Context-Aware Sentence/Passage Term Importance Estimation For First Stage Retrieval

Term frequency is a common method for identifying the importance of a term in a query or document. But it is a weak signal, especially when the frequency distribution is flat, such as in long queries or short documents where the text is of sentence/passage-length. This paper proposes a Deep Contextualized Term Weighting framework that learns to map BERT's contextualized text representations to context-aware term weights for sentences and passages. When applied to passages, DeepCT-Index produces term weights that can be stored in an ordinary inverted index for passage retrieval. When applied to query text, DeepCT-Query generates a weighted bag-of-words query. Both types of term weight can be used directly by typical first-stage retrieval algorithms. This is novel because most deep neural network based ranking models have higher computational costs, and thus are restricted to later-stage rankers. Experiments on four datasets demonstrate that DeepCT's deep contextualized text understanding greatly improves the accuracy of first-stage retrieval algorithms.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> sections/bak-reweght-example.tex <==
This section provides two qualitative analysis of \texttt{DeepCT-Index}. It first compare the term weights generated from \texttt{DeepCT-Index} to term weights from baseline term weighting approaches. Next, it investigates how the weights affect retrieval accucary by studying winning/losing cases of \texttt{DeepCT-Index}

\begin{table*}[t]
\caption{An example of re-weighted documents generated from baseline methods and \texttt{DeepCT-Index}. The query and the document are from MS MARCO.}\label{tab:river_example}
\begin{tabular}{ll}
\hline \hline
Query          & Where does the Delaware River start and end                                                                                                                                                                                                                        \\
Document & \begin{tabular}[c]{@{}l@{}}The Delaware River flows through Philadelphia into the Delaware Bay. It flows through and aqueduct\\ in the Roundout Reservoir and then flows through Philadelphia and New Jersey before emptying into\\ the Delaware Bay.\end{tabular} \\ \hline
\texttt{Origin}        & (flows,3)   \textbf{(delaware,3)}  (philadelphia,2)  (bay,2) (roundout,1)  \textbf{(river,1)}  (reservoir, 1) (empty,1) (aqueduct, 1)\\
TextRank        & (emptying,14)   (philadelphia,10)  (flows,10)  (reservoir,9) (roundout,9)  \textbf{(delaware,5)}  (bay,5) (aqueduct,5)   \textbf{(river,1)}                                                                                                                                                                   \\
\texttt{DeepTR}       & \textbf{(delaware,30)}  (aqueduct,14)  (bay,12)  (reservoir,10)  (philadelphia,8)  \textbf{(river,7)}  (flows,6) (roundout,2)                                                                                                                                                                        \\ \hline
\texttt{Doc2Query}     & 
\begin{tabular}[c]{@{}l@{}}what river flows through delaware; what year did the delaware river flow; when did the delaware river flow;\\  what river flows through the delaware river; where does the river river river river flow    \end{tabular}
                                                     \\ \hline                                                                                                                                                             
\texttt{DeepCT-Index}   & \textbf{(delaware,97)} \textbf{(river,93)} (flows,66) (emptying,22) (bay,12) (philadelphia,8) (roundout,2) (aqueduct,2)                                                                                 \\ \hline \hline                                                                                           
\end{tabular}
\end{table*}
Table~\ref{tab:river_example} gives an example of term weights predicted by \texttt{TextRank}, \texttt{DeepTR}, and \texttt{DeepCT-Index}; we also show the expanded query from \texttt{Doc2Query} using the example from~\citet{nogueira2019doc2qry}. \texttt{TextRank} estimate term importance with PageRank on the term co-occurrence graph. However, most words appear 1 or 2 times in the passages, hence the co-occurrence probabilities are rather flat and cannot well reflect term centralities. \texttt{DeepTR} takes word meanings into consideration by representing words with word2vec. It can identify some important words with the linguistic properties encoded in word2vec such as part-of-speech tags and certain word classes. However, \texttt{DeepTR} often assign high weights to nouns or less-freuquent words even though they are not central to the meaning of the passage. As shown in Table~\ref{tab:river_example}, `aqueduct' and `reservoir' were mistankenly asigned high weights by \texttt{DeepTR}. \texttt{Doc2Query} is the most effective baseline. It learns a transoforms-based encoder to encode the passage and generates potential queries based on the encoded context. As shown in Table~\ref{tab:river_example}, it puts important document words `delaware' and `river' into the predicted query and added the query back to the document. However, adding a query can only increase the term frequency by 1, which may not put enough emphasize on the central words. 

\texttt{DeepCT} explicitly generate a contextualized representation to every individual term and directly learn a weights for each term. The embedding from BERT captures a words' meaning, position, and relation to other words.

==> sections/exp-elmo.tex <==
\section{ELMo vs. BERT in D\MakeLowercase{eep}CT}\label{sec:elmo}

The last experiment studied how the \texttt{DeeCT} framework works with another strong contextualized word representation, ELMo~\cite{Peters:2018}. The ELMo-based \texttt{DeepCT} is based on the PyTorch-based NLP library AllenNLP; parameters are initialized with the pre-trained ELMo described by~\citet{Peters:2018}.

Figure~\ref{fig:elmo} compares ELMo-base and BERT-based \texttt{DeepCT} on both query/document weighting tasks. It shows the relative improvements of \texttt{DeepCT-Query} and \texttt{DeepCT-Index} over the original query and document representations on the corresponding retrieval tasks. Due to space constraints, we present results for just one dataset. 

ELMo-based \texttt{DeepCT} improved ranking accuracy compared to the unweighted query and document representations, indicating that the \texttt{DeepCT} approach is not restricted to BERT. %Their linear regression layer, the supervision signals, and the ways of using estimated weights are all compatible with another contextualized word presentation. 
However, BERT consistently outperforms ELMo.  The difference is greater as text length increases (description < narrative < passage), suggesting that BERT may be more effective at modeling longer dependencies. 
%The inference time of ELMo-based \texttt{DeepCT} was more than $3\times$ slower than BERT-based \texttt{DeepCT}. This is due to the fact that ELMo uses a RNN-based architecture
%probably due to the framework (pytorch vs. Tensorflow) and the parallelism of the neural network (Bi-LSTMs vs. Transformers). 
We recommend using BERT in \texttt{DeepCT-Query} and \texttt{DeepCT-Index}.  However, this experiment suggests that the \texttt{DeepCT} framework is likely to be compatible with more powerful neural word representations that may be developed in the future.


\begin{figure}[tb]
\centering
\begin{subfigure}[b]{0.16\textwidth}
\includegraphics[width=\textwidth]{figures/deepct_elmo_qdesc.pdf}
\end{subfigure}%
\begin{subfigure}[b]{0.16\textwidth}
\includegraphics[width=\textwidth]{figures/deepct_elmo_qnarr.pdf}
\end{subfigure}%
\begin{subfigure}[b]{0.16\textwidth}
\includegraphics[width=\textwidth]{figures/deepct_elmo_marco.pdf}
\end{subfigure}%
\caption{Relative gain of ELMo- and BERT-based \texttt{DeepCT} over original queries/documents. The left and middle figures used \texttt{DeepCT-Query} to generate weighted \texttt{BOW} queries for Robust04 query descriptions/narratives. The right figure used \texttt{DeepCT-Index} to index MS MARCO passages and search queries with \texttt{BM25}.
}~\label{fig:term_dist}
\label{fig:elmo}
\end{figure}

==> sections/exp-res-doc-trainsize.tex <==
\subsection{Effects of Training Data Size}\label{subsection:train-size}

%Previous experiments in this section used hundreds of thousands of relevant query-passage pairs to fine-tune \texttt{DeepCT}'s BERT model and to learn the regression layer. Large amounts of relevant labels may be expensive to obtain. 
The last experiment studied \texttt{DeepCT-Index}'s performance with varying amounts of training data. It randomly sampled the training data in a log scale ($1/4, 1/16, ..., 1/1024$). Figure~\ref{fig:train_size} shows results on MS MARCO.  

Perhaps surprisingly, \texttt{DeepCT-Index} achieved relatively good performance with small amounts of training data.
When only 392 training examples are available ($1/1024$ of the total training data), \texttt{DeepCT-Index} already outperforms the original BM25 by $14\%$.  \texttt{DeepCT-Index}'s accuracy grows
with more training sessions. The increasing trends has not yet plateaued with 0.4M training passages, suggesting that \texttt{DeepCT-Index} can utilize more training data than was available in this dataset.

\texttt{DeepCT-Index}'s data efficiency is due to the fact that the underlying BERT is pre-trained on large, open-domain text corpora. Our results show that the patterns learned from those pre-training tasks are effective in identifying important terms. A small amount of additional data enables fine-tuning \texttt{DeepCT} to produce good term weights. Meanwhile, \texttt{DeepCT} has a large learning capacity and keeps improving with more training data.




\begin{figure}[tb]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/deepct_train_size.pdf}
    \caption{The ranking accuracy of BM25 using \texttt{DeepCT-Index} with varying amounts of training data.  X-axis shows the ratio of passages used for training (first row) and the corresponding number of training instances (second row). Y-axis shows MRR@10 of BM25 retrieval on \texttt{DeepCT-Index}.}
    \label{fig:train_size}
\end{figure}


==> sections/sigir19/conclusion.tex <==
\section{Conclusion}
Text understanding is a long-desired feature for text retrieval.  Bag-of-words approaches only provide a shallow representation of text. Contextual neural language models open new possibilities for understanding word context and modeling language structures. This paper studies the effect of a recently-proposed deep neural language model, BERT, on ad-hoc document retrieval tasks.

Adapting and fine-tuning BERT achieves high accuracy on two different search tasks, showing the effectiveness of BERT's language modeling for IR. %The power comes from the transformer architecture that supports different types of word associations, and the pre-trained model that provide off-the-shelf language modeling. 
%Moreover, minimal search-specific architecture is required: the attention of BERT spans over query and document, organically supporting query-document interaction in addition to query/document understanding. 
The contextualized model brings large improvements to natural language queries. 
The corpus-trained language model can be complemented with search knowledge through simple domain adaptation, leading to a strong ranker that models both  meanings of text and relevance in search.
%For two decades

People have been trained to use keyword queries because bag-of-words retrieval models cannot effectively extract key information from natural language. %Even for systems that do take natural language queries, such as retrieval-based question-answering systems, many of them actually convert the query into keywords by filtering out stopwords and punctuations in order to reduce noise. 
We found that queries written in natural language actually enable \textit{better} search results when the system can model language structures. Our findings encourage additional research on search systems with natural language interfaces.  %to gradually move towards interacting with people in natural languages. %It will not only provides a more natural user experience, but will also provide better search results, as shown in this work. 
%Pre-trained BERT is especially helpful for search tasks with few training data. However, it does not know search-related knowledge such as user search preferences. Fine tune on the search task may not provide sufficient example when labels are limited. 
 %The resulting search-enhanced BERT demonstrated that, a good retrieval model should be able to understand the general language knowledge and search knowledge, and it is possible to gain both types of knowledge in a pre-trained way to benefit low-resource search tasks. 

%Previous IR models find difficult to leverage natural languages as sparse word representations cannot well represent word meanings, and bag-of-words models are not able to model structures.  Neural IR models also not able to effectively use them as many of them are still bag-of-words, and most IR models focuses on q-d relations without explicitly goal to model the language itself. 

==> sections/sigir19/evaluation.tex <==
\section{Results and Discussion}

This section studies the effectiveness of BERT on document retrieval tasks, the difference among different types of queries, and the impact of enhancing BERT with search logs.

\input{sections/exp1-overall.tex}


\input{sections/exp2-query.tex}

\input{sections/exp3-enhance.tex}



==> sections/sigir19/exp1-overall.tex <==
\subsection{Pre-trained BERT for Document Retrieval}



\begin{table}[t]
\caption{Search accuracy on \textbf{Robust04} and \textbf{ClueWeb09-B}. $\dagger$ indicates statistically significant improvements over \texttt{Coor-Ascent} by permutation test with p< 0.05.}\label{tab:overall}

\def\arraystretch{0.9}
\vspace{-0.15in}
\begin{tabular}{l|cc||cc}
\hline \hline
  &  \multicolumn{4}{c}{nDCG@20}\\
\multirow{3}{*}{Model} & \multicolumn{2}{c||}{Robust04} & \multicolumn{2}{c}{ClueWeb09-B} \\
 & \multicolumn{1}{c}{Title  } & \multicolumn{1}{c||}{Description  } & \multicolumn{1}{c}{Title  } & \multicolumn{1}{c}{Description }  \\
                            \hline
\texttt{BOW}                         & 0.417    & 0.409   
 & 0.268  & 0.234  \\
\texttt{SDM}                         & 0.427           & 0.427         & 0.279 & 0.235  \\ \hline
%QE                         & 0.424     & 0.239          & 0.416       & 0.248     & 0.264 & 0.272 & 0.168 & 0.232 & 0.236 & 0.133 \\ \hline
\texttt{RankSVM}                    & 0.420         &   0.435        & 0.289  & 0.245  \\
\texttt{Coor-Ascent}                & 0.427            &     0.441               & \textbf{0.295}  & 0.251  \\ \hline
\texttt{DRMM}                       & 0.422          & 0.412            & 0.275  & 0.245  \\ 
\texttt{Conv-KNRM}                       &  0.416        &  0.406          & 0.270  &  0.242 \\ \hline\hline
%K-NRM                  & 0.418           &   0.396        & 0.192     &  0.361            & 0.333           &   0.179      & & & & & &  \\ \hline
%Conv-KNRM-fixemb                  &           &           &         &              &             &         & & & & & &  \\ \hline
\texttt{BERT-FirstP}           & 0.444$^\dagger$            & 0.491$^\dagger$             & 0.286  & \textbf{0.272}$^\dagger$    \\
\texttt{BERT-MaxP}            & \textbf{0.469}$^\dagger$           & \textbf{0.529}$^\dagger$          & 0.293  & 0.262$^\dagger$   \\ 
\texttt{BERT-SumP}        &  0.467$^\dagger$     &   0.524$^\dagger$    &   0.289 &   0.261      \\ 
\hline \hline 
 

\end{tabular}
\end{table}

The ranking accuracy of each ranking method is shown in Table~\ref{tab:overall}.  On Robust04,  BERT models consistently achieve better search accuracy than the baselines, with a $10\%$ margin on query titles and a $20\%$ margin on description queries. On ClueWeb09-B,  BERT is comparable to 
\texttt{Coor-Ascent} on title queries, and better on description queries. The results demonstrate the effectiveness of BERT for document retrieval, especially on description queries. 

Among the neural rankers, \texttt{Conv-KNRM} has the lowest accuracy. \texttt{Conv-KNRM} needs to learn n-gram embeddings from scratch. It is strong when 
trained on a large search log~\cite{dai2018convolutional}, but it tends to overfit when 
trained with only a small amount of data. BERT is pre-trained and is less prone to overfitting. \texttt{DRMM} represents words with pre-trained word embeddings. The better performance of BERT models demonstrates that the contextualized text representations are more effective for IR than bag-of-words embeddings. 

\textbf{Sources of effectiveness}. Figure~\ref{fig:bertviz} visualizes two layers from the \texttt{BERT-MaxP} model when predicting the relevance between a description query \textit{`Where are wind power installations located?'} and a sentence \textit{`There were 1,200 wind power installations in Germany'}. Example 1 shows the attention received by the document word \textit{`power'}. The strongest attention comes from \textit{`power'} in the query (query-document exact term matching), and the previous and next word of \textit{`power'} (bi-gram modeling). 
Local matching of words and n-grams have proven to be strong neural IR features ~\cite{DRMM, dai2018convolutional}; BERT is also able to capture them.
Example 2 shows that the document word \textit{`in'} receives the strongest attention from the query word \textit{`where'}. The word \textit{`in'} appears in the context of \textit{`in Germany'}, so it satisfies the \textit{`where'} question. Words like \textit{`in'} and \textit{`where'} are often ignored by traditional IR methods due to their high document frequency in the corpus. This example shows that with a deeper text understanding, these stop words actually provide important evidence about relevance. 
In summary, the advantages of BERT lie in the architecture and the data. The transformer architecture allows BERT to extract a variety of effective matching features. The transformers are already pre-trained on a large corpus, so search tasks with few training data can also benefit from this deep network.

%Among the baselines, ~\texttt{Coor-Ascent} performs the best, showing that a good combination word frequency signals is powerful. \texttt{DRMM} incoperates soft-match signals harvest from a pre-trained word2vec with traditional frequency signals (TF and IDF). The soft-match signals provide DRMM with word-level text understanding, improving its search performance in some cases. However, term frequency signals are crucial for DRMM; previous research shown that its performace was lower than LM if used without IDF~\cite{DRMM}. \texttt{BERT} models outperforms frequency-based baselines and \texttt{DRMM} without explicitly extracting term frequencies. This may seem in contrast with previous neural IR research that exact term-matching signals are impportant~\cite{DRMM, K-NRM}. To better understand  

%This is due to that \texttt{BERT} pre-trained models is deep and contuxtual, whereas word embeddings are shallow bag-of-words.  Comparing \texttt{BERT} to \texttt{Conv-KNRM} shows the advantage of having a pre-trained model.  \texttt{conv-KNRM} needs to end-to-end learn the contextual word embeddings (n-grams). However, our datasets only have limited training data and are not sufficient for it to learn generalizable patterns. \texttt{BERT} alreadly learns language modeling from high-quality, general domain documents, making it suitable for low-resource search tasks.
%\texttt{DRMM} rely on the IDF weight to determine word importance. \texttt{K-NRM-fixemb} can be viewed as a \texttt{DRMM} without IDF weight, whose performance drops dramatically. \text{BERT} models do not have IDF weight, either, but were albe to achieve good performance. This is due to by learning from large number of documents, the model already identifies unimportant words; the self-attention further helps the model to pay attention to important words. 
%The main advantages of \texttt{BERT} lie in 1) the multi-head self-attention architecture, and 2) the pre-trained language model. The self-attention spans over the concatenation of query and document tokens, performing query self-attention, document self-attention, and the attention across query and document. The last piece makes it possible to directly use BERT for search without adding search-specific architecture. The multi-head attention allows the model to learn different types of word dependencies. \todo{illustration}. More importantly, the model is pre-trained on high-quality documents with well-defined language modeling tasks. The Wikipeida and bookcorpus allows the model to learn general language knowledge such as related concepts, language structures, word importances, ect.  Comparing \texttt{BERT} to \texttt{Conv-KNRM} shows the advantage of having a pre-trained model.  \texttt{conv-KNRM} needs to end-to-end learn the contextual word embeddings (n-grams). However, our datasets only have limited training data and are not sufficient for it to learn generalizable patterns. \texttt{BERT} alreadly learns language modeling from high-quality, general domain documents, making it suitable for low-resource search tasks. Besides, trained on the next-sentence prediction task, the model already learns interaction two sentence, similar to interacting query-document.

\begin{figure}[tb]
     \centering
     
     \includegraphics[width=0.5\textwidth]{figures/bertviz5.png}
     \caption{Visualization of BERT.  Different colors represent different attention heads of the multi-head attention; deeper color indicates higher attention. } \label{fig:bertviz}
 \end{figure}
 
 

\textbf{Title queries vs. description queries}. \texttt{BERT} models have larger gains on description queries. On Robust04, using description queries with \texttt{BERT-MaxP} brings a $23\%$ improvement over the best title query baseline (\texttt{SDM}). Most other ranking methods only get similar or worse performance on descriptions compared to titles. To the best of our knowledge, this is the first time we see that description queries outperform title queries with such a large margin. On ClueWeb09-B,  \texttt{BERT} manages to shrink the gap between titles and descriptions. %It is harder to make description queries better than title queries due to lower recall from the initial retrieval stage. 
Although intuitively, description queries should carry richer information, it is hard to fully utilize them in traditional bag-of-words methods due to difficulties in estimating term importance. Our results show that longer natural language queries are indeed more expressive than keywords, and the richer information can be effectively leveraged to improve search using a deep, contextualized neural language model. Further analysis of BERT's ability to understand different types of search queries is given in Section 5.2.

\textbf{Robust04 vs. ClueWeb09-B.} BERT models perform better on Robust04 than on ClueWeb09-B. This is probably due to that Robust04 is closer to the pre-trained model. Robust04 has well-written articles; its queries look for facts that depend largely on understanding text meaning. ClueWeb09-B documents are webpages that include tables, navigation bars, and other discontinuous text. The task also involves web-search specific issues such as page authority. More training data may be required to learn such search-specific knowledge. We investigate this possibility in Section 5.3.






==> sections/sigir19/exp2-query.tex <==
\subsection{Understanding Natural Language Queries}

%Natural language queries differ from keywords queries in that they are longer, with well-formed grammar structures, and have more complex logic.  %In traditional bag-of-words retrieval models, longer queries require better term re-weighting; the grammar structures and logic are even more difficult to leverage, requiring sophisticate parsing and feature engineering. This section tries to understand how these differences affect BERT's contextual language model in understanding a query. 

This section examines BERT on 3 types of queries that require different levels of text understanding: title, description, and narrative.  To test the effect of grammar structures, a keyword version of description and narrative is generated by removing stopwords and punctuation. To test how BERT understands the logic in narratives, a `positive' version of narrative is generated by removing negative conditions (e.g. \textit{"Not relevant are documents..."}).
Table~\ref{tab:query-types} shows the performance of \texttt{SDM}, \texttt{Coor-Ascent} and \texttt{BERT-MaxP} on Robust04. Supervised methods use narratives to re-rank title query initial results due to low recall of \texttt{BOW} on narratives, which gives narratives 
an advantage over the other types of queries.

\texttt{SDM} works best with titles. \texttt{Coor-Ascent} is moderately better with descriptions and narratives. The two methods weight words solely based on term frequencies, but word importance should depend on the meaning of the word and the meaning of the entire query. \texttt{BERT-MaxP} makes much larger improvement on longer queries by modeling word meaning and context.  For both \texttt{SDM} and \texttt{Coor-Ascent}, keywords versions perform better than the original query, because stopwords are noisy to traditional match signals like TF.
In contrast, BERT is more effective on the original natural languages queries. Although stopwords and punctuation do not define the information need, they build the structures in a language. The deep transformer architecture of BERT is able to capture such structures, achieving a deeper query understanding than flat bag-of-words. Table~\ref{tab:query-types} also shows the limitations of BERT. It is unable to leverage evidence from negative logic conditions in narratives; removing negative conditions does not hurt performance. %Adding title improves the performance of narratives, showing the need of better ways to extracting the most important information.

%Narratives have a higher requirement of logic inference such as NOT ("A document is not relevant if...") and OR ("Also relevant are..."). For description and narratives, we generated a keyword version which removes grammar structure by removing stopwords and punctuations. To test how BERT understand the logic in narratives, we also generate a `positive' version where all negative logic conditions were manually removed.


\begin{table}[tb]
 \centering
\caption{Accuracy on different types of Robust04 queries. Percentages show relative gain/loss over title queries.}\label{tab:query-types}
\def\arraystretch{0.9}
\vspace{-0.15in}
\setlength\tabcolsep{3pt}

\begin{tabular}{l|c|cr|cr|cr}
\hline \hline
\multirow{2}{*}{Query} & Avg & \multicolumn{6}{c}{nDCG@20} \\ 
  & Len & \multicolumn{2}{c}{\texttt{SDM}}   & \multicolumn{2}{c}{\texttt{Coor-Ascent}}  & \multicolumn{2}{c}{\texttt{BERT-MaxP}} \\ \hline
 
%Title                   & 3   & 0.427   & -- & 0.427 & +0\% & 0.469    & +10\% \\    \hline
%Desc        & 14  & 0.404   & -5\%   & 0.422  & -1\% & 0.529    & +24\% \\ 

%Desc, keywords   & 7  & 0.427   & -0\%  & 0.441 & +5\%& 0.503    & +18\% \\  \hline

%Narr          & 40   &  0.278  &  -35\%   & 0.424 & -1\% & 0.487  & +14\%  \\
%Narr, keywords     &  18 &  0.332  & -22\%   & 0.439  & +3\%&    0.471 &  +10\%  \\ 
%Narr, positive          & 31   & 0.272   &  -36\%    & 0.432 & +1\% & 0.489  & +15\%  \\ 
%Title+Narr, origin          & 43   &    &    & &  & 0.501  & +17\%  \\

Title                   & 3   & 0.427   & -- & 0.427 & -- & 0.469    & -- \\    \hline
Desc        & 14  & 0.404   & -5\%   & 0.422  & -1\% & 0.529    & +13\% \\ 

Desc, keywords   & 7  & 0.427   & -0\%  & 0.441  & +5\%& 0.503     & +7\% \\  \hline

Narr          & 40   &  0.278  &  -35\%   & 0.424 & -1\% & 0.487  & +4\%  \\
Narr, keywords     &  18 &  0.332  & -22\%   & 0.439  & +3\%&    0.471 &  +0\%  \\ 
Narr, positive          & 31   & 0.272   &  -36\%    & 0.432 & +1\% & 0.489   & +4\%  \\

\hline \hline
\end{tabular}
\end{table}


==> sections/sigir19/exp3-enhance.tex <==
\subsection{Understanding the Search Task}

Corpus-trained text representations do not always align with the search task~\cite{K-NRM}. Search specific knowledge is necessary, but requires labeled data to train.  ~\citet{dai2018convolutional} show promising results on learning search patterns from related domains for a low-resource search task. The last section investigates if BERT's language modeling knowledge can be stacked with additional search knowledge to build a better ranker, and if the search knowledge can be learned in a domain-adaptation manner to alleviate cold-start problems. 
%1) if contextual language models, which are much larger and likely to overfit, can also learn knowledge about search in a similar domain-adaptation way; and 2) if the natural language modeling knowledge and the search knowledge can be stacked to generate a better neural ranker.
%Results from Section 5.1 indicate that for some search tasks, text content understanding is not sufficient; search-specific features are also important. %In many cases, such data are expensive to obtain and takes time to collect, causing cold-start problem for new search tasks. 


%One of the most attractive advantage of \texttt{BERT} is that the model is pre-trained, so that downstream tasks can avoid training from scratch, which is time-consuming, error-prone and data-hungry. 
 


\begin{table}[tb]
\caption{Accuracy of Bing augmented BERT on ClueWeb09-B. $\dagger$: statistically significant improvements over \texttt{Coor-Ascent}.}\label{tab:enhance}
\def\arraystretch{0.85}
\vspace{-0.15in}

\begin{tabular}{l|cc|ll}
\hline \hline
    \multirow{2}{*}{Model}  & \multicolumn{2}{c|}{Knowledge} & \multicolumn{2}{c}{nDCG@20} \\
              & Text &  Search         & {Title} & {Desc}\\ \hline
\texttt{Coor-Ascent}              & Low & Low   & 0.295     & 0.251    \\ \hline
\texttt{BERT-FirstP}  & High & Low & 0.286     & 0.272$^{\dagger}$    \\ 

%Conv-KNRM+Bing     &  & \checkmark &      &    \\ 
\texttt{Conv-KNRM+Bing}    &  Low & High   & 0.314 $^{\dagger}$     &  0.275 $^{\dagger}$    \\ 
\texttt{BERT-FirstP+Bing}  & High  & High  & \textbf{0.333}$^{\dagger}$      & \textbf{0.300}$^{\dagger}$   \\ 
 \hline \hline

\end{tabular}
\end{table}

%\texttt{BERT-First} is the model directly fine-tuned on the target task. The model learn language modeling from a large amount of documents, but only sees a limited amount of search examples. It fails to beat  \text{Coor-Ascent}.

We train BERT on a sample of Bing search log with 0.1M queries and fine-tune it on ClueWeb09-B. Results are shown in Table~\ref{tab:enhance}. \texttt{BERT-FirstP} is the best in-domain BERT model on ClueWeb09-B (Table~\ref{tab:overall}). Its pre-trained language model encodes general word associations like (`Honda', `car'), but lacks search-specifc knowledge like  (`Honda', `special offer').
\texttt{Conv-KNRM+Bing} was the previous state-of-the-art domain adapted neural IR model~\cite{dai2018convolutional}.  It is trained on millions of query-document pairs to learn search-specific n-gram embeddings, but does not explicitly model general language patterns. %Combining its n-gram matching features with \texttt{SDM} has better performance than feature-based learning-to-rank and \texttt{BERT-FristP}, showing the importance of search-specific knowledge.
\texttt{BERT-FirstP+Bing}  achieves the best performance, confirming that text retrieval requires understanding both the text content and the search task. Simple domain adaptation of BERT leads to a pre-trained model with both types of knowledge that can improve related search tasks where labeled data are limited. %For search tasks where relevance labels are limited, off-the-shelf pre-trained BERT provides text understanding knowledge, while the search knowledge can be enhanced by learning from related search tasks in a simple yet effective way. For search tasks where labeled data is limited, it is desirable to have 

==> sections/sigir19/experimental_setup.tex <==
\section{Experimental Setup} \label{section:exp-setup}

\begin{table}
\caption{Example of Robust04 search topic (Topic 697).}\label{tab:query-example}
\small
\vspace{-0.15in}
%\def\arraystretch{0.85}


\begin{tabular}{p{0.15\columnwidth} p{0.76\columnwidth}}
\hline \hline
%\multicolumn{2}{c}{Topic }                                                                                                                                                                                %                                                                            \\\hline
Title       & air traffic controller                                                                                                                                                                                                                                                  \\
Description & What are working conditions and pay for U.S. air traffic controllers?                                                                                                                                                                                             \\
Narrative   &  Relevant documents tell something about working conditions or pay for American controllers.  Documents about foreign controllers or individuals are not relevant.
\\ \hline \hline
\end{tabular}
\end{table}

\textbf{Datasets.} We use two standard text retrieval collections with different characteristics. \textbf{Robust04} is a news corpus with 0.5M documents and 249 queries. Two versions of queries are included: a short keyword query (\textit{title}) and a longer natural language query (\textit{description}). A \textit{narrative} is also included as the guidance for relevance assessment. An example is shown in Table \ref{tab:query-example}. \textbf{ClueWeb09-B} contains 50M web pages and 200 queries with title and description. Passages are generated using a $150$-word sliding window with a stride of $75$ words. For ClueWeb09-B, document titles are added to the beginning of each passage. %We evaluate the search effectiveness of ranking models on title queries and description queries; robust04 narratives are used in Section~\ref{section:exp-query} to gain better understanding of BERT's language understanding ability.
%Both datasets have limited relevance labels (200-250 queries), making pre-trained models like BERT desirable. The two datasets also enable us to compare BERT's generalization ability for text retrieval in terms of query styles (keywords vs. natural language) and document quality (well-written news articles vs. noisy web pages). 
For augmenting BERT with search data, we follow the domain adaptation setting from ~\citet{dai2018convolutional} and use the same Bing search log sample. The sample contains 0.1M queries and 5M query-document pairs.%The Bing-log dataset pre-processing and training label generation all follow~\citep{dai2018convolutional}.

\textbf{Baselines and Implementations}. Unsupervised baselines use Indri's bag of words (\texttt{BOW}) and sequential dependency model queries (\texttt{SDM}). 
Learning-to-rank baselines include \texttt{RankSVM} and \texttt{Coor-Ascent} with bag-of-words features~\cite{dai2018convolutional}. Neural baselines include \texttt{DRMM}~\cite{DRMM} and \texttt{Conv-KNRM}. \texttt{DRMM} uses word2vec~\cite{word2vec} to model word soft-match; it was shown to be among the best performing neural models on our two datasets~\cite{DRMM}. \texttt{Conv-KNRM} learns n-gram embeddings for the search task and show strong performance when 
trained on large search logs~\cite{dai2018convolutional}.  %\texttt{K-NRM} end-to-end learns a word embedding from relevance labels, tailoring the word embeddings for soft-matching queries and documents.
The Bing-adapted \texttt{Conv-KNRM} was the state-of-the-art neural IR model when trained with domain adaptation~\cite{dai2018convolutional}, and is compared to the Bing-augmented BERT. BERT models are based on the implementation released by Google\footnote{https://github.com/google-research/bert}. Baselines use standard stopword removal and stemming; BERT uses raw text. Supervised models are used to re-rank the top 100 documents retrieved by \texttt{BOW} with 5-fold cross-validation. Due to space limit, we only report \textbf{nDCG@20}, one of the official
TREC ad-hoc task metrics; similar trends were observed with nDCG@10 and MAP@100.




 

==> sections/sigir19/model.tex <==
\section{Document Search with BERT}\label{sec:model}

\begin{figure}[!t]
\centering
\includegraphics[width=0.8\linewidth]{figures/bert2.png}
\caption{BERT sentence pair classification architecture~\cite{devlin2018bert}. %Query tokens and document tokens are concatenated. Token embeddings are added with position embeiddings and segment embeddings. The transformers learn interactions among query and document tokens. A multi-layer perceptron (MLP) is used to predict the relevant label.
}
\label{fig:bert}
\end{figure}

This work uses an off-the-shelf BERT architecture, the sentence pair classification architecture described by~\citet{devlin2018bert}, as shown in Figure~\ref{fig:bert}. The model takes as input the concatenation of the query tokens and the document tokens, with a special token `[SEP]'  separating the two segments. Tokens are embedded into embeddings. To further separate the query from the document, segment embeddings `Q' (for query tokens) and `D' (for document tokens) are added to the token embeddings. To capture word order, position embeddings are added. The tokens go through several layers of \emph{transformers}. At each layer, a new contextualized embedding is generated for each token by weighted-summing all other tokens' embeddings. The weights are decided by several attention matrices (multi-head attention). Words with stronger attentions are considered more related to the target word. Different attention matrices capture different types of word relations, such as exact match and synonyms . The attention spans over the query and the document so that query-document interactions are taken into consideration. Finally, the output embedding of the first token is used as a representation for the entire query-document pair. It is fed into a multi-layer perceptron (MLP) to predict the possibility of relevance (binary classification).
The model is initialized with a pre-trained BERT model\footnote{We use uncased BERT-Base model from \url{https://github.com/google-research/bert}} to leverage the pre-trained language model, while the last MLP layer is learned from scratch. During training, the entire model is tuned to learn more IR-specific representations. 


\textbf{Passage-Level Evidence.} Applying BERT to long documents causes increasing memory usage and run time due to the complexity in interacting every pair of tokens. The sentence-trained model may also be less effective on long text. We adopt a simple passage-level approach for document retrieval. We split a document into overlapping passages. The neural ranker predicts the relevance of each passage independently.  document score is the score of the first passage (\texttt{BERT-FirstP}), the best passage (\texttt{BERT-MaxP}), or the sum of all passage scores (\texttt{BERT-SumP}). For training, passage-level labels are not available in this work. We consider all passages from a relevant document as relevant and vice versa. When the document title is available, the title is added to the beginning of every passage to provide context. 


\textbf{Augmenting BERT with Search Knowledge.}  
Some search tasks require both general text understanding (e.g. Honda is a motor company) and more-specific search knowledge (e.g. people want to see special offers about Honda). While pre-trained BERT encodes general language patterns, the search knowledge must be learned from labeled search data.  Such data are often expensive to obtain and take time to collect. It is desirable to have a pre-trained ranking model that is equipped with both language understanding knowledge and search knowledge. We augment BERT with search knowledge by tuning it on a large search log. The rich search knowledge is expected to benefit related search tasks where only dozens or hundreds of labeled search examples are available. %The resulting search-enhance model is fine-tuned on the target search domain.  


%A main advantage of pre-trained BERT is that it provides downstream NLP tasks with general knowledge about the English language without the need to learn from scratch. In search tasks, this ability helps the ranker to understand the meaning of the query and the topic of the document. However, text search tasks also require specific knowledge about the search problem. For example, people often write search queries in a few keywords rather than verbose natural language with grammar structures; people also have preferences over documents from certain sources than from the others. BERT pre-trained on high quality documents does not have knowledge about user queries and user preferences. Fine-tuning BERT on the target search task is one way to equip BERT with search knowledge. However, when the target search task only has a small amount of labeled data, it may not be sufficient to fill this gap. In this work, 


\textbf{Discussion.} 
Only small adaptations are made to apply BERT to search tasks:  
a passage-based approach to handle long documents, and a concatenation approach to handle multiple document fields.  Our goal is to study the value of BERT's contextualized language models for search, not to make major 
extensions to the architecture.
%This work focuses on whether a contextual language model can provide better text understanding for IR, so we made minimal changes to the BERT architecture.
%We believe that the off-the-shelf BERT already supports many important features for IR. Search-specific architectural adaptations are promising but require much more engineering and training data.

==> sections/sigir19/related_work.tex <==
\section{Related Work}\label{section:related-work}

%There are two focuses of neural models for text search tasks:  1) how to understand the document and query, and 2) how to model the relevance patterns between queries and documents. 

Recent neural IR models have made promising progress in learning query-document relevance patterns. One line of research learns text presentations tailored for the search task~\cite{K-NRM, dai2018convolutional, WeakNeuIR} with search signals from click logs~\cite{K-NRM, dai2018convolutional} or pseudo-relevance feedback~\cite{WeakNeuIR}. Another line of research designs neural architectures to capture diverse matching features such as exact match signals~\cite{DRMM, mitra2017learning} and passage-level signals~\cite{pang2017deeprank}. How to understand the text content of the query/document is less explored. Most neural IR models represent text with word embeddings such as Word2Vec~\cite{word2vec} and GloVE~\cite{pennington2014glove}. 
%Solely learning from relevance labels causes problems as the labels are expensive to obtain and have bias on frequent queries. A search system should also be able to understand the text content, which can be learned from the corpus without search data. 
%Relevance labels are sparse. To avoid overfitting, most neural IR models are based on pre-trained word embeddings such as Word2Vec~\cite{word2vec} and GloVE~\cite{pennington2014glove}. They have proven helpful to some search tasks by providing word synthetic and semantic similarities~\cite{DRMM, zheng2015learning}. 
%With most existing neural IR models focusing on query-document relevance patterns, another fundamental problem of text search, understanding the text content o a document or a query, is less explored. 
%Most neural IR methods gain use pre-trained word embeddings~\cite{word2vec, pennington2014glove} which captures syntactic and semantic information of words from large scale unlabeled text. The word similarities encoded in such pre-trained word embeddings have proven helpful to bridge the vocabulary gap between queries and documents~\cite{DRMM}, and in identify important words in a query~\cite{zheng2015learning}.  
%But word embeddings does not consider context of a word and the structure in a sentence, causing topic shifting~\cite{diazquery} for IR tasks. It often requires additional network layers and training to leverage word embeddings for longer documents. %IR tasks requires deeper understanding of the text, such as identifying synonyms, understand word classes, finding the paraphrases, etc. Hence, it is common for neural IR models to add additional CNN/RNN layers on top of word embeddings to capture phrases and sentence level information. But they usually need a lot of training data, and the supervision is from query-document relevance, so they only implicitly learn text understanding. 

Contextual neural language models are proposed to improve traditional word embeddings by incorporating the context~\cite{Peters:2018, devlin2018bert}. %They use more complex architectures to capture contextual information from a text, showing stronger representation power than word embeddings. 
One of the best performing neural language models is BERT~\cite{devlin2018bert}.  BERT consists of dozens of multi-head self-attention layers (`transformers'), where a word is represented by the weighted sum of related words' embeddings. 
The word representation is contextual as it depends on all other words. %The full connection among words provides a flexible way to model word dependencies and language structures. Besides, BERT uses multiple-head attention to learn different types of word relations (e.g. exact-match, bi-grams, etc), which is shown effective for IR~\cite{DRMM, dai2018convolutional}.
BERT is pre-trained on large-scale, open-domain documents (Wikipedia and BooksCorpus) to learn general patterns in a language. Pre-training tasks include predicting words within a sentence and the relationship of two sentences. BERT has advanced the state-of-the-art on a variety of NLP tasks, including the MS MARCO passage ranking task~\cite{nogueira2019passage}. Its effectiveness on standard document retrieval tasks remains to be studied.

%Besides the good performance, BERT has several points that make it a good fit for IR tasks. First, prior neural IR research show that it is crucial for a nerual IR model to model query-document word interactions. However, most pre-trained word embeeding or language models only generate word or sentence vectors, but requires extensive archtiecture engineering to design architectures for the search task. BERT's attention based architecture is essentially modeling word-word interactions, so that the model archtiecture already support query-document interaction, making it possible to simply take the pre-trained model without adding task-specific layers (and to train these parameters). Second, BERT uses multi-head attention, each attention capturing a different type of word associations (same word, next word, synonyms, etc). This aligns with ~\citep{K-NRM}'s findings that having multiple types of word associations are beneficial for search tasks. 



==> sections/visualization/03.tex <==
\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut All} \colorbox{red!1}{\strut These} \colorbox{red!11}{\strut Things} \colorbox{red!0}{\strut LyricsThird} \colorbox{red!12}{\strut Eye} \colorbox{red!0}{\strut BlindDopamineLyrics} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut These} \colorbox{red!11}{\strut Things} \colorbox{red!0}{\strut Lyricsmania} \colorbox{red!0}{\strut staff} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut working} \colorbox{red!0}{\strut hard} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut These} \colorbox{red!11}{\strut Things} \colorbox{red!11}{\strut lyrics} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut soon} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut released} \colorbox{red!0}{\strut by} \colorbox{red!12}{\strut Third} \colorbox{red!12}{\strut Eye} \colorbox{red!12}{\strut Blind} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut check} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut soon} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut lyrics} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut These} \colorbox{red!11}{\strut Things} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut send} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fill} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Artist} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Third} \colorbox{red!12}{\strut Eye} \colorbox{red!12}{\strut Blind} \colorbox{red!11}{\strut lyrics} \colorbox{red!0}{\strut Album} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Dopamine} \colorbox{red!1}{\strut Title} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut These} \colorbox{red!11}{\strut Things} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut E-Mail} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Lyrics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Print} 
}}}
\end{CJK*}


D2233036

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Santiago} \colorbox{red!6}{\strut Calatrava} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!7}{\strut World} \colorbox{red!7}{\strut Trade} \colorbox{red!7}{\strut Center} \colorbox{red!3}{\strut Transportation} \colorbox{red!3}{\strut Hub} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut nothing} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut beams} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cranes} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut recently} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut essence} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut structure} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut finally} \colorbox{red!0}{\strut beginning} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut emerge} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!8}{\strut Port} \colorbox{red!7}{\strut Authority} \colorbox{red!0}{\strut released} \colorbox{red!2}{\strut new} \colorbox{red!0}{\strut images} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut week} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut interior} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 800,000-square-foot} \colorbox{red!1}{\strut structure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut Oculus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut revealing} \colorbox{red!0}{\strut white} \colorbox{red!0}{\strut marble} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut soaring} \colorbox{red!0}{\strut articulated} \colorbox{red!0}{\strut ribs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut opulence} \colorbox{red!0}{\strut doesn} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut cheap} \colorbox{red!0}{\strut though} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut project} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut turning} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut expensive} \colorbox{red!0}{\strut train} \colorbox{red!0}{\strut stations} \colorbox{red!0}{\strut ever.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut World} \colorbox{red!7}{\strut Trade} \colorbox{red!7}{\strut Center} \colorbox{red!3}{\strut Transportation} \colorbox{red!3}{\strut Hub} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut going} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut serve} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut critical} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut functional} \colorbox{red!3}{\strut transportation} \colorbox{red!1}{\strut purpose} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut Patrick} \colorbox{red!0}{\strut J.} \colorbox{red!2}{\strut Foye} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!0}{\strut Times} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.74} \colorbox{red!0}{\strut billion} \colorbox{red!0}{\strut dollar} \colorbox{red!1}{\strut project} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut criticism} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut expanding} \colorbox{red!0}{\strut budget} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut originally} \colorbox{red!0}{\strut estimated} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut billion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut extended} \colorbox{red!2}{\strut completion} \colorbox{red!0}{\strut date} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut going} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut viewed} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut grand} \colorbox{red!0}{\strut public} \colorbox{red!0}{\strut space.} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Foye} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut executive} \colorbox{red!0}{\strut director} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut Port} \colorbox{red!7}{\strut Authority} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut New} \colorbox{red!1}{\strut Jersey} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut owner} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut trade} \colorbox{red!7}{\strut center} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut builder} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut hub} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut serve} \colorbox{red!0}{\strut 200,000} \colorbox{red!0}{\strut subway} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut PATH} \colorbox{red!0}{\strut train} \colorbox{red!0}{\strut commuters} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut day.The} \colorbox{red!8}{\strut Port} \colorbox{red!7}{\strut Authority} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut establishing} \colorbox{red!0}{\strut plans} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut rent} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut sections} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut hub} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut private} \colorbox{red!0}{\strut events} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut charity} \colorbox{red!0}{\strut fundraisers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut art} \colorbox{red!0}{\strut shows} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut perhaps} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut weddings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut blocked} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut public} \colorbox{red!0}{\strut commuters} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Special} \colorbox{red!0}{\strut infrastructure} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut screens} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lighting} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sound} \colorbox{red!0}{\strut systems} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut installed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut ensure} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut events} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut served} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut dramatic} \colorbox{red!0}{\strut effect} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut structure.The} \colorbox{red!0}{\strut multistory} \colorbox{red!3}{\strut hub} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut equivalent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut two-and-a-half} \colorbox{red!0}{\strut Grand} \colorbox{red!0}{\strut Central} \colorbox{red!0}{\strut Terminals} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut fit} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut project} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut doubled} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut costs} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut expanding} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut originally} \colorbox{red!0}{\strut estimated} \colorbox{red!0}{\strut four-year} \colorbox{red!2}{\strut completion} \colorbox{red!0}{\strut date} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut ten} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Completion} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut PATH} \colorbox{red!0}{\strut passenger} \colorbox{red!0}{\strut platforms} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut slated} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut year.} \colorbox{red!4}{\strut Santiago} \colorbox{red!0}{\strut Calatrava} \colorbox{red!8}{\strut Port} \colorbox{red!7}{\strut Authority} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut New} \colorbox{red!0}{\strut JerseyVia} \colorbox{red!0}{\strut Archpaper} 
}}}
\end{CJK*}


D23522_passage_0_11

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!12}{\strut Region} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut TurkeyMediterranean} \colorbox{red!12}{\strut region} \colorbox{red!0}{\strut takes} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!0}{\strut Sea} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut occupies} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!11}{\strut Turkey} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut 120.000} \colorbox{red!0}{\strut square} \colorbox{red!0}{\strut kilometers} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut land} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut bordered} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Aegean} \colorbox{red!12}{\strut Region} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut west} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Central} \colorbox{red!0}{\strut Anatolia} \colorbox{red!12}{\strut Region} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut north} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Eastern} \colorbox{red!0}{\strut Anatolia} \colorbox{red!12}{\strut Region} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut northeast} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Southeastern} \colorbox{red!0}{\strut Anatolia} \colorbox{red!12}{\strut Region} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut east} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Syria} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut southeast} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!0}{\strut Sea} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut south} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Mid-Taurus} \colorbox{red!0}{\strut mountains} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut parallel} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut coast} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Because} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut steep} \colorbox{red!0}{\strut mountains} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut valleys} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sea} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut mountain} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut narrow} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut width} \colorbox{red!0}{\strut varies} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 120-180} \colorbox{red!0}{\strut kilometers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut rivers} \colorbox{red!0}{\strut rising} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Spring} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut snow} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut melting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut lakes} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut highlands} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut nature} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut population} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut concentrated} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut locations} \colorbox{red!0}{\strut suitable} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut agriculture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tourism} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut commerce.The} \colorbox{red!0}{\strut plains} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!12}{\strut region} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut rich} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut agricultural} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fertile} \colorbox{red!0}{\strut soils} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut warm} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!3}{\strut climate} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut ideal} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut growing} \colorbox{red!0}{\strut citrus} \colorbox{red!0}{\strut fruits} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut grapes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cereals} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut irrigated} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rice} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cotton} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Summers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut hot} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut droughts} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut uncommon} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut industrial} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut agricultural} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut wheat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut barley} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tobacco} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut green} \colorbox{red!0}{\strut houses} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut carpet} \colorbox{red!0}{\strut weaving} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut aluminum} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut steel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut of} \colorbox{red!11}{\strut Turkey} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut oranges} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut mandarins} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut grown} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut meanwhile} \colorbox{red!0}{\strut bananas} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut region.Climate} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut nature} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!12}{\strut Region} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!3}{\strut climate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut characterized} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut warm} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut relatively} \colorbox{red!0}{\strut humid} \colorbox{red!0}{\strut winters} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut hot} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut dry} \colorbox{red!0}{\strut summers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Temperatures} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut winter} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut 24C} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut reach} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut upper} \colorbox{red!0}{\strut 30ssProvinces} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Antalya} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Adana} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mersin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hatay} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Isparta} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Burdur} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Kahramanmaras} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Osmaniye} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}


D2343647_passage_0_13

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Interested} \colorbox{red!5}{\strut Person} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Probate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Law} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Legal} \colorbox{red!0}{\strut DefinitionAn} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut whose} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut relationship} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut affected} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut appointment} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut guardian} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut conservator} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut An} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut property} \colorbox{red!0}{\strut interests} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut affected} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut probate} \colorbox{red!0}{\strut proceedings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut ward} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut considered} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut an} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut appointment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut nominated} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut guardian} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut conservator} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Interested} \colorbox{red!5}{\strut persons} \colorbox{red!0}{\strut include} \colorbox{red!1}{\strut legal} \colorbox{red!0}{\strut representatives} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut spouse} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut parents} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adult} \colorbox{red!0}{\strut children} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adult} \colorbox{red!0}{\strut siblings} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut adults} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Government} \colorbox{red!0}{\strut agencies} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut health} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut agents} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut proxies} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut be} \colorbox{red!5}{\strut interested} \colorbox{red!0}{\strut persons.Pursuant} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Section} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut 201} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Uniform} \colorbox{red!3}{\strut Probate} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut persons} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut heirs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut devisees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut children} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut spouses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut creditors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut beneficiaries} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut property} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut claim} \colorbox{red!0}{\strut against} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut trust} \colorbox{red!0}{\strut estate} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut estate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut decedent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ward} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut protected} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Interested} \colorbox{red!5}{\strut persons} \colorbox{red!0}{\strut include} \colorbox{red!5}{\strut persons} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut priority} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut appointment} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut personal} \colorbox{red!0}{\strut representative} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut fiduciaries} \colorbox{red!0}{\strut representing} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut persons} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut meaning} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut term} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut varies} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut meaning} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut determined} \colorbox{red!0}{\strut according} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut particular} \colorbox{red!0}{\strut purposes} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut matter} \colorbox{red!0}{\strut involved} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut proceeding.In} \colorbox{red!0}{\strut Spicer} \colorbox{red!0}{\strut v.} \colorbox{red!0}{\strut Estate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Spicer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 55} \colorbox{red!0}{\strut Ark} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut App} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 267} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 268} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ark} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ct.} \colorbox{red!0}{\strut App} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1996} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut an} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut defined} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut heir} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut devisee} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut spouse} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut creditor} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut property} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut interest} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut claim} \colorbox{red!0}{\strut against} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut estate} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut administered} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fiduciary} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut An} \colorbox{red!5}{\strut interested} \colorbox{red!5}{\strut person} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut contest} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut probate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut thereof} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut stating} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut writing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut grounds} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut objection} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut filing} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut court.Legal} \colorbox{red!3}{\strut Definition} \colorbox{red!0}{\strut listInterested} \colorbox{red!5}{\strut Person} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Probate} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Interested} \colorbox{red!5}{\strut Person} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Guardianship} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Interested} \colorbox{red!0}{\strut Governmental} \colorbox{red!0}{\strut ParticipantInterested} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut PartyInterest-Only} \colorbox{red!0}{\strut StripInterests} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Property} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Internal} \colorbox{red!0}{\strut Revenue} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Interfaith} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Corporate} \colorbox{red!0}{\strut ResponsibilityInterferenceInterference} \colorbox{red!0}{\strut Proceedings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Trademark} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Interference} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut OfficerInterference} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut BurialRelated} \colorbox{red!1}{\strut Legal} \colorbox{red!0}{\strut TermsAbsent} \colorbox{red!0}{\strut PersonAccidental} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut InjuryAccountable} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut PropertyActio} \colorbox{red!0}{\strut Personalis} \colorbox{red!0}{\strut Moritur} \colorbox{red!0}{\strut Cum} \colorbox{red!0}{\strut PersonaAction} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut PersonamActus} \colorbox{red!0}{\strut Inceptus} \colorbox{red!0}{\strut Cujus} \colorbox{red!0}{\strut Perfectio} \colorbox{red!0}{\strut Pendet} \colorbox{red!0}{\strut Ex} \colorbox{red!0}{\strut Voluntate} \colorbox{red!0}{\strut Partium} \colorbox{red!0}{\strut Revocari} \colorbox{red!0}{\strut Potest} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Si} \colorbox{red!0}{\strut Autem} \colorbox{red!0}{\strut Pendet} \colorbox{red!0}{\strut Ex} \colorbox{red!0}{\strut Voluntate} \colorbox{red!0}{\strut Tertiae} \colorbox{red!0}{\strut Personae} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Vel} \colorbox{red!0}{\strut Ex} \colorbox{red!0}{\strut Contingenti} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut RevocarAdministration} \colorbox{red!0}{\strut Expenses} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Probate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adverse} \colorbox{red!0}{\strut Personnel} \colorbox{red!0}{\strut ActionAffiliated} \colorbox{red!5}{\strut Persons} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Securities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Agency} \colorbox{red!0}{\strut Designee} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Administrative} \colorbox{red!0}{\strut Personnel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}


D2459260 passage 0-14

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 15} \colorbox{red!4}{\strut Best} \colorbox{red!6}{\strut Herbal} \colorbox{red!15}{\strut Tea} \colorbox{red!13}{\strut Ingredients} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut HealingJackie} \colorbox{red!0}{\strut LeavittMarch} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2045} \colorbox{red!0}{\strut PMShare} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Staring} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut grocery} \colorbox{red!0}{\strut store} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut wall} \colorbox{red!0}{\strut of} \colorbox{red!14}{\strut teas} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut intimidating} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut options} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut scan} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut picking} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut eventually} \colorbox{red!0}{\strut ring} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut register} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut purpose} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut soothing} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut throat} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut helping} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut lose} \colorbox{red!0}{\strut weight} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut tasting} \colorbox{red!0}{\strut pretty} \colorbox{red!0}{\strut darn} \colorbox{red!1}{\strut good} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Having} \colorbox{red!0}{\strut recently} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut sick} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut combination} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut allergies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut move} \colorbox{red!0}{\strut cross} \colorbox{red!0}{\strut country} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut plants} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut assume} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut common} \colorbox{red!0}{\strut cold} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut instead} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut going} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut buy} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!14}{\strut teas} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut ailments} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut concocted} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ginger} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut garlic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rosemary} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tumeric} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut oregano} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut plus} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut honey} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Making} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut own} \colorbox{red!15}{\strut tea} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut surprisingly} \colorbox{red!0}{\strut simple} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut like} \colorbox{red!1}{\strut making} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut soup} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut whole} \colorbox{red!0}{\strut bunch} \colorbox{red!0}{\strut of} \colorbox{red!13}{\strut ingredients} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut chop} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut throw} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut boiling} \colorbox{red!0}{\strut pot} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut five} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut ten} \colorbox{red!0}{\strut minutes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut strain} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut flavored} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut favorite} \colorbox{red!0}{\strut mug.The} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut figure} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut what} \colorbox{red!13}{\strut ingredients} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut So} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!3}{\strut helpful} \colorbox{red!15}{\strut tea} \colorbox{red!13}{\strut ingredients} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut health} \colorbox{red!1}{\strut food} \colorbox{red!0}{\strut store} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut combat} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut ailments} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut experience.1} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Ginger} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Anti-viral} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Containing} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut dozen} \colorbox{red!1}{\strut antiviral} \colorbox{red!6}{\strut compounds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut pain-relieving} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut antiseptic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut antioxidant} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Helps} \colorbox{red!0}{\strut prevent} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut treats} \colorbox{red!1}{\strut colds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sore} \colorbox{red!1}{\strut throats} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut inflamation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut mucus} \colorbox{red!0}{\strut membranes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut reduces} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fever} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut mild} \colorbox{red!0}{\strut sedative} \colorbox{red!0}{\strut effect} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut encourages} \colorbox{red!0}{\strut rest.2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Echinacea} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut leaves} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut flower} \colorbox{red!0}{\strut petals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Anti-bacterial} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Increases} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut properdin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut chemical} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut activates} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut immune} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut responsible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut increasing} \colorbox{red!0}{\strut defence} \colorbox{red!0}{\strut mechanisms} \colorbox{red!0}{\strut against} \colorbox{red!2}{\strut viral} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut bacterial} \colorbox{red!0}{\strut attacks.3} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Garlic} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Anti-bacterial} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-fungal} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Contains} \colorbox{red!0}{\strut several} \colorbox{red!3}{\strut helpful} \colorbox{red!0}{\strut immune-boosting} \colorbox{red!6}{\strut compounds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!1}{\strut allicin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut potent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut natural} \colorbox{red!1}{\strut antibiotic} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}


D2459260 passage 15-39

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Best} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut raw.4} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Goldenseal} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Anti-viral} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-bacterial} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-fungal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut both} \colorbox{red!3}{\strut antiseptic} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut immune} \colorbox{red!1}{\strut stimulating} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut increasing} \colorbox{red!10}{\strut blood} \colorbox{red!0}{\strut supply} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut spleen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut chemical} \colorbox{red!1}{\strut berberine} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut goldenseal} \colorbox{red!0}{\strut activates} \colorbox{red!0}{\strut white} \colorbox{red!10}{\strut blood} \colorbox{red!0}{\strut cells} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut destruct} \colorbox{red!0}{\strut bacteria} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fungi} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut viruses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tumour} \colorbox{red!0}{\strut cells.5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sage} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Antiseptic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-bacterial} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sooths} \colorbox{red!0}{\strut sore} \colorbox{red!0}{\strut throats} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut promotes} \colorbox{red!4}{\strut good} \colorbox{red!0}{\strut digestion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut helps} \colorbox{red!0}{\strut ease} \colorbox{red!0}{\strut menstrual} \colorbox{red!0}{\strut cramps.6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Peppermint} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut painkiller} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut headaches} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut reduces} \colorbox{red!0}{\strut fevers} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut inducing} \colorbox{red!0}{\strut sweating} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cooling} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut body} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut it} \colorbox{red!3}{\strut helps} \colorbox{red!0}{\strut bring} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut mucus} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lungs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut bronchi} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut trachea} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut bronchitis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut colds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut flu.7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Blackberry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut leaves} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut fruit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut fruit} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut rich} \colorbox{red!0}{\strut in} \colorbox{red!10}{\strut vitamin} \colorbox{red!5}{\strut C} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut leaves} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut teas.8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Cinnamon} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Anti-bacterial} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut antiviral} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut antifungal} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Helps} \colorbox{red!1}{\strut stop} \colorbox{red!0}{\strut vomiting} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut relieve} \colorbox{red!0}{\strut nausea} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut increases} \colorbox{red!0}{\strut restricted} \colorbox{red!10}{\strut blood} \colorbox{red!0}{\strut flow.9} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Clove} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Antiviral} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut antifungal} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut antimicrobial} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut antioxidant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-inflammatory} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Helps} \colorbox{red!0}{\strut fight} \colorbox{red!0}{\strut infection} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ease} \colorbox{red!0}{\strut pain.10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lemon} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Another} \colorbox{red!0}{\strut rich} \colorbox{red!0}{\strut source} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut vitamin} \colorbox{red!5}{\strut C} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut squeeze} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut tea.11} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Chamomile} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Anti-fungal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-bacterial} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut antiseptic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-inflammatory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Natural} \colorbox{red!0}{\strut sedative.12} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lemongrass} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Antibacterial} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-inflammatory} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-parasitic} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut antifungal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Relieves} \colorbox{red!0}{\strut digestive} \colorbox{red!0}{\strut ailments} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fluid} \colorbox{red!0}{\strut retention} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut improves} \colorbox{red!10}{\strut blood} \colorbox{red!1}{\strut circulation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dilates} \colorbox{red!10}{\strut blood} \colorbox{red!0}{\strut vessels.13} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Oregano} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut tonic} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut immune} \colorbox{red!0}{\strut booster.14} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rosemary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Antibacterial} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut antiseptic} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut antiparasitic} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut antifungal} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Good} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nerves} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut stimulating} \colorbox{red!0}{\strut effect.15} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tumeric} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Antioxident} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-imflammatory} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut antifungal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut anticancer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!10}{\strut blood} \colorbox{red!0}{\strut purifier} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut helps} \colorbox{red!0}{\strut lower} \colorbox{red!10}{\strut blood} \colorbox{red!1}{\strut sugar} \colorbox{red!0}{\strut levels.} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut food} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut healing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut healthy} \colorbox{red!6}{\strut foods} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut healthy} \colorbox{red!0}{\strut recipes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mind} \colorbox{red!0}{\strut body} \colorbox{red!0}{\strut connectionJackie} \colorbox{red!0}{\strut LeavittJackie} \colorbox{red!0}{\strut Leavitt} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut traveler} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut passion} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut writing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Or} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut writer} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut passion} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut travel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut She} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut lives} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Francisco} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pursuing} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut loves} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dabbling} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut PostsSpiritualityWhat} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Mercury} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Says} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut How} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Voice} \colorbox{red!0}{\strut HeardThe} \colorbox{red!0}{\strut AstroTwinsRecovery5} \colorbox{red!0}{\strut Things} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Need} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Know} \colorbox{red!0}{\strut Today} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2018} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Gretchen} \colorbox{red!0}{\strut LidickerPersonal} \colorbox{red!0}{\strut GrowthThe} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut Self-Care} \colorbox{red!0}{\strut Topic} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut Wants} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Talk} \colorbox{red!0}{\strut AboutKrysten} \colorbox{red!0}{\strut Peck} 
}}}
\end{CJK*}


D1359598 passage 0-11

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Pouch} \colorbox{red!0}{\strut ProcessingT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Scott} \colorbox{red!0}{\strut Williams} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Vice} \colorbox{red!0}{\strut President} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Allpax} \colorbox{red!0}{\strut ProductsIntroductionThere} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut doubt} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut advantages} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut packaging} \colorbox{red!0}{\strut food} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut retort} \colorbox{red!8}{\strut pouch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Generally} \colorbox{red!4}{\strut processing} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut reduced} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut comparable} \colorbox{red!0}{\strut sized} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut jar} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut cylindrical} \colorbox{red!0}{\strut container} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut additional} \colorbox{red!1}{\strut advantages} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut reduced} \colorbox{red!0}{\strut shipping} \colorbox{red!0}{\strut costs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut storage} \colorbox{red!0}{\strut space} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut empty} \colorbox{red!0}{\strut containers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!8}{\strut pouch} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut shelf} \colorbox{red!0}{\strut appeal} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut growing} \colorbox{red!0}{\strut acceptance} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut consumers.There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut many} \colorbox{red!4}{\strut processing} \colorbox{red!0}{\strut challenges} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut retortable} \colorbox{red!8}{\strut pouch} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut metal} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut significant} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut pouch} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut fill} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut seal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut handle} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut equipment} \colorbox{red!0}{\strut needed} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut fill} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut seal} \colorbox{red!8}{\strut pouches} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut sophisticated} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut expensive} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut sealing} \colorbox{red!1}{\strut equipment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut handling} \colorbox{red!0}{\strut systems} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut pouch} \colorbox{red!2}{\strut loaders} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut unloaders} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .The} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut follows} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut overview} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut covers} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut considerations} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut taken} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut planning} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut designing} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut retort} \colorbox{red!8}{\strut pouch} \colorbox{red!0}{\strut line.Major} \colorbox{red!1}{\strut Equipment} \colorbox{red!0}{\strut ComponentsThere} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut seven} \colorbox{red!0}{\strut major} \colorbox{red!1}{\strut equipment} \colorbox{red!0}{\strut categories} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut comprise} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut retort} \colorbox{red!8}{\strut pouch} \colorbox{red!1}{\strut line} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Pouch} \colorbox{red!0}{\strut FillerPouch} \colorbox{red!0}{\strut LoaderTrays} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut house} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut pouches} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut stacked} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut cubesRetortsRetort} \colorbox{red!1}{\strut Loading} \colorbox{red!1}{\strut System} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Drone} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ribbi} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Conveyor} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut Retort} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Shuttle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Manually} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Pouch} \colorbox{red!0}{\strut UnloaderCase} \colorbox{red!0}{\strut PackerFor} \colorbox{red!0}{\strut reference} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut red} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut produced} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Allpax} \colorbox{red!0}{\strut Products.In} \colorbox{red!0}{\strut designing} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut pouch} \colorbox{red!1}{\strut line} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut desired} \colorbox{red!1}{\strut line} \colorbox{red!0}{\strut speed} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut drives} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut decisions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut line} \colorbox{red!0}{\strut speed} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut dictate} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut brand} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut pouch} \colorbox{red!0}{\strut fillersealer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut fillersealer} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut characteristic} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut format} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut filled} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut sealed} \colorbox{red!8}{\strut pouches} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut single} \colorbox{red!0}{\strut file} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut strong} \colorbox{red!0}{\strut possibility} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut fillersealer} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut line.The} \colorbox{red!0}{\strut piece} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut equipment} \colorbox{red!0}{\strut immediately} \colorbox{red!0}{\strut downstream} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut fillersealer} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut pouch} \colorbox{red!1}{\strut loading} \colorbox{red!0}{\strut station} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut loader} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut collate} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut pouches} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut manner} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut placed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut racking} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

D1359598 passage 12-23

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut fillersealer} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut fillersealers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut loader} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut presented} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut pouches} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut single} \colorbox{red!0}{\strut file} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut two} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut four} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut fillersealer} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut direct} \colorbox{red!0}{\strut impact} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut design} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut loader} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut detail} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut presented} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut below.Tray} \colorbox{red!0}{\strut DesignAllpax} \colorbox{red!0}{\strut 304L} \colorbox{red!0}{\strut stainless} \colorbox{red!1}{\strut steel} \colorbox{red!3}{\strut pouch} \colorbox{red!0}{\strut racksOnce} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut speed} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut filler} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut sealer} \colorbox{red!0}{\strut decision} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tray} \colorbox{red!2}{\strut design} \colorbox{red!0}{\strut becomes} \colorbox{red!0}{\strut critical} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut layout} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut pattern} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut rack} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut efficiently} \colorbox{red!1}{\strut work} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut robotic} \colorbox{red!3}{\strut pouch} \colorbox{red!2}{\strut loader} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut loader} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut operate} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut efficiently} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut highest} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut speed} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut rows} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut rack} \colorbox{red!0}{\strut match} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut devisable} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut rows} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut filler} \colorbox{red!0}{\strut sealers.For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut two} \colorbox{red!2}{\strut filler} \colorbox{red!2}{\strut sealers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut lanes} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut pouches} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut optimal} \colorbox{red!9}{\strut rack} \colorbox{red!2}{\strut design} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut 12} \colorbox{red!1}{\strut rows} \colorbox{red!1}{\strut wide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut devisable} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut lanes} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut produced} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!9}{\strut rack} \colorbox{red!2}{\strut design} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut 9} \colorbox{red!1}{\strut rows} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut work.Once} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut conceptual} \colorbox{red!9}{\strut rack} \colorbox{red!2}{\strut design} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut done} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut retort} \colorbox{red!0}{\strut sizing} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut sometime} \colorbox{red!0}{\strut necessary} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut revisit} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut pouch} \colorbox{red!3}{\strut size} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut change} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut dimensions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut pouch} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut sometime} \colorbox{red!0}{\strut greatly} \colorbox{red!0}{\strut enhance} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut efficiency} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut design.Pouches} \colorbox{red!10}{\strut racks} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut fabricated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut two} \colorbox{red!0}{\strut ways} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stainless} \colorbox{red!1}{\strut steel} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut aluminum} \colorbox{red!0}{\strut constructionInjection} \colorbox{red!0}{\strut molded} \colorbox{red!0}{\strut plastic} \colorbox{red!0}{\strut constructionAllpax} \colorbox{red!1}{\strut injection} \colorbox{red!0}{\strut molded} \colorbox{red!0}{\strut trays} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut GE} \colorbox{red!0}{\strut resinsBoth} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut stainless} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut plastic} \colorbox{red!10}{\strut racks} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut advantages} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut disadvantages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stainless} \colorbox{red!10}{\strut racks} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut long} \colorbox{red!0}{\strut service} \colorbox{red!1}{\strut life} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut produced} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut numbers} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut individual} \colorbox{red!8}{\strut cost} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Injection} \colorbox{red!0}{\strut molded} \colorbox{red!10}{\strut racks} \colorbox{red!0}{\strut typically} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut 110} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut stainless} \colorbox{red!1}{\strut steel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tooling} \colorbox{red!8}{\strut cost} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 100,000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Plastic} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut choice} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut rack} \colorbox{red!3}{\strut size} \colorbox{red!0}{\strut exceeds} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 40.Allpax} \colorbox{red!0}{\strut basketIn} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut basket} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cans} \colorbox{red!0}{\strut nest} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pattern} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut themselves} \colorbox{red!0}{\strut into} \colorbox{red!1}{\strut rows} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut columns} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut separated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut thin} \colorbox{red!0}{\strut divider} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut slip} \colorbox{red!0}{\strut sheet} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

D1359598 passage 24-37

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut Pouches} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut placed} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tray} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut cradle} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut protect} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut integrity} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut prevent} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut other} \colorbox{red!7}{\strut pouches} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut resting} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut tray} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut simple} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut well} \colorbox{red!1}{\strut designed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut stiff} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!5}{\strut loader} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut stack} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut destack} \colorbox{red!0}{\strut cubes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut incorporate} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut promotes} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut thermal} \colorbox{red!0}{\strut distribution} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut allow} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut adequate} \colorbox{red!1}{\strut flow} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut strong} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut allow} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut load} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut whole} \colorbox{red!0}{\strut cube} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut supported} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut frame} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut burrs} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut defects} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut damage} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut integrity} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut pouch.Handling} \colorbox{red!0}{\strut PouchesAllpax} \colorbox{red!0}{\strut Model} \colorbox{red!1}{\strut 400x} \colorbox{red!0}{\strut high} \colorbox{red!1}{\strut speed} \colorbox{red!0}{\strut loaderAs} \colorbox{red!0}{\strut stated} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut decisions} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut flow} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut line} \colorbox{red!1}{\strut speed} \colorbox{red!0}{\strut definition} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!0}{\strut geometry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut cans} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut line} \colorbox{red!1}{\strut speeds} \colorbox{red!0}{\strut for} \colorbox{red!7}{\strut pouch} \colorbox{red!1}{\strut lines} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut generally} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut slower.The} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut aspect} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut understanding} \colorbox{red!7}{\strut pouch} \colorbox{red!3}{\strut handling} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut break} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut preconceived} \colorbox{red!0}{\strut notion} \colorbox{red!0}{\strut that} \colorbox{red!7}{\strut pouches} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut similar} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut cans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut quote} \colorbox{red!0}{\strut about} \colorbox{red!7}{\strut pouch} \colorbox{red!2}{\strut loading} \colorbox{red!0}{\strut equipment} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut recent} \colorbox{red!0}{\strut newsletters} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Allpax} \colorbox{red!1}{\strut 400x} \colorbox{red!7}{\strut pouch} \colorbox{red!1}{\strut staging} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 4} \colorbox{red!1}{\strut fillers} \colorbox{red!0}{\strut producing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 2-up} \colorbox{red!0}{\strut patternOne} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut misconceptions} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut folks} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut regarding} \colorbox{red!7}{\strut pouches} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut material} \colorbox{red!3}{\strut handling} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut cans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut untrue} \colorbox{red!0}{\strut !} \colorbox{red!7}{\strut Pouches} \colorbox{red!0}{\strut behave} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut differently} \colorbox{red!0}{\strut than} \colorbox{red!1}{\strut cans} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut require} \colorbox{red!0}{\strut completely} \colorbox{red!0}{\strut different} \colorbox{red!3}{\strut handling} \colorbox{red!0}{\strut techniques} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Cans} \colorbox{red!0}{\strut behave} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut well-trained} \colorbox{red!0}{\strut soldiers} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut stay} \colorbox{red!0}{\strut organized} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut move} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut unison} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut hand} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut pouches} \colorbox{red!0}{\strut behave} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut felines} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut uncooperative.The} \colorbox{red!7}{\strut pouch} \colorbox{red!5}{\strut loader} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut stage} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tray} \colorbox{red!0}{\strut pattern} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut relate} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut manner} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut pouch} \colorbox{red!1}{\strut filler} \colorbox{red!0}{\strut feeds} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut loader} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Pouches} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut staged} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tray} \colorbox{red!0}{\strut pattern} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pneumatic} \colorbox{red!0}{\strut pick} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut head} \colorbox{red!0}{\strut lifts} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut staged} \colorbox{red!0}{\strut pattern} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut places} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tray} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}


D1359598 passage 38-52

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!0}{\strut fully} \colorbox{red!0}{\strut loaded} \colorbox{red!0}{\strut tray} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut stacked} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut create} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut cube} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut cube} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut roughly} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut shape} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut retort} \colorbox{red!0}{\strut basket.Retort} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Cube} \colorbox{red!0}{\strut CapacityOne} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut tradeoff} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut note} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut considering} \colorbox{red!1}{\strut pouches} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut won} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut quantity} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut pouches} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut retort} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut cans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Again} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nature} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut cans} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut nest} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut overlapping} \colorbox{red!0}{\strut rows} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut columns} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut pouch} \colorbox{red!0}{\strut eats} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lot} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut room} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut reside} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut compartment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Take} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut comparative} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut capacities} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Allpax} \colorbox{red!0}{\strut Jumbo} \colorbox{red!0}{\strut 6-basketcube} \colorbox{red!0}{\strut spray} \colorbox{red!9}{\strut retort} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut oz} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 85} \colorbox{red!0}{\strut gram} \colorbox{red!0}{\strut pouch3oz} \colorbox{red!1}{\strut Cans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6156085g} \colorbox{red!1}{\strut Pouches} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 95mm} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 125mm} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 20mm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 22032The} \colorbox{red!9}{\strut Retort} \colorbox{red!3}{\strut Process} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Overpressure} \colorbox{red!0}{\strut RetortsSterilization} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pouch} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut accomplished} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut overpressure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut means} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut air} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut retort} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut sterilization} \colorbox{red!0}{\strut phases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut process} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut come-up} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cook} \colorbox{red!0}{\strut phases} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut three} \colorbox{red!6}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut process} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut perform} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut overpressure} \colorbox{red!3}{\strut process} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut describes} \colorbox{red!0}{\strut these} \colorbox{red!3}{\strut process} \colorbox{red!0}{\strut types.General} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Overpressure} \colorbox{red!9}{\strut retorts} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut required} \colorbox{red!0}{\strut when} \colorbox{red!2}{\strut sterilizing} \colorbox{red!0}{\strut glass} \colorbox{red!1}{\strut containers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut flexible} \colorbox{red!1}{\strut pouches} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut semi-rigid} \colorbox{red!0}{\strut plastic} \colorbox{red!1}{\strut containers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut tend} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut complex} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut expensive} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut comparable} \colorbox{red!0}{\strut sized} \colorbox{red!1}{\strut steam} \colorbox{red!9}{\strut retorts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut pumps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut motors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut drive} \colorbox{red!0}{\strut units} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut automated} \colorbox{red!0}{\strut valves} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sophisticated} \colorbox{red!0}{\strut controls} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut three} \colorbox{red!6}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut overpressure} \colorbox{red!9}{\strut retorts} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut commonly} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Full} \colorbox{red!1}{\strut water} \colorbox{red!1}{\strut immersion} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Water} \colorbox{red!0}{\strut spraysteam-air} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Forced} \colorbox{red!0}{\strut SteamAir} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut fan} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut brief} \colorbox{red!0}{\strut discussion} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut follows.Allpax} \colorbox{red!0}{\strut Model} \colorbox{red!0}{\strut 1600} \colorbox{red!1}{\strut water} \colorbox{red!1}{\strut immersion} \colorbox{red!0}{\strut retortWater} \colorbox{red!1}{\strut immersion} \colorbox{red!9}{\strut retorts} \colorbox{red!0}{\strut generally} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut flexibility} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut processing} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut container} \colorbox{red!6}{\strut types} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Water} \colorbox{red!1}{\strut immersion} \colorbox{red!9}{\strut retorts} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut effectively} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut rotary} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut non} \colorbox{red!0}{\strut rotary} \colorbox{red!0}{\strut modes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut will} \colorbox{red!3}{\strut process} \colorbox{red!0}{\strut all} \colorbox{red!6}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut containers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut accommodate} \colorbox{red!1}{\strut containers} \colorbox{red!0}{\strut loaded} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dense} \colorbox{red!0}{\strut pack} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut configurations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut i.e} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut cans} \colorbox{red!0}{\strut stacked} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut divider} \colorbox{red!0}{\strut sheets} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Full} \colorbox{red!1}{\strut immersion} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut partial} \colorbox{red!1}{\strut immersion} \colorbox{red!3}{\strut processes} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut providing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut wide} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut processing} \colorbox{red!0}{\strut flexibility} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}



==> sections/visualization/cwbloss.tex <==
query: mitchell college

98:mitchell, 97:colleges, 96:college, 40:costs, 28:enrollment, 28:enrolled, 21:new, 21:london, 19:students, 19:average


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Mitchell} \colorbox{red!8}{\strut College} \colorbox{red!1}{\strut 437} \colorbox{red!1}{\strut Pequot} \colorbox{red!0}{\strut Avenue} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut London} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut CT} \colorbox{red!0}{\strut 06320-4498} \colorbox{red!0}{\strut Office} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Admissions} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Financial} \colorbox{red!1}{\strut Aid} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 443-2811} \colorbox{red!0}{\strut FAX} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 860} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 444-4498} \colorbox{red!0}{\strut e-mail} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut admissions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mitchell.edu} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.mitchell.edu} \colorbox{red!2}{\strut ENROLLMENT} \colorbox{red!0}{\strut Full-time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Total} \colorbox{red!0}{\strut 708} \colorbox{red!1}{\strut men} \colorbox{red!0}{\strut 427women} \colorbox{red!0}{\strut 281} \colorbox{red!0}{\strut Part-time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Total} \colorbox{red!0}{\strut 120} \colorbox{red!1}{\strut men} \colorbox{red!0}{\strut 41women} \colorbox{red!0}{\strut 79} \colorbox{red!1}{\strut FRESHMAN} \colorbox{red!1}{\strut ADMISSION} \colorbox{red!0}{\strut PROFILE} \colorbox{red!1}{\strut Number} \colorbox{red!1}{\strut who} \colorbox{red!1}{\strut applied} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1024} \colorbox{red!1}{\strut Number} \colorbox{red!1}{\strut accepted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 641} \colorbox{red!1}{\strut Number} \colorbox{red!2}{\strut enrolled} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 346} \colorbox{red!2}{\strut Average} \colorbox{red!1}{\strut SAT} \colorbox{red!1}{\strut scores} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut V} \colorbox{red!0}{\strut 500} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut 500} \colorbox{red!2}{\strut Average} \colorbox{red!1}{\strut ACT} \colorbox{red!1}{\strut score} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19} \colorbox{red!1}{\strut Freshman} \colorbox{red!1}{\strut retention} \colorbox{red!0}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2006-2007} \colorbox{red!3}{\strut COSTS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tuition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19,199} \colorbox{red!1}{\strut Room} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9,268} \colorbox{red!1}{\strut Fees} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 929} \colorbox{red!1}{\strut FINANCIAL} \colorbox{red!1}{\strut AID} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Freshmen} \colorbox{red!1}{\strut receiving} \colorbox{red!1}{\strut aid} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 85} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Average} \colorbox{red!1}{\strut financial} \colorbox{red!1}{\strut aid} \colorbox{red!0}{\strut package} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8,000} \colorbox{red!1}{\strut FACULTY} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Full-time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut Part-time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut Ph.D.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut Student-faculty} \colorbox{red!0}{\strut ratio} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121} \colorbox{red!0}{\strut IN} \colorbox{red!0}{\strut ADDITION} \colorbox{red!8}{\strut Mitchell} \colorbox{red!8}{\strut College} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut built} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut reputation} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut giving} \colorbox{red!2}{\strut students} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut outstanding} \colorbox{red!0}{\strut foundation} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut their} \colorbox{red!8}{\strut college} \colorbox{red!1}{\strut studies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut nationally} \colorbox{red!0}{\strut respected} \colorbox{red!1}{\strut Learning} \colorbox{red!0}{\strut Resource} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut LRC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut students} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut diagnosed} \colorbox{red!1}{\strut learning} \colorbox{red!1}{\strut disabilities} \colorbox{red!0}{\strut andor} \colorbox{red!0}{\strut ADDADHD} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut related} \colorbox{red!1}{\strut disabilities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut fact} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut colleges} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut universities} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut country} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut used} \colorbox{red!8}{\strut Mitchell} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut LRC} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut model} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut developing} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut own} \colorbox{red!1}{\strut programs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Because} \colorbox{red!0}{\strut each} \colorbox{red!8}{\strut Mitchell} \colorbox{red!1}{\strut student} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut unique} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut academic} \colorbox{red!0}{\strut strengths} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut weaknesses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut LRC} \colorbox{red!1}{\strut program} \colorbox{red!0}{\strut addresses} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut participany} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut individual} \colorbox{red!0}{\strut basis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Our} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut size} \colorbox{red!0}{\strut enables} \colorbox{red!8}{\strut Mitchell} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut offer} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut exceptionally} \colorbox{red!0}{\strut personalized} \colorbox{red!1}{\strut academic} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut classroom} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Go} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Profile} \colorbox{red!0}{\strut Index} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut Go} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Page} \colorbox{red!8}{\strut Mitchell} \colorbox{red!8}{\strut College} \colorbox{red!1}{\strut 437} \colorbox{red!1}{\strut Pequot} \colorbox{red!0}{\strut Avenue} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut London} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Connecticut} \colorbox{red!0}{\strut 06320-4498} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.mitchell.edu} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut loading} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut scroll} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut read} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut profile} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut about} \colorbox{red!8}{\strut Mitchell} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut play} \colorbox{red!0}{\strut automatically} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut loaded} 
}}}
\end{CJK*}

28:rhodes, 26:scholarships, 24:mitchell, 23:marshall, 17:scholarship, 15:college, 14:school, 13:lyric, 13:arts, 12:university


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut For} \colorbox{red!1}{\strut Students} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Faculty} \colorbox{red!1}{\strut Available} \colorbox{red!2}{\strut Scholarships} \colorbox{red!1}{\strut Nominees} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Recipients} \colorbox{red!0}{\strut FAQ} \colorbox{red!0}{\strut Calendar} \colorbox{red!0}{\strut RECENT} \colorbox{red!1}{\strut NOMINEES} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut RECIPIENTS} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Article} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Six} \colorbox{red!0}{\strut Honored} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Scholarship} \colorbox{red!1}{\strut Nominations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut University} \colorbox{red!1}{\strut Record} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 101208} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2005} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2004} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2003} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2002} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Christine} \colorbox{red!1}{\strut Beamer} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut RHODES} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Theatre} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Dance} \colorbox{red!1}{\strut Maia} \colorbox{red!1}{\strut Dedrick} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Theatre} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Dance} \colorbox{red!0}{\strut Abdul} \colorbox{red!0}{\strut El-Sayed} \colorbox{red!2}{\strut RHODES} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut offered} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut accepted} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut offered} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut declined} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Public} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut Sam} \colorbox{red!0}{\strut Espahbodi} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut Megan} \colorbox{red!0}{\strut Hildebrandt} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut finalist} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Art} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Design} \colorbox{red!0}{\strut Neil} \colorbox{red!0}{\strut Rao} \colorbox{red!2}{\strut MITCHELL} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut RHODES} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Public} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Kendal} \colorbox{red!1}{\strut Sparks} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut RHODES} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Theatre} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Dance} \colorbox{red!1}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut top} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut Michael} \colorbox{red!0}{\strut Cromwell} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut RHODES} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stephen} \colorbox{red!0}{\strut M.} \colorbox{red!0}{\strut Ross} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut Stephanie} \colorbox{red!0}{\strut Ketchum} \colorbox{red!2}{\strut RHODES} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut Loc} \colorbox{red!0}{\strut Thang} \colorbox{red!2}{\strut RHODES} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Engineering} \colorbox{red!1}{\strut Colin} \colorbox{red!1}{\strut Tucker} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Theatre} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Dance} \colorbox{red!0}{\strut Thomas} \colorbox{red!1}{\strut Wisniewski} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut RHODES} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Theatre} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Dance} \colorbox{red!1}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut top} \colorbox{red!1}{\strut 2007} \colorbox{red!1}{\strut Lyric} \colorbox{red!1}{\strut Chen} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut offered} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut accepted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut RHODES} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut finalist} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut Lucas} \colorbox{red!0}{\strut Polcyn} \colorbox{red!2}{\strut MARSHALL} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut RHODES} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut MITCHELL} \colorbox{red!1}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Literature} 
}}}
\end{CJK*}

query: car parts

99:parts, 83:car, 81:cars, 27:foreign, 26:recycler, 25:auto, 24:inventories, 22:used, 22:domestic, 22:american


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Auto} \colorbox{red!2}{\strut Recycling} \colorbox{red!1}{\strut since} \colorbox{red!1}{\strut 1946} \colorbox{red!2}{\strut Used} \colorbox{red!2}{\strut Auto} \colorbox{red!9}{\strut Parts} \colorbox{red!1}{\strut For} \colorbox{red!2}{\strut Foreign} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut American} \colorbox{red!7}{\strut Cars} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Trucks} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Vans} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut SUV} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut We} \colorbox{red!1}{\strut Ship} \colorbox{red!1}{\strut Quality} \colorbox{red!2}{\strut Used} \colorbox{red!2}{\strut Auto} \colorbox{red!9}{\strut Parts} \colorbox{red!1}{\strut World} \colorbox{red!1}{\strut Wide} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut largest} \colorbox{red!2}{\strut inventories} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut late-model} \colorbox{red!2}{\strut used} \colorbox{red!2}{\strut Foreign} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Domestic} \colorbox{red!8}{\strut Car} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Truck} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut SUV} \colorbox{red!9}{\strut parts} \colorbox{red!1}{\strut For} \colorbox{red!1}{\strut ALL} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut used} \colorbox{red!9}{\strut parts} \colorbox{red!1}{\strut needs} \colorbox{red!1}{\strut Call} \colorbox{red!1}{\strut ALL} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 797-4595} \colorbox{red!1}{\strut sales} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eallauto.com} \colorbox{red!1}{\strut all} \colorbox{red!2}{\strut auto} \colorbox{red!2}{\strut used} \colorbox{red!9}{\strut parts} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut all} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut used} \colorbox{red!8}{\strut car} \colorbox{red!1}{\strut pa} \colorbox{red!0}{\strut 15755} \colorbox{red!0}{\strut Arrow} \colorbox{red!0}{\strut Highway} \colorbox{red!0}{\strut Fontana} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut CA} \colorbox{red!0}{\strut 92335} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 797-4595} \colorbox{red!1}{\strut All} \colorbox{red!2}{\strut auto} \colorbox{red!2}{\strut used} \colorbox{red!9}{\strut parts} \colorbox{red!1}{\strut wrecking} \colorbox{red!1}{\strut yard} \colorbox{red!2}{\strut recycler} \colorbox{red!2}{\strut foreign} \colorbox{red!2}{\strut domestic} \colorbox{red!9}{\strut parts} \colorbox{red!1}{\strut Copyright} \colorbox{red!0}{\strut 2002-2006} \colorbox{red!1}{\strut All} \colorbox{red!1}{\strut Rights} \colorbox{red!1}{\strut Reserved} \colorbox{red!1}{\strut All} \colorbox{red!2}{\strut Auto} \colorbox{red!9}{\strut Parts} \colorbox{red!0}{\strut Co.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eAllAuto.com} \colorbox{red!0}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut MediaSugar} \colorbox{red!1}{\strut all} \colorbox{red!2}{\strut auto} \colorbox{red!9}{\strut parts} \colorbox{red!1}{\strut carries} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut huge} \colorbox{red!0}{\strut selection} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut mercedes} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut honda} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut toyota} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lexus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut acura} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut jaguar} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut porsche} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut ford} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

97:parts, 97:cars, 96:detroit, 96:car, 25:accessories, 22:part, 20:vehicles, 20:sale, 17:customizing, 17:custom


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Used} \colorbox{red!4}{\strut car} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut sale} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Locanto} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Change} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut Personals} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut Pets} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Rent} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Estate} \colorbox{red!0}{\strut For} \colorbox{red!1}{\strut Sale} \colorbox{red!0}{\strut Jobs} \colorbox{red!1}{\strut Services} \colorbox{red!0}{\strut Post} \colorbox{red!1}{\strut Ad} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut offer} \colorbox{red!1}{\strut wanted} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut classified} \colorbox{red!1}{\strut ad} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Results} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut Detroit.Page} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut motorcyclesmotorbikes} \colorbox{red!1}{\strut used} \colorbox{red!4}{\strut cars} \colorbox{red!1}{\strut commercial} \colorbox{red!0}{\strut trucks} \colorbox{red!0}{\strut boats} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut RVstrailers} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut categories} \colorbox{red!0}{\strut automotive} \colorbox{red!1}{\strut services} \colorbox{red!1}{\strut used} \colorbox{red!4}{\strut cars} \colorbox{red!0}{\strut Users} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut browsed} \colorbox{red!0}{\strut our} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut classifieds} \colorbox{red!1}{\strut category} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Yalwa} \colorbox{red!4}{\strut Car} \colorbox{red!4}{\strut Parts} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Accessories} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut directory} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Used} \colorbox{red!1}{\strut Auto} \colorbox{red!4}{\strut Parts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Johns} \colorbox{red!1}{\strut Auto} \colorbox{red!4}{\strut Parts} \colorbox{red!4}{\strut detroit} \colorbox{red!0}{\strut Save} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut Used} \colorbox{red!1}{\strut Auto} \colorbox{red!4}{\strut Parts} \colorbox{red!0}{\strut Just} \colorbox{red!0}{\strut print} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut ad} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut present} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut purchase} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Auto} \colorbox{red!0}{\strut Salvage} \colorbox{red!0}{\strut 5166} \colorbox{red!0}{\strut Grand} \colorbox{red!0}{\strut River} \colorbox{red!0}{\strut Ave} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut MI} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut Found} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut neighbouring} \colorbox{red!1}{\strut cities} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!1}{\strut Wanted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s10} \colorbox{red!0}{\strut door} \colorbox{red!0}{\strut cromwell} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut door} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut s10} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut Fort} \colorbox{red!0}{\strut Wayne} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut Fort} \colorbox{red!0}{\strut Wayne} \colorbox{red!0}{\strut Taylors} \colorbox{red!1}{\strut Custom} \colorbox{red!1}{\strut Accessories} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Exhaust} \colorbox{red!0}{\strut Thigur} \colorbox{red!0}{\strut alders} \colorbox{red!0}{\strut algeria} \colorbox{red!1}{\strut Auto} \colorbox{red!1}{\strut Customizing} \colorbox{red!1}{\strut Auto} \colorbox{red!0}{\strut Race} \colorbox{red!4}{\strut Cars} \colorbox{red!1}{\strut Mufflers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Exhaust} \colorbox{red!0}{\strut Systems} \colorbox{red!0}{\strut Restoration} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Reconditioning} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut Akron} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut Akron} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Taylors} \colorbox{red!1}{\strut Custom} \colorbox{red!1}{\strut Accessories} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Exhaust} \colorbox{red!0}{\strut Thigur} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut alders} \colorbox{red!1}{\strut Auto} \colorbox{red!1}{\strut Customizing} \colorbox{red!1}{\strut Auto} \colorbox{red!0}{\strut Race} \colorbox{red!4}{\strut Cars} \colorbox{red!1}{\strut Mufflers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Exhaust} \colorbox{red!0}{\strut Systems} \colorbox{red!0}{\strut Restoration} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Reconditioning} \colorbox{red!0}{\strut website} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.taacc.com} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut Akron} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut Akron} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Sat} \colorbox{red!0}{\strut 17} \colorbox{red!0}{\strut Jan} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut 065135} \colorbox{red!0}{\strut PM} \colorbox{red!0}{\strut Results} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut car} \colorbox{red!0}{\strut partsaccessories} \colorbox{red!0}{\strut Detroit.Page} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1} \colorbox{red!1}{\strut Used} \colorbox{red!1}{\strut auto} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut sale} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut classified} \colorbox{red!1}{\strut ad} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Locanto} \colorbox{red!1}{\strut Used} \colorbox{red!4}{\strut car} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut sale} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Detroit} \colorbox{red!0}{\strut classifieds} \colorbox{red!1}{\strut category} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: dinosaurs

96:dinosaur, 95:dinosaurs, 60:reptiles, 37:dinosauric, 26:lizards, 20:lizard, 20:carnivorous, 18:extinct, 17:name, 15:saurischia


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut contents} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut contents} \colorbox{red!1}{\strut Animals} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut Finance} \colorbox{red!1}{\strut Food} \colorbox{red!0}{\strut Garden} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Law} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut Miscellaneous} \colorbox{red!0}{\strut Religion} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut Shopping} \colorbox{red!0}{\strut Sports} \colorbox{red!0}{\strut Technology} \colorbox{red!0}{\strut Travel} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Looking} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut Year} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Review} \colorbox{red!10}{\strut dinosaur} \colorbox{red!1}{\strut Dictionary} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut dinosaur} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dnY-sr} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Library} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Literature} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Language} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Dictionary} \colorbox{red!0}{\strut n.} \colorbox{red!0}{\strut Any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut various} \colorbox{red!2}{\strut extinct} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut often} \colorbox{red!1}{\strut gigantic} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut carnivorous} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut herbivorous} \colorbox{red!6}{\strut reptiles} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut orders} \colorbox{red!2}{\strut Saurischia} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Ornithischia} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut chiefly} \colorbox{red!1}{\strut terrestrial} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut existed} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Mesozoic} \colorbox{red!1}{\strut Era} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!0}{\strut relic} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut past} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut living} \colorbox{red!10}{\strut dinosaurs} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut world} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut vegetation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut John} \colorbox{red!1}{\strut Olmsted} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut hopelessly} \colorbox{red!0}{\strut outmoded} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut unwieldy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut big-city} \colorbox{red!0}{\strut teaching} \colorbox{red!0}{\strut hospital} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!10}{\strut dinosaur} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Peggy} \colorbox{red!0}{\strut Breault} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut New} \colorbox{red!1}{\strut Latin} \colorbox{red!0}{\strut Dnosauria} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut group} \colorbox{red!2}{\strut name} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Dnosaurus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut former} \colorbox{red!2}{\strut genus} \colorbox{red!2}{\strut name} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Greek} \colorbox{red!1}{\strut deinos} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut monstrous} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Greek} \colorbox{red!1}{\strut sauros} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut lizard} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut dinosauric} \colorbox{red!0}{\strut dinosauric} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -sr-k} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut adj} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Answers.com} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut Personalize} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut Translate} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut WikiAnswers.com} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut Recent} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut Advanced} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut unanswered} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut library} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut Q} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!0}{\strut Reference} \colorbox{red!0}{\strut topics} \colorbox{red!0}{\strut Sci-Tech} \colorbox{red!0}{\strut Encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut Dinosaur} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Library} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sci-Tech} \colorbox{red!0}{\strut Encyclopedia} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut term} \colorbox{red!1}{\strut Dinosauria} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Greek} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut terrible} \colorbox{red!3}{\strut lizards} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut coined} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut British} \colorbox{red!0}{\strut comparative} \colorbox{red!1}{\strut anatomist} \colorbox{red!0}{\strut Richard} \colorbox{red!0}{\strut Owen} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1842} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut represent} \colorbox{red!1}{\strut three} \colorbox{red!0}{\strut partly} \colorbox{red!1}{\strut known} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut impressively} \colorbox{red!1}{\strut large} \colorbox{red!1}{\strut fossil} \colorbox{red!6}{\strut reptiles} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut countryside} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut carnivore} \colorbox{red!1}{\strut Megalosaurus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut duckbilled} \colorbox{red!1}{\strut Iguanodon} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut armored} \colorbox{red!1}{\strut Hylaeosaurus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!10}{\strut dinosaurs} \colorbox{red!0}{\strut became} \colorbox{red!0}{\strut better} \colorbox{red!1}{\strut known} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut taxonomy} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut classification} \colorbox{red!0}{\strut developed} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut diversity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 1888} \colorbox{red!0}{\strut H.} \colorbox{red!0}{\strut G.} \colorbox{red!0}{\strut Seeley} \colorbox{red!0}{\strut recognized} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut quite} \colorbox{red!1}{\strut different} \colorbox{red!1}{\strut hip} \colorbox{red!1}{\strut structures} \colorbox{red!0}{\strut in} \colorbox{red!10}{\strut dinosaurs} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut grouped} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut accordingly} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Saurischia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut carnivorous} \colorbox{red!0}{\strut Theropoda} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut giant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut long-necked} \colorbox{red!1}{\strut Sauropoda} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut retained} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut generalized} \colorbox{red!1}{\strut reptilian} \colorbox{red!1}{\strut hip} \colorbox{red!1}{\strut structure} \colorbox{red!0}{\strut in} 
}}}
\end{CJK*}

100:dinosaur, 99:dinosaurs, 98:party, 55:birthday, 32:price, 30:sale, 23:napkins, 23:invitations, 22:table, 21:plates


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Dinosaur} \colorbox{red!1}{\strut Birthday} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut High} \colorbox{red!0}{\strut quality} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut dinosaur} \colorbox{red!2}{\strut party} \colorbox{red!0}{\strut supplies} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!1}{\strut invitations} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!1}{\strut birthday} \colorbox{red!1}{\strut invitations} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!1}{\strut birthday} \colorbox{red!0}{\strut bags} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!1}{\strut birthday} \colorbox{red!0}{\strut gifts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut toys} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut plates} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut cups} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut mural} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut balloons} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut candy} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!1}{\strut napkins} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut tableware} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!0}{\strut posters} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut school} \colorbox{red!0}{\strut stationary} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut masks} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut bones} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut skeletons} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut eggs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut stickers} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut tattoos} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut coloring} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut puppets} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut cups} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pterodactyl} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut growing} \colorbox{red!2}{\strut dinosaurs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaurs} \colorbox{red!0}{\strut eggs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut candy} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut necklaces} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut skulls} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut cookie} \colorbox{red!0}{\strut cutters} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut plush} \colorbox{red!0}{\strut toys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut t-shirts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut inflatable} \colorbox{red!2}{\strut dinosaurs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut T-rex} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Velociraptor} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Pterodactyl} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Tyrannosaurus} \colorbox{red!0}{\strut rex} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Triceratops} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut masks} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut costumes} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dinosaur} \colorbox{red!0}{\strut keychains} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut T-rex} \colorbox{red!0}{\strut toys} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FREE} \colorbox{red!0}{\strut 1} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!0}{\strut Gift} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 70} \colorbox{red!0}{\strut Purchase} \colorbox{red!0}{\strut FREE} \colorbox{red!0}{\strut 2} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!0}{\strut Gifts} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 150} \colorbox{red!0}{\strut Purchase} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Pack} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Tableware} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut Guests} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 41.35} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Pack} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Tableware} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut Guests} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 46.15} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Favors} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.95} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Bags} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.95} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Plates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Beverage} \colorbox{red!0}{\strut Plates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut pcs} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.85} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Plates} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!0}{\strut Beverage} \colorbox{red!0}{\strut Plates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut pcs} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.25} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!1}{\strut Napkins} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Beverage} \colorbox{red!1}{\strut Napkins} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut pcs} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.65} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!1}{\strut Napkins} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!0}{\strut Beverage} \colorbox{red!1}{\strut Napkins} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut pcs} \colorbox{red!0}{\strut Regular} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.95} \colorbox{red!1}{\strut Sale} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dinosaur} \colorbox{red!2}{\strut Party} \colorbox{red!0}{\strut Plates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Luncheon} \colorbox{red!0}{\strut Plates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

query: lower heart rate

83:benefits, 69:cardiorespiratory, 65:rate, 50:cardio, 45:heart, 41:muscle, 40:resting, 39:lower, 34:muscles, 30:blood


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Fitness} \colorbox{red!0}{\strut Study} \colorbox{red!1}{\strut Guide} \colorbox{red!7}{\strut Benefits} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Flexibility-} \colorbox{red!2}{\strut Better} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut motion} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut joints} \colorbox{red!2}{\strut Avoid} \colorbox{red!4}{\strut muscle} \colorbox{red!2}{\strut injuries} \colorbox{red!1}{\strut Ease} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut doing} \colorbox{red!0}{\strut everyday} \colorbox{red!0}{\strut tasks} \colorbox{red!7}{\strut Benefits} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Cardiorespiratory-} \colorbox{red!3}{\strut Lower} \colorbox{red!4}{\strut resting} \colorbox{red!4}{\strut heart} \colorbox{red!6}{\strut rate} \colorbox{red!1}{\strut Overall} \colorbox{red!0}{\strut feeling} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut better} \colorbox{red!1}{\strut health} \colorbox{red!7}{\strut Benefits} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Strength} \colorbox{red!0}{\strut Training-} \colorbox{red!1}{\strut Stronger} \colorbox{red!3}{\strut muscles} \colorbox{red!1}{\strut Stronger} \colorbox{red!1}{\strut bones} \colorbox{red!2}{\strut Avoid} \colorbox{red!4}{\strut muscle} \colorbox{red!2}{\strut injuries} \colorbox{red!4}{\strut Cardio} \colorbox{red!0}{\strut healthlower} \colorbox{red!3}{\strut blood} \colorbox{red!3}{\strut pressure} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Weights} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut lifted} \colorbox{red!0}{\strut slowly} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 10-15} \colorbox{red!1}{\strut repetitions} \colorbox{red!0}{\strut per} \colorbox{red!1}{\strut set} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut B} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut heart} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut training} \colorbox{red!2}{\strut zone} \colorbox{red!0}{\strut while} \colorbox{red!2}{\strut exercising} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut working} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut lower} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut resting} \colorbox{red!4}{\strut heart} \colorbox{red!6}{\strut rate} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut improving} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut endurance} \colorbox{red!1}{\strut burning} \colorbox{red!1}{\strut fat} \colorbox{red!1}{\strut calories} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut target} \colorbox{red!4}{\strut heart} \colorbox{red!2}{\strut zone} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 60-80} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut maximum} \colorbox{red!4}{\strut heart} \colorbox{red!6}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut youre} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut zone} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut getting} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut benefits} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut cardiorespiratory} \colorbox{red!2}{\strut work} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut D.} \colorbox{red!3}{\strut Muscles} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut examples} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut exercises} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut work} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Abdominals} \colorbox{red!0}{\strut -crunches} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut sit-ups} \colorbox{red!1}{\strut Trapezius} \colorbox{red!0}{\strut -shoulder} \colorbox{red!1}{\strut press} \colorbox{red!1}{\strut Biceps} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut arm} \colorbox{red!0}{\strut curls} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut push-ups} \colorbox{red!1}{\strut Quadriceps} \colorbox{red!0}{\strut -leg} \colorbox{red!1}{\strut extension} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut leg} \colorbox{red!1}{\strut press} \colorbox{red!1}{\strut Pectoralis} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut flys} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut bench} \colorbox{red!1}{\strut press} \colorbox{red!0}{\strut Deltoid} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut shoulder} \colorbox{red!1}{\strut press} \colorbox{red!1}{\strut Triceps} \colorbox{red!0}{\strut -upright} \colorbox{red!1}{\strut rows} \colorbox{red!0}{\strut Gluteus} \colorbox{red!0}{\strut maximus} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut leg} \colorbox{red!1}{\strut press} \colorbox{red!0}{\strut KNOW} \colorbox{red!1}{\strut WHERE} \colorbox{red!0}{\strut ALL} \colorbox{red!0}{\strut THE} \colorbox{red!0}{\strut ABOVE} \colorbox{red!3}{\strut MUSCLES} \colorbox{red!0}{\strut ARE} \colorbox{red!0}{\strut ON} \colorbox{red!0}{\strut THE} \colorbox{red!0}{\strut BODY-STUDY} \colorbox{red!0}{\strut THE} \colorbox{red!0}{\strut WALL} \colorbox{red!0}{\strut PICTURES} \colorbox{red!0}{\strut IN} \colorbox{red!1}{\strut CLASS} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

97:rate, 95:heart, 77:how, 67:training, 62:calculate, 60:calculating, 31:resting, 27:zone, 24:pulse, 23:zones


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tips} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Techniques} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Calculating} \colorbox{red!0}{\strut Your} \colorbox{red!3}{\strut Training} \colorbox{red!4}{\strut Heart} \colorbox{red!4}{\strut Rate} \colorbox{red!1}{\strut High} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut disciplinespecially} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut elite} \colorbox{red!0}{\strut athleticsequires} \colorbox{red!0}{\strut measuring} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut recording} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tracking} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut key} \colorbox{red!0}{\strut metrics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut discussing} \colorbox{red!3}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut calculate} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut training} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut monitors} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut monitor} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut optimize} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reduce} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut injuries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut show} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut calculate} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut training} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut formula} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut accounts} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut fitness} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut resting} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Training} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut THR} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut zones} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut doing} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut aerobic} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut workout} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Take} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut pulse} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut workout} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut ensure} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut training} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut target} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!1}{\strut zone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut training} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!1}{\strut zone} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut roughly} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 60} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut maximum} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MHR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Training} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut computed} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut follows} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Take} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut pulse} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut soon} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut wake} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut morning} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut resting} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RHR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Subtract} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut age} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 220} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut number} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut MHR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut values} \colorbox{red!0}{\strut obtained} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut equation} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut determine} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut target} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut training} \colorbox{red!0}{\strut purposes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut heart} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut calculate} \colorbox{red!0}{\strut upper} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut lower} \colorbox{red!1}{\strut limits} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut THR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut i.e.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 60} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut TARGET} \colorbox{red!0}{\strut HR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MHR} \colorbox{red!0}{\strut RHR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RHR} \colorbox{red!1}{\strut THR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RHR} \colorbox{red!0}{\strut Example} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MHR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 220} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 190} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RHR} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 60} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut determined} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut morning} 
}}}
\end{CJK*}

query: atari

100:atari, 99:ataris, 64:what, 27:owned, 20:games, 20:founded, 19:company, 17:corporation, 16:brand, 14:game


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut disambiguation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut refer} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut video} \colorbox{red!1}{\strut game} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut computer} \colorbox{red!1}{\strut brand} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Inc} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut defunct} \colorbox{red!1}{\strut corporation} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut founded} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut brand} \colorbox{red!7}{\strut Atari} \colorbox{red!1}{\strut Corporation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut company} \colorbox{red!1}{\strut formed} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut original} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut consumer} \colorbox{red!0}{\strut assets} \colorbox{red!7}{\strut Atari} \colorbox{red!1}{\strut Games} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut spun} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut original} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut later} \colorbox{red!2}{\strut owned} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Midway} \colorbox{red!1}{\strut Games} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Infogrames} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut corporation} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut leases} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut brand} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut Interactive} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut current} \colorbox{red!0}{\strut owner} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut Atari} \colorbox{red!1}{\strut brand} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut privately} \colorbox{red!0}{\strut held} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Infogrames} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Japanese} \colorbox{red!1}{\strut word} \colorbox{red!0}{\strut which} \colorbox{red!1}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut hit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut game} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Go} \colorbox{red!0}{\strut The} \colorbox{red!6}{\strut Ataris} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut alternative} \colorbox{red!0}{\strut rock} \colorbox{red!1}{\strut band} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Italian} \colorbox{red!0}{\strut electropop} \colorbox{red!1}{\strut group} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut Bigby} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut born} \colorbox{red!0}{\strut 1981} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut football} \colorbox{red!1}{\strut player} \colorbox{red!0}{\strut Gali} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut born} \colorbox{red!0}{\strut 1953} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Israeli} \colorbox{red!0}{\strut singer} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut actress} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut abbreviation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Finnish} \colorbox{red!0}{\strut registry} \colorbox{red!0}{\strut term} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ammatti-} \colorbox{red!0}{\strut ja} \colorbox{red!0}{\strut taparikollinen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut professional} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut custom} \colorbox{red!0}{\strut criminal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Finnish} \colorbox{red!0}{\strut police} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Natsume} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut pachinko} \colorbox{red!0}{\strut branch} \colorbox{red!1}{\strut company} \colorbox{red!7}{\strut Atari} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Pakistan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut town} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Punjab} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Pakistan} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut Attari} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Indian} \colorbox{red!0}{\strut side} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut official} \colorbox{red!0}{\strut border} \colorbox{red!0}{\strut crossing} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut India} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Pakistan} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut disambiguation} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut lists} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut title} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut internal} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut led} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut wish} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut change} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut directly} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Retrieved} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut en.wikipedia.orgwikiAtari} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut disambiguation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Category} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Disambiguation} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut Hidden} \colorbox{red!0}{\strut categories} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut disambiguation} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut article} \colorbox{red!1}{\strut disambiguation} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut Views} \colorbox{red!0}{\strut Article} \colorbox{red!0}{\strut Discussion} \colorbox{red!0}{\strut Edit} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut tools} \colorbox{red!0}{\strut Log} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut create} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut Navigation} \colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut Featured} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut Current} \colorbox{red!0}{\strut events} \colorbox{red!0}{\strut Random} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Interaction} 
}}}
\end{CJK*}

100:atari, 71:released, 47:release, 18:7800, 17:publisher, 17:game, 15:titles, 15:name, 14:ace, 12:jr


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Atari} \colorbox{red!1}{\strut 7800} \colorbox{red!2}{\strut Release} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut Complete} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Atari} \colorbox{red!1}{\strut 7800} \colorbox{red!1}{\strut Titles} \colorbox{red!3}{\strut Released} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!1}{\strut GAME} \colorbox{red!0}{\strut CARTRIDGE} \colorbox{red!1}{\strut NAME} \colorbox{red!1}{\strut PUBLISHER} \colorbox{red!1}{\strut Ace} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Aces} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Alien} \colorbox{red!0}{\strut Brigade} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Asteroids} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut BallBlazer} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Barnyard} \colorbox{red!0}{\strut Blaster} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Basketbrawl} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Centipede} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Choplifter} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Commando} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Cracked} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Crossbow} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Dark} \colorbox{red!0}{\strut Chambers} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Desert} \colorbox{red!0}{\strut Falcon} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Dig} \colorbox{red!0}{\strut Dug} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Donkey} \colorbox{red!0}{\strut Kong} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Donkey} \colorbox{red!0}{\strut Kong} \colorbox{red!0}{\strut Jr.} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Double} \colorbox{red!0}{\strut Dragon} \colorbox{red!0}{\strut Activision} \colorbox{red!0}{\strut F-18} \colorbox{red!0}{\strut Hornet} \colorbox{red!0}{\strut Absolute} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Fatal} \colorbox{red!0}{\strut Run} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Fight} \colorbox{red!0}{\strut Night} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Food} \colorbox{red!0}{\strut Fight} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Galaga} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Hat} \colorbox{red!0}{\strut Trick} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Ikari} \colorbox{red!0}{\strut Warriors} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Impossible} \colorbox{red!0}{\strut Mission} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Jinks} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Joust} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Karateka} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Kung} \colorbox{red!0}{\strut Fu} \colorbox{red!0}{\strut Master} \colorbox{red!0}{\strut Absolute} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Mario} \colorbox{red!0}{\strut Bros.} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Mat} \colorbox{red!0}{\strut Mania} \colorbox{red!0}{\strut Challenge} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Mean} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut Ultimate} \colorbox{red!0}{\strut Golf} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Meltdown} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Midnight} \colorbox{red!0}{\strut Mutants} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut MotoPsycho} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Ms.} \colorbox{red!0}{\strut Pac-Man} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Ninja} \colorbox{red!0}{\strut Golf} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut One-on-One} \colorbox{red!0}{\strut Basketball} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Pete} \colorbox{red!0}{\strut Rose} \colorbox{red!0}{\strut Baseball} \colorbox{red!0}{\strut Absolute} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Planet} \colorbox{red!0}{\strut Smashers} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Pole} \colorbox{red!0}{\strut Position} \colorbox{red!0}{\strut II} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Rampage} \colorbox{red!0}{\strut Activision} \colorbox{red!0}{\strut RealSports} \colorbox{red!0}{\strut Baseball} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Robotron} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2084} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Scrapyard} \colorbox{red!0}{\strut Dog} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Summer} \colorbox{red!0}{\strut Games} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Super} \colorbox{red!0}{\strut Huey} \colorbox{red!0}{\strut UH-IX} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Super} \colorbox{red!0}{\strut Skateboardin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Absolute} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Tank} \colorbox{red!0}{\strut Command} \colorbox{red!0}{\strut Froggo} \colorbox{red!0}{\strut Title} \colorbox{red!0}{\strut Match} \colorbox{red!0}{\strut Pro} \colorbox{red!0}{\strut Wrestling} \colorbox{red!0}{\strut Absolute} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Tomcat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F-14} \colorbox{red!0}{\strut Fighter} \colorbox{red!0}{\strut Simulator} \colorbox{red!0}{\strut Absolute} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Touchdown} \colorbox{red!0}{\strut Football} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Tower} \colorbox{red!0}{\strut Toppler} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Water} \colorbox{red!0}{\strut Ski} \colorbox{red!0}{\strut Froggo} \colorbox{red!0}{\strut Winter} \colorbox{red!0}{\strut Games} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Xenophobe} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut Xevious} \colorbox{red!4}{\strut Atari} \colorbox{red!0}{\strut E-Mail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GOOD} \colorbox{red!0}{\strut DEAL} \colorbox{red!0}{\strut GAMES} \colorbox{red!0}{\strut GOOD} \colorbox{red!0}{\strut DEAL} \colorbox{red!0}{\strut GAMES} \colorbox{red!0}{\strut HOMEPAGE} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2003} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut GOOD} \colorbox{red!0}{\strut DEAL} \colorbox{red!0}{\strut GAMES} 
}}}
\end{CJK*}

query: hoboken

100:hoboken, 99:hobokens, 72:museum, 40:historical, 37:history, 15:musical, 15:events, 13:exhibit, 12:railroad, 12:house


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lastest} \colorbox{red!8}{\strut Hoboken} \colorbox{red!3}{\strut Historical} \colorbox{red!6}{\strut Museum} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut pdf} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Nov.} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut November} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut December} \colorbox{red!1}{\strut Events} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut --} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Oct.} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut Stunning} \colorbox{red!0}{\strut Variety} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Homes} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Display} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Annual} \colorbox{red!8}{\strut Hoboken} \colorbox{red!3}{\strut Historical} \colorbox{red!6}{\strut Museum} \colorbox{red!1}{\strut House} \colorbox{red!1}{\strut Tour} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Oct.} \colorbox{red!0}{\strut 26} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Aug.} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Heaven} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hell} \colorbox{red!0}{\strut or} \colorbox{red!8}{\strut Hoboken} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Exhibit} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lecture} \colorbox{red!0}{\strut Series} \colorbox{red!0}{\strut Bring} \colorbox{red!8}{\strut Hoboken} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut War} \colorbox{red!0}{\strut Experience} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Life} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Aug.} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!8}{\strut Hoboken} \colorbox{red!3}{\strut Historical} \colorbox{red!6}{\strut Museum} \colorbox{red!0}{\strut Fall} \colorbox{red!1}{\strut Events} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!8}{\strut Hoboken} \colorbox{red!3}{\strut Historical} \colorbox{red!6}{\strut Museum} \colorbox{red!0}{\strut 11th} \colorbox{red!0}{\strut Annual} \colorbox{red!0}{\strut Secret} \colorbox{red!0}{\strut GardenTour} \colorbox{red!0}{\strut Covers} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Town} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Northeast} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Southwest} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!1}{\strut Make} \colorbox{red!3}{\strut History} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut Year} \colorbox{red!0}{\strut Great} \colorbox{red!8}{\strut Hoboken} \colorbox{red!0}{\strut Auction} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Support} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut Hoboken} \colorbox{red!3}{\strut Historical} \colorbox{red!6}{\strut Museum} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!8}{\strut Hoboken} \colorbox{red!3}{\strut Historical} \colorbox{red!6}{\strut Museum} \colorbox{red!0}{\strut Hosts} \colorbox{red!0}{\strut Publication} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Oral} \colorbox{red!3}{\strut History} \colorbox{red!0}{\strut Chapbook} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Nice} \colorbox{red!0}{\strut Tavern} \colorbox{red!0}{\strut Book} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut recollections} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Paul} \colorbox{red!0}{\strut Samperi} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut fathers} \colorbox{red!0}{\strut lively} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut owner} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut Hobokens} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut popular} \colorbox{red!1}{\strut celebration} \colorbox{red!0}{\strut halls} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -Feb.} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut Celebrate} \colorbox{red!0}{\strut Black} \colorbox{red!3}{\strut History} \colorbox{red!0}{\strut Month} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Tribute} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Civil} \colorbox{red!0}{\strut Rights} \colorbox{red!0}{\strut Activists} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Leo} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Sarah} \colorbox{red!0}{\strut Smith} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut latest} \colorbox{red!0}{\strut oral} \colorbox{red!3}{\strut history} \colorbox{red!0}{\strut chapbook} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Always} \colorbox{red!0}{\strut Helping} \colorbox{red!0}{\strut People} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Release} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut -Nov.} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut Features} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Musical} \colorbox{red!1}{\strut Guests} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Authors} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Sinatra} \colorbox{red!0}{\strut Idol} \colorbox{red!0}{\strut Contest} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Wrap} \colorbox{red!0}{\strut Up} \colorbox{red!8}{\strut Hoboken} \colorbox{red!1}{\strut Tunes} \colorbox{red!1}{\strut Exhibit} 
}}}
\end{CJK*}

100:hoboken, 80:what, 35:jobs, 33:job, 30:where, 26:company, 24:host, 22:companies, 20:location, 20:city


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut my.indeed} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Create} \colorbox{red!0}{\strut Account} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Jobs} \colorbox{red!1}{\strut Salaries} \colorbox{red!0}{\strut Trends} \colorbox{red!0}{\strut Forums} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut job} \colorbox{red!1}{\strut title} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut keywords} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut Forums} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut City} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut Jersey} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut Forum} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut new} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut cancel} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut alerts} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut anytime} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Current} \colorbox{red!0}{\strut Discussions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Start} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Discussion} \colorbox{red!1}{\strut Host} \colorbox{red!1}{\strut Best} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut work} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut What} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut fueling} \colorbox{red!0}{\strut growth} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Why} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut employer} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Host} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut activities} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut recreation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut vacation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut plain} \colorbox{red!0}{\strut fun} \colorbox{red!0}{\strut around} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Host} \colorbox{red!0}{\strut Newcomer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut guide} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut newcomers} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut settle} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut enjoy} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Car} \colorbox{red!0}{\strut registration} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pet} \colorbox{red!0}{\strut laws} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut services} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Host} \colorbox{red!1}{\strut Job} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut local} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut boards} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut clubs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut recruiters} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut temp} \colorbox{red!0}{\strut agencies} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Host} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut coming} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!3}{\strut What} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rise} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Host} \colorbox{red!4}{\strut Hoboken} \colorbox{red!1}{\strut causes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut charities} \colorbox{red!3}{\strut What} \colorbox{red!1}{\strut causes} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Where} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut volunteer} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Host} \colorbox{red!0}{\strut Weather} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut seasons} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut How} \colorbox{red!0}{\strut do} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut dwellers} \colorbox{red!0}{\strut cope} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Host} \colorbox{red!1}{\strut Best} \colorbox{red!0}{\strut schools} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Where} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut schools} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut districts} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Host} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut neigborhoods} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Hoboken} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Where} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut life} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut families} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Singles} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut work} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut change} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut what} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Got} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut worst} \colorbox{red!0}{\strut about} \colorbox{red!3}{\strut what} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut work} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut joining} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut discussion} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut starting} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Subscribe} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut forum} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut RSS} \colorbox{red!0}{\strut feed} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: alexian brothers hospital

98:alexian, 95:brothers, 84:hospitals, 81:hospital, 35:network, 26:medical, 20:which, 17:care, 16:locations, 15:comprised


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Main} \colorbox{red!1}{\strut Navigation} \colorbox{red!1}{\strut Jobs} \colorbox{red!2}{\strut Locations} \colorbox{red!1}{\strut Services} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Doctor} \colorbox{red!1}{\strut Classes} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Events} \colorbox{red!1}{\strut Donate} \colorbox{red!1}{\strut About} \colorbox{red!1}{\strut Us} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut Like} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Learn} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut Alexian} \colorbox{red!10}{\strut Brothers} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Doctor} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Job} \colorbox{red!1}{\strut View} \colorbox{red!1}{\strut Maps} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Directions} \colorbox{red!1}{\strut Volunteer} \colorbox{red!1}{\strut Learn} \colorbox{red!0}{\strut More} \colorbox{red!1}{\strut About} \colorbox{red!1}{\strut Quality} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Patient} \colorbox{red!1}{\strut Safety} \colorbox{red!1}{\strut Pay} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Bill} \colorbox{red!0}{\strut Search} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut Encyclopedia} \colorbox{red!0}{\strut Busque} \colorbox{red!1}{\strut en} \colorbox{red!1}{\strut la} \colorbox{red!1}{\strut Enciclopedia} \colorbox{red!1}{\strut de} \colorbox{red!1}{\strut Salud} \colorbox{red!1}{\strut en} \colorbox{red!1}{\strut espaol} \colorbox{red!1}{\strut Live} \colorbox{red!1}{\strut Healthier} \colorbox{red!1}{\strut View} \colorbox{red!0}{\strut Baby} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut Find} \colorbox{red!1}{\strut Information} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Healthcare} \colorbox{red!1}{\strut Professionals} \colorbox{red!11}{\strut Alexian} \colorbox{red!10}{\strut Brothers} \colorbox{red!9}{\strut Hospital} \colorbox{red!4}{\strut Network} \colorbox{red!11}{\strut Alexian} \colorbox{red!10}{\strut Brothers} \colorbox{red!9}{\strut Hospital} \colorbox{red!4}{\strut Network} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut comprised} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut four} \colorbox{red!9}{\strut hospitals} \colorbox{red!2}{\strut which} \colorbox{red!1}{\strut serve} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut two} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut residents} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut Chicago} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut growing} \colorbox{red!1}{\strut Northwest} \colorbox{red!1}{\strut suburbs} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!1}{\strut offer} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut broad} \colorbox{red!0}{\strut continuum} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut innovative} \colorbox{red!2}{\strut care} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut leading} \colorbox{red!3}{\strut medical} \colorbox{red!1}{\strut specialists} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut state-of-the-art} \colorbox{red!1}{\strut technology} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut reflecting} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut commitment} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut provide} \colorbox{red!0}{\strut unsurpassed} \colorbox{red!1}{\strut treatment} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut care} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut benefit} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut patients} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut community} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Job} \colorbox{red!0}{\strut Privacy} \colorbox{red!1}{\strut Policy} \colorbox{red!0}{\strut Advertising} \colorbox{red!1}{\strut Policy} \colorbox{red!3}{\strut Medical} \colorbox{red!1}{\strut Disclaimer} \colorbox{red!1}{\strut Media} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2009} \colorbox{red!1}{\strut Congregation} \colorbox{red!1}{\strut of} \colorbox{red!11}{\strut Alexian} \colorbox{red!10}{\strut Brothers} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

100:alexian, 76:brothers, 62:hospitals, 38:hospital, 38:center, 33:locations, 31:centers, 29:medical, 25:home, 24:facilities


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut Navigation} \colorbox{red!0}{\strut Jobs} \colorbox{red!1}{\strut Locations} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Doctor} \colorbox{red!0}{\strut Classes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Events} \colorbox{red!0}{\strut Donate} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Contact} \colorbox{red!1}{\strut Locations} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut News} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Dominican} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut Form} \colorbox{red!0}{\strut Partnership} \colorbox{red!0}{\strut Resource} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Veterans} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut ABMC} \colorbox{red!0}{\strut ABHN} \colorbox{red!0}{\strut Receives} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Stroke} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Guidelines} \colorbox{red!0}{\strut Gold} \colorbox{red!0}{\strut Performance} \colorbox{red!0}{\strut Achievement} \colorbox{red!0}{\strut Award} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Hospital} \colorbox{red!0}{\strut Network} \colorbox{red!0}{\strut Participating} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Phase} \colorbox{red!0}{\strut III} \colorbox{red!0}{\strut MS} \colorbox{red!0}{\strut Study} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Cancer} \colorbox{red!0}{\strut Institute} \colorbox{red!0}{\strut Broadens} \colorbox{red!0}{\strut Genetics} \colorbox{red!0}{\strut Testing} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Joint} \colorbox{red!0}{\strut Commission} \colorbox{red!0}{\strut Awards} \colorbox{red!0}{\strut Gold} \colorbox{red!0}{\strut Seal} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Approval} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Disease} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut Programs} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Locations} \colorbox{red!0}{\strut Our} \colorbox{red!1}{\strut Locations} \colorbox{red!2}{\strut Hospitals} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Behavioral} \colorbox{red!1}{\strut Health} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!3}{\strut Alexian} \colorbox{red!0}{\strut Rehabilitation} \colorbox{red!1}{\strut Hospital} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut Alexius} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut Emergency} \colorbox{red!1}{\strut Care} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Behavioral} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Hospital} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut Alexius} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ImmediateCare} \colorbox{red!0}{\strut CentersDiagnostic} \colorbox{red!0}{\strut Imaging} \colorbox{red!0}{\strut Services} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Immediate} \colorbox{red!1}{\strut Care} \colorbox{red!0}{\strut CenterDiagnostic} \colorbox{red!0}{\strut Imaging} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Addison} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Diagnostic} \colorbox{red!0}{\strut Imaging} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mount} \colorbox{red!0}{\strut Prospect} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut Alexius} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ImmediateCare} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hanover} \colorbox{red!0}{\strut Park} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut Alexius} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ImmediateCare} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Palatine} \colorbox{red!0}{\strut Occupational} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Clinics} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!0}{\strut Occupational} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Clinics} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Care} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Care} \colorbox{red!0}{\strut Supportive} \colorbox{red!0}{\strut Housing} \colorbox{red!3}{\strut Alexian} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Mental} \colorbox{red!1}{\strut Health} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!0}{\strut AIDS} \colorbox{red!0}{\strut Ministry} \colorbox{red!0}{\strut Outpatient} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Brock} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Plaza} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Eberle} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Building} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Niehoff} \colorbox{red!0}{\strut Pavilion} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Pavilion} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Roncoli} \colorbox{red!1}{\strut Center} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Wimmer} \colorbox{red!1}{\strut Center} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Group} \colorbox{red!3}{\strut Alexian} \colorbox{red!0}{\strut Rehabilitation} \colorbox{red!1}{\strut Hospital} \colorbox{red!3}{\strut Alexian} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Mall} \colorbox{red!0}{\strut Outpatient} \colorbox{red!0}{\strut Mental} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Facilities} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Behavioral} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Hospital} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Behavioral} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Hospital} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Group} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Plaza} \colorbox{red!3}{\strut Alexian} \colorbox{red!2}{\strut Brothers} \colorbox{red!1}{\strut Behavioral} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Hospital} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Eberle} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Office} \colorbox{red!0}{\strut Building} \colorbox{red!0}{\strut AlexianBrothersCenter} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Mental} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Job} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut Advertising} \colorbox{red!0}{\strut Policy} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Disclaimer} \colorbox{red!0}{\strut Media} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Congregation} 
}}}
\end{CJK*}

query: indexed annuity

99:annuity, 98:index, 98:annuitys, 98:annuities, 97:indexed, 84:equity, 75:what, 27:insurance, 27:buying, 25:cancel


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut EIA} \colorbox{red!0}{\strut Book} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Book} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Equity-Indexed} \colorbox{red!6}{\strut Annuities} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut Securities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Exchange} \colorbox{red!0}{\strut Commission} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SEC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Equity-Indexed} \colorbox{red!6}{\strut Annuities} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut considering} \colorbox{red!2}{\strut buying} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut equity-indexed} \colorbox{red!6}{\strut annuity} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut brochure} \colorbox{red!0}{\strut explains} \colorbox{red!0}{\strut equity-indexed} \colorbox{red!6}{\strut annuities} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut obtaining} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut Equity-Indexed} \colorbox{red!6}{\strut Annuity} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut equity-indexed} \colorbox{red!6}{\strut annuity} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut contract} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut insurance} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut During} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut accumulation} \colorbox{red!0}{\strut period} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut make} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut lump} \colorbox{red!1}{\strut sum} \colorbox{red!1}{\strut payment} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut payments} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut insurance} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut credits} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut return} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut changes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!5}{\strut equity} \colorbox{red!6}{\strut index} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut S} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut P} \colorbox{red!0}{\strut 500Composite} \colorbox{red!1}{\strut Stock} \colorbox{red!1}{\strut Price} \colorbox{red!6}{\strut Index} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut insurance} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut typically} \colorbox{red!1}{\strut guarantees} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut minimum} \colorbox{red!1}{\strut return} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Guaranteed} \colorbox{red!1}{\strut minimum} \colorbox{red!1}{\strut return} \colorbox{red!0}{\strut rates} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut accumulation} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut insurance} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut make} \colorbox{red!0}{\strut periodic} \colorbox{red!1}{\strut payments} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut contract} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut unless} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut receive} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut contract} \colorbox{red!0}{\strut value} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut lump} \colorbox{red!1}{\strut sum} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut Lose} \colorbox{red!1}{\strut money} \colorbox{red!2}{\strut Buying} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut Equity-Indexed} \colorbox{red!6}{\strut Annuity} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut lose} \colorbox{red!1}{\strut money} \colorbox{red!2}{\strut buying} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut equity-indexed} \colorbox{red!6}{\strut annuity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut cancel} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut annuity} \colorbox{red!1}{\strut early} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Even} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut guarantee} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut still} \colorbox{red!1}{\strut lose} \colorbox{red!1}{\strut money} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut guarantee} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut amount} \colorbox{red!0}{\strut thats} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut full} \colorbox{red!1}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut purchase} \colorbox{red!1}{\strut payments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut take} \colorbox{red!0}{\strut several} \colorbox{red!1}{\strut years} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut equity-index} \colorbox{red!6}{\strut annuitys} \colorbox{red!1}{\strut minimum} \colorbox{red!1}{\strut guarantee} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut break} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut significant} \colorbox{red!0}{\strut surrender} \colorbox{red!0}{\strut charge} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tax} \colorbox{red!0}{\strut penalties} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut cancel} \colorbox{red!1}{\strut early} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut insurance} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut credit} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut index-linked} \colorbox{red!1}{\strut interest} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut hold} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut contract} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut maturity} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Contract} \colorbox{red!0}{\strut Features} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Equity-Indexed} \colorbox{red!6}{\strut Annuities} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Equity-indexed} \colorbox{red!6}{\strut annuities} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut complicated} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut contain} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut affect} \colorbox{red!0}{\strut your} 
}}}
\end{CJK*}

101:annuity, 101:annuities, 50:what, 20:variable, 20:fixed, 19:rate, 19:cash, 15:index, 15:guaranteed, 14:life


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Welcome} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut bestannuities.com} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut Annuities} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Cash} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut annuity} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Searches} \colorbox{red!5}{\strut Annuities} \colorbox{red!1}{\strut Cash} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut annuity} \colorbox{red!1}{\strut Immediate} \colorbox{red!5}{\strut annuities} \colorbox{red!1}{\strut Fixed} \colorbox{red!5}{\strut Annuity} \colorbox{red!1}{\strut Rates} \colorbox{red!1}{\strut Retirement} \colorbox{red!5}{\strut annuities} \colorbox{red!1}{\strut Immediate} \colorbox{red!5}{\strut annuity} \colorbox{red!1}{\strut Best} \colorbox{red!5}{\strut annuity} \colorbox{red!1}{\strut rate} \colorbox{red!1}{\strut Index} \colorbox{red!5}{\strut annuity} \colorbox{red!1}{\strut Income} \colorbox{red!5}{\strut annuity} \colorbox{red!1}{\strut Equity} \colorbox{red!1}{\strut indexed} \colorbox{red!5}{\strut annuity} \colorbox{red!0}{\strut Single} \colorbox{red!0}{\strut premium} \colorbox{red!1}{\strut immediate} \colorbox{red!5}{\strut annuity} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Searches} \colorbox{red!0}{\strut TIAA} \colorbox{red!0}{\strut CREF} \colorbox{red!5}{\strut Annuities} \colorbox{red!1}{\strut Tax} \colorbox{red!1}{\strut sheltered} \colorbox{red!5}{\strut annuity} \colorbox{red!1}{\strut Insurance} \colorbox{red!5}{\strut annuity} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut Jackson} \colorbox{red!0}{\strut National} \colorbox{red!5}{\strut Annuities} \colorbox{red!0}{\strut Compare} \colorbox{red!5}{\strut Annuities} \colorbox{red!1}{\strut Indexed} \colorbox{red!5}{\strut annuities} \colorbox{red!1}{\strut Deferred} \colorbox{red!1}{\strut Fixed} \colorbox{red!5}{\strut Annuities} \colorbox{red!1}{\strut IRA} \colorbox{red!5}{\strut annuities} \colorbox{red!1}{\strut Impaired} \colorbox{red!1}{\strut Life} \colorbox{red!5}{\strut Annuities} \colorbox{red!1}{\strut Best} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut America} \colorbox{red!5}{\strut Annuity} \colorbox{red!1}{\strut Guaranteed} \colorbox{red!1}{\strut Variable} \colorbox{red!5}{\strut Annuity} \colorbox{red!1}{\strut CD} \colorbox{red!5}{\strut annuity} \colorbox{red!0}{\strut Have} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut found} \colorbox{red!3}{\strut what} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Then} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Best} \colorbox{red!5}{\strut Annuity} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Best} \colorbox{red!1}{\strut variable} \colorbox{red!5}{\strut annuities} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Charitable} \colorbox{red!1}{\strut gift} \colorbox{red!5}{\strut annuity} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Ing} \colorbox{red!5}{\strut annuities} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Indexed} \colorbox{red!5}{\strut annuity} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut bestannuities.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Rights} \colorbox{red!0}{\strut Reserved} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} 
}}}
\end{CJK*}

query: wilson antenna

102:antennas, 102:antenna, 64:wilson, 41:cb, 32:mobile, 26:base, 25:whip, 24:radios, 24:power, 22:priced


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut CB} \colorbox{red!1}{\strut Radios} \colorbox{red!0}{\strut 10} \colorbox{red!1}{\strut Meter} \colorbox{red!0}{\strut Amateur} \colorbox{red!1}{\strut Radios} \colorbox{red!1}{\strut Bearcat} \colorbox{red!0}{\strut Scanners} \colorbox{red!0}{\strut 2-Way} \colorbox{red!1}{\strut Radios} \colorbox{red!2}{\strut CB} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut 2} \colorbox{red!1}{\strut Meter} \colorbox{red!5}{\strut Antenna} \colorbox{red!5}{\strut Antenna} \colorbox{red!1}{\strut Mounting} \colorbox{red!0}{\strut Coax} \colorbox{red!0}{\strut Microphones} \colorbox{red!0}{\strut Speakers} \colorbox{red!1}{\strut Power} \colorbox{red!0}{\strut Supplies} \colorbox{red!0}{\strut Test} \colorbox{red!1}{\strut Meters} \colorbox{red!0}{\strut Accessories} \colorbox{red!0}{\strut Pepper} \colorbox{red!0}{\strut Elec} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Store} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut CB} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Mobile} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut CB} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Mobile} \colorbox{red!2}{\strut CB} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Car} \colorbox{red!5}{\strut Antennas} \colorbox{red!3}{\strut Wilson} \colorbox{red!1}{\strut Car} \colorbox{red!2}{\strut CB} \colorbox{red!5}{\strut Antennas} \colorbox{red!3}{\strut Wilson} \colorbox{red!1}{\strut Short} \colorbox{red!1}{\strut Load} \colorbox{red!0}{\strut 900817} \colorbox{red!0}{\strut 39} \colorbox{red!0}{\strut Inch} \colorbox{red!0}{\strut Center} \colorbox{red!1}{\strut Load} \colorbox{red!1}{\strut Whip} \colorbox{red!0}{\strut Designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Replace} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Original} \colorbox{red!0}{\strut Longer} \colorbox{red!1}{\strut Whip} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut 500} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 5000} \colorbox{red!1}{\strut Base} \colorbox{red!1}{\strut Load} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16.95} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Little} \colorbox{red!0}{\strut Wil} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Antenna} \colorbox{red!1}{\strut Economically} \colorbox{red!1}{\strut priced} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Little} \colorbox{red!0}{\strut Wil} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut beaten} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut verses} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut comparison} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut perfect} \colorbox{red!5}{\strut antenna} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut vacationer} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Little} \colorbox{red!0}{\strut Wil} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Specifications} \colorbox{red!0}{\strut 300} \colorbox{red!1}{\strut Watt} \colorbox{red!1}{\strut power} \colorbox{red!0}{\strut handling} \colorbox{red!0}{\strut capability} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ICAS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Made} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut high} \colorbox{red!1}{\strut impact} \colorbox{red!0}{\strut Thermoplastic} \colorbox{red!1}{\strut Heavy} \colorbox{red!1}{\strut duty} \colorbox{red!1}{\strut coil} \colorbox{red!0}{\strut uses} \colorbox{red!0}{\strut 14} \colorbox{red!1}{\strut gauge} \colorbox{red!0}{\strut copper} \colorbox{red!1}{\strut wire} \colorbox{red!0}{\strut Exclusive} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut loss} \colorbox{red!1}{\strut coil} \colorbox{red!1}{\strut design} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Patent} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4,882,591} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Same} \colorbox{red!0}{\strut as} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut 36} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 17-7} \colorbox{red!0}{\strut PH} \colorbox{red!0}{\strut stainless} \colorbox{red!1}{\strut steel} \colorbox{red!1}{\strut whip} \colorbox{red!1}{\strut Frequency} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut MHz} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut MHz} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Year} \colorbox{red!0}{\strut Warranty} \colorbox{red!1}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 39.95} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut 500} \colorbox{red!5}{\strut Antenna} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut Higher} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Little} \colorbox{red!0}{\strut Will} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut priced} \colorbox{red!0}{\strut lower} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut perfect} \colorbox{red!0}{\strut mid} \colorbox{red!1}{\strut range} \colorbox{red!5}{\strut antenna} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 500} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Specifications} \colorbox{red!0}{\strut 2000} \colorbox{red!1}{\strut Watt} \colorbox{red!1}{\strut power} \colorbox{red!0}{\strut handling} \colorbox{red!0}{\strut capability} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ICAS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Made} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut high} \colorbox{red!1}{\strut impact} \colorbox{red!0}{\strut Thermoplastic} \colorbox{red!1}{\strut Heavy} \colorbox{red!1}{\strut duty} \colorbox{red!1}{\strut coil} \colorbox{red!0}{\strut uses} \colorbox{red!0}{\strut 12} \colorbox{red!1}{\strut gauge} \colorbox{red!0}{\strut copper} \colorbox{red!1}{\strut wire} \colorbox{red!0}{\strut Exclusive} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut loss} \colorbox{red!1}{\strut coil} \colorbox{red!1}{\strut design} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Patent} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4,882,591} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Same} \colorbox{red!0}{\strut as} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut 54} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 17-7} \colorbox{red!0}{\strut PH} \colorbox{red!0}{\strut stainless} \colorbox{red!1}{\strut steel} \colorbox{red!1}{\strut whip} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut warranty} \colorbox{red!1}{\strut Frequency} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut MHz} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut MHz} \colorbox{red!0}{\strut Weather} \colorbox{red!0}{\strut Channel} \colorbox{red!0}{\strut Ready} \colorbox{red!1}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 64.95} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut 1000} \colorbox{red!5}{\strut Antenna} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut recognized} \colorbox{red!5}{\strut antenna} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut market} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Available} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Roof} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Trunk} \colorbox{red!0}{\strut Lip} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Magnetic} \colorbox{red!1}{\strut mounts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Magnetic} \colorbox{red!1}{\strut Mount} \colorbox{red!0}{\strut Shown} \colorbox{red!3}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1000} 
}}}
\end{CJK*}

101:antennas, 101:antenna, 51:type, 36:phone, 31:wilson, 31:dt, 30:cell, 29:mobile, 29:cellular, 27:wireless


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Set} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Add} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Favorites} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut map} \colorbox{red!1}{\strut Customer} \colorbox{red!1}{\strut Service} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 888} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 512-6774} \colorbox{red!0}{\strut Purchase} \colorbox{red!1}{\strut Orders} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut accepted} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut Day} \colorbox{red!0}{\strut Satisfaction} \colorbox{red!0}{\strut Guarantee} \colorbox{red!0}{\strut Reviews} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Catalog} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut View} \colorbox{red!1}{\strut cart} \colorbox{red!0}{\strut Quick} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut pattern} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Advanced} \colorbox{red!0}{\strut search} \colorbox{red!1}{\strut Reception} \colorbox{red!0}{\strut Products} \colorbox{red!1}{\strut Amplifiers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Repeaters} \colorbox{red!5}{\strut Antenna} \colorbox{red!1}{\strut Adapters} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut Coax} \colorbox{red!0}{\strut Cables} \colorbox{red!0}{\strut Complete} \colorbox{red!0}{\strut Kits} \colorbox{red!0}{\strut Components} \colorbox{red!0}{\strut Connectors} \colorbox{red!0}{\strut Crimps} \colorbox{red!1}{\strut Mounts} \colorbox{red!0}{\strut Power} \colorbox{red!0}{\strut Supplies} \colorbox{red!1}{\strut Splitters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Taps} \colorbox{red!0}{\strut Accessory} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut Type} \colorbox{red!1}{\strut Bluetooth} \colorbox{red!1}{\strut Car} \colorbox{red!0}{\strut Kits} \colorbox{red!1}{\strut Bluetooth} \colorbox{red!0}{\strut Headsets} \colorbox{red!0}{\strut GPS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Navigation} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Carrier} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut equipment} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut wireless} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut provider} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut AT} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut T} \colorbox{red!1}{\strut Bell} \colorbox{red!0}{\strut Nextel} \colorbox{red!1}{\strut Sprint} \colorbox{red!0}{\strut T-Mobile} \colorbox{red!1}{\strut Verizon} \colorbox{red!1}{\strut Wireless} \colorbox{red!0}{\strut Manufacturers} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!1}{\strut Customer} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut Returns} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut Testimonials} \colorbox{red!0}{\strut Latest} \colorbox{red!0}{\strut Posts} \colorbox{red!0}{\strut AT} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut T} \colorbox{red!0}{\strut Moving} \colorbox{red!0}{\strut EDGE} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 1900} \colorbox{red!0}{\strut Mhz} \colorbox{red!1}{\strut Band} \colorbox{red!2}{\strut Wilson} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut powerful} \colorbox{red!1}{\strut amplifiers} \colorbox{red!0}{\strut yet} \colorbox{red!2}{\strut Wilson} \colorbox{red!1}{\strut Electronics} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Wireless} \colorbox{red!1}{\strut Technology} \colorbox{red!0}{\strut Leader} \colorbox{red!0}{\strut Why} \colorbox{red!2}{\strut Wilson} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Fire} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ice} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut break} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut signal} \colorbox{red!0}{\strut Testimonials} \colorbox{red!0}{\strut Author} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tom} \colorbox{red!0}{\strut worked} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut well} \colorbox{red!1}{\strut Home} \colorbox{red!5}{\strut Antennas} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut Our} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut patented} \colorbox{red!2}{\strut cell} \colorbox{red!2}{\strut phone} \colorbox{red!5}{\strut antennas} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut commited} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut bringing} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut highest} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut possible} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!1}{\strut carry} \colorbox{red!0}{\strut an} \colorbox{red!5}{\strut antenna} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut almost} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut application} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut situation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Whether} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut car} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Wilson} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Cellularantennas} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reduce} \colorbox{red!0}{\strut disconnects} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut drop} \colorbox{red!0}{\strut outs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut noise} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut these} \colorbox{red!5}{\strut antennas} \colorbox{red!0}{\strut significantly} \colorbox{red!0}{\strut increase} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut cell} \colorbox{red!2}{\strut phone} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut reception} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut eliminate} \colorbox{red!0}{\strut dead} \colorbox{red!0}{\strut zones} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Most} \colorbox{red!2}{\strut cell} \colorbox{red!2}{\strut phone} \colorbox{red!5}{\strut antennas} \colorbox{red!1}{\strut install} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut minutes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut tools} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut narrow} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut select} \colorbox{red!5}{\strut antenna} \colorbox{red!3}{\strut type} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Mobile} \colorbox{red!5}{\strut Antennas} \colorbox{red!1}{\strut Building} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Yagi} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Dome} \colorbox{red!5}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Cell} \colorbox{red!2}{\strut Phone} \colorbox{red!5}{\strut Antenna} \colorbox{red!1}{\strut Adapters} \colorbox{red!0}{\strut Pages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 3} \colorbox{red!1}{\strut Range} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sort} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Product} \colorbox{red!1}{\strut Price} \colorbox{red!1}{\strut Default} \colorbox{red!2}{\strut Wilson} \colorbox{red!1}{\strut Black} \colorbox{red!1}{\strut Rubber} \colorbox{red!5}{\strut Antenna} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut TNC} \colorbox{red!0}{\strut Male} \colorbox{red!0}{\strut Connector} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 301144} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Wilson} \colorbox{red!1}{\strut Black} \colorbox{red!1}{\strut Rubber} \colorbox{red!5}{\strut Antenna} \colorbox{red!0}{\strut with} 
}}}
\end{CJK*}

query: avp

100:avps, 100:avp, 39:when, 27:established, 21:olympics, 20:volleyball, 18:beach, 16:pro, 16:2008, 14:mens


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut AVPs} \colorbox{red!1}{\strut 2008} \colorbox{red!2}{\strut Olympics} \colorbox{red!1}{\strut Blog} \colorbox{red!1}{\strut Site} \colorbox{red!9}{\strut AVPs} \colorbox{red!1}{\strut 2008} \colorbox{red!2}{\strut Olympics} \colorbox{red!1}{\strut Blog} \colorbox{red!1}{\strut Site} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut theAVP} \colorbox{red!0}{\strut The} \colorbox{red!9}{\strut AVP} \colorbox{red!0}{\strut was} \colorbox{red!3}{\strut established} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1983} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut comprised} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut best} \colorbox{red!1}{\strut mens} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut womens} \colorbox{red!1}{\strut pro} \colorbox{red!2}{\strut beach} \colorbox{red!2}{\strut volleyball} \colorbox{red!1}{\strut players} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut arguably} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut world} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!9}{\strut AVPs} \colorbox{red!1}{\strut main} \colorbox{red!1}{\strut goal} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut deliver} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut fans} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut amazing} \colorbox{red!0}{\strut athletic} \colorbox{red!0}{\strut contest} \colorbox{red!0}{\strut surrounded} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut unforgettable} \colorbox{red!2}{\strut beach} \colorbox{red!0}{\strut party} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut million} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut expected} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut attend} \colorbox{red!0}{\strut an} \colorbox{red!9}{\strut AVP} \colorbox{red!1}{\strut event} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 31} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2001} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut AVP} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut reorganized} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut new} \colorbox{red!1}{\strut management} \colorbox{red!1}{\strut team} \colorbox{red!0}{\strut led} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut agent} \colorbox{red!0}{\strut Leonard} \colorbox{red!1}{\strut Armato} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut his} \colorbox{red!1}{\strut company} \colorbox{red!1}{\strut Management} \colorbox{red!0}{\strut Plus} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut When} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut announced} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut acquisition} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut tour} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Manhattan} \colorbox{red!2}{\strut Beach} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Calif.} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut historic} \colorbox{red!0}{\strut move} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut uniting} \colorbox{red!0}{\strut both} \colorbox{red!1}{\strut men} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut women} \colorbox{red!0}{\strut professional} \colorbox{red!2}{\strut beach} \colorbox{red!2}{\strut volleyball} \colorbox{red!1}{\strut players} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut umbrella} \colorbox{red!1}{\strut organization} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut historic} \colorbox{red!0}{\strut unification} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut mens} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut womens} \colorbox{red!1}{\strut competitions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut new} \colorbox{red!9}{\strut AVP} \colorbox{red!1}{\strut Tour} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut able} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut capitalize} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut having} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut property} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut maximize} \colorbox{red!1}{\strut sponsor} \colorbox{red!0}{\strut dollars} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut marketing} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut media} \colorbox{red!0}{\strut coverage} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut prize} \colorbox{red!1}{\strut money} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!9}{\strut AVP} \colorbox{red!0}{\strut now} \colorbox{red!1}{\strut stands} \colorbox{red!0}{\strut alone} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut only} \colorbox{red!1}{\strut pro} \colorbox{red!2}{\strut beach} \colorbox{red!2}{\strut volleyball} \colorbox{red!1}{\strut tour} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut country} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut cooperative} \colorbox{red!0}{\strut relationship} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut USA} \colorbox{red!2}{\strut Volleyball} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Federation} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut de} \colorbox{red!2}{\strut Volleyball} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FIVB} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut Response} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut theAVP} \colorbox{red!1}{\strut Barbara} \colorbox{red!0}{\strut Says} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 31} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut 2008} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 1045} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut Love} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut website} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut current-tourney} \colorbox{red!0}{\strut statistics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut bios} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut blogs} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut job} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut thanks} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut continue} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut return} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Mason} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Cincinnati} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut love} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Leave} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Reply} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut cancel} \colorbox{red!0}{\strut reply} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Name} \colorbox{red!0}{\strut Mail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut published} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Website} \colorbox{red!0}{\strut Notify} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut followup} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut via} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pages} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut theAVP} \colorbox{red!1}{\strut Archives} \colorbox{red!0}{\strut August} \colorbox{red!1}{\strut 2008} \colorbox{red!0}{\strut Categories} \colorbox{red!0}{\strut avpblog} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Chris} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Geeter} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

77:avp, 53:jobs, 49:job, 30:industry, 26:title, 22:hr, 22:company, 22:claims, 18:atv, 17:mortgage


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Browse} \colorbox{red!2}{\strut Jobs} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Category} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Location} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Company} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Keyword} \colorbox{red!0}{\strut Keywords} \colorbox{red!2}{\strut Job} \colorbox{red!1}{\strut Title} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Industry} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Employer} \colorbox{red!1}{\strut Location} \colorbox{red!0}{\strut City} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut State} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Zip} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut Advanced} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Keyword} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ATV} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Behavioral} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut AVP} \colorbox{red!1}{\strut Mortgage} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Avphr} \colorbox{red!0}{\strut Keywords} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut Popular} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Avphr} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!1}{\strut Title} \colorbox{red!0}{\strut Insurance} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Training} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Operations} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Sales} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Estate} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Systems} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Of} \colorbox{red!1}{\strut Claims} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!1}{\strut Payroll} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Quality} \colorbox{red!0}{\strut Assurance} \colorbox{red!3}{\strut AVP} \colorbox{red!1}{\strut Mortgage} \colorbox{red!3}{\strut AVP} \colorbox{red!1}{\strut Mortgage} \colorbox{red!0}{\strut Collections} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Auto} \colorbox{red!1}{\strut Claims} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Branches} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Of} \colorbox{red!1}{\strut Claims} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Nursing} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut P} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut c} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Product} \colorbox{red!0}{\strut Management} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Operations} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Organizational} \colorbox{red!0}{\strut Development} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Organizational} \colorbox{red!0}{\strut Learning} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Patient} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut Services} \colorbox{red!3}{\strut AVP} \colorbox{red!1}{\strut Payroll} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Public} \colorbox{red!0}{\strut Relations} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut QA} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Quality} \colorbox{red!0}{\strut Assurance} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Quantitative} \colorbox{red!0}{\strut Strategies} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Estate} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Reporting} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Reporting} \colorbox{red!0}{\strut Analytics} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Reporting} \colorbox{red!0}{\strut Manager} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Risk} \colorbox{red!0}{\strut Management} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Risk} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut Insurance} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Safety} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Sales} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Secondary} \colorbox{red!0}{\strut Marketing} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Strategic} \colorbox{red!0}{\strut Giving} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Syndications} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Systems} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut T} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut od} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Talent} \colorbox{red!0}{\strut Management} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Technology} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Telecom} \colorbox{red!3}{\strut AVP} \colorbox{red!1}{\strut Title} \colorbox{red!0}{\strut Insurance} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Training} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Training} \colorbox{red!0}{\strut Development} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Training} \colorbox{red!0}{\strut OD} \colorbox{red!3}{\strut AVP} \colorbox{red!0}{\strut Workforce} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut Avpdirector} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Compensation} \colorbox{red!0}{\strut Avphr} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut Juju} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Add} \colorbox{red!2}{\strut Jobs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Advertise} \colorbox{red!2}{\strut Jobs} 
}}}
\end{CJK*}

query: penguins

101:penguin, 100:penguins, 46:species, 37:gentoo, 25:world, 14:listed, 14:distribution, 13:eudyptes, 13:emperor, 11:king


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Gentoo} \colorbox{red!6}{\strut Penguins} \colorbox{red!6}{\strut Penguins} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut Species} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut 17} \colorbox{red!3}{\strut species} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut world-wide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut listed} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut linking} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut each} \colorbox{red!6}{\strut penguin} \colorbox{red!3}{\strut species} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut find} \colorbox{red!6}{\strut penguins} \colorbox{red!1}{\strut listed} \colorbox{red!0}{\strut according} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut geographical} \colorbox{red!1}{\strut distribution} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut interactive} \colorbox{red!6}{\strut Penguins} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut World} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut Adelie} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pygoscelis} \colorbox{red!0}{\strut adeliae} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut African} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Spheniscus} \colorbox{red!0}{\strut demersus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Chinstrap} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pygoscelis} \colorbox{red!1}{\strut antarctica} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Emperor} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Aptenodytes} \colorbox{red!0}{\strut forsteri} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Erect-crested} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eudyptes} \colorbox{red!1}{\strut sclateri} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fiordland} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eudyptes} \colorbox{red!0}{\strut pachyrhynchus} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Galapagos} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Spheniscus} \colorbox{red!0}{\strut mendiculus} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Gentoo} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pygoscelis} \colorbox{red!0}{\strut papua} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Humboldt} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Spheniscus} \colorbox{red!0}{\strut humboldti} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut King} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Aptenodytes} \colorbox{red!0}{\strut patagonicus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Little} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Blue} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eudyptula} \colorbox{red!0}{\strut minor} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Macaroni} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eudyptes} \colorbox{red!1}{\strut chrysolophus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Magellanic} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Spheniscus} \colorbox{red!0}{\strut magellanicus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rockhopper} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eudyptes} \colorbox{red!0}{\strut chrysocome} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Royal} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eudyptes} \colorbox{red!0}{\strut schlegeli} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Snares} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eudyptes} \colorbox{red!0}{\strut robustus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Yellow-eyed} \colorbox{red!6}{\strut penguins} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Megadyptes} \colorbox{red!0}{\strut antipodes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Mike} \colorbox{red!0}{\strut Bingham} 
}}}
\end{CJK*}

100:penguins, 100:penguin, 44:names, 40:which, 26:genus, 24:emperor, 23:lists, 21:king, 19:appear, 17:table


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut This} \colorbox{red!1}{\strut table} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut lists} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut penguins} \colorbox{red!2}{\strut which} \colorbox{red!1}{\strut appear} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut Which} \colorbox{red!5}{\strut Penguin} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut click} \colorbox{red!2}{\strut names} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut penguins} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut pages} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut displayed} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Which} \colorbox{red!5}{\strut Penguin} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Iwish} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut try} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Which} \colorbox{red!5}{\strut Penguin} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Emperor} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut genus} \colorbox{red!1}{\strut Emperor} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut King} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut Adelie} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut genus} \colorbox{red!1}{\strut Adelie} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Gentoo} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Chinstrap} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut Macaroni} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut genus} \colorbox{red!0}{\strut Rockhopper} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut Royal} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut Macaroni} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Snares} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Erect-crested} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Fioldland} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Huboldt} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut genus} \colorbox{red!0}{\strut Huboldt} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Magellan} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut Cape} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Galapagos} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Fairy} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut genus} \colorbox{red!0}{\strut Fairy} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut Yellow-eyed} \colorbox{red!5}{\strut penguin} \colorbox{red!1}{\strut genus} \colorbox{red!0}{\strut Yellow-eyed} \colorbox{red!5}{\strut penguin} \colorbox{red!5}{\strut Penguin} \colorbox{red!0}{\strut Fossil} \colorbox{red!1}{\strut Giant} \colorbox{red!5}{\strut penguin} \colorbox{red!2}{\strut Which} \colorbox{red!5}{\strut penguin} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut webmaster} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Japanese} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut sent} \colorbox{red!0}{\strut mail} \colorbox{red!0}{\strut -Never} \colorbox{red!0}{\strut Spam} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut -} 
}}}
\end{CJK*}

query: build fence

95:dogs, 95:dog, 91:fences, 91:fenced, 89:fence, 82:fencing, 79:how, 58:square, 47:building, 37:feet


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut ChainFree} \colorbox{red!1}{\strut Asheville} \colorbox{red!1}{\strut Breaking} \colorbox{red!1}{\strut Chains} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Building} \colorbox{red!4}{\strut Fences} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Love} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Dogs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut Facts} \colorbox{red!0}{\strut About} \colorbox{red!1}{\strut Chaining} \colorbox{red!1}{\strut Valentine} \colorbox{red!0}{\strut Have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Heart} \colorbox{red!0}{\strut !} \colorbox{red!4}{\strut HOW} \colorbox{red!0}{\strut YOU} \colorbox{red!0}{\strut CAN} \colorbox{red!0}{\strut HELP} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut Gallery} \colorbox{red!0}{\strut Know} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Law} \colorbox{red!4}{\strut Fences} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Alternatives} \colorbox{red!0}{\strut Videos} \colorbox{red!0}{\strut Neighbor} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut Dog} \colorbox{red!1}{\strut Chained} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Build} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut Fence} \colorbox{red!1}{\strut Animal} \colorbox{red!0}{\strut Control} \colorbox{red!0}{\strut Contacts} \colorbox{red!0}{\strut Child} \colorbox{red!0}{\strut Safety} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Outside} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Dogs} \colorbox{red!0}{\strut LINKS} \colorbox{red!0}{\strut Habitats} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Hounds} \colorbox{red!0}{\strut Wish} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut Volunteer} \colorbox{red!0}{\strut Jobs} \colorbox{red!0}{\strut !} \colorbox{red!4}{\strut Dogs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Vehicles} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!1}{\strut FREE} \colorbox{red!4}{\strut FENCING} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Yes} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut now} \colorbox{red!2}{\strut building} \colorbox{red!4}{\strut fences} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Send} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut telling} \colorbox{red!0}{\strut us} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut dog} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ChainFreeAsheville} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut gmail.com} \colorbox{red!4}{\strut Fencing} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Yard} \colorbox{red!4}{\strut Fencing} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut popular} \colorbox{red!1}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut allow} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut dog} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut roam} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut chain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!4}{\strut dog} \colorbox{red!0}{\strut guardians} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut bring} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut dog} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut dog} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut leash} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut apartment} \colorbox{red!0}{\strut dwellers} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut bringing} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut dog} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut option} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut building} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut secure} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut humane} \colorbox{red!4}{\strut fenced} \colorbox{red!1}{\strut enclosure} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Chain} \colorbox{red!1}{\strut Free} \colorbox{red!1}{\strut Asheville} \colorbox{red!0}{\strut recommends} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut minimum} \colorbox{red!4}{\strut fenced} \colorbox{red!1}{\strut enclosure} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 200} \colorbox{red!3}{\strut square} \colorbox{red!2}{\strut feet} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut each} \colorbox{red!4}{\strut dog} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut value} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut recently} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut adopted} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut cities} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut requirement} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut laws} \colorbox{red!0}{\strut governing} \colorbox{red!0}{\strut humane} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut animals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 200} \colorbox{red!3}{\strut square} \colorbox{red!2}{\strut feet} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut equivalent} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut side} \colorbox{red!1}{\strut dimensions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 10} \colorbox{red!2}{\strut feet} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut 20} \colorbox{red!2}{\strut feet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut requires} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 60} \colorbox{red!1}{\strut linear} \colorbox{red!2}{\strut feet} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut fence} \colorbox{red!0}{\strut fabric} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut perimeter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10102020} \colorbox{red!0}{\strut 60} \colorbox{red!1}{\strut linear} \colorbox{red!2}{\strut feet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Other} \colorbox{red!1}{\strut side} \colorbox{red!1}{\strut dimensions} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut yield} \colorbox{red!0}{\strut 200} \colorbox{red!3}{\strut square} \colorbox{red!2}{\strut feet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut required} \colorbox{red!4}{\strut fence} \colorbox{red!0}{\strut fabric} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut posts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut hardware} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut reduced} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut one} \colorbox{red!1}{\strut side} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut house} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut side} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut dogs} \colorbox{red!1}{\strut enclosure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Note} 
}}}
\end{CJK*}

97:fencing, 96:fences, 96:fence, 85:ostriches, 81:ostrich, 47:how, 46:build, 30:long, 29:posts, 20:high


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut How} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut Just} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Everything} \colorbox{red!0}{\strut How-To} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Videos} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Members} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Start} \colorbox{red!0}{\strut contributing} \colorbox{red!0}{\strut today} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Join} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut HOME} \colorbox{red!2}{\strut HOW} \colorbox{red!0}{\strut TOs} \colorbox{red!0}{\strut VIDEOS} \colorbox{red!0}{\strut WRITE} \colorbox{red!0}{\strut RESOURCES} \colorbox{red!0}{\strut COMMUNITY} \colorbox{red!0}{\strut MY} \colorbox{red!0}{\strut PROFILE} \colorbox{red!0}{\strut Home} \colorbox{red!1}{\strut Pets} \colorbox{red!1}{\strut Farm} \colorbox{red!1}{\strut Animals} \colorbox{red!1}{\strut Breeding} \colorbox{red!1}{\strut Farm} \colorbox{red!1}{\strut Animals} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Build} \colorbox{red!5}{\strut Fences} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut Ostriches} \colorbox{red!0}{\strut BROWSE} \colorbox{red!2}{\strut HOW} \colorbox{red!0}{\strut TOs} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut Like} \colorbox{red!0}{\strut This} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Purchase} \colorbox{red!1}{\strut Chicks} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Hatch} \colorbox{red!1}{\strut Chicks} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Choose} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Breeding} \colorbox{red!1}{\strut Pair} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Ostriches} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Determine} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Sex} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut Ostrich} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Hatch} \colorbox{red!1}{\strut Duck} \colorbox{red!1}{\strut Eggs} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut Author} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Train} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Dog} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Lie} \colorbox{red!0}{\strut Down} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Stop} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Dog} \colorbox{red!0}{\strut Fight} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Handle} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Found} \colorbox{red!1}{\strut Dog} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Shave} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Goat} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Show} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Show} \colorbox{red!0}{\strut 4-H} \colorbox{red!0}{\strut Broilers} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut To} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Build} \colorbox{red!5}{\strut Fences} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut Ostriches} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut eHow} \colorbox{red!1}{\strut Pets} \colorbox{red!0}{\strut Editor} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut Did} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut Rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Ratings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut height} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut long} \colorbox{red!1}{\strut legs} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut ostrich} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut behavior} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut males} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mean} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut build} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut special} \colorbox{red!5}{\strut fence} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut ostriches} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!4}{\strut ostrich} \colorbox{red!1}{\strut chicks} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut being} \colorbox{red!1}{\strut raised} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut different} \colorbox{red!5}{\strut fence} \colorbox{red!1}{\strut design} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut ostrich} \colorbox{red!5}{\strut fence} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut five} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut five} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut half} \colorbox{red!1}{\strut feet} \colorbox{red!1}{\strut high} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Send} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Phone} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut Article} \colorbox{red!0}{\strut Add} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Favorites} \colorbox{red!0}{\strut Flag} \colorbox{red!0}{\strut Article} \colorbox{red!0}{\strut Instructions} \colorbox{red!0}{\strut Difficulty} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Moderately} \colorbox{red!0}{\strut Challenging} \colorbox{red!0}{\strut Things} \colorbox{red!0}{\strut Youll} \colorbox{red!0}{\strut Need} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Fence} \colorbox{red!2}{\strut posts} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut five} \colorbox{red!1}{\strut foot} \colorbox{red!1}{\strut high} \colorbox{red!5}{\strut fence} \colorbox{red!1}{\strut High} \colorbox{red!0}{\strut tensile} \colorbox{red!1}{\strut wire} \colorbox{red!5}{\strut fence} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut wire} \colorbox{red!1}{\strut mesh} \colorbox{red!0}{\strut Wooden} \colorbox{red!0}{\strut droppers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut battens} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Step1} \colorbox{red!0}{\strut Choose} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut close} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut barn} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut shelter} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut ostriches} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Make} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut build} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut grassy} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut actual} \colorbox{red!0}{\strut size} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut bird} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut room} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut yet} \colorbox{red!0}{\strut still} \colorbox{red!0}{\strut manageable} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut ostrich} \colorbox{red!0}{\strut keeper} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut maintain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Step2} \colorbox{red!0}{\strut Prepare} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut placing} \colorbox{red!5}{\strut fence} \colorbox{red!2}{\strut posts} \colorbox{red!0}{\strut in} 
}}}
\end{CJK*}

query: continental plates

99:plates, 99:plate, 94:continental, 63:what, 48:tectonics, 45:tectonic, 28:types, 25:boundaries, 22:lithospheric, 22:earth


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Plate} \colorbox{red!3}{\strut tectonics} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut Continental} \colorbox{red!6}{\strut plates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut tectonic} \colorbox{red!6}{\strut plates} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut were} \colorbox{red!1}{\strut mapped} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut half} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 20th} \colorbox{red!0}{\strut century} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Plate} \colorbox{red!3}{\strut tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Greek} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut tektn} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut builder} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mason} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut describes} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut large} \colorbox{red!1}{\strut scale} \colorbox{red!1}{\strut motions} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Earth} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut lithosphere} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut theory} \colorbox{red!0}{\strut encompasses} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut older} \colorbox{red!1}{\strut concepts} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut continental} \colorbox{red!1}{\strut drift} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut developed} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut half} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 20th} \colorbox{red!0}{\strut century} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut seafloor} \colorbox{red!1}{\strut spreading} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut understood} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 1960s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut outermost} \colorbox{red!1}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Earth} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut interior} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut two} \colorbox{red!1}{\strut layers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut lithosphere} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut comprising} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut crust} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rigid} \colorbox{red!0}{\strut uppermost} \colorbox{red!1}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut mantle} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Below} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut lithosphere} \colorbox{red!0}{\strut lies} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut asthenosphere} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Although} \colorbox{red!0}{\strut solid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut asthenosphere} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut relatively} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut viscosity} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut shear} \colorbox{red!0}{\strut strength} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut flow} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut liquid} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut geological} \colorbox{red!1}{\strut time} \colorbox{red!1}{\strut scales} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut deeper} \colorbox{red!1}{\strut mantle} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut asthenosphere} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut rigid} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut higher} \colorbox{red!0}{\strut pressure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut lithosphere} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut broken} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut into} \colorbox{red!4}{\strut what} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut called} \colorbox{red!3}{\strut tectonic} \colorbox{red!6}{\strut plates} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Earth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut seven} \colorbox{red!1}{\strut major} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut minor} \colorbox{red!6}{\strut plates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut list} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut lithospheric} \colorbox{red!6}{\strut plates} \colorbox{red!0}{\strut ride} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut asthenosphere} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!6}{\strut plates} \colorbox{red!1}{\strut move} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut relation} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut three} \colorbox{red!2}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut plate} \colorbox{red!1}{\strut boundaries} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut convergent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut collisional} \colorbox{red!1}{\strut boundaries} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut divergent} \colorbox{red!1}{\strut boundaries} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut called} \colorbox{red!1}{\strut spreading} \colorbox{red!0}{\strut centers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut transform} \colorbox{red!1}{\strut boundaries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Earthquakes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut volcanic} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mountain} \colorbox{red!0}{\strut -building} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut oceanic} \colorbox{red!1}{\strut trench} \colorbox{red!1}{\strut formation} \colorbox{red!1}{\strut occur} \colorbox{red!0}{\strut along} \colorbox{red!6}{\strut plate} \colorbox{red!1}{\strut boundaries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut lateral} \colorbox{red!1}{\strut movement} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut plates} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut typically} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut speeds} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 50100} \colorbox{red!0}{\strut mm} \colorbox{red!0}{\strut annually} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Synopsis} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut development} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut theory} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Key} \colorbox{red!0}{\strut principles} \colorbox{red!0}{\strut 3} \colorbox{red!2}{\strut Types} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut plate} \colorbox{red!1}{\strut boundaries} \colorbox{red!0}{\strut 3.1} \colorbox{red!1}{\strut Transform} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut conservative} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

98:plate, 97:tectonics, 74:what, 36:theory, 23:continental, 20:earth, 20:drift, 19:rocks, 19:drives, 18:earthquakes


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Pete} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Presentations} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Presentations} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut PowerPoint} \colorbox{red!0}{\strut format} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut earth} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut augusta} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut graves} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut bloomington} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut rockwood} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eastchester} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Theory} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut step} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut 1} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut 2} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Rocks} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mountain} \colorbox{red!0}{\strut Building} \colorbox{red!1}{\strut Understanding} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!1}{\strut Continental} \colorbox{red!1}{\strut Drift} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Andreas} \colorbox{red!0}{\strut Fault} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ppt} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut audio} \colorbox{red!0}{\strut narrative} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut Also} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Earthquakes} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Volcanoes} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Rocks} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Minerals} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Introduction} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Geology} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Kids} \colorbox{red!3}{\strut What} \colorbox{red!1}{\strut drives} \colorbox{red!4}{\strut plate} \colorbox{red!4}{\strut tectonics} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut what} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Pangaea} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pangea} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Theory} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut move} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut animation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut movie} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut thinkquest} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut About} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut Dynamic} \colorbox{red!1}{\strut Earth} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut interactive} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Continental} \colorbox{red!1}{\strut Drift} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut animated} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut movie} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Continental} \colorbox{red!1}{\strut Drift} \colorbox{red!1}{\strut Continental} \colorbox{red!1}{\strut Drift} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Interactive} \colorbox{red!0}{\strut Quiz} \colorbox{red!1}{\strut Continental} \colorbox{red!0}{\strut Rift} \colorbox{red!0}{\strut game} \colorbox{red!1}{\strut Earthquakes} \colorbox{red!1}{\strut Volcanoes} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Teachers} \colorbox{red!4}{\strut Plate} \colorbox{red!4}{\strut Tectonics} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Wilson} \colorbox{red!0}{\strut Cycle} \colorbox{red!0}{\strut Rifting} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Clipart} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Science} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Templates} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut partnership} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut mrdonn.org} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut phillipmartin.info} \colorbox{red!0}{\strut ALL} \colorbox{red!0}{\strut ART} \colorbox{red!0}{\strut OWNED} \colorbox{red!0}{\strut BY} \colorbox{red!0}{\strut PHILLIP} \colorbox{red!0}{\strut MARTIN} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Rights} \colorbox{red!0}{\strut Reserved} 
}}}
\end{CJK*}

query: madam cj walker

94:walker, 72:c, 71:madame, 70:j, 67:madam, 58:who, 54:cj, 35:when, 32:died, 30:born


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Madam} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut J.} \colorbox{red!7}{\strut Walker} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut Madame} \colorbox{red!4}{\strut CJ} \colorbox{red!7}{\strut Walker} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!5}{\strut Madam} \colorbox{red!7}{\strut Walker} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut photograph} \colorbox{red!0}{\strut ca} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 1914} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Addison} \colorbox{red!1}{\strut Scurlock} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Madam} \colorbox{red!0}{\strut C.J} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Walker} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 23} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1867} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1919} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut was} \colorbox{red!1}{\strut an} \colorbox{red!1}{\strut American} \colorbox{red!1}{\strut businesswoman} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut hair} \colorbox{red!1}{\strut care} \colorbox{red!1}{\strut entrepreneur} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tycoon} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut philanthropist} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut She} \colorbox{red!2}{\strut died} \colorbox{red!0}{\strut after} \colorbox{red!1}{\strut World} \colorbox{red!0}{\strut War} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Her} \colorbox{red!1}{\strut fortune} \colorbox{red!1}{\strut was} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut developing} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut marketing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut hugely} \colorbox{red!1}{\strut successful} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut beauty} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut hair} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut black} \colorbox{red!1}{\strut women} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut she} \colorbox{red!2}{\strut founded} \colorbox{red!5}{\strut Madam} \colorbox{red!0}{\strut C.J} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Walker} \colorbox{red!1}{\strut Manufacturing} \colorbox{red!1}{\strut Company} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Guinness} \colorbox{red!0}{\strut Book} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Records} \colorbox{red!0}{\strut cites} \colorbox{red!7}{\strut Walker} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut female} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut black} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut white} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut who} \colorbox{red!1}{\strut became} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut millionaire} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut achievements} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 2002} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut scholar} \colorbox{red!0}{\strut Molefi} \colorbox{red!0}{\strut Kete} \colorbox{red!0}{\strut Asante} \colorbox{red!0}{\strut listed} \colorbox{red!5}{\strut Madam} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut J.} \colorbox{red!7}{\strut Walker} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut Greatest} \colorbox{red!1}{\strut African} \colorbox{red!1}{\strut Americans} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Biography} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Further} \colorbox{red!0}{\strut reading} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut Biography} \colorbox{red!0}{\strut She} \colorbox{red!1}{\strut was} \colorbox{red!2}{\strut born} \colorbox{red!2}{\strut Sarah} \colorbox{red!0}{\strut Breedlove} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Delta} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut member} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut her} \colorbox{red!1}{\strut family} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut born} \colorbox{red!1}{\strut free} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Her} \colorbox{red!1}{\strut parents} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut been} \colorbox{red!1}{\strut slaves} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!1}{\strut age} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut she} \colorbox{red!1}{\strut married} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut man} \colorbox{red!1}{\strut named} \colorbox{red!0}{\strut Moses} \colorbox{red!0}{\strut McWilliams} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut was} \colorbox{red!0}{\strut widowed} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut age} \colorbox{red!0}{\strut 20} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut She} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut moved} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut St.} \colorbox{red!1}{\strut Louis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Missouri} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut join} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut brothers} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Sarah} \colorbox{red!1}{\strut worked} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut laundress} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut dollar} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut half} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut she} \colorbox{red!1}{\strut was} \colorbox{red!0}{\strut able} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut educate} \colorbox{red!0}{\strut her} \colorbox{red!1}{\strut daughter} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut living} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut St.} \colorbox{red!1}{\strut Louis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut joined} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut Paul} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut African} \colorbox{red!0}{\strut Methodist} \colorbox{red!0}{\strut Episcopal} \colorbox{red!0}{\strut Church} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!1}{\strut helped} \colorbox{red!0}{\strut develop} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut speaking} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut interpersonal} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut organizational} \colorbox{red!0}{\strut skills} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut She} \colorbox{red!1}{\strut was} \colorbox{red!1}{\strut married} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1894} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut John} \colorbox{red!1}{\strut Davis} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut divorced} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut nine} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut later} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut When} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut began} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut lose} 
}}}
\end{CJK*}

99:walker, 71:madam, 70:madame, 58:what, 52:c, 46:cj, 40:j, 30:house, 24:famous, 23:hudson


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!1}{\strut Inventors} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Finance} \colorbox{red!1}{\strut Inventors} \colorbox{red!0}{\strut Email} \colorbox{red!1}{\strut Inventors} \colorbox{red!0}{\strut Basics} \colorbox{red!1}{\strut Black} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Month} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Bios} \colorbox{red!0}{\strut Free} \colorbox{red!1}{\strut Inventors} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut Forum} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut House} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Mary} \colorbox{red!0}{\strut Bellis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut About.com} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut madam} \colorbox{red!4}{\strut walker} \colorbox{red!0}{\strut beauty} \colorbox{red!1}{\strut black} \colorbox{red!0}{\strut inventor} \colorbox{red!0}{\strut photo} \colorbox{red!0}{\strut gallery} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut House} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Villa} \colorbox{red!1}{\strut Lewaro} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Irvington-on-the-Hudson} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut circa} \colorbox{red!0}{\strut 1987} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Gallery} \colorbox{red!0}{\strut Index} \colorbox{red!0}{\strut Prev} \colorbox{red!0}{\strut Next} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut House} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Villa} \colorbox{red!1}{\strut Lewaro} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Irvington-on-the-Hudson} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut circa} \colorbox{red!0}{\strut 1987} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut LOC} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut designed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1918} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut African} \colorbox{red!1}{\strut American} \colorbox{red!0}{\strut architect} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Vertner} \colorbox{red!0}{\strut Woodson} \colorbox{red!1}{\strut Tandy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut African} \colorbox{red!1}{\strut American} \colorbox{red!1}{\strut cosmetics} \colorbox{red!0}{\strut magnate} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Hudson} \colorbox{red!0}{\strut River} \colorbox{red!0}{\strut north} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut asked} \colorbox{red!1}{\strut why} \colorbox{red!0}{\strut she} \colorbox{red!1}{\strut built} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut palatial} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut replied} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut built} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut herself} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut blacks} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut see} \colorbox{red!2}{\strut what} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut accomplished} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut hard} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut determination} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Villa} \colorbox{red!1}{\strut Lewaro} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut estate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut significance} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut architect} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut original} \colorbox{red!1}{\strut owner} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tandy} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut licensed} \colorbox{red!1}{\strut black} \colorbox{red!0}{\strut architect} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut building} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut knows} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut exact} \colorbox{red!0}{\strut worth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut considered} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nation} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut African} \colorbox{red!1}{\strut American} \colorbox{red!1}{\strut woman} \colorbox{red!0}{\strut millionaire} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Learn} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Madam} \colorbox{red!0}{\strut C.J} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut Prev} \colorbox{red!0}{\strut Next} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Biography} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut Her} \colorbox{red!0}{\strut Own} \colorbox{red!0}{\strut Ground} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Times} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Madam} \colorbox{red!2}{\strut C} \colorbox{red!2}{\strut J} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut Books} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut Madame} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Compare} \colorbox{red!0}{\strut Prices} \colorbox{red!1}{\strut Famous} \colorbox{red!1}{\strut Black} \colorbox{red!1}{\strut Inventors} \colorbox{red!1}{\strut Famous} \colorbox{red!1}{\strut Black} \colorbox{red!1}{\strut Inventors} \colorbox{red!1}{\strut Inventors} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Finance} \colorbox{red!1}{\strut Inventors} \colorbox{red!1}{\strut African} \colorbox{red!1}{\strut Americans} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut Gallery} \colorbox{red!3}{\strut Madame} \colorbox{red!2}{\strut CJ} \colorbox{red!4}{\strut Walker} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut House} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut Popular} \colorbox{red!0}{\strut Latest} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut Add} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut iGoogle} \colorbox{red!0}{\strut My} 
}}}
\end{CJK*}

query: cass county missouri

98:cass, 96:county, 96:counties, 52:missouri, 28:location, 28:located, 27:population, 27:kansas, 22:harrisonville, 13:state


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Cass} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Missouri} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!5}{\strut Cass} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Missouri} \colorbox{red!0}{\strut Map} \colorbox{red!1}{\strut Location} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Missouri} \colorbox{red!2}{\strut Missouri} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut location} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Statistics} \colorbox{red!0}{\strut Founded} \colorbox{red!0}{\strut 1835} \colorbox{red!1}{\strut Seat} \colorbox{red!1}{\strut Harrisonville} \colorbox{red!1}{\strut Area} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Total} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Land} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Water} \colorbox{red!0}{\strut 703} \colorbox{red!0}{\strut sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,821} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 699sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,810km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 0.52} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Population} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Density} \colorbox{red!0}{\strut 97,133} \colorbox{red!0}{\strut 138sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 53.3km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Website} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.casscounty.com} \colorbox{red!5}{\strut Cass} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut county} \colorbox{red!1}{\strut located} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Missouri} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut population} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut 82,092} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Its} \colorbox{red!5}{\strut county} \colorbox{red!1}{\strut seat} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut Harrisonville} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut county} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut organized} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1835} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut Van} \colorbox{red!0}{\strut Buren} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut renamed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1848} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut Michigan} \colorbox{red!0}{\strut U.S} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Senator} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut presidential} \colorbox{red!0}{\strut candidate} \colorbox{red!0}{\strut Lewis} \colorbox{red!5}{\strut Cass} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Cass} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Kansas} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut Metropolitan} \colorbox{red!1}{\strut Area} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Geography} \colorbox{red!0}{\strut 1.1} \colorbox{red!0}{\strut Adjacent} \colorbox{red!5}{\strut counties} \colorbox{red!0}{\strut 1.2} \colorbox{red!0}{\strut Major} \colorbox{red!0}{\strut highways} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Demographics} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Cities} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut towns} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Geography} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Census} \colorbox{red!0}{\strut Bureau} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut county} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut total} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 703square} \colorbox{red!1}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,820km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 699square} \colorbox{red!1}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,810km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut land} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 4square} \colorbox{red!1}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0.52} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut water} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adjacent} \colorbox{red!5}{\strut counties} \colorbox{red!1}{\strut Jackson} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut north} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Johnson} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut east} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Henry} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut southeast} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Bates} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut south} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Miami} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Kansas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut west} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Johnson} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Kansas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut northwest} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Johnson} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Kansas} \colorbox{red!1}{\strut Jackson} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut v} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut e} \colorbox{red!0}{\strut Miami} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Kansas} \colorbox{red!0}{\strut Johnson} \colorbox{red!5}{\strut County} \colorbox{red!5}{\strut Cass} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Missouri} \colorbox{red!0}{\strut Bates} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut Henry} \colorbox{red!5}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Major} \colorbox{red!0}{\strut highways} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Route} \colorbox{red!0}{\strut 71} \colorbox{red!0}{\strut Route} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Route} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Route} \colorbox{red!0}{\strut 58} \colorbox{red!0}{\strut Route} \colorbox{red!0}{\strut 291} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Demographics} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut census} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} 
}}}
\end{CJK*}

100:cass, 88:lewis, 86:named, 73:places, 39:cities, 32:towns, 24:county, 24:city, 22:list, 21:town


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut places} \colorbox{red!3}{\strut named} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut Lewis} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut places} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!3}{\strut named} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut Lewis} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut 1} \colorbox{red!1}{\strut Counties} \colorbox{red!0}{\strut 2} \colorbox{red!1}{\strut Cities} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut towns} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut villages} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Townships} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Geographical} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Buildings} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Streets} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut Notes} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Counties} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Illinois} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Michigan} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Minnesota} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Missouri} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Nebraska} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Texas} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Bartow} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut formerly} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Civil} \colorbox{red!0}{\strut War} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Cities} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut towns} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut villages} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut Virginia} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Michigan} \colorbox{red!0}{\strut Cassopolis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Michigan} \colorbox{red!0}{\strut Casstown} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ohio} \colorbox{red!0}{\strut Cassville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut formerly} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut county} \colorbox{red!0}{\strut seat} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Bartow} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut formerly} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Civil} \colorbox{red!0}{\strut War} \colorbox{red!0}{\strut Cassville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Missouri} \colorbox{red!0}{\strut Cassville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Pennsylvania} \colorbox{red!0}{\strut Cassville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Wisconsin} \colorbox{red!0}{\strut Cassville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Townships} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Illinois} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Fulton} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Illinois} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Clay} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Dubois} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Greene} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut LaPorte} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ohio} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Pulaksi} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Sullivan} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut White} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Indiana} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Boone} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Cass} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Cedar} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Clayton} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Guthrie} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hamilton} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Harrison} \colorbox{red!1}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iowa} \colorbox{red!3}{\strut Cass} \colorbox{red!0}{\strut Township} 
}}}
\end{CJK*}

query: adobe indian houses

96:adobe, 92:house, 63:what, 63:style, 61:styles, 33:homes, 33:home, 27:built, 25:designed, 24:pueblo


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Adobe} \colorbox{red!5}{\strut House} \colorbox{red!1}{\strut Plans} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Southwestern} \colorbox{red!5}{\strut House} \colorbox{red!1}{\strut Plans} \colorbox{red!0}{\strut From} \colorbox{red!1}{\strut Southwestern} \colorbox{red!4}{\strut Style} \colorbox{red!2}{\strut Homes} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Plans} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Southwest} \colorbox{red!5}{\strut House} \colorbox{red!1}{\strut Plans} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Favorites} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut Cart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Search} \colorbox{red!5}{\strut Adobe} \colorbox{red!5}{\strut House} \colorbox{red!1}{\strut Plans} \colorbox{red!0}{\strut Our} \colorbox{red!5}{\strut adobe} \colorbox{red!5}{\strut house} \colorbox{red!1}{\strut plans} \colorbox{red!0}{\strut were} \colorbox{red!1}{\strut designed} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut architects} \colorbox{red!0}{\strut working} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Southwest} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut popular} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut regions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut country} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Our} \colorbox{red!0}{\strut adobe-style} \colorbox{red!1}{\strut floor} \colorbox{red!1}{\strut plans} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut unique} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut distinctive} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut thick} \colorbox{red!1}{\strut walls} \colorbox{red!0}{\strut allow} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut unusual} \colorbox{red!1}{\strut design} \colorbox{red!0}{\strut elements} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Common} \colorbox{red!1}{\strut Characteristics} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Adobe-Style} \colorbox{red!2}{\strut Home} \colorbox{red!1}{\strut Plans} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Popular} \colorbox{red!1}{\strut Revival} \colorbox{red!4}{\strut Style} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Southwest} \colorbox{red!0}{\strut Also} \colorbox{red!0}{\strut called} \colorbox{red!0}{\strut Santa} \colorbox{red!1}{\strut Fe} \colorbox{red!4}{\strut Style} \colorbox{red!0}{\strut Low-pitched} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut flat} \colorbox{red!1}{\strut roof} \colorbox{red!1}{\strut Pitched} \colorbox{red!1}{\strut roof} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut ceramic} \colorbox{red!0}{\strut tiles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Spanish} \colorbox{red!0}{\strut Colonial} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Monterey} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Flat} \colorbox{red!1}{\strut roof} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut surrounding} \colorbox{red!0}{\strut parapet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Santa} \colorbox{red!1}{\strut Fe} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Pueblo} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thick} \colorbox{red!1}{\strut masonry} \colorbox{red!1}{\strut walls} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Revival} \colorbox{red!3}{\strut styles} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut strawbale} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut standard} \colorbox{red!1}{\strut construction} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Recessed} \colorbox{red!0}{\strut windows} \colorbox{red!0}{\strut Simple} \colorbox{red!0}{\strut doors} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut smaller} \colorbox{red!0}{\strut windows} \colorbox{red!1}{\strut Roof} \colorbox{red!0}{\strut beams} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cross-members} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut exposed} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut button} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut browse} \colorbox{red!0}{\strut our} \colorbox{red!5}{\strut adobe} \colorbox{red!2}{\strut home} \colorbox{red!1}{\strut plans} \colorbox{red!0}{\strut !} \colorbox{red!4}{\strut What} \colorbox{red!0}{\strut follows} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut excerpts} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Shelter} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Lester} \colorbox{red!0}{\strut Walker} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut published} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Overlook} \colorbox{red!0}{\strut Press} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1997} \colorbox{red!1}{\strut Pueblo} \colorbox{red!1}{\strut Revival} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Adobe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Pueblo} \colorbox{red!1}{\strut Revival} \colorbox{red!4}{\strut Style} \colorbox{red!0}{\strut takes} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut prototypical} \colorbox{red!5}{\strut adobe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut flat-roofed} \colorbox{red!1}{\strut pueblos} \colorbox{red!2}{\strut built} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Hopi} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Pueblo} \colorbox{red!1}{\strut Indians} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut Mexico} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut northern} \colorbox{red!1}{\strut Arizona} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut introduced} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut California} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Boston} \colorbox{red!1}{\strut architect} \colorbox{red!0}{\strut A.C.} \colorbox{red!0}{\strut Schweinfurth} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut hotel} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Montalvo} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1894} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Later} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut he} \colorbox{red!1}{\strut designed} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut buildings} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Hearst} \colorbox{red!0}{\strut ranch} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Pleasanton} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut style} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut 1915} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut Mexico} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Arizona} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Pueblo} \colorbox{red!1}{\strut Revival} \colorbox{red!4}{\strut Style} \colorbox{red!0}{\strut became} \colorbox{red!1}{\strut popular} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut hotels} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut college} \colorbox{red!0}{\strut campus} \colorbox{red!1}{\strut buildings} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut churches} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut public} \colorbox{red!1}{\strut buildings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut marriage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut archeological} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut modern} \colorbox{red!0}{\strut spirit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Pueblo} \colorbox{red!1}{\strut Revival} \colorbox{red!5}{\strut house} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut original} \colorbox{red!1}{\strut pueblo} 
}}}
\end{CJK*}

66:what, 47:grants, 44:housing, 43:grant, 38:block, 36:pih, 28:development, 27:program, 27:hud, 26:indian


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Public} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Indian} \colorbox{red!3}{\strut Housing} \colorbox{red!0}{\strut About} \colorbox{red!2}{\strut PIH} \colorbox{red!1}{\strut Public} \colorbox{red!3}{\strut housing} \colorbox{red!1}{\strut Asset} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut Senior} \colorbox{red!3}{\strut Housing} \colorbox{red!0}{\strut Clearinghouse} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut CapFund} \colorbox{red!0}{\strut HOPE} \colorbox{red!0}{\strut VI} \colorbox{red!3}{\strut Housing} \colorbox{red!0}{\strut Choice} \colorbox{red!1}{\strut Vouchers} \colorbox{red!1}{\strut Public} \colorbox{red!3}{\strut Housing} \colorbox{red!0}{\strut Reform} \colorbox{red!2}{\strut Indian} \colorbox{red!3}{\strut Housing} \colorbox{red!0}{\strut CODETALK} \colorbox{red!1}{\strut Community} \colorbox{red!2}{\strut development} \colorbox{red!0}{\strut Homeownership} \colorbox{red!3}{\strut Grants} \colorbox{red!0}{\strut Common} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut events} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut regulations} \colorbox{red!0}{\strut Publications} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut Online} \colorbox{red!0}{\strut systems} \colorbox{red!0}{\strut Training} \colorbox{red!0}{\strut Rental} \colorbox{red!3}{\strut Housing} \colorbox{red!0}{\strut Integrity} \colorbox{red!0}{\strut Improvement} \colorbox{red!0}{\strut Project} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Estate} \colorbox{red!0}{\strut Assessment} \colorbox{red!3}{\strut Grants} \colorbox{red!1}{\strut Notices} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rules} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut regulations} \colorbox{red!0}{\strut Library} \colorbox{red!0}{\strut Forums} \colorbox{red!0}{\strut Online} \colorbox{red!0}{\strut systems} \colorbox{red!2}{\strut HUD} \colorbox{red!0}{\strut news} \colorbox{red!1}{\strut Homes} \colorbox{red!0}{\strut Resources} \colorbox{red!1}{\strut Communities} \colorbox{red!0}{\strut Working} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut HUD} \colorbox{red!0}{\strut Tools} \colorbox{red!0}{\strut Webcasts} \colorbox{red!0}{\strut Mailing} \colorbox{red!0}{\strut lists} \colorbox{red!0}{\strut RSS} \colorbox{red!0}{\strut Feeds} \colorbox{red!0}{\strut Help} \colorbox{red!3}{\strut Grants} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut State} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut version} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Information} \colorbox{red!2}{\strut PIH} \colorbox{red!3}{\strut grant} \colorbox{red!0}{\strut information} \colorbox{red!1}{\strut Funds} \colorbox{red!1}{\strut available} \colorbox{red!3}{\strut Grants} \colorbox{red!0}{\strut Inventory} \colorbox{red!1}{\strut Did} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Know} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Office} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Native} \colorbox{red!1}{\strut American} \colorbox{red!2}{\strut Programs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ONAP} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut developed} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut guidebooks} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut assist} \colorbox{red!3}{\strut grant} \colorbox{red!0}{\strut staff} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut recipients} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Grants} \colorbox{red!1}{\strut Evaluation} \colorbox{red!0}{\strut Guidebook} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 259} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Provides} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut processing} \colorbox{red!1}{\strut requirements} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut procedures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tools} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut Grants} \colorbox{red!1}{\strut Evaluation} \colorbox{red!0}{\strut staff} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Revisions} \colorbox{red!0}{\strut APR} \colorbox{red!0}{\strut Review} \colorbox{red!0}{\strut Guidelines} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut APR} \colorbox{red!0}{\strut Reviewer} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Revisions} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Grants} \colorbox{red!1}{\strut Evaluation} \colorbox{red!0}{\strut Guidebook} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 105} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Revision} \colorbox{red!0}{\strut Procedures} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Pursuing} \colorbox{red!0}{\strut Enforcement} \colorbox{red!0}{\strut Actions} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Delinquent} \colorbox{red!0}{\strut Annual} \colorbox{red!0}{\strut Performance} \colorbox{red!0}{\strut Reports} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 35} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Revised} \colorbox{red!1}{\strut Sanction} \colorbox{red!1}{\strut Process} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 56} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Self-Monitoring} \colorbox{red!0}{\strut Guidebook} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 177} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Assists} \colorbox{red!2}{\strut IHBG} \colorbox{red!0}{\strut recipients} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut meeting} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut self-monitoring} \colorbox{red!0}{\strut responsibilities} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut NAHASDA} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut What} \colorbox{red!1}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut grants} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut available} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut Indian} \colorbox{red!3}{\strut housing} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut community} \colorbox{red!2}{\strut development} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut HUD} \colorbox{red!1}{\strut awards} \colorbox{red!3}{\strut grants} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut tribes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!2}{\strut Indian} \colorbox{red!0}{\strut entities} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut competitive} \colorbox{red!1}{\strut process} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut discretionary} \colorbox{red!3}{\strut grants} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut formula} \colorbox{red!0}{\strut basis} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Indian} \colorbox{red!3}{\strut Housing} \colorbox{red!2}{\strut Block} \colorbox{red!3}{\strut Grant} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut IHBG} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Program} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut competitions} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut discretionary} \colorbox{red!3}{\strut grant} \colorbox{red!2}{\strut programs} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut announced} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut HUD} \colorbox{red!0}{\strut SuperNOFA} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut published} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut each} \colorbox{red!1}{\strut Federal} \colorbox{red!0}{\strut fiscal} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Program} \colorbox{red!0}{\strut Descriptions} \colorbox{red!2}{\strut Indian} \colorbox{red!1}{\strut Community} \colorbox{red!2}{\strut Development} \colorbox{red!2}{\strut Block} \colorbox{red!3}{\strut Grant} \colorbox{red!2}{\strut Program} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ICDBG} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Provides} \colorbox{red!2}{\strut Indian} 
}}}
\end{CJK*}

query: interview thank

97:thanking, 97:thank, 91:notes, 90:note, 46:interview, 45:interviewers, 43:job, 42:send, 40:interviews, 38:what


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Fast} \colorbox{red!0}{\strut Find} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Looking} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut Main} \colorbox{red!1}{\strut Articles} \colorbox{red!1}{\strut Art} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Culture} \colorbox{red!3}{\strut Business} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut Entertaining} \colorbox{red!1}{\strut Fashion} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Holidays} \colorbox{red!1}{\strut Home} \colorbox{red!2}{\strut Life} \colorbox{red!1}{\strut Internet} \colorbox{red!1}{\strut Legal} \colorbox{red!1}{\strut Guide} \colorbox{red!1}{\strut Pets} \colorbox{red!0}{\strut Pop} \colorbox{red!1}{\strut Culture} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut Recreation} \colorbox{red!0}{\strut Science} \colorbox{red!0}{\strut Shopping} \colorbox{red!1}{\strut Society} \colorbox{red!0}{\strut Sports} \colorbox{red!0}{\strut Technology} \colorbox{red!1}{\strut Tax} \colorbox{red!1}{\strut Guides} \colorbox{red!0}{\strut Toy} \colorbox{red!0}{\strut Reviews} \colorbox{red!1}{\strut Travel} \colorbox{red!1}{\strut Guides} \colorbox{red!1}{\strut Wine} \colorbox{red!1}{\strut Guides} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Money} \colorbox{red!1}{\strut MAIN} \colorbox{red!3}{\strut Business} \colorbox{red!3}{\strut Office} \colorbox{red!2}{\strut Life} \colorbox{red!3}{\strut Interviews} \colorbox{red!0}{\strut Thank-You} \colorbox{red!7}{\strut Notes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut Integral} \colorbox{red!1}{\strut Part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Your} \colorbox{red!2}{\strut Career} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut little} \colorbox{red!1}{\strut practice} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut vital} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut generating} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut interest} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut potential} \colorbox{red!2}{\strut employers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut critical} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut few} \colorbox{red!3}{\strut job} \colorbox{red!0}{\strut seekers} \colorbox{red!0}{\strut actually} \colorbox{red!1}{\strut do} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!8}{\strut THANK} \colorbox{red!1}{\strut YOU} \colorbox{red!7}{\strut NOTE} \colorbox{red!0}{\strut !} \colorbox{red!4}{\strut Interview} \colorbox{red!1}{\strut experts} \colorbox{red!0}{\strut agree} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut EVERY} \colorbox{red!3}{\strut job} \colorbox{red!1}{\strut hunter} \colorbox{red!0}{\strut MUST} \colorbox{red!3}{\strut send} \colorbox{red!0}{\strut thank-you} \colorbox{red!7}{\strut notes} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut EVERY} \colorbox{red!4}{\strut interview} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut completely} \colorbox{red!0}{\strut ignore} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut bit} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut wisdom} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut order} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut huge} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut candidates} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut job} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut send} \colorbox{red!0}{\strut thank-you} \colorbox{red!7}{\strut notes} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut EVERYONE} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut meet} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut interviewadministrative} \colorbox{red!1}{\strut assistants} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut managers} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut interviewers} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut people} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut met} \colorbox{red!2}{\strut who} \colorbox{red!0}{\strut already} \colorbox{red!1}{\strut do} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut job} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut targeting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut resume} \colorbox{red!0}{\strut clients} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut let} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut call} \colorbox{red!0}{\strut him} \colorbox{red!0}{\strut Mike} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Certified} \colorbox{red!1}{\strut Arborist} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Tree} \colorbox{red!1}{\strut Care} \colorbox{red!1}{\strut Professional} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut San} \colorbox{red!0}{\strut Diego} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut His} \colorbox{red!0}{\strut goal} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut move} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut consulting} \colorbox{red!0}{\strut arena} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Very} \colorbox{red!0}{\strut soon} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut speaking} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut phone} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut owner} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut prominent} \colorbox{red!1}{\strut tree} \colorbox{red!1}{\strut care} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mike} \colorbox{red!1}{\strut mailed} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut brief} \colorbox{red!7}{\strut note} \colorbox{red!8}{\strut thanking} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut owner} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut his} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut consideration} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

100:thank, 99:letter, 98:letters, 90:email, 46:how, 42:writing, 38:interviews, 38:interview, 35:write, 23:example


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Tech} \colorbox{red!0}{\strut Careers} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Careers} \colorbox{red!0}{\strut Tech} \colorbox{red!0}{\strut Careers} \colorbox{red!3}{\strut Email} \colorbox{red!0}{\strut Tech} \colorbox{red!0}{\strut Careers} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Job} \colorbox{red!0}{\strut Career} \colorbox{red!0}{\strut Advancement} \colorbox{red!0}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut Forum} \colorbox{red!0}{\strut Apply} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut guide} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut About} \colorbox{red!1}{\strut Interview} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letters} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut About.com} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letters} \colorbox{red!0}{\strut job} \colorbox{red!1}{\strut interviews} \colorbox{red!0}{\strut business} \colorbox{red!3}{\strut letter} \colorbox{red!1}{\strut writing} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut interview} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut good} \colorbox{red!0}{\strut idea} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut follow} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tech} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut email} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut appropriate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut guidelines} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut examples} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut writing} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut several} \colorbox{red!1}{\strut examples} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut interview} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letters} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut appropriate} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut different} \colorbox{red!1}{\strut interview} \colorbox{red!0}{\strut situations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Interview} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letters} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Guidelines} \colorbox{red!0}{\strut Guidelines} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut writing} \colorbox{red!1}{\strut interview} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letters} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut write} \colorbox{red!1}{\strut interview} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letters} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut write} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut send} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Interview} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut General} \colorbox{red!0}{\strut Format} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut general} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut sent} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut interview} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Interview} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letter} \colorbox{red!0}{\strut An} \colorbox{red!1}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut general} \colorbox{red!1}{\strut interview} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut mentions} \colorbox{red!1}{\strut follow} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut discussions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Interview} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letter} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Additional} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut interview} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut convey} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut training} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut forgot} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut mention} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut interview} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Campus} \colorbox{red!1}{\strut Interview} \colorbox{red!0}{\strut An} \colorbox{red!1}{\strut interview} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut appropriate} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut on-campus} \colorbox{red!1}{\strut interview} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Interview} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Scheduling} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Follow} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut sample} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut mentions} \colorbox{red!1}{\strut scheduling} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut follow} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut discussion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Interview} \colorbox{red!3}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Addressing} \colorbox{red!0}{\strut Concerns} \colorbox{red!0}{\strut An} \colorbox{red!1}{\strut interview} \colorbox{red!3}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut addresses} \colorbox{red!0}{\strut concerns} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut brought} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut interview} 
}}}
\end{CJK*}

query: culpeper national cemetery

92:cemeteries, 91:cemetery, 71:culpeper, 59:located, 49:virginia, 48:what, 46:locate, 40:quantico, 36:resting, 36:open


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut National} \colorbox{red!1}{\strut Veterans} \colorbox{red!5}{\strut Cemeteries} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut numerous} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemeteries} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Virginia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut remain} \colorbox{red!2}{\strut open} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut burial} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Arlington} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!2}{\strut Quantico} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!4}{\strut Culpeper} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!1}{\strut Arlington} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut only} \colorbox{red!2}{\strut national} \colorbox{red!5}{\strut cemetery} \colorbox{red!1}{\strut administered} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Army} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Arlington} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut final} \colorbox{red!2}{\strut resting} \colorbox{red!1}{\strut place} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut presidents} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Supreme} \colorbox{red!0}{\strut Court} \colorbox{red!0}{\strut justices} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut astronauts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Medal} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Honor} \colorbox{red!0}{\strut recipients} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut notable} \colorbox{red!0}{\strut Americans} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut perhaps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Tomb} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Unknown} \colorbox{red!0}{\strut Soldier} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Arlington} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut strict} \colorbox{red!1}{\strut eligibility} \colorbox{red!1}{\strut requirements} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Nelsen} \colorbox{red!1}{\strut Funeral} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Crematory} \colorbox{red!0}{\strut personnel} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut assist} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut determining} \colorbox{red!1}{\strut eligibility} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Quantico} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut located} \colorbox{red!0}{\strut midway} \colorbox{red!0}{\strut between} \colorbox{red!1}{\strut Fredericksburg} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Washington} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut DC.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut land} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut Marine} \colorbox{red!0}{\strut Corps} \colorbox{red!1}{\strut Base} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Quantico} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut hosted} \colorbox{red!1}{\strut military} \colorbox{red!0}{\strut operations} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 200} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut Virginia} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut naval} \colorbox{red!0}{\strut operations} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1775} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut blockade} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Confederate} \colorbox{red!0}{\strut army} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 1977} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Marine} \colorbox{red!0}{\strut Corps} \colorbox{red!0}{\strut donated} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut land} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!0}{\strut Administration} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut cemetery} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut dedicated} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1983} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Culpeper} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut located} \colorbox{red!0}{\strut approximately} \colorbox{red!0}{\strut 35} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut west} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Fredericksburg} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut Culpeper} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut site} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut Civil} \colorbox{red!0}{\strut War} \colorbox{red!0}{\strut battles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Following} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut war} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut reburial} \colorbox{red!0}{\strut program} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut initiated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut federal} \colorbox{red!0}{\strut government} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut locate} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut remains} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut Union} \colorbox{red!0}{\strut soldiers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut reinter} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut national} \colorbox{red!5}{\strut cemeteries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut scattered} \colorbox{red!0}{\strut Union} \colorbox{red!1}{\strut dead} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut vicinity} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Culpeper} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut established} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1867} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 1996} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Culpeper} \colorbox{red!2}{\strut National} \colorbox{red!5}{\strut Cemetery} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut placed} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut National} \colorbox{red!0}{\strut Register} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Historic} \colorbox{red!1}{\strut Places} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4650} \colorbox{red!0}{\strut S.} \colorbox{red!0}{\strut Laburnum} \colorbox{red!0}{\strut Ave.Richmond} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut VA23231804.222.8601} \colorbox{red!0}{\strut info} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut nelsencares.com} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2008} \colorbox{red!1}{\strut Nelsen} \colorbox{red!1}{\strut Funeral} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut FuneralNet} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Staff} 
}}}
\end{CJK*}

96:culpeper, 94:county, 31:cemetery, 18:graveyard, 16:renfrow, 15:photos, 13:near, 13:joan, 10:teresa, 10:hill


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Culpeper} \colorbox{red!4}{\strut County} \colorbox{red!1}{\strut Cemetery} \colorbox{red!1}{\strut Photos} \colorbox{red!0}{\strut RecorderSubmitter} \colorbox{red!0}{\strut Instructions} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Submitting} \colorbox{red!0}{\strut Transcriptions} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Photos} \colorbox{red!0}{\strut USGenWeb} \colorbox{red!0}{\strut Archives} \colorbox{red!0}{\strut National} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Feature} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Camera} \colorbox{red!0}{\strut icon} \colorbox{red!0}{\strut indicates} \colorbox{red!1}{\strut photos} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Culpeper} \colorbox{red!4}{\strut County} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Listing} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Saints} \colorbox{red!0}{\strut Episcopal} \colorbox{red!0}{\strut Church} \colorbox{red!1}{\strut Graveyard} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Apperson} \colorbox{red!1}{\strut Graveyard} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Armstrong} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Bell} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Bethel} \colorbox{red!0}{\strut Baptist} \colorbox{red!0}{\strut Church} \colorbox{red!1}{\strut Graveyard} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Bickers} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut aka} \colorbox{red!0}{\strut Mountain} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Bleak} \colorbox{red!0}{\strut Hill} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Alanthus} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Bolen} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Broadus} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Brown} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Brown} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Store} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Brown} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Slate} \colorbox{red!0}{\strut Mills} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Brown} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Rixeyville} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Brown} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Reva} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Clatterbuck} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Colvin} \colorbox{red!1}{\strut Cemetery} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Colvin} \colorbox{red!1}{\strut Graveyard} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Clover} \colorbox{red!0}{\strut Hill} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Cloverdale} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Compton} \colorbox{red!1}{\strut Graveyard} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Cooke} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Coons} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Coons} \colorbox{red!1}{\strut Cemetery} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Coon} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Cemetery} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Corbin} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Crane} \colorbox{red!1}{\strut Graveyard} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Crigler} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Daniel} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Davenport-Thompson} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Dowlman} \colorbox{red!0}{\strut Tomb} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Eggborn} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Teresa} \colorbox{red!0}{\strut Kelley} \colorbox{red!0}{\strut Fairview} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Fant} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Griffinsburg} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Farish} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Mitchells} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Ficklin} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Eggbornsville} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Fishback} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Jeffersonton} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Fleetwood} \colorbox{red!0}{\strut Hill} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Elkwood} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Francis} \colorbox{red!0}{\strut Browning} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Lebanon} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Freeman} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Rixeyville} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Gaines} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut Karen} \colorbox{red!0}{\strut Bennett} \colorbox{red!0}{\strut Garnett} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Gourdvine} \colorbox{red!0}{\strut Church} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Guinn} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Winston} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Hall} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Winston} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Hitt} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!5}{\strut Culpeper} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Hoffman} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut near} \colorbox{red!0}{\strut Rixeyville} \colorbox{red!1}{\strut Joan} \colorbox{red!1}{\strut Renfrow} \colorbox{red!0}{\strut Jameson} \colorbox{red!1}{\strut Cemetery} \colorbox{red!0}{\strut -} 
}}}
\end{CJK*}

query: iowa food stamp program

95:food, 87:stamp, 72:iowa, 55:what, 42:survey, 41:fsp, 39:leavers, 37:leaver, 31:program, 30:when


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut or} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Publications} \colorbox{red!0}{\strut Publications} \colorbox{red!4}{\strut Iowa} \colorbox{red!6}{\strut Food} \colorbox{red!5}{\strut Stamp} \colorbox{red!2}{\strut Leavers} \colorbox{red!2}{\strut Survey} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Final} \colorbox{red!2}{\strut Report} \colorbox{red!0}{\strut Helen} \colorbox{red!0}{\strut H.} \colorbox{red!0}{\strut Jensen} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Steven} \colorbox{red!0}{\strut Garasky} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Cory} \colorbox{red!0}{\strut Wessman} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut S.M} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Nusser} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ERS} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Elizabeth} \colorbox{red!0}{\strut Dagata} \colorbox{red!0}{\strut E-FAN} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 02014-1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut pp} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 2002} \colorbox{red!1}{\strut Enrollment} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Iowa} \colorbox{red!0}{\strut s} \colorbox{red!6}{\strut Food} \colorbox{red!5}{\strut Stamp} \colorbox{red!2}{\strut Program} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut FSP} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut sharply} \colorbox{red!0}{\strut decreased} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 1990s} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut significant} \colorbox{red!0}{\strut changes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut social} \colorbox{red!1}{\strut assistance} \colorbox{red!1}{\strut programs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut State} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut passage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut Responsibility} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Work} \colorbox{red!0}{\strut Opportunity} \colorbox{red!0}{\strut Reconciliation} \colorbox{red!0}{\strut Act} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1996} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut good} \colorbox{red!1}{\strut economic} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Data} \colorbox{red!0}{\strut collected} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 1999} \colorbox{red!2}{\strut survey} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut well-being} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut families} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut had} \colorbox{red!1}{\strut participated} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Iowa} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut FSP} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1997} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut immediately} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut introduction} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut regulations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Nearly} \colorbox{red!0}{\strut 58} \colorbox{red!1}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut those} \colorbox{red!1}{\strut participating} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut FSP} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1997} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut participating} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut program} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut interviewed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1999} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Those} \colorbox{red!1}{\strut who} \colorbox{red!1}{\strut left} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut FSP} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1997} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut including} \colorbox{red!1}{\strut working} \colorbox{red!1}{\strut age} \colorbox{red!1}{\strut adults} \colorbox{red!0}{\strut without} \colorbox{red!1}{\strut dependents} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut disability} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut better} \colorbox{red!1}{\strut economic} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut employment} \colorbox{red!0}{\strut outcomes} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Adults} \colorbox{red!0}{\strut without} \colorbox{red!1}{\strut dependents} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut disability} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut remained} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut FSP} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1997} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut greatest} \colorbox{red!0}{\strut hardships} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut income} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut less} \colorbox{red!1}{\strut contribution} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut earned} \colorbox{red!0}{\strut income} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut experience} \colorbox{red!6}{\strut food} \colorbox{red!0}{\strut insecurity} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut hunger} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut half} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut households} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut survey} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut private} \colorbox{red!6}{\strut food} \colorbox{red!1}{\strut assistance} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut description} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut methodology} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut study} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!4}{\strut Iowa} \colorbox{red!6}{\strut Food} \colorbox{red!5}{\strut Stamp} \colorbox{red!2}{\strut Leavers} \colorbox{red!2}{\strut Survey} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Methodology} \colorbox{red!2}{\strut Report} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut E-FAN} \colorbox{red!0}{\strut 02014-2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Keywords} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Food} \colorbox{red!5}{\strut Stamp} \colorbox{red!2}{\strut Program} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut PRWORA} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ABAWD} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut leaver} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut report} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Chapters} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut Acrobat} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut format} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Abstract} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

99:stamps, 99:stamp, 99:food, 45:did, 42:program, 41:programs, 22:benefits, 20:welfare, 19:south, 17:legal


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Overview} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Programs} \colorbox{red!3}{\strut Program} \colorbox{red!0}{\strut Components} \colorbox{red!1}{\strut Children} \colorbox{red!0}{\strut Special} \colorbox{red!0}{\strut Populations} \colorbox{red!0}{\strut Caseload} \colorbox{red!1}{\strut Characteristics} \colorbox{red!3}{\strut Program} \colorbox{red!0}{\strut Outcomes} \colorbox{red!0}{\strut Family} \colorbox{red!0}{\strut Formation} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Database} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Database} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Database} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Key} \colorbox{red!0}{\strut Topics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Caseload} \colorbox{red!1}{\strut Characteristics} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Food} \colorbox{red!6}{\strut Stamps} \colorbox{red!0}{\strut Caseload} \colorbox{red!1}{\strut Characteristics} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 1996} \colorbox{red!1}{\strut welfare} \colorbox{red!1}{\strut law} \colorbox{red!1}{\strut mandated} \colorbox{red!1}{\strut changes} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut food} \colorbox{red!1}{\strut nutrition} \colorbox{red!3}{\strut programs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut notably} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut scaling} \colorbox{red!1}{\strut back} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut Food} \colorbox{red!6}{\strut Stamp} \colorbox{red!3}{\strut Program} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Following} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut implementation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut PRWORA} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut participation} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut Food} \colorbox{red!6}{\strut Stamp} \colorbox{red!3}{\strut Program} \colorbox{red!0}{\strut declined} \colorbox{red!0}{\strut considerably} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut approximately} \colorbox{red!0}{\strut 28} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 1995} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 1998} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut trend} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut reverse} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut Food} \colorbox{red!6}{\strut Stamps} \colorbox{red!1}{\strut caseloads} \colorbox{red!1}{\strut increasing} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 28} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut 32} \colorbox{red!0}{\strut months} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut increase} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut slowed} \colorbox{red!0}{\strut economy} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut growing} \colorbox{red!0}{\strut efforts} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut connect} \colorbox{red!0}{\strut eligible} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut benefits} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Four} \colorbox{red!0}{\strut studies} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Arizona} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Illinois} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Iowa} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut South} \colorbox{red!1}{\strut Carolina} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut examine} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut status} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut those} \colorbox{red!1}{\strut who} \colorbox{red!1}{\strut leave} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut Food} \colorbox{red!6}{\strut Stamp} \colorbox{red!3}{\strut Program} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut South} \colorbox{red!1}{\strut Carolina} \colorbox{red!0}{\strut project} \colorbox{red!0}{\strut expands} \colorbox{red!0}{\strut upon} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut welfare} \colorbox{red!0}{\strut leavers} \colorbox{red!0}{\strut study} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut projects} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut pay} \colorbox{red!0}{\strut close} \colorbox{red!0}{\strut attention} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut able-bodied} \colorbox{red!1}{\strut adults} \colorbox{red!1}{\strut ages} \colorbox{red!0}{\strut 18-50} \colorbox{red!0}{\strut without} \colorbox{red!1}{\strut dependents} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut time} \colorbox{red!1}{\strut limits} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut meet} \colorbox{red!0}{\strut specific} \colorbox{red!1}{\strut work} \colorbox{red!1}{\strut requirements} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Researchers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut administrative} \colorbox{red!0}{\strut records} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut surveys} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut analyze} \colorbox{red!0}{\strut employment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut earnings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut income} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut publicprivate} \colorbox{red!3}{\strut programs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Illinois} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Arizona} \colorbox{red!1}{\strut released} \colorbox{red!0}{\strut final} \colorbox{red!1}{\strut reports} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut early} \colorbox{red!0}{\strut 2001} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut final} \colorbox{red!1}{\strut report} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut South} \colorbox{red!1}{\strut Carolina} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut released} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 2001} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut final} \colorbox{red!1}{\strut report} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Iowa} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut released} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 2002} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Farm} \colorbox{red!1}{\strut Bill} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut passed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut late} \colorbox{red!0}{\strut 2001} \colorbox{red!0}{\strut restored} \colorbox{red!6}{\strut Food} \colorbox{red!6}{\strut Stamps} \colorbox{red!1}{\strut benefits} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut immigrants} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut country} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut immigrant} \colorbox{red!1}{\strut children} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut regardless} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut entry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut immigrants} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut disabilities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Selected} \colorbox{red!0}{\strut Summary} \colorbox{red!1}{\strut Findings} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Brief} 
}}}
\end{CJK*}

query: american military university

93:american, 89:military, 86:university, 86:universities, 46:what, 37:campus, 31:amu, 24:colleges, 21:apus, 16:engineering


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!18}{\strut American} \colorbox{red!17}{\strut Military} \colorbox{red!17}{\strut University} \colorbox{red!7}{\strut Campus} \colorbox{red!2}{\strut Login} \colorbox{red!1}{\strut User} \colorbox{red!1}{\strut ID} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Password} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Forgot} \colorbox{red!1}{\strut Your} \colorbox{red!2}{\strut Password} \colorbox{red!1}{\strut or} \colorbox{red!1}{\strut User} \colorbox{red!1}{\strut ID} \colorbox{red!1}{\strut ?} \colorbox{red!1}{\strut Call} \colorbox{red!3}{\strut Admissions} \colorbox{red!0}{\strut 1-877-777-9081} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Other} \colorbox{red!1}{\strut Calls} \colorbox{red!0}{\strut 1-877-755-2787} \colorbox{red!0}{\strut E-mail} \colorbox{red!3}{\strut Admissions} \colorbox{red!1}{\strut Live} \colorbox{red!1}{\strut Chat} \colorbox{red!1}{\strut Find} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut Rep} \colorbox{red!1}{\strut Near} \colorbox{red!1}{\strut You} \colorbox{red!1}{\strut Schedule} \colorbox{red!0}{\strut ofClasses} \colorbox{red!0}{\strut E-mail} \colorbox{red!0}{\strut StudentServices} \colorbox{red!1}{\strut Transfer} \colorbox{red!2}{\strut Credit} \colorbox{red!2}{\strut Center} \colorbox{red!9}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut New} \colorbox{red!1}{\strut Interested} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut BS} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut Engineering} \colorbox{red!1}{\strut ?} \colorbox{red!1}{\strut Take} \colorbox{red!1}{\strut Our} \colorbox{red!1}{\strut Survey} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut Internet} \colorbox{red!1}{\strut Connectivity} \colorbox{red!1}{\strut Issues} \colorbox{red!1}{\strut Overseas} \colorbox{red!4}{\strut APUS} \colorbox{red!1}{\strut Announces} \colorbox{red!2}{\strut President} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Honor} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut Dean} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Lists} \colorbox{red!6}{\strut AMU} \colorbox{red!1}{\strut Makes} \colorbox{red!1}{\strut It} \colorbox{red!1}{\strut on} \colorbox{red!2}{\strut List} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut Top} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut Military-Friendly} \colorbox{red!5}{\strut Colleges} \colorbox{red!1}{\strut and} \colorbox{red!17}{\strut Universities} \colorbox{red!1}{\strut Online} \colorbox{red!3}{\strut Programs} \colorbox{red!1}{\strut Over} \colorbox{red!0}{\strut 50} \colorbox{red!1}{\strut Online} \colorbox{red!2}{\strut Associate} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Bachelor} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut Master} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Degrees} \colorbox{red!1}{\strut Homeland} \colorbox{red!1}{\strut Security} \colorbox{red!1}{\strut Sports} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut Sciences} \colorbox{red!1}{\strut Intelligence} \colorbox{red!1}{\strut Public} \colorbox{red!1}{\strut Administration} \colorbox{red!1}{\strut Emergency} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Disaster} \colorbox{red!1}{\strut Management} \colorbox{red!1}{\strut Transportation} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Logistics} \colorbox{red!1}{\strut Management} \colorbox{red!1}{\strut History} \colorbox{red!1}{\strut Security} \colorbox{red!1}{\strut Ma} 
}}}
\end{CJK*}

99:articulation, 97:agreements, 95:agreement, 79:what, 47:vccs, 45:transfer, 32:colleges, 28:university, 28:universities, 28:college


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut HOME} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SITE} \colorbox{red!0}{\strut INDEX} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Z} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SEARCH} \colorbox{red!0}{\strut Current} \colorbox{red!0}{\strut Students} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Academic} \colorbox{red!1}{\strut Advising} \colorbox{red!1}{\strut ADMISSIONS} \colorbox{red!1}{\strut REGISTRATION} \colorbox{red!1}{\strut ACADEMIC} \colorbox{red!1}{\strut ADVISING} \colorbox{red!3}{\strut TRANSFER} \colorbox{red!1}{\strut PLANNING} \colorbox{red!3}{\strut Transfer} \colorbox{red!1}{\strut Program} \colorbox{red!3}{\strut Transfer} \colorbox{red!6}{\strut Agreement} \colorbox{red!1}{\strut Types} \colorbox{red!1}{\strut Guaranteed} \colorbox{red!1}{\strut Admissions} \colorbox{red!6}{\strut Agreements} \colorbox{red!6}{\strut Articulation} \colorbox{red!6}{\strut Agreements} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut BRCC} \colorbox{red!1}{\strut Degree} \colorbox{red!3}{\strut Transfer} \colorbox{red!1}{\strut Advising} \colorbox{red!0}{\strut Guides} \colorbox{red!3}{\strut Transfer} \colorbox{red!0}{\strut Links} \colorbox{red!1}{\strut ORIENTATION} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Students} \colorbox{red!1}{\strut General} \colorbox{red!1}{\strut ADVISING} \colorbox{red!0}{\strut Advanced} \colorbox{red!0}{\strut Standing} \colorbox{red!0}{\strut Faculty} \colorbox{red!0}{\strut Advisors} \colorbox{red!1}{\strut Graduation} \colorbox{red!0}{\strut Honors} \colorbox{red!1}{\strut Program} \colorbox{red!1}{\strut Program} \colorbox{red!0}{\strut Selection} \colorbox{red!0}{\strut DISABILITY} \colorbox{red!0}{\strut SERVICES} \colorbox{red!1}{\strut PEER} \colorbox{red!0}{\strut TUTORING} \colorbox{red!0}{\strut LEARNING} \colorbox{red!0}{\strut ASSISTANCE} \colorbox{red!0}{\strut CTR} \colorbox{red!0}{\strut CLUBS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ORGANIZATIONS} \colorbox{red!1}{\strut STUDENT} \colorbox{red!0}{\strut ACTIVITIES} \colorbox{red!0}{\strut CAREER} \colorbox{red!0}{\strut RESOURCES} \colorbox{red!6}{\strut Articulation} \colorbox{red!6}{\strut Agreements} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut BRCC} \colorbox{red!1}{\strut Degree} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut articulation} \colorbox{red!6}{\strut agreement} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Associate} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Arts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Sciences} \colorbox{red!1}{\strut Degree} \colorbox{red!0}{\strut CollegeUniversity} \colorbox{red!3}{\strut Transfer} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut VCCS} \colorbox{red!0}{\strut has} \colorbox{red!6}{\strut articulation} \colorbox{red!6}{\strut agreements} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut four} \colorbox{red!1}{\strut year} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut public} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut collegesuniversities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Students} \colorbox{red!1}{\strut graduating} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut degree} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut granted} \colorbox{red!1}{\strut junior} \colorbox{red!0}{\strut status} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut collegesuniversities} \colorbox{red!0}{\strut waive} \colorbox{red!1}{\strut general} \colorbox{red!1}{\strut education} \colorbox{red!1}{\strut requirements} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut may} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut general} \colorbox{red!1}{\strut education} \colorbox{red!1}{\strut requirements} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut met} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!3}{\strut Transfer} \colorbox{red!1}{\strut Advising} \colorbox{red!0}{\strut Guides} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut transfer} \colorbox{red!0}{\strut institution-specific} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut Associates} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Applied} \colorbox{red!0}{\strut Science} \colorbox{red!1}{\strut Degrees} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut files} \colorbox{red!0}{\strut linked} \colorbox{red!0}{\strut below} \colorbox{red!1}{\strut require} \colorbox{red!0}{\strut Adobe} \colorbox{red!0}{\strut Acrobat} \colorbox{red!0}{\strut Reader} \colorbox{red!0}{\strut Accounting} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Administration} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Justice} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Eastern} \colorbox{red!0}{\strut Kentucky} \colorbox{red!0}{\strut University-} \colorbox{red!2}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Justice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Safety} \colorbox{red!0}{\strut Ferrum} \colorbox{red!2}{\strut College} \colorbox{red!0}{\strut Criminal} \colorbox{red!0}{\strut Justice} \colorbox{red!1}{\strut Program} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Computer} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Electronic} \colorbox{red!0}{\strut Technology} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Old} \colorbox{red!0}{\strut Dominion} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Computer} \colorbox{red!0}{\strut Science} \colorbox{red!0}{\strut James} \colorbox{red!0}{\strut Madison} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Human} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut Systems} \colorbox{red!0}{\strut Technology} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Radford} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Manufacturing} \colorbox{red!0}{\strut Technology} \colorbox{red!0}{\strut Old} \colorbox{red!0}{\strut Dominion} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Mechanical} \colorbox{red!0}{\strut Design} \colorbox{red!0}{\strut Technology} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Old} \colorbox{red!0}{\strut Dominion} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Nursing} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Old} \colorbox{red!0}{\strut Dominion} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Technical} \colorbox{red!0}{\strut Studies} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Old} \colorbox{red!0}{\strut Dominion} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Veterinary} \colorbox{red!0}{\strut Technology} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Military} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut CONTACT} \colorbox{red!0}{\strut Counseling} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut Houff} \colorbox{red!1}{\strut Student} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut M-Th} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 815} \colorbox{red!0}{\strut am-500} \colorbox{red!0}{\strut pm} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: supper painting

99:supper, 66:did, 63:painting, 62:painted, 62:paint, 54:how, 44:leonardo, 34:why, 34:last, 32:who


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!1}{\strut Art} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Education} \colorbox{red!1}{\strut Art} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Email} \colorbox{red!1}{\strut Art} \colorbox{red!0}{\strut History} \colorbox{red!1}{\strut Artists} \colorbox{red!0}{\strut Styles} \colorbox{red!1}{\strut Works} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Art} \colorbox{red!0}{\strut Free} \colorbox{red!1}{\strut Art} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut Forum} \colorbox{red!3}{\strut Leonardo} \colorbox{red!1}{\strut da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut Last} \colorbox{red!7}{\strut Supper} \colorbox{red!0}{\strut Ten} \colorbox{red!0}{\strut Common} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Painting} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Shelley} \colorbox{red!0}{\strut Esaak} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut About.com} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut leonardo} \colorbox{red!1}{\strut da} \colorbox{red!2}{\strut vinci} \colorbox{red!2}{\strut last} \colorbox{red!7}{\strut supper} \colorbox{red!1}{\strut italian} \colorbox{red!1}{\strut renaissance} \colorbox{red!2}{\strut frescoes} \colorbox{red!1}{\strut murals} \colorbox{red!3}{\strut Leonardo} \colorbox{red!1}{\strut da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Italian} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1452-1519} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Last} \colorbox{red!7}{\strut Supper} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1495-98} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tempera} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut mixed} \colorbox{red!0}{\strut media} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut plaster} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 460} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 880} \colorbox{red!0}{\strut cm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 15.09} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 28.87} \colorbox{red!0}{\strut ft.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Convent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Santa} \colorbox{red!1}{\strut Maria} \colorbox{red!0}{\strut delle} \colorbox{red!1}{\strut Grazie} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Milan} \colorbox{red!2}{\strut Why} \colorbox{red!5}{\strut did} \colorbox{red!3}{\strut Leonardo} \colorbox{red!4}{\strut paint} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Because} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut employer} \colorbox{red!0}{\strut requested} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Leonardo} \colorbox{red!1}{\strut worked} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Ludovico} \colorbox{red!1}{\strut Sforza} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Duke} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Milan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut eighteen} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1482-99} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Duke} \colorbox{red!1}{\strut decided} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut wanted} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut particular} \colorbox{red!0}{\strut religious} \colorbox{red!0}{\strut scene} \colorbox{red!4}{\strut painted} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut Leonardo} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut who} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut stupid} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut decided} \colorbox{red!4}{\strut painting} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut perfect} \colorbox{red!0}{\strut financial} \colorbox{red!0}{\strut sense} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut How} \colorbox{red!1}{\strut big} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut huge} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 460} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 880} \colorbox{red!0}{\strut cm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 29} \colorbox{red!0}{\strut feet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut covers} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut entire} \colorbox{red!0}{\strut large} \colorbox{red!1}{\strut wall} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut unlike} \colorbox{red!0}{\strut reproductions} \colorbox{red!1}{\strut sized} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut hang} \colorbox{red!0}{\strut neatly} \colorbox{red!0}{\strut behind} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut sofa} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Where} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut original} \colorbox{red!1}{\strut mural} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut wall} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut refectory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dining} \colorbox{red!0}{\strut hall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Convent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Santa} \colorbox{red!1}{\strut Maria} \colorbox{red!0}{\strut delle} \colorbox{red!1}{\strut Grazie} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Milan} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Italy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut reproduction} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut fifty} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut easily} \colorbox{red!1}{\strut found} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut image} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Last} \colorbox{red!7}{\strut Supper} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut put} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut everything} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut mirrors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut mouse} \colorbox{red!0}{\strut pads} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut musical} \colorbox{red!0}{\strut pillows} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!3}{\strut Leonardo} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut still} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut earning} \colorbox{red!0}{\strut billions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut insert} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut currency} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut licensing} \colorbox{red!0}{\strut fees} \colorbox{red!0}{\strut alone} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut How} \colorbox{red!2}{\strut long} \colorbox{red!5}{\strut did} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut take} \colorbox{red!3}{\strut Leonardo} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut paint} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut began} 
}}}
\end{CJK*}

87:painting, 79:painted, 58:paint, 55:supper, 53:italian, 45:italy, 31:fresco, 30:vinci, 30:art, 29:renaissance


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Italian} \colorbox{red!2}{\strut Renaissance} \colorbox{red!1}{\strut Artists} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut L} \colorbox{red!3}{\strut Italian} \colorbox{red!2}{\strut Renaissance} \colorbox{red!1}{\strut Artists} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Z} \colorbox{red!3}{\strut Italian} \colorbox{red!2}{\strut Renaissance} \colorbox{red!0}{\strut MovementsPeriods} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Art} \colorbox{red!0}{\strut Glossary} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Terms} \colorbox{red!0}{\strut Contemporary} \colorbox{red!0}{\strut Abstract} \colorbox{red!2}{\strut Art} \colorbox{red!0}{\strut Unique} \colorbox{red!0}{\strut Gifts} \colorbox{red!1}{\strut Oil} \colorbox{red!6}{\strut Painting} \colorbox{red!1}{\strut Reproductions} \colorbox{red!1}{\strut Sculpture} \colorbox{red!1}{\strut Reproductions} \colorbox{red!2}{\strut Art} \colorbox{red!0}{\strut Puzzles} \colorbox{red!1}{\strut Da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!6}{\strut Painting} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!1}{\strut 1498} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mixed} \colorbox{red!1}{\strut technique} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 460} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 880} \colorbox{red!0}{\strut cm} \colorbox{red!1}{\strut Convent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Santa} \colorbox{red!1}{\strut Maria} \colorbox{red!0}{\strut delle} \colorbox{red!1}{\strut Grazie} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Milan} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut fine} \colorbox{red!2}{\strut art} \colorbox{red!1}{\strut reproductions} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!6}{\strut painting} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut 1498} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut traditional} \colorbox{red!0}{\strut true} \colorbox{red!2}{\strut fresco} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut buon} \colorbox{red!2}{\strut fresco} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut painted} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut wet} \colorbox{red!1}{\strut plaster} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!5}{\strut painted} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut dry} \colorbox{red!1}{\strut plaster} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut tempera} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut fresco} \colorbox{red!0}{\strut secco} \colorbox{red!0}{\strut technique.Da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!6}{\strut painting} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut refectory} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut dining} \colorbox{red!0}{\strut hall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut convent} \colorbox{red!0}{\strut ofSanta} \colorbox{red!1}{\strut Maria} \colorbox{red!0}{\strut della} \colorbox{red!1}{\strut Grazie} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Milan} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Italy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut stone} \colorbox{red!1}{\strut wall} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut prepared} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!6}{\strut painting} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut sealing} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut stone} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut pitch} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mastic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut gesso} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut experimental} \colorbox{red!1}{\strut technique} \colorbox{red!0}{\strut caused} \colorbox{red!0}{\strut rapid} \colorbox{red!0}{\strut deterioration} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!6}{\strut painting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut described} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Vasari} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Leonardo} \colorbox{red!0}{\strut biographer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ruined} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut 1556} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut dry} \colorbox{red!4}{\strut paint} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!6}{\strut painting} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut flaking} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut early} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut 1517} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut consequence} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut experimental} \colorbox{red!1}{\strut technique} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Da} \colorbox{red!2}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Last} \colorbox{red!3}{\strut Supper} \colorbox{red!6}{\strut painting} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut undergone} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut restorations} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1726} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut last} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1999} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut took} \colorbox{red!0}{\strut 21} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut finish} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: hobby stores

82:stores, 82:store, 82:hobby, 67:shop, 58:hobbies, 38:tools, 29:games, 25:toys, 22:hobbyist, 21:shopping


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut Gr8} \colorbox{red!1}{\strut Shopping} \colorbox{red!1}{\strut Sites} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut WWW} \colorbox{red!1}{\strut Sponsored} \colorbox{red!0}{\strut Listing} \colorbox{red!0}{\strut Navigate} \colorbox{red!1}{\strut Antiques} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Collectibles} \colorbox{red!1}{\strut Auctions} \colorbox{red!1}{\strut Autos} \colorbox{red!0}{\strut Beauty} \colorbox{red!1}{\strut Products} \colorbox{red!0}{\strut Books} \colorbox{red!1}{\strut Children} \colorbox{red!0}{\strut Classifieds} \colorbox{red!1}{\strut Clothing} \colorbox{red!1}{\strut Consumer} \colorbox{red!1}{\strut Electronics} \colorbox{red!1}{\strut Crafts} \colorbox{red!0}{\strut Death} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut Directories} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Ethnic} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Regional} \colorbox{red!0}{\strut Flowers} \colorbox{red!0}{\strut Food} \colorbox{red!0}{\strut Furniture} \colorbox{red!0}{\strut General} \colorbox{red!1}{\strut Merchandise} \colorbox{red!0}{\strut Gifts} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Holidays} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Garden} \colorbox{red!0}{\strut Jewelry} \colorbox{red!0}{\strut Major} \colorbox{red!1}{\strut Retailers} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut Niche} \colorbox{red!0}{\strut Office} \colorbox{red!1}{\strut Products} \colorbox{red!1}{\strut Pets} \colorbox{red!0}{\strut Photography} \colorbox{red!0}{\strut Publications} \colorbox{red!1}{\strut Recreation} \colorbox{red!0}{\strut Sports} \colorbox{red!1}{\strut Tobacco} \colorbox{red!3}{\strut Tools} \colorbox{red!2}{\strut Toys} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Games} \colorbox{red!0}{\strut Travel} \colorbox{red!1}{\strut Vehicles} \colorbox{red!0}{\strut Visual} \colorbox{red!0}{\strut Arts} \colorbox{red!0}{\strut Weddings} \colorbox{red!0}{\strut Submission} \colorbox{red!1}{\strut Policies} \colorbox{red!0}{\strut Article} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut Submissions} \colorbox{red!1}{\strut Copyright} \colorbox{red!1}{\strut License} \colorbox{red!1}{\strut Agreement} \colorbox{red!0}{\strut Guidelines} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Authors} \colorbox{red!1}{\strut Corporate} \colorbox{red!1}{\strut Policies} \colorbox{red!0}{\strut Advertising} \colorbox{red!1}{\strut Childrens} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Use} \colorbox{red!1}{\strut Site} \colorbox{red!3}{\strut Tools} \colorbox{red!1}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Home} \colorbox{red!2}{\strut Toys} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Games} \colorbox{red!5}{\strut Hobby} \colorbox{red!5}{\strut Stores} \colorbox{red!1}{\strut Categories} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Models} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,802} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Shopping} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Crafts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Supplies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4,126} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Shopping} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Recreation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5,820} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Gr8} \colorbox{red!1}{\strut Sites} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Might} \colorbox{red!0}{\strut Find} \colorbox{red!1}{\strut Useful} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Clock} \colorbox{red!0}{\strut And} \colorbox{red!1}{\strut Craft} \colorbox{red!1}{\strut Supplies} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Clock} \colorbox{red!1}{\strut movements} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut clock} \colorbox{red!0}{\strut kits} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut clock} \colorbox{red!1}{\strut parts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut craft} \colorbox{red!1}{\strut supplies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut UK} \colorbox{red!1}{\strut based} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Downtown} \colorbox{red!4}{\strut Hobbies} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Offers} \colorbox{red!1}{\strut radio} \colorbox{red!1}{\strut controlled} \colorbox{red!1}{\strut aircraft} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut boats} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut cars} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut trucks} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut rockets} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Frontline} \colorbox{red!4}{\strut Hobbies} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut A} \colorbox{red!1}{\strut full} \colorbox{red!0}{\strut line} \colorbox{red!5}{\strut hobby} \colorbox{red!4}{\strut shop} \colorbox{red!1}{\strut offering} \colorbox{red!0}{\strut online} \colorbox{red!0}{\strut sales} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Gizmo-Guru.Com} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Takara} \colorbox{red!0}{\strut Beyblades} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut RC} \colorbox{red!0}{\strut planes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Bit} \colorbox{red!0}{\strut Char-G} \colorbox{red!1}{\strut cars} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Crush} \colorbox{red!0}{\strut gear} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Astrojax} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Digimon} \colorbox{red!1}{\strut digivice} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Konami} \colorbox{red!0}{\strut Digi-Q} \colorbox{red!0}{\strut tanks} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Tomy} \colorbox{red!1}{\strut Micro} \colorbox{red!1}{\strut pets} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Yu-Gi-Oh} \colorbox{red!0}{\strut cards} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Also} \colorbox{red!0}{\strut Playstation} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Xbox} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Game} \colorbox{red!0}{\strut Boy} \colorbox{red!0}{\strut Advanced} \colorbox{red!0}{\strut accessories} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MP3} \colorbox{red!0}{\strut players} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Gooding} \colorbox{red!5}{\strut Store} \colorbox{red!5}{\strut Hobby} \colorbox{red!4}{\strut Shop} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Diecast} \colorbox{red!1}{\strut models} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut HO} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut N} \colorbox{red!1}{\strut scale} \colorbox{red!1}{\strut model} \colorbox{red!0}{\strut railroads} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut nostalgic} \colorbox{red!0}{\strut tin} \colorbox{red!0}{\strut thermometers} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Hammond} \colorbox{red!4}{\strut Hobbies} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Toys} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Offering} \colorbox{red!1}{\strut dolls} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut telescopes} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut model} \colorbox{red!1}{\strut trains} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rockets} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut games} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut puzzles} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut collectibles} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Hobbies} \colorbox{red!1}{\strut Plus} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Offers} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut wide} \colorbox{red!0}{\strut selection} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut games} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut toys} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut crafts} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut model} \colorbox{red!0}{\strut kits} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut puzzles} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Hobby} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Scale} \colorbox{red!1}{\strut model} \colorbox{red!4}{\strut shop} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut Japan} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Military} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ships} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut airplanes} 
}}}
\end{CJK*}

99:hobby, 98:lobby, 41:stores, 35:store, 25:manager, 25:management, 18:retail, 14:sales, 11:louisiana, 10:alabama


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Retail} \colorbox{red!0}{\strut Careers} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sales} \colorbox{red!0}{\strut Associate} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Grand} \colorbox{red!0}{\strut Island} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Nebraska} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Essential} \colorbox{red!0}{\strut Personnel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 011609} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Design} \colorbox{red!0}{\strut ConsultantSales} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Omaha} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Nebraska} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Incentive} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut pay} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut guaranteed} \colorbox{red!0}{\strut minimum} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Bassett} \colorbox{red!1}{\strut Sales} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut SalesDesign} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Bassett} \colorbox{red!0}{\strut Furniture} \colorbox{red!0}{\strut Direct} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 010309} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lawrence} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Kansas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Atlanta} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Zanesville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ohio} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Dallas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Texas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Baton} \colorbox{red!0}{\strut Rouge} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Florence} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Carolina} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Greenville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Carolina} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Spartanburg} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Carolina} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Gadsden} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Alabama} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Montgomery} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Alabama} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Biloxi} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mississippi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Hammond} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lake} \colorbox{red!0}{\strut Charles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Co-Manager} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut Monroe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Hobby} \colorbox{red!4}{\strut Lobby} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 121808} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut Applied} \colorbox{red!0}{\strut Information} \colorbox{red!1}{\strut Management} \colorbox{red!0}{\strut Institute} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Rights} 
}}}
\end{CJK*}

query: civil right movement

99:rights, 99:civil, 98:right, 98:movements, 98:movement, 41:who, 35:african, 33:american, 26:blacks, 26:americans


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut African-American} \colorbox{red!4}{\strut Civil} \colorbox{red!4}{\strut Rights} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19551968} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut American} \colorbox{red!4}{\strut civil} \colorbox{red!4}{\strut rights} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut references} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut external} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut sources} \colorbox{red!0}{\strut remain} \colorbox{red!0}{\strut unclear} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut insufficient} \colorbox{red!0}{\strut inline} \colorbox{red!0}{\strut citations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut improve} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut introducing} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut precise} \colorbox{red!0}{\strut citations} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut appropriate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut November} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut American} \colorbox{red!4}{\strut Civil} \colorbox{red!4}{\strut Rights} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut redirects} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut African-American} \colorbox{red!4}{\strut Civil} \colorbox{red!4}{\strut Rights} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 18961954} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Prominent} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!4}{\strut Civil} \colorbox{red!4}{\strut Rights} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut W.} \colorbox{red!0}{\strut E.} \colorbox{red!0}{\strut B} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Du} \colorbox{red!1}{\strut Bois} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut top} \colorbox{red!4}{\strut right} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Malcolm} \colorbox{red!0}{\strut X} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut bottom} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Martin} \colorbox{red!1}{\strut Luther} \colorbox{red!0}{\strut King} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Jr.} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut bottom} \colorbox{red!4}{\strut right} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rosa} \colorbox{red!0}{\strut Parks} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut American} \colorbox{red!4}{\strut Civil} \colorbox{red!4}{\strut Rights} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19551968} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut refers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut reform} \colorbox{red!4}{\strut movements} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut aimed} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut abolishing} \colorbox{red!1}{\strut racial} \colorbox{red!0}{\strut discrimination} \colorbox{red!0}{\strut against} \colorbox{red!2}{\strut African} \colorbox{red!1}{\strut Americans} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut restoring} \colorbox{red!0}{\strut suffrage} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Southern} \colorbox{red!1}{\strut states} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut covers} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut phase} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut movement} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 1954} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 1968} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut particularly} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut 1966} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut emergence} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Black} \colorbox{red!0}{\strut Power} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut lasted} \colorbox{red!0}{\strut roughly} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 1966} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 1975} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut enlarged} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut aims} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Civil} \colorbox{red!4}{\strut Rights} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut include} \colorbox{red!1}{\strut racial} \colorbox{red!0}{\strut dignity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut economic} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut political} \colorbox{red!0}{\strut self-sufficiency} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut freedom} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut oppression} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut whites} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut those} \colorbox{red!2}{\strut who} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut active} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Civil} \colorbox{red!4}{\strut Rights} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut organizations} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut SNCC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut CORE} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut SCLC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut prefer} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut term} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Southern} \colorbox{red!1}{\strut Freedom} \colorbox{red!4}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut struggle} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut far} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut just} \colorbox{red!4}{\strut civil} \colorbox{red!4}{\strut rights} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut law} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut fundamental} \colorbox{red!0}{\strut issues} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut freedom} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut respect} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut dignity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut economic} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut social} \colorbox{red!1}{\strut equality} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut disputed} \colorbox{red!0}{\strut election} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1876} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Reconstruction} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

102:rights, 101:civil, 100:movement, 55:african, 36:american, 31:timeline, 25:free, 21:human, 20:close, 19:which


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Powerset} \colorbox{red!0}{\strut Microsoft} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut Feedback} \colorbox{red!0}{\strut Need} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Powerlabs} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut Keyboard} \colorbox{red!0}{\strut shortcuts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut toggle} \colorbox{red!0}{\strut Off} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut Finding} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Freebase} \colorbox{red!0}{\strut searching} \colorbox{red!0}{\strut Factz} \colorbox{red!0}{\strut searching} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut searching} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1209} \colorbox{red!0}{\strut advanced} \colorbox{red!0}{\strut sort} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut sort} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut sentence} \colorbox{red!0}{\strut help} \colorbox{red!1}{\strut close} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1600} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1799} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19551968} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Prominent} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Integrating} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Deliberate} \colorbox{red!0}{\strut Speed} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut contains} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut history} \colorbox{red!0}{\strut interviews} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut African} \colorbox{red!1}{\strut American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!0}{\strut pioneers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut primary} \colorbox{red!0}{\strut source} \colorbox{red!0}{\strut materials} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut photographs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut speeches} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut historical} \colorbox{red!0}{\strut documents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut Jim} \colorbox{red!0}{\strut Crow} \colorbox{red!0}{\strut laws} \colorbox{red!0}{\strut Rosa} \colorbox{red!0}{\strut Parks} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1955} \colorbox{red!0}{\strut act} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut civil} \colorbox{red!0}{\strut disobedience} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut refused} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut give} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut seat} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut bus} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut white} \colorbox{red!0}{\strut man} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut catalyst} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Anti-miscegenation} \colorbox{red!0}{\strut laws} \colorbox{red!0}{\strut Black} \colorbox{red!0}{\strut Codes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut USA} \colorbox{red!0}{\strut Racial} \colorbox{red!0}{\strut segregation} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!0}{\strut Disfranchisement} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Civil} \colorbox{red!0}{\strut War} \colorbox{red!0}{\strut Dunning} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut Group} \colorbox{red!0}{\strut Areas} \colorbox{red!0}{\strut Act} \colorbox{red!0}{\strut Second-class} \colorbox{red!0}{\strut citizen} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut Bernice} \colorbox{red!0}{\strut Fisher} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut Cleveland} \colorbox{red!0}{\strut Sellers} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut Government} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut Forest} \colorbox{red!0}{\strut Park} \colorbox{red!0}{\strut High} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Beaumont} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Texas} \colorbox{red!0}{\strut 1962} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 1982} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 18961954} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19th-century} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut civil} \colorbox{red!3}{\strut rights} \colorbox{red!0}{\strut activists} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!1}{\strut close} \colorbox{red!1}{\strut American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 18961954} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19th-century} \colorbox{red!0}{\strut African-American} \colorbox{red!3}{\strut civil} \colorbox{red!3}{\strut rights} \colorbox{red!0}{\strut activists} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Timeline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut American} \colorbox{red!3}{\strut Civil} \colorbox{red!3}{\strut Rights} \colorbox{red!3}{\strut Movement} \colorbox{red!1}{\strut close} 
}}}
\end{CJK*}

query: gs pay rate

99:pay, 94:locality, 64:gs, 36:rate, 34:rates, 30:government, 22:federal, 21:wage, 21:tables, 19:employees


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Federal} \colorbox{red!1}{\strut Jobs} \colorbox{red!1}{\strut Net} \colorbox{red!3}{\strut GS} \colorbox{red!5}{\strut Pay} \colorbox{red!0}{\strut Scales} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Feedback} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Office} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Personnel} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Official} \colorbox{red!5}{\strut Pay} \colorbox{red!0}{\strut Chart} \colorbox{red!0}{\strut 2009} \colorbox{red!1}{\strut General} \colorbox{red!1}{\strut Schedule} \colorbox{red!0}{\strut INCORPORATING} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut 2.9} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut GENERAL} \colorbox{red!0}{\strut INCREASE} \colorbox{red!0}{\strut Effective} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut BASE} \colorbox{red!2}{\strut RATE} \colorbox{red!1}{\strut TABLE} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut reference} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut General} \colorbox{red!1}{\strut Schedule} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut GS} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut government} \colorbox{red!1}{\strut employees} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut make} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut base} \colorbox{red!2}{\strut rate} \colorbox{red!5}{\strut pay} \colorbox{red!0}{\strut with} \colorbox{red!5}{\strut locality} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Locality} \colorbox{red!5}{\strut pay} \colorbox{red!2}{\strut rates} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut areas} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut specific} \colorbox{red!5}{\strut locality} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut table} \colorbox{red!0}{\strut titled} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rest} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Pay} \colorbox{red!0}{\strut varies} \colorbox{red!0}{\strut per} \colorbox{red!5}{\strut locality} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Look} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut locality} \colorbox{red!1}{\strut tables} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut metropolitan} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut determine} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut actual} \colorbox{red!1}{\strut salary} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut given} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Wage} \colorbox{red!2}{\strut rate} \colorbox{red!1}{\strut tables} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut major} \colorbox{red!0}{\strut metropolitan} \colorbox{red!1}{\strut areas} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut located} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.cpms.osd.milwage} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut comparison} \colorbox{red!0}{\strut purposes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut current} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut years} \colorbox{red!5}{\strut locality} \colorbox{red!1}{\strut tables} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut review} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2009} \colorbox{red!5}{\strut locality} \colorbox{red!5}{\strut pay} \colorbox{red!2}{\strut rates} \colorbox{red!0}{\strut 2008} \colorbox{red!5}{\strut locality} \colorbox{red!5}{\strut pay} \colorbox{red!2}{\strut rates} \colorbox{red!0}{\strut 2007} \colorbox{red!5}{\strut locality} \colorbox{red!5}{\strut pay} \colorbox{red!2}{\strut rates} \colorbox{red!0}{\strut 2006} \colorbox{red!5}{\strut locality} \colorbox{red!5}{\strut pay} \colorbox{red!2}{\strut rates} \colorbox{red!0}{\strut 2005} \colorbox{red!5}{\strut locality} \colorbox{red!5}{\strut pay} \colorbox{red!2}{\strut rates} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut upward} \colorbox{red!0}{\strut mobility} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut promotions} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Visit} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut Federal} \colorbox{red!0}{\strut Career} \colorbox{red!0}{\strut Planning} \colorbox{red!0}{\strut web} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut assists} \colorbox{red!1}{\strut federal} \colorbox{red!2}{\strut government} \colorbox{red!1}{\strut employees} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut realistic} \colorbox{red!0}{\strut Individual} \colorbox{red!0}{\strut Development} \colorbox{red!0}{\strut Plans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut IDPs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut target} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut promotions} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut government} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Federal} \colorbox{red!2}{\strut government} \colorbox{red!1}{\strut employees} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut numerous} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut attractive} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut upward} \colorbox{red!0}{\strut mobility} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Developed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut fed} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 35} \colorbox{red!0}{\strut years} \colorbox{red!1}{\strut federal} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Annual} \colorbox{red!2}{\strut Rates} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Grade} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut Grade} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut WITHIN} \colorbox{red!0}{\strut GRADE} \colorbox{red!0}{\strut AMOUNTS} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut 17540} \colorbox{red!0}{\strut 18126} \colorbox{red!0}{\strut 18709} \colorbox{red!0}{\strut 19290} \colorbox{red!0}{\strut 19873} \colorbox{red!0}{\strut 20216} \colorbox{red!0}{\strut 20792} \colorbox{red!0}{\strut 21373} \colorbox{red!0}{\strut 21396} \colorbox{red!0}{\strut 21944} \colorbox{red!0}{\strut VARIES} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 19721} \colorbox{red!0}{\strut 20190} \colorbox{red!0}{\strut 20842} \colorbox{red!0}{\strut 21396} \colorbox{red!0}{\strut 21635} \colorbox{red!0}{\strut 22271} \colorbox{red!0}{\strut 22907} \colorbox{red!0}{\strut 23543} \colorbox{red!0}{\strut 24179} \colorbox{red!0}{\strut 24815} \colorbox{red!0}{\strut VARIES} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut 21517} 
}}}
\end{CJK*}

50:rate, 41:pay, 41:gs, 33:set, 32:locality, 31:employees, 31:employee, 30:fws, 29:wage, 29:range


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut skip} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut OPM.gov} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Subject} \colorbox{red!0}{\strut Index} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Important} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Office} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Personnel} \colorbox{red!1}{\strut Management} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Ensuring} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Federal} \colorbox{red!0}{\strut Government} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut effective} \colorbox{red!0}{\strut civilian} \colorbox{red!0}{\strut workforce} \colorbox{red!1}{\strut Advanced} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Alert} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Paysetting} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Federal} \colorbox{red!1}{\strut Wage} \colorbox{red!1}{\strut System} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut General} \colorbox{red!1}{\strut Schedule} \colorbox{red!0}{\strut Movements} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut reminder} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Office} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Personnel} \colorbox{red!1}{\strut Management} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut OPM} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut issued} \colorbox{red!0}{\strut interim} \colorbox{red!1}{\strut regulations} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 31} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2005} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut changed} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut way} \colorbox{red!2}{\strut pay} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut set} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Federal} \colorbox{red!1}{\strut Wage} \colorbox{red!1}{\strut System} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut FWS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut non-General} \colorbox{red!1}{\strut Schedule} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut GS} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut employees} \colorbox{red!0}{\strut upon} \colorbox{red!1}{\strut movement} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut GS} \colorbox{red!1}{\strut position} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut maximum} \colorbox{red!1}{\strut payable} \colorbox{red!3}{\strut rate} \colorbox{red!1}{\strut rule} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut CFR} \colorbox{red!0}{\strut 531.221-223} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut pay} \colorbox{red!1}{\strut retention} \colorbox{red!1}{\strut rules} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut CFR} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut 536} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut subpart} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!1}{\strut CPM} \colorbox{red!0}{\strut 2005-10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!1}{\strut rules} \colorbox{red!0}{\strut became} \colorbox{red!1}{\strut effective} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2005} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Under} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut former} \colorbox{red!1}{\strut maximum} \colorbox{red!1}{\strut payable} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut pay} \colorbox{red!1}{\strut retention} \colorbox{red!1}{\strut rules} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut FWS} \colorbox{red!2}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut pay} \colorbox{red!0}{\strut was} \colorbox{red!2}{\strut set} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut comparing} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut FWS} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut underlying} \colorbox{red!2}{\strut GS} \colorbox{red!1}{\strut base} \colorbox{red!3}{\strut rate} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut grade} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut excluding} \colorbox{red!2}{\strut locality} \colorbox{red!2}{\strut pay} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Once} \colorbox{red!2}{\strut pay} \colorbox{red!0}{\strut was} \colorbox{red!2}{\strut set} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut underlying} \colorbox{red!2}{\strut GS} \colorbox{red!1}{\strut base} \colorbox{red!3}{\strut rate} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut pay} \colorbox{red!1}{\strut retention} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut retained} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut FWS} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut exceeded} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut step} \colorbox{red!0}{\strut 10} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut applicable} \colorbox{red!2}{\strut GS} \colorbox{red!2}{\strut locality} \colorbox{red!1}{\strut payment} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut added} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut comparing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut locality-based} \colorbox{red!2}{\strut FWS} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut GS} \colorbox{red!3}{\strut rate} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut did} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut locality} \colorbox{red!1}{\strut adjustment} \colorbox{red!0}{\strut resulted} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut substantial} \colorbox{red!2}{\strut pay} \colorbox{red!1}{\strut increases} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut affected} \colorbox{red!0}{\strut employees-an} \colorbox{red!0}{\strut anomalous} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut maximum} \colorbox{red!1}{\strut payable} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut pay} \colorbox{red!1}{\strut retention} \colorbox{red!1}{\strut rules} \colorbox{red!0}{\strut Under} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut maximum} \colorbox{red!1}{\strut payable} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut pay} \colorbox{red!1}{\strut retention} \colorbox{red!1}{\strut rules} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut employee} \colorbox{red!1}{\strut moves} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut FWS} \colorbox{red!1}{\strut position} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut GS} \colorbox{red!1}{\strut position} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut her} \colorbox{red!2}{\strut FWS} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut compared} 
}}}
\end{CJK*}

query: indiana state fairgrounds

85:state, 80:indiana, 77:fair, 75:fairgrounds, 36:largest, 35:indianapolis, 27:venue, 21:pavilion, 17:building, 14:show


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Administrative} \colorbox{red!1}{\strut Hours} \colorbox{red!1}{\strut Parking} \colorbox{red!0}{\strut Fees} \colorbox{red!0}{\strut Camping} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Hotels} \colorbox{red!7}{\strut Fairgrounds} \colorbox{red!0}{\strut 101} \colorbox{red!0}{\strut Employment} \colorbox{red!0}{\strut Press} \colorbox{red!0}{\strut Releases} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut General} \colorbox{red!1}{\strut Email} \colorbox{red!8}{\strut State} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut Largest} \colorbox{red!1}{\strut Classroom} \colorbox{red!7}{\strut Fairgrounds} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut Driving} \colorbox{red!0}{\strut Directions} \colorbox{red!1}{\strut Indy} \colorbox{red!1}{\strut Visitor} \colorbox{red!0}{\strut Information} \colorbox{red!7}{\strut Fairgrounds} \colorbox{red!1}{\strut Mission} \colorbox{red!8}{\strut State} \colorbox{red!7}{\strut Fair} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Commission} \colorbox{red!0}{\strut Inside} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Grounds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Magazine} \colorbox{red!1}{\strut Meetings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Notices} \colorbox{red!7}{\strut Fairgrounds} \colorbox{red!0}{\strut Managers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Staff} \colorbox{red!0}{\strut Year-round} \colorbox{red!1}{\strut Sponsors} \colorbox{red!0}{\strut Yearly} \colorbox{red!0}{\strut Calendar} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Events} \colorbox{red!0}{\strut Monthly} \colorbox{red!0}{\strut E-Calendar} \colorbox{red!3}{\strut Venue} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut Contract} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut Request} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Information} \colorbox{red!1}{\strut Public} \colorbox{red!1}{\strut Skating} \colorbox{red!0}{\strut Pro} \colorbox{red!0}{\strut Skate} \colorbox{red!0}{\strut Shop} \colorbox{red!0}{\strut Pepsi} \colorbox{red!1}{\strut Coliseum} \colorbox{red!0}{\strut Youth} \colorbox{red!1}{\strut Hockey} \colorbox{red!1}{\strut League} \colorbox{red!0}{\strut Winter} \colorbox{red!1}{\strut Club} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Indianapolis} \colorbox{red!8}{\strut Indiana} \colorbox{red!1}{\strut Ice} \colorbox{red!3}{\strut Venue} \colorbox{red!0}{\strut Information} \colorbox{red!1}{\strut Northwest} \colorbox{red!2}{\strut Pavilion} \colorbox{red!0}{\strut 31,800} \colorbox{red!0}{\strut sq} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ft.} \colorbox{red!1}{\strut Northwest} \colorbox{red!2}{\strut Pavilion} \colorbox{red!1}{\strut Occupancy} \colorbox{red!0}{\strut 1,000} \colorbox{red!0}{\strut 10x10} \colorbox{red!1}{\strut booths} \colorbox{red!0}{\strut 214} \colorbox{red!1}{\strut Ceiling} \colorbox{red!1}{\strut Height} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut clearance} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut center} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut clearance} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut middle} \colorbox{red!1}{\strut aisle} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut clearance} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut outer} \colorbox{red!1}{\strut aisle} \colorbox{red!1}{\strut Move} \colorbox{red!0}{\strut inout} \colorbox{red!0}{\strut daily} \colorbox{red!1}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 400} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut Daily} \colorbox{red!1}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut larger} \colorbox{red!0}{\strut version} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut layout} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut pdf} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut historic} \colorbox{red!0}{\strut 1927} \colorbox{red!1}{\strut structure} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut accommodate} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut auction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut trade} \colorbox{red!1}{\strut show} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut livestock} \colorbox{red!1}{\strut event} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut ceilings} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut flexibility} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut large} \colorbox{red!1}{\strut exhibits} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Complete} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut heat} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut overhead} \colorbox{red!0}{\strut fans} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut facility} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut round} \colorbox{red!0}{\strut comfort} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Office} \colorbox{red!1}{\strut space} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut supply} \colorbox{red!1}{\strut show} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut allows} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ease} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut show} \colorbox{red!1}{\strut operations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Wheelchair} \colorbox{red!0}{\strut accessible} \colorbox{red!0}{\strut restrooms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut overhead} \colorbox{red!0}{\strut doors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut concessions} \colorbox{red!1}{\strut space} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut additional} \colorbox{red!1}{\strut features} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut building} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Clientele} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Stewart} \colorbox{red!0}{\strut s} \colorbox{red!8}{\strut Indiana} \colorbox{red!1}{\strut Flea} \colorbox{red!1}{\strut Market} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!1}{\strut Rabbit} \colorbox{red!0}{\strut Breeders} \colorbox{red!1}{\strut Show} \colorbox{red!8}{\strut Indiana} \colorbox{red!8}{\strut State} \colorbox{red!7}{\strut Fairgrounds} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1202} \colorbox{red!0}{\strut E.} \colorbox{red!0}{\strut 38th} \colorbox{red!0}{\strut St} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Indpls.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut IN} \colorbox{red!0}{\strut 46205} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 317927-7500} \colorbox{red!1}{\strut fax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 317-927-7695} 
}}}
\end{CJK*}

97:fair, 91:indiana, 89:barn, 86:state, 20:governed, 18:fairgrounds, 14:commission, 13:education, 12:site, 12:educational


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!9}{\strut Barn} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut Indiana} \colorbox{red!8}{\strut State} \colorbox{red!2}{\strut Fairgrounds} \colorbox{red!0}{\strut The} \colorbox{red!9}{\strut Barn} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut Indiana} \colorbox{red!8}{\strut State} \colorbox{red!2}{\strut Fairgrounds} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut governed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Board} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Trustees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut Indiana} \colorbox{red!8}{\strut State} \colorbox{red!9}{\strut Fair} \colorbox{red!1}{\strut Commission} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut works} \colorbox{red!0}{\strut toward} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut mission} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut bridging} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut agricultural} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut consumer} \colorbox{red!1}{\strut public} \colorbox{red!0}{\strut through} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!9}{\strut Barn} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut Indiana} \colorbox{red!8}{\strut State} \colorbox{red!2}{\strut Fairgrounds} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut provide} \colorbox{red!0}{\strut on-site} \colorbox{red!1}{\strut educational} \colorbox{red!1}{\strut programming} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut northside} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut Indiana} \colorbox{red!8}{\strut State} \colorbox{red!2}{\strut Fairgrounds} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut beyond} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Educational} \colorbox{red!1}{\strut Programming} \colorbox{red!1}{\strut Professional} \colorbox{red!1}{\strut Development} \colorbox{red!1}{\strut Events} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Exhibitions} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut Barn} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut Involved} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Contact} \colorbox{red!1}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Indiana} \colorbox{red!8}{\strut State} \colorbox{red!9}{\strut Fair} 
}}}
\end{CJK*}

query: fybromyalgia

90:fibromyalgia, 86:fybromyalgia, 36:symptoms, 26:disorder, 25:pain, 25:fibrous, 25:fibro, 19:disease, 19:affective, 18:tissue


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Fibromyalgia} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!8}{\strut Fybromyalgia} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!8}{\strut Fibromyalgia} \colorbox{red!0}{\strut Classification} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut external} \colorbox{red!0}{\strut resources} \colorbox{red!2}{\strut ICD} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut 79.7} \colorbox{red!2}{\strut ICD} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut 729.1} \colorbox{red!0}{\strut MedlinePlus} \colorbox{red!0}{\strut 000427} \colorbox{red!0}{\strut eMedicine} \colorbox{red!0}{\strut med790} \colorbox{red!0}{\strut med2934} \colorbox{red!0}{\strut ped777} \colorbox{red!0}{\strut pmr47} \colorbox{red!0}{\strut MeSH} \colorbox{red!0}{\strut D005356} \colorbox{red!8}{\strut Fibromyalgia} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut new} \colorbox{red!0}{\strut lat.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fibro-} \colorbox{red!2}{\strut fibrous} \colorbox{red!2}{\strut tissue} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Gk} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut myo-} \colorbox{red!2}{\strut muscle} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Gk} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut algos-} \colorbox{red!2}{\strut pain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut meaning} \colorbox{red!2}{\strut muscle} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut connective} \colorbox{red!2}{\strut tissue} \colorbox{red!2}{\strut pain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut referred} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut FM} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut FMS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut disorder} \colorbox{red!1}{\strut classified} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut presence} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut chronic} \colorbox{red!0}{\strut widespread} \colorbox{red!2}{\strut pain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut heightened} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut painful} \colorbox{red!1}{\strut response} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut gentle} \colorbox{red!0}{\strut touch} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut tactile} \colorbox{red!1}{\strut allodynia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut core} \colorbox{red!1}{\strut features} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut disorder} \colorbox{red!0}{\strut include} \colorbox{red!1}{\strut debilitating} \colorbox{red!1}{\strut fatigue} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut sleep} \colorbox{red!1}{\strut disturbance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut joint} \colorbox{red!1}{\strut stiffness} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut persons} \colorbox{red!1}{\strut affected} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut disorder} \colorbox{red!0}{\strut frequently} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut other} \colorbox{red!3}{\strut symptoms} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut involve} \colorbox{red!0}{\strut multiple} \colorbox{red!1}{\strut body} \colorbox{red!1}{\strut systems} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut difficulty} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut swallowing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut functional} \colorbox{red!1}{\strut bowel} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut bladder} \colorbox{red!1}{\strut abnormalities} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut difficulty} \colorbox{red!1}{\strut breathing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut diffuse} \colorbox{red!1}{\strut sensations} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut numbness} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut tingling} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut non-dermatomal} \colorbox{red!0}{\strut paresthesia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut abnormal} \colorbox{red!1}{\strut motor} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut i.e} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut nocturnal} \colorbox{red!1}{\strut myoclonus} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut sleep} \colorbox{red!0}{\strut bruxism} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut cognitive} \colorbox{red!1}{\strut dysfunction} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut increased} \colorbox{red!1}{\strut prevalence} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut affective} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut anxiety-related} \colorbox{red!3}{\strut symptoms} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut While} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut criteria} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut entity} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut yet} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut thoroughly} \colorbox{red!0}{\strut developed} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut recognition} \colorbox{red!0}{\strut that} \colorbox{red!8}{\strut fibromyalgia} \colorbox{red!1}{\strut involves} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut just} \colorbox{red!2}{\strut pain} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut led} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut frequent} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut term} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut fibromyalgia} \colorbox{red!1}{\strut syndrome} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Not} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut affected} \colorbox{red!0}{\strut persons} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut symptoms} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut greater} \colorbox{red!1}{\strut syndrome} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Fibromyalgia} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut considered} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut controversial} \colorbox{red!1}{\strut diagnosis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut authors} \colorbox{red!0}{\strut contending} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut disorder} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut non-disease} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lack} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut objective} \colorbox{red!0}{\strut laboratory} 
}}}
\end{CJK*}

75:rsds, 75:rsd, 54:what, 28:pain, 24:mental, 24:illness, 24:advisory, 23:syndrome, 23:diseases, 22:disorders


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut RSD} \colorbox{red!0}{\strut Advisory-} \colorbox{red!1}{\strut Where} \colorbox{red!1}{\strut Chronic} \colorbox{red!2}{\strut Pain} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Mental} \colorbox{red!1}{\strut Illness} \colorbox{red!1}{\strut Collide} \colorbox{red!0}{\strut October} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2006} \colorbox{red!1}{\strut Promoting} \colorbox{red!0}{\strut Awareness-} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut thoughts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut storieswelcome} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Filed} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 360.yahoo.comelllajC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Blogroll} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Blogs} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Blogging} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut CRPS} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Chronic} \colorbox{red!2}{\strut Pain} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Complex} \colorbox{red!1}{\strut Regional} \colorbox{red!2}{\strut Pain} \colorbox{red!1}{\strut Syndrome} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Depression} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Fybromyalgia} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Incurable} \colorbox{red!1}{\strut Diseases} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Mental} \colorbox{red!1}{\strut Illness} \colorbox{red!1}{\strut Advocacy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut MySpace} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut NINDS} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Neurological} \colorbox{red!1}{\strut Disorder} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Pain} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Pain} \colorbox{red!1}{\strut Syndrome} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut Essays} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut RSD} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut RSDS} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Rare} \colorbox{red!1}{\strut Disorders} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Reflex} \colorbox{red!1}{\strut Sympathetic} \colorbox{red!1}{\strut Dystrophy} \colorbox{red!1}{\strut Syndrome} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut Publications} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut authors} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut what} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut www.RSDAdvisor.com} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut www.RSDAdvisory.com} \colorbox{red!0}{\strut twinklev} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 456} \colorbox{red!0}{\strut pm} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut effort} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut promote} \colorbox{red!1}{\strut awareness} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut regarding} \colorbox{red!1}{\strut Reflex} \colorbox{red!1}{\strut Sympathetic} \colorbox{red!1}{\strut Dystrophy} \colorbox{red!0}{\strut SyndromeComplex} \colorbox{red!1}{\strut Regional} \colorbox{red!2}{\strut Pain} \colorbox{red!1}{\strut Syndrome} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut aka} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut RSD} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut RSDS} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut CRPS} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut sites} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut understanding} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut RSD} \colorbox{red!1}{\strut Advisory} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut RSD} \colorbox{red!1}{\strut Advisor} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut mirror} \colorbox{red!0}{\strut dot.com} \colorbox{red!0}{\strut sites} \colorbox{red!0}{\strut www.RSDAdvisor.com} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut www.RSDAdvisory.com} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut at} \colorbox{red!4}{\strut RSD} \colorbox{red!0}{\strut Advisory-WordPress} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut leave} \colorbox{red!1}{\strut comments} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut stories} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tell} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Just} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut comment} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut post} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut blogs} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut fits} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thank} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut supporting} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut passion} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut promote} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut date} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut still} \colorbox{red!0}{\strut no} \colorbox{red!1}{\strut cure} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Best} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut wishes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut twinkleellaj} \colorbox{red!1}{\strut Comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut October} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Universal} \colorbox{red!0}{\strut Disorder-} \colorbox{red!0}{\strut Part} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut conclusion} \colorbox{red!1}{\strut Filed} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 360.yahoo.comelllajC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Answers} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Bipolar} \colorbox{red!1}{\strut Disorder} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Blogroll} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut CRPS} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Chronic} \colorbox{red!2}{\strut Pain} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Complex} \colorbox{red!1}{\strut Regional} \colorbox{red!2}{\strut Pain} \colorbox{red!1}{\strut Syndrome} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Depression} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Fybromyalgia} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Incurable} \colorbox{red!1}{\strut Diseases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mania} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Mental} \colorbox{red!1}{\strut Illness} \colorbox{red!1}{\strut Advocacy} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut NINDS} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Neurological} \colorbox{red!1}{\strut Disorder} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Pain} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Pain} \colorbox{red!1}{\strut Syndrome} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut RSD} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut RSDS} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Rare} \colorbox{red!1}{\strut Disorders} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Reflex} \colorbox{red!1}{\strut Sympathetic} \colorbox{red!1}{\strut Dystrophy} \colorbox{red!1}{\strut Syndrome} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Salacious} \colorbox{red!0}{\strut Surrender} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut what} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut www.RSDAdvisor.com} 
}}}
\end{CJK*}

query: gmat prep classes

101:gmat, 64:prep, 60:cost, 44:class, 41:classes, 34:courses, 34:course, 25:tests, 24:hours, 22:classroom


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Order} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut FAQ} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Home} \colorbox{red!1}{\strut Order} \colorbox{red!5}{\strut GMAT} \colorbox{red!3}{\strut Prep} \colorbox{red!1}{\strut Order} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 800score.com} \colorbox{red!3}{\strut Prep} \colorbox{red!2}{\strut Course} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut 5} \colorbox{red!5}{\strut GMAT} \colorbox{red!1}{\strut exams} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut GMAT} \colorbox{red!0}{\strut Sections} \colorbox{red!0}{\strut Download} \colorbox{red!0}{\strut 5} \colorbox{red!5}{\strut GMAT} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Essay} \colorbox{red!0}{\strut Section} \colorbox{red!0}{\strut Guide} \colorbox{red!1}{\strut Math} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Verbal} \colorbox{red!0}{\strut Guide} \colorbox{red!5}{\strut GMAT} \colorbox{red!0}{\strut Resources} \colorbox{red!0}{\strut Intro} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut GMAT} \colorbox{red!0}{\strut 24} \colorbox{red!1}{\strut Hour} \colorbox{red!0}{\strut Tutor} \colorbox{red!0}{\strut Support} \colorbox{red!0}{\strut Free} \colorbox{red!1}{\strut Practice} \colorbox{red!0}{\strut Essays} \colorbox{red!0}{\strut Free} \colorbox{red!5}{\strut GMAT} \colorbox{red!0}{\strut Download} \colorbox{red!1}{\strut Test} \colorbox{red!1}{\strut Pacer} \colorbox{red!1}{\strut Training} \colorbox{red!5}{\strut GMAT} \colorbox{red!1}{\strut Online} \colorbox{red!3}{\strut Prep} \colorbox{red!2}{\strut Course} \colorbox{red!5}{\strut GMAT} \colorbox{red!1}{\strut Classroom} \colorbox{red!2}{\strut Course} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut GMAT} \colorbox{red!2}{\strut Class} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut 800score} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut value-priced} \colorbox{red!1}{\strut online} \colorbox{red!2}{\strut course} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut 500} \colorbox{red!1}{\strut pages} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 5} \colorbox{red!5}{\strut GMAT} \colorbox{red!1}{\strut CAT} \colorbox{red!1}{\strut tests} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 39.95} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut students} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut cost-no-object} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut approach} \colorbox{red!0}{\strut to} \colorbox{red!5}{\strut GMAT} \colorbox{red!3}{\strut prep} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut prefer} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut classroom} \colorbox{red!0}{\strut environment} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut these} \colorbox{red!5}{\strut GMAT} \colorbox{red!1}{\strut classroom} \colorbox{red!3}{\strut prep} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Veritas} \colorbox{red!3}{\strut Prep} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut recently} \colorbox{red!0}{\strut profiled} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut BusinessWeek} \colorbox{red!0}{\strut magazine} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut rapidly} \colorbox{red!0}{\strut growing} \colorbox{red!5}{\strut GMAT} \colorbox{red!3}{\strut prep} \colorbox{red!0}{\strut company} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 5,000} \colorbox{red!5}{\strut GMAT} \colorbox{red!1}{\strut students} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 65} \colorbox{red!0}{\strut locations} \colorbox{red!0}{\strut worldwide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Their} \colorbox{red!0}{\strut admissions} \colorbox{red!0}{\strut consultant} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut former} \colorbox{red!0}{\strut admissions} \colorbox{red!0}{\strut officers} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut schools} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut 2000} \colorbox{red!1}{\strut pages} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut materials} \colorbox{red!0}{\strut 15} \colorbox{red!1}{\strut practice} \colorbox{red!1}{\strut tests} \colorbox{red!0}{\strut 42} \colorbox{red!1}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut class} \colorbox{red!0}{\strut instruction} \colorbox{red!0}{\strut Unlimited} \colorbox{red!0}{\strut instructor} \colorbox{red!0}{\strut phone} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut tutoring} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut Instructors} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut scored} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 99th} \colorbox{red!0}{\strut percentile} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 760} \colorbox{red!5}{\strut GMAT} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Classroom} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Weekend} \colorbox{red!0}{\strut Focus} \colorbox{red!2}{\strut course} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 700} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 42-hour} \colorbox{red!2}{\strut course} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1400} \colorbox{red!1}{\strut Online} \colorbox{red!2}{\strut courses} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 750} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1100} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut live} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Continue} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Veritas} \colorbox{red!3}{\strut Prep} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut GMAT} \colorbox{red!2}{\strut Classes} \colorbox{red!0}{\strut ManhattanGMAT} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut cities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut LA} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Chicago} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut DC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Boston} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Austin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Philladelphia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut reputation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut clients} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Goldman} \colorbox{red!0}{\strut Sachs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut JP} \colorbox{red!0}{\strut Morgan} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut 1500} \colorbox{red!1}{\strut pages} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut materials} \colorbox{red!0}{\strut 6} \colorbox{red!1}{\strut practice} \colorbox{red!5}{\strut GMAT} \colorbox{red!1}{\strut CAT} \colorbox{red!1}{\strut tests} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut full} \colorbox{red!1}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut class} \colorbox{red!0}{\strut instruction} \colorbox{red!0}{\strut Instructors} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut scored} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 99th} \colorbox{red!0}{\strut percentile} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 760} \colorbox{red!5}{\strut GMAT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Location} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 138} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut 25th} \colorbox{red!0}{\strut Street} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 9th} \colorbox{red!0}{\strut floor} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut NY} \colorbox{red!0}{\strut Continue} \colorbox{red!0}{\strut to} 
}}}
\end{CJK*}

98:prep, 97:preparatory, 97:gmat, 87:classes, 85:class, 26:test, 21:program, 19:programs, 16:preparation, 15:exam


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Academic} \colorbox{red!1}{\strut Credit} \colorbox{red!1}{\strut Academic} \colorbox{red!1}{\strut Noncredit} \colorbox{red!1}{\strut Distance} \colorbox{red!1}{\strut Education} \colorbox{red!1}{\strut English} \colorbox{red!0}{\strut Language} \colorbox{red!0}{\strut Lifelong} \colorbox{red!1}{\strut Learning} \colorbox{red!0}{\strut Osher} \colorbox{red!0}{\strut Institute} \colorbox{red!0}{\strut Professional} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut Technology} \colorbox{red!1}{\strut Education} \colorbox{red!2}{\strut Test} \colorbox{red!1}{\strut Preparation} \colorbox{red!0}{\strut Youth} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut Programs} \colorbox{red!1}{\strut Locations} \colorbox{red!7}{\strut GMAT} \colorbox{red!7}{\strut Preparatory} \colorbox{red!6}{\strut Class} \colorbox{red!0}{\strut Our} \colorbox{red!7}{\strut preparatory} \colorbox{red!2}{\strut program} \colorbox{red!1}{\strut offers} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut class} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut GMAT} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut improve} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut chances} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut gaining} \colorbox{red!1}{\strut admission} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut graduate} \colorbox{red!1}{\strut schools} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut comprehensive} \colorbox{red!6}{\strut class} \colorbox{red!0}{\strut covers} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut exam} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut strategies} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut suggestions} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut improve} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lets} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut practice} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut analytical} \colorbox{red!1}{\strut writing} \colorbox{red!1}{\strut assessment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut practice} \colorbox{red!1}{\strut exams} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Once} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut paid} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut preparatory} \colorbox{red!6}{\strut class} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut 3} \colorbox{red!1}{\strut years} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut retake} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut class} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut charge} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut extra} \colorbox{red!0}{\strut material} \colorbox{red!1}{\strut costs} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut included} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut upon} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut space} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut dates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut registration} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut for} \colorbox{red!7}{\strut classes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut view} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut syllabus} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Cart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut All} \colorbox{red!7}{\strut Prep} \colorbox{red!7}{\strut Classes} \colorbox{red!7}{\strut GMAT} \colorbox{red!1}{\strut GRE} \colorbox{red!1}{\strut LSAT} \colorbox{red!0}{\strut Meet} \colorbox{red!0}{\strut Our} \colorbox{red!1}{\strut Instructors} \colorbox{red!0}{\strut Frequently} \colorbox{red!0}{\strut Asked} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut about} \colorbox{red!7}{\strut Prep} \colorbox{red!7}{\strut Classes} \colorbox{red!0}{\strut Already} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut Test} \colorbox{red!7}{\strut Prep} \colorbox{red!1}{\strut student} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut WebCT} \colorbox{red!2}{\strut Test} \colorbox{red!7}{\strut Prep} \colorbox{red!0}{\strut home} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut Continuing} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Utah} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut reserved} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1901} \colorbox{red!0}{\strut E.} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Campus} \colorbox{red!0}{\strut Dr.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1215} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Salt} \colorbox{red!0}{\strut Lake} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut UT} \colorbox{red!0}{\strut 84112-9359} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 801-581-5361} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut fax} \colorbox{red!0}{\strut 801-585-5414} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Comments} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Disclaimer} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: djs

103:djs, 103:dj, 66:how, 53:what, 27:find, 27:disc, 23:where, 15:look, 15:hired, 14:jockey


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 1-800-DJS-ARE-US} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Supply} \colorbox{red!0}{\strut Store-} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut America} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Disc} \colorbox{red!0}{\strut Jockey} \colorbox{red!0}{\strut Resource} \colorbox{red!0}{\strut 1800djsareus.com} \colorbox{red!0}{\strut Looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut find} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut near} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut State} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut event} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut info} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Renew} \colorbox{red!0}{\strut Monthly} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut Listing} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut past} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut Renew} \colorbox{red!0}{\strut Annual} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut Listing} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut past} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut Cancel} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut Listing} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut current} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Never} \colorbox{red!0}{\strut hired} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut disc} \colorbox{red!0}{\strut jockey} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!1}{\strut what} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 1999-2008} \colorbox{red!2}{\strut DJ} \colorbox{red!0}{\strut S} \colorbox{red!0}{\strut ARE} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut agree} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut terms} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut advertise} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut request} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut webmaster} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Clipart} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.ace-clipart.com} \colorbox{red!0}{\strut Alabama} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Alaska} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Arizona} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Arkansas} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut California} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Colorado} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Connecticut} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Delaware} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Florida} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Georgia} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Hawaii} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Idaho} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Illinois} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Indiana} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Iowa} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Kansas} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Kentucky} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Maine} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Maryland} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Massachusetts} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Michigan} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Minnesota} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Mississippi} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Missouri} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Montana} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Nebraska} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Nevada} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Hampshire} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Jersey} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Mexico} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Carolina} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Dakota} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Ohio} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Oklahoma} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Oregon} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Pennsylvania} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Rhode} \colorbox{red!0}{\strut Island} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Carolina} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Dakota} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Tennessee} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Texas} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Utah} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Vermont} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Virginia} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Washington} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut Virginia} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Wisconsin} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Wyoming} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Los} \colorbox{red!0}{\strut Angeles} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Chicago} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Houston} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Arkansas} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Philadelphia} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Phoenix} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Diego} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Antonio} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Dallas} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Detroit} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut Hawaii} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Jose} 
}}}
\end{CJK*}

104:djs, 103:dj, 95:miami, 34:florida, 21:party, 19:parties, 12:disc, 8:when, 7:weddings, 7:south


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Miami} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Planners} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Weddings} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Mobile} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Professional} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut miami} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Planners} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Weddings} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Mobile} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Professional} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut miami} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Planners} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Weddings} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Mobile} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Professional} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut miami} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Planners} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Weddings} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Mobile} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Professional} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut miami} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Planners} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Weddings} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Mobile} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Professional} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut miami} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Planners} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Florida} \colorbox{red!0}{\strut Disc} \colorbox{red!0}{\strut Jockeys} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Weddings} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Mobile} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Professional} \colorbox{red!2}{\strut DJs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Miami} \colorbox{red!0}{\strut Party} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut miami} \colorbox{red!2}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

query: arizona game fish

96:fishing, 95:fish, 76:arizona, 42:number, 39:licenses, 38:license, 29:state, 21:hunting, 18:records, 14:trout


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut FinTalk} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Fish} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Game} \colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!0}{\strut Information} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut fishing} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut many} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut fishing} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut web} \colorbox{red!0}{\strut sites} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut fishing} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fish} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Game} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut heading} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut fishing} \colorbox{red!0}{\strut trip} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut reserviors} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut lakes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut fishing} \colorbox{red!1}{\strut licenses} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut hunting} \colorbox{red!1}{\strut licenses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut fishing} \colorbox{red!1}{\strut records} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut ARIZONA} \colorbox{red!3}{\strut Fish} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Game} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut 2222} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut Greenway} \colorbox{red!0}{\strut Road} \colorbox{red!0}{\strut Phoenix} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AZ} \colorbox{red!0}{\strut 85023-4312} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 602} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 942-3000} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.gf.state.az.us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut image} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut map} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fish} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Game} \colorbox{red!3}{\strut Arizona} \colorbox{red!0}{\strut Online} \colorbox{red!1}{\strut Licenses} \colorbox{red!3}{\strut Arizona} \colorbox{red!0}{\strut Public} \colorbox{red!1}{\strut Records} \colorbox{red!0}{\strut Federal} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut State} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Conservation} \colorbox{red!0}{\strut Resources} \colorbox{red!3}{\strut Arizona} \colorbox{red!0}{\strut Conservation} \colorbox{red!0}{\strut Resources} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Fish} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Wildlife} \colorbox{red!0}{\strut Agencies} \colorbox{red!0}{\strut Trout} \colorbox{red!0}{\strut Unlimited} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Arizona} \colorbox{red!1}{\strut State} \colorbox{red!0}{\strut Chapter} \colorbox{red!3}{\strut Arizona} \colorbox{red!0}{\strut Marine} \colorbox{red!0}{\strut Conservation} \colorbox{red!0}{\strut Directory} \colorbox{red!0}{\strut Wildlife} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Tomorrow} \colorbox{red!0}{\strut Government} \colorbox{red!0}{\strut Resources} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Arizona} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Federal} \colorbox{red!0}{\strut Recreation} \colorbox{red!0}{\strut --} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!0}{\strut Areas} \colorbox{red!3}{\strut Arizona} \colorbox{red!0}{\strut Farm} \colorbox{red!0}{\strut Service} \colorbox{red!0}{\strut Agency} \colorbox{red!0}{\strut Invasive} \colorbox{red!0}{\strut Species} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!1}{\strut Records} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!1}{\strut Records} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!0}{\strut Regulations} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!0}{\strut Report} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Add} \colorbox{red!0}{\strut An} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!0}{\strut Report} \colorbox{red!0}{\strut Talk} \colorbox{red!0}{\strut about} \colorbox{red!3}{\strut Arizona} \colorbox{red!3}{\strut Fishing} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Forum} \colorbox{red!3}{\strut Fishing} \colorbox{red!1}{\strut License} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut Buy} \colorbox{red!3}{\strut Fishing} \colorbox{red!1}{\strut Licenses} \colorbox{red!0}{\strut Online} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut fee} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut charged} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut temporary} \colorbox{red!1}{\strut license} \colorbox{red!1}{\strut number} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut recognized} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut law} \colorbox{red!0}{\strut enforcement} \colorbox{red!0}{\strut officers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut field} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut permanent} \colorbox{red!1}{\strut license} \colorbox{red!0}{\strut arrives} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut mail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut blank} \colorbox{red!1}{\strut license} \colorbox{red!0}{\strut forms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fill} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mail-in} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut regarding} \colorbox{red!1}{\strut licenses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut call} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Arizona} \colorbox{red!0}{\strut Game} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Fish} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 602} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 942-3000} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Hunting} \colorbox{red!1}{\strut License} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut Buy} \colorbox{red!1}{\strut Hunting} \colorbox{red!1}{\strut Licenses} \colorbox{red!0}{\strut Online} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut fee} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut charged} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut service} 
}}}
\end{CJK*}

78:arizona, 77:arizonas, 68:fish, 56:game, 36:conserve, 31:wildlife, 27:fishing, 27:department, 24:ohv, 23:conservation


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut RSS} \colorbox{red!0}{\strut Feed} \colorbox{red!0}{\strut Subscribe} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut BUY} \colorbox{red!1}{\strut LICENSES} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut BIG} \colorbox{red!5}{\strut GAME} \colorbox{red!1}{\strut DRAW} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eNEWS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CALENDAR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut VIDEO} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut HUNTING} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut FISHING} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut WILDLIFE} \colorbox{red!0}{\strut VIEWING} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut CONSERVATION} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut EDUCATION} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut BOATING} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SHOOTING} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut OHV} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SITE} \colorbox{red!0}{\strut MAP} \colorbox{red!0}{\strut About} \colorbox{red!1}{\strut The} \colorbox{red!7}{\strut Arizona} \colorbox{red!5}{\strut Game} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Fish} \colorbox{red!2}{\strut Department} \colorbox{red!1}{\strut Mission} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut To} \colorbox{red!3}{\strut conserve} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut enhance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut restore} \colorbox{red!0}{\strut Arizonas} \colorbox{red!1}{\strut diverse} \colorbox{red!3}{\strut wildlife} \colorbox{red!1}{\strut resources} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut habitats} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut aggressive} \colorbox{red!1}{\strut protection} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut management} \colorbox{red!1}{\strut programs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut provide} \colorbox{red!3}{\strut wildlife} \colorbox{red!1}{\strut resources} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut safe} \colorbox{red!1}{\strut watercraft} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut off-highway} \colorbox{red!1}{\strut vehicle} \colorbox{red!1}{\strut recreation} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut enjoyment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut appreciation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut present} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut future} \colorbox{red!0}{\strut generations.View} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut agency} \colorbox{red!0}{\strut directory} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut commission} \colorbox{red!1}{\strut meeting} \colorbox{red!0}{\strut minutes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut strategic} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut annual} \colorbox{red!0}{\strut report} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut opportunity} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut join} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut team} \colorbox{red!0}{\strut within} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut employment} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Recent} \colorbox{red!0}{\strut Entries} \colorbox{red!1}{\strut Archery} \colorbox{red!0}{\strut 3-D} \colorbox{red!0}{\strut fun} \colorbox{red!0}{\strut shoot} \colorbox{red!1}{\strut open} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Outdoor} \colorbox{red!1}{\strut Expo} \colorbox{red!0}{\strut slated} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut late} \colorbox{red!0}{\strut March} \colorbox{red!7}{\strut Arizona} \colorbox{red!3}{\strut Wildlife} \colorbox{red!1}{\strut Views} \colorbox{red!1}{\strut television} \colorbox{red!1}{\strut series} \colorbox{red!1}{\strut begins} \colorbox{red!1}{\strut new} \colorbox{red!1}{\strut season} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut PBS} \colorbox{red!1}{\strut Give} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut magazine} \colorbox{red!0}{\strut gift} \colorbox{red!0}{\strut subscription} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut free} \colorbox{red!3}{\strut wildlife} \colorbox{red!0}{\strut calendar} \colorbox{red!1}{\strut Annual} \colorbox{red!1}{\strut Bald} \colorbox{red!1}{\strut Eagle} \colorbox{red!0}{\strut Workshop} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Flagstaff} \colorbox{red!1}{\strut Yuma} \colorbox{red!1}{\strut open} \colorbox{red!0}{\strut house} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut provide} \colorbox{red!0}{\strut details} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut Lower} \colorbox{red!2}{\strut Colorado} \colorbox{red!1}{\strut River} \colorbox{red!0}{\strut Multi-Species} \colorbox{red!2}{\strut Conservation} \colorbox{red!1}{\strut Program} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut backwater} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut selection} \colorbox{red!0}{\strut Reminder} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Hunting} \colorbox{red!1}{\strut seasons} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut carry} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut January} \colorbox{red!1}{\strut require} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 2009} \colorbox{red!2}{\strut hunting} \colorbox{red!1}{\strut license} \colorbox{red!0}{\strut Honor} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut fellow} \colorbox{red!1}{\strut conservationists} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut Commission} \colorbox{red!1}{\strut Awards} \colorbox{red!0}{\strut Banquet} \colorbox{red!1}{\strut Meet} \colorbox{red!1}{\strut the} \colorbox{red!7}{\strut Arizona} \colorbox{red!5}{\strut Game} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Fish} \colorbox{red!2}{\strut Commission} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut January} \colorbox{red!1}{\strut meeting} \colorbox{red!1}{\strut New} \colorbox{red!2}{\strut state} \colorbox{red!2}{\strut OHV} \colorbox{red!1}{\strut laws} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut into} \colorbox{red!1}{\strut effect} \colorbox{red!0}{\strut Jan.} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut 2009-10} \colorbox{red!2}{\strut Fishing} \colorbox{red!0}{\strut Regulations} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut Should} \colorbox{red!1}{\strut make} \colorbox{red!0}{\strut superb} \colorbox{red!1}{\strut seasonal} \colorbox{red!1}{\strut stocking} \colorbox{red!0}{\strut stuffers} \colorbox{red!0}{\strut Off-highway} \colorbox{red!1}{\strut vehicle} \colorbox{red!0}{\strut decal} \colorbox{red!1}{\strut price} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut Last-minute} \colorbox{red!0}{\strut gift} \colorbox{red!0}{\strut ideas} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut Game} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Fish} \colorbox{red!1}{\strut Archery} \colorbox{red!0}{\strut leagues} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut New} \colorbox{red!0}{\strut Year} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Ben} \colorbox{red!0}{\strut Avery} \colorbox{red!1}{\strut Shooting} \colorbox{red!1}{\strut Facility} \colorbox{red!0}{\strut Brackets} \colorbox{red!0}{\strut offered} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut men} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut women} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut children} \colorbox{red!2}{\strut Commission} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut hold} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut 09} \colorbox{red!1}{\strut meetings} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Phoenix} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut save} \colorbox{red!1}{\strut costs} \colorbox{red!0}{\strut Two} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut California} \colorbox{red!0}{\strut condor} \colorbox{red!0}{\strut chicks} \colorbox{red!0}{\strut flying} \colorbox{red!1}{\strut free} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Grand} \colorbox{red!0}{\strut Canyon} 
}}}
\end{CJK*}

query: wedding budget calculator

96:wedding, 81:budget, 60:costs, 23:tags, 23:planning, 22:invitations, 21:tagged, 21:calculator, 20:item, 19:cakes


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Popular} \colorbox{red!4}{\strut Wedding} \colorbox{red!1}{\strut Tags} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Wedding} \colorbox{red!1}{\strut Dresses} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Wedding} \colorbox{red!1}{\strut Cakes} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Wedding} \colorbox{red!1}{\strut Rings} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Wedding} \colorbox{red!1}{\strut Invitations} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Give} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Feedback} \colorbox{red!4}{\strut Wedding} \colorbox{red!1}{\strut Planning} \colorbox{red!0}{\strut Tips} \colorbox{red!1}{\strut Planning} \colorbox{red!0}{\strut Tips} \colorbox{red!0}{\strut Photographs} \colorbox{red!0}{\strut Bridal} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Perfect} \colorbox{red!1}{\strut Planner} \colorbox{red!0}{\strut Tools} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Check} \colorbox{red!1}{\strut Lists} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Guest} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Seating} \colorbox{red!0}{\strut Chart} \colorbox{red!0}{\strut My} \colorbox{red!4}{\strut Budget} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Calendar} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Tags} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Website} \colorbox{red!0}{\strut Local} \colorbox{red!4}{\strut Wedding} \colorbox{red!0}{\strut Professionals} \colorbox{red!0}{\strut Giveaways} \colorbox{red!4}{\strut Wedding} \colorbox{red!0}{\strut Favors} \colorbox{red!0}{\strut Bridal} \colorbox{red!0}{\strut Shows} \colorbox{red!4}{\strut Wedding} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Calculator} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut Local} \colorbox{red!0}{\strut Vendors} \colorbox{red!0}{\strut Local} \colorbox{red!4}{\strut Wedding} \colorbox{red!0}{\strut Vendors} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Perfect} \colorbox{red!1}{\strut Planner} \colorbox{red!0}{\strut Tools} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Checklists} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Guest} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Bridal} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Seating} \colorbox{red!0}{\strut Chart} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Tagged} \colorbox{red!1}{\strut Items} \colorbox{red!0}{\strut My} \colorbox{red!4}{\strut Budget} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Calendar} \colorbox{red!4}{\strut Wedding} \colorbox{red!0}{\strut Website} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Calculator} \colorbox{red!1}{\strut Planning} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut budget} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut sticking} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut difficult} \colorbox{red!0}{\strut task} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Using} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Calculator} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut budget} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut actual} \colorbox{red!3}{\strut costs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Rings} \colorbox{red!1}{\strut Item} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Actual} \colorbox{red!1}{\strut Brides} \colorbox{red!1}{\strut Band} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Grooms} \colorbox{red!1}{\strut Band} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Subtotals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 500.00} \colorbox{red!0}{\strut 0} \colorbox{red!1}{\strut Ceremony} \colorbox{red!1}{\strut Item} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Actual} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Rental} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Officiate} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Fee} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Marriage} \colorbox{red!0}{\strut License} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Subtotals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 875.00} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Bridal} \colorbox{red!1}{\strut Attire} \colorbox{red!1}{\strut Item} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Actual} \colorbox{red!0}{\strut Gown} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Veil} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Alterations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Shoes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stockings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lingerie} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Garter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jewelery} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Gown} \colorbox{red!0}{\strut Preservation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Subtotals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,550.00} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Reception} \colorbox{red!1}{\strut Item} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Actual} \colorbox{red!0}{\strut Reception} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Rental} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Food} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Beverage} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Dance} \colorbox{red!0}{\strut Lessons} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Subtotals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6,824.00} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Photography} \colorbox{red!1}{\strut Item} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Actual} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Wedding} \colorbox{red!0}{\strut Portrait} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Wedding} \colorbox{red!0}{\strut Photographs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Wedding} \colorbox{red!0}{\strut Album} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Subtotals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800.00} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Music} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Entertainment} \colorbox{red!1}{\strut Item} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Actual} \colorbox{red!1}{\strut Band} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Ceremony} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DJ} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Ceremony} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Band} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Reception} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DJ} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Reception} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Subtotals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 700.00} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Videography} \colorbox{red!1}{\strut Item} \colorbox{red!4}{\strut Budget} \colorbox{red!1}{\strut Actual} \colorbox{red!0}{\strut Videotaping} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Editing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Subtotals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut 0} 
}}}
\end{CJK*}

80:budget, 76:weddings, 72:wedding, 70:how, 49:elegant, 42:spend, 32:sarasota, 27:calculator, 26:spent, 23:amount


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!10}{\strut Budget} \colorbox{red!3}{\strut Calculator} \colorbox{red!1}{\strut Use} \colorbox{red!0}{\strut our} \colorbox{red!10}{\strut Budget} \colorbox{red!3}{\strut Calculator} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut determine} \colorbox{red!9}{\strut how} \colorbox{red!1}{\strut much} \colorbox{red!0}{\strut to} \colorbox{red!5}{\strut spend} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut where} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut ll} \colorbox{red!1}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut plan} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut start} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut finish} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut get} \colorbox{red!1}{\strut started} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut estimate} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut total} \colorbox{red!10}{\strut budget} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut guests} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut attendants} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut required} \colorbox{red!1}{\strut fields} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut right} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut TOTAL} \colorbox{red!10}{\strut BUDGET} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0.00} \colorbox{red!3}{\strut SPENT} \colorbox{red!0}{\strut TO} \colorbox{red!0}{\strut DATE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0.00} \colorbox{red!3}{\strut AMOUNT} \colorbox{red!1}{\strut LEFT} \colorbox{red!0}{\strut TO} \colorbox{red!5}{\strut SPEND} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0.00} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut required} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut My} \colorbox{red!10}{\strut Budget} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Guests} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Female} \colorbox{red!2}{\strut Attendants} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Male} \colorbox{red!2}{\strut Attendants} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Mission} \colorbox{red!0}{\strut Statement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Become} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Member} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Link} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut 2009} \colorbox{red!6}{\strut Elegant} \colorbox{red!4}{\strut Sarasota} \colorbox{red!9}{\strut Weddings} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Rights} \colorbox{red!0}{\strut Reserved} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut LOG} \colorbox{red!0}{\strut IN} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut JOIN} \colorbox{red!0}{\strut FREE} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut SEARCH} \colorbox{red!0}{\strut OUR} \colorbox{red!0}{\strut SITE} \colorbox{red!1}{\strut Accommodations} \colorbox{red!1}{\strut Bakers} \colorbox{red!1}{\strut Bridal} \colorbox{red!1}{\strut Wear} \colorbox{red!1}{\strut Butterfly} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Dove} \colorbox{red!0}{\strut Release} \colorbox{red!1}{\strut Catering} \colorbox{red!0}{\strut DJs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Entertainment} \colorbox{red!1}{\strut Florists} \colorbox{red!1}{\strut Formal} \colorbox{red!1}{\strut Wear} \colorbox{red!1}{\strut Invitations} \colorbox{red!1}{\strut Musicians} \colorbox{red!1}{\strut Officiants} \colorbox{red!0}{\strut Photographers} \colorbox{red!1}{\strut Reception} \colorbox{red!1}{\strut Locations} \colorbox{red!1}{\strut Receptions} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Waterfront} \colorbox{red!1}{\strut Rentals} \colorbox{red!1}{\strut Salon} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Spa} \colorbox{red!0}{\strut Transportation} \colorbox{red!0}{\strut Travel} \colorbox{red!0}{\strut Agencies} \colorbox{red!0}{\strut Videographers} \colorbox{red!9}{\strut Wedding} \colorbox{red!1}{\strut Planners} \colorbox{red!1}{\strut Yacht} \colorbox{red!1}{\strut Charter} \colorbox{red!1}{\strut Visit} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut sites} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!6}{\strut Elegant} \colorbox{red!9}{\strut Weddings} \colorbox{red!1}{\strut Network} \colorbox{red!1}{\strut Tampa} 
}}}
\end{CJK*}

query: rick warren

100:obama, 73:rick, 70:warren, 64:invocation, 60:inauguration, 56:green, 54:what, 42:who, 36:president, 25:barack


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Welcome} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Logout} \colorbox{red!0}{\strut Log} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Huffington} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Politics} \colorbox{red!0}{\strut Media} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut Living} \colorbox{red!0}{\strut Style} \colorbox{red!2}{\strut Green} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut Chicago} \colorbox{red!0}{\strut 236} \colorbox{red!0}{\strut Video} \colorbox{red!0}{\strut bignews} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Inauguration} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Slideshows} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut George} \colorbox{red!0}{\strut Bush} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Make} \colorbox{red!0}{\strut HuffPost} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut HomePage} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut HuffPost} \colorbox{red!0}{\strut Firefox} \colorbox{red!0}{\strut Toolbar} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Rev} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Inauguration} \colorbox{red!0}{\strut Byron} \colorbox{red!0}{\strut Williams} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Posted} \colorbox{red!0}{\strut 12.20.2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Politics} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Barack} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Inauguration} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut Saddleback} \colorbox{red!1}{\strut Church} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Barack} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Politics} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut piece} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut friend} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut colleague} \colorbox{red!0}{\strut Dr.} \colorbox{red!0}{\strut Sylvia} \colorbox{red!0}{\strut Rhue} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Director} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Religious} \colorbox{red!0}{\strut Affairs} \colorbox{red!0}{\strut National} \colorbox{red!0}{\strut Black} \colorbox{red!0}{\strut Justice} \colorbox{red!0}{\strut Coalition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut passi} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Days} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Green} \colorbox{red!0}{\strut Jobs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Caroline} \colorbox{red!0}{\strut Kennedy} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!1}{\strut Mark} \colorbox{red!2}{\strut Green} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Posted} \colorbox{red!0}{\strut 12.20.2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Politics} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Barack} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Air} \colorbox{red!0}{\strut America} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Mark} \colorbox{red!2}{\strut Green} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Green} \colorbox{red!0}{\strut Jobs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Inauguration} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Green} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Green} \colorbox{red!0}{\strut Energy} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut Saddleback} \colorbox{red!1}{\strut Church} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Barack} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Days} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut America} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Caroline} \colorbox{red!0}{\strut Kennedy} \colorbox{red!1}{\strut Senate} \colorbox{red!0}{\strut Seat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Caroline} \colorbox{red!0}{\strut Kennedy} \colorbox{red!1}{\strut Senate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Caroline} \colorbox{red!0}{\strut Kennedy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut Senate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hillary} \colorbox{red!0}{\strut Clinton} \colorbox{red!1}{\strut Senate} \colorbox{red!0}{\strut Seat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Politics} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Is} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut choice} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut president-elect} \colorbox{red!0}{\strut giving} \colorbox{red!0}{\strut conservatives} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut visual} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut giving} \colorbox{red!0}{\strut progressives} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut policy} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut Post} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut Was} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut Thinking} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut William} \colorbox{red!0}{\strut Fisher} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Posted} \colorbox{red!0}{\strut 12.20.2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Politics} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!2}{\strut Invocation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Inauguration} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Barack} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Barack} \colorbox{red!3}{\strut Obama} \colorbox{red!2}{\strut Rick} \colorbox{red!2}{\strut Warren} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Rick} 
}}}
\end{CJK*}

100:warrens, 100:warren, 96:rick, 84:invocation, 62:inauguration, 52:why, 44:obamas, 44:obama, 34:president, 31:inaugural


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Saturday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Nation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Money} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut Opinion} \colorbox{red!0}{\strut Science} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut Video} \colorbox{red!0}{\strut Rankings} \colorbox{red!0}{\strut Nation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut Article} \colorbox{red!0}{\strut Index} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Subscribe} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Nation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut God} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Country} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Why} \colorbox{red!6}{\strut Rick} \colorbox{red!0}{\strut Warrens} \colorbox{red!5}{\strut Invocation} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Obamas} \colorbox{red!4}{\strut Inauguration} \colorbox{red!1}{\strut Matters} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Focus} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Family} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Tricky} \colorbox{red!1}{\strut Invitation} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut President-Elect} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut Rick} \colorbox{red!6}{\strut Warren} \colorbox{red!1}{\strut Flap} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Can} \colorbox{red!3}{\strut Obama} \colorbox{red!1}{\strut Appeal} \colorbox{red!0}{\strut Both} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Gays} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Evangelicals} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Blog} \colorbox{red!0}{\strut Entry} \colorbox{red!1}{\strut Comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 145} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Why} \colorbox{red!6}{\strut Rick} \colorbox{red!0}{\strut Warrens} \colorbox{red!5}{\strut Invocation} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Obamas} \colorbox{red!4}{\strut Inauguration} \colorbox{red!1}{\strut Matters} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 17} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut 0544} \colorbox{red!0}{\strut PM} \colorbox{red!0}{\strut ET} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Dan} \colorbox{red!0}{\strut Gilgoff} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Permanent} \colorbox{red!0}{\strut Link} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Dan} \colorbox{red!0}{\strut Gilgoff} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut God} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Country} \colorbox{red!1}{\strut Evangelical} \colorbox{red!0}{\strut megachurch} \colorbox{red!1}{\strut pastor} \colorbox{red!6}{\strut Rick} \colorbox{red!6}{\strut Warren} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut author} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Purpose-Driven} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut deliver} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut invocation} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Barack} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut inauguration} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut month} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Joint} \colorbox{red!1}{\strut Congressional} \colorbox{red!0}{\strut Committee} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut Inaugural} \colorbox{red!1}{\strut Ceremonies} \colorbox{red!1}{\strut announced} \colorbox{red!0}{\strut today} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut selection} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Warren} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut whose} \colorbox{red!0}{\strut Saddleback} \colorbox{red!0}{\strut Church} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut California} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut candidate} \colorbox{red!0}{\strut forum} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Republican} \colorbox{red!1}{\strut presidential} \colorbox{red!0}{\strut nominee} \colorbox{red!1}{\strut John} \colorbox{red!0}{\strut McCain} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut early} \colorbox{red!0}{\strut taste} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Democrats} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut post-election} \colorbox{red!0}{\strut effort} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reach} \colorbox{red!1}{\strut evangelical} \colorbox{red!0}{\strut Americans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut effort} \colorbox{red!0}{\strut continues} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut though} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut evangelical} \colorbox{red!0}{\strut offensive} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut presidential} \colorbox{red!0}{\strut campaign} \colorbox{red!0}{\strut yielded} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut modest} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut Election} \colorbox{red!0}{\strut Day} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut White} \colorbox{red!1}{\strut evangelicals} \colorbox{red!0}{\strut supported} \colorbox{red!0}{\strut McCain} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Democratic} \colorbox{red!0}{\strut nominee} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut 73} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut represented} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 4-percentage-point} \colorbox{red!0}{\strut improvement} \colorbox{red!0}{\strut over} \colorbox{red!1}{\strut John} \colorbox{red!0}{\strut Kerry} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut showing} \colorbox{red!0}{\strut among} \colorbox{red!1}{\strut white} \colorbox{red!1}{\strut evangelicals} \colorbox{red!0}{\strut four} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Another} \colorbox{red!0}{\strut reason} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut mildly} \colorbox{red!0}{\strut surprised} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut Warren} \colorbox{red!0}{\strut pick} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut backers} \colorbox{red!0}{\strut felt} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut man} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut bamboozled} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut candidate} \colorbox{red!0}{\strut summit} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut both} \colorbox{red!1}{\strut candidates} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut supposed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut kept} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut dark} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut questions} \colorbox{red!6}{\strut Warren} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut asking} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut With} \colorbox{red!6}{\strut Warren} \colorbox{red!1}{\strut sitting} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut Obama} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut pastor} \colorbox{red!0}{\strut asserted} 
}}}
\end{CJK*}

query: yahoo

100:yahoo, 49:privacy, 28:policy, 15:centre, 15:center, 14:email, 10:services, 10:security, 10:search, 10:practices


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Asia} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Help} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Privacy} \colorbox{red!1}{\strut Centre} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Info} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Privacy} \colorbox{red!1}{\strut Centre} \colorbox{red!1}{\strut Email} \colorbox{red!0}{\strut Print} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Privacy} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Privacy} \colorbox{red!1}{\strut Policy} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut detailed} \colorbox{red!0}{\strut reference} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut describing} \colorbox{red!0}{\strut our} \colorbox{red!2}{\strut privacy} \colorbox{red!0}{\strut practices} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut wide} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut services} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Assistance} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Account} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Privacy} \colorbox{red!1}{\strut Centre} \colorbox{red!0}{\strut Special} \colorbox{red!0}{\strut Topics} \colorbox{red!0}{\strut Cookies} \colorbox{red!0}{\strut Data} \colorbox{red!0}{\strut Storage} \colorbox{red!0}{\strut IP} \colorbox{red!0}{\strut Addresses} \colorbox{red!0}{\strut Mobile} \colorbox{red!0}{\strut Devices} \colorbox{red!0}{\strut Promotions} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut Security} \colorbox{red!0}{\strut at} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Third} \colorbox{red!0}{\strut Party} \colorbox{red!0}{\strut Cookies} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut Beacons} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Services} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Address} \colorbox{red!0}{\strut Book} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Briefcase} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Calendar} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Chat} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Delivers} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Games} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut GeoCities} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Greetings} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Help} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Mail} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Messenger} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Mobile} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut News} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Notepad} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut People} \colorbox{red!0}{\strut Search} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Photos} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Search} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Weather} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2009} \colorbox{red!5}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Singapore} \colorbox{red!0}{\strut Pte} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ltd.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Co.} \colorbox{red!0}{\strut Reg} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 199700735D} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Rights} \colorbox{red!0}{\strut Reserved} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Privacy} \colorbox{red!1}{\strut Policy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Service} 
}}}
\end{CJK*}

99:yahoos, 99:yahoo, 38:mail, 30:app, 28:launch, 26:platform, 25:launching, 20:network, 17:soon, 17:labs


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut GigaOM} \colorbox{red!0}{\strut GigaOM} \colorbox{red!0}{\strut Earth2Tech} \colorbox{red!0}{\strut jkOnTheRun} \colorbox{red!0}{\strut NewTeeVee} \colorbox{red!0}{\strut OStatic} \colorbox{red!0}{\strut TheAppleBlog} \colorbox{red!0}{\strut WebWorkerDaily} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut Live} \colorbox{red!0}{\strut Events} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Posts} \colorbox{red!1}{\strut Web} \colorbox{red!0}{\strut Broadband} \colorbox{red!0}{\strut Infrastructure} \colorbox{red!1}{\strut Mobile} \colorbox{red!0}{\strut Voice} \colorbox{red!0}{\strut Briefings} \colorbox{red!0}{\strut Archives} \colorbox{red!9}{\strut Yahoo} \colorbox{red!4}{\strut Mail} \colorbox{red!3}{\strut App} \colorbox{red!2}{\strut Platform} \colorbox{red!1}{\strut To} \colorbox{red!0}{\strut LaunchTomorrow} \colorbox{red!0}{\strut Om} \colorbox{red!0}{\strut Malik} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sunday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 729} \colorbox{red!0}{\strut PM} \colorbox{red!1}{\strut PT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut comments} \colorbox{red!9}{\strut Yahoo} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut rotten} \colorbox{red!0}{\strut week} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut actually} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut positive} \colorbox{red!1}{\strut press} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut company} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut launching} \colorbox{red!9}{\strut Yahoo} \colorbox{red!4}{\strut Mail} \colorbox{red!1}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut platform} \colorbox{red!1}{\strut tomorrow} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut organizing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut big} \colorbox{red!0}{\strut shin-dig} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Francisco} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut launch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Last} \colorbox{red!0}{\strut week} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut that} \colorbox{red!9}{\strut Yahoo} \colorbox{red!0}{\strut would} \colorbox{red!3}{\strut launch} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut platform} \colorbox{red!0}{\strut relatively} \colorbox{red!2}{\strut soon} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut company} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut getting} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!1}{\strut applications} \colorbox{red!1}{\strut ready} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut launch} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut five} \colorbox{red!1}{\strut apps} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut launch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut response} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut previous} \colorbox{red!0}{\strut post} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut folks} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut links} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut blog} \colorbox{red!0}{\strut posts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut bits} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut give} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut clear} \colorbox{red!0}{\strut outline} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut Yahoos} \colorbox{red!1}{\strut plans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ShareEmail} \colorbox{red!0}{\strut Previous} \colorbox{red!0}{\strut Next} \colorbox{red!0}{\strut Job} \colorbox{red!0}{\strut Postings} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!1}{\strut Product} \colorbox{red!0}{\strut ManagerArchitect} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Orange} \colorbox{red!2}{\strut Labs} \colorbox{red!1}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut aka} \colorbox{red!0}{\strut France} \colorbox{red!1}{\strut Telecom} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut LLC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Francisco} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut Principal} \colorbox{red!1}{\strut IP} \colorbox{red!2}{\strut Network} \colorbox{red!1}{\strut Architect} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Orange} \colorbox{red!2}{\strut Labs} \colorbox{red!1}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut aka} \colorbox{red!0}{\strut France} \colorbox{red!1}{\strut Telecom} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut LLC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Francisco} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut Senior} \colorbox{red!1}{\strut IP} \colorbox{red!2}{\strut Network} \colorbox{red!1}{\strut Architect} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Orange} \colorbox{red!2}{\strut Labs} \colorbox{red!1}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut aka} \colorbox{red!0}{\strut France} \colorbox{red!1}{\strut Telecom} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut LLC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Francisco} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!1}{\strut Software} \colorbox{red!0}{\strut Engineer} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Home} \colorbox{red!1}{\strut Group} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Orange} \colorbox{red!2}{\strut Labs} \colorbox{red!1}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut aka} \colorbox{red!0}{\strut France} \colorbox{red!1}{\strut Telecom} \colorbox{red!1}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut LLC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Francisco} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut trackbacks} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut far} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 14th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut 814} \colorbox{red!0}{\strut PM} \colorbox{red!1}{\strut PT} \colorbox{red!9}{\strut Yahoo} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut Expand} \colorbox{red!0}{\strut Its} \colorbox{red!1}{\strut Email} \colorbox{red!1}{\strut as} \colorbox{red!3}{\strut App} \colorbox{red!2}{\strut Platform} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SolSie.com} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut recent} \colorbox{red!0}{\strut tarnished} \colorbox{red!0}{\strut image} \colorbox{red!0}{\strut ,} \colorbox{red!9}{\strut Yahoo} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut rumored} 
}}}
\end{CJK*}

query: euclid

87:elements, 84:euclid, 74:lived, 28:father, 27:geometry, 27:born, 24:which, 24:background, 21:study, 20:why


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Mahalo.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mahalo} \colorbox{red!0}{\strut Answers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mahalo} \colorbox{red!0}{\strut Daily} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mahalo} \colorbox{red!0}{\strut Greenhouse} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Liveblog} \colorbox{red!4}{\strut Euclid} \colorbox{red!1}{\strut Known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Father} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Geometry} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!3}{\strut lived} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut reign} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Ptolemy} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Alexandria} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Egypt} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut His} \colorbox{red!0}{\strut thirteen} \colorbox{red!0}{\strut volume} \colorbox{red!1}{\strut textbook} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut considered} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut preeminent} \colorbox{red!1}{\strut treatise} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut mathematics} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 2,000} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut studied} \colorbox{red!1}{\strut textbook} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut selling} \colorbox{red!1}{\strut book} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut history} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Bible} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fast} \colorbox{red!0}{\strut Facts} \colorbox{red!1}{\strut Born} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 325-330} \colorbox{red!0}{\strut B.C} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Died} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 265-260} \colorbox{red!0}{\strut B.C} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Studied} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Plato} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Academy} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Greece} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut established} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Alexandria} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut 1,000} \colorbox{red!0}{\strut editions} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut produced} \colorbox{red!0}{\strut Optica} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut published} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut earliest} \colorbox{red!0}{\strut surviving} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut study} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut visible} \colorbox{red!1}{\strut light} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut entitled} \colorbox{red!0}{\strut Optica} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut background} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut later} \colorbox{red!1}{\strut study} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut astronomy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Categories} \colorbox{red!1}{\strut History} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Science} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Mathematics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut Note} \colorbox{red!1}{\strut History} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Mahalo} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Alexandria} \colorbox{red!1}{\strut Math} \colorbox{red!0}{\strut Open} \colorbox{red!0}{\strut Reference} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut Clark} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut Molecular} \colorbox{red!0}{\strut Expressions} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut 325-265} \colorbox{red!0}{\strut BC} \colorbox{red!0}{\strut OBKB.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut Engineering.com} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Alexandria} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Mathematical} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Computational} \colorbox{red!0}{\strut Sciences} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut St} \colorbox{red!0}{\strut Andrews} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!4}{\strut Euclid} \colorbox{red!1}{\strut Background} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Works} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Background} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Perseus} \colorbox{red!0}{\strut Digital} \colorbox{red!0}{\strut Library} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Traditions} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Him} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Works} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut Clark} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut Internet} \colorbox{red!0}{\strut Archive} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut 1st} \colorbox{red!0}{\strut Six} \colorbox{red!1}{\strut Books} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 76.24} \colorbox{red!0}{\strut MB} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Data} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Catoptrics} \colorbox{red!0}{\strut OBKB.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Works} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Elements} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lost} \colorbox{red!1}{\strut Works} \colorbox{red!0}{\strut Dr.} \colorbox{red!0}{\strut Tuttle} \colorbox{red!0}{\strut Professor} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Engineering} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Denver} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Theorem} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Optics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Phaenomena} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut Images} \colorbox{red!0}{\strut Google} \colorbox{red!0}{\strut Image} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut Image} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Ask.com} \colorbox{red!0}{\strut Image} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} \colorbox{red!0}{\strut Image} \colorbox{red!0}{\strut Search} \colorbox{red!4}{\strut Euclid} \colorbox{red!1}{\strut Books} \colorbox{red!0}{\strut Amazon.com} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Euclid} 
}}}
\end{CJK*}

97:euclides, 96:euclid, 90:craters, 89:crater, 38:located, 20:impact, 19:latitude, 18:named, 17:name, 17:eppinger


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Euclides} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut crater} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!6}{\strut Euclides} \colorbox{red!5}{\strut crater} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!5}{\strut Crater} \colorbox{red!0}{\strut characteristics} \colorbox{red!1}{\strut Coordinates} \colorbox{red!0}{\strut 7.4} \colorbox{red!0}{\strut S} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 29.5} \colorbox{red!0}{\strut W} \colorbox{red!1}{\strut Diameter} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut km} \colorbox{red!1}{\strut Depth} \colorbox{red!0}{\strut 1.3} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut Colongitude} \colorbox{red!0}{\strut 29} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut sunrise} \colorbox{red!0}{\strut Eponym} \colorbox{red!6}{\strut Euclid} \colorbox{red!6}{\strut Euclides} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut small} \colorbox{red!1}{\strut lunar} \colorbox{red!1}{\strut impact} \colorbox{red!5}{\strut crater} \colorbox{red!2}{\strut located} \colorbox{red!0}{\strut near} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut eastern} \colorbox{red!0}{\strut edge} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Oceanus} \colorbox{red!0}{\strut Procellarum} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut kilometers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut west} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Montes} \colorbox{red!1}{\strut Riphaeus} \colorbox{red!1}{\strut mountains} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut mare} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut vicinity} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut devoid} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut significant} \colorbox{red!5}{\strut craters} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut west} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut rises} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut crater} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut named} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Greek} \colorbox{red!0}{\strut mathematician} \colorbox{red!6}{\strut Euclid} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Euclides} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut bowl-shaped} \colorbox{red!0}{\strut formation} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut circular} \colorbox{red!0}{\strut rim} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut surrounded} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut streaks} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut ejecta} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut higher} \colorbox{red!1}{\strut albedo} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nearby} \colorbox{red!0}{\strut maria} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut nebulous} \colorbox{red!0}{\strut skirt} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut light-hued} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut makes} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut feature} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut prominent} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut Sun} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut brightest} \colorbox{red!0}{\strut sites} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Moon} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Euclides} \colorbox{red!1}{\strut D} \colorbox{red!6}{\strut Euclides} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut small} \colorbox{red!1}{\strut lunar} \colorbox{red!1}{\strut impact} \colorbox{red!5}{\strut crater} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Mare} \colorbox{red!0}{\strut Cognitum} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut diameter} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut kilometers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut depth} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1.3} \colorbox{red!0}{\strut kilometers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut lies} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut southeast} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Euclides} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut beyond} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Montes} \colorbox{red!1}{\strut Riphaeus} \colorbox{red!1}{\strut mountains} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 1976} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut Euclides} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut renamed} \colorbox{red!1}{\strut Eppinger} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut IAU} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut honor} \colorbox{red!0}{\strut Hans} \colorbox{red!1}{\strut Eppinger} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut professor} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut pathological} \colorbox{red!0}{\strut anatomy} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Graz} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2002} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut after} \colorbox{red!1}{\strut Eppinger} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut association} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Nazi} \colorbox{red!0}{\strut prison} \colorbox{red!0}{\strut camps} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut brought} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut attention} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut IAU} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Working} \colorbox{red!0}{\strut Group} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Planetary} \colorbox{red!0}{\strut System} \colorbox{red!0}{\strut Nomenclature} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut changed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Satellite} \colorbox{red!5}{\strut craters} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut convention} \colorbox{red!0}{\strut these} \colorbox{red!1}{\strut features} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut identified} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut lunar} \colorbox{red!0}{\strut maps} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut placing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut letter} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut side} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut crater} \colorbox{red!0}{\strut mid-point} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut closest} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut Euclides} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Euclides} \colorbox{red!1}{\strut Latitude} \colorbox{red!1}{\strut Longitude} \colorbox{red!1}{\strut Diameter} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut 13.2} \colorbox{red!0}{\strut S} \colorbox{red!0}{\strut 30.0} 
}}}
\end{CJK*}

query: starbucks

99:starbucks, 62:union, 42:iww, 32:labor, 30:workers, 23:fired, 22:workplace, 19:swu, 19:pay, 19:join


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Starbucks} \colorbox{red!3}{\strut Union} \colorbox{red!2}{\strut IWW} \colorbox{red!5}{\strut Starbucks} \colorbox{red!1}{\strut Workers} \colorbox{red!3}{\strut Union} \colorbox{red!1}{\strut Register} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut us} \colorbox{red!1}{\strut phone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 917-577-1110} \colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut Menu} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Bean2Cup} \colorbox{red!0}{\strut Campus} \colorbox{red!1}{\strut Campaign} \colorbox{red!0}{\strut E-mail} \colorbox{red!0}{\strut Action} \colorbox{red!0}{\strut Updates} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut Involved} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Archive} \colorbox{red!0}{\strut Forums} \colorbox{red!0}{\strut Documentary} \colorbox{red!0}{\strut Govt} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut Settlement} \colorbox{red!0}{\strut Events} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut User} \colorbox{red!0}{\strut login} \colorbox{red!0}{\strut Username} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Password} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Create} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut Request} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut password} \colorbox{red!5}{\strut Starbucks} \colorbox{red!3}{\strut Union} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut receive} \colorbox{red!1}{\strut campaign} \colorbox{red!0}{\strut bulletins} \colorbox{red!0}{\strut E-mail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Subscribe} \colorbox{red!0}{\strut Unsubscribe} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut feed} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!5}{\strut Starbucks} \colorbox{red!1}{\strut Workers} \colorbox{red!0}{\strut Coming} \colorbox{red!0}{\strut Together} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Increased} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut raises} \colorbox{red!0}{\strut Guaranteed} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut option} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut fulltime} \colorbox{red!0}{\strut status} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut understaffing} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut healthier} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut safer} \colorbox{red!1}{\strut workplace} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut Involved} \colorbox{red!1}{\strut Join} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Union} \colorbox{red!0}{\strut Contribute} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Recent} \colorbox{red!0}{\strut blog} \colorbox{red!0}{\strut posts} \colorbox{red!0}{\strut Swedish} \colorbox{red!3}{\strut Union} \colorbox{red!0}{\strut Seeks} \colorbox{red!0}{\strut Support} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut Nazi} \colorbox{red!0}{\strut Murder} \colorbox{red!0}{\strut Attempt} \colorbox{red!1}{\strut SWU} \colorbox{red!0}{\strut Member} \colorbox{red!0}{\strut Daniel} \colorbox{red!0}{\strut Gross} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Chicago} \colorbox{red!0}{\strut Sit-Down} \colorbox{red!1}{\strut Strike} \colorbox{red!1}{\strut Members} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut SWU} \colorbox{red!0}{\strut Sister} \colorbox{red!3}{\strut Union} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Sweden} \colorbox{red!0}{\strut Survive} \colorbox{red!0}{\strut Nazi} \colorbox{red!0}{\strut Attack} \colorbox{red!0}{\strut Blast} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut IWW} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MOA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut TC} \colorbox{red!0}{\strut Daily} \colorbox{red!0}{\strut Planet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mall} \colorbox{red!5}{\strut Starbucks} \colorbox{red!1}{\strut workers} \colorbox{red!1}{\strut join} \colorbox{red!3}{\strut union} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Star} \colorbox{red!0}{\strut Tribune} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mall} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut America} \colorbox{red!5}{\strut Starbucks} \colorbox{red!1}{\strut Baristas} \colorbox{red!0}{\strut Walk} \colorbox{red!0}{\strut Off} \colorbox{red!0}{\strut Job} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Protest} \colorbox{red!0}{\strut Closures} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fox} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SWU} \colorbox{red!0}{\strut Allies} \colorbox{red!0}{\strut Hit} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Spain} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut Day} \colorbox{red!0}{\strut Judge} \colorbox{red!0}{\strut draws} \colorbox{red!0}{\strut clear} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut tip} \colorbox{red!0}{\strut jar} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut Will} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut reveal} \colorbox{red!1}{\strut Calorie} \colorbox{red!0}{\strut count} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Appeal} \colorbox{red!0}{\strut Tip-Sharing} \colorbox{red!1}{\strut Ruling} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut Sbux} \colorbox{red!3}{\strut Union} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut E-Mail} \colorbox{red!0}{\strut Action} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tell} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Year} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Honor} \colorbox{red!0}{\strut Dr.} \colorbox{red!0}{\strut King} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Holiday} \colorbox{red!0}{\strut !} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Union} \colorbox{red!0}{\strut Blues} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut BusinessWeek} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut Loses} \colorbox{red!0}{\strut Round} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Battle} \colorbox{red!0}{\strut Over} \colorbox{red!3}{\strut Union} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!0}{\strut Times} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Judge} \colorbox{red!0}{\strut Finds} \colorbox{red!5}{\strut Starbucks} \colorbox{red!1}{\strut Guilty} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Extensive} \colorbox{red!0}{\strut Union-Busting} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut Wo} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut Back} \colorbox{red!0}{\strut Down} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut Manager} \colorbox{red!0}{\strut Threatens} \colorbox{red!1}{\strut Lawsuit} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Criminal} \colorbox{red!1}{\strut Complaint} \colorbox{red!0}{\strut Against} \colorbox{red!2}{\strut IWW} \colorbox{red!1}{\strut Baristas} \colorbox{red!0}{\strut Present} \colorbox{red!0}{\strut 500} \colorbox{red!0}{\strut Petition} \colorbox{red!0}{\strut Signatures} \colorbox{red!0}{\strut Demanding} \colorbox{red!0}{\strut Improved} \colorbox{red!0}{\strut Security} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Minneapolis} \colorbox{red!5}{\strut Starbucks} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut Blues} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Slate} \colorbox{red!0}{\strut Magazine} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Starbucks} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut Conference} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Orleans} \colorbox{red!0}{\strut Hit} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Unexpected} \colorbox{red!3}{\strut Union} \colorbox{red!1}{\strut Protest} \colorbox{red!5}{\strut Starbucks} \colorbox{red!1}{\strut settles} \colorbox{red!0}{\strut NLRB} \colorbox{red!1}{\strut complaint} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut fired} \colorbox{red!1}{\strut barista} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut AP} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Baristas} \colorbox{red!0}{\strut Defeat} 
}}}
\end{CJK*}

97:starbucks, 56:what, 50:starbuck, 34:coffee, 33:coffees, 23:where, 21:t, 21:outlets, 19:jeeves, 17:money


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut From} \colorbox{red!1}{\strut Uncyclopedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut content-free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut search} \colorbox{red!1}{\strut Whoops} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Maybe} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Capitalism} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut told} \colorbox{red!1}{\strut Jeeves} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut did} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut my} \colorbox{red!3}{\strut coffee} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 5-minutes} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut would} \colorbox{red!1}{\strut replace} \colorbox{red!0}{\strut him} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut house} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut service} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut shit} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut stisfaction} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut knowing} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut Jeeves} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut searching} \colorbox{red!0}{\strut through} \colorbox{red!1}{\strut shit} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut coffee} \colorbox{red!1}{\strut beans} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 2.00} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut millenium} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Cocky} \colorbox{red!1}{\strut Mcrew} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Oscar} \colorbox{red!0}{\strut Wilde} \colorbox{red!0}{\strut on} \colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut wrong} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut many} \colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut uming} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut money} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut economy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mor} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut wt} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut priou} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mony} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut George} \colorbox{red!0}{\strut Dubya} \colorbox{red!0}{\strut Bush} \colorbox{red!0}{\strut on} \colorbox{red!8}{\strut Starbucks} \colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut computer} \colorbox{red!1}{\strut virus} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut escaped} \colorbox{red!0}{\strut cyberspace} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut infected} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut real} \colorbox{red!1}{\strut world} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut chain} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut coffee} \colorbox{red!1}{\strut shops} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut hugest} \colorbox{red!1}{\strut moneymaking} \colorbox{red!0}{\strut schemes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut world} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut virus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut creator} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Dirk} \colorbox{red!1}{\strut Benedict} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut now} \colorbox{red!1}{\strut owning} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut whole} \colorbox{red!1}{\strut planet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Neptune} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Overview} \colorbox{red!0}{\strut 2} \colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut Formation} \colorbox{red!0}{\strut 3} \colorbox{red!4}{\strut What} \colorbox{red!1}{\strut happened} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Dirk} \colorbox{red!0}{\strut Starbuck} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Benedict} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut little} \colorbox{red!3}{\strut coffee} \colorbox{red!1}{\strut stall} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 4} \colorbox{red!1}{\strut Tall} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Grande} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Venti} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Downfall} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut Milan} \colorbox{red!0}{\strut Massacre} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut In-Store} \colorbox{red!0}{\strut Promotions} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Coffee} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut Various} \colorbox{red!3}{\strut Coffees} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sizes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut Competitors} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Overview} \colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Coffee} \colorbox{red!1}{\strut Corporation} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Promotion} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Image} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Starbuck} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Starbucks} \colorbox{red!3}{\strut Coffee} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut simply} \colorbox{red!8}{\strut Starbucks} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut not-for-profit} \colorbox{red!1}{\strut organization} \colorbox{red!2}{\strut where} \colorbox{red!0}{\strut bastard} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut children} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut drink} \colorbox{red!0}{\strut tea} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut consume} \colorbox{red!0}{\strut pre-huffed} \colorbox{red!0}{\strut kittens} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Its} \colorbox{red!1}{\strut three} \colorbox{red!1}{\strut corporate} \colorbox{red!1}{\strut values} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut promote} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut well-being} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut communities} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut increased} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut contact} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: diabetes education

101:diabetic, 92:diabetes, 50:menus, 47:menu, 31:recipes, 31:lists, 24:grocery, 22:list, 20:planner, 20:medications


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut web} \colorbox{red!0}{\strut resource} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut professional} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut educators} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Recipes} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Diabetes} \colorbox{red!2}{\strut Menus} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Grocery} \colorbox{red!1}{\strut Lists} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Nutrition} \colorbox{red!0}{\strut Facts} \colorbox{red!0}{\strut !} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Certified} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Educator} \colorbox{red!0}{\strut CDE} \colorbox{red!0}{\strut Home} \colorbox{red!3}{\strut Diabetes} \colorbox{red!2}{\strut Menus} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut Educators} \colorbox{red!0}{\strut FAQs} \colorbox{red!0}{\strut Sign-Up} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut e-mail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut password} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FREE} \colorbox{red!3}{\strut Diabetes} \colorbox{red!2}{\strut Menu} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Week} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Body} \colorbox{red!0}{\strut Calculator} \colorbox{red!1}{\strut Food} \colorbox{red!0}{\strut Picker} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Recipes} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut Pre-Diabetes} \colorbox{red!0}{\strut Recently} \colorbox{red!0}{\strut Diagnosed} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut Groups} \colorbox{red!0}{\strut Weight} \colorbox{red!0}{\strut Loss} \colorbox{red!0}{\strut Live} \colorbox{red!0}{\strut Chat} \colorbox{red!0}{\strut Feedback} \colorbox{red!0}{\strut Sign-Up} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut Educators} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!0}{\strut services} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut Educators} \colorbox{red!0}{\strut Add} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut Locator} \colorbox{red!0}{\strut database} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut educator} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Educator} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut diabetes} \colorbox{red!1}{\strut educator} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut diabetes} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut request} \colorbox{red!0}{\strut brochures} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Diabetes} \colorbox{red!1}{\strut Educator} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut submitting} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!0}{\strut Write} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut becoming} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut CDE} \colorbox{red!0}{\strut Become} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut CDE} \colorbox{red!0}{\strut Interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut becoming} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut Certified} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Advanced} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut Educators} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Diabetes} \colorbox{red!2}{\strut Menus} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut Educators} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sign-up} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FAQs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2001} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2002} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2003} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!0}{\strut Presented} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Nutrition} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut Inc.} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut topics} \colorbox{red!0}{\strut covering} \colorbox{red!3}{\strut diabetes} \colorbox{red!1}{\strut medications} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut complications} \colorbox{red!4}{\strut diabetic} \colorbox{red!1}{\strut diet} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut nutrition} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut diagnosed} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Menus} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut prepared} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut professional} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut educators} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Weekly} \colorbox{red!3}{\strut diabetes} \colorbox{red!2}{\strut menu} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut grocery} \colorbox{red!1}{\strut list} \colorbox{red!3}{\strut diabetes} \colorbox{red!1}{\strut recipes} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut nutrition} \colorbox{red!0}{\strut analysis} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!0}{\strut website} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut apply} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Our} \colorbox{red!3}{\strut diabetes} \colorbox{red!2}{\strut menus} \colorbox{red!3}{\strut diabetes} \colorbox{red!1}{\strut recipes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut replace} \colorbox{red!0}{\strut professional} \colorbox{red!0}{\strut medical} \colorbox{red!0}{\strut advice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut aware} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut complications} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut issues} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Always} \colorbox{red!0}{\strut check} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut physician} \colorbox{red!0}{\strut prior} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut starting} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut diabetic} \colorbox{red!1}{\strut diet} \colorbox{red!3}{\strut diabetes} \colorbox{red!1}{\strut medications} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut program} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

96:diabetes, 85:what, 70:educational, 68:educator, 66:educators, 63:education, 58:cde, 51:certified, 43:certification, 26:nurse


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Certified} \colorbox{red!4}{\strut diabetes} \colorbox{red!3}{\strut educator} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut A} \colorbox{red!2}{\strut Certified} \colorbox{red!4}{\strut diabetes} \colorbox{red!3}{\strut educator} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut CDE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut health} \colorbox{red!1}{\strut care} \colorbox{red!1}{\strut professional} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut specialized} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut certified} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut teach} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut with} \colorbox{red!4}{\strut diabetes} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut manage} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut condition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut CDE} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut invaluable} \colorbox{red!0}{\strut asset} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut those} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tools} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut skills} \colorbox{red!0}{\strut necessary} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut blood} \colorbox{red!0}{\strut sugar} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut avoid} \colorbox{red!0}{\strut long-term} \colorbox{red!0}{\strut complications} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut hyperglycemia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Unlike} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut endocrinologist} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut CDE} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut spend} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut newly} \colorbox{red!0}{\strut diagnosed} \colorbox{red!0}{\strut person} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut needed} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut educational} \colorbox{red!0}{\strut purposes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut emotional} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Typically} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut CDE} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut nurse} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut dietitian} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pharmacist} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut worker} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut specialized} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut diabetes} \colorbox{red!3}{\strut education} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut care} \colorbox{red!0}{\strut management} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Formal} \colorbox{red!3}{\strut education} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut practical} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut required} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut formal} \colorbox{red!0}{\strut examination} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut diabetes} \colorbox{red!3}{\strut educator} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut certified} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut certification} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut awarded} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut National} \colorbox{red!2}{\strut Certification} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut Diabetes} \colorbox{red!3}{\strut Educators} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Canada} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut certification} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut awarded} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Canadian} \colorbox{red!4}{\strut Diabetes} \colorbox{red!3}{\strut Educator} \colorbox{red!2}{\strut Certification} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CDECB} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Philippines} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut allied} \colorbox{red!1}{\strut health} \colorbox{red!1}{\strut care} \colorbox{red!1}{\strut professional} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut apply} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut diabetes} \colorbox{red!3}{\strut educator} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut courses} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Philippine} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Diabetes} \colorbox{red!3}{\strut Educators} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PADE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Diabetes} \colorbox{red!1}{\strut Nurse} \colorbox{red!3}{\strut Educators} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Philippines} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ADNEP} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Qualified} \colorbox{red!0}{\strut graduates} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut diabetes} \colorbox{red!3}{\strut educator} \colorbox{red!0}{\strut courses} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut practice} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut professional} \colorbox{red!4}{\strut diabetes} \colorbox{red!3}{\strut educator} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut Diabetes} \colorbox{red!1}{\strut Care} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CDC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut clinic} \colorbox{red!0}{\strut network} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut Diabetes} \colorbox{red!1}{\strut Nurse} \colorbox{red!3}{\strut Educator} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DNE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Certified} \colorbox{red!0}{\strut Lay} \colorbox{red!3}{\strut Educator} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut CLE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut equivalent} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut CDE} \colorbox{red!1}{\strut certificate} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Philippines} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut American} \colorbox{red!4}{\strut Diabetes} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Center} 
}}}
\end{CJK*}

query: website design hosting

38:cms, 30:hosting, 28:fire, 25:angel, 24:design, 20:website, 19:site, 18:web, 16:albuquerque, 15:database


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!2}{\strut CMS} \colorbox{red!1}{\strut Website} \colorbox{red!0}{\strut SEO} \colorbox{red!1}{\strut Blog} \colorbox{red!1}{\strut Web} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut eCommerce} \colorbox{red!0}{\strut Affiliate} \colorbox{red!0}{\strut Store} \colorbox{red!0}{\strut Shopping} \colorbox{red!0}{\strut Cart} \colorbox{red!1}{\strut Web} \colorbox{red!0}{\strut Evaluation} \colorbox{red!1}{\strut Database} \colorbox{red!2}{\strut Hosting} \colorbox{red!1}{\strut Database} \colorbox{red!0}{\strut Demos} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Engines} \colorbox{red!0}{\strut Free} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!0}{\strut Portfolio} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Company} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut ImageBuilders} \colorbox{red!0}{\strut PO} \colorbox{red!0}{\strut Box} \colorbox{red!0}{\strut 995} \colorbox{red!1}{\strut Angel} \colorbox{red!1}{\strut Fire} \colorbox{red!0}{\strut NM} \colorbox{red!0}{\strut 87710} \colorbox{red!0}{\strut Phone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 505.377.2372} \colorbox{red!0}{\strut Email} \colorbox{red!1}{\strut Albuquerque} \colorbox{red!1}{\strut Angel} \colorbox{red!1}{\strut Fire} \colorbox{red!0}{\strut Santa} \colorbox{red!0}{\strut Fe} \colorbox{red!1}{\strut Houston} \colorbox{red!0}{\strut Dallas} \colorbox{red!1}{\strut Taos} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2003} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut ImageBuilders} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut Business} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Web} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Database} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ImageBuilders} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Web} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Database} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Design} \colorbox{red!1}{\strut Houston} \colorbox{red!0}{\strut Small} \colorbox{red!0}{\strut Business} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Website} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Database} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut Free} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Blog} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Engine} \colorbox{red!0}{\strut Optimization} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut Free} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Blog} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Albuquerque} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Engine} \colorbox{red!0}{\strut Optimization} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut Free} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Blog} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Santa} \colorbox{red!0}{\strut Fe} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Engine} \colorbox{red!0}{\strut Optimization} \colorbox{red!0}{\strut Services} \colorbox{red!1}{\strut Albuquerque} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!2}{\strut Hosting} \colorbox{red!1}{\strut Houston} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Web} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut Dallas} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Web} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut Santa} \colorbox{red!0}{\strut Fe} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Mexico} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Website} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut Nationwide} \colorbox{red!1}{\strut Web} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Albuquerque} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Santa} \colorbox{red!0}{\strut Fe} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Taos} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Angel} \colorbox{red!1}{\strut Fire} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Houston} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Dallas} \colorbox{red!0}{\strut Phoenix} \colorbox{red!0}{\strut Arizona} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eCommerce} \colorbox{red!1}{\strut Website} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut Mesa} \colorbox{red!0}{\strut Phoenix} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Website} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut FSBO} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Estate} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut Alamosa} \colorbox{red!0}{\strut Colorado} \colorbox{red!0}{\strut eCommerce} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Web} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut php} \colorbox{red!0}{\strut Conejos} \colorbox{red!0}{\strut Colorado} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Estate} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Luis} \colorbox{red!0}{\strut Colorado} \colorbox{red!1}{\strut Web} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Website} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut Washington} \colorbox{red!0}{\strut DC} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eCommerce} \colorbox{red!1}{\strut Website} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut Alpharetta} \colorbox{red!0}{\strut Atlanta} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut CMS} \colorbox{red!1}{\strut Website} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut Atlanta} \colorbox{red!0}{\strut Georgia} \colorbox{red!2}{\strut CMS} \colorbox{red!1}{\strut Database} \colorbox{red!1}{\strut Web} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eCommerce} \colorbox{red!1}{\strut Website} \colorbox{red!2}{\strut Hosting} \colorbox{red!0}{\strut Brazil} 
}}}
\end{CJK*}

86:website, 86:designs, 85:websites, 79:design, 78:designer, 74:designing, 56:web, 49:ascend, 48:yahoo, 38:host


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Ascend} \colorbox{red!4}{\strut Web} \colorbox{red!6}{\strut Designs} \colorbox{red!1}{\strut offers} \colorbox{red!6}{\strut website} \colorbox{red!5}{\strut design} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut hosting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut internet} \colorbox{red!2}{\strut marketing} \colorbox{red!1}{\strut services} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut tailored} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut small} \colorbox{red!1}{\strut business} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut personal} \colorbox{red!1}{\strut needs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut pride} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut designing} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut quality} \colorbox{red!6}{\strut websites} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut quick} \colorbox{red!0}{\strut turnaround} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut consultative} \colorbox{red!0}{\strut approach} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut recommending} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut effective} \colorbox{red!6}{\strut website} \colorbox{red!5}{\strut design} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut delivers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Choosing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut local} \colorbox{red!6}{\strut website} \colorbox{red!5}{\strut design} \colorbox{red!0}{\strut firm} \colorbox{red!0}{\strut means} \colorbox{red!0}{\strut face-to-face} \colorbox{red!0}{\strut collaboration} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut customers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut own} \colorbox{red!2}{\strut site} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut middle} \colorbox{red!0}{\strut man} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut do} \colorbox{red!6}{\strut website} \colorbox{red!5}{\strut design} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut pay} \colorbox{red!3}{\strut Yahoo} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11.95} \colorbox{red!0}{\strut per} \colorbox{red!1}{\strut month} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut host} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut website} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut as} \colorbox{red!3}{\strut long} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Great} \colorbox{red!1}{\strut value} \colorbox{red!0}{\strut Basic} \colorbox{red!6}{\strut website} \colorbox{red!5}{\strut design} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut three} \colorbox{red!1}{\strut pages} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 299} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Professional} \colorbox{red!0}{\strut look} \colorbox{red!1}{\strut Custom} \colorbox{red!6}{\strut website} \colorbox{red!5}{\strut design} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut scratch} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 400} \colorbox{red!6}{\strut website} \colorbox{red!0}{\strut templates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eCommerce} \colorbox{red!0}{\strut capable} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PayPal} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut shopping} \colorbox{red!0}{\strut carts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On-page} \colorbox{red!0}{\strut search} \colorbox{red!1}{\strut engine} \colorbox{red!1}{\strut optimization} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SEO} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut standard} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Off-page} \colorbox{red!1}{\strut SEO} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Hosted} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut trusted} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut also} \colorbox{red!5}{\strut design} \colorbox{red!0}{\strut Blog-sites} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut HTML} \colorbox{red!0}{\strut programming} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut marketing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sales} \colorbox{red!0}{\strut positioning} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut make} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut break} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut web} \colorbox{red!2}{\strut site} \colorbox{red!0}{\strut investment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Take} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut opportunity} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut team} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut professionals} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut selling} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut marketing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut CEO} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut President} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut CIO} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Chief} \colorbox{red!2}{\strut Marketing} \colorbox{red!0}{\strut Officers} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GM} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut GNC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Borgota} \colorbox{red!0}{\strut Casino} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Nextel} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lexis-Nexis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Laureate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lincoln} \colorbox{red!0}{\strut Financial} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Let} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Servicing} \colorbox{red!0}{\strut everywhere} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut specializing} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Baltimore} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Annapolis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut D.C.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Northern} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Central} \colorbox{red!0}{\strut Virginia} \colorbox{red!0}{\strut Our} \colorbox{red!0}{\strut search} \colorbox{red!1}{\strut engine} \colorbox{red!1}{\strut optimization} \colorbox{red!1}{\strut services} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut keywords} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut meta} \colorbox{red!0}{\strut tags} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

query: elliptical trainer

100:trainers, 97:trainer, 97:cross, 91:marcy, 46:elliptical, 24:treadmills, 17:fitness, 16:weight, 16:price, 16:machines


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Home} \colorbox{red!1}{\strut Treadmills} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Exercise} \colorbox{red!0}{\strut Bikes} \colorbox{red!0}{\strut Multi} \colorbox{red!0}{\strut Gyms} \colorbox{red!0}{\strut Rowing} \colorbox{red!0}{\strut Machines} \colorbox{red!0}{\strut Weight} \colorbox{red!0}{\strut Benches} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut Will} \colorbox{red!0}{\strut Not} \colorbox{red!0}{\strut Be} \colorbox{red!0}{\strut Beaten} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut Price} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut Marcy} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Call} \colorbox{red!0}{\strut Now} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Details} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut 01942} \colorbox{red!0}{\strut 495695} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ProductsSearch} \colorbox{red!0}{\strut Advanced} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Select} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Brand} \colorbox{red!0}{\strut ProductCategories} \colorbox{red!0}{\strut Special} \colorbox{red!0}{\strut Offers} \colorbox{red!1}{\strut Treadmills} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut Fitness} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Horizon} \colorbox{red!0}{\strut Fitness} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Bremshey} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Tunturi} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Vision} \colorbox{red!0}{\strut Fitness} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Pro-Form} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Beny} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Reebok} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut TrimMaster} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Johnson} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Nordic} \colorbox{red!0}{\strut Track} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!2}{\strut Marcy} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Motive} \colorbox{red!0}{\strut Fitness} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut York} \colorbox{red!0}{\strut Fitness} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Exercise} \colorbox{red!0}{\strut Bikes} \colorbox{red!0}{\strut Multi} \colorbox{red!0}{\strut Gyms} \colorbox{red!0}{\strut Rowing} \colorbox{red!0}{\strut Machines} \colorbox{red!0}{\strut Weight} \colorbox{red!0}{\strut Benches} \colorbox{red!0}{\strut Smith} \colorbox{red!0}{\strut Machines} \colorbox{red!0}{\strut Leg} \colorbox{red!0}{\strut Machines} \colorbox{red!0}{\strut Mid} \colorbox{red!0}{\strut Section} \colorbox{red!0}{\strut Machines} \colorbox{red!0}{\strut Upper} \colorbox{red!0}{\strut Body} \colorbox{red!0}{\strut Machines} \colorbox{red!0}{\strut Powerblock} \colorbox{red!0}{\strut Dumbells} \colorbox{red!0}{\strut Commercial} \colorbox{red!0}{\strut Equipment} \colorbox{red!0}{\strut Vibration} \colorbox{red!0}{\strut Plates} \colorbox{red!0}{\strut Boxing} \colorbox{red!0}{\strut Equipment} \colorbox{red!0}{\strut Heart} \colorbox{red!0}{\strut Rate} \colorbox{red!0}{\strut Monitors} \colorbox{red!0}{\strut Powerbreathe} \colorbox{red!0}{\strut Snooker} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pool} \colorbox{red!0}{\strut Tables} \colorbox{red!0}{\strut Table} \colorbox{red!0}{\strut Games} \colorbox{red!0}{\strut Table} \colorbox{red!0}{\strut Tennis} \colorbox{red!0}{\strut Tables} \colorbox{red!0}{\strut Steppers} \colorbox{red!0}{\strut Kid-e-Fit} \colorbox{red!0}{\strut Exercise} \colorbox{red!0}{\strut Equipment} \colorbox{red!0}{\strut Football} \colorbox{red!0}{\strut Tables} \colorbox{red!0}{\strut Powerbar} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Premier} \colorbox{red!0}{\strut Sports} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Fitness} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Delivery} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut Secure} \colorbox{red!0}{\strut Ordering} \colorbox{red!0}{\strut Returns} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut Guide} \colorbox{red!1}{\strut Treadmills} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut Guide} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Exercise} \colorbox{red!0}{\strut Bikes} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Multi} \colorbox{red!0}{\strut Gyms} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Rowing} \colorbox{red!0}{\strut Machines} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Weight} \colorbox{red!0}{\strut Benches} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Heart} \colorbox{red!0}{\strut Rate} \colorbox{red!0}{\strut Monitor} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut Products} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!2}{\strut Marcy} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!2}{\strut Marcy} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!2}{\strut Marcy} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut offer} \colorbox{red!0}{\strut excellent} \colorbox{red!0}{\strut functionality} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut budget} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut break} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut bank} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Designed} \colorbox{red!0}{\strut primarily} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut beginners} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Marcy} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainers} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut easy} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut display} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut magnetic} \colorbox{red!0}{\strut resistance} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut handgrip} \colorbox{red!0}{\strut pulse} \colorbox{red!0}{\strut sensors} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut budget} \colorbox{red!0}{\strut buy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Filter} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Marcy} \colorbox{red!0}{\strut E8820D} \colorbox{red!1}{\strut Elliptical} \colorbox{red!2}{\strut Cross} \colorbox{red!2}{\strut Trainer} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Save} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.97} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut E8820D} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut compact} \colorbox{red!0}{\strut dual} \colorbox{red!0}{\strut action} \colorbox{red!1}{\strut elliptical} \colorbox{red!2}{\strut cross} \colorbox{red!2}{\strut trainer} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut varying} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Price29.00} 
}}}
\end{CJK*}

99:ellipticals, 99:elliptical, 81:trainers, 71:trainer, 64:warranty, 52:warranties, 18:ratings, 18:fitness, 18:best, 14:importance


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Elliptical} \colorbox{red!6}{\strut Trainer} \colorbox{red!1}{\strut Online} \colorbox{red!1}{\strut Stores} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Elliptical} \colorbox{red!0}{\strut Buyer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!1}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Warranty} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Send} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Reviews} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Best} \colorbox{red!1}{\strut Buy} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Ellipticals} \colorbox{red!9}{\strut Elliptical} \colorbox{red!2}{\strut Ratings} \colorbox{red!9}{\strut Elliptical} \colorbox{red!1}{\strut Reviews} \colorbox{red!0}{\strut NordicTrack} \colorbox{red!0}{\strut 990} \colorbox{red!0}{\strut NordicTrack} \colorbox{red!0}{\strut 1300} \colorbox{red!1}{\strut Sole} \colorbox{red!2}{\strut Fitness} \colorbox{red!1}{\strut E55} \colorbox{red!1}{\strut Sole} \colorbox{red!2}{\strut Fitness} \colorbox{red!1}{\strut E35} \colorbox{red!1}{\strut Smooth} \colorbox{red!0}{\strut CE} \colorbox{red!0}{\strut 3.2} \colorbox{red!1}{\strut Smooth} \colorbox{red!0}{\strut CE} \colorbox{red!0}{\strut 7.4} \colorbox{red!1}{\strut Schwinn} \colorbox{red!0}{\strut 430} \colorbox{red!1}{\strut Schwinn} \colorbox{red!0}{\strut 460} \colorbox{red!0}{\strut ProForm} \colorbox{red!0}{\strut 1200} \colorbox{red!0}{\strut Reebok} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut ZX} \colorbox{red!1}{\strut Horizon} \colorbox{red!0}{\strut EX-77} \colorbox{red!1}{\strut Life} \colorbox{red!2}{\strut Fitness} \colorbox{red!0}{\strut X3} \colorbox{red!0}{\strut New} \colorbox{red!1}{\strut Balance} \colorbox{red!0}{\strut 9.0} \colorbox{red!1}{\strut Octane} \colorbox{red!1}{\strut Q47} \colorbox{red!1}{\strut Precor} \colorbox{red!0}{\strut EFX} \colorbox{red!0}{\strut 5.17} \colorbox{red!1}{\strut Spirit} \colorbox{red!0}{\strut ZE110} \colorbox{red!0}{\strut True} \colorbox{red!1}{\strut TSXa} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut More} \colorbox{red!1}{\strut Reviews} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Best} \colorbox{red!1}{\strut Buy} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Treadmills} \colorbox{red!1}{\strut Treadmill} \colorbox{red!2}{\strut Ratings} \colorbox{red!9}{\strut Elliptical} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Fitness} \colorbox{red!1}{\strut Articles} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Importance} \colorbox{red!1}{\strut of} \colorbox{red!9}{\strut Elliptical} \colorbox{red!6}{\strut Trainer} \colorbox{red!5}{\strut Warranties} \colorbox{red!1}{\strut One} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut best} \colorbox{red!1}{\strut indicators} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut quality} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!9}{\strut elliptical} \colorbox{red!6}{\strut trainer} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut extent} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut warranty} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!6}{\strut warranty} \colorbox{red!0}{\strut lets} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut beyond} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut hype} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut reveals} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut degree} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut confidence} \colorbox{red!0}{\strut an} \colorbox{red!9}{\strut elliptical} \colorbox{red!1}{\strut manufacturer} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut example} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Weslo} \colorbox{red!9}{\strut elliptical} \colorbox{red!7}{\strut trainers} \colorbox{red!1}{\strut come} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 90} \colorbox{red!1}{\strut parts} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut labor} \colorbox{red!6}{\strut warranty} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: gps

100:gps, 76:bluetooth, 29:price, 19:navigation, 17:name, 16:mk, 15:supply, 15:products, 15:product, 15:new


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Welcome} \colorbox{red!0}{\strut buyer-} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut Visit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2009-1-20} \colorbox{red!0}{\strut 84154} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Message} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut reply} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Buy} \colorbox{red!0}{\strut Offer} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut Not} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut member} \colorbox{red!0}{\strut yet} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Join} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut FREE} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Product} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Product} \colorbox{red!0}{\strut Name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mk-722} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7gps} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut bluetooth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut FM} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AV} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sd} \colorbox{red!0}{\strut card} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Detail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Touch} \colorbox{red!0}{\strut screen} \colorbox{red!0}{\strut TFT} \colorbox{red!0}{\strut LCD} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut build-in} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut receiver} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Bluetooth} \colorbox{red!0}{\strut Shirf} \colorbox{red!0}{\strut star} \colorbox{red!0}{\strut IIIBuilt-in} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut antenna} \colorbox{red!0}{\strut CPU} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut S3C2440A} \colorbox{red!0}{\strut 400MHz} \colorbox{red!0}{\strut WinCE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Net} \colorbox{red!0}{\strut 4.2} \colorbox{red!0}{\strut Core} \colorbox{red!0}{\strut SDRAM} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Low} \colorbox{red!0}{\strut Power} \colorbox{red!0}{\strut 64MB} \colorbox{red!0}{\strut Nand} \colorbox{red!0}{\strut Flash} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3264128256512MB1GB} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut optional} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SD} \colorbox{red!0}{\strut memory} \colorbox{red!0}{\strut Slot} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut SD} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 128MB-2GB} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Support} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MP3} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Movie} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut E-Book} \colorbox{red!0}{\strut With} \colorbox{red!2}{\strut Bluetooth} \colorbox{red!0}{\strut More} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut Exporters} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Waimao8} \colorbox{red!0}{\strut mk-722} \colorbox{red!0}{\strut mk-308} \colorbox{red!0}{\strut mk-488} \colorbox{red!0}{\strut 4.3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut touch} \colorbox{red!0}{\strut screen} \colorbox{red!0}{\strut DVB-T} \colorbox{red!0}{\strut tv} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut mp4} \colorbox{red!0}{\strut functions} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut Navigation} \colorbox{red!0}{\strut System} \colorbox{red!0}{\strut Weltone} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut Anti-theft} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -robbing} \colorbox{red!0}{\strut System} \colorbox{red!0}{\strut 7.0inch} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut 4.3inch} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut G-1.47} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut item} \colorbox{red!0}{\strut 3.5inch} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut Navigation} \colorbox{red!0}{\strut 3.5inch} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut Navigation} \colorbox{red!0}{\strut 4.3inch} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut 3.5inch} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut Navigation} \colorbox{red!0}{\strut supply} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut gps} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!0}{\strut GPS20081121} \colorbox{red!0}{\strut supply} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut gps} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut 20081121} \colorbox{red!0}{\strut supply} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut gps} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut 20081121} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut gps} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut gps} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut gps} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut manufacturer20081121} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut manufacturer20081121} \colorbox{red!0}{\strut supply} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut gps} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut GPS20081121} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!0}{\strut supply} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut 20081121} \colorbox{red!0}{\strut supply} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut 20081121} \colorbox{red!0}{\strut supply} \colorbox{red!0}{\strut daobao} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut 20081121} \colorbox{red!3}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut GPS} \colorbox{red!1}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut china} 
}}}
\end{CJK*}

102:register, 100:gp, 52:how, 44:what, 38:entered, 26:who, 26:registration, 25:work, 25:take, 25:long


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut GMChome} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GMCScotland} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GMCWalesCMC} \colorbox{red!0}{\strut Cymru} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GMCNorthern} \colorbox{red!0}{\strut Ireland} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pressoffice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MyGMC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Freedomofinformation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contactus} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut medical} \colorbox{red!3}{\strut register} \colorbox{red!1}{\strut Registration} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut doctors} \colorbox{red!0}{\strut Concerns} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut doctors} \colorbox{red!0}{\strut Guidance} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut practice} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut Publications} \colorbox{red!0}{\strut Aboutus} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut finding} \colorbox{red!1}{\strut what} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Frequently} \colorbox{red!0}{\strut Asked} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Frequently} \colorbox{red!0}{\strut Asked} \colorbox{red!0}{\strut Questions} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Frequently} \colorbox{red!0}{\strut Asked} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut Background} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Who} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut purpose} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut benefits} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Specialist} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Medical} \colorbox{red!1}{\strut Performers} \colorbox{red!1}{\strut List} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Applying} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut entered} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut do} \colorbox{red!1}{\strut doctors} \colorbox{red!1}{\strut apply} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut entered} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut How} \colorbox{red!1}{\strut long} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut application} \colorbox{red!0}{\strut process} \colorbox{red!1}{\strut take} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut charge} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut entry} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Eligibility} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Register} \colorbox{red!1}{\strut Who} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut entitled} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut entered} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut acquired} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut retired} \colorbox{red!1}{\strut doctors} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut doctors} \colorbox{red!1}{\strut taking} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut break} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut about} \colorbox{red!3}{\strut GP} \colorbox{red!1}{\strut Registrars} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut locums} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut questions} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut T} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut GP} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut indicator} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut entries} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Medical} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut access} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut fact} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut contain} \colorbox{red!3}{\strut GP} \colorbox{red!1}{\strut registrars} \colorbox{red!0}{\strut confusing} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Can} \colorbox{red!1}{\strut doctors} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut still} \colorbox{red!1}{\strut practise} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut managers} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut performers} \colorbox{red!1}{\strut lists} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Background} \colorbox{red!1}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut GP} \colorbox{red!3}{\strut Register} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut register} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut eligible} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut work} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut practice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut apart} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut doctors} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut training} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!3}{\strut GP} \colorbox{red!1}{\strut registrars} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut UK} \colorbox{red!0}{\strut health} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut came} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut effect} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut midnight} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut 31} 
}}}
\end{CJK*}

query: michworks

99:county, 86:calhoun, 73:mi, 60:michigan, 34:marshall, 14:government, 11:site, 9:working, 9:map, 9:green


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Employment} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut Building} \colorbox{red!0}{\strut Building} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Better} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut Through} \colorbox{red!0}{\strut Responsive} \colorbox{red!0}{\strut Leadership} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut details} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut employment} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut latest} \colorbox{red!0}{\strut job} \colorbox{red!0}{\strut openings} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut Human} \colorbox{red!0}{\strut Resources} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut discover} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut job} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut outside} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!1}{\strut Government} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!1}{\strut sites} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Talent} \colorbox{red!0}{\strut Bank} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut MTBEMPL.EntryMainPage} \colorbox{red!0}{\strut Michworks} \colorbox{red!0}{\strut Partner} \colorbox{red!1}{\strut Site} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.michpartners.org} \colorbox{red!0}{\strut CENTS} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut www.centjobs.com} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!1}{\strut Government} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Visiting} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Living} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!1}{\strut Working} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut Departments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Online} \colorbox{red!0}{\strut Reference} \colorbox{red!0}{\strut Desk} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Event} \colorbox{red!0}{\strut Calendar} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Weather} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Map} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut 315} \colorbox{red!0}{\strut West} \colorbox{red!1}{\strut Green} \colorbox{red!0}{\strut Street} \colorbox{red!2}{\strut Marshall} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut MI} \colorbox{red!0}{\strut 49068} \colorbox{red!1}{\strut Phone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 269} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 781-0700} \colorbox{red!0}{\strut Fax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 269} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 781-0140} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut contact} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut webmaster} \colorbox{red!0}{\strut at} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut commentsfeedback} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut website} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut technical} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut website} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut i.e.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut broken} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Several} \colorbox{red!0}{\strut photos} \colorbox{red!0}{\strut included} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut web} \colorbox{red!1}{\strut site} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut courtesy} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Scene} \colorbox{red!0}{\strut Magazine} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut modified} \colorbox{red!0}{\strut 080305} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut 2004} \colorbox{red!6}{\strut Calhoun} \colorbox{red!7}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Michigan} \colorbox{red!0}{\strut DHTML} \colorbox{red!0}{\strut Menu} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Milonic} \colorbox{red!0}{\strut JavaScript} \colorbox{red!1}{\strut Site} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut Policy} \colorbox{red!1}{\strut Site} \colorbox{red!0}{\strut DesignDevelopment} \colorbox{red!0}{\strut by} 
}}}
\end{CJK*}

97:michigan, 75:number, 43:phone, 41:works, 23:association, 21:employer, 20:mwa, 17:michworks, 17:disabilities, 16:name


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut If} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Job} \colorbox{red!0}{\strut Seeker} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut Employer} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut are} \colorbox{red!1}{\strut looking} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!12}{\strut Michigan} \colorbox{red!2}{\strut Talent} \colorbox{red!2}{\strut Bank} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut follow} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.michworks.org} \colorbox{red!0}{\strut If} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut MWA} \colorbox{red!2}{\strut Member} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut Associate} \colorbox{red!2}{\strut Member} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut remove} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut UserName} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Password} \colorbox{red!1}{\strut Boxes} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut boxes} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut meet} \colorbox{red!2}{\strut ADA} \colorbox{red!2}{\strut requirements} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Michigan} \colorbox{red!5}{\strut Works} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Login} \colorbox{red!0}{\strut Use} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut form} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut log} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut site} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut UserName} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Password} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Michigan} \colorbox{red!5}{\strut Works} \colorbox{red!0}{\strut !} \colorbox{red!3}{\strut Association} \colorbox{red!1}{\strut The} \colorbox{red!3}{\strut Association} \colorbox{red!1}{\strut of} \colorbox{red!12}{\strut Michigan} \colorbox{red!5}{\strut Works} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Agencies} \colorbox{red!1}{\strut 2500} \colorbox{red!0}{\strut Kerry} \colorbox{red!1}{\strut Street} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Suite} \colorbox{red!0}{\strut 210} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Lansing} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut MI} \colorbox{red!0}{\strut 48912} \colorbox{red!5}{\strut Phone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 517-371-1100} \colorbox{red!1}{\strut Fax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 517-371-1140} \colorbox{red!0}{\strut e-mail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut info} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut michiganworks.org} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut accordance} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut Americans} \colorbox{red!0}{\strut With} \colorbox{red!2}{\strut Disabilities} \colorbox{red!1}{\strut Act} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ADA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut site} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut alternative} \colorbox{red!0}{\strut format} \colorbox{red!0}{\strut upon} \colorbox{red!1}{\strut request} \colorbox{red!1}{\strut received} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut office} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Michigan} \colorbox{red!2}{\strut Relay} \colorbox{red!9}{\strut number} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut Deaf} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 649-3777} \colorbox{red!1}{\strut The} \colorbox{red!12}{\strut Michigan} \colorbox{red!5}{\strut Works} \colorbox{red!0}{\strut !} \colorbox{red!3}{\strut Association} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut Equal} \colorbox{red!1}{\strut Opportunity} \colorbox{red!0}{\strut EmployerTrainer} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Security} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Disclaimer} \colorbox{red!0}{\strut Statements} 
}}}
\end{CJK*}

query: map united states

84:states, 56:state, 45:map, 44:maps, 34:york, 33:united, 32:city, 31:new, 28:cities, 26:usa


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut About} \colorbox{red!1}{\strut Road} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!1}{\strut Physical} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut USA} \colorbox{red!3}{\strut States} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut Shower} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut Home} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut More} \colorbox{red!2}{\strut maps} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut imagine} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut US} \colorbox{red!2}{\strut Maps} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut State} \colorbox{red!2}{\strut Maps} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Maps} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Europe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mar} \colorbox{red!0}{\strut 31} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut 0} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!1}{\strut City} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut Never} \colorbox{red!0}{\strut Sleeps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut populous} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut largest} \colorbox{red!0}{\strut urban} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut densely} \colorbox{red!1}{\strut populated} \colorbox{red!0}{\strut major} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 8.2} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut residents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut comprised} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut boroughs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Bronx} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Brooklyn} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Manhattan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Queens} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Staten} \colorbox{red!0}{\strut Island} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut visited} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut almost} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut foreign} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut american} \colorbox{red!0}{\strut tourists} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Statue} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Liberty} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut major} \colorbox{red!0}{\strut tourist} \colorbox{red!0}{\strut attraction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut recognizable} \colorbox{red!0}{\strut icons} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Written} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut anniesfamouscookies} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut America} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tags} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut animated} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut individual} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut large} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut America} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut USA} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut us} \colorbox{red!3}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut usa} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut map} \colorbox{red!1}{\strut united} \colorbox{red!3}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mapoftheunitedstates} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut maps} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut maps} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!1}{\strut City} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut physical} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut political} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut religious} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Religious} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut USA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut road} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut standard} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut united} \colorbox{red!3}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut united} \colorbox{red!3}{\strut states} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut united} \colorbox{red!3}{\strut states} \colorbox{red!2}{\strut maps} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut United} \colorbox{red!3}{\strut States} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut America} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut united} \colorbox{red!3}{\strut states} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut america} \colorbox{red!2}{\strut maps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut us} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut usa} \colorbox{red!2}{\strut map} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

87:states, 82:map, 81:america, 78:united, 61:state, 60:what, 43:how, 33:geography, 29:which, 20:swim


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut TEACHING} \colorbox{red!0}{\strut AND} \colorbox{red!1}{\strut LEARNING} \colorbox{red!1}{\strut BEGINNING} \colorbox{red!5}{\strut MAP} \colorbox{red!1}{\strut READING} \colorbox{red!1}{\strut LESSON} \colorbox{red!0}{\strut PLAN} \colorbox{red!1}{\strut BEGINNING} \colorbox{red!1}{\strut TEACHER} \colorbox{red!5}{\strut MAP} \colorbox{red!0}{\strut SKILL} \colorbox{red!1}{\strut LESSON} \colorbox{red!0}{\strut PLAN} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut TEACH} \colorbox{red!1}{\strut ELEMENTARY} \colorbox{red!0}{\strut FREE} \colorbox{red!1}{\strut LESSON} \colorbox{red!5}{\strut UNITED} \colorbox{red!6}{\strut STATES} \colorbox{red!0}{\strut INTRODUCTION} \colorbox{red!1}{\strut TOPOGRAPHICAL} \colorbox{red!1}{\strut US} \colorbox{red!2}{\strut GEOGRAPHY} \colorbox{red!1}{\strut LEARNING} \colorbox{red!0}{\strut THE} \colorbox{red!5}{\strut UNITED} \colorbox{red!6}{\strut STATES} \colorbox{red!5}{\strut MAP} \colorbox{red!0}{\strut Suggested} \colorbox{red!1}{\strut Grade} \colorbox{red!0}{\strut Levels} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Third} \colorbox{red!1}{\strut Grade} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Fourth} \colorbox{red!1}{\strut Grade} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Fifth} \colorbox{red!1}{\strut Grade} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Good} \colorbox{red!1}{\strut lesson} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut ESOL} \colorbox{red!1}{\strut students} \colorbox{red!0}{\strut using} \colorbox{red!1}{\strut TPR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Total} \colorbox{red!1}{\strut Physical} \colorbox{red!1}{\strut Response} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Getting} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Know} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut United} \colorbox{red!6}{\strut States} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut America} \colorbox{red!1}{\strut TPR} \colorbox{red!1}{\strut Commands} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tap} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut Florida} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Swim} \colorbox{red!0}{\strut directly} \colorbox{red!1}{\strut west} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Gulf} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Mexico} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pretend} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut swim} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Trace} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut circle} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut state} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut now} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Trace} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut name} \colorbox{red!1}{\strut Texas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Fly} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut northwest} \colorbox{red!1}{\strut direction} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pretend} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut fly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Land} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut state} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut capital} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Sacramento} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Point} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Walk} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut beach} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!1}{\strut fingers} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut walk} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut shoreline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Look} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut ocean} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pretend} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut glasses} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut look} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut room} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut creature} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Students} \colorbox{red!1}{\strut say} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut creative} \colorbox{red!1}{\strut response} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Dive} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Pacific} \colorbox{red!1}{\strut Ocean} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pretend} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut dive} \colorbox{red!0}{\strut into} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut hands} \colorbox{red!0}{\strut overhead} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Swim} \colorbox{red!0}{\strut north} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pretend} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut swim} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Washington} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!1}{\strut fingers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut step} \colorbox{red!0}{\strut onto} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut shore} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut How} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut feel} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut long} \colorbox{red!1}{\strut swim} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Students} \colorbox{red!1}{\strut say} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut creative} \colorbox{red!1}{\strut response} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 13} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Hike} \colorbox{red!1}{\strut east} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut capital} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Mississippi} \colorbox{red!1}{\strut River} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!1}{\strut fingers} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut walk} \colorbox{red!1}{\strut east} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut map} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: solar panels

99:panels, 99:panel, 97:solar, 67:what, 42:photovoltaic, 37:installed, 37:installation, 36:energy, 32:installer, 32:installations


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut loading} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut italiano} \colorbox{red!0}{\strut english} \colorbox{red!0}{\strut contact} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut Energy} \colorbox{red!1}{\strut Account} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Earn} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut income} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut away} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Energy} \colorbox{red!1}{\strut Account} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut today} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut possible} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut earn} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut producing} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut twenty} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut incentive} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut kwh} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut Solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut transform} \colorbox{red!0}{\strut sunlight} \colorbox{red!0}{\strut into} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut heat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut types} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut photovoltaic} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Photovoltaic} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut mentioned} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut photovoltaic} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut transform} \colorbox{red!3}{\strut solar} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut electricity} \colorbox{red!0}{\strut utilized} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Thermal} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!1}{\strut Thermal} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut replace} \colorbox{red!0}{\strut traditional} \colorbox{red!0}{\strut gas} \colorbox{red!0}{\strut boilers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut allowing} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut heat} \colorbox{red!0}{\strut water} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut home} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Incentives} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut concessions} \colorbox{red!0}{\strut Finally} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut waiting} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Italian} \colorbox{red!0}{\strut citizens} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut financing} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut called} \colorbox{red!1}{\strut Energy} \colorbox{red!1}{\strut Account} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut effective} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Installation} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut costs} \colorbox{red!0}{\strut Depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut location} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut residence} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut installed} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut functioning} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut installation} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Solar} \colorbox{red!0}{\strut panels-} \colorbox{red!1}{\strut photovoltaic} \colorbox{red!0}{\strut panels-} \colorbox{red!0}{\strut water} \colorbox{red!3}{\strut solar} \colorbox{red!0}{\strut panels-} \colorbox{red!1}{\strut photovoltaic} \colorbox{red!3}{\strut solar} \colorbox{red!0}{\strut panels-} \colorbox{red!1}{\strut thermal} \colorbox{red!3}{\strut solar} \colorbox{red!0}{\strut panels-} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panel} \colorbox{red!0}{\strut production-} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panel} \colorbox{red!0}{\strut sales} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut portal} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut established} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fulfil} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut publics} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut photovoltaic} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut understand} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut contact} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut installation} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panel} \colorbox{red!1}{\strut installations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut businesses} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut offering} \colorbox{red!0}{\strut advice} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut planning} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut assembly} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Thermal} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panel} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut able} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut understand} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut photovoltaic} \colorbox{red!3}{\strut panel} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut perhaps} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut able} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut incentives} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut financing} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Thermal} \colorbox{red!3}{\strut solar} \colorbox{red!3}{\strut panels} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut short} 
}}}
\end{CJK*}

97:solars, 97:solar, 91:panels, 90:panel, 50:power, 34:systems, 30:energy, 30:cells, 25:cell, 20:watt


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Solar} \colorbox{red!1}{\strut Energy} \colorbox{red!0}{\strut Publication} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Pros} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cons} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut solar} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut solar} \colorbox{red!4}{\strut panels} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut renewable} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut sustainable} \colorbox{red!2}{\strut power} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut menu} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Home} \colorbox{red!4}{\strut Solar} \colorbox{red!4}{\strut Panels} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Systems} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Subpages} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut Solar} \colorbox{red!4}{\strut Panels} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Systems} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Solar} \colorbox{red!4}{\strut Panels} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Systems} \colorbox{red!0}{\strut Browse} \colorbox{red!4}{\strut solar} \colorbox{red!2}{\strut systems} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut alternative} \colorbox{red!1}{\strut energy} \colorbox{red!1}{\strut solutions} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut GoGreenSolar.com} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut online} \colorbox{red!0}{\strut destination} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut solar} \colorbox{red!4}{\strut panels} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut wind} \colorbox{red!2}{\strut power} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Protect} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut environment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eliminate} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut bills} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut become} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut independent} \colorbox{red!0}{\strut PopShops} \colorbox{red!0}{\strut affiliate} \colorbox{red!0}{\strut stores} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut wind} \colorbox{red!2}{\strut power} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut alternative} \colorbox{red!1}{\strut energy} \colorbox{red!1}{\strut solutions} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut GoGreenSolar.com} \colorbox{red!0}{\strut UniSolar} \colorbox{red!0}{\strut 62} \colorbox{red!1}{\strut Watt} \colorbox{red!0}{\strut Thin} \colorbox{red!0}{\strut Film} \colorbox{red!4}{\strut Solar} \colorbox{red!4}{\strut Panel} \colorbox{red!0}{\strut United} \colorbox{red!4}{\strut Solars} \colorbox{red!0}{\strut proprietary} \colorbox{red!0}{\strut Triple} \colorbox{red!0}{\strut Junction} \colorbox{red!0}{\strut spectrum-splitting} \colorbox{red!0}{\strut amorphous} \colorbox{red!1}{\strut silicon} \colorbox{red!1}{\strut cell} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut achieves} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut performance.These} \colorbox{red!1}{\strut cells} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut constructed} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut separate} \colorbox{red!0}{\strut p-i-n} \colorbox{red!1}{\strut type} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut amorphous} \colorbox{red!0}{\strut semiconductor} \colorbox{red!4}{\strut solar} \colorbox{red!0}{\strut sub-cells} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut different} \colorbox{red!0}{\strut spectral} \colorbox{red!0}{\strut response} \colorbox{red!0}{\strut characteristic} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut allows} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut cell} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut convert} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut different} \colorbox{red!0}{\strut visible} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut near} \colorbox{red!0}{\strut infrared} \colorbox{red!1}{\strut wavelengths} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut sunlight} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut optimal} \colorbox{red!0}{\strut efficiency} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Everlite} \colorbox{red!0}{\strut Compact} \colorbox{red!4}{\strut Solar} \colorbox{red!0}{\strut Spotlight} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut high-tech} \colorbox{red!4}{\strut solar} \colorbox{red!0}{\strut spotlight} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut eight} \colorbox{red!0}{\strut ultra-bright} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 000} \colorbox{red!0}{\strut mcd} \colorbox{red!0}{\strut white} \colorbox{red!1}{\strut LEDs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut built} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut nickel-metal} \colorbox{red!0}{\strut hydride} \colorbox{red!0}{\strut battery} \colorbox{red!0}{\strut pack} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut lightweight} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut pound} \colorbox{red!0}{\strut Everlite} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ideal} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut emergency} \colorbox{red!0}{\strut lighting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut camping} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut outdoor} \colorbox{red!0}{\strut activities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut runs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut charge} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut light} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut sun} \colorbox{red!0}{\strut charging} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut BP} \colorbox{red!4}{\strut Solar} \colorbox{red!0}{\strut BP350J} \colorbox{red!0}{\strut 50W} \colorbox{red!4}{\strut Solar} \colorbox{red!4}{\strut Panel} \colorbox{red!0}{\strut High-efficiency} \colorbox{red!0}{\strut photovoltaic} \colorbox{red!0}{\strut module} \colorbox{red!0}{\strut using} \colorbox{red!1}{\strut silicon} \colorbox{red!0}{\strut nitride} \colorbox{red!0}{\strut multicrystalline} \colorbox{red!1}{\strut silicon} \colorbox{red!1}{\strut cells} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ideal} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut remote} \colorbox{red!0}{\strut telemetry} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut instrumentation} \colorbox{red!2}{\strut systems} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut security} \colorbox{red!0}{\strut sensors} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut land-based} \colorbox{red!0}{\strut aids} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Evergreen} \colorbox{red!0}{\strut ES-190} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 190} \colorbox{red!1}{\strut Watt} \colorbox{red!4}{\strut Solar} \colorbox{red!4}{\strut Panel} \colorbox{red!0}{\strut Evergreen} \colorbox{red!4}{\strut Solar} \colorbox{red!0}{\strut Spruce} \colorbox{red!0}{\strut Line} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut high} \colorbox{red!2}{\strut power} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut state-of-the-art} \colorbox{red!4}{\strut solar} \colorbox{red!4}{\strut panels} \colorbox{red!1}{\strut designed} \colorbox{red!0}{\strut specifically} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut residential} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut commercial} \colorbox{red!0}{\strut applications} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!4}{\strut solar} \colorbox{red!4}{\strut panels} \colorbox{red!0}{\strut offer} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut end-user} \colorbox{red!0}{\strut superior} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut complete} \colorbox{red!0}{\strut peace} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut mind} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut providing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut utmost} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut installation} \colorbox{red!0}{\strut flexibility} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: horse hooves

96:horse, 51:cleaning, 50:clean, 49:cleaned, 48:cleanings, 44:hoof, 35:hooves, 28:good, 27:helps, 27:help


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Topics} \colorbox{red!5}{\strut Horse} \colorbox{red!1}{\strut Care} \colorbox{red!2}{\strut Hoof} \colorbox{red!1}{\strut Care} \colorbox{red!5}{\strut Horse} \colorbox{red!2}{\strut Hoof} \colorbox{red!1}{\strut Care} \colorbox{red!0}{\strut Pointers} \colorbox{red!1}{\strut Making} \colorbox{red!1}{\strut sure} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut has} \colorbox{red!3}{\strut clean} \colorbox{red!2}{\strut hooves} \colorbox{red!1}{\strut helps} \colorbox{red!0}{\strut maintain} \colorbox{red!0}{\strut his} \colorbox{red!1}{\strut health} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut beautiful} \colorbox{red!0}{\strut appearance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut hoof} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut highly} \colorbox{red!0}{\strut specialized} \colorbox{red!0}{\strut horny} \colorbox{red!0}{\strut shell} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut covers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut protects} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sensitive} \colorbox{red!0}{\strut structures} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut foot} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut seem} \colorbox{red!0}{\strut indestructible} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut careful} \colorbox{red!1}{\strut when} \colorbox{red!1}{\strut working} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut hooves} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Hoof} \colorbox{red!1}{\strut Care} \colorbox{red!1}{\strut Helps} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Hindrances} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut help} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut strong} \colorbox{red!2}{\strut hooves} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut old} \colorbox{red!1}{\strut age} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adhering} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut routine} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut good} \colorbox{red!1}{\strut trimming} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut shoeing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Allow} \colorbox{red!0}{\strut you} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut periods} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut barefoot} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut promote} \colorbox{red!2}{\strut hoof} \colorbox{red!1}{\strut health} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Daily} \colorbox{red!2}{\strut cleanings} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut hoof} \colorbox{red!1}{\strut dressings} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut hand} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut improper} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut careless} \colorbox{red!1}{\strut shoeing} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut sure} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut harm} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut hooves} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut insufficient} \colorbox{red!1}{\strut exercise} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut poor} \colorbox{red!0}{\strut nutrition} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dryness} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut hoof} \colorbox{red!0}{\strut wall} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut poor} \colorbox{red!2}{\strut hoof} \colorbox{red!1}{\strut health} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Why} \colorbox{red!3}{\strut Clean} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut Horse} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Hooves} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Keeping} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut hooves} \colorbox{red!3}{\strut clean} \colorbox{red!1}{\strut keeps} \colorbox{red!0}{\strut them} \colorbox{red!1}{\strut healthy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut hoof} \colorbox{red!1}{\strut pick} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut remove} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut buildup} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut dirt} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut debris} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Long-term} \colorbox{red!0}{\strut exposure} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut bacteria} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut eventually} \colorbox{red!0}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut infections} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stones} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut collect} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut hooves} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut cause} \colorbox{red!0}{\strut bruising} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Hoof} \colorbox{red!1}{\strut Picking} \colorbox{red!0}{\strut Tips} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut basics} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut horse} \colorbox{red!2}{\strut hoof} \colorbox{red!1}{\strut care} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut cleaning} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Be} \colorbox{red!0}{\strut patient} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut calm} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut gentle} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut his} \colorbox{red!2}{\strut hooves} \colorbox{red!2}{\strut cleaned} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Always} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut pick} \colorbox{red!0}{\strut towards} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut toe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut front} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut hoof} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pulling} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut pick} \colorbox{red!0}{\strut towards} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut allow} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut pick} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut caught} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut frog} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut hurt} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut quick} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut lose} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut confidence} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pick} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut hooves} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut each} \colorbox{red!1}{\strut ride} 
}}}
\end{CJK*}

93:hooves, 92:horses, 91:horse, 91:dancing, 86:stable, 49:owned, 42:jackson, 40:county, 32:brandon, 30:located


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Dancing} \colorbox{red!9}{\strut Hooves} \colorbox{red!9}{\strut Stable} \colorbox{red!0}{\strut .com} \colorbox{red!9}{\strut Horse} \colorbox{red!9}{\strut Stable} \colorbox{red!1}{\strut Accommodations} \colorbox{red!0}{\strut Great} \colorbox{red!1}{\strut Company} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut 4} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!1}{\strut Listen} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut great} \colorbox{red!1}{\strut Christian} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Brandon} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut Mississippi} \colorbox{red!1}{\strut area} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 100.9} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut 93.5} \colorbox{red!0}{\strut FM} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 601} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 940-1818} \colorbox{red!5}{\strut Owned} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Operated} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Dawn} \colorbox{red!1}{\strut Clarke} \colorbox{red!0}{\strut 1575} \colorbox{red!1}{\strut Carsley} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Jackson} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut MS} \colorbox{red!0}{\strut 39209} \colorbox{red!9}{\strut Dancing} \colorbox{red!9}{\strut Hooves} \colorbox{red!9}{\strut Stable} \colorbox{red!0}{\strut offers} \colorbox{red!1}{\strut Haven} \colorbox{red!0}{\strut for} \colorbox{red!9}{\strut Horses} \colorbox{red!2}{\strut Who} \colorbox{red!0}{\strut Are} \colorbox{red!1}{\strut Retired} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut Recuperating} \colorbox{red!9}{\strut Dancing} \colorbox{red!9}{\strut Hooves} \colorbox{red!9}{\strut Stable} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut paradise} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut green} \colorbox{red!1}{\strut grass} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut shade} \colorbox{red!1}{\strut trees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut loving} \colorbox{red!1}{\strut care} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut located} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut 35.5} \colorbox{red!1}{\strut acres} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut North} \colorbox{red!1}{\strut Hinds} \colorbox{red!4}{\strut County} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut Jackson} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut MS} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!9}{\strut horses} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut given} \colorbox{red!1}{\strut care} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut individual} \colorbox{red!1}{\strut need} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut unique} \colorbox{red!0}{\strut personality} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Care} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut consistent} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut provided} \colorbox{red!0}{\strut 247} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 365} \colorbox{red!1}{\strut days} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut year} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut your} \colorbox{red!9}{\strut horse} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut attention} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut regular} \colorbox{red!1}{\strut care} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut available} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

query: discovery channel store

63:uncover, 58:discovery, 50:found, 48:find, 42:gift, 39:gifts, 27:ideas, 23:meanings, 21:store, 21:channel


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Giving} \colorbox{red!0}{\strut Made} \colorbox{red!0}{\strut Easy} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Dedicated} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut helping} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut find} \colorbox{red!0}{\strut creative} \colorbox{red!2}{\strut gift} \colorbox{red!1}{\strut ideas} \colorbox{red!0}{\strut Personalize} \colorbox{red!0}{\strut FindGift.com} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Overview} \colorbox{red!1}{\strut Looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut gift} \colorbox{red!1}{\strut registry} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Top} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Ideas} \colorbox{red!0}{\strut Saved} \colorbox{red!2}{\strut Gifts} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Registry} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Shops} \colorbox{red!0}{\strut Email} \colorbox{red!2}{\strut Gifts} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Shops} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Ideas} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Biology} \colorbox{red!0}{\strut undo} \colorbox{red!0}{\strut All} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Ideas} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut viewing} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 14} \colorbox{red!2}{\strut gift} \colorbox{red!1}{\strut ideas} \colorbox{red!2}{\strut found} \colorbox{red!3}{\strut Uncover} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Human} \colorbox{red!1}{\strut Body} \colorbox{red!1}{\strut Book} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 18.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Botanicals} \colorbox{red!0}{\strut Exotic} \colorbox{red!0}{\strut Jungle} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 29.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Critter} \colorbox{red!0}{\strut Projector} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Turbo} \colorbox{red!0}{\strut Critter} \colorbox{red!0}{\strut Catcher} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!1}{\strut Spark} \colorbox{red!0}{\strut Talking} \colorbox{red!1}{\strut Microscope} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 24.47} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Genetics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DNA} \colorbox{red!0}{\strut Kit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 34.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!3}{\strut Discovery} \colorbox{red!0}{\strut Macro} \colorbox{red!1}{\strut Microscope} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 79.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut SparkTalking} \colorbox{red!0}{\strut Bug} \colorbox{red!0}{\strut Identifier} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Antlantis} \colorbox{red!1}{\strut Island} \colorbox{red!0}{\strut Adventure} \colorbox{red!0}{\strut Habitat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 29.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Dissect} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Frog} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 24.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Praying} \colorbox{red!0}{\strut Mantis} \colorbox{red!0}{\strut Encounter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 13.97} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Frog} \colorbox{red!0}{\strut Pond} \colorbox{red!0}{\strut Habitat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 22.99} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!3}{\strut Discovery} \colorbox{red!0}{\strut Whodunit} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Forensics} \colorbox{red!0}{\strut Lab} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 79.95} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Evolution} \colorbox{red!0}{\strut Game} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 24.99} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Discovery} \colorbox{red!1}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut viewing} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 14} \colorbox{red!2}{\strut gift} \colorbox{red!1}{\strut ideas} \colorbox{red!2}{\strut found} \colorbox{red!0}{\strut 29} \colorbox{red!0}{\strut Days} \colorbox{red!0}{\strut Until} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Valentine} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Day} \colorbox{red!0}{\strut Feb} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Valentine} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Day} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Ideas} \colorbox{red!0}{\strut Upcoming} \colorbox{red!0}{\strut Holidays} \colorbox{red!0}{\strut Super} \colorbox{red!0}{\strut Bowl} \colorbox{red!0}{\strut Feb} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Academy} \colorbox{red!0}{\strut Awards} \colorbox{red!0}{\strut Feb} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut Mardi} \colorbox{red!0}{\strut Gras} \colorbox{red!0}{\strut Feb} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Seasonal} \colorbox{red!2}{\strut Gifts} \colorbox{red!0}{\strut Anniversary} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Ideas} \colorbox{red!0}{\strut Birthday} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Ideas} \colorbox{red!0}{\strut Winter} \colorbox{red!0}{\strut Theme} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut Top} \colorbox{red!2}{\strut Gift} \colorbox{red!1}{\strut Ideas} \colorbox{red!2}{\strut Gift} \colorbox{red!0}{\strut Helpers} \colorbox{red!0}{\strut Anniversary} \colorbox{red!2}{\strut Gifts} \colorbox{red!0}{\strut Table} \colorbox{red!0}{\strut Flower} \colorbox{red!1}{\strut Meanings} \colorbox{red!0}{\strut Monthly} \colorbox{red!0}{\strut Flowers} \colorbox{red!0}{\strut Monthly} \colorbox{red!0}{\strut Birthstones} \colorbox{red!0}{\strut Signs} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Zodiac} \colorbox{red!0}{\strut Additional} \colorbox{red!0}{\strut Resources} \colorbox{red!2}{\strut Find} \colorbox{red!0}{\strut unique} \colorbox{red!2}{\strut gift} \colorbox{red!1}{\strut ideas} 
}}}
\end{CJK*}

99:discovery, 98:channel, 68:cash, 47:what, 43:ebates, 35:back, 29:stores, 27:store, 24:rebates, 23:coupons


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut --} \colorbox{red!0}{\strut Select} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut store} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Ebates} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut saving} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Members} \colorbox{red!0}{\strut Log} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Stores} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut My} \colorbox{red!2}{\strut Ebates} \colorbox{red!0}{\strut Tell-A-Friend} \colorbox{red!0}{\strut Blog} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut receive} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut sales} \colorbox{red!0}{\strut commission} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut stores} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut buy} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut pass} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut portion} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut commission} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut Ebates} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut four} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut forms} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fill} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut Ebates} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut buy} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut earn} \colorbox{red!3}{\strut cash} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!1}{\strut coupon} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DESCRIPTION} \colorbox{red!1}{\strut COUPONS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SPECIALS} \colorbox{red!0}{\strut DESCRIPTION} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut leading} \colorbox{red!0}{\strut destination} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut educational} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut carries} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut complete} \colorbox{red!0}{\strut inventory} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut books} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut dvds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut health} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fitness} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut toys} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut games} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut deals} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!1}{\strut coupons} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut specials} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut sales} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!1}{\strut coupon} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut promo} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut offer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut simply} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut shopping} \colorbox{red!0}{\strut cart} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut redeem} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut COUPONS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SPECIALS} \colorbox{red!0}{\strut SAVE} \colorbox{red!0}{\strut AT} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!1}{\strut Rebates} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Receive} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Use} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!1}{\strut coupons} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut Discounts} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut latest} \colorbox{red!4}{\strut Discovery} \colorbox{red!4}{\strut Channel} \colorbox{red!1}{\strut Store} \colorbox{red!0}{\strut discounts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut deals} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Appliances} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Hardware} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut stores} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut category} \colorbox{red!0}{\strut Sears} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Depot} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Compact} \colorbox{red!0}{\strut Appliance} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Ace} \colorbox{red!0}{\strut Hardware} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Target} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Baby} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Kids} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut stores} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut category} \colorbox{red!0}{\strut Diapers.com} 
}}}
\end{CJK*}

query: ct jobs

88:ct, 66:lyme, 22:jobs, 16:job, 15:city, 14:cities, 11:located, 9:why, 9:sprague, 9:point


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut help} \colorbox{red!0}{\strut post} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut get} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut alerts} \colorbox{red!0}{\strut search} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Create} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut profile} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut employers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Already} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut sign} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut why} \colorbox{red!0}{\strut register} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut get} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut alerts} \colorbox{red!0}{\strut Refine} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut Posted} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut Located} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut Sort} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Best} \colorbox{red!0}{\strut match} \colorbox{red!0}{\strut Date} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Distance} \colorbox{red!1}{\strut Cities} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Baltic} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Borough} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Bozrah} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Canterbury} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut Groton} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Chesterfield} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Colchester} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut East} \colorbox{red!2}{\strut Lyme} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Exeter} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Fitchville} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Fort} \colorbox{red!0}{\strut Trumbull} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Franklin} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Franklin} \colorbox{red!0}{\strut Hill} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Gales} \colorbox{red!0}{\strut Ferry} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Gilman} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Griswold} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Groton} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Groton} \colorbox{red!0}{\strut Long} \colorbox{red!0}{\strut Point} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Hadlyme} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Hamburg} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Hanover} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Hopeville} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Jewett} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Jordan} \colorbox{red!0}{\strut Village} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Jupiter} \colorbox{red!0}{\strut Point} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Lebanon} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Ledyard} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Lisbon} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Lords} \colorbox{red!0}{\strut Point} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Lyme} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Mashantucket} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Masons} \colorbox{red!0}{\strut Island} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Millstone} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Montville} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Mystic} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Naval} \colorbox{red!0}{\strut Submarine} \colorbox{red!0}{\strut Base} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut London} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Niantic} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Noank} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Franklin} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut CT} \colorbox{red!1}{\strut Jobs} 
}}}
\end{CJK*}

100:jobs, 98:ct, 97:job, 30:hiring, 27:employment, 26:why, 19:career, 17:careers, 16:openings, 15:salary


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Help} \colorbox{red!1}{\strut Home} \colorbox{red!6}{\strut CT} \colorbox{red!6}{\strut Job} \colorbox{red!1}{\strut Search} \colorbox{red!6}{\strut Job} \colorbox{red!1}{\strut Seekers} \colorbox{red!1}{\strut Career} \colorbox{red!1}{\strut Central} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!1}{\strut Advertising} \colorbox{red!1}{\strut Employers} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Regular} \colorbox{red!6}{\strut Job} \colorbox{red!1}{\strut Openings} \colorbox{red!0}{\strut 170} \colorbox{red!1}{\strut Temp} \colorbox{red!6}{\strut Job} \colorbox{red!0}{\strut Openings2} \colorbox{red!0}{\strut Companies659} \colorbox{red!0}{\strut Resumes8906} \colorbox{red!0}{\strut Advanced} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut CategoryCity} \colorbox{red!1}{\strut New} \colorbox{red!6}{\strut Jobs} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut Temp} \colorbox{red!6}{\strut Jobs} \colorbox{red!0}{\strut Seasonal} \colorbox{red!6}{\strut Jobs} \colorbox{red!1}{\strut Company} \colorbox{red!1}{\strut Profiles} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Register} \colorbox{red!2}{\strut Why} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut PostEdit} \colorbox{red!1}{\strut Resume} \colorbox{red!1}{\strut Career} \colorbox{red!0}{\strut Agent} \colorbox{red!1}{\strut Career} \colorbox{red!1}{\strut Central} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Career} \colorbox{red!0}{\strut Advice} \colorbox{red!0}{\strut Articles} \colorbox{red!1}{\strut Career} \colorbox{red!0}{\strut Events} \colorbox{red!1}{\strut Salary} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut Links} \colorbox{red!1}{\strut Career} \colorbox{red!0}{\strut Connection} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!0}{\strut Join} \colorbox{red!0}{\strut Our} \colorbox{red!0}{\strut Team} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Statement} \colorbox{red!0}{\strut Acceptable} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut Banner} \colorbox{red!1}{\strut Advertising} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Register} \colorbox{red!2}{\strut Why} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Products} \colorbox{red!1}{\strut Rate} \colorbox{red!0}{\strut Card} \colorbox{red!0}{\strut Competitive} \colorbox{red!1}{\strut Salary} \colorbox{red!0}{\strut Reports} \colorbox{red!0}{\strut Testimonials} \colorbox{red!0}{\strut HR} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut B2B} \colorbox{red!0}{\strut Events} \colorbox{red!0}{\strut JiUS} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut Username} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Password} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Remember} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut Forgot} \colorbox{red!0}{\strut password} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut ?} \colorbox{red!6}{\strut Job} \colorbox{red!1}{\strut Seeker} \colorbox{red!0}{\strut Resources} \colorbox{red!0}{\strut Featured} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Donts} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Today} \colorbox{red!0}{\strut s} \colorbox{red!6}{\strut Job} \colorbox{red!1}{\strut Seeker} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut today} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut tough} \colorbox{red!6}{\strut job} \colorbox{red!0}{\strut market} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut differentiate} \colorbox{red!0}{\strut yourself} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut competition} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut plum} \colorbox{red!6}{\strut job} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Bright} \colorbox{red!0}{\strut Spots} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Becoming} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut RN} \colorbox{red!0}{\strut Switching} \colorbox{red!1}{\strut careers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut registered} \colorbox{red!0}{\strut nurse} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut easy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut worth} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Career} \colorbox{red!0}{\strut Connection} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut Now} \colorbox{red!2}{\strut Hiring} \colorbox{red!1}{\strut Advertising} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut mission} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut help} \colorbox{red!6}{\strut job} \colorbox{red!1}{\strut seekers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut local} \colorbox{red!1}{\strut Connecticut} \colorbox{red!2}{\strut employment} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut careers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut job} \colorbox{red!1}{\strut listings} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut careers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut employment} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut conveniently} \colorbox{red!0}{\strut organized} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut facilitate} \colorbox{red!6}{\strut job} \colorbox{red!1}{\strut seeker} \colorbox{red!1}{\strut searches} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!0}{\strut offers} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut latest} \colorbox{red!1}{\strut career} \colorbox{red!0}{\strut advice} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut resume} \colorbox{red!0}{\strut posting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut automated} \colorbox{red!1}{\strut career} \colorbox{red!0}{\strut agents} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut meet} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Connecticut} \colorbox{red!6}{\strut job} \colorbox{red!1}{\strut seekers} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SearchJobs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut New} \colorbox{red!6}{\strut Jobs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CompanyProfiles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CareerCentral} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RegisterLogin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SiteMap} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ContactJobsInCT.com} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Employers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Testimonials} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Advertise} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Banner} \colorbox{red!1}{\strut Advertising} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2009JobsInTheUS.com} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut reserved} \colorbox{red!0}{\strut Acceptable} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Statement} \colorbox{red!0}{\strut Other} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut serve} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut JobsInAL.com} 
}}}
\end{CJK*}

query: texas border patrol

87:aguilar, 81:border, 77:patrol, 46:chief, 38:david, 32:agents, 30:agent, 19:v, 17:states, 17:ranking


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut David} \colorbox{red!0}{\strut V.} \colorbox{red!4}{\strut Aguilar} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut citations} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut verification} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut improve} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut reliable} \colorbox{red!0}{\strut references} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Unsourced} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut challenged} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut removed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut David} \colorbox{red!0}{\strut V.} \colorbox{red!4}{\strut Aguilar} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Chief} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Agent} \colorbox{red!2}{\strut David} \colorbox{red!0}{\strut V.} \colorbox{red!4}{\strut Aguilar} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Chief} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut having} \colorbox{red!1}{\strut assumed} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut position} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2004} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nation} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut highest} \colorbox{red!1}{\strut ranking} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut agent} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Chief} \colorbox{red!4}{\strut Aguilar} \colorbox{red!0}{\strut directs} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut enforcement} \colorbox{red!0}{\strut efforts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 18,000} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!2}{\strut Agents} \colorbox{red!0}{\strut nationwide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut 2} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Accolades} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Dissatisfaction} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Subordinates} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Education} \colorbox{red!4}{\strut Aguilar} \colorbox{red!0}{\strut received} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Associates} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Accounting} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Laredo} \colorbox{red!0}{\strut Junior} \colorbox{red!0}{\strut College} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut attended} \colorbox{red!0}{\strut Laredo} \colorbox{red!0}{\strut State} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Texas} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Arlington} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut graduate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut F.} \colorbox{red!0}{\strut Kennedy} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Government} \colorbox{red!0}{\strut Harvard} \colorbox{red!0}{\strut Senior} \colorbox{red!0}{\strut Executive} \colorbox{red!0}{\strut Fellows} \colorbox{red!0}{\strut Spring} \colorbox{red!0}{\strut Class} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1999} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!0}{\strut experience} \colorbox{red!4}{\strut Aguilar} \colorbox{red!0}{\strut entered} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut duty} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut June} \colorbox{red!0}{\strut 1978} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut His} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut station} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Laredo} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Texas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut Laredo} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut served} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut positions} \colorbox{red!0}{\strut including} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Agent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut Supervisory} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Agent} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Assistant} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Agent} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Charge} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Aguilar} \colorbox{red!0}{\strut served} \colorbox{red!0}{\strut as} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Agent} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Charge} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut different} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Stations} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Texas} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 1988} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 1996} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut promoted} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Agent} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Charge} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Dallas} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Station} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 1988} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut promoted} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Rio} \colorbox{red!0}{\strut Grande} \colorbox{red!1}{\strut City} \colorbox{red!4}{\strut Border} \colorbox{red!4}{\strut Patrol} \colorbox{red!1}{\strut Station} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1992} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Rio} \colorbox{red!0}{\strut Grande} \colorbox{red!1}{\strut City} \colorbox{red!1}{\strut Station} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut active} \colorbox{red!1}{\strut stations} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut narcotics} \colorbox{red!0}{\strut interdiction} \colorbox{red!0}{\strut along} 
}}}
\end{CJK*}

92:border, 91:patrol, 91:borders, 46:who, 34:prison, 32:sentences, 25:texas, 24:free, 24:agents, 22:smuggler


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sign-up} \colorbox{red!0}{\strut Logout} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Edit} \colorbox{red!0}{\strut Profile} \colorbox{red!1}{\strut Immigration} \colorbox{red!0}{\strut Chronicles} \colorbox{red!0}{\strut Blogging} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Chronicle} \colorbox{red!0}{\strut staff} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut permit} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut hire} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut undocumented} \colorbox{red!1}{\strut worker} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Where} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut fence} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut More} \colorbox{red!1}{\strut calls} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut free} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut Border} \colorbox{red!6}{\strut Patrol} \colorbox{red!1}{\strut Two} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut White} \colorbox{red!1}{\strut House} \colorbox{red!1}{\strut fax} \colorbox{red!1}{\strut machine} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut working} \colorbox{red!1}{\strut overtime} \colorbox{red!0}{\strut cranking} \colorbox{red!0}{\strut out} \colorbox{red!1}{\strut letters} \colorbox{red!1}{\strut demanding} \colorbox{red!1}{\strut clemency} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut two} \colorbox{red!6}{\strut Border} \colorbox{red!6}{\strut Patrol} \colorbox{red!2}{\strut agents} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut Texas} \colorbox{red!1}{\strut imprisoned} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut shooting} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut fleeing} \colorbox{red!1}{\strut Mexican} \colorbox{red!1}{\strut drug} \colorbox{red!1}{\strut smuggler} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut latest} \colorbox{red!1}{\strut entry} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Rep.} \colorbox{red!1}{\strut John} \colorbox{red!1}{\strut Culberson} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R-Houston} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut House} \colorbox{red!0}{\strut colleagues} \colorbox{red!3}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut asking} \colorbox{red!1}{\strut President} \colorbox{red!1}{\strut Bush} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut commute} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ex-agents} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut prison} \colorbox{red!2}{\strut sentences} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Ignacio} \colorbox{red!1}{\strut Ramos} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Jose} \colorbox{red!1}{\strut Compean} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut began} \colorbox{red!1}{\strut serving} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut respective} \colorbox{red!0}{\strut 11-} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 12-year} \colorbox{red!2}{\strut sentences} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut wounding} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut smuggler} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut concealing} \colorbox{red!0}{\strut evidence} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut February} \colorbox{red!0}{\strut 2005} \colorbox{red!1}{\strut shooting} \colorbox{red!0}{\strut outside} \colorbox{red!1}{\strut El} \colorbox{red!1}{\strut Paso} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut letter} \colorbox{red!0}{\strut today} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Bush} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lawmakers} \colorbox{red!0}{\strut wrote} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut extremely} \colorbox{red!1}{\strut harsh} \colorbox{red!2}{\strut prison} \colorbox{red!2}{\strut sentences} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut received} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut unjustified} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut case} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut prosecution} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut prison} \colorbox{red!2}{\strut sentences} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut demoralizing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut other} \colorbox{red!6}{\strut Border} \colorbox{red!6}{\strut Patrol} \colorbox{red!2}{\strut agents} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut undoubtedly} \colorbox{red!0}{\strut harmed} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut security} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut nation} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut causing} \colorbox{red!6}{\strut Border} \colorbox{red!6}{\strut Patrol} \colorbox{red!2}{\strut agents} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut hesitate} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut weapons} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut defense} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut our} \colorbox{red!6}{\strut borders} \colorbox{red!0}{\strut against} \colorbox{red!1}{\strut criminals} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut terrorists} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Texans} \colorbox{red!1}{\strut signing} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut letter} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut Reps.} \colorbox{red!0}{\strut Ted} \colorbox{red!1}{\strut Poe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R-Humble} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louie} \colorbox{red!0}{\strut Gohmert} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R-Tyler} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Michael} \colorbox{red!0}{\strut McCaul} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R-Austin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Kay} \colorbox{red!0}{\strut Granger} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R-Fort} \colorbox{red!0}{\strut Worth} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut John} \colorbox{red!0}{\strut Carter} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R-Round} \colorbox{red!0}{\strut Rock} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Sens} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut John} \colorbox{red!0}{\strut Cornyn} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R-Texas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Dianne} \colorbox{red!0}{\strut Feinstein} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut D-Calif.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut week} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut requested} \colorbox{red!1}{\strut clemency} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ex-agents} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut congressman} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Rep.} \colorbox{red!1}{\strut Silvestre} \colorbox{red!1}{\strut Reyes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut D-El} \colorbox{red!1}{\strut Paso} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut added} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut voice} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut chorus} \colorbox{red!0}{\strut --} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut particularly} \colorbox{red!0}{\strut significant} \colorbox{red!0}{\strut because} \colorbox{red!1}{\strut Reyes} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut former} \colorbox{red!6}{\strut Border} \colorbox{red!6}{\strut Patrol} \colorbox{red!1}{\strut supervisor} \colorbox{red!3}{\strut who} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut largely} 
}}}
\end{CJK*}

query: pvc

92:pipe, 85:pvc, 40:sewer, 34:water, 21:installation, 20:requirements, 19:temperature, 19:dwv, 17:burial, 16:pw


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut PW} \colorbox{red!1}{\strut Eagle} \colorbox{red!0}{\strut Home} \colorbox{red!1}{\strut Support} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut FAQ} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Tech} \colorbox{red!1}{\strut Support} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Technical} \colorbox{red!0}{\strut Bulletins} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Depth} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Burial} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Print} \colorbox{red!1}{\strut Line} \colorbox{red!1}{\strut Requirements} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Nonmetallic} \colorbox{red!1}{\strut Conduit} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Utility} \colorbox{red!1}{\strut Duct} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Max} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bell} \colorbox{red!0}{\strut OS} \colorbox{red!0}{\strut Diameter} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Effects} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Temperature} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut VacuumExternal} \colorbox{red!1}{\strut Pressure} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Support} \colorbox{red!1}{\strut Spacing} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Longitudinal} \colorbox{red!1}{\strut Bending} \colorbox{red!5}{\strut PVC} \colorbox{red!2}{\strut Sewer} \colorbox{red!5}{\strut Pipe} \colorbox{red!1}{\strut Burial} \colorbox{red!1}{\strut Depths} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut 1428} \colorbox{red!1}{\strut Storm} \colorbox{red!1}{\strut Drain} \colorbox{red!1}{\strut Burial} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut AWWA} \colorbox{red!0}{\strut C900} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut C905} \colorbox{red!1}{\strut Burial} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Effects} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Sunlight} \colorbox{red!5}{\strut PVC} \colorbox{red!5}{\strut Pipe} \colorbox{red!1}{\strut Trench} \colorbox{red!1}{\strut Construction} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Air} \colorbox{red!1}{\strut testing} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut DWV} \colorbox{red!5}{\strut Pipe} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Gasketed} \colorbox{red!5}{\strut Pipe} \colorbox{red!1}{\strut Assembly} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Print} \colorbox{red!1}{\strut Line} \colorbox{red!1}{\strut Requirements} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut WaterSewer} \colorbox{red!5}{\strut PVC} \colorbox{red!5}{\strut Pipe} \colorbox{red!1}{\strut Compound} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Fire} \colorbox{red!1}{\strut Protection} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Firestop} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Material} \colorbox{red!0}{\strut Safety} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut Sheet} \colorbox{red!1}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut top} \colorbox{red!1}{\strut Installation} \colorbox{red!0}{\strut Guides} \colorbox{red!1}{\strut Installation} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut PVC} \colorbox{red!2}{\strut Sewer} \colorbox{red!5}{\strut Pipe} \colorbox{red!1}{\strut Installation} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut PVC} \colorbox{red!2}{\strut Water} \colorbox{red!5}{\strut Pipe} \colorbox{red!1}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut top} \colorbox{red!1}{\strut Misc} \colorbox{red!0}{\strut Limited} \colorbox{red!0}{\strut Warranty} \colorbox{red!0}{\strut Metric} \colorbox{red!0}{\strut Sizes} \colorbox{red!1}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut Search} \colorbox{red!1}{\strut Support} \colorbox{red!0}{\strut 2004} \colorbox{red!1}{\strut PW} \colorbox{red!1}{\strut Eagle} \colorbox{red!0}{\strut Inc} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

92:pvc, 89:pvcs, 37:poison, 36:banned, 35:plastic, 33:phthalates, 33:ban, 32:bans, 24:restrictions, 21:toys


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Poison} \colorbox{red!2}{\strut Plastic} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Video} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sam} \colorbox{red!0}{\strut Suds} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Case} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Poison} \colorbox{red!2}{\strut Plastic} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Products} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut Near} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Plants} \colorbox{red!0}{\strut Companies} \colorbox{red!0}{\strut with} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Products} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Company} \colorbox{red!1}{\strut Policies} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Governmental} \colorbox{red!1}{\strut Policies} \colorbox{red!0}{\strut Reports} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Hazards} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut About} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Governmental} \colorbox{red!1}{\strut Policies} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Governmental} \colorbox{red!1}{\strut Policies} \colorbox{red!0}{\strut Around} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut World} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut response} \colorbox{red!0}{\strut to} \colorbox{red!5}{\strut PVCs} \colorbox{red!1}{\strut toxic} \colorbox{red!0}{\strut threats} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut governments} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut world} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut passed} \colorbox{red!0}{\strut sweeping} \colorbox{red!1}{\strut policies} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut phase} \colorbox{red!0}{\strut out} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut switch} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut safer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut healthier} \colorbox{red!1}{\strut consumer} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Weve} \colorbox{red!0}{\strut highlighted} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut PVC-free} \colorbox{red!1}{\strut policies} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut included} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut in-depth} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut PVC-free} \colorbox{red!0}{\strut governmental} \colorbox{red!1}{\strut policies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Nationwide} \colorbox{red!2}{\strut Bans} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut Sweden} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut proposed} \colorbox{red!1}{\strut restrictions} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1995} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut working} \colorbox{red!0}{\strut toward} \colorbox{red!0}{\strut discontinuing} \colorbox{red!0}{\strut all} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut uses} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Spain} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 60} \colorbox{red!1}{\strut cities} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut declared} \colorbox{red!0}{\strut PVC-free} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Germany} \colorbox{red!0}{\strut has} \colorbox{red!2}{\strut banned} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut disposal} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut landfills} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2005} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut minimizing} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut incineration} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut encouraging} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut phaseout} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut easily} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut recycled} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Since} \colorbox{red!0}{\strut 1986} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 274} \colorbox{red!0}{\strut communities} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Germany} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut enacted} \colorbox{red!1}{\strut restrictions} \colorbox{red!0}{\strut against} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Restrictions} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut Childrens} \colorbox{red!1}{\strut Toys} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Baby} \colorbox{red!1}{\strut Products} \colorbox{red!1}{\strut Restrictions} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut bans} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut placed} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut phthalates} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut toys} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut entire} \colorbox{red!0}{\strut European} \colorbox{red!0}{\strut Union} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Austria} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Denmark} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Finland} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut France} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Germany} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Greece} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Italy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Japan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Iceland} \colorbox{red!0}{\strut Mexico} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Norway} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Sweden} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 1998} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut Consumer} \colorbox{red!1}{\strut Product} \colorbox{red!0}{\strut Safety} \colorbox{red!0}{\strut Commission} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CPSC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut reached} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut voluntary} \colorbox{red!0}{\strut agreement} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut manufacturers} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut remove} \colorbox{red!0}{\strut two} \colorbox{red!2}{\strut phthalates} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut PVC} \colorbox{red!0}{\strut rattles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut teethers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pacifiers} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut baby} \colorbox{red!0}{\strut bottle} \colorbox{red!0}{\strut nipples} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Despite} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut phthalates} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut still} \colorbox{red!0}{\strut commonly} \colorbox{red!0}{\strut added} \colorbox{red!0}{\strut to} \colorbox{red!5}{\strut PVC} \colorbox{red!1}{\strut childrens} \colorbox{red!1}{\strut toys} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut baby} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Francisco} \colorbox{red!0}{\strut became} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut in} 
}}}
\end{CJK*}

query: raised gardens

98:beds, 97:raised, 96:bed, 71:what, 43:gardens, 43:garden, 41:gardening, 38:how, 31:gardeners, 30:soil


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Organic} \colorbox{red!1}{\strut Gardening} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Garden} \colorbox{red!0}{\strut Organic} \colorbox{red!1}{\strut Gardening} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Organic} \colorbox{red!1}{\strut Gardening} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Organic} \colorbox{red!1}{\strut Gardening} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut Forum} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Beds} \colorbox{red!1}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Make} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Bed} \colorbox{red!1}{\strut Garden} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Colleen} \colorbox{red!0}{\strut Vanderlinden} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut About.com} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut garden} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut bed} \colorbox{red!1}{\strut garden} \colorbox{red!1}{\strut garden} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut garden} \colorbox{red!1}{\strut gardening} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Bed} \colorbox{red!1}{\strut Vegetable} \colorbox{red!1}{\strut Gardens} \colorbox{red!0}{\strut Colleen} \colorbox{red!0}{\strut Vanderlinden} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut bed} \colorbox{red!1}{\strut gardens} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut saviors} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut gardeners} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut poor} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut everywhere} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut basic} \colorbox{red!0}{\strut idea} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut bed} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut instead} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut battling} \colorbox{red!0}{\strut against} \colorbox{red!0}{\strut poor} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut build} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut ground} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut absolute} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut texture} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ingredients} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Bed} \colorbox{red!1}{\strut Garden} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut bed} \colorbox{red!1}{\strut garden} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut garden} \colorbox{red!0}{\strut built} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut native} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut incorporating} \colorbox{red!0}{\strut native} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut bed} \colorbox{red!1}{\strut gardens} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut contained} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut build} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut wood} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut stone} \colorbox{red!0}{\strut structure} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut bed} \colorbox{red!0}{\strut intact} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut amendments} \colorbox{red!0}{\strut merely} \colorbox{red!0}{\strut piled} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut inches} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut plant} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut herbs} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut vegetables} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut perennials} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut shrubs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut bed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Advantages} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Bed} \colorbox{red!1}{\strut Garden} \colorbox{red!0}{\strut Aside} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut avoiding} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut gardening} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut poor} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut bed} \colorbox{red!1}{\strut gardens} \colorbox{red!0}{\strut offer} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut advantages} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut warm} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut quickly} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut spring} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut allowing} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut plant} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut drain} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut compacted} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut constructed} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut accessibility} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut mind} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut easy} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut tailor} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut soil} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut bed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut plants} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut grow} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut initial} \colorbox{red!0}{\strut construction} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut require} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut maintenance} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut conventional} \colorbox{red!1}{\strut garden} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Make} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Raised} 
}}}
\end{CJK*}

97:garden, 95:raised, 94:raising, 94:gardens, 86:gardening, 76:beds, 69:bed, 39:gardeners, 38:why, 32:gardener


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut No} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Shopping} \colorbox{red!0}{\strut Cart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Product} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Compost} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut Compost} \colorbox{red!0}{\strut Bins} \colorbox{red!0}{\strut Compost} \colorbox{red!0}{\strut Tumblers} \colorbox{red!0}{\strut Compost} \colorbox{red!0}{\strut Supplies} \colorbox{red!0}{\strut Vermiculture} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Worms} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Green} \colorbox{red!0}{\strut Mowers} \colorbox{red!0}{\strut Lawn} \colorbox{red!0}{\strut Care} \colorbox{red!3}{\strut Garden} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut Season} \colorbox{red!0}{\strut Extenders} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!3}{\strut Beds} \colorbox{red!0}{\strut Rain} \colorbox{red!0}{\strut Barrels} \colorbox{red!0}{\strut Water} \colorbox{red!0}{\strut Accessories} \colorbox{red!0}{\strut Pet} \colorbox{red!0}{\strut Waste} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut Ecological} \colorbox{red!0}{\strut Toilets} \colorbox{red!0}{\strut Recycling} \colorbox{red!0}{\strut Systems} \colorbox{red!0}{\strut Winter} \colorbox{red!0}{\strut Assistance} \colorbox{red!0}{\strut Chipper} \colorbox{red!0}{\strut Shredder} \colorbox{red!0}{\strut Best} \colorbox{red!0}{\strut Sellers} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Additions} \colorbox{red!0}{\strut FAQ} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut Composting} \colorbox{red!0}{\strut Blog} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!3}{\strut Beds} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!3}{\strut Beds} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut gardener} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut joy} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut leisure} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut gardening} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut never} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut jeopardized} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut burden} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut recreational} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut comfort} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut gardening} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut ought} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut felt} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut gardeners} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut gardens} \colorbox{red!0}{\strut alike} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut why} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut garden} \colorbox{red!3}{\strut beds} \colorbox{red!1}{\strut close} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut space} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut beautiful} \colorbox{red!0}{\strut healthy} \colorbox{red!3}{\strut garden} \colorbox{red!0}{\strut cared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut perfection} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut garden} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut space-efficient} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dcor-friendly} \colorbox{red!0}{\strut perks} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut notably} \colorbox{red!0}{\strut presents} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut secure} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut valuable} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut plants} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut vegetables} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Filter} \colorbox{red!0}{\strut Options} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!3}{\strut Beds} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!2}{\strut Bed} \colorbox{red!0}{\strut Planter} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Sand} \colorbox{red!0}{\strut Box} \colorbox{red!0}{\strut Multi-Season} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!2}{\strut Bed} \colorbox{red!0}{\strut Systems} \colorbox{red!0}{\strut ReNew} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!2}{\strut Bed} \colorbox{red!0}{\strut Kits} \colorbox{red!0}{\strut Four} \colorbox{red!0}{\strut Level} \colorbox{red!0}{\strut Pyramid} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!2}{\strut Bed} \colorbox{red!0}{\strut Strawberry} \colorbox{red!0}{\strut Tower} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Herb} \colorbox{red!0}{\strut Terrace} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!2}{\strut Bed} \colorbox{red!0}{\strut Kit} \colorbox{red!0}{\strut Faux} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut Garden} \colorbox{red!2}{\strut Bed} \colorbox{red!0}{\strut Rock} \colorbox{red!0}{\strut Wall} \colorbox{red!0}{\strut Collection} \colorbox{red!0}{\strut Recycled} \colorbox{red!0}{\strut Plastic} \colorbox{red!0}{\strut Landscapes} \colorbox{red!0}{\strut Timber} \colorbox{red!0}{\strut Ties} \colorbox{red!0}{\strut Soil} \colorbox{red!0}{\strut Moisture} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut pH} \colorbox{red!0}{\strut Meters} \colorbox{red!3}{\strut Raising} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut patch} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut garden} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut ground} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut advantages} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raised} \colorbox{red!3}{\strut garden} \colorbox{red!3}{\strut beds} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut accessible} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut convenient} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Giving} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut soil} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut space} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut soil} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut monitored} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut exceptional} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut keep} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut garden} \colorbox{red!0}{\strut rich} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut healthy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut raised} \colorbox{red!2}{\strut bed} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut allow} \colorbox{red!3}{\strut gardening} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut yard} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut poor} \colorbox{red!0}{\strut soil} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut unfit} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut gardening} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut longer} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Watering} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut raised} \colorbox{red!3}{\strut garden} \colorbox{red!2}{\strut bed} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut significant} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut quicker} \colorbox{red!0}{\strut drainage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut moisture} \colorbox{red!0}{\strut from} 
}}}
\end{CJK*}

query: bart sf

101:bart, 80:stations, 80:station, 29:sf, 27:oakland, 27:berkeley, 25:city, 20:tv, 19:san, 19:bay


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Enter} \colorbox{red!0}{\strut Query} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Skip} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut Content} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut View} \colorbox{red!6}{\strut BART} \colorbox{red!1}{\strut Map} \colorbox{red!0}{\strut Home} \colorbox{red!5}{\strut Stations} \colorbox{red!5}{\strut Station} \colorbox{red!1}{\strut List} \colorbox{red!1}{\strut Find} \colorbox{red!0}{\strut Closest} \colorbox{red!5}{\strut Station} \colorbox{red!0}{\strut Schedules} \colorbox{red!0}{\strut Overview} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Time} \colorbox{red!0}{\strut Arrivals} \colorbox{red!1}{\strut Service} \colorbox{red!0}{\strut Advisories} \colorbox{red!0}{\strut Mobile} \colorbox{red!0}{\strut Options} \colorbox{red!0}{\strut Developer} \colorbox{red!0}{\strut Resources} \colorbox{red!0}{\strut Tickets} \colorbox{red!0}{\strut Overview} \colorbox{red!0}{\strut Ticket} \colorbox{red!0}{\strut Sales} \colorbox{red!0}{\strut Fare} \colorbox{red!0}{\strut Calculator} \colorbox{red!0}{\strut Rider} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Overview} \colorbox{red!0}{\strut Parking} \colorbox{red!1}{\strut Airport} \colorbox{red!0}{\strut Connections} \colorbox{red!0}{\strut Transit} \colorbox{red!0}{\strut Connections} \colorbox{red!0}{\strut Bikes} \colorbox{red!0}{\strut on} \colorbox{red!6}{\strut BART} \colorbox{red!0}{\strut Accessible} \colorbox{red!1}{\strut Services} \colorbox{red!0}{\strut Destinations} \colorbox{red!0}{\strut Lost} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Found} \colorbox{red!0}{\strut Safety} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Security} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Articles} \colorbox{red!6}{\strut BART} \colorbox{red!1}{\strut TV} \colorbox{red!6}{\strut BART} \colorbox{red!0}{\strut Times} \colorbox{red!1}{\strut Email} \colorbox{red!0}{\strut Alerts} \colorbox{red!0}{\strut RSS} \colorbox{red!0}{\strut Feeds} \colorbox{red!0}{\strut myBART} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Widget} \colorbox{red!0}{\strut About} \colorbox{red!6}{\strut BART} \colorbox{red!0}{\strut Overview} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Directors} \colorbox{red!0}{\strut Financials} \colorbox{red!0}{\strut Projects} \colorbox{red!0}{\strut Planning} \colorbox{red!0}{\strut Doing} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut Jobs} \colorbox{red!0}{\strut Reports} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Facts} \colorbox{red!6}{\strut BART} \colorbox{red!0}{\strut Police} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Stations} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Station} \colorbox{red!1}{\strut List} \colorbox{red!5}{\strut Station} \colorbox{red!1}{\strut List} \colorbox{red!5}{\strut Station} \colorbox{red!1}{\strut List} \colorbox{red!1}{\strut Find} \colorbox{red!0}{\strut Closest} \colorbox{red!5}{\strut Station} \colorbox{red!1}{\strut Email} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut 12th} \colorbox{red!0}{\strut St.} \colorbox{red!2}{\strut Oakland} \colorbox{red!2}{\strut City} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut 16th} \colorbox{red!0}{\strut St.} \colorbox{red!1}{\strut Mission} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19th} \colorbox{red!0}{\strut St.} \colorbox{red!2}{\strut Oakland} \colorbox{red!0}{\strut 24th} \colorbox{red!0}{\strut St.} \colorbox{red!1}{\strut Mission} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ashby} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Berkeley} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Balboa} \colorbox{red!0}{\strut Park} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bay} \colorbox{red!0}{\strut Fair} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut San} \colorbox{red!0}{\strut Leandro} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Castro} \colorbox{red!0}{\strut Valley} \colorbox{red!0}{\strut Civic} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ColiseumOakland} \colorbox{red!1}{\strut Airport} \colorbox{red!0}{\strut Colma} \colorbox{red!1}{\strut Concord} \colorbox{red!0}{\strut Daly} \colorbox{red!2}{\strut City} \colorbox{red!0}{\strut Downtown} \colorbox{red!2}{\strut Berkeley} \colorbox{red!0}{\strut DublinPleasanton} \colorbox{red!0}{\strut El} \colorbox{red!0}{\strut Cerrito} \colorbox{red!0}{\strut del} \colorbox{red!0}{\strut Norte} \colorbox{red!0}{\strut El} \colorbox{red!0}{\strut Cerrito} \colorbox{red!0}{\strut Plaza} \colorbox{red!0}{\strut Embarcadero} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fremont} \colorbox{red!0}{\strut Fruitvale} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Oakland} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Glen} \colorbox{red!0}{\strut Park} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Hayward} \colorbox{red!0}{\strut Lafayette} \colorbox{red!0}{\strut Lake} \colorbox{red!0}{\strut Merritt} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Oakland} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MacArthur} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Oakland} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Millbrae} \colorbox{red!0}{\strut Montgomery} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut North} \colorbox{red!2}{\strut Berkeley} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut ConcordMartinez} \colorbox{red!0}{\strut Orinda} \colorbox{red!0}{\strut PittsburgBay} \colorbox{red!0}{\strut Point} \colorbox{red!0}{\strut Pleasant} \colorbox{red!0}{\strut Hill} \colorbox{red!0}{\strut Powell} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Richmond} \colorbox{red!0}{\strut Rockridge} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Oakland} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut San} \colorbox{red!0}{\strut Bruno} \colorbox{red!1}{\strut San} \colorbox{red!1}{\strut Francisco} \colorbox{red!0}{\strut Int} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut l} \colorbox{red!1}{\strut Airport} \colorbox{red!1}{\strut San} \colorbox{red!0}{\strut Leandro} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut Hayward} \colorbox{red!0}{\strut South} \colorbox{red!1}{\strut San} \colorbox{red!1}{\strut Francisco} \colorbox{red!0}{\strut Union} \colorbox{red!2}{\strut City} \colorbox{red!0}{\strut Walnut} \colorbox{red!0}{\strut Creek} \colorbox{red!0}{\strut West} \colorbox{red!2}{\strut Oakland} \colorbox{red!6}{\strut BART} \colorbox{red!0}{\strut System} \colorbox{red!1}{\strut Map} \colorbox{red!6}{\strut BART} \colorbox{red!0}{\strut Rider} \colorbox{red!0}{\strut Rewards} \colorbox{red!0}{\strut Card} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut myBART} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut BART} \colorbox{red!1}{\strut TV} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut 2009} \colorbox{red!1}{\strut San} \colorbox{red!1}{\strut Francisco} \colorbox{red!1}{\strut Bay} \colorbox{red!0}{\strut Area} \colorbox{red!0}{\strut Rapid} \colorbox{red!0}{\strut Transit} \colorbox{red!0}{\strut District} 
}}}
\end{CJK*}

100:tiles, 100:tile, 98:bart, 77:stops, 75:sf, 74:stop, 40:civic, 33:symphony, 31:center, 29:where


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Welcome} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut Design} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut NY} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut LA} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut SF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Chicago} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut apartmenttherapy.com} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Nursery} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut ohdeedoh.com} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Kitchen} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut thekitchn.com} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Tech} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut unplggd.com} \colorbox{red!0}{\strut Green} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut re-nest.com} \colorbox{red!1}{\strut apartment} \colorbox{red!1}{\strut therapy} \colorbox{red!0}{\strut changing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!1}{\strut room} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut time} \colorbox{red!1}{\strut Main} \colorbox{red!1}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!0}{\strut Los} \colorbox{red!0}{\strut Angeles} \colorbox{red!1}{\strut San} \colorbox{red!1}{\strut Francisco} \colorbox{red!2}{\strut Chicago} \colorbox{red!0}{\strut DC} \colorbox{red!0}{\strut Boston} \colorbox{red!1}{\strut House} \colorbox{red!0}{\strut Tours} \colorbox{red!0}{\strut Shopping} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut Archive} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Big} \colorbox{red!0}{\strut Window} \colorbox{red!0}{\strut Challenge} \colorbox{red!0}{\strut Community} \colorbox{red!5}{\strut SF} \colorbox{red!1}{\strut Good} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Tiles} \colorbox{red!0}{\strut at} \colorbox{red!6}{\strut BART} \colorbox{red!5}{\strut Stops} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut AT} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut SF} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut idea} \colorbox{red!2}{\strut where} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut find} \colorbox{red!6}{\strut tiles} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Civic} \colorbox{red!2}{\strut Center} \colorbox{red!6}{\strut BART} \colorbox{red!4}{\strut stop} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Thanks} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut -Laura} \colorbox{red!0}{\strut Laura} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!6}{\strut tile} \colorbox{red!0}{\strut Shannon} \colorbox{red!0}{\strut asked} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut months} \colorbox{red!0}{\strut ago} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut never} \colorbox{red!0}{\strut heard} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut from} \colorbox{red!6}{\strut BART} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut anyone} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut QUESTIONS} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut sf} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut apartmenttherapy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dot} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut com} \colorbox{red!0}{\strut Note} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Include} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut picture} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut gets} \colorbox{red!0}{\strut posted} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut San} \colorbox{red!1}{\strut Francisco} \colorbox{red!0}{\strut leslie} \colorbox{red!0}{\strut June} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut 0445PM} \colorbox{red!0}{\strut Comments} \colorbox{red!0}{\strut Tags} \colorbox{red!6}{\strut tile} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut stone} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut countertops} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Good} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut TileVault} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sunset} \colorbox{red!1}{\strut Idea} \colorbox{red!1}{\strut House} \colorbox{red!5}{\strut SF} \colorbox{red!1}{\strut Good} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Tiles} \colorbox{red!0}{\strut at} \colorbox{red!6}{\strut BART} \colorbox{red!5}{\strut Stops} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut Symphony} \colorbox{red!2}{\strut Wall} \colorbox{red!6}{\strut Tiles} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Dominic} \colorbox{red!0}{\strut Crinson} \colorbox{red!0}{\strut TileVault} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Small} \colorbox{red!0}{\strut Blue} \colorbox{red!1}{\strut Squares} \colorbox{red!0}{\strut Look} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Spacious} \colorbox{red!0}{\strut Blue} \colorbox{red!1}{\strut Bathroom} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut Comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut subconscious} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut hexagon} \colorbox{red!1}{\strut patterns} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut late} \colorbox{red!0}{\strut 60s-early} \colorbox{red!0}{\strut 70s} \colorbox{red!0}{\strut vibe} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut posted} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut pantzini} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut June} \colorbox{red!0}{\strut 26th} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 1246pm} \colorbox{red!0}{\strut view} \colorbox{red!1}{\strut pantzini} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut profile} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut anymore} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut certainly} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut up} \colorbox{red!1}{\strut making} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!6}{\strut tile} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut tile} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut listening} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut People} \colorbox{red!0}{\strut seem} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut love} \colorbox{red!0}{\strut that} \colorbox{red!6}{\strut tile} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotosjayfish129710344inset-72157600356591088} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotospetebeck12389105} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotosjbergen1200303453inset-72157601592381820} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotoselithebearded1450203895inset-72157594574414547} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotosjef145597993} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut know} 
}}}
\end{CJK*}

query: raffles

100:raffles, 100:hotel, 99:hotels, 62:what, 56:famous, 10:english, 10:bangkok, 10:asia, 9:oriental, 9:guests


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikimedia} \colorbox{red!0}{\strut Commons} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut media} \colorbox{red!0}{\strut repository} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!2}{\strut famous} \colorbox{red!3}{\strut hotels} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Asia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut among} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Oriental} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Bangkok} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut hotel} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut many} \colorbox{red!2}{\strut famous} \colorbox{red!0}{\strut guests} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut among} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut Rudyard} \colorbox{red!0}{\strut Kipling} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!0}{\strut Courtyard} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Lawn} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!0}{\strut Fountain} \colorbox{red!0}{\strut at} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!0}{\strut Retrieved} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut commons.wikimedia.orgwikiRafflesHotel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Category} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Raffles} \colorbox{red!3}{\strut Hotel} \colorbox{red!0}{\strut Views} \colorbox{red!0}{\strut Gallery} \colorbox{red!0}{\strut Discussion} \colorbox{red!0}{\strut Edit} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut tools} \colorbox{red!0}{\strut Log} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut create} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Navigation} \colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut Welcome} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut portal} \colorbox{red!0}{\strut Village} \colorbox{red!0}{\strut pump} \colorbox{red!0}{\strut Participate} \colorbox{red!0}{\strut Upload} \colorbox{red!0}{\strut file} \colorbox{red!0}{\strut Recent} \colorbox{red!0}{\strut changes} \colorbox{red!0}{\strut Latest} \colorbox{red!0}{\strut files} \colorbox{red!0}{\strut Random} \colorbox{red!0}{\strut file} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut Donate} \colorbox{red!0}{\strut Toolbox} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut changes} \colorbox{red!0}{\strut Special} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut Printable} \colorbox{red!0}{\strut version} \colorbox{red!0}{\strut Permanent} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut Cite} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut Deutsch} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Svenska} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut modified} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut November} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 1623} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Text} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut GNU} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Documentation} \colorbox{red!0}{\strut License} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Wikimedia} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut registered} \colorbox{red!0}{\strut trademark} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Wikimedia} \colorbox{red!0}{\strut Foundation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut policy} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Wikimedia} \colorbox{red!0}{\strut Commons} \colorbox{red!0}{\strut Disclaimers} 
}}}
\end{CJK*}

85:raffle, 84:raffling, 83:raffled, 81:raffles, 78:what, 71:parrots, 70:parrot, 57:birds, 54:bird, 51:prizes


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Avian} \colorbox{red!1}{\strut Protection} \colorbox{red!1}{\strut Society} \colorbox{red!6}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Wrong} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut Raffling} \colorbox{red!4}{\strut Birds} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut interesting} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut us} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut avian} \colorbox{red!1}{\strut welfare} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut tend} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut agree} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut live} \colorbox{red!4}{\strut birds} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut never} \colorbox{red!0}{\strut be} \colorbox{red!6}{\strut raffled} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut given} \colorbox{red!1}{\strut away} \colorbox{red!1}{\strut as} \colorbox{red!4}{\strut prizes} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut contests} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!1}{\strut reasons} \colorbox{red!2}{\strut why} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut feel} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut practice} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut unethical} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut illegal} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut In} \colorbox{red!0}{\strut some} \colorbox{red!1}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut actually} \colorbox{red!1}{\strut illegal} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!3}{\strut live} \colorbox{red!2}{\strut animals} \colorbox{red!1}{\strut as} \colorbox{red!4}{\strut prizes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Check} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut laws} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut going} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut homepage} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut checking} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut legislation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut irresponsible} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Considering} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut parrots} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut given} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut normal} \colorbox{red!0}{\strut behaviors} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut screaming} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut destruction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut messiness} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut biting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut behavioral} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut excessive} \colorbox{red!0}{\strut screaming} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut feather} \colorbox{red!0}{\strut destructive} \colorbox{red!0}{\strut behaviors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut conclude} \colorbox{red!0}{\strut that} \colorbox{red!5}{\strut parrots} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut difficult} \colorbox{red!2}{\strut animals} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut live} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Given} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut condone} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut practice} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut giving} \colorbox{red!1}{\strut away} \colorbox{red!0}{\strut these} \colorbox{red!2}{\strut animals} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut clearly} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut live} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut humans} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut thought} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut decision} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut care} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut parrot} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut feel} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut organizations} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut hold} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut kinds} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut raffles} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut able} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut screen} \colorbox{red!1}{\strut new} \colorbox{red!1}{\strut owners} \colorbox{red!1}{\strut properly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Education} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut radio} \colorbox{red!0}{\strut stations} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut businesses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut organizations} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut feel} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut potential} \colorbox{red!4}{\strut prize} \colorbox{red!1}{\strut winners} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut appropriate} \colorbox{red!0}{\strut training} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut regard} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut intense} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut parrots} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut In} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut potential} \colorbox{red!4}{\strut prize} \colorbox{red!1}{\strut winners} \colorbox{red!1}{\strut make} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut decision} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut enter} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut contest} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut impulse} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Impulse} \colorbox{red!1}{\strut buys} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut parrots} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut birds} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut re-homed} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut year} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut country} 
}}}
\end{CJK*}

query: rice

102:rice, 26:recipes, 23:fried, 21:treats, 19:chicken, 18:spanish, 17:chilled, 15:shrimp, 15:mexican, 14:contact


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut XML} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut Copyright} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut 2} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Index} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Links} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut XML} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Chicken} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Casserole} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Spanish} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Chicken} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Pudding} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Baked} \colorbox{red!0}{\strut Chicken} \colorbox{red!0}{\strut And} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Krispies} \colorbox{red!0}{\strut Treats} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Chicken} \colorbox{red!0}{\strut And} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Soup} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Basmati} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Mexican} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Red} \colorbox{red!0}{\strut Beans} \colorbox{red!0}{\strut And} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Cake} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Chinese} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Sticky} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Sushi} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Bayou} \colorbox{red!0}{\strut Shrimp} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Turkey} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Homemade} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Milk} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Lemon} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Garlic} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Cajun} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Beef} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Mexican} \colorbox{red!0}{\strut Fire} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Pilaf} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Minute} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Spicy} \colorbox{red!0}{\strut Jalapeno} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Balls} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Southwestern} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Pork} \colorbox{red!0}{\strut Fried} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Onion} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Chilled} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Salad} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Chocolate} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Pudding} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Pineapple} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Casserole} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Mushroom} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Honey} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Wild} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Casserole} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Calamari} \colorbox{red!0}{\strut And} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Cheesy} \colorbox{red!0}{\strut Confetti} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Okra} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Taco} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Asian} \colorbox{red!0}{\strut Coconut} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Green} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Jamaican} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Indian} \colorbox{red!2}{\strut Rice} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Hamburger} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Soup} \colorbox{red!2}{\strut Rice} \colorbox{red!0}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Ham} 
}}}
\end{CJK*}

98:rices, 97:rice, 89:river, 68:farms, 21:trade, 18:shows, 17:show, 15:wild, 14:schedule, 14:beans


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!10}{\strut Rice} \colorbox{red!9}{\strut River} \colorbox{red!7}{\strut Farms} \colorbox{red!2}{\strut Trade} \colorbox{red!2}{\strut Show} \colorbox{red!1}{\strut Schedule} \colorbox{red!10}{\strut Rice} \colorbox{red!9}{\strut River} \colorbox{red!7}{\strut Farms} \colorbox{red!0}{\strut does} \colorbox{red!1}{\strut not} \colorbox{red!1}{\strut have} \colorbox{red!0}{\strut any} \colorbox{red!2}{\strut trade} \colorbox{red!2}{\strut shows} \colorbox{red!1}{\strut scheduled} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut time} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!1}{\strut continue} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut updated} \colorbox{red!0}{\strut information} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 2005} \colorbox{red!10}{\strut Rice} \colorbox{red!9}{\strut River} \colorbox{red!7}{\strut Farms} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut Rights} \colorbox{red!0}{\strut Reserved} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut HOME} \colorbox{red!1}{\strut PRODUCTS} \colorbox{red!2}{\strut Wild} \colorbox{red!10}{\strut Rice} \colorbox{red!1}{\strut Blends} \colorbox{red!2}{\strut Wild} \colorbox{red!10}{\strut Rice} \colorbox{red!1}{\strut Boxed} \colorbox{red!1}{\strut Products} \colorbox{red!1}{\strut Bagged} \colorbox{red!1}{\strut Products} \colorbox{red!1}{\strut Beans} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Lentils} \colorbox{red!1}{\strut Beans} \colorbox{red!1}{\strut Lentils} \colorbox{red!1}{\strut Chiles} \colorbox{red!1}{\strut Chiles} \colorbox{red!1}{\strut Processed} \colorbox{red!1}{\strut Chiles} \colorbox{red!1}{\strut Corn} \colorbox{red!1}{\strut Corn} \colorbox{red!1}{\strut Dried} \colorbox{red!1}{\strut Fruits} \colorbox{red!1}{\strut Dried} \colorbox{red!1}{\strut Fruits} \colorbox{red!1}{\strut Grains} \colorbox{red!1}{\strut Grains} \colorbox{red!1}{\strut Mushrooms} \colorbox{red!1}{\strut Mushrooms} \colorbox{red!1}{\strut Nuts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Seeds} \colorbox{red!1}{\strut Nuts} \colorbox{red!1}{\strut Seeds} \colorbox{red!1}{\strut Pasta} \colorbox{red!1}{\strut Couscous} \colorbox{red!0}{\strut Orzo} \colorbox{red!1}{\strut Polenta} \colorbox{red!0}{\strut Other} \colorbox{red!1}{\strut Specialty} \colorbox{red!10}{\strut Rices} \colorbox{red!1}{\strut Specialty} \colorbox{red!10}{\strut Rices} \colorbox{red!1}{\strut Spices} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Herbs} \colorbox{red!0}{\strut Peppercorns} \colorbox{red!1}{\strut Sea} \colorbox{red!1}{\strut Salt} \colorbox{red!1}{\strut Spices} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Herbs} \colorbox{red!1}{\strut ORDER} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Consumer} \colorbox{red!1}{\strut Retail} \colorbox{red!1}{\strut Business} \colorbox{red!0}{\strut ADDITIONAL} \colorbox{red!0}{\strut INFO} \colorbox{red!0}{\strut Foodservice} \colorbox{red!1}{\strut Retail} \colorbox{red!1}{\strut Promotional} \colorbox{red!0}{\strut Suggestions} \colorbox{red!1}{\strut Recipes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tips} \colorbox{red!0}{\strut Links} \colorbox{red!1}{\strut COMPANY} \colorbox{red!0}{\strut INFO} \colorbox{red!0}{\strut Tradeshows} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

query: sat

85:vocabulary, 53:sat, 38:words, 34:lists, 24:list, 20:business, 19:practice, 18:school, 15:score, 13:high


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut Admissions} \colorbox{red!0}{\strut Careers} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut Filed} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SAT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GMAT} \colorbox{red!0}{\strut Preparation} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut score} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut SAT} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut essential} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut vocabulary} \colorbox{red!1}{\strut words} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut vocabulary} \colorbox{red!1}{\strut lists} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut practice} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut prepare} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut SAT} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 25} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 25} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 24} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 24} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 23} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 23} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 22} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 22} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 21} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 21} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 20} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 20} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 19} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 19} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 18} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 18} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 17} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 17} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 16} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 16} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 15} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 15} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 14} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 14} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 13} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 13} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 12} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 12} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 11} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 11} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut SAT} \colorbox{red!2}{\strut Vocabulary} \colorbox{red!0}{\strut Practice} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut SAT} 
}}}
\end{CJK*}

100:sat, 99:sats, 77:test, 66:what, 63:tests, 34:assessment, 32:diagnostic, 28:prep, 27:score, 25:scholastic


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut SAT} \colorbox{red!2}{\strut Scholastic} \colorbox{red!2}{\strut Assessment} \colorbox{red!5}{\strut Test} \colorbox{red!0}{\strut Ogni} \colorbox{red!1}{\strut anno} \colorbox{red!0}{\strut circa} \colorbox{red!0}{\strut 2} \colorbox{red!1}{\strut milioni} \colorbox{red!0}{\strut di} \colorbox{red!1}{\strut studenti} \colorbox{red!0}{\strut che} \colorbox{red!0}{\strut si} \colorbox{red!0}{\strut iscrivono} \colorbox{red!0}{\strut alle} \colorbox{red!0}{\strut universitamericane} \colorbox{red!0}{\strut devono} \colorbox{red!0}{\strut superare} \colorbox{red!0}{\strut lsame} \colorbox{red!6}{\strut SAT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Il} \colorbox{red!5}{\strut test} \colorbox{red!0}{\strut ha} \colorbox{red!0}{\strut lo} \colorbox{red!1}{\strut scopo} \colorbox{red!0}{\strut di} \colorbox{red!0}{\strut fornire} \colorbox{red!0}{\strut alle} \colorbox{red!0}{\strut commissioni} \colorbox{red!0}{\strut dmmissione} \colorbox{red!0}{\strut delle} \colorbox{red!0}{\strut universitelementi} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut determinare} \colorbox{red!0}{\strut le} \colorbox{red!0}{\strut capacitdegli} \colorbox{red!1}{\strut studenti} \colorbox{red!0}{\strut e} \colorbox{red!0}{\strut le} \colorbox{red!0}{\strut probabilitdi} \colorbox{red!0}{\strut successo} \colorbox{red!0}{\strut nei} \colorbox{red!0}{\strut loro} \colorbox{red!0}{\strut studi} \colorbox{red!1}{\strut universitari} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Le} \colorbox{red!0}{\strut sessioni} \colorbox{red!0}{\strut dellsame} \colorbox{red!6}{\strut SAT} \colorbox{red!0}{\strut hanno} \colorbox{red!0}{\strut luogo} \colorbox{red!0}{\strut sei} \colorbox{red!0}{\strut volte} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut un} \colorbox{red!1}{\strut anno} \colorbox{red!0}{\strut ed} \colorbox{red!0}{\strut il} \colorbox{red!5}{\strut test} \colorbox{red!0}{\strut su} \colorbox{red!0}{\strut carta} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut non} \colorbox{red!0}{\strut si} \colorbox{red!0}{\strut effettua} \colorbox{red!0}{\strut al} \colorbox{red!1}{\strut computer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Prepare} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut October} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut November} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 1} \colorbox{red!6}{\strut SATs} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut FlexPrep} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut SAT} \colorbox{red!1}{\strut Taught} \colorbox{red!0}{\strut by} \colorbox{red!6}{\strut SAT} \colorbox{red!0}{\strut specialist} \colorbox{red!0}{\strut Bob} \colorbox{red!0}{\strut Stanton} \colorbox{red!0}{\strut Here} \colorbox{red!4}{\strut what} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut SAT} \colorbox{red!2}{\strut Diagnostic} \colorbox{red!1}{\strut Make} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut appointment} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut Monday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Tuesday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Wednesday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thursday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Saturday} \colorbox{red!0}{\strut afternoon} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut SAT} \colorbox{red!2}{\strut Diagnostic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut specifically} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut reliable} \colorbox{red!0}{\strut estimate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut current} \colorbox{red!2}{\strut score} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reveal} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut strength} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut weakness} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Consultation} \colorbox{red!0}{\strut Sit} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut our} \colorbox{red!6}{\strut SAT} \colorbox{red!0}{\strut expert} \colorbox{red!0}{\strut Bob} \colorbox{red!0}{\strut Stanton} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut review} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut results} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut SAT} \colorbox{red!2}{\strut Diagnostic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut discuss} \colorbox{red!0}{\strut objectives} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut develop} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut personalized} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut attack} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut reaching} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut SAT} \colorbox{red!0}{\strut goal} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Official} \colorbox{red!6}{\strut SAT} \colorbox{red!1}{\strut Study} \colorbox{red!0}{\strut Guide} \colorbox{red!1}{\strut Practice} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut comprehensive} \colorbox{red!1}{\strut study} \colorbox{red!0}{\strut guide} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut in-depth} \colorbox{red!5}{\strut test} \colorbox{red!0}{\strut coverage} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut packed} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut eight} \colorbox{red!0}{\strut full-length} \colorbox{red!1}{\strut practice} \colorbox{red!4}{\strut tests} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut hundred} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut questionsll} \colorbox{red!0}{\strut prepared} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut makers} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut SAT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Private} \colorbox{red!1}{\strut Lessons} \colorbox{red!0}{\strut Profit} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut personalized} \colorbox{red!1}{\strut instruction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut scheduled} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut times} \colorbox{red!0}{\strut convenient} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut concentrating} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut topics} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut help} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Small-Group} \colorbox{red!1}{\strut Lessons} \colorbox{red!0}{\strut Join} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut weekly} \colorbox{red!0}{\strut Monday} \colorbox{red!0}{\strut workshops} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16.309.00} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut focused} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut essay} \colorbox{red!1}{\strut writing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut vocabulary} \colorbox{red!0}{\strut building} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut reading} \colorbox{red!0}{\strut skills} \colorbox{red!1}{\strut development} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut grammar} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut math} \colorbox{red!1}{\strut review} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut test-taking} \colorbox{red!0}{\strut strategies} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: butter margarine

95:margarine, 88:butter, 74:healthier, 62:what, 36:made, 22:better, 17:health, 17:benefits, 13:medical, 12:rich


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Appointments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jobs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Podcast} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Margarine} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut it} \colorbox{red!5}{\strut healthier} \colorbox{red!0}{\strut than} \colorbox{red!6}{\strut butter} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut expert} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!1}{\strut Zeratsky} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R.D.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut L.D} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Total} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 00542} \colorbox{red!0}{\strut minutes} \colorbox{red!0}{\strut Subscribe} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut podcasts} \colorbox{red!0}{\strut TRANSCRIPT} \colorbox{red!0}{\strut Welcome} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Mayo} \colorbox{red!1}{\strut Clinic} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut podcast} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut month} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut topic} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Margarine} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut it} \colorbox{red!5}{\strut healthier} \colorbox{red!0}{\strut than} \colorbox{red!6}{\strut butter} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut host} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Rich} \colorbox{red!1}{\strut Dietman} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut today} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut podcast} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut talking} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut relative} \colorbox{red!1}{\strut health} \colorbox{red!1}{\strut benefits} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut vs.} \colorbox{red!6}{\strut butter} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Katherine} \colorbox{red!1}{\strut Zeratsky} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut registered} \colorbox{red!0}{\strut dietitian} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Mayo} \colorbox{red!1}{\strut Clinic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut specialty} \colorbox{red!0}{\strut editor} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Food} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Nutrition} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut MayoClinic.com} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut thanks} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut today} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!1}{\strut Zeratsky} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thank} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut me} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Rich} \colorbox{red!1}{\strut Dietman} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Let} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Katherine} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut better} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut heart} \colorbox{red!6}{\strut butter} \colorbox{red!0}{\strut or} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Katherine} \colorbox{red!1}{\strut Zeratsky} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Quite} \colorbox{red!0}{\strut generally} \colorbox{red!0}{\strut speaking} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut better} \colorbox{red!0}{\strut choice} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut grocery} \colorbox{red!0}{\strut store} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut checked} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut butter-margarine} \colorbox{red!0}{\strut aisle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut necessarily} \colorbox{red!1}{\strut mean} \colorbox{red!0}{\strut picking} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut easy} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Rich} \colorbox{red!1}{\strut Dietman} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut choices} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!1}{\strut Zeratsky} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut choices} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut different} \colorbox{red!1}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut butter} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut straight} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut different} \colorbox{red!0}{\strut kinds} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut margarine-like} \colorbox{red!0}{\strut spreads} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Rich} \colorbox{red!1}{\strut Dietman} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Why} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut difficult} \colorbox{red!0}{\strut choice} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut why} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tricky} \colorbox{red!0}{\strut proposition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut choosing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut between} \colorbox{red!6}{\strut butter} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut say} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut trying} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut pick} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut best} \colorbox{red!6}{\strut margarine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut probably} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut better} \colorbox{red!1}{\strut product} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut us} 
}}}
\end{CJK*}

93:margarine, 92:margarines, 59:butter, 58:what, 34:how, 30:which, 24:oils, 23:oil, 20:fat, 20:cholesterol


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut HealthPlans} \colorbox{red!0}{\strut Providers} \colorbox{red!0}{\strut Programs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut Hospitals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Clinics} \colorbox{red!0}{\strut HealthInfo} \colorbox{red!0}{\strut Employment} \colorbox{red!0}{\strut Foundations} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Nutrition} \colorbox{red!0}{\strut Center} \colorbox{red!0}{\strut Ask} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Expert} \colorbox{red!0}{\strut Healthwise} \colorbox{red!0}{\strut Library} \colorbox{red!0}{\strut AudioLibrary} \colorbox{red!0}{\strut myProvidence} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut Register} \colorbox{red!0}{\strut Ask} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut Expert} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Butter} \colorbox{red!0}{\strut vs.} \colorbox{red!7}{\strut Margarine} \colorbox{red!2}{\strut Which} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut Better} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Q} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Years} \colorbox{red!0}{\strut ago} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut switched} \colorbox{red!0}{\strut from} \colorbox{red!4}{\strut butter} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut margarine} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reduce} \colorbox{red!0}{\strut my} \colorbox{red!2}{\strut cholesterol} \colorbox{red!0}{\strut intake} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Now} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut hear} \colorbox{red!0}{\strut that} \colorbox{red!7}{\strut margarine} \colorbox{red!1}{\strut contains} \colorbox{red!0}{\strut something} \colorbox{red!0}{\strut even} \colorbox{red!1}{\strut worse} \colorbox{red!0}{\strut than} \colorbox{red!2}{\strut cholesterol} \colorbox{red!1}{\strut trans} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut Im} \colorbox{red!0}{\strut thinking} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut switching} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut butter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Weighing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut pros} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cons} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut healthier} \colorbox{red!1}{\strut choice} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut butter} \colorbox{red!1}{\strut or} \colorbox{red!7}{\strut margarine} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Terese} \colorbox{red!0}{\strut Scollard} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut MBA} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R.D.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut L.D.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut regional} \colorbox{red!0}{\strut clinical} \colorbox{red!0}{\strut nutrition} \colorbox{red!0}{\strut manager} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Providence} \colorbox{red!0}{\strut Nutrition} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Butter} \colorbox{red!1}{\strut contains} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lot} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut artery-clogging} \colorbox{red!1}{\strut saturated} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut margarine} \colorbox{red!1}{\strut contains} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut unhealthy} \colorbox{red!0}{\strut combination} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut saturated} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut trans} \colorbox{red!1}{\strut fats} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut healthiest} \colorbox{red!1}{\strut choice} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut skip} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut use} \colorbox{red!1}{\strut liquid} \colorbox{red!2}{\strut oils} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut olive} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut canola} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut safflower} \colorbox{red!2}{\strut oil} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut instead} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut dietitians} \colorbox{red!0}{\strut understand} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut some} \colorbox{red!1}{\strut foods} \colorbox{red!0}{\strut benefit} \colorbox{red!0}{\strut greatly} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut little} \colorbox{red!1}{\strut buttery} \colorbox{red!1}{\strut flavor} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut wouldnt} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut realistic} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut suggest} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut give} \colorbox{red!0}{\strut up} \colorbox{red!4}{\strut butter} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut margarine} \colorbox{red!0}{\strut altogether} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut one} \colorbox{red!1}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut occasion} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut margarine} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut healthier} \colorbox{red!1}{\strut choice} \colorbox{red!0}{\strut overall} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut long} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut right} \colorbox{red!1}{\strut type} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut margarine} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Margarine} \colorbox{red!1}{\strut comes} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut stick} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut tub} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut liquid} \colorbox{red!0}{\strut forms} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut created} \colorbox{red!1}{\strut equal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!1}{\strut stick} \colorbox{red!7}{\strut margarines} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut no} \colorbox{red!1}{\strut better} \colorbox{red!0}{\strut than} \colorbox{red!4}{\strut butter} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut health} \colorbox{red!1}{\strut effects} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut best} \colorbox{red!1}{\strut choices} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut soft} \colorbox{red!1}{\strut or} \colorbox{red!1}{\strut liquid} \colorbox{red!7}{\strut margarines} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut or} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut trans} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 3} \colorbox{red!1}{\strut grams} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut saturated} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut serving} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Understanding} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut pros} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cons} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut option} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut you} 
}}}
\end{CJK*}

query: fact uranus

99:uranus, 44:how, 35:did, 29:names, 27:mean, 27:big, 23:who, 22:planet, 21:spelled, 16:surface


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Dictionary} \colorbox{red!0}{\strut Thesaurus} \colorbox{red!0}{\strut Reference} \colorbox{red!0}{\strut Translate} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Register} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Suggestions} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Searches} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Ask.com} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut facts} \colorbox{red!1}{\strut planet} \colorbox{red!5}{\strut uranus} \colorbox{red!5}{\strut uranus} \colorbox{red!1}{\strut moons} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut rings} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut atmosphere} \colorbox{red!0}{\strut interesting} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut ...} \colorbox{red!5}{\strut uranus} \colorbox{red!1}{\strut surface} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut informatio} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut greek} \colorbox{red!1}{\strut god} \colorbox{red!5}{\strut uranus} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut fact} \colorbox{red!0}{\strut sheet} \colorbox{red!2}{\strut names} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut ...} \colorbox{red!2}{\strut how} \colorbox{red!2}{\strut did} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut ge} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut fun} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut about} \colorbox{red!5}{\strut uranus} \colorbox{red!2}{\strut how} \colorbox{red!1}{\strut big} \colorbox{red!0}{\strut is} \colorbox{red!5}{\strut uranus} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut gravity} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut weather} \colorbox{red!0}{\strut amazing} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut facts} \colorbox{red!5}{\strut uranus} \colorbox{red!1}{\strut symbol} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut discovered} \colorbox{red!5}{\strut uranus} \colorbox{red!5}{\strut uranus} \colorbox{red!1}{\strut mythology} \colorbox{red!0}{\strut life} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut uranus} \colorbox{red!1}{\strut surface} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut uranus} \colorbox{red!0}{\strut Nearby} \colorbox{red!0}{\strut Entries} \colorbox{red!0}{\strut uranologist} \colorbox{red!0}{\strut Uranology} \colorbox{red!0}{\strut Uranometria} \colorbox{red!0}{\strut uranometrical} \colorbox{red!0}{\strut Uranometry} \colorbox{red!0}{\strut uranophobia} \colorbox{red!0}{\strut uranoplasty} \colorbox{red!0}{\strut uranorrhaphy} \colorbox{red!0}{\strut uranoschisis} \colorbox{red!0}{\strut uranoscopid} \colorbox{red!0}{\strut uranoscopidae} \colorbox{red!0}{\strut Uranoscopy} \colorbox{red!0}{\strut Uranoso-} \colorbox{red!0}{\strut uranostaphyloplas} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut uranostaphyloschi} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Uranous} \colorbox{red!5}{\strut Uranus} \colorbox{red!0}{\strut Uranyl} \colorbox{red!0}{\strut uranyl} \colorbox{red!0}{\strut acetate} \colorbox{red!0}{\strut uranyl} \colorbox{red!0}{\strut group} \colorbox{red!0}{\strut uranyl} \colorbox{red!0}{\strut nitrate} \colorbox{red!0}{\strut uranyl} \colorbox{red!0}{\strut oxalate} \colorbox{red!0}{\strut uranyl} \colorbox{red!0}{\strut radical} \colorbox{red!0}{\strut uranylic} \colorbox{red!0}{\strut Urao} \colorbox{red!0}{\strut URAQT} \colorbox{red!0}{\strut Urare} \colorbox{red!0}{\strut urarthritis} \colorbox{red!0}{\strut urartian} \colorbox{red!0}{\strut urartu} \colorbox{red!0}{\strut urase} \colorbox{red!0}{\strut urate} \colorbox{red!0}{\strut urate} \colorbox{red!0}{\strut oxidase} \colorbox{red!5}{\strut Uranus} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut dictionary} \colorbox{red!0}{\strut results} \colorbox{red!5}{\strut Uranus} \colorbox{red!0}{\strut yYr} \colorbox{red!0}{\strut Y} \colorbox{red!0}{\strut nYs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut yrej-} \colorbox{red!0}{\strut Show} \colorbox{red!1}{\strut Spelled} \colorbox{red!1}{\strut Pronunciation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut yoo} \colorbox{red!0}{\strut r-uh-nuh} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut yoo-rey-} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Show} \colorbox{red!0}{\strut IPA} \colorbox{red!1}{\strut Pronunciation} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Astronomy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut planet} \colorbox{red!0}{\strut seventh} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sun} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut equatorial} \colorbox{red!0}{\strut diameter} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 32,600} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 56,460} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut mean} \colorbox{red!1}{\strut distance} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sun} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1,784} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2,871} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut revolution} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 84.07} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 15} \colorbox{red!1}{\strut moons} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Also} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ouranos} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Classical} \colorbox{red!1}{\strut Mythology} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut personification} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Heaven} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ruler} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut son} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut husband} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Gaea} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Earth} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut father} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Titans} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut castrated} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dethroned} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut youngest} \colorbox{red!0}{\strut son} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Cronus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut instigation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Gaea} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Dictionary.com} \colorbox{red!0}{\strut Unabridged} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut v} \colorbox{red!0}{\strut 1.1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Random} \colorbox{red!0}{\strut House} \colorbox{red!0}{\strut Unabridged} \colorbox{red!0}{\strut Dictionary} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Random} \colorbox{red!0}{\strut House} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Cite} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut Source} \colorbox{red!5}{\strut Uranus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut yOOr} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Y-nYs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut yOO-rnYs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pronunciation} \colorbox{red!0}{\strut Key} \colorbox{red!0}{\strut n.} \colorbox{red!1}{\strut Greek} \colorbox{red!1}{\strut Mythology} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut earliest} \colorbox{red!0}{\strut supreme} \colorbox{red!1}{\strut god} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut personification} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sky} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut who} 
}}}
\end{CJK*}

101:logos, 81:uranus, 61:fact, 55:planetary, 44:earth, 42:solar, 35:saturn, 31:planets, 30:neptune, 21:body


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut URANUS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut THE} \colorbox{red!1}{\strut DIAMOND} \colorbox{red!1}{\strut SOUL} \colorbox{red!0}{\strut Thinking} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut question} \colorbox{red!1}{\strut s} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Planetary} \colorbox{red!5}{\strut Logos} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Earth} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut fact} \colorbox{red!0}{\strut theLogos} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Uranus} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut p} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut following} \colorbox{red!0}{\strut speculations} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Uranus} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Neptune} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Saturn} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut synthesizing} \colorbox{red!1}{\strut planets} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut following} \colorbox{red!1}{\strut correspondences} \colorbox{red!4}{\strut Uranus} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut petals} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Solar} \colorbox{red!0}{\strut Egoic} \colorbox{red!0}{\strut Lotus} \colorbox{red!1}{\strut cosmic} \colorbox{red!1}{\strut mental} \colorbox{red!1}{\strut plane} \colorbox{red!0}{\strut higher} \colorbox{red!1}{\strut three} \colorbox{red!1}{\strut planes} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut cosmic} \colorbox{red!1}{\strut physical} \colorbox{red!1}{\strut Neptune} \colorbox{red!0}{\strut love} \colorbox{red!1}{\strut petals} \colorbox{red!0}{\strut ofSolar} \colorbox{red!0}{\strut lotus} \colorbox{red!1}{\strut cosmic} \colorbox{red!0}{\strut astral} \colorbox{red!1}{\strut plane} \colorbox{red!0}{\strut triadal} \colorbox{red!1}{\strut planes} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut cosmic} \colorbox{red!1}{\strut physical} \colorbox{red!2}{\strut Saturn} \colorbox{red!0}{\strut intelligence} \colorbox{red!1}{\strut petals} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Solar} \colorbox{red!0}{\strut Lotus} \colorbox{red!1}{\strut cosmic} \colorbox{red!1}{\strut physical} \colorbox{red!1}{\strut plane} \colorbox{red!0}{\strut lower} \colorbox{red!1}{\strut three} \colorbox{red!1}{\strut planes} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut cosmic} \colorbox{red!1}{\strut physical} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut synthesizers} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut three} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut our} \colorbox{red!3}{\strut Planetary} \colorbox{red!5}{\strut Logos} \colorbox{red!4}{\strut Uranus} \colorbox{red!3}{\strut Planetary} \colorbox{red!1}{\strut Spirit} \colorbox{red!1}{\strut Neptune} \colorbox{red!1}{\strut Nameless} \colorbox{red!0}{\strut One} \colorbox{red!2}{\strut Saturn} \colorbox{red!1}{\strut Sanat} \colorbox{red!0}{\strut Kumara} \colorbox{red!0}{\strut Lets} \colorbox{red!0}{\strut suppose} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut ask} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut following} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut thought} \colorbox{red!0}{\strut experiment} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut planetary} \colorbox{red!5}{\strut logos} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut fact} \colorbox{red!2}{\strut Saturn} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut Yes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut extent} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut contacting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut relating} \colorbox{red!0}{\strut through} \colorbox{red!1}{\strut Sanat} \colorbox{red!0}{\strut Kumara} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut synthesizing} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut cosmic} \colorbox{red!1}{\strut physical} \colorbox{red!1}{\strut plane} \colorbox{red!0}{\strut b} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut planetary} \colorbox{red!5}{\strut logos} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut fact} \colorbox{red!1}{\strut Neptune} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut Yes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut extent} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut contacting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut relating} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Nameless} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut synthesizing} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut cosmic} \colorbox{red!0}{\strut astral} \colorbox{red!1}{\strut plane} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut c} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut planetary} \colorbox{red!5}{\strut logos} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut fact} \colorbox{red!4}{\strut Uranus} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut Yes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut extent} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut contacting} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut relating} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Planetary} \colorbox{red!1}{\strut Spirit} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut synthesizing} \colorbox{red!1}{\strut energy} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut cosmic} \colorbox{red!1}{\strut mental} \colorbox{red!1}{\strut plane} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut perhaps} \colorbox{red!0}{\strut reveal} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut stage} \colorbox{red!0}{\strut reached} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut questioning} \colorbox{red!1}{\strut consciousness} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut fixed} \colorbox{red!0}{\strut underlying} \colorbox{red!1}{\strut reality} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut beg} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut final} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Planetary} \colorbox{red!5}{\strut Logos} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut fact} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Solar} \colorbox{red!5}{\strut Logos} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut Yes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut extent} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut expression} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Solar} \colorbox{red!0}{\strut Will} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut manifestation} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut correspondence} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut human} \colorbox{red!0}{\strut arena} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut Am} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut body} \colorbox{red!0}{\strut ?} 
}}}
\end{CJK*}

query: vines shade

94:zones, 88:shade, 53:flowers, 49:flower, 35:size, 27:common, 26:plant, 25:name, 24:scarified, 23:scientific


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Common} \colorbox{red!2}{\strut name} \colorbox{red!1}{\strut Scientific} \colorbox{red!2}{\strut name} \colorbox{red!6}{\strut Zones} \colorbox{red!3}{\strut Flower} \colorbox{red!2}{\strut Size} \colorbox{red!1}{\strut Exposure} \colorbox{red!0}{\strut Comments} \colorbox{red!1}{\strut Canary} \colorbox{red!1}{\strut bird} \colorbox{red!1}{\strut vine} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Canary} \colorbox{red!1}{\strut creeper} \colorbox{red!0}{\strut Tropaeolum} \colorbox{red!0}{\strut peregrium} \colorbox{red!1}{\strut Annual} \colorbox{red!1}{\strut Yellow} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!0}{\strut Edible} \colorbox{red!3}{\strut flowers} \colorbox{red!1}{\strut produced} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut frost} \colorbox{red!1}{\strut Cape} \colorbox{red!1}{\strut honeysuckle} \colorbox{red!0}{\strut Tecomaria} \colorbox{red!0}{\strut capensis} \colorbox{red!0}{\strut 8-9} \colorbox{red!0}{\strut Orange-scarlet} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!0}{\strut Quasiclimber} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut tolerant} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut heat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut drought} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut coastal} \colorbox{red!0}{\strut conditions} \colorbox{red!1}{\strut Cardinal} \colorbox{red!0}{\strut climber} \colorbox{red!0}{\strut Ipomoea} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut multifida} \colorbox{red!1}{\strut Annual} \colorbox{red!1}{\strut Red} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!1}{\strut Seeds} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut scarified} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut soaked} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut aid} \colorbox{red!1}{\strut germination} \colorbox{red!0}{\strut Carolina} \colorbox{red!0}{\strut jasmine} \colorbox{red!0}{\strut Gelsemium} \colorbox{red!0}{\strut sempervirens} \colorbox{red!0}{\strut 7-9} \colorbox{red!1}{\strut Yellow} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!1}{\strut Yellow} \colorbox{red!3}{\strut flowers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut spring} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut native} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut foliage} \colorbox{red!0}{\strut bronzes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut winter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut plant} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut toxic} \colorbox{red!0}{\strut Chilean} \colorbox{red!1}{\strut glory} \colorbox{red!3}{\strut flower} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Glory} \colorbox{red!1}{\strut vine} \colorbox{red!0}{\strut Eccremocarpus} \colorbox{red!1}{\strut scaber} \colorbox{red!1}{\strut Annual} \colorbox{red!1}{\strut Yellow} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut red} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut Start} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut seeds} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut transplant} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut thrives} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut heat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut tubular} \colorbox{red!3}{\strut flowers} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut summer} \colorbox{red!0}{\strut Cross} \colorbox{red!1}{\strut vine} \colorbox{red!0}{\strut Bignonia} \colorbox{red!0}{\strut capreolata} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Anisostichus} \colorbox{red!0}{\strut capreolata} \colorbox{red!0}{\strut 6-9} \colorbox{red!0}{\strut Orange-red} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!0}{\strut Evergreen} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut semi-evergreen} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut native} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut flowers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut mid-spring} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut leaves} \colorbox{red!1}{\strut take} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut purplish} \colorbox{red!1}{\strut color} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut winter} \colorbox{red!0}{\strut Cypress} \colorbox{red!1}{\strut vine} \colorbox{red!0}{\strut Ipomoea} \colorbox{red!0}{\strut quamoclit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Quamoclit} \colorbox{red!0}{\strut pennata} \colorbox{red!1}{\strut Annual} \colorbox{red!1}{\strut Red} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!1}{\strut Seeds} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut scarified} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut soaked} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut aid} \colorbox{red!1}{\strut germination} \colorbox{red!0}{\strut Firecracker} \colorbox{red!1}{\strut vine} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Spanish} \colorbox{red!0}{\strut flag} \colorbox{red!0}{\strut Mina} \colorbox{red!0}{\strut lobata} \colorbox{red!1}{\strut Annual} \colorbox{red!0}{\strut Reddish-orange} \colorbox{red!1}{\strut fading} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut orange} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut yellow} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut white} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!1}{\strut Seeds} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut scarified} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut soaked} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut aid} \colorbox{red!1}{\strut germination} \colorbox{red!1}{\strut Honeysuckle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Coral} \colorbox{red!0}{\strut Lonicera} \colorbox{red!0}{\strut sempervirens} \colorbox{red!0}{\strut 5-9} \colorbox{red!0}{\strut Coral} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut red} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut yellow} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sun} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partial} \colorbox{red!6}{\strut shade} \colorbox{red!0}{\strut Trumpet-shaped} \colorbox{red!3}{\strut flowers} \colorbox{red!0}{\strut mid-spring} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fall} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut native} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut cultivars} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sulfurea} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut yellow} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Superba} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Magnifica} 
}}}
\end{CJK*}

98:shade, 71:what, 56:vine, 55:plants, 49:plant, 47:good, 43:gardening, 30:grow, 27:nature, 24:hydrangea


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 19} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Subscribe} \colorbox{red!0}{\strut Today} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Text} \colorbox{red!0}{\strut size} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Q} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!4}{\strut good} \colorbox{red!4}{\strut vine} \colorbox{red!1}{\strut for} \colorbox{red!8}{\strut shade} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut BY} \colorbox{red!0}{\strut KATHY} \colorbox{red!0}{\strut VAN} \colorbox{red!1}{\strut MULLEKOM} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 757-247-4781} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 24} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut NEWPORT} \colorbox{red!0}{\strut NEWS} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Q.} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut enjoyed} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut talk} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Ford} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Colony} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut morning} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut practical} \colorbox{red!0}{\strut advice} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut maintenance} \colorbox{red!4}{\strut plants} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut poet} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut laurel} \colorbox{red!0}{\strut finally} \colorbox{red!0}{\strut got} \colorbox{red!1}{\strut named} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut wondering} \colorbox{red!6}{\strut what} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut inherited} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut garden} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ago} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut moved} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut shed} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut pesticides} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!1}{\strut experimenting} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut see} \colorbox{red!6}{\strut what} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut survive} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Periwinkle} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut yarrow} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut huge} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut lily-of-the-valley} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut eaten} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut thought} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut were} \colorbox{red!1}{\strut poisonous} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut glad} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut hear} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ca} \colorbox{red!0}{\strut nt} \colorbox{red!2}{\strut grow} \colorbox{red!1}{\strut daphne} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut killed} \colorbox{red!0}{\strut two} \colorbox{red!1}{\strut pretty} \colorbox{red!0}{\strut ones} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Daphne} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut middle} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut trellis} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut shade} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut recommend} \colorbox{red!1}{\strut a} \colorbox{red!4}{\strut vine} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut likes} \colorbox{red!8}{\strut shade} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Thank} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Hazel} \colorbox{red!1}{\strut Daphne} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut e-mail} \colorbox{red!0}{\strut A.} \colorbox{red!1}{\strut Hazel} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut climbing} \colorbox{red!2}{\strut hydrangea} \colorbox{red!2}{\strut likes} \colorbox{red!8}{\strut shade} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut look} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut Moonlight} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut few} \colorbox{red!2}{\strut flowers} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut silvery} \colorbox{red!1}{\strut foliage} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Autumn} \colorbox{red!1}{\strut clematis} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut wonderful} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut blooms} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut late} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Our} \colorbox{red!0}{\strut native} \colorbox{red!1}{\strut Virginia} \colorbox{red!1}{\strut creeper} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut nice} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut vigorous} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut needs} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut strong} \colorbox{red!1}{\strut trellis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fatshedra} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut nice} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!1}{\strut grown} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut bush} \colorbox{red!2}{\strut ivy} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut needs} \colorbox{red!1}{\strut help} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut climb} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut ties} \colorbox{red!1}{\strut are} \colorbox{red!4}{\strut good} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut vote} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut Moonlight} \colorbox{red!2}{\strut hydrangea} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut happy} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut are} \colorbox{red!3}{\strut gardening} \colorbox{red!0}{\strut without} \colorbox{red!1}{\strut pesticides} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!1}{\strut found} \colorbox{red!1}{\strut having} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut plants} \colorbox{red!0}{\strut attracts} \colorbox{red!1}{\strut beneficial} \colorbox{red!4}{\strut plants} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut seldom} \colorbox{red!0}{\strut have} \colorbox{red!4}{\strut plant} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Take} \colorbox{red!0}{\strut care} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Kathy} \colorbox{red!0}{\strut Want} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut home} 
}}}
\end{CJK*}

query: septic system design

35:types, 29:septic, 28:apedia, 27:systems, 27:system, 25:septics, 21:water, 19:tank, 16:designs, 16:building


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut InspectAPedia} \colorbox{red!1}{\strut Building} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Environmental} \colorbox{red!1}{\strut Inspection} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Testing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Diagnosis} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Repair} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Problem} \colorbox{red!0}{\strut Prevention} \colorbox{red!0}{\strut Advice} \colorbox{red!0}{\strut InspectAPedia} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Air} \colorbox{red!1}{\strut Conditioning} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Electrical} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Environment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Exteriors} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Heating} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Inspection} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Insulate} \colorbox{red!1}{\strut Ventilate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Interiors} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Mold} \colorbox{red!0}{\strut InspectTest} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Plumbing} \colorbox{red!1}{\strut Water} \colorbox{red!2}{\strut Septic} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Roofing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Structure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Directory} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Professionals} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Inspect} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut Test} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Building} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!1}{\strut HOME} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut INFO} \colorbox{red!0}{\strut ARTICLES} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Owners} \colorbox{red!2}{\strut Septic} \colorbox{red!2}{\strut System} \colorbox{red!1}{\strut Design} \colorbox{red!2}{\strut Septic} \colorbox{red!1}{\strut Inspection} \colorbox{red!1}{\strut Testing} \colorbox{red!2}{\strut Septic} \colorbox{red!0}{\strut Maintenance} \colorbox{red!1}{\strut Repair} \colorbox{red!2}{\strut Septic} \colorbox{red!0}{\strut Component} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Product} \colorbox{red!0}{\strut Suppliers} \colorbox{red!2}{\strut Septic} \colorbox{red!0}{\strut Videos} \colorbox{red!1}{\strut HOME} \colorbox{red!0}{\strut BUYERS} \colorbox{red!0}{\strut GUIDE} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut ONLINE} \colorbox{red!0}{\strut BOOK} \colorbox{red!0}{\strut INTRODUCTION} \colorbox{red!0}{\strut SAFETY} \colorbox{red!0}{\strut WARNINGS} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!2}{\strut SYSTEM} \colorbox{red!1}{\strut DESIGN} \colorbox{red!0}{\strut BASICS} \colorbox{red!0}{\strut PERC} \colorbox{red!1}{\strut TESTS} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut TANK} \colorbox{red!1}{\strut SIZE} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut TANK} \colorbox{red!0}{\strut DEPTH} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut TANK} \colorbox{red!0}{\strut TEES} \colorbox{red!0}{\strut FIELD} \colorbox{red!1}{\strut SIZE} \colorbox{red!0}{\strut FIELD} \colorbox{red!0}{\strut SHAPE} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut CLEARANCES} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut TANK} \colorbox{red!0}{\strut PUMPING} \colorbox{red!0}{\strut FREQUENCY} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut TANK} \colorbox{red!0}{\strut PUMPING} \colorbox{red!0}{\strut PROCEDURE} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut PUMPING} \colorbox{red!1}{\strut REPAIR} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut TREATMENTS} \colorbox{red!0}{\strut STEEP} \colorbox{red!0}{\strut SLOPE} \colorbox{red!1}{\strut DESIGNS} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut DESIGN} \colorbox{red!0}{\strut ALTERNATIVES} \colorbox{red!1}{\strut Wastewater} \colorbox{red!1}{\strut Treatment} \colorbox{red!0}{\strut Levels} \colorbox{red!1}{\strut Wastewater} \colorbox{red!0}{\strut Dispersal} \colorbox{red!1}{\strut Methods} \colorbox{red!0}{\strut Master} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Septic} \colorbox{red!2}{\strut System} \colorbox{red!2}{\strut Types} \colorbox{red!1}{\strut AEROBIC} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut CESSPOOLS} \colorbox{red!1}{\strut DOSING} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut GRAVITYSIPHON} \colorbox{red!1}{\strut DOSING} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut PRESSURE} \colorbox{red!0}{\strut DRYWELLS} \colorbox{red!0}{\strut EVAPORATION-TRANSPIRATION} \colorbox{red!0}{\strut GRAVELLESS} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut GREYWATER} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut LAGOON} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut MEDIA} \colorbox{red!0}{\strut FILTER} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GREYWATER} \colorbox{red!0}{\strut FILTERS} \colorbox{red!1}{\strut MOUND} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut RAISED} \colorbox{red!1}{\strut BED} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut SAND} \colorbox{red!1}{\strut BED} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!1}{\strut SEWAGE} \colorbox{red!1}{\strut TREATMENT} \colorbox{red!2}{\strut SYSTEMS} \colorbox{red!0}{\strut STEEP} \colorbox{red!0}{\strut SLOPE} \colorbox{red!1}{\strut DESIGNS} \colorbox{red!0}{\strut TOILET} \colorbox{red!0}{\strut ALTERNATIVES} \colorbox{red!1}{\strut ALTERNATIVE} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut DESIGNERS} \colorbox{red!1}{\strut ALTERNATIVE} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!1}{\strut PRODUCTS} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut INSPECTIONS} \colorbox{red!0}{\strut DEFINITIONS} \colorbox{red!0}{\strut FAILURE} \colorbox{red!0}{\strut LAWSUIT} \colorbox{red!0}{\strut FLOOD} \colorbox{red!0}{\strut RESPONSE} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut REFERENCES} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut CONSULTANTS} \colorbox{red!2}{\strut SEPTIC} \colorbox{red!0}{\strut AUTHORITIES} \colorbox{red!0}{\strut BOOKS} \colorbox{red!0}{\strut REFS} \colorbox{red!0}{\strut CODES} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut InspectAPedia} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!1}{\strut Air} \colorbox{red!1}{\strut Conditioning} \colorbox{red!0}{\strut InspectAPedia} \colorbox{red!0}{\strut Bookstore} \colorbox{red!1}{\strut Electrical} \colorbox{red!1}{\strut Environment} \colorbox{red!0}{\strut Exteriors} \colorbox{red!1}{\strut Heating} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Inspection} \colorbox{red!0}{\strut Insulate} \colorbox{red!1}{\strut Ventilate} \colorbox{red!0}{\strut Interiors} \colorbox{red!1}{\strut Mold} \colorbox{red!0}{\strut InspectTest} \colorbox{red!1}{\strut Roofing} \colorbox{red!1}{\strut Plumbing} \colorbox{red!1}{\strut Water} \colorbox{red!2}{\strut Septic} \colorbox{red!0}{\strut Structure} \colorbox{red!0}{\strut Accuracy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Bias} \colorbox{red!0}{\strut Pledge} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Master} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Types} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Septic} \colorbox{red!2}{\strut Systems} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Septic} \colorbox{red!2}{\strut System} \colorbox{red!1}{\strut Designs} \colorbox{red!0}{\strut SepticAPedia} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut inspect-ny.com} \colorbox{red!2}{\strut Types} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Septic} \colorbox{red!2}{\strut Systems} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Alternative} \colorbox{red!2}{\strut Septic} \colorbox{red!2}{\strut System} \colorbox{red!1}{\strut Designs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Master} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Descriptions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Kinds} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Septic} \colorbox{red!2}{\strut Systems} \colorbox{red!1}{\strut Alternative} \colorbox{red!2}{\strut septic} \colorbox{red!2}{\strut system} \colorbox{red!1}{\strut designs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut problem} \colorbox{red!0}{\strut sites} \colorbox{red!0}{\strut Description} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut alternative} \colorbox{red!2}{\strut septic} \colorbox{red!2}{\strut systems} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut design} \colorbox{red!0}{\strut criteria} 
}}}
\end{CJK*}

89:septics, 88:septic, 86:engineering, 85:system, 83:systems, 82:engineers, 71:south, 68:jersey, 49:new, 22:design


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 1-866-SEPTICS} \colorbox{red!7}{\strut engineers} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut septics.com} \colorbox{red!6}{\strut South} \colorbox{red!6}{\strut jersey} \colorbox{red!7}{\strut engineers} \colorbox{red!1}{\strut llc} \colorbox{red!1}{\strut Professional} \colorbox{red!7}{\strut Septic} \colorbox{red!7}{\strut System} \colorbox{red!2}{\strut Design} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Engineering} \colorbox{red!1}{\strut Soil} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Site} \colorbox{red!1}{\strut Analysis} \colorbox{red!1}{\strut Repair} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Remediation} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Renovation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Restoration} \colorbox{red!0}{\strut Feasibility} \colorbox{red!0}{\strut andPermitting} \colorbox{red!1}{\strut services} \colorbox{red!1}{\strut Advanced} \colorbox{red!1}{\strut Pinelands} \colorbox{red!8}{\strut Septics} \colorbox{red!7}{\strut Systems} \colorbox{red!1}{\strut Inspection} \colorbox{red!1}{\strut Services} \colorbox{red!7}{\strut Engineering} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Innovative} \colorbox{red!1}{\strut Solutions} \colorbox{red!0}{\strut 1-866-SEPTICS} \colorbox{red!7}{\strut engineers} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut septics.com} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut septic} \colorbox{red!7}{\strut systems} \colorbox{red!6}{\strut South} \colorbox{red!6}{\strut Jersey} \colorbox{red!7}{\strut Engineers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut L.L.C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut has} \colorbox{red!1}{\strut successfully} \colorbox{red!2}{\strut designed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut 12312006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10,000} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut year} \colorbox{red!1}{\strut count} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut SOME} \colorbox{red!0}{\strut OF} \colorbox{red!0}{\strut OUR} \colorbox{red!1}{\strut SERVICES} \colorbox{red!1}{\strut Active} \colorbox{red!1}{\strut Member} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut New} \colorbox{red!6}{\strut Jersey} \colorbox{red!0}{\strut BuildersAssociation} \colorbox{red!1}{\strut Builders} \colorbox{red!1}{\strut League} \colorbox{red!0}{\strut ofSouth} \colorbox{red!6}{\strut Jersey} \colorbox{red!1}{\strut American} \colorbox{red!1}{\strut Society} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Civil} \colorbox{red!7}{\strut Engineers} \colorbox{red!4}{\strut New} \colorbox{red!6}{\strut Jersey} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pennsylvania} \colorbox{red!7}{\strut Septic} \colorbox{red!1}{\strut Management} \colorbox{red!1}{\strut Association} \colorbox{red!4}{\strut New} \colorbox{red!6}{\strut Jersey} \colorbox{red!1}{\strut Society} \colorbox{red!0}{\strut ofProfessional} \colorbox{red!7}{\strut Engineers} 
}}}
\end{CJK*}

query: paralegal

100:paralegal, 99:paralegals, 61:texas, 42:lake, 38:clear, 32:schools, 29:school, 29:degree, 28:degrees, 26:training


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 800-446-6931} \colorbox{red!2}{\strut Texas} \colorbox{red!3}{\strut Paralegal} \colorbox{red!1}{\strut Training} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Paralegal} \colorbox{red!1}{\strut Schools} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut paralegal} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut clear} \colorbox{red!1}{\strut lake} \colorbox{red!2}{\strut texas} \colorbox{red!2}{\strut Texas} \colorbox{red!3}{\strut Paralegal} \colorbox{red!1}{\strut Training} \colorbox{red!3}{\strut Paralegal} \colorbox{red!1}{\strut Schools} \colorbox{red!3}{\strut Paralegal} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut Houston} \colorbox{red!0}{\strut Houston} \colorbox{red!3}{\strut Paralegal} \colorbox{red!1}{\strut Program} \colorbox{red!0}{\strut conroe} \colorbox{red!2}{\strut texas} \colorbox{red!3}{\strut paralegal} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut pearland} \colorbox{red!2}{\strut texas} \colorbox{red!3}{\strut paralegal} \colorbox{red!1}{\strut training} \colorbox{red!1}{\strut program} \colorbox{red!2}{\strut texas} \colorbox{red!0}{\strut accredited} \colorbox{red!3}{\strut paralegal} \colorbox{red!1}{\strut schools} \colorbox{red!0}{\strut houston} \colorbox{red!2}{\strut texas} \colorbox{red!3}{\strut paralegal} \colorbox{red!1}{\strut training} \colorbox{red!0}{\strut baytown} \colorbox{red!2}{\strut texas} \colorbox{red!3}{\strut paralegal} \colorbox{red!0}{\strut certification} \colorbox{red!0}{\strut cypress} \colorbox{red!2}{\strut texas} \colorbox{red!3}{\strut paralegal} \colorbox{red!0}{\strut university} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut paralegal} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut clear} \colorbox{red!1}{\strut lake} \colorbox{red!2}{\strut texas} \colorbox{red!0}{\strut humble} \colorbox{red!2}{\strut texas} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut assistant} \colorbox{red!1}{\strut training} \colorbox{red!0}{\strut richmond} \colorbox{red!2}{\strut texas} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut assistant} \colorbox{red!0}{\strut classes} \colorbox{red!0}{\strut pasadena} \colorbox{red!2}{\strut texas} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut assistant} \colorbox{red!1}{\strut schools} \colorbox{red!0}{\strut top} \colorbox{red!3}{\strut paralegal} \colorbox{red!1}{\strut schools} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut houston} \colorbox{red!2}{\strut texas} \colorbox{red!3}{\strut paralegal} \colorbox{red!0}{\strut studies} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut cypress} \colorbox{red!2}{\strut texas} \colorbox{red!0}{\strut pasadena} \colorbox{red!2}{\strut texas} \colorbox{red!3}{\strut paralegal} \colorbox{red!1}{\strut education} \colorbox{red!3}{\strut paralegal} \colorbox{red!0}{\strut certificate} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut galveston} \colorbox{red!2}{\strut texas} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut assistant} \colorbox{red!0}{\strut certification} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut houston} \colorbox{red!0}{\strut best} \colorbox{red!3}{\strut paralegal} \colorbox{red!1}{\strut schools} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut pearland} \colorbox{red!2}{\strut texas} \colorbox{red!1}{\strut legal} \colorbox{red!1}{\strut assistant} \colorbox{red!1}{\strut degree} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut sugar} \colorbox{red!0}{\strut land} \colorbox{red!2}{\strut texas} \colorbox{red!0}{\strut ABA} \colorbox{red!3}{\strut Paralegal} \colorbox{red!1}{\strut Schools} \colorbox{red!0}{\strut Become} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Paralegal} \colorbox{red!0}{\strut In} \colorbox{red!1}{\strut Clear} \colorbox{red!1}{\strut Lake} \colorbox{red!2}{\strut Texas} \colorbox{red!0}{\strut Become} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Paralegal} \colorbox{red!0}{\strut Today} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut expected} \colorbox{red!0}{\strut growth} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut field} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut individuals} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut interest} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut law} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut consider} \colorbox{red!0}{\strut pursuing} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut enable} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!3}{\strut paralegals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut prospective} \colorbox{red!0}{\strut employers} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut paralegals} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!1}{\strut law} \colorbox{red!0}{\strut firms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut government} \colorbox{red!0}{\strut agencies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut private} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Individuals} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!3}{\strut paralegals} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut pursue} \colorbox{red!0}{\strut careers} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut organizations} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut immigration} \colorbox{red!1}{\strut law} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut family} \colorbox{red!1}{\strut law} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Different} \colorbox{red!0}{\strut Paths} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Become} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Paralegal} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut single} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut training} \colorbox{red!0}{\strut path} \colorbox{red!0}{\strut required} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut jobs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut ways} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut paralegal} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut choosing} \colorbox{red!0}{\strut among} \colorbox{red!1}{\strut education} \colorbox{red!0}{\strut centers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut prospective} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut beyond} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut jobs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut consider} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut long-term} \colorbox{red!0}{\strut careers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut obtaining} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut associate} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut degree} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut student} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut open} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut doors} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut otherwise} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Those} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut college} \colorbox{red!1}{\strut degrees} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut further} \colorbox{red!1}{\strut training} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut changing} \colorbox{red!0}{\strut careers} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut attend} \colorbox{red!0}{\strut certificate} \colorbox{red!1}{\strut programs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Programs} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut approved} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Bar} 
}}}
\end{CJK*}

96:accounting, 96:accountant, 94:paralegal, 62:what, 44:how, 39:old, 31:cpa, 31:career, 29:salaries, 29:job


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut my.indeed} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Create} \colorbox{red!1}{\strut Account} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Jobs} \colorbox{red!2}{\strut Salaries} \colorbox{red!1}{\strut Trends} \colorbox{red!0}{\strut Forums} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut job} \colorbox{red!1}{\strut title} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut keywords} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut Forums} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Job} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Accountant} \colorbox{red!2}{\strut Career} \colorbox{red!2}{\strut Change} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Accountant} \colorbox{red!0}{\strut or} \colorbox{red!7}{\strut Paralegal} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut new} \colorbox{red!1}{\strut comments} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut email} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Email} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut cancel} \colorbox{red!1}{\strut email} \colorbox{red!0}{\strut alerts} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut anytime} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tara} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Chicago} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Illinois} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut months} \colorbox{red!0}{\strut ago} \colorbox{red!0}{\strut Hello} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut 35} \colorbox{red!1}{\strut years} \colorbox{red!3}{\strut old} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut would} \colorbox{red!1}{\strut like} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut start} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut new} \colorbox{red!2}{\strut career} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut varied} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut experienced} \colorbox{red!0}{\strut past} \colorbox{red!2}{\strut job} \colorbox{red!0}{\strut profile} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut model} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut bartender} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut administrative} \colorbox{red!0}{\strut assistant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut photography} \colorbox{red!0}{\strut assistant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut film} \colorbox{red!0}{\strut production} \colorbox{red!1}{\strut manager} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut media} \colorbox{red!0}{\strut analyst} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut pharmaceutical} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut relatively} \colorbox{red!0}{\strut stable} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut well-paying} \colorbox{red!2}{\strut career} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut willing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut land} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut job} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut BA} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Anthropology} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut paralegal} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut should} \colorbox{red!1}{\strut obtain} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut certificate} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut ABA-approved} \colorbox{red!1}{\strut program} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut become} \colorbox{red!0}{\strut an} \colorbox{red!7}{\strut accountant} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 2nd} \colorbox{red!1}{\strut Bachelor} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut try} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Master} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut Accounting} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Also} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut what} \colorbox{red!1}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut jobs} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut salaries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut non-CPA} \colorbox{red!7}{\strut accountant} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut degree} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut Accounting} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Which} \colorbox{red!2}{\strut job} \colorbox{red!1}{\strut would} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut understand} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut ultimately} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut choice} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut industries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut brand} \colorbox{red!1}{\strut new} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut would} \colorbox{red!1}{\strut like} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut objective} \colorbox{red!0}{\strut opinions} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut people} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Becoming} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut paralegal} \colorbox{red!0}{\strut seems} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut quicker} \colorbox{red!1}{\strut process} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut multiple} \colorbox{red!0}{\strut forums} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut heard} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut horrors} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut stress} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut field} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut note} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut would} \colorbox{red!0}{\strut enjoy} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!2}{\strut jobs} \colorbox{red!0}{\strut equally} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut How} \colorbox{red!1}{\strut would} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut compare} \colorbox{red!2}{\strut job} \colorbox{red!0}{\strut stability} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut job} \colorbox{red!0}{\strut growthopenings} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

query: hip fractures

98:fractures, 98:fracture, 88:hip, 66:what, 52:causes, 48:cause, 32:symptoms, 27:injury, 27:definition, 23:cost


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut HealthCentral.com} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Diseases} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Injuries} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut Encyclopedia} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Diseases} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Conditions} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut partner} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut chronic} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ChronicPainConnection.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut ways} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut chronic} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut relief} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut right} \colorbox{red!1}{\strut treatment} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut chronic} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut Join} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut chronic} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut group} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut B} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut D} \colorbox{red!0}{\strut E} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut H} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut J} \colorbox{red!0}{\strut K} \colorbox{red!0}{\strut L} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut N} \colorbox{red!0}{\strut O} \colorbox{red!0}{\strut P} \colorbox{red!0}{\strut R} \colorbox{red!0}{\strut S} \colorbox{red!0}{\strut T} \colorbox{red!0}{\strut U} \colorbox{red!0}{\strut V} \colorbox{red!0}{\strut W} \colorbox{red!0}{\strut Y} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Definition} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Description} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!2}{\strut Causes} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!1}{\strut Symptoms} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!1}{\strut Treatment} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!0}{\strut Prevention} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut ask} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Doctor} \colorbox{red!0}{\strut About} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Definition} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut fractures} \colorbox{red!0}{\strut are} \colorbox{red!4}{\strut fractures} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut neck} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut femur} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut long} \colorbox{red!1}{\strut bone} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut comprises} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut upper} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut leg} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut femoral} \colorbox{red!1}{\strut neck} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut shaft} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut bone} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut head} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut femur} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ball} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut fits} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut socket} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut hip} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Description} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut fractures} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut major} \colorbox{red!0}{\strut public} \colorbox{red!1}{\strut health} \colorbox{red!0}{\strut problem} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut approximately} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut billion} \colorbox{red!0}{\strut dollars} \colorbox{red!0}{\strut annually} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut common} \colorbox{red!2}{\strut cause} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut admission} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut nursing} \colorbox{red!0}{\strut homes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut accounting} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut 60,000} \colorbox{red!0}{\strut admissions} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Osteoporosis} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut elderly} \colorbox{red!0}{\strut contributes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!4}{\strut fractures} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!1}{\strut elderly} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut break} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut hip} \colorbox{red!0}{\strut face} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut broad} \colorbox{red!0}{\strut array} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut transcend} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut treatment} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut injury} \colorbox{red!0}{\strut itself} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut elderly} \colorbox{red!0}{\strut person} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut independent} \colorbox{red!0}{\strut existence} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut impacted} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fall} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut causes} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut event} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut forever} \colorbox{red!0}{\strut lessen} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut patient} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut level} 
}}}
\end{CJK*}

89:fractures, 89:fracture, 83:hip, 72:hips, 64:what, 62:fractured, 53:broken, 46:causes, 44:caused, 35:break


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Orthopedics} \colorbox{red!0}{\strut Home} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut Orthopedics} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Orthopedics} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut Hurts} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Treatment} \colorbox{red!0}{\strut Options} \colorbox{red!2}{\strut Broken} \colorbox{red!1}{\strut Bones} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Orthopedics} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut Forum} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut Fracture} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Jonathan} \colorbox{red!0}{\strut Cluett} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut M.D} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut About.com} \colorbox{red!0}{\strut Updated} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut About.com} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Disease} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Condition} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut reviewed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Medical} \colorbox{red!0}{\strut Review} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut hip} \colorbox{red!1}{\strut pain} \colorbox{red!1}{\strut osteoporosis} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut versus} \colorbox{red!2}{\strut break} \colorbox{red!4}{\strut hip} \colorbox{red!1}{\strut replacement} \colorbox{red!0}{\strut A} \colorbox{red!2}{\strut broken} \colorbox{red!4}{\strut hip} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut common} \colorbox{red!1}{\strut injury} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut elderly} \colorbox{red!0}{\strut individuals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fractures} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut common} \colorbox{red!2}{\strut broken} \colorbox{red!1}{\strut bone} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut requires} \colorbox{red!1}{\strut hospitalization} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 300,000} \colorbox{red!0}{\strut Americans} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut hospitalized} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut broken} \colorbox{red!4}{\strut hip} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut mean} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut How} \colorbox{red!0}{\strut do} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fractures} \colorbox{red!1}{\strut happen} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut fractures} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut elderly} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut often} \colorbox{red!2}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut fall} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut seemingly} \colorbox{red!0}{\strut insignificant} \colorbox{red!1}{\strut fall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut younger} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut stronger} \colorbox{red!1}{\strut bones} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut common} \colorbox{red!2}{\strut causes} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut broken} \colorbox{red!4}{\strut hip} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut high-energy} \colorbox{red!1}{\strut injuries} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut car} \colorbox{red!0}{\strut accidents} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Hip} \colorbox{red!4}{\strut fractures} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut bone} \colorbox{red!0}{\strut weakened} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut tumor} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut infection} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut problem} \colorbox{red!0}{\strut called} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pathologic} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!2}{\strut broken} \colorbox{red!4}{\strut hip} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut elderly} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut explained} \colorbox{red!0}{\strut primarily} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut weak} \colorbox{red!1}{\strut bones} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut osteoporosis} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Elderly} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut osteoporosis} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut higher} \colorbox{red!0}{\strut risk} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut developing} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut without} \colorbox{red!1}{\strut osteoporosis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut risk} \colorbox{red!0}{\strut factors} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!4}{\strut hip} \colorbox{red!4}{\strut fracture} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut female} \colorbox{red!0}{\strut sex} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Caucasian} \colorbox{red!0}{\strut race} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut slightly} \colorbox{red!0}{\strut built} \colorbox{red!0}{\strut individuals} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut physical} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut How} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut problem} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut broken} \colorbox{red!3}{\strut hips} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut osteoporosis} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Osteoporosis} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut condition} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut causes} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut bone} \colorbox{red!0}{\strut mass} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut composition} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut bone} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut normal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut thinner} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut normal} \colorbox{red!0}{\strut individuals} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut thinner} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

query: brooks brothers clearance

101:brooks, 97:brothers, 45:what, 31:ebates, 31:cash, 24:sales, 22:back, 21:coupons, 21:buy, 20:coupon


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut --} \colorbox{red!0}{\strut Select} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut store} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Ebates} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Sign} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut saving} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Members} \colorbox{red!0}{\strut Log} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Stores} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Ebates} \colorbox{red!0}{\strut Tell-A-Friend} \colorbox{red!0}{\strut Blog} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut receive} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut sales} \colorbox{red!0}{\strut commission} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut stores} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut buy} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut pass} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut portion} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut commission} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut amount} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut Ebates} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut four} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut forms} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fill} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut Ebates} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut buy} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut earn} \colorbox{red!1}{\strut cash} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SAVINGS} \colorbox{red!0}{\strut AT} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DESCRIPTION} \colorbox{red!1}{\strut COUPONS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SPECIALS} \colorbox{red!0}{\strut DESCRIPTION} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut leading} \colorbox{red!0}{\strut destination} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut women} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut men} \colorbox{red!0}{\strut apparel} \colorbox{red!1}{\strut purchases} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!0}{\strut carries} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut complete} \colorbox{red!0}{\strut inventory} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut dresses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut women} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut men} \colorbox{red!0}{\strut suits} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut shoes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut accessories} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Browse} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!1}{\strut deals} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!1}{\strut coupons} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut specials} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut sales} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!1}{\strut coupon} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut promo} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut offer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut simply} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!0}{\strut shopping} \colorbox{red!0}{\strut cart} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut redeem} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut COUPONS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SPECIALS} \colorbox{red!0}{\strut Save} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 60} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut men} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut women} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut clearance} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut at} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!1}{\strut Sales} \colorbox{red!0}{\strut Save} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut Boys} \colorbox{red!0}{\strut Clearance} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut at} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut Sales} \colorbox{red!0}{\strut SAVE} \colorbox{red!0}{\strut AT} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!1}{\strut Rebates} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Receive} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Use} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!1}{\strut coupons} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!0}{\strut Discounts} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut latest} \colorbox{red!4}{\strut Brooks} \colorbox{red!4}{\strut Brothers} \colorbox{red!0}{\strut discounts} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut deals} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Appliances} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Hardware} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut stores} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut category} \colorbox{red!0}{\strut Sears} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Depot} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Compact} \colorbox{red!0}{\strut Appliance} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Cash} \colorbox{red!1}{\strut Back} \colorbox{red!0}{\strut Ace} 
}}}
\end{CJK*}

97:brooks, 89:brothers, 24:clearance, 22:deals, 20:stores, 17:shop, 15:coupons, 15:couponing, 14:grocery, 14:discounts


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut Business} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Finance} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!1}{\strut Email} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!1}{\strut Local} \colorbox{red!1}{\strut Bargains} \colorbox{red!1}{\strut Couponing} \colorbox{red!0}{\strut 101} \colorbox{red!1}{\strut Online} \colorbox{red!2}{\strut Deals} \colorbox{red!1}{\strut Free} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut Forum} \colorbox{red!1}{\strut Donna} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!1}{\strut Blog} \colorbox{red!0}{\strut By} \colorbox{red!1}{\strut Donna} \colorbox{red!0}{\strut L} \colorbox{red!0}{\strut Montaldo} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut About.com} \colorbox{red!1}{\strut Guide} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut 2001} \colorbox{red!0}{\strut MyBio} \colorbox{red!0}{\strut MyBlog} \colorbox{red!0}{\strut MyForum} \colorbox{red!1}{\strut Add} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut iGoogle} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut Yahoo} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut RSS} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut 60} \colorbox{red!1}{\strut Percent} \colorbox{red!1}{\strut Off} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut BrooksBrothers.com} \colorbox{red!0}{\strut Wednesday} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut BrooksBrothers.com} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut just} \colorbox{red!1}{\strut launched} \colorbox{red!0}{\strut their} \colorbox{red!2}{\strut Clearance} \colorbox{red!1}{\strut Event} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 60} \colorbox{red!1}{\strut percent} \colorbox{red!1}{\strut off} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut men} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut women} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut clearance} \colorbox{red!1}{\strut items} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 50} \colorbox{red!1}{\strut percent} \colorbox{red!1}{\strut off} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut boy} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut clearance} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Brooks} \colorbox{red!8}{\strut Brothers} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut known} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut excellent} \colorbox{red!0}{\strut quality} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut styling} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut classic} \colorbox{red!1}{\strut apparel} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut accessories} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Clearance} \colorbox{red!1}{\strut items} \colorbox{red!0}{\strut include} \colorbox{red!1}{\strut blazers} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut outerwear} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut dresses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut slacks} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut sweaters} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cashmere} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut handbags} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut shoes} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut ties} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Shop} \colorbox{red!1}{\strut Direct} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Men} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Women} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Clearance} \colorbox{red!2}{\strut Shop} \colorbox{red!1}{\strut Direct} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Boys} \colorbox{red!2}{\strut Clearance} \colorbox{red!0}{\strut Comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Posts} \colorbox{red!0}{\strut Prev} \colorbox{red!0}{\strut Comments} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut yet} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Leave} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Comment} \colorbox{red!1}{\strut Leave} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Comment} \colorbox{red!0}{\strut Name} \colorbox{red!1}{\strut Email} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut never} \colorbox{red!0}{\strut displayed} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut URL} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Comment} \colorbox{red!0}{\strut Line} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut paragraph} \colorbox{red!0}{\strut breaks} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut automatic} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut HTML} \colorbox{red!1}{\strut allowed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Say} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Discuss} \colorbox{red!0}{\strut Recent} \colorbox{red!1}{\strut Blog} \colorbox{red!0}{\strut Posts} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut 60} \colorbox{red!1}{\strut Percent} \colorbox{red!1}{\strut Off} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut BrooksBrothers.com} \colorbox{red!1}{\strut Printable} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Quit} \colorbox{red!1}{\strut Smoking} \colorbox{red!0}{\strut Aides} \colorbox{red!1}{\strut Grocery} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Community} \colorbox{red!1}{\strut Forum} \colorbox{red!0}{\strut Explore} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!1}{\strut Must} \colorbox{red!0}{\strut Reads} \colorbox{red!1}{\strut Grocery} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut Double} \colorbox{red!1}{\strut Coupons} \colorbox{red!1}{\strut Outlet} \colorbox{red!1}{\strut Mall} \colorbox{red!1}{\strut Shopping} \colorbox{red!1}{\strut Online} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Z} \colorbox{red!1}{\strut Cut} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Entertainment} \colorbox{red!1}{\strut Costs} \colorbox{red!1}{\strut Hotel} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Nationwide} \colorbox{red!0}{\strut Most} \colorbox{red!1}{\strut Popular} \colorbox{red!1}{\strut Printable} \colorbox{red!1}{\strut Pizza} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut Abercrombie} \colorbox{red!0}{\strut Fitch} \colorbox{red!1}{\strut Outlets} \colorbox{red!1}{\strut Printable} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Food} \colorbox{red!2}{\strut Stores} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut Double} \colorbox{red!1}{\strut Coupons} \colorbox{red!1}{\strut Discounts} \colorbox{red!0}{\strut For} \colorbox{red!1}{\strut Smoking} \colorbox{red!0}{\strut Aides} \colorbox{red!1}{\strut Free} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bargains} \colorbox{red!0}{\strut Newsletter} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Category} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut Online} \colorbox{red!1}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Deals} \colorbox{red!1}{\strut Apparel} \colorbox{red!2}{\strut Deals} \colorbox{red!1}{\strut Shopping} \colorbox{red!0}{\strut Tips} \colorbox{red!1}{\strut Baby} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Toy} \colorbox{red!2}{\strut Deals} \colorbox{red!0}{\strut Beauty} 
}}}
\end{CJK*}

query: sore throat

98:throats, 98:throat, 94:soreness, 94:sore, 58:caused, 58:cause, 56:causes, 32:pain, 29:symptoms, 26:painful


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Departments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut Patients} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Trials} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Doctor} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Topics} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut Internal} \colorbox{red!0}{\strut Medicine} \colorbox{red!4}{\strut Sore} \colorbox{red!4}{\strut throat} \colorbox{red!4}{\strut Sore} \colorbox{red!4}{\strut throat} \colorbox{red!4}{\strut Throat} \colorbox{red!0}{\strut anatomy} \colorbox{red!1}{\strut Strep} \colorbox{red!4}{\strut throat} \colorbox{red!1}{\strut Definition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut discomfort} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut scratchiness} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut makes} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut painful} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut swallow} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Alternative} \colorbox{red!0}{\strut Names} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Throat} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut sore} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pain} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut Considerations} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Sore} \colorbox{red!4}{\strut throats} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut common} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut soreness} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut worse} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut morning} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut improves} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut progresses} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Like} \colorbox{red!1}{\strut colds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut vast} \colorbox{red!0}{\strut majority} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throats} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut viral} \colorbox{red!1}{\strut infections} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut means} \colorbox{red!0}{\strut most} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throats} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut NOT} \colorbox{red!0}{\strut respond} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut antibiotics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut mild} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut beginning} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut every} \colorbox{red!1}{\strut cold} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut When} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nose} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut sinuses} \colorbox{red!0}{\strut become} \colorbox{red!1}{\strut infected} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut drainage} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut irritate} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut night} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Or} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut itself} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut infected} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut viruses} \colorbox{red!0}{\strut can} \colorbox{red!2}{\strut cause} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Coxsackievirus} \colorbox{red!0}{\strut sometimes} \colorbox{red!2}{\strut causes} \colorbox{red!1}{\strut blisters} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut late} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut early} \colorbox{red!0}{\strut fall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mono} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut flu} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!2}{\strut cause} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut viral} \colorbox{red!4}{\strut throat} \colorbox{red!1}{\strut infections} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Strep} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut common} \colorbox{red!0}{\strut bacterial} \colorbox{red!2}{\strut cause} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Because} \colorbox{red!1}{\strut strep} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut occasionally} \colorbox{red!0}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut rheumatic} \colorbox{red!0}{\strut fever} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut antibiotics} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Strep} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fever} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut greater} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 101F} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut white} \colorbox{red!0}{\strut draining} \colorbox{red!0}{\strut patches} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut swollen} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut tender} \colorbox{red!0}{\strut lymph} \colorbox{red!0}{\strut glands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut neck} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Children} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut headache} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut stomach} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!4}{\strut sore} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut strep} \colorbox{red!4}{\strut throat} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut minor} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut typical} \colorbox{red!1}{\strut cold} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut runny} \colorbox{red!0}{\strut nose} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut stuffy} \colorbox{red!0}{\strut ears} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

99:throats, 99:throat, 99:sores, 98:soreness, 97:sore, 69:what, 64:remedies, 46:lime, 46:health, 43:nature


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Tuesday} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 13th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut shop} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut podcasts} \colorbox{red!1}{\strut tv} \colorbox{red!0}{\strut lime.com} \colorbox{red!1}{\strut Food} \colorbox{red!3}{\strut Health} \colorbox{red!1}{\strut Green} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Balance} \colorbox{red!0}{\strut Planet} \colorbox{red!0}{\strut Live} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Change} \colorbox{red!0}{\strut Home} \colorbox{red!5}{\strut sore} \colorbox{red!5}{\strut throat} \colorbox{red!2}{\strut Natural} \colorbox{red!4}{\strut Remedies} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut SORE} \colorbox{red!5}{\strut THROATS} \colorbox{red!1}{\strut Sea} \colorbox{red!1}{\strut Salt} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Water} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut draw} \colorbox{red!0}{\strut excess} \colorbox{red!0}{\strut moisture} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut inflamed} \colorbox{red!5}{\strut throat} \colorbox{red!0}{\strut tissues} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut draws} \colorbox{red!0}{\strut moisture} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut mixture} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut drying} \colorbox{red!1}{\strut effect} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut makes} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut ideal} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut treating} \colorbox{red!5}{\strut sore} \colorbox{red!5}{\strut throats} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut mosquito} \colorbox{red!1}{\strut bites} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Salt} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut has} \colorbox{red!1}{\strut disinfectant} \colorbox{red!0}{\strut properties} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!2}{\strut help} \colorbox{red!1}{\strut kill} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut bacteria} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut caused} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut sore} \colorbox{red!5}{\strut throat} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stir} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut tablespoon} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut sea} \colorbox{red!1}{\strut salt} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut half} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut cup} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut warm} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut dissolved} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut mixture} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut gargle} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut needed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Soak} \colorbox{red!1}{\strut bites} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut salt} \colorbox{red!1}{\strut water} \colorbox{red!1}{\strut mixture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut mix} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut sea} \colorbox{red!1}{\strut salt} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut lard} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut cold} \colorbox{red!0}{\strut cream} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut apply} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut paste} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut bites} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut register} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut post} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut Topics} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut LIME} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Natural} \colorbox{red!0}{\strut First} \colorbox{red!1}{\strut Aid} \colorbox{red!3}{\strut Health} \colorbox{red!5}{\strut sore} \colorbox{red!5}{\strut throat} \colorbox{red!2}{\strut Natural} \colorbox{red!0}{\strut First} \colorbox{red!1}{\strut Aid} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut What} \colorbox{red!0}{\strut Ails} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Posted} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut LIME} \colorbox{red!0}{\strut Team} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 1008am} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Step} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut bee} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Swallow} \colorbox{red!0}{\strut something} \colorbox{red!0}{\strut scratchy} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Touch} \colorbox{red!0}{\strut something} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut hot} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut LIME} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut feel} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut ASAP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut mostly} \colorbox{red!2}{\strut natural} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut herbal} \colorbox{red!0}{\strut approaches} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut whatever} \colorbox{red!0}{\strut ails} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut waiting} \colorbox{red!0}{\strut room} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut consultation} \colorbox{red!0}{\strut fee} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut insurance} \colorbox{red!0}{\strut paper} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fill} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut just} \colorbox{red!2}{\strut good} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut solid} \colorbox{red!0}{\strut advice} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut treating} \colorbox{red!0}{\strut household} \colorbox{red!0}{\strut boo-boos} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut bang-ups} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut best} \colorbox{red!2}{\strut nature} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut offer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut Topics} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut LIME} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Natural} \colorbox{red!0}{\strut First} \colorbox{red!1}{\strut Aid} \colorbox{red!3}{\strut Health} \colorbox{red!0}{\strut ant} \colorbox{red!1}{\strut bites} \colorbox{red!1}{\strut bee} \colorbox{red!0}{\strut stings} \colorbox{red!0}{\strut blisters} \colorbox{red!0}{\strut bruises} \colorbox{red!0}{\strut burns} \colorbox{red!0}{\strut chapped} \colorbox{red!0}{\strut lips} \colorbox{red!0}{\strut chigger} \colorbox{red!1}{\strut bites} \colorbox{red!1}{\strut cold} \colorbox{red!5}{\strut sores} \colorbox{red!0}{\strut constipation} \colorbox{red!0}{\strut coughs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut congestion} \colorbox{red!0}{\strut cuts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut scrapes} \colorbox{red!0}{\strut diarrhea} \colorbox{red!0}{\strut ear} \colorbox{red!0}{\strut infections} \colorbox{red!0}{\strut eczema} \colorbox{red!0}{\strut Growing} \colorbox{red!0}{\strut Greener} \colorbox{red!0}{\strut Kids} \colorbox{red!0}{\strut hay} \colorbox{red!0}{\strut fever} 
}}}
\end{CJK*}

query: ontario california airport

98:airport, 97:airports, 96:ontario, 41:ont, 35:la, 34:california, 27:canada, 24:airlines, 23:international, 21:location


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut LAOntario} \colorbox{red!1}{\strut International} \colorbox{red!6}{\strut Airport} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut L.A.Ontario} \colorbox{red!6}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut airport} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut California} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!6}{\strut airports} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut Ontario} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Canada} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut airports} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Canada} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut LAOntario} \colorbox{red!1}{\strut International} \colorbox{red!6}{\strut Airport} \colorbox{red!0}{\strut IATA} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ONT} \colorbox{red!1}{\strut ICAO} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut KONT} \colorbox{red!1}{\strut FAA} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ONT} \colorbox{red!0}{\strut Summary} \colorbox{red!6}{\strut Airport} \colorbox{red!1}{\strut type} \colorbox{red!0}{\strut Public} \colorbox{red!0}{\strut Owner} \colorbox{red!1}{\strut Los} \colorbox{red!1}{\strut Angeles} \colorbox{red!0}{\strut World} \colorbox{red!6}{\strut Airports} \colorbox{red!0}{\strut Serves} \colorbox{red!5}{\strut Ontario} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Inland} \colorbox{red!0}{\strut Empire} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut California} \colorbox{red!1}{\strut Location} \colorbox{red!5}{\strut Ontario} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut California} \colorbox{red!0}{\strut Elevation} \colorbox{red!0}{\strut AMSL} \colorbox{red!0}{\strut 944} \colorbox{red!0}{\strut ft} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 288} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut Coordinates} \colorbox{red!0}{\strut 340322N} \colorbox{red!0}{\strut 1173604W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 34.05611N} \colorbox{red!0}{\strut 117.60111W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 34.05611} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -117.60111} \colorbox{red!0}{\strut Website} \colorbox{red!0}{\strut www.lawa.orgont} \colorbox{red!1}{\strut Runways} \colorbox{red!0}{\strut Direction} \colorbox{red!0}{\strut Length} \colorbox{red!0}{\strut Surface} \colorbox{red!0}{\strut ft} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut 8L26R} \colorbox{red!0}{\strut 12,197} \colorbox{red!0}{\strut 3,718} \colorbox{red!0}{\strut Concrete} \colorbox{red!0}{\strut 8R26L} \colorbox{red!0}{\strut 10,200} \colorbox{red!0}{\strut 3,109} \colorbox{red!0}{\strut Concrete} \colorbox{red!0}{\strut Statistics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Aircraft} \colorbox{red!0}{\strut operations} \colorbox{red!0}{\strut 136,410} \colorbox{red!0}{\strut Based} \colorbox{red!0}{\strut aircraft} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut Source} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Federal} \colorbox{red!0}{\strut Aviation} \colorbox{red!0}{\strut Administration} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Terminal} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut at} \colorbox{red!2}{\strut ONT} \colorbox{red!0}{\strut LAOntario} \colorbox{red!1}{\strut International} \colorbox{red!6}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut IATA} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ONT} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut ICAO} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut KONT} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut FAA} \colorbox{red!0}{\strut LID} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ONT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut formerly} \colorbox{red!5}{\strut Ontario} \colorbox{red!1}{\strut International} \colorbox{red!6}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut public} \colorbox{red!6}{\strut airport} \colorbox{red!1}{\strut located} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut east} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut central} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut district} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CBD} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Ontario} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Bernardino} \colorbox{red!0}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut California} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut USA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!6}{\strut airport} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut owned} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut operated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Los} \colorbox{red!1}{\strut Angeles} \colorbox{red!0}{\strut World} \colorbox{red!6}{\strut Airports} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut agency} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Los} \colorbox{red!1}{\strut Angeles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 6.2} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut passengers} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut airport} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut decline} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 13.5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!6}{\strut airport} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut dominated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Southwest} \colorbox{red!1}{\strut Airlines} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut carried} \colorbox{red!0}{\strut 49.38} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut passengers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut four} \colorbox{red!1}{\strut airlines} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut five} \colorbox{red!0}{\strut were} \colorbox{red!1}{\strut United} \colorbox{red!0}{\strut AirlinesUnited} \colorbox{red!0}{\strut Express} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8.64} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Delta} \colorbox{red!0}{\strut Air} \colorbox{red!0}{\strut Lines} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7.93} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut Airways} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7.08} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Airlines} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6.18} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Expressjet} \colorbox{red!1}{\strut operated} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut hub} \colorbox{red!0}{\strut at} 
}}}
\end{CJK*}

92:airports, 91:airport, 82:ontario, 72:california, 26:aviation, 23:state, 18:new, 17:usa, 15:maine, 14:runways


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut PHOTOVALET} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut tm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Enter} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut term} \colorbox{red!1}{\strut PHOTOVAULT} \colorbox{red!3}{\strut AVIATION} \colorbox{red!1}{\strut Museum} \colorbox{red!9}{\strut Airports} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Ontario} \colorbox{red!7}{\strut California} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Customs} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Traffic} \colorbox{red!1}{\strut Control} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Runways} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut images} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Wernher} \colorbox{red!1}{\strut Krutein} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut PHOTOVAULT} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut contains} \colorbox{red!0}{\strut samples} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut picture} \colorbox{red!1}{\strut files} \colorbox{red!9}{\strut Airports} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Ontario} \colorbox{red!7}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!1}{\strut pictures} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut licensing} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut media} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!1}{\strut Pricing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut General} \colorbox{red!0}{\strut Guidelines} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Delivery} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut may} \colorbox{red!1}{\strut contact} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut thru} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut phone} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut These} \colorbox{red!1}{\strut pictures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut files} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut shown} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut ask} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut These} \colorbox{red!1}{\strut pictures} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Included} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut PHOTOVAULT} \colorbox{red!3}{\strut AVIATION} \colorbox{red!1}{\strut Museum} \colorbox{red!0}{\strut are} \colorbox{red!9}{\strut Airport} \colorbox{red!1}{\strut images} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut USA} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Adak} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Albuquerque} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Alton} \colorbox{red!1}{\strut Bay} \colorbox{red!2}{\strut New} \colorbox{red!1}{\strut Hampshire} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Anchorage} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Atlanta} \colorbox{red!0}{\strut Hartsfield} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Austin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Bakersfield} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Baltimore} \colorbox{red!1}{\strut Washington} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Boise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Boulder} \colorbox{red!1}{\strut Nevada} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Burbank} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Calistoga} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Canyonlands} \colorbox{red!1}{\strut Field} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Catalina} \colorbox{red!1}{\strut Island} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Chandler} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Charlotte} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Charleston} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Chester} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Chicago} \colorbox{red!0}{\strut Midway} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Chicago} \colorbox{red!0}{\strut Ohare} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Cincinnati} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Concord} \colorbox{red!7}{\strut California} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Dallas} \colorbox{red!1}{\strut Fort} \colorbox{red!0}{\strut Worth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Dallas} \colorbox{red!0}{\strut Love} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Denver} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Detroit} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Dulles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut El} \colorbox{red!0}{\strut Paso} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut El} \colorbox{red!0}{\strut Toro} \colorbox{red!7}{\strut California} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Fairbanks} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Fortuna} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Fremont} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Fresno} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut General} \colorbox{red!0}{\strut Mitchell} \colorbox{red!0}{\strut Intl} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Grand} \colorbox{red!0}{\strut Junction} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Gulfport} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hailey} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Half} \colorbox{red!0}{\strut Moon} \colorbox{red!1}{\strut Bay} \colorbox{red!7}{\strut California} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hampton} \colorbox{red!2}{\strut New} \colorbox{red!0}{\strut H} \colorbox{red!0}{\strut ampshire} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hayward} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hilo} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Honolulu} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Houston} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Jackson} \colorbox{red!0}{\strut Hole} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut F.} \colorbox{red!0}{\strut Kennedy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut Wayne} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Kahului} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Kansas} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Kauai} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Knox} \colorbox{red!1}{\strut County} \colorbox{red!1}{\strut Maine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Kona} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut La} \colorbox{red!0}{\strut Guardia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lake} \colorbox{red!0}{\strut Tahoe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Las} \colorbox{red!0}{\strut Vegas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lawrence} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lebanon} \colorbox{red!2}{\strut New} \colorbox{red!1}{\strut Hampshire} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Little} \colorbox{red!1}{\strut Rock} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Livermore} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Logan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Long} \colorbox{red!1}{\strut Beach} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}



==> sections/visualization/cwbloss2.tex <==
query: mitchell college

98:mitchell, 96:college, 40:costs, 28:enrollment, 21:new, 21:london, 19:average, 17:programs, 17:admissions, 16:universities


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!97}{\strut Mitchell} \colorbox{red!95}{\strut College} \colorbox{red!9}{\strut 437} \colorbox{red!12}{\strut Pequot} \colorbox{red!3}{\strut Avenue} \colorbox{red!20}{\strut New} \colorbox{red!20}{\strut London} \colorbox{red!1}{\strut ,} \colorbox{red!9}{\strut CT} \colorbox{red!0}{\strut 06320-4498} \colorbox{red!2}{\strut Office} \colorbox{red!2}{\strut of} \colorbox{red!16}{\strut Admissions} \colorbox{red!4}{\strut and} \colorbox{red!5}{\strut Financial} \colorbox{red!7}{\strut Aid} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 443-2811} \colorbox{red!4}{\strut FAX} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 860} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 444-4498} \colorbox{red!0}{\strut e-mail} \colorbox{red!2}{\strut .} \colorbox{red!16}{\strut admissions} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut mitchell.edu} \colorbox{red!2}{\strut http} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut www.mitchell.edu} \colorbox{red!27}{\strut ENROLLMENT} \colorbox{red!0}{\strut Full-time} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Total} \colorbox{red!0}{\strut 708} \colorbox{red!7}{\strut men} \colorbox{red!0}{\strut 427women} \colorbox{red!2}{\strut 281} \colorbox{red!0}{\strut Part-time} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Total} \colorbox{red!0}{\strut 120} \colorbox{red!7}{\strut men} \colorbox{red!0}{\strut 41women} \colorbox{red!0}{\strut 79} \colorbox{red!14}{\strut FRESHMAN} \colorbox{red!0}{\strut ADMISSION} \colorbox{red!4}{\strut PROFILE} \colorbox{red!10}{\strut Number} \colorbox{red!5}{\strut who} \colorbox{red!5}{\strut applied} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1024} \colorbox{red!10}{\strut Number} \colorbox{red!13}{\strut accepted} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 641} \colorbox{red!10}{\strut Number} \colorbox{red!0}{\strut enrolled} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 346} \colorbox{red!18}{\strut Average} \colorbox{red!5}{\strut SAT} \colorbox{red!5}{\strut scores} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut V} \colorbox{red!0}{\strut 500} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut 500} \colorbox{red!18}{\strut Average} \colorbox{red!6}{\strut ACT} \colorbox{red!0}{\strut score} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 19} \colorbox{red!14}{\strut Freshman} \colorbox{red!5}{\strut retention} \colorbox{red!4}{\strut rate} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2006-2007} \colorbox{red!39}{\strut COSTS} \colorbox{red!2}{\strut .} \colorbox{red!14}{\strut Tuition} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19,199} \colorbox{red!5}{\strut Room} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut Board} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9,268} \colorbox{red!6}{\strut Fees} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 929} \colorbox{red!5}{\strut FINANCIAL} \colorbox{red!7}{\strut AID} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Freshmen} \colorbox{red!6}{\strut receiving} \colorbox{red!7}{\strut aid} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 85} \colorbox{red!0}{\strut .} \colorbox{red!18}{\strut Average} \colorbox{red!5}{\strut financial} \colorbox{red!7}{\strut aid} \colorbox{red!1}{\strut package} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8,000} \colorbox{red!8}{\strut FACULTY} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Full-time} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut Part-time} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut Ph.D.} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 12} \colorbox{red!0}{\strut Student-faculty} \colorbox{red!3}{\strut ratio} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 121} \colorbox{red!0}{\strut IN} \colorbox{red!0}{\strut ADDITION} \colorbox{red!97}{\strut Mitchell} \colorbox{red!95}{\strut College} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut built} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut reputation} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut giving} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut outstanding} \colorbox{red!0}{\strut foundation} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut their} \colorbox{red!95}{\strut college} \colorbox{red!7}{\strut studies} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut known} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut our} \colorbox{red!2}{\strut nationally} \colorbox{red!0}{\strut respected} \colorbox{red!7}{\strut Learning} \colorbox{red!2}{\strut Resource} \colorbox{red!4}{\strut Center} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut LRC} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut diagnosed} \colorbox{red!7}{\strut learning} \colorbox{red!7}{\strut disabilities} \colorbox{red!0}{\strut andor} \colorbox{red!0}{\strut ADDADHD} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut related} \colorbox{red!7}{\strut disabilities} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!2}{\strut fact} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut colleges} \colorbox{red!4}{\strut and} \colorbox{red!15}{\strut universities} \colorbox{red!0}{\strut across} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut country} \colorbox{red!1}{\strut have} \colorbox{red!0}{\strut used} \colorbox{red!97}{\strut Mitchell} \colorbox{red!0}{\strut s} \colorbox{red!14}{\strut LRC} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut model} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut developing} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut own} \colorbox{red!16}{\strut programs} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Because} \colorbox{red!0}{\strut each} \colorbox{red!97}{\strut Mitchell} \colorbox{red!13}{\strut student} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut her} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut unique} \colorbox{red!2}{\strut set} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut academic} \colorbox{red!0}{\strut strengths} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut weaknesses} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!14}{\strut LRC} \colorbox{red!0}{\strut program} \colorbox{red!2}{\strut addresses} \colorbox{red!0}{\strut each} \colorbox{red!2}{\strut participany} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut individual} \colorbox{red!0}{\strut basis} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut Our} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut size} \colorbox{red!0}{\strut enables} \colorbox{red!97}{\strut Mitchell} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut offer} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut exceptionally} \colorbox{red!1}{\strut personalized} \colorbox{red!6}{\strut academic} \colorbox{red!2}{\strut experience} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut out} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut classroom} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Go} \colorbox{red!0}{\strut To} \colorbox{red!4}{\strut Profile} \colorbox{red!0}{\strut Index} \colorbox{red!2}{\strut Page} \colorbox{red!0}{\strut Go} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Top} \colorbox{red!2}{\strut Of} \colorbox{red!2}{\strut Page} \colorbox{red!97}{\strut Mitchell} \colorbox{red!95}{\strut College} \colorbox{red!9}{\strut 437} \colorbox{red!12}{\strut Pequot} \colorbox{red!3}{\strut Avenue} \colorbox{red!20}{\strut New} \colorbox{red!20}{\strut London} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Connecticut} \colorbox{red!0}{\strut 06320-4498} \colorbox{red!2}{\strut http} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut www.mitchell.edu} \colorbox{red!0}{\strut While} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut video} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut loading} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut please} \colorbox{red!0}{\strut scroll} \colorbox{red!0}{\strut down} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut read} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut profile} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut about} \colorbox{red!97}{\strut Mitchell} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!2}{\strut video} \colorbox{red!2}{\strut will} \colorbox{red!4}{\strut play} \colorbox{red!0}{\strut automatically} \colorbox{red!6}{\strut when} \colorbox{red!0}{\strut loaded} 
}}}
\end{CJK*}

28:rhodes, 26:scholarships, 24:mitchell, 23:marshall, 15:college, 14:school, 13:lyric, 13:arts, 12:university, 10:science


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut For} \colorbox{red!4}{\strut Students} \colorbox{red!3}{\strut For} \colorbox{red!2}{\strut Faculty} \colorbox{red!4}{\strut Available} \colorbox{red!19}{\strut Scholarships} \colorbox{red!4}{\strut Nominees} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Recipients} \colorbox{red!3}{\strut FAQ} \colorbox{red!1}{\strut Calendar} \colorbox{red!0}{\strut RECENT} \colorbox{red!4}{\strut NOMINEES} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut RECIPIENTS} \colorbox{red!0}{\strut Read} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut Article} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Six} \colorbox{red!3}{\strut Honored} \colorbox{red!3}{\strut for} \colorbox{red!0}{\strut Scholarship} \colorbox{red!4}{\strut Nominations} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut University} \colorbox{red!4}{\strut Record} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut 101208} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut 2009} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut 2008} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 2007} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2006} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut 2005} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2004} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut 2003} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut 2002} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut 2009} \colorbox{red!3}{\strut Christine} \colorbox{red!4}{\strut Beamer} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!3}{\strut ,} \colorbox{red!21}{\strut RHODES} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Music} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Theatre} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut Dance} \colorbox{red!5}{\strut Maia} \colorbox{red!4}{\strut Dedrick} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Music} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Theatre} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut Dance} \colorbox{red!3}{\strut Abdul} \colorbox{red!0}{\strut El-Sayed} \colorbox{red!21}{\strut RHODES} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut offered} \colorbox{red!3}{\strut and} \colorbox{red!7}{\strut accepted} \colorbox{red!3}{\strut .} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut offered} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut declined} \colorbox{red!3}{\strut .} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut Public} \colorbox{red!5}{\strut Health} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut Medical} \colorbox{red!10}{\strut School} \colorbox{red!3}{\strut Sam} \colorbox{red!2}{\strut Espahbodi} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut Megan} \colorbox{red!3}{\strut Hildebrandt} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut finalist} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut Art} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Design} \colorbox{red!3}{\strut Neil} \colorbox{red!2}{\strut Rao} \colorbox{red!18}{\strut MITCHELL} \colorbox{red!3}{\strut ,} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!3}{\strut ,} \colorbox{red!21}{\strut RHODES} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut Public} \colorbox{red!5}{\strut Health} \colorbox{red!4}{\strut Kendal} \colorbox{red!4}{\strut Sparks} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!3}{\strut ,} \colorbox{red!21}{\strut RHODES} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Music} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Theatre} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut Dance} \colorbox{red!6}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut top} \colorbox{red!3}{\strut 2008} \colorbox{red!3}{\strut Michael} \colorbox{red!3}{\strut Cromwell} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!3}{\strut ,} \colorbox{red!21}{\strut RHODES} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut Stephen} \colorbox{red!0}{\strut M.} \colorbox{red!3}{\strut Ross} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut Business} \colorbox{red!3}{\strut Stephanie} \colorbox{red!3}{\strut Ketchum} \colorbox{red!21}{\strut RHODES} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut Loc} \colorbox{red!3}{\strut Thang} \colorbox{red!21}{\strut RHODES} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut Engineering} \colorbox{red!4}{\strut Colin} \colorbox{red!4}{\strut Tucker} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Music} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Theatre} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut Dance} \colorbox{red!3}{\strut Thomas} \colorbox{red!4}{\strut Wisniewski} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!3}{\strut ,} \colorbox{red!21}{\strut RHODES} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Music} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Theatre} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut Dance} \colorbox{red!6}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut top} \colorbox{red!4}{\strut 2007} \colorbox{red!9}{\strut Lyric} \colorbox{red!7}{\strut Chen} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut offered} \colorbox{red!3}{\strut and} \colorbox{red!7}{\strut accepted} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut ,} \colorbox{red!21}{\strut RHODES} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut finalist} \colorbox{red!3}{\strut .} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Science} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut Arts} \colorbox{red!3}{\strut Lucas} \colorbox{red!3}{\strut Polcyn} \colorbox{red!17}{\strut MARSHALL} \colorbox{red!3}{\strut ,} \colorbox{red!21}{\strut RHODES} \colorbox{red!3}{\strut ,} \colorbox{red!18}{\strut MITCHELL} \colorbox{red!11}{\strut College} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Literature} 
}}}
\end{CJK*}

query: lower heart rate

83:benefits, 69:cardiorespiratory, 65:rate, 50:cardio, 45:heart, 41:muscle, 40:resting, 39:lower, 30:blood, 29:pressure


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!10}{\strut Fitness} \colorbox{red!4}{\strut Study} \colorbox{red!4}{\strut Guide} \colorbox{red!68}{\strut Benefits} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut Flexibility-} \colorbox{red!16}{\strut Better} \colorbox{red!9}{\strut range} \colorbox{red!3}{\strut of} \colorbox{red!11}{\strut motion} \colorbox{red!0}{\strut for} \colorbox{red!9}{\strut joints} \colorbox{red!22}{\strut Avoid} \colorbox{red!33}{\strut muscle} \colorbox{red!22}{\strut injuries} \colorbox{red!7}{\strut Ease} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut doing} \colorbox{red!1}{\strut everyday} \colorbox{red!2}{\strut tasks} \colorbox{red!68}{\strut Benefits} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut Cardiorespiratory-} \colorbox{red!32}{\strut Lower} \colorbox{red!33}{\strut resting} \colorbox{red!37}{\strut heart} \colorbox{red!53}{\strut rate} \colorbox{red!7}{\strut Overall} \colorbox{red!1}{\strut feeling} \colorbox{red!3}{\strut of} \colorbox{red!16}{\strut better} \colorbox{red!11}{\strut health} \colorbox{red!68}{\strut Benefits} \colorbox{red!3}{\strut of} \colorbox{red!11}{\strut Strength} \colorbox{red!0}{\strut Training-} \colorbox{red!7}{\strut Stronger} \colorbox{red!0}{\strut muscles} \colorbox{red!7}{\strut Stronger} \colorbox{red!5}{\strut bones} \colorbox{red!22}{\strut Avoid} \colorbox{red!33}{\strut muscle} \colorbox{red!22}{\strut injuries} \colorbox{red!41}{\strut Cardio} \colorbox{red!0}{\strut healthlower} \colorbox{red!24}{\strut blood} \colorbox{red!24}{\strut pressure} \colorbox{red!0}{\strut A} \colorbox{red!1}{\strut .} \colorbox{red!14}{\strut Weights} \colorbox{red!2}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!11}{\strut lifted} \colorbox{red!4}{\strut slowly} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 10-15} \colorbox{red!7}{\strut repetitions} \colorbox{red!0}{\strut per} \colorbox{red!11}{\strut set} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut day} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut B} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut your} \colorbox{red!37}{\strut heart} \colorbox{red!1}{\strut is} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!17}{\strut training} \colorbox{red!16}{\strut zone} \colorbox{red!4}{\strut while} \colorbox{red!20}{\strut exercising} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!18}{\strut working} \colorbox{red!0}{\strut to} \colorbox{red!32}{\strut lower} \colorbox{red!0}{\strut your} \colorbox{red!33}{\strut resting} \colorbox{red!37}{\strut heart} \colorbox{red!53}{\strut rate} \colorbox{red!1}{\strut ,} \colorbox{red!12}{\strut improving} \colorbox{red!0}{\strut your} \colorbox{red!7}{\strut endurance} \colorbox{red!9}{\strut burning} \colorbox{red!6}{\strut fat} \colorbox{red!7}{\strut calories} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut Your} \colorbox{red!8}{\strut target} \colorbox{red!37}{\strut heart} \colorbox{red!16}{\strut zone} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 60-80} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!11}{\strut maximum} \colorbox{red!37}{\strut heart} \colorbox{red!53}{\strut rate} \colorbox{red!1}{\strut .} \colorbox{red!9}{\strut When} \colorbox{red!0}{\strut youre} \colorbox{red!3}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!16}{\strut zone} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut are} \colorbox{red!2}{\strut getting} \colorbox{red!2}{\strut the} \colorbox{red!68}{\strut benefits} \colorbox{red!3}{\strut of} \colorbox{red!57}{\strut cardiorespiratory} \colorbox{red!0}{\strut work} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut D.} \colorbox{red!0}{\strut Muscles} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut examples} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut exercises} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Abdominals} \colorbox{red!0}{\strut -crunches} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut sit-ups} \colorbox{red!4}{\strut Trapezius} \colorbox{red!0}{\strut -shoulder} \colorbox{red!11}{\strut press} \colorbox{red!6}{\strut Biceps} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut arm} \colorbox{red!4}{\strut curls} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut push-ups} \colorbox{red!10}{\strut Quadriceps} \colorbox{red!0}{\strut -leg} \colorbox{red!7}{\strut extension} \colorbox{red!1}{\strut ,} \colorbox{red!10}{\strut leg} \colorbox{red!11}{\strut press} \colorbox{red!5}{\strut Pectoralis} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut flys} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut bench} \colorbox{red!11}{\strut press} \colorbox{red!2}{\strut Deltoid} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut shoulder} \colorbox{red!11}{\strut press} \colorbox{red!7}{\strut Triceps} \colorbox{red!0}{\strut -upright} \colorbox{red!4}{\strut rows} \colorbox{red!4}{\strut Gluteus} \colorbox{red!3}{\strut maximus} \colorbox{red!0}{\strut -} \colorbox{red!10}{\strut leg} \colorbox{red!11}{\strut press} \colorbox{red!0}{\strut KNOW} \colorbox{red!5}{\strut WHERE} \colorbox{red!0}{\strut ALL} \colorbox{red!2}{\strut THE} \colorbox{red!0}{\strut ABOVE} \colorbox{red!0}{\strut MUSCLES} \colorbox{red!3}{\strut ARE} \colorbox{red!0}{\strut ON} \colorbox{red!2}{\strut THE} \colorbox{red!0}{\strut BODY-STUDY} \colorbox{red!2}{\strut THE} \colorbox{red!0}{\strut WALL} \colorbox{red!0}{\strut PICTURES} \colorbox{red!3}{\strut IN} \colorbox{red!6}{\strut CLASS} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

97:rate, 95:heart, 77:how, 67:training, 60:calculating, 31:resting, 24:pulse, 23:zones, 23:thr, 22:workout


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tips} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut Techniques} \colorbox{red!1}{\strut .} \colorbox{red!27}{\strut Calculating} \colorbox{red!0}{\strut Your} \colorbox{red!30}{\strut Training} \colorbox{red!43}{\strut Heart} \colorbox{red!44}{\strut Rate} \colorbox{red!7}{\strut High} \colorbox{red!5}{\strut performance} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut disciplinespecially} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut elite} \colorbox{red!0}{\strut athleticsequires} \colorbox{red!4}{\strut measuring} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut recording} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut tracking} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut key} \colorbox{red!2}{\strut metrics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut discussing} \colorbox{red!35}{\strut how} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut calculate} \colorbox{red!0}{\strut a} \colorbox{red!30}{\strut training} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!1}{\strut ,} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!3}{\strut monitors} \colorbox{red!1}{\strut ,} \colorbox{red!35}{\strut how} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut use} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut monitor} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut optimize} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut performance} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!35}{\strut how} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut reduce} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut chance} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut injuries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!1}{\strut will} \colorbox{red!2}{\strut show} \colorbox{red!0}{\strut you} \colorbox{red!35}{\strut how} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut calculate} \colorbox{red!0}{\strut your} \colorbox{red!30}{\strut training} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut formula} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut accounts} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut level} \colorbox{red!1}{\strut of} \colorbox{red!4}{\strut fitness} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut your} \colorbox{red!14}{\strut resting} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!1}{\strut .} \colorbox{red!30}{\strut Training} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!1}{\strut .} \colorbox{red!10}{\strut THR} \colorbox{red!1}{\strut .} \colorbox{red!10}{\strut zones} \colorbox{red!1}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!5}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut are} \colorbox{red!1}{\strut doing} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut aerobic} \colorbox{red!2}{\strut part} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!10}{\strut workout} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Take} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut pulse} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!3}{\strut times} \colorbox{red!2}{\strut during} \colorbox{red!0}{\strut your} \colorbox{red!10}{\strut workout} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut ensure} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut are} \colorbox{red!30}{\strut training} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut target} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!0}{\strut zone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!30}{\strut training} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!0}{\strut zone} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut roughly} \colorbox{red!0}{\strut between} \colorbox{red!1}{\strut 60} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut 90} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut maximum} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut MHR} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!30}{\strut Training} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!0}{\strut is} \colorbox{red!7}{\strut computed} \colorbox{red!1}{\strut as} \colorbox{red!0}{\strut follows} \colorbox{red!1}{\strut .} \colorbox{red!9}{\strut Take} \colorbox{red!0}{\strut your} \colorbox{red!10}{\strut pulse} \colorbox{red!1}{\strut as} \colorbox{red!2}{\strut soon} \colorbox{red!1}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut wake} \colorbox{red!1}{\strut up} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut morning} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut your} \colorbox{red!14}{\strut resting} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut RHR} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Subtract} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut age} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut 220} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut this} \colorbox{red!7}{\strut number} \colorbox{red!1}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut MHR} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Use} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut values} \colorbox{red!0}{\strut obtained} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut equation} \colorbox{red!0}{\strut below} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut determine} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut target} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!0}{\strut for} \colorbox{red!30}{\strut training} \colorbox{red!3}{\strut purposes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut percent} \colorbox{red!1}{\strut of} \colorbox{red!43}{\strut heart} \colorbox{red!44}{\strut rate} \colorbox{red!0}{\strut used} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut calculate} \colorbox{red!4}{\strut upper} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut lower} \colorbox{red!9}{\strut limits} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut THR} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut i.e.} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut 60} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut 90} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut TARGET} \colorbox{red!2}{\strut HR} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut MHR} \colorbox{red!3}{\strut RHR} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut RHR} \colorbox{red!10}{\strut THR} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut RHR} \colorbox{red!1}{\strut Example} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut are} \colorbox{red!1}{\strut 30} \colorbox{red!1}{\strut years} \colorbox{red!2}{\strut old} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut MHR} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut 220} \colorbox{red!1}{\strut 30} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut 190} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut RHR} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut 60} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut determined} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut morning} 
}}}
\end{CJK*}

query: alexian brothers hospital

98:alexian, 95:brothers, 81:hospital, 35:network, 26:medical, 20:which, 17:care, 16:locations, 15:comprised, 12:chicago


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!12}{\strut Main} \colorbox{red!8}{\strut Navigation} \colorbox{red!12}{\strut Jobs} \colorbox{red!17}{\strut Locations} \colorbox{red!8}{\strut Services} \colorbox{red!0}{\strut Find} \colorbox{red!4}{\strut a} \colorbox{red!12}{\strut Doctor} \colorbox{red!5}{\strut Classes} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Events} \colorbox{red!8}{\strut Donate} \colorbox{red!5}{\strut About} \colorbox{red!5}{\strut Us} \colorbox{red!9}{\strut Contact} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut Like} \colorbox{red!4}{\strut To} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Learn} \colorbox{red!3}{\strut more} \colorbox{red!5}{\strut about} \colorbox{red!2}{\strut the} \colorbox{red!100}{\strut Alexian} \colorbox{red!100}{\strut Brothers} \colorbox{red!0}{\strut Find} \colorbox{red!4}{\strut a} \colorbox{red!12}{\strut Doctor} \colorbox{red!0}{\strut Find} \colorbox{red!4}{\strut a} \colorbox{red!0}{\strut Job} \colorbox{red!7}{\strut View} \colorbox{red!6}{\strut Maps} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Directions} \colorbox{red!5}{\strut Volunteer} \colorbox{red!6}{\strut Learn} \colorbox{red!3}{\strut More} \colorbox{red!5}{\strut About} \colorbox{red!6}{\strut Quality} \colorbox{red!2}{\strut .} \colorbox{red!11}{\strut Patient} \colorbox{red!6}{\strut Safety} \colorbox{red!6}{\strut Pay} \colorbox{red!0}{\strut My} \colorbox{red!4}{\strut Bill} \colorbox{red!3}{\strut Search} \colorbox{red!11}{\strut Health} \colorbox{red!3}{\strut Encyclopedia} \colorbox{red!4}{\strut Busque} \colorbox{red!6}{\strut en} \colorbox{red!5}{\strut la} \colorbox{red!6}{\strut Enciclopedia} \colorbox{red!11}{\strut de} \colorbox{red!7}{\strut Salud} \colorbox{red!6}{\strut en} \colorbox{red!8}{\strut espaol} \colorbox{red!7}{\strut Live} \colorbox{red!7}{\strut Healthier} \colorbox{red!7}{\strut View} \colorbox{red!4}{\strut Baby} \colorbox{red!4}{\strut Photos} \colorbox{red!0}{\strut Find} \colorbox{red!6}{\strut Information} \colorbox{red!3}{\strut for} \colorbox{red!11}{\strut Healthcare} \colorbox{red!7}{\strut Professionals} \colorbox{red!100}{\strut Alexian} \colorbox{red!100}{\strut Brothers} \colorbox{red!89}{\strut Hospital} \colorbox{red!38}{\strut Network} \colorbox{red!100}{\strut Alexian} \colorbox{red!100}{\strut Brothers} \colorbox{red!89}{\strut Hospital} \colorbox{red!38}{\strut Network} \colorbox{red!8}{\strut is} \colorbox{red!16}{\strut comprised} \colorbox{red!12}{\strut of} \colorbox{red!12}{\strut four} \colorbox{red!0}{\strut hospitals} \colorbox{red!22}{\strut which} \colorbox{red!9}{\strut serve} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut two} \colorbox{red!5}{\strut million} \colorbox{red!4}{\strut residents} \colorbox{red!12}{\strut of} \colorbox{red!13}{\strut Chicago} \colorbox{red!0}{\strut s} \colorbox{red!7}{\strut growing} \colorbox{red!5}{\strut Northwest} \colorbox{red!7}{\strut suburbs} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut We} \colorbox{red!7}{\strut offer} \colorbox{red!4}{\strut a} \colorbox{red!5}{\strut broad} \colorbox{red!4}{\strut continuum} \colorbox{red!12}{\strut of} \colorbox{red!5}{\strut innovative} \colorbox{red!18}{\strut care} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut leading} \colorbox{red!28}{\strut medical} \colorbox{red!6}{\strut specialists} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut state-of-the-art} \colorbox{red!8}{\strut technology} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut reflecting} \colorbox{red!0}{\strut our} \colorbox{red!6}{\strut commitment} \colorbox{red!4}{\strut to} \colorbox{red!7}{\strut provide} \colorbox{red!4}{\strut unsurpassed} \colorbox{red!11}{\strut treatment} \colorbox{red!1}{\strut and} \colorbox{red!18}{\strut care} \colorbox{red!4}{\strut to} \colorbox{red!8}{\strut benefit} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut patients} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut community} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!4}{\strut a} \colorbox{red!0}{\strut Job} \colorbox{red!4}{\strut Privacy} \colorbox{red!5}{\strut Policy} \colorbox{red!0}{\strut Advertising} \colorbox{red!5}{\strut Policy} \colorbox{red!28}{\strut Medical} \colorbox{red!5}{\strut Disclaimer} \colorbox{red!5}{\strut Media} \colorbox{red!3}{\strut Copyright} \colorbox{red!0}{\strut 2009} \colorbox{red!12}{\strut Congregation} \colorbox{red!12}{\strut of} \colorbox{red!100}{\strut Alexian} \colorbox{red!100}{\strut Brothers} \colorbox{red!5}{\strut .} 
}}}
\end{CJK*}

100:alexian, 76:brothers, 38:hospital, 38:center, 33:locations, 29:medical, 25:home, 24:facilities, 23:health, 20:clinics


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Main} \colorbox{red!0}{\strut Navigation} \colorbox{red!4}{\strut Jobs} \colorbox{red!20}{\strut Locations} \colorbox{red!9}{\strut Services} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut Doctor} \colorbox{red!4}{\strut Classes} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Events} \colorbox{red!0}{\strut Donate} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Contact} \colorbox{red!20}{\strut Locations} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut News} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut Dominican} \colorbox{red!10}{\strut University} \colorbox{red!1}{\strut Form} \colorbox{red!2}{\strut Partnership} \colorbox{red!2}{\strut Resource} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut Veterans} \colorbox{red!2}{\strut at} \colorbox{red!4}{\strut ABMC} \colorbox{red!2}{\strut ABHN} \colorbox{red!0}{\strut Receives} \colorbox{red!0}{\strut American} \colorbox{red!3}{\strut Stroke} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Guidelines} \colorbox{red!0}{\strut Gold} \colorbox{red!0}{\strut Performance} \colorbox{red!0}{\strut Achievement} \colorbox{red!1}{\strut Award} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!23}{\strut Hospital} \colorbox{red!4}{\strut Network} \colorbox{red!2}{\strut Participating} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Phase} \colorbox{red!0}{\strut III} \colorbox{red!0}{\strut MS} \colorbox{red!0}{\strut Study} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Cancer} \colorbox{red!3}{\strut Institute} \colorbox{red!0}{\strut Broadens} \colorbox{red!3}{\strut Genetics} \colorbox{red!2}{\strut Testing} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Joint} \colorbox{red!1}{\strut Commission} \colorbox{red!0}{\strut Awards} \colorbox{red!0}{\strut Gold} \colorbox{red!0}{\strut Seal} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Approval} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Disease} \colorbox{red!3}{\strut Management} \colorbox{red!4}{\strut Programs} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!15}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Locations} \colorbox{red!0}{\strut Our} \colorbox{red!20}{\strut Locations} \colorbox{red!0}{\strut Hospitals} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!12}{\strut Behavioral} \colorbox{red!13}{\strut Health} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!60}{\strut Alexian} \colorbox{red!9}{\strut Rehabilitation} \colorbox{red!23}{\strut Hospital} \colorbox{red!0}{\strut St.} \colorbox{red!6}{\strut Alexius} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!5}{\strut Emergency} \colorbox{red!12}{\strut Care} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!12}{\strut Behavioral} \colorbox{red!13}{\strut Health} \colorbox{red!23}{\strut Hospital} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut St.} \colorbox{red!6}{\strut Alexius} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ImmediateCare} \colorbox{red!0}{\strut CentersDiagnostic} \colorbox{red!4}{\strut Imaging} \colorbox{red!9}{\strut Services} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Immediate} \colorbox{red!12}{\strut Care} \colorbox{red!0}{\strut CenterDiagnostic} \colorbox{red!4}{\strut Imaging} \colorbox{red!9}{\strut Services} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Addison} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut Diagnostic} \colorbox{red!4}{\strut Imaging} \colorbox{red!9}{\strut Services} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mount} \colorbox{red!0}{\strut Prospect} \colorbox{red!0}{\strut St.} \colorbox{red!6}{\strut Alexius} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ImmediateCare} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Hanover} \colorbox{red!2}{\strut Park} \colorbox{red!0}{\strut St.} \colorbox{red!6}{\strut Alexius} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ImmediateCare} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Palatine} \colorbox{red!5}{\strut Occupational} \colorbox{red!13}{\strut Health} \colorbox{red!12}{\strut Clinics} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!5}{\strut Occupational} \colorbox{red!13}{\strut Health} \colorbox{red!12}{\strut Clinics} \colorbox{red!15}{\strut Home} \colorbox{red!13}{\strut Health} \colorbox{red!12}{\strut Care} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!15}{\strut Home} \colorbox{red!13}{\strut Health} \colorbox{red!12}{\strut Care} \colorbox{red!2}{\strut Supportive} \colorbox{red!4}{\strut Housing} \colorbox{red!60}{\strut Alexian} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut for} \colorbox{red!7}{\strut Mental} \colorbox{red!13}{\strut Health} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!0}{\strut AIDS} \colorbox{red!0}{\strut Ministry} \colorbox{red!4}{\strut Outpatient} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Brock} \colorbox{red!17}{\strut Medical} \colorbox{red!4}{\strut Plaza} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Eberle} \colorbox{red!17}{\strut Medical} \colorbox{red!9}{\strut Building} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Niehoff} \colorbox{red!0}{\strut Pavilion} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Pavilion} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Roncoli} \colorbox{red!23}{\strut Center} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!23}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Wimmer} \colorbox{red!23}{\strut Center} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!7}{\strut Group} \colorbox{red!60}{\strut Alexian} \colorbox{red!9}{\strut Rehabilitation} \colorbox{red!23}{\strut Hospital} \colorbox{red!60}{\strut Alexian} \colorbox{red!17}{\strut Medical} \colorbox{red!3}{\strut Mall} \colorbox{red!4}{\strut Outpatient} \colorbox{red!7}{\strut Mental} \colorbox{red!13}{\strut Health} \colorbox{red!14}{\strut Facilities} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!12}{\strut Behavioral} \colorbox{red!13}{\strut Health} \colorbox{red!23}{\strut Hospital} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!12}{\strut Behavioral} \colorbox{red!13}{\strut Health} \colorbox{red!23}{\strut Hospital} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut Group} \colorbox{red!4}{\strut Practice} \colorbox{red!0}{\strut ,} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!17}{\strut Medical} \colorbox{red!4}{\strut Plaza} \colorbox{red!60}{\strut Alexian} \colorbox{red!46}{\strut Brothers} \colorbox{red!12}{\strut Behavioral} \colorbox{red!13}{\strut Health} \colorbox{red!23}{\strut Hospital} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Eberle} \colorbox{red!17}{\strut Medical} \colorbox{red!4}{\strut Office} \colorbox{red!9}{\strut Building} \colorbox{red!0}{\strut AlexianBrothersCenter} \colorbox{red!0}{\strut for} \colorbox{red!7}{\strut Mental} \colorbox{red!13}{\strut Health} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Job} \colorbox{red!0}{\strut Privacy} \colorbox{red!0}{\strut Policy} \colorbox{red!0}{\strut Advertising} \colorbox{red!0}{\strut Policy} \colorbox{red!17}{\strut Medical} \colorbox{red!0}{\strut Disclaimer} \colorbox{red!0}{\strut Media} \colorbox{red!0}{\strut Copyright} \colorbox{red!0}{\strut 2009} \colorbox{red!6}{\strut Congregation} 
}}}
\end{CJK*}

query: wilson antenna

102:antennas, 64:wilson, 41:cb, 32:mobile, 26:base, 25:whip, 24:radios, 24:power, 22:made, 22:load


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!37}{\strut CB} \colorbox{red!22}{\strut Radios} \colorbox{red!4}{\strut 10} \colorbox{red!12}{\strut Meter} \colorbox{red!10}{\strut Amateur} \colorbox{red!22}{\strut Radios} \colorbox{red!16}{\strut Bearcat} \colorbox{red!6}{\strut Scanners} \colorbox{red!0}{\strut 2-Way} \colorbox{red!22}{\strut Radios} \colorbox{red!37}{\strut CB} \colorbox{red!94}{\strut Antennas} \colorbox{red!5}{\strut 2} \colorbox{red!12}{\strut Meter} \colorbox{red!0}{\strut Antenna} \colorbox{red!0}{\strut Antenna} \colorbox{red!12}{\strut Mounting} \colorbox{red!1}{\strut Coax} \colorbox{red!7}{\strut Microphones} \colorbox{red!9}{\strut Speakers} \colorbox{red!22}{\strut Power} \colorbox{red!1}{\strut Supplies} \colorbox{red!3}{\strut Test} \colorbox{red!0}{\strut Meters} \colorbox{red!1}{\strut Accessories} \colorbox{red!1}{\strut Pepper} \colorbox{red!0}{\strut Elec} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Store} \colorbox{red!3}{\strut .} \colorbox{red!37}{\strut CB} \colorbox{red!94}{\strut Antennas} \colorbox{red!3}{\strut .} \colorbox{red!29}{\strut Mobile} \colorbox{red!0}{\strut -} \colorbox{red!37}{\strut CB} \colorbox{red!94}{\strut Antennas} \colorbox{red!3}{\strut .} \colorbox{red!59}{\strut Wilson} \colorbox{red!0}{\strut -} \colorbox{red!29}{\strut Mobile} \colorbox{red!37}{\strut CB} \colorbox{red!94}{\strut Antennas} \colorbox{red!3}{\strut .} \colorbox{red!59}{\strut Wilson} \colorbox{red!0}{\strut -} \colorbox{red!20}{\strut Car} \colorbox{red!94}{\strut Antennas} \colorbox{red!59}{\strut Wilson} \colorbox{red!20}{\strut Car} \colorbox{red!37}{\strut CB} \colorbox{red!94}{\strut Antennas} \colorbox{red!59}{\strut Wilson} \colorbox{red!13}{\strut Short} \colorbox{red!20}{\strut Load} \colorbox{red!2}{\strut 900817} \colorbox{red!0}{\strut 39} \colorbox{red!0}{\strut Inch} \colorbox{red!9}{\strut Center} \colorbox{red!20}{\strut Load} \colorbox{red!23}{\strut Whip} \colorbox{red!10}{\strut Designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Replace} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut Original} \colorbox{red!0}{\strut Longer} \colorbox{red!23}{\strut Whip} \colorbox{red!2}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!59}{\strut Wilson} \colorbox{red!5}{\strut 500} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut 1000} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut 5000} \colorbox{red!24}{\strut Base} \colorbox{red!20}{\strut Load} \colorbox{red!94}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!19}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16.95} \colorbox{red!59}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Little} \colorbox{red!5}{\strut Wil} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Antenna} \colorbox{red!12}{\strut Economically} \colorbox{red!0}{\strut priced} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut Little} \colorbox{red!5}{\strut Wil} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut beaten} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!19}{\strut price} \colorbox{red!0}{\strut verses} \colorbox{red!7}{\strut performance} \colorbox{red!2}{\strut comparison} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut perfect} \colorbox{red!0}{\strut antenna} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut the} \colorbox{red!10}{\strut vacationer} \colorbox{red!0}{\strut .} \colorbox{red!59}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Little} \colorbox{red!5}{\strut Wil} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Specifications} \colorbox{red!0}{\strut 300} \colorbox{red!12}{\strut Watt} \colorbox{red!22}{\strut power} \colorbox{red!5}{\strut handling} \colorbox{red!3}{\strut capability} \colorbox{red!0}{\strut .} \colorbox{red!16}{\strut ICAS} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Made} \colorbox{red!0}{\strut with} \colorbox{red!9}{\strut high} \colorbox{red!16}{\strut impact} \colorbox{red!7}{\strut Thermoplastic} \colorbox{red!16}{\strut Heavy} \colorbox{red!11}{\strut duty} \colorbox{red!16}{\strut coil} \colorbox{red!3}{\strut uses} \colorbox{red!0}{\strut 14} \colorbox{red!12}{\strut gauge} \colorbox{red!4}{\strut copper} \colorbox{red!15}{\strut wire} \colorbox{red!1}{\strut Exclusive} \colorbox{red!6}{\strut low} \colorbox{red!7}{\strut loss} \colorbox{red!16}{\strut coil} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut Patent} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4,882,591} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Same} \colorbox{red!0}{\strut as} \colorbox{red!59}{\strut Wilson} \colorbox{red!7}{\strut 1000} \colorbox{red!1}{\strut 36} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 17-7} \colorbox{red!9}{\strut PH} \colorbox{red!2}{\strut stainless} \colorbox{red!12}{\strut steel} \colorbox{red!23}{\strut whip} \colorbox{red!19}{\strut Frequency} \colorbox{red!15}{\strut range} \colorbox{red!0}{\strut 26} \colorbox{red!7}{\strut MHz} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 30} \colorbox{red!7}{\strut MHz} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Year} \colorbox{red!7}{\strut Warranty} \colorbox{red!19}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 39.95} \colorbox{red!59}{\strut Wilson} \colorbox{red!5}{\strut 500} \colorbox{red!0}{\strut Antenna} \colorbox{red!0}{\strut With} \colorbox{red!2}{\strut Higher} \colorbox{red!7}{\strut performance} \colorbox{red!0}{\strut than} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut Little} \colorbox{red!0}{\strut Will} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut priced} \colorbox{red!0}{\strut lower} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut a} \colorbox{red!59}{\strut Wilson} \colorbox{red!7}{\strut 1000} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut perfect} \colorbox{red!7}{\strut mid} \colorbox{red!15}{\strut range} \colorbox{red!0}{\strut antenna} \colorbox{red!0}{\strut .} \colorbox{red!59}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut 500} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Specifications} \colorbox{red!0}{\strut 2000} \colorbox{red!12}{\strut Watt} \colorbox{red!22}{\strut power} \colorbox{red!5}{\strut handling} \colorbox{red!3}{\strut capability} \colorbox{red!0}{\strut .} \colorbox{red!16}{\strut ICAS} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Made} \colorbox{red!0}{\strut with} \colorbox{red!9}{\strut high} \colorbox{red!16}{\strut impact} \colorbox{red!7}{\strut Thermoplastic} \colorbox{red!16}{\strut Heavy} \colorbox{red!11}{\strut duty} \colorbox{red!16}{\strut coil} \colorbox{red!3}{\strut uses} \colorbox{red!0}{\strut 12} \colorbox{red!12}{\strut gauge} \colorbox{red!4}{\strut copper} \colorbox{red!15}{\strut wire} \colorbox{red!1}{\strut Exclusive} \colorbox{red!6}{\strut low} \colorbox{red!7}{\strut loss} \colorbox{red!16}{\strut coil} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut Patent} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4,882,591} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Same} \colorbox{red!0}{\strut as} \colorbox{red!59}{\strut Wilson} \colorbox{red!7}{\strut 1000} \colorbox{red!0}{\strut 54} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 17-7} \colorbox{red!9}{\strut PH} \colorbox{red!2}{\strut stainless} \colorbox{red!12}{\strut steel} \colorbox{red!23}{\strut whip} \colorbox{red!5}{\strut 2} \colorbox{red!0}{\strut year} \colorbox{red!7}{\strut warranty} \colorbox{red!19}{\strut Frequency} \colorbox{red!15}{\strut range} \colorbox{red!0}{\strut 26} \colorbox{red!7}{\strut MHz} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 30} \colorbox{red!7}{\strut MHz} \colorbox{red!8}{\strut Weather} \colorbox{red!8}{\strut Channel} \colorbox{red!1}{\strut Ready} \colorbox{red!19}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 64.95} \colorbox{red!59}{\strut Wilson} \colorbox{red!7}{\strut 1000} \colorbox{red!0}{\strut Antenna} \colorbox{red!2}{\strut The} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut recognized} \colorbox{red!0}{\strut antenna} \colorbox{red!2}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut market} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Available} \colorbox{red!0}{\strut in} \colorbox{red!15}{\strut Roof} \colorbox{red!4}{\strut Top} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut Trunk} \colorbox{red!5}{\strut Lip} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!7}{\strut Magnetic} \colorbox{red!0}{\strut mounts} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Magnetic} \colorbox{red!0}{\strut Mount} \colorbox{red!0}{\strut Shown} \colorbox{red!59}{\strut Wilson} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut 1000} 
}}}
\end{CJK*}

101:antenna, 51:type, 36:phone, 31:wilson, 31:dt, 30:cell, 29:mobile, 29:cellular, 27:wireless, 26:cart


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Set} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Add} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Favorites} \colorbox{red!4}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut About} \colorbox{red!2}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Contact} \colorbox{red!2}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Site} \colorbox{red!1}{\strut map} \colorbox{red!4}{\strut Customer} \colorbox{red!5}{\strut Service} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 888} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 512-6774} \colorbox{red!2}{\strut Purchase} \colorbox{red!3}{\strut Orders} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut accepted} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut Day} \colorbox{red!0}{\strut Satisfaction} \colorbox{red!1}{\strut Guarantee} \colorbox{red!0}{\strut Reviews} \colorbox{red!4}{\strut Home} \colorbox{red!0}{\strut Catalog} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut account} \colorbox{red!1}{\strut View} \colorbox{red!8}{\strut cart} \colorbox{red!0}{\strut Quick} \colorbox{red!2}{\strut Search} \colorbox{red!2}{\strut Search} \colorbox{red!1}{\strut for} \colorbox{red!3}{\strut pattern} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Advanced} \colorbox{red!2}{\strut search} \colorbox{red!5}{\strut Reception} \colorbox{red!1}{\strut Products} \colorbox{red!4}{\strut Amplifiers} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Repeaters} \colorbox{red!32}{\strut Antenna} \colorbox{red!4}{\strut Adapters} \colorbox{red!0}{\strut Antennas} \colorbox{red!1}{\strut Coax} \colorbox{red!1}{\strut Cables} \colorbox{red!1}{\strut Complete} \colorbox{red!1}{\strut Kits} \colorbox{red!1}{\strut Components} \colorbox{red!1}{\strut Connectors} \colorbox{red!1}{\strut Crimps} \colorbox{red!4}{\strut Mounts} \colorbox{red!2}{\strut Power} \colorbox{red!2}{\strut Supplies} \colorbox{red!3}{\strut Splitters} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Taps} \colorbox{red!1}{\strut Accessory} \colorbox{red!1}{\strut by} \colorbox{red!16}{\strut Type} \colorbox{red!6}{\strut Bluetooth} \colorbox{red!7}{\strut Car} \colorbox{red!1}{\strut Kits} \colorbox{red!6}{\strut Bluetooth} \colorbox{red!1}{\strut Headsets} \colorbox{red!1}{\strut GPS} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Navigation} \colorbox{red!2}{\strut Search} \colorbox{red!1}{\strut by} \colorbox{red!3}{\strut Carrier} \colorbox{red!0}{\strut Browse} \colorbox{red!1}{\strut for} \colorbox{red!3}{\strut equipment} \colorbox{red!1}{\strut by} \colorbox{red!0}{\strut your} \colorbox{red!8}{\strut wireless} \colorbox{red!5}{\strut service} \colorbox{red!4}{\strut provider} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut AT} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut T} \colorbox{red!4}{\strut Bell} \colorbox{red!2}{\strut Nextel} \colorbox{red!6}{\strut Sprint} \colorbox{red!0}{\strut T-Mobile} \colorbox{red!3}{\strut Verizon} \colorbox{red!8}{\strut Wireless} \colorbox{red!2}{\strut Manufacturers} \colorbox{red!0}{\strut Information} \colorbox{red!1}{\strut About} \colorbox{red!2}{\strut Us} \colorbox{red!2}{\strut Contact} \colorbox{red!2}{\strut Us} \colorbox{red!4}{\strut Customer} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut Returns} \colorbox{red!0}{\strut Privacy} \colorbox{red!1}{\strut Policy} \colorbox{red!1}{\strut Testimonials} \colorbox{red!0}{\strut Latest} \colorbox{red!0}{\strut Posts} \colorbox{red!1}{\strut AT} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut T} \colorbox{red!2}{\strut Moving} \colorbox{red!1}{\strut EDGE} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 1900} \colorbox{red!2}{\strut Mhz} \colorbox{red!5}{\strut Band} \colorbox{red!9}{\strut Wilson} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut powerful} \colorbox{red!4}{\strut amplifiers} \colorbox{red!0}{\strut yet} \colorbox{red!9}{\strut Wilson} \colorbox{red!3}{\strut Electronics} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut The} \colorbox{red!8}{\strut Wireless} \colorbox{red!4}{\strut Technology} \colorbox{red!1}{\strut Leader} \colorbox{red!2}{\strut Why} \colorbox{red!9}{\strut Wilson} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Fire} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Ice} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut The} \colorbox{red!1}{\strut only} \colorbox{red!2}{\strut break} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut signal} \colorbox{red!1}{\strut Testimonials} \colorbox{red!0}{\strut Author} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tom} \colorbox{red!2}{\strut worked} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut well} \colorbox{red!4}{\strut Home} \colorbox{red!0}{\strut Antennas} \colorbox{red!0}{\strut Antennas} \colorbox{red!0}{\strut Our} \colorbox{red!1}{\strut full} \colorbox{red!2}{\strut line} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut patented} \colorbox{red!9}{\strut cell} \colorbox{red!11}{\strut phone} \colorbox{red!0}{\strut antennas} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut commited} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut bringing} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut highest} \colorbox{red!1}{\strut performance} \colorbox{red!0}{\strut possible} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!3}{\strut carry} \colorbox{red!0}{\strut an} \colorbox{red!32}{\strut antenna} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut almost} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut application} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut situation} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Whether} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!7}{\strut car} \colorbox{red!0}{\strut or} \colorbox{red!4}{\strut home} \colorbox{red!0}{\strut ,} \colorbox{red!9}{\strut Wilson} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Cellularantennas} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reduce} \colorbox{red!2}{\strut disconnects} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut drop} \colorbox{red!0}{\strut outs} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut noise} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut antennas} \colorbox{red!0}{\strut significantly} \colorbox{red!2}{\strut increase} \colorbox{red!0}{\strut your} \colorbox{red!9}{\strut cell} \colorbox{red!11}{\strut phone} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut range} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut reception} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut also} \colorbox{red!2}{\strut help} \colorbox{red!0}{\strut eliminate} \colorbox{red!0}{\strut dead} \colorbox{red!2}{\strut zones} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Most} \colorbox{red!9}{\strut cell} \colorbox{red!11}{\strut phone} \colorbox{red!0}{\strut antennas} \colorbox{red!5}{\strut install} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut minutes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut tools} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!1}{\strut narrow} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut search} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut select} \colorbox{red!32}{\strut antenna} \colorbox{red!16}{\strut type} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Mobile} \colorbox{red!0}{\strut Antennas} \colorbox{red!5}{\strut Building} \colorbox{red!0}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Yagi} \colorbox{red!0}{\strut Antennas} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut Dome} \colorbox{red!0}{\strut Antennas} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Cell} \colorbox{red!11}{\strut Phone} \colorbox{red!32}{\strut Antenna} \colorbox{red!4}{\strut Adapters} \colorbox{red!2}{\strut Pages} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!1}{\strut 2} \colorbox{red!1}{\strut 3} \colorbox{red!4}{\strut Range} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Sort} \colorbox{red!1}{\strut by} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Product} \colorbox{red!5}{\strut Price} \colorbox{red!3}{\strut Default} \colorbox{red!9}{\strut Wilson} \colorbox{red!3}{\strut Black} \colorbox{red!3}{\strut Rubber} \colorbox{red!32}{\strut Antenna} \colorbox{red!0}{\strut with} \colorbox{red!5}{\strut TNC} \colorbox{red!2}{\strut Male} \colorbox{red!0}{\strut Connector} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 301144} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Wilson} \colorbox{red!3}{\strut Black} \colorbox{red!3}{\strut Rubber} \colorbox{red!32}{\strut Antenna} \colorbox{red!0}{\strut with} 
}}}
\end{CJK*}

query: continental plates

99:plate, 94:continental, 63:what, 48:tectonics, 28:types, 25:boundaries, 22:earth, 20:theory, 20:lithosphere, 19:major


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!68}{\strut Plate} \colorbox{red!33}{\strut tectonics} \colorbox{red!4}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Redirected} \colorbox{red!4}{\strut from} \colorbox{red!65}{\strut Continental} \colorbox{red!0}{\strut plates} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Jump} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut navigation} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut search} \colorbox{red!3}{\strut The} \colorbox{red!0}{\strut tectonic} \colorbox{red!0}{\strut plates} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut world} \colorbox{red!2}{\strut were} \colorbox{red!10}{\strut mapped} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut second} \colorbox{red!1}{\strut half} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut 20th} \colorbox{red!3}{\strut century} \colorbox{red!2}{\strut .} \colorbox{red!68}{\strut Plate} \colorbox{red!33}{\strut tectonics} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut from} \colorbox{red!4}{\strut Greek} \colorbox{red!2}{\strut ,} \colorbox{red!7}{\strut tektn} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut builder} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut mason} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut describes} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut large} \colorbox{red!6}{\strut scale} \colorbox{red!11}{\strut motions} \colorbox{red!5}{\strut of} \colorbox{red!15}{\strut Earth} \colorbox{red!0}{\strut s} \colorbox{red!13}{\strut lithosphere} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!13}{\strut theory} \colorbox{red!2}{\strut encompasses} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut older} \colorbox{red!7}{\strut concepts} \colorbox{red!5}{\strut of} \colorbox{red!65}{\strut continental} \colorbox{red!13}{\strut drift} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut developed} \colorbox{red!2}{\strut during} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut first} \colorbox{red!1}{\strut half} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut 20th} \colorbox{red!3}{\strut century} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!5}{\strut seafloor} \colorbox{red!9}{\strut spreading} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut understood} \colorbox{red!2}{\strut during} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut 1960s} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!4}{\strut outermost} \colorbox{red!7}{\strut part} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!15}{\strut Earth} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut interior} \colorbox{red!2}{\strut is} \colorbox{red!9}{\strut made} \colorbox{red!1}{\strut up} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut two} \colorbox{red!11}{\strut layers} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut above} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut the} \colorbox{red!13}{\strut lithosphere} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut comprising} \colorbox{red!3}{\strut the} \colorbox{red!11}{\strut crust} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut rigid} \colorbox{red!4}{\strut uppermost} \colorbox{red!7}{\strut part} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut mantle} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Below} \colorbox{red!3}{\strut the} \colorbox{red!13}{\strut lithosphere} \colorbox{red!2}{\strut lies} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut asthenosphere} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Although} \colorbox{red!5}{\strut solid} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut asthenosphere} \colorbox{red!0}{\strut has} \colorbox{red!2}{\strut relatively} \colorbox{red!2}{\strut low} \colorbox{red!4}{\strut viscosity} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut shear} \colorbox{red!2}{\strut strength} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut can} \colorbox{red!4}{\strut flow} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut liquid} \colorbox{red!0}{\strut on} \colorbox{red!13}{\strut geological} \colorbox{red!6}{\strut time} \colorbox{red!0}{\strut scales} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!2}{\strut deeper} \colorbox{red!8}{\strut mantle} \colorbox{red!2}{\strut below} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut asthenosphere} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut more} \colorbox{red!3}{\strut rigid} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut due} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut higher} \colorbox{red!2}{\strut pressure} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!13}{\strut lithosphere} \colorbox{red!2}{\strut is} \colorbox{red!7}{\strut broken} \colorbox{red!1}{\strut up} \colorbox{red!2}{\strut into} \colorbox{red!43}{\strut what} \colorbox{red!3}{\strut are} \colorbox{red!11}{\strut called} \colorbox{red!0}{\strut tectonic} \colorbox{red!0}{\strut plates} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut case} \colorbox{red!5}{\strut of} \colorbox{red!15}{\strut Earth} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!3}{\strut are} \colorbox{red!2}{\strut seven} \colorbox{red!13}{\strut major} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut minor} \colorbox{red!0}{\strut plates} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!2}{\strut list} \colorbox{red!2}{\strut below} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!0}{\strut lithospheric} \colorbox{red!0}{\strut plates} \colorbox{red!4}{\strut ride} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut asthenosphere} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut These} \colorbox{red!0}{\strut plates} \colorbox{red!9}{\strut move} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut relation} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut one} \colorbox{red!2}{\strut another} \colorbox{red!2}{\strut at} \colorbox{red!0}{\strut one} \colorbox{red!5}{\strut of} \colorbox{red!4}{\strut three} \colorbox{red!19}{\strut types} \colorbox{red!5}{\strut of} \colorbox{red!68}{\strut plate} \colorbox{red!17}{\strut boundaries} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut convergent} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!5}{\strut collisional} \colorbox{red!17}{\strut boundaries} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut divergent} \colorbox{red!17}{\strut boundaries} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!11}{\strut called} \colorbox{red!9}{\strut spreading} \colorbox{red!3}{\strut centers} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut and} \colorbox{red!8}{\strut transform} \colorbox{red!17}{\strut boundaries} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Earthquakes} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut volcanic} \colorbox{red!5}{\strut activity} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut mountain} \colorbox{red!0}{\strut -building} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!9}{\strut oceanic} \colorbox{red!10}{\strut trench} \colorbox{red!6}{\strut formation} \colorbox{red!10}{\strut occur} \colorbox{red!2}{\strut along} \colorbox{red!68}{\strut plate} \colorbox{red!17}{\strut boundaries} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!4}{\strut lateral} \colorbox{red!12}{\strut movement} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut plates} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut typically} \colorbox{red!2}{\strut at} \colorbox{red!3}{\strut speeds} \colorbox{red!5}{\strut of} \colorbox{red!0}{\strut 50100} \colorbox{red!1}{\strut mm} \colorbox{red!3}{\strut annually} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Contents} \colorbox{red!3}{\strut 1} \colorbox{red!3}{\strut Synopsis} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut development} \colorbox{red!5}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!13}{\strut theory} \colorbox{red!2}{\strut 2} \colorbox{red!2}{\strut Key} \colorbox{red!2}{\strut principles} \colorbox{red!2}{\strut 3} \colorbox{red!19}{\strut Types} \colorbox{red!5}{\strut of} \colorbox{red!68}{\strut plate} \colorbox{red!17}{\strut boundaries} \colorbox{red!0}{\strut 3.1} \colorbox{red!8}{\strut Transform} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut conservative} \colorbox{red!2}{\strut .} 
}}}
\end{CJK*}

98:plate, 97:tectonics, 74:what, 36:theory, 23:continental, 20:earth, 20:drift, 19:rocks, 19:drives, 18:earthquakes


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Home} \colorbox{red!1}{\strut Pete} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut Presentations} \colorbox{red!8}{\strut Science} \colorbox{red!3}{\strut Free} \colorbox{red!3}{\strut Presentations} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut PowerPoint} \colorbox{red!6}{\strut format} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!1}{\strut -} \colorbox{red!10}{\strut earth} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut augusta} \colorbox{red!2}{\strut .} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut graves} \colorbox{red!2}{\strut .} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut bloomington} \colorbox{red!2}{\strut .} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut rockwood} \colorbox{red!2}{\strut .} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut eastchester} \colorbox{red!2}{\strut .} \colorbox{red!19}{\strut Theory} \colorbox{red!3}{\strut of} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut step} \colorbox{red!2}{\strut .} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!4}{\strut 1} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!5}{\strut 2} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!3}{\strut ,} \colorbox{red!10}{\strut Rocks} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Mountain} \colorbox{red!5}{\strut Building} \colorbox{red!7}{\strut Understanding} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!1}{\strut around} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut world} \colorbox{red!12}{\strut Continental} \colorbox{red!10}{\strut Drift} \colorbox{red!3}{\strut San} \colorbox{red!4}{\strut Andreas} \colorbox{red!4}{\strut Fault} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut ppt} \colorbox{red!1}{\strut with} \colorbox{red!3}{\strut audio} \colorbox{red!3}{\strut narrative} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut Also} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut Earthquakes} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Volcanoes} \colorbox{red!3}{\strut ,} \colorbox{red!10}{\strut Rocks} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Minerals} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut Introduction} \colorbox{red!2}{\strut to} \colorbox{red!7}{\strut Geology} \colorbox{red!2}{\strut For} \colorbox{red!2}{\strut Kids} \colorbox{red!39}{\strut What} \colorbox{red!10}{\strut drives} \colorbox{red!51}{\strut plate} \colorbox{red!51}{\strut tectonics} \colorbox{red!0}{\strut ?} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!1}{\strut -} \colorbox{red!39}{\strut what} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut Pangaea} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Pangea} \colorbox{red!2}{\strut .} \colorbox{red!19}{\strut Theory} \colorbox{red!0}{\strut On} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut move} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!1}{\strut -} \colorbox{red!4}{\strut animation} \colorbox{red!2}{\strut and} \colorbox{red!6}{\strut movie} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut thinkquest} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut All} \colorbox{red!0}{\strut About} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!5}{\strut Dynamic} \colorbox{red!10}{\strut Earth} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut interactive} \colorbox{red!2}{\strut .} \colorbox{red!12}{\strut Continental} \colorbox{red!10}{\strut Drift} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut animated} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut movie} \colorbox{red!2}{\strut .} \colorbox{red!12}{\strut Continental} \colorbox{red!10}{\strut Drift} \colorbox{red!12}{\strut Continental} \colorbox{red!10}{\strut Drift} \colorbox{red!1}{\strut -} \colorbox{red!3}{\strut Interactive} \colorbox{red!3}{\strut Quiz} \colorbox{red!12}{\strut Continental} \colorbox{red!5}{\strut Rift} \colorbox{red!4}{\strut game} \colorbox{red!9}{\strut Earthquakes} \colorbox{red!7}{\strut Volcanoes} \colorbox{red!2}{\strut For} \colorbox{red!3}{\strut Teachers} \colorbox{red!51}{\strut Plate} \colorbox{red!51}{\strut Tectonics} \colorbox{red!1}{\strut -} \colorbox{red!3}{\strut Wilson} \colorbox{red!3}{\strut Cycle} \colorbox{red!0}{\strut Rifting} \colorbox{red!3}{\strut Free} \colorbox{red!2}{\strut Clipart} \colorbox{red!2}{\strut for} \colorbox{red!8}{\strut Science} \colorbox{red!3}{\strut Free} \colorbox{red!2}{\strut Templates} \colorbox{red!2}{\strut This} \colorbox{red!3}{\strut free} \colorbox{red!3}{\strut site} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut a} \colorbox{red!2}{\strut partnership} \colorbox{red!2}{\strut between} \colorbox{red!0}{\strut mrdonn.org} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut phillipmartin.info} \colorbox{red!1}{\strut ALL} \colorbox{red!4}{\strut ART} \colorbox{red!3}{\strut OWNED} \colorbox{red!1}{\strut BY} \colorbox{red!2}{\strut PHILLIP} \colorbox{red!2}{\strut MARTIN} \colorbox{red!1}{\strut All} \colorbox{red!1}{\strut Rights} \colorbox{red!0}{\strut Reserved} 
}}}
\end{CJK*}

query: ocd

100:ocd, 62:pure, 24:causes, 22:disorder, 16:suffer, 13:who, 12:obsessive, 10:written, 10:anxiety, 9:effects


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut .} \colorbox{red!8}{\strut Taking} \colorbox{red!5}{\strut a} \colorbox{red!4}{\strut look} \colorbox{red!0}{\strut into} \colorbox{red!5}{\strut the} \colorbox{red!6}{\strut world} \colorbox{red!5}{\strut of} \colorbox{red!100}{\strut OCD} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut pure-ocd} \colorbox{red!5}{\strut .} \colorbox{red!2}{\strut This} \colorbox{red!8}{\strut website} \colorbox{red!5}{\strut is} \colorbox{red!8}{\strut designed} \colorbox{red!5}{\strut to} \colorbox{red!9}{\strut educate} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut inform} \colorbox{red!4}{\strut people} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!13}{\strut anxiety} \colorbox{red!29}{\strut disorder} \colorbox{red!5}{\strut ,} \colorbox{red!100}{\strut OCD} \colorbox{red!6}{\strut .} \colorbox{red!16}{\strut Obsessive} \colorbox{red!12}{\strut Compulsive} \colorbox{red!29}{\strut Disorder} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut .} \colorbox{red!100}{\strut OCD} \colorbox{red!5}{\strut is} \colorbox{red!8}{\strut ananxiety} \colorbox{red!29}{\strut disorder} \colorbox{red!5}{\strut that} \colorbox{red!32}{\strut causes} \colorbox{red!5}{\strut a} \colorbox{red!6}{\strut person} \colorbox{red!5}{\strut to} \colorbox{red!21}{\strut suffer} \colorbox{red!2}{\strut unwanted} \colorbox{red!10}{\strut thoughts} \colorbox{red!5}{\strut ,} \colorbox{red!6}{\strut urges} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!9}{\strut feelings} \colorbox{red!5}{\strut .} \colorbox{red!2}{\strut This} \colorbox{red!8}{\strut website} \colorbox{red!0}{\strut showcases} \colorbox{red!4}{\strut many} \colorbox{red!9}{\strut forms} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!29}{\strut disorder} \colorbox{red!2}{\strut in} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut shortstory} \colorbox{red!5}{\strut ,} \colorbox{red!8}{\strut script} \colorbox{red!6}{\strut stye} \colorbox{red!6}{\strut format} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut The} \colorbox{red!9}{\strut aim} \colorbox{red!5}{\strut is} \colorbox{red!5}{\strut to} \colorbox{red!4}{\strut promote} \colorbox{red!2}{\strut awareness} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut justof} \colorbox{red!0}{\strut OCDitself} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!4}{\strut its} \colorbox{red!4}{\strut many} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut ignored} \colorbox{red!9}{\strut forms} \colorbox{red!4}{\strut and} \colorbox{red!5}{\strut the} \colorbox{red!12}{\strut effects} \colorbox{red!0}{\strut it} \colorbox{red!5}{\strut has} \colorbox{red!1}{\strut on} \colorbox{red!6}{\strut asufferer} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut life} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut all} \colorbox{red!5}{\strut ,} \colorbox{red!5}{\strut as} \colorbox{red!5}{\strut one} \colorbox{red!0}{\strut sufferer} \colorbox{red!2}{\strut remarked} \colorbox{red!1}{\strut .} \colorbox{red!100}{\strut OCD} \colorbox{red!5}{\strut IS} \colorbox{red!5}{\strut A} \colorbox{red!4}{\strut MULTIFACETED} \colorbox{red!29}{\strut DISORDER} \colorbox{red!4}{\strut AND} \colorbox{red!0}{\strut SHOULDBE} \colorbox{red!9}{\strut TREATED} \colorbox{red!4}{\strut LIKEWISE} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut this} \colorbox{red!0}{\strut quote} \colorbox{red!2}{\strut in} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut waysums} \colorbox{red!0}{\strut up} \colorbox{red!2}{\strut this} \colorbox{red!0}{\strut whole} \colorbox{red!8}{\strut website} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut The} \colorbox{red!5}{\strut site} \colorbox{red!1}{\strut features} \colorbox{red!5}{\strut fictional} \colorbox{red!5}{\strut accounts} \colorbox{red!5}{\strut of} \colorbox{red!0}{\strut livesaffected} \colorbox{red!2}{\strut by} \colorbox{red!100}{\strut OCD} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut some} \colorbox{red!5}{\strut of} \colorbox{red!9}{\strut which} \colorbox{red!4}{\strut are} \colorbox{red!8}{\strut based} \colorbox{red!1}{\strut on} \colorbox{red!6}{\strut real} \colorbox{red!0}{\strut sufferers} \colorbox{red!5}{\strut ,} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut although} \colorbox{red!2}{\strut thenames} \colorbox{red!2}{\strut have} \colorbox{red!4}{\strut been} \colorbox{red!6}{\strut changed} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!5}{\strut has} \colorbox{red!4}{\strut been} \colorbox{red!13}{\strut written} \colorbox{red!2}{\strut by} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut sufferer} \colorbox{red!4}{\strut and} \colorbox{red!5}{\strut has} \colorbox{red!2}{\strut beenendorsed} \colorbox{red!2}{\strut by} \colorbox{red!0}{\strut sufferers} \colorbox{red!0}{\strut too} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut The} \colorbox{red!8}{\strut stories} \colorbox{red!0}{\strut themselves} \colorbox{red!4}{\strut are} \colorbox{red!4}{\strut short} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!1}{\strut highlight} \colorbox{red!5}{\strut the} \colorbox{red!5}{\strut constant} \colorbox{red!5}{\strut battle} \colorbox{red!5}{\strut aperson} \colorbox{red!5}{\strut has} \colorbox{red!2}{\strut with} \colorbox{red!100}{\strut OCD} \colorbox{red!5}{\strut ,} \colorbox{red!1}{\strut or} \colorbox{red!2}{\strut in} \colorbox{red!5}{\strut the} \colorbox{red!8}{\strut stories} \colorbox{red!6}{\strut case} \colorbox{red!0}{\strut Mr} \colorbox{red!100}{\strut OCD} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut Many} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!8}{\strut stories} \colorbox{red!0}{\strut arehumorous} \colorbox{red!5}{\strut ,} \colorbox{red!1}{\strut dark} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut thought} \colorbox{red!6}{\strut provoking} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut showsides} \colorbox{red!5}{\strut that} \colorbox{red!4}{\strut are} \colorbox{red!0}{\strut often} \colorbox{red!1}{\strut inignoredby} \colorbox{red!5}{\strut the} \colorbox{red!5}{\strut media} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!1}{\strut sadly} \colorbox{red!2}{\strut in} \colorbox{red!4}{\strut some} \colorbox{red!0}{\strut cases} \colorbox{red!5}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!8}{\strut medical} \colorbox{red!5}{\strut proffession} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut We} \colorbox{red!4}{\strut want} \colorbox{red!5}{\strut toput} \colorbox{red!4}{\strut those} \colorbox{red!17}{\strut who} \colorbox{red!4}{\strut are} \colorbox{red!2}{\strut unaware} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!29}{\strut disorder} \colorbox{red!2}{\strut in} \colorbox{red!5}{\strut the} \colorbox{red!5}{\strut picture} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut we} \colorbox{red!0}{\strut hopethat} \colorbox{red!1}{\strut you} \colorbox{red!5}{\strut learn} \colorbox{red!5}{\strut a} \colorbox{red!4}{\strut great} \colorbox{red!4}{\strut deal} \colorbox{red!2}{\strut from} \colorbox{red!0}{\strut it} \colorbox{red!5}{\strut ,} \colorbox{red!5}{\strut as} \colorbox{red!2}{\strut this} \colorbox{red!5}{\strut is} \colorbox{red!0}{\strut so} \colorbox{red!4}{\strut important} \colorbox{red!4}{\strut for} \colorbox{red!2}{\strut future} \colorbox{red!2}{\strut andpresent} \colorbox{red!0}{\strut awarness} \colorbox{red!5}{\strut .} \colorbox{red!8}{\strut TRIGGER} \colorbox{red!9}{\strut WARNING} \colorbox{red!5}{\strut !} \colorbox{red!0}{\strut If} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut sufferer} \colorbox{red!0}{\strut ofOCD} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut want} \colorbox{red!5}{\strut to} \colorbox{red!5}{\strut read} \colorbox{red!5}{\strut the} \colorbox{red!8}{\strut stories} \colorbox{red!5}{\strut ,} \colorbox{red!2}{\strut please} \colorbox{red!5}{\strut be} \colorbox{red!0}{\strut aware} \colorbox{red!5}{\strut that} \colorbox{red!1}{\strut they} \colorbox{red!2}{\strut may} \colorbox{red!4}{\strut contain} \colorbox{red!0}{\strut triggers} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut pure-ocd} \colorbox{red!0}{\strut ContaminationChecking} \colorbox{red!4}{\strut Hoarding} \colorbox{red!8}{\strut Magical} \colorbox{red!0}{\strut ThinkingLinking} \colorbox{red!83}{\strut Pure} \colorbox{red!10}{\strut O} \colorbox{red!5}{\strut Symmetry} \colorbox{red!4}{\strut Help} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut support} \colorbox{red!2}{\strut Guestbook} \colorbox{red!5}{\strut Create} \colorbox{red!5}{\strut a} \colorbox{red!4}{\strut free} \colorbox{red!8}{\strut website} \colorbox{red!4}{\strut at} \colorbox{red!0}{\strut Webs.com} \colorbox{red!0}{\strut kirktacey005llightseserved} \colorbox{red!5}{\strut .} 
}}}
\end{CJK*}

100:ocd, 91:what, 23:center, 19:treatment, 17:therapy, 17:obsessional, 16:disorders, 15:spectrum, 15:phobias, 14:oc


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Contact} \colorbox{red!2}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut here} \colorbox{red!1}{\strut to} \colorbox{red!6}{\strut email} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut L.A.} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 310} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 335-5443} \colorbox{red!4}{\strut Specializing} \colorbox{red!3}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut Treatment} \colorbox{red!2}{\strut of} \colorbox{red!66}{\strut OCD} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut Related} \colorbox{red!4}{\strut Conditions} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut CENTER} \colorbox{red!2}{\strut OF} \colorbox{red!7}{\strut LOS} \colorbox{red!5}{\strut ANGELES} \colorbox{red!5}{\strut SITE} \colorbox{red!5}{\strut MAP} \colorbox{red!60}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!66}{\strut OCD} \colorbox{red!2}{\strut ?} \colorbox{red!8}{\strut Pure} \colorbox{red!11}{\strut Obsessional} \colorbox{red!66}{\strut OCD} \colorbox{red!4}{\strut Postpartum} \colorbox{red!66}{\strut OCD} \colorbox{red!4}{\strut Childhood} \colorbox{red!1}{\strut .} \colorbox{red!8}{\strut Adolescent} \colorbox{red!66}{\strut OCD} \colorbox{red!2}{\strut The} \colorbox{red!6}{\strut Obsessive} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Compulsive} \colorbox{red!4}{\strut Cycle} \colorbox{red!0}{\strut Obsessive-Compulsive} \colorbox{red!10}{\strut Spectrum} \colorbox{red!10}{\strut Disorders} \colorbox{red!6}{\strut Body} \colorbox{red!8}{\strut Dysmorphic} \colorbox{red!0}{\strut Disorder} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut BDD} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut Hypochondria} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Health} \colorbox{red!8}{\strut Anxiety} \colorbox{red!10}{\strut Phobias} \colorbox{red!4}{\strut Panic} \colorbox{red!0}{\strut Disorder} \colorbox{red!7}{\strut Social} \colorbox{red!8}{\strut Anxiety} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Social} \colorbox{red!0}{\strut Phobia} \colorbox{red!6}{\strut Trichotillomania} \colorbox{red!8}{\strut Compulsive} \colorbox{red!4}{\strut Skin} \colorbox{red!2}{\strut Picking} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Dermatillomania} \colorbox{red!5}{\strut Olfactory} \colorbox{red!4}{\strut Reference} \colorbox{red!5}{\strut Syndrome} \colorbox{red!66}{\strut OCD} \colorbox{red!12}{\strut Treatment} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Cognitive} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut Behavioral} \colorbox{red!11}{\strut Therapy} \colorbox{red!66}{\strut OCD} \colorbox{red!7}{\strut Test} \colorbox{red!66}{\strut OCD} \colorbox{red!0}{\strut TherapySupport} \colorbox{red!5}{\strut Groups} \colorbox{red!1}{\strut For} \colorbox{red!5}{\strut Adults} \colorbox{red!66}{\strut OCD} \colorbox{red!0}{\strut TherapySupport} \colorbox{red!5}{\strut Groups} \colorbox{red!1}{\strut for} \colorbox{red!5}{\strut Children} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Adolescents} \colorbox{red!66}{\strut OCD} \colorbox{red!6}{\strut Readings} \colorbox{red!66}{\strut OCD} \colorbox{red!4}{\strut Resources} \colorbox{red!2}{\strut About} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!4}{\strut Staff} \colorbox{red!4}{\strut Directions} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!6}{\strut Email} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!3}{\strut Home} \colorbox{red!60}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!66}{\strut OCD} \colorbox{red!2}{\strut ?} \colorbox{red!8}{\strut Pure} \colorbox{red!11}{\strut Obsessional} \colorbox{red!66}{\strut OCD} \colorbox{red!4}{\strut Postpartum} \colorbox{red!66}{\strut OCD} \colorbox{red!4}{\strut Childhood} \colorbox{red!1}{\strut .} \colorbox{red!8}{\strut Adolescent} \colorbox{red!66}{\strut OCD} \colorbox{red!6}{\strut Body} \colorbox{red!8}{\strut Dysmorphic} \colorbox{red!0}{\strut Disorder} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut BDD} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut Hypochondria} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Health} \colorbox{red!8}{\strut Anxiety} \colorbox{red!10}{\strut Phobias} \colorbox{red!4}{\strut Panic} \colorbox{red!0}{\strut Disorder} \colorbox{red!7}{\strut Social} \colorbox{red!8}{\strut Anxiety} \colorbox{red!6}{\strut Trichotillomania} \colorbox{red!8}{\strut Compulsive} \colorbox{red!4}{\strut Skin} \colorbox{red!2}{\strut Picking} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut CSP} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Olfactory} \colorbox{red!4}{\strut Reference} \colorbox{red!5}{\strut Syndrome} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut ORS} \colorbox{red!3}{\strut .} \colorbox{red!66}{\strut OCD} \colorbox{red!12}{\strut Treatment} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Cognitive} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut Behavioral} \colorbox{red!11}{\strut Therapy} \colorbox{red!2}{\strut The} \colorbox{red!6}{\strut Obsessive} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Compulsive} \colorbox{red!4}{\strut Cycle} \colorbox{red!9}{\strut OC} \colorbox{red!10}{\strut Spectrum} \colorbox{red!10}{\strut Disorders} \colorbox{red!66}{\strut OCD} \colorbox{red!7}{\strut Test} \colorbox{red!66}{\strut OCD} \colorbox{red!0}{\strut TherapySupport} \colorbox{red!5}{\strut Groups} \colorbox{red!66}{\strut OCD} \colorbox{red!6}{\strut Readings} \colorbox{red!66}{\strut OCD} \colorbox{red!4}{\strut Resources} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!4}{\strut Staff} \colorbox{red!6}{\strut Email} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!4}{\strut Directions} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!5}{\strut Site} \colorbox{red!5}{\strut Map} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!3}{\strut Home} \colorbox{red!0}{\strut 1999} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 2007} \colorbox{red!66}{\strut OCD} \colorbox{red!15}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!7}{\strut Los} \colorbox{red!5}{\strut Angeles} \colorbox{red!5}{\strut Site} \colorbox{red!2}{\strut Created} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: er tv show

98:er, 75:cast, 56:show, 46:tv, 46:series, 28:seasons, 28:chief, 27:medicine, 24:emergency, 23:run


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!85}{\strut ER} \colorbox{red!2}{\strut .} \colorbox{red!39}{\strut TV} \colorbox{red!39}{\strut series} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!24}{\strut Chief} \colorbox{red!3}{\strut of} \colorbox{red!20}{\strut Emergency} \colorbox{red!23}{\strut Medicine} \colorbox{red!2}{\strut .} \colorbox{red!85}{\strut ER} \colorbox{red!39}{\strut TV} \colorbox{red!48}{\strut show} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!8}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut contain} \colorbox{red!13}{\strut original} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut unverified} \colorbox{red!0}{\strut claims} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!3}{\strut improve} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adding} \colorbox{red!5}{\strut references} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut talk} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut details} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut February} \colorbox{red!0}{\strut 2009} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!1}{\strut needs} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut citations} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut verification} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut help} \colorbox{red!3}{\strut improve} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut reliable} \colorbox{red!5}{\strut references} \colorbox{red!4}{\strut .} \colorbox{red!5}{\strut Unsourced} \colorbox{red!1}{\strut material} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut challenged} \colorbox{red!3}{\strut and} \colorbox{red!1}{\strut removed} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut February} \colorbox{red!0}{\strut 2009} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut about} \colorbox{red!2}{\strut the} \colorbox{red!17}{\strut medical} \colorbox{red!13}{\strut drama} \colorbox{red!39}{\strut series} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!2}{\strut the} \colorbox{red!13}{\strut sitcom} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut ER} \colorbox{red!4}{\strut .} \colorbox{red!85}{\strut ER} \colorbox{red!85}{\strut ER} \colorbox{red!4}{\strut intertitle} \colorbox{red!4}{\strut .} \colorbox{red!9}{\strut Format} \colorbox{red!17}{\strut Medical} \colorbox{red!13}{\strut Drama} \colorbox{red!7}{\strut Created} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut Michael} \colorbox{red!8}{\strut Crichton} \colorbox{red!14}{\strut Starring} \colorbox{red!9}{\strut Current} \colorbox{red!65}{\strut cast} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Noah} \colorbox{red!4}{\strut Wyle} \colorbox{red!2}{\strut Parminder} \colorbox{red!0}{\strut Nagra} \colorbox{red!1}{\strut John} \colorbox{red!0}{\strut Stamos} \colorbox{red!0}{\strut Linda} \colorbox{red!1}{\strut Cardellini} \colorbox{red!1}{\strut Scott} \colorbox{red!1}{\strut Grimes} \colorbox{red!2}{\strut David} \colorbox{red!3}{\strut Lyons} \colorbox{red!2}{\strut Angela} \colorbox{red!2}{\strut Bassett} \colorbox{red!0}{\strut Openingtheme} \colorbox{red!3}{\strut James} \colorbox{red!0}{\strut Newton} \colorbox{red!0}{\strut Howard} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 19942006} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Martin} \colorbox{red!2}{\strut Davich} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 2006Present} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Countryoforigin} \colorbox{red!5}{\strut USA} \colorbox{red!1}{\strut No} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut of} \colorbox{red!24}{\strut seasons} \colorbox{red!2}{\strut 15} \colorbox{red!0}{\strut No.ofepisodes} \colorbox{red!0}{\strut 325} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Listofepisodes} \colorbox{red!3}{\strut .} \colorbox{red!18}{\strut Production} \colorbox{red!0}{\strut Camerasetup} \colorbox{red!2}{\strut Single} \colorbox{red!6}{\strut Runningtime} \colorbox{red!0}{\strut 60} \colorbox{red!5}{\strut minutes} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut including} \colorbox{red!4}{\strut commercials} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut approx} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut 45} \colorbox{red!5}{\strut minutes} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut without} \colorbox{red!4}{\strut commercials} \colorbox{red!3}{\strut .} \colorbox{red!18}{\strut Production} \colorbox{red!5}{\strut company} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut s} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut Constant} \colorbox{red!4}{\strut c} \colorbox{red!0}{\strut Productions} \colorbox{red!4}{\strut Amblin} \colorbox{red!12}{\strut Television} \colorbox{red!3}{\strut Warner} \colorbox{red!0}{\strut Bros.} \colorbox{red!12}{\strut Television} \colorbox{red!11}{\strut Broadcast} \colorbox{red!13}{\strut Original} \colorbox{red!8}{\strut channel} \colorbox{red!14}{\strut NBC} \colorbox{red!0}{\strut Pictureformat} \colorbox{red!2}{\strut 480i} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut SDTV} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut 1080i} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut HDTV} \colorbox{red!3}{\strut .} \colorbox{red!13}{\strut Original} \colorbox{red!19}{\strut run} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 19} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut 1994} \colorbox{red!1}{\strut present} \colorbox{red!0}{\strut External} \colorbox{red!1}{\strut links} \colorbox{red!0}{\strut Official} \colorbox{red!0}{\strut website} \colorbox{red!0}{\strut IMDb} \colorbox{red!1}{\strut profile} \colorbox{red!0}{\strut TV.com} \colorbox{red!0}{\strut summary} \colorbox{red!85}{\strut ER} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!8}{\strut Emmy} \colorbox{red!7}{\strut Award} \colorbox{red!0}{\strut -winning} \colorbox{red!6}{\strut American} \colorbox{red!17}{\strut medical} \colorbox{red!13}{\strut drama} \colorbox{red!39}{\strut series} \colorbox{red!7}{\strut created} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut late} \colorbox{red!0}{\strut novelist} \colorbox{red!3}{\strut Michael} \colorbox{red!8}{\strut Crichton} \colorbox{red!3}{\strut and} \colorbox{red!10}{\strut airing} \colorbox{red!3}{\strut on} \colorbox{red!14}{\strut NBC} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut It} \colorbox{red!2}{\strut is} \colorbox{red!5}{\strut set} \colorbox{red!0}{\strut primarily} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!20}{\strut emergency} \colorbox{red!8}{\strut room} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut fictional} \colorbox{red!3}{\strut County} \colorbox{red!0}{\strut General} \colorbox{red!6}{\strut Hospital} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Chicago} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut Illinois} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut It} \colorbox{red!2}{\strut is} \colorbox{red!6}{\strut produced} \colorbox{red!0}{\strut by} \colorbox{red!4}{\strut Constant} \colorbox{red!4}{\strut c} \colorbox{red!0}{\strut Productions} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut Amblin} \colorbox{red!5}{\strut Entertainment} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut association} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut Warner} \colorbox{red!0}{\strut Bros.} \colorbox{red!12}{\strut Television} \colorbox{red!18}{\strut Production} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut Inc} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut Contents} \colorbox{red!2}{\strut 1} \colorbox{red!39}{\strut Series} \colorbox{red!19}{\strut run} \colorbox{red!3}{\strut 2} \colorbox{red!6}{\strut History} \colorbox{red!3}{\strut and} \colorbox{red!18}{\strut production} \colorbox{red!1}{\strut 3} \colorbox{red!15}{\strut Episodes} \colorbox{red!1}{\strut 4} \colorbox{red!65}{\strut Cast} \colorbox{red!0}{\strut 4.1} \colorbox{red!13}{\strut Main} \colorbox{red!65}{\strut cast} \colorbox{red!0}{\strut 4.1.1} \colorbox{red!13}{\strut Original} \colorbox{red!65}{\strut cast} \colorbox{red!0}{\strut 4.1.2} \colorbox{red!0}{\strut Additions} \colorbox{red!0}{\strut to} \colorbox{red!13}{\strut main} 
}}}
\end{CJK*}

100:ray, 92:barnett, 86:dr, 41:er, 18:shows, 16:prev, 15:medical, 14:actor, 13:nbc, 13:dramas


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Search} \colorbox{red!5}{\strut TV} \colorbox{red!7}{\strut Dramas} \colorbox{red!5}{\strut Home} \colorbox{red!5}{\strut Entertainment} \colorbox{red!5}{\strut TV} \colorbox{red!7}{\strut Dramas} \colorbox{red!4}{\strut Email} \colorbox{red!5}{\strut TV} \colorbox{red!7}{\strut Dramas} \colorbox{red!10}{\strut Shows} \colorbox{red!0}{\strut A-Z} \colorbox{red!5}{\strut TV} \colorbox{red!5}{\strut Celebrities} \colorbox{red!5}{\strut TV} \colorbox{red!3}{\strut Extras} \colorbox{red!2}{\strut Free} \colorbox{red!5}{\strut TV} \colorbox{red!7}{\strut Dramas} \colorbox{red!2}{\strut Newsletter} \colorbox{red!2}{\strut !} \colorbox{red!3}{\strut Sign} \colorbox{red!1}{\strut Up} \colorbox{red!3}{\strut Discuss} \colorbox{red!2}{\strut in} \colorbox{red!2}{\strut my} \colorbox{red!3}{\strut Forum} \colorbox{red!5}{\strut Shane} \colorbox{red!4}{\strut West} \colorbox{red!2}{\strut as} \colorbox{red!0}{\strut Dr.} \colorbox{red!58}{\strut Ray} \colorbox{red!53}{\strut Barnett} \colorbox{red!2}{\strut From} \colorbox{red!4}{\strut Rachel} \colorbox{red!6}{\strut Thomas} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut About.com} \colorbox{red!0}{\strut See} \colorbox{red!2}{\strut More} \colorbox{red!1}{\strut About} \colorbox{red!2}{\strut .} \colorbox{red!23}{\strut er} \colorbox{red!23}{\strut er} \colorbox{red!4}{\strut photo} \colorbox{red!5}{\strut gallery} \colorbox{red!5}{\strut shane} \colorbox{red!4}{\strut west} \colorbox{red!8}{\strut actor} \colorbox{red!2}{\strut 10} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut 10} \colorbox{red!5}{\strut Gallery} \colorbox{red!4}{\strut Index} \colorbox{red!9}{\strut Prev} \colorbox{red!3}{\strut Next} \colorbox{red!7}{\strut NBC} \colorbox{red!5}{\strut Universal} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!5}{\strut Shane} \colorbox{red!4}{\strut West} \colorbox{red!4}{\strut stars} \colorbox{red!2}{\strut as} \colorbox{red!0}{\strut Dr.} \colorbox{red!58}{\strut Ray} \colorbox{red!53}{\strut Barnett} \colorbox{red!2}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut hit} \colorbox{red!7}{\strut NBC} \colorbox{red!8}{\strut medical} \colorbox{red!0}{\strut drama} \colorbox{red!23}{\strut ER} \colorbox{red!3}{\strut .} \colorbox{red!9}{\strut Prev} \colorbox{red!3}{\strut Next} \colorbox{red!5}{\strut TV} \colorbox{red!7}{\strut Dramas} \colorbox{red!5}{\strut Home} \colorbox{red!5}{\strut Entertainment} \colorbox{red!5}{\strut TV} \colorbox{red!7}{\strut Dramas} \colorbox{red!5}{\strut TV} \colorbox{red!10}{\strut Shows} \colorbox{red!4}{\strut A} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Z} \colorbox{red!0}{\strut ER} \colorbox{red!1}{\strut .} \colorbox{red!23}{\strut ER} \colorbox{red!4}{\strut Photo} \colorbox{red!5}{\strut Gallery} \colorbox{red!1}{\strut Most} \colorbox{red!2}{\strut Popular} \colorbox{red!1}{\strut Latest} \colorbox{red!2}{\strut Articles} \colorbox{red!2}{\strut Add} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut iGoogle} \colorbox{red!2}{\strut My} \colorbox{red!2}{\strut Yahoo} \colorbox{red!2}{\strut !} \colorbox{red!2}{\strut RSS} \colorbox{red!2}{\strut Advertising} \colorbox{red!2}{\strut Info} \colorbox{red!3}{\strut News} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Events} \colorbox{red!4}{\strut Work} \colorbox{red!2}{\strut at} \colorbox{red!1}{\strut About} \colorbox{red!0}{\strut SiteMap} \colorbox{red!1}{\strut All} \colorbox{red!3}{\strut Topics} \colorbox{red!2}{\strut Reprints} \colorbox{red!2}{\strut Help} \colorbox{red!1}{\strut User} \colorbox{red!3}{\strut Agreement} \colorbox{red!3}{\strut Ethics} \colorbox{red!4}{\strut Policy} \colorbox{red!4}{\strut Patent} \colorbox{red!2}{\strut Info} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut Privacy} \colorbox{red!4}{\strut Policy} \colorbox{red!1}{\strut Our} \colorbox{red!2}{\strut Story} \colorbox{red!2}{\strut Be} \colorbox{red!4}{\strut a} \colorbox{red!2}{\strut Guide} \colorbox{red!1}{\strut 2009} \colorbox{red!0}{\strut About.com} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut a} \colorbox{red!5}{\strut part} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut The} \colorbox{red!4}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!3}{\strut Times} \colorbox{red!4}{\strut Company} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut All} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut reserved} \colorbox{red!3}{\strut .} 
}}}
\end{CJK*}

query: south africa

100:sport, 100:south, 100:africa, 35:category, 16:teams, 13:african, 10:athletics, 9:football, 7:soccer, 7:city


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!54}{\strut Category} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Sport} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!4}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!4}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!4}{\strut The} \colorbox{red!0}{\strut main} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut for} \colorbox{red!6}{\strut this} \colorbox{red!54}{\strut category} \colorbox{red!0}{\strut is} \colorbox{red!100}{\strut Sport} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!9}{\strut .} \colorbox{red!9}{\strut Wikimedia} \colorbox{red!0}{\strut Commons} \colorbox{red!4}{\strut has} \colorbox{red!3}{\strut media} \colorbox{red!6}{\strut related} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sports} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!9}{\strut Subcategories} \colorbox{red!6}{\strut This} \colorbox{red!54}{\strut category} \colorbox{red!4}{\strut has} \colorbox{red!4}{\strut the} \colorbox{red!9}{\strut following} \colorbox{red!3}{\strut 33} \colorbox{red!9}{\strut subcategories} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut 33} \colorbox{red!7}{\strut total} \colorbox{red!9}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut Sport} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!4}{\strut by} \colorbox{red!10}{\strut city} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!4}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Sports} \colorbox{red!24}{\strut teams} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!4}{\strut .} \colorbox{red!6}{\strut A} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!15}{\strut Athletics} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!7}{\strut Australian} \colorbox{red!4}{\strut rules} \colorbox{red!14}{\strut football} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!7}{\strut B} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!6}{\strut Badminton} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut C} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!7}{\strut Chess} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!1}{\strut Climbing} \colorbox{red!1}{\strut areas} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!6}{\strut at} \colorbox{red!4}{\strut the} \colorbox{red!9}{\strut Commonwealth} \colorbox{red!7}{\strut Games} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!9}{\strut Cricket} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut 9} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!1}{\strut Cycle} \colorbox{red!7}{\strut racing} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut D} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut Sport} \colorbox{red!7}{\strut deaths} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut F} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Sports} \colorbox{red!7}{\strut festivals} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!3}{\strut Field} \colorbox{red!7}{\strut hockey} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!4}{\strut Figure} \colorbox{red!6}{\strut skating} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!14}{\strut Football} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut soccer} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut 9} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut G} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Gliding} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!4}{\strut Golf} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut H} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!4}{\strut Horse} \colorbox{red!7}{\strut racing} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut 5} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!1}{\strut Ice} \colorbox{red!7}{\strut hockey} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!6}{\strut J} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut Sport} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut Johannesburg} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut M} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut South} \colorbox{red!100}{\strut Africa} \colorbox{red!6}{\strut at} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut Maccabiah} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut .} \colorbox{red!4}{\strut Motorsport} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut South} 
}}}
\end{CJK*}

99:africa, 92:south, 31:years, 16:category, 7:subcategories, 7:jump, 7:], 7:1850, 6:next, 6:1851


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!14}{\strut Category} \colorbox{red!2}{\strut .} \colorbox{red!27}{\strut Years} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!1}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut free} \colorbox{red!2}{\strut encyclopedia} \colorbox{red!6}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!4}{\strut Contents} \colorbox{red!3}{\strut Top} \colorbox{red!3}{\strut 09} \colorbox{red!1}{\strut A} \colorbox{red!2}{\strut B} \colorbox{red!2}{\strut C} \colorbox{red!1}{\strut D} \colorbox{red!0}{\strut E} \colorbox{red!2}{\strut F} \colorbox{red!1}{\strut G} \colorbox{red!1}{\strut H} \colorbox{red!0}{\strut I} \colorbox{red!3}{\strut J} \colorbox{red!2}{\strut K} \colorbox{red!0}{\strut L} \colorbox{red!2}{\strut M} \colorbox{red!3}{\strut N} \colorbox{red!2}{\strut O} \colorbox{red!2}{\strut P} \colorbox{red!2}{\strut Q} \colorbox{red!0}{\strut R} \colorbox{red!2}{\strut S} \colorbox{red!0}{\strut T} \colorbox{red!0}{\strut U} \colorbox{red!0}{\strut V} \colorbox{red!4}{\strut W} \colorbox{red!1}{\strut X} \colorbox{red!0}{\strut Y} \colorbox{red!0}{\strut Z} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut previous} \colorbox{red!3}{\strut 200} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut next} \colorbox{red!3}{\strut 200} \colorbox{red!4}{\strut .} \colorbox{red!6}{\strut Subcategories} \colorbox{red!0}{\strut This} \colorbox{red!14}{\strut category} \colorbox{red!2}{\strut has} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut following} \colorbox{red!0}{\strut 89} \colorbox{red!6}{\strut subcategories} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 155} \colorbox{red!3}{\strut total} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!5}{\strut 1815} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!6}{\strut 1850} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!5}{\strut 1851} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut 1852} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut 1853} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1854} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1855} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1856} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!1}{\strut 1857} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 1858} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut 1859} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1860} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1861} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut 1862} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut 1863} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut 1864} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!1}{\strut 1865} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1870} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut 1871} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1872} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut 1873} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut 1875} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 1876} \colorbox{red!3}{\strut in} \colorbox{red!80}{\strut South} \colorbox{red!86}{\strut Africa} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut 0} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

query: cass county missouri

98:cass, 96:county, 52:missouri, 28:location, 27:population, 27:kansas, 22:harrisonville, 13:state, 13:organized, 12:seat


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Cass} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!67}{\strut Missouri} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!7}{\strut ,} \colorbox{red!6}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!7}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!100}{\strut Cass} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!67}{\strut Missouri} \colorbox{red!5}{\strut Map} \colorbox{red!36}{\strut Location} \colorbox{red!6}{\strut in} \colorbox{red!6}{\strut the} \colorbox{red!16}{\strut state} \colorbox{red!6}{\strut of} \colorbox{red!67}{\strut Missouri} \colorbox{red!67}{\strut Missouri} \colorbox{red!0}{\strut s} \colorbox{red!36}{\strut location} \colorbox{red!6}{\strut in} \colorbox{red!6}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut Statistics} \colorbox{red!10}{\strut Founded} \colorbox{red!0}{\strut 1835} \colorbox{red!15}{\strut Seat} \colorbox{red!28}{\strut Harrisonville} \colorbox{red!14}{\strut Area} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut Total} \colorbox{red!0}{\strut -} \colorbox{red!10}{\strut Land} \colorbox{red!0}{\strut -} \colorbox{red!11}{\strut Water} \colorbox{red!2}{\strut 703} \colorbox{red!6}{\strut sqmi} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1,821} \colorbox{red!3}{\strut km} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 699sqmi} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1,810km} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 4sqmi} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 10km} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut ,} \colorbox{red!0}{\strut 0.52} \colorbox{red!1}{\strut .} \colorbox{red!34}{\strut Population} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 2007} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!9}{\strut Density} \colorbox{red!0}{\strut 97,133} \colorbox{red!0}{\strut 138sqmi} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 53.3km} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Website} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.casscounty.com} \colorbox{red!100}{\strut Cass} \colorbox{red!100}{\strut County} \colorbox{red!5}{\strut is} \colorbox{red!5}{\strut a} \colorbox{red!100}{\strut county} \colorbox{red!0}{\strut located} \colorbox{red!6}{\strut in} \colorbox{red!6}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!16}{\strut state} \colorbox{red!6}{\strut of} \colorbox{red!67}{\strut Missouri} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut As} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut 2000} \colorbox{red!7}{\strut ,} \colorbox{red!6}{\strut the} \colorbox{red!34}{\strut population} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut 82,092} \colorbox{red!6}{\strut .} \colorbox{red!6}{\strut Its} \colorbox{red!100}{\strut county} \colorbox{red!15}{\strut seat} \colorbox{red!5}{\strut is} \colorbox{red!28}{\strut Harrisonville} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!6}{\strut The} \colorbox{red!100}{\strut county} \colorbox{red!0}{\strut was} \colorbox{red!16}{\strut organized} \colorbox{red!6}{\strut in} \colorbox{red!0}{\strut 1835} \colorbox{red!2}{\strut as} \colorbox{red!2}{\strut Van} \colorbox{red!0}{\strut Buren} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!6}{\strut renamed} \colorbox{red!6}{\strut in} \colorbox{red!0}{\strut 1848} \colorbox{red!0}{\strut after} \colorbox{red!7}{\strut Michigan} \colorbox{red!0}{\strut U.S} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut Senator} \colorbox{red!3}{\strut and} \colorbox{red!0}{\strut presidential} \colorbox{red!0}{\strut candidate} \colorbox{red!3}{\strut Lewis} \colorbox{red!100}{\strut Cass} \colorbox{red!6}{\strut .} \colorbox{red!100}{\strut Cass} \colorbox{red!5}{\strut is} \colorbox{red!12}{\strut part} \colorbox{red!6}{\strut of} \colorbox{red!6}{\strut the} \colorbox{red!34}{\strut Kansas} \colorbox{red!15}{\strut City} \colorbox{red!2}{\strut Metropolitan} \colorbox{red!14}{\strut Area} \colorbox{red!0}{\strut Contents} \colorbox{red!5}{\strut 1} \colorbox{red!2}{\strut Geography} \colorbox{red!0}{\strut 1.1} \colorbox{red!5}{\strut Adjacent} \colorbox{red!0}{\strut counties} \colorbox{red!0}{\strut 1.2} \colorbox{red!5}{\strut Major} \colorbox{red!5}{\strut highways} \colorbox{red!1}{\strut 2} \colorbox{red!6}{\strut Demographics} \colorbox{red!0}{\strut 3} \colorbox{red!3}{\strut History} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Cities} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut towns} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Geography} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!5}{\strut Census} \colorbox{red!0}{\strut Bureau} \colorbox{red!7}{\strut ,} \colorbox{red!6}{\strut the} \colorbox{red!100}{\strut county} \colorbox{red!2}{\strut has} \colorbox{red!5}{\strut a} \colorbox{red!5}{\strut total} \colorbox{red!14}{\strut area} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut 703square} \colorbox{red!14}{\strut miles} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1,820km} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 699square} \colorbox{red!14}{\strut miles} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1,810km} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!5}{\strut is} \colorbox{red!10}{\strut land} \colorbox{red!3}{\strut and} \colorbox{red!1}{\strut 4square} \colorbox{red!14}{\strut miles} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 10km} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 0.52} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut is} \colorbox{red!11}{\strut water} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Adjacent} \colorbox{red!0}{\strut counties} \colorbox{red!14}{\strut Jackson} \colorbox{red!100}{\strut County} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut north} \colorbox{red!3}{\strut .} \colorbox{red!9}{\strut Johnson} \colorbox{red!100}{\strut County} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut east} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Henry} \colorbox{red!100}{\strut County} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut southeast} \colorbox{red!3}{\strut .} \colorbox{red!11}{\strut Bates} \colorbox{red!100}{\strut County} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut south} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Miami} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!34}{\strut Kansas} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut west} \colorbox{red!3}{\strut .} \colorbox{red!9}{\strut Johnson} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!34}{\strut Kansas} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut northwest} \colorbox{red!3}{\strut .} \colorbox{red!9}{\strut Johnson} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!34}{\strut Kansas} \colorbox{red!14}{\strut Jackson} \colorbox{red!100}{\strut County} \colorbox{red!0}{\strut v} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut e} \colorbox{red!5}{\strut Miami} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!34}{\strut Kansas} \colorbox{red!9}{\strut Johnson} \colorbox{red!100}{\strut County} \colorbox{red!100}{\strut Cass} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut ,} \colorbox{red!67}{\strut Missouri} \colorbox{red!11}{\strut Bates} \colorbox{red!100}{\strut County} \colorbox{red!0}{\strut Henry} \colorbox{red!100}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Major} \colorbox{red!5}{\strut highways} \colorbox{red!0}{\strut U.S.} \colorbox{red!3}{\strut Route} \colorbox{red!0}{\strut 71} \colorbox{red!3}{\strut Route} \colorbox{red!1}{\strut 2} \colorbox{red!3}{\strut Route} \colorbox{red!0}{\strut 7} \colorbox{red!3}{\strut Route} \colorbox{red!0}{\strut 58} \colorbox{red!3}{\strut Route} \colorbox{red!0}{\strut 291} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Demographics} \colorbox{red!2}{\strut As} \colorbox{red!6}{\strut of} \colorbox{red!6}{\strut the} \colorbox{red!5}{\strut census} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 2} 
}}}
\end{CJK*}

100:cass, 88:lewis, 86:named, 73:places, 39:cities, 32:towns, 22:list, 21:counties, 16:which, 15:illinois


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!13}{\strut List} \colorbox{red!2}{\strut of} \colorbox{red!44}{\strut places} \colorbox{red!52}{\strut named} \colorbox{red!0}{\strut for} \colorbox{red!53}{\strut Lewis} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut From} \colorbox{red!1}{\strut Wikipedia} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!2}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut navigation} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!3}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!13}{\strut list} \colorbox{red!2}{\strut of} \colorbox{red!44}{\strut places} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut United} \colorbox{red!6}{\strut States} \colorbox{red!52}{\strut named} \colorbox{red!0}{\strut for} \colorbox{red!53}{\strut Lewis} \colorbox{red!61}{\strut Cass} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!1}{\strut 1} \colorbox{red!12}{\strut Counties} \colorbox{red!0}{\strut 2} \colorbox{red!23}{\strut Cities} \colorbox{red!4}{\strut ,} \colorbox{red!19}{\strut towns} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut or} \colorbox{red!4}{\strut villages} \colorbox{red!0}{\strut 3} \colorbox{red!5}{\strut Townships} \colorbox{red!0}{\strut 4} \colorbox{red!4}{\strut Geographical} \colorbox{red!4}{\strut features} \colorbox{red!0}{\strut 5} \colorbox{red!4}{\strut Buildings} \colorbox{red!0}{\strut 6} \colorbox{red!3}{\strut Other} \colorbox{red!0}{\strut 7} \colorbox{red!2}{\strut Streets} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut Notes} \colorbox{red!1}{\strut 9} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Counties} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!9}{\strut Illinois} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut Michigan} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Minnesota} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Missouri} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut Nebraska} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Texas} \colorbox{red!1}{\strut In} \colorbox{red!3}{\strut addition} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut Bartow} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Georgia} \colorbox{red!3}{\strut was} \colorbox{red!5}{\strut formerly} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Georgia} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut until} \colorbox{red!0}{\strut after} \colorbox{red!3}{\strut the} \colorbox{red!1}{\strut American} \colorbox{red!2}{\strut Civil} \colorbox{red!3}{\strut War} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!23}{\strut Cities} \colorbox{red!4}{\strut ,} \colorbox{red!19}{\strut towns} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut or} \colorbox{red!4}{\strut villages} \colorbox{red!61}{\strut Cass} \colorbox{red!4}{\strut ,} \colorbox{red!1}{\strut West} \colorbox{red!0}{\strut Virginia} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut City} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut Michigan} \colorbox{red!0}{\strut Cassopolis} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut Michigan} \colorbox{red!0}{\strut Casstown} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut Ohio} \colorbox{red!1}{\strut Cassville} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Georgia} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut formerly} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut county} \colorbox{red!5}{\strut seat} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut Bartow} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Georgia} \colorbox{red!4}{\strut ,} \colorbox{red!9}{\strut which} \colorbox{red!3}{\strut was} \colorbox{red!5}{\strut formerly} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Georgia} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut until} \colorbox{red!0}{\strut after} \colorbox{red!3}{\strut the} \colorbox{red!1}{\strut American} \colorbox{red!2}{\strut Civil} \colorbox{red!3}{\strut War} \colorbox{red!1}{\strut Cassville} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Missouri} \colorbox{red!1}{\strut Cassville} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Pennsylvania} \colorbox{red!1}{\strut Cassville} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut Wisconsin} \colorbox{red!1}{\strut Cassville} \colorbox{red!4}{\strut ,} \colorbox{red!2}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Townships} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!9}{\strut Illinois} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Fulton} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!9}{\strut Illinois} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Clay} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Dubois} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Greene} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut LaPorte} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut Ohio} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Pulaksi} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Sullivan} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut White} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Boone} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Cedar} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Clayton} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Guthrie} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Hamilton} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Harrison} \colorbox{red!0}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut Iowa} \colorbox{red!61}{\strut Cass} \colorbox{red!0}{\strut Township} 
}}}
\end{CJK*}

query: adobe indian houses

96:adobe, 92:house, 63:what, 63:style, 33:homes, 27:built, 25:designed, 24:pueblo, 22:revival, 22:buildings


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!81}{\strut Adobe} \colorbox{red!78}{\strut House} \colorbox{red!17}{\strut Plans} \colorbox{red!1}{\strut .} \colorbox{red!15}{\strut Southwestern} \colorbox{red!78}{\strut House} \colorbox{red!17}{\strut Plans} \colorbox{red!1}{\strut From} \colorbox{red!15}{\strut Southwestern} \colorbox{red!53}{\strut Style} \colorbox{red!28}{\strut Homes} \colorbox{red!2}{\strut and} \colorbox{red!17}{\strut Plans} \colorbox{red!1}{\strut .} \colorbox{red!11}{\strut Southwest} \colorbox{red!78}{\strut House} \colorbox{red!17}{\strut Plans} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Favorites} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut View} \colorbox{red!0}{\strut Cart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Search} \colorbox{red!81}{\strut Adobe} \colorbox{red!78}{\strut House} \colorbox{red!17}{\strut Plans} \colorbox{red!2}{\strut Our} \colorbox{red!81}{\strut adobe} \colorbox{red!78}{\strut house} \colorbox{red!17}{\strut plans} \colorbox{red!3}{\strut were} \colorbox{red!21}{\strut designed} \colorbox{red!2}{\strut by} \colorbox{red!9}{\strut architects} \colorbox{red!5}{\strut working} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!11}{\strut Southwest} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!8}{\strut popular} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut other} \colorbox{red!3}{\strut regions} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut country} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut Our} \colorbox{red!0}{\strut adobe-style} \colorbox{red!11}{\strut floor} \colorbox{red!17}{\strut plans} \colorbox{red!0}{\strut are} \colorbox{red!6}{\strut unique} \colorbox{red!2}{\strut and} \colorbox{red!7}{\strut distinctive} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut thick} \colorbox{red!15}{\strut walls} \colorbox{red!1}{\strut allow} \colorbox{red!0}{\strut for} \colorbox{red!10}{\strut unusual} \colorbox{red!0}{\strut design} \colorbox{red!5}{\strut elements} \colorbox{red!2}{\strut inside} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut home} \colorbox{red!4}{\strut .} \colorbox{red!11}{\strut Common} \colorbox{red!13}{\strut Characteristics} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut Adobe-Style} \colorbox{red!0}{\strut Home} \colorbox{red!17}{\strut Plans} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Popular} \colorbox{red!18}{\strut Revival} \colorbox{red!53}{\strut Style} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut especially} \colorbox{red!1}{\strut in} \colorbox{red!11}{\strut Southwest} \colorbox{red!0}{\strut Also} \colorbox{red!5}{\strut called} \colorbox{red!6}{\strut Santa} \colorbox{red!10}{\strut Fe} \colorbox{red!53}{\strut Style} \colorbox{red!0}{\strut Low-pitched} \colorbox{red!0}{\strut or} \colorbox{red!8}{\strut flat} \colorbox{red!13}{\strut roof} \colorbox{red!9}{\strut Pitched} \colorbox{red!13}{\strut roof} \colorbox{red!3}{\strut often} \colorbox{red!1}{\strut with} \colorbox{red!4}{\strut ceramic} \colorbox{red!5}{\strut tiles} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Spanish} \colorbox{red!5}{\strut Colonial} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Monterey} \colorbox{red!1}{\strut .} \colorbox{red!8}{\strut Flat} \colorbox{red!13}{\strut roof} \colorbox{red!3}{\strut usually} \colorbox{red!1}{\strut with} \colorbox{red!0}{\strut surrounding} \colorbox{red!5}{\strut parapet} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Santa} \colorbox{red!10}{\strut Fe} \colorbox{red!2}{\strut ,} \colorbox{red!20}{\strut Pueblo} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Thick} \colorbox{red!8}{\strut masonry} \colorbox{red!15}{\strut walls} \colorbox{red!0}{\strut .} \colorbox{red!18}{\strut Revival} \colorbox{red!0}{\strut styles} \colorbox{red!3}{\strut often} \colorbox{red!3}{\strut strawbale} \colorbox{red!0}{\strut or} \colorbox{red!4}{\strut standard} \colorbox{red!12}{\strut construction} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Recessed} \colorbox{red!6}{\strut windows} \colorbox{red!4}{\strut Simple} \colorbox{red!4}{\strut doors} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut smaller} \colorbox{red!6}{\strut windows} \colorbox{red!13}{\strut Roof} \colorbox{red!1}{\strut beams} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut cross-members} \colorbox{red!3}{\strut often} \colorbox{red!0}{\strut exposed} \colorbox{red!2}{\strut inside} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut button} \colorbox{red!1}{\strut below} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut browse} \colorbox{red!2}{\strut our} \colorbox{red!81}{\strut adobe} \colorbox{red!0}{\strut home} \colorbox{red!17}{\strut plans} \colorbox{red!0}{\strut !} \colorbox{red!53}{\strut What} \colorbox{red!1}{\strut follows} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut excerpts} \colorbox{red!1}{\strut from} \colorbox{red!5}{\strut American} \colorbox{red!5}{\strut Shelter} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut written} \colorbox{red!2}{\strut by} \colorbox{red!0}{\strut Lester} \colorbox{red!0}{\strut Walker} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut published} \colorbox{red!2}{\strut by} \colorbox{red!3}{\strut Overlook} \colorbox{red!1}{\strut Press} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut 1997} \colorbox{red!20}{\strut Pueblo} \colorbox{red!18}{\strut Revival} \colorbox{red!0}{\strut .} \colorbox{red!81}{\strut Adobe} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!20}{\strut Pueblo} \colorbox{red!18}{\strut Revival} \colorbox{red!53}{\strut Style} \colorbox{red!6}{\strut takes} \colorbox{red!0}{\strut its} \colorbox{red!7}{\strut name} \colorbox{red!1}{\strut from} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut prototypical} \colorbox{red!81}{\strut adobe} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut flat-roofed} \colorbox{red!0}{\strut pueblos} \colorbox{red!23}{\strut built} \colorbox{red!2}{\strut by} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut Hopi} \colorbox{red!2}{\strut and} \colorbox{red!20}{\strut Pueblo} \colorbox{red!11}{\strut Indians} \colorbox{red!1}{\strut in} \colorbox{red!7}{\strut New} \colorbox{red!7}{\strut Mexico} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut northern} \colorbox{red!13}{\strut Arizona} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut It} \colorbox{red!3}{\strut was} \colorbox{red!5}{\strut introduced} \colorbox{red!1}{\strut in} \colorbox{red!9}{\strut California} \colorbox{red!2}{\strut by} \colorbox{red!3}{\strut Boston} \colorbox{red!0}{\strut architect} \colorbox{red!0}{\strut A.C.} \colorbox{red!5}{\strut Schweinfurth} \colorbox{red!1}{\strut with} \colorbox{red!2}{\strut a} \colorbox{red!12}{\strut hotel} \colorbox{red!1}{\strut in} \colorbox{red!4}{\strut Montalvo} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut 1894} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Later} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut he} \colorbox{red!21}{\strut designed} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!1}{\strut of} \colorbox{red!18}{\strut buildings} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut Hearst} \colorbox{red!4}{\strut ranch} \colorbox{red!1}{\strut in} \colorbox{red!4}{\strut Pleasanton} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!53}{\strut style} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut By} \colorbox{red!0}{\strut 1915} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut in} \colorbox{red!7}{\strut New} \colorbox{red!7}{\strut Mexico} \colorbox{red!2}{\strut and} \colorbox{red!13}{\strut Arizona} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!20}{\strut Pueblo} \colorbox{red!18}{\strut Revival} \colorbox{red!53}{\strut Style} \colorbox{red!0}{\strut became} \colorbox{red!8}{\strut popular} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut hotels} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut college} \colorbox{red!3}{\strut campus} \colorbox{red!18}{\strut buildings} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut churches} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!5}{\strut public} \colorbox{red!18}{\strut buildings} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut It} \colorbox{red!3}{\strut was} \colorbox{red!2}{\strut seen} \colorbox{red!0}{\strut as} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut marriage} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut archeological} \colorbox{red!2}{\strut and} \colorbox{red!4}{\strut modern} \colorbox{red!3}{\strut spirit} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!20}{\strut Pueblo} \colorbox{red!18}{\strut Revival} \colorbox{red!78}{\strut house} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut like} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut original} \colorbox{red!20}{\strut pueblo} 
}}}
\end{CJK*}

66:what, 47:grants, 44:housing, 38:block, 36:pih, 28:development, 27:hud, 26:indian, 26:ihbg, 25:programs


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Public} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut Indian} \colorbox{red!16}{\strut Housing} \colorbox{red!1}{\strut About} \colorbox{red!13}{\strut PIH} \colorbox{red!6}{\strut Public} \colorbox{red!16}{\strut housing} \colorbox{red!3}{\strut Asset} \colorbox{red!1}{\strut Management} \colorbox{red!2}{\strut Senior} \colorbox{red!16}{\strut Housing} \colorbox{red!2}{\strut Clearinghouse} \colorbox{red!2}{\strut Center} \colorbox{red!0}{\strut CapFund} \colorbox{red!1}{\strut HOPE} \colorbox{red!2}{\strut VI} \colorbox{red!16}{\strut Housing} \colorbox{red!2}{\strut Choice} \colorbox{red!3}{\strut Vouchers} \colorbox{red!6}{\strut Public} \colorbox{red!16}{\strut Housing} \colorbox{red!1}{\strut Reform} \colorbox{red!9}{\strut Indian} \colorbox{red!16}{\strut Housing} \colorbox{red!1}{\strut CODETALK} \colorbox{red!6}{\strut Community} \colorbox{red!10}{\strut development} \colorbox{red!1}{\strut Homeownership} \colorbox{red!17}{\strut Grants} \colorbox{red!2}{\strut Common} \colorbox{red!1}{\strut questions} \colorbox{red!1}{\strut News} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut events} \colorbox{red!2}{\strut Policy} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut regulations} \colorbox{red!0}{\strut Publications} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut resources} \colorbox{red!1}{\strut Online} \colorbox{red!2}{\strut systems} \colorbox{red!1}{\strut Training} \colorbox{red!2}{\strut Rental} \colorbox{red!16}{\strut Housing} \colorbox{red!1}{\strut Integrity} \colorbox{red!2}{\strut Improvement} \colorbox{red!2}{\strut Project} \colorbox{red!1}{\strut Real} \colorbox{red!2}{\strut Estate} \colorbox{red!2}{\strut Assessment} \colorbox{red!17}{\strut Grants} \colorbox{red!3}{\strut Notices} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut rules} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut regulations} \colorbox{red!0}{\strut Library} \colorbox{red!1}{\strut Forums} \colorbox{red!1}{\strut Online} \colorbox{red!2}{\strut systems} \colorbox{red!9}{\strut HUD} \colorbox{red!1}{\strut news} \colorbox{red!5}{\strut Homes} \colorbox{red!1}{\strut Resources} \colorbox{red!0}{\strut Communities} \colorbox{red!2}{\strut Working} \colorbox{red!1}{\strut with} \colorbox{red!9}{\strut HUD} \colorbox{red!1}{\strut Tools} \colorbox{red!1}{\strut Webcasts} \colorbox{red!1}{\strut Mailing} \colorbox{red!2}{\strut lists} \colorbox{red!1}{\strut RSS} \colorbox{red!1}{\strut Feeds} \colorbox{red!1}{\strut Help} \colorbox{red!17}{\strut Grants} \colorbox{red!1}{\strut Information} \colorbox{red!0}{\strut by} \colorbox{red!4}{\strut State} \colorbox{red!1}{\strut Print} \colorbox{red!1}{\strut version} \colorbox{red!0}{\strut Related} \colorbox{red!1}{\strut Information} \colorbox{red!13}{\strut PIH} \colorbox{red!0}{\strut grant} \colorbox{red!1}{\strut information} \colorbox{red!0}{\strut Funds} \colorbox{red!5}{\strut available} \colorbox{red!17}{\strut Grants} \colorbox{red!2}{\strut Inventory} \colorbox{red!3}{\strut Did} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Know} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut The} \colorbox{red!3}{\strut Office} \colorbox{red!1}{\strut of} \colorbox{red!8}{\strut Native} \colorbox{red!6}{\strut American} \colorbox{red!9}{\strut Programs} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut ONAP} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut developed} \colorbox{red!1}{\strut two} \colorbox{red!2}{\strut guidebooks} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut assist} \colorbox{red!0}{\strut grant} \colorbox{red!2}{\strut staff} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut recipients} \colorbox{red!1}{\strut .} \colorbox{red!17}{\strut Grants} \colorbox{red!5}{\strut Evaluation} \colorbox{red!0}{\strut Guidebook} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Adobe} \colorbox{red!1}{\strut PDF} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 259} \colorbox{red!1}{\strut pages} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Provides} \colorbox{red!1}{\strut general} \colorbox{red!2}{\strut processing} \colorbox{red!4}{\strut requirements} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut procedures} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut tools} \colorbox{red!1}{\strut for} \colorbox{red!17}{\strut Grants} \colorbox{red!5}{\strut Evaluation} \colorbox{red!2}{\strut staff} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Revisions} \colorbox{red!0}{\strut APR} \colorbox{red!2}{\strut Review} \colorbox{red!1}{\strut Guidelines} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut APR} \colorbox{red!0}{\strut Reviewer} \colorbox{red!1}{\strut Questions} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Adobe} \colorbox{red!1}{\strut PDF} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 10} \colorbox{red!1}{\strut pages} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Revisions} \colorbox{red!1}{\strut to} \colorbox{red!17}{\strut Grants} \colorbox{red!5}{\strut Evaluation} \colorbox{red!0}{\strut Guidebook} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Adobe} \colorbox{red!1}{\strut PDF} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 105} \colorbox{red!1}{\strut pages} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Revision} \colorbox{red!2}{\strut Procedures} \colorbox{red!1}{\strut for} \colorbox{red!2}{\strut Pursuing} \colorbox{red!1}{\strut Enforcement} \colorbox{red!1}{\strut Actions} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut Delinquent} \colorbox{red!1}{\strut Annual} \colorbox{red!1}{\strut Performance} \colorbox{red!1}{\strut Reports} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Adobe} \colorbox{red!1}{\strut PDF} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 35} \colorbox{red!1}{\strut pages} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Revised} \colorbox{red!4}{\strut Sanction} \colorbox{red!0}{\strut Process} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Adobe} \colorbox{red!1}{\strut PDF} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 56} \colorbox{red!1}{\strut pages} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Self-Monitoring} \colorbox{red!0}{\strut Guidebook} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Adobe} \colorbox{red!1}{\strut PDF} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 177} \colorbox{red!1}{\strut pages} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Assists} \colorbox{red!9}{\strut IHBG} \colorbox{red!2}{\strut recipients} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut meeting} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut self-monitoring} \colorbox{red!1}{\strut responsibilities} \colorbox{red!1}{\strut under} \colorbox{red!2}{\strut NAHASDA} \colorbox{red!1}{\strut .} \colorbox{red!24}{\strut What} \colorbox{red!5}{\strut types} \colorbox{red!1}{\strut of} \colorbox{red!17}{\strut grants} \colorbox{red!0}{\strut are} \colorbox{red!5}{\strut available} \colorbox{red!1}{\strut for} \colorbox{red!9}{\strut Indian} \colorbox{red!16}{\strut housing} \colorbox{red!1}{\strut and} \colorbox{red!6}{\strut community} \colorbox{red!10}{\strut development} \colorbox{red!0}{\strut ?} \colorbox{red!9}{\strut HUD} \colorbox{red!5}{\strut awards} \colorbox{red!17}{\strut grants} \colorbox{red!1}{\strut to} \colorbox{red!8}{\strut tribes} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut other} \colorbox{red!9}{\strut Indian} \colorbox{red!2}{\strut entities} \colorbox{red!1}{\strut through} \colorbox{red!1}{\strut either} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut competitive} \colorbox{red!0}{\strut process} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut discretionary} \colorbox{red!17}{\strut grants} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut formula} \colorbox{red!1}{\strut basis} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut case} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!9}{\strut Indian} \colorbox{red!16}{\strut Housing} \colorbox{red!13}{\strut Block} \colorbox{red!0}{\strut Grant} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut IHBG} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Program} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!0}{\strut competitions} \colorbox{red!1}{\strut for} \colorbox{red!3}{\strut discretionary} \colorbox{red!0}{\strut grant} \colorbox{red!9}{\strut programs} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut announced} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!9}{\strut HUD} \colorbox{red!0}{\strut SuperNOFA} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut which} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut published} \colorbox{red!1}{\strut once} \colorbox{red!0}{\strut each} \colorbox{red!4}{\strut Federal} \colorbox{red!2}{\strut fiscal} \colorbox{red!1}{\strut year} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Program} \colorbox{red!2}{\strut Descriptions} \colorbox{red!9}{\strut Indian} \colorbox{red!6}{\strut Community} \colorbox{red!10}{\strut Development} \colorbox{red!13}{\strut Block} \colorbox{red!0}{\strut Grant} \colorbox{red!0}{\strut Program} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut ICDBG} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Provides} \colorbox{red!9}{\strut Indian} 
}}}
\end{CJK*}

query: interview thank

97:thank, 93:interview, 62:send, 55:letter, 53:how, 39:note, 29:job, 27:write, 24:follow, 18:typed


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!62}{\strut Send} \colorbox{red!7}{\strut a} \colorbox{red!98}{\strut Thank} \colorbox{red!7}{\strut You} \colorbox{red!39}{\strut Note} \colorbox{red!5}{\strut After} \colorbox{red!7}{\strut the} \colorbox{red!29}{\strut Job} \colorbox{red!94}{\strut Interview} \colorbox{red!7}{\strut A} \colorbox{red!0}{\strut follow-up} \colorbox{red!98}{\strut thank} \colorbox{red!7}{\strut you} \colorbox{red!55}{\strut letter} \colorbox{red!8}{\strut to} \colorbox{red!7}{\strut the} \colorbox{red!0}{\strut interviewer} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!8}{\strut important} \colorbox{red!0}{\strut step} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut the} \colorbox{red!0}{\strut interviewing} \colorbox{red!11}{\strut process} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!1}{\strut that} \colorbox{red!13}{\strut candidates} \colorbox{red!0}{\strut often} \colorbox{red!3}{\strut forget} \colorbox{red!8}{\strut to} \colorbox{red!12}{\strut take} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Sending} \colorbox{red!1}{\strut such} \colorbox{red!7}{\strut a} \colorbox{red!55}{\strut letter} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut only} \colorbox{red!6}{\strut proper} \colorbox{red!14}{\strut business} \colorbox{red!6}{\strut etiquette} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut also} \colorbox{red!5}{\strut makes} \colorbox{red!7}{\strut you} \colorbox{red!6}{\strut stand} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut from} \colorbox{red!7}{\strut the} \colorbox{red!2}{\strut other} \colorbox{red!13}{\strut candidates} \colorbox{red!6}{\strut competing} \colorbox{red!2}{\strut for} \colorbox{red!7}{\strut the} \colorbox{red!3}{\strut same} \colorbox{red!9}{\strut position} \colorbox{red!5}{\strut .} \colorbox{red!27}{\strut Write} \colorbox{red!6}{\strut your} \colorbox{red!98}{\strut thank} \colorbox{red!7}{\strut you} \colorbox{red!55}{\strut letter} \colorbox{red!0}{\strut as} \colorbox{red!10}{\strut soon} \colorbox{red!0}{\strut as} \colorbox{red!6}{\strut possible} \colorbox{red!5}{\strut after} \colorbox{red!7}{\strut the} \colorbox{red!94}{\strut interview} \colorbox{red!5}{\strut .} \colorbox{red!7}{\strut You} \colorbox{red!4}{\strut should} \colorbox{red!62}{\strut send} \colorbox{red!7}{\strut a} \colorbox{red!0}{\strut follow-up} \colorbox{red!98}{\strut thank} \colorbox{red!7}{\strut you} \colorbox{red!55}{\strut letter} \colorbox{red!5}{\strut even} \colorbox{red!0}{\strut if} \colorbox{red!7}{\strut you} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!3}{\strut want} \colorbox{red!7}{\strut the} \colorbox{red!29}{\strut job} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!1}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!7}{\strut the} \colorbox{red!4}{\strut case} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut let} \colorbox{red!7}{\strut the} \colorbox{red!0}{\strut interviewer} \colorbox{red!1}{\strut know} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut your} \colorbox{red!98}{\strut thank} \colorbox{red!7}{\strut you} \colorbox{red!55}{\strut letter} \colorbox{red!5}{\strut .} \colorbox{red!6}{\strut Ask} \colorbox{red!7}{\strut the} \colorbox{red!0}{\strut interviewer} \colorbox{red!8}{\strut to} \colorbox{red!3}{\strut keep} \colorbox{red!7}{\strut you} \colorbox{red!3}{\strut in} \colorbox{red!2}{\strut mind} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut positions} \colorbox{red!2}{\strut with} \colorbox{red!7}{\strut the} \colorbox{red!7}{\strut company} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut be} \colorbox{red!4}{\strut available} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut the} \colorbox{red!4}{\strut future} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Components} \colorbox{red!6}{\strut of} \colorbox{red!7}{\strut the} \colorbox{red!0}{\strut Follow-up} \colorbox{red!98}{\strut Thank} \colorbox{red!7}{\strut You} \colorbox{red!55}{\strut Letter} \colorbox{red!6}{\strut Your} \colorbox{red!98}{\strut thank} \colorbox{red!7}{\strut you} \colorbox{red!55}{\strut letter} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!18}{\strut typed} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut a} \colorbox{red!14}{\strut business} \colorbox{red!55}{\strut letter} \colorbox{red!6}{\strut format} \colorbox{red!4}{\strut or} \colorbox{red!6}{\strut handwritten} \colorbox{red!0}{\strut using} \colorbox{red!7}{\strut a} \colorbox{red!0}{\strut pre-printed} \colorbox{red!98}{\strut thank} \colorbox{red!7}{\strut you} \colorbox{red!39}{\strut note} \colorbox{red!5}{\strut .} \colorbox{red!7}{\strut The} \colorbox{red!55}{\strut letter} \colorbox{red!4}{\strut or} \colorbox{red!39}{\strut note} \colorbox{red!4}{\strut should} \colorbox{red!12}{\strut express} \colorbox{red!5}{\strut appreciation} \colorbox{red!2}{\strut for} \colorbox{red!7}{\strut the} \colorbox{red!5}{\strut opportunity} \colorbox{red!8}{\strut to} \colorbox{red!94}{\strut interview} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut tour} \colorbox{red!7}{\strut the} \colorbox{red!4}{\strut facilities} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut meet} \colorbox{red!2}{\strut other} \colorbox{red!6}{\strut employees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!5}{\strut .} \colorbox{red!7}{\strut You} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut also} \colorbox{red!3}{\strut want} \colorbox{red!8}{\strut to} \colorbox{red!27}{\strut write} \colorbox{red!0}{\strut about} \colorbox{red!7}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut Mention} \colorbox{red!7}{\strut the} \colorbox{red!2}{\strut day} \colorbox{red!6}{\strut of} \colorbox{red!6}{\strut your} \colorbox{red!94}{\strut interview} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut the} \colorbox{red!9}{\strut position} \colorbox{red!2}{\strut for} \colorbox{red!8}{\strut which} \colorbox{red!7}{\strut you} \colorbox{red!0}{\strut interviewed} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut --} \colorbox{red!12}{\strut Express} \colorbox{red!4}{\strut continued} \colorbox{red!2}{\strut interest} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut the} \colorbox{red!9}{\strut position} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut the} \colorbox{red!7}{\strut company} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut Re-emphasize} \colorbox{red!6}{\strut your} \colorbox{red!0}{\strut most} \colorbox{red!8}{\strut important} \colorbox{red!1}{\strut skills} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut qualifications} \colorbox{red!0}{\strut and} \colorbox{red!53}{\strut how} \colorbox{red!7}{\strut you} \colorbox{red!7}{\strut expect} \colorbox{red!8}{\strut to} \colorbox{red!3}{\strut contribute} \colorbox{red!8}{\strut to} \colorbox{red!7}{\strut the} \colorbox{red!5}{\strut organization} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut Include} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut information} \colorbox{red!7}{\strut you} \colorbox{red!3}{\strut forgot} \colorbox{red!8}{\strut to} \colorbox{red!0}{\strut mention} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut the} \colorbox{red!94}{\strut interview} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!6}{\strut necessary} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut be} \colorbox{red!5}{\strut brief} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut --} \colorbox{red!9}{\strut Close} \colorbox{red!6}{\strut your} \colorbox{red!55}{\strut letter} \colorbox{red!2}{\strut with} \colorbox{red!7}{\strut a} \colorbox{red!4}{\strut comment} \colorbox{red!0}{\strut about} \colorbox{red!4}{\strut future} \colorbox{red!4}{\strut contact} \colorbox{red!2}{\strut with} \colorbox{red!7}{\strut the} \colorbox{red!7}{\strut employer} \colorbox{red!5}{\strut .} \colorbox{red!6}{\strut Sample} \colorbox{red!98}{\strut Thank} \colorbox{red!7}{\strut You} \colorbox{red!55}{\strut Letter} \colorbox{red!3}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut appreciated} \colorbox{red!7}{\strut the} \colorbox{red!5}{\strut opportunity} \colorbox{red!8}{\strut to} \colorbox{red!94}{\strut interview} \colorbox{red!2}{\strut at} \colorbox{red!6}{\strut your} \colorbox{red!9}{\strut hospital} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut Monday} \colorbox{red!5}{\strut .} \colorbox{red!7}{\strut The} \colorbox{red!10}{\strut tour} \colorbox{red!6}{\strut of} \colorbox{red!7}{\strut the} \colorbox{red!4}{\strut facilities} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut conversations} \colorbox{red!2}{\strut with} \colorbox{red!11}{\strut Acme} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut laboratory} \colorbox{red!4}{\strut staff} \colorbox{red!5}{\strut gave} 
}}}
\end{CJK*}

100:thank, 98:letters, 90:email, 46:how, 42:writing, 38:interview, 23:appropriate, 22:when, 22:follow, 20:examples


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Search} \colorbox{red!2}{\strut Tech} \colorbox{red!3}{\strut Careers} \colorbox{red!0}{\strut Home} \colorbox{red!3}{\strut Careers} \colorbox{red!2}{\strut Tech} \colorbox{red!3}{\strut Careers} \colorbox{red!40}{\strut Email} \colorbox{red!2}{\strut Tech} \colorbox{red!3}{\strut Careers} \colorbox{red!5}{\strut Education} \colorbox{red!6}{\strut Find} \colorbox{red!2}{\strut A} \colorbox{red!6}{\strut Job} \colorbox{red!0}{\strut Career} \colorbox{red!2}{\strut Advancement} \colorbox{red!1}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut Forum} \colorbox{red!4}{\strut Apply} \colorbox{red!0}{\strut now} \colorbox{red!3}{\strut to} \colorbox{red!1}{\strut guide} \colorbox{red!2}{\strut this} \colorbox{red!1}{\strut site} \colorbox{red!0}{\strut All} \colorbox{red!2}{\strut About} \colorbox{red!16}{\strut Interview} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!43}{\strut Letters} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut About.com} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut More} \colorbox{red!2}{\strut About} \colorbox{red!0}{\strut .} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!43}{\strut letters} \colorbox{red!6}{\strut job} \colorbox{red!0}{\strut interviews} \colorbox{red!4}{\strut business} \colorbox{red!0}{\strut letter} \colorbox{red!18}{\strut writing} \colorbox{red!0}{\strut After} \colorbox{red!2}{\strut your} \colorbox{red!16}{\strut interview} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut always} \colorbox{red!2}{\strut a} \colorbox{red!8}{\strut good} \colorbox{red!4}{\strut idea} \colorbox{red!3}{\strut to} \colorbox{red!9}{\strut follow} \colorbox{red!2}{\strut up} \colorbox{red!1}{\strut with} \colorbox{red!2}{\strut a} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut letter} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut tech} \colorbox{red!4}{\strut industry} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut a} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!40}{\strut email} \colorbox{red!1}{\strut is} \colorbox{red!10}{\strut appropriate} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut some} \colorbox{red!4}{\strut guidelines} \colorbox{red!0}{\strut and} \colorbox{red!8}{\strut examples} \colorbox{red!2}{\strut for} \colorbox{red!18}{\strut writing} \colorbox{red!2}{\strut your} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!43}{\strut letters} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut links} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut several} \colorbox{red!8}{\strut examples} \colorbox{red!3}{\strut of} \colorbox{red!16}{\strut interview} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!43}{\strut letters} \colorbox{red!2}{\strut ,} \colorbox{red!10}{\strut appropriate} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut several} \colorbox{red!4}{\strut different} \colorbox{red!16}{\strut interview} \colorbox{red!4}{\strut situations} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!2}{\strut .} \colorbox{red!16}{\strut Interview} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!43}{\strut Letters} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Guidelines} \colorbox{red!4}{\strut Guidelines} \colorbox{red!2}{\strut for} \colorbox{red!18}{\strut writing} \colorbox{red!16}{\strut interview} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!43}{\strut letters} \colorbox{red!2}{\strut .} \colorbox{red!20}{\strut How} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut write} \colorbox{red!16}{\strut interview} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!43}{\strut letters} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!9}{\strut when} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut write} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut and} \colorbox{red!20}{\strut how} \colorbox{red!3}{\strut to} \colorbox{red!5}{\strut send} \colorbox{red!0}{\strut them} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 2} \colorbox{red!2}{\strut .} \colorbox{red!16}{\strut Interview} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!0}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut General} \colorbox{red!2}{\strut Format} \colorbox{red!2}{\strut A} \colorbox{red!3}{\strut general} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!4}{\strut sent} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut any} \colorbox{red!16}{\strut interview} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 3} \colorbox{red!2}{\strut .} \colorbox{red!16}{\strut Interview} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!0}{\strut Letter} \colorbox{red!2}{\strut An} \colorbox{red!0}{\strut example} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut general} \colorbox{red!16}{\strut interview} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!5}{\strut mentions} \colorbox{red!9}{\strut follow} \colorbox{red!2}{\strut up} \colorbox{red!0}{\strut discussions} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 4} \colorbox{red!2}{\strut .} \colorbox{red!16}{\strut Interview} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!0}{\strut Letter} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut Additional} \colorbox{red!0}{\strut Information} \colorbox{red!2}{\strut This} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut an} \colorbox{red!0}{\strut example} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut an} \colorbox{red!16}{\strut interview} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut used} \colorbox{red!3}{\strut to} \colorbox{red!3}{\strut convey} \colorbox{red!1}{\strut additional} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!3}{\strut experience} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut training} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut forgot} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut mention} \colorbox{red!1}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!16}{\strut interview} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 5} \colorbox{red!2}{\strut .} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!0}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Campus} \colorbox{red!16}{\strut Interview} \colorbox{red!2}{\strut An} \colorbox{red!16}{\strut interview} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut is} \colorbox{red!10}{\strut appropriate} \colorbox{red!0}{\strut after} \colorbox{red!2}{\strut an} \colorbox{red!0}{\strut on-campus} \colorbox{red!16}{\strut interview} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 6} \colorbox{red!2}{\strut .} \colorbox{red!16}{\strut Interview} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!0}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Scheduling} \colorbox{red!2}{\strut a} \colorbox{red!9}{\strut Follow} \colorbox{red!2}{\strut Up} \colorbox{red!2}{\strut A} \colorbox{red!3}{\strut sample} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!5}{\strut mentions} \colorbox{red!8}{\strut scheduling} \colorbox{red!2}{\strut a} \colorbox{red!9}{\strut follow} \colorbox{red!2}{\strut up} \colorbox{red!0}{\strut discussion} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 7} \colorbox{red!2}{\strut .} \colorbox{red!16}{\strut Interview} \colorbox{red!44}{\strut Thank} \colorbox{red!4}{\strut You} \colorbox{red!0}{\strut Letter} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Addressing} \colorbox{red!1}{\strut Concerns} \colorbox{red!2}{\strut An} \colorbox{red!16}{\strut interview} \colorbox{red!44}{\strut thank} \colorbox{red!4}{\strut you} \colorbox{red!0}{\strut letter} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut addresses} \colorbox{red!1}{\strut concerns} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut were} \colorbox{red!2}{\strut brought} \colorbox{red!2}{\strut up} \colorbox{red!1}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!16}{\strut interview} 
}}}
\end{CJK*}

query: culpeper national cemetery

92:cemeteries, 71:culpeper, 59:located, 49:virginia, 48:what, 40:quantico, 36:resting, 36:open, 35:national, 27:fredericksburg


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!25}{\strut National} \colorbox{red!18}{\strut Veterans} \colorbox{red!66}{\strut Cemeteries} \colorbox{red!5}{\strut While} \colorbox{red!1}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut numerous} \colorbox{red!25}{\strut National} \colorbox{red!66}{\strut Cemeteries} \colorbox{red!3}{\strut in} \colorbox{red!35}{\strut Virginia} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut only} \colorbox{red!2}{\strut three} \colorbox{red!3}{\strut remain} \colorbox{red!25}{\strut open} \colorbox{red!1}{\strut for} \colorbox{red!18}{\strut burial} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut These} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut .} \colorbox{red!17}{\strut Arlington} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!28}{\strut Quantico} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!51}{\strut Culpeper} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!17}{\strut Arlington} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!5}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut only} \colorbox{red!25}{\strut national} \colorbox{red!0}{\strut cemetery} \colorbox{red!7}{\strut administered} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut Department} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut Army} \colorbox{red!2}{\strut .} \colorbox{red!17}{\strut Arlington} \colorbox{red!5}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut final} \colorbox{red!25}{\strut resting} \colorbox{red!7}{\strut place} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut presidents} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Supreme} \colorbox{red!4}{\strut Court} \colorbox{red!3}{\strut justices} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut astronauts} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut Medal} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut Honor} \colorbox{red!4}{\strut recipients} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!3}{\strut notable} \colorbox{red!2}{\strut Americans} \colorbox{red!1}{\strut and} \colorbox{red!5}{\strut is} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut perhaps} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut best} \colorbox{red!2}{\strut known} \colorbox{red!1}{\strut for} \colorbox{red!2}{\strut the} \colorbox{red!10}{\strut Tomb} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!1}{\strut Unknown} \colorbox{red!5}{\strut Soldier} \colorbox{red!2}{\strut .} \colorbox{red!17}{\strut Arlington} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!2}{\strut has} \colorbox{red!2}{\strut strict} \colorbox{red!7}{\strut eligibility} \colorbox{red!7}{\strut requirements} \colorbox{red!2}{\strut .} \colorbox{red!12}{\strut Nelsen} \colorbox{red!16}{\strut Funeral} \colorbox{red!7}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Crematory} \colorbox{red!4}{\strut personnel} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut assist} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut determining} \colorbox{red!7}{\strut eligibility} \colorbox{red!2}{\strut .} \colorbox{red!28}{\strut Quantico} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!5}{\strut is} \colorbox{red!42}{\strut located} \colorbox{red!2}{\strut midway} \colorbox{red!0}{\strut between} \colorbox{red!19}{\strut Fredericksburg} \colorbox{red!1}{\strut and} \colorbox{red!12}{\strut Washington} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut DC.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut land} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut was} \colorbox{red!5}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!7}{\strut Marine} \colorbox{red!4}{\strut Corps} \colorbox{red!7}{\strut Base} \colorbox{red!2}{\strut .} \colorbox{red!28}{\strut Quantico} \colorbox{red!2}{\strut has} \colorbox{red!3}{\strut hosted} \colorbox{red!10}{\strut military} \colorbox{red!1}{\strut operations} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 200} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut first} \colorbox{red!1}{\strut used} \colorbox{red!0}{\strut by} \colorbox{red!35}{\strut Virginia} \colorbox{red!1}{\strut for} \colorbox{red!3}{\strut naval} \colorbox{red!1}{\strut operations} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut 1775} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut blockade} \colorbox{red!0}{\strut point} \colorbox{red!1}{\strut for} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut Confederate} \colorbox{red!6}{\strut army} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut In} \colorbox{red!0}{\strut 1977} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut Marine} \colorbox{red!4}{\strut Corps} \colorbox{red!4}{\strut donated} \colorbox{red!0}{\strut this} \colorbox{red!5}{\strut land} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!3}{\strut Administration} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!0}{\strut cemetery} \colorbox{red!2}{\strut was} \colorbox{red!13}{\strut dedicated} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1983} \colorbox{red!2}{\strut .} \colorbox{red!51}{\strut Culpeper} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!5}{\strut is} \colorbox{red!42}{\strut located} \colorbox{red!4}{\strut approximately} \colorbox{red!0}{\strut 35} \colorbox{red!2}{\strut miles} \colorbox{red!4}{\strut west} \colorbox{red!0}{\strut of} \colorbox{red!19}{\strut Fredericksburg} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!51}{\strut Culpeper} \colorbox{red!6}{\strut area} \colorbox{red!2}{\strut was} \colorbox{red!2}{\strut the} \colorbox{red!8}{\strut site} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut many} \colorbox{red!2}{\strut Civil} \colorbox{red!5}{\strut War} \colorbox{red!1}{\strut battles} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Following} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut war} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut reburial} \colorbox{red!2}{\strut program} \colorbox{red!2}{\strut was} \colorbox{red!2}{\strut initiated} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut federal} \colorbox{red!3}{\strut government} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut locate} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut remains} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!5}{\strut Union} \colorbox{red!0}{\strut soldiers} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut reinter} \colorbox{red!2}{\strut them} \colorbox{red!3}{\strut in} \colorbox{red!25}{\strut national} \colorbox{red!66}{\strut cemeteries} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut scattered} \colorbox{red!5}{\strut Union} \colorbox{red!8}{\strut dead} \colorbox{red!3}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut vicinity} \colorbox{red!0}{\strut ,} \colorbox{red!51}{\strut Culpeper} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!2}{\strut was} \colorbox{red!6}{\strut established} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut 1867} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut In} \colorbox{red!0}{\strut 1996} \colorbox{red!0}{\strut ,} \colorbox{red!51}{\strut Culpeper} \colorbox{red!25}{\strut National} \colorbox{red!0}{\strut Cemetery} \colorbox{red!2}{\strut was} \colorbox{red!0}{\strut placed} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!25}{\strut National} \colorbox{red!6}{\strut Register} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Historic} \colorbox{red!0}{\strut Places} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 4650} \colorbox{red!0}{\strut S.} \colorbox{red!0}{\strut Laburnum} \colorbox{red!0}{\strut Ave.Richmond} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut VA23231804.222.8601} \colorbox{red!0}{\strut info} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut nelsencares.com} \colorbox{red!2}{\strut Copyright} \colorbox{red!0}{\strut 2008} \colorbox{red!12}{\strut Nelsen} \colorbox{red!16}{\strut Funeral} \colorbox{red!7}{\strut Home} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut FuneralNet} \colorbox{red!7}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!2}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Staff} 
}}}
\end{CJK*}

96:culpeper, 94:county, 31:cemetery, 18:graveyard, 16:renfrow, 15:photos, 13:near, 13:joan, 10:teresa, 10:hill


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!95}{\strut Culpeper} \colorbox{red!93}{\strut County} \colorbox{red!30}{\strut Cemetery} \colorbox{red!14}{\strut Photos} \colorbox{red!0}{\strut RecorderSubmitter} \colorbox{red!0}{\strut Instructions} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Submitting} \colorbox{red!4}{\strut Transcriptions} \colorbox{red!0}{\strut and} \colorbox{red!14}{\strut Photos} \colorbox{red!0}{\strut USGenWeb} \colorbox{red!2}{\strut Archives} \colorbox{red!0}{\strut National} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Feature} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Camera} \colorbox{red!0}{\strut icon} \colorbox{red!0}{\strut indicates} \colorbox{red!14}{\strut photos} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut .} \colorbox{red!95}{\strut Culpeper} \colorbox{red!93}{\strut County} \colorbox{red!30}{\strut Cemetery} \colorbox{red!5}{\strut Listing} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut All} \colorbox{red!6}{\strut Saints} \colorbox{red!3}{\strut Episcopal} \colorbox{red!7}{\strut Church} \colorbox{red!17}{\strut Graveyard} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!3}{\strut Apperson} \colorbox{red!17}{\strut Graveyard} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Armstrong} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Bell} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!2}{\strut Bethel} \colorbox{red!0}{\strut Baptist} \colorbox{red!7}{\strut Church} \colorbox{red!17}{\strut Graveyard} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!7}{\strut Bickers} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut aka} \colorbox{red!7}{\strut Mountain} \colorbox{red!6}{\strut View} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!4}{\strut Bleak} \colorbox{red!9}{\strut Hill} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!1}{\strut Alanthus} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Bolen} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!6}{\strut Broadus} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!5}{\strut Brown} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!5}{\strut Brown} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut Store} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!5}{\strut Brown} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!6}{\strut Slate} \colorbox{red!5}{\strut Mills} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!5}{\strut Brown} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!1}{\strut Rixeyville} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!5}{\strut Brown} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!5}{\strut Reva} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!7}{\strut Clatterbuck} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!5}{\strut Colvin} \colorbox{red!30}{\strut Cemetery} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!5}{\strut Colvin} \colorbox{red!17}{\strut Graveyard} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!5}{\strut Clover} \colorbox{red!9}{\strut Hill} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!2}{\strut Cloverdale} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Compton} \colorbox{red!17}{\strut Graveyard} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Cooke} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Coons} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Coons} \colorbox{red!30}{\strut Cemetery} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Coon} \colorbox{red!0}{\strut s} \colorbox{red!30}{\strut Cemetery} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Corbin} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Crane} \colorbox{red!17}{\strut Graveyard} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!6}{\strut Crigler} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Daniel} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Davenport-Thompson} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!0}{\strut Dowlman} \colorbox{red!0}{\strut Tomb} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!2}{\strut Eggborn} \colorbox{red!30}{\strut Cemetery} \colorbox{red!9}{\strut Teresa} \colorbox{red!8}{\strut Kelley} \colorbox{red!3}{\strut Fairview} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Fant} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!0}{\strut Griffinsburg} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Farish} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!4}{\strut Mitchells} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!3}{\strut Ficklin} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!3}{\strut Eggbornsville} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Fishback} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!0}{\strut Jeffersonton} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Fleetwood} \colorbox{red!9}{\strut Hill} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!0}{\strut Elkwood} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Francis} \colorbox{red!0}{\strut Browning} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!0}{\strut Lebanon} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Freeman} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!1}{\strut Rixeyville} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!2}{\strut Gaines} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut Karen} \colorbox{red!0}{\strut Bennett} \colorbox{red!3}{\strut Garnett} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Gourdvine} \colorbox{red!7}{\strut Church} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Guinn} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!0}{\strut Winston} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Hall} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!0}{\strut Winston} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Hitt} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!95}{\strut Culpeper} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Hoffman} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut near} \colorbox{red!1}{\strut Rixeyville} \colorbox{red!12}{\strut Joan} \colorbox{red!15}{\strut Renfrow} \colorbox{red!0}{\strut Jameson} \colorbox{red!30}{\strut Cemetery} \colorbox{red!0}{\strut -} 
}}}
\end{CJK*}

query: iowa food stamp program

95:food, 87:stamp, 72:iowa, 55:what, 42:survey, 41:fsp, 39:leavers, 31:program, 30:when, 29:report


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut or} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut here} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Publications} \colorbox{red!3}{\strut Publications} \colorbox{red!47}{\strut Iowa} \colorbox{red!62}{\strut Food} \colorbox{red!57}{\strut Stamp} \colorbox{red!25}{\strut Leavers} \colorbox{red!27}{\strut Survey} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Final} \colorbox{red!19}{\strut Report} \colorbox{red!3}{\strut Helen} \colorbox{red!0}{\strut H.} \colorbox{red!0}{\strut Jensen} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut Steven} \colorbox{red!4}{\strut Garasky} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut Cory} \colorbox{red!1}{\strut Wessman} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut S.M} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Nusser} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut ERS} \colorbox{red!5}{\strut Contact} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Elizabeth} \colorbox{red!2}{\strut Dagata} \colorbox{red!0}{\strut E-FAN} \colorbox{red!0}{\strut No} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 02014-1} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut pp} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut July} \colorbox{red!3}{\strut 2002} \colorbox{red!10}{\strut Enrollment} \colorbox{red!3}{\strut in} \colorbox{red!47}{\strut Iowa} \colorbox{red!0}{\strut s} \colorbox{red!62}{\strut Food} \colorbox{red!57}{\strut Stamp} \colorbox{red!20}{\strut Program} \colorbox{red!5}{\strut .} \colorbox{red!27}{\strut FSP} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut sharply} \colorbox{red!5}{\strut decreased} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut last} \colorbox{red!3}{\strut years} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut 1990s} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut following} \colorbox{red!3}{\strut significant} \colorbox{red!4}{\strut changes} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut social} \colorbox{red!13}{\strut assistance} \colorbox{red!0}{\strut programs} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!12}{\strut State} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut passage} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut Personal} \colorbox{red!4}{\strut Responsibility} \colorbox{red!1}{\strut and} \colorbox{red!6}{\strut Work} \colorbox{red!4}{\strut Opportunity} \colorbox{red!3}{\strut Reconciliation} \colorbox{red!5}{\strut Act} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut 1996} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut period} \colorbox{red!3}{\strut of} \colorbox{red!5}{\strut good} \colorbox{red!8}{\strut economic} \colorbox{red!3}{\strut conditions} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Data} \colorbox{red!2}{\strut collected} \colorbox{red!3}{\strut in} \colorbox{red!2}{\strut a} \colorbox{red!5}{\strut 1999} \colorbox{red!27}{\strut survey} \colorbox{red!1}{\strut provide} \colorbox{red!2}{\strut information} \colorbox{red!2}{\strut about} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut well-being} \colorbox{red!3}{\strut of} \colorbox{red!5}{\strut families} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut had} \colorbox{red!13}{\strut participated} \colorbox{red!3}{\strut in} \colorbox{red!47}{\strut Iowa} \colorbox{red!0}{\strut s} \colorbox{red!27}{\strut FSP} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut 1997} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!7}{\strut time} \colorbox{red!3}{\strut immediately} \colorbox{red!2}{\strut following} \colorbox{red!2}{\strut introduction} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut new} \colorbox{red!5}{\strut regulations} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Nearly} \colorbox{red!1}{\strut 58} \colorbox{red!9}{\strut percent} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut those} \colorbox{red!0}{\strut participating} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!27}{\strut FSP} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut 1997} \colorbox{red!1}{\strut were} \colorbox{red!4}{\strut not} \colorbox{red!0}{\strut participating} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!20}{\strut program} \colorbox{red!19}{\strut when} \colorbox{red!4}{\strut interviewed} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut 1999} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Those} \colorbox{red!13}{\strut who} \colorbox{red!8}{\strut left} \colorbox{red!3}{\strut the} \colorbox{red!27}{\strut FSP} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut 1997} \colorbox{red!5}{\strut .} \colorbox{red!2}{\strut including} \colorbox{red!0}{\strut working} \colorbox{red!8}{\strut age} \colorbox{red!8}{\strut adults} \colorbox{red!1}{\strut without} \colorbox{red!7}{\strut dependents} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut a} \colorbox{red!8}{\strut disability} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut had} \colorbox{red!3}{\strut better} \colorbox{red!8}{\strut economic} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut employment} \colorbox{red!3}{\strut outcomes} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut others} \colorbox{red!2}{\strut .} \colorbox{red!8}{\strut Adults} \colorbox{red!1}{\strut without} \colorbox{red!7}{\strut dependents} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut a} \colorbox{red!8}{\strut disability} \colorbox{red!13}{\strut who} \colorbox{red!3}{\strut remained} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!27}{\strut FSP} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut 1997} \colorbox{red!3}{\strut had} \colorbox{red!3}{\strut the} \colorbox{red!1}{\strut greatest} \colorbox{red!2}{\strut hardships} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!1}{\strut were} \colorbox{red!0}{\strut most} \colorbox{red!3}{\strut likely} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut have} \colorbox{red!1}{\strut very} \colorbox{red!3}{\strut low} \colorbox{red!5}{\strut income} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut had} \colorbox{red!0}{\strut less} \colorbox{red!7}{\strut contribution} \colorbox{red!0}{\strut from} \colorbox{red!3}{\strut earned} \colorbox{red!5}{\strut income} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut were} \colorbox{red!0}{\strut more} \colorbox{red!3}{\strut likely} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut experience} \colorbox{red!62}{\strut food} \colorbox{red!3}{\strut insecurity} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut hunger} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut last} \colorbox{red!0}{\strut year} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Over} \colorbox{red!2}{\strut half} \colorbox{red!3}{\strut of} \colorbox{red!1}{\strut all} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut households} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!27}{\strut survey} \colorbox{red!3}{\strut had} \colorbox{red!1}{\strut used} \colorbox{red!5}{\strut private} \colorbox{red!62}{\strut food} \colorbox{red!13}{\strut assistance} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut past} \colorbox{red!0}{\strut year} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut For} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut description} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut methodology} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut study} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!47}{\strut Iowa} \colorbox{red!62}{\strut Food} \colorbox{red!57}{\strut Stamp} \colorbox{red!25}{\strut Leavers} \colorbox{red!27}{\strut Survey} \colorbox{red!1}{\strut .} \colorbox{red!8}{\strut Methodology} \colorbox{red!19}{\strut Report} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut E-FAN} \colorbox{red!0}{\strut 02014-2} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Keywords} \colorbox{red!1}{\strut .} \colorbox{red!62}{\strut Food} \colorbox{red!57}{\strut Stamp} \colorbox{red!20}{\strut Program} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut PRWORA} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut ABAWD} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut leaver} \colorbox{red!3}{\strut In} \colorbox{red!1}{\strut this} \colorbox{red!19}{\strut report} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut Chapters} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut Adobe} \colorbox{red!2}{\strut Acrobat} \colorbox{red!0}{\strut PDF} \colorbox{red!1}{\strut format} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Abstract} \colorbox{red!2}{\strut ,} 
}}}
\end{CJK*}

99:stamps, 99:food, 45:did, 41:programs, 22:benefits, 20:welfare, 19:south, 17:legal, 17:carolina, 17:arizona


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Overview} \colorbox{red!1}{\strut of} \colorbox{red!15}{\strut Programs} \colorbox{red!0}{\strut Program} \colorbox{red!1}{\strut Components} \colorbox{red!5}{\strut Children} \colorbox{red!2}{\strut Special} \colorbox{red!1}{\strut Populations} \colorbox{red!2}{\strut Caseload} \colorbox{red!3}{\strut Characteristics} \colorbox{red!0}{\strut Program} \colorbox{red!2}{\strut Outcomes} \colorbox{red!2}{\strut Family} \colorbox{red!0}{\strut Formation} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut Search} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut Database} \colorbox{red!0}{\strut Browse} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut Database} \colorbox{red!0}{\strut About} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut Database} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut Links} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Key} \colorbox{red!1}{\strut Topics} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Caseload} \colorbox{red!3}{\strut Characteristics} \colorbox{red!0}{\strut .} \colorbox{red!36}{\strut Food} \colorbox{red!36}{\strut Stamps} \colorbox{red!2}{\strut Caseload} \colorbox{red!3}{\strut Characteristics} \colorbox{red!1}{\strut The} \colorbox{red!1}{\strut 1996} \colorbox{red!7}{\strut welfare} \colorbox{red!5}{\strut law} \colorbox{red!4}{\strut mandated} \colorbox{red!5}{\strut changes} \colorbox{red!1}{\strut in} \colorbox{red!36}{\strut food} \colorbox{red!5}{\strut nutrition} \colorbox{red!15}{\strut programs} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut notably} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut scaling} \colorbox{red!3}{\strut back} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!36}{\strut Food} \colorbox{red!0}{\strut Stamp} \colorbox{red!0}{\strut Program} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Following} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut implementation} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut PRWORA} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut participation} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!36}{\strut Food} \colorbox{red!0}{\strut Stamp} \colorbox{red!0}{\strut Program} \colorbox{red!2}{\strut declined} \colorbox{red!0}{\strut considerably} \colorbox{red!1}{\strut -} \colorbox{red!1}{\strut approximately} \colorbox{red!1}{\strut 28} \colorbox{red!2}{\strut percent} \colorbox{red!1}{\strut between} \colorbox{red!2}{\strut December} \colorbox{red!2}{\strut 1995} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut December} \colorbox{red!2}{\strut 1998} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut However} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut this} \colorbox{red!3}{\strut trend} \colorbox{red!1}{\strut has} \colorbox{red!0}{\strut seen} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut reverse} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut with} \colorbox{red!36}{\strut Food} \colorbox{red!36}{\strut Stamps} \colorbox{red!0}{\strut caseloads} \colorbox{red!3}{\strut increasing} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut 28} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut past} \colorbox{red!1}{\strut 32} \colorbox{red!2}{\strut months} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut This} \colorbox{red!0}{\strut increase} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut due} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut slowed} \colorbox{red!1}{\strut economy} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut growing} \colorbox{red!2}{\strut efforts} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut connect} \colorbox{red!2}{\strut eligible} \colorbox{red!4}{\strut people} \colorbox{red!1}{\strut with} \colorbox{red!8}{\strut benefits} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Four} \colorbox{red!2}{\strut studies} \colorbox{red!1}{\strut in} \colorbox{red!6}{\strut Arizona} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Illinois} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Iowa} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!7}{\strut South} \colorbox{red!6}{\strut Carolina} \colorbox{red!1}{\strut were} \colorbox{red!2}{\strut designed} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut examine} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut status} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut those} \colorbox{red!4}{\strut who} \colorbox{red!4}{\strut leave} \colorbox{red!1}{\strut the} \colorbox{red!36}{\strut Food} \colorbox{red!0}{\strut Stamp} \colorbox{red!0}{\strut Program} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!7}{\strut South} \colorbox{red!6}{\strut Carolina} \colorbox{red!2}{\strut project} \colorbox{red!0}{\strut expands} \colorbox{red!0}{\strut upon} \colorbox{red!1}{\strut a} \colorbox{red!7}{\strut welfare} \colorbox{red!2}{\strut leavers} \colorbox{red!0}{\strut study} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!0}{\strut projects} \colorbox{red!0}{\strut all} \colorbox{red!2}{\strut pay} \colorbox{red!0}{\strut close} \colorbox{red!0}{\strut attention} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut able-bodied} \colorbox{red!4}{\strut adults} \colorbox{red!4}{\strut ages} \colorbox{red!0}{\strut 18-50} \colorbox{red!0}{\strut without} \colorbox{red!4}{\strut dependents} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut now} \colorbox{red!1}{\strut subject} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut time} \colorbox{red!5}{\strut limits} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut they} \colorbox{red!2}{\strut do} \colorbox{red!1}{\strut not} \colorbox{red!0}{\strut meet} \colorbox{red!0}{\strut specific} \colorbox{red!3}{\strut work} \colorbox{red!4}{\strut requirements} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Researchers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut using} \colorbox{red!2}{\strut administrative} \colorbox{red!1}{\strut records} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut surveys} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut analyze} \colorbox{red!2}{\strut employment} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut support} \colorbox{red!0}{\strut from} \colorbox{red!3}{\strut earnings} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut income} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut support} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut publicprivate} \colorbox{red!15}{\strut programs} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Illinois} \colorbox{red!1}{\strut and} \colorbox{red!6}{\strut Arizona} \colorbox{red!3}{\strut released} \colorbox{red!1}{\strut final} \colorbox{red!3}{\strut reports} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut early} \colorbox{red!2}{\strut 2001} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!1}{\strut final} \colorbox{red!0}{\strut report} \colorbox{red!1}{\strut for} \colorbox{red!7}{\strut South} \colorbox{red!6}{\strut Carolina} \colorbox{red!1}{\strut was} \colorbox{red!3}{\strut released} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut September} \colorbox{red!2}{\strut 2001} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!1}{\strut final} \colorbox{red!0}{\strut report} \colorbox{red!1}{\strut for} \colorbox{red!5}{\strut Iowa} \colorbox{red!1}{\strut was} \colorbox{red!3}{\strut released} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut July} \colorbox{red!2}{\strut 2002} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!3}{\strut Farm} \colorbox{red!3}{\strut Bill} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut was} \colorbox{red!2}{\strut passed} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut late} \colorbox{red!2}{\strut 2001} \colorbox{red!2}{\strut restored} \colorbox{red!36}{\strut Food} \colorbox{red!36}{\strut Stamps} \colorbox{red!8}{\strut benefits} \colorbox{red!1}{\strut to} \colorbox{red!6}{\strut legal} \colorbox{red!4}{\strut immigrants} \colorbox{red!4}{\strut who} \colorbox{red!1}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut country} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut 5} \colorbox{red!2}{\strut years} \colorbox{red!1}{\strut ,} \colorbox{red!6}{\strut legal} \colorbox{red!0}{\strut immigrant} \colorbox{red!5}{\strut children} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut regardless} \colorbox{red!1}{\strut of} \colorbox{red!4}{\strut time} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut entry} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!6}{\strut legal} \colorbox{red!4}{\strut immigrants} \colorbox{red!1}{\strut with} \colorbox{red!3}{\strut disabilities} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Selected} \colorbox{red!1}{\strut Summary} \colorbox{red!3}{\strut Findings} \colorbox{red!1}{\strut In} \colorbox{red!1}{\strut Brief} 
}}}
\end{CJK*}

query: source nile

98:source, 98:nile, 40:game, 22:playing, 21:board, 16:discovery, 15:river, 15:released, 15:players, 14:who


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Source} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!100}{\strut Nile} \colorbox{red!2}{\strut .} \colorbox{red!25}{\strut board} \colorbox{red!49}{\strut game} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!4}{\strut Wikipedia} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!2}{\strut free} \colorbox{red!7}{\strut encyclopedia} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!100}{\strut Source} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!100}{\strut nile} \colorbox{red!2}{\strut .} \colorbox{red!49}{\strut game} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!12}{\strut Jump} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut search} \colorbox{red!100}{\strut Source} \colorbox{red!6}{\strut Of} \colorbox{red!4}{\strut The} \colorbox{red!100}{\strut Nile} \colorbox{red!100}{\strut Source} \colorbox{red!6}{\strut Of} \colorbox{red!4}{\strut The} \colorbox{red!100}{\strut Nile} \colorbox{red!2}{\strut .} \colorbox{red!8}{\strut 1979} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut by} \colorbox{red!15}{\strut Avalon} \colorbox{red!13}{\strut Hill} \colorbox{red!18}{\strut Players} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!13}{\strut Age} \colorbox{red!8}{\strut range} \colorbox{red!0}{\strut 12} \colorbox{red!6}{\strut Setup} \colorbox{red!14}{\strut time} \colorbox{red!0}{\strut 15} \colorbox{red!6}{\strut minutes} \colorbox{red!26}{\strut Playing} \colorbox{red!14}{\strut time} \colorbox{red!2}{\strut 2} \colorbox{red!3}{\strut hours} \colorbox{red!6}{\strut Random} \colorbox{red!2}{\strut chance} \colorbox{red!0}{\strut Medium} \colorbox{red!4}{\strut Skills} \colorbox{red!7}{\strut required} \colorbox{red!6}{\strut Tactics} \colorbox{red!3}{\strut ,} \colorbox{red!8}{\strut Strategy} \colorbox{red!1}{\strut For} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut literal} \colorbox{red!100}{\strut source} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!100}{\strut Nile} \colorbox{red!18}{\strut River} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!100}{\strut Nile} \colorbox{red!100}{\strut Source} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!100}{\strut Nile} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!25}{\strut board} \colorbox{red!49}{\strut game} \colorbox{red!3}{\strut by} \colorbox{red!7}{\strut Ross} \colorbox{red!9}{\strut Maker} \colorbox{red!4}{\strut and} \colorbox{red!7}{\strut David} \colorbox{red!4}{\strut Wesely} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!18}{\strut released} \colorbox{red!3}{\strut by} \colorbox{red!19}{\strut Discovery} \colorbox{red!0}{\strut Games} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut 1977} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut re-released} \colorbox{red!3}{\strut by} \colorbox{red!15}{\strut Avalon} \colorbox{red!13}{\strut Hill} \colorbox{red!2}{\strut in} \colorbox{red!8}{\strut 1979} \colorbox{red!3}{\strut .} \colorbox{red!11}{\strut Set} \colorbox{red!2}{\strut in} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut 19th} \colorbox{red!4}{\strut century} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!3}{\strut object} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!49}{\strut game} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut to} \colorbox{red!11}{\strut explore} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut interior} \colorbox{red!6}{\strut of} \colorbox{red!12}{\strut Africa} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut make} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut important} \colorbox{red!19}{\strut discovery} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut back} \colorbox{red!2}{\strut to} \colorbox{red!7}{\strut European} \colorbox{red!8}{\strut civilization} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!0}{\strut explorers} \colorbox{red!1}{\strut must} \colorbox{red!2}{\strut outfit} \colorbox{red!0}{\strut their} \colorbox{red!4}{\strut expeditions} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut method} \colorbox{red!6}{\strut of} \colorbox{red!8}{\strut travel} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut it} \colorbox{red!4}{\strut canoe} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut camel} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut foot} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut At} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut outset} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!49}{\strut game} \colorbox{red!4}{\strut the} \colorbox{red!12}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut interior} \colorbox{red!6}{\strut of} \colorbox{red!12}{\strut Africa} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut blank} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut As} \colorbox{red!0}{\strut explorers} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut unexplored} \colorbox{red!3}{\strut hex} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut card} \colorbox{red!2}{\strut is} \colorbox{red!4}{\strut drawn} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut determine} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut terrain} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut events} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut any} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut befall} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut explorers} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut Crayons} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut used} \colorbox{red!2}{\strut to} \colorbox{red!12}{\strut draw} \colorbox{red!6}{\strut terrain} \colorbox{red!0}{\strut on} \colorbox{red!4}{\strut the} \colorbox{red!12}{\strut map} \colorbox{red!2}{\strut as} \colorbox{red!0}{\strut it} \colorbox{red!2}{\strut is} \colorbox{red!6}{\strut discovered} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!0}{\strut explorers} \colorbox{red!1}{\strut must} \colorbox{red!0}{\strut confront} \colorbox{red!1}{\strut dangers} \colorbox{red!0}{\strut such} \colorbox{red!2}{\strut as} \colorbox{red!2}{\strut starvation} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut disease} \colorbox{red!3}{\strut ,} \colorbox{red!18}{\strut river} \colorbox{red!7}{\strut cataracts} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut hostile} \colorbox{red!7}{\strut natives} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!49}{\strut game} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut in} \colorbox{red!1}{\strut fact} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut highly} \colorbox{red!3}{\strut lethal} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut explorers} \colorbox{red!3}{\strut ,} \colorbox{red!1}{\strut but} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut player} \colorbox{red!6}{\strut loses} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut explorer} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut she} \colorbox{red!0}{\strut may} \colorbox{red!2}{\strut create} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut new} \colorbox{red!0}{\strut one} \colorbox{red!17}{\strut who} \colorbox{red!0}{\strut re-enters} \colorbox{red!4}{\strut the} \colorbox{red!49}{\strut game} \colorbox{red!3}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut coastal} \colorbox{red!4}{\strut port} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!0}{\strut player} \colorbox{red!1}{\strut must} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut profession} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut the} \colorbox{red!1}{\strut amount} \colorbox{red!6}{\strut of} \colorbox{red!7}{\strut points} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut player} \colorbox{red!6}{\strut gains} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut particular} \colorbox{red!0}{\strut discoveries} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut choice} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut In} \colorbox{red!1}{\strut particular} \colorbox{red!2}{\strut .} 
}}}
\end{CJK*}

89:nile, 76:egypt, 63:water, 59:source, 59:river, 29:flows, 27:white, 26:world, 26:formed, 24:main


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Photos} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!51}{\strut Nile} \colorbox{red!0}{\strut -} \colorbox{red!43}{\strut Egypt} \colorbox{red!0}{\strut .} \colorbox{red!43}{\strut Egypt} \colorbox{red!3}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut Gift} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!51}{\strut Nile} \colorbox{red!0}{\strut .} \colorbox{red!43}{\strut Egypt} \colorbox{red!0}{\strut s} \colorbox{red!13}{\strut main} \colorbox{red!34}{\strut source} \colorbox{red!2}{\strut of} \colorbox{red!36}{\strut water} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!51}{\strut Nile} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut longest} \colorbox{red!34}{\strut river} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!14}{\strut world} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut it} \colorbox{red!3}{\strut is} \colorbox{red!2}{\strut 6695} \colorbox{red!4}{\strut Kms} \colorbox{red!1}{\strut from} \colorbox{red!2}{\strut the} \colorbox{red!34}{\strut source} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!15}{\strut White} \colorbox{red!51}{\strut Nile} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Other} \colorbox{red!0}{\strut sources} \colorbox{red!2}{\strut of} \colorbox{red!36}{\strut water} \colorbox{red!1}{\strut in} \colorbox{red!43}{\strut Egypt} \colorbox{red!1}{\strut are} \colorbox{red!5}{\strut negligible} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut without} \colorbox{red!2}{\strut the} \colorbox{red!51}{\strut Nile} \colorbox{red!3}{\strut ,} \colorbox{red!43}{\strut Egypt} \colorbox{red!3}{\strut would} \colorbox{red!2}{\strut not} \colorbox{red!2}{\strut have} \colorbox{red!2}{\strut enough} \colorbox{red!36}{\strut water} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut everyone} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!51}{\strut Nile} \colorbox{red!3}{\strut is} \colorbox{red!14}{\strut formed} \colorbox{red!12}{\strut when} \colorbox{red!2}{\strut the} \colorbox{red!15}{\strut White} \colorbox{red!51}{\strut Nile} \colorbox{red!1}{\strut .} \colorbox{red!14}{\strut formed} \colorbox{red!1}{\strut from} \colorbox{red!9}{\strut Lake} \colorbox{red!3}{\strut Victoria} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut Uganda} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut meets} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut Blue} \colorbox{red!51}{\strut Nile} \colorbox{red!1}{\strut .} \colorbox{red!14}{\strut formed} \colorbox{red!1}{\strut from} \colorbox{red!9}{\strut Lake} \colorbox{red!3}{\strut Tana} \colorbox{red!1}{\strut in} \colorbox{red!4}{\strut Ethiopia} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut then} \colorbox{red!16}{\strut flows} \colorbox{red!1}{\strut all} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut way} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut Mediterranean} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Life} \colorbox{red!1}{\strut in} \colorbox{red!43}{\strut Egypt} \colorbox{red!3}{\strut is} \colorbox{red!1}{\strut along} \colorbox{red!2}{\strut the} \colorbox{red!51}{\strut Nile} \colorbox{red!3}{\strut ,} \colorbox{red!1}{\strut 94} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut Egyptian} \colorbox{red!4}{\strut Population} \colorbox{red!6}{\strut live} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut edges} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!51}{\strut Nile} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut 4} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut land} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut In} \colorbox{red!8}{\strut Cairo} \colorbox{red!0}{\strut Outside} \colorbox{red!8}{\strut Cairo} \colorbox{red!3}{\strut People} \colorbox{red!0}{\strut living} \colorbox{red!0}{\strut off} \colorbox{red!2}{\strut the} \colorbox{red!51}{\strut Nile} \colorbox{red!2}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut About} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Places} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Portfolio} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Buy} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Site} \colorbox{red!2}{\strut Map} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Contact} \colorbox{red!0}{\strut Me} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Wallpaper} 
}}}
\end{CJK*}

query: american military university

93:american, 89:military, 86:university, 46:what, 37:campus, 31:amu, 24:colleges, 21:apus, 16:engineering, 16:classes


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!99}{\strut American} \colorbox{red!94}{\strut Military} \colorbox{red!91}{\strut University} \colorbox{red!39}{\strut Campus} \colorbox{red!10}{\strut Login} \colorbox{red!5}{\strut User} \colorbox{red!5}{\strut ID} \colorbox{red!5}{\strut .} \colorbox{red!9}{\strut Password} \colorbox{red!5}{\strut .} \colorbox{red!3}{\strut Forgot} \colorbox{red!4}{\strut Your} \colorbox{red!9}{\strut Password} \colorbox{red!4}{\strut or} \colorbox{red!5}{\strut User} \colorbox{red!5}{\strut ID} \colorbox{red!3}{\strut ?} \colorbox{red!6}{\strut Call} \colorbox{red!14}{\strut Admissions} \colorbox{red!0}{\strut 1-877-777-9081} \colorbox{red!2}{\strut All} \colorbox{red!2}{\strut Other} \colorbox{red!0}{\strut Calls} \colorbox{red!0}{\strut 1-877-755-2787} \colorbox{red!0}{\strut E-mail} \colorbox{red!14}{\strut Admissions} \colorbox{red!4}{\strut Live} \colorbox{red!3}{\strut Chat} \colorbox{red!6}{\strut Find} \colorbox{red!4}{\strut a} \colorbox{red!4}{\strut Rep} \colorbox{red!5}{\strut Near} \colorbox{red!4}{\strut You} \colorbox{red!7}{\strut Schedule} \colorbox{red!0}{\strut ofClasses} \colorbox{red!0}{\strut E-mail} \colorbox{red!0}{\strut StudentServices} \colorbox{red!6}{\strut Transfer} \colorbox{red!8}{\strut Credit} \colorbox{red!8}{\strut Center} \colorbox{red!49}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!11}{\strut New} \colorbox{red!7}{\strut Interested} \colorbox{red!3}{\strut in} \colorbox{red!4}{\strut a} \colorbox{red!9}{\strut BS} \colorbox{red!3}{\strut in} \colorbox{red!17}{\strut Engineering} \colorbox{red!3}{\strut ?} \colorbox{red!7}{\strut Take} \colorbox{red!4}{\strut Our} \colorbox{red!4}{\strut Survey} \colorbox{red!3}{\strut !} \colorbox{red!7}{\strut Internet} \colorbox{red!4}{\strut Connectivity} \colorbox{red!5}{\strut Issues} \colorbox{red!7}{\strut Overseas} \colorbox{red!22}{\strut APUS} \colorbox{red!5}{\strut Announces} \colorbox{red!11}{\strut President} \colorbox{red!0}{\strut s} \colorbox{red!9}{\strut Honor} \colorbox{red!5}{\strut and} \colorbox{red!8}{\strut Dean} \colorbox{red!0}{\strut s} \colorbox{red!9}{\strut Lists} \colorbox{red!33}{\strut AMU} \colorbox{red!5}{\strut Makes} \colorbox{red!3}{\strut It} \colorbox{red!6}{\strut on} \colorbox{red!0}{\strut List} \colorbox{red!4}{\strut of} \colorbox{red!6}{\strut Top} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut Military-Friendly} \colorbox{red!25}{\strut Colleges} \colorbox{red!5}{\strut and} \colorbox{red!0}{\strut Universities} \colorbox{red!7}{\strut Online} \colorbox{red!14}{\strut Programs} \colorbox{red!4}{\strut Over} \colorbox{red!1}{\strut 50} \colorbox{red!7}{\strut Online} \colorbox{red!12}{\strut Associate} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut Bachelor} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut and} \colorbox{red!8}{\strut Master} \colorbox{red!0}{\strut s} \colorbox{red!12}{\strut Degrees} \colorbox{red!7}{\strut Homeland} \colorbox{red!5}{\strut Security} \colorbox{red!6}{\strut Sports} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Health} \colorbox{red!6}{\strut Sciences} \colorbox{red!3}{\strut Intelligence} \colorbox{red!6}{\strut Public} \colorbox{red!5}{\strut Administration} \colorbox{red!6}{\strut Emergency} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Disaster} \colorbox{red!3}{\strut Management} \colorbox{red!5}{\strut Transportation} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Logistics} \colorbox{red!3}{\strut Management} \colorbox{red!3}{\strut History} \colorbox{red!5}{\strut Security} \colorbox{red!5}{\strut Ma} 
}}}
\end{CJK*}

99:articulation, 95:agreement, 79:what, 47:vccs, 45:transfer, 28:university, 28:college, 24:brcc, 22:requirements, 19:state


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut HOME} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SITE} \colorbox{red!2}{\strut INDEX} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Z} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SEARCH} \colorbox{red!1}{\strut Current} \colorbox{red!3}{\strut Students} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Academic} \colorbox{red!5}{\strut Advising} \colorbox{red!8}{\strut ADMISSIONS} \colorbox{red!6}{\strut REGISTRATION} \colorbox{red!5}{\strut ACADEMIC} \colorbox{red!5}{\strut ADVISING} \colorbox{red!22}{\strut TRANSFER} \colorbox{red!4}{\strut PLANNING} \colorbox{red!22}{\strut Transfer} \colorbox{red!7}{\strut Program} \colorbox{red!22}{\strut Transfer} \colorbox{red!46}{\strut Agreement} \colorbox{red!4}{\strut Types} \colorbox{red!5}{\strut Guaranteed} \colorbox{red!8}{\strut Admissions} \colorbox{red!0}{\strut Agreements} \colorbox{red!48}{\strut Articulation} \colorbox{red!0}{\strut Agreements} \colorbox{red!0}{\strut by} \colorbox{red!11}{\strut BRCC} \colorbox{red!9}{\strut Degree} \colorbox{red!22}{\strut Transfer} \colorbox{red!5}{\strut Advising} \colorbox{red!1}{\strut Guides} \colorbox{red!22}{\strut Transfer} \colorbox{red!1}{\strut Links} \colorbox{red!4}{\strut ORIENTATION} \colorbox{red!3}{\strut New} \colorbox{red!3}{\strut Students} \colorbox{red!4}{\strut General} \colorbox{red!5}{\strut ADVISING} \colorbox{red!3}{\strut Advanced} \colorbox{red!2}{\strut Standing} \colorbox{red!2}{\strut Faculty} \colorbox{red!3}{\strut Advisors} \colorbox{red!6}{\strut Graduation} \colorbox{red!2}{\strut Honors} \colorbox{red!7}{\strut Program} \colorbox{red!7}{\strut Program} \colorbox{red!1}{\strut Selection} \colorbox{red!2}{\strut DISABILITY} \colorbox{red!1}{\strut SERVICES} \colorbox{red!4}{\strut PEER} \colorbox{red!1}{\strut TUTORING} \colorbox{red!3}{\strut LEARNING} \colorbox{red!1}{\strut ASSISTANCE} \colorbox{red!2}{\strut CTR} \colorbox{red!1}{\strut CLUBS} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ORGANIZATIONS} \colorbox{red!0}{\strut STUDENT} \colorbox{red!1}{\strut ACTIVITIES} \colorbox{red!1}{\strut CAREER} \colorbox{red!2}{\strut RESOURCES} \colorbox{red!48}{\strut Articulation} \colorbox{red!0}{\strut Agreements} \colorbox{red!0}{\strut by} \colorbox{red!11}{\strut BRCC} \colorbox{red!9}{\strut Degree} \colorbox{red!38}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!48}{\strut articulation} \colorbox{red!46}{\strut agreement} \colorbox{red!0}{\strut ?} \colorbox{red!8}{\strut Associate} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Arts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Sciences} \colorbox{red!9}{\strut Degree} \colorbox{red!0}{\strut CollegeUniversity} \colorbox{red!22}{\strut Transfer} \colorbox{red!0}{\strut The} \colorbox{red!23}{\strut VCCS} \colorbox{red!0}{\strut has} \colorbox{red!48}{\strut articulation} \colorbox{red!0}{\strut agreements} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut all} \colorbox{red!3}{\strut four} \colorbox{red!4}{\strut year} \colorbox{red!9}{\strut state} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut public} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut collegesuniversities} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Students} \colorbox{red!0}{\strut graduating} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut this} \colorbox{red!9}{\strut degree} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut granted} \colorbox{red!4}{\strut junior} \colorbox{red!3}{\strut status} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut collegesuniversities} \colorbox{red!3}{\strut waive} \colorbox{red!4}{\strut general} \colorbox{red!8}{\strut education} \colorbox{red!10}{\strut requirements} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut may} \colorbox{red!9}{\strut state} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut general} \colorbox{red!8}{\strut education} \colorbox{red!10}{\strut requirements} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut met} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!22}{\strut Transfer} \colorbox{red!5}{\strut Advising} \colorbox{red!1}{\strut Guides} \colorbox{red!0}{\strut for} \colorbox{red!22}{\strut transfer} \colorbox{red!0}{\strut institution-specific} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut Associates} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Applied} \colorbox{red!2}{\strut Science} \colorbox{red!0}{\strut Degrees} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut files} \colorbox{red!0}{\strut linked} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut require} \colorbox{red!0}{\strut Adobe} \colorbox{red!1}{\strut Acrobat} \colorbox{red!0}{\strut Reader} \colorbox{red!1}{\strut Accounting} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!2}{\strut Administration} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Justice} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!2}{\strut Eastern} \colorbox{red!2}{\strut Kentucky} \colorbox{red!0}{\strut University-} \colorbox{red!13}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Justice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Safety} \colorbox{red!2}{\strut Ferrum} \colorbox{red!13}{\strut College} \colorbox{red!1}{\strut Criminal} \colorbox{red!3}{\strut Justice} \colorbox{red!7}{\strut Program} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut Management} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut Computer} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Electronic} \colorbox{red!1}{\strut Technology} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!2}{\strut Old} \colorbox{red!1}{\strut Dominion} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut Computer} \colorbox{red!2}{\strut Science} \colorbox{red!0}{\strut James} \colorbox{red!0}{\strut Madison} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut Human} \colorbox{red!1}{\strut Services} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut Information} \colorbox{red!1}{\strut Systems} \colorbox{red!1}{\strut Technology} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!1}{\strut Radford} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut Manufacturing} \colorbox{red!1}{\strut Technology} \colorbox{red!2}{\strut Old} \colorbox{red!1}{\strut Dominion} \colorbox{red!13}{\strut University} \colorbox{red!1}{\strut Mechanical} \colorbox{red!1}{\strut Design} \colorbox{red!1}{\strut Technology} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!2}{\strut Old} \colorbox{red!1}{\strut Dominion} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut Nursing} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!2}{\strut Old} \colorbox{red!1}{\strut Dominion} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut Technical} \colorbox{red!1}{\strut Studies} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!2}{\strut Old} \colorbox{red!1}{\strut Dominion} \colorbox{red!13}{\strut University} \colorbox{red!1}{\strut Veterinary} \colorbox{red!1}{\strut Technology} \colorbox{red!2}{\strut American} \colorbox{red!6}{\strut Military} \colorbox{red!13}{\strut University} \colorbox{red!0}{\strut CONTACT} \colorbox{red!1}{\strut Counseling} \colorbox{red!1}{\strut Center} \colorbox{red!3}{\strut Houff} \colorbox{red!0}{\strut Student} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut M-Th} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 815} \colorbox{red!0}{\strut am-500} \colorbox{red!0}{\strut pm} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: rock gem shows

98:gem, 96:rock, 95:show, 32:n, 26:hop, 23:where, 23:farm, 21:park, 19:uk, 17:how


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Skip} \colorbox{red!1}{\strut To} \colorbox{red!2}{\strut Content} \colorbox{red!5}{\strut The} \colorbox{red!23}{\strut Hop} \colorbox{red!20}{\strut Farm} \colorbox{red!13}{\strut Country} \colorbox{red!18}{\strut Park} \colorbox{red!3}{\strut Keywords} \colorbox{red!4}{\strut Submit} \colorbox{red!14}{\strut Attractions} \colorbox{red!14}{\strut Events} \colorbox{red!5}{\strut Corporate} \colorbox{red!6}{\strut Weddings} \colorbox{red!5}{\strut Home} \colorbox{red!5}{\strut Visitor} \colorbox{red!1}{\strut Information} \colorbox{red!4}{\strut Groups} \colorbox{red!1}{\strut .} \colorbox{red!8}{\strut Schools} \colorbox{red!3}{\strut Trade} \colorbox{red!4}{\strut Camping} \colorbox{red!5}{\strut Season} \colorbox{red!8}{\strut Ticket} \colorbox{red!8}{\strut Children} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut Parties} \colorbox{red!14}{\strut Events} \colorbox{red!10}{\strut Calendar} \colorbox{red!2}{\strut Back} \colorbox{red!1}{\strut to} \colorbox{red!14}{\strut Events} \colorbox{red!10}{\strut Calendar} \colorbox{red!5}{\strut The} \colorbox{red!85}{\strut Rock} \colorbox{red!8}{\strut and} \colorbox{red!87}{\strut Gem} \colorbox{red!84}{\strut Show} \colorbox{red!7}{\strut Saturday} \colorbox{red!4}{\strut 24th} \colorbox{red!1}{\strut to} \colorbox{red!6}{\strut Sunday} \colorbox{red!5}{\strut 25th} \colorbox{red!5}{\strut January} \colorbox{red!0}{\strut 2009} \colorbox{red!4}{\strut Visit} \colorbox{red!5}{\strut the} \colorbox{red!85}{\strut Rock} \colorbox{red!7}{\strut .} \colorbox{red!28}{\strut n} \colorbox{red!7}{\strut .} \colorbox{red!87}{\strut Gem} \colorbox{red!84}{\strut Show} \colorbox{red!8}{\strut and} \colorbox{red!4}{\strut be} \colorbox{red!1}{\strut fascinated} \colorbox{red!2}{\strut by} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut whole} \colorbox{red!0}{\strut range} \colorbox{red!1}{\strut of} \colorbox{red!13}{\strut natural} \colorbox{red!10}{\strut stone} \colorbox{red!11}{\strut products} \colorbox{red!3}{\strut from} \colorbox{red!5}{\strut around} \colorbox{red!5}{\strut the} \colorbox{red!9}{\strut world} \colorbox{red!4}{\strut .} \colorbox{red!8}{\strut Available} \colorbox{red!2}{\strut at} \colorbox{red!4}{\strut reasonable} \colorbox{red!8}{\strut prices} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!84}{\strut show} \colorbox{red!0}{\strut includes} \colorbox{red!6}{\strut spectacular} \colorbox{red!13}{\strut mineral} \colorbox{red!6}{\strut specimens} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut sparkling} \colorbox{red!8}{\strut crystals} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut every} \colorbox{red!8}{\strut colour} \colorbox{red!8}{\strut and} \colorbox{red!6}{\strut ancient} \colorbox{red!8}{\strut fossils} \colorbox{red!4}{\strut .} \colorbox{red!8}{\strut Created} \colorbox{red!3}{\strut from} \colorbox{red!5}{\strut the} \colorbox{red!13}{\strut natural} \colorbox{red!11}{\strut products} \colorbox{red!1}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!6}{\strut beads} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut polished} \colorbox{red!8}{\strut and} \colorbox{red!5}{\strut carved} \colorbox{red!0}{\strut stones} \colorbox{red!8}{\strut and} \colorbox{red!6}{\strut gold} \colorbox{red!8}{\strut and} \colorbox{red!5}{\strut silver} \colorbox{red!5}{\strut jewellery} \colorbox{red!2}{\strut inset} \colorbox{red!4}{\strut with} \colorbox{red!0}{\strut them} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut Experienced} \colorbox{red!8}{\strut exhibitors} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut happy} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut discuss} \colorbox{red!5}{\strut the} \colorbox{red!11}{\strut products} \colorbox{red!8}{\strut available} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut whether} \colorbox{red!0}{\strut it} \colorbox{red!2}{\strut is} \colorbox{red!20}{\strut where} \colorbox{red!8}{\strut and} \colorbox{red!15}{\strut how} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut were} \colorbox{red!12}{\strut mined} \colorbox{red!0}{\strut or} \colorbox{red!15}{\strut how} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut were} \colorbox{red!9}{\strut formed} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Young} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut old} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut experienced} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut novice} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut see} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut event} \colorbox{red!4}{\strut .} \colorbox{red!7}{\strut Entrance} \colorbox{red!1}{\strut to} \colorbox{red!5}{\strut The} \colorbox{red!85}{\strut Rock} \colorbox{red!8}{\strut and} \colorbox{red!87}{\strut Gem} \colorbox{red!84}{\strut show} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!2}{\strut include} \colorbox{red!7}{\strut entrance} \colorbox{red!1}{\strut to} \colorbox{red!5}{\strut The} \colorbox{red!23}{\strut Hop} \colorbox{red!20}{\strut Farm} \colorbox{red!14}{\strut attractions} \colorbox{red!8}{\strut Ticket} \colorbox{red!8}{\strut Prices} \colorbox{red!4}{\strut Advance} \colorbox{red!4}{\strut Booking} \colorbox{red!3}{\strut Gate} \colorbox{red!0}{\strut Price} \colorbox{red!5}{\strut Adult} \colorbox{red!0}{\strut 3.00} \colorbox{red!7}{\strut Senior} \colorbox{red!0}{\strut 1.50} \colorbox{red!4}{\strut Child} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8-15} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1.00} \colorbox{red!0}{\strut Downloads} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Links} \colorbox{red!0}{\strut www.rockngem.co.uk} \colorbox{red!4}{\strut Site} \colorbox{red!1}{\strut Tools} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Normal} \colorbox{red!4}{\strut Text} \colorbox{red!1}{\strut Size} \colorbox{red!1}{\strut Decrease} \colorbox{red!4}{\strut Text} \colorbox{red!1}{\strut Size} \colorbox{red!2}{\strut Increase} \colorbox{red!4}{\strut Text} \colorbox{red!1}{\strut Size} \colorbox{red!4}{\strut Text} \colorbox{red!0}{\strut Only} \colorbox{red!1}{\strut Print} \colorbox{red!0}{\strut Page} \colorbox{red!3}{\strut Accommodation} \colorbox{red!2}{\strut Contact} \colorbox{red!3}{\strut Us} \colorbox{red!2}{\strut Work} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut Us} \colorbox{red!2}{\strut Links} \colorbox{red!3}{\strut Media} \colorbox{red!3}{\strut Centre} \colorbox{red!4}{\strut Site} \colorbox{red!3}{\strut Map} \colorbox{red!5}{\strut Terms} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Conditions} \colorbox{red!5}{\strut Privacy} \colorbox{red!4}{\strut Policy} \colorbox{red!8}{\strut Created} \colorbox{red!2}{\strut by} \colorbox{red!4}{\strut Tangerine} \colorbox{red!3}{\strut New} \colorbox{red!3}{\strut Media} 
}}}
\end{CJK*}

91:what, 86:gem, 82:shows, 80:rock, 26:minerals, 23:gemstones, 21:fossils, 12:history, 12:exhibit, 11:subject


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!51}{\strut What} \colorbox{red!2}{\strut are} \colorbox{red!45}{\strut ROCK} \colorbox{red!5}{\strut .} \colorbox{red!6}{\strut n} \colorbox{red!5}{\strut .} \colorbox{red!48}{\strut GEM} \colorbox{red!46}{\strut Shows} \colorbox{red!2}{\strut ?} \colorbox{red!0}{\strut Rocks} \colorbox{red!2}{\strut ,} \colorbox{red!14}{\strut minerals} \colorbox{red!2}{\strut and} \colorbox{red!11}{\strut fossils} \colorbox{red!1}{\strut have} \colorbox{red!3}{\strut fascinated} \colorbox{red!2}{\strut humanity} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut our} \colorbox{red!3}{\strut earliest} \colorbox{red!6}{\strut history} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut They} \colorbox{red!1}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!1}{\strut used} \colorbox{red!2}{\strut as} \colorbox{red!3}{\strut weapons} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut talismans} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut tokens} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut love} \colorbox{red!2}{\strut and} \colorbox{red!6}{\strut objects} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut desire} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut obsession} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Today} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut they} \colorbox{red!1}{\strut still} \colorbox{red!2}{\strut exert} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut same} \colorbox{red!2}{\strut mysterious} \colorbox{red!2}{\strut force} \colorbox{red!0}{\strut over} \colorbox{red!2}{\strut us} \colorbox{red!2}{\strut as} \colorbox{red!1}{\strut they} \colorbox{red!2}{\strut did} \colorbox{red!0}{\strut upon} \colorbox{red!2}{\strut our} \colorbox{red!2}{\strut distant} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut more} \colorbox{red!2}{\strut recent} \colorbox{red!2}{\strut ancestors} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut ROCKS} \colorbox{red!2}{\strut ,} \colorbox{red!14}{\strut MINERALS} \colorbox{red!2}{\strut ,} \colorbox{red!11}{\strut FOSSILS} \colorbox{red!2}{\strut ,} \colorbox{red!13}{\strut GEMSTONES} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut GEM-SET} \colorbox{red!4}{\strut jewellery} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut LAPIDARY} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut HEALING} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut other} \colorbox{red!5}{\strut facet} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut wonderful} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut fascinating} \colorbox{red!6}{\strut subject} \colorbox{red!2}{\strut are} \colorbox{red!0}{\strut all} \colorbox{red!4}{\strut available} \colorbox{red!3}{\strut at} \colorbox{red!45}{\strut ROCK} \colorbox{red!5}{\strut .} \colorbox{red!6}{\strut n} \colorbox{red!5}{\strut .} \colorbox{red!48}{\strut GEM} \colorbox{red!46}{\strut shows} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut If} \colorbox{red!2}{\strut you} \colorbox{red!2}{\strut are} \colorbox{red!2}{\strut a} \colorbox{red!2}{\strut serious} \colorbox{red!4}{\strut collector} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut a} \colorbox{red!2}{\strut hobbyist} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut a} \colorbox{red!5}{\strut geologist} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut lapidarist} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut Club} \colorbox{red!1}{\strut member} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut Professional} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut then} \colorbox{red!45}{\strut ROCK} \colorbox{red!5}{\strut .} \colorbox{red!6}{\strut n} \colorbox{red!5}{\strut .} \colorbox{red!48}{\strut GEM} \colorbox{red!46}{\strut shows} \colorbox{red!1}{\strut have} \colorbox{red!3}{\strut something} \colorbox{red!3}{\strut for} \colorbox{red!2}{\strut you} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut Some} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.K.} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut leading} \colorbox{red!4}{\strut dealers} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut an} \colorbox{red!0}{\strut ever} \colorbox{red!0}{\strut increasing} \colorbox{red!0}{\strut number} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut European} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut International} \colorbox{red!4}{\strut dealers} \colorbox{red!6}{\strut exhibit} \colorbox{red!3}{\strut at} \colorbox{red!45}{\strut ROCK} \colorbox{red!5}{\strut .} \colorbox{red!6}{\strut n} \colorbox{red!5}{\strut .} \colorbox{red!48}{\strut GEM} \colorbox{red!46}{\strut Shows} \colorbox{red!3}{\strut offering} \colorbox{red!2}{\strut a} \colorbox{red!2}{\strut wide} \colorbox{red!1}{\strut range} \colorbox{red!2}{\strut of} \colorbox{red!13}{\strut gemstones} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut geological} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut mineral} \colorbox{red!3}{\strut samples} \colorbox{red!2}{\strut Home} \colorbox{red!3}{\strut -} \colorbox{red!0}{\strut About} \colorbox{red!3}{\strut -} \colorbox{red!2}{\strut Magazine} \colorbox{red!3}{\strut -} \colorbox{red!3}{\strut Events} \colorbox{red!4}{\strut Copyright} \colorbox{red!0}{\strut 2006-09} \colorbox{red!45}{\strut Rock} \colorbox{red!2}{\strut and} \colorbox{red!48}{\strut Gem} \colorbox{red!4}{\strut Ltd} 
}}}
\end{CJK*}

query: rocky mountain news

98:news, 96:rocky, 94:mountain, 44:newspaper, 41:owned, 38:who, 26:colorado, 22:circulation, 21:denver, 20:running


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Rocky} \colorbox{red!100}{\strut Mountain} \colorbox{red!100}{\strut News} \colorbox{red!0}{\strut From} \colorbox{red!2}{\strut Wikipedia} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!3}{\strut encyclopedia} \colorbox{red!2}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!4}{\strut ,} \colorbox{red!1}{\strut search} \colorbox{red!100}{\strut Rocky} \colorbox{red!100}{\strut Mountain} \colorbox{red!100}{\strut News} \colorbox{red!5}{\strut The} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 2} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut front} \colorbox{red!2}{\strut page} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!100}{\strut Rocky} \colorbox{red!100}{\strut Mountain} \colorbox{red!100}{\strut News} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut before} \colorbox{red!5}{\strut the} \colorbox{red!1}{\strut 2007} \colorbox{red!6}{\strut redesign} \colorbox{red!6}{\strut Type} \colorbox{red!16}{\strut Daily} \colorbox{red!48}{\strut newspaper} \colorbox{red!7}{\strut Format} \colorbox{red!9}{\strut Tabloid} \colorbox{red!6}{\strut Owner} \colorbox{red!0}{\strut E.} \colorbox{red!0}{\strut W.} \colorbox{red!19}{\strut Scripps} \colorbox{red!16}{\strut Company} \colorbox{red!4}{\strut ,} \colorbox{red!14}{\strut Operated} \colorbox{red!0}{\strut by} \colorbox{red!22}{\strut Denver} \colorbox{red!48}{\strut Newspaper} \colorbox{red!1}{\strut Agency} \colorbox{red!10}{\strut Publisher} \colorbox{red!3}{\strut John} \colorbox{red!8}{\strut Temple} \colorbox{red!5}{\strut Editor} \colorbox{red!3}{\strut John} \colorbox{red!8}{\strut Temple} \colorbox{red!15}{\strut Founded} \colorbox{red!0}{\strut 1859} \colorbox{red!2}{\strut Headquarters} \colorbox{red!0}{\strut 101} \colorbox{red!0}{\strut West} \colorbox{red!2}{\strut Colfax} \colorbox{red!0}{\strut Ave.} \colorbox{red!0}{\strut Suite} \colorbox{red!0}{\strut 500} \colorbox{red!22}{\strut Denver} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut CO} \colorbox{red!0}{\strut 80202} \colorbox{red!8}{\strut United} \colorbox{red!8}{\strut States} \colorbox{red!24}{\strut Circulation} \colorbox{red!0}{\strut 255,427} \colorbox{red!16}{\strut Daily} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 704,806} \colorbox{red!5}{\strut Sunday} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Website} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut rockymountainnews.com} \colorbox{red!5}{\strut The} \colorbox{red!100}{\strut Rocky} \colorbox{red!100}{\strut Mountain} \colorbox{red!100}{\strut News} \colorbox{red!5}{\strut is} \colorbox{red!4}{\strut a} \colorbox{red!0}{\strut Monday-Saturday} \colorbox{red!5}{\strut morning} \colorbox{red!9}{\strut tabloid} \colorbox{red!0}{\strut -format} \colorbox{red!48}{\strut newspaper} \colorbox{red!0}{\strut published} \colorbox{red!3}{\strut in} \colorbox{red!22}{\strut Denver} \colorbox{red!4}{\strut ,} \colorbox{red!28}{\strut Colorado} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut United} \colorbox{red!8}{\strut States} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut It} \colorbox{red!5}{\strut is} \colorbox{red!44}{\strut owned} \colorbox{red!0}{\strut by} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut E.} \colorbox{red!0}{\strut W.} \colorbox{red!19}{\strut Scripps} \colorbox{red!16}{\strut Company} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Despite} \colorbox{red!19}{\strut Scripps} \colorbox{red!4}{\strut still} \colorbox{red!21}{\strut running} \colorbox{red!5}{\strut the} \colorbox{red!19}{\strut paper} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut only} \colorbox{red!48}{\strut newspaper} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut the} \colorbox{red!19}{\strut Scripps} \colorbox{red!0}{\strut family} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!5}{\strut the} \colorbox{red!5}{\strut corporate} \colorbox{red!4}{\strut lighthouse} \colorbox{red!0}{\strut logo} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut front} \colorbox{red!2}{\strut page} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut As} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut March} \colorbox{red!0}{\strut 2006} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut Monday-Friday} \colorbox{red!24}{\strut circulation} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut 255,427} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Under} \colorbox{red!5}{\strut the} \colorbox{red!3}{\strut leadership} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut President} \colorbox{red!4}{\strut ,} \colorbox{red!10}{\strut Publisher} \colorbox{red!2}{\strut and} \colorbox{red!5}{\strut Editor} \colorbox{red!3}{\strut John} \colorbox{red!8}{\strut Temple} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!100}{\strut Rocky} \colorbox{red!100}{\strut Mountain} \colorbox{red!100}{\strut News} \colorbox{red!2}{\strut has} \colorbox{red!5}{\strut won} \colorbox{red!0}{\strut four} \colorbox{red!13}{\strut Pulitzer} \colorbox{red!5}{\strut Prizes} \colorbox{red!0}{\strut since} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut 2000} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut recently} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut 2006} \colorbox{red!4}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!48}{\strut newspaper} \colorbox{red!5}{\strut won} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut Pulitzers} \colorbox{red!3}{\strut in} \colorbox{red!2}{\strut Feature} \colorbox{red!2}{\strut Writing} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut Feature} \colorbox{red!0}{\strut Photography} \colorbox{red!5}{\strut .} \colorbox{red!1}{\strut Contents} \colorbox{red!3}{\strut 1} \colorbox{red!4}{\strut History} \colorbox{red!0}{\strut 1.1} \colorbox{red!0}{\strut First} \colorbox{red!12}{\strut issue} \colorbox{red!0}{\strut 1.2} \colorbox{red!2}{\strut Jack} \colorbox{red!3}{\strut Foster} \colorbox{red!0}{\strut 1.3} \colorbox{red!5}{\strut The} \colorbox{red!2}{\strut joint} \colorbox{red!0}{\strut operating} \colorbox{red!1}{\strut agreement} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Recent} \colorbox{red!3}{\strut Awards} \colorbox{red!0}{\strut 2.1} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut 2.2} \colorbox{red!0}{\strut 2003} \colorbox{red!0}{\strut 2.3} \colorbox{red!0}{\strut 2002} \colorbox{red!0}{\strut 2.4} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut 3} \colorbox{red!100}{\strut Rocky} \colorbox{red!0}{\strut redesigned} \colorbox{red!1}{\strut 4} \colorbox{red!100}{\strut News} \colorbox{red!2}{\strut Put} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut For} \colorbox{red!3}{\strut Sale} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut History} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!12}{\strut issue} \colorbox{red!5}{\strut The} \colorbox{red!100}{\strut Rocky} \colorbox{red!100}{\strut Mountain} \colorbox{red!100}{\strut News} \colorbox{red!5}{\strut is} \colorbox{red!28}{\strut Colorado} \colorbox{red!0}{\strut s} \colorbox{red!12}{\strut oldest} \colorbox{red!48}{\strut newspaper} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut continuously} \colorbox{red!14}{\strut operated} \colorbox{red!1}{\strut business} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Its} \colorbox{red!0}{\strut first} \colorbox{red!12}{\strut issue} \colorbox{red!0}{\strut was} \colorbox{red!9}{\strut printed} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut April} \colorbox{red!0}{\strut 23} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut 1859} \colorbox{red!0}{\strut by} \colorbox{red!4}{\strut founder} \colorbox{red!3}{\strut William} \colorbox{red!0}{\strut N.} \colorbox{red!3}{\strut Byers} \colorbox{red!4}{\strut ,} \colorbox{red!41}{\strut who} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut hauled} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut printing} \colorbox{red!3}{\strut press} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Omaha} \colorbox{red!4}{\strut ,} \colorbox{red!2}{\strut Nebraska} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut oxcart} \colorbox{red!0}{\strut during} \colorbox{red!5}{\strut the} \colorbox{red!6}{\strut start} \colorbox{red!0}{\strut of} 
}}}
\end{CJK*}

99:rocky, 98:mountain, 22:range, 22:county, 21:georgia, 16:colorado, 15:states, 15:california, 14:arkansas, 13:movie


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut disambiguation} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!2}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!2}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut refer} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 46} \colorbox{red!7}{\strut summits} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut United} \colorbox{red!10}{\strut States} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Alaska} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Arkansas} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut San} \colorbox{red!0}{\strut Diego} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut California} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Sonoma} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut California} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -1} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Sonoma} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut California} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -2} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Colorado} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Fannin} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Gilmer} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lumpkin} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rabun} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Towns} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Union} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -1} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Union} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -2} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Union} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -3} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut White} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut Georgia} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Idaho} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Kentucky} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Aroostook} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut Maine} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Knox} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut Maine} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Mississippi} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Missouri} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Montana} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut New} \colorbox{red!0}{\strut Hampshire} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut Jersey} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Essex} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Hamilton} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut Lawrence} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Ulster} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut New} \colorbox{red!2}{\strut York} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Henderson} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut North} \colorbox{red!5}{\strut Carolina} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Jackson} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut North} \colorbox{red!5}{\strut Carolina} \colorbox{red!2}{\strut .} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut McDowell} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut North} \colorbox{red!5}{\strut Carolina} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -1} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut McDowell} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut North} \colorbox{red!5}{\strut Carolina} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -2} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Transylvania} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut North} \colorbox{red!5}{\strut Carolina} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -1} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Transylvania} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut North} \colorbox{red!5}{\strut Carolina} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut -2} \colorbox{red!70}{\strut Rocky} \colorbox{red!69}{\strut Mountain} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: supper painting

98:supper, 92:painted, 58:what, 38:when, 35:last, 32:why, 29:leonardo, 25:did, 24:famous, 23:fresco


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut LisaShea.com} \colorbox{red!3}{\strut Homepage} \colorbox{red!3}{\strut Site} \colorbox{red!5}{\strut Map} \colorbox{red!0}{\strut Most} \colorbox{red!8}{\strut Popular} \colorbox{red!0}{\strut DaVinci} \colorbox{red!17}{\strut Code} \colorbox{red!8}{\strut Parakeets} \colorbox{red!3}{\strut Origami} \colorbox{red!2}{\strut Travelogues} \colorbox{red!3}{\strut Forums} \colorbox{red!1}{\strut My} \colorbox{red!4}{\strut Books} \colorbox{red!4}{\strut Irish} \colorbox{red!5}{\strut Weddings} \colorbox{red!7}{\strut Italian} \colorbox{red!5}{\strut Weddings} \colorbox{red!6}{\strut French} \colorbox{red!5}{\strut Weddings} \colorbox{red!3}{\strut The} \colorbox{red!26}{\strut Last} \colorbox{red!73}{\strut Supper} \colorbox{red!21}{\strut Leonardo} \colorbox{red!11}{\strut da} \colorbox{red!16}{\strut Vinci} \colorbox{red!3}{\strut ,} \colorbox{red!7}{\strut Mary} \colorbox{red!12}{\strut Magdalene} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut The} \colorbox{red!12}{\strut Hand} \colorbox{red!3}{\strut and} \colorbox{red!5}{\strut Knife} \colorbox{red!21}{\strut Leonardo} \colorbox{red!11}{\strut da} \colorbox{red!16}{\strut Vinci} \colorbox{red!4}{\strut was} \colorbox{red!2}{\strut already} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut well} \colorbox{red!11}{\strut known} \colorbox{red!16}{\strut artist} \colorbox{red!28}{\strut when} \colorbox{red!3}{\strut he} \colorbox{red!13}{\strut created} \colorbox{red!3}{\strut his} \colorbox{red!9}{\strut masterpiece} \colorbox{red!3}{\strut The} \colorbox{red!26}{\strut Last} \colorbox{red!73}{\strut Supper} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut He} \colorbox{red!69}{\strut painted} \colorbox{red!3}{\strut it} \colorbox{red!2}{\strut on} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut back} \colorbox{red!6}{\strut wall} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!7}{\strut dining} \colorbox{red!9}{\strut hall} \colorbox{red!3}{\strut at} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut Dominican} \colorbox{red!4}{\strut convent} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut Sta} \colorbox{red!3}{\strut Maria} \colorbox{red!0}{\strut delle} \colorbox{red!4}{\strut Grazie} \colorbox{red!2}{\strut in} \colorbox{red!7}{\strut Italy} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!9}{\strut reason} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut painting} \colorbox{red!2}{\strut is} \colorbox{red!7}{\strut laid} \colorbox{red!3}{\strut out} \colorbox{red!3}{\strut the} \colorbox{red!10}{\strut way} \colorbox{red!3}{\strut it} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut that} \colorbox{red!21}{\strut Leonardo} \colorbox{red!4}{\strut was} \colorbox{red!1}{\strut trying} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut extend} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut room} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut to} \colorbox{red!5}{\strut make} \colorbox{red!3}{\strut it} \colorbox{red!4}{\strut look} \colorbox{red!2}{\strut like} \colorbox{red!9}{\strut Jesus} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut his} \colorbox{red!7}{\strut apostles} \colorbox{red!3}{\strut were} \colorbox{red!3}{\strut sitting} \colorbox{red!3}{\strut at} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!7}{\strut dining} \colorbox{red!9}{\strut hall} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut This} \colorbox{red!0}{\strut painting} \colorbox{red!3}{\strut became} \colorbox{red!2}{\strut an} \colorbox{red!4}{\strut instant} \colorbox{red!18}{\strut famous} \colorbox{red!10}{\strut work} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut many} \colorbox{red!0}{\strut reasons} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!0}{\strut painting} \colorbox{red!5}{\strut depicts} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut very} \colorbox{red!5}{\strut moment} \colorbox{red!3}{\strut that} \colorbox{red!9}{\strut Jesus} \colorbox{red!0}{\strut has} \colorbox{red!6}{\strut said} \colorbox{red!3}{\strut to} \colorbox{red!3}{\strut his} \colorbox{red!9}{\strut disciples} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Now} \colorbox{red!28}{\strut when} \colorbox{red!3}{\strut the} \colorbox{red!1}{\strut even} \colorbox{red!4}{\strut was} \colorbox{red!9}{\strut come} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut he} \colorbox{red!6}{\strut sat} \colorbox{red!1}{\strut down} \colorbox{red!2}{\strut with} \colorbox{red!3}{\strut the} \colorbox{red!9}{\strut twelve} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut And} \colorbox{red!2}{\strut as} \colorbox{red!1}{\strut they} \colorbox{red!18}{\strut did} \colorbox{red!3}{\strut eat} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut he} \colorbox{red!6}{\strut said} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut Verily} \colorbox{red!0}{\strut I} \colorbox{red!5}{\strut say} \colorbox{red!2}{\strut unto} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut that} \colorbox{red!1}{\strut one} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut shall} \colorbox{red!6}{\strut betray} \colorbox{red!0}{\strut me} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut And} \colorbox{red!1}{\strut they} \colorbox{red!3}{\strut were} \colorbox{red!3}{\strut exceeding} \colorbox{red!0}{\strut sorrowful} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut began} \colorbox{red!0}{\strut every} \colorbox{red!1}{\strut one} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut them} \colorbox{red!3}{\strut to} \colorbox{red!5}{\strut say} \colorbox{red!2}{\strut unto} \colorbox{red!0}{\strut him} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut Lord} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut it} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut And} \colorbox{red!3}{\strut he} \colorbox{red!2}{\strut answered} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut said} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut He} \colorbox{red!3}{\strut that} \colorbox{red!3}{\strut dippeth} \colorbox{red!3}{\strut his} \colorbox{red!12}{\strut hand} \colorbox{red!2}{\strut with} \colorbox{red!0}{\strut me} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut dish} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!3}{\strut shall} \colorbox{red!6}{\strut betray} \colorbox{red!0}{\strut me} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut --} \colorbox{red!5}{\strut Matthew} \colorbox{red!2}{\strut 26} \colorbox{red!3}{\strut The} \colorbox{red!9}{\strut disciples} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut all} \colorbox{red!4}{\strut reacting} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut horror} \colorbox{red!3}{\strut to} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut thought} \colorbox{red!3}{\strut that} \colorbox{red!2}{\strut someone} \colorbox{red!3}{\strut at} \colorbox{red!3}{\strut that} \colorbox{red!6}{\strut table} \colorbox{red!3}{\strut would} \colorbox{red!6}{\strut betray} \colorbox{red!0}{\strut their} \colorbox{red!6}{\strut master} \colorbox{red!4}{\strut .} \colorbox{red!17}{\strut Fresco} \colorbox{red!1}{\strut vs} \colorbox{red!4}{\strut Tempera} \colorbox{red!0}{\strut Dan} \colorbox{red!1}{\strut Brown} \colorbox{red!0}{\strut s} \colorbox{red!9}{\strut error} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut The} \colorbox{red!11}{\strut Da} \colorbox{red!16}{\strut Vinci} \colorbox{red!17}{\strut Code} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut that} \colorbox{red!3}{\strut he} \colorbox{red!6}{\strut calls} \colorbox{red!3}{\strut the} \colorbox{red!26}{\strut Last} \colorbox{red!73}{\strut Supper} \colorbox{red!2}{\strut a} \colorbox{red!17}{\strut FRESCO} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut This} \colorbox{red!0}{\strut painting} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!2}{\strut a} \colorbox{red!17}{\strut fresco} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut This} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut critical} \colorbox{red!5}{\strut mistake} \colorbox{red!3}{\strut because} \colorbox{red!0}{\strut if} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut painting} \colorbox{red!1}{\strut had} \colorbox{red!1}{\strut been} \colorbox{red!2}{\strut a} \colorbox{red!17}{\strut fresco} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!3}{\strut would} \colorbox{red!3}{\strut still} \colorbox{red!1}{\strut have} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut superb} \colorbox{red!4}{\strut image} \colorbox{red!3}{\strut to} 
}}}
\end{CJK*}

87:painting, 55:supper, 53:italian, 45:italy, 31:fresco, 30:vinci, 30:art, 29:renaissance, 25:last, 23:artists


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!30}{\strut Italian} \colorbox{red!16}{\strut Renaissance} \colorbox{red!13}{\strut Artists} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut L} \colorbox{red!30}{\strut Italian} \colorbox{red!16}{\strut Renaissance} \colorbox{red!13}{\strut Artists} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Z} \colorbox{red!30}{\strut Italian} \colorbox{red!16}{\strut Renaissance} \colorbox{red!0}{\strut MovementsPeriods} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut in} \colorbox{red!17}{\strut Art} \colorbox{red!1}{\strut Glossary} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut Terms} \colorbox{red!2}{\strut Contemporary} \colorbox{red!2}{\strut Abstract} \colorbox{red!17}{\strut Art} \colorbox{red!2}{\strut Unique} \colorbox{red!1}{\strut Gifts} \colorbox{red!5}{\strut Oil} \colorbox{red!50}{\strut Painting} \colorbox{red!5}{\strut Reproductions} \colorbox{red!4}{\strut Sculpture} \colorbox{red!5}{\strut Reproductions} \colorbox{red!17}{\strut Art} \colorbox{red!0}{\strut Puzzles} \colorbox{red!10}{\strut Da} \colorbox{red!17}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!50}{\strut Painting} \colorbox{red!2}{\strut The} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!5}{\strut 1498} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Mixed} \colorbox{red!12}{\strut technique} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut 460} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 880} \colorbox{red!3}{\strut cm} \colorbox{red!5}{\strut Convent} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut Santa} \colorbox{red!4}{\strut Maria} \colorbox{red!2}{\strut delle} \colorbox{red!6}{\strut Grazie} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Milan} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut see} \colorbox{red!1}{\strut our} \colorbox{red!3}{\strut fine} \colorbox{red!17}{\strut art} \colorbox{red!5}{\strut reproductions} \colorbox{red!2}{\strut .} \colorbox{red!10}{\strut Da} \colorbox{red!17}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!50}{\strut painting} \colorbox{red!1}{\strut of} \colorbox{red!5}{\strut 1498} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut traditional} \colorbox{red!1}{\strut true} \colorbox{red!17}{\strut fresco} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut buon} \colorbox{red!17}{\strut fresco} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut painted} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut wet} \colorbox{red!8}{\strut plaster} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut painted} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut dry} \colorbox{red!8}{\strut plaster} \colorbox{red!1}{\strut with} \colorbox{red!4}{\strut tempera} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!17}{\strut fresco} \colorbox{red!2}{\strut secco} \colorbox{red!0}{\strut technique.Da} \colorbox{red!17}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!50}{\strut painting} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!3}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut refectory} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut dining} \colorbox{red!2}{\strut hall} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut convent} \colorbox{red!0}{\strut ofSanta} \colorbox{red!4}{\strut Maria} \colorbox{red!2}{\strut della} \colorbox{red!6}{\strut Grazie} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut Milan} \colorbox{red!1}{\strut ,} \colorbox{red!25}{\strut Italy} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!4}{\strut stone} \colorbox{red!5}{\strut wall} \colorbox{red!0}{\strut was} \colorbox{red!2}{\strut first} \colorbox{red!3}{\strut prepared} \colorbox{red!0}{\strut for} \colorbox{red!10}{\strut Da} \colorbox{red!17}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!50}{\strut painting} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut sealing} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut stone} \colorbox{red!1}{\strut with} \colorbox{red!2}{\strut pitch} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut mastic} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut gesso} \colorbox{red!2}{\strut .} \colorbox{red!10}{\strut Da} \colorbox{red!17}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut experimental} \colorbox{red!12}{\strut technique} \colorbox{red!4}{\strut caused} \colorbox{red!0}{\strut rapid} \colorbox{red!1}{\strut deterioration} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!50}{\strut painting} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut as} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut described} \colorbox{red!0}{\strut by} \colorbox{red!4}{\strut Vasari} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut a} \colorbox{red!9}{\strut Leonardo} \colorbox{red!0}{\strut biographer} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut as} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ruined} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut 1556} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!5}{\strut dry} \colorbox{red!0}{\strut paint} \colorbox{red!1}{\strut of} \colorbox{red!10}{\strut Da} \colorbox{red!17}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!50}{\strut painting} \colorbox{red!0}{\strut was} \colorbox{red!2}{\strut reported} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut be} \colorbox{red!4}{\strut flaking} \colorbox{red!1}{\strut off} \colorbox{red!2}{\strut as} \colorbox{red!1}{\strut early} \colorbox{red!2}{\strut as} \colorbox{red!2}{\strut 1517} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut consequence} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut his} \colorbox{red!2}{\strut experimental} \colorbox{red!12}{\strut technique} \colorbox{red!2}{\strut .} \colorbox{red!10}{\strut Da} \colorbox{red!17}{\strut Vinci} \colorbox{red!0}{\strut s} \colorbox{red!14}{\strut Last} \colorbox{red!31}{\strut Supper} \colorbox{red!50}{\strut painting} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut undergone} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut restorations} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut first} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut 1726} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!14}{\strut last} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1999} \colorbox{red!7}{\strut which} \colorbox{red!2}{\strut took} \colorbox{red!0}{\strut 21} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut finish} \colorbox{red!2}{\strut .} 
}}}
\end{CJK*}

query: porterville

99:porterville, 77:county, 42:california, 21:population, 16:location, 15:city, 12:area, 9:tulare, 6:which, 6:united


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Porterville} \colorbox{red!9}{\strut ,} \colorbox{red!83}{\strut California} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!9}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!9}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!100}{\strut Porterville} \colorbox{red!9}{\strut ,} \colorbox{red!83}{\strut California} \colorbox{red!5}{\strut Motto} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!5}{\strut Good} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut .} \colorbox{red!31}{\strut Location} \colorbox{red!3}{\strut in} \colorbox{red!17}{\strut Tulare} \colorbox{red!100}{\strut County} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut the} \colorbox{red!11}{\strut state} \colorbox{red!1}{\strut of} \colorbox{red!83}{\strut California} \colorbox{red!7}{\strut Coordinates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3647N} \colorbox{red!0}{\strut 119139W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 36.06861N} \colorbox{red!0}{\strut 119.0275W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 36.06861} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -119.0275} \colorbox{red!3}{\strut Country} \colorbox{red!11}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!11}{\strut State} \colorbox{red!83}{\strut California} \colorbox{red!100}{\strut County} \colorbox{red!17}{\strut Tulare} \colorbox{red!5}{\strut Settled} \colorbox{red!0}{\strut approx} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 1826} \colorbox{red!5}{\strut Incorperated} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 7} \colorbox{red!9}{\strut ,} \colorbox{red!0}{\strut 1902} \colorbox{red!5}{\strut Government} \colorbox{red!0}{\strut -Type} \colorbox{red!0}{\strut Council-Manager} \colorbox{red!0}{\strut -City} \colorbox{red!0}{\strut Manager} \colorbox{red!0}{\strut John} \colorbox{red!5}{\strut Longley} \colorbox{red!0}{\strut -Mayor} \colorbox{red!1}{\strut Cameron} \colorbox{red!0}{\strut J.} \colorbox{red!3}{\strut Hamilton} \colorbox{red!0}{\strut -Mayor} \colorbox{red!5}{\strut Pro} \colorbox{red!0}{\strut Tempore} \colorbox{red!0}{\strut Felipe} \colorbox{red!0}{\strut A.} \colorbox{red!5}{\strut Martinez} \colorbox{red!23}{\strut Area} \colorbox{red!0}{\strut -Total} \colorbox{red!0}{\strut 14.1sqmi} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 36.5km2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -Land} \colorbox{red!3}{\strut 14sqmi} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 36.3km2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut Water} \colorbox{red!0}{\strut 0.1sqmi} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 0.2km2} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Elevation} \colorbox{red!0}{\strut 456ft} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 139m} \colorbox{red!0}{\strut .} \colorbox{red!41}{\strut Population} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -Total} \colorbox{red!0}{\strut 39,615} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Density} \colorbox{red!0}{\strut 2,809.6sqmi} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 1,085.3km2} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Time} \colorbox{red!3}{\strut zone} \colorbox{red!3}{\strut Pacific} \colorbox{red!5}{\strut .} \colorbox{red!1}{\strut PST} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut UTC-8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -Summer} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut DST} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut PDT} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut UTC-7} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut ZIP} \colorbox{red!3}{\strut codes} \colorbox{red!0}{\strut 93257-93258} \colorbox{red!23}{\strut Area} \colorbox{red!0}{\strut code} \colorbox{red!5}{\strut .} \colorbox{red!3}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 559} \colorbox{red!3}{\strut FIPS} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut 06-58240} \colorbox{red!3}{\strut GNIS} \colorbox{red!3}{\strut feature} \colorbox{red!3}{\strut ID} \colorbox{red!1}{\strut 1652779} \colorbox{red!100}{\strut Porterville} \colorbox{red!5}{\strut is} \colorbox{red!5}{\strut a} \colorbox{red!29}{\strut city} \colorbox{red!3}{\strut in} \colorbox{red!17}{\strut Tulare} \colorbox{red!100}{\strut County} \colorbox{red!9}{\strut ,} \colorbox{red!83}{\strut California} \colorbox{red!9}{\strut ,} \colorbox{red!11}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!41}{\strut population} \colorbox{red!3}{\strut was} \colorbox{red!0}{\strut 39,615} \colorbox{red!3}{\strut at} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut 2000} \colorbox{red!9}{\strut census} \colorbox{red!3}{\strut .} \colorbox{red!29}{\strut City} \colorbox{red!3}{\strut limit} \colorbox{red!0}{\strut signs} \colorbox{red!1}{\strut currently} \colorbox{red!3}{\strut have} \colorbox{red!3}{\strut the} \colorbox{red!41}{\strut population} \colorbox{red!3}{\strut at} \colorbox{red!0}{\strut 51,467} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!29}{\strut city} \colorbox{red!0}{\strut s} \colorbox{red!41}{\strut population} \colorbox{red!0}{\strut grew} \colorbox{red!0}{\strut dramatically} \colorbox{red!0}{\strut as} \colorbox{red!3}{\strut the} \colorbox{red!29}{\strut city} \colorbox{red!0}{\strut annexed} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut properties} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut unincorporated} \colorbox{red!0}{\strut areas} \colorbox{red!3}{\strut in} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut around} \colorbox{red!100}{\strut Porterville} \colorbox{red!3}{\strut .} \colorbox{red!100}{\strut Porterville} \colorbox{red!5}{\strut is} \colorbox{red!3}{\strut considered} \colorbox{red!9}{\strut part} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!9}{\strut Census} \colorbox{red!1}{\strut Bureau} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut designation} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut Visalia-Porterville} \colorbox{red!5}{\strut metropolitan} \colorbox{red!7}{\strut statistical} \colorbox{red!23}{\strut area} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!3}{\strut 1} \colorbox{red!5}{\strut Geography} \colorbox{red!0}{\strut 2} \colorbox{red!5}{\strut Demographics} \colorbox{red!0}{\strut 3} \colorbox{red!1}{\strut Politics} \colorbox{red!0}{\strut 4} \colorbox{red!1}{\strut Local} \colorbox{red!3}{\strut Trivia} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Notable} \colorbox{red!0}{\strut locals} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut Media} \colorbox{red!0}{\strut 7} \colorbox{red!7}{\strut Education} \colorbox{red!0}{\strut 7.1} \colorbox{red!7}{\strut Schools} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!100}{\strut Porterville} \colorbox{red!11}{\strut Unified} \colorbox{red!0}{\strut School} \colorbox{red!7}{\strut District} \colorbox{red!0}{\strut 7.2} \colorbox{red!7}{\strut Schools} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!1}{\strut Burton} \colorbox{red!0}{\strut School} \colorbox{red!7}{\strut District} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut Higher} \colorbox{red!7}{\strut Education} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut Sister} \colorbox{red!0}{\strut cities} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Geography} \colorbox{red!100}{\strut Porterville} \colorbox{red!5}{\strut is} \colorbox{red!0}{\strut located} \colorbox{red!3}{\strut at} \colorbox{red!0}{\strut 3647N} \colorbox{red!0}{\strut 119139W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 36.06861N} \colorbox{red!0}{\strut 119.0275W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 36.06861} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -119.0275} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut 36.068550} \colorbox{red!9}{\strut ,} \colorbox{red!0}{\strut -119.027536} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut the} \colorbox{red!11}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!9}{\strut Census} \colorbox{red!1}{\strut Bureau} \colorbox{red!9}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!29}{\strut city} \colorbox{red!5}{\strut has} \colorbox{red!5}{\strut a} \colorbox{red!3}{\strut total} \colorbox{red!23}{\strut area} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut 14.1} \colorbox{red!5}{\strut square} 
}}}
\end{CJK*}

98:porterville, 96:college, 15:school, 14:update, 12:produced, 12:district, 12:california, 11:news, 10:pc, 10:kern


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!70}{\strut Porterville} \colorbox{red!69}{\strut College} \colorbox{red!3}{\strut With} \colorbox{red!5}{\strut students} \colorbox{red!4}{\strut as} \colorbox{red!0}{\strut our} \colorbox{red!5}{\strut focus} \colorbox{red!2}{\strut ,} \colorbox{red!7}{\strut PC} \colorbox{red!3}{\strut provides} \colorbox{red!1}{\strut an} \colorbox{red!2}{\strut excellent} \colorbox{red!7}{\strut educational} \colorbox{red!3}{\strut experience} \colorbox{red!0}{\strut ...} \colorbox{red!7}{\strut News} \colorbox{red!7}{\strut PC} \colorbox{red!4}{\strut Home} \colorbox{red!5}{\strut Office} \colorbox{red!3}{\strut of} \colorbox{red!5}{\strut Public} \colorbox{red!5}{\strut Information} \colorbox{red!3}{\strut Monte} \colorbox{red!4}{\strut Moore} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut Public} \colorbox{red!5}{\strut Information} \colorbox{red!0}{\strut Officer} \colorbox{red!70}{\strut PORTERVILLE} \colorbox{red!69}{\strut COLLEGE} \colorbox{red!4}{\strut 100} \colorbox{red!5}{\strut East} \colorbox{red!69}{\strut College} \colorbox{red!4}{\strut Avenue} \colorbox{red!70}{\strut Porterville} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut California} \colorbox{red!4}{\strut 93257} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut 559} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 791-2200} \colorbox{red!2}{\strut 2009} \colorbox{red!7}{\strut Issues} \colorbox{red!5}{\strut January} \colorbox{red!2}{\strut 2008} \colorbox{red!7}{\strut Issues} \colorbox{red!3}{\strut December} \colorbox{red!4}{\strut November} \colorbox{red!3}{\strut October} \colorbox{red!4}{\strut September} \colorbox{red!4}{\strut August} \colorbox{red!4}{\strut July} \colorbox{red!4}{\strut June} \colorbox{red!4}{\strut May} \colorbox{red!5}{\strut April} \colorbox{red!5}{\strut March} \colorbox{red!5}{\strut February} \colorbox{red!3}{\strut 2007} \colorbox{red!7}{\strut Issues} \colorbox{red!3}{\strut December} \colorbox{red!4}{\strut November} \colorbox{red!3}{\strut October} \colorbox{red!4}{\strut September} \colorbox{red!4}{\strut June} \colorbox{red!4}{\strut May} \colorbox{red!5}{\strut April} \colorbox{red!5}{\strut March} \colorbox{red!5}{\strut February} \colorbox{red!5}{\strut January} \colorbox{red!70}{\strut Porterville} \colorbox{red!69}{\strut College} \colorbox{red!7}{\strut News} \colorbox{red!2}{\strut The} \colorbox{red!7}{\strut PC} \colorbox{red!10}{\strut Update} \colorbox{red!2}{\strut is} \colorbox{red!8}{\strut produced} \colorbox{red!4}{\strut monthly} \colorbox{red!2}{\strut by} \colorbox{red!2}{\strut the} \colorbox{red!70}{\strut Porterville} \colorbox{red!69}{\strut College} \colorbox{red!5}{\strut Office} \colorbox{red!3}{\strut of} \colorbox{red!5}{\strut Public} \colorbox{red!5}{\strut Information} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!0}{\strut publication} \colorbox{red!2}{\strut is} \colorbox{red!4}{\strut distributed} \colorbox{red!4}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut Kern} \colorbox{red!5}{\strut Community} \colorbox{red!69}{\strut College} \colorbox{red!8}{\strut District} \colorbox{red!5}{\strut Board} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut Trustees} \colorbox{red!2}{\strut ,} \colorbox{red!70}{\strut Porterville} \colorbox{red!69}{\strut College} \colorbox{red!5}{\strut employees} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut retirees} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut local} \colorbox{red!10}{\strut school} \colorbox{red!5}{\strut administrators} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut counselors} \colorbox{red!2}{\strut ,} \colorbox{red!7}{\strut PC} \colorbox{red!5}{\strut Foundation} \colorbox{red!5}{\strut board} \colorbox{red!2}{\strut members} \colorbox{red!2}{\strut and} \colorbox{red!70}{\strut Porterville} \colorbox{red!2}{\strut Chamber} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut Commerce} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut Issues} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut available} \colorbox{red!3}{\strut for} \colorbox{red!3}{\strut viewing} \colorbox{red!2}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut web} \colorbox{red!2}{\strut using} \colorbox{red!3}{\strut Acrobat} \colorbox{red!4}{\strut reader} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut Get} \colorbox{red!2}{\strut Adobe} \colorbox{red!4}{\strut Reader} \colorbox{red!3}{\strut copyright} \colorbox{red!3}{\strut 2007} \colorbox{red!70}{\strut Porterville} \colorbox{red!69}{\strut College} 
}}}
\end{CJK*}

query: rock art

99:art, 98:rock, 31:artist, 28:paintings, 16:stone, 16:craft, 15:critters, 14:pond, 14:form, 14:dogs


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Rock} \colorbox{red!100}{\strut Art} \colorbox{red!7}{\strut By} \colorbox{red!14}{\strut Julie} \colorbox{red!14}{\strut Home} \colorbox{red!17}{\strut Pet} \colorbox{red!15}{\strut Portraits} \colorbox{red!10}{\strut Seasonal} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Winter} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut Leaf} \colorbox{red!36}{\strut Paintings} \colorbox{red!18}{\strut Pond} \colorbox{red!0}{\strut rocks} \colorbox{red!1}{\strut and} \colorbox{red!14}{\strut fishy} \colorbox{red!11}{\strut things} \colorbox{red!10}{\strut Houses} \colorbox{red!6}{\strut ,} \colorbox{red!9}{\strut Huts} \colorbox{red!6}{\strut ,} \colorbox{red!7}{\strut buildings} \colorbox{red!15}{\strut Garden} \colorbox{red!0}{\strut Rocks} \colorbox{red!6}{\strut Artic} \colorbox{red!19}{\strut Critters} \colorbox{red!14}{\strut Fantasy} \colorbox{red!10}{\strut Wild} \colorbox{red!9}{\strut Life} \colorbox{red!14}{\strut Cats} \colorbox{red!18}{\strut Dogs} \colorbox{red!0}{\strut Rocks} \colorbox{red!14}{\strut Sold} \colorbox{red!10}{\strut Gallery} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Favorite} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Add} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Link} \colorbox{red!3}{\strut Welcome} \colorbox{red!5}{\strut My} \colorbox{red!9}{\strut current} \colorbox{red!6}{\strut ebay} \colorbox{red!11}{\strut auctions} \colorbox{red!1}{\strut Hello} \colorbox{red!10}{\strut .} \colorbox{red!3}{\strut Welcome} \colorbox{red!3}{\strut to} \colorbox{red!5}{\strut my} \colorbox{red!100}{\strut rock} \colorbox{red!100}{\strut art} \colorbox{red!10}{\strut site} \colorbox{red!10}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!7}{\strut of} \colorbox{red!5}{\strut my} \colorbox{red!100}{\strut art} \colorbox{red!6}{\strut is} \colorbox{red!6}{\strut for} \colorbox{red!0}{\strut sale.You} \colorbox{red!3}{\strut will} \colorbox{red!3}{\strut note} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut callit} \colorbox{red!100}{\strut Rock} \colorbox{red!100}{\strut Art} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut not} \colorbox{red!100}{\strut rock} \colorbox{red!0}{\strut craft.Rock} \colorbox{red!100}{\strut art} \colorbox{red!6}{\strut is} \colorbox{red!7}{\strut a} \colorbox{red!18}{\strut form} \colorbox{red!7}{\strut of} \colorbox{red!100}{\strut art} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut believe} \colorbox{red!0}{\strut it} \colorbox{red!6}{\strut is} \colorbox{red!7}{\strut a} \colorbox{red!20}{\strut craft} \colorbox{red!0}{\strut becausewe} \colorbox{red!3}{\strut use} \colorbox{red!7}{\strut a} \colorbox{red!14}{\strut meer} \colorbox{red!20}{\strut stone} \colorbox{red!3}{\strut or} \colorbox{red!100}{\strut rock} \colorbox{red!0}{\strut instead} \colorbox{red!0}{\strut ofstore} \colorbox{red!13}{\strut bought} \colorbox{red!11}{\strut canvas} \colorbox{red!10}{\strut .} \colorbox{red!100}{\strut Rock} \colorbox{red!40}{\strut Artist} \colorbox{red!15}{\strut put} \colorbox{red!0}{\strut lots} \colorbox{red!0}{\strut oftime} \colorbox{red!0}{\strut andskill} \colorbox{red!7}{\strut into} \colorbox{red!0}{\strut each} \colorbox{red!7}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!13}{\strut pieces} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut paint.The} \colorbox{red!13}{\strut pieces} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!10}{\strut site} \colorbox{red!3}{\strut are} \colorbox{red!10}{\strut priced} \colorbox{red!1}{\strut as} \colorbox{red!100}{\strut Art} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut as} \colorbox{red!0}{\strut crafts} \colorbox{red!10}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!3}{\strut you} \colorbox{red!3}{\strut are} \colorbox{red!5}{\strut interested} \colorbox{red!2}{\strut in} \colorbox{red!7}{\strut buying} \colorbox{red!0}{\strut apiece} \colorbox{red!7}{\strut of} \colorbox{red!100}{\strut art} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut will} \colorbox{red!0}{\strut bring} \colorbox{red!3}{\strut you} \colorbox{red!3}{\strut many} \colorbox{red!5}{\strut years} \colorbox{red!7}{\strut of} \colorbox{red!3}{\strut enjoyment} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut feel} \colorbox{red!0}{\strut free} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut browse} \colorbox{red!5}{\strut threw} \colorbox{red!5}{\strut my} \colorbox{red!0}{\strut pages.Each} \colorbox{red!0}{\strut piece} \colorbox{red!6}{\strut is} \colorbox{red!7}{\strut a} \colorbox{red!0}{\strut one} \colorbox{red!7}{\strut of} \colorbox{red!7}{\strut a} \colorbox{red!1}{\strut kind} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!3}{\strut are} \colorbox{red!3}{\strut no} \colorbox{red!13}{\strut two} \colorbox{red!0}{\strut rocks} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut are} \colorbox{red!2}{\strut the} \colorbox{red!1}{\strut same} \colorbox{red!3}{\strut although} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut may} \colorbox{red!9}{\strut look} \colorbox{red!5}{\strut simular} \colorbox{red!10}{\strut .} 
}}}
\end{CJK*}

99:rock, 98:roll, 30:degrees, 19:university, 19:arts, 16:digital, 14:fashion, 14:cola, 11:rockstars, 10:coca


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut I} \colorbox{red!8}{\strut was} \colorbox{red!6}{\strut drinking} \colorbox{red!9}{\strut Coca} \colorbox{red!13}{\strut Cola} \colorbox{red!5}{\strut young} \colorbox{red!8}{\strut hip} \colorbox{red!10}{\strut rockstars} \colorbox{red!13}{\strut fashion} \colorbox{red!5}{\strut New} \colorbox{red!5}{\strut York} \colorbox{red!9}{\strut City} \colorbox{red!8}{\strut Manhattan} \colorbox{red!2}{\strut .} \colorbox{red!97}{\strut Rock} \colorbox{red!4}{\strut n} \colorbox{red!96}{\strut Roll} \colorbox{red!9}{\strut Coca} \colorbox{red!13}{\strut Cola} \colorbox{red!1}{\strut on} \colorbox{red!4}{\strut Apple} \colorbox{red!6}{\strut COmputers} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut iPOd} \colorbox{red!6}{\strut gave} \colorbox{red!3}{\strut soft} \colorbox{red!0}{\strut drink} \colorbox{red!4}{\strut games} \colorbox{red!3}{\strut Ideas} \colorbox{red!2}{\strut Telcel} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut SIEMENS} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut gave} \colorbox{red!0}{\strut some} \colorbox{red!9}{\strut coca} \colorbox{red!13}{\strut cola} \colorbox{red!3}{\strut cool} \colorbox{red!8}{\strut kids} \colorbox{red!8}{\strut make} \colorbox{red!3}{\strut friends} \colorbox{red!5}{\strut online} \colorbox{red!2}{\strut .} \colorbox{red!18}{\strut University} \colorbox{red!15}{\strut Digital} \colorbox{red!29}{\strut degrees} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!13}{\strut Fashion} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!15}{\strut digital} \colorbox{red!18}{\strut arts} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} \colorbox{red!5}{\strut and} \colorbox{red!96}{\strut roll} \colorbox{red!3}{\strut ,} \colorbox{red!97}{\strut rock} 
}}}
\end{CJK*}

query: unc

101:unc, 43:uncg, 29:unct, 29:system, 27:students, 23:today, 21:carolina, 20:tomorrow, 20:north, 17:enrollment


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Skip} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut Main} \colorbox{red!0}{\strut Content} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut PROSPECTIVE} \colorbox{red!31}{\strut STUDENTS} \colorbox{red!6}{\strut CURRENT} \colorbox{red!31}{\strut STUDENTS} \colorbox{red!10}{\strut FACULTY} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut STAFF} \colorbox{red!3}{\strut ALUMNI} \colorbox{red!3}{\strut COMMUNITY} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FRIENDS} \colorbox{red!0}{\strut Search} \colorbox{red!50}{\strut UNCG} \colorbox{red!17}{\strut UNCGENIE} \colorbox{red!0}{\strut SITE} \colorbox{red!0}{\strut TOOLS} \colorbox{red!13}{\strut CAMPUS} \colorbox{red!0}{\strut LINKS} \colorbox{red!1}{\strut Inside} \colorbox{red!50}{\strut UNCG} \colorbox{red!9}{\strut Admissions} \colorbox{red!4}{\strut Academics} \colorbox{red!0}{\strut Libraries} \colorbox{red!9}{\strut Administration} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Centers} \colorbox{red!3}{\strut International} \colorbox{red!18}{\strut Programs} \colorbox{red!0}{\strut Continuing} \colorbox{red!8}{\strut Education} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Outreach} \colorbox{red!0}{\strut Technology} \colorbox{red!0}{\strut Arts} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Entertainment} \colorbox{red!2}{\strut Employment} \colorbox{red!4}{\strut Corporate} \colorbox{red!0}{\strut Resources} \colorbox{red!3}{\strut Giving} \colorbox{red!2}{\strut to} \colorbox{red!50}{\strut UNCG} \colorbox{red!50}{\strut UNCG} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!8}{\strut Home} \colorbox{red!100}{\strut UNC} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!9}{\strut Summary} \colorbox{red!50}{\strut UNCG} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!13}{\strut Strategic} \colorbox{red!13}{\strut Planning} \colorbox{red!2}{\strut Committee} \colorbox{red!33}{\strut UNCT} \colorbox{red!11}{\strut Phase} \colorbox{red!10}{\strut II} \colorbox{red!15}{\strut Response} \colorbox{red!1}{\strut Template} \colorbox{red!2}{\strut A} \colorbox{red!3}{\strut Bridge} \colorbox{red!0}{\strut between} \colorbox{red!50}{\strut UNCG} \colorbox{red!26}{\strut Today} \colorbox{red!4}{\strut and} \colorbox{red!50}{\strut UNCG} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!100}{\strut UNC} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!15}{\strut Response} \colorbox{red!11}{\strut Phase} \colorbox{red!4}{\strut I} \colorbox{red!2}{\strut Strengthening} \colorbox{red!50}{\strut UNCG} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!8}{\strut Proposed} \colorbox{red!3}{\strut Major} \colorbox{red!0}{\strut Initiatves} \colorbox{red!13}{\strut Planning} \colorbox{red!3}{\strut Preparation} \colorbox{red!2}{\strut Committee} \colorbox{red!100}{\strut UNC} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!10}{\strut Commission} \colorbox{red!100}{\strut UNC} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!9}{\strut Summary} \colorbox{red!3}{\strut Final} \colorbox{red!3}{\strut Report} \colorbox{red!2}{\strut Contact} \colorbox{red!4}{\strut Us} \colorbox{red!100}{\strut UNC} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!9}{\strut Summary} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut http} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut www.nctomorrow.org} \colorbox{red!5}{\strut for} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut detailed} \colorbox{red!0}{\strut information} \colorbox{red!5}{\strut .} \colorbox{red!23}{\strut North} \colorbox{red!24}{\strut Carolina} \colorbox{red!10}{\strut is} \colorbox{red!10}{\strut undergoing} \colorbox{red!1}{\strut several} \colorbox{red!10}{\strut economic} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut demographic} \colorbox{red!12}{\strut changes} \colorbox{red!3}{\strut .} \colorbox{red!26}{\strut Today} \colorbox{red!0}{\strut ,} \colorbox{red!100}{\strut UNC} \colorbox{red!33}{\strut system} \colorbox{red!19}{\strut enrollment} \colorbox{red!10}{\strut is} \colorbox{red!0}{\strut 200,000} \colorbox{red!31}{\strut students} \colorbox{red!4}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!100}{\strut UNC} \colorbox{red!33}{\strut system} \colorbox{red!9}{\strut projections} \colorbox{red!5}{\strut for} \colorbox{red!3}{\strut 2017} \colorbox{red!0}{\strut are} \colorbox{red!5}{\strut for} \colorbox{red!0}{\strut 280,000} \colorbox{red!31}{\strut students} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut By} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!10}{\strut state} \colorbox{red!1}{\strut of} \colorbox{red!23}{\strut North} \colorbox{red!24}{\strut Carolina} \colorbox{red!6}{\strut will} \colorbox{red!6}{\strut need} \colorbox{red!0}{\strut 400,000} \colorbox{red!11}{\strut new} \colorbox{red!3}{\strut workers} \colorbox{red!4}{\strut .} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut The} \colorbox{red!100}{\strut UNC} \colorbox{red!33}{\strut system} \colorbox{red!1}{\strut generates} \colorbox{red!0}{\strut 50,000} \colorbox{red!6}{\strut jobs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1.5} \colorbox{red!1}{\strut billion} \colorbox{red!5}{\strut payroll} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut 1} \colorbox{red!1}{\strut billion} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut grants} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut contracts} \colorbox{red!0}{\strut each} \colorbox{red!4}{\strut year} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!100}{\strut UNC} \colorbox{red!23}{\strut Tomorrow} \colorbox{red!4}{\strut .} \colorbox{red!33}{\strut UNCT} \colorbox{red!5}{\strut .} \colorbox{red!9}{\strut initiative} \colorbox{red!10}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut effort} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut meet} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut needs} \colorbox{red!1}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!23}{\strut North} \colorbox{red!24}{\strut Carolina} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut 20-year} \colorbox{red!13}{\strut strategic} \colorbox{red!0}{\strut plan} \colorbox{red!5}{\strut for} \colorbox{red!4}{\strut the} \colorbox{red!100}{\strut UNC} \colorbox{red!33}{\strut system} \colorbox{red!2}{\strut was} \colorbox{red!6}{\strut developed} \colorbox{red!4}{\strut as} \colorbox{red!4}{\strut follows} \colorbox{red!3}{\strut .} \colorbox{red!13}{\strut Campus} \colorbox{red!5}{\strut Visits} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Spring} \colorbox{red!4}{\strut 2007} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Community} \colorbox{red!3}{\strut Listening} \colorbox{red!3}{\strut Forums} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut early} \colorbox{red!4}{\strut Fall} \colorbox{red!4}{\strut 2007} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut Faculty} \colorbox{red!3}{\strut Listening} \colorbox{red!3}{\strut Forums} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut late} \colorbox{red!4}{\strut Fall} \colorbox{red!4}{\strut 2007} \colorbox{red!0}{\strut ,} \colorbox{red!33}{\strut UNCT} \colorbox{red!5}{\strut Scholars} \colorbox{red!3}{\strut Council} \colorbox{red!4}{\strut and} \colorbox{red!100}{\strut UNC} \colorbox{red!0}{\strut General} \colorbox{red!9}{\strut Administration} \colorbox{red!33}{\strut UNCT} \colorbox{red!3}{\strut Report} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut late} \colorbox{red!4}{\strut Fall} \colorbox{red!4}{\strut 2007} \colorbox{red!0}{\strut ,} \colorbox{red!33}{\strut UNCT} \colorbox{red!10}{\strut Commission} \colorbox{red!4}{\strut unanimous} \colorbox{red!3}{\strut vote} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut support} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut December} \colorbox{red!4}{\strut 2007} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!100}{\strut UNC} \colorbox{red!2}{\strut Board} \colorbox{red!1}{\strut of} \colorbox{red!6}{\strut Governors} \colorbox{red!4}{\strut unanimous} \colorbox{red!3}{\strut vote} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut support} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut January} \colorbox{red!2}{\strut 2008} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Each} \colorbox{red!13}{\strut campus} \colorbox{red!10}{\strut is} \colorbox{red!2}{\strut charged} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut provide} \colorbox{red!2}{\strut a} \colorbox{red!33}{\strut UNCT} \colorbox{red!15}{\strut Response} \colorbox{red!0}{\strut Plan} \colorbox{red!11}{\strut Phase} \colorbox{red!4}{\strut I} \colorbox{red!3}{\strut by} \colorbox{red!3}{\strut May} \colorbox{red!2}{\strut 1} \colorbox{red!4}{\strut and} \colorbox{red!2}{\strut a} \colorbox{red!15}{\strut Response} \colorbox{red!0}{\strut Plan} \colorbox{red!11}{\strut Phase} \colorbox{red!10}{\strut II} \colorbox{red!3}{\strut by} \colorbox{red!2}{\strut December} \colorbox{red!2}{\strut 1} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut During} \colorbox{red!11}{\strut Phase} \colorbox{red!4}{\strut I} \colorbox{red!0}{\strut each} 
}}}
\end{CJK*}

100:unc, 92:tickets, 90:basketball, 38:what, 29:find, 23:team, 23:buy, 21:who, 19:seats, 18:game


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Home} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!55}{\strut UNC} \colorbox{red!9}{\strut schedule} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!55}{\strut UNC} \colorbox{red!8}{\strut mens} \colorbox{red!49}{\strut basketball} \colorbox{red!3}{\strut Need} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut Basketball} \colorbox{red!50}{\strut tickets} \colorbox{red!2}{\strut ?} \colorbox{red!2}{\strut Hi} \colorbox{red!0}{\strut there} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut thanks} \colorbox{red!1}{\strut for} \colorbox{red!4}{\strut visiting} \colorbox{red!0}{\strut my} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!3}{\strut site} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!6}{\strut Tarheels} \colorbox{red!1}{\strut are} \colorbox{red!7}{\strut set} \colorbox{red!3}{\strut to} \colorbox{red!1}{\strut have} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut monster} \colorbox{red!1}{\strut year} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut i} \colorbox{red!0}{\strut decided} \colorbox{red!3}{\strut to} \colorbox{red!7}{\strut set} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut site} \colorbox{red!3}{\strut to} \colorbox{red!4}{\strut help} \colorbox{red!3}{\strut visitors} \colorbox{red!15}{\strut find} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut best} \colorbox{red!4}{\strut deals} \colorbox{red!2}{\strut on} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut With} \colorbox{red!1}{\strut a} \colorbox{red!12}{\strut team} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut talented} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut one} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut its} \colorbox{red!0}{\strut gon} \colorbox{red!0}{\strut na} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut great} \colorbox{red!1}{\strut year} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut at} \colorbox{red!1}{\strut a} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!9}{\strut game} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Finding} \colorbox{red!50}{\strut tickets} \colorbox{red!3}{\strut to} \colorbox{red!55}{\strut UNC} \colorbox{red!6}{\strut Tarheels} \colorbox{red!0}{\strut games} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut not} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut mention} \colorbox{red!6}{\strut cheap} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut bit} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut challenge} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut have} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut best} \colorbox{red!3}{\strut site} \colorbox{red!3}{\strut to} \colorbox{red!15}{\strut find} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!50}{\strut tickets} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Ticket} \colorbox{red!4}{\strut Liquidator} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut They} \colorbox{red!1}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut extensive} \colorbox{red!0}{\strut collection} \colorbox{red!1}{\strut of} \colorbox{red!55}{\strut UNC} \colorbox{red!10}{\strut seats} \colorbox{red!0}{\strut that} \colorbox{red!4}{\strut come} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut brokers} \colorbox{red!11}{\strut who} \colorbox{red!3}{\strut make} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut living} \colorbox{red!0}{\strut wheeling} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dealing} \colorbox{red!1}{\strut in} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!50}{\strut tickets} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Sometimes} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut might} \colorbox{red!1}{\strut have} \colorbox{red!3}{\strut to} \colorbox{red!4}{\strut pay} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut bit} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut face-value} \colorbox{red!1}{\strut for} \colorbox{red!7}{\strut good} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut see} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut team} \colorbox{red!4}{\strut take} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut court} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut be} \colorbox{red!6}{\strut worth} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!1}{\strut are} \colorbox{red!0}{\strut all} \colorbox{red!7}{\strut set} \colorbox{red!1}{\strut for} \colorbox{red!20}{\strut what} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut one} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut biggest} \colorbox{red!0}{\strut years} \colorbox{red!1}{\strut in} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!6}{\strut history} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut loving} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut this} \colorbox{red!12}{\strut team} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cant} \colorbox{red!2}{\strut wait} \colorbox{red!1}{\strut for} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!3}{\strut to} \colorbox{red!3}{\strut go} \colorbox{red!0}{\strut all} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut way} \colorbox{red!2}{\strut baby} \colorbox{red!1}{\strut !} \colorbox{red!0}{\strut Sure} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut watching} \colorbox{red!0}{\strut them} \colorbox{red!2}{\strut on} \colorbox{red!2}{\strut TV} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut great} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut all} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut cant} \colorbox{red!2}{\strut beat} \colorbox{red!1}{\strut a} \colorbox{red!7}{\strut set} \colorbox{red!1}{\strut of} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut see} \colorbox{red!6}{\strut Tarheels} \colorbox{red!49}{\strut basketball} \colorbox{red!3}{\strut live} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut person} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Ed} \colorbox{red!1}{\strut Cota} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut alltime} \colorbox{red!2}{\strut assist} \colorbox{red!0}{\strut leader} \colorbox{red!2}{\strut at} \colorbox{red!55}{\strut UNC} \colorbox{red!12}{\strut Buy} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!50}{\strut TICKETS} \colorbox{red!0}{\strut Recent} \colorbox{red!1}{\strut Posts} \colorbox{red!1}{\strut 2008} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut 2009} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut Basketball} \colorbox{red!6}{\strut season} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!2}{\strut launches} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut Tickets} \colorbox{red!1}{\strut With} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut incredible} \colorbox{red!12}{\strut team} \colorbox{red!55}{\strut UNC} \colorbox{red!49}{\strut basketball} \colorbox{red!1}{\strut has} \colorbox{red!3}{\strut put} \colorbox{red!1}{\strut together} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut year} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!3}{\strut bet} \colorbox{red!0}{\strut that} \colorbox{red!55}{\strut UNC} \colorbox{red!50}{\strut tickets} \colorbox{red!1}{\strut are} \colorbox{red!0}{\strut going} \colorbox{red!3}{\strut fast} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Luckily} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut know} \colorbox{red!8}{\strut where} \colorbox{red!3}{\strut to} \colorbox{red!2}{\strut look} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!15}{\strut find} \colorbox{red!0}{\strut some} 
}}}
\end{CJK*}

query: gs pay rate

99:pay, 94:locality, 64:gs, 36:rate, 30:government, 22:federal, 21:wage, 19:employees, 17:table, 17:schedule


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!22}{\strut Federal} \colorbox{red!10}{\strut Jobs} \colorbox{red!13}{\strut Net} \colorbox{red!66}{\strut GS} \colorbox{red!100}{\strut Pay} \colorbox{red!3}{\strut Scales} \colorbox{red!3}{\strut Home} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut About} \colorbox{red!4}{\strut Us} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Site} \colorbox{red!4}{\strut Map} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Feedback} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Search} \colorbox{red!0}{\strut U.S.} \colorbox{red!3}{\strut Office} \colorbox{red!5}{\strut of} \colorbox{red!6}{\strut Personnel} \colorbox{red!5}{\strut Management} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut Official} \colorbox{red!100}{\strut Pay} \colorbox{red!6}{\strut Chart} \colorbox{red!5}{\strut 2009} \colorbox{red!16}{\strut General} \colorbox{red!17}{\strut Schedule} \colorbox{red!3}{\strut INCORPORATING} \colorbox{red!3}{\strut A} \colorbox{red!0}{\strut 2.9} \colorbox{red!3}{\strut .} \colorbox{red!16}{\strut GENERAL} \colorbox{red!6}{\strut INCREASE} \colorbox{red!3}{\strut Effective} \colorbox{red!3}{\strut January} \colorbox{red!5}{\strut 2009} \colorbox{red!8}{\strut BASE} \colorbox{red!37}{\strut RATE} \colorbox{red!17}{\strut TABLE} \colorbox{red!2}{\strut Use} \colorbox{red!4}{\strut for} \colorbox{red!2}{\strut reference} \colorbox{red!1}{\strut only} \colorbox{red!5}{\strut .} \colorbox{red!3}{\strut All} \colorbox{red!16}{\strut General} \colorbox{red!17}{\strut Schedule} \colorbox{red!5}{\strut .} \colorbox{red!66}{\strut GS} \colorbox{red!2}{\strut .} \colorbox{red!31}{\strut government} \colorbox{red!19}{\strut employees} \colorbox{red!4}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!16}{\strut make} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut base} \colorbox{red!37}{\strut rate} \colorbox{red!100}{\strut pay} \colorbox{red!2}{\strut with} \colorbox{red!97}{\strut locality} \colorbox{red!5}{\strut .} \colorbox{red!97}{\strut Locality} \colorbox{red!100}{\strut pay} \colorbox{red!0}{\strut rates} \colorbox{red!4}{\strut for} \colorbox{red!3}{\strut all} \colorbox{red!14}{\strut areas} \colorbox{red!3}{\strut are} \colorbox{red!6}{\strut listed} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut this} \colorbox{red!4}{\strut site} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut For} \colorbox{red!0}{\strut those} \colorbox{red!1}{\strut not} \colorbox{red!4}{\strut in} \colorbox{red!3}{\strut a} \colorbox{red!4}{\strut specific} \colorbox{red!97}{\strut locality} \colorbox{red!0}{\strut area} \colorbox{red!2}{\strut use} \colorbox{red!3}{\strut the} \colorbox{red!17}{\strut table} \colorbox{red!3}{\strut titled} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Rest} \colorbox{red!5}{\strut of} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Pay} \colorbox{red!7}{\strut varies} \colorbox{red!3}{\strut per} \colorbox{red!97}{\strut locality} \colorbox{red!0}{\strut area} \colorbox{red!5}{\strut .} \colorbox{red!3}{\strut Look} \colorbox{red!3}{\strut up} \colorbox{red!3}{\strut the} \colorbox{red!97}{\strut locality} \colorbox{red!0}{\strut tables} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!9}{\strut metropolitan} \colorbox{red!0}{\strut area} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut determine} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut actual} \colorbox{red!14}{\strut salary} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut area} \colorbox{red!5}{\strut .} \colorbox{red!21}{\strut Wage} \colorbox{red!37}{\strut rate} \colorbox{red!0}{\strut tables} \colorbox{red!4}{\strut for} \colorbox{red!3}{\strut all} \colorbox{red!6}{\strut major} \colorbox{red!9}{\strut metropolitan} \colorbox{red!14}{\strut areas} \colorbox{red!3}{\strut are} \colorbox{red!7}{\strut located} \colorbox{red!3}{\strut at} \colorbox{red!3}{\strut http} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut www.cpms.osd.milwage} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut For} \colorbox{red!0}{\strut comparison} \colorbox{red!0}{\strut purposes} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut current} \colorbox{red!2}{\strut and} \colorbox{red!5}{\strut past} \colorbox{red!0}{\strut three} \colorbox{red!4}{\strut years} \colorbox{red!97}{\strut locality} \colorbox{red!0}{\strut tables} \colorbox{red!3}{\strut are} \colorbox{red!3}{\strut available} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!5}{\strut review} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut 2009} \colorbox{red!97}{\strut locality} \colorbox{red!100}{\strut pay} \colorbox{red!0}{\strut rates} \colorbox{red!6}{\strut 2008} \colorbox{red!97}{\strut locality} \colorbox{red!100}{\strut pay} \colorbox{red!0}{\strut rates} \colorbox{red!4}{\strut 2007} \colorbox{red!97}{\strut locality} \colorbox{red!100}{\strut pay} \colorbox{red!0}{\strut rates} \colorbox{red!4}{\strut 2006} \colorbox{red!97}{\strut locality} \colorbox{red!100}{\strut pay} \colorbox{red!0}{\strut rates} \colorbox{red!4}{\strut 2005} \colorbox{red!97}{\strut locality} \colorbox{red!100}{\strut pay} \colorbox{red!0}{\strut rates} \colorbox{red!3}{\strut Are} \colorbox{red!3}{\strut you} \colorbox{red!3}{\strut interested} \colorbox{red!4}{\strut in} \colorbox{red!3}{\strut upward} \colorbox{red!4}{\strut mobility} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut promotions} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Visit} \colorbox{red!0}{\strut our} \colorbox{red!22}{\strut Federal} \colorbox{red!4}{\strut Career} \colorbox{red!4}{\strut Planning} \colorbox{red!0}{\strut web} \colorbox{red!4}{\strut site} \colorbox{red!5}{\strut .} \colorbox{red!2}{\strut This} \colorbox{red!4}{\strut site} \colorbox{red!4}{\strut assists} \colorbox{red!22}{\strut federal} \colorbox{red!31}{\strut government} \colorbox{red!19}{\strut employees} \colorbox{red!2}{\strut to} \colorbox{red!4}{\strut design} \colorbox{red!3}{\strut realistic} \colorbox{red!3}{\strut Individual} \colorbox{red!3}{\strut Development} \colorbox{red!0}{\strut Plans} \colorbox{red!5}{\strut .} \colorbox{red!3}{\strut IDPs} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut target} \colorbox{red!4}{\strut new} \colorbox{red!10}{\strut jobs} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut promotions} \colorbox{red!4}{\strut in} \colorbox{red!31}{\strut government} \colorbox{red!5}{\strut .} \colorbox{red!22}{\strut Federal} \colorbox{red!31}{\strut government} \colorbox{red!19}{\strut employees} \colorbox{red!3}{\strut have} \colorbox{red!2}{\strut numerous} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut attractive} \colorbox{red!4}{\strut career} \colorbox{red!3}{\strut development} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut upward} \colorbox{red!4}{\strut mobility} \colorbox{red!2}{\strut opportunities} \colorbox{red!3}{\strut available} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut them} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Developed} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut a} \colorbox{red!4}{\strut career} \colorbox{red!3}{\strut fed} \colorbox{red!2}{\strut with} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 35} \colorbox{red!4}{\strut years} \colorbox{red!22}{\strut federal} \colorbox{red!6}{\strut service} \colorbox{red!5}{\strut .} \colorbox{red!8}{\strut Annual} \colorbox{red!0}{\strut Rates} \colorbox{red!0}{\strut by} \colorbox{red!5}{\strut Grade} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut Step} \colorbox{red!5}{\strut Grade} \colorbox{red!3}{\strut Step} \colorbox{red!4}{\strut 1} \colorbox{red!3}{\strut Step} \colorbox{red!4}{\strut 2} \colorbox{red!3}{\strut Step} \colorbox{red!2}{\strut 3} \colorbox{red!3}{\strut Step} \colorbox{red!2}{\strut 4} \colorbox{red!3}{\strut Step} \colorbox{red!4}{\strut 5} \colorbox{red!3}{\strut Step} \colorbox{red!1}{\strut 6} \colorbox{red!3}{\strut Step} \colorbox{red!4}{\strut 7} \colorbox{red!3}{\strut Step} \colorbox{red!4}{\strut 8} \colorbox{red!3}{\strut Step} \colorbox{red!2}{\strut 9} \colorbox{red!3}{\strut Step} \colorbox{red!3}{\strut 10} \colorbox{red!0}{\strut WITHIN} \colorbox{red!5}{\strut GRADE} \colorbox{red!7}{\strut AMOUNTS} \colorbox{red!4}{\strut 1} \colorbox{red!0}{\strut 17540} \colorbox{red!1}{\strut 18126} \colorbox{red!0}{\strut 18709} \colorbox{red!0}{\strut 19290} \colorbox{red!0}{\strut 19873} \colorbox{red!1}{\strut 20216} \colorbox{red!0}{\strut 20792} \colorbox{red!0}{\strut 21373} \colorbox{red!0}{\strut 21396} \colorbox{red!1}{\strut 21944} \colorbox{red!7}{\strut VARIES} \colorbox{red!4}{\strut 2} \colorbox{red!0}{\strut 19721} \colorbox{red!2}{\strut 20190} \colorbox{red!0}{\strut 20842} \colorbox{red!0}{\strut 21396} \colorbox{red!1}{\strut 21635} \colorbox{red!1}{\strut 22271} \colorbox{red!0}{\strut 22907} \colorbox{red!0}{\strut 23543} \colorbox{red!0}{\strut 24179} \colorbox{red!0}{\strut 24815} \colorbox{red!7}{\strut VARIES} \colorbox{red!2}{\strut 3} \colorbox{red!1}{\strut 21517} 
}}}
\end{CJK*}

50:rate, 41:pay, 41:gs, 33:set, 32:locality, 31:employees, 30:fws, 29:wage, 29:range, 27:retention


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut skip} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut OPM.gov} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Subject} \colorbox{red!2}{\strut Index} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Important} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut U.S.} \colorbox{red!2}{\strut Office} \colorbox{red!1}{\strut of} \colorbox{red!6}{\strut Personnel} \colorbox{red!4}{\strut Management} \colorbox{red!1}{\strut -} \colorbox{red!1}{\strut Ensuring} \colorbox{red!1}{\strut the} \colorbox{red!7}{\strut Federal} \colorbox{red!2}{\strut Government} \colorbox{red!1}{\strut has} \colorbox{red!1}{\strut an} \colorbox{red!4}{\strut effective} \colorbox{red!1}{\strut civilian} \colorbox{red!2}{\strut workforce} \colorbox{red!3}{\strut Advanced} \colorbox{red!0}{\strut Search} \colorbox{red!3}{\strut Alert} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut Paysetting} \colorbox{red!1}{\strut for} \colorbox{red!7}{\strut Federal} \colorbox{red!11}{\strut Wage} \colorbox{red!9}{\strut System} \colorbox{red!1}{\strut to} \colorbox{red!7}{\strut General} \colorbox{red!8}{\strut Schedule} \colorbox{red!3}{\strut Movements} \colorbox{red!1}{\strut This} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut reminder} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut Office} \colorbox{red!1}{\strut of} \colorbox{red!6}{\strut Personnel} \colorbox{red!4}{\strut Management} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut OPM} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut issued} \colorbox{red!1}{\strut interim} \colorbox{red!5}{\strut regulations} \colorbox{red!1}{\strut on} \colorbox{red!1}{\strut May} \colorbox{red!1}{\strut 31} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut 2005} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut changed} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut way} \colorbox{red!16}{\strut pay} \colorbox{red!1}{\strut is} \colorbox{red!12}{\strut set} \colorbox{red!1}{\strut for} \colorbox{red!7}{\strut Federal} \colorbox{red!11}{\strut Wage} \colorbox{red!9}{\strut System} \colorbox{red!1}{\strut .} \colorbox{red!11}{\strut FWS} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut other} \colorbox{red!0}{\strut non-General} \colorbox{red!8}{\strut Schedule} \colorbox{red!1}{\strut .} \colorbox{red!16}{\strut GS} \colorbox{red!1}{\strut .} \colorbox{red!12}{\strut employees} \colorbox{red!1}{\strut upon} \colorbox{red!0}{\strut movement} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut a} \colorbox{red!16}{\strut GS} \colorbox{red!6}{\strut position} \colorbox{red!1}{\strut using} \colorbox{red!1}{\strut the} \colorbox{red!10}{\strut maximum} \colorbox{red!10}{\strut payable} \colorbox{red!19}{\strut rate} \colorbox{red!9}{\strut rule} \colorbox{red!1}{\strut at} \colorbox{red!1}{\strut 5} \colorbox{red!3}{\strut CFR} \colorbox{red!0}{\strut 531.221-223} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut the} \colorbox{red!16}{\strut pay} \colorbox{red!10}{\strut retention} \colorbox{red!0}{\strut rules} \colorbox{red!2}{\strut under} \colorbox{red!1}{\strut 5} \colorbox{red!3}{\strut CFR} \colorbox{red!1}{\strut part} \colorbox{red!1}{\strut 536} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut subpart} \colorbox{red!0}{\strut C.} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!4}{\strut CPM} \colorbox{red!0}{\strut 2005-10} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!0}{\strut rules} \colorbox{red!0}{\strut became} \colorbox{red!4}{\strut effective} \colorbox{red!1}{\strut on} \colorbox{red!1}{\strut May} \colorbox{red!0}{\strut 1} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut 2005} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Under} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut former} \colorbox{red!10}{\strut maximum} \colorbox{red!10}{\strut payable} \colorbox{red!19}{\strut rate} \colorbox{red!1}{\strut and} \colorbox{red!16}{\strut pay} \colorbox{red!10}{\strut retention} \colorbox{red!0}{\strut rules} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut an} \colorbox{red!11}{\strut FWS} \colorbox{red!0}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!16}{\strut pay} \colorbox{red!1}{\strut was} \colorbox{red!12}{\strut set} \colorbox{red!0}{\strut by} \colorbox{red!5}{\strut comparing} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!11}{\strut FWS} \colorbox{red!19}{\strut rate} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut underlying} \colorbox{red!16}{\strut GS} \colorbox{red!9}{\strut base} \colorbox{red!19}{\strut rate} \colorbox{red!11}{\strut range} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!7}{\strut grade} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut excluding} \colorbox{red!12}{\strut locality} \colorbox{red!16}{\strut pay} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Once} \colorbox{red!16}{\strut pay} \colorbox{red!1}{\strut was} \colorbox{red!12}{\strut set} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut underlying} \colorbox{red!16}{\strut GS} \colorbox{red!9}{\strut base} \colorbox{red!19}{\strut rate} \colorbox{red!11}{\strut range} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut or} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut case} \colorbox{red!1}{\strut of} \colorbox{red!16}{\strut pay} \colorbox{red!10}{\strut retention} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut as} \colorbox{red!1}{\strut a} \colorbox{red!5}{\strut retained} \colorbox{red!19}{\strut rate} \colorbox{red!0}{\strut if} \colorbox{red!1}{\strut the} \colorbox{red!11}{\strut FWS} \colorbox{red!19}{\strut rate} \colorbox{red!2}{\strut exceeded} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut step} \colorbox{red!3}{\strut 10} \colorbox{red!19}{\strut rate} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut employee} \colorbox{red!0}{\strut s} \colorbox{red!7}{\strut grade} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut applicable} \colorbox{red!16}{\strut GS} \colorbox{red!12}{\strut locality} \colorbox{red!5}{\strut payment} \colorbox{red!1}{\strut was} \colorbox{red!2}{\strut added} \colorbox{red!1}{\strut on} \colorbox{red!3}{\strut top} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut This} \colorbox{red!3}{\strut process} \colorbox{red!1}{\strut of} \colorbox{red!5}{\strut comparing} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut locality-based} \colorbox{red!11}{\strut FWS} \colorbox{red!19}{\strut rate} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut a} \colorbox{red!16}{\strut GS} \colorbox{red!19}{\strut rate} \colorbox{red!11}{\strut range} \colorbox{red!0}{\strut that} \colorbox{red!9}{\strut did} \colorbox{red!1}{\strut not} \colorbox{red!1}{\strut include} \colorbox{red!1}{\strut a} \colorbox{red!12}{\strut locality} \colorbox{red!3}{\strut adjustment} \colorbox{red!1}{\strut resulted} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut substantial} \colorbox{red!16}{\strut pay} \colorbox{red!8}{\strut increases} \colorbox{red!1}{\strut for} \colorbox{red!3}{\strut affected} \colorbox{red!0}{\strut employees-an} \colorbox{red!1}{\strut anomalous} \colorbox{red!0}{\strut result} \colorbox{red!1}{\strut not} \colorbox{red!2}{\strut intended} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut the} \colorbox{red!10}{\strut maximum} \colorbox{red!10}{\strut payable} \colorbox{red!19}{\strut rate} \colorbox{red!1}{\strut or} \colorbox{red!16}{\strut pay} \colorbox{red!10}{\strut retention} \colorbox{red!0}{\strut rules} \colorbox{red!2}{\strut Under} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut new} \colorbox{red!10}{\strut maximum} \colorbox{red!10}{\strut payable} \colorbox{red!19}{\strut rate} \colorbox{red!1}{\strut and} \colorbox{red!16}{\strut pay} \colorbox{red!10}{\strut retention} \colorbox{red!0}{\strut rules} \colorbox{red!1}{\strut ,} \colorbox{red!7}{\strut when} \colorbox{red!1}{\strut an} \colorbox{red!0}{\strut employee} \colorbox{red!4}{\strut moves} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut an} \colorbox{red!11}{\strut FWS} \colorbox{red!6}{\strut position} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut a} \colorbox{red!16}{\strut GS} \colorbox{red!6}{\strut position} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut his} \colorbox{red!1}{\strut or} \colorbox{red!0}{\strut her} \colorbox{red!11}{\strut FWS} \colorbox{red!19}{\strut rate} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut compared} 
}}}
\end{CJK*}

query: dog clean bags

90:bags, 84:dogs, 34:board, 28:walkies, 24:pick, 23:pack, 20:friendly, 19:environmentally, 19:doggy, 18:clean


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Bags} \colorbox{red!0}{\strut on} \colorbox{red!44}{\strut Board} \colorbox{red!24}{\strut Doggy} \colorbox{red!31}{\strut Pick} \colorbox{red!6}{\strut Up} \colorbox{red!20}{\strut Dispenser} \colorbox{red!30}{\strut Pack} \colorbox{red!5}{\strut For} \colorbox{red!100}{\strut Dogs} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Sake} \colorbox{red!6}{\strut ,} \colorbox{red!31}{\strut Pick} \colorbox{red!6}{\strut Up} \colorbox{red!6}{\strut !} \colorbox{red!100}{\strut Bags} \colorbox{red!0}{\strut on} \colorbox{red!44}{\strut Board} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut clean-up} \colorbox{red!7}{\strut product} \colorbox{red!3}{\strut that} \colorbox{red!9}{\strut attaches} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!18}{\strut leash} \colorbox{red!6}{\strut !} \colorbox{red!2}{\strut 2} \colorbox{red!6}{\strut rolls} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut 12} \colorbox{red!13}{\strut large} \colorbox{red!100}{\strut bags} \colorbox{red!9}{\strut come} \colorbox{red!6}{\strut with} \colorbox{red!3}{\strut a} \colorbox{red!7}{\strut handy} \colorbox{red!20}{\strut dispenser} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!20}{\strut Dispenser} \colorbox{red!30}{\strut Pack} \colorbox{red!0}{\strut comes} \colorbox{red!6}{\strut with} \colorbox{red!10}{\strut container} \colorbox{red!6}{\strut ,} \colorbox{red!13}{\strut tie} \colorbox{red!5}{\strut for} \colorbox{red!9}{\strut lead} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut 24} \colorbox{red!22}{\strut disposable} \colorbox{red!100}{\strut bags} \colorbox{red!6}{\strut .} \colorbox{red!24}{\strut Environmentally} \colorbox{red!26}{\strut Friendly} \colorbox{red!0}{\strut -100} \colorbox{red!3}{\strut .} \colorbox{red!23}{\strut Biodegradable} \colorbox{red!100}{\strut Bags} \colorbox{red!6}{\strut !} \colorbox{red!100}{\strut Bags} \colorbox{red!0}{\strut on} \colorbox{red!44}{\strut Board} \colorbox{red!5}{\strut provide} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut easy} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut no-mess} \colorbox{red!5}{\strut solution} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut always} \colorbox{red!6}{\strut having} \colorbox{red!31}{\strut pick} \colorbox{red!6}{\strut up} \colorbox{red!100}{\strut bags} \colorbox{red!6}{\strut with} \colorbox{red!1}{\strut you} \colorbox{red!14}{\strut when} \colorbox{red!1}{\strut you} \colorbox{red!7}{\strut go} \colorbox{red!0}{\strut Walkies} \colorbox{red!6}{\strut !} \colorbox{red!7}{\strut .} \colorbox{red!6}{\strut with} \colorbox{red!3}{\strut your} \colorbox{red!0}{\strut dog..} \colorbox{red!2}{\strut The} \colorbox{red!3}{\strut good} \colorbox{red!0}{\strut news} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut that} \colorbox{red!2}{\strut these} \colorbox{red!100}{\strut bags} \colorbox{red!1}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut dog-friendly} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut are} \colorbox{red!0}{\strut environmentally-friendly} \colorbox{red!0}{\strut too} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut being} \colorbox{red!7}{\strut 100} \colorbox{red!3}{\strut .} \colorbox{red!23}{\strut biodegradable} \colorbox{red!6}{\strut !} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut always} \colorbox{red!23}{\strut clean} \colorbox{red!6}{\strut up} \colorbox{red!0}{\strut after} \colorbox{red!3}{\strut your} \colorbox{red!0}{\strut dog} \colorbox{red!3}{\strut to} \colorbox{red!2}{\strut ensure} \colorbox{red!100}{\strut dogs} \colorbox{red!5}{\strut retain} \colorbox{red!0}{\strut their} \colorbox{red!6}{\strut rights} \colorbox{red!3}{\strut to} \colorbox{red!10}{\strut parks} \colorbox{red!6}{\strut ,} \colorbox{red!9}{\strut beaches} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut dog-friendly} \colorbox{red!11}{\strut accommodation} \colorbox{red!5}{\strut facilities} \colorbox{red!6}{\strut ,} \colorbox{red!9}{\strut walking} \colorbox{red!5}{\strut trails} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut other} \colorbox{red!14}{\strut public} \colorbox{red!9}{\strut places} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut Remember} \colorbox{red!0}{\strut dog} \colorbox{red!11}{\strut poo} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut commonest} \colorbox{red!6}{\strut complaint} \colorbox{red!5}{\strut against} \colorbox{red!100}{\strut dogs} \colorbox{red!2}{\strut using} \colorbox{red!14}{\strut public} \colorbox{red!5}{\strut areas} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut Do} \colorbox{red!5}{\strut it} \colorbox{red!5}{\strut for} \colorbox{red!2}{\strut the} \colorbox{red!10}{\strut environment} \colorbox{red!6}{\strut !} \colorbox{red!3}{\strut Do} \colorbox{red!5}{\strut it} \colorbox{red!5}{\strut for} \colorbox{red!3}{\strut your} \colorbox{red!0}{\strut dog} \colorbox{red!6}{\strut !} \colorbox{red!2}{\strut And} \colorbox{red!3}{\strut do} \colorbox{red!5}{\strut it} \colorbox{red!6}{\strut ,} \colorbox{red!1}{\strut so} \colorbox{red!0}{\strut others} \colorbox{red!3}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!3}{\strut complain} \colorbox{red!3}{\strut to} \colorbox{red!3}{\strut your} \colorbox{red!6}{\strut council} \colorbox{red!2}{\strut and} \colorbox{red!9}{\strut places} \colorbox{red!3}{\strut that} \colorbox{red!0}{\strut we} \colorbox{red!3}{\strut can} \colorbox{red!17}{\strut take} \colorbox{red!0}{\strut our} \colorbox{red!100}{\strut dogs} \colorbox{red!5}{\strut increase} \colorbox{red!0}{\strut rather} \colorbox{red!2}{\strut than} \colorbox{red!6}{\strut decrease} \colorbox{red!6}{\strut !} 
}}}
\end{CJK*}

87:dogs, 60:what, 59:cats, 24:bags, 22:clean, 19:fencing, 16:tie, 16:paws, 15:tame, 15:tags


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Search} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut SIGN} \colorbox{red!1}{\strut IN} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut REGISTER} \colorbox{red!0}{\strut User} \colorbox{red!2}{\strut Name} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Password} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Forgot} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut password} \colorbox{red!1}{\strut ?} \colorbox{red!1}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!3}{\strut Home} \colorbox{red!31}{\strut Dogs} \colorbox{red!21}{\strut Cats} \colorbox{red!5}{\strut Birds} \colorbox{red!4}{\strut Fish} \colorbox{red!3}{\strut Horses} \colorbox{red!3}{\strut Reptiles} \colorbox{red!3}{\strut Small} \colorbox{red!4}{\strut Mammals} \colorbox{red!2}{\strut Quick} \colorbox{red!2}{\strut Picks} \colorbox{red!31}{\strut DOGS} \colorbox{red!2}{\strut Apparel} \colorbox{red!4}{\strut Beds} \colorbox{red!4}{\strut Bones} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut Chews} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Rawhides} \colorbox{red!5}{\strut Bowls} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Feeders} \colorbox{red!5}{\strut Carriers} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Crates} \colorbox{red!7}{\strut Clean} \colorbox{red!1}{\strut Up} \colorbox{red!3}{\strut Collars} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut Leashes} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut Harnesses} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Tie} \colorbox{red!2}{\strut Outs} \colorbox{red!6}{\strut Fencing} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Kennels} \colorbox{red!1}{\strut First} \colorbox{red!3}{\strut Aid} \colorbox{red!5}{\strut Flea} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Tick} \colorbox{red!4}{\strut Food} \colorbox{red!2}{\strut Furniture} \colorbox{red!4}{\strut Gates} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Doors} \colorbox{red!3}{\strut Grooming} \colorbox{red!3}{\strut Health} \colorbox{red!2}{\strut Care} \colorbox{red!1}{\strut Heartworm} \colorbox{red!3}{\strut Prevention} \colorbox{red!3}{\strut Houses} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Pens} \colorbox{red!3}{\strut ID} \colorbox{red!5}{\strut Tags} \colorbox{red!2}{\strut Magazines} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut Movies} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Books} \colorbox{red!4}{\strut Muzzles} \colorbox{red!5}{\strut Pets} \colorbox{red!2}{\strut Ramps} \colorbox{red!3}{\strut Stain} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Odor} \colorbox{red!3}{\strut Toys} \colorbox{red!3}{\strut Training} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Behavior} \colorbox{red!2}{\strut Tools} \colorbox{red!2}{\strut Travel} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Outdoors} \colorbox{red!3}{\strut Treats} \colorbox{red!3}{\strut Vitamins} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Supplements} \colorbox{red!2}{\strut Whelping} \colorbox{red!2}{\strut Supplies} \colorbox{red!31}{\strut Dogs} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Clean} \colorbox{red!1}{\strut Up} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Clean} \colorbox{red!1}{\strut Up} \colorbox{red!2}{\strut Accessories} \colorbox{red!7}{\strut CLEAN} \colorbox{red!1}{\strut UP} \colorbox{red!2}{\strut ACCESSORIES} \colorbox{red!1}{\strut -} \colorbox{red!1}{\strut PRODUCTS} \colorbox{red!1}{\strut Four} \colorbox{red!5}{\strut Paws} \colorbox{red!4}{\strut Doggie} \colorbox{red!2}{\strut Doo} \colorbox{red!8}{\strut Bags} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 25} \colorbox{red!3}{\strut scented} \colorbox{red!8}{\strut bags} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Baby} \colorbox{red!2}{\strut powder} \colorbox{red!3}{\strut scented} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut easy} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut use} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Simply} \colorbox{red!2}{\strut place} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut hand} \colorbox{red!1}{\strut inside} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut bag} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut scoop} \colorbox{red!1}{\strut up} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut waste} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut pull} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut bag} \colorbox{red!1}{\strut inside} \colorbox{red!0}{\strut out} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Tie} \colorbox{red!3}{\strut handles} \colorbox{red!1}{\strut on} \colorbox{red!0}{\strut bag} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!2}{\strut done} \colorbox{red!1}{\strut !} \colorbox{red!7}{\strut Clean} \colorbox{red!1}{\strut up} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut breeze} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Tame} \colorbox{red!8}{\strut Bags} \colorbox{red!1}{\strut on} \colorbox{red!3}{\strut Board} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 60} \colorbox{red!3}{\strut refill} \colorbox{red!8}{\strut bags} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Doggie} \colorbox{red!0}{\strut clean-up} \colorbox{red!8}{\strut bags} \colorbox{red!3}{\strut come} \colorbox{red!3}{\strut rolled} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut handy} \colorbox{red!2}{\strut dispenser} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut With} \colorbox{red!8}{\strut Bags} \colorbox{red!1}{\strut on} \colorbox{red!3}{\strut Board} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!1}{\strut always} \colorbox{red!1}{\strut have} \colorbox{red!8}{\strut bags} \colorbox{red!2}{\strut with} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut !} \colorbox{red!5}{\strut Tame} \colorbox{red!8}{\strut Bags} \colorbox{red!1}{\strut on} \colorbox{red!3}{\strut Board} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 105} \colorbox{red!3}{\strut refill} \colorbox{red!8}{\strut bags} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Doggie} \colorbox{red!0}{\strut clean-up} \colorbox{red!8}{\strut bags} \colorbox{red!3}{\strut come} \colorbox{red!3}{\strut rolled} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut handy} \colorbox{red!2}{\strut dispenser} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut With} \colorbox{red!8}{\strut Bags} \colorbox{red!1}{\strut on} \colorbox{red!3}{\strut Board} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!1}{\strut always} \colorbox{red!1}{\strut have} \colorbox{red!8}{\strut bags} \colorbox{red!2}{\strut with} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut Subscribe} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut More} \colorbox{red!1}{\strut Reviews} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut RSS} \colorbox{red!2}{\strut Feed} \colorbox{red!1}{\strut -} \colorbox{red!1}{\strut Add} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut My} \colorbox{red!1}{\strut Yahoo} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut -} \colorbox{red!1}{\strut Add} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut Google} \colorbox{red!2}{\strut Homepage} \colorbox{red!21}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut Hot} \colorbox{red!0}{\strut Cat} \colorbox{red!4}{\strut Beds} \colorbox{red!0}{\strut Cat} \colorbox{red!5}{\strut Bowls} \colorbox{red!0}{\strut Cat} \colorbox{red!5}{\strut Carriers} \colorbox{red!0}{\strut Cat} \colorbox{red!5}{\strut Flea} \colorbox{red!3}{\strut Control} \colorbox{red!0}{\strut Cat} \colorbox{red!3}{\strut ID} \colorbox{red!5}{\strut Tags} \colorbox{red!0}{\strut Cat} \colorbox{red!3}{\strut Litter} \colorbox{red!3}{\strut Box} \colorbox{red!0}{\strut Cat} \colorbox{red!3}{\strut Toys} \colorbox{red!0}{\strut Cat} \colorbox{red!3}{\strut Urine} \colorbox{red!3}{\strut Odor} \colorbox{red!0}{\strut Dog} \colorbox{red!4}{\strut Beds} \colorbox{red!0}{\strut Dog} \colorbox{red!5}{\strut Bowls} \colorbox{red!0}{\strut Dog} \colorbox{red!3}{\strut Crates} \colorbox{red!0}{\strut Dog} \colorbox{red!6}{\strut Fencing} \colorbox{red!0}{\strut Dog} \colorbox{red!5}{\strut Flea} \colorbox{red!0}{\strut Dog} \colorbox{red!4}{\strut Food} \colorbox{red!0}{\strut Dog} \colorbox{red!4}{\strut Gates} \colorbox{red!0}{\strut Dog} \colorbox{red!3}{\strut ID} \colorbox{red!5}{\strut Tags} \colorbox{red!0}{\strut Dog} \colorbox{red!2}{\strut Ramps} \colorbox{red!0}{\strut Dog} \colorbox{red!3}{\strut Tick} \colorbox{red!0}{\strut Dog} \colorbox{red!3}{\strut Toys} \colorbox{red!0}{\strut Site} \colorbox{red!1}{\strut Map} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: indiana state fairgrounds

85:state, 80:indiana, 77:fair, 75:fairgrounds, 36:largest, 35:indianapolis, 27:venue, 21:pavilion, 17:building, 14:show


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Administrative} \colorbox{red!5}{\strut Hours} \colorbox{red!12}{\strut Parking} \colorbox{red!4}{\strut Fees} \colorbox{red!3}{\strut Camping} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Hotels} \colorbox{red!66}{\strut Fairgrounds} \colorbox{red!1}{\strut 101} \colorbox{red!3}{\strut Employment} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut Releases} \colorbox{red!3}{\strut Photos} \colorbox{red!0}{\strut Related} \colorbox{red!1}{\strut Links} \colorbox{red!2}{\strut General} \colorbox{red!6}{\strut Email} \colorbox{red!75}{\strut State} \colorbox{red!0}{\strut s} \colorbox{red!32}{\strut Largest} \colorbox{red!10}{\strut Classroom} \colorbox{red!66}{\strut Fairgrounds} \colorbox{red!4}{\strut Map} \colorbox{red!4}{\strut Driving} \colorbox{red!3}{\strut Directions} \colorbox{red!8}{\strut Indy} \colorbox{red!5}{\strut Visitor} \colorbox{red!3}{\strut Information} \colorbox{red!66}{\strut Fairgrounds} \colorbox{red!5}{\strut Mission} \colorbox{red!75}{\strut State} \colorbox{red!68}{\strut Fair} \colorbox{red!1}{\strut Board} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Commission} \colorbox{red!0}{\strut Inside} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut Grounds} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Magazine} \colorbox{red!9}{\strut Meetings} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut Notices} \colorbox{red!66}{\strut Fairgrounds} \colorbox{red!4}{\strut Managers} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut Staff} \colorbox{red!0}{\strut Year-round} \colorbox{red!5}{\strut Sponsors} \colorbox{red!2}{\strut Yearly} \colorbox{red!4}{\strut Calendar} \colorbox{red!2}{\strut of} \colorbox{red!9}{\strut Events} \colorbox{red!2}{\strut Monthly} \colorbox{red!0}{\strut E-Calendar} \colorbox{red!24}{\strut Venue} \colorbox{red!3}{\strut Information} \colorbox{red!4}{\strut Contract} \colorbox{red!3}{\strut Services} \colorbox{red!3}{\strut Request} \colorbox{red!3}{\strut for} \colorbox{red!3}{\strut Information} \colorbox{red!5}{\strut Public} \colorbox{red!5}{\strut Skating} \colorbox{red!3}{\strut Pro} \colorbox{red!0}{\strut Skate} \colorbox{red!1}{\strut Shop} \colorbox{red!4}{\strut Pepsi} \colorbox{red!6}{\strut Coliseum} \colorbox{red!4}{\strut Youth} \colorbox{red!5}{\strut Hockey} \colorbox{red!5}{\strut League} \colorbox{red!4}{\strut Winter} \colorbox{red!5}{\strut Club} \colorbox{red!2}{\strut of} \colorbox{red!31}{\strut Indianapolis} \colorbox{red!71}{\strut Indiana} \colorbox{red!7}{\strut Ice} \colorbox{red!24}{\strut Venue} \colorbox{red!3}{\strut Information} \colorbox{red!8}{\strut Northwest} \colorbox{red!18}{\strut Pavilion} \colorbox{red!0}{\strut 31,800} \colorbox{red!1}{\strut sq} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut ft.} \colorbox{red!8}{\strut Northwest} \colorbox{red!18}{\strut Pavilion} \colorbox{red!7}{\strut Occupancy} \colorbox{red!0}{\strut 1,000} \colorbox{red!3}{\strut 10x10} \colorbox{red!5}{\strut booths} \colorbox{red!0}{\strut 214} \colorbox{red!5}{\strut Ceiling} \colorbox{red!6}{\strut Height} \colorbox{red!1}{\strut 20} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut clearance} \colorbox{red!0}{\strut at} \colorbox{red!5}{\strut center} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 13} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut clearance} \colorbox{red!0}{\strut at} \colorbox{red!3}{\strut middle} \colorbox{red!6}{\strut aisle} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut clearance} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut outer} \colorbox{red!6}{\strut aisle} \colorbox{red!5}{\strut Move} \colorbox{red!0}{\strut inout} \colorbox{red!2}{\strut daily} \colorbox{red!6}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut 400} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut day} \colorbox{red!2}{\strut Daily} \colorbox{red!6}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 800} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut day} \colorbox{red!3}{\strut View} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut larger} \colorbox{red!0}{\strut version} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!6}{\strut layout} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut pdf} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!7}{\strut historic} \colorbox{red!0}{\strut 1927} \colorbox{red!8}{\strut structure} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut accommodate} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut auction} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut trade} \colorbox{red!12}{\strut show} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut livestock} \colorbox{red!0}{\strut event} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut high} \colorbox{red!0}{\strut ceilings} \colorbox{red!3}{\strut add} \colorbox{red!2}{\strut flexibility} \colorbox{red!3}{\strut for} \colorbox{red!4}{\strut large} \colorbox{red!6}{\strut exhibits} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Complete} \colorbox{red!1}{\strut with} \colorbox{red!2}{\strut heat} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut large} \colorbox{red!3}{\strut overhead} \colorbox{red!3}{\strut fans} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!10}{\strut facility} \colorbox{red!0}{\strut can} \colorbox{red!2}{\strut provide} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut round} \colorbox{red!4}{\strut comfort} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Office} \colorbox{red!10}{\strut space} \colorbox{red!3}{\strut and} \colorbox{red!2}{\strut supply} \colorbox{red!12}{\strut show} \colorbox{red!2}{\strut area} \colorbox{red!2}{\strut allows} \colorbox{red!3}{\strut for} \colorbox{red!2}{\strut ease} \colorbox{red!3}{\strut in} \colorbox{red!12}{\strut show} \colorbox{red!6}{\strut operations} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Wheelchair} \colorbox{red!1}{\strut accessible} \colorbox{red!3}{\strut restrooms} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut overhead} \colorbox{red!3}{\strut doors} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!8}{\strut concessions} \colorbox{red!10}{\strut space} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut additional} \colorbox{red!5}{\strut features} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!15}{\strut building} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Clientele} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Stewart} \colorbox{red!0}{\strut s} \colorbox{red!71}{\strut Indiana} \colorbox{red!5}{\strut Flea} \colorbox{red!5}{\strut Market} \colorbox{red!3}{\strut ,} \colorbox{red!71}{\strut Indiana} \colorbox{red!5}{\strut Rabbit} \colorbox{red!4}{\strut Breeders} \colorbox{red!12}{\strut Show} \colorbox{red!71}{\strut Indiana} \colorbox{red!75}{\strut State} \colorbox{red!66}{\strut Fairgrounds} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 1202} \colorbox{red!0}{\strut E.} \colorbox{red!4}{\strut 38th} \colorbox{red!3}{\strut St} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Indpls.} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut IN} \colorbox{red!3}{\strut 46205} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 317927-7500} \colorbox{red!5}{\strut fax} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 317-927-7695} 
}}}
\end{CJK*}

97:fair, 91:indiana, 89:barn, 86:state, 20:governed, 18:fairgrounds, 14:commission, 13:education, 12:site, 10:trustees


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut The} \colorbox{red!65}{\strut Barn} \colorbox{red!5}{\strut at} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut Indiana} \colorbox{red!63}{\strut State} \colorbox{red!13}{\strut Fairgrounds} \colorbox{red!2}{\strut The} \colorbox{red!65}{\strut Barn} \colorbox{red!5}{\strut at} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut Indiana} \colorbox{red!63}{\strut State} \colorbox{red!13}{\strut Fairgrounds} \colorbox{red!3}{\strut is} \colorbox{red!14}{\strut governed} \colorbox{red!2}{\strut by} \colorbox{red!3}{\strut a} \colorbox{red!6}{\strut Board} \colorbox{red!3}{\strut of} \colorbox{red!7}{\strut Trustees} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut Indiana} \colorbox{red!63}{\strut State} \colorbox{red!71}{\strut Fair} \colorbox{red!10}{\strut Commission} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut also} \colorbox{red!5}{\strut works} \colorbox{red!2}{\strut toward} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut mission} \colorbox{red!3}{\strut of} \colorbox{red!7}{\strut bridging} \colorbox{red!3}{\strut members} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut agricultural} \colorbox{red!2}{\strut community} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut consumer} \colorbox{red!6}{\strut public} \colorbox{red!2}{\strut through} \colorbox{red!9}{\strut education} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!65}{\strut Barn} \colorbox{red!5}{\strut at} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut Indiana} \colorbox{red!63}{\strut State} \colorbox{red!13}{\strut Fairgrounds} \colorbox{red!3}{\strut will} \colorbox{red!5}{\strut provide} \colorbox{red!0}{\strut on-site} \colorbox{red!0}{\strut educational} \colorbox{red!7}{\strut programming} \colorbox{red!2}{\strut for} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut northside} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!66}{\strut Indiana} \colorbox{red!63}{\strut State} \colorbox{red!13}{\strut Fairgrounds} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut 2007} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut beyond} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Educational} \colorbox{red!7}{\strut Programming} \colorbox{red!4}{\strut Professional} \colorbox{red!5}{\strut Development} \colorbox{red!7}{\strut Events} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Exhibitions} \colorbox{red!3}{\strut About} \colorbox{red!2}{\strut the} \colorbox{red!65}{\strut Barn} \colorbox{red!0}{\strut Get} \colorbox{red!4}{\strut Involved} \colorbox{red!3}{\strut Home} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Links} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Contact} \colorbox{red!4}{\strut Us} \colorbox{red!1}{\strut .} \colorbox{red!66}{\strut Indiana} \colorbox{red!63}{\strut State} \colorbox{red!71}{\strut Fair} 
}}}
\end{CJK*}

query: fybromyalgia

90:fibromyalgia, 86:fybromyalgia, 36:symptoms, 26:disorder, 25:pain, 25:fibrous, 25:fibro, 19:disease, 18:tissue, 18:muscle


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!68}{\strut Fibromyalgia} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!1}{\strut free} \colorbox{red!1}{\strut encyclopedia} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!65}{\strut Fybromyalgia} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut Jump} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut navigation} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut search} \colorbox{red!68}{\strut Fibromyalgia} \colorbox{red!3}{\strut Classification} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut external} \colorbox{red!1}{\strut resources} \colorbox{red!12}{\strut ICD} \colorbox{red!3}{\strut -} \colorbox{red!3}{\strut 10} \colorbox{red!1}{\strut M} \colorbox{red!0}{\strut 79.7} \colorbox{red!12}{\strut ICD} \colorbox{red!3}{\strut -} \colorbox{red!3}{\strut 9} \colorbox{red!0}{\strut 729.1} \colorbox{red!0}{\strut MedlinePlus} \colorbox{red!2}{\strut 000427} \colorbox{red!0}{\strut eMedicine} \colorbox{red!0}{\strut med790} \colorbox{red!0}{\strut med2934} \colorbox{red!0}{\strut ped777} \colorbox{red!0}{\strut pmr47} \colorbox{red!0}{\strut MeSH} \colorbox{red!2}{\strut D005356} \colorbox{red!68}{\strut Fibromyalgia} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut new} \colorbox{red!0}{\strut lat.} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut fibro-} \colorbox{red!19}{\strut fibrous} \colorbox{red!13}{\strut tissue} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut Gk} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut myo-} \colorbox{red!13}{\strut muscle} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut Gk} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut algos-} \colorbox{red!19}{\strut pain} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!13}{\strut meaning} \colorbox{red!13}{\strut muscle} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut connective} \colorbox{red!13}{\strut tissue} \colorbox{red!19}{\strut pain} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut also} \colorbox{red!2}{\strut referred} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut as} \colorbox{red!6}{\strut FM} \colorbox{red!1}{\strut or} \colorbox{red!0}{\strut FMS} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut a} \colorbox{red!19}{\strut disorder} \colorbox{red!4}{\strut classified} \colorbox{red!1}{\strut by} \colorbox{red!4}{\strut the} \colorbox{red!4}{\strut presence} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut chronic} \colorbox{red!2}{\strut widespread} \colorbox{red!19}{\strut pain} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut a} \colorbox{red!4}{\strut heightened} \colorbox{red!3}{\strut and} \colorbox{red!0}{\strut painful} \colorbox{red!6}{\strut response} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut gentle} \colorbox{red!3}{\strut touch} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut tactile} \colorbox{red!4}{\strut allodynia} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 1} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Other} \colorbox{red!3}{\strut core} \colorbox{red!4}{\strut features} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!19}{\strut disorder} \colorbox{red!2}{\strut include} \colorbox{red!5}{\strut debilitating} \colorbox{red!5}{\strut fatigue} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut sleep} \colorbox{red!4}{\strut disturbance} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut joint} \colorbox{red!4}{\strut stiffness} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut In} \colorbox{red!2}{\strut addition} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut persons} \colorbox{red!7}{\strut affected} \colorbox{red!1}{\strut by} \colorbox{red!4}{\strut the} \colorbox{red!19}{\strut disorder} \colorbox{red!1}{\strut frequently} \colorbox{red!2}{\strut experience} \colorbox{red!3}{\strut a} \colorbox{red!0}{\strut range} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut other} \colorbox{red!27}{\strut symptoms} \colorbox{red!2}{\strut that} \colorbox{red!3}{\strut involve} \colorbox{red!3}{\strut multiple} \colorbox{red!4}{\strut body} \colorbox{red!5}{\strut systems} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!3}{\strut difficulty} \colorbox{red!3}{\strut with} \colorbox{red!4}{\strut swallowing} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 2} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut functional} \colorbox{red!5}{\strut bowel} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut bladder} \colorbox{red!8}{\strut abnormalities} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 3} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut difficulty} \colorbox{red!4}{\strut breathing} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 4} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut diffuse} \colorbox{red!4}{\strut sensations} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut numbness} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut tingling} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut non-dermatomal} \colorbox{red!3}{\strut paresthesia} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 5} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut abnormal} \colorbox{red!4}{\strut motor} \colorbox{red!3}{\strut activity} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut i.e} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut nocturnal} \colorbox{red!4}{\strut myoclonus} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut sleep} \colorbox{red!3}{\strut bruxism} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 6} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut cognitive} \colorbox{red!4}{\strut dysfunction} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 7} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut An} \colorbox{red!2}{\strut increased} \colorbox{red!4}{\strut prevalence} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut affective} \colorbox{red!3}{\strut and} \colorbox{red!0}{\strut anxiety-related} \colorbox{red!27}{\strut symptoms} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut also} \colorbox{red!2}{\strut well} \colorbox{red!3}{\strut known} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 8} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut While} \colorbox{red!4}{\strut the} \colorbox{red!3}{\strut criteria} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut such} \colorbox{red!2}{\strut an} \colorbox{red!3}{\strut entity} \colorbox{red!3}{\strut have} \colorbox{red!0}{\strut not} \colorbox{red!3}{\strut yet} \colorbox{red!2}{\strut been} \colorbox{red!1}{\strut thoroughly} \colorbox{red!3}{\strut developed} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut recognition} \colorbox{red!2}{\strut that} \colorbox{red!68}{\strut fibromyalgia} \colorbox{red!0}{\strut involves} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut than} \colorbox{red!1}{\strut just} \colorbox{red!19}{\strut pain} \colorbox{red!1}{\strut has} \colorbox{red!1}{\strut led} \colorbox{red!2}{\strut to} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut frequent} \colorbox{red!3}{\strut use} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut term} \colorbox{red!0}{\strut .} \colorbox{red!68}{\strut fibromyalgia} \colorbox{red!9}{\strut syndrome} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 9} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Not} \colorbox{red!1}{\strut all} \colorbox{red!7}{\strut affected} \colorbox{red!3}{\strut persons} \colorbox{red!2}{\strut experience} \colorbox{red!1}{\strut all} \colorbox{red!4}{\strut the} \colorbox{red!27}{\strut symptoms} \colorbox{red!1}{\strut associated} \colorbox{red!3}{\strut with} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut greater} \colorbox{red!9}{\strut syndrome} \colorbox{red!3}{\strut .} \colorbox{red!68}{\strut Fibromyalgia} \colorbox{red!2}{\strut is} \colorbox{red!5}{\strut considered} \colorbox{red!3}{\strut a} \colorbox{red!0}{\strut controversial} \colorbox{red!6}{\strut diagnosis} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut with} \colorbox{red!1}{\strut some} \colorbox{red!2}{\strut authors} \colorbox{red!0}{\strut contending} \colorbox{red!2}{\strut that} \colorbox{red!4}{\strut the} \colorbox{red!19}{\strut disorder} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut a} \colorbox{red!0}{\strut non-disease} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut due} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut part} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut a} \colorbox{red!3}{\strut lack} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut objective} \colorbox{red!3}{\strut laboratory} 
}}}
\end{CJK*}

75:rsd, 54:what, 28:pain, 24:mental, 24:illness, 24:advisory, 23:syndrome, 23:diseases, 22:complex, 21:disorder


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!31}{\strut RSD} \colorbox{red!0}{\strut Advisory-} \colorbox{red!8}{\strut Where} \colorbox{red!5}{\strut Chronic} \colorbox{red!11}{\strut Pain} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Mental} \colorbox{red!9}{\strut Illness} \colorbox{red!7}{\strut Collide} \colorbox{red!2}{\strut October} \colorbox{red!2}{\strut 24} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut 2006} \colorbox{red!4}{\strut Promoting} \colorbox{red!0}{\strut Awareness-} \colorbox{red!1}{\strut Your} \colorbox{red!3}{\strut thoughts} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut storieswelcome} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Filed} \colorbox{red!1}{\strut under} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 360.yahoo.comelllajC} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut Blogroll} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut Blogs} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut Blogging} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut CRPS} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut Chronic} \colorbox{red!11}{\strut Pain} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut Complex} \colorbox{red!7}{\strut Regional} \colorbox{red!11}{\strut Pain} \colorbox{red!9}{\strut Syndrome} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut Depression} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut Fybromyalgia} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut Incurable} \colorbox{red!9}{\strut Diseases} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut Mental} \colorbox{red!9}{\strut Illness} \colorbox{red!5}{\strut Advocacy} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut MySpace} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut NINDS} \colorbox{red!2}{\strut ,} \colorbox{red!7}{\strut Neurological} \colorbox{red!8}{\strut Disorder} \colorbox{red!2}{\strut ,} \colorbox{red!11}{\strut Pain} \colorbox{red!2}{\strut ,} \colorbox{red!11}{\strut Pain} \colorbox{red!9}{\strut Syndrome} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut Personal} \colorbox{red!2}{\strut Essays} \colorbox{red!2}{\strut ,} \colorbox{red!31}{\strut RSD} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut RSDS} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut Rare} \colorbox{red!0}{\strut Disorders} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut Reflex} \colorbox{red!8}{\strut Sympathetic} \colorbox{red!7}{\strut Dystrophy} \colorbox{red!9}{\strut Syndrome} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut Web} \colorbox{red!2}{\strut Publications} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut Web} \colorbox{red!3}{\strut authors} \colorbox{red!2}{\strut ,} \colorbox{red!22}{\strut what} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut www.RSDAdvisor.com} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut www.RSDAdvisory.com} \colorbox{red!2}{\strut twinklev} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 456} \colorbox{red!1}{\strut pm} \colorbox{red!1}{\strut In} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut effort} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut promote} \colorbox{red!5}{\strut awareness} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut resources} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut information} \colorbox{red!1}{\strut regarding} \colorbox{red!8}{\strut Reflex} \colorbox{red!8}{\strut Sympathetic} \colorbox{red!7}{\strut Dystrophy} \colorbox{red!0}{\strut SyndromeComplex} \colorbox{red!7}{\strut Regional} \colorbox{red!11}{\strut Pain} \colorbox{red!9}{\strut Syndrome} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut aka} \colorbox{red!2}{\strut ,} \colorbox{red!31}{\strut RSD} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut RSDS} \colorbox{red!2}{\strut and} \colorbox{red!8}{\strut CRPS} \colorbox{red!2}{\strut these} \colorbox{red!3}{\strut sites} \colorbox{red!1}{\strut have} \colorbox{red!2}{\strut been} \colorbox{red!3}{\strut created} \colorbox{red!1}{\strut so} \colorbox{red!1}{\strut that} \colorbox{red!2}{\strut understanding} \colorbox{red!1}{\strut might} \colorbox{red!2}{\strut come} \colorbox{red!1}{\strut from} \colorbox{red!2}{\strut them} \colorbox{red!1}{\strut .} \colorbox{red!31}{\strut RSD} \colorbox{red!9}{\strut Advisory} \colorbox{red!2}{\strut and} \colorbox{red!31}{\strut RSD} \colorbox{red!4}{\strut Advisor} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut mirror} \colorbox{red!0}{\strut dot.com} \colorbox{red!3}{\strut sites} \colorbox{red!0}{\strut www.RSDAdvisor.com} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut www.RSDAdvisory.com} \colorbox{red!2}{\strut Here} \colorbox{red!1}{\strut at} \colorbox{red!31}{\strut RSD} \colorbox{red!0}{\strut Advisory-WordPress} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut can} \colorbox{red!2}{\strut leave} \colorbox{red!3}{\strut comments} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut add} \colorbox{red!1}{\strut your} \colorbox{red!1}{\strut own} \colorbox{red!2}{\strut stories} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut tell} \colorbox{red!2}{\strut the} \colorbox{red!1}{\strut world} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut anything} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut might} \colorbox{red!1}{\strut like} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut add} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Just} \colorbox{red!2}{\strut add} \colorbox{red!2}{\strut it} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut comment} \colorbox{red!1}{\strut area} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut this} \colorbox{red!2}{\strut post} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut one} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut blogs} \colorbox{red!1}{\strut that} \colorbox{red!3}{\strut best} \colorbox{red!1}{\strut fits} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Thank} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut for} \colorbox{red!2}{\strut supporting} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut passion} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut promote} \colorbox{red!4}{\strut education} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut date} \colorbox{red!1}{\strut there} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut still} \colorbox{red!1}{\strut no} \colorbox{red!5}{\strut cure} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Best} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut wishes} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut twinkleellaj} \colorbox{red!3}{\strut Comments} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 8} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut October} \colorbox{red!2}{\strut 22} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut 2006} \colorbox{red!2}{\strut The} \colorbox{red!5}{\strut Universal} \colorbox{red!0}{\strut Disorder-} \colorbox{red!3}{\strut Part} \colorbox{red!2}{\strut 3} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut conclusion} \colorbox{red!4}{\strut Filed} \colorbox{red!1}{\strut under} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 360.yahoo.comelllajC} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut Answers} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut Bipolar} \colorbox{red!8}{\strut Disorder} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut Blogroll} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut CRPS} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut Chronic} \colorbox{red!11}{\strut Pain} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut Complex} \colorbox{red!7}{\strut Regional} \colorbox{red!11}{\strut Pain} \colorbox{red!9}{\strut Syndrome} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut Depression} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut Fybromyalgia} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut Incurable} \colorbox{red!9}{\strut Diseases} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut Mania} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut Mental} \colorbox{red!9}{\strut Illness} \colorbox{red!5}{\strut Advocacy} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut NINDS} \colorbox{red!2}{\strut ,} \colorbox{red!7}{\strut Neurological} \colorbox{red!8}{\strut Disorder} \colorbox{red!2}{\strut ,} \colorbox{red!11}{\strut Pain} \colorbox{red!2}{\strut ,} \colorbox{red!11}{\strut Pain} \colorbox{red!9}{\strut Syndrome} \colorbox{red!2}{\strut ,} \colorbox{red!31}{\strut RSD} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut RSDS} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut Rare} \colorbox{red!0}{\strut Disorders} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut Reflex} \colorbox{red!8}{\strut Sympathetic} \colorbox{red!7}{\strut Dystrophy} \colorbox{red!9}{\strut Syndrome} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut Salacious} \colorbox{red!3}{\strut Surrender} \colorbox{red!2}{\strut ,} \colorbox{red!22}{\strut what} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut www.RSDAdvisor.com} 
}}}
\end{CJK*}

query: french lick resort casino

101:lick, 100:french, 90:casino, 62:indiana, 36:resort, 29:how, 23:places, 22:address, 18:poker, 13:hotels


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!0}{\strut .} \colorbox{red!24}{\strut Places} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!11}{\strut Played} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Ratings} \colorbox{red!9}{\strut Check} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut .} \colorbox{red!24}{\strut Places} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!11}{\strut Played} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut FIRST} \colorbox{red!3}{\strut Facebook} \colorbox{red!4}{\strut application} \colorbox{red!6}{\strut created} \colorbox{red!2}{\strut for} \colorbox{red!8}{\strut ranking} \colorbox{red!0}{\strut Casinos} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut see} \colorbox{red!31}{\strut how} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut rate} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!7}{\strut .} \colorbox{red!5}{\strut Currently} \colorbox{red!7}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!4}{\strut site} \colorbox{red!3}{\strut has} \colorbox{red!0}{\strut not} \colorbox{red!2}{\strut yet} \colorbox{red!2}{\strut been} \colorbox{red!0}{\strut rated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut .} \colorbox{red!24}{\strut Places} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!11}{\strut Played} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut users} \colorbox{red!7}{\strut ,} \colorbox{red!3}{\strut which} \colorbox{red!0}{\strut means} \colorbox{red!0}{\strut YOU} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut first} \colorbox{red!4}{\strut !} \colorbox{red!0}{\strut Rate} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!9}{\strut Coupons} \colorbox{red!1}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut 20} \colorbox{red!9}{\strut Slot} \colorbox{red!7}{\strut Dollars} \colorbox{red!1}{\strut from} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!4}{\strut !} \colorbox{red!2}{\strut The} \colorbox{red!5}{\strut American} \colorbox{red!96}{\strut Casino} \colorbox{red!4}{\strut Guide} \colorbox{red!3}{\strut has} \colorbox{red!2}{\strut over} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,000} \colorbox{red!5}{\strut in} \colorbox{red!0}{\strut money-saving} \colorbox{red!9}{\strut coupons} \colorbox{red!1}{\strut from} \colorbox{red!0}{\strut all} \colorbox{red!2}{\strut over} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut country} \colorbox{red!4}{\strut !} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut stationary} \colorbox{red!8}{\strut boat} \colorbox{red!96}{\strut Casino} \colorbox{red!5}{\strut in} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!7}{\strut ,} \colorbox{red!66}{\strut Indiana} \colorbox{red!7}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!96}{\strut casino} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut 42,000} \colorbox{red!8}{\strut square} \colorbox{red!8}{\strut foot} \colorbox{red!11}{\strut gaming} \colorbox{red!6}{\strut space} \colorbox{red!5}{\strut features} \colorbox{red!0}{\strut 1,335} \colorbox{red!11}{\strut gaming} \colorbox{red!3}{\strut machines} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut fifty} \colorbox{red!9}{\strut table} \colorbox{red!1}{\strut and} \colorbox{red!19}{\strut poker} \colorbox{red!0}{\strut games} \colorbox{red!7}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!7}{\strut property} \colorbox{red!3}{\strut has} \colorbox{red!0}{\strut nine} \colorbox{red!12}{\strut restaurants} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut two} \colorbox{red!13}{\strut hotels} \colorbox{red!3}{\strut with} \colorbox{red!2}{\strut 689} \colorbox{red!12}{\strut rooms} \colorbox{red!7}{\strut .} \colorbox{red!9}{\strut Check} \colorbox{red!5}{\strut in} \colorbox{red!1}{\strut .} \colorbox{red!9}{\strut Check} \colorbox{red!0}{\strut out} \colorbox{red!1}{\strut .} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!23}{\strut Address} \colorbox{red!4}{\strut 8670} \colorbox{red!4}{\strut West} \colorbox{red!10}{\strut State} \colorbox{red!3}{\strut Road} \colorbox{red!0}{\strut 56} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!7}{\strut ,} \colorbox{red!66}{\strut Indiana} \colorbox{red!2}{\strut 47432} \colorbox{red!5}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!5}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut News} \colorbox{red!0}{\strut PokerTek} \colorbox{red!6}{\strut installs} \colorbox{red!0}{\strut PokerPro} \colorbox{red!5}{\strut at} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!2}{\strut 2} \colorbox{red!2}{\strut September} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut PokerTek} \colorbox{red!7}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!3}{\strut has} \colorbox{red!0}{\strut installed} \colorbox{red!0}{\strut PokerPro} \colorbox{red!5}{\strut at} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!38}{\strut Resort} \colorbox{red!96}{\strut Casino} \colorbox{red!5}{\strut in} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!7}{\strut ,} \colorbox{red!66}{\strut Indiana} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!4}{\strut issues} \colorbox{red!6}{\strut notes} \colorbox{red!0}{\strut 29} \colorbox{red!4}{\strut April} \colorbox{red!0}{\strut 2008} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!0}{\strut Resorts} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!7}{\strut ,} \colorbox{red!11}{\strut LLC} \colorbox{red!1}{\strut and} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!0}{\strut Resorts} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!0}{\strut Corp.} \colorbox{red!6}{\strut report} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut results} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut their} \colorbox{red!6}{\strut offer} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut purchase} \colorbox{red!2}{\strut for} \colorbox{red!7}{\strut cash} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 150,000,000} \colorbox{red!4}{\strut aggregate} \colorbox{red!5}{\strut principal} \colorbox{red!6}{\strut amount} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut outstanding} \colorbox{red!0}{\strut 10-34} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut First} \colorbox{red!6}{\strut Mortgage} \colorbox{red!6}{\strut Notes} \colorbox{red!4}{\strut due} \colorbox{red!0}{\strut 2014} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!3}{\strut amends} \colorbox{red!2}{\strut tender} \colorbox{red!6}{\strut offer} \colorbox{red!2}{\strut 3} \colorbox{red!4}{\strut April} \colorbox{red!0}{\strut 2008} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!0}{\strut Resorts} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!7}{\strut ,} \colorbox{red!11}{\strut LLC} \colorbox{red!1}{\strut and} \colorbox{red!100}{\strut French} \colorbox{red!100}{\strut Lick} \colorbox{red!0}{\strut Resorts} \colorbox{red!3}{\strut .} \colorbox{red!96}{\strut Casino} \colorbox{red!0}{\strut Corp.} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut amended} \colorbox{red!0}{\strut their} \colorbox{red!2}{\strut tender} \colorbox{red!6}{\strut offer} \colorbox{red!3}{\strut launched} \colorbox{red!1}{\strut on} \colorbox{red!3}{\strut March} \colorbox{red!0}{\strut 31} 
}}}
\end{CJK*}

97:french, 96:lick, 91:casino, 60:resort, 38:coupons, 32:how, 27:price, 24:gambling, 18:legal, 17:sale


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!47}{\strut French} \colorbox{red!46}{\strut Lick} \colorbox{red!29}{\strut Resort} \colorbox{red!0}{\strut .} \colorbox{red!44}{\strut Casino} \colorbox{red!18}{\strut Coupons} \colorbox{red!6}{\strut American} \colorbox{red!44}{\strut Casino} \colorbox{red!3}{\strut Guide} \colorbox{red!3}{\strut List} \colorbox{red!13}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 16.95} \colorbox{red!8}{\strut Sale} \colorbox{red!13}{\strut Price} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 11.53} \colorbox{red!3}{\strut Save} \colorbox{red!1}{\strut 30} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut !} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut coupon} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 205} \colorbox{red!18}{\strut coupons} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut can} \colorbox{red!3}{\strut save} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut over} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 1,000} \colorbox{red!0}{\strut included} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut American} \colorbox{red!44}{\strut Casino} \colorbox{red!3}{\strut Guide} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Published} \colorbox{red!2}{\strut annually} \colorbox{red!1}{\strut since} \colorbox{red!0}{\strut 1992} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut edition} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut best-selling} \colorbox{red!3}{\strut guide} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut jam-packed} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut detailed} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut casinoresort} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut riverboat} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut Indian} \colorbox{red!44}{\strut casino} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut useful} \colorbox{red!0}{\strut advice} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut top} \colorbox{red!11}{\strut gambling} \colorbox{red!0}{\strut experts} \colorbox{red!0}{\strut on} \colorbox{red!15}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut play} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut win} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!5}{\strut popular} \colorbox{red!44}{\strut casino} \colorbox{red!6}{\strut games} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!2}{\strut arranged} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut special} \colorbox{red!1}{\strut discount} \colorbox{red!2}{\strut rate} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut book} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!18}{\strut coupons} \colorbox{red!1}{\strut for} \colorbox{red!44}{\strut Casino} \colorbox{red!7}{\strut City} \colorbox{red!2}{\strut visitors} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut save} \colorbox{red!1}{\strut 30} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Only} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 11.53} \colorbox{red!1}{\strut plus} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 3.50} \colorbox{red!1}{\strut shipping} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut US} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Complete} \colorbox{red!0}{\strut Details} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!2}{\strut Slot} \colorbox{red!3}{\strut Dollars} \colorbox{red!0}{\strut NON-REDEEMABLE} \colorbox{red!0}{\strut SAMPLE} \colorbox{red!1}{\strut ONLY} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Coupon} \colorbox{red!0}{\strut Front} \colorbox{red!1}{\strut Present} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut coupon} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut valid} \colorbox{red!0}{\strut photo} \colorbox{red!0}{\strut i.d} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!47}{\strut French} \colorbox{red!46}{\strut Lick} \colorbox{red!3}{\strut Players} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Club} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut receive} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!2}{\strut Slot} \colorbox{red!3}{\strut Dollars} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut NON-REDEEMABLE} \colorbox{red!0}{\strut SAMPLE} \colorbox{red!1}{\strut ONLY} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Coupon} \colorbox{red!1}{\strut Back} \colorbox{red!1}{\strut Join} \colorbox{red!0}{\strut the} \colorbox{red!29}{\strut Resort} \colorbox{red!1}{\strut Rewards} \colorbox{red!0}{\strut at} \colorbox{red!47}{\strut French} \colorbox{red!46}{\strut Lick} \colorbox{red!3}{\strut players} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut club} \colorbox{red!1}{\strut today} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut receive} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut offer} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut fast} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut FREE} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut easy} \colorbox{red!2}{\strut !} \colorbox{red!3}{\strut Expires} \colorbox{red!0}{\strut 12312009} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut 21} \colorbox{red!2}{\strut years} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut older} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Not} \colorbox{red!4}{\strut redeemable} \colorbox{red!1}{\strut for} \colorbox{red!3}{\strut Cash} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Coupon} \colorbox{red!1}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut combined} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut other} \colorbox{red!18}{\strut coupons} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut offer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut promotions} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Offer} \colorbox{red!4}{\strut valid} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut new} \colorbox{red!1}{\strut member} \colorbox{red!1}{\strut sign} \colorbox{red!0}{\strut up} \colorbox{red!1}{\strut only} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Coupon} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut present} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut recieve} \colorbox{red!3}{\strut offer} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Valid} \colorbox{red!1}{\strut January} \colorbox{red!2}{\strut 1} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009-December} \colorbox{red!1}{\strut 30} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut 2009} \colorbox{red!1}{\strut .} \colorbox{red!11}{\strut Gambling} \colorbox{red!0}{\strut Problem} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut CALL} \colorbox{red!0}{\strut 1-800-9-WITH-IT} \colorbox{red!2}{\strut !} \colorbox{red!3}{\strut Expires} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut 30} \colorbox{red!0}{\strut December} \colorbox{red!1}{\strut 2009} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!2}{\strut us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Feedback} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Advertising} \colorbox{red!44}{\strut CASINO} \colorbox{red!7}{\strut CITY} \colorbox{red!1}{\strut NETWORK} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Online} \colorbox{red!44}{\strut Casino} \colorbox{red!7}{\strut City} \colorbox{red!0}{\strut .} \colorbox{red!44}{\strut Casino} \colorbox{red!7}{\strut City} \colorbox{red!0}{\strut Times} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RGT} \colorbox{red!1}{\strut Online} \colorbox{red!0}{\strut .} \colorbox{red!44}{\strut Casino} \colorbox{red!7}{\strut City} \colorbox{red!1}{\strut Press} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GBDonline} \colorbox{red!44}{\strut Casino} \colorbox{red!7}{\strut City} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut independent} \colorbox{red!1}{\strut directory} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut information} \colorbox{red!1}{\strut service} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut affiliated} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut any} \colorbox{red!44}{\strut casino} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

query: gmat prep classes

101:gmat, 64:prep, 60:cost, 44:class, 34:course, 22:classroom, 21:test, 19:cat, 18:training, 18:exams


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!18}{\strut Order} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut About} \colorbox{red!4}{\strut Us} \colorbox{red!1}{\strut FAQ} \colorbox{red!3}{\strut Contact} \colorbox{red!4}{\strut Us} \colorbox{red!4}{\strut Home} \colorbox{red!18}{\strut Order} \colorbox{red!100}{\strut GMAT} \colorbox{red!67}{\strut Prep} \colorbox{red!18}{\strut Order} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut 800score.com} \colorbox{red!67}{\strut Prep} \colorbox{red!36}{\strut Course} \colorbox{red!1}{\strut with} \colorbox{red!3}{\strut 5} \colorbox{red!100}{\strut GMAT} \colorbox{red!19}{\strut exams} \colorbox{red!1}{\strut .} \colorbox{red!100}{\strut GMAT} \colorbox{red!5}{\strut Sections} \colorbox{red!4}{\strut Download} \colorbox{red!3}{\strut 5} \colorbox{red!100}{\strut GMAT} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut Essay} \colorbox{red!0}{\strut Section} \colorbox{red!5}{\strut Guide} \colorbox{red!13}{\strut Math} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Verbal} \colorbox{red!5}{\strut Guide} \colorbox{red!100}{\strut GMAT} \colorbox{red!4}{\strut Resources} \colorbox{red!5}{\strut Intro} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!100}{\strut GMAT} \colorbox{red!2}{\strut 24} \colorbox{red!18}{\strut Hour} \colorbox{red!9}{\strut Tutor} \colorbox{red!8}{\strut Support} \colorbox{red!4}{\strut Free} \colorbox{red!12}{\strut Practice} \colorbox{red!0}{\strut Essays} \colorbox{red!4}{\strut Free} \colorbox{red!100}{\strut GMAT} \colorbox{red!4}{\strut Download} \colorbox{red!22}{\strut Test} \colorbox{red!11}{\strut Pacer} \colorbox{red!19}{\strut Training} \colorbox{red!100}{\strut GMAT} \colorbox{red!13}{\strut Online} \colorbox{red!67}{\strut Prep} \colorbox{red!36}{\strut Course} \colorbox{red!100}{\strut GMAT} \colorbox{red!23}{\strut Classroom} \colorbox{red!36}{\strut Course} \colorbox{red!5}{\strut Find} \colorbox{red!1}{\strut a} \colorbox{red!100}{\strut GMAT} \colorbox{red!46}{\strut Class} \colorbox{red!0}{\strut While} \colorbox{red!9}{\strut 800score} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut value-priced} \colorbox{red!13}{\strut online} \colorbox{red!36}{\strut course} \colorbox{red!3}{\strut product} \colorbox{red!1}{\strut with} \colorbox{red!0}{\strut 500} \colorbox{red!12}{\strut pages} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut content} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut 5} \colorbox{red!100}{\strut GMAT} \colorbox{red!20}{\strut CAT} \colorbox{red!0}{\strut tests} \colorbox{red!3}{\strut for} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 39.95} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut many} \colorbox{red!13}{\strut students} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut cost-no-object} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut approach} \colorbox{red!2}{\strut to} \colorbox{red!100}{\strut GMAT} \colorbox{red!67}{\strut prep} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut those} \colorbox{red!7}{\strut who} \colorbox{red!0}{\strut prefer} \colorbox{red!1}{\strut a} \colorbox{red!23}{\strut classroom} \colorbox{red!0}{\strut environment} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut these} \colorbox{red!100}{\strut GMAT} \colorbox{red!23}{\strut classroom} \colorbox{red!67}{\strut prep} \colorbox{red!6}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Veritas} \colorbox{red!67}{\strut Prep} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut recently} \colorbox{red!2}{\strut profiled} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut BusinessWeek} \colorbox{red!4}{\strut magazine} \colorbox{red!2}{\strut as} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut rapidly} \colorbox{red!0}{\strut growing} \colorbox{red!100}{\strut GMAT} \colorbox{red!67}{\strut prep} \colorbox{red!0}{\strut company} \colorbox{red!1}{\strut with} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 5,000} \colorbox{red!100}{\strut GMAT} \colorbox{red!13}{\strut students} \colorbox{red!3}{\strut at} \colorbox{red!0}{\strut 65} \colorbox{red!7}{\strut locations} \colorbox{red!6}{\strut worldwide} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Their} \colorbox{red!6}{\strut admissions} \colorbox{red!1}{\strut consultant} \colorbox{red!5}{\strut service} \colorbox{red!2}{\strut has} \colorbox{red!0}{\strut former} \colorbox{red!6}{\strut admissions} \colorbox{red!2}{\strut officers} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut top} \colorbox{red!0}{\strut 20} \colorbox{red!5}{\strut business} \colorbox{red!8}{\strut schools} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut 2000} \colorbox{red!12}{\strut pages} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut materials} \colorbox{red!0}{\strut 15} \colorbox{red!12}{\strut practice} \colorbox{red!0}{\strut tests} \colorbox{red!0}{\strut 42} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!46}{\strut class} \colorbox{red!9}{\strut instruction} \colorbox{red!0}{\strut Unlimited} \colorbox{red!7}{\strut instructor} \colorbox{red!4}{\strut phone} \colorbox{red!1}{\strut and} \colorbox{red!5}{\strut email} \colorbox{red!0}{\strut tutoring} \colorbox{red!8}{\strut support} \colorbox{red!0}{\strut Instructors} \colorbox{red!1}{\strut have} \colorbox{red!14}{\strut scored} \colorbox{red!0}{\strut above} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut 99th} \colorbox{red!4}{\strut percentile} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 760} \colorbox{red!100}{\strut GMAT} \colorbox{red!2}{\strut .} \colorbox{red!23}{\strut Classroom} \colorbox{red!0}{\strut Products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Weekend} \colorbox{red!2}{\strut Focus} \colorbox{red!36}{\strut course} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 700} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 42-hour} \colorbox{red!36}{\strut course} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 1400} \colorbox{red!13}{\strut Online} \colorbox{red!0}{\strut courses} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 750} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 1100} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut live} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Continue} \colorbox{red!2}{\strut to} \colorbox{red!14}{\strut Veritas} \colorbox{red!67}{\strut Prep} \colorbox{red!0}{\strut s} \colorbox{red!100}{\strut GMAT} \colorbox{red!0}{\strut Classes} \colorbox{red!0}{\strut ManhattanGMAT} \colorbox{red!2}{\strut is} \colorbox{red!5}{\strut limited} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!4}{\strut cities} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut New} \colorbox{red!5}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut LA} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Chicago} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut DC} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Boston} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Austin} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut Philladelphia} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!2}{\strut has} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut great} \colorbox{red!1}{\strut reputation} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut clients} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Goldman} \colorbox{red!3}{\strut Sachs} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut JP} \colorbox{red!0}{\strut Morgan} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut 1500} \colorbox{red!12}{\strut pages} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut materials} \colorbox{red!2}{\strut 6} \colorbox{red!12}{\strut practice} \colorbox{red!100}{\strut GMAT} \colorbox{red!20}{\strut CAT} \colorbox{red!0}{\strut tests} \colorbox{red!0}{\strut 40} \colorbox{red!3}{\strut full} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!46}{\strut class} \colorbox{red!9}{\strut instruction} \colorbox{red!0}{\strut Instructors} \colorbox{red!1}{\strut have} \colorbox{red!14}{\strut scored} \colorbox{red!0}{\strut above} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut 99th} \colorbox{red!4}{\strut percentile} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 760} \colorbox{red!100}{\strut GMAT} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Location} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 138} \colorbox{red!2}{\strut West} \colorbox{red!0}{\strut 25th} \colorbox{red!2}{\strut Street} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 9th} \colorbox{red!2}{\strut floor} \colorbox{red!6}{\strut New} \colorbox{red!5}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut NY} \colorbox{red!3}{\strut Continue} \colorbox{red!2}{\strut to} 
}}}
\end{CJK*}

98:prep, 97:preparatory, 97:gmat, 85:class, 26:test, 19:programs, 16:preparation, 15:exam, 14:locations, 14:education


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Academic} \colorbox{red!5}{\strut Credit} \colorbox{red!6}{\strut Academic} \colorbox{red!4}{\strut Noncredit} \colorbox{red!5}{\strut Distance} \colorbox{red!6}{\strut Education} \colorbox{red!3}{\strut English} \colorbox{red!2}{\strut Language} \colorbox{red!2}{\strut Lifelong} \colorbox{red!3}{\strut Learning} \colorbox{red!2}{\strut Osher} \colorbox{red!0}{\strut Institute} \colorbox{red!2}{\strut Professional} \colorbox{red!6}{\strut Education} \colorbox{red!2}{\strut Technology} \colorbox{red!6}{\strut Education} \colorbox{red!12}{\strut Test} \colorbox{red!7}{\strut Preparation} \colorbox{red!2}{\strut Youth} \colorbox{red!6}{\strut Education} \colorbox{red!0}{\strut All} \colorbox{red!9}{\strut Programs} \colorbox{red!6}{\strut Locations} \colorbox{red!46}{\strut GMAT} \colorbox{red!46}{\strut Preparatory} \colorbox{red!40}{\strut Class} \colorbox{red!2}{\strut Our} \colorbox{red!46}{\strut preparatory} \colorbox{red!0}{\strut program} \colorbox{red!3}{\strut offers} \colorbox{red!1}{\strut a} \colorbox{red!40}{\strut class} \colorbox{red!1}{\strut designed} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut do} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!46}{\strut GMAT} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut improve} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut chances} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut gaining} \colorbox{red!3}{\strut admission} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut graduate} \colorbox{red!4}{\strut schools} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut business} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut comprehensive} \colorbox{red!40}{\strut class} \colorbox{red!0}{\strut covers} \colorbox{red!0}{\strut each} \colorbox{red!2}{\strut section} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut exam} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut provides} \colorbox{red!2}{\strut strategies} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut suggestions} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut improve} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut performance} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut lets} \colorbox{red!0}{\strut you} \colorbox{red!4}{\strut practice} \colorbox{red!2}{\strut for} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut analytical} \colorbox{red!3}{\strut writing} \colorbox{red!4}{\strut assessment} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut includes} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut practice} \colorbox{red!0}{\strut exams} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Once} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!2}{\strut paid} \colorbox{red!2}{\strut for} \colorbox{red!1}{\strut a} \colorbox{red!46}{\strut preparatory} \colorbox{red!40}{\strut class} \colorbox{red!2}{\strut with} \colorbox{red!2}{\strut us} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!2}{\strut come} \colorbox{red!2}{\strut back} \colorbox{red!0}{\strut any} \colorbox{red!3}{\strut time} \colorbox{red!0}{\strut within} \colorbox{red!2}{\strut the} \colorbox{red!1}{\strut next} \colorbox{red!1}{\strut 3} \colorbox{red!4}{\strut years} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut retake} \colorbox{red!2}{\strut the} \colorbox{red!40}{\strut class} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut charge} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut extra} \colorbox{red!2}{\strut material} \colorbox{red!5}{\strut costs} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut included} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut upon} \colorbox{red!1}{\strut available} \colorbox{red!1}{\strut space} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut dates} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut times} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut registration} \colorbox{red!0}{\strut information} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut classes} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut view} \colorbox{red!1}{\strut a} \colorbox{red!5}{\strut syllabus} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Cart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut All} \colorbox{red!47}{\strut Prep} \colorbox{red!0}{\strut Classes} \colorbox{red!46}{\strut GMAT} \colorbox{red!3}{\strut GRE} \colorbox{red!4}{\strut LSAT} \colorbox{red!1}{\strut Meet} \colorbox{red!2}{\strut Our} \colorbox{red!3}{\strut Instructors} \colorbox{red!0}{\strut Frequently} \colorbox{red!1}{\strut Asked} \colorbox{red!1}{\strut Questions} \colorbox{red!0}{\strut about} \colorbox{red!47}{\strut Prep} \colorbox{red!0}{\strut Classes} \colorbox{red!2}{\strut Already} \colorbox{red!1}{\strut a} \colorbox{red!12}{\strut Test} \colorbox{red!47}{\strut Prep} \colorbox{red!4}{\strut student} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Login} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut WebCT} \colorbox{red!12}{\strut Test} \colorbox{red!47}{\strut Prep} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut 2008} \colorbox{red!2}{\strut Continuing} \colorbox{red!6}{\strut Education} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Utah} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut reserved} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 1901} \colorbox{red!0}{\strut E.} \colorbox{red!2}{\strut South} \colorbox{red!2}{\strut Campus} \colorbox{red!0}{\strut Dr.} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1215} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Salt} \colorbox{red!1}{\strut Lake} \colorbox{red!3}{\strut City} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut UT} \colorbox{red!0}{\strut 84112-9359} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 801-581-5361} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut fax} \colorbox{red!0}{\strut 801-585-5414} \colorbox{red!1}{\strut Questions} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Comments} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Contact} \colorbox{red!2}{\strut us} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Disclaimer} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

query: djs

103:djs, 66:how, 53:what, 27:find, 27:disc, 23:where, 15:hired, 14:jockey, 13:current, 11:party


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 1-800-DJS-ARE-US} \colorbox{red!15}{\strut Party} \colorbox{red!8}{\strut Supply} \colorbox{red!0}{\strut Store-} \colorbox{red!9}{\strut Click} \colorbox{red!0}{\strut Here} \colorbox{red!8}{\strut America} \colorbox{red!0}{\strut s} \colorbox{red!36}{\strut Disc} \colorbox{red!19}{\strut Jockey} \colorbox{red!9}{\strut Resource} \colorbox{red!0}{\strut 1800djsareus.com} \colorbox{red!15}{\strut Looking} \colorbox{red!8}{\strut for} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut DJ} \colorbox{red!2}{\strut ?} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut can} \colorbox{red!6}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!36}{\strut find} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut DJ} \colorbox{red!5}{\strut near} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut To} \colorbox{red!0}{\strut get} \colorbox{red!13}{\strut started} \colorbox{red!0}{\strut ,} \colorbox{red!9}{\strut click} \colorbox{red!1}{\strut on} \colorbox{red!36}{\strut Find} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut DJ} \colorbox{red!0}{\strut or} \colorbox{red!9}{\strut click} \colorbox{red!1}{\strut on} \colorbox{red!5}{\strut a} \colorbox{red!6}{\strut State} \colorbox{red!31}{\strut where} \colorbox{red!0}{\strut your} \colorbox{red!8}{\strut event} \colorbox{red!0}{\strut is} \colorbox{red!5}{\strut taking} \colorbox{red!6}{\strut place} \colorbox{red!2}{\strut .} \colorbox{red!36}{\strut Find} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut DJ} \colorbox{red!2}{\strut Are} \colorbox{red!0}{\strut you} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut DJ} \colorbox{red!2}{\strut ?} \colorbox{red!9}{\strut Click} \colorbox{red!0}{\strut Here} \colorbox{red!8}{\strut for} \colorbox{red!5}{\strut info} \colorbox{red!1}{\strut on} \colorbox{red!90}{\strut how} \colorbox{red!5}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!6}{\strut listed} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Renew} \colorbox{red!6}{\strut Monthly} \colorbox{red!0}{\strut DJ} \colorbox{red!0}{\strut Listing} \colorbox{red!8}{\strut -} \colorbox{red!8}{\strut For} \colorbox{red!12}{\strut past} \colorbox{red!0}{\strut DJ} \colorbox{red!9}{\strut members} \colorbox{red!5}{\strut Renew} \colorbox{red!6}{\strut Annual} \colorbox{red!0}{\strut DJ} \colorbox{red!0}{\strut Listing} \colorbox{red!8}{\strut -} \colorbox{red!8}{\strut For} \colorbox{red!12}{\strut past} \colorbox{red!0}{\strut DJ} \colorbox{red!9}{\strut members} \colorbox{red!0}{\strut Cancel} \colorbox{red!0}{\strut DJ} \colorbox{red!0}{\strut Listing} \colorbox{red!8}{\strut -} \colorbox{red!8}{\strut For} \colorbox{red!17}{\strut current} \colorbox{red!0}{\strut DJ} \colorbox{red!9}{\strut members} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Never} \colorbox{red!20}{\strut hired} \colorbox{red!5}{\strut a} \colorbox{red!36}{\strut disc} \colorbox{red!19}{\strut jockey} \colorbox{red!1}{\strut before} \colorbox{red!2}{\strut ?} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut article} \colorbox{red!5}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!72}{\strut what} \colorbox{red!5}{\strut to} \colorbox{red!0}{\strut look} \colorbox{red!8}{\strut for} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut DJ} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!72}{\strut What} \colorbox{red!5}{\strut to} \colorbox{red!0}{\strut look} \colorbox{red!8}{\strut for} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut a} \colorbox{red!0}{\strut DJ} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Copyright} \colorbox{red!0}{\strut 1999-2008} \colorbox{red!0}{\strut DJ} \colorbox{red!0}{\strut S} \colorbox{red!2}{\strut ARE} \colorbox{red!9}{\strut US} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut our} \colorbox{red!2}{\strut site} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!4}{\strut agree} \colorbox{red!5}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!9}{\strut terms} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut conditions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut use} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut To} \colorbox{red!5}{\strut advertise} \colorbox{red!1}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut site} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut email} \colorbox{red!0}{\strut your} \colorbox{red!12}{\strut request} \colorbox{red!5}{\strut to} \colorbox{red!0}{\strut webmaster} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Free} \colorbox{red!0}{\strut Clipart} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Photos} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.ace-clipart.com} \colorbox{red!6}{\strut Alabama} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut Alaska} \colorbox{red!100}{\strut DJs} \colorbox{red!6}{\strut Arizona} \colorbox{red!100}{\strut DJs} \colorbox{red!6}{\strut Arkansas} \colorbox{red!100}{\strut DJs} \colorbox{red!5}{\strut California} \colorbox{red!100}{\strut DJs} \colorbox{red!5}{\strut Colorado} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut Connecticut} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Delaware} \colorbox{red!100}{\strut DJs} \colorbox{red!5}{\strut Florida} \colorbox{red!100}{\strut DJs} \colorbox{red!5}{\strut Georgia} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut Hawaii} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Idaho} \colorbox{red!100}{\strut DJs} \colorbox{red!5}{\strut Illinois} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Indiana} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Iowa} \colorbox{red!100}{\strut DJs} \colorbox{red!6}{\strut Kansas} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Kentucky} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Louisiana} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut Maine} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Maryland} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut Massachusetts} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut Michigan} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Minnesota} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Mississippi} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Missouri} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Montana} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Nebraska} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Nevada} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut New} \colorbox{red!0}{\strut Hampshire} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut New} \colorbox{red!5}{\strut Jersey} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut New} \colorbox{red!0}{\strut Mexico} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Carolina} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Dakota} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut Ohio} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut Oklahoma} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Oregon} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Pennsylvania} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Rhode} \colorbox{red!1}{\strut Island} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Carolina} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Dakota} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Tennessee} \colorbox{red!100}{\strut DJs} \colorbox{red!6}{\strut Texas} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Utah} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Vermont} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Virginia} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Washington} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut Virginia} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Wisconsin} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Wyoming} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Los} \colorbox{red!0}{\strut Angeles} \colorbox{red!100}{\strut DJs} \colorbox{red!8}{\strut Chicago} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut Houston} \colorbox{red!100}{\strut DJs} \colorbox{red!6}{\strut Arkansas} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut Philadelphia} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Phoenix} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Diego} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Antonio} \colorbox{red!100}{\strut DJs} \colorbox{red!2}{\strut Dallas} \colorbox{red!100}{\strut DJs} \colorbox{red!4}{\strut Detroit} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut Hawaii} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Jose} 
}}}
\end{CJK*}

104:djs, 95:miami, 34:florida, 21:party, 12:disc, 8:when, 7:weddings, 7:south, 7:jockeys, 6:professional


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Miami} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Miami} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!3}{\strut Planners} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Entertainment} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!8}{\strut Weddings} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Mobile} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Professional} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!100}{\strut djs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut miami} \colorbox{red!100}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Miami} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!3}{\strut Planners} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Entertainment} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!8}{\strut Weddings} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Mobile} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Professional} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!100}{\strut djs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut miami} \colorbox{red!100}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Miami} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!3}{\strut Planners} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Entertainment} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!8}{\strut Weddings} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Mobile} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Professional} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!100}{\strut djs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut miami} \colorbox{red!100}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Miami} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!3}{\strut Planners} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Entertainment} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!8}{\strut Weddings} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Mobile} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Professional} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!100}{\strut djs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut miami} \colorbox{red!100}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Miami} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!3}{\strut Planners} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Entertainment} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!8}{\strut Weddings} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Mobile} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Professional} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!100}{\strut djs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut miami} \colorbox{red!100}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut DJs} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Miami} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!3}{\strut Planners} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!0}{\strut Parties} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Entertainment} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut South} \colorbox{red!41}{\strut Florida} \colorbox{red!14}{\strut Disc} \colorbox{red!8}{\strut Jockeys} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!8}{\strut Weddings} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Mobile} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!7}{\strut Professional} \colorbox{red!100}{\strut DJs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut Miami} \colorbox{red!25}{\strut Party} \colorbox{red!100}{\strut djs} \colorbox{red!1}{\strut ,} \colorbox{red!100}{\strut miami} \colorbox{red!100}{\strut djs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut ,} 
}}}
\end{CJK*}

query: espn sports

100:espn, 59:network, 24:company, 23:sports, 22:radio, 21:news, 21:magazine, 21:businesses, 20:international, 20:classic


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!25}{\strut businesses} \colorbox{red!4}{\strut include} \colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut ,} \colorbox{red!12}{\strut ESPN2} \colorbox{red!6}{\strut ,} \colorbox{red!3}{\strut ESPNEWS} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!24}{\strut Classic} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut ESPN.com} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!26}{\strut Radio} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!24}{\strut International} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut The} \colorbox{red!25}{\strut Magazine} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!14}{\strut Regional} \colorbox{red!21}{\strut Television} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!16}{\strut Deportes} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!19}{\strut ENTERPRISES} \colorbox{red!4}{\strut and} \colorbox{red!100}{\strut ESPN} \colorbox{red!8}{\strut Outdoors} \colorbox{red!6}{\strut ,} \colorbox{red!15}{\strut which} \colorbox{red!0}{\strut includes} \colorbox{red!12}{\strut BASS} \colorbox{red!8}{\strut .} \colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!6}{\strut ,} \colorbox{red!3}{\strut with} \colorbox{red!4}{\strut its} \colorbox{red!2}{\strut critically} \colorbox{red!3}{\strut acclaimed} \colorbox{red!27}{\strut sports} \colorbox{red!25}{\strut news} \colorbox{red!4}{\strut and} \colorbox{red!9}{\strut live} \colorbox{red!8}{\strut event} \colorbox{red!9}{\strut coverage} \colorbox{red!6}{\strut ,} \colorbox{red!3}{\strut has} \colorbox{red!7}{\strut established} \colorbox{red!4}{\strut itself} \colorbox{red!2}{\strut as} \colorbox{red!6}{\strut the} \colorbox{red!12}{\strut worldwide} \colorbox{red!6}{\strut leader} \colorbox{red!2}{\strut in} \colorbox{red!27}{\strut sports} \colorbox{red!8}{\strut .} \colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!3}{\strut has} \colorbox{red!6}{\strut grown} \colorbox{red!0}{\strut from} \colorbox{red!6}{\strut the} \colorbox{red!0}{\strut first-ever} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut 24-hour} \colorbox{red!27}{\strut sports} \colorbox{red!71}{\strut network} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut consist} \colorbox{red!7}{\strut today} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut four} \colorbox{red!7}{\strut domestic} \colorbox{red!21}{\strut television} \colorbox{red!0}{\strut networks} \colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut ,} \colorbox{red!12}{\strut ESPN2} \colorbox{red!6}{\strut ,} \colorbox{red!100}{\strut ESPN} \colorbox{red!24}{\strut Classic} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut ESPNEWS} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut 24} \colorbox{red!100}{\strut ESPN} \colorbox{red!24}{\strut international} \colorbox{red!0}{\strut networks} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut 11} \colorbox{red!7}{\strut languages} \colorbox{red!6}{\strut ,} \colorbox{red!2}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!2}{\strut as} \colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut The} \colorbox{red!25}{\strut Magazine} \colorbox{red!6}{\strut ,} \colorbox{red!4}{\strut a} \colorbox{red!4}{\strut provocative} \colorbox{red!4}{\strut and} \colorbox{red!1}{\strut innovative} \colorbox{red!10}{\strut biweekly} \colorbox{red!14}{\strut publication} \colorbox{red!8}{\strut .} \colorbox{red!100}{\strut ESPN} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut includes} \colorbox{red!100}{\strut ESPN} \colorbox{red!14}{\strut Regional} \colorbox{red!21}{\strut Television} \colorbox{red!6}{\strut ,} \colorbox{red!6}{\strut the} \colorbox{red!6}{\strut nation} \colorbox{red!0}{\strut s} \colorbox{red!13}{\strut largest} \colorbox{red!27}{\strut sports} \colorbox{red!18}{\strut syndication} \colorbox{red!29}{\strut company} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut SportsTicker} \colorbox{red!6}{\strut ,} \colorbox{red!4}{\strut a} \colorbox{red!0}{\strut 24-hour} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut real-time} \colorbox{red!27}{\strut sports} \colorbox{red!25}{\strut news} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut information} \colorbox{red!10}{\strut service} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut pay} \colorbox{red!9}{\strut subscription} \colorbox{red!6}{\strut packages} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut consumer} \colorbox{red!10}{\strut products} \colorbox{red!0}{\strut including} \colorbox{red!6}{\strut video} \colorbox{red!12}{\strut games} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut compact} \colorbox{red!7}{\strut discs} \colorbox{red!8}{\strut .} \colorbox{red!6}{\strut Opportunities} \colorbox{red!4}{\strut are} \colorbox{red!20}{\strut located} \colorbox{red!3}{\strut primarily} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut Bristol} \colorbox{red!6}{\strut ,} \colorbox{red!6}{\strut CT} \colorbox{red!4}{\strut and} \colorbox{red!6}{\strut New} \colorbox{red!3}{\strut York} \colorbox{red!6}{\strut ,} \colorbox{red!6}{\strut NY} \colorbox{red!8}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!4}{\strut information} \colorbox{red!6}{\strut about} \colorbox{red!10}{\strut openings} \colorbox{red!6}{\strut ,} \colorbox{red!1}{\strut visit} \colorbox{red!0}{\strut joinourteam.espn.com} \colorbox{red!8}{\strut .} 
}}}
\end{CJK*}

95:espn, 93:sports, 63:networks, 42:airing, 30:tv, 28:date, 22:schedule, 21:days, 21:abc, 20:who


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!42}{\strut ESPN} \colorbox{red!5}{\strut Search} \colorbox{red!13}{\strut TV} \colorbox{red!7}{\strut RADIO} \colorbox{red!4}{\strut MAGAZINE} \colorbox{red!3}{\strut INSIDER} \colorbox{red!2}{\strut PODCENTER} \colorbox{red!2}{\strut ESPN360} \colorbox{red!0}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut a.espncdn.comprod} \colorbox{red!0}{\strut https} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut r.espn.go.com} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut U} \colorbox{red!0}{\strut false} \colorbox{red!3}{\strut Register} \colorbox{red!2}{\strut Now} \colorbox{red!0}{\strut myESPN} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Sign} \colorbox{red!1}{\strut In} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Search} \colorbox{red!0}{\strut ESPN.com} \colorbox{red!0}{\strut ESPNTV.com} \colorbox{red!1}{\strut Index} \colorbox{red!5}{\strut Listings} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!42}{\strut sports} \colorbox{red!18}{\strut airing} \colorbox{red!5}{\strut on} \colorbox{red!3}{\strut the} \colorbox{red!42}{\strut ESPN} \colorbox{red!3}{\strut and} \colorbox{red!9}{\strut ABC} \colorbox{red!42}{\strut Sports} \colorbox{red!28}{\strut networks} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Refine} \colorbox{red!5}{\strut Search} \colorbox{red!1}{\strut Outdoors} \colorbox{red!0}{\strut By} \colorbox{red!2}{\strut Type} \colorbox{red!1}{\strut Stories} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1055} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Photo} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 90} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!12}{\strut Date} \colorbox{red!5}{\strut Last} \colorbox{red!1}{\strut 7} \colorbox{red!9}{\strut Days} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 9} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Last} \colorbox{red!2}{\strut 30} \colorbox{red!9}{\strut Days} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 15} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Last} \colorbox{red!0}{\strut 365} \colorbox{red!9}{\strut Days} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 112} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Past} \colorbox{red!4}{\strut Years} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 1034} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Sport} \colorbox{red!4}{\strut NFL} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 16} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Racing} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 15} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut Golf} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 9} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut NHL} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut NBA} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Columnist} \colorbox{red!0}{\strut Ron} \colorbox{red!0}{\strut Schara} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 97} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Lynn} \colorbox{red!1}{\strut Burkhead} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Ken} \colorbox{red!1}{\strut Schultz} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 32} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut George} \colorbox{red!2}{\strut Poveromo} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 27} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Sam} \colorbox{red!0}{\strut Eifling} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 26} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Andrew} \colorbox{red!0}{\strut Canulette} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 15} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Angie} \colorbox{red!0}{\strut Thompson} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut 9} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut 1145} \colorbox{red!1}{\strut Results} \colorbox{red!2}{\strut for} \colorbox{red!5}{\strut espn2} \colorbox{red!1}{\strut 1} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut 77} \colorbox{red!0}{\strut Day} \colorbox{red!5}{\strut On} \colorbox{red!3}{\strut The} \colorbox{red!6}{\strut Lake} \colorbox{red!5}{\strut features} \colorbox{red!1}{\strut Kevin} \colorbox{red!0}{\strut Langill} \colorbox{red!0}{\strut ESPNOutdoors.com} \colorbox{red!4}{\strut Staff} \colorbox{red!0}{\strut Day} \colorbox{red!5}{\strut On} \colorbox{red!3}{\strut The} \colorbox{red!6}{\strut Lake} \colorbox{red!5}{\strut features} \colorbox{red!1}{\strut Kevin} \colorbox{red!0}{\strut Langill} \colorbox{red!0}{\strut Story} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Conversation} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut January} \colorbox{red!2}{\strut 16} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut 2009} \colorbox{red!0}{\strut Day} \colorbox{red!5}{\strut On} \colorbox{red!3}{\strut The} \colorbox{red!6}{\strut Lake} \colorbox{red!5}{\strut features} \colorbox{red!2}{\strut Gary} \colorbox{red!4}{\strut Klein} \colorbox{red!0}{\strut ESPNOutdoors.com} \colorbox{red!4}{\strut Staff} \colorbox{red!0}{\strut Day} \colorbox{red!5}{\strut On} \colorbox{red!3}{\strut The} \colorbox{red!6}{\strut Lake} \colorbox{red!5}{\strut features} \colorbox{red!2}{\strut Gary} \colorbox{red!4}{\strut Klein} \colorbox{red!0}{\strut Story} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Conversation} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut January} \colorbox{red!2}{\strut 16} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut 2009} \colorbox{red!3}{\strut The} \colorbox{red!0}{\strut overlooked} \colorbox{red!2}{\strut Miami} \colorbox{red!2}{\strut George} \colorbox{red!2}{\strut Poveromo} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ESPNOutdoors.com} \colorbox{red!2}{\strut Poveromo} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut World} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut Saltwater} \colorbox{red!1}{\strut Fishing} \colorbox{red!0}{\strut Story} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Conversation} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut January} \colorbox{red!2}{\strut 16} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut 2009} \colorbox{red!0}{\strut Saltwater} \colorbox{red!5}{\strut Series} \colorbox{red!3}{\strut unveils} \colorbox{red!3}{\strut 2009} \colorbox{red!9}{\strut schedule} \colorbox{red!0}{\strut ESPNOutdoors.com} \colorbox{red!4}{\strut Staff} \colorbox{red!0}{\strut Saltwater} \colorbox{red!5}{\strut Series} \colorbox{red!3}{\strut unveils} \colorbox{red!3}{\strut 2009} \colorbox{red!9}{\strut schedule} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut includes} \colorbox{red!1}{\strut five} \colorbox{red!0}{\strut redbone} \colorbox{red!3}{\strut events} \colorbox{red!0}{\strut Story} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Conversation} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut January} \colorbox{red!2}{\strut 15} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut 2009} \colorbox{red!0}{\strut Saltwater} \colorbox{red!5}{\strut Series} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut include} \colorbox{red!1}{\strut IGFA} \colorbox{red!1}{\strut Inshore} \colorbox{red!0}{\strut ESPNOutdoors.com} \colorbox{red!3}{\strut Florida} \colorbox{red!1}{\strut Keys} \colorbox{red!1}{\strut Outfitters} \colorbox{red!1}{\strut IGFA} \colorbox{red!1}{\strut Inshore} \colorbox{red!3}{\strut World} \colorbox{red!2}{\strut Championship} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut part} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut 2009} \colorbox{red!5}{\strut series} \colorbox{red!0}{\strut Story} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Conversation} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut January} \colorbox{red!1}{\strut 13} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut 2009} \colorbox{red!4}{\strut Elite} \colorbox{red!2}{\strut pro} \colorbox{red!0}{\strut Byron} \colorbox{red!0}{\strut Velvick} \colorbox{red!7}{\strut starts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Going} \colorbox{red!2}{\strut Coastal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ESPNOutdoors.com} \colorbox{red!4}{\strut Staff} \colorbox{red!4}{\strut Elite} \colorbox{red!2}{\strut pro} \colorbox{red!0}{\strut Byron} \colorbox{red!0}{\strut Velvick} \colorbox{red!7}{\strut starts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Going} \colorbox{red!2}{\strut Coastal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Story} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Conversation} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut January} \colorbox{red!2}{\strut 10} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut 2009} \colorbox{red!0}{\strut Day} 
}}}
\end{CJK*}

query: arizona game fish

95:fish, 76:arizona, 42:number, 39:licenses, 29:state, 21:hunting, 18:records, 14:trout, 14:game, 14:az


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut FinTalk} \colorbox{red!3}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Fish} \colorbox{red!2}{\strut .} \colorbox{red!15}{\strut Game} \colorbox{red!3}{\strut Main} \colorbox{red!0}{\strut .} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!7}{\strut Information} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut fishing} \colorbox{red!7}{\strut information} \colorbox{red!2}{\strut includes} \colorbox{red!3}{\strut links} \colorbox{red!4}{\strut to} \colorbox{red!4}{\strut many} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut fishing} \colorbox{red!4}{\strut related} \colorbox{red!4}{\strut web} \colorbox{red!5}{\strut sites} \colorbox{red!5}{\strut ,} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut fishing} \colorbox{red!7}{\strut resources} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut the} \colorbox{red!86}{\strut Arizona} \colorbox{red!100}{\strut Fish} \colorbox{red!2}{\strut .} \colorbox{red!15}{\strut Game} \colorbox{red!6}{\strut Department} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut If} \colorbox{red!3}{\strut you} \colorbox{red!4}{\strut are} \colorbox{red!5}{\strut heading} \colorbox{red!4}{\strut out} \colorbox{red!3}{\strut on} \colorbox{red!3}{\strut a} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut fishing} \colorbox{red!3}{\strut trip} \colorbox{red!4}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut many} \colorbox{red!5}{\strut reserviors} \colorbox{red!4}{\strut and} \colorbox{red!9}{\strut lakes} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!33}{\strut state} \colorbox{red!0}{\strut then} \colorbox{red!1}{\strut these} \colorbox{red!7}{\strut resources} \colorbox{red!4}{\strut will} \colorbox{red!4}{\strut help} \colorbox{red!3}{\strut you} \colorbox{red!3}{\strut on} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut way} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut Find} \colorbox{red!7}{\strut information} \colorbox{red!5}{\strut for} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut fishing} \colorbox{red!44}{\strut licenses} \colorbox{red!5}{\strut ,} \colorbox{red!23}{\strut hunting} \colorbox{red!44}{\strut licenses} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut fishing} \colorbox{red!20}{\strut records} \colorbox{red!3}{\strut .} \colorbox{red!86}{\strut ARIZONA} \colorbox{red!100}{\strut Fish} \colorbox{red!2}{\strut .} \colorbox{red!15}{\strut Game} \colorbox{red!6}{\strut Department} \colorbox{red!3}{\strut 2222} \colorbox{red!4}{\strut West} \colorbox{red!5}{\strut Greenway} \colorbox{red!5}{\strut Road} \colorbox{red!12}{\strut Phoenix} \colorbox{red!5}{\strut ,} \colorbox{red!15}{\strut AZ} \colorbox{red!0}{\strut 85023-4312} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut 602} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 942-3000} \colorbox{red!1}{\strut http} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut www.gf.state.az.us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut click} \colorbox{red!3}{\strut image} \colorbox{red!5}{\strut for} \colorbox{red!3}{\strut map} \colorbox{red!1}{\strut .} \colorbox{red!86}{\strut Arizona} \colorbox{red!100}{\strut Fish} \colorbox{red!4}{\strut and} \colorbox{red!15}{\strut Game} \colorbox{red!86}{\strut Arizona} \colorbox{red!7}{\strut Online} \colorbox{red!44}{\strut Licenses} \colorbox{red!86}{\strut Arizona} \colorbox{red!9}{\strut Public} \colorbox{red!20}{\strut Records} \colorbox{red!7}{\strut Federal} \colorbox{red!5}{\strut ,} \colorbox{red!33}{\strut State} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut and} \colorbox{red!7}{\strut Conservation} \colorbox{red!7}{\strut Resources} \colorbox{red!86}{\strut Arizona} \colorbox{red!7}{\strut Conservation} \colorbox{red!7}{\strut Resources} \colorbox{red!4}{\strut .} \colorbox{red!4}{\strut International} \colorbox{red!1}{\strut Association} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Fish} \colorbox{red!4}{\strut and} \colorbox{red!7}{\strut Wildlife} \colorbox{red!6}{\strut Agencies} \colorbox{red!15}{\strut Trout} \colorbox{red!5}{\strut Unlimited} \colorbox{red!0}{\strut -} \colorbox{red!86}{\strut Arizona} \colorbox{red!33}{\strut State} \colorbox{red!4}{\strut Chapter} \colorbox{red!86}{\strut Arizona} \colorbox{red!6}{\strut Marine} \colorbox{red!7}{\strut Conservation} \colorbox{red!3}{\strut Directory} \colorbox{red!7}{\strut Wildlife} \colorbox{red!5}{\strut for} \colorbox{red!0}{\strut Tomorrow} \colorbox{red!5}{\strut Government} \colorbox{red!7}{\strut Resources} \colorbox{red!0}{\strut -} \colorbox{red!86}{\strut Arizona} \colorbox{red!4}{\strut .} \colorbox{red!7}{\strut Federal} \colorbox{red!5}{\strut Recreation} \colorbox{red!0}{\strut --} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!7}{\strut Areas} \colorbox{red!86}{\strut Arizona} \colorbox{red!5}{\strut Farm} \colorbox{red!7}{\strut Service} \colorbox{red!0}{\strut Agency} \colorbox{red!6}{\strut Invasive} \colorbox{red!9}{\strut Species} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!20}{\strut Records} \colorbox{red!4}{\strut .} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!20}{\strut Records} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!12}{\strut Regulations} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!6}{\strut Report} \colorbox{red!4}{\strut .} \colorbox{red!4}{\strut Add} \colorbox{red!2}{\strut An} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!6}{\strut Report} \colorbox{red!6}{\strut Talk} \colorbox{red!3}{\strut about} \colorbox{red!86}{\strut Arizona} \colorbox{red!0}{\strut Fishing} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut Forum} \colorbox{red!0}{\strut Fishing} \colorbox{red!0}{\strut License} \colorbox{red!9}{\strut Info} \colorbox{red!10}{\strut Buy} \colorbox{red!0}{\strut Fishing} \colorbox{red!44}{\strut Licenses} \colorbox{red!7}{\strut Online} \colorbox{red!3}{\strut !} \colorbox{red!2}{\strut An} \colorbox{red!3}{\strut additional} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 2} \colorbox{red!12}{\strut fee} \colorbox{red!4}{\strut will} \colorbox{red!3}{\strut be} \colorbox{red!14}{\strut charged} \colorbox{red!5}{\strut for} \colorbox{red!3}{\strut this} \colorbox{red!7}{\strut service} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut You} \colorbox{red!4}{\strut will} \colorbox{red!3}{\strut be} \colorbox{red!4}{\strut provided} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut a} \colorbox{red!10}{\strut temporary} \colorbox{red!0}{\strut license} \colorbox{red!47}{\strut number} \colorbox{red!1}{\strut that} \colorbox{red!4}{\strut will} \colorbox{red!3}{\strut be} \colorbox{red!5}{\strut recognized} \colorbox{red!0}{\strut by} \colorbox{red!9}{\strut law} \colorbox{red!6}{\strut enforcement} \colorbox{red!5}{\strut officers} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut field} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut You} \colorbox{red!2}{\strut can} \colorbox{red!0}{\strut use} \colorbox{red!3}{\strut this} \colorbox{red!4}{\strut until} \colorbox{red!0}{\strut your} \colorbox{red!10}{\strut permanent} \colorbox{red!0}{\strut license} \colorbox{red!6}{\strut arrives} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut mail} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Print} \colorbox{red!5}{\strut blank} \colorbox{red!0}{\strut license} \colorbox{red!7}{\strut forms} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut fill} \colorbox{red!0}{\strut them} \colorbox{red!4}{\strut out} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut mail-in} \colorbox{red!4}{\strut to} \colorbox{red!3}{\strut the} \colorbox{red!33}{\strut state} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut For} \colorbox{red!7}{\strut information} \colorbox{red!4}{\strut regarding} \colorbox{red!44}{\strut licenses} \colorbox{red!5}{\strut ,} \colorbox{red!1}{\strut please} \colorbox{red!7}{\strut call} \colorbox{red!3}{\strut the} \colorbox{red!86}{\strut Arizona} \colorbox{red!15}{\strut Game} \colorbox{red!2}{\strut .} \colorbox{red!100}{\strut Fish} \colorbox{red!6}{\strut Department} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut 602} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 942-3000} \colorbox{red!3}{\strut .} \colorbox{red!23}{\strut Hunting} \colorbox{red!0}{\strut License} \colorbox{red!9}{\strut Info} \colorbox{red!10}{\strut Buy} \colorbox{red!23}{\strut Hunting} \colorbox{red!44}{\strut Licenses} \colorbox{red!7}{\strut Online} \colorbox{red!3}{\strut !} \colorbox{red!2}{\strut An} \colorbox{red!3}{\strut additional} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut 2} \colorbox{red!12}{\strut fee} \colorbox{red!4}{\strut will} \colorbox{red!3}{\strut be} \colorbox{red!14}{\strut charged} \colorbox{red!5}{\strut for} \colorbox{red!3}{\strut this} \colorbox{red!7}{\strut service} 
}}}
\end{CJK*}

99:fishing, 72:arizona, 62:licenses, 48:regulations, 34:limit, 28:2009, 25:10, 23:available, 20:stocking, 20:game


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut RSS} \colorbox{red!1}{\strut Feed} \colorbox{red!1}{\strut Subscribe} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Email} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut BUY} \colorbox{red!25}{\strut LICENSES} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut BIG} \colorbox{red!8}{\strut GAME} \colorbox{red!2}{\strut DRAW} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eNEWS} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut CALENDAR} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut VIDEO} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut HUNTING} \colorbox{red!0}{\strut .} \colorbox{red!41}{\strut FISHING} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut WILDLIFE} \colorbox{red!1}{\strut VIEWING} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut CONSERVATION} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut EDUCATION} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut BOATING} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SHOOTING} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut OHV} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut SITE} \colorbox{red!1}{\strut MAP} \colorbox{red!1}{\strut Southeastern} \colorbox{red!30}{\strut Arizona} \colorbox{red!5}{\strut HOLIDAY} \colorbox{red!3}{\strut CHECKLIST} \colorbox{red!2}{\strut REMINDERS} \colorbox{red!0}{\strut 2009-10} \colorbox{red!41}{\strut Fishing} \colorbox{red!20}{\strut Regulations} \colorbox{red!3}{\strut are} \colorbox{red!3}{\strut now} \colorbox{red!9}{\strut available} \colorbox{red!0}{\strut Should} \colorbox{red!5}{\strut make} \colorbox{red!0}{\strut superb} \colorbox{red!6}{\strut seasonal} \colorbox{red!8}{\strut stocking} \colorbox{red!2}{\strut stuffers} \colorbox{red!0}{\strut December} \colorbox{red!1}{\strut 22nd} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut 2008} \colorbox{red!5}{\strut PHOENIX} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Just} \colorbox{red!1}{\strut in} \colorbox{red!4}{\strut time} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut be} \colorbox{red!8}{\strut stocking} \colorbox{red!2}{\strut stuffers} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut favorite} \colorbox{red!2}{\strut outdoor} \colorbox{red!0}{\strut enthusiast} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut newly} \colorbox{red!4}{\strut printed} \colorbox{red!0}{\strut 2009-10} \colorbox{red!30}{\strut Arizona} \colorbox{red!41}{\strut Fishing} \colorbox{red!20}{\strut Regulations} \colorbox{red!3}{\strut are} \colorbox{red!3}{\strut now} \colorbox{red!9}{\strut available} \colorbox{red!2}{\strut for} \colorbox{red!5}{\strut free} \colorbox{red!2}{\strut at} \colorbox{red!0}{\strut all} \colorbox{red!41}{\strut fishing} \colorbox{red!0}{\strut license} \colorbox{red!6}{\strut dealers} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut state} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut all} \colorbox{red!30}{\strut Arizona} \colorbox{red!8}{\strut Game} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Fish} \colorbox{red!2}{\strut Department} \colorbox{red!2}{\strut offices} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut theme} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut years} \colorbox{red!41}{\strut fishing} \colorbox{red!20}{\strut regulations} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut dovetail} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut seasonal} \colorbox{red!0}{\strut spirit} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut holidays} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Kids} \colorbox{red!0}{\strut dont} \colorbox{red!0}{\strut remember} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut watching} \colorbox{red!1}{\strut television} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Whether} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut childs} \colorbox{red!2}{\strut Christmas} \colorbox{red!3}{\strut wish} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut own} \colorbox{red!3}{\strut New} \colorbox{red!0}{\strut Years} \colorbox{red!2}{\strut vow} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut take} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut children} \colorbox{red!41}{\strut fishing} \colorbox{red!0}{\strut this} \colorbox{red!5}{\strut coming} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut guarantee} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut memories} \colorbox{red!0}{\strut you} \colorbox{red!5}{\strut make} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut outlast} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut video} \colorbox{red!8}{\strut game} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut she} \colorbox{red!1}{\strut wants} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut said} \colorbox{red!4}{\strut Fisheries} \colorbox{red!0}{\strut Chief} \colorbox{red!0}{\strut Kirk} \colorbox{red!2}{\strut Young} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Dont} \colorbox{red!0}{\strut forget} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut 2009} \colorbox{red!41}{\strut fishing} \colorbox{red!25}{\strut licenses} \colorbox{red!3}{\strut are} \colorbox{red!0}{\strut also} \colorbox{red!9}{\strut available} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut license} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut ultimate} \colorbox{red!2}{\strut gift} \colorbox{red!0}{\strut that} \colorbox{red!4}{\strut keeps} \colorbox{red!1}{\strut on} \colorbox{red!6}{\strut giving} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut year} \colorbox{red!6}{\strut long} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut There} \colorbox{red!3}{\strut are} \colorbox{red!0}{\strut even} \colorbox{red!3}{\strut family} \colorbox{red!25}{\strut licenses} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut youth} \colorbox{red!2}{\strut combination} \colorbox{red!25}{\strut licenses} \colorbox{red!9}{\strut available} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Just} \colorbox{red!3}{\strut check} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut out} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut easy-to-use} \colorbox{red!0}{\strut regulation} \colorbox{red!1}{\strut booklet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thanks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Arizonas} \colorbox{red!0}{\strut abundant} \colorbox{red!0}{\strut snowpack} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut superb} \colorbox{red!1}{\strut runoff} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut filled} \colorbox{red!0}{\strut our} \colorbox{red!6}{\strut lakes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut overflowing} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut year} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!41}{\strut fishing} \colorbox{red!2}{\strut prognosis} \colorbox{red!1}{\strut going} \colorbox{red!2}{\strut into} \colorbox{red!11}{\strut 2009} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut very} \colorbox{red!6}{\strut good} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut recent} \colorbox{red!2}{\strut winter} \colorbox{red!1}{\strut storms} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut hopeful} \colorbox{red!0}{\strut promise} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut good} \colorbox{red!1}{\strut things} \colorbox{red!0}{\strut headed} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut way} \colorbox{red!0}{\strut this} \colorbox{red!5}{\strut coming} \colorbox{red!0}{\strut year} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Young} \colorbox{red!1}{\strut said} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Keep} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut mind} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut there} \colorbox{red!3}{\strut are} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut regulation} \colorbox{red!2}{\strut changes} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut heading} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut way} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut 2009-10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!8}{\strut Game} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Fish} \colorbox{red!2}{\strut Department} \colorbox{red!0}{\strut has} \colorbox{red!1}{\strut instituted} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut protective} \colorbox{red!2}{\strut slot} \colorbox{red!14}{\strut limit} 
}}}
\end{CJK*}

query: yahoo

100:yahoo, 49:privacy, 28:policy, 15:centre, 15:center, 14:email, 10:services, 10:security, 10:search, 10:practices


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!19}{\strut Asia} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!19}{\strut Search} \colorbox{red!15}{\strut Help} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!96}{\strut Privacy} \colorbox{red!29}{\strut Centre} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!15}{\strut Info} \colorbox{red!29}{\strut Center} \colorbox{red!1}{\strut .} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!96}{\strut Privacy} \colorbox{red!29}{\strut Centre} \colorbox{red!27}{\strut Email} \colorbox{red!9}{\strut Print} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!96}{\strut Privacy} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!96}{\strut Privacy} \colorbox{red!55}{\strut Policy} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut have} \colorbox{red!5}{\strut detailed} \colorbox{red!7}{\strut reference} \colorbox{red!5}{\strut links} \colorbox{red!17}{\strut describing} \colorbox{red!0}{\strut our} \colorbox{red!96}{\strut privacy} \colorbox{red!19}{\strut practices} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut wide} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!11}{\strut products} \colorbox{red!1}{\strut and} \colorbox{red!19}{\strut services} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut here} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Assistance} \colorbox{red!15}{\strut Help} \colorbox{red!11}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut My} \colorbox{red!11}{\strut Account} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!96}{\strut Privacy} \colorbox{red!29}{\strut Centre} \colorbox{red!5}{\strut Special} \colorbox{red!11}{\strut Topics} \colorbox{red!11}{\strut Cookies} \colorbox{red!13}{\strut Data} \colorbox{red!7}{\strut Storage} \colorbox{red!9}{\strut IP} \colorbox{red!9}{\strut Addresses} \colorbox{red!11}{\strut Mobile} \colorbox{red!9}{\strut Devices} \colorbox{red!5}{\strut Promotions} \colorbox{red!0}{\strut on} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!17}{\strut Research} \colorbox{red!19}{\strut Security} \colorbox{red!3}{\strut at} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!7}{\strut Third} \colorbox{red!5}{\strut Party} \colorbox{red!11}{\strut Cookies} \colorbox{red!0}{\strut on} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!11}{\strut Web} \colorbox{red!7}{\strut Beacons} \colorbox{red!11}{\strut Products} \colorbox{red!1}{\strut and} \colorbox{red!19}{\strut Services} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!0}{\strut Address} \colorbox{red!7}{\strut Book} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!5}{\strut Briefcase} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!7}{\strut Calendar} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!9}{\strut Chat} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!0}{\strut Delivers} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!7}{\strut Games} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!0}{\strut GeoCities} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!7}{\strut Greetings} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!15}{\strut Help} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!7}{\strut Mail} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!0}{\strut Messenger} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!11}{\strut Mobile} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!5}{\strut News} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!0}{\strut Notepad} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!17}{\strut People} \colorbox{red!19}{\strut Search} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!7}{\strut Photos} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!19}{\strut Search} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!9}{\strut Weather} \colorbox{red!17}{\strut Copyright} \colorbox{red!3}{\strut 2009} \colorbox{red!100}{\strut Yahoo} \colorbox{red!9}{\strut !} \colorbox{red!15}{\strut Singapore} \colorbox{red!0}{\strut Pte} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Ltd.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Co.} \colorbox{red!0}{\strut Reg} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 199700735D} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!7}{\strut Rights} \colorbox{red!0}{\strut Reserved} \colorbox{red!1}{\strut .} \colorbox{red!96}{\strut Privacy} \colorbox{red!55}{\strut Policy} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Service} 
}}}
\end{CJK*}

99:yahoo, 17:contact, 15:registration, 15:email, 14:international, 13:help, 13:customer, 13:account, 11:password, 11:id


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Sign-in} \colorbox{red!5}{\strut and} \colorbox{red!16}{\strut Registration} \colorbox{red!13}{\strut Help} \colorbox{red!18}{\strut Contact} \colorbox{red!5}{\strut Us} \colorbox{red!7}{\strut Go} \colorbox{red!8}{\strut Back} \colorbox{red!6}{\strut to} \colorbox{red!100}{\strut Yahoo} \colorbox{red!6}{\strut !} \colorbox{red!0}{\strut Sign-in} \colorbox{red!5}{\strut and} \colorbox{red!16}{\strut Registration} \colorbox{red!100}{\strut Yahoo} \colorbox{red!6}{\strut !} \colorbox{red!0}{\strut Sign-in} \colorbox{red!5}{\strut and} \colorbox{red!16}{\strut Registration} \colorbox{red!7}{\strut .} \colorbox{red!100}{\strut Yahoo} \colorbox{red!6}{\strut !} \colorbox{red!0}{\strut Sign-in} \colorbox{red!5}{\strut and} \colorbox{red!16}{\strut Registration} \colorbox{red!13}{\strut Help} \colorbox{red!7}{\strut .} \colorbox{red!18}{\strut Contact} \colorbox{red!5}{\strut Us} \colorbox{red!18}{\strut Contact} \colorbox{red!100}{\strut Yahoo} \colorbox{red!6}{\strut !} \colorbox{red!13}{\strut Customer} \colorbox{red!9}{\strut Care} \colorbox{red!16}{\strut Email} \colorbox{red!100}{\strut Yahoo} \colorbox{red!6}{\strut !} \colorbox{red!13}{\strut Account} \colorbox{red!10}{\strut Services} \colorbox{red!13}{\strut Help} \colorbox{red!10}{\strut Form} \colorbox{red!100}{\strut Yahoo} \colorbox{red!6}{\strut !} \colorbox{red!15}{\strut INTERNATIONAL} \colorbox{red!13}{\strut Help} \colorbox{red!10}{\strut Form} \colorbox{red!6}{\strut For} \colorbox{red!9}{\strut Sign} \colorbox{red!6}{\strut in} \colorbox{red!5}{\strut .} \colorbox{red!16}{\strut registration} \colorbox{red!8}{\strut issues} \colorbox{red!6}{\strut for} \colorbox{red!100}{\strut Yahoo} \colorbox{red!6}{\strut !} \colorbox{red!8}{\strut users} \colorbox{red!9}{\strut who} \colorbox{red!5}{\strut are} \colorbox{red!6}{\strut outside} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!8}{\strut United} \colorbox{red!9}{\strut States} \colorbox{red!6}{\strut .} \colorbox{red!5}{\strut My} \colorbox{red!13}{\strut Help} \colorbox{red!5}{\strut Forgot} \colorbox{red!2}{\strut your} \colorbox{red!11}{\strut ID} \colorbox{red!1}{\strut or} \colorbox{red!11}{\strut password} \colorbox{red!3}{\strut ?} \colorbox{red!9}{\strut Sign} \colorbox{red!6}{\strut In} \colorbox{red!9}{\strut Sign} \colorbox{red!6}{\strut in} \colorbox{red!6}{\strut to} \colorbox{red!5}{\strut see} \colorbox{red!2}{\strut your} \colorbox{red!13}{\strut account} \colorbox{red!8}{\strut information} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut saved} \colorbox{red!7}{\strut articles} \colorbox{red!5}{\strut and} \colorbox{red!6}{\strut more} \colorbox{red!6}{\strut .} \colorbox{red!5}{\strut Recent} \colorbox{red!7}{\strut Searches} \colorbox{red!3}{\strut No} \colorbox{red!5}{\strut recent} \colorbox{red!7}{\strut searches} \colorbox{red!6}{\strut Clear} \colorbox{red!3}{\strut all} 
}}}
\end{CJK*}

query: euclid

87:elements, 84:euclid, 74:lived, 28:father, 27:geometry, 27:born, 24:which, 24:background, 20:why, 20:treatise


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Mahalo.com} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Mahalo} \colorbox{red!0}{\strut Answers} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Mahalo} \colorbox{red!0}{\strut Daily} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Mahalo} \colorbox{red!1}{\strut Greenhouse} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Liveblog} \colorbox{red!63}{\strut Euclid} \colorbox{red!11}{\strut Known} \colorbox{red!3}{\strut as} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!21}{\strut Father} \colorbox{red!6}{\strut of} \colorbox{red!20}{\strut Geometry} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!55}{\strut lived} \colorbox{red!0}{\strut during} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut reign} \colorbox{red!6}{\strut of} \colorbox{red!13}{\strut Ptolemy} \colorbox{red!2}{\strut in} \colorbox{red!14}{\strut Alexandria} \colorbox{red!4}{\strut ,} \colorbox{red!9}{\strut Egypt} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut His} \colorbox{red!4}{\strut thirteen} \colorbox{red!5}{\strut volume} \colorbox{red!13}{\strut textbook} \colorbox{red!4}{\strut ,} \colorbox{red!65}{\strut Elements} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut was} \colorbox{red!9}{\strut considered} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut preeminent} \colorbox{red!15}{\strut treatise} \colorbox{red!5}{\strut on} \colorbox{red!15}{\strut mathematics} \colorbox{red!3}{\strut for} \colorbox{red!2}{\strut over} \colorbox{red!0}{\strut 2,000} \colorbox{red!6}{\strut years} \colorbox{red!2}{\strut .} \colorbox{red!65}{\strut Elements} \colorbox{red!1}{\strut is} \colorbox{red!3}{\strut the} \colorbox{red!1}{\strut most} \colorbox{red!15}{\strut studied} \colorbox{red!13}{\strut textbook} \colorbox{red!6}{\strut of} \colorbox{red!2}{\strut all} \colorbox{red!9}{\strut time} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut best} \colorbox{red!6}{\strut selling} \colorbox{red!10}{\strut book} \colorbox{red!2}{\strut in} \colorbox{red!9}{\strut history} \colorbox{red!3}{\strut next} \colorbox{red!3}{\strut to} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut Bible} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Fast} \colorbox{red!4}{\strut Facts} \colorbox{red!20}{\strut Born} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 325-330} \colorbox{red!0}{\strut B.C} \colorbox{red!2}{\strut .} \colorbox{red!10}{\strut Died} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 265-260} \colorbox{red!0}{\strut B.C} \colorbox{red!2}{\strut .} \colorbox{red!15}{\strut Studied} \colorbox{red!3}{\strut at} \colorbox{red!3}{\strut Plato} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut Academy} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut Greece} \colorbox{red!63}{\strut Euclid} \colorbox{red!8}{\strut established} \colorbox{red!2}{\strut a} \colorbox{red!13}{\strut school} \colorbox{red!2}{\strut in} \colorbox{red!14}{\strut Alexandria} \colorbox{red!2}{\strut Over} \colorbox{red!0}{\strut 1,000} \colorbox{red!4}{\strut editions} \colorbox{red!6}{\strut of} \colorbox{red!65}{\strut Elements} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!4}{\strut produced} \colorbox{red!7}{\strut Optica} \colorbox{red!2}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!3}{\strut to} \colorbox{red!65}{\strut Elements} \colorbox{red!4}{\strut ,} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut also} \colorbox{red!9}{\strut published} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut earliest} \colorbox{red!7}{\strut surviving} \colorbox{red!6}{\strut Western} \colorbox{red!0}{\strut study} \colorbox{red!5}{\strut on} \colorbox{red!6}{\strut visible} \colorbox{red!14}{\strut light} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut entitled} \colorbox{red!7}{\strut Optica} \colorbox{red!4}{\strut ,} \colorbox{red!18}{\strut which} \colorbox{red!3}{\strut provided} \colorbox{red!3}{\strut the} \colorbox{red!18}{\strut background} \colorbox{red!3}{\strut for} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut later} \colorbox{red!0}{\strut study} \colorbox{red!6}{\strut of} \colorbox{red!12}{\strut astronomy} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Categories} \colorbox{red!9}{\strut History} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Science} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Mathematics} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut View} \colorbox{red!2}{\strut Note} \colorbox{red!9}{\strut History} \colorbox{red!3}{\strut The} \colorbox{red!3}{\strut Mahalo} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut 7} \colorbox{red!3}{\strut Wikipedia} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!6}{\strut of} \colorbox{red!14}{\strut Alexandria} \colorbox{red!12}{\strut Math} \colorbox{red!0}{\strut Open} \colorbox{red!2}{\strut Reference} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!6}{\strut Clark} \colorbox{red!7}{\strut University} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!65}{\strut Elements} \colorbox{red!4}{\strut Molecular} \colorbox{red!5}{\strut Expressions} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut 325-265} \colorbox{red!3}{\strut BC} \colorbox{red!0}{\strut OBKB.com} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!6}{\strut Life} \colorbox{red!6}{\strut of} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut Engineering.com} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!6}{\strut of} \colorbox{red!14}{\strut Alexandria} \colorbox{red!13}{\strut School} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut Mathematical} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Computational} \colorbox{red!0}{\strut Sciences} \colorbox{red!7}{\strut University} \colorbox{red!6}{\strut of} \colorbox{red!2}{\strut St} \colorbox{red!3}{\strut Andrews} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!63}{\strut Euclid} \colorbox{red!18}{\strut Background} \colorbox{red!3}{\strut and} \colorbox{red!11}{\strut Works} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!18}{\strut Background} \colorbox{red!3}{\strut The} \colorbox{red!0}{\strut Perseus} \colorbox{red!2}{\strut Digital} \colorbox{red!2}{\strut Library} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut Traditions} \colorbox{red!5}{\strut About} \colorbox{red!3}{\strut Him} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!11}{\strut Works} \colorbox{red!3}{\strut Wikipedia} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!65}{\strut Elements} \colorbox{red!6}{\strut Clark} \colorbox{red!7}{\strut University} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!65}{\strut Elements} \colorbox{red!3}{\strut Internet} \colorbox{red!2}{\strut Archive} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut 1st} \colorbox{red!2}{\strut Six} \colorbox{red!0}{\strut Books} \colorbox{red!6}{\strut of} \colorbox{red!65}{\strut Elements} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 76.24} \colorbox{red!0}{\strut MB} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Wikipedia} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Data} \colorbox{red!0}{\strut -} \colorbox{red!63}{\strut Euclid} \colorbox{red!3}{\strut Wikipedia} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Catoptrics} \colorbox{red!0}{\strut OBKB.com} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!11}{\strut Works} \colorbox{red!6}{\strut of} \colorbox{red!63}{\strut Euclid} \colorbox{red!3}{\strut Other} \colorbox{red!2}{\strut than} \colorbox{red!3}{\strut the} \colorbox{red!65}{\strut Elements} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Lost} \colorbox{red!11}{\strut Works} \colorbox{red!0}{\strut Dr.} \colorbox{red!3}{\strut Tuttle} \colorbox{red!5}{\strut Professor} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut Engineering} \colorbox{red!4}{\strut ,} \colorbox{red!7}{\strut University} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut Denver} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut Theorem} \colorbox{red!0}{\strut from} \colorbox{red!3}{\strut the} \colorbox{red!14}{\strut Optics} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Phaenomena} \colorbox{red!63}{\strut Euclid} \colorbox{red!4}{\strut Images} \colorbox{red!6}{\strut Google} \colorbox{red!0}{\strut Image} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut Image} \colorbox{red!3}{\strut Search} \colorbox{red!0}{\strut Ask.com} \colorbox{red!0}{\strut Image} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut Image} \colorbox{red!3}{\strut Search} \colorbox{red!63}{\strut Euclid} \colorbox{red!0}{\strut Books} \colorbox{red!0}{\strut Amazon.com} \colorbox{red!2}{\strut .} \colorbox{red!63}{\strut Euclid} 
}}}
\end{CJK*}

98:euclid, 60:ohio, 18:city, 13:waste, 13:republic, 12:recycling, 11:hall, 10:refuse, 10:contract, 9:neighborhood


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Homes} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Properties} \colorbox{red!100}{\strut Euclid} \colorbox{red!8}{\strut Public} \colorbox{red!0}{\strut Library} \colorbox{red!9}{\strut Neighborhood} \colorbox{red!4}{\strut Programs} \colorbox{red!6}{\strut Social} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut Safety} \colorbox{red!7}{\strut Services} \colorbox{red!3}{\strut Community} \colorbox{red!6}{\strut TV} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut ECTV} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Maps} \colorbox{red!1}{\strut The} \colorbox{red!18}{\strut City} \colorbox{red!4}{\strut of} \colorbox{red!100}{\strut Euclid} \colorbox{red!3}{\strut is} \colorbox{red!6}{\strut under} \colorbox{red!10}{\strut contract} \colorbox{red!5}{\strut with} \colorbox{red!13}{\strut Republic} \colorbox{red!13}{\strut Waste} \colorbox{red!7}{\strut Services} \colorbox{red!4}{\strut of} \colorbox{red!61}{\strut Ohio} \colorbox{red!7}{\strut Hauling} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut collection} \colorbox{red!4}{\strut and} \colorbox{red!5}{\strut disposal} \colorbox{red!4}{\strut of} \colorbox{red!10}{\strut refuse} \colorbox{red!8}{\strut materials} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut bi-weekly} \colorbox{red!12}{\strut recycling} \colorbox{red!4}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!4}{\strut following} \colorbox{red!4}{\strut procedures} \colorbox{red!0}{\strut are} \colorbox{red!4}{\strut recommended} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!1}{\strut this} \colorbox{red!0}{\strut program} \colorbox{red!4}{\strut running} \colorbox{red!0}{\strut smoothly} \colorbox{red!4}{\strut .} \colorbox{red!8}{\strut Resident} \colorbox{red!0}{\strut Notice.pdf} \colorbox{red!0}{\strut home} \colorbox{red!4}{\strut about} \colorbox{red!100}{\strut euclid} \colorbox{red!18}{\strut city} \colorbox{red!11}{\strut hall} \colorbox{red!18}{\strut city} \colorbox{red!6}{\strut departments} \colorbox{red!8}{\strut resident} \colorbox{red!0}{\strut information} \colorbox{red!4}{\strut seniors} \colorbox{red!3}{\strut recreation} \colorbox{red!2}{\strut calendar} \colorbox{red!3}{\strut news} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut announcements} \colorbox{red!2}{\strut contact} \colorbox{red!3}{\strut us} \colorbox{red!5}{\strut form} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut permits} \colorbox{red!4}{\strut faq} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut sitemap} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut search} \colorbox{red!4}{\strut Copyright} \colorbox{red!0}{\strut 2009} \colorbox{red!1}{\strut The} \colorbox{red!18}{\strut City} \colorbox{red!4}{\strut of} \colorbox{red!100}{\strut Euclid} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut reserved} \colorbox{red!4}{\strut .} \colorbox{red!5}{\strut Employee} \colorbox{red!3}{\strut Signon} 
}}}
\end{CJK*}

query: starbucks

99:starbucks, 62:union, 42:iww, 32:labor, 30:workers, 23:fired, 22:workplace, 19:swu, 19:pay, 19:join


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!64}{\strut Starbucks} \colorbox{red!40}{\strut Union} \colorbox{red!27}{\strut IWW} \colorbox{red!64}{\strut Starbucks} \colorbox{red!19}{\strut Workers} \colorbox{red!40}{\strut Union} \colorbox{red!9}{\strut Register} \colorbox{red!5}{\strut Login} \colorbox{red!6}{\strut email} \colorbox{red!3}{\strut us} \colorbox{red!11}{\strut phone} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 917-577-1110} \colorbox{red!2}{\strut Main} \colorbox{red!3}{\strut Menu} \colorbox{red!3}{\strut Home} \colorbox{red!2}{\strut About} \colorbox{red!3}{\strut Us} \colorbox{red!1}{\strut Bean2Cup} \colorbox{red!5}{\strut Campus} \colorbox{red!7}{\strut Campaign} \colorbox{red!0}{\strut E-mail} \colorbox{red!5}{\strut Action} \colorbox{red!2}{\strut Updates} \colorbox{red!0}{\strut Get} \colorbox{red!9}{\strut Involved} \colorbox{red!5}{\strut Contact} \colorbox{red!3}{\strut Us} \colorbox{red!4}{\strut News} \colorbox{red!2}{\strut Archive} \colorbox{red!2}{\strut Forums} \colorbox{red!2}{\strut Documentary} \colorbox{red!0}{\strut Govt} \colorbox{red!64}{\strut Starbucks} \colorbox{red!6}{\strut Settlement} \colorbox{red!3}{\strut Events} \colorbox{red!1}{\strut Search} \colorbox{red!1}{\strut User} \colorbox{red!5}{\strut login} \colorbox{red!0}{\strut Username} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Password} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Create} \colorbox{red!5}{\strut new} \colorbox{red!3}{\strut account} \colorbox{red!5}{\strut Request} \colorbox{red!5}{\strut new} \colorbox{red!5}{\strut password} \colorbox{red!64}{\strut Starbucks} \colorbox{red!40}{\strut Union} \colorbox{red!5}{\strut Sign} \colorbox{red!2}{\strut up} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut receive} \colorbox{red!7}{\strut campaign} \colorbox{red!2}{\strut bulletins} \colorbox{red!0}{\strut E-mail} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Subscribe} \colorbox{red!1}{\strut Unsubscribe} \colorbox{red!2}{\strut Read} \colorbox{red!1}{\strut our} \colorbox{red!3}{\strut feed} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!64}{\strut Starbucks} \colorbox{red!19}{\strut Workers} \colorbox{red!5}{\strut Coming} \colorbox{red!3}{\strut Together} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Increased} \colorbox{red!12}{\strut pay} \colorbox{red!1}{\strut and} \colorbox{red!8}{\strut raises} \colorbox{red!2}{\strut Guaranteed} \colorbox{red!4}{\strut hours} \colorbox{red!2}{\strut with} \colorbox{red!2}{\strut the} \colorbox{red!1}{\strut option} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut fulltime} \colorbox{red!5}{\strut status} \colorbox{red!0}{\strut An} \colorbox{red!3}{\strut end} \colorbox{red!1}{\strut to} \colorbox{red!8}{\strut understaffing} \colorbox{red!1}{\strut A} \colorbox{red!3}{\strut healthier} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut safer} \colorbox{red!14}{\strut workplace} \colorbox{red!0}{\strut Get} \colorbox{red!9}{\strut Involved} \colorbox{red!12}{\strut Join} \colorbox{red!2}{\strut the} \colorbox{red!40}{\strut Union} \colorbox{red!3}{\strut Contribute} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Recent} \colorbox{red!2}{\strut blog} \colorbox{red!3}{\strut posts} \colorbox{red!3}{\strut Swedish} \colorbox{red!40}{\strut Union} \colorbox{red!2}{\strut Seeks} \colorbox{red!4}{\strut Support} \colorbox{red!0}{\strut After} \colorbox{red!3}{\strut Nazi} \colorbox{red!5}{\strut Murder} \colorbox{red!3}{\strut Attempt} \colorbox{red!12}{\strut SWU} \colorbox{red!4}{\strut Member} \colorbox{red!1}{\strut Daniel} \colorbox{red!2}{\strut Gross} \colorbox{red!2}{\strut on} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut Chicago} \colorbox{red!0}{\strut Sit-Down} \colorbox{red!9}{\strut Strike} \colorbox{red!0}{\strut Members} \colorbox{red!3}{\strut of} \colorbox{red!12}{\strut SWU} \colorbox{red!3}{\strut Sister} \colorbox{red!40}{\strut Union} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut Sweden} \colorbox{red!4}{\strut Survive} \colorbox{red!3}{\strut Nazi} \colorbox{red!5}{\strut Attack} \colorbox{red!1}{\strut Blast} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut past} \colorbox{red!1}{\strut .} \colorbox{red!27}{\strut IWW} \colorbox{red!0}{\strut comes} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut MOA} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut TC} \colorbox{red!2}{\strut Daily} \colorbox{red!1}{\strut Planet} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Mall} \colorbox{red!64}{\strut Starbucks} \colorbox{red!19}{\strut workers} \colorbox{red!12}{\strut join} \colorbox{red!40}{\strut union} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Star} \colorbox{red!1}{\strut Tribune} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Mall} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut America} \colorbox{red!64}{\strut Starbucks} \colorbox{red!8}{\strut Baristas} \colorbox{red!2}{\strut Walk} \colorbox{red!0}{\strut Off} \colorbox{red!5}{\strut Job} \colorbox{red!1}{\strut ,} \colorbox{red!7}{\strut Protest} \colorbox{red!3}{\strut Closures} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Fox} \colorbox{red!0}{\strut 9} \colorbox{red!1}{\strut .} \colorbox{red!12}{\strut SWU} \colorbox{red!3}{\strut Allies} \colorbox{red!5}{\strut Hit} \colorbox{red!64}{\strut Starbucks} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut Spain} \colorbox{red!2}{\strut on} \colorbox{red!1}{\strut May} \colorbox{red!1}{\strut Day} \colorbox{red!5}{\strut Judge} \colorbox{red!1}{\strut draws} \colorbox{red!1}{\strut clear} \colorbox{red!1}{\strut line} \colorbox{red!3}{\strut at} \colorbox{red!2}{\strut tip} \colorbox{red!2}{\strut jar} \colorbox{red!1}{\strut in} \colorbox{red!64}{\strut Starbucks} \colorbox{red!5}{\strut case} \colorbox{red!4}{\strut Will} \colorbox{red!64}{\strut Starbucks} \colorbox{red!3}{\strut reveal} \colorbox{red!11}{\strut Calorie} \colorbox{red!4}{\strut count} \colorbox{red!64}{\strut Starbucks} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut Appeal} \colorbox{red!0}{\strut Tip-Sharing} \colorbox{red!7}{\strut Ruling} \colorbox{red!0}{\strut more} \colorbox{red!3}{\strut Sbux} \colorbox{red!40}{\strut Union} \colorbox{red!4}{\strut News} \colorbox{red!0}{\strut E-Mail} \colorbox{red!5}{\strut Action} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Tell} \colorbox{red!64}{\strut Starbucks} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut Year} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut Honor} \colorbox{red!0}{\strut Dr.} \colorbox{red!6}{\strut King} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Holiday} \colorbox{red!2}{\strut !} \colorbox{red!64}{\strut Starbucks} \colorbox{red!2}{\strut .} \colorbox{red!40}{\strut Union} \colorbox{red!3}{\strut Blues} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut BusinessWeek} \colorbox{red!1}{\strut .} \colorbox{red!64}{\strut Starbucks} \colorbox{red!4}{\strut Loses} \colorbox{red!0}{\strut Round} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut Battle} \colorbox{red!2}{\strut Over} \colorbox{red!40}{\strut Union} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut New} \colorbox{red!1}{\strut York} \colorbox{red!2}{\strut Times} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Judge} \colorbox{red!6}{\strut Finds} \colorbox{red!64}{\strut Starbucks} \colorbox{red!7}{\strut Guilty} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut Extensive} \colorbox{red!0}{\strut Union-Busting} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut Wo} \colorbox{red!0}{\strut nt} \colorbox{red!5}{\strut Back} \colorbox{red!3}{\strut Down} \colorbox{red!1}{\strut .} \colorbox{red!64}{\strut Starbucks} \colorbox{red!5}{\strut Manager} \colorbox{red!3}{\strut Threatens} \colorbox{red!7}{\strut Lawsuit} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut Criminal} \colorbox{red!7}{\strut Complaint} \colorbox{red!5}{\strut Against} \colorbox{red!27}{\strut IWW} \colorbox{red!8}{\strut Baristas} \colorbox{red!2}{\strut Present} \colorbox{red!1}{\strut 500} \colorbox{red!3}{\strut Petition} \colorbox{red!4}{\strut Signatures} \colorbox{red!3}{\strut Demanding} \colorbox{red!1}{\strut Improved} \colorbox{red!3}{\strut Security} \colorbox{red!3}{\strut at} \colorbox{red!1}{\strut a} \colorbox{red!7}{\strut Minneapolis} \colorbox{red!64}{\strut Starbucks} \colorbox{red!64}{\strut Starbucks} \colorbox{red!3}{\strut Blues} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Slate} \colorbox{red!4}{\strut Magazine} \colorbox{red!1}{\strut .} \colorbox{red!64}{\strut Starbucks} \colorbox{red!0}{\strut Management} \colorbox{red!3}{\strut Conference} \colorbox{red!1}{\strut in} \colorbox{red!5}{\strut New} \colorbox{red!1}{\strut Orleans} \colorbox{red!5}{\strut Hit} \colorbox{red!2}{\strut with} \colorbox{red!1}{\strut Unexpected} \colorbox{red!40}{\strut Union} \colorbox{red!7}{\strut Protest} \colorbox{red!64}{\strut Starbucks} \colorbox{red!8}{\strut settles} \colorbox{red!3}{\strut NLRB} \colorbox{red!7}{\strut complaint} \colorbox{red!3}{\strut of} \colorbox{red!15}{\strut fired} \colorbox{red!0}{\strut barista} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut AP} \colorbox{red!1}{\strut .} \colorbox{red!8}{\strut Baristas} \colorbox{red!3}{\strut Defeat} 
}}}
\end{CJK*}

98:starbuck, 75:county, 41:minnesota, 30:location, 27:population, 14:pope, 14:city, 14:area, 13:states, 13:coordinates


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!87}{\strut Starbuck} \colorbox{red!6}{\strut ,} \colorbox{red!36}{\strut Minnesota} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!6}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!87}{\strut Starbuck} \colorbox{red!6}{\strut ,} \colorbox{red!36}{\strut Minnesota} \colorbox{red!26}{\strut Location} \colorbox{red!1}{\strut of} \colorbox{red!87}{\strut Starbuck} \colorbox{red!6}{\strut ,} \colorbox{red!36}{\strut Minnesota} \colorbox{red!11}{\strut Coordinates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 453650N} \colorbox{red!0}{\strut 953150W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 45.61389N} \colorbox{red!0}{\strut 95.53056W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 45.61389} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -95.53056} \colorbox{red!3}{\strut Country} \colorbox{red!5}{\strut United} \colorbox{red!11}{\strut States} \colorbox{red!0}{\strut State} \colorbox{red!36}{\strut Minnesota} \colorbox{red!66}{\strut County} \colorbox{red!12}{\strut Pope} \colorbox{red!12}{\strut Area} \colorbox{red!0}{\strut -Total} \colorbox{red!0}{\strut 1.6sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.1km2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -Land} \colorbox{red!0}{\strut 1.6sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.1km2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Water} \colorbox{red!0}{\strut 0.0sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0.0km2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Elevation} \colorbox{red!0}{\strut 1,171ft} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 357m} \colorbox{red!0}{\strut .} \colorbox{red!24}{\strut Population} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -Total} \colorbox{red!0}{\strut 1,314} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Density} \colorbox{red!0}{\strut 834.0sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 322.0km2} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Time} \colorbox{red!0}{\strut zone} \colorbox{red!0}{\strut Central} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CST} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut UTC-6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -Summer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DST} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut CDT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut UTC-5} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut ZIP} \colorbox{red!4}{\strut code} \colorbox{red!0}{\strut 56381} \colorbox{red!12}{\strut Area} \colorbox{red!4}{\strut code} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 320} \colorbox{red!1}{\strut FIPS} \colorbox{red!4}{\strut code} \colorbox{red!0}{\strut 27-62500} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut GNIS} \colorbox{red!0}{\strut feature} \colorbox{red!7}{\strut ID} \colorbox{red!0}{\strut 0652561} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!87}{\strut Starbuck} \colorbox{red!4}{\strut is} \colorbox{red!4}{\strut a} \colorbox{red!12}{\strut city} \colorbox{red!4}{\strut in} \colorbox{red!12}{\strut Pope} \colorbox{red!66}{\strut County} \colorbox{red!6}{\strut ,} \colorbox{red!36}{\strut Minnesota} \colorbox{red!6}{\strut ,} \colorbox{red!5}{\strut United} \colorbox{red!11}{\strut States} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!24}{\strut population} \colorbox{red!1}{\strut was} \colorbox{red!0}{\strut 1,314} \colorbox{red!1}{\strut at} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut 2000} \colorbox{red!5}{\strut census} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!1}{\strut 1} \colorbox{red!4}{\strut Geography} \colorbox{red!0}{\strut 2} \colorbox{red!3}{\strut Demographics} \colorbox{red!0}{\strut 3} \colorbox{red!2}{\strut Trivia} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Geography} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut United} \colorbox{red!11}{\strut States} \colorbox{red!5}{\strut Census} \colorbox{red!0}{\strut Bureau} \colorbox{red!6}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut city} \colorbox{red!0}{\strut has} \colorbox{red!4}{\strut a} \colorbox{red!0}{\strut total} \colorbox{red!12}{\strut area} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut 1.6} \colorbox{red!4}{\strut square} \colorbox{red!5}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.1} \colorbox{red!3}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!4}{\strut land} \colorbox{red!2}{\strut .} \colorbox{red!36}{\strut Minnesota} \colorbox{red!0}{\strut State} \colorbox{red!2}{\strut Highways} \colorbox{red!0}{\strut 28} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut 29} \colorbox{red!6}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut 114} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut three} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut main} \colorbox{red!0}{\strut routes} \colorbox{red!4}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut city} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Demographics} \colorbox{red!2}{\strut As} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut census} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut 2000} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!2}{\strut were} \colorbox{red!0}{\strut 1,314} \colorbox{red!6}{\strut people} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut 565} \colorbox{red!1}{\strut households} \colorbox{red!6}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut 328} \colorbox{red!0}{\strut families} \colorbox{red!3}{\strut residing} \colorbox{red!4}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut city} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!24}{\strut population} \colorbox{red!1}{\strut density} \colorbox{red!1}{\strut was} \colorbox{red!0}{\strut 834.0} \colorbox{red!6}{\strut people} \colorbox{red!0}{\strut per} \colorbox{red!4}{\strut square} \colorbox{red!0}{\strut mile} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 321.1km} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!2}{\strut were} \colorbox{red!0}{\strut 633} \colorbox{red!1}{\strut housing} \colorbox{red!0}{\strut units} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut an} \colorbox{red!3}{\strut average} \colorbox{red!1}{\strut density} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut 401.8sqmi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 154.7km} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!5}{\strut racial} \colorbox{red!4}{\strut makeup} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut city} \colorbox{red!1}{\strut was} \colorbox{red!0}{\strut 99.01} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut White} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut 0.23} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut other} \colorbox{red!2}{\strut races} \colorbox{red!6}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut 0.76} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut races} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Hispanic} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Latino} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut race} \colorbox{red!2}{\strut were} \colorbox{red!0}{\strut 0.46} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!24}{\strut population} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!2}{\strut were} \colorbox{red!0}{\strut 565} \colorbox{red!1}{\strut households} 
}}}
\end{CJK*}

query: diabetes education

92:diabetes, 50:menus, 31:recipes, 31:lists, 24:grocery, 20:planner, 20:medications, 19:nutrition, 18:diet, 15:food


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!4}{\strut A} \colorbox{red!6}{\strut web} \colorbox{red!5}{\strut resource} \colorbox{red!6}{\strut for} \colorbox{red!93}{\strut diabetes} \colorbox{red!13}{\strut patients} \colorbox{red!4}{\strut and} \colorbox{red!11}{\strut professional} \colorbox{red!93}{\strut diabetes} \colorbox{red!14}{\strut educators} \colorbox{red!5}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!93}{\strut Diabetes} \colorbox{red!31}{\strut Recipes} \colorbox{red!5}{\strut ,} \colorbox{red!93}{\strut Diabetes} \colorbox{red!50}{\strut Menus} \colorbox{red!5}{\strut ,} \colorbox{red!24}{\strut Grocery} \colorbox{red!31}{\strut Lists} \colorbox{red!4}{\strut .} \colorbox{red!19}{\strut Nutrition} \colorbox{red!9}{\strut Facts} \colorbox{red!5}{\strut !} \colorbox{red!93}{\strut Diabetes} \colorbox{red!0}{\strut Education} \colorbox{red!5}{\strut -} \colorbox{red!12}{\strut Certified} \colorbox{red!93}{\strut Diabetes} \colorbox{red!0}{\strut Educator} \colorbox{red!10}{\strut CDE} \colorbox{red!11}{\strut Home} \colorbox{red!93}{\strut Diabetes} \colorbox{red!50}{\strut Menus} \colorbox{red!93}{\strut Diabetes} \colorbox{red!14}{\strut Educators} \colorbox{red!7}{\strut FAQs} \colorbox{red!0}{\strut Sign-Up} \colorbox{red!7}{\strut Contact} \colorbox{red!5}{\strut Us} \colorbox{red!11}{\strut Articles} \colorbox{red!11}{\strut Newsletter} \colorbox{red!0}{\strut e-mail} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut password} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut FREE} \colorbox{red!93}{\strut Diabetes} \colorbox{red!0}{\strut Menu} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!7}{\strut Week} \colorbox{red!5}{\strut !} \colorbox{red!9}{\strut Body} \colorbox{red!12}{\strut Calculator} \colorbox{red!15}{\strut Food} \colorbox{red!5}{\strut Picker} \colorbox{red!93}{\strut Diabetes} \colorbox{red!31}{\strut Recipes} \colorbox{red!93}{\strut Diabetes} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut Pre-Diabetes} \colorbox{red!4}{\strut Recently} \colorbox{red!9}{\strut Diagnosed} \colorbox{red!93}{\strut Diabetes} \colorbox{red!8}{\strut Groups} \colorbox{red!12}{\strut Weight} \colorbox{red!6}{\strut Loss} \colorbox{red!5}{\strut Live} \colorbox{red!4}{\strut Chat} \colorbox{red!6}{\strut Feedback} \colorbox{red!0}{\strut Sign-Up} \colorbox{red!93}{\strut Diabetes} \colorbox{red!14}{\strut Educators} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!7}{\strut services} \colorbox{red!6}{\strut for} \colorbox{red!93}{\strut Diabetes} \colorbox{red!14}{\strut Educators} \colorbox{red!6}{\strut Add} \colorbox{red!2}{\strut your} \colorbox{red!8}{\strut name} \colorbox{red!5}{\strut to} \colorbox{red!5}{\strut our} \colorbox{red!93}{\strut Diabetes} \colorbox{red!0}{\strut Education} \colorbox{red!2}{\strut Locator} \colorbox{red!7}{\strut database} \colorbox{red!2}{\strut I} \colorbox{red!5}{\strut am} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut educator} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut please} \colorbox{red!6}{\strut add} \colorbox{red!1}{\strut my} \colorbox{red!8}{\strut name} \colorbox{red!5}{\strut Help} \colorbox{red!3}{\strut me} \colorbox{red!8}{\strut find} \colorbox{red!4}{\strut a} \colorbox{red!93}{\strut Diabetes} \colorbox{red!0}{\strut Educator} \colorbox{red!2}{\strut I} \colorbox{red!5}{\strut am} \colorbox{red!4}{\strut looking} \colorbox{red!6}{\strut for} \colorbox{red!4}{\strut a} \colorbox{red!93}{\strut diabetes} \colorbox{red!0}{\strut educator} \colorbox{red!2}{\strut or} \colorbox{red!93}{\strut diabetes} \colorbox{red!0}{\strut education} \colorbox{red!2}{\strut I} \colorbox{red!4}{\strut would} \colorbox{red!2}{\strut like} \colorbox{red!5}{\strut to} \colorbox{red!5}{\strut request} \colorbox{red!5}{\strut brochures} \colorbox{red!7}{\strut Contact} \colorbox{red!5}{\strut Us} \colorbox{red!2}{\strut I} \colorbox{red!5}{\strut am} \colorbox{red!4}{\strut a} \colorbox{red!93}{\strut Diabetes} \colorbox{red!0}{\strut Educator} \colorbox{red!4}{\strut and} \colorbox{red!7}{\strut interested} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut submitting} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut article} \colorbox{red!6}{\strut for} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!8}{\strut Write} \colorbox{red!6}{\strut for} \colorbox{red!5}{\strut us} \colorbox{red!5}{\strut !} \colorbox{red!7}{\strut Interested} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut becoming} \colorbox{red!4}{\strut a} \colorbox{red!10}{\strut CDE} \colorbox{red!0}{\strut Become} \colorbox{red!4}{\strut a} \colorbox{red!10}{\strut CDE} \colorbox{red!7}{\strut Interested} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut becoming} \colorbox{red!5}{\strut Board} \colorbox{red!12}{\strut Certified} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Advanced} \colorbox{red!93}{\strut Diabetes} \colorbox{red!6}{\strut Management} \colorbox{red!5}{\strut American} \colorbox{red!7}{\strut Association} \colorbox{red!5}{\strut of} \colorbox{red!93}{\strut Diabetes} \colorbox{red!14}{\strut Educators} \colorbox{red!11}{\strut Home} \colorbox{red!3}{\strut .} \colorbox{red!93}{\strut Diabetes} \colorbox{red!50}{\strut Menus} \colorbox{red!3}{\strut .} \colorbox{red!93}{\strut Diabetes} \colorbox{red!14}{\strut Educators} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Sign-up} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut FAQs} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut Contact} \colorbox{red!5}{\strut Us} \colorbox{red!3}{\strut .} \colorbox{red!11}{\strut Articles} \colorbox{red!3}{\strut .} \colorbox{red!11}{\strut Newsletter} \colorbox{red!6}{\strut Copyright} \colorbox{red!3}{\strut 2001} \colorbox{red!5}{\strut ,} \colorbox{red!1}{\strut 2002} \colorbox{red!5}{\strut ,} \colorbox{red!3}{\strut 2003} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!6}{\strut Presented} \colorbox{red!3}{\strut by} \colorbox{red!19}{\strut Nutrition} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut Inc.} \colorbox{red!93}{\strut Diabetes} \colorbox{red!11}{\strut articles} \colorbox{red!4}{\strut with} \colorbox{red!6}{\strut topics} \colorbox{red!5}{\strut covering} \colorbox{red!93}{\strut diabetes} \colorbox{red!20}{\strut medications} \colorbox{red!93}{\strut diabetes} \colorbox{red!12}{\strut complications} \colorbox{red!0}{\strut diabetic} \colorbox{red!18}{\strut diet} \colorbox{red!4}{\strut and} \colorbox{red!19}{\strut nutrition} \colorbox{red!9}{\strut facts} \colorbox{red!6}{\strut for} \colorbox{red!0}{\strut those} \colorbox{red!9}{\strut diagnosed} \colorbox{red!4}{\strut with} \colorbox{red!93}{\strut diabetes} \colorbox{red!5}{\strut .} \colorbox{red!50}{\strut Menus} \colorbox{red!3}{\strut are} \colorbox{red!6}{\strut prepared} \colorbox{red!3}{\strut by} \colorbox{red!11}{\strut professional} \colorbox{red!93}{\strut diabetes} \colorbox{red!14}{\strut educators} \colorbox{red!5}{\strut .} \colorbox{red!10}{\strut Weekly} \colorbox{red!93}{\strut diabetes} \colorbox{red!0}{\strut menu} \colorbox{red!5}{\strut includes} \colorbox{red!4}{\strut a} \colorbox{red!24}{\strut grocery} \colorbox{red!0}{\strut list} \colorbox{red!93}{\strut diabetes} \colorbox{red!31}{\strut recipes} \colorbox{red!4}{\strut and} \colorbox{red!19}{\strut nutrition} \colorbox{red!4}{\strut analysis} \colorbox{red!5}{\strut .} \colorbox{red!93}{\strut Diabetes} \colorbox{red!8}{\strut care} \colorbox{red!3}{\strut is} \colorbox{red!6}{\strut specific} \colorbox{red!4}{\strut and} \colorbox{red!2}{\strut all} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!5}{\strut information} \colorbox{red!4}{\strut on} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut DiabetesPlanner.com} \colorbox{red!8}{\strut website} \colorbox{red!2}{\strut may} \colorbox{red!2}{\strut not} \colorbox{red!3}{\strut apply} \colorbox{red!5}{\strut to} \colorbox{red!2}{\strut you} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut Our} \colorbox{red!93}{\strut diabetes} \colorbox{red!50}{\strut menus} \colorbox{red!93}{\strut diabetes} \colorbox{red!31}{\strut recipes} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut other} \colorbox{red!93}{\strut diabetes} \colorbox{red!5}{\strut information} \colorbox{red!3}{\strut are} \colorbox{red!2}{\strut not} \colorbox{red!5}{\strut intended} \colorbox{red!5}{\strut to} \colorbox{red!5}{\strut replace} \colorbox{red!11}{\strut professional} \colorbox{red!0}{\strut medical} \colorbox{red!6}{\strut advice} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut be} \colorbox{red!3}{\strut aware} \colorbox{red!5}{\strut of} \colorbox{red!93}{\strut diabetes} \colorbox{red!12}{\strut complications} \colorbox{red!4}{\strut and} \colorbox{red!4}{\strut other} \colorbox{red!5}{\strut issues} \colorbox{red!5}{\strut .} \colorbox{red!4}{\strut Always} \colorbox{red!5}{\strut check} \colorbox{red!4}{\strut with} \colorbox{red!2}{\strut your} \colorbox{red!8}{\strut physician} \colorbox{red!1}{\strut prior} \colorbox{red!5}{\strut to} \colorbox{red!7}{\strut starting} \colorbox{red!4}{\strut a} \colorbox{red!0}{\strut diabetic} \colorbox{red!18}{\strut diet} \colorbox{red!93}{\strut diabetes} \colorbox{red!20}{\strut medications} \colorbox{red!2}{\strut or} \colorbox{red!8}{\strut exercise} \colorbox{red!8}{\strut program} \colorbox{red!5}{\strut .} 
}}}
\end{CJK*}

98:diabetes, 93:education, 41:japan, 32:nurses, 24:who, 22:which, 21:pharmacists, 19:patients, 19:english, 19:concerned


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut English} \colorbox{red!3}{\strut HOME} \colorbox{red!2}{\strut .} \colorbox{red!8}{\strut English} \colorbox{red!8}{\strut English} \colorbox{red!1}{\strut A} \colorbox{red!1}{\strut result} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut increase} \colorbox{red!1}{\strut in} \colorbox{red!44}{\strut diabetes} \colorbox{red!8}{\strut patients} \colorbox{red!1}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut increase} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut need} \colorbox{red!1}{\strut for} \colorbox{red!5}{\strut human} \colorbox{red!3}{\strut resources} \colorbox{red!2}{\strut to} \colorbox{red!4}{\strut provide} \colorbox{red!8}{\strut patients} \colorbox{red!1}{\strut with} \colorbox{red!44}{\strut diabetes} \colorbox{red!42}{\strut education} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut At} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!2}{\strut time} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut rising} \colorbox{red!8}{\strut expectations} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut part} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut public} \colorbox{red!1}{\strut for} \colorbox{red!42}{\strut education} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut be} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!14}{\strut nurses} \colorbox{red!1}{\strut ,} \colorbox{red!6}{\strut nutritionists} \colorbox{red!1}{\strut ,} \colorbox{red!9}{\strut pharmacists} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut technicians} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut others} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut In} \colorbox{red!2}{\strut order} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut respond} \colorbox{red!2}{\strut adequately} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut these} \colorbox{red!8}{\strut expectations} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut a} \colorbox{red!4}{\strut context} \colorbox{red!1}{\strut in} \colorbox{red!9}{\strut which} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut would} \colorbox{red!1}{\strut be} \colorbox{red!2}{\strut difficult} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut say} \colorbox{red!1}{\strut that} \colorbox{red!42}{\strut education} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut being} \colorbox{red!2}{\strut carried} \colorbox{red!1}{\strut out} \colorbox{red!3}{\strut effectively} \colorbox{red!1}{\strut or} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut light} \colorbox{red!2}{\strut of} \colorbox{red!4}{\strut experience} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut there} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!4}{\strut need} \colorbox{red!2}{\strut to} \colorbox{red!4}{\strut provide} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut qualitative} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut quantitative} \colorbox{red!3}{\strut improvement} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut patient} \colorbox{red!42}{\strut education} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut With} \colorbox{red!1}{\strut these} \colorbox{red!1}{\strut points} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut mind} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut JADEN} \colorbox{red!0}{\strut intends} \colorbox{red!2}{\strut to} \colorbox{red!4}{\strut promote} \colorbox{red!7}{\strut research} \colorbox{red!1}{\strut that} \colorbox{red!4}{\strut specialists} \colorbox{red!1}{\strut in} \colorbox{red!44}{\strut diabetes} \colorbox{red!42}{\strut education} \colorbox{red!1}{\strut will} \colorbox{red!1}{\strut be} \colorbox{red!2}{\strut able} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut apply} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut their} \colorbox{red!2}{\strut own} \colorbox{red!4}{\strut practice} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!4}{\strut Association} \colorbox{red!1}{\strut will} \colorbox{red!2}{\strut serve} \colorbox{red!1}{\strut as} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut forum} \colorbox{red!1}{\strut in} \colorbox{red!9}{\strut which} \colorbox{red!0}{\strut researchers} \colorbox{red!1}{\strut can} \colorbox{red!3}{\strut present} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut findings} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut field} \colorbox{red!2}{\strut of} \colorbox{red!44}{\strut diabetes} \colorbox{red!42}{\strut education} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut or} \colorbox{red!1}{\strut as} \colorbox{red!1}{\strut one} \colorbox{red!1}{\strut in} \colorbox{red!9}{\strut which} \colorbox{red!4}{\strut practitioners} \colorbox{red!1}{\strut can} \colorbox{red!3}{\strut make} \colorbox{red!2}{\strut reports} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut addition} \colorbox{red!1}{\strut as} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut place} \colorbox{red!1}{\strut in} \colorbox{red!9}{\strut which} \colorbox{red!0}{\strut researchers} \colorbox{red!2}{\strut and} \colorbox{red!4}{\strut practitioners} \colorbox{red!1}{\strut can} \colorbox{red!3}{\strut engage} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut mutual} \colorbox{red!2}{\strut exchange} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut views} \colorbox{red!2}{\strut and} \colorbox{red!4}{\strut experience} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!1}{\strut will} \colorbox{red!4}{\strut systematize} \colorbox{red!2}{\strut and} \colorbox{red!4}{\strut unify} \colorbox{red!4}{\strut theory} \colorbox{red!2}{\strut and} \colorbox{red!7}{\strut research} \colorbox{red!8}{\strut concerned} \colorbox{red!1}{\strut with} \colorbox{red!44}{\strut diabetes} \colorbox{red!42}{\strut education} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut objective} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut making} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut contribution} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut raising} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut level} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut such} \colorbox{red!42}{\strut education} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Turning} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut establishment} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!18}{\strut Japan} \colorbox{red!4}{\strut Academy} \colorbox{red!2}{\strut of} \colorbox{red!44}{\strut Diabetes} \colorbox{red!42}{\strut Education} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut Nursing} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut its} \colorbox{red!4}{\strut beginnings} \colorbox{red!1}{\strut can} \colorbox{red!1}{\strut be} \colorbox{red!1}{\strut traced} \colorbox{red!1}{\strut back} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut meeting} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut February} \colorbox{red!0}{\strut 1996} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut number} \colorbox{red!2}{\strut of} \colorbox{red!8}{\strut concerned} \colorbox{red!5}{\strut persons} \colorbox{red!10}{\strut who} \colorbox{red!1}{\strut shared} \colorbox{red!2}{\strut common} \colorbox{red!1}{\strut feelings} \colorbox{red!2}{\strut of} \colorbox{red!8}{\strut expectations} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut unease} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut arrangements} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut being} \colorbox{red!3}{\strut put} \colorbox{red!1}{\strut in} \colorbox{red!2}{\strut place} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut certification} \colorbox{red!2}{\strut examination} \colorbox{red!1}{\strut for} \colorbox{red!4}{\strut Certified} \colorbox{red!44}{\strut Diabetes} \colorbox{red!0}{\strut Educators} \colorbox{red!2}{\strut of} \colorbox{red!18}{\strut Japan} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut At} \colorbox{red!1}{\strut that} \colorbox{red!2}{\strut time} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut the} \colorbox{red!8}{\strut concerned} \colorbox{red!5}{\strut persons} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut nurses} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut tried} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut protest} \colorbox{red!0}{\strut against} \colorbox{red!0}{\strut this} \colorbox{red!4}{\strut development} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut because} \colorbox{red!1}{\strut there} \colorbox{red!1}{\strut was} \colorbox{red!0}{\strut no} \colorbox{red!7}{\strut research} 
}}}
\end{CJK*}

query: website design hosting

38:cms, 30:hosting, 28:fire, 25:angel, 24:design, 20:website, 19:site, 18:web, 16:albuquerque, 15:database


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Home} \colorbox{red!3}{\strut News} \colorbox{red!0}{\strut About} \colorbox{red!5}{\strut Us} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!68}{\strut CMS} \colorbox{red!35}{\strut Website} \colorbox{red!14}{\strut SEO} \colorbox{red!21}{\strut Blog} \colorbox{red!32}{\strut Web} \colorbox{red!53}{\strut Hosting} \colorbox{red!0}{\strut eCommerce} \colorbox{red!12}{\strut Affiliate} \colorbox{red!5}{\strut Store} \colorbox{red!7}{\strut Shopping} \colorbox{red!5}{\strut Cart} \colorbox{red!32}{\strut Web} \colorbox{red!7}{\strut Evaluation} \colorbox{red!26}{\strut Database} \colorbox{red!53}{\strut Hosting} \colorbox{red!26}{\strut Database} \colorbox{red!5}{\strut Demos} \colorbox{red!12}{\strut Search} \colorbox{red!7}{\strut Engines} \colorbox{red!8}{\strut Free} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!8}{\strut Portfolio} \colorbox{red!7}{\strut Contact} \colorbox{red!5}{\strut Us} \colorbox{red!12}{\strut Company} \colorbox{red!8}{\strut Info} \colorbox{red!0}{\strut ImageBuilders} \colorbox{red!3}{\strut PO} \colorbox{red!0}{\strut Box} \colorbox{red!0}{\strut 995} \colorbox{red!44}{\strut Angel} \colorbox{red!50}{\strut Fire} \colorbox{red!5}{\strut NM} \colorbox{red!0}{\strut 87710} \colorbox{red!5}{\strut Phone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 505.377.2372} \colorbox{red!8}{\strut Email} \colorbox{red!28}{\strut Albuquerque} \colorbox{red!44}{\strut Angel} \colorbox{red!50}{\strut Fire} \colorbox{red!7}{\strut Santa} \colorbox{red!10}{\strut Fe} \colorbox{red!17}{\strut Houston} \colorbox{red!16}{\strut Dallas} \colorbox{red!17}{\strut Taos} \colorbox{red!12}{\strut Copyright} \colorbox{red!0}{\strut 2003} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut ImageBuilders} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!10}{\strut Contents} \colorbox{red!10}{\strut Business} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!32}{\strut Web} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!26}{\strut Database} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut and} \colorbox{red!26}{\strut Database} \colorbox{red!43}{\strut Design} \colorbox{red!0}{\strut ImageBuilders} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!32}{\strut Web} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!26}{\strut Database} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut and} \colorbox{red!26}{\strut Database} \colorbox{red!43}{\strut Design} \colorbox{red!17}{\strut Houston} \colorbox{red!7}{\strut Small} \colorbox{red!10}{\strut Business} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!35}{\strut Website} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!26}{\strut Database} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut and} \colorbox{red!26}{\strut Database} \colorbox{red!43}{\strut Design} \colorbox{red!8}{\strut Free} \colorbox{red!35}{\strut Website} \colorbox{red!21}{\strut Blog} \colorbox{red!5}{\strut ,} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!12}{\strut Search} \colorbox{red!0}{\strut Engine} \colorbox{red!12}{\strut Optimization} \colorbox{red!8}{\strut Services} \colorbox{red!8}{\strut Free} \colorbox{red!35}{\strut Website} \colorbox{red!21}{\strut Blog} \colorbox{red!5}{\strut ,} \colorbox{red!28}{\strut Albuquerque} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!12}{\strut Search} \colorbox{red!0}{\strut Engine} \colorbox{red!12}{\strut Optimization} \colorbox{red!8}{\strut Services} \colorbox{red!8}{\strut Free} \colorbox{red!35}{\strut Website} \colorbox{red!21}{\strut Blog} \colorbox{red!5}{\strut ,} \colorbox{red!7}{\strut Santa} \colorbox{red!10}{\strut Fe} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!12}{\strut Search} \colorbox{red!0}{\strut Engine} \colorbox{red!12}{\strut Optimization} \colorbox{red!8}{\strut Services} \colorbox{red!28}{\strut Albuquerque} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!35}{\strut Website} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut and} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!53}{\strut Hosting} \colorbox{red!17}{\strut Houston} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!35}{\strut Website} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut and} \colorbox{red!32}{\strut Web} \colorbox{red!53}{\strut Hosting} \colorbox{red!16}{\strut Dallas} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!35}{\strut Website} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut and} \colorbox{red!32}{\strut Web} \colorbox{red!53}{\strut Hosting} \colorbox{red!7}{\strut Santa} \colorbox{red!10}{\strut Fe} \colorbox{red!10}{\strut New} \colorbox{red!14}{\strut Mexico} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!35}{\strut Website} \colorbox{red!53}{\strut Hosting} \colorbox{red!8}{\strut Nationwide} \colorbox{red!32}{\strut Web} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut and} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!0}{\strut -} \colorbox{red!28}{\strut Albuquerque} \colorbox{red!5}{\strut ,} \colorbox{red!7}{\strut Santa} \colorbox{red!10}{\strut Fe} \colorbox{red!5}{\strut ,} \colorbox{red!17}{\strut Taos} \colorbox{red!5}{\strut ,} \colorbox{red!44}{\strut Angel} \colorbox{red!50}{\strut Fire} \colorbox{red!5}{\strut ,} \colorbox{red!17}{\strut Houston} \colorbox{red!5}{\strut ,} \colorbox{red!16}{\strut Dallas} \colorbox{red!8}{\strut Phoenix} \colorbox{red!8}{\strut Arizona} \colorbox{red!26}{\strut Database} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut eCommerce} \colorbox{red!35}{\strut Website} \colorbox{red!53}{\strut Hosting} \colorbox{red!1}{\strut Mesa} \colorbox{red!8}{\strut Phoenix} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!35}{\strut Website} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!5}{\strut FSBO} \colorbox{red!0}{\strut Real} \colorbox{red!8}{\strut Estate} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!0}{\strut Alamosa} \colorbox{red!14}{\strut Colorado} \colorbox{red!0}{\strut eCommerce} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!26}{\strut Database} \colorbox{red!32}{\strut Web} \colorbox{red!8}{\strut Services} \colorbox{red!3}{\strut with} \colorbox{red!7}{\strut php} \colorbox{red!0}{\strut Conejos} \colorbox{red!14}{\strut Colorado} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut Real} \colorbox{red!8}{\strut Estate} \colorbox{red!35}{\strut Website} \colorbox{red!43}{\strut Design} \colorbox{red!3}{\strut San} \colorbox{red!1}{\strut Luis} \colorbox{red!14}{\strut Colorado} \colorbox{red!32}{\strut Web} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut and} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!35}{\strut Website} \colorbox{red!53}{\strut Hosting} \colorbox{red!3}{\strut Washington} \colorbox{red!1}{\strut DC} \colorbox{red!26}{\strut Database} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut eCommerce} \colorbox{red!35}{\strut Website} \colorbox{red!53}{\strut Hosting} \colorbox{red!0}{\strut Alpharetta} \colorbox{red!8}{\strut Atlanta} \colorbox{red!26}{\strut Database} \colorbox{red!32}{\strut Web} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut ,} \colorbox{red!68}{\strut CMS} \colorbox{red!35}{\strut Website} \colorbox{red!43}{\strut Design} \colorbox{red!8}{\strut Atlanta} \colorbox{red!10}{\strut Georgia} \colorbox{red!68}{\strut CMS} \colorbox{red!26}{\strut Database} \colorbox{red!32}{\strut Web} \colorbox{red!34}{\strut Site} \colorbox{red!43}{\strut Design} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut eCommerce} \colorbox{red!35}{\strut Website} \colorbox{red!53}{\strut Hosting} \colorbox{red!5}{\strut Brazil} 
}}}
\end{CJK*}

98:website, 89:design, 59:what, 44:hosting, 21:email, 20:web, 20:services, 19:professional, 18:online, 18:business


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 61} \colorbox{red!1}{\strut 3} \colorbox{red!0}{\strut 8624} \colorbox{red!0}{\strut 2300Call} \colorbox{red!1}{\strut us} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut speak} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut realeBusiness} \colorbox{red!5}{\strut Consultant} \colorbox{red!4}{\strut PRODUCTS} \colorbox{red!3}{\strut Domain} \colorbox{red!1}{\strut Names} \colorbox{red!7}{\strut Email} \colorbox{red!7}{\strut Services} \colorbox{red!34}{\strut Website} \colorbox{red!15}{\strut Hosting} \colorbox{red!34}{\strut Website} \colorbox{red!31}{\strut Design} \colorbox{red!6}{\strut Online} \colorbox{red!3}{\strut Marketing} \colorbox{red!2}{\strut Dedicated} \colorbox{red!2}{\strut Servers} \colorbox{red!2}{\strut Office} \colorbox{red!5}{\strut Tools} \colorbox{red!34}{\strut Website} \colorbox{red!3}{\strut Security} \colorbox{red!1}{\strut MY} \colorbox{red!1}{\strut ACCOUNT} \colorbox{red!2}{\strut Log} \colorbox{red!1}{\strut In} \colorbox{red!2}{\strut New} \colorbox{red!1}{\strut Account} \colorbox{red!2}{\strut Password} \colorbox{red!1}{\strut Recovery} \colorbox{red!1}{\strut RENEW} \colorbox{red!1}{\strut Renew} \colorbox{red!3}{\strut Domain} \colorbox{red!1}{\strut PROGRAMS} \colorbox{red!2}{\strut Reseller} \colorbox{red!2}{\strut Affiliate} \colorbox{red!0}{\strut Program} \colorbox{red!3}{\strut WHOIS} \colorbox{red!3}{\strut Whois} \colorbox{red!2}{\strut Lookup} \colorbox{red!2}{\strut HELP} \colorbox{red!1}{\strut Sitemap} \colorbox{red!2}{\strut Help} \colorbox{red!1}{\strut Centre} \colorbox{red!2}{\strut Contact} \colorbox{red!1}{\strut Us} \colorbox{red!2}{\strut Pricing} \colorbox{red!0}{\strut ABOUT} \colorbox{red!3}{\strut Company} \colorbox{red!4}{\strut People} \colorbox{red!2}{\strut Investors} \colorbox{red!2}{\strut Careers} \colorbox{red!2}{\strut Log} \colorbox{red!1}{\strut In} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Order} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut .} \colorbox{red!34}{\strut Website} \colorbox{red!31}{\strut Design} \colorbox{red!34}{\strut Website} \colorbox{red!31}{\strut Design} \colorbox{red!1}{\strut and} \colorbox{red!7}{\strut Web} \colorbox{red!5}{\strut Development} \colorbox{red!6}{\strut Professional} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut effective} \colorbox{red!0}{\strut websites} \colorbox{red!4}{\strut Stand} \colorbox{red!1}{\strut out} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut a} \colorbox{red!34}{\strut website} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut your} \colorbox{red!6}{\strut business} \colorbox{red!1}{\strut In} \colorbox{red!3}{\strut today} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut marketplace} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut a} \colorbox{red!6}{\strut professional} \colorbox{red!1}{\strut and} \colorbox{red!5}{\strut effective} \colorbox{red!34}{\strut website} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut essential} \colorbox{red!0}{\strut if} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut want} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut stand-out} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut your} \colorbox{red!2}{\strut competitors} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Research} \colorbox{red!0}{\strut shows} \colorbox{red!1}{\strut that} \colorbox{red!1}{\strut more} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut more} \colorbox{red!2}{\strut consumers} \colorbox{red!1}{\strut use} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Internet} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut research} \colorbox{red!2}{\strut buying} \colorbox{red!2}{\strut decisions} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut wide} \colorbox{red!1}{\strut range} \colorbox{red!1}{\strut of} \colorbox{red!4}{\strut products} \colorbox{red!1}{\strut and} \colorbox{red!7}{\strut services} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut In} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut recent} \colorbox{red!0}{\strut Nielson} \colorbox{red!6}{\strut Online} \colorbox{red!1}{\strut survey} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 58} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut consumers} \colorbox{red!1}{\strut indicated} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Internet} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut preferred} \colorbox{red!1}{\strut information} \colorbox{red!1}{\strut source} \colorbox{red!0}{\strut This} \colorbox{red!2}{\strut means} \colorbox{red!0}{\strut if} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!1}{\strut have} \colorbox{red!1}{\strut a} \colorbox{red!34}{\strut website} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut missing} \colorbox{red!1}{\strut out} \colorbox{red!0}{\strut on} \colorbox{red!6}{\strut business} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut At} \colorbox{red!2}{\strut Melbourne} \colorbox{red!1}{\strut IT} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!1}{\strut understand} \colorbox{red!1}{\strut that} \colorbox{red!1}{\strut building} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut redesigning} \colorbox{red!1}{\strut your} \colorbox{red!34}{\strut website} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut hard} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Our} \colorbox{red!1}{\strut local} \colorbox{red!0}{\strut eBusiness} \colorbox{red!0}{\strut consultants} \colorbox{red!2}{\strut speak} \colorbox{red!1}{\strut your} \colorbox{red!1}{\strut language} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut work} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut understand} \colorbox{red!1}{\strut your} \colorbox{red!6}{\strut business} \colorbox{red!3}{\strut needs} \colorbox{red!1}{\strut before} \colorbox{red!1}{\strut recommending} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut best} \colorbox{red!1}{\strut solution} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut you} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut helped} \colorbox{red!0}{\strut thousands} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut businesses} \colorbox{red!1}{\strut create} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut update} \colorbox{red!1}{\strut a} \colorbox{red!34}{\strut website} \colorbox{red!2}{\strut customised} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut their} \colorbox{red!2}{\strut requirements} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Next} \colorbox{red!1}{\strut steps} \colorbox{red!1}{\strut Try} \colorbox{red!1}{\strut it} \colorbox{red!1}{\strut out} \colorbox{red!3}{\strut today} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut use} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut real} \colorbox{red!1}{\strut demo} \colorbox{red!1}{\strut Login} \colorbox{red!1}{\strut as} \colorbox{red!2}{\strut sitedemo} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut melbourneitwebsites.com} \colorbox{red!0}{\strut using} \colorbox{red!2}{\strut password} \colorbox{red!2}{\strut sitedemo} \colorbox{red!1}{\strut View} \colorbox{red!0}{\strut sample} \colorbox{red!1}{\strut templates} \colorbox{red!1}{\strut Get} \colorbox{red!1}{\strut started} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut free} \colorbox{red!1}{\strut quote} \colorbox{red!4}{\strut Which} \colorbox{red!4}{\strut site} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut right} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut you} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Do-It-Yourself} \colorbox{red!1}{\strut Get} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut starter} \colorbox{red!34}{\strut website} \colorbox{red!1}{\strut fast} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Stunning} \colorbox{red!1}{\strut templates} \colorbox{red!0}{\strut No} \colorbox{red!1}{\strut technical} \colorbox{red!3}{\strut skills} \colorbox{red!0}{\strut needed} \colorbox{red!0}{\strut Product} \colorbox{red!1}{\strut image} \colorbox{red!1}{\strut gallery} \colorbox{red!1}{\strut Easy} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut use} \colorbox{red!1}{\strut builder} \colorbox{red!0}{\strut tool} \colorbox{red!7}{\strut Email} \colorbox{red!1}{\strut and} \colorbox{red!15}{\strut hosting} \colorbox{red!2}{\strut included} \colorbox{red!1}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut find} \colorbox{red!1}{\strut out} \colorbox{red!1}{\strut more} \colorbox{red!0}{\strut Done-For-You} \colorbox{red!1}{\strut Your} \colorbox{red!2}{\strut content} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut our} \colorbox{red!31}{\strut design} \colorbox{red!1}{\strut Stunning} \colorbox{red!1}{\strut templates} \colorbox{red!0}{\strut No} \colorbox{red!1}{\strut technical} \colorbox{red!3}{\strut skills} \colorbox{red!0}{\strut needed} \colorbox{red!1}{\strut Easy} \colorbox{red!1}{\strut to} 
}}}
\end{CJK*}

query: gps

100:gps, 76:bluetooth, 29:price, 19:navigation, 17:name, 16:mk, 15:supply, 15:products, 15:new, 15:chinese


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Welcome} \colorbox{red!0}{\strut buyer-} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut First} \colorbox{red!3}{\strut Visit} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2009-1-20} \colorbox{red!0}{\strut 84154} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut Your} \colorbox{red!6}{\strut Message} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 0} \colorbox{red!14}{\strut companies} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 0} \colorbox{red!18}{\strut new} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 0} \colorbox{red!3}{\strut reply} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut Post} \colorbox{red!2}{\strut Your} \colorbox{red!12}{\strut Buy} \colorbox{red!13}{\strut Offer} \colorbox{red!100}{\strut GPS} \colorbox{red!18}{\strut Products} \colorbox{red!0}{\strut Not} \colorbox{red!4}{\strut a} \colorbox{red!7}{\strut member} \colorbox{red!2}{\strut yet} \colorbox{red!0}{\strut ?} \colorbox{red!6}{\strut Join} \colorbox{red!3}{\strut For} \colorbox{red!3}{\strut FREE} \colorbox{red!18}{\strut New} \colorbox{red!0}{\strut Product} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Product} \colorbox{red!20}{\strut Name} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut mk-722} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 7gps} \colorbox{red!4}{\strut with} \colorbox{red!91}{\strut bluetooth} \colorbox{red!3}{\strut ,} \colorbox{red!9}{\strut FM} \colorbox{red!3}{\strut ,} \colorbox{red!9}{\strut AV} \colorbox{red!4}{\strut in} \colorbox{red!3}{\strut ,} \colorbox{red!12}{\strut sd} \colorbox{red!12}{\strut card} \colorbox{red!6}{\strut .} \colorbox{red!34}{\strut Price} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut US} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Detail} \colorbox{red!3}{\strut .} \colorbox{red!9}{\strut Touch} \colorbox{red!14}{\strut screen} \colorbox{red!8}{\strut TFT} \colorbox{red!7}{\strut LCD} \colorbox{red!10}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut with} \colorbox{red!0}{\strut build-in} \colorbox{red!100}{\strut GPS} \colorbox{red!12}{\strut receiver} \colorbox{red!4}{\strut and} \colorbox{red!91}{\strut Bluetooth} \colorbox{red!0}{\strut Shirf} \colorbox{red!10}{\strut star} \colorbox{red!0}{\strut IIIBuilt-in} \colorbox{red!100}{\strut GPS} \colorbox{red!7}{\strut antenna} \colorbox{red!6}{\strut CPU} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut S3C2440A} \colorbox{red!1}{\strut 400MHz} \colorbox{red!0}{\strut WinCE} \colorbox{red!4}{\strut .} \colorbox{red!4}{\strut Net} \colorbox{red!0}{\strut 4.2} \colorbox{red!0}{\strut Core} \colorbox{red!4}{\strut SDRAM} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Low} \colorbox{red!6}{\strut Power} \colorbox{red!0}{\strut 64MB} \colorbox{red!2}{\strut Nand} \colorbox{red!4}{\strut Flash} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 3264128256512MB1GB} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut optional} \colorbox{red!6}{\strut .} \colorbox{red!12}{\strut SD} \colorbox{red!4}{\strut memory} \colorbox{red!4}{\strut Slot} \colorbox{red!3}{\strut ,} \colorbox{red!12}{\strut SD} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 128MB-2GB} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut Support} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut MP3} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut Movie} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut Photo} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut E-Book} \colorbox{red!4}{\strut With} \colorbox{red!91}{\strut Bluetooth} \colorbox{red!1}{\strut More} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut More} \colorbox{red!100}{\strut GPS} \colorbox{red!9}{\strut Exporters} \colorbox{red!4}{\strut at} \colorbox{red!3}{\strut Waimao8} \colorbox{red!0}{\strut mk-722} \colorbox{red!0}{\strut mk-308} \colorbox{red!0}{\strut mk-488} \colorbox{red!0}{\strut 4.3} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut touch} \colorbox{red!14}{\strut screen} \colorbox{red!0}{\strut DVB-T} \colorbox{red!9}{\strut tv} \colorbox{red!4}{\strut with} \colorbox{red!100}{\strut GPS} \colorbox{red!9}{\strut mp4} \colorbox{red!13}{\strut functions} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut Navigation} \colorbox{red!15}{\strut System} \colorbox{red!6}{\strut Weltone} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut Anti-theft} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -robbing} \colorbox{red!15}{\strut System} \colorbox{red!0}{\strut 7.0inch} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut 4.3inch} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut G-1.47} \colorbox{red!18}{\strut New} \colorbox{red!8}{\strut item} \colorbox{red!0}{\strut 3.5inch} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut Navigation} \colorbox{red!0}{\strut 3.5inch} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut Navigation} \colorbox{red!0}{\strut 4.3inch} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut 3.5inch} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut Navigation} \colorbox{red!18}{\strut supply} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut gps} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!0}{\strut GPS20081121} \colorbox{red!18}{\strut supply} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut gps} \colorbox{red!22}{\strut navigation} \colorbox{red!1}{\strut 20081121} \colorbox{red!18}{\strut supply} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut gps} \colorbox{red!22}{\strut navigation} \colorbox{red!1}{\strut 20081121} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut gps} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut gps} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut gps} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut manufacturer20081121} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut manufacturer20081121} \colorbox{red!18}{\strut supply} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut gps} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut GPS20081121} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut navigation20081121} \colorbox{red!18}{\strut supply} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!1}{\strut 20081121} \colorbox{red!18}{\strut supply} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!1}{\strut 20081121} \colorbox{red!18}{\strut supply} \colorbox{red!15}{\strut daobao} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!1}{\strut 20081121} \colorbox{red!100}{\strut GPS} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut GPS} \colorbox{red!22}{\strut navigation} \colorbox{red!3}{\strut ,} \colorbox{red!16}{\strut china} 
}}}
\end{CJK*}

99:gps, 90:invented, 47:broadcom, 31:team, 21:company, 16:that, 15:fast, 12:part, 10:live, 7:scobleizer


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!53}{\strut Broadcom} \colorbox{red!17}{\strut Fast} \colorbox{red!23}{\strut Company} \colorbox{red!11}{\strut Live} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!2}{\strut 5} \colorbox{red!3}{\strut Thursday} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut November} \colorbox{red!6}{\strut 27th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!2}{\strut 5} \colorbox{red!17}{\strut Fast} \colorbox{red!23}{\strut Company} \colorbox{red!11}{\strut Live} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!1}{\strut 3} \colorbox{red!3}{\strut Thursday} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut November} \colorbox{red!6}{\strut 27th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!1}{\strut 3} \colorbox{red!17}{\strut Fast} \colorbox{red!23}{\strut Company} \colorbox{red!11}{\strut Live} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!3}{\strut 1} \colorbox{red!3}{\strut Thursday} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut November} \colorbox{red!6}{\strut 27th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!3}{\strut 1} \colorbox{red!17}{\strut Fast} \colorbox{red!23}{\strut Company} \colorbox{red!11}{\strut Live} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!2}{\strut 4} \colorbox{red!3}{\strut Thursday} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut November} \colorbox{red!6}{\strut 27th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!2}{\strut 4} \colorbox{red!17}{\strut Fast} \colorbox{red!23}{\strut Company} \colorbox{red!11}{\strut Live} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!4}{\strut 2} \colorbox{red!3}{\strut Thursday} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut November} \colorbox{red!6}{\strut 27th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!53}{\strut Broadcom} \colorbox{red!35}{\strut team} \colorbox{red!18}{\strut that} \colorbox{red!100}{\strut invented} \colorbox{red!100}{\strut GPS} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Part} \colorbox{red!4}{\strut 2} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!3}{\strut Home} \colorbox{red!7}{\strut Scobleizer} \colorbox{red!6}{\strut TV} \colorbox{red!17}{\strut Fast} \colorbox{red!23}{\strut Company} \colorbox{red!11}{\strut Live} \colorbox{red!0}{\strut WorkFast} \colorbox{red!6}{\strut TV} \colorbox{red!0}{\strut Recent} \colorbox{red!0}{\strut Comments} \colorbox{red!0}{\strut About} \colorbox{red!17}{\strut Fast} \colorbox{red!23}{\strut Company} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Privacy} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Terms} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Service} \colorbox{red!3}{\strut Mansueto} \colorbox{red!4}{\strut Digital} \colorbox{red!4}{\strut Network} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Inc.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FastCompany.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut IncBizNet.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut IncTechnology.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FastCompany.TV} \colorbox{red!0}{\strut Advertise} \colorbox{red!1}{\strut Copyright} \colorbox{red!3}{\strut Mansueto} \colorbox{red!4}{\strut Ventures} \colorbox{red!2}{\strut LLC} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut reserved} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Inc.com} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 7} \colorbox{red!5}{\strut World} \colorbox{red!3}{\strut Trade} \colorbox{red!2}{\strut Center} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut New} \colorbox{red!0}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut NY} \colorbox{red!0}{\strut 10007-2195} 
}}}
\end{CJK*}

query: michworks

99:county, 86:calhoun, 73:mi, 60:michigan, 34:marshall, 14:government, 9:working, 9:map, 9:green, 9:employment


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!11}{\strut Employment} \colorbox{red!100}{\strut County} \colorbox{red!7}{\strut Building} \colorbox{red!7}{\strut Building} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Better} \colorbox{red!100}{\strut County} \colorbox{red!2}{\strut Through} \colorbox{red!2}{\strut Responsive} \colorbox{red!5}{\strut Leadership} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut more} \colorbox{red!5}{\strut details} \colorbox{red!0}{\strut about} \colorbox{red!11}{\strut employment} \colorbox{red!7}{\strut opportunities} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!3}{\strut latest} \colorbox{red!7}{\strut job} \colorbox{red!7}{\strut openings} \colorbox{red!5}{\strut with} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut please} \colorbox{red!1}{\strut click} \colorbox{red!0}{\strut here} \colorbox{red!5}{\strut to} \colorbox{red!6}{\strut visit} \colorbox{red!0}{\strut our} \colorbox{red!6}{\strut Human} \colorbox{red!5}{\strut Resources} \colorbox{red!2}{\strut Department} \colorbox{red!6}{\strut .} \colorbox{red!5}{\strut To} \colorbox{red!0}{\strut discover} \colorbox{red!0}{\strut other} \colorbox{red!7}{\strut job} \colorbox{red!7}{\strut opportunities} \colorbox{red!0}{\strut outside} \colorbox{red!5}{\strut of} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!18}{\strut Government} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut please} \colorbox{red!6}{\strut visit} \colorbox{red!2}{\strut the} \colorbox{red!1}{\strut following} \colorbox{red!10}{\strut sites} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Talent} \colorbox{red!6}{\strut Bank} \colorbox{red!3}{\strut -} \colorbox{red!0}{\strut MTBEMPL.EntryMainPage} \colorbox{red!9}{\strut Michworks} \colorbox{red!5}{\strut Partner} \colorbox{red!0}{\strut Site} \colorbox{red!3}{\strut -} \colorbox{red!1}{\strut http} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut www.michpartners.org} \colorbox{red!6}{\strut CENTS} \colorbox{red!7}{\strut Home} \colorbox{red!7}{\strut Page} \colorbox{red!3}{\strut -} \colorbox{red!0}{\strut www.centjobs.com} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!18}{\strut Government} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Visiting} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!3}{\strut .} \colorbox{red!9}{\strut Living} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!11}{\strut Working} \colorbox{red!0}{\strut in} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!3}{\strut .} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!0}{\strut Departments} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut Online} \colorbox{red!5}{\strut Reference} \colorbox{red!5}{\strut Desk} \colorbox{red!3}{\strut Help} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut Home} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut Event} \colorbox{red!5}{\strut Calendar} \colorbox{red!3}{\strut .} \colorbox{red!9}{\strut Weather} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut Search} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Site} \colorbox{red!11}{\strut Map} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!6}{\strut 315} \colorbox{red!7}{\strut West} \colorbox{red!11}{\strut Green} \colorbox{red!7}{\strut Street} \colorbox{red!44}{\strut Marshall} \colorbox{red!3}{\strut ,} \colorbox{red!94}{\strut MI} \colorbox{red!3}{\strut 49068} \colorbox{red!10}{\strut Phone} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 269} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 781-0700} \colorbox{red!6}{\strut Fax} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 269} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 781-0140} \colorbox{red!1}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!5}{\strut to} \colorbox{red!5}{\strut contact} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut webmaster} \colorbox{red!6}{\strut at} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!5}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut commentsfeedback} \colorbox{red!2}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!5}{\strut website} \colorbox{red!6}{\strut .} \colorbox{red!1}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!5}{\strut to} \colorbox{red!3}{\strut report} \colorbox{red!1}{\strut technical} \colorbox{red!0}{\strut problems} \colorbox{red!5}{\strut with} \colorbox{red!0}{\strut this} \colorbox{red!5}{\strut website} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut i.e.} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut broken} \colorbox{red!2}{\strut links} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut pages} \colorbox{red!2}{\strut not} \colorbox{red!7}{\strut found} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut Several} \colorbox{red!5}{\strut photos} \colorbox{red!3}{\strut included} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut web} \colorbox{red!0}{\strut site} \colorbox{red!2}{\strut were} \colorbox{red!3}{\strut provided} \colorbox{red!3}{\strut courtesy} \colorbox{red!5}{\strut of} \colorbox{red!5}{\strut Scene} \colorbox{red!2}{\strut Magazine} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!7}{\strut page} \colorbox{red!0}{\strut last} \colorbox{red!3}{\strut modified} \colorbox{red!0}{\strut 080305} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!5}{\strut information} \colorbox{red!0}{\strut 2004} \colorbox{red!100}{\strut Calhoun} \colorbox{red!100}{\strut County} \colorbox{red!3}{\strut ,} \colorbox{red!78}{\strut Michigan} \colorbox{red!3}{\strut DHTML} \colorbox{red!3}{\strut Menu} \colorbox{red!3}{\strut By} \colorbox{red!5}{\strut Milonic} \colorbox{red!0}{\strut JavaScript} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut Use} \colorbox{red!7}{\strut Policy} \colorbox{red!0}{\strut Site} \colorbox{red!0}{\strut DesignDevelopment} \colorbox{red!3}{\strut by} 
}}}
\end{CJK*}

97:michigan, 75:number, 43:phone, 41:works, 21:employer, 20:mwa, 17:michworks, 17:disabilities, 16:name, 16:agencies


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut If} \colorbox{red!3}{\strut you} \colorbox{red!3}{\strut are} \colorbox{red!2}{\strut a} \colorbox{red!6}{\strut Job} \colorbox{red!2}{\strut Seeker} \colorbox{red!1}{\strut or} \colorbox{red!12}{\strut Employer} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut are} \colorbox{red!4}{\strut looking} \colorbox{red!3}{\strut for} \colorbox{red!5}{\strut the} \colorbox{red!59}{\strut Michigan} \colorbox{red!8}{\strut Talent} \colorbox{red!8}{\strut Bank} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut follow} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut link} \colorbox{red!1}{\strut below} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut www.michworks.org} \colorbox{red!1}{\strut If} \colorbox{red!3}{\strut you} \colorbox{red!3}{\strut are} \colorbox{red!2}{\strut a} \colorbox{red!12}{\strut MWA} \colorbox{red!8}{\strut Member} \colorbox{red!1}{\strut or} \colorbox{red!4}{\strut Associate} \colorbox{red!8}{\strut Member} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!2}{\strut remove} \colorbox{red!5}{\strut the} \colorbox{red!1}{\strut information} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut UserName} \colorbox{red!1}{\strut and} \colorbox{red!8}{\strut Password} \colorbox{red!4}{\strut Boxes} \colorbox{red!1}{\strut below} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut The} \colorbox{red!1}{\strut information} \colorbox{red!2}{\strut in} \colorbox{red!5}{\strut the} \colorbox{red!4}{\strut boxes} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut meet} \colorbox{red!9}{\strut ADA} \colorbox{red!8}{\strut requirements} \colorbox{red!2}{\strut .} \colorbox{red!59}{\strut Michigan} \colorbox{red!25}{\strut Works} \colorbox{red!1}{\strut -} \colorbox{red!3}{\strut Login} \colorbox{red!0}{\strut Use} \colorbox{red!5}{\strut the} \colorbox{red!3}{\strut form} \colorbox{red!1}{\strut below} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut log} \colorbox{red!2}{\strut in} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!3}{\strut site} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut UserName} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Password} \colorbox{red!0}{\strut .} \colorbox{red!59}{\strut Michigan} \colorbox{red!25}{\strut Works} \colorbox{red!2}{\strut !} \colorbox{red!0}{\strut Association} \colorbox{red!5}{\strut The} \colorbox{red!0}{\strut Association} \colorbox{red!4}{\strut of} \colorbox{red!59}{\strut Michigan} \colorbox{red!25}{\strut Works} \colorbox{red!2}{\strut !} \colorbox{red!9}{\strut Agencies} \colorbox{red!3}{\strut 2500} \colorbox{red!2}{\strut Kerry} \colorbox{red!5}{\strut Street} \colorbox{red!1}{\strut -} \colorbox{red!4}{\strut Suite} \colorbox{red!0}{\strut 210} \colorbox{red!1}{\strut -} \colorbox{red!4}{\strut Lansing} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut MI} \colorbox{red!2}{\strut 48912} \colorbox{red!26}{\strut Phone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 517-371-1100} \colorbox{red!5}{\strut Fax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 517-371-1140} \colorbox{red!0}{\strut e-mail} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut info} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut michiganworks.org} \colorbox{red!2}{\strut In} \colorbox{red!1}{\strut accordance} \colorbox{red!2}{\strut with} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut Americans} \colorbox{red!2}{\strut With} \colorbox{red!10}{\strut Disabilities} \colorbox{red!6}{\strut Act} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut ADA} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!1}{\strut information} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut site} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut available} \colorbox{red!2}{\strut in} \colorbox{red!2}{\strut an} \colorbox{red!0}{\strut alternative} \colorbox{red!0}{\strut format} \colorbox{red!0}{\strut upon} \colorbox{red!3}{\strut request} \colorbox{red!3}{\strut received} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut office} \colorbox{red!2}{\strut .} \colorbox{red!59}{\strut Michigan} \colorbox{red!8}{\strut Relay} \colorbox{red!46}{\strut number} \colorbox{red!3}{\strut for} \colorbox{red!5}{\strut the} \colorbox{red!6}{\strut Deaf} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 800} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 649-3777} \colorbox{red!5}{\strut The} \colorbox{red!59}{\strut Michigan} \colorbox{red!25}{\strut Works} \colorbox{red!2}{\strut !} \colorbox{red!0}{\strut Association} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut an} \colorbox{red!3}{\strut Equal} \colorbox{red!7}{\strut Opportunity} \colorbox{red!0}{\strut EmployerTrainer} \colorbox{red!2}{\strut Privacy} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut Security} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut Disclaimer} \colorbox{red!1}{\strut Statements} 
}}}
\end{CJK*}

query: orange county convention center

93:county, 92:convention, 78:center, 57:orange, 46:occc, 43:florida, 35:orlando, 25:located, 18:facility, 16:hotel


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Community} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Public} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!73}{\strut Center} \colorbox{red!2}{\strut of} \colorbox{red!14}{\strut Hospitality} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Since} \colorbox{red!3}{\strut 1983} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!86}{\strut Convention} \colorbox{red!73}{\strut Center} \colorbox{red!4}{\strut .} \colorbox{red!43}{\strut OCCC} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut has} \colorbox{red!4}{\strut served} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut clients} \colorbox{red!3}{\strut as} \colorbox{red!2}{\strut a} \colorbox{red!11}{\strut venue} \colorbox{red!2}{\strut for} \colorbox{red!8}{\strut trade} \colorbox{red!7}{\strut shows} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut assemblies} \colorbox{red!4}{\strut and} \colorbox{red!0}{\strut meetings.During} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut span} \colorbox{red!3}{\strut the} \colorbox{red!16}{\strut facility} \colorbox{red!3}{\strut has} \colorbox{red!3}{\strut undergone} \colorbox{red!2}{\strut five} \colorbox{red!2}{\strut extensive} \colorbox{red!7}{\strut expansion} \colorbox{red!0}{\strut periods.It} \colorbox{red!4}{\strut is} \colorbox{red!2}{\strut now} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut nation} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut second} \colorbox{red!6}{\strut largest} \colorbox{red!86}{\strut convention} \colorbox{red!73}{\strut center} \colorbox{red!4}{\strut .} \colorbox{red!12}{\strut Owned} \colorbox{red!4}{\strut and} \colorbox{red!11}{\strut operated} \colorbox{red!1}{\strut by} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!9}{\strut Government} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!43}{\strut OCCC} \colorbox{red!4}{\strut provides} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1.4} \colorbox{red!3}{\strut billion} \colorbox{red!3}{\strut dollar} \colorbox{red!2}{\strut total} \colorbox{red!10}{\strut economic} \colorbox{red!6}{\strut impact} \colorbox{red!2}{\strut annually} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut Central} \colorbox{red!40}{\strut Florida} \colorbox{red!8}{\strut economy} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut all} \colorbox{red!4}{\strut at} \colorbox{red!0}{\strut no} \colorbox{red!14}{\strut cost} \colorbox{red!1}{\strut to} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!3}{\strut Citizens} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Choose} \colorbox{red!3}{\strut from} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut links} \colorbox{red!1}{\strut below} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!1}{\strut more} \colorbox{red!2}{\strut about} \colorbox{red!3}{\strut the} \colorbox{red!43}{\strut OCCC} \colorbox{red!16}{\strut facility} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut note} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut need} \colorbox{red!2}{\strut Adobe} \colorbox{red!1}{\strut Acrobat} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut read} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut documents} \colorbox{red!4}{\strut and} \colorbox{red!1}{\strut maps} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Follow} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut link} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut download} \colorbox{red!2}{\strut Adobe} \colorbox{red!1}{\strut Acrobat} \colorbox{red!4}{\strut .} \colorbox{red!4}{\strut Fiscal} \colorbox{red!0}{\strut Year} \colorbox{red!1}{\strut Analysis} \colorbox{red!0}{\strut 2006-07} \colorbox{red!16}{\strut Facility} \colorbox{red!0}{\strut Facts} \colorbox{red!0}{\strut Fun} \colorbox{red!0}{\strut Facts} \colorbox{red!3}{\strut Features} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut NorthSouth} \colorbox{red!15}{\strut Building} \colorbox{red!3}{\strut Features} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut West} \colorbox{red!15}{\strut Building} \colorbox{red!0}{\strut Boosting} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut Local} \colorbox{red!8}{\strut Economy} \colorbox{red!0}{\strut Every} \colorbox{red!0}{\strut year} \colorbox{red!3}{\strut the} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!86}{\strut Convention} \colorbox{red!73}{\strut Center} \colorbox{red!5}{\strut plays} \colorbox{red!5}{\strut host} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut million} \colorbox{red!7}{\strut attendees} \colorbox{red!3}{\strut ,} \colorbox{red!1}{\strut generating} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut impressive} \colorbox{red!10}{\strut economic} \colorbox{red!6}{\strut impact} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut local} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!8}{\strut economy} \colorbox{red!4}{\strut .} \colorbox{red!8}{\strut Community} \colorbox{red!0}{\strut Frequently} \colorbox{red!0}{\strut Asked} \colorbox{red!0}{\strut Questions} \colorbox{red!10}{\strut Economic} \colorbox{red!6}{\strut Impact} \colorbox{red!2}{\strut Be} \colorbox{red!2}{\strut a} \colorbox{red!8}{\strut Community} \colorbox{red!0}{\strut Ambassador} \colorbox{red!2}{\strut !} \colorbox{red!4}{\strut Help} \colorbox{red!0}{\strut bring} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut organization} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut meeting} \colorbox{red!1}{\strut to} \colorbox{red!32}{\strut Orlando} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut the} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!86}{\strut Convention} \colorbox{red!73}{\strut Center} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Click} \colorbox{red!2}{\strut here} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut read} \colorbox{red!1}{\strut more} \colorbox{red!4}{\strut .} \colorbox{red!11}{\strut Downtown} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Shining} \colorbox{red!4}{\strut Star} \colorbox{red!3}{\strut The} \colorbox{red!43}{\strut OCCC} \colorbox{red!3}{\strut ,} \colorbox{red!23}{\strut located} \colorbox{red!0}{\strut 12} \colorbox{red!4}{\strut miles} \colorbox{red!3}{\strut from} \colorbox{red!3}{\strut the} \colorbox{red!32}{\strut Orlando} \colorbox{red!4}{\strut International} \colorbox{red!7}{\strut Airport} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut is} \colorbox{red!10}{\strut situated} \colorbox{red!2}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut heart} \colorbox{red!2}{\strut of} \colorbox{red!11}{\strut Downtown} \colorbox{red!53}{\strut Orange} \colorbox{red!87}{\strut County} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut area} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut tourism} \colorbox{red!0}{\strut core} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!43}{\strut OCCC} \colorbox{red!4}{\strut is} \colorbox{red!3}{\strut within} \colorbox{red!2}{\strut close} \colorbox{red!5}{\strut proximity} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 8,000} \colorbox{red!15}{\strut hotel} \colorbox{red!4}{\strut rooms} \colorbox{red!4}{\strut and} \colorbox{red!3}{\strut within} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut 45-minute} \colorbox{red!1}{\strut driving} \colorbox{red!6}{\strut distance} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut 113,000} \colorbox{red!1}{\strut more} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut For} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut map} \colorbox{red!2}{\strut of} \colorbox{red!4}{\strut nearby} \colorbox{red!0}{\strut hotels} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut click} \colorbox{red!2}{\strut here} \colorbox{red!4}{\strut .} \colorbox{red!3}{\strut The} \colorbox{red!43}{\strut OCCC} \colorbox{red!1}{\strut also} \colorbox{red!2}{\strut works} \colorbox{red!0}{\strut closely} \colorbox{red!1}{\strut with} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut OrlandoOrange} \colorbox{red!87}{\strut County} \colorbox{red!86}{\strut Convention} \colorbox{red!4}{\strut and} \colorbox{red!7}{\strut Visitors} \colorbox{red!0}{\strut Bureau} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut Working} \colorbox{red!0}{\strut Hand} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut Hand} \colorbox{red!1}{\strut with} \colorbox{red!3}{\strut the} \colorbox{red!53}{\strut Orange} 
}}}
\end{CJK*}

99:center, 98:convention, 91:county, 87:orange, 37:florida, 34:price, 34:orlando, 30:service, 26:ny, 26:canaveral


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut HAPPY} \colorbox{red!0}{\strut PEOPLE} \colorbox{red!0}{\strut ON} \colorbox{red!0}{\strut THE} \colorbox{red!1}{\strut MOVE} \colorbox{red!0}{\strut InterPlex} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!13}{\strut Orlando} \colorbox{red!6}{\strut Transportation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Attractions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!33}{\strut Orange} \colorbox{red!35}{\strut County} \colorbox{red!37}{\strut Convention} \colorbox{red!38}{\strut Center} \colorbox{red!1}{\strut For} \colorbox{red!11}{\strut Service} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut other} \colorbox{red!6}{\strut Metro} \colorbox{red!2}{\strut Areas} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Chicago} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut IL} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut USA} \colorbox{red!5}{\strut New} \colorbox{red!4}{\strut York} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut NY} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut USA} \colorbox{red!7}{\strut Port} \colorbox{red!10}{\strut Canaveral} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut FL} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut USA} \colorbox{red!2}{\strut Sofia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Bulgaria} \colorbox{red!0}{\strut InterPlex} \colorbox{red!2}{\strut provides} \colorbox{red!2}{\strut shuttle} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut limo} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut town} \colorbox{red!8}{\strut car} \colorbox{red!6}{\strut transportation} \colorbox{red!0}{\strut to} \colorbox{red!33}{\strut Orange} \colorbox{red!35}{\strut County} \colorbox{red!37}{\strut Convention} \colorbox{red!38}{\strut Center} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!1}{\strut addition} \colorbox{red!0}{\strut we} \colorbox{red!11}{\strut service} \colorbox{red!1}{\strut theme} \colorbox{red!3}{\strut parks} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut attractions} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut all} \colorbox{red!2}{\strut Central} \colorbox{red!14}{\strut Florida} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut South} \colorbox{red!14}{\strut Florida} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut North} \colorbox{red!14}{\strut Florida} \colorbox{red!7}{\strut locations} \colorbox{red!0}{\strut .} \colorbox{red!33}{\strut Orange} \colorbox{red!35}{\strut County} \colorbox{red!37}{\strut Convention} \colorbox{red!38}{\strut Center} \colorbox{red!3}{\strut offers} \colorbox{red!5}{\strut space} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut large} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut host} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut business-related} \colorbox{red!6}{\strut international} \colorbox{red!37}{\strut convention} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut good} \colorbox{red!1}{\strut hands} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut InterPlex} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Check} \colorbox{red!1}{\strut our} \colorbox{red!1}{\strut references} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut proceed} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut confidence} \colorbox{red!1}{\strut !} \colorbox{red!33}{\strut Orange} \colorbox{red!35}{\strut County} \colorbox{red!37}{\strut Convention} \colorbox{red!38}{\strut Center} \colorbox{red!3}{\strut offers} \colorbox{red!0}{\strut 2.1} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut sq.ft} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut exhibition} \colorbox{red!5}{\strut space} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut two} \colorbox{red!0}{\strut 92,000} \colorbox{red!0}{\strut sq.ft} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut assembly} \colorbox{red!2}{\strut areas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 74} \colorbox{red!1}{\strut meeting} \colorbox{red!1}{\strut rooms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2,643-seat} \colorbox{red!0}{\strut Chapin} \colorbox{red!2}{\strut Theater} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 160-seat} \colorbox{red!0}{\strut Lecture} \colorbox{red!0}{\strut Hall} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 62,000} \colorbox{red!0}{\strut sq.ft} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut multi-purpose} \colorbox{red!0}{\strut room} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut full-service} \colorbox{red!3}{\strut restaurants} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut on-site} \colorbox{red!0}{\strut parking} \colorbox{red!0}{\strut lot} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 6000} \colorbox{red!0}{\strut cars} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Simply} \colorbox{red!1}{\strut position} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut cursor} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut relevant} \colorbox{red!0}{\strut price-cell} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut follow} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut proceed} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut confidence} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut book} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut trip} \colorbox{red!1}{\strut online} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut Our} \colorbox{red!11}{\strut service} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut guaranteed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut backed} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Better} \colorbox{red!1}{\strut Business} \colorbox{red!0}{\strut Bureau} \colorbox{red!0}{\strut seal} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut approval} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NO} \colorbox{red!1}{\strut payment} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut collected} \colorbox{red!0}{\strut during} \colorbox{red!1}{\strut online} \colorbox{red!0}{\strut booking} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut For} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut assistance} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!1}{\strut call} \colorbox{red!1}{\strut our} \colorbox{red!3}{\strut reservation} \colorbox{red!0}{\strut specialists} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut 1-888-398-5392} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut use} \colorbox{red!1}{\strut our} \colorbox{red!1}{\strut free} \colorbox{red!0}{\strut call-back} \colorbox{red!0}{\strut button} \colorbox{red!0}{\strut or} \colorbox{red!33}{\strut Orange} \colorbox{red!35}{\strut County} \colorbox{red!37}{\strut Convention} \colorbox{red!38}{\strut Center} \colorbox{red!3}{\strut OCCC} \colorbox{red!0}{\strut From} \colorbox{red!33}{\strut Orange} \colorbox{red!35}{\strut County} \colorbox{red!37}{\strut Convention} \colorbox{red!38}{\strut Center} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Estimated} \colorbox{red!3}{\strut Travel} \colorbox{red!3}{\strut Time} \colorbox{red!2}{\strut Lincoln} \colorbox{red!2}{\strut Town} \colorbox{red!8}{\strut Car} \colorbox{red!3}{\strut Mercedes} \colorbox{red!1}{\strut S550} \colorbox{red!1}{\strut Ford} \colorbox{red!1}{\strut E350} \colorbox{red!3}{\strut Mercedes} \colorbox{red!1}{\strut Luxury} \colorbox{red!4}{\strut Van} \colorbox{red!1}{\strut Cadillac} \colorbox{red!2}{\strut Escalade} \colorbox{red!2}{\strut Lincoln} \colorbox{red!3}{\strut Limo} \colorbox{red!1}{\strut Hummer} \colorbox{red!3}{\strut Limo} \colorbox{red!2}{\strut SUV} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 4} \colorbox{red!5}{\strut Passengers} \colorbox{red!13}{\strut price} \colorbox{red!0}{\strut per} \colorbox{red!5}{\strut vehicle} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 4} \colorbox{red!5}{\strut Passengers} \colorbox{red!13}{\strut price} \colorbox{red!0}{\strut per} \colorbox{red!5}{\strut vehicle} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 9} \colorbox{red!5}{\strut Passengers} \colorbox{red!13}{\strut price} \colorbox{red!0}{\strut per} \colorbox{red!5}{\strut vehicle} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 8} \colorbox{red!5}{\strut Passengers} \colorbox{red!13}{\strut price} \colorbox{red!0}{\strut per} \colorbox{red!5}{\strut vehicle} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 5} \colorbox{red!5}{\strut Passengers} \colorbox{red!13}{\strut price} \colorbox{red!0}{\strut per} \colorbox{red!5}{\strut vehicle} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut to} 
}}}
\end{CJK*}

query: map united states

84:states, 45:map, 34:york, 33:united, 32:city, 31:new, 26:usa, 18:america, 17:populous, 15:road


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut About} \colorbox{red!25}{\strut Road} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!23}{\strut Physical} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!43}{\strut USA} \colorbox{red!100}{\strut States} \colorbox{red!75}{\strut Map} \colorbox{red!0}{\strut Shower} \colorbox{red!75}{\strut Map} \colorbox{red!10}{\strut Home} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut maps} \colorbox{red!5}{\strut than} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!6}{\strut imagine} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut US} \colorbox{red!0}{\strut Maps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut State} \colorbox{red!0}{\strut Maps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Maps} \colorbox{red!6}{\strut of} \colorbox{red!13}{\strut Europe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut more} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Mar} \colorbox{red!0}{\strut 31} \colorbox{red!0}{\strut 2008} \colorbox{red!5}{\strut 0} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!52}{\strut New} \colorbox{red!57}{\strut York} \colorbox{red!53}{\strut City} \colorbox{red!52}{\strut New} \colorbox{red!57}{\strut York} \colorbox{red!53}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut The} \colorbox{red!53}{\strut City} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut Never} \colorbox{red!0}{\strut Sleeps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut most} \colorbox{red!28}{\strut populous} \colorbox{red!53}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!3}{\strut the} \colorbox{red!10}{\strut largest} \colorbox{red!11}{\strut urban} \colorbox{red!6}{\strut areas} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!13}{\strut world} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut most} \colorbox{red!0}{\strut densely} \colorbox{red!0}{\strut populated} \colorbox{red!16}{\strut major} \colorbox{red!53}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 8.2} \colorbox{red!6}{\strut million} \colorbox{red!11}{\strut residents} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!52}{\strut New} \colorbox{red!57}{\strut York} \colorbox{red!53}{\strut City} \colorbox{red!0}{\strut is} \colorbox{red!6}{\strut comprised} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!15}{\strut boroughs} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Bronx} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut Brooklyn} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Manhattan} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Queens} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Staten} \colorbox{red!8}{\strut Island} \colorbox{red!3}{\strut .} \colorbox{red!52}{\strut New} \colorbox{red!57}{\strut York} \colorbox{red!53}{\strut City} \colorbox{red!0}{\strut is} \colorbox{red!15}{\strut visited} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut almost} \colorbox{red!0}{\strut 40} \colorbox{red!6}{\strut million} \colorbox{red!10}{\strut foreign} \colorbox{red!0}{\strut and} \colorbox{red!18}{\strut american} \colorbox{red!5}{\strut tourists} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut Statue} \colorbox{red!6}{\strut of} \colorbox{red!6}{\strut Liberty} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut a} \colorbox{red!16}{\strut major} \colorbox{red!0}{\strut tourist} \colorbox{red!6}{\strut attraction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut one} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!5}{\strut most} \colorbox{red!0}{\strut recognizable} \colorbox{red!0}{\strut icons} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!3}{\strut .} \colorbox{red!10}{\strut Written} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut anniesfamouscookies} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!6}{\strut of} \colorbox{red!30}{\strut America} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Tags} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut animated} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut individual} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut large} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!30}{\strut America} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!52}{\strut New} \colorbox{red!57}{\strut York} \colorbox{red!53}{\strut City} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!100}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!100}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut The} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!15}{\strut us} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!43}{\strut USA} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!15}{\strut us} \colorbox{red!100}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!6}{\strut of} \colorbox{red!43}{\strut usa} \colorbox{red!0}{\strut ,} \colorbox{red!75}{\strut map} \colorbox{red!55}{\strut united} \colorbox{red!100}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mapoftheunitedstates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut maps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut maps} \colorbox{red!15}{\strut us} \colorbox{red!0}{\strut ,} \colorbox{red!52}{\strut New} \colorbox{red!57}{\strut York} \colorbox{red!53}{\strut City} \colorbox{red!75}{\strut Map} \colorbox{red!0}{\strut ,} \colorbox{red!23}{\strut physical} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut political} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut religious} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Religious} \colorbox{red!75}{\strut Map} \colorbox{red!6}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!43}{\strut USA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!25}{\strut road} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut standard} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!55}{\strut united} \colorbox{red!100}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!55}{\strut united} \colorbox{red!100}{\strut states} \colorbox{red!75}{\strut map} \colorbox{red!10}{\strut large} \colorbox{red!0}{\strut ,} \colorbox{red!55}{\strut united} \colorbox{red!100}{\strut states} \colorbox{red!0}{\strut maps} \colorbox{red!0}{\strut ,} \colorbox{red!55}{\strut United} \colorbox{red!100}{\strut States} \colorbox{red!6}{\strut of} \colorbox{red!30}{\strut America} \colorbox{red!0}{\strut ,} \colorbox{red!55}{\strut united} \colorbox{red!100}{\strut states} \colorbox{red!6}{\strut of} \colorbox{red!30}{\strut america} \colorbox{red!0}{\strut maps} \colorbox{red!0}{\strut ,} \colorbox{red!15}{\strut us} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} \colorbox{red!43}{\strut usa} \colorbox{red!75}{\strut map} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

87:states, 82:map, 81:america, 78:united, 60:what, 43:how, 33:geography, 29:which, 20:swim, 20:name


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut TEACHING} \colorbox{red!1}{\strut AND} \colorbox{red!4}{\strut LEARNING} \colorbox{red!2}{\strut BEGINNING} \colorbox{red!28}{\strut MAP} \colorbox{red!4}{\strut READING} \colorbox{red!3}{\strut LESSON} \colorbox{red!2}{\strut PLAN} \colorbox{red!2}{\strut BEGINNING} \colorbox{red!3}{\strut TEACHER} \colorbox{red!28}{\strut MAP} \colorbox{red!2}{\strut SKILL} \colorbox{red!3}{\strut LESSON} \colorbox{red!2}{\strut PLAN} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut TEACH} \colorbox{red!3}{\strut ELEMENTARY} \colorbox{red!0}{\strut FREE} \colorbox{red!3}{\strut LESSON} \colorbox{red!27}{\strut UNITED} \colorbox{red!30}{\strut STATES} \colorbox{red!2}{\strut INTRODUCTION} \colorbox{red!5}{\strut TOPOGRAPHICAL} \colorbox{red!3}{\strut US} \colorbox{red!11}{\strut GEOGRAPHY} \colorbox{red!4}{\strut LEARNING} \colorbox{red!1}{\strut THE} \colorbox{red!27}{\strut UNITED} \colorbox{red!30}{\strut STATES} \colorbox{red!28}{\strut MAP} \colorbox{red!1}{\strut Suggested} \colorbox{red!3}{\strut Grade} \colorbox{red!2}{\strut Levels} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Third} \colorbox{red!3}{\strut Grade} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Fourth} \colorbox{red!3}{\strut Grade} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Fifth} \colorbox{red!3}{\strut Grade} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Good} \colorbox{red!3}{\strut lesson} \colorbox{red!0}{\strut for} \colorbox{red!5}{\strut ESOL} \colorbox{red!2}{\strut students} \colorbox{red!0}{\strut using} \colorbox{red!6}{\strut TPR} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Total} \colorbox{red!4}{\strut Physical} \colorbox{red!3}{\strut Response} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Getting} \colorbox{red!1}{\strut to} \colorbox{red!5}{\strut Know} \colorbox{red!1}{\strut the} \colorbox{red!28}{\strut Map} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!27}{\strut United} \colorbox{red!30}{\strut States} \colorbox{red!0}{\strut of} \colorbox{red!28}{\strut America} \colorbox{red!6}{\strut TPR} \colorbox{red!3}{\strut Commands} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Tap} \colorbox{red!1}{\strut on} \colorbox{red!4}{\strut Florida} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut 2} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Swim} \colorbox{red!1}{\strut directly} \colorbox{red!3}{\strut west} \colorbox{red!1}{\strut across} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut Gulf} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Mexico} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Pretend} \colorbox{red!1}{\strut to} \colorbox{red!6}{\strut swim} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut 3} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Trace} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut circle} \colorbox{red!0}{\strut around} \colorbox{red!1}{\strut the} \colorbox{red!6}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut now} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Trace} \colorbox{red!1}{\strut the} \colorbox{red!6}{\strut name} \colorbox{red!4}{\strut Texas} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 4} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Fly} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut northwest} \colorbox{red!4}{\strut direction} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Pretend} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut fly} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut 5} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Land} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut state} \colorbox{red!1}{\strut ,} \colorbox{red!10}{\strut which} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut capital} \colorbox{red!1}{\strut is} \colorbox{red!2}{\strut Sacramento} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Point} \colorbox{red!1}{\strut to} \colorbox{red!5}{\strut California} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 6} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Walk} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut beach} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!2}{\strut fingers} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut walk} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut shoreline} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 7} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Look} \colorbox{red!2}{\strut into} \colorbox{red!1}{\strut the} \colorbox{red!6}{\strut ocean} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Pretend} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut have} \colorbox{red!1}{\strut glasses} \colorbox{red!1}{\strut on} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut look} \colorbox{red!1}{\strut across} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut room} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 8} \colorbox{red!1}{\strut .} \colorbox{red!20}{\strut What} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut creature} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut see} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Students} \colorbox{red!4}{\strut say} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut creative} \colorbox{red!3}{\strut response} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 9} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Dive} \colorbox{red!2}{\strut into} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut Pacific} \colorbox{red!6}{\strut Ocean} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Pretend} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut dive} \colorbox{red!2}{\strut into} \colorbox{red!5}{\strut water} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut hands} \colorbox{red!1}{\strut overhead} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 10} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Swim} \colorbox{red!2}{\strut north} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Pretend} \colorbox{red!1}{\strut to} \colorbox{red!6}{\strut swim} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 11} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut water} \colorbox{red!1}{\strut in} \colorbox{red!3}{\strut Washington} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!2}{\strut fingers} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut step} \colorbox{red!1}{\strut onto} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut shore} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 12} \colorbox{red!1}{\strut .} \colorbox{red!15}{\strut How} \colorbox{red!1}{\strut do} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut feel} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut that} \colorbox{red!6}{\strut long} \colorbox{red!6}{\strut swim} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Students} \colorbox{red!4}{\strut say} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut creative} \colorbox{red!3}{\strut response} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut 13} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Hike} \colorbox{red!3}{\strut east} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut first} \colorbox{red!4}{\strut capital} \colorbox{red!1}{\strut on} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut Mississippi} \colorbox{red!4}{\strut River} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!2}{\strut fingers} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut walk} \colorbox{red!3}{\strut east} \colorbox{red!1}{\strut across} \colorbox{red!1}{\strut the} \colorbox{red!28}{\strut map} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} 
}}}
\end{CJK*}

query: solar panels

99:panels, 97:solar, 67:what, 42:photovoltaic, 37:installation, 36:energy, 28:how, 27:account, 26:thermal, 23:italian


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut loading} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut italiano} \colorbox{red!2}{\strut english} \colorbox{red!13}{\strut contact} \colorbox{red!2}{\strut video} \colorbox{red!13}{\strut New} \colorbox{red!0}{\strut !} \colorbox{red!60}{\strut What} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!32}{\strut Energy} \colorbox{red!24}{\strut Account} \colorbox{red!3}{\strut ?} \colorbox{red!10}{\strut Earn} \colorbox{red!0}{\strut an} \colorbox{red!7}{\strut income} \colorbox{red!2}{\strut right} \colorbox{red!3}{\strut away} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut the} \colorbox{red!32}{\strut Energy} \colorbox{red!24}{\strut Account} \colorbox{red!0}{\strut From} \colorbox{red!5}{\strut today} \colorbox{red!1}{\strut it} \colorbox{red!1}{\strut is} \colorbox{red!3}{\strut possible} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut earn} \colorbox{red!0}{\strut by} \colorbox{red!6}{\strut producing} \colorbox{red!32}{\strut energy} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut !} \colorbox{red!4}{\strut For} \colorbox{red!3}{\strut twenty} \colorbox{red!4}{\strut years} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut through} \colorbox{red!1}{\strut a} \colorbox{red!7}{\strut state} \colorbox{red!6}{\strut incentive} \colorbox{red!2}{\strut ,} \colorbox{red!4}{\strut every} \colorbox{red!0}{\strut kwh} \colorbox{red!4}{\strut of} \colorbox{red!0}{\strut ...} \colorbox{red!13}{\strut New} \colorbox{red!0}{\strut !} \colorbox{red!60}{\strut What} \colorbox{red!2}{\strut are} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!3}{\strut ?} \colorbox{red!86}{\strut Solar} \colorbox{red!88}{\strut panels} \colorbox{red!2}{\strut are} \colorbox{red!5}{\strut used} \colorbox{red!2}{\strut to} \colorbox{red!14}{\strut transform} \colorbox{red!14}{\strut sunlight} \colorbox{red!4}{\strut into} \colorbox{red!32}{\strut energy} \colorbox{red!5}{\strut and} \colorbox{red!13}{\strut heat} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!2}{\strut are} \colorbox{red!7}{\strut two} \colorbox{red!13}{\strut types} \colorbox{red!2}{\strut .} \colorbox{red!37}{\strut photovoltaic} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!5}{\strut and} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!0}{\strut ...} \colorbox{red!37}{\strut Photovoltaic} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut mentioned} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!37}{\strut photovoltaic} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!14}{\strut transform} \colorbox{red!86}{\strut solar} \colorbox{red!32}{\strut energy} \colorbox{red!4}{\strut into} \colorbox{red!12}{\strut electricity} \colorbox{red!6}{\strut utilized} \colorbox{red!4}{\strut every} \colorbox{red!5}{\strut day} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut ...} \colorbox{red!23}{\strut Thermal} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!23}{\strut Thermal} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!2}{\strut replace} \colorbox{red!0}{\strut traditional} \colorbox{red!6}{\strut gas} \colorbox{red!4}{\strut boilers} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut allowing} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut to} \colorbox{red!13}{\strut heat} \colorbox{red!14}{\strut water} \colorbox{red!5}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!9}{\strut home} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut ...} \colorbox{red!13}{\strut New} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Incentives} \colorbox{red!5}{\strut and} \colorbox{red!2}{\strut concessions} \colorbox{red!2}{\strut Finally} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut after} \colorbox{red!4}{\strut years} \colorbox{red!4}{\strut of} \colorbox{red!5}{\strut waiting} \colorbox{red!2}{\strut ,} \colorbox{red!20}{\strut Italian} \colorbox{red!2}{\strut citizens} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut can} \colorbox{red!8}{\strut take} \colorbox{red!7}{\strut advantage} \colorbox{red!4}{\strut of} \colorbox{red!12}{\strut financing} \colorbox{red!4}{\strut for} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut It} \colorbox{red!1}{\strut is} \colorbox{red!6}{\strut called} \colorbox{red!32}{\strut Energy} \colorbox{red!24}{\strut Account} \colorbox{red!5}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!1}{\strut become} \colorbox{red!6}{\strut effective} \colorbox{red!0}{\strut ...} \colorbox{red!33}{\strut Installation} \colorbox{red!5}{\strut and} \colorbox{red!19}{\strut costs} \colorbox{red!1}{\strut Depending} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut the} \colorbox{red!7}{\strut location} \colorbox{red!4}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!6}{\strut residence} \colorbox{red!0}{\strut in} \colorbox{red!17}{\strut which} \colorbox{red!3}{\strut the} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!0}{\strut must} \colorbox{red!2}{\strut be} \colorbox{red!0}{\strut installed} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut functioning} \colorbox{red!4}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!33}{\strut installation} \colorbox{red!8}{\strut system} \colorbox{red!1}{\strut will} \colorbox{red!2}{\strut be} \colorbox{red!2}{\strut better} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Home} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut .} \colorbox{red!86}{\strut Solar} \colorbox{red!0}{\strut panels-} \colorbox{red!37}{\strut photovoltaic} \colorbox{red!0}{\strut panels-} \colorbox{red!14}{\strut water} \colorbox{red!86}{\strut solar} \colorbox{red!0}{\strut panels-} \colorbox{red!37}{\strut photovoltaic} \colorbox{red!86}{\strut solar} \colorbox{red!0}{\strut panels-} \colorbox{red!23}{\strut thermal} \colorbox{red!86}{\strut solar} \colorbox{red!0}{\strut panels-} \colorbox{red!86}{\strut solar} \colorbox{red!0}{\strut panel} \colorbox{red!0}{\strut production-} \colorbox{red!86}{\strut solar} \colorbox{red!0}{\strut panel} \colorbox{red!7}{\strut sales} \colorbox{red!0}{\strut This} \colorbox{red!4}{\strut portal} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!4}{\strut established} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut fulfil} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut publics} \colorbox{red!0}{\strut need} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut know} \colorbox{red!3}{\strut about} \colorbox{red!37}{\strut photovoltaic} \colorbox{red!88}{\strut panels} \colorbox{red!5}{\strut and} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut to} \colorbox{red!5}{\strut understand} \colorbox{red!25}{\strut how} \colorbox{red!5}{\strut and} \colorbox{red!8}{\strut who} \colorbox{red!2}{\strut to} \colorbox{red!13}{\strut contact} \colorbox{red!4}{\strut for} \colorbox{red!3}{\strut the} \colorbox{red!33}{\strut installation} \colorbox{red!4}{\strut of} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!3}{\strut .} \colorbox{red!86}{\strut solar} \colorbox{red!0}{\strut panel} \colorbox{red!0}{\strut installations} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut find} \colorbox{red!4}{\strut businesses} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut area} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut offering} \colorbox{red!0}{\strut advice} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut planning} \colorbox{red!5}{\strut and} \colorbox{red!12}{\strut assembly} \colorbox{red!4}{\strut of} \colorbox{red!23}{\strut Thermal} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!3}{\strut .} \colorbox{red!86}{\strut solar} \colorbox{red!0}{\strut panel} \colorbox{red!7}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut be} \colorbox{red!1}{\strut able} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut better} \colorbox{red!5}{\strut understand} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut cost} \colorbox{red!4}{\strut of} \colorbox{red!37}{\strut photovoltaic} \colorbox{red!0}{\strut panel} \colorbox{red!5}{\strut and} \colorbox{red!0}{\strut perhaps} \colorbox{red!2}{\strut be} \colorbox{red!1}{\strut able} \colorbox{red!2}{\strut to} \colorbox{red!5}{\strut find} \colorbox{red!0}{\strut incentives} \colorbox{red!4}{\strut for} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!0}{\strut or} \colorbox{red!12}{\strut financing} \colorbox{red!4}{\strut for} \colorbox{red!23}{\strut Thermal} \colorbox{red!86}{\strut solar} \colorbox{red!88}{\strut panels} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut short} 
}}}
\end{CJK*}

99:solar, 98:panels, 29:bp, 21:power, 18:watt, 17:cells, 16:sx320j, 15:number, 14:systems, 14:heaters


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!71}{\strut Solar} \colorbox{red!70}{\strut Panels} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut FAQs} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Site} \colorbox{red!5}{\strut Map} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Product} \colorbox{red!2}{\strut Catalog} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Bookmark} \colorbox{red!2}{\strut this} \colorbox{red!5}{\strut site} \colorbox{red!1}{\strut !} \colorbox{red!6}{\strut Home} \colorbox{red!4}{\strut .} \colorbox{red!71}{\strut Solar} \colorbox{red!15}{\strut Power} \colorbox{red!10}{\strut Systems} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Components} \colorbox{red!4}{\strut .} \colorbox{red!71}{\strut Solar} \colorbox{red!70}{\strut Panels} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut by} \colorbox{red!5}{\strut Brand} \colorbox{red!4}{\strut .} \colorbox{red!20}{\strut Bp} \colorbox{red!71}{\strut Solar} \colorbox{red!4}{\strut .} \colorbox{red!20}{\strut BP} \colorbox{red!11}{\strut SX320J} \colorbox{red!71}{\strut Solar} \colorbox{red!70}{\strut Panels} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut 20} \colorbox{red!12}{\strut Watt} \colorbox{red!2}{\strut .} \colorbox{red!20}{\strut BP} \colorbox{red!11}{\strut SX320J} \colorbox{red!71}{\strut Solar} \colorbox{red!70}{\strut Panels} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut 20} \colorbox{red!12}{\strut Watt} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut View} \colorbox{red!3}{\strut Larger} \colorbox{red!4}{\strut Image} \colorbox{red!5}{\strut MSRP} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 323.95} \colorbox{red!2}{\strut ONLY} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 209.00} \colorbox{red!3}{\strut Item} \colorbox{red!10}{\strut Number} \colorbox{red!3}{\strut .} \colorbox{red!11}{\strut SX320J} \colorbox{red!2}{\strut Quantity} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut Email} \colorbox{red!2}{\strut this} \colorbox{red!1}{\strut page} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut friend} \colorbox{red!20}{\strut BP} \colorbox{red!11}{\strut SX320J} \colorbox{red!71}{\strut Solar} \colorbox{red!70}{\strut Panels} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut 20} \colorbox{red!12}{\strut Watt} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Product} \colorbox{red!5}{\strut Reviews} \colorbox{red!3}{\strut Rate} \colorbox{red!2}{\strut This} \colorbox{red!5}{\strut Product} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut Create} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut Review} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 0} \colorbox{red!0}{\strut Ratings} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut 0} \colorbox{red!5}{\strut Reviews} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Jump} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut most} \colorbox{red!1}{\strut popular} \colorbox{red!2}{\strut search} \colorbox{red!0}{\strut results} \colorbox{red!3}{\strut .} \colorbox{red!71}{\strut Solar} \colorbox{red!70}{\strut Panels} \colorbox{red!2}{\strut .} \colorbox{red!8}{\strut Lighting} \colorbox{red!2}{\strut .} \colorbox{red!12}{\strut Cells} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut Home} \colorbox{red!2}{\strut Kits} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Fountains} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Security} \colorbox{red!2}{\strut Kits} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Outdoor} \colorbox{red!2}{\strut Garden} \colorbox{red!0}{\strut Lights} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Battery} \colorbox{red!7}{\strut Chargers} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Pool} \colorbox{red!2}{\strut Covers} \colorbox{red!2}{\strut .} \colorbox{red!10}{\strut Heaters} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Residential} \colorbox{red!71}{\strut Solar} \colorbox{red!70}{\strut Panels} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut RV} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Pumps} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut Home} \colorbox{red!5}{\strut Security} \colorbox{red!2}{\strut .} \colorbox{red!71}{\strut Solar} \colorbox{red!15}{\strut Power} \colorbox{red!3}{\strut View} \colorbox{red!2}{\strut Catalog} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Security} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Return} \colorbox{red!4}{\strut Policy} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Contact} \colorbox{red!4}{\strut us} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut About} \colorbox{red!4}{\strut us} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Shipping} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Links} \colorbox{red!2}{\strut .} \colorbox{red!71}{\strut Solar} \colorbox{red!9}{\strut Calculator} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut Tax} \colorbox{red!3}{\strut Incentives} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Information} \colorbox{red!2}{\strut Copyright} \colorbox{red!0}{\strut 1998} \colorbox{red!2}{\strut -} \colorbox{red!3}{\strut 2008} 
}}}
\end{CJK*}

query: horse hooves

96:horse, 50:clean, 44:hoof, 35:hooves, 28:good, 27:helps, 27:care, 25:keeping, 21:pick, 19:why


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Home} \colorbox{red!2}{\strut Topics} \colorbox{red!88}{\strut Horse} \colorbox{red!24}{\strut Care} \colorbox{red!40}{\strut Hoof} \colorbox{red!24}{\strut Care} \colorbox{red!88}{\strut Horse} \colorbox{red!40}{\strut Hoof} \colorbox{red!24}{\strut Care} \colorbox{red!7}{\strut Pointers} \colorbox{red!14}{\strut Making} \colorbox{red!10}{\strut sure} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!1}{\strut has} \colorbox{red!46}{\strut clean} \colorbox{red!32}{\strut hooves} \colorbox{red!24}{\strut helps} \colorbox{red!7}{\strut maintain} \colorbox{red!0}{\strut his} \colorbox{red!17}{\strut health} \colorbox{red!1}{\strut and} \colorbox{red!6}{\strut beautiful} \colorbox{red!6}{\strut appearance} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!40}{\strut hoof} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut highly} \colorbox{red!0}{\strut specialized} \colorbox{red!5}{\strut horny} \colorbox{red!1}{\strut shell} \colorbox{red!2}{\strut that} \colorbox{red!4}{\strut covers} \colorbox{red!1}{\strut and} \colorbox{red!8}{\strut protects} \colorbox{red!1}{\strut the} \colorbox{red!6}{\strut sensitive} \colorbox{red!2}{\strut structures} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!88}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!12}{\strut foot} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut may} \colorbox{red!1}{\strut seem} \colorbox{red!4}{\strut indestructible} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!1}{\strut have} \colorbox{red!2}{\strut to} \colorbox{red!5}{\strut be} \colorbox{red!0}{\strut careful} \colorbox{red!12}{\strut when} \colorbox{red!14}{\strut working} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!32}{\strut hooves} \colorbox{red!2}{\strut .} \colorbox{red!40}{\strut Hoof} \colorbox{red!24}{\strut Care} \colorbox{red!24}{\strut Helps} \colorbox{red!1}{\strut and} \colorbox{red!8}{\strut Hindrances} \colorbox{red!0}{\strut You} \colorbox{red!3}{\strut can} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!1}{\strut have} \colorbox{red!5}{\strut strong} \colorbox{red!32}{\strut hooves} \colorbox{red!2}{\strut into} \colorbox{red!0}{\strut his} \colorbox{red!2}{\strut old} \colorbox{red!10}{\strut age} \colorbox{red!1}{\strut by} \colorbox{red!2}{\strut adhering} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut a} \colorbox{red!4}{\strut routine} \colorbox{red!0}{\strut of} \colorbox{red!25}{\strut good} \colorbox{red!10}{\strut trimming} \colorbox{red!1}{\strut and} \colorbox{red!12}{\strut shoeing} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Allow} \colorbox{red!0}{\strut you} \colorbox{red!88}{\strut horse} \colorbox{red!4}{\strut periods} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut being} \colorbox{red!8}{\strut barefoot} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut further} \colorbox{red!3}{\strut promote} \colorbox{red!40}{\strut hoof} \colorbox{red!17}{\strut health} \colorbox{red!2}{\strut .} \colorbox{red!11}{\strut Daily} \colorbox{red!0}{\strut cleanings} \colorbox{red!1}{\strut and} \colorbox{red!40}{\strut hoof} \colorbox{red!13}{\strut dressings} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut help} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut hand} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut improper} \colorbox{red!2}{\strut or} \colorbox{red!2}{\strut careless} \colorbox{red!12}{\strut shoeing} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!10}{\strut sure} \colorbox{red!8}{\strut way} \colorbox{red!2}{\strut to} \colorbox{red!8}{\strut harm} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!32}{\strut hooves} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut In} \colorbox{red!2}{\strut addition} \colorbox{red!2}{\strut ,} \colorbox{red!6}{\strut insufficient} \colorbox{red!12}{\strut exercise} \colorbox{red!2}{\strut ,} \colorbox{red!10}{\strut poor} \colorbox{red!3}{\strut nutrition} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut dryness} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!40}{\strut hoof} \colorbox{red!6}{\strut wall} \colorbox{red!3}{\strut can} \colorbox{red!5}{\strut lead} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut poor} \colorbox{red!40}{\strut hoof} \colorbox{red!17}{\strut health} \colorbox{red!2}{\strut .} \colorbox{red!17}{\strut Why} \colorbox{red!46}{\strut Clean} \colorbox{red!1}{\strut a} \colorbox{red!88}{\strut Horse} \colorbox{red!0}{\strut s} \colorbox{red!32}{\strut Hooves} \colorbox{red!0}{\strut ?} \colorbox{red!23}{\strut Keeping} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!32}{\strut hooves} \colorbox{red!46}{\strut clean} \colorbox{red!0}{\strut keeps} \colorbox{red!0}{\strut them} \colorbox{red!15}{\strut healthy} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Use} \colorbox{red!1}{\strut a} \colorbox{red!40}{\strut hoof} \colorbox{red!19}{\strut pick} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut day} \colorbox{red!2}{\strut to} \colorbox{red!11}{\strut remove} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut buildup} \colorbox{red!0}{\strut of} \colorbox{red!11}{\strut dirt} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut debris} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Long-term} \colorbox{red!3}{\strut exposure} \colorbox{red!2}{\strut to} \colorbox{red!8}{\strut bacteria} \colorbox{red!3}{\strut can} \colorbox{red!0}{\strut eventually} \colorbox{red!5}{\strut lead} \colorbox{red!2}{\strut to} \colorbox{red!8}{\strut infections} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Stones} \colorbox{red!3}{\strut can} \colorbox{red!6}{\strut collect} \colorbox{red!3}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!32}{\strut hooves} \colorbox{red!1}{\strut and} \colorbox{red!15}{\strut cause} \colorbox{red!8}{\strut bruising} \colorbox{red!2}{\strut .} \colorbox{red!40}{\strut Hoof} \colorbox{red!0}{\strut Picking} \colorbox{red!0}{\strut Tips} \colorbox{red!1}{\strut Here} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut basics} \colorbox{red!0}{\strut of} \colorbox{red!88}{\strut horse} \colorbox{red!40}{\strut hoof} \colorbox{red!24}{\strut care} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut cleaning} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Be} \colorbox{red!5}{\strut patient} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut calm} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut gentle} \colorbox{red!1}{\strut if} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut used} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut his} \colorbox{red!32}{\strut hooves} \colorbox{red!0}{\strut cleaned} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Always} \colorbox{red!5}{\strut use} \colorbox{red!1}{\strut the} \colorbox{red!19}{\strut pick} \colorbox{red!0}{\strut towards} \colorbox{red!1}{\strut the} \colorbox{red!9}{\strut toe} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut front} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!40}{\strut hoof} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut Pulling} \colorbox{red!1}{\strut the} \colorbox{red!19}{\strut pick} \colorbox{red!0}{\strut towards} \colorbox{red!1}{\strut the} \colorbox{red!8}{\strut back} \colorbox{red!3}{\strut can} \colorbox{red!4}{\strut allow} \colorbox{red!1}{\strut the} \colorbox{red!19}{\strut pick} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!7}{\strut caught} \colorbox{red!3}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut frog} \colorbox{red!1}{\strut and} \colorbox{red!8}{\strut hurt} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!3}{\strut quick} \colorbox{red!8}{\strut way} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut lose} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut confidence} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut .} \colorbox{red!19}{\strut Pick} \colorbox{red!0}{\strut your} \colorbox{red!88}{\strut horse} \colorbox{red!0}{\strut s} \colorbox{red!32}{\strut hooves} \colorbox{red!0}{\strut before} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut each} \colorbox{red!12}{\strut ride} 
}}}
\end{CJK*}

93:hooves, 91:horse, 91:dancing, 86:stable, 49:owned, 42:jackson, 40:county, 32:brandon, 30:located, 29:mississippi


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!48}{\strut Dancing} \colorbox{red!49}{\strut Hooves} \colorbox{red!45}{\strut Stable} \colorbox{red!0}{\strut .com} \colorbox{red!48}{\strut Horse} \colorbox{red!45}{\strut Stable} \colorbox{red!5}{\strut Accommodations} \colorbox{red!1}{\strut Great} \colorbox{red!5}{\strut Company} \colorbox{red!1}{\strut Photos} \colorbox{red!1}{\strut Photos} \colorbox{red!0}{\strut 2} \colorbox{red!1}{\strut Photos} \colorbox{red!0}{\strut 3} \colorbox{red!1}{\strut Photos} \colorbox{red!0}{\strut 4} \colorbox{red!3}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!2}{\strut Listen} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut great} \colorbox{red!5}{\strut Christian} \colorbox{red!3}{\strut Music} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!17}{\strut Brandon} \colorbox{red!2}{\strut ,} \colorbox{red!15}{\strut Mississippi} \colorbox{red!3}{\strut area} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 100.9} \colorbox{red!1}{\strut or} \colorbox{red!0}{\strut 93.5} \colorbox{red!1}{\strut FM} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut 601} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 940-1818} \colorbox{red!26}{\strut Owned} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Operated} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut Dawn} \colorbox{red!3}{\strut Clarke} \colorbox{red!1}{\strut 1575} \colorbox{red!4}{\strut Carsley} \colorbox{red!5}{\strut Road} \colorbox{red!1}{\strut .} \colorbox{red!22}{\strut Jackson} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut MS} \colorbox{red!1}{\strut 39209} \colorbox{red!48}{\strut Dancing} \colorbox{red!49}{\strut Hooves} \colorbox{red!45}{\strut Stable} \colorbox{red!2}{\strut offers} \colorbox{red!4}{\strut Haven} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Horses} \colorbox{red!8}{\strut Who} \colorbox{red!0}{\strut Are} \colorbox{red!6}{\strut Retired} \colorbox{red!1}{\strut or} \colorbox{red!6}{\strut Recuperating} \colorbox{red!48}{\strut Dancing} \colorbox{red!49}{\strut Hooves} \colorbox{red!45}{\strut Stable} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut paradise} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut green} \colorbox{red!2}{\strut grass} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut large} \colorbox{red!2}{\strut shade} \colorbox{red!2}{\strut trees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut loving} \colorbox{red!5}{\strut care} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!16}{\strut located} \colorbox{red!1}{\strut on} \colorbox{red!0}{\strut 35.5} \colorbox{red!2}{\strut acres} \colorbox{red!1}{\strut in} \colorbox{red!8}{\strut North} \colorbox{red!3}{\strut Hinds} \colorbox{red!21}{\strut County} \colorbox{red!2}{\strut ,} \colorbox{red!22}{\strut Jackson} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut MS} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut horses} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut given} \colorbox{red!5}{\strut care} \colorbox{red!0}{\strut based} \colorbox{red!1}{\strut on} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut individual} \colorbox{red!3}{\strut need} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut unique} \colorbox{red!2}{\strut personality} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Care} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut consistent} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut provided} \colorbox{red!0}{\strut 247} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut 365} \colorbox{red!2}{\strut days} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut year} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut When} \colorbox{red!0}{\strut your} \colorbox{red!48}{\strut horse} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut special} \colorbox{red!1}{\strut attention} \colorbox{red!1}{\strut or} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut regular} \colorbox{red!5}{\strut care} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut always} \colorbox{red!1}{\strut available} \colorbox{red!3}{\strut .} 
}}}
\end{CJK*}

query: ct jobs

88:ct, 66:lyme, 16:job, 14:cities, 11:located, 9:why, 9:sprague, 9:point, 9:griswold, 9:borough


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut help} \colorbox{red!7}{\strut post} \colorbox{red!0}{\strut a} \colorbox{red!24}{\strut job} \colorbox{red!4}{\strut get} \colorbox{red!24}{\strut job} \colorbox{red!9}{\strut alerts} \colorbox{red!6}{\strut search} \colorbox{red!0}{\strut jobs} \colorbox{red!6}{\strut search} \colorbox{red!0}{\strut people} \colorbox{red!6}{\strut Search} \colorbox{red!3}{\strut Create} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut profile} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut get} \colorbox{red!4}{\strut found} \colorbox{red!0}{\strut by} \colorbox{red!12}{\strut employers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut get} \colorbox{red!9}{\strut started} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Already} \colorbox{red!3}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut account} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut sign} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut here} \colorbox{red!6}{\strut .} \colorbox{red!13}{\strut why} \colorbox{red!12}{\strut register} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut get} \colorbox{red!24}{\strut job} \colorbox{red!9}{\strut alerts} \colorbox{red!4}{\strut Refine} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut search} \colorbox{red!0}{\strut Posted} \colorbox{red!4}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut last} \colorbox{red!3}{\strut 1} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 14} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 30} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 90} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!6}{\strut .} \colorbox{red!6}{\strut days} \colorbox{red!16}{\strut Located} \colorbox{red!4}{\strut within} \colorbox{red!4}{\strut 5} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut 10} \colorbox{red!6}{\strut .} \colorbox{red!1}{\strut 15} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 25} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!6}{\strut .} \colorbox{red!6}{\strut miles} \colorbox{red!4}{\strut Sort} \colorbox{red!0}{\strut by} \colorbox{red!6}{\strut Best} \colorbox{red!0}{\strut match} \colorbox{red!4}{\strut Date} \colorbox{red!6}{\strut .} \colorbox{red!10}{\strut Distance} \colorbox{red!21}{\strut Cities} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!10}{\strut Baltic} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!13}{\strut Borough} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Bozrah} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Canterbury} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!10}{\strut Center} \colorbox{red!12}{\strut Groton} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Chesterfield} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Colchester} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut East} \colorbox{red!100}{\strut Lyme} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Exeter} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Fitchville} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Fort} \colorbox{red!7}{\strut Trumbull} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Franklin} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Franklin} \colorbox{red!6}{\strut Hill} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!4}{\strut Gales} \colorbox{red!6}{\strut Ferry} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Gilman} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!13}{\strut Griswold} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!12}{\strut Groton} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!12}{\strut Groton} \colorbox{red!9}{\strut Long} \colorbox{red!13}{\strut Point} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!4}{\strut Hadlyme} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Hamburg} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Hanover} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Hopeville} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Jewett} \colorbox{red!0}{\strut City} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Jordan} \colorbox{red!9}{\strut Village} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Jupiter} \colorbox{red!13}{\strut Point} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Lebanon} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!4}{\strut Ledyard} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Lisbon} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Lords} \colorbox{red!13}{\strut Point} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!100}{\strut Lyme} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Mashantucket} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Masons} \colorbox{red!7}{\strut Island} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Millstone} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Montville} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!9}{\strut Mystic} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Naval} \colorbox{red!6}{\strut Submarine} \colorbox{red!6}{\strut Base} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut New} \colorbox{red!4}{\strut London} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!6}{\strut Niantic} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut Noank} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} \colorbox{red!3}{\strut in} \colorbox{red!7}{\strut North} \colorbox{red!9}{\strut Franklin} \colorbox{red!3}{\strut ,} \colorbox{red!100}{\strut CT} \colorbox{red!0}{\strut Jobs} 
}}}
\end{CJK*}

98:ct, 97:job, 30:hiring, 26:why, 19:career, 16:openings, 15:salary, 15:company, 14:employers, 14:connecticut


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut My} \colorbox{red!5}{\strut Home} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Login} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Help} \colorbox{red!5}{\strut Home} \colorbox{red!46}{\strut CT} \colorbox{red!45}{\strut Job} \colorbox{red!5}{\strut Search} \colorbox{red!45}{\strut Job} \colorbox{red!6}{\strut Seekers} \colorbox{red!8}{\strut Career} \colorbox{red!4}{\strut Central} \colorbox{red!2}{\strut About} \colorbox{red!2}{\strut Us} \colorbox{red!6}{\strut Advertising} \colorbox{red!6}{\strut Employers} \colorbox{red!1}{\strut January} \colorbox{red!0}{\strut 13} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut 2009} \colorbox{red!2}{\strut Regular} \colorbox{red!45}{\strut Job} \colorbox{red!7}{\strut Openings} \colorbox{red!0}{\strut 170} \colorbox{red!5}{\strut Temp} \colorbox{red!45}{\strut Job} \colorbox{red!1}{\strut Openings2} \colorbox{red!0}{\strut Companies659} \colorbox{red!1}{\strut Resumes8906} \colorbox{red!1}{\strut Advanced} \colorbox{red!5}{\strut Search} \colorbox{red!1}{\strut Browse} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut CategoryCity} \colorbox{red!5}{\strut New} \colorbox{red!0}{\strut Jobs} \colorbox{red!5}{\strut New} \colorbox{red!5}{\strut Temp} \colorbox{red!0}{\strut Jobs} \colorbox{red!2}{\strut Seasonal} \colorbox{red!0}{\strut Jobs} \colorbox{red!7}{\strut Company} \colorbox{red!4}{\strut Profiles} \colorbox{red!1}{\strut My} \colorbox{red!5}{\strut Home} \colorbox{red!4}{\strut Register} \colorbox{red!12}{\strut Why} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!1}{\strut ?} \colorbox{red!0}{\strut PostEdit} \colorbox{red!5}{\strut Resume} \colorbox{red!8}{\strut Career} \colorbox{red!3}{\strut Agent} \colorbox{red!8}{\strut Career} \colorbox{red!4}{\strut Central} \colorbox{red!5}{\strut Home} \colorbox{red!8}{\strut Career} \colorbox{red!2}{\strut Advice} \colorbox{red!2}{\strut Articles} \colorbox{red!8}{\strut Career} \colorbox{red!2}{\strut Events} \colorbox{red!7}{\strut Salary} \colorbox{red!1}{\strut Information} \colorbox{red!2}{\strut Education} \colorbox{red!1}{\strut Links} \colorbox{red!8}{\strut Career} \colorbox{red!3}{\strut Connection} \colorbox{red!3}{\strut Newsletter} \colorbox{red!2}{\strut Site} \colorbox{red!3}{\strut Map} \colorbox{red!2}{\strut About} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!3}{\strut Join} \colorbox{red!1}{\strut Our} \colorbox{red!1}{\strut Team} \colorbox{red!4}{\strut Contact} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!3}{\strut Privacy} \colorbox{red!2}{\strut Statement} \colorbox{red!3}{\strut Acceptable} \colorbox{red!1}{\strut Use} \colorbox{red!3}{\strut Policy} \colorbox{red!2}{\strut Banner} \colorbox{red!6}{\strut Advertising} \colorbox{red!3}{\strut Products} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut Services} \colorbox{red!1}{\strut My} \colorbox{red!5}{\strut Home} \colorbox{red!4}{\strut Register} \colorbox{red!12}{\strut Why} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!1}{\strut ?} \colorbox{red!3}{\strut Products} \colorbox{red!5}{\strut Rate} \colorbox{red!2}{\strut Card} \colorbox{red!2}{\strut Competitive} \colorbox{red!7}{\strut Salary} \colorbox{red!1}{\strut Reports} \colorbox{red!1}{\strut Testimonials} \colorbox{red!1}{\strut HR} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut B2B} \colorbox{red!2}{\strut Events} \colorbox{red!0}{\strut JiUS} \colorbox{red!2}{\strut University} \colorbox{red!0}{\strut Username} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Password} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Remember} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut Forgot} \colorbox{red!2}{\strut password} \colorbox{red!1}{\strut ?} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!1}{\strut time} \colorbox{red!1}{\strut user} \colorbox{red!1}{\strut ?} \colorbox{red!45}{\strut Job} \colorbox{red!0}{\strut Seeker} \colorbox{red!1}{\strut Resources} \colorbox{red!1}{\strut Featured} \colorbox{red!2}{\strut Articles} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut December} \colorbox{red!1}{\strut 5} \colorbox{red!0}{\strut Donts} \colorbox{red!1}{\strut For} \colorbox{red!3}{\strut Today} \colorbox{red!0}{\strut s} \colorbox{red!45}{\strut Job} \colorbox{red!0}{\strut Seeker} \colorbox{red!1}{\strut In} \colorbox{red!3}{\strut today} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut tough} \colorbox{red!45}{\strut job} \colorbox{red!2}{\strut market} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut need} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut differentiate} \colorbox{red!0}{\strut yourself} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut competition} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut order} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut plum} \colorbox{red!45}{\strut job} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Bright} \colorbox{red!0}{\strut Spots} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Becoming} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut RN} \colorbox{red!1}{\strut Switching} \colorbox{red!0}{\strut careers} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut registered} \colorbox{red!2}{\strut nurse} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!2}{\strut easy} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut well} \colorbox{red!2}{\strut worth} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut these} \colorbox{red!2}{\strut articles} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!8}{\strut Career} \colorbox{red!3}{\strut Connection} \colorbox{red!3}{\strut Newsletter} \colorbox{red!2}{\strut Now} \colorbox{red!14}{\strut Hiring} \colorbox{red!6}{\strut Advertising} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut mission} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut help} \colorbox{red!45}{\strut job} \colorbox{red!6}{\strut seekers} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut find} \colorbox{red!1}{\strut local} \colorbox{red!6}{\strut Connecticut} \colorbox{red!0}{\strut employment} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut careers} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut the} \colorbox{red!45}{\strut job} \colorbox{red!4}{\strut listings} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut careers} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut employment} \colorbox{red!2}{\strut opportunities} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut conveniently} \colorbox{red!2}{\strut organized} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut facilitate} \colorbox{red!45}{\strut job} \colorbox{red!0}{\strut seeker} \colorbox{red!0}{\strut searches} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut JobsInCT.com} \colorbox{red!3}{\strut offers} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut latest} \colorbox{red!8}{\strut career} \colorbox{red!2}{\strut advice} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut resume} \colorbox{red!0}{\strut posting} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut automated} \colorbox{red!8}{\strut career} \colorbox{red!0}{\strut agents} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut best} \colorbox{red!1}{\strut meet} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Connecticut} \colorbox{red!45}{\strut job} \colorbox{red!6}{\strut seekers} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Home} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut SearchJobs} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut New} \colorbox{red!0}{\strut Jobs} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut CompanyProfiles} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut CareerCentral} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut RegisterLogin} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut SiteMap} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut ContactJobsInCT.com} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Employers} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Testimonials} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Advertise} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Banner} \colorbox{red!6}{\strut Advertising} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Links} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut About} \colorbox{red!2}{\strut Us} \colorbox{red!2}{\strut Copyright} \colorbox{red!0}{\strut 2009JobsInTheUS.com} \colorbox{red!0}{\strut All} \colorbox{red!1}{\strut rights} \colorbox{red!1}{\strut reserved} \colorbox{red!3}{\strut Acceptable} \colorbox{red!1}{\strut Use} \colorbox{red!3}{\strut Policy} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Privacy} \colorbox{red!2}{\strut Statement} \colorbox{red!0}{\strut Other} \colorbox{red!5}{\strut States} \colorbox{red!1}{\strut we} \colorbox{red!2}{\strut serve} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut JobsInAL.com} 
}}}
\end{CJK*}

query: texas border patrol

87:aguilar, 81:border, 77:patrol, 46:chief, 38:david, 30:agent, 19:v, 17:states, 17:ranking, 17:assumed


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!38}{\strut David} \colorbox{red!0}{\strut V.} \colorbox{red!87}{\strut Aguilar} \colorbox{red!1}{\strut From} \colorbox{red!4}{\strut Wikipedia} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!2}{\strut free} \colorbox{red!3}{\strut encyclopedia} \colorbox{red!8}{\strut Jump} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut navigation} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut search} \colorbox{red!2}{\strut This} \colorbox{red!3}{\strut article} \colorbox{red!1}{\strut needs} \colorbox{red!3}{\strut additional} \colorbox{red!4}{\strut citations} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut verification} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut Please} \colorbox{red!3}{\strut help} \colorbox{red!3}{\strut improve} \colorbox{red!2}{\strut this} \colorbox{red!3}{\strut article} \colorbox{red!4}{\strut by} \colorbox{red!2}{\strut adding} \colorbox{red!2}{\strut reliable} \colorbox{red!3}{\strut references} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut Unsourced} \colorbox{red!3}{\strut material} \colorbox{red!1}{\strut may} \colorbox{red!1}{\strut be} \colorbox{red!3}{\strut challenged} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut removed} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut September} \colorbox{red!3}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!38}{\strut David} \colorbox{red!0}{\strut V.} \colorbox{red!87}{\strut Aguilar} \colorbox{red!5}{\strut ,} \colorbox{red!46}{\strut Chief} \colorbox{red!77}{\strut Patrol} \colorbox{red!30}{\strut Agent} \colorbox{red!38}{\strut David} \colorbox{red!0}{\strut V.} \colorbox{red!87}{\strut Aguilar} \colorbox{red!4}{\strut is} \colorbox{red!4}{\strut the} \colorbox{red!46}{\strut Chief} \colorbox{red!2}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!10}{\strut United} \colorbox{red!17}{\strut States} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut 1} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut ,} \colorbox{red!4}{\strut having} \colorbox{red!17}{\strut assumed} \colorbox{red!4}{\strut the} \colorbox{red!11}{\strut position} \colorbox{red!4}{\strut on} \colorbox{red!5}{\strut July} \colorbox{red!4}{\strut 1} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut 2004} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut As} \colorbox{red!4}{\strut the} \colorbox{red!8}{\strut nation} \colorbox{red!0}{\strut s} \colorbox{red!11}{\strut highest} \colorbox{red!17}{\strut ranking} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!30}{\strut agent} \colorbox{red!5}{\strut ,} \colorbox{red!46}{\strut Chief} \colorbox{red!87}{\strut Aguilar} \colorbox{red!9}{\strut directs} \colorbox{red!4}{\strut the} \colorbox{red!9}{\strut enforcement} \colorbox{red!2}{\strut efforts} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut than} \colorbox{red!0}{\strut 18,000} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!0}{\strut Agents} \colorbox{red!3}{\strut nationwide} \colorbox{red!6}{\strut .} \colorbox{red!1}{\strut Contents} \colorbox{red!4}{\strut 1} \colorbox{red!7}{\strut Education} \colorbox{red!0}{\strut 2} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!4}{\strut experience} \colorbox{red!0}{\strut 3} \colorbox{red!4}{\strut Accolades} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Dissatisfaction} \colorbox{red!2}{\strut of} \colorbox{red!5}{\strut Subordinates} \colorbox{red!0}{\strut 5} \colorbox{red!2}{\strut Personal} \colorbox{red!0}{\strut 6} \colorbox{red!3}{\strut References} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut edit} \colorbox{red!3}{\strut .} \colorbox{red!7}{\strut Education} \colorbox{red!87}{\strut Aguilar} \colorbox{red!5}{\strut received} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Associates} \colorbox{red!6}{\strut Degree} \colorbox{red!4}{\strut in} \colorbox{red!2}{\strut Accounting} \colorbox{red!1}{\strut from} \colorbox{red!9}{\strut Laredo} \colorbox{red!2}{\strut Junior} \colorbox{red!4}{\strut College} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut also} \colorbox{red!6}{\strut attended} \colorbox{red!9}{\strut Laredo} \colorbox{red!0}{\strut State} \colorbox{red!4}{\strut University} \colorbox{red!3}{\strut and} \colorbox{red!4}{\strut University} \colorbox{red!2}{\strut of} \colorbox{red!16}{\strut Texas} \colorbox{red!4}{\strut at} \colorbox{red!2}{\strut Arlington} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!4}{\strut is} \colorbox{red!3}{\strut a} \colorbox{red!3}{\strut graduate} \colorbox{red!2}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!5}{\strut John} \colorbox{red!0}{\strut F.} \colorbox{red!5}{\strut Kennedy} \colorbox{red!4}{\strut School} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut Government} \colorbox{red!5}{\strut Harvard} \colorbox{red!4}{\strut Senior} \colorbox{red!5}{\strut Executive} \colorbox{red!0}{\strut Fellows} \colorbox{red!3}{\strut Spring} \colorbox{red!3}{\strut Class} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut 1999} \colorbox{red!6}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut edit} \colorbox{red!3}{\strut .} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!4}{\strut experience} \colorbox{red!87}{\strut Aguilar} \colorbox{red!6}{\strut entered} \colorbox{red!4}{\strut on} \colorbox{red!9}{\strut duty} \colorbox{red!2}{\strut with} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!4}{\strut in} \colorbox{red!3}{\strut June} \colorbox{red!0}{\strut 1978} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut His} \colorbox{red!3}{\strut first} \colorbox{red!15}{\strut station} \colorbox{red!3}{\strut was} \colorbox{red!4}{\strut at} \colorbox{red!9}{\strut Laredo} \colorbox{red!5}{\strut ,} \colorbox{red!16}{\strut Texas} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut At} \colorbox{red!9}{\strut Laredo} \colorbox{red!0}{\strut he} \colorbox{red!6}{\strut served} \colorbox{red!4}{\strut in} \colorbox{red!3}{\strut a} \colorbox{red!0}{\strut variety} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut positions} \colorbox{red!2}{\strut including} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!30}{\strut Agent} \colorbox{red!5}{\strut ,} \colorbox{red!3}{\strut a} \colorbox{red!3}{\strut first} \colorbox{red!6}{\strut line} \colorbox{red!5}{\strut Supervisory} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!30}{\strut Agent} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut Assistant} \colorbox{red!77}{\strut Patrol} \colorbox{red!30}{\strut Agent} \colorbox{red!4}{\strut in} \colorbox{red!10}{\strut Charge} \colorbox{red!6}{\strut .} \colorbox{red!87}{\strut Aguilar} \colorbox{red!6}{\strut served} \colorbox{red!2}{\strut as} \colorbox{red!77}{\strut Patrol} \colorbox{red!30}{\strut Agent} \colorbox{red!4}{\strut in} \colorbox{red!10}{\strut Charge} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut three} \colorbox{red!3}{\strut different} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!0}{\strut Stations} \colorbox{red!4}{\strut in} \colorbox{red!16}{\strut Texas} \colorbox{red!1}{\strut from} \colorbox{red!4}{\strut January} \colorbox{red!2}{\strut 1988} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut August} \colorbox{red!3}{\strut 1996} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!3}{\strut was} \colorbox{red!3}{\strut first} \colorbox{red!3}{\strut promoted} \colorbox{red!2}{\strut to} \colorbox{red!77}{\strut Patrol} \colorbox{red!30}{\strut Agent} \colorbox{red!4}{\strut in} \colorbox{red!10}{\strut Charge} \colorbox{red!2}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!12}{\strut Dallas} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!15}{\strut Station} \colorbox{red!4}{\strut in} \colorbox{red!4}{\strut January} \colorbox{red!2}{\strut 1988} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!3}{\strut was} \colorbox{red!3}{\strut promoted} \colorbox{red!2}{\strut to} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut Rio} \colorbox{red!6}{\strut Grande} \colorbox{red!16}{\strut City} \colorbox{red!81}{\strut Border} \colorbox{red!77}{\strut Patrol} \colorbox{red!15}{\strut Station} \colorbox{red!4}{\strut in} \colorbox{red!0}{\strut 1992} \colorbox{red!6}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!6}{\strut Rio} \colorbox{red!6}{\strut Grande} \colorbox{red!16}{\strut City} \colorbox{red!15}{\strut Station} \colorbox{red!4}{\strut is} \colorbox{red!2}{\strut one} \colorbox{red!2}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!2}{\strut most} \colorbox{red!5}{\strut active} \colorbox{red!0}{\strut stations} \colorbox{red!2}{\strut for} \colorbox{red!7}{\strut narcotics} \colorbox{red!5}{\strut interdiction} \colorbox{red!0}{\strut along} 
}}}
\end{CJK*}

98:border, 97:patrol, 45:mexico, 41:hernandez, 34:who, 34:ezequiel, 30:military, 29:when, 27:shot, 24:texas


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut The} \colorbox{red!11}{\strut Military} \colorbox{red!0}{\strut Should} \colorbox{red!1}{\strut Not} \colorbox{red!0}{\strut Be} \colorbox{red!2}{\strut Used} \colorbox{red!0}{\strut to} \colorbox{red!37}{\strut Patrol} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut U.S.-Mexico} \colorbox{red!37}{\strut Border} \colorbox{red!2}{\strut On} \colorbox{red!1}{\strut May} \colorbox{red!1}{\strut 20} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut 1997} \colorbox{red!2}{\strut ,} \colorbox{red!13}{\strut Ezequiel} \colorbox{red!15}{\strut Hernandez} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut an} \colorbox{red!2}{\strut 18} \colorbox{red!0}{\strut year-old} \colorbox{red!3}{\strut high} \colorbox{red!4}{\strut school} \colorbox{red!3}{\strut student} \colorbox{red!1}{\strut from} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut town} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut Redford} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut West} \colorbox{red!9}{\strut Texas} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut was} \colorbox{red!10}{\strut shot} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut death} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut unit} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut four} \colorbox{red!5}{\strut Marines} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut Esequiel} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut U.S.} \colorbox{red!2}{\strut Citizen} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!6}{\strut soldiers} \colorbox{red!0}{\strut were} \colorbox{red!2}{\strut members} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Joint} \colorbox{red!5}{\strut Task} \colorbox{red!9}{\strut Force} \colorbox{red!1}{\strut 6} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!11}{\strut military} \colorbox{red!9}{\strut force} \colorbox{red!2}{\strut established} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut anti-drug} \colorbox{red!0}{\strut activites} \colorbox{red!1}{\strut along} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut U.S.-Mexico} \colorbox{red!37}{\strut border} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut were} \colorbox{red!3}{\strut operating} \colorbox{red!0}{\strut under} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut authorization} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!37}{\strut Border} \colorbox{red!37}{\strut Patrol} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!9}{\strut Texas} \colorbox{red!3}{\strut Rangers} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut state} \colorbox{red!2}{\strut police} \colorbox{red!9}{\strut force} \colorbox{red!3}{\strut investigating} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut shooting} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut say} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut inconsistencies} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut Marines} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut account} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut incident} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut which} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut present} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut grand} \colorbox{red!0}{\strut jury} \colorbox{red!3}{\strut investigating} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Opposition} \colorbox{red!0}{\strut to} \colorbox{red!11}{\strut Military} \colorbox{red!2}{\strut on} \colorbox{red!37}{\strut Border} \colorbox{red!0}{\strut Grows} \colorbox{red!1}{\strut From} \colorbox{red!1}{\strut presidential} \colorbox{red!0}{\strut advisers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut those} \colorbox{red!1}{\strut living} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut small} \colorbox{red!3}{\strut town} \colorbox{red!9}{\strut Texas} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut sentiments} \colorbox{red!0}{\strut seem} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut swaying} \colorbox{red!0}{\strut against} \colorbox{red!3}{\strut deploying} \colorbox{red!6}{\strut soldiers} \colorbox{red!2}{\strut on} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut soil} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut anti-drug} \colorbox{red!2}{\strut surveillance} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut do} \colorbox{red!1}{\strut not} \colorbox{red!0}{\strut believe} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut militarizing} \colorbox{red!1}{\strut the} \colorbox{red!37}{\strut border} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut Brian} \colorbox{red!1}{\strut Morton} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut spokesman} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut Office} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut National} \colorbox{red!7}{\strut Drug} \colorbox{red!1}{\strut Control} \colorbox{red!1}{\strut Policy} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut which} \colorbox{red!1}{\strut coordinates} \colorbox{red!3}{\strut President} \colorbox{red!1}{\strut Clinton} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut anti-drug} \colorbox{red!0}{\strut efforts} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut believe} \colorbox{red!1}{\strut that} \colorbox{red!37}{\strut Border} \colorbox{red!37}{\strut Patrol} \colorbox{red!3}{\strut agents} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut civilian} \colorbox{red!2}{\strut law} \colorbox{red!2}{\strut enforcement} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut best} \colorbox{red!6}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!37}{\strut patrol} \colorbox{red!1}{\strut that} \colorbox{red!2}{\strut area} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Numerous} \colorbox{red!3}{\strut federal} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut state} \colorbox{red!2}{\strut agencies} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut reviewing} \colorbox{red!1}{\strut the} \colorbox{red!11}{\strut military} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut role} \colorbox{red!2}{\strut on} \colorbox{red!1}{\strut the} \colorbox{red!37}{\strut border} \colorbox{red!0}{\strut since} \colorbox{red!1}{\strut May} \colorbox{red!1}{\strut 20} \colorbox{red!2}{\strut ,} \colorbox{red!11}{\strut when} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Marine} \colorbox{red!2}{\strut assigned} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!11}{\strut military} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut Joint} \colorbox{red!5}{\strut Task} \colorbox{red!9}{\strut Force} \colorbox{red!2}{\strut Six} \colorbox{red!10}{\strut shot} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut killed} \colorbox{red!0}{\strut 18-year-old} \colorbox{red!13}{\strut Ezequiel} \colorbox{red!15}{\strut Hernandez} \colorbox{red!1}{\strut while} \colorbox{red!2}{\strut on} \colorbox{red!37}{\strut patrol} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut Redford} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut Texas} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!37}{\strut Border} \colorbox{red!37}{\strut Patrol} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut El} \colorbox{red!2}{\strut Paso} \colorbox{red!2}{\strut sector} \colorbox{red!0}{\strut announced} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut week} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut had} \colorbox{red!2}{\strut suspended} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut JTF-Six} \colorbox{red!0}{\strut operations} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut West} \colorbox{red!9}{\strut Texas} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut New} \colorbox{red!17}{\strut Mexico} \colorbox{red!0}{\strut until} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut shooting} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut investigated} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut El} \colorbox{red!2}{\strut Paso} \colorbox{red!0}{\strut Times} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Laura} \colorbox{red!0}{\strut Smitherman} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut July} \colorbox{red!0}{\strut 13} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut 1997} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Military} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut Role} 
}}}
\end{CJK*}

query: pvc

92:pipe, 85:pvc, 40:sewer, 34:water, 21:installation, 20:requirements, 19:temperature, 19:dwv, 17:burial, 16:pw


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!16}{\strut PW} \colorbox{red!9}{\strut Eagle} \colorbox{red!8}{\strut Home} \colorbox{red!11}{\strut Support} \colorbox{red!8}{\strut Home} \colorbox{red!6}{\strut FAQ} \colorbox{red!0}{\strut s} \colorbox{red!7}{\strut Contact} \colorbox{red!6}{\strut Tech} \colorbox{red!11}{\strut Support} \colorbox{red!9}{\strut Back} \colorbox{red!6}{\strut Technical} \colorbox{red!6}{\strut Bulletins} \colorbox{red!87}{\strut PVC} \colorbox{red!14}{\strut Depth} \colorbox{red!6}{\strut of} \colorbox{red!17}{\strut Burial} \colorbox{red!87}{\strut PVC} \colorbox{red!9}{\strut Print} \colorbox{red!12}{\strut Line} \colorbox{red!20}{\strut Requirements} \colorbox{red!87}{\strut PVC} \colorbox{red!15}{\strut Nonmetallic} \colorbox{red!16}{\strut Conduit} \colorbox{red!7}{\strut and} \colorbox{red!12}{\strut Utility} \colorbox{red!12}{\strut Duct} \colorbox{red!87}{\strut PVC} \colorbox{red!8}{\strut Max} \colorbox{red!6}{\strut .} \colorbox{red!9}{\strut Bell} \colorbox{red!0}{\strut OS} \colorbox{red!7}{\strut Diameter} \colorbox{red!87}{\strut PVC} \colorbox{red!14}{\strut Effects} \colorbox{red!6}{\strut of} \colorbox{red!19}{\strut Temperature} \colorbox{red!87}{\strut PVC} \colorbox{red!0}{\strut VacuumExternal} \colorbox{red!10}{\strut Pressure} \colorbox{red!87}{\strut PVC} \colorbox{red!11}{\strut Support} \colorbox{red!15}{\strut Spacing} \colorbox{red!87}{\strut PVC} \colorbox{red!8}{\strut Longitudinal} \colorbox{red!10}{\strut Bending} \colorbox{red!87}{\strut PVC} \colorbox{red!41}{\strut Sewer} \colorbox{red!95}{\strut Pipe} \colorbox{red!17}{\strut Burial} \colorbox{red!0}{\strut Depths} \colorbox{red!87}{\strut PVC} \colorbox{red!0}{\strut 1428} \colorbox{red!9}{\strut Storm} \colorbox{red!14}{\strut Drain} \colorbox{red!17}{\strut Burial} \colorbox{red!87}{\strut PVC} \colorbox{red!8}{\strut AWWA} \colorbox{red!7}{\strut C900} \colorbox{red!7}{\strut and} \colorbox{red!7}{\strut C905} \colorbox{red!17}{\strut Burial} \colorbox{red!87}{\strut PVC} \colorbox{red!14}{\strut Effects} \colorbox{red!6}{\strut of} \colorbox{red!11}{\strut Sunlight} \colorbox{red!87}{\strut PVC} \colorbox{red!95}{\strut Pipe} \colorbox{red!12}{\strut Trench} \colorbox{red!14}{\strut Construction} \colorbox{red!87}{\strut PVC} \colorbox{red!10}{\strut Air} \colorbox{red!9}{\strut testing} \colorbox{red!6}{\strut of} \colorbox{red!19}{\strut DWV} \colorbox{red!95}{\strut Pipe} \colorbox{red!87}{\strut PVC} \colorbox{red!16}{\strut Gasketed} \colorbox{red!95}{\strut Pipe} \colorbox{red!12}{\strut Assembly} \colorbox{red!87}{\strut PVC} \colorbox{red!9}{\strut Print} \colorbox{red!12}{\strut Line} \colorbox{red!20}{\strut Requirements} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut WaterSewer} \colorbox{red!87}{\strut PVC} \colorbox{red!95}{\strut Pipe} \colorbox{red!15}{\strut Compound} \colorbox{red!87}{\strut PVC} \colorbox{red!12}{\strut Fire} \colorbox{red!9}{\strut Protection} \colorbox{red!7}{\strut and} \colorbox{red!10}{\strut Firestop} \colorbox{red!87}{\strut PVC} \colorbox{red!7}{\strut Material} \colorbox{red!7}{\strut Safety} \colorbox{red!5}{\strut Information} \colorbox{red!4}{\strut Sheet} \colorbox{red!9}{\strut back} \colorbox{red!6}{\strut to} \colorbox{red!8}{\strut top} \colorbox{red!21}{\strut Installation} \colorbox{red!5}{\strut Guides} \colorbox{red!21}{\strut Installation} \colorbox{red!0}{\strut Guide} \colorbox{red!6}{\strut for} \colorbox{red!87}{\strut PVC} \colorbox{red!41}{\strut Sewer} \colorbox{red!95}{\strut Pipe} \colorbox{red!21}{\strut Installation} \colorbox{red!0}{\strut Guide} \colorbox{red!6}{\strut for} \colorbox{red!87}{\strut PVC} \colorbox{red!35}{\strut Water} \colorbox{red!95}{\strut Pipe} \colorbox{red!9}{\strut back} \colorbox{red!6}{\strut to} \colorbox{red!8}{\strut top} \colorbox{red!9}{\strut Misc} \colorbox{red!6}{\strut Limited} \colorbox{red!8}{\strut Warranty} \colorbox{red!6}{\strut Metric} \colorbox{red!6}{\strut Sizes} \colorbox{red!9}{\strut back} \colorbox{red!6}{\strut to} \colorbox{red!8}{\strut top} \colorbox{red!8}{\strut Home} \colorbox{red!5}{\strut Products} \colorbox{red!6}{\strut Search} \colorbox{red!11}{\strut Support} \colorbox{red!5}{\strut 2004} \colorbox{red!16}{\strut PW} \colorbox{red!9}{\strut Eagle} \colorbox{red!6}{\strut Inc} \colorbox{red!6}{\strut .} 
}}}
\end{CJK*}

99:pvc, 44:pipes, 28:why, 23:pvc4pipes, 23:founded, 15:association, 13:work, 12:brussels, 11:systems, 11:new


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!11}{\strut New} \colorbox{red!6}{\strut Website} \colorbox{red!5}{\strut for} \colorbox{red!24}{\strut PVC4Pipes} \colorbox{red!3}{\strut !} \colorbox{red!5}{\strut Welcome} \colorbox{red!4}{\strut on} \colorbox{red!0}{\strut our} \colorbox{red!11}{\strut new} \colorbox{red!6}{\strut website} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut NEW} \colorbox{red!0}{\strut Posters} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut presentations} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut the} \colorbox{red!11}{\strut Documents} \colorbox{red!1}{\strut Sections} \colorbox{red!2}{\strut Visit} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut document} \colorbox{red!0}{\strut section} \colorbox{red!5}{\strut for} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut interesting} \colorbox{red!0}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!11}{\strut documents} \colorbox{red!4}{\strut on} \colorbox{red!100}{\strut PVC} \colorbox{red!47}{\strut Pipes} \colorbox{red!5}{\strut Home} \colorbox{red!5}{\strut Contact} \colorbox{red!2}{\strut Sitemap} \colorbox{red!8}{\strut Disclaimer} \colorbox{red!2}{\strut WHYISPVCUSEDINPIPES} \colorbox{red!4}{\strut ?} \colorbox{red!3}{\strut ABOUTUS} \colorbox{red!7}{\strut PVCPIPESANDSUSTAINABILITY} \colorbox{red!11}{\strut DOCUMENTS} \colorbox{red!1}{\strut NEWS} \colorbox{red!4}{\strut LINKS} \colorbox{red!4}{\strut FAQ} \colorbox{red!0}{\strut .} \colorbox{red!24}{\strut PVC4Pipes} \colorbox{red!5}{\strut is} \colorbox{red!5}{\strut the} \colorbox{red!16}{\strut association} \colorbox{red!24}{\strut founded} \colorbox{red!3}{\strut in} \colorbox{red!12}{\strut Brussels} \colorbox{red!3}{\strut in} \colorbox{red!3}{\strut 2003} \colorbox{red!4}{\strut with} \colorbox{red!5}{\strut the} \colorbox{red!6}{\strut mission} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut developing} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut promoting} \colorbox{red!7}{\strut sustainable} \colorbox{red!100}{\strut PVC} \colorbox{red!0}{\strut piping} \colorbox{red!11}{\strut systems} \colorbox{red!3}{\strut in} \colorbox{red!5}{\strut the} \colorbox{red!5}{\strut global} \colorbox{red!6}{\strut market} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!6}{\strut will} \colorbox{red!0}{\strut also} \colorbox{red!13}{\strut work} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut complement} \colorbox{red!5}{\strut the} \colorbox{red!4}{\strut existing} \colorbox{red!0}{\strut associations} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut industry} \colorbox{red!6}{\strut bodies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!3}{\strut us} \colorbox{red!1}{\strut .} \colorbox{red!29}{\strut Why} \colorbox{red!5}{\strut is} \colorbox{red!100}{\strut PVC} \colorbox{red!8}{\strut used} \colorbox{red!3}{\strut in} \colorbox{red!47}{\strut pipes} \colorbox{red!4}{\strut ?} \colorbox{red!1}{\strut .} \colorbox{red!100}{\strut PVC} \colorbox{red!47}{\strut pipes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sustainability} \colorbox{red!1}{\strut .} \colorbox{red!11}{\strut Documents} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Links} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Contact} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut FAQ} \colorbox{red!6}{\strut Copyright} \colorbox{red!0}{\strut 2004} \colorbox{red!24}{\strut PVC4Pipes} \colorbox{red!0}{\strut all} \colorbox{red!5}{\strut rights} \colorbox{red!0}{\strut reserved} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Disclaimer} 
}}}
\end{CJK*}

query: voyager

100:voyager, 56:star, 35:trek, 26:lg, 23:verizon, 21:phone, 16:space, 14:language, 12:spelled, 12:seas


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!10}{\strut Dictionary} \colorbox{red!0}{\strut Thesaurus} \colorbox{red!3}{\strut Reference} \colorbox{red!7}{\strut Translate} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Register} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Login} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Suggestions} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Searches} \colorbox{red!2}{\strut on} \colorbox{red!0}{\strut Ask.com} \colorbox{red!100}{\strut voyager} \colorbox{red!6}{\strut 1} \colorbox{red!70}{\strut star} \colorbox{red!43}{\strut trek} \colorbox{red!100}{\strut voyager} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut spacecraf} \colorbox{red!0}{\strut ...} \colorbox{red!100}{\strut voyager} \colorbox{red!20}{\strut space} \colorbox{red!3}{\strut mis} \colorbox{red!0}{\strut ...} \colorbox{red!100}{\strut voyager} \colorbox{red!20}{\strut space} \colorbox{red!6}{\strut pro} \colorbox{red!0}{\strut ...} \colorbox{red!28}{\strut verizon} \colorbox{red!100}{\strut voyager} \colorbox{red!32}{\strut lg} \colorbox{red!100}{\strut voyager} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!8}{\strut se} \colorbox{red!0}{\strut ...} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!8}{\strut se} \colorbox{red!0}{\strut ...} \colorbox{red!70}{\strut star} \colorbox{red!43}{\strut trek} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut ...} \colorbox{red!100}{\strut voyager} \colorbox{red!11}{\strut missions} \colorbox{red!100}{\strut voyager} \colorbox{red!26}{\strut phone} \colorbox{red!100}{\strut voyager} \colorbox{red!11}{\strut trike} \colorbox{red!7}{\strut kit} \colorbox{red!100}{\strut voyager} \colorbox{red!7}{\strut mobile} \colorbox{red!26}{\strut phone} \colorbox{red!5}{\strut chrysler} \colorbox{red!100}{\strut voyager} \colorbox{red!100}{\strut voyager} \colorbox{red!7}{\strut reading} \colorbox{red!15}{\strut program} \colorbox{red!100}{\strut voyager} \colorbox{red!6}{\strut 1} \colorbox{red!7}{\strut facts} \colorbox{red!100}{\strut voyager} \colorbox{red!11}{\strut episode} \colorbox{red!3}{\strut guide} \colorbox{red!3}{\strut kawasaki} \colorbox{red!100}{\strut voyager} \colorbox{red!5}{\strut royal} \colorbox{red!3}{\strut caribbean} \colorbox{red!1}{\strut download} \colorbox{red!70}{\strut star} \colorbox{red!43}{\strut trek} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut episodes} \colorbox{red!2}{\strut plymouth} \colorbox{red!100}{\strut voyager} \colorbox{red!100}{\strut voyager} \colorbox{red!3}{\strut airplane} \colorbox{red!100}{\strut voyager} \colorbox{red!6}{\strut pontoon} \colorbox{red!7}{\strut boats} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!15}{\strut seas} \colorbox{red!3}{\strut reviews} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!15}{\strut seas} \colorbox{red!6}{\strut design} \colorbox{red!100}{\strut voyager} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!15}{\strut seas} \colorbox{red!0}{\strut webcam} \colorbox{red!32}{\strut lg} \colorbox{red!100}{\strut voyager} \colorbox{red!2}{\strut accessories} \colorbox{red!5}{\strut saa} \colorbox{red!100}{\strut voyager} \colorbox{red!100}{\strut voyager} \colorbox{red!6}{\strut passport} \colorbox{red!7}{\strut reading} \colorbox{red!15}{\strut program} \colorbox{red!100}{\strut voyager} \colorbox{red!7}{\strut books} \colorbox{red!100}{\strut voyager} \colorbox{red!7}{\strut publishing} \colorbox{red!100}{\strut voyager} \colorbox{red!12}{\strut fleet} \colorbox{red!5}{\strut card} \colorbox{red!100}{\strut voyager} \colorbox{red!3}{\strut ii} \colorbox{red!100}{\strut voyager} \colorbox{red!5}{\strut aircraft} \colorbox{red!1}{\strut Nearby} \colorbox{red!2}{\strut Entries} \colorbox{red!3}{\strut vowing} \colorbox{red!2}{\strut vowless} \colorbox{red!6}{\strut Vox} \colorbox{red!6}{\strut Vox} \colorbox{red!2}{\strut angelica} \colorbox{red!6}{\strut vox} \colorbox{red!0}{\strut barbara} \colorbox{red!6}{\strut vox} \colorbox{red!0}{\strut et} \colorbox{red!3}{\strut praeterea} \colorbox{red!0}{\strut ...} \colorbox{red!6}{\strut vox} \colorbox{red!6}{\strut humana} \colorbox{red!6}{\strut vox} \colorbox{red!2}{\strut pop} \colorbox{red!6}{\strut vox} \colorbox{red!2}{\strut pop} \colorbox{red!6}{\strut .} \colorbox{red!6}{\strut vox} \colorbox{red!3}{\strut populi} \colorbox{red!6}{\strut vox} \colorbox{red!3}{\strut populi} \colorbox{red!1}{\strut ,} \colorbox{red!6}{\strut vox} \colorbox{red!1}{\strut d} \colorbox{red!0}{\strut ...} \colorbox{red!2}{\strut voxel} \colorbox{red!0}{\strut Voyage} \colorbox{red!0}{\strut voyage} \colorbox{red!5}{\strut policy} \colorbox{red!0}{\strut Voyageable} \colorbox{red!0}{\strut voyaged} \colorbox{red!100}{\strut Voyager} \colorbox{red!6}{\strut Voyageur} \colorbox{red!0}{\strut voyageurs} \colorbox{red!3}{\strut nationa} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut voyaging} \colorbox{red!8}{\strut voyeur} \colorbox{red!0}{\strut voyeurism} \colorbox{red!7}{\strut voyeuristic} \colorbox{red!0}{\strut voyeuristical} \colorbox{red!0}{\strut voyeuristically} \colorbox{red!6}{\strut voyeuse} \colorbox{red!3}{\strut Voyol} \colorbox{red!5}{\strut Voysey} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Charles} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut ...} \colorbox{red!3}{\strut voznesenski} \colorbox{red!3}{\strut Voznesenski} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Andr} \colorbox{red!0}{\strut ...} \colorbox{red!3}{\strut voznesenski} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut andr} \colorbox{red!0}{\strut ...} \colorbox{red!3}{\strut voznesenski} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut andr} \colorbox{red!0}{\strut ...} \colorbox{red!3}{\strut VP} \colorbox{red!100}{\strut Voyager} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut 5} \colorbox{red!10}{\strut dictionary} \colorbox{red!0}{\strut results} \colorbox{red!3}{\strut Sponsored} \colorbox{red!3}{\strut Links} \colorbox{red!32}{\strut LG} \colorbox{red!100}{\strut Voyager} \colorbox{red!2}{\strut Get} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Great} \colorbox{red!3}{\strut Deal} \colorbox{red!2}{\strut On} \colorbox{red!0}{\strut A} \colorbox{red!13}{\strut New} \colorbox{red!32}{\strut LG} \colorbox{red!100}{\strut Voyager} \colorbox{red!1}{\strut With} \colorbox{red!28}{\strut Verizon} \colorbox{red!10}{\strut Plan} \colorbox{red!0}{\strut Wirefly.comLGVoyager} \colorbox{red!100}{\strut Voyager} \colorbox{red!2}{\strut Get} \colorbox{red!5}{\strut the} \colorbox{red!13}{\strut new} \colorbox{red!100}{\strut Voyager} \colorbox{red!26}{\strut Phone} \colorbox{red!2}{\strut by} \colorbox{red!32}{\strut LG} \colorbox{red!2}{\strut at} \colorbox{red!0}{\strut VzW} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut Free} \colorbox{red!3}{\strut Activation} \colorbox{red!0}{\strut Fri-Mon} \colorbox{red!2}{\strut !} \colorbox{red!0}{\strut VerizonWireless.VzW.com} \colorbox{red!70}{\strut Star} \colorbox{red!43}{\strut Trek} \colorbox{red!100}{\strut Voyager} \colorbox{red!6}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Complete} \colorbox{red!13}{\strut Seasons} \colorbox{red!6}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 7} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut Brand} \colorbox{red!13}{\strut New} \colorbox{red!6}{\strut .} \colorbox{red!0}{\strut 47} \colorbox{red!0}{\strut DVDs} \colorbox{red!6}{\strut .} \colorbox{red!2}{\strut Only} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 129.90} \colorbox{red!0}{\strut Free} \colorbox{red!7}{\strut shipping} \colorbox{red!0}{\strut www.dealsworld.net} \colorbox{red!100}{\strut Voyager} \colorbox{red!0}{\strut vTj} \colorbox{red!0}{\strut Y} \colorbox{red!0}{\strut dYr} \colorbox{red!12}{\strut Show} \colorbox{red!15}{\strut Spelled} \colorbox{red!8}{\strut Pronunciation} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut voi-uh-jer} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Show} \colorbox{red!2}{\strut IPA} \colorbox{red!8}{\strut Pronunciation} \colorbox{red!5}{\strut noun} \colorbox{red!3}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut U.S.} \colorbox{red!20}{\strut space} \colorbox{red!5}{\strut probes} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut obtained} \colorbox{red!3}{\strut scientific} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut while} \colorbox{red!7}{\strut flying} \colorbox{red!2}{\strut by} \colorbox{red!5}{\strut the} \colorbox{red!7}{\strut planets} \colorbox{red!5}{\strut Jupiter} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Saturn} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut Uranus} \colorbox{red!6}{\strut .} \colorbox{red!17}{\strut Language} \colorbox{red!0}{\strut Translation} \colorbox{red!0}{\strut for} \colorbox{red!3}{\strut .} \colorbox{red!100}{\strut Voyager} \colorbox{red!8}{\strut Spanish} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut viajero} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut German} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut der} 
}}}
\end{CJK*}

98:voyager, 20:oceanography, 20:home, 19:scripps, 17:pier, 16:q, 15:kids, 15:ages, 14:archives, 11:topics


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!3}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut SEARCH} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Home} \colorbox{red!8}{\strut Features} \colorbox{red!9}{\strut Research} \colorbox{red!0}{\strut Highlights} \colorbox{red!0}{\strut Around} \colorbox{red!3}{\strut the} \colorbox{red!17}{\strut Pier} \colorbox{red!98}{\strut Voyager} \colorbox{red!5}{\strut for} \colorbox{red!15}{\strut Kids} \colorbox{red!6}{\strut Multimedia} \colorbox{red!9}{\strut explorations} \colorbox{red!5}{\strut .} \colorbox{red!19}{\strut scripps} \colorbox{red!20}{\strut Home} \colorbox{red!98}{\strut Voyager} \colorbox{red!98}{\strut Voyager} \colorbox{red!5}{\strut for} \colorbox{red!15}{\strut Kids} \colorbox{red!8}{\strut Web} \colorbox{red!8}{\strut Features} \colorbox{red!7}{\strut Activities} \colorbox{red!14}{\strut Archives} \colorbox{red!98}{\strut Voyager} \colorbox{red!16}{\strut Q} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut A} \colorbox{red!98}{\strut Voyager} \colorbox{red!8}{\strut features} \colorbox{red!10}{\strut stories} \colorbox{red!0}{\strut about} \colorbox{red!5}{\strut a} \colorbox{red!3}{\strut wide} \colorbox{red!5}{\strut range} \colorbox{red!6}{\strut of} \colorbox{red!20}{\strut oceanography} \colorbox{red!11}{\strut topics} \colorbox{red!5}{\strut for} \colorbox{red!10}{\strut children} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!15}{\strut ages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!4}{\strut addition} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!6}{\strut section} \colorbox{red!2}{\strut includes} \colorbox{red!11}{\strut science} \colorbox{red!7}{\strut experiments} \colorbox{red!15}{\strut kids} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut try} \colorbox{red!4}{\strut at} \colorbox{red!20}{\strut home} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut answers} \colorbox{red!3}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut researchers} \colorbox{red!6}{\strut submitted} \colorbox{red!4}{\strut by} \colorbox{red!7}{\strut students} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Selected} \colorbox{red!10}{\strut stories} \colorbox{red!3}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!14}{\strut archives} \colorbox{red!3}{\strut and} \colorbox{red!6}{\strut answers} \colorbox{red!3}{\strut from} \colorbox{red!3}{\strut the} \colorbox{red!98}{\strut Voyager} \colorbox{red!16}{\strut Q} \colorbox{red!3}{\strut and} \colorbox{red!5}{\strut A} \colorbox{red!7}{\strut library} \colorbox{red!0}{\strut are} \colorbox{red!6}{\strut available} \colorbox{red!5}{\strut as} \colorbox{red!0}{\strut print-friendly} \colorbox{red!6}{\strut PDF} \colorbox{red!9}{\strut files} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2009} \colorbox{red!19}{\strut Scripps} \colorbox{red!9}{\strut Institution} \colorbox{red!6}{\strut of} \colorbox{red!20}{\strut Oceanography} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut University} \colorbox{red!6}{\strut of} \colorbox{red!5}{\strut California} \colorbox{red!3}{\strut ,} \colorbox{red!5}{\strut San} \colorbox{red!4}{\strut Diego} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut Rights} \colorbox{red!0}{\strut Reserved} 
}}}
\end{CJK*}

query: bart sf

101:bart, 80:stations, 29:sf, 27:oakland, 27:berkeley, 25:city, 20:tv, 19:san, 19:bay, 16:mission


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Enter} \colorbox{red!1}{\strut Query} \colorbox{red!2}{\strut Search} \colorbox{red!3}{\strut Skip} \colorbox{red!2}{\strut to} \colorbox{red!6}{\strut Main} \colorbox{red!2}{\strut Content} \colorbox{red!8}{\strut Contact} \colorbox{red!4}{\strut Us} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut View} \colorbox{red!97}{\strut BART} \colorbox{red!10}{\strut Map} \colorbox{red!7}{\strut Home} \colorbox{red!76}{\strut Stations} \colorbox{red!0}{\strut Station} \colorbox{red!10}{\strut List} \colorbox{red!8}{\strut Find} \colorbox{red!4}{\strut Closest} \colorbox{red!0}{\strut Station} \colorbox{red!6}{\strut Schedules} \colorbox{red!4}{\strut Overview} \colorbox{red!2}{\strut Real} \colorbox{red!7}{\strut Time} \colorbox{red!5}{\strut Arrivals} \colorbox{red!9}{\strut Service} \colorbox{red!1}{\strut Advisories} \colorbox{red!4}{\strut Mobile} \colorbox{red!2}{\strut Options} \colorbox{red!1}{\strut Developer} \colorbox{red!2}{\strut Resources} \colorbox{red!5}{\strut Tickets} \colorbox{red!4}{\strut Overview} \colorbox{red!0}{\strut Ticket} \colorbox{red!1}{\strut Sales} \colorbox{red!4}{\strut Fare} \colorbox{red!4}{\strut Calculator} \colorbox{red!6}{\strut Rider} \colorbox{red!2}{\strut Guide} \colorbox{red!4}{\strut Overview} \colorbox{red!5}{\strut Parking} \colorbox{red!12}{\strut Airport} \colorbox{red!2}{\strut Connections} \colorbox{red!5}{\strut Transit} \colorbox{red!2}{\strut Connections} \colorbox{red!4}{\strut Bikes} \colorbox{red!2}{\strut on} \colorbox{red!97}{\strut BART} \colorbox{red!2}{\strut Accessible} \colorbox{red!0}{\strut Services} \colorbox{red!4}{\strut Destinations} \colorbox{red!5}{\strut Lost} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Found} \colorbox{red!2}{\strut Safety} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Security} \colorbox{red!4}{\strut News} \colorbox{red!4}{\strut News} \colorbox{red!3}{\strut Articles} \colorbox{red!97}{\strut BART} \colorbox{red!19}{\strut TV} \colorbox{red!97}{\strut BART} \colorbox{red!0}{\strut Times} \colorbox{red!8}{\strut Email} \colorbox{red!3}{\strut Alerts} \colorbox{red!4}{\strut RSS} \colorbox{red!1}{\strut Feeds} \colorbox{red!0}{\strut myBART} \colorbox{red!4}{\strut News} \colorbox{red!6}{\strut Widget} \colorbox{red!3}{\strut About} \colorbox{red!97}{\strut BART} \colorbox{red!4}{\strut Overview} \colorbox{red!3}{\strut Board} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Directors} \colorbox{red!4}{\strut Financials} \colorbox{red!3}{\strut Projects} \colorbox{red!4}{\strut Planning} \colorbox{red!2}{\strut Doing} \colorbox{red!2}{\strut Business} \colorbox{red!2}{\strut Jobs} \colorbox{red!3}{\strut Reports} \colorbox{red!4}{\strut History} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut Facts} \colorbox{red!97}{\strut BART} \colorbox{red!3}{\strut Police} \colorbox{red!7}{\strut Home} \colorbox{red!2}{\strut .} \colorbox{red!76}{\strut Stations} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Station} \colorbox{red!10}{\strut List} \colorbox{red!0}{\strut Station} \colorbox{red!10}{\strut List} \colorbox{red!0}{\strut Station} \colorbox{red!10}{\strut List} \colorbox{red!8}{\strut Find} \colorbox{red!4}{\strut Closest} \colorbox{red!0}{\strut Station} \colorbox{red!8}{\strut Email} \colorbox{red!1}{\strut this} \colorbox{red!3}{\strut page} \colorbox{red!3}{\strut Print} \colorbox{red!1}{\strut this} \colorbox{red!3}{\strut page} \colorbox{red!4}{\strut 12th} \colorbox{red!0}{\strut St.} \colorbox{red!25}{\strut Oakland} \colorbox{red!24}{\strut City} \colorbox{red!8}{\strut Center} \colorbox{red!6}{\strut 16th} \colorbox{red!0}{\strut St.} \colorbox{red!15}{\strut Mission} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut 19th} \colorbox{red!0}{\strut St.} \colorbox{red!25}{\strut Oakland} \colorbox{red!7}{\strut 24th} \colorbox{red!0}{\strut St.} \colorbox{red!15}{\strut Mission} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Ashby} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Berkeley} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Balboa} \colorbox{red!0}{\strut Park} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!18}{\strut Bay} \colorbox{red!4}{\strut Fair} \colorbox{red!0}{\strut .} \colorbox{red!18}{\strut San} \colorbox{red!3}{\strut Leandro} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Castro} \colorbox{red!2}{\strut Valley} \colorbox{red!5}{\strut Civic} \colorbox{red!8}{\strut Center} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut ColiseumOakland} \colorbox{red!12}{\strut Airport} \colorbox{red!3}{\strut Colma} \colorbox{red!9}{\strut Concord} \colorbox{red!6}{\strut Daly} \colorbox{red!24}{\strut City} \colorbox{red!7}{\strut Downtown} \colorbox{red!25}{\strut Berkeley} \colorbox{red!0}{\strut DublinPleasanton} \colorbox{red!4}{\strut El} \colorbox{red!7}{\strut Cerrito} \colorbox{red!4}{\strut del} \colorbox{red!1}{\strut Norte} \colorbox{red!4}{\strut El} \colorbox{red!7}{\strut Cerrito} \colorbox{red!2}{\strut Plaza} \colorbox{red!2}{\strut Embarcadero} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Fremont} \colorbox{red!1}{\strut Fruitvale} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Oakland} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Glen} \colorbox{red!0}{\strut Park} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!8}{\strut Hayward} \colorbox{red!4}{\strut Lafayette} \colorbox{red!5}{\strut Lake} \colorbox{red!0}{\strut Merritt} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Oakland} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut MacArthur} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Oakland} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Millbrae} \colorbox{red!5}{\strut Montgomery} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut North} \colorbox{red!25}{\strut Berkeley} \colorbox{red!5}{\strut North} \colorbox{red!0}{\strut ConcordMartinez} \colorbox{red!0}{\strut Orinda} \colorbox{red!0}{\strut PittsburgBay} \colorbox{red!5}{\strut Point} \colorbox{red!7}{\strut Pleasant} \colorbox{red!4}{\strut Hill} \colorbox{red!0}{\strut Powell} \colorbox{red!0}{\strut St.} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut SF} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Richmond} \colorbox{red!4}{\strut Rockridge} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Oakland} \colorbox{red!1}{\strut .} \colorbox{red!18}{\strut San} \colorbox{red!2}{\strut Bruno} \colorbox{red!18}{\strut San} \colorbox{red!11}{\strut Francisco} \colorbox{red!2}{\strut Int} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut l} \colorbox{red!12}{\strut Airport} \colorbox{red!18}{\strut San} \colorbox{red!3}{\strut Leandro} \colorbox{red!5}{\strut South} \colorbox{red!8}{\strut Hayward} \colorbox{red!5}{\strut South} \colorbox{red!18}{\strut San} \colorbox{red!11}{\strut Francisco} \colorbox{red!5}{\strut Union} \colorbox{red!24}{\strut City} \colorbox{red!4}{\strut Walnut} \colorbox{red!6}{\strut Creek} \colorbox{red!6}{\strut West} \colorbox{red!25}{\strut Oakland} \colorbox{red!97}{\strut BART} \colorbox{red!5}{\strut System} \colorbox{red!10}{\strut Map} \colorbox{red!97}{\strut BART} \colorbox{red!6}{\strut Rider} \colorbox{red!3}{\strut Rewards} \colorbox{red!3}{\strut Card} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut myBART} \colorbox{red!2}{\strut .} \colorbox{red!97}{\strut BART} \colorbox{red!19}{\strut TV} \colorbox{red!8}{\strut Contact} \colorbox{red!4}{\strut Us} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Your} \colorbox{red!2}{\strut Privacy} \colorbox{red!2}{\strut 2009} \colorbox{red!18}{\strut San} \colorbox{red!11}{\strut Francisco} \colorbox{red!18}{\strut Bay} \colorbox{red!0}{\strut Area} \colorbox{red!7}{\strut Rapid} \colorbox{red!5}{\strut Transit} \colorbox{red!5}{\strut District} 
}}}
\end{CJK*}

100:tiles, 98:bart, 77:stops, 75:sf, 40:civic, 33:symphony, 31:center, 29:where, 29:chicago, 27:wall


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Welcome} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!4}{\strut New} \colorbox{red!4}{\strut Design} \colorbox{red!1}{\strut !} \colorbox{red!6}{\strut NY} \colorbox{red!2}{\strut ,} \colorbox{red!7}{\strut LA} \colorbox{red!2}{\strut ,} \colorbox{red!25}{\strut SF} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut Chicago} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut apartmenttherapy.com} \colorbox{red!1}{\strut The} \colorbox{red!4}{\strut Nursery} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut now} \colorbox{red!0}{\strut ohdeedoh.com} \colorbox{red!1}{\strut The} \colorbox{red!2}{\strut Kitchen} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut now} \colorbox{red!0}{\strut thekitchn.com} \colorbox{red!3}{\strut Home} \colorbox{red!1}{\strut Tech} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut now} \colorbox{red!0}{\strut unplggd.com} \colorbox{red!2}{\strut Green} \colorbox{red!3}{\strut Home} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut now} \colorbox{red!0}{\strut re-nest.com} \colorbox{red!3}{\strut apartment} \colorbox{red!3}{\strut therapy} \colorbox{red!1}{\strut changing} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut world} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut one} \colorbox{red!3}{\strut room} \colorbox{red!2}{\strut at} \colorbox{red!2}{\strut a} \colorbox{red!4}{\strut time} \colorbox{red!3}{\strut Main} \colorbox{red!4}{\strut New} \colorbox{red!3}{\strut York} \colorbox{red!2}{\strut Los} \colorbox{red!1}{\strut Angeles} \colorbox{red!6}{\strut San} \colorbox{red!4}{\strut Francisco} \colorbox{red!10}{\strut Chicago} \colorbox{red!2}{\strut DC} \colorbox{red!2}{\strut Boston} \colorbox{red!4}{\strut House} \colorbox{red!1}{\strut Tours} \colorbox{red!0}{\strut Shopping} \colorbox{red!0}{\strut Guide} \colorbox{red!1}{\strut Archive} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!1}{\strut The} \colorbox{red!1}{\strut Big} \colorbox{red!2}{\strut Window} \colorbox{red!1}{\strut Challenge} \colorbox{red!0}{\strut Community} \colorbox{red!25}{\strut SF} \colorbox{red!3}{\strut Good} \colorbox{red!0}{\strut Questions} \colorbox{red!1}{\strut .} \colorbox{red!34}{\strut Tiles} \colorbox{red!2}{\strut at} \colorbox{red!33}{\strut BART} \colorbox{red!26}{\strut Stops} \colorbox{red!1}{\strut ?} \colorbox{red!2}{\strut AT} \colorbox{red!1}{\strut .} \colorbox{red!25}{\strut SF} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut Any} \colorbox{red!3}{\strut idea} \colorbox{red!10}{\strut where} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut can} \colorbox{red!7}{\strut find} \colorbox{red!34}{\strut tiles} \colorbox{red!0}{\strut like} \colorbox{red!1}{\strut these} \colorbox{red!2}{\strut at} \colorbox{red!1}{\strut the} \colorbox{red!13}{\strut Civic} \colorbox{red!10}{\strut Center} \colorbox{red!33}{\strut BART} \colorbox{red!0}{\strut stop} \colorbox{red!1}{\strut ?} \colorbox{red!0}{\strut Thanks} \colorbox{red!1}{\strut !} \colorbox{red!0}{\strut -Laura} \colorbox{red!1}{\strut Laura} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut tile} \colorbox{red!1}{\strut Shannon} \colorbox{red!0}{\strut asked} \colorbox{red!0}{\strut about} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut months} \colorbox{red!0}{\strut ago} \colorbox{red!1}{\strut here} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut here} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut never} \colorbox{red!0}{\strut heard} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut from} \colorbox{red!33}{\strut BART} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Can} \colorbox{red!0}{\strut anyone} \colorbox{red!0}{\strut help} \colorbox{red!1}{\strut ?} \colorbox{red!2}{\strut Email} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut QUESTIONS} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut subject} \colorbox{red!1}{\strut line} \colorbox{red!1}{\strut .} \colorbox{red!25}{\strut sf} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut at} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut apartmenttherapy} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut dot} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut com} \colorbox{red!0}{\strut Note} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Include} \colorbox{red!2}{\strut a} \colorbox{red!1}{\strut picture} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut question} \colorbox{red!0}{\strut gets} \colorbox{red!2}{\strut posted} \colorbox{red!1}{\strut first} \colorbox{red!6}{\strut San} \colorbox{red!4}{\strut Francisco} \colorbox{red!0}{\strut leslie} \colorbox{red!1}{\strut June} \colorbox{red!0}{\strut 26} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut 2008} \colorbox{red!0}{\strut 0445PM} \colorbox{red!1}{\strut Comments} \colorbox{red!1}{\strut Tags} \colorbox{red!0}{\strut tile} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut stone} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut countertops} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut Good} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut TileVault} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Sunset} \colorbox{red!3}{\strut Idea} \colorbox{red!4}{\strut House} \colorbox{red!25}{\strut SF} \colorbox{red!3}{\strut Good} \colorbox{red!0}{\strut Questions} \colorbox{red!1}{\strut .} \colorbox{red!34}{\strut Tiles} \colorbox{red!2}{\strut at} \colorbox{red!33}{\strut BART} \colorbox{red!26}{\strut Stops} \colorbox{red!1}{\strut ?} \colorbox{red!11}{\strut Symphony} \colorbox{red!9}{\strut Wall} \colorbox{red!34}{\strut Tiles} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Dominic} \colorbox{red!2}{\strut Crinson} \colorbox{red!0}{\strut TileVault} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Small} \colorbox{red!2}{\strut Blue} \colorbox{red!5}{\strut Squares} \colorbox{red!1}{\strut Look} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Spacious} \colorbox{red!2}{\strut Blue} \colorbox{red!3}{\strut Bathroom} \colorbox{red!1}{\strut Share} \colorbox{red!1}{\strut Comments} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut 7} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!1}{\strut it} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut subconscious} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut hexagon} \colorbox{red!4}{\strut patterns} \colorbox{red!1}{\strut do} \colorbox{red!1}{\strut have} \colorbox{red!2}{\strut a} \colorbox{red!1}{\strut late} \colorbox{red!0}{\strut 60s-early} \colorbox{red!0}{\strut 70s} \colorbox{red!1}{\strut vibe} \colorbox{red!1}{\strut ?} \colorbox{red!2}{\strut posted} \colorbox{red!0}{\strut by} \colorbox{red!5}{\strut pantzini} \colorbox{red!1}{\strut on} \colorbox{red!1}{\strut June} \colorbox{red!2}{\strut 26th} \colorbox{red!1}{\strut 2008} \colorbox{red!2}{\strut at} \colorbox{red!0}{\strut 1246pm} \colorbox{red!1}{\strut view} \colorbox{red!5}{\strut pantzini} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut profile} \colorbox{red!0}{\strut If} \colorbox{red!1}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut not} \colorbox{red!5}{\strut made} \colorbox{red!1}{\strut anymore} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut someone} \colorbox{red!0}{\strut certainly} \colorbox{red!0}{\strut should} \colorbox{red!2}{\strut take} \colorbox{red!1}{\strut up} \colorbox{red!3}{\strut making} \colorbox{red!1}{\strut it} \colorbox{red!0}{\strut again} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut tile} \colorbox{red!3}{\strut company} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut tile} \colorbox{red!0}{\strut companies} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut listening} \colorbox{red!1}{\strut ?} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut People} \colorbox{red!1}{\strut seem} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut love} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut tile} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotosjayfish129710344inset-72157600356591088} \colorbox{red!1}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotospetebeck12389105} \colorbox{red!1}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotosjbergen1200303453inset-72157601592381820} \colorbox{red!1}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotoselithebearded1450203895inset-72157594574414547} \colorbox{red!1}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut www.flickr.comphotosjef145597993} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut know} 
}}}
\end{CJK*}

query: raffles

100:raffles, 100:hotel, 62:what, 56:famous, 10:english, 10:bangkok, 10:asia, 9:oriental, 9:guests, 8:views


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!0}{\strut From} \colorbox{red!12}{\strut Wikimedia} \colorbox{red!0}{\strut Commons} \colorbox{red!5}{\strut ,} \colorbox{red!5}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!3}{\strut media} \colorbox{red!1}{\strut repository} \colorbox{red!7}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut .} \colorbox{red!8}{\strut navigation} \colorbox{red!5}{\strut ,} \colorbox{red!7}{\strut search} \colorbox{red!17}{\strut English} \colorbox{red!3}{\strut .} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!5}{\strut is} \colorbox{red!8}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!10}{\strut most} \colorbox{red!99}{\strut famous} \colorbox{red!0}{\strut hotels} \colorbox{red!8}{\strut in} \colorbox{red!17}{\strut Asia} \colorbox{red!5}{\strut ,} \colorbox{red!3}{\strut among} \colorbox{red!8}{\strut with} \colorbox{red!5}{\strut The} \colorbox{red!15}{\strut Oriental} \colorbox{red!8}{\strut in} \colorbox{red!17}{\strut Bangkok} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut The} \colorbox{red!100}{\strut hotel} \colorbox{red!7}{\strut have} \colorbox{red!8}{\strut had} \colorbox{red!3}{\strut many} \colorbox{red!99}{\strut famous} \colorbox{red!15}{\strut guests} \colorbox{red!5}{\strut ,} \colorbox{red!3}{\strut among} \colorbox{red!3}{\strut them} \colorbox{red!7}{\strut Rudyard} \colorbox{red!7}{\strut Kipling} \colorbox{red!3}{\strut .} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!7}{\strut Courtyard} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!5}{\strut The} \colorbox{red!10}{\strut Lawn} \colorbox{red!5}{\strut ,} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!12}{\strut Fountain} \colorbox{red!7}{\strut at} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!8}{\strut Retrieved} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut http} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut commons.wikimedia.orgwikiRafflesHotel} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Category} \colorbox{red!3}{\strut .} \colorbox{red!100}{\strut Raffles} \colorbox{red!100}{\strut Hotel} \colorbox{red!14}{\strut Views} \colorbox{red!7}{\strut Gallery} \colorbox{red!0}{\strut Discussion} \colorbox{red!1}{\strut Edit} \colorbox{red!7}{\strut History} \colorbox{red!5}{\strut Personal} \colorbox{red!0}{\strut tools} \colorbox{red!0}{\strut Log} \colorbox{red!8}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut create} \colorbox{red!5}{\strut account} \colorbox{red!7}{\strut Search} \colorbox{red!8}{\strut Navigation} \colorbox{red!0}{\strut Main} \colorbox{red!0}{\strut Page} \colorbox{red!3}{\strut Welcome} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut portal} \colorbox{red!3}{\strut Village} \colorbox{red!0}{\strut pump} \colorbox{red!0}{\strut Participate} \colorbox{red!0}{\strut Upload} \colorbox{red!7}{\strut file} \colorbox{red!0}{\strut Recent} \colorbox{red!3}{\strut changes} \colorbox{red!1}{\strut Latest} \colorbox{red!0}{\strut files} \colorbox{red!0}{\strut Random} \colorbox{red!7}{\strut file} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut Donate} \colorbox{red!0}{\strut Toolbox} \colorbox{red!100}{\strut What} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut Related} \colorbox{red!3}{\strut changes} \colorbox{red!0}{\strut Special} \colorbox{red!0}{\strut pages} \colorbox{red!1}{\strut Printable} \colorbox{red!0}{\strut version} \colorbox{red!3}{\strut Permanent} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut Cite} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!8}{\strut In} \colorbox{red!5}{\strut Wikipedia} \colorbox{red!0}{\strut Deutsch} \colorbox{red!17}{\strut English} \colorbox{red!5}{\strut ,} \colorbox{red!1}{\strut Svenska} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut last} \colorbox{red!0}{\strut modified} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut 22} \colorbox{red!3}{\strut November} \colorbox{red!0}{\strut 2008} \colorbox{red!5}{\strut ,} \colorbox{red!7}{\strut at} \colorbox{red!0}{\strut 1623} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Text} \colorbox{red!5}{\strut is} \colorbox{red!0}{\strut available} \colorbox{red!1}{\strut under} \colorbox{red!3}{\strut GNU} \colorbox{red!0}{\strut Free} \colorbox{red!7}{\strut Documentation} \colorbox{red!5}{\strut License} \colorbox{red!3}{\strut .} \colorbox{red!12}{\strut Wikimedia} \colorbox{red!5}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!14}{\strut registered} \colorbox{red!10}{\strut trademark} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut the} \colorbox{red!12}{\strut Wikimedia} \colorbox{red!0}{\strut Foundation} \colorbox{red!5}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!10}{\strut Privacy} \colorbox{red!7}{\strut policy} \colorbox{red!7}{\strut About} \colorbox{red!12}{\strut Wikimedia} \colorbox{red!0}{\strut Commons} \colorbox{red!0}{\strut Disclaimers} 
}}}
\end{CJK*}

100:raffles, 41:hotel, 20:destinations, 11:home, 10:china, 9:weddings, 9:singapore, 9:resorts, 9:airline, 8:social


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!40}{\strut Hotel} \colorbox{red!19}{\strut Destinations} \colorbox{red!7}{\strut Beijing} \colorbox{red!1}{\strut ,} \colorbox{red!9}{\strut China} \colorbox{red!0}{\strut Beverly} \colorbox{red!2}{\strut Hills} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut California} \colorbox{red!4}{\strut Dubai} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut United} \colorbox{red!2}{\strut Arab} \colorbox{red!3}{\strut Emirates} \colorbox{red!4}{\strut Phnom} \colorbox{red!0}{\strut Penh} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Cambodia} \colorbox{red!0}{\strut Siem} \colorbox{red!2}{\strut Reap} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Cambodia} \colorbox{red!8}{\strut Singapore} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut Grenadines} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Caribbean} \colorbox{red!2}{\strut Select} \colorbox{red!3}{\strut Language} \colorbox{red!3}{\strut English} \colorbox{red!4}{\strut Contact} \colorbox{red!4}{\strut us} \colorbox{red!99}{\strut Raffles} \colorbox{red!10}{\strut Home} \colorbox{red!0}{\strut About} \colorbox{red!99}{\strut Raffles} \colorbox{red!7}{\strut Exclusive} \colorbox{red!7}{\strut Offers} \colorbox{red!8}{\strut Weddings} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Celebrations} \colorbox{red!6}{\strut Meetings} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Events} \colorbox{red!0}{\strut RafflesAmrita} \colorbox{red!5}{\strut Spa} \colorbox{red!99}{\strut Raffles} \colorbox{red!6}{\strut Ambassadors} \colorbox{red!5}{\strut Private} \colorbox{red!5}{\strut Ownership} \colorbox{red!4}{\strut Media} \colorbox{red!4}{\strut Room} \colorbox{red!99}{\strut Raffles} \colorbox{red!40}{\strut Hotel} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Resorts} \colorbox{red!7}{\strut Corporate} \colorbox{red!7}{\strut Social} \colorbox{red!4}{\strut Responsibilty} \colorbox{red!4}{\strut History} \colorbox{red!3}{\strut Core} \colorbox{red!6}{\strut Competencies} \colorbox{red!99}{\strut Raffles} \colorbox{red!6}{\strut News} \colorbox{red!99}{\strut Raffles} \colorbox{red!3}{\strut Experiences} \colorbox{red!8}{\strut Airline} \colorbox{red!6}{\strut Partners} \colorbox{red!3}{\strut Credit} \colorbox{red!3}{\strut Card} \colorbox{red!6}{\strut Partners} \colorbox{red!4}{\strut Gift} \colorbox{red!2}{\strut Certificates} \colorbox{red!4}{\strut Ovation} \colorbox{red!6}{\strut Rewards} \colorbox{red!6}{\strut Travel} \colorbox{red!3}{\strut Agents} \colorbox{red!99}{\strut Raffles} \colorbox{red!4}{\strut Romance} \colorbox{red!99}{\strut Raffles} \colorbox{red!3}{\strut Revelry} \colorbox{red!3}{\strut Press} \colorbox{red!3}{\strut Release} \colorbox{red!4}{\strut Awards} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Accolades} \colorbox{red!2}{\strut Bouquets} \colorbox{red!99}{\strut Raffles} \colorbox{red!6}{\strut News} \colorbox{red!2}{\strut Gallery} \colorbox{red!0}{\strut Overview} \colorbox{red!10}{\strut Home} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Media} \colorbox{red!4}{\strut Room} \colorbox{red!1}{\strut .} \colorbox{red!99}{\strut Raffles} \colorbox{red!6}{\strut News} 
}}}
\end{CJK*}

query: rice

102:rice, 26:recipes, 23:fried, 21:treats, 19:chicken, 18:spanish, 17:chilled, 15:shrimp, 15:mexican, 14:contact


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!9}{\strut Home} \colorbox{red!18}{\strut Contact} \colorbox{red!2}{\strut Us} \colorbox{red!12}{\strut Links} \colorbox{red!8}{\strut XML} \colorbox{red!6}{\strut Site} \colorbox{red!10}{\strut Map} \colorbox{red!6}{\strut Site} \colorbox{red!10}{\strut Map} \colorbox{red!10}{\strut Copyright} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut Page} \colorbox{red!6}{\strut 1} \colorbox{red!9}{\strut 2} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!9}{\strut Index} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!18}{\strut Contact} \colorbox{red!2}{\strut Us} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!18}{\strut Contact} \colorbox{red!2}{\strut Us} \colorbox{red!5}{\strut Thank} \colorbox{red!0}{\strut You} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut Links} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut Site} \colorbox{red!10}{\strut Map} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut XML} \colorbox{red!6}{\strut Site} \colorbox{red!10}{\strut Map} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!25}{\strut Chicken} \colorbox{red!100}{\strut Rice} \colorbox{red!16}{\strut Casserole} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!24}{\strut Spanish} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!25}{\strut Chicken} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!100}{\strut Rice} \colorbox{red!14}{\strut Pudding} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!10}{\strut Baked} \colorbox{red!25}{\strut Chicken} \colorbox{red!1}{\strut And} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!100}{\strut Rice} \colorbox{red!5}{\strut Krispies} \colorbox{red!28}{\strut Treats} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!25}{\strut Chicken} \colorbox{red!1}{\strut And} \colorbox{red!100}{\strut Rice} \colorbox{red!16}{\strut Soup} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Basmati} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!20}{\strut Mexican} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!17}{\strut Red} \colorbox{red!16}{\strut Beans} \colorbox{red!1}{\strut And} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!100}{\strut Rice} \colorbox{red!18}{\strut Cake} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!17}{\strut Chinese} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!13}{\strut Sticky} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!9}{\strut Sushi} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!17}{\strut Bayou} \colorbox{red!20}{\strut Shrimp} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!14}{\strut Turkey} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!17}{\strut Homemade} \colorbox{red!100}{\strut Rice} \colorbox{red!13}{\strut Milk} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Lemon} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Garlic} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut Cajun} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!10}{\strut Beef} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!20}{\strut Mexican} \colorbox{red!14}{\strut Fire} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!100}{\strut Rice} \colorbox{red!6}{\strut Pilaf} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut Minute} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut Spicy} \colorbox{red!10}{\strut Jalapeno} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!100}{\strut Rice} \colorbox{red!13}{\strut Balls} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut Southwestern} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!9}{\strut Pork} \colorbox{red!30}{\strut Fried} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!10}{\strut Onion} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!22}{\strut Chilled} \colorbox{red!100}{\strut Rice} \colorbox{red!13}{\strut Salad} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut Chocolate} \colorbox{red!100}{\strut Rice} \colorbox{red!14}{\strut Pudding} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Pineapple} \colorbox{red!100}{\strut Rice} \colorbox{red!16}{\strut Casserole} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut Mushroom} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut Honey} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!10}{\strut Wild} \colorbox{red!100}{\strut Rice} \colorbox{red!16}{\strut Casserole} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!5}{\strut Calamari} \colorbox{red!1}{\strut And} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Cheesy} \colorbox{red!4}{\strut Confetti} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Okra} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut Taco} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!12}{\strut Asian} \colorbox{red!16}{\strut Coconut} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!14}{\strut Green} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!14}{\strut Jamaican} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!17}{\strut Indian} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!13}{\strut Hamburger} \colorbox{red!100}{\strut Rice} \colorbox{red!16}{\strut Soup} \colorbox{red!100}{\strut Rice} \colorbox{red!35}{\strut Recipes} \colorbox{red!0}{\strut -} \colorbox{red!8}{\strut Ham} 
}}}
\end{CJK*}

99:rice, 99:lake, 37:minnesota, 26:county, 11:name, 11:aitkin, 8:cass, 7:crow, 6:blue, 6:anoka


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!0}{\strut .} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!4}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut search} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut refer} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut dozen} \colorbox{red!0}{\strut lakes} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!15}{\strut name} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!15}{\strut Aitkin} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!15}{\strut Aitkin} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!15}{\strut Aitkin} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!15}{\strut Aitkin} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!8}{\strut Anoka} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!8}{\strut Anoka} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!7}{\strut Becker} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!7}{\strut Becker} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!7}{\strut Becker} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!7}{\strut Becker} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!7}{\strut Becker} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!5}{\strut Beltrami} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!5}{\strut Beltrami} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!5}{\strut Beltrami} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!5}{\strut Beltrami} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!5}{\strut Beltrami} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!8}{\strut Blue} \colorbox{red!4}{\strut Earth} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!5}{\strut Carver} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!11}{\strut Cass} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!11}{\strut Cass} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!11}{\strut Cass} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!11}{\strut Cass} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!11}{\strut Cass} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!11}{\strut Cass} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!7}{\strut Cook} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!9}{\strut Crow} \colorbox{red!5}{\strut Wing} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!9}{\strut Crow} \colorbox{red!5}{\strut Wing} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!9}{\strut Crow} \colorbox{red!5}{\strut Wing} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!9}{\strut Crow} \colorbox{red!5}{\strut Wing} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!9}{\strut Crow} \colorbox{red!5}{\strut Wing} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!9}{\strut Crow} \colorbox{red!5}{\strut Wing} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} \colorbox{red!9}{\strut Crow} \colorbox{red!5}{\strut Wing} \colorbox{red!36}{\strut County} \colorbox{red!4}{\strut ,} \colorbox{red!51}{\strut Minnesota} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Rice} \colorbox{red!100}{\strut Lake} \colorbox{red!7}{\strut in} 
}}}
\end{CJK*}

query: sat

85:vocabulary, 53:sat, 38:words, 34:lists, 20:business, 19:practice, 18:school, 15:score, 13:high, 12:education


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!18}{\strut Search} \colorbox{red!40}{\strut Business} \colorbox{red!36}{\strut School} \colorbox{red!8}{\strut Home} \colorbox{red!24}{\strut Education} \colorbox{red!40}{\strut Business} \colorbox{red!36}{\strut School} \colorbox{red!40}{\strut Business} \colorbox{red!36}{\strut School} \colorbox{red!6}{\strut Admissions} \colorbox{red!0}{\strut Careers} \colorbox{red!40}{\strut Business} \colorbox{red!36}{\strut School} \colorbox{red!0}{\strut Life} \colorbox{red!4}{\strut Filed} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut SAT} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut GMAT} \colorbox{red!22}{\strut Preparation} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!10}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!30}{\strut score} \colorbox{red!26}{\strut high} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut the} \colorbox{red!100}{\strut SAT} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!8}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!12}{\strut know} \colorbox{red!18}{\strut essential} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut vocabulary} \colorbox{red!76}{\strut words} \colorbox{red!12}{\strut .} \colorbox{red!18}{\strut Here} \colorbox{red!14}{\strut are} \colorbox{red!8}{\strut a} \colorbox{red!4}{\strut few} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut vocabulary} \colorbox{red!68}{\strut lists} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!6}{\strut can} \colorbox{red!6}{\strut use} \colorbox{red!0}{\strut to} \colorbox{red!38}{\strut practice} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut prepare} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!100}{\strut SAT} \colorbox{red!12}{\strut .} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!16}{\strut 25} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!16}{\strut 25} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 24} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 24} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 23} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 23} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!6}{\strut 22} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!6}{\strut 22} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 21} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 21} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!4}{\strut 20} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!4}{\strut 20} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 19} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 19} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 18} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut 18} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!4}{\strut 17} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!4}{\strut 17} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!2}{\strut 16} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!2}{\strut 16} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!10}{\strut 15} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!10}{\strut 15} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!10}{\strut 14} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!10}{\strut 14} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 13} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 13} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 12} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 12} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 11} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!12}{\strut 11} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!0}{\strut List} \colorbox{red!16}{\strut Ten} \colorbox{red!100}{\strut SAT} \colorbox{red!100}{\strut Vocabulary} \colorbox{red!38}{\strut Practice} \colorbox{red!6}{\strut -} \colorbox{red!100}{\strut SAT} 
}}}
\end{CJK*}

98:sat, 98:man, 47:limited, 26:company, 21:offices, 18:uk, 17:registered, 16:isle, 11:liability, 10:london


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut ManSat} \colorbox{red!52}{\strut Limited} \colorbox{red!0}{\strut -} \colorbox{red!20}{\strut UK} \colorbox{red!23}{\strut Offices} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut ManSat} \colorbox{red!7}{\strut Ltd} \colorbox{red!0}{\strut 12} \colorbox{red!2}{\strut Tybenham} \colorbox{red!4}{\strut Road} \colorbox{red!11}{\strut London} \colorbox{red!0}{\strut SW19} \colorbox{red!0}{\strut 3LA} \colorbox{red!6}{\strut United} \colorbox{red!6}{\strut Kingdom} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Tel.} \colorbox{red!0}{\strut 44} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut 8542} \colorbox{red!0}{\strut 5762} \colorbox{red!7}{\strut Fax} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 44} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut 8404} \colorbox{red!2}{\strut 2940} \colorbox{red!10}{\strut Mobile} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 44} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 77} \colorbox{red!0}{\strut 70} \colorbox{red!0}{\strut 415} \colorbox{red!0}{\strut 545} \colorbox{red!4}{\strut information} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mansat.com} \colorbox{red!6}{\strut Copyright} \colorbox{red!6}{\strut 2000} \colorbox{red!4}{\strut ManSat} \colorbox{red!52}{\strut Limited} \colorbox{red!4}{\strut ManSat} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut an} \colorbox{red!17}{\strut Isle} \colorbox{red!2}{\strut of} \colorbox{red!100}{\strut Man} \colorbox{red!19}{\strut registered} \colorbox{red!52}{\strut Limited} \colorbox{red!12}{\strut Liability} \colorbox{red!29}{\strut Company} \colorbox{red!4}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut 92219C} 
}}}
\end{CJK*}

query: butter margarine

95:margarine, 88:butter, 74:healthier, 62:what, 36:made, 22:better, 17:health, 17:benefits, 13:medical, 12:rich


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!12}{\strut Medical} \colorbox{red!0}{\strut Services} \colorbox{red!1}{\strut .} \colorbox{red!15}{\strut Health} \colorbox{red!0}{\strut Information} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Appointments} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Education} \colorbox{red!6}{\strut and} \colorbox{red!2}{\strut Research} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Jobs} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Podcast} \colorbox{red!1}{\strut .} \colorbox{red!88}{\strut Margarine} \colorbox{red!4}{\strut Is} \colorbox{red!6}{\strut it} \colorbox{red!68}{\strut healthier} \colorbox{red!0}{\strut than} \colorbox{red!81}{\strut butter} \colorbox{red!0}{\strut ?} \colorbox{red!12}{\strut Medical} \colorbox{red!0}{\strut expert} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!8}{\strut Zeratsky} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut R.D.} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut L.D} \colorbox{red!8}{\strut .} \colorbox{red!4}{\strut Total} \colorbox{red!4}{\strut time} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 00542} \colorbox{red!3}{\strut minutes} \colorbox{red!2}{\strut Subscribe} \colorbox{red!4}{\strut to} \colorbox{red!2}{\strut podcasts} \colorbox{red!5}{\strut TRANSCRIPT} \colorbox{red!4}{\strut Welcome} \colorbox{red!4}{\strut to} \colorbox{red!8}{\strut Mayo} \colorbox{red!7}{\strut Clinic} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut podcast} \colorbox{red!8}{\strut .} \colorbox{red!2}{\strut This} \colorbox{red!2}{\strut month} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut topic} \colorbox{red!4}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!88}{\strut Margarine} \colorbox{red!4}{\strut Is} \colorbox{red!6}{\strut it} \colorbox{red!68}{\strut healthier} \colorbox{red!0}{\strut than} \colorbox{red!81}{\strut butter} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut I} \colorbox{red!0}{\strut m} \colorbox{red!2}{\strut your} \colorbox{red!2}{\strut host} \colorbox{red!6}{\strut ,} \colorbox{red!11}{\strut Rich} \colorbox{red!8}{\strut Dietman} \colorbox{red!8}{\strut .} \colorbox{red!2}{\strut In} \colorbox{red!5}{\strut today} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut podcast} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut talking} \colorbox{red!0}{\strut about} \colorbox{red!3}{\strut the} \colorbox{red!2}{\strut relative} \colorbox{red!15}{\strut health} \colorbox{red!15}{\strut benefits} \colorbox{red!6}{\strut of} \colorbox{red!88}{\strut margarine} \colorbox{red!0}{\strut vs.} \colorbox{red!81}{\strut butter} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Katherine} \colorbox{red!8}{\strut Zeratsky} \colorbox{red!6}{\strut ,} \colorbox{red!4}{\strut a} \colorbox{red!6}{\strut registered} \colorbox{red!4}{\strut dietitian} \colorbox{red!3}{\strut at} \colorbox{red!8}{\strut Mayo} \colorbox{red!7}{\strut Clinic} \colorbox{red!6}{\strut ,} \colorbox{red!6}{\strut and} \colorbox{red!3}{\strut specialty} \colorbox{red!2}{\strut editor} \colorbox{red!4}{\strut for} \colorbox{red!3}{\strut the} \colorbox{red!8}{\strut Food} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Nutrition} \colorbox{red!3}{\strut Center} \colorbox{red!2}{\strut on} \colorbox{red!0}{\strut MayoClinic.com} \colorbox{red!8}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut thanks} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut us} \colorbox{red!5}{\strut today} \colorbox{red!8}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!8}{\strut Zeratsky} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Thank} \colorbox{red!2}{\strut you} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut having} \colorbox{red!3}{\strut me} \colorbox{red!8}{\strut .} \colorbox{red!11}{\strut Rich} \colorbox{red!8}{\strut Dietman} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Let} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut get} \colorbox{red!4}{\strut right} \colorbox{red!4}{\strut to} \colorbox{red!6}{\strut it} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut Katherine} \colorbox{red!8}{\strut .} \colorbox{red!57}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!20}{\strut better} \colorbox{red!4}{\strut for} \colorbox{red!2}{\strut your} \colorbox{red!7}{\strut heart} \colorbox{red!81}{\strut butter} \colorbox{red!0}{\strut or} \colorbox{red!88}{\strut margarine} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Katherine} \colorbox{red!8}{\strut Zeratsky} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Quite} \colorbox{red!0}{\strut generally} \colorbox{red!0}{\strut speaking} \colorbox{red!6}{\strut ,} \colorbox{red!88}{\strut margarine} \colorbox{red!4}{\strut is} \colorbox{red!4}{\strut a} \colorbox{red!20}{\strut better} \colorbox{red!6}{\strut choice} \colorbox{red!8}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!2}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!2}{\strut been} \colorbox{red!4}{\strut to} \colorbox{red!2}{\strut your} \colorbox{red!0}{\strut local} \colorbox{red!5}{\strut grocery} \colorbox{red!4}{\strut store} \colorbox{red!6}{\strut and} \colorbox{red!3}{\strut checked} \colorbox{red!3}{\strut out} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut butter-margarine} \colorbox{red!3}{\strut aisle} \colorbox{red!6}{\strut ,} \colorbox{red!2}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut see} \colorbox{red!1}{\strut that} \colorbox{red!2}{\strut my} \colorbox{red!0}{\strut answer} \colorbox{red!6}{\strut of} \colorbox{red!88}{\strut margarine} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut necessarily} \colorbox{red!7}{\strut mean} \colorbox{red!5}{\strut picking} \colorbox{red!3}{\strut out} \colorbox{red!4}{\strut a} \colorbox{red!88}{\strut margarine} \colorbox{red!4}{\strut is} \colorbox{red!3}{\strut an} \colorbox{red!6}{\strut easy} \colorbox{red!0}{\strut thing} \colorbox{red!4}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!8}{\strut .} \colorbox{red!11}{\strut Rich} \colorbox{red!8}{\strut Dietman} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut And} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut because} \colorbox{red!4}{\strut there} \colorbox{red!3}{\strut are} \colorbox{red!3}{\strut just} \colorbox{red!0}{\strut so} \colorbox{red!4}{\strut many} \colorbox{red!0}{\strut choices} \colorbox{red!8}{\strut .} \colorbox{red!0}{\strut Katherine} \colorbox{red!8}{\strut Zeratsky} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut That} \colorbox{red!4}{\strut is} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut there} \colorbox{red!3}{\strut are} \colorbox{red!4}{\strut many} \colorbox{red!0}{\strut choices} \colorbox{red!2}{\strut from} \colorbox{red!10}{\strut different} \colorbox{red!10}{\strut types} \colorbox{red!6}{\strut of} \colorbox{red!81}{\strut butter} \colorbox{red!6}{\strut ,} \colorbox{red!8}{\strut straight} \colorbox{red!88}{\strut margarine} \colorbox{red!6}{\strut ,} \colorbox{red!4}{\strut to} \colorbox{red!10}{\strut different} \colorbox{red!5}{\strut kinds} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut margarine-like} \colorbox{red!5}{\strut spreads} \colorbox{red!8}{\strut .} \colorbox{red!11}{\strut Rich} \colorbox{red!8}{\strut Dietman} \colorbox{red!1}{\strut .} \colorbox{red!9}{\strut Why} \colorbox{red!4}{\strut is} \colorbox{red!2}{\strut this} \colorbox{red!2}{\strut such} \colorbox{red!4}{\strut a} \colorbox{red!4}{\strut difficult} \colorbox{red!6}{\strut choice} \colorbox{red!6}{\strut ,} \colorbox{red!6}{\strut and} \colorbox{red!9}{\strut why} \colorbox{red!4}{\strut is} \colorbox{red!6}{\strut it} \colorbox{red!2}{\strut such} \colorbox{red!4}{\strut a} \colorbox{red!3}{\strut tricky} \colorbox{red!2}{\strut proposition} \colorbox{red!4}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!4}{\strut choosing} \colorbox{red!6}{\strut ,} \colorbox{red!1}{\strut first} \colorbox{red!6}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!6}{\strut ,} \colorbox{red!0}{\strut between} \colorbox{red!81}{\strut butter} \colorbox{red!6}{\strut and} \colorbox{red!88}{\strut margarine} \colorbox{red!6}{\strut ,} \colorbox{red!6}{\strut and} \colorbox{red!2}{\strut then} \colorbox{red!0}{\strut as} \colorbox{red!2}{\strut you} \colorbox{red!4}{\strut say} \colorbox{red!6}{\strut ,} \colorbox{red!3}{\strut trying} \colorbox{red!4}{\strut to} \colorbox{red!0}{\strut pick} \colorbox{red!3}{\strut the} \colorbox{red!7}{\strut best} \colorbox{red!88}{\strut margarine} \colorbox{red!6}{\strut ,} \colorbox{red!1}{\strut since} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut probably} \colorbox{red!3}{\strut the} \colorbox{red!20}{\strut better} \colorbox{red!11}{\strut product} \colorbox{red!4}{\strut for} \colorbox{red!0}{\strut us} 
}}}
\end{CJK*}

97:butter, 95:margarine, 65:what, 54:difference, 45:how, 23:tastes, 21:benefits, 20:turkeys, 19:eating, 17:grams


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Homeopathy} \colorbox{red!5}{\strut Arizona} \colorbox{red!0}{\strut Dedicated} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut integrative} \colorbox{red!2}{\strut medicine} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut advancing} \colorbox{red!5}{\strut Homeopathy} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut alternative} \colorbox{red!2}{\strut medicine} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut Arizona} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut globally} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Nutrition} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2008} \colorbox{red!3}{\strut Pass} \colorbox{red!1}{\strut The} \colorbox{red!46}{\strut Butter} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Nutritional} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Must} \colorbox{red!2}{\strut Know} \colorbox{red!45}{\strut Margarine} \colorbox{red!0}{\strut was} \colorbox{red!4}{\strut originally} \colorbox{red!2}{\strut manufactured} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut fatten} \colorbox{red!9}{\strut turkeys} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut When} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut killed} \colorbox{red!1}{\strut the} \colorbox{red!9}{\strut turkeys} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut the} \colorbox{red!2}{\strut people} \colorbox{red!2}{\strut who} \colorbox{red!0}{\strut had} \colorbox{red!2}{\strut put} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut money} \colorbox{red!0}{\strut into} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut research} \colorbox{red!0}{\strut wanted} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut payback} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut they} \colorbox{red!2}{\strut put} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut heads} \colorbox{red!1}{\strut together} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut figure} \colorbox{red!0}{\strut out} \colorbox{red!31}{\strut what} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut money} \colorbox{red!1}{\strut back} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut white} \colorbox{red!1}{\strut substance} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut no} \colorbox{red!7}{\strut food} \colorbox{red!0}{\strut appeal} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut they} \colorbox{red!2}{\strut added} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut yellow} \colorbox{red!8}{\strut coloring} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut sold} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut people} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut pla} \colorbox{red!0}{\strut ce} \colorbox{red!1}{\strut of} \colorbox{red!46}{\strut butter} \colorbox{red!1}{\strut .} \colorbox{red!21}{\strut How} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut come} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut clever} \colorbox{red!1}{\strut new} \colorbox{red!5}{\strut flavorings} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut DO} \colorbox{red!0}{\strut YOU} \colorbox{red!2}{\strut KNOW} \colorbox{red!1}{\strut the} \colorbox{red!26}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!45}{\strut margarine} \colorbox{red!1}{\strut and} \colorbox{red!46}{\strut butter} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut gets} \colorbox{red!0}{\strut very} \colorbox{red!1}{\strut interesting} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Both} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut same} \colorbox{red!4}{\strut amount} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut ca} \colorbox{red!2}{\strut lories} \colorbox{red!1}{\strut .} \colorbox{red!46}{\strut Butter} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut slightly} \colorbox{red!4}{\strut higher} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut saturated} \colorbox{red!7}{\strut fats} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 8} \colorbox{red!8}{\strut grams} \colorbox{red!2}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 5} \colorbox{red!8}{\strut grams} \colorbox{red!1}{\strut .} \colorbox{red!9}{\strut Eating} \colorbox{red!45}{\strut margarine} \colorbox{red!1}{\strut can} \colorbox{red!6}{\strut increase} \colorbox{red!3}{\strut heart} \colorbox{red!4}{\strut disease} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut women} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut 53} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut over} \colorbox{red!9}{\strut eating} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut same} \colorbox{red!4}{\strut amount} \colorbox{red!1}{\strut of} \colorbox{red!46}{\strut butter} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut according} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut recent} \colorbox{red!0}{\strut Harvard} \colorbox{red!3}{\strut Medical} \colorbox{red!1}{\strut Study} \colorbox{red!9}{\strut Eating} \colorbox{red!46}{\strut butter} \colorbox{red!0}{\strut increases} \colorbox{red!1}{\strut the} \colorbox{red!1}{\strut absorption} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut many} \colorbox{red!0}{\strut other} \colorbox{red!4}{\strut nutrients} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut foods} \colorbox{red!1}{\strut .} \colorbox{red!46}{\strut Butter} \colorbox{red!0}{\strut has} \colorbox{red!1}{\strut many} \colorbox{red!0}{\strut nutritional} \colorbox{red!10}{\strut benefits} \colorbox{red!2}{\strut where} \colorbox{red!0}{\strut m} \colorbox{red!2}{\strut argari} \colorbox{red!0}{\strut ne} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!1}{\strut only} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut added} \colorbox{red!0}{\strut !} \colorbox{red!46}{\strut Butter} \colorbox{red!11}{\strut tastes} \colorbox{red!0}{\strut much} \colorbox{red!5}{\strut better} \colorbox{red!1}{\strut than} \colorbox{red!45}{\strut margarine} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut can} \colorbox{red!1}{\strut enhance} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut flavors} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut ot} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut foods} \colorbox{red!1}{\strut .} \colorbox{red!46}{\strut Butter} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut centuries} \colorbox{red!2}{\strut where} \colorbox{red!45}{\strut margarine} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut less} \colorbox{red!1}{\strut than} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut years} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut And} \colorbox{red!1}{\strut now} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut for} \colorbox{red!45}{\strut Margarine} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Very} \colorbox{red!4}{\strut high} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut trans} \colorbox{red!1}{\strut fatty} \colorbox{red!2}{\strut acids} \colorbox{red!1}{\strut Triple} \colorbox{red!0}{\strut risk} \colorbox{red!1}{\strut of} \colorbox{red!3}{\strut coronary} \colorbox{red!3}{\strut heart} \colorbox{red!4}{\strut disease} \colorbox{red!0}{\strut Increases} \colorbox{red!1}{\strut total} \colorbox{red!6}{\strut cholesterol} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut LDL} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut bad} \colorbox{red!6}{\strut cholesterol} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut and} \colorbox{red!6}{\strut lowers} \colorbox{red!3}{\strut HDL} \colorbox{red!6}{\strut cholesterol} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut the} \colorbox{red!7}{\strut good} \colorbox{red!6}{\strut cholesterol} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: fact uranus

99:uranus, 44:how, 35:did, 29:names, 27:mean, 27:big, 23:who, 22:planet, 21:spelled, 16:surface


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Dictionary} \colorbox{red!3}{\strut Thesaurus} \colorbox{red!7}{\strut Reference} \colorbox{red!5}{\strut Translate} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Register} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Suggestions} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Searches} \colorbox{red!2}{\strut on} \colorbox{red!0}{\strut Ask.com} \colorbox{red!100}{\strut uranus} \colorbox{red!10}{\strut facts} \colorbox{red!25}{\strut planet} \colorbox{red!100}{\strut uranus} \colorbox{red!100}{\strut uranus} \colorbox{red!17}{\strut moons} \colorbox{red!100}{\strut uranus} \colorbox{red!7}{\strut rings} \colorbox{red!100}{\strut uranus} \colorbox{red!5}{\strut atmosphere} \colorbox{red!0}{\strut interesting} \colorbox{red!10}{\strut facts} \colorbox{red!0}{\strut ...} \colorbox{red!100}{\strut uranus} \colorbox{red!18}{\strut surface} \colorbox{red!100}{\strut uranus} \colorbox{red!0}{\strut informatio} \colorbox{red!0}{\strut ...} \colorbox{red!17}{\strut greek} \colorbox{red!12}{\strut god} \colorbox{red!100}{\strut uranus} \colorbox{red!100}{\strut uranus} \colorbox{red!0}{\strut fact} \colorbox{red!5}{\strut sheet} \colorbox{red!32}{\strut names} \colorbox{red!3}{\strut of} \colorbox{red!100}{\strut uranus} \colorbox{red!7}{\strut m} \colorbox{red!0}{\strut ...} \colorbox{red!50}{\strut how} \colorbox{red!39}{\strut did} \colorbox{red!100}{\strut uranus} \colorbox{red!7}{\strut ge} \colorbox{red!0}{\strut ...} \colorbox{red!4}{\strut fun} \colorbox{red!10}{\strut facts} \colorbox{red!4}{\strut about} \colorbox{red!100}{\strut uranus} \colorbox{red!50}{\strut how} \colorbox{red!30}{\strut big} \colorbox{red!0}{\strut is} \colorbox{red!100}{\strut uranus} \colorbox{red!100}{\strut uranus} \colorbox{red!6}{\strut gravity} \colorbox{red!100}{\strut uranus} \colorbox{red!6}{\strut weather} \colorbox{red!3}{\strut amazing} \colorbox{red!100}{\strut uranus} \colorbox{red!10}{\strut facts} \colorbox{red!100}{\strut uranus} \colorbox{red!12}{\strut symbol} \colorbox{red!26}{\strut who} \colorbox{red!10}{\strut discovered} \colorbox{red!100}{\strut uranus} \colorbox{red!100}{\strut uranus} \colorbox{red!17}{\strut mythology} \colorbox{red!9}{\strut life} \colorbox{red!2}{\strut on} \colorbox{red!100}{\strut uranus} \colorbox{red!18}{\strut surface} \colorbox{red!9}{\strut features} \colorbox{red!3}{\strut of} \colorbox{red!100}{\strut uranus} \colorbox{red!4}{\strut Nearby} \colorbox{red!4}{\strut Entries} \colorbox{red!6}{\strut uranologist} \colorbox{red!6}{\strut Uranology} \colorbox{red!0}{\strut Uranometria} \colorbox{red!0}{\strut uranometrical} \colorbox{red!0}{\strut Uranometry} \colorbox{red!0}{\strut uranophobia} \colorbox{red!2}{\strut uranoplasty} \colorbox{red!0}{\strut uranorrhaphy} \colorbox{red!0}{\strut uranoschisis} \colorbox{red!0}{\strut uranoscopid} \colorbox{red!0}{\strut uranoscopidae} \colorbox{red!0}{\strut Uranoscopy} \colorbox{red!0}{\strut Uranoso-} \colorbox{red!0}{\strut uranostaphyloplas} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut uranostaphyloschi} \colorbox{red!0}{\strut ...} \colorbox{red!9}{\strut Uranous} \colorbox{red!100}{\strut Uranus} \colorbox{red!2}{\strut Uranyl} \colorbox{red!2}{\strut uranyl} \colorbox{red!0}{\strut acetate} \colorbox{red!2}{\strut uranyl} \colorbox{red!5}{\strut group} \colorbox{red!2}{\strut uranyl} \colorbox{red!2}{\strut nitrate} \colorbox{red!2}{\strut uranyl} \colorbox{red!0}{\strut oxalate} \colorbox{red!2}{\strut uranyl} \colorbox{red!4}{\strut radical} \colorbox{red!0}{\strut uranylic} \colorbox{red!4}{\strut Urao} \colorbox{red!2}{\strut URAQT} \colorbox{red!3}{\strut Urare} \colorbox{red!0}{\strut urarthritis} \colorbox{red!2}{\strut urartian} \colorbox{red!1}{\strut urartu} \colorbox{red!5}{\strut urase} \colorbox{red!6}{\strut urate} \colorbox{red!6}{\strut urate} \colorbox{red!2}{\strut oxidase} \colorbox{red!100}{\strut Uranus} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 8} \colorbox{red!9}{\strut dictionary} \colorbox{red!2}{\strut results} \colorbox{red!100}{\strut Uranus} \colorbox{red!0}{\strut yYr} \colorbox{red!5}{\strut Y} \colorbox{red!0}{\strut nYs} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut yrej-} \colorbox{red!4}{\strut Show} \colorbox{red!23}{\strut Spelled} \colorbox{red!14}{\strut Pronunciation} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut yoo} \colorbox{red!0}{\strut r-uh-nuh} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut yoo-rey-} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Show} \colorbox{red!2}{\strut IPA} \colorbox{red!14}{\strut Pronunciation} \colorbox{red!3}{\strut noun} \colorbox{red!3}{\strut 1} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut Astronomy} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut the} \colorbox{red!25}{\strut planet} \colorbox{red!2}{\strut seventh} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut order} \colorbox{red!2}{\strut from} \colorbox{red!4}{\strut the} \colorbox{red!7}{\strut sun} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut having} \colorbox{red!0}{\strut an} \colorbox{red!5}{\strut equatorial} \colorbox{red!5}{\strut diameter} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut 32,600} \colorbox{red!5}{\strut miles} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 56,460} \colorbox{red!3}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut a} \colorbox{red!30}{\strut mean} \colorbox{red!15}{\strut distance} \colorbox{red!2}{\strut from} \colorbox{red!4}{\strut the} \colorbox{red!7}{\strut sun} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut 1,784} \colorbox{red!5}{\strut million} \colorbox{red!5}{\strut miles} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 2,871} \colorbox{red!5}{\strut million} \colorbox{red!3}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut a} \colorbox{red!5}{\strut period} \colorbox{red!3}{\strut of} \colorbox{red!2}{\strut revolution} \colorbox{red!3}{\strut of} \colorbox{red!0}{\strut 84.07} \colorbox{red!5}{\strut years} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut and} \colorbox{red!0}{\strut 15} \colorbox{red!17}{\strut moons} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Also} \colorbox{red!4}{\strut ,} \colorbox{red!1}{\strut Ouranos} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut Classical} \colorbox{red!17}{\strut Mythology} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut the} \colorbox{red!4}{\strut personification} \colorbox{red!3}{\strut of} \colorbox{red!6}{\strut Heaven} \colorbox{red!3}{\strut and} \colorbox{red!7}{\strut ruler} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!9}{\strut world} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut son} \colorbox{red!3}{\strut and} \colorbox{red!0}{\strut husband} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut Gaea} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut Earth} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut and} \colorbox{red!9}{\strut father} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut Titans} \colorbox{red!4}{\strut ,} \colorbox{red!26}{\strut who} \colorbox{red!5}{\strut was} \colorbox{red!11}{\strut castrated} \colorbox{red!3}{\strut and} \colorbox{red!3}{\strut dethroned} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut his} \colorbox{red!7}{\strut youngest} \colorbox{red!6}{\strut son} \colorbox{red!4}{\strut ,} \colorbox{red!9}{\strut Cronus} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut at} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut instigation} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut Gaea} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Dictionary.com} \colorbox{red!0}{\strut Unabridged} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut v} \colorbox{red!0}{\strut 1.1} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Based} \colorbox{red!2}{\strut on} \colorbox{red!4}{\strut the} \colorbox{red!4}{\strut Random} \colorbox{red!2}{\strut House} \colorbox{red!0}{\strut Unabridged} \colorbox{red!9}{\strut Dictionary} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut Random} \colorbox{red!2}{\strut House} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut 2006} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Cite} \colorbox{red!1}{\strut This} \colorbox{red!9}{\strut Source} \colorbox{red!100}{\strut Uranus} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut yOOr} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Y-nYs} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut yOO-rnYs} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Pronunciation} \colorbox{red!3}{\strut Key} \colorbox{red!0}{\strut n.} \colorbox{red!17}{\strut Greek} \colorbox{red!17}{\strut Mythology} \colorbox{red!4}{\strut The} \colorbox{red!3}{\strut earliest} \colorbox{red!4}{\strut supreme} \colorbox{red!12}{\strut god} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut a} \colorbox{red!4}{\strut personification} \colorbox{red!3}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!7}{\strut sky} \colorbox{red!4}{\strut ,} \colorbox{red!26}{\strut who} 
}}}
\end{CJK*}

101:logos, 81:uranus, 61:fact, 55:planetary, 44:earth, 42:solar, 35:saturn, 31:planets, 30:neptune, 21:body


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!35}{\strut URANUS} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut THE} \colorbox{red!6}{\strut DIAMOND} \colorbox{red!7}{\strut SOUL} \colorbox{red!3}{\strut Thinking} \colorbox{red!1}{\strut about} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut question} \colorbox{red!5}{\strut s} \colorbox{red!2}{\strut the} \colorbox{red!23}{\strut Planetary} \colorbox{red!43}{\strut Logos} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!19}{\strut Earth} \colorbox{red!2}{\strut in} \colorbox{red!26}{\strut fact} \colorbox{red!0}{\strut theLogos} \colorbox{red!2}{\strut of} \colorbox{red!35}{\strut Uranus} \colorbox{red!2}{\strut ?} \colorbox{red!0}{\strut p} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!2}{\strut have} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut following} \colorbox{red!1}{\strut speculations} \colorbox{red!2}{\strut .} \colorbox{red!35}{\strut Uranus} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut Neptune} \colorbox{red!1}{\strut and} \colorbox{red!15}{\strut Saturn} \colorbox{red!2}{\strut are} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut synthesizing} \colorbox{red!13}{\strut planets} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut would} \colorbox{red!2}{\strut have} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut following} \colorbox{red!7}{\strut correspondences} \colorbox{red!35}{\strut Uranus} \colorbox{red!3}{\strut will} \colorbox{red!6}{\strut petals} \colorbox{red!2}{\strut of} \colorbox{red!18}{\strut Solar} \colorbox{red!2}{\strut Egoic} \colorbox{red!3}{\strut Lotus} \colorbox{red!6}{\strut cosmic} \colorbox{red!6}{\strut mental} \colorbox{red!4}{\strut plane} \colorbox{red!1}{\strut higher} \colorbox{red!6}{\strut three} \colorbox{red!0}{\strut planes} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut cosmic} \colorbox{red!8}{\strut physical} \colorbox{red!13}{\strut Neptune} \colorbox{red!1}{\strut love} \colorbox{red!6}{\strut petals} \colorbox{red!0}{\strut ofSolar} \colorbox{red!3}{\strut lotus} \colorbox{red!6}{\strut cosmic} \colorbox{red!3}{\strut astral} \colorbox{red!4}{\strut plane} \colorbox{red!2}{\strut triadal} \colorbox{red!0}{\strut planes} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut cosmic} \colorbox{red!8}{\strut physical} \colorbox{red!15}{\strut Saturn} \colorbox{red!2}{\strut intelligence} \colorbox{red!6}{\strut petals} \colorbox{red!2}{\strut of} \colorbox{red!18}{\strut Solar} \colorbox{red!3}{\strut Lotus} \colorbox{red!6}{\strut cosmic} \colorbox{red!8}{\strut physical} \colorbox{red!4}{\strut plane} \colorbox{red!1}{\strut lower} \colorbox{red!6}{\strut three} \colorbox{red!0}{\strut planes} \colorbox{red!2}{\strut of} \colorbox{red!6}{\strut cosmic} \colorbox{red!8}{\strut physical} \colorbox{red!1}{\strut As} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut synthesizers} \colorbox{red!0}{\strut they} \colorbox{red!2}{\strut would} \colorbox{red!1}{\strut be} \colorbox{red!3}{\strut related} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut three} \colorbox{red!3}{\strut levels} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut our} \colorbox{red!23}{\strut Planetary} \colorbox{red!43}{\strut Logos} \colorbox{red!35}{\strut Uranus} \colorbox{red!23}{\strut Planetary} \colorbox{red!7}{\strut Spirit} \colorbox{red!13}{\strut Neptune} \colorbox{red!7}{\strut Nameless} \colorbox{red!2}{\strut One} \colorbox{red!15}{\strut Saturn} \colorbox{red!6}{\strut Sanat} \colorbox{red!1}{\strut Kumara} \colorbox{red!1}{\strut Lets} \colorbox{red!1}{\strut suppose} \colorbox{red!3}{\strut we} \colorbox{red!3}{\strut ask} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut following} \colorbox{red!0}{\strut questions} \colorbox{red!1}{\strut as} \colorbox{red!3}{\strut a} \colorbox{red!4}{\strut thought} \colorbox{red!2}{\strut experiment} \colorbox{red!3}{\strut a} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut Is} \colorbox{red!2}{\strut the} \colorbox{red!23}{\strut planetary} \colorbox{red!43}{\strut logos} \colorbox{red!2}{\strut in} \colorbox{red!26}{\strut fact} \colorbox{red!15}{\strut Saturn} \colorbox{red!2}{\strut ?} \colorbox{red!3}{\strut Answer} \colorbox{red!2}{\strut Yes} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut extent} \colorbox{red!3}{\strut we} \colorbox{red!2}{\strut are} \colorbox{red!4}{\strut contacting} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut relating} \colorbox{red!1}{\strut through} \colorbox{red!6}{\strut Sanat} \colorbox{red!1}{\strut Kumara} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut synthesizing} \colorbox{red!5}{\strut energy} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut cosmic} \colorbox{red!8}{\strut physical} \colorbox{red!4}{\strut plane} \colorbox{red!3}{\strut b} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut Is} \colorbox{red!2}{\strut the} \colorbox{red!23}{\strut planetary} \colorbox{red!43}{\strut logos} \colorbox{red!2}{\strut in} \colorbox{red!26}{\strut fact} \colorbox{red!13}{\strut Neptune} \colorbox{red!2}{\strut ?} \colorbox{red!3}{\strut Answer} \colorbox{red!2}{\strut Yes} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut extent} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut we} \colorbox{red!2}{\strut are} \colorbox{red!4}{\strut contacting} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut relating} \colorbox{red!1}{\strut through} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut Nameless} \colorbox{red!2}{\strut One} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut synthesizing} \colorbox{red!5}{\strut energy} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut cosmic} \colorbox{red!3}{\strut astral} \colorbox{red!4}{\strut plane} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut c} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut Is} \colorbox{red!2}{\strut the} \colorbox{red!23}{\strut planetary} \colorbox{red!43}{\strut logos} \colorbox{red!2}{\strut in} \colorbox{red!26}{\strut fact} \colorbox{red!35}{\strut Uranus} \colorbox{red!2}{\strut ?} \colorbox{red!3}{\strut Answer} \colorbox{red!2}{\strut Yes} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut extent} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut we} \colorbox{red!2}{\strut are} \colorbox{red!4}{\strut contacting} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut relating} \colorbox{red!1}{\strut through} \colorbox{red!2}{\strut the} \colorbox{red!23}{\strut Planetary} \colorbox{red!7}{\strut Spirit} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut synthesizing} \colorbox{red!5}{\strut energy} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut cosmic} \colorbox{red!6}{\strut mental} \colorbox{red!4}{\strut plane} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut These} \colorbox{red!0}{\strut questions} \colorbox{red!1}{\strut perhaps} \colorbox{red!1}{\strut reveal} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut about} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut stage} \colorbox{red!2}{\strut reached} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut questioning} \colorbox{red!5}{\strut consciousness} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut do} \colorbox{red!1}{\strut about} \colorbox{red!0}{\strut any} \colorbox{red!3}{\strut fixed} \colorbox{red!2}{\strut underlying} \colorbox{red!6}{\strut reality} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut beg} \colorbox{red!2}{\strut one} \colorbox{red!2}{\strut final} \colorbox{red!2}{\strut question} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut d} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut Is} \colorbox{red!2}{\strut the} \colorbox{red!23}{\strut Planetary} \colorbox{red!43}{\strut Logos} \colorbox{red!2}{\strut in} \colorbox{red!26}{\strut fact} \colorbox{red!2}{\strut the} \colorbox{red!18}{\strut Solar} \colorbox{red!43}{\strut Logos} \colorbox{red!2}{\strut ?} \colorbox{red!3}{\strut Answer} \colorbox{red!2}{\strut Yes} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut extent} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut He} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut an} \colorbox{red!3}{\strut expression} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!18}{\strut Solar} \colorbox{red!3}{\strut Will} \colorbox{red!2}{\strut in} \colorbox{red!1}{\strut full} \colorbox{red!3}{\strut manifestation} \colorbox{red!2}{\strut The} \colorbox{red!0}{\strut correspondence} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut these} \colorbox{red!0}{\strut questions} \colorbox{red!2}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut human} \colorbox{red!2}{\strut arena} \colorbox{red!2}{\strut would} \colorbox{red!1}{\strut be} \colorbox{red!0}{\strut Am} \colorbox{red!1}{\strut I} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut body} \colorbox{red!2}{\strut ?} 
}}}
\end{CJK*}

query: vines shade

94:zones, 88:shade, 49:flower, 35:size, 27:common, 26:plant, 25:name, 24:scarified, 23:scientific, 22:seeds


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!22}{\strut Common} \colorbox{red!20}{\strut name} \colorbox{red!18}{\strut Scientific} \colorbox{red!20}{\strut name} \colorbox{red!77}{\strut Zones} \colorbox{red!40}{\strut Flower} \colorbox{red!28}{\strut Size} \colorbox{red!7}{\strut Exposure} \colorbox{red!2}{\strut Comments} \colorbox{red!13}{\strut Canary} \colorbox{red!9}{\strut bird} \colorbox{red!10}{\strut vine} \colorbox{red!2}{\strut .} \colorbox{red!13}{\strut Canary} \colorbox{red!9}{\strut creeper} \colorbox{red!5}{\strut Tropaeolum} \colorbox{red!4}{\strut peregrium} \colorbox{red!13}{\strut Annual} \colorbox{red!14}{\strut Yellow} \colorbox{red!2}{\strut 8} \colorbox{red!2}{\strut to} \colorbox{red!4}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!3}{\strut Edible} \colorbox{red!0}{\strut flowers} \colorbox{red!6}{\strut produced} \colorbox{red!2}{\strut from} \colorbox{red!1}{\strut July} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut frost} \colorbox{red!6}{\strut Cape} \colorbox{red!10}{\strut honeysuckle} \colorbox{red!3}{\strut Tecomaria} \colorbox{red!4}{\strut capensis} \colorbox{red!0}{\strut 8-9} \colorbox{red!0}{\strut Orange-scarlet} \colorbox{red!3}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!2}{\strut Quasiclimber} \colorbox{red!2}{\strut .} \colorbox{red!8}{\strut tolerant} \colorbox{red!3}{\strut of} \colorbox{red!6}{\strut heat} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut drought} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut coastal} \colorbox{red!5}{\strut conditions} \colorbox{red!6}{\strut Cardinal} \colorbox{red!3}{\strut climber} \colorbox{red!4}{\strut Ipomoea} \colorbox{red!2}{\strut x} \colorbox{red!3}{\strut multifida} \colorbox{red!13}{\strut Annual} \colorbox{red!10}{\strut Red} \colorbox{red!4}{\strut 10} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!18}{\strut Seeds} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!19}{\strut scarified} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut soaked} \colorbox{red!0}{\strut in} \colorbox{red!13}{\strut water} \colorbox{red!2}{\strut for} \colorbox{red!1}{\strut 12} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut 24} \colorbox{red!4}{\strut hours} \colorbox{red!2}{\strut to} \colorbox{red!7}{\strut aid} \colorbox{red!14}{\strut germination} \colorbox{red!2}{\strut Carolina} \colorbox{red!5}{\strut jasmine} \colorbox{red!0}{\strut Gelsemium} \colorbox{red!5}{\strut sempervirens} \colorbox{red!0}{\strut 7-9} \colorbox{red!14}{\strut Yellow} \colorbox{red!4}{\strut 10} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!14}{\strut Yellow} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut spring} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut native} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut foliage} \colorbox{red!2}{\strut bronzes} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut winter} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!4}{\strut parts} \colorbox{red!3}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!21}{\strut plant} \colorbox{red!2}{\strut are} \colorbox{red!2}{\strut toxic} \colorbox{red!2}{\strut Chilean} \colorbox{red!17}{\strut glory} \colorbox{red!40}{\strut flower} \colorbox{red!2}{\strut .} \colorbox{red!17}{\strut Glory} \colorbox{red!10}{\strut vine} \colorbox{red!0}{\strut Eccremocarpus} \colorbox{red!8}{\strut scaber} \colorbox{red!13}{\strut Annual} \colorbox{red!14}{\strut Yellow} \colorbox{red!1}{\strut ,} \colorbox{red!10}{\strut red} \colorbox{red!4}{\strut 10} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut 12} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!4}{\strut Start} \colorbox{red!2}{\strut from} \colorbox{red!18}{\strut seeds} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!3}{\strut transplant} \colorbox{red!0}{\strut well} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut thrives} \colorbox{red!1}{\strut on} \colorbox{red!6}{\strut heat} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut tubular} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut all} \colorbox{red!7}{\strut summer} \colorbox{red!1}{\strut Cross} \colorbox{red!10}{\strut vine} \colorbox{red!0}{\strut Bignonia} \colorbox{red!4}{\strut capreolata} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Anisostichus} \colorbox{red!4}{\strut capreolata} \colorbox{red!0}{\strut 6-9} \colorbox{red!0}{\strut Orange-red} \colorbox{red!0}{\strut 30} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!4}{\strut Evergreen} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut semi-evergreen} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut native} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut mid-spring} \colorbox{red!2}{\strut .} \colorbox{red!14}{\strut leaves} \colorbox{red!9}{\strut take} \colorbox{red!1}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut purplish} \colorbox{red!16}{\strut color} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut winter} \colorbox{red!4}{\strut Cypress} \colorbox{red!10}{\strut vine} \colorbox{red!4}{\strut Ipomoea} \colorbox{red!3}{\strut quamoclit} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Quamoclit} \colorbox{red!3}{\strut pennata} \colorbox{red!13}{\strut Annual} \colorbox{red!10}{\strut Red} \colorbox{red!4}{\strut 10} \colorbox{red!2}{\strut to} \colorbox{red!1}{\strut 15} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!18}{\strut Seeds} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!19}{\strut scarified} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut soaked} \colorbox{red!0}{\strut in} \colorbox{red!13}{\strut water} \colorbox{red!2}{\strut for} \colorbox{red!1}{\strut 12} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut 24} \colorbox{red!4}{\strut hours} \colorbox{red!2}{\strut to} \colorbox{red!7}{\strut aid} \colorbox{red!14}{\strut germination} \colorbox{red!3}{\strut Firecracker} \colorbox{red!10}{\strut vine} \colorbox{red!2}{\strut .} \colorbox{red!8}{\strut Spanish} \colorbox{red!4}{\strut flag} \colorbox{red!3}{\strut Mina} \colorbox{red!4}{\strut lobata} \colorbox{red!13}{\strut Annual} \colorbox{red!0}{\strut Reddish-orange} \colorbox{red!9}{\strut fading} \colorbox{red!2}{\strut to} \colorbox{red!13}{\strut orange} \colorbox{red!1}{\strut ,} \colorbox{red!14}{\strut yellow} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut white} \colorbox{red!4}{\strut 10} \colorbox{red!2}{\strut to} \colorbox{red!3}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!18}{\strut Seeds} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!19}{\strut scarified} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut soaked} \colorbox{red!0}{\strut in} \colorbox{red!13}{\strut water} \colorbox{red!2}{\strut for} \colorbox{red!1}{\strut 12} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut 24} \colorbox{red!4}{\strut hours} \colorbox{red!2}{\strut to} \colorbox{red!7}{\strut aid} \colorbox{red!14}{\strut germination} \colorbox{red!10}{\strut Honeysuckle} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut Coral} \colorbox{red!5}{\strut Lonicera} \colorbox{red!5}{\strut sempervirens} \colorbox{red!0}{\strut 5-9} \colorbox{red!4}{\strut Coral} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut red} \colorbox{red!1}{\strut ,} \colorbox{red!14}{\strut yellow} \colorbox{red!1}{\strut 15} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Sun} \colorbox{red!2}{\strut to} \colorbox{red!10}{\strut partial} \colorbox{red!72}{\strut shade} \colorbox{red!0}{\strut Trumpet-shaped} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut mid-spring} \colorbox{red!2}{\strut to} \colorbox{red!2}{\strut fall} \colorbox{red!2}{\strut .} \colorbox{red!9}{\strut native} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut cultivars} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Sulfurea} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut yellow} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut Superba} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Magnifica} 
}}}
\end{CJK*}

98:shade, 71:what, 56:vine, 55:plants, 47:good, 30:grow, 27:nature, 24:hydrangea, 23:which, 23:climbing


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 19} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Subscribe} \colorbox{red!0}{\strut Today} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut Text} \colorbox{red!1}{\strut size} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Q} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut A} \colorbox{red!1}{\strut .} \colorbox{red!26}{\strut What} \colorbox{red!2}{\strut is} \colorbox{red!4}{\strut a} \colorbox{red!17}{\strut good} \colorbox{red!20}{\strut vine} \colorbox{red!2}{\strut for} \colorbox{red!36}{\strut shade} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut BY} \colorbox{red!0}{\strut KATHY} \colorbox{red!1}{\strut VAN} \colorbox{red!2}{\strut MULLEKOM} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 757-247-4781} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 24} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut 2007} \colorbox{red!1}{\strut NEWPORT} \colorbox{red!1}{\strut NEWS} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Q.} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut really} \colorbox{red!0}{\strut enjoyed} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut talk} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Ford} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Colony} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut morning} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut practical} \colorbox{red!1}{\strut advice} \colorbox{red!1}{\strut on} \colorbox{red!1}{\strut low} \colorbox{red!0}{\strut maintenance} \colorbox{red!20}{\strut plants} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut great} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut My} \colorbox{red!4}{\strut poet} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut laurel} \colorbox{red!0}{\strut finally} \colorbox{red!0}{\strut got} \colorbox{red!3}{\strut named} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut wondering} \colorbox{red!26}{\strut what} \colorbox{red!1}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut inherited} \colorbox{red!4}{\strut a} \colorbox{red!4}{\strut garden} \colorbox{red!1}{\strut two} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ago} \colorbox{red!3}{\strut when} \colorbox{red!1}{\strut we} \colorbox{red!1}{\strut moved} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut also} \colorbox{red!4}{\strut a} \colorbox{red!0}{\strut shed} \colorbox{red!0}{\strut full} \colorbox{red!1}{\strut of} \colorbox{red!4}{\strut pesticides} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!1}{\strut want} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut am} \colorbox{red!3}{\strut experimenting} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut see} \colorbox{red!26}{\strut what} \colorbox{red!1}{\strut will} \colorbox{red!2}{\strut survive} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Periwinkle} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut yarrow} \colorbox{red!1}{\strut take} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut huge} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut lily-of-the-valley} \colorbox{red!0}{\strut get} \colorbox{red!2}{\strut eaten} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut thought} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut were} \colorbox{red!6}{\strut poisonous} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut glad} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut hear} \colorbox{red!2}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ca} \colorbox{red!0}{\strut nt} \colorbox{red!11}{\strut grow} \colorbox{red!5}{\strut daphne} \colorbox{red!0}{\strut either} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut killed} \colorbox{red!1}{\strut two} \colorbox{red!3}{\strut pretty} \colorbox{red!1}{\strut ones} \colorbox{red!1}{\strut and} \colorbox{red!5}{\strut Daphne} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut really} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut middle} \colorbox{red!0}{\strut name} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut We} \colorbox{red!0}{\strut have} \colorbox{red!4}{\strut a} \colorbox{red!4}{\strut trellis} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!36}{\strut shade} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut question} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut recommend} \colorbox{red!4}{\strut a} \colorbox{red!20}{\strut vine} \colorbox{red!2}{\strut that} \colorbox{red!7}{\strut likes} \colorbox{red!36}{\strut shade} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Thank} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Hazel} \colorbox{red!5}{\strut Daphne} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut e-mail} \colorbox{red!0}{\strut A.} \colorbox{red!5}{\strut Hazel} \colorbox{red!4}{\strut ,} \colorbox{red!8}{\strut climbing} \colorbox{red!8}{\strut hydrangea} \colorbox{red!7}{\strut likes} \colorbox{red!36}{\strut shade} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut look} \colorbox{red!2}{\strut for} \colorbox{red!4}{\strut Moonlight} \colorbox{red!8}{\strut which} \colorbox{red!1}{\strut has} \colorbox{red!1}{\strut few} \colorbox{red!7}{\strut flowers} \colorbox{red!0}{\strut but} \colorbox{red!1}{\strut great} \colorbox{red!0}{\strut silvery} \colorbox{red!2}{\strut foliage} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Autumn} \colorbox{red!3}{\strut clematis} \colorbox{red!2}{\strut is} \colorbox{red!4}{\strut a} \colorbox{red!1}{\strut wonderful} \colorbox{red!0}{\strut one} \colorbox{red!2}{\strut that} \colorbox{red!5}{\strut blooms} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut late} \colorbox{red!1}{\strut summer} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Our} \colorbox{red!1}{\strut native} \colorbox{red!3}{\strut Virginia} \colorbox{red!4}{\strut creeper} \colorbox{red!2}{\strut is} \colorbox{red!1}{\strut also} \colorbox{red!3}{\strut nice} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!2}{\strut vigorous} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut needs} \colorbox{red!4}{\strut a} \colorbox{red!1}{\strut strong} \colorbox{red!4}{\strut trellis} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Fatshedra} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut nice} \colorbox{red!4}{\strut ,} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!2}{\strut grown} \colorbox{red!1}{\strut it} \colorbox{red!4}{\strut ,} \colorbox{red!1}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut a} \colorbox{red!5}{\strut bush} \colorbox{red!7}{\strut ivy} \colorbox{red!2}{\strut that} \colorbox{red!2}{\strut needs} \colorbox{red!2}{\strut help} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut climb} \colorbox{red!4}{\strut ,} \colorbox{red!2}{\strut ties} \colorbox{red!2}{\strut are} \colorbox{red!17}{\strut good} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut My} \colorbox{red!1}{\strut vote} \colorbox{red!1}{\strut would} \colorbox{red!1}{\strut be} \colorbox{red!4}{\strut Moonlight} \colorbox{red!8}{\strut hydrangea} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut m} \colorbox{red!1}{\strut so} \colorbox{red!1}{\strut happy} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut are} \colorbox{red!0}{\strut gardening} \colorbox{red!0}{\strut without} \colorbox{red!4}{\strut pesticides} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!4}{\strut found} \colorbox{red!4}{\strut having} \colorbox{red!4}{\strut a} \colorbox{red!3}{\strut variety} \colorbox{red!1}{\strut of} \colorbox{red!20}{\strut plants} \colorbox{red!2}{\strut attracts} \colorbox{red!2}{\strut beneficial} \colorbox{red!20}{\strut plants} \colorbox{red!1}{\strut so} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut seldom} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut plant} \colorbox{red!0}{\strut problems} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Take} \colorbox{red!1}{\strut care} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Kathy} \colorbox{red!1}{\strut Want} \colorbox{red!1}{\strut more} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Get} \colorbox{red!1}{\strut home} 
}}}
\end{CJK*}

query: university phoenix

100:university, 99:phoenix, 73:campuses, 65:campus, 50:what, 41:locations, 34:how, 27:online, 17:when, 17:programs


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!17}{\strut Programs} \colorbox{red!0}{\strut .} \colorbox{red!35}{\strut How} \colorbox{red!0}{\strut it} \colorbox{red!4}{\strut Works} \colorbox{red!0}{\strut .} \colorbox{red!17}{\strut Financial} \colorbox{red!6}{\strut Options} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Accreditation} \colorbox{red!0}{\strut .} \colorbox{red!68}{\strut Campus} \colorbox{red!43}{\strut Locations} \colorbox{red!17}{\strut PROGRAMS} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Associate} \colorbox{red!10}{\strut Degrees} \colorbox{red!0}{\strut Bachelors} \colorbox{red!10}{\strut Degrees} \colorbox{red!0}{\strut Masters} \colorbox{red!10}{\strut Degrees} \colorbox{red!0}{\strut Accounting} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut Degree} \colorbox{red!3}{\strut Communications} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut Criminal} \colorbox{red!0}{\strut Justice} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut E-Business} \colorbox{red!0}{\strut Degree} \colorbox{red!6}{\strut Education} \colorbox{red!0}{\strut Degree} \colorbox{red!11}{\strut Finance} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut IT} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut Marketing} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut MBA} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut Nursing} \colorbox{red!0}{\strut Degree} \colorbox{red!3}{\strut Technology} \colorbox{red!0}{\strut Degree} \colorbox{red!35}{\strut How} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut is} \colorbox{red!12}{\strut tuition} \colorbox{red!0}{\strut ?} \colorbox{red!17}{\strut When} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut classes} \colorbox{red!2}{\strut starting} \colorbox{red!0}{\strut ?} \colorbox{red!52}{\strut What} \colorbox{red!0}{\strut about} \colorbox{red!17}{\strut financial} \colorbox{red!0}{\strut aid} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut Enter} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut ZipPostal} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut .} \colorbox{red!28}{\strut Online} \colorbox{red!0}{\strut Degree} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!0}{\strut .} \colorbox{red!68}{\strut Campus} \colorbox{red!43}{\strut Locations} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!68}{\strut Campus} \colorbox{red!43}{\strut Locations} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 190} \colorbox{red!77}{\strut campuses} \colorbox{red!0}{\strut and} \colorbox{red!9}{\strut learning} \colorbox{red!16}{\strut centers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 38} \colorbox{red!12}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Puerto} \colorbox{red!2}{\strut Rico} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Alberta} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut British} \colorbox{red!0}{\strut Columbia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Canada} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut Netherlands} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!28}{\strut Online} \colorbox{red!0}{\strut ,} \colorbox{red!77}{\strut Campuses} \colorbox{red!0}{\strut and} \colorbox{red!68}{\strut Campus} \colorbox{red!43}{\strut Locations} \colorbox{red!5}{\strut As} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut list} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut ,} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!28}{\strut Online} \colorbox{red!0}{\strut ,} \colorbox{red!77}{\strut Campuses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!68}{\strut Campus} \colorbox{red!0}{\strut Location} \colorbox{red!6}{\strut options} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut encourage} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut explore} \colorbox{red!0}{\strut all} \colorbox{red!2}{\strut the} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!28}{\strut Online} \colorbox{red!0}{\strut ,} \colorbox{red!77}{\strut Campuses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!68}{\strut Campus} \colorbox{red!0}{\strut Location} \colorbox{red!6}{\strut options} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut choose} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut learning} \colorbox{red!6}{\strut format} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!5}{\strut right} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!28}{\strut Online} \colorbox{red!0}{\strut and} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!28}{\strut Online} \colorbox{red!68}{\strut Campus} \colorbox{red!6}{\strut options} \colorbox{red!0}{\strut such} \colorbox{red!5}{\strut as} \colorbox{red!0}{\strut FLEXNET} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut advance} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut need} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut determining} \colorbox{red!2}{\strut the} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!28}{\strut Online} \colorbox{red!0}{\strut ,} \colorbox{red!77}{\strut Campuses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!68}{\strut Campus} \colorbox{red!0}{\strut Location} \colorbox{red!0}{\strut option} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!5}{\strut right} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut connect} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut an} \colorbox{red!10}{\strut enrollment} \colorbox{red!0}{\strut advisor} \colorbox{red!2}{\strut today} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut UNITED} \colorbox{red!12}{\strut STATES} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!8}{\strut Alabama} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!0}{\strut Alaska} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!9}{\strut Arizona} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!3}{\strut Tucson} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!100}{\strut Phoenix} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!7}{\strut Arkansas} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!0}{\strut Little} \colorbox{red!4}{\strut Rock} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!3}{\strut Northwest} \colorbox{red!7}{\strut Arkansas} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!11}{\strut California} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!0}{\strut Sacramento} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!4}{\strut Central} \colorbox{red!3}{\strut Valley} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!4}{\strut Bay} \colorbox{red!5}{\strut Area} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!4}{\strut San} \colorbox{red!2}{\strut Diego} \colorbox{red!68}{\strut Campus} \colorbox{red!100}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!100}{\strut Phoenix} \colorbox{red!4}{\strut Southern} 
}}}
\end{CJK*}

99:phoenix, 97:university, 40:campus, 34:locations, 33:arkansas, 29:rogers, 23:northwest, 21:college, 17:classes, 14:county


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!67}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!68}{\strut Phoenix} \colorbox{red!8}{\strut Axia} \colorbox{red!14}{\strut College} \colorbox{red!0}{\strut 866.766.0766} \colorbox{red!0}{\strut Colleges} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Divisions} \colorbox{red!8}{\strut Axia} \colorbox{red!14}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!67}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!68}{\strut Phoenix} \colorbox{red!14}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Arts} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut Sciences} \colorbox{red!0}{\strut Colleges} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Business} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut Management} \colorbox{red!14}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Education} \colorbox{red!14}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Health} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut Human} \colorbox{red!0}{\strut Services} \colorbox{red!14}{\strut College} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Information} \colorbox{red!0}{\strut Systems} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut Technology} \colorbox{red!3}{\strut Military} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Domestic} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut School} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Advanced} \colorbox{red!2}{\strut Studies} \colorbox{red!2}{\strut Online} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut Campus} \colorbox{red!9}{\strut Programs} \colorbox{red!6}{\strut Degree} \colorbox{red!9}{\strut Programs} \colorbox{red!0}{\strut Certificate} \colorbox{red!9}{\strut Programs} \colorbox{red!0}{\strut Continuing} \colorbox{red!1}{\strut Teacher} \colorbox{red!5}{\strut Education} \colorbox{red!0}{\strut Individual} \colorbox{red!6}{\strut Courses} \colorbox{red!1}{\strut Professional} \colorbox{red!0}{\strut Development} \colorbox{red!6}{\strut Courses} \colorbox{red!4}{\strut Tuition} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Financial} \colorbox{red!1}{\strut Options} \colorbox{red!2}{\strut Financial} \colorbox{red!1}{\strut Options} \colorbox{red!2}{\strut Financial} \colorbox{red!2}{\strut Information} \colorbox{red!0}{\strut Scholarships} \colorbox{red!0}{\strut Policies} \colorbox{red!6}{\strut Student} \colorbox{red!0}{\strut Loan} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Conduct} \colorbox{red!0}{\strut Apply} \colorbox{red!2}{\strut Online} \colorbox{red!2}{\strut Admissions} \colorbox{red!0}{\strut Admission} \colorbox{red!1}{\strut Requirements} \colorbox{red!6}{\strut Student} \colorbox{red!0}{\strut Experience} \colorbox{red!0}{\strut Transfer} \colorbox{red!2}{\strut Information} \colorbox{red!0}{\strut Prior} \colorbox{red!3}{\strut Learning} \colorbox{red!0}{\strut Assessment} \colorbox{red!27}{\strut Campus} \colorbox{red!23}{\strut Locations} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut Students} \colorbox{red!2}{\strut Alumni} \colorbox{red!0}{\strut Faculty} \colorbox{red!2}{\strut Online} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut About} \colorbox{red!67}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!68}{\strut Phoenix} \colorbox{red!2}{\strut Mission} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut Purposes} \colorbox{red!4}{\strut Accreditation} \colorbox{red!0}{\strut Green} \colorbox{red!0}{\strut Initiative} \colorbox{red!67}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!68}{\strut Phoenix} \colorbox{red!0}{\strut Foundation} \colorbox{red!0}{\strut Publications} \colorbox{red!27}{\strut Campus} \colorbox{red!0}{\strut Safety} \colorbox{red!0}{\strut Regulatory} \colorbox{red!1}{\strut Employment} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!6}{\strut Degree} \colorbox{red!9}{\strut Programs} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Associate} \colorbox{red!2}{\strut Arts} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut Sciences} \colorbox{red!6}{\strut Business} \colorbox{red!2}{\strut Management} \colorbox{red!0}{\strut Criminal} \colorbox{red!0}{\strut Justice} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut Security} \colorbox{red!5}{\strut Education} \colorbox{red!0}{\strut Human} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut Nursing} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut Health} \colorbox{red!0}{\strut Care} \colorbox{red!3}{\strut Psychology} \colorbox{red!0}{\strut Technology} \colorbox{red!2}{\strut Undergraduate} \colorbox{red!2}{\strut Graduate} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut Del.icio.us} \colorbox{red!0}{\strut Digg} \colorbox{red!0}{\strut Facebook} \colorbox{red!0}{\strut MySpace} \colorbox{red!0}{\strut Reddit} \colorbox{red!0}{\strut StumbleUpon} \colorbox{red!0}{\strut Bookmark} \colorbox{red!4}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut Campus} \colorbox{red!23}{\strut Locations} \colorbox{red!2}{\strut Welcome} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!15}{\strut Northwest} \colorbox{red!22}{\strut Arkansas} \colorbox{red!27}{\strut Campus} \colorbox{red!15}{\strut Northwest} \colorbox{red!22}{\strut Arkansas} \colorbox{red!27}{\strut Campus} \colorbox{red!0}{\strut 903} \colorbox{red!0}{\strut N.} \colorbox{red!0}{\strut 47th} \colorbox{red!0}{\strut Street} \colorbox{red!0}{\strut Suite} \colorbox{red!0}{\strut 400} \colorbox{red!20}{\strut Rogers} \colorbox{red!3}{\strut ,} \colorbox{red!22}{\strut Arkansas} \colorbox{red!0}{\strut 72756} \colorbox{red!4}{\strut Phone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 479.986.0385} \colorbox{red!0}{\strut Local} \colorbox{red!67}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!68}{\strut Phoenix} \colorbox{red!0}{\strut in} \colorbox{red!20}{\strut Rogers} \colorbox{red!3}{\strut ,} \colorbox{red!22}{\strut Arkansas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!15}{\strut Northwest} \colorbox{red!22}{\strut Arkansas} \colorbox{red!27}{\strut Campus} \colorbox{red!0}{\strut The} \colorbox{red!67}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!68}{\strut Phoenix} \colorbox{red!15}{\strut Northwest} \colorbox{red!22}{\strut Arkansas} \colorbox{red!27}{\strut Campus} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut located} \colorbox{red!0}{\strut in} \colorbox{red!20}{\strut Rogers} \colorbox{red!3}{\strut ,} \colorbox{red!22}{\strut Arkansas} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Located} \colorbox{red!3}{\strut near} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Highway} \colorbox{red!0}{\strut 62} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut Interstate} \colorbox{red!0}{\strut 540} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut NW} \colorbox{red!22}{\strut Arkansas} \colorbox{red!27}{\strut Campus} \colorbox{red!2}{\strut is} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut driving} \colorbox{red!4}{\strut distance} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Fayetteville} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut Bentonville} \colorbox{red!3}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Benton} \colorbox{red!9}{\strut County} \colorbox{red!3}{\strut ,} \colorbox{red!22}{\strut Arkansas} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Our} \colorbox{red!2}{\strut convenient} \colorbox{red!0}{\strut location} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut scheduling} \colorbox{red!0}{\strut enable} \colorbox{red!2}{\strut working} \colorbox{red!0}{\strut adults} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut earn} \colorbox{red!0}{\strut their} \colorbox{red!14}{\strut college} \colorbox{red!6}{\strut degree} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut giving} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut commitments} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut work} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut home} \colorbox{red!2}{\strut .} \colorbox{red!15}{\strut Northwest} \colorbox{red!22}{\strut Arkansas} \colorbox{red!0}{\strut Campus-Options} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Flexible} \colorbox{red!3}{\strut Learning} \colorbox{red!0}{\strut The} \colorbox{red!15}{\strut Northwest} \colorbox{red!22}{\strut Arkansas} \colorbox{red!27}{\strut Campus} \colorbox{red!4}{\strut offers} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut bachelor} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut master} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut options} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut on-campus} \colorbox{red!0}{\strut students} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Students} \colorbox{red!3}{\strut learning} \colorbox{red!0}{\strut on-campus} \colorbox{red!8}{\strut attend} \colorbox{red!11}{\strut classes} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut week} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut evening} \colorbox{red!2}{\strut .} \colorbox{red!6}{\strut Courses} 
}}}
\end{CJK*}

query: septic system design

35:types, 29:septic, 28:apedia, 27:systems, 21:water, 19:tank, 16:building, 16:air, 15:testing, 14:roofing


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut InspectAPedia} \colorbox{red!21}{\strut Building} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut Environmental} \colorbox{red!11}{\strut Inspection} \colorbox{red!7}{\strut ,} \colorbox{red!19}{\strut Testing} \colorbox{red!7}{\strut ,} \colorbox{red!0}{\strut Diagnosis} \colorbox{red!7}{\strut ,} \colorbox{red!13}{\strut Repair} \colorbox{red!7}{\strut ,} \colorbox{red!5}{\strut .} \colorbox{red!7}{\strut Problem} \colorbox{red!0}{\strut Prevention} \colorbox{red!0}{\strut Advice} \colorbox{red!0}{\strut InspectAPedia} \colorbox{red!17}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!21}{\strut Air} \colorbox{red!14}{\strut Conditioning} \colorbox{red!0}{\strut .} \colorbox{red!17}{\strut Electrical} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Environment} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Exteriors} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Heating} \colorbox{red!0}{\strut .} \colorbox{red!17}{\strut Home} \colorbox{red!11}{\strut Inspection} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Insulate} \colorbox{red!11}{\strut Ventilate} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Interiors} \colorbox{red!0}{\strut .} \colorbox{red!13}{\strut Mold} \colorbox{red!0}{\strut InspectTest} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Plumbing} \colorbox{red!27}{\strut Water} \colorbox{red!38}{\strut Septic} \colorbox{red!0}{\strut .} \colorbox{red!18}{\strut Roofing} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Structure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut Directory} \colorbox{red!7}{\strut of} \colorbox{red!0}{\strut Professionals} \colorbox{red!2}{\strut to} \colorbox{red!0}{\strut Inspect} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Test} \colorbox{red!0}{\strut a} \colorbox{red!21}{\strut Building} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!17}{\strut HOME} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!0}{\strut INFO} \colorbox{red!0}{\strut ARTICLES} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut for} \colorbox{red!17}{\strut Home} \colorbox{red!0}{\strut Buyers} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut Owners} \colorbox{red!38}{\strut Septic} \colorbox{red!0}{\strut System} \colorbox{red!18}{\strut Design} \colorbox{red!38}{\strut Septic} \colorbox{red!11}{\strut Inspection} \colorbox{red!19}{\strut Testing} \colorbox{red!38}{\strut Septic} \colorbox{red!5}{\strut Maintenance} \colorbox{red!13}{\strut Repair} \colorbox{red!38}{\strut Septic} \colorbox{red!7}{\strut Component} \colorbox{red!5}{\strut .} \colorbox{red!10}{\strut Product} \colorbox{red!3}{\strut Suppliers} \colorbox{red!38}{\strut Septic} \colorbox{red!3}{\strut Videos} \colorbox{red!17}{\strut HOME} \colorbox{red!0}{\strut BUYERS} \colorbox{red!0}{\strut GUIDE} \colorbox{red!2}{\strut to} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!0}{\strut ONLINE} \colorbox{red!0}{\strut BOOK} \colorbox{red!0}{\strut INTRODUCTION} \colorbox{red!0}{\strut SAFETY} \colorbox{red!1}{\strut WARNINGS} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!0}{\strut SYSTEM} \colorbox{red!18}{\strut DESIGN} \colorbox{red!0}{\strut BASICS} \colorbox{red!10}{\strut PERC} \colorbox{red!0}{\strut TESTS} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!25}{\strut TANK} \colorbox{red!13}{\strut SIZE} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!25}{\strut TANK} \colorbox{red!10}{\strut DEPTH} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!25}{\strut TANK} \colorbox{red!3}{\strut TEES} \colorbox{red!3}{\strut FIELD} \colorbox{red!13}{\strut SIZE} \colorbox{red!3}{\strut FIELD} \colorbox{red!10}{\strut SHAPE} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!9}{\strut CLEARANCES} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!25}{\strut TANK} \colorbox{red!9}{\strut PUMPING} \colorbox{red!7}{\strut FREQUENCY} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!25}{\strut TANK} \colorbox{red!9}{\strut PUMPING} \colorbox{red!10}{\strut PROCEDURE} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!9}{\strut PUMPING} \colorbox{red!13}{\strut REPAIR} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!13}{\strut TREATMENTS} \colorbox{red!6}{\strut STEEP} \colorbox{red!2}{\strut SLOPE} \colorbox{red!0}{\strut DESIGNS} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!18}{\strut DESIGN} \colorbox{red!9}{\strut ALTERNATIVES} \colorbox{red!14}{\strut Wastewater} \colorbox{red!0}{\strut Treatment} \colorbox{red!7}{\strut Levels} \colorbox{red!14}{\strut Wastewater} \colorbox{red!5}{\strut Dispersal} \colorbox{red!13}{\strut Methods} \colorbox{red!10}{\strut Master} \colorbox{red!10}{\strut List} \colorbox{red!7}{\strut of} \colorbox{red!38}{\strut Septic} \colorbox{red!0}{\strut System} \colorbox{red!46}{\strut Types} \colorbox{red!15}{\strut AEROBIC} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!9}{\strut CESSPOOLS} \colorbox{red!14}{\strut DOSING} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!0}{\strut GRAVITYSIPHON} \colorbox{red!14}{\strut DOSING} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!2}{\strut PRESSURE} \colorbox{red!7}{\strut DRYWELLS} \colorbox{red!0}{\strut EVAPORATION-TRANSPIRATION} \colorbox{red!1}{\strut GRAVELLESS} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!5}{\strut GREYWATER} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!7}{\strut LAGOON} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!6}{\strut MEDIA} \colorbox{red!5}{\strut FILTER} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut GREYWATER} \colorbox{red!0}{\strut FILTERS} \colorbox{red!13}{\strut MOUND} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!9}{\strut RAISED} \colorbox{red!14}{\strut BED} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!9}{\strut SAND} \colorbox{red!14}{\strut BED} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!11}{\strut SEWAGE} \colorbox{red!0}{\strut TREATMENT} \colorbox{red!35}{\strut SYSTEMS} \colorbox{red!6}{\strut STEEP} \colorbox{red!2}{\strut SLOPE} \colorbox{red!0}{\strut DESIGNS} \colorbox{red!5}{\strut TOILET} \colorbox{red!9}{\strut ALTERNATIVES} \colorbox{red!0}{\strut ALTERNATIVE} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!0}{\strut DESIGNERS} \colorbox{red!0}{\strut ALTERNATIVE} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!0}{\strut PRODUCTS} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!0}{\strut INSPECTIONS} \colorbox{red!10}{\strut DEFINITIONS} \colorbox{red!0}{\strut FAILURE} \colorbox{red!2}{\strut LAWSUIT} \colorbox{red!1}{\strut FLOOD} \colorbox{red!5}{\strut RESPONSE} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!0}{\strut REFERENCES} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!6}{\strut CONSULTANTS} \colorbox{red!38}{\strut SEPTIC} \colorbox{red!7}{\strut AUTHORITIES} \colorbox{red!0}{\strut BOOKS} \colorbox{red!0}{\strut REFS} \colorbox{red!6}{\strut CODES} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut InspectAPedia} \colorbox{red!17}{\strut Home} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut Site} \colorbox{red!0}{\strut Map} \colorbox{red!21}{\strut Air} \colorbox{red!14}{\strut Conditioning} \colorbox{red!0}{\strut InspectAPedia} \colorbox{red!0}{\strut Bookstore} \colorbox{red!17}{\strut Electrical} \colorbox{red!11}{\strut Environment} \colorbox{red!7}{\strut Exteriors} \colorbox{red!11}{\strut Heating} \colorbox{red!17}{\strut Home} \colorbox{red!11}{\strut Inspection} \colorbox{red!5}{\strut Insulate} \colorbox{red!11}{\strut Ventilate} \colorbox{red!5}{\strut Interiors} \colorbox{red!13}{\strut Mold} \colorbox{red!0}{\strut InspectTest} \colorbox{red!18}{\strut Roofing} \colorbox{red!14}{\strut Plumbing} \colorbox{red!27}{\strut Water} \colorbox{red!38}{\strut Septic} \colorbox{red!9}{\strut Structure} \colorbox{red!0}{\strut Accuracy} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Bias} \colorbox{red!0}{\strut Pledge} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!10}{\strut Master} \colorbox{red!10}{\strut List} \colorbox{red!7}{\strut of} \colorbox{red!46}{\strut Types} \colorbox{red!7}{\strut of} \colorbox{red!38}{\strut Septic} \colorbox{red!35}{\strut Systems} \colorbox{red!5}{\strut .} \colorbox{red!38}{\strut Septic} \colorbox{red!0}{\strut System} \colorbox{red!0}{\strut Designs} \colorbox{red!0}{\strut SepticAPedia} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut Web} \colorbox{red!5}{\strut site} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut inspect-ny.com} \colorbox{red!46}{\strut Types} \colorbox{red!7}{\strut of} \colorbox{red!38}{\strut Septic} \colorbox{red!35}{\strut Systems} \colorbox{red!7}{\strut ,} \colorbox{red!0}{\strut Alternative} \colorbox{red!38}{\strut Septic} \colorbox{red!0}{\strut System} \colorbox{red!0}{\strut Designs} \colorbox{red!7}{\strut ,} \colorbox{red!10}{\strut Master} \colorbox{red!10}{\strut List} \colorbox{red!5}{\strut .} \colorbox{red!7}{\strut Descriptions} \colorbox{red!7}{\strut of} \colorbox{red!1}{\strut Kinds} \colorbox{red!7}{\strut of} \colorbox{red!38}{\strut Septic} \colorbox{red!35}{\strut Systems} \colorbox{red!0}{\strut Alternative} \colorbox{red!38}{\strut septic} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut designs} \colorbox{red!0}{\strut for} \colorbox{red!7}{\strut problem} \colorbox{red!0}{\strut sites} \colorbox{red!0}{\strut Description} \colorbox{red!7}{\strut of} \colorbox{red!0}{\strut alternative} \colorbox{red!38}{\strut septic} \colorbox{red!35}{\strut systems} \colorbox{red!7}{\strut ,} \colorbox{red!18}{\strut design} \colorbox{red!0}{\strut criteria} 
}}}
\end{CJK*}

89:septics, 85:system, 82:engineers, 71:south, 68:jersey, 49:new, 22:design, 17:professional, 16:llc, 14:services


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 1-866-SEPTICS} \colorbox{red!49}{\strut engineers} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut septics.com} \colorbox{red!43}{\strut South} \colorbox{red!41}{\strut jersey} \colorbox{red!49}{\strut engineers} \colorbox{red!9}{\strut llc} \colorbox{red!10}{\strut Professional} \colorbox{red!0}{\strut Septic} \colorbox{red!51}{\strut System} \colorbox{red!13}{\strut Design} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Engineering} \colorbox{red!3}{\strut Soil} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut Site} \colorbox{red!3}{\strut Analysis} \colorbox{red!6}{\strut Repair} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Remediation} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Renovation} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Restoration} \colorbox{red!3}{\strut Feasibility} \colorbox{red!0}{\strut andPermitting} \colorbox{red!8}{\strut services} \colorbox{red!6}{\strut Advanced} \colorbox{red!6}{\strut Pinelands} \colorbox{red!54}{\strut Septics} \colorbox{red!0}{\strut Systems} \colorbox{red!5}{\strut Inspection} \colorbox{red!8}{\strut Services} \colorbox{red!0}{\strut Engineering} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut Innovative} \colorbox{red!7}{\strut Solutions} \colorbox{red!0}{\strut 1-866-SEPTICS} \colorbox{red!49}{\strut engineers} \colorbox{red!4}{\strut .} \colorbox{red!0}{\strut septics.com} \colorbox{red!1}{\strut That} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut number} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut septic} \colorbox{red!0}{\strut systems} \colorbox{red!43}{\strut South} \colorbox{red!41}{\strut Jersey} \colorbox{red!49}{\strut Engineers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut L.L.C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut has} \colorbox{red!4}{\strut successfully} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut through} \colorbox{red!0}{\strut 12312006} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut 10,000} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut we} \colorbox{red!2}{\strut include} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut year} \colorbox{red!5}{\strut count} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut SOME} \colorbox{red!1}{\strut OF} \colorbox{red!0}{\strut OUR} \colorbox{red!8}{\strut SERVICES} \colorbox{red!3}{\strut Active} \colorbox{red!3}{\strut Member} \colorbox{red!0}{\strut .} \colorbox{red!29}{\strut New} \colorbox{red!41}{\strut Jersey} \colorbox{red!0}{\strut BuildersAssociation} \colorbox{red!8}{\strut Builders} \colorbox{red!6}{\strut League} \colorbox{red!0}{\strut ofSouth} \colorbox{red!41}{\strut Jersey} \colorbox{red!3}{\strut American} \colorbox{red!6}{\strut Society} \colorbox{red!1}{\strut of} \colorbox{red!6}{\strut Civil} \colorbox{red!49}{\strut Engineers} \colorbox{red!29}{\strut New} \colorbox{red!41}{\strut Jersey} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Pennsylvania} \colorbox{red!0}{\strut Septic} \colorbox{red!4}{\strut Management} \colorbox{red!5}{\strut Association} \colorbox{red!29}{\strut New} \colorbox{red!41}{\strut Jersey} \colorbox{red!6}{\strut Society} \colorbox{red!0}{\strut ofProfessional} \colorbox{red!49}{\strut Engineers} 
}}}
\end{CJK*}

query: paralegal

100:paralegal, 61:texas, 42:lake, 38:clear, 32:schools, 29:degree, 26:training, 26:law, 26:education, 25:legal


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 800-446-6931} \colorbox{red!75}{\strut Texas} \colorbox{red!100}{\strut Paralegal} \colorbox{red!32}{\strut Training} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Paralegal} \colorbox{red!39}{\strut Schools} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!100}{\strut paralegal} \colorbox{red!0}{\strut in} \colorbox{red!46}{\strut clear} \colorbox{red!51}{\strut lake} \colorbox{red!75}{\strut texas} \colorbox{red!75}{\strut Texas} \colorbox{red!100}{\strut Paralegal} \colorbox{red!32}{\strut Training} \colorbox{red!100}{\strut Paralegal} \colorbox{red!39}{\strut Schools} \colorbox{red!100}{\strut Paralegal} \colorbox{red!0}{\strut School} \colorbox{red!13}{\strut Houston} \colorbox{red!13}{\strut Houston} \colorbox{red!100}{\strut Paralegal} \colorbox{red!20}{\strut Program} \colorbox{red!12}{\strut conroe} \colorbox{red!75}{\strut texas} \colorbox{red!100}{\strut paralegal} \colorbox{red!32}{\strut education} \colorbox{red!11}{\strut pearland} \colorbox{red!75}{\strut texas} \colorbox{red!100}{\strut paralegal} \colorbox{red!32}{\strut training} \colorbox{red!20}{\strut program} \colorbox{red!75}{\strut texas} \colorbox{red!7}{\strut accredited} \colorbox{red!100}{\strut paralegal} \colorbox{red!39}{\strut schools} \colorbox{red!13}{\strut houston} \colorbox{red!75}{\strut texas} \colorbox{red!100}{\strut paralegal} \colorbox{red!32}{\strut training} \colorbox{red!0}{\strut baytown} \colorbox{red!75}{\strut texas} \colorbox{red!100}{\strut paralegal} \colorbox{red!9}{\strut certification} \colorbox{red!17}{\strut cypress} \colorbox{red!75}{\strut texas} \colorbox{red!100}{\strut paralegal} \colorbox{red!13}{\strut university} \colorbox{red!7}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!100}{\strut paralegal} \colorbox{red!0}{\strut in} \colorbox{red!46}{\strut clear} \colorbox{red!51}{\strut lake} \colorbox{red!75}{\strut texas} \colorbox{red!6}{\strut humble} \colorbox{red!75}{\strut texas} \colorbox{red!30}{\strut legal} \colorbox{red!23}{\strut assistant} \colorbox{red!32}{\strut training} \colorbox{red!3}{\strut richmond} \colorbox{red!75}{\strut texas} \colorbox{red!30}{\strut legal} \colorbox{red!23}{\strut assistant} \colorbox{red!11}{\strut classes} \colorbox{red!7}{\strut pasadena} \colorbox{red!75}{\strut texas} \colorbox{red!30}{\strut legal} \colorbox{red!23}{\strut assistant} \colorbox{red!39}{\strut schools} \colorbox{red!6}{\strut top} \colorbox{red!100}{\strut paralegal} \colorbox{red!39}{\strut schools} \colorbox{red!0}{\strut in} \colorbox{red!13}{\strut houston} \colorbox{red!75}{\strut texas} \colorbox{red!100}{\strut paralegal} \colorbox{red!12}{\strut studies} \colorbox{red!0}{\strut in} \colorbox{red!17}{\strut cypress} \colorbox{red!75}{\strut texas} \colorbox{red!7}{\strut pasadena} \colorbox{red!75}{\strut texas} \colorbox{red!100}{\strut paralegal} \colorbox{red!32}{\strut education} \colorbox{red!100}{\strut paralegal} \colorbox{red!0}{\strut certificate} \colorbox{red!14}{\strut course} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut galveston} \colorbox{red!75}{\strut texas} \colorbox{red!30}{\strut legal} \colorbox{red!23}{\strut assistant} \colorbox{red!9}{\strut certification} \colorbox{red!0}{\strut in} \colorbox{red!13}{\strut houston} \colorbox{red!6}{\strut best} \colorbox{red!100}{\strut paralegal} \colorbox{red!39}{\strut schools} \colorbox{red!0}{\strut in} \colorbox{red!11}{\strut pearland} \colorbox{red!75}{\strut texas} \colorbox{red!30}{\strut legal} \colorbox{red!23}{\strut assistant} \colorbox{red!35}{\strut degree} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut sugar} \colorbox{red!3}{\strut land} \colorbox{red!75}{\strut texas} \colorbox{red!4}{\strut ABA} \colorbox{red!100}{\strut Paralegal} \colorbox{red!39}{\strut Schools} \colorbox{red!7}{\strut Become} \colorbox{red!0}{\strut A} \colorbox{red!100}{\strut Paralegal} \colorbox{red!0}{\strut In} \colorbox{red!46}{\strut Clear} \colorbox{red!51}{\strut Lake} \colorbox{red!75}{\strut Texas} \colorbox{red!7}{\strut Become} \colorbox{red!0}{\strut A} \colorbox{red!100}{\strut Paralegal} \colorbox{red!11}{\strut Today} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut expected} \colorbox{red!0}{\strut growth} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut field} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut individuals} \colorbox{red!12}{\strut who} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!3}{\strut interest} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!32}{\strut law} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut consider} \colorbox{red!6}{\strut pursuing} \colorbox{red!0}{\strut an} \colorbox{red!32}{\strut education} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut will} \colorbox{red!0}{\strut enable} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut become} \colorbox{red!0}{\strut paralegals} \colorbox{red!7}{\strut .} \colorbox{red!2}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!7}{\strut prospective} \colorbox{red!4}{\strut employers} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut paralegals} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!32}{\strut law} \colorbox{red!3}{\strut firms} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut government} \colorbox{red!0}{\strut agencies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut private} \colorbox{red!3}{\strut companies} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Individuals} \colorbox{red!12}{\strut who} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut become} \colorbox{red!0}{\strut paralegals} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut pursue} \colorbox{red!4}{\strut careers} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!3}{\strut organizations} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut like} \colorbox{red!7}{\strut immigration} \colorbox{red!32}{\strut law} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut family} \colorbox{red!32}{\strut law} \colorbox{red!7}{\strut .} \colorbox{red!9}{\strut Different} \colorbox{red!1}{\strut Paths} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut Become} \colorbox{red!0}{\strut a} \colorbox{red!100}{\strut Paralegal} \colorbox{red!0}{\strut While} \colorbox{red!2}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut single} \colorbox{red!32}{\strut education} \colorbox{red!0}{\strut or} \colorbox{red!32}{\strut training} \colorbox{red!0}{\strut path} \colorbox{red!17}{\strut required} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut most} \colorbox{red!13}{\strut jobs} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut several} \colorbox{red!9}{\strut different} \colorbox{red!9}{\strut ways} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!100}{\strut paralegal} \colorbox{red!7}{\strut .} \colorbox{red!19}{\strut When} \colorbox{red!1}{\strut choosing} \colorbox{red!0}{\strut among} \colorbox{red!32}{\strut education} \colorbox{red!4}{\strut centers} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut prospective} \colorbox{red!7}{\strut students} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut beyond} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut first} \colorbox{red!13}{\strut jobs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut consider} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut long-term} \colorbox{red!4}{\strut careers} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!6}{\strut obtaining} \colorbox{red!0}{\strut an} \colorbox{red!9}{\strut associate} \colorbox{red!0}{\strut s} \colorbox{red!35}{\strut degree} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut student} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut open} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut doors} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut otherwise} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Those} \colorbox{red!12}{\strut who} \colorbox{red!1}{\strut already} \colorbox{red!0}{\strut have} \colorbox{red!17}{\strut college} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut further} \colorbox{red!32}{\strut training} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut changing} \colorbox{red!4}{\strut careers} \colorbox{red!0}{\strut can} \colorbox{red!9}{\strut attend} \colorbox{red!0}{\strut certificate} \colorbox{red!0}{\strut programs} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Programs} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut approved} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut American} \colorbox{red!12}{\strut Bar} 
}}}
\end{CJK*}

94:paralegal, 62:what, 44:how, 39:old, 31:cpa, 31:career, 29:salaries, 27:change, 26:jobs, 23:start


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut my.indeed} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Create} \colorbox{red!4}{\strut Account} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Sign} \colorbox{red!0}{\strut in} \colorbox{red!11}{\strut Jobs} \colorbox{red!12}{\strut Salaries} \colorbox{red!3}{\strut Trends} \colorbox{red!1}{\strut Forums} \colorbox{red!26}{\strut What} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut job} \colorbox{red!8}{\strut title} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut keywords} \colorbox{red!2}{\strut or} \colorbox{red!7}{\strut company} \colorbox{red!1}{\strut Forums} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Job} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Accountant} \colorbox{red!13}{\strut Career} \colorbox{red!11}{\strut Change} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Accountant} \colorbox{red!2}{\strut or} \colorbox{red!40}{\strut Paralegal} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut Get} \colorbox{red!7}{\strut new} \colorbox{red!3}{\strut comments} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut email} \colorbox{red!0}{\strut My} \colorbox{red!3}{\strut Email} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut cancel} \colorbox{red!3}{\strut email} \colorbox{red!1}{\strut alerts} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut anytime} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Tara} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut Chicago} \colorbox{red!2}{\strut ,} \colorbox{red!5}{\strut Illinois} \colorbox{red!1}{\strut 4} \colorbox{red!1}{\strut months} \colorbox{red!0}{\strut ago} \colorbox{red!2}{\strut Hello} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut am} \colorbox{red!0}{\strut 35} \colorbox{red!4}{\strut years} \colorbox{red!16}{\strut old} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut I} \colorbox{red!3}{\strut would} \colorbox{red!3}{\strut like} \colorbox{red!1}{\strut to} \colorbox{red!9}{\strut start} \colorbox{red!2}{\strut a} \colorbox{red!7}{\strut new} \colorbox{red!13}{\strut career} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut have} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut varied} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut experienced} \colorbox{red!1}{\strut past} \colorbox{red!0}{\strut job} \colorbox{red!1}{\strut profile} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut model} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut bartender} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut administrative} \colorbox{red!1}{\strut assistant} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut photography} \colorbox{red!1}{\strut assistant} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut film} \colorbox{red!1}{\strut production} \colorbox{red!3}{\strut manager} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut currently} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut a} \colorbox{red!1}{\strut media} \colorbox{red!0}{\strut analyst} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut top} \colorbox{red!2}{\strut pharmaceutical} \colorbox{red!0}{\strut companies} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut need} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut relatively} \colorbox{red!2}{\strut stable} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut well-paying} \colorbox{red!13}{\strut career} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut am} \colorbox{red!0}{\strut willing} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut go} \colorbox{red!1}{\strut back} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut school} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut land} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut job} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!2}{\strut already} \colorbox{red!1}{\strut have} \colorbox{red!2}{\strut a} \colorbox{red!6}{\strut BA} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Anthropology} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut become} \colorbox{red!2}{\strut a} \colorbox{red!40}{\strut paralegal} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut should} \colorbox{red!3}{\strut obtain} \colorbox{red!2}{\strut a} \colorbox{red!4}{\strut certificate} \colorbox{red!0}{\strut through} \colorbox{red!2}{\strut an} \colorbox{red!0}{\strut ABA-approved} \colorbox{red!3}{\strut program} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut become} \colorbox{red!2}{\strut an} \colorbox{red!0}{\strut accountant} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut either} \colorbox{red!2}{\strut get} \colorbox{red!2}{\strut a} \colorbox{red!1}{\strut 2nd} \colorbox{red!3}{\strut Bachelor} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut or} \colorbox{red!0}{\strut try} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut a} \colorbox{red!3}{\strut Master} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Accounting} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Also} \colorbox{red!2}{\strut ,} \colorbox{red!26}{\strut what} \colorbox{red!5}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!11}{\strut jobs} \colorbox{red!0}{\strut and} \colorbox{red!12}{\strut salaries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut non-CPA} \colorbox{red!0}{\strut accountant} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut a} \colorbox{red!7}{\strut degree} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Accounting} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut Which} \colorbox{red!0}{\strut job} \colorbox{red!3}{\strut would} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut understand} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut ultimately} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut my} \colorbox{red!2}{\strut choice} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut these} \colorbox{red!1}{\strut industries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut brand} \colorbox{red!7}{\strut new} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut me} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut I} \colorbox{red!3}{\strut would} \colorbox{red!3}{\strut like} \colorbox{red!0}{\strut some} \colorbox{red!1}{\strut objective} \colorbox{red!2}{\strut opinions} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut people} \colorbox{red!4}{\strut who} \colorbox{red!1}{\strut know} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Becoming} \colorbox{red!2}{\strut a} \colorbox{red!40}{\strut paralegal} \colorbox{red!1}{\strut seems} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut quicker} \colorbox{red!3}{\strut process} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut multiple} \colorbox{red!1}{\strut forums} \colorbox{red!1}{\strut I} \colorbox{red!1}{\strut have} \colorbox{red!0}{\strut heard} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut horrors} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut stress} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut field} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut note} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut I} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut I} \colorbox{red!3}{\strut would} \colorbox{red!1}{\strut enjoy} \colorbox{red!1}{\strut either} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut these} \colorbox{red!11}{\strut jobs} \colorbox{red!0}{\strut equally} \colorbox{red!1}{\strut .} \colorbox{red!18}{\strut How} \colorbox{red!3}{\strut would} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut compare} \colorbox{red!0}{\strut job} \colorbox{red!1}{\strut stability} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut job} \colorbox{red!0}{\strut growthopenings} \colorbox{red!2}{\strut ,} 
}}}
\end{CJK*}

query: hip fractures

98:fracture, 88:hip, 66:what, 52:causes, 32:symptoms, 27:definition, 23:cost, 19:treatment, 17:femur, 16:injuries


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut HealthCentral.com} \colorbox{red!5}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Diseases} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Injuries} \colorbox{red!0}{\strut .} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!12}{\strut Health} \colorbox{red!0}{\strut Encyclopedia} \colorbox{red!0}{\strut -} \colorbox{red!15}{\strut Diseases} \colorbox{red!2}{\strut and} \colorbox{red!4}{\strut Conditions} \colorbox{red!1}{\strut From} \colorbox{red!0}{\strut our} \colorbox{red!2}{\strut partner} \colorbox{red!3}{\strut site} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut chronic} \colorbox{red!13}{\strut pain} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut ChronicPainConnection.com} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut Find} \colorbox{red!3}{\strut ways} \colorbox{red!3}{\strut to} \colorbox{red!1}{\strut get} \colorbox{red!3}{\strut chronic} \colorbox{red!13}{\strut pain} \colorbox{red!2}{\strut relief} \colorbox{red!1}{\strut !} \colorbox{red!6}{\strut Find} \colorbox{red!2}{\strut a} \colorbox{red!6}{\strut right} \colorbox{red!18}{\strut treatment} \colorbox{red!2}{\strut for} \colorbox{red!2}{\strut your} \colorbox{red!3}{\strut chronic} \colorbox{red!13}{\strut pain} \colorbox{red!2}{\strut Join} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut your} \colorbox{red!3}{\strut chronic} \colorbox{red!13}{\strut pain} \colorbox{red!1}{\strut support} \colorbox{red!2}{\strut group} \colorbox{red!3}{\strut .} \colorbox{red!2}{\strut A} \colorbox{red!1}{\strut B} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut D} \colorbox{red!0}{\strut E} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut H} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut J} \colorbox{red!1}{\strut K} \colorbox{red!0}{\strut L} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut N} \colorbox{red!0}{\strut O} \colorbox{red!0}{\strut P} \colorbox{red!0}{\strut R} \colorbox{red!7}{\strut S} \colorbox{red!0}{\strut T} \colorbox{red!6}{\strut U} \colorbox{red!0}{\strut V} \colorbox{red!0}{\strut W} \colorbox{red!0}{\strut Y} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!63}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut the} \colorbox{red!25}{\strut Definition} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!3}{\strut ?} \colorbox{red!11}{\strut Description} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!49}{\strut Causes} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!30}{\strut Symptoms} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!18}{\strut Treatment} \colorbox{red!2}{\strut for} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!10}{\strut Prevention} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!63}{\strut What} \colorbox{red!4}{\strut Questions} \colorbox{red!3}{\strut to} \colorbox{red!0}{\strut ask} \colorbox{red!2}{\strut Your} \colorbox{red!6}{\strut Doctor} \colorbox{red!1}{\strut About} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!3}{\strut ?} \colorbox{red!63}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut the} \colorbox{red!25}{\strut Definition} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!3}{\strut ?} \colorbox{red!84}{\strut Hip} \colorbox{red!0}{\strut fractures} \colorbox{red!3}{\strut are} \colorbox{red!0}{\strut fractures} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut neck} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!16}{\strut femur} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut the} \colorbox{red!12}{\strut long} \colorbox{red!15}{\strut bone} \colorbox{red!1}{\strut that} \colorbox{red!4}{\strut comprises} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut upper} \colorbox{red!10}{\strut part} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!14}{\strut leg} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut The} \colorbox{red!15}{\strut femoral} \colorbox{red!14}{\strut neck} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut the} \colorbox{red!4}{\strut area} \colorbox{red!0}{\strut between} \colorbox{red!4}{\strut the} \colorbox{red!2}{\strut shaft} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!15}{\strut bone} \colorbox{red!2}{\strut and} \colorbox{red!4}{\strut the} \colorbox{red!6}{\strut head} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!16}{\strut femur} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut ball} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut that} \colorbox{red!4}{\strut fits} \colorbox{red!0}{\strut into} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut socket} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!84}{\strut hip} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut top} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Description} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut Hip} \colorbox{red!93}{\strut Fracture} \colorbox{red!84}{\strut Hip} \colorbox{red!0}{\strut fractures} \colorbox{red!3}{\strut are} \colorbox{red!2}{\strut a} \colorbox{red!4}{\strut major} \colorbox{red!5}{\strut public} \colorbox{red!12}{\strut health} \colorbox{red!6}{\strut problem} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut In} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut the} \colorbox{red!22}{\strut cost} \colorbox{red!4}{\strut of} \colorbox{red!84}{\strut hip} \colorbox{red!93}{\strut fracture} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut approximately} \colorbox{red!0}{\strut 7} \colorbox{red!3}{\strut billion} \colorbox{red!4}{\strut dollars} \colorbox{red!8}{\strut annually} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!84}{\strut hip} \colorbox{red!93}{\strut fracture} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut the} \colorbox{red!3}{\strut second} \colorbox{red!1}{\strut most} \colorbox{red!10}{\strut common} \colorbox{red!0}{\strut cause} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut admission} \colorbox{red!3}{\strut to} \colorbox{red!4}{\strut nursing} \colorbox{red!0}{\strut homes} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut accounting} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut 60,000} \colorbox{red!0}{\strut admissions} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut year} \colorbox{red!3}{\strut .} \colorbox{red!6}{\strut Osteoporosis} \colorbox{red!3}{\strut in} \colorbox{red!4}{\strut the} \colorbox{red!13}{\strut elderly} \colorbox{red!3}{\strut contributes} \colorbox{red!3}{\strut to} \colorbox{red!1}{\strut most} \colorbox{red!4}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut fractures} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut Many} \colorbox{red!13}{\strut elderly} \colorbox{red!5}{\strut patients} \colorbox{red!4}{\strut who} \colorbox{red!8}{\strut break} \colorbox{red!2}{\strut a} \colorbox{red!84}{\strut hip} \colorbox{red!2}{\strut face} \colorbox{red!2}{\strut a} \colorbox{red!1}{\strut broad} \colorbox{red!0}{\strut array} \colorbox{red!4}{\strut of} \colorbox{red!0}{\strut problems} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut transcend} \colorbox{red!4}{\strut the} \colorbox{red!18}{\strut treatment} \colorbox{red!4}{\strut of} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut injury} \colorbox{red!0}{\strut itself} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut In} \colorbox{red!1}{\strut many} \colorbox{red!4}{\strut cases} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut an} \colorbox{red!13}{\strut elderly} \colorbox{red!6}{\strut person} \colorbox{red!0}{\strut s} \colorbox{red!3}{\strut independent} \colorbox{red!1}{\strut existence} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut impacted} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut a} \colorbox{red!4}{\strut fall} \colorbox{red!1}{\strut that} \colorbox{red!49}{\strut causes} \colorbox{red!2}{\strut a} \colorbox{red!84}{\strut hip} \colorbox{red!93}{\strut fracture} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut an} \colorbox{red!4}{\strut event} \colorbox{red!1}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut forever} \colorbox{red!0}{\strut lessen} \colorbox{red!4}{\strut the} \colorbox{red!0}{\strut patient} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut level} 
}}}
\end{CJK*}

99:fracture, 98:hip, 64:average, 43:stay, 41:nsw, 36:wales, 33:care, 32:hospital, 31:australia, 30:new


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut eMJA} \colorbox{red!1}{\strut The} \colorbox{red!7}{\strut Medical} \colorbox{red!1}{\strut Journal} \colorbox{red!2}{\strut of} \colorbox{red!13}{\strut Australia} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Issues} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eMJA} \colorbox{red!0}{\strut shop} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Classifieds} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Contact} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Topics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Login} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Buy} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut access} \colorbox{red!0}{\strut Next} \colorbox{red!0}{\strut article} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut Previous} \colorbox{red!0}{\strut article} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut list} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut on} \colorbox{red!5}{\strut Public} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut environmental} \colorbox{red!8}{\strut health} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut Geriatrics} \colorbox{red!0}{\strut Pdf} \colorbox{red!0}{\strut version} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut PubMed} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut articles} \colorbox{red!5}{\strut Public} \colorbox{red!8}{\strut Health} \colorbox{red!7}{\strut Incidence} \colorbox{red!2}{\strut of} \colorbox{red!43}{\strut hip} \colorbox{red!44}{\strut fracture} \colorbox{red!2}{\strut in} \colorbox{red!13}{\strut New} \colorbox{red!10}{\strut South} \colorbox{red!16}{\strut Wales} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut efforts} \colorbox{red!1}{\strut having} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut effect} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Soufiane} \colorbox{red!0}{\strut Boufous} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Caroline} \colorbox{red!0}{\strut F} \colorbox{red!1}{\strut Finch} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Stephen} \colorbox{red!0}{\strut R} \colorbox{red!3}{\strut Lord} \colorbox{red!4}{\strut MJA} \colorbox{red!0}{\strut 2004} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 180} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 12} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 623-626} \colorbox{red!0}{\strut Introduction} \colorbox{red!0}{\strut Methods} \colorbox{red!3}{\strut Data} \colorbox{red!0}{\strut sources} \colorbox{red!0}{\strut Case} \colorbox{red!11}{\strut definition} \colorbox{red!4}{\strut Statistical} \colorbox{red!1}{\strut analyses} \colorbox{red!1}{\strut Results} \colorbox{red!0}{\strut Discussion} \colorbox{red!0}{\strut Acknowledgements} \colorbox{red!0}{\strut Competing} \colorbox{red!0}{\strut interests} \colorbox{red!0}{\strut References} \colorbox{red!0}{\strut Author} \colorbox{red!0}{\strut details} \colorbox{red!0}{\strut Abstract} \colorbox{red!0}{\strut Objective} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut To} \colorbox{red!0}{\strut examine} \colorbox{red!2}{\strut trends} \colorbox{red!2}{\strut in} \colorbox{red!14}{\strut hospital} \colorbox{red!12}{\strut admission} \colorbox{red!2}{\strut for} \colorbox{red!43}{\strut hip} \colorbox{red!44}{\strut fracture} \colorbox{red!2}{\strut in} \colorbox{red!13}{\strut New} \colorbox{red!10}{\strut South} \colorbox{red!16}{\strut Wales} \colorbox{red!1}{\strut between} \colorbox{red!2}{\strut July} \colorbox{red!0}{\strut 1990and} \colorbox{red!2}{\strut June} \colorbox{red!2}{\strut 2000} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Design} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Analysis} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut routinely} \colorbox{red!0}{\strut collected} \colorbox{red!14}{\strut hospital} \colorbox{red!1}{\strut separation} \colorbox{red!3}{\strut data} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Setting} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Public} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut private} \colorbox{red!0}{\strut acute-care} \colorbox{red!0}{\strut hospitals} \colorbox{red!2}{\strut in} \colorbox{red!18}{\strut NSW} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Participants} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut Admissions} \colorbox{red!2}{\strut of} \colorbox{red!5}{\strut patients} \colorbox{red!7}{\strut aged} \colorbox{red!0}{\strut 50years} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut primary} \colorbox{red!3}{\strut diagnosis} \colorbox{red!2}{\strut of} \colorbox{red!44}{\strut fracture} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut neck} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut femur} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut International} \colorbox{red!1}{\strut classification} \colorbox{red!2}{\strut of} \colorbox{red!4}{\strut diseases} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut 9th} \colorbox{red!0}{\strut revision} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ICD-9} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut 820or} \colorbox{red!0}{\strut ICD-10codes} \colorbox{red!0}{\strut S72.0S72.2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Main} \colorbox{red!2}{\strut outcome} \colorbox{red!2}{\strut measures} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut Number} \colorbox{red!0}{\strut and} \colorbox{red!8}{\strut rates} \colorbox{red!2}{\strut of} \colorbox{red!14}{\strut hospital} \colorbox{red!12}{\strut admission} \colorbox{red!2}{\strut for} \colorbox{red!44}{\strut fracture} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut the} \colorbox{red!3}{\strut neck} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut femur} \colorbox{red!1}{\strut per} \colorbox{red!0}{\strut 1000population} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut inpatient} \colorbox{red!4}{\strut mortality} \colorbox{red!8}{\strut rates} \colorbox{red!1}{\strut per} \colorbox{red!0}{\strut 1000admissions} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Results} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Between} \colorbox{red!2}{\strut July} \colorbox{red!0}{\strut 1990and} \colorbox{red!2}{\strut June} \colorbox{red!2}{\strut 2000} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut number} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut admissions} \colorbox{red!3}{\strut to} \colorbox{red!18}{\strut NSW} \colorbox{red!0}{\strut acute-care} \colorbox{red!0}{\strut hospitals} \colorbox{red!2}{\strut for} \colorbox{red!43}{\strut hip} \colorbox{red!44}{\strut fracture} \colorbox{red!2}{\strut increased} \colorbox{red!1}{\strut by} \colorbox{red!0}{\strut 41.9} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut in} \colorbox{red!2}{\strut men} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 1059to} \colorbox{red!0}{\strut 1503per} \colorbox{red!1}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut by} \colorbox{red!0}{\strut 31.2} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut in} \colorbox{red!4}{\strut women} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 3160to} \colorbox{red!0}{\strut 4145per} \colorbox{red!1}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut However} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut age-specific} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut age-adjusted} \colorbox{red!8}{\strut rates} \colorbox{red!1}{\strut remained} \colorbox{red!0}{\strut practically} \colorbox{red!0}{\strut unchanged} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!28}{\strut average} \colorbox{red!6}{\strut length} \colorbox{red!2}{\strut of} \colorbox{red!19}{\strut stay} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut admissions} \colorbox{red!2}{\strut for} \colorbox{red!43}{\strut hip} \colorbox{red!44}{\strut fracture} \colorbox{red!0}{\strut decreased} \colorbox{red!0}{\strut significantly} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 19.2days} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 95} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CI} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 18.519.8days} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut in} \colorbox{red!0}{\strut 19901991to} 
}}}
\end{CJK*}

query: quit smoking

97:smoking, 84:cigarettes, 59:quit, 41:help, 40:drug, 35:smokers, 28:benefits, 25:aids, 24:when, 21:new


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!30}{\strut drug} \colorbox{red!0}{\strut -} \colorbox{red!13}{\strut chantix} \colorbox{red!5}{\strut by} \colorbox{red!12}{\strut pfizer} \colorbox{red!5}{\strut to} \colorbox{red!31}{\strut help} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!13}{\strut Home} \colorbox{red!13}{\strut Chantix} \colorbox{red!8}{\strut Buy} \colorbox{red!13}{\strut Chantix} \colorbox{red!13}{\strut Chantix} \colorbox{red!13}{\strut Side} \colorbox{red!14}{\strut Effects} \colorbox{red!45}{\strut Quit} \colorbox{red!74}{\strut Smoking} \colorbox{red!31}{\strut Help} \colorbox{red!45}{\strut Quit} \colorbox{red!74}{\strut Smoking} \colorbox{red!19}{\strut Aids} \colorbox{red!45}{\strut Quit} \colorbox{red!74}{\strut Smoking} \colorbox{red!21}{\strut Benefits} \colorbox{red!0}{\strut Sitemap} \colorbox{red!4}{\strut Links} \colorbox{red!6}{\strut Contact} \colorbox{red!0}{\strut Us} \colorbox{red!45}{\strut Quit} \colorbox{red!74}{\strut Smoking} \colorbox{red!30}{\strut Drug} \colorbox{red!74}{\strut Smoking} \colorbox{red!2}{\strut is} \colorbox{red!11}{\strut Suicide} \colorbox{red!3}{\strut !} \colorbox{red!45}{\strut Quit} \colorbox{red!74}{\strut Smoking} \colorbox{red!3}{\strut now} \colorbox{red!3}{\strut ,} \colorbox{red!8}{\strut buy} \colorbox{red!13}{\strut Chantix} \colorbox{red!1}{\strut the} \colorbox{red!7}{\strut ultimate} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!30}{\strut drug} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut It} \colorbox{red!2}{\strut is} \colorbox{red!5}{\strut not} \colorbox{red!9}{\strut easy} \colorbox{red!5}{\strut to} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!3}{\strut ,} \colorbox{red!0}{\strut everybody} \colorbox{red!15}{\strut who} \colorbox{red!3}{\strut has} \colorbox{red!3}{\strut tried} \colorbox{red!3}{\strut it} \colorbox{red!1}{\strut can} \colorbox{red!3}{\strut tell} \colorbox{red!3}{\strut you} \colorbox{red!4}{\strut this} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut But} \colorbox{red!2}{\strut with} \colorbox{red!1}{\strut the} \colorbox{red!16}{\strut new} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!30}{\strut drug} \colorbox{red!3}{\strut ,} \colorbox{red!13}{\strut Chantix} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut it} \colorbox{red!3}{\strut has} \colorbox{red!5}{\strut become} \colorbox{red!5}{\strut relatively} \colorbox{red!6}{\strut easier} \colorbox{red!2}{\strut for} \colorbox{red!26}{\strut smokers} \colorbox{red!5}{\strut to} \colorbox{red!8}{\strut break} \colorbox{red!1}{\strut the} \colorbox{red!5}{\strut old} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut ugly} \colorbox{red!74}{\strut smoking} \colorbox{red!15}{\strut habit} \colorbox{red!3}{\strut .} \colorbox{red!45}{\strut Quit} \colorbox{red!74}{\strut Smoking} \colorbox{red!30}{\strut Drug} \colorbox{red!0}{\strut -} \colorbox{red!13}{\strut chantix} \colorbox{red!4}{\strut 70} \colorbox{red!7}{\strut .} \colorbox{red!6}{\strut of} \colorbox{red!26}{\strut smokers} \colorbox{red!7}{\strut say} \colorbox{red!3}{\strut they} \colorbox{red!5}{\strut want} \colorbox{red!5}{\strut to} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!3}{\strut ,} \colorbox{red!1}{\strut but} \colorbox{red!3}{\strut most} \colorbox{red!4}{\strut believe} \colorbox{red!3}{\strut they} \colorbox{red!4}{\strut will} \colorbox{red!2}{\strut be} \colorbox{red!5}{\strut unable} \colorbox{red!5}{\strut to} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut However} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut almost} \colorbox{red!6}{\strut half} \colorbox{red!6}{\strut of} \colorbox{red!6}{\strut all} \colorbox{red!26}{\strut smokers} \colorbox{red!5}{\strut eventually} \colorbox{red!5}{\strut manage} \colorbox{red!5}{\strut to} \colorbox{red!6}{\strut achieve} \colorbox{red!4}{\strut this} \colorbox{red!8}{\strut goal} \colorbox{red!2}{\strut with} \colorbox{red!1}{\strut the} \colorbox{red!31}{\strut help} \colorbox{red!6}{\strut of} \colorbox{red!13}{\strut Chantix} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!30}{\strut drug} \colorbox{red!3}{\strut .} \colorbox{red!4}{\strut This} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!30}{\strut drug} \colorbox{red!7}{\strut increases} \colorbox{red!4}{\strut your} \colorbox{red!7}{\strut chances} \colorbox{red!5}{\strut to} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!3}{\strut four} \colorbox{red!6}{\strut times} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut than} \colorbox{red!5}{\strut going} \colorbox{red!0}{\strut cold} \colorbox{red!0}{\strut turkey} \colorbox{red!3}{\strut .} \colorbox{red!5}{\strut Even} \colorbox{red!2}{\strut if} \colorbox{red!3}{\strut you} \colorbox{red!0}{\strut go} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut other} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!0}{\strut drugs} \colorbox{red!4}{\strut such} \colorbox{red!2}{\strut as} \colorbox{red!5}{\strut Zyban} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut they} \colorbox{red!6}{\strut dont} \colorbox{red!31}{\strut help} \colorbox{red!3}{\strut you} \colorbox{red!3}{\strut nearly} \colorbox{red!6}{\strut half} \colorbox{red!2}{\strut as} \colorbox{red!3}{\strut much} \colorbox{red!2}{\strut as} \colorbox{red!13}{\strut Chantix} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Increase} \colorbox{red!4}{\strut your} \colorbox{red!7}{\strut chances} \colorbox{red!5}{\strut to} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!3}{\strut .} \colorbox{red!8}{\strut Buy} \colorbox{red!13}{\strut Chantix} \colorbox{red!3}{\strut a} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!30}{\strut drug} \colorbox{red!10}{\strut which} \colorbox{red!5}{\strut actually} \colorbox{red!14}{\strut works} \colorbox{red!3}{\strut .} \colorbox{red!18}{\strut When} \colorbox{red!3}{\strut you} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!2}{\strut with} \colorbox{red!13}{\strut Chantix} \colorbox{red!3}{\strut ,} \colorbox{red!2}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut many} \colorbox{red!21}{\strut benefits} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut Let} \colorbox{red!0}{\strut us} \colorbox{red!6}{\strut consider} \colorbox{red!6}{\strut all} \colorbox{red!1}{\strut the} \colorbox{red!21}{\strut benefits} \colorbox{red!6}{\strut of} \colorbox{red!4}{\strut this} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!30}{\strut drug} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Non-Nicotine} \colorbox{red!45}{\strut Quit} \colorbox{red!74}{\strut Smoking} \colorbox{red!30}{\strut Drug} \colorbox{red!0}{\strut From} \colorbox{red!1}{\strut the} \colorbox{red!6}{\strut conventional} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!0}{\strut drugs} \colorbox{red!4}{\strut such} \colorbox{red!2}{\strut as} \colorbox{red!9}{\strut nicotine} \colorbox{red!4}{\strut gums} \colorbox{red!3}{\strut ,} \colorbox{red!6}{\strut patches} \colorbox{red!3}{\strut ,} \colorbox{red!3}{\strut lozenges} \colorbox{red!3}{\strut ,} \colorbox{red!4}{\strut inhalers} \colorbox{red!1}{\strut and} \colorbox{red!5}{\strut sprays} \colorbox{red!3}{\strut ,} \colorbox{red!8}{\strut science} \colorbox{red!3}{\strut has} \colorbox{red!5}{\strut advanced} \colorbox{red!5}{\strut to} \colorbox{red!0}{\strut non-nicotine} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!0}{\strut drugs} \colorbox{red!3}{\strut .} \colorbox{red!1}{\strut The} \colorbox{red!3}{\strut older} \colorbox{red!9}{\strut nicotine} \colorbox{red!9}{\strut replacement} \colorbox{red!9}{\strut therapies} \colorbox{red!0}{\strut work} \colorbox{red!5}{\strut by} \colorbox{red!3}{\strut supplying} \colorbox{red!9}{\strut nicotine} \colorbox{red!5}{\strut to} \colorbox{red!4}{\strut your} \colorbox{red!7}{\strut body} \colorbox{red!1}{\strut .} \colorbox{red!9}{\strut nicotine} \colorbox{red!2}{\strut is} \colorbox{red!5}{\strut to} \colorbox{red!5}{\strut blame} \colorbox{red!2}{\strut for} \colorbox{red!4}{\strut your} \colorbox{red!74}{\strut smoking} \colorbox{red!15}{\strut habit} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut thereby} \colorbox{red!8}{\strut weaning} \colorbox{red!3}{\strut you} \colorbox{red!0}{\strut from} \colorbox{red!64}{\strut cigarettes} \colorbox{red!1}{\strut slowly} \colorbox{red!3}{\strut .} \colorbox{red!3}{\strut You} \colorbox{red!6}{\strut dont} \colorbox{red!4}{\strut feel} \colorbox{red!6}{\strut like} \colorbox{red!74}{\strut smoking} \colorbox{red!18}{\strut when} \colorbox{red!3}{\strut you} \colorbox{red!4}{\strut avail} \colorbox{red!6}{\strut of} \colorbox{red!6}{\strut these} \colorbox{red!45}{\strut quit} \colorbox{red!74}{\strut smoking} \colorbox{red!0}{\strut drugs} \colorbox{red!1}{\strut and} 
}}}
\end{CJK*}

96:smoking, 93:quit, 27:tool, 22:application, 20:program, 20:pda, 19:interactive, 18:ppc, 18:palm, 18:computer


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!47}{\strut Quit} \colorbox{red!49}{\strut Smoking} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Consumer} \colorbox{red!9}{\strut Interactive} \colorbox{red!13}{\strut Tool} \colorbox{red!3}{\strut This} \colorbox{red!10}{\strut program} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut a} \colorbox{red!10}{\strut PDA} \colorbox{red!13}{\strut tool} \colorbox{red!2}{\strut that} \colorbox{red!4}{\strut helps} \colorbox{red!0}{\strut consumers} \colorbox{red!1}{\strut to} \colorbox{red!4}{\strut prepare} \colorbox{red!1}{\strut to} \colorbox{red!47}{\strut quit} \colorbox{red!49}{\strut smoking} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Included} \colorbox{red!2}{\strut is} \colorbox{red!2}{\strut a} \colorbox{red!0}{\strut 5-day} \colorbox{red!5}{\strut countdown} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut their} \colorbox{red!47}{\strut quit} \colorbox{red!5}{\strut date} \colorbox{red!2}{\strut that} \colorbox{red!1}{\strut can} \colorbox{red!1}{\strut be} \colorbox{red!2}{\strut inserted} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut Calendar} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!2}{\strut as} \colorbox{red!2}{\strut a} \colorbox{red!1}{\strut number} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut helpful} \colorbox{red!2}{\strut resources} \colorbox{red!1}{\strut .} \colorbox{red!11}{\strut Application} \colorbox{red!4}{\strut Downloads} \colorbox{red!4}{\strut Installation} \colorbox{red!4}{\strut Instructions} \colorbox{red!3}{\strut Feedback} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut Help} \colorbox{red!6}{\strut Copyright} \colorbox{red!7}{\strut Constraints} \colorbox{red!0}{\strut Related} \colorbox{red!2}{\strut Resources} \colorbox{red!11}{\strut Application} \colorbox{red!4}{\strut Downloads} \colorbox{red!9}{\strut Palm} \colorbox{red!6}{\strut OS} \colorbox{red!0}{\strut 3.2} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut above} \colorbox{red!7}{\strut File} \colorbox{red!5}{\strut Size} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 27} \colorbox{red!1}{\strut KB} \colorbox{red!0}{\strut Download} \colorbox{red!11}{\strut Application} \colorbox{red!6}{\strut Pocket} \colorbox{red!5}{\strut PC} \colorbox{red!3}{\strut Version} \colorbox{red!7}{\strut File} \colorbox{red!5}{\strut Size} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 74} \colorbox{red!1}{\strut KB} \colorbox{red!0}{\strut Download} \colorbox{red!11}{\strut Application} \colorbox{red!2}{\strut Web} \colorbox{red!3}{\strut Version} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut HTML} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 5-Day} \colorbox{red!5}{\strut Countdown} \colorbox{red!4}{\strut Installation} \colorbox{red!4}{\strut Instructions} \colorbox{red!9}{\strut Palm} \colorbox{red!6}{\strut OS} \colorbox{red!5}{\strut Device} \colorbox{red!0}{\strut Download} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut file} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut QuitPalm.prc} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut your} \colorbox{red!9}{\strut computer} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Double} \colorbox{red!2}{\strut Click} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut QuitPalm.prc} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut to} \colorbox{red!3}{\strut add} \colorbox{red!2}{\strut the} \colorbox{red!11}{\strut application} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut your} \colorbox{red!9}{\strut Palm} \colorbox{red!3}{\strut Desktop} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Sync} \colorbox{red!1}{\strut your} \colorbox{red!9}{\strut Palm} \colorbox{red!1}{\strut with} \colorbox{red!1}{\strut your} \colorbox{red!5}{\strut PC} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut install} \colorbox{red!2}{\strut the} \colorbox{red!11}{\strut application} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Pocket} \colorbox{red!5}{\strut PC} \colorbox{red!0}{\strut Download} \colorbox{red!2}{\strut the} \colorbox{red!7}{\strut file} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut QuitPPC.exe} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut your} \colorbox{red!9}{\strut computer} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Start} \colorbox{red!4}{\strut Microsoft} \colorbox{red!0}{\strut ActiveSync} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut attach} \colorbox{red!2}{\strut the} \colorbox{red!6}{\strut Pocket} \colorbox{red!5}{\strut PC} \colorbox{red!1}{\strut to} \colorbox{red!1}{\strut your} \colorbox{red!9}{\strut computer} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Double} \colorbox{red!2}{\strut click} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut QuitPPC.exe} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut file} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut install} \colorbox{red!2}{\strut the} \colorbox{red!11}{\strut application} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Feedback} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut Help} \colorbox{red!2}{\strut Submit} \colorbox{red!1}{\strut your} \colorbox{red!2}{\strut comments} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut questions} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut suggestions} \colorbox{red!0}{\strut regarding} \colorbox{red!3}{\strut this} \colorbox{red!11}{\strut application} \colorbox{red!0}{\strut via} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut info.ahrq.gov} \colorbox{red!6}{\strut Copyright} \colorbox{red!7}{\strut Constraints} \colorbox{red!3}{\strut AHRQ} \colorbox{red!1}{\strut makes} \colorbox{red!3}{\strut this} \colorbox{red!3}{\strut product} \colorbox{red!3}{\strut available} \colorbox{red!2}{\strut under} \colorbox{red!2}{\strut the} \colorbox{red!2}{\strut following} \colorbox{red!2}{\strut conditions} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!47}{\strut Quit} \colorbox{red!49}{\strut Smoking} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Consumer} \colorbox{red!9}{\strut Interactive} \colorbox{red!13}{\strut Tool} \colorbox{red!1}{\strut may} \colorbox{red!1}{\strut be} \colorbox{red!0}{\strut downloaded} \colorbox{red!2}{\strut for} \colorbox{red!2}{\strut specific} \colorbox{red!1}{\strut individual} \colorbox{red!0}{\strut applications} \colorbox{red!1}{\strut by} \colorbox{red!2}{\strut organizations} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut personal} \colorbox{red!3}{\strut use} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut providing} \colorbox{red!1}{\strut citation} \colorbox{red!2}{\strut as} \colorbox{red!1}{\strut to} \colorbox{red!2}{\strut source} \colorbox{red!2}{\strut is} \colorbox{red!3}{\strut included} \colorbox{red!1}{\strut .} \colorbox{red!47}{\strut Quit} \colorbox{red!49}{\strut Smoking} \colorbox{red!1}{\strut .} \colorbox{red!6}{\strut Consumer} \colorbox{red!9}{\strut Interactive} \colorbox{red!13}{\strut Tool} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Agency} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut Healthcare} \colorbox{red!2}{\strut Research} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut Quality} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut November} \colorbox{red!1}{\strut 2004} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Rockville} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut MD} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut http} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut pda.ahrq.gov} \colorbox{red!3}{\strut This} \colorbox{red!3}{\strut product} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut any} \colorbox{red!2}{\strut modifications} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut adaptations} \colorbox{red!1}{\strut may} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut be} \colorbox{red!0}{\strut reproduced} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut sold} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut used} \colorbox{red!2}{\strut for} \colorbox{red!3}{\strut commercial} \colorbox{red!1}{\strut purposes} \colorbox{red!0}{\strut without} \colorbox{red!2}{\strut specific} \colorbox{red!3}{\strut permission} \colorbox{red!2}{\strut granted} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut a} \colorbox{red!7}{\strut licensing} \colorbox{red!2}{\strut agreement} \colorbox{red!1}{\strut from} \colorbox{red!3}{\strut AHRQ} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut In} \colorbox{red!1}{\strut addition} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut this} \colorbox{red!11}{\strut application} \colorbox{red!2}{\strut and} \colorbox{red!1}{\strut links} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut any} \colorbox{red!2}{\strut direct} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut indirect} \colorbox{red!2}{\strut endorsement} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut a} 
}}}
\end{CJK*}

query: brooks brothers clearance

101:brooks, 97:brothers, 45:what, 31:ebates, 31:cash, 24:sales, 22:back, 21:coupons, 21:buy, 19:rebates


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut --} \colorbox{red!0}{\strut Select} \colorbox{red!1}{\strut a} \colorbox{red!11}{\strut store} \colorbox{red!0}{\strut --} \colorbox{red!6}{\strut New} \colorbox{red!0}{\strut to} \colorbox{red!27}{\strut Ebates} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut Sign} \colorbox{red!0}{\strut up} \colorbox{red!1}{\strut and} \colorbox{red!8}{\strut start} \colorbox{red!6}{\strut saving} \colorbox{red!3}{\strut !} \colorbox{red!5}{\strut Members} \colorbox{red!0}{\strut Log} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Stores} \colorbox{red!18}{\strut Coupons} \colorbox{red!3}{\strut Products} \colorbox{red!0}{\strut My} \colorbox{red!27}{\strut Ebates} \colorbox{red!0}{\strut Tell-A-Friend} \colorbox{red!2}{\strut Blog} \colorbox{red!1}{\strut Help} \colorbox{red!0}{\strut We} \colorbox{red!7}{\strut receive} \colorbox{red!1}{\strut a} \colorbox{red!21}{\strut sales} \colorbox{red!7}{\strut commission} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut stores} \colorbox{red!9}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!18}{\strut buy} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut pass} \colorbox{red!0}{\strut along} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut portion} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!7}{\strut commission} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut this} \colorbox{red!10}{\strut amount} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!27}{\strut Ebates} \colorbox{red!7}{\strut account} \colorbox{red!1}{\strut and} \colorbox{red!16}{\strut pay} \colorbox{red!1}{\strut it} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut four} \colorbox{red!4}{\strut times} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut year} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!5}{\strut forms} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut fill} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut from} \colorbox{red!27}{\strut Ebates} \colorbox{red!0}{\strut ,} \colorbox{red!18}{\strut buy} \colorbox{red!1}{\strut and} \colorbox{red!10}{\strut earn} \colorbox{red!27}{\strut cash} \colorbox{red!3}{\strut !} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut SAVINGS} \colorbox{red!4}{\strut AT} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!7}{\strut 4} \colorbox{red!3}{\strut .} \colorbox{red!27}{\strut Cash} \colorbox{red!19}{\strut Back} \colorbox{red!0}{\strut .} \colorbox{red!39}{\strut What} \colorbox{red!1}{\strut is} \colorbox{red!27}{\strut Cash} \colorbox{red!19}{\strut Back} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut DESCRIPTION} \colorbox{red!18}{\strut COUPONS} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut SPECIALS} \colorbox{red!0}{\strut DESCRIPTION} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!1}{\strut leading} \colorbox{red!0}{\strut destination} \colorbox{red!1}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!8}{\strut women} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut men} \colorbox{red!6}{\strut apparel} \colorbox{red!11}{\strut purchases} \colorbox{red!7}{\strut .} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!7}{\strut carries} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut complete} \colorbox{red!2}{\strut inventory} \colorbox{red!2}{\strut of} \colorbox{red!5}{\strut dresses} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut women} \colorbox{red!1}{\strut and} \colorbox{red!9}{\strut men} \colorbox{red!5}{\strut suits} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut shoes} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut accessories} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut Browse} \colorbox{red!3}{\strut the} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!11}{\strut deals} \colorbox{red!2}{\strut listed} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!3}{\strut !} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut the} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut take} \colorbox{red!1}{\strut advantage} \colorbox{red!2}{\strut of} \colorbox{red!3}{\strut the} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!18}{\strut coupons} \colorbox{red!0}{\strut ,} \colorbox{red!15}{\strut specials} \colorbox{red!0}{\strut or} \colorbox{red!21}{\strut sales} \colorbox{red!7}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!1}{\strut there} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!0}{\strut coupon} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut promo} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut the} \colorbox{red!4}{\strut offer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut simply} \colorbox{red!1}{\strut enter} \colorbox{red!1}{\strut it} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut the} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!6}{\strut shopping} \colorbox{red!4}{\strut cart} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut redeem} \colorbox{red!1}{\strut it} \colorbox{red!7}{\strut .} \colorbox{red!18}{\strut COUPONS} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut SPECIALS} \colorbox{red!0}{\strut Save} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut 60} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut all} \colorbox{red!9}{\strut men} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut and} \colorbox{red!8}{\strut women} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut clearance} \colorbox{red!5}{\strut items} \colorbox{red!4}{\strut at} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!21}{\strut Sales} \colorbox{red!0}{\strut Save} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 50} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut all} \colorbox{red!7}{\strut Boys} \colorbox{red!5}{\strut Clearance} \colorbox{red!5}{\strut items} \colorbox{red!3}{\strut only} \colorbox{red!4}{\strut at} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!3}{\strut !} \colorbox{red!21}{\strut Sales} \colorbox{red!0}{\strut SAVE} \colorbox{red!4}{\strut AT} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!16}{\strut Rebates} \colorbox{red!0}{\strut -} \colorbox{red!7}{\strut Receive} \colorbox{red!7}{\strut 4} \colorbox{red!3}{\strut .} \colorbox{red!27}{\strut Cash} \colorbox{red!19}{\strut Back} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!18}{\strut Coupons} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Use} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!18}{\strut coupons} \colorbox{red!2}{\strut listed} \colorbox{red!0}{\strut above} \colorbox{red!7}{\strut .} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!9}{\strut Discounts} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Find} \colorbox{red!3}{\strut the} \colorbox{red!3}{\strut latest} \colorbox{red!89}{\strut Brooks} \colorbox{red!85}{\strut Brothers} \colorbox{red!9}{\strut discounts} \colorbox{red!1}{\strut and} \colorbox{red!11}{\strut deals} \colorbox{red!2}{\strut listed} \colorbox{red!0}{\strut above} \colorbox{red!7}{\strut .} \colorbox{red!6}{\strut Appliances} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Hardware} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut stores} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!4}{\strut category} \colorbox{red!3}{\strut Sears} \colorbox{red!7}{\strut 2} \colorbox{red!3}{\strut .} \colorbox{red!27}{\strut Cash} \colorbox{red!19}{\strut Back} \colorbox{red!6}{\strut Home} \colorbox{red!4}{\strut Depot} \colorbox{red!7}{\strut 3} \colorbox{red!3}{\strut .} \colorbox{red!27}{\strut Cash} \colorbox{red!19}{\strut Back} \colorbox{red!5}{\strut Compact} \colorbox{red!0}{\strut Appliance} \colorbox{red!7}{\strut 3} \colorbox{red!3}{\strut .} \colorbox{red!27}{\strut Cash} \colorbox{red!19}{\strut Back} \colorbox{red!4}{\strut Ace} 
}}}
\end{CJK*}

97:brooks, 89:brothers, 24:clearance, 22:deals, 20:stores, 17:shop, 15:coupons, 14:grocery, 14:discounts, 14:boy


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Search} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!4}{\strut Home} \colorbox{red!3}{\strut Business} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Finance} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!4}{\strut Email} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!3}{\strut Local} \colorbox{red!5}{\strut Bargains} \colorbox{red!0}{\strut Couponing} \colorbox{red!0}{\strut 101} \colorbox{red!5}{\strut Online} \colorbox{red!9}{\strut Deals} \colorbox{red!3}{\strut Free} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!2}{\strut Newsletter} \colorbox{red!1}{\strut !} \colorbox{red!2}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!1}{\strut Discuss} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut my} \colorbox{red!3}{\strut Forum} \colorbox{red!5}{\strut Donna} \colorbox{red!0}{\strut s} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!3}{\strut Blog} \colorbox{red!0}{\strut By} \colorbox{red!5}{\strut Donna} \colorbox{red!0}{\strut L} \colorbox{red!1}{\strut Montaldo} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut About.com} \colorbox{red!3}{\strut Guide} \colorbox{red!1}{\strut to} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!1}{\strut since} \colorbox{red!1}{\strut 2001} \colorbox{red!0}{\strut MyBio} \colorbox{red!0}{\strut MyBlog} \colorbox{red!0}{\strut MyForum} \colorbox{red!2}{\strut Add} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut iGoogle} \colorbox{red!1}{\strut My} \colorbox{red!3}{\strut Yahoo} \colorbox{red!1}{\strut !} \colorbox{red!3}{\strut RSS} \colorbox{red!0}{\strut Up} \colorbox{red!1}{\strut To} \colorbox{red!0}{\strut 60} \colorbox{red!2}{\strut Percent} \colorbox{red!2}{\strut Off} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut BrooksBrothers.com} \colorbox{red!1}{\strut Wednesday} \colorbox{red!1}{\strut January} \colorbox{red!1}{\strut 7} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut BrooksBrothers.com} \colorbox{red!2}{\strut has} \colorbox{red!0}{\strut just} \colorbox{red!2}{\strut launched} \colorbox{red!0}{\strut their} \colorbox{red!10}{\strut Clearance} \colorbox{red!3}{\strut Event} \colorbox{red!2}{\strut with} \colorbox{red!0}{\strut up} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut 60} \colorbox{red!2}{\strut percent} \colorbox{red!2}{\strut off} \colorbox{red!0}{\strut all} \colorbox{red!4}{\strut men} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut women} \colorbox{red!0}{\strut s} \colorbox{red!10}{\strut clearance} \colorbox{red!4}{\strut items} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut up} \colorbox{red!1}{\strut to} \colorbox{red!0}{\strut 50} \colorbox{red!2}{\strut percent} \colorbox{red!2}{\strut off} \colorbox{red!0}{\strut all} \colorbox{red!6}{\strut boy} \colorbox{red!0}{\strut s} \colorbox{red!10}{\strut clearance} \colorbox{red!1}{\strut .} \colorbox{red!42}{\strut Brooks} \colorbox{red!38}{\strut Brothers} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut known} \colorbox{red!2}{\strut for} \colorbox{red!0}{\strut its} \colorbox{red!3}{\strut excellent} \colorbox{red!2}{\strut quality} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut styling} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut classic} \colorbox{red!4}{\strut apparel} \colorbox{red!1}{\strut and} \colorbox{red!3}{\strut accessories} \colorbox{red!1}{\strut .} \colorbox{red!10}{\strut Clearance} \colorbox{red!4}{\strut items} \colorbox{red!1}{\strut include} \colorbox{red!2}{\strut blazers} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut outerwear} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut dresses} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut slacks} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut sweaters} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut cashmere} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut handbags} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut shoes} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut ties} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!1}{\strut more} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut Shop} \colorbox{red!3}{\strut Direct} \colorbox{red!1}{\strut -} \colorbox{red!4}{\strut Men} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut Women} \colorbox{red!0}{\strut s} \colorbox{red!10}{\strut Clearance} \colorbox{red!7}{\strut Shop} \colorbox{red!3}{\strut Direct} \colorbox{red!1}{\strut -} \colorbox{red!0}{\strut Boys} \colorbox{red!10}{\strut Clearance} \colorbox{red!2}{\strut Comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut All} \colorbox{red!2}{\strut Posts} \colorbox{red!2}{\strut Prev} \colorbox{red!2}{\strut Comments} \colorbox{red!0}{\strut No} \colorbox{red!2}{\strut comments} \colorbox{red!0}{\strut yet} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut Leave} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Comment} \colorbox{red!2}{\strut Leave} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Comment} \colorbox{red!0}{\strut Name} \colorbox{red!4}{\strut Email} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut never} \colorbox{red!1}{\strut displayed} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut URL} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Comment} \colorbox{red!1}{\strut Line} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut paragraph} \colorbox{red!2}{\strut breaks} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut automatic} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Some} \colorbox{red!1}{\strut HTML} \colorbox{red!2}{\strut allowed} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Say} \colorbox{red!1}{\strut It} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut Discuss} \colorbox{red!1}{\strut Recent} \colorbox{red!3}{\strut Blog} \colorbox{red!2}{\strut Posts} \colorbox{red!0}{\strut Up} \colorbox{red!1}{\strut To} \colorbox{red!0}{\strut 60} \colorbox{red!2}{\strut Percent} \colorbox{red!2}{\strut Off} \colorbox{red!1}{\strut at} \colorbox{red!0}{\strut BrooksBrothers.com} \colorbox{red!4}{\strut Printable} \colorbox{red!6}{\strut Coupons} \colorbox{red!2}{\strut for} \colorbox{red!2}{\strut Quit} \colorbox{red!2}{\strut Smoking} \colorbox{red!2}{\strut Aides} \colorbox{red!6}{\strut Grocery} \colorbox{red!2}{\strut News} \colorbox{red!1}{\strut Community} \colorbox{red!3}{\strut Forum} \colorbox{red!2}{\strut Explore} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!2}{\strut Must} \colorbox{red!1}{\strut Reads} \colorbox{red!6}{\strut Grocery} \colorbox{red!8}{\strut Stores} \colorbox{red!1}{\strut That} \colorbox{red!2}{\strut Double} \colorbox{red!6}{\strut Coupons} \colorbox{red!3}{\strut Outlet} \colorbox{red!3}{\strut Mall} \colorbox{red!0}{\strut Shopping} \colorbox{red!5}{\strut Online} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut ,} \colorbox{red!8}{\strut Stores} \colorbox{red!0}{\strut A} \colorbox{red!1}{\strut -} \colorbox{red!2}{\strut Z} \colorbox{red!3}{\strut Cut} \colorbox{red!0}{\strut Your} \colorbox{red!4}{\strut Entertainment} \colorbox{red!3}{\strut Costs} \colorbox{red!3}{\strut Hotel} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut -} \colorbox{red!1}{\strut Nationwide} \colorbox{red!1}{\strut Most} \colorbox{red!3}{\strut Popular} \colorbox{red!4}{\strut Printable} \colorbox{red!4}{\strut Pizza} \colorbox{red!6}{\strut Coupons} \colorbox{red!2}{\strut Abercrombie} \colorbox{red!2}{\strut Fitch} \colorbox{red!0}{\strut Outlets} \colorbox{red!4}{\strut Printable} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut -} \colorbox{red!2}{\strut Food} \colorbox{red!8}{\strut Stores} \colorbox{red!1}{\strut That} \colorbox{red!2}{\strut Double} \colorbox{red!6}{\strut Coupons} \colorbox{red!6}{\strut Discounts} \colorbox{red!2}{\strut For} \colorbox{red!2}{\strut Smoking} \colorbox{red!2}{\strut Aides} \colorbox{red!3}{\strut Free} \colorbox{red!6}{\strut Coupons} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut Bargains} \colorbox{red!2}{\strut Newsletter} \colorbox{red!1}{\strut !} \colorbox{red!2}{\strut Sign} \colorbox{red!0}{\strut Up} \colorbox{red!0}{\strut By} \colorbox{red!1}{\strut Category} \colorbox{red!0}{\strut All} \colorbox{red!5}{\strut Online} \colorbox{red!6}{\strut Coupons} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Deals} \colorbox{red!4}{\strut Apparel} \colorbox{red!9}{\strut Deals} \colorbox{red!0}{\strut Shopping} \colorbox{red!2}{\strut Tips} \colorbox{red!3}{\strut Baby} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Toy} \colorbox{red!9}{\strut Deals} \colorbox{red!1}{\strut Beauty} 
}}}
\end{CJK*}

query: sore throat

98:throat, 94:sore, 58:caused, 32:pain, 29:symptoms, 24:strep, 24:means, 21:colds, 20:infections, 20:definition


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Departments} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Services} \colorbox{red!1}{\strut For} \colorbox{red!4}{\strut Patients} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Trials} \colorbox{red!3}{\strut Education} \colorbox{red!5}{\strut Find} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut Doctor} \colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut Encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut List} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut Topics} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut Page} \colorbox{red!8}{\strut Internal} \colorbox{red!9}{\strut Medicine} \colorbox{red!96}{\strut Sore} \colorbox{red!100}{\strut throat} \colorbox{red!96}{\strut Sore} \colorbox{red!100}{\strut throat} \colorbox{red!100}{\strut Throat} \colorbox{red!4}{\strut anatomy} \colorbox{red!24}{\strut Strep} \colorbox{red!100}{\strut throat} \colorbox{red!20}{\strut Definition} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!96}{\strut sore} \colorbox{red!100}{\strut throat} \colorbox{red!5}{\strut is} \colorbox{red!13}{\strut discomfort} \colorbox{red!4}{\strut ,} \colorbox{red!32}{\strut pain} \colorbox{red!4}{\strut ,} \colorbox{red!3}{\strut or} \colorbox{red!12}{\strut scratchiness} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!100}{\strut throat} \colorbox{red!5}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!96}{\strut sore} \colorbox{red!100}{\strut throat} \colorbox{red!3}{\strut often} \colorbox{red!8}{\strut makes} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut painful} \colorbox{red!4}{\strut to} \colorbox{red!7}{\strut swallow} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut Alternative} \colorbox{red!8}{\strut Names} \colorbox{red!0}{\strut .} \colorbox{red!100}{\strut Throat} \colorbox{red!2}{\strut -} \colorbox{red!96}{\strut sore} \colorbox{red!0}{\strut .} \colorbox{red!32}{\strut Pain} \colorbox{red!2}{\strut -} \colorbox{red!100}{\strut throat} \colorbox{red!4}{\strut Considerations} \colorbox{red!0}{\strut .} \colorbox{red!96}{\strut Sore} \colorbox{red!0}{\strut throats} \colorbox{red!0}{\strut are} \colorbox{red!13}{\strut common} \colorbox{red!5}{\strut .} \colorbox{red!2}{\strut Most} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut time} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut soreness} \colorbox{red!5}{\strut is} \colorbox{red!6}{\strut worse} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut morning} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut improves} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut day} \colorbox{red!2}{\strut progresses} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Like} \colorbox{red!21}{\strut colds} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut vast} \colorbox{red!0}{\strut majority} \colorbox{red!2}{\strut of} \colorbox{red!96}{\strut sore} \colorbox{red!0}{\strut throats} \colorbox{red!0}{\strut are} \colorbox{red!59}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!10}{\strut viral} \colorbox{red!20}{\strut infections} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!24}{\strut means} \colorbox{red!2}{\strut most} \colorbox{red!96}{\strut sore} \colorbox{red!0}{\strut throats} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut NOT} \colorbox{red!1}{\strut respond} \colorbox{red!4}{\strut to} \colorbox{red!12}{\strut antibiotics} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!5}{\strut people} \colorbox{red!2}{\strut have} \colorbox{red!1}{\strut a} \colorbox{red!7}{\strut mild} \colorbox{red!96}{\strut sore} \colorbox{red!100}{\strut throat} \colorbox{red!2}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut beginning} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut cold} \colorbox{red!5}{\strut .} \colorbox{red!7}{\strut When} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut nose} \colorbox{red!3}{\strut or} \colorbox{red!4}{\strut sinuses} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut infected} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut drainage} \colorbox{red!0}{\strut can} \colorbox{red!5}{\strut run} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut back} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!100}{\strut throat} \colorbox{red!2}{\strut and} \colorbox{red!8}{\strut irritate} \colorbox{red!0}{\strut it} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!2}{\strut at} \colorbox{red!5}{\strut night} \colorbox{red!5}{\strut .} \colorbox{red!3}{\strut Or} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!100}{\strut throat} \colorbox{red!0}{\strut itself} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut infected} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!6}{\strut viruses} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut cause} \colorbox{red!5}{\strut specific} \colorbox{red!10}{\strut types} \colorbox{red!2}{\strut of} \colorbox{red!96}{\strut sore} \colorbox{red!100}{\strut throat} \colorbox{red!5}{\strut .} \colorbox{red!1}{\strut For} \colorbox{red!6}{\strut example} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut Coxsackievirus} \colorbox{red!3}{\strut sometimes} \colorbox{red!0}{\strut causes} \colorbox{red!20}{\strut blisters} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!100}{\strut throat} \colorbox{red!4}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut late} \colorbox{red!4}{\strut summer} \colorbox{red!2}{\strut and} \colorbox{red!3}{\strut early} \colorbox{red!3}{\strut fall} \colorbox{red!5}{\strut .} \colorbox{red!6}{\strut Mono} \colorbox{red!2}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut flu} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut cause} \colorbox{red!5}{\strut specific} \colorbox{red!10}{\strut viral} \colorbox{red!100}{\strut throat} \colorbox{red!20}{\strut infections} \colorbox{red!5}{\strut .} \colorbox{red!24}{\strut Strep} \colorbox{red!100}{\strut throat} \colorbox{red!5}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut most} \colorbox{red!13}{\strut common} \colorbox{red!12}{\strut bacterial} \colorbox{red!0}{\strut cause} \colorbox{red!2}{\strut of} \colorbox{red!96}{\strut sore} \colorbox{red!100}{\strut throat} \colorbox{red!5}{\strut .} \colorbox{red!0}{\strut Because} \colorbox{red!24}{\strut strep} \colorbox{red!100}{\strut throat} \colorbox{red!0}{\strut can} \colorbox{red!2}{\strut occasionally} \colorbox{red!4}{\strut lead} \colorbox{red!4}{\strut to} \colorbox{red!5}{\strut rheumatic} \colorbox{red!9}{\strut fever} \colorbox{red!4}{\strut ,} \colorbox{red!12}{\strut antibiotics} \colorbox{red!0}{\strut are} \colorbox{red!5}{\strut given} \colorbox{red!5}{\strut .} \colorbox{red!24}{\strut Strep} \colorbox{red!100}{\strut throat} \colorbox{red!3}{\strut often} \colorbox{red!2}{\strut includes} \colorbox{red!1}{\strut a} \colorbox{red!9}{\strut fever} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut greater} \colorbox{red!2}{\strut than} \colorbox{red!3}{\strut 101F} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut ,} \colorbox{red!6}{\strut white} \colorbox{red!3}{\strut draining} \colorbox{red!4}{\strut patches} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!100}{\strut throat} \colorbox{red!4}{\strut ,} \colorbox{red!2}{\strut and} \colorbox{red!5}{\strut swollen} \colorbox{red!3}{\strut or} \colorbox{red!4}{\strut tender} \colorbox{red!6}{\strut lymph} \colorbox{red!5}{\strut glands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut neck} \colorbox{red!5}{\strut .} \colorbox{red!5}{\strut Children} \colorbox{red!3}{\strut may} \colorbox{red!2}{\strut have} \colorbox{red!1}{\strut a} \colorbox{red!8}{\strut headache} \colorbox{red!2}{\strut and} \colorbox{red!8}{\strut stomach} \colorbox{red!32}{\strut pain} \colorbox{red!5}{\strut .} \colorbox{red!1}{\strut A} \colorbox{red!96}{\strut sore} \colorbox{red!100}{\strut throat} \colorbox{red!5}{\strut is} \colorbox{red!0}{\strut less} \colorbox{red!4}{\strut likely} \colorbox{red!4}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!24}{\strut strep} \colorbox{red!100}{\strut throat} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut it} \colorbox{red!5}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut minor} \colorbox{red!5}{\strut part} \colorbox{red!2}{\strut of} \colorbox{red!1}{\strut a} \colorbox{red!3}{\strut typical} \colorbox{red!0}{\strut cold} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut runny} \colorbox{red!10}{\strut nose} \colorbox{red!4}{\strut ,} \colorbox{red!4}{\strut stuffy} \colorbox{red!5}{\strut ears} \colorbox{red!4}{\strut ,} 
}}}
\end{CJK*}

98:throat, 97:sore, 45:caused, 39:disease, 27:pharynx, 22:pharyngitis, 21:health, 19:effect, 18:inflammation, 14:virus


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!68}{\strut Sore} \colorbox{red!68}{\strut throat} \colorbox{red!0}{\strut From} \colorbox{red!14}{\strut Health} \colorbox{red!8}{\strut Encyclopedia} \colorbox{red!5}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut navigation} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut search} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut edit} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Use} \colorbox{red!15}{\strut pharyngitis} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut edit} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Facts} \colorbox{red!4}{\strut A} \colorbox{red!68}{\strut sore} \colorbox{red!68}{\strut throat} \colorbox{red!2}{\strut is} \colorbox{red!9}{\strut partly} \colorbox{red!4}{\strut a} \colorbox{red!27}{\strut disease} \colorbox{red!3}{\strut in} \colorbox{red!4}{\strut itself} \colorbox{red!2}{\strut and} \colorbox{red!9}{\strut partly} \colorbox{red!2}{\strut an} \colorbox{red!13}{\strut effect} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut other} \colorbox{red!0}{\strut diseases} \colorbox{red!2}{\strut such} \colorbox{red!2}{\strut as} \colorbox{red!8}{\strut flu} \colorbox{red!2}{\strut and} \colorbox{red!7}{\strut glandular} \colorbox{red!9}{\strut fever} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut A} \colorbox{red!68}{\strut sore} \colorbox{red!68}{\strut throat} \colorbox{red!12}{\strut inflammation} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!5}{\strut fauces} \colorbox{red!2}{\strut and} \colorbox{red!18}{\strut pharynx} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut can} \colorbox{red!1}{\strut be} \colorbox{red!31}{\strut caused} \colorbox{red!1}{\strut by} \colorbox{red!0}{\strut either} \colorbox{red!4}{\strut a} \colorbox{red!9}{\strut virus} \colorbox{red!2}{\strut or} \colorbox{red!4}{\strut a} \colorbox{red!7}{\strut bacterium} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut Retrieved} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut http} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut www.steadyhealth.comencyclopediaSorethroat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Would} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut discuss} \colorbox{red!2}{\strut or} \colorbox{red!3}{\strut post} \colorbox{red!2}{\strut question} \colorbox{red!2}{\strut about} \colorbox{red!68}{\strut Sore} \colorbox{red!68}{\strut throat} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut !} \colorbox{red!5}{\strut Views} \colorbox{red!4}{\strut Article} \colorbox{red!7}{\strut Edit} \colorbox{red!3}{\strut Personal} \colorbox{red!3}{\strut tools} \colorbox{red!1}{\strut Log} \colorbox{red!3}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut create} \colorbox{red!3}{\strut account} \colorbox{red!5}{\strut Search} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut Navigator} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Discussion} \colorbox{red!2}{\strut Boards} \colorbox{red!0}{\strut Free} \colorbox{red!4}{\strut Blogs} \colorbox{red!3}{\strut Pregnancy} \colorbox{red!2}{\strut Tickers} \colorbox{red!0}{\strut This} \colorbox{red!2}{\strut page} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut last} \colorbox{red!2}{\strut modified} \colorbox{red!0}{\strut 0932} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 20} \colorbox{red!2}{\strut September} \colorbox{red!0}{\strut 2007} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!2}{\strut page} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!2}{\strut accessed} \colorbox{red!0}{\strut 3,040} \colorbox{red!3}{\strut times} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut Privacy} \colorbox{red!4}{\strut policy} \colorbox{red!2}{\strut About} \colorbox{red!14}{\strut Health} \colorbox{red!8}{\strut Encyclopedia} \colorbox{red!2}{\strut Disclaimers} 
}}}
\end{CJK*}

query: ontario california airport

98:airport, 96:ontario, 41:ont, 35:la, 34:california, 27:canada, 24:airlines, 23:international, 21:location, 21:kont


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut LAOntario} \colorbox{red!22}{\strut International} \colorbox{red!96}{\strut Airport} \colorbox{red!0}{\strut From} \colorbox{red!2}{\strut Wikipedia} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut L.A.Ontario} \colorbox{red!96}{\strut Airport} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Jump} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut navigation} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut search} \colorbox{red!1}{\strut This} \colorbox{red!2}{\strut article} \colorbox{red!1}{\strut is} \colorbox{red!4}{\strut about} \colorbox{red!2}{\strut an} \colorbox{red!96}{\strut airport} \colorbox{red!4}{\strut in} \colorbox{red!33}{\strut California} \colorbox{red!4}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!11}{\strut United} \colorbox{red!17}{\strut States} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut For} \colorbox{red!0}{\strut airports} \colorbox{red!4}{\strut in} \colorbox{red!94}{\strut Ontario} \colorbox{red!2}{\strut ,} \colorbox{red!26}{\strut Canada} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!2}{\strut List} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut airports} \colorbox{red!4}{\strut in} \colorbox{red!26}{\strut Canada} \colorbox{red!2}{\strut .} \colorbox{red!0}{\strut LAOntario} \colorbox{red!22}{\strut International} \colorbox{red!96}{\strut Airport} \colorbox{red!7}{\strut IATA} \colorbox{red!2}{\strut .} \colorbox{red!40}{\strut ONT} \colorbox{red!9}{\strut ICAO} \colorbox{red!2}{\strut .} \colorbox{red!20}{\strut KONT} \colorbox{red!9}{\strut FAA} \colorbox{red!2}{\strut .} \colorbox{red!40}{\strut ONT} \colorbox{red!2}{\strut Summary} \colorbox{red!96}{\strut Airport} \colorbox{red!14}{\strut type} \colorbox{red!5}{\strut Public} \colorbox{red!4}{\strut Owner} \colorbox{red!13}{\strut Los} \colorbox{red!12}{\strut Angeles} \colorbox{red!6}{\strut World} \colorbox{red!0}{\strut Airports} \colorbox{red!6}{\strut Serves} \colorbox{red!94}{\strut Ontario} \colorbox{red!2}{\strut ,} \colorbox{red!33}{\strut California} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut Inland} \colorbox{red!5}{\strut Empire} \colorbox{red!2}{\strut ,} \colorbox{red!33}{\strut California} \colorbox{red!20}{\strut Location} \colorbox{red!94}{\strut Ontario} \colorbox{red!2}{\strut ,} \colorbox{red!33}{\strut California} \colorbox{red!3}{\strut Elevation} \colorbox{red!4}{\strut AMSL} \colorbox{red!2}{\strut 944} \colorbox{red!0}{\strut ft} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut 288} \colorbox{red!0}{\strut m} \colorbox{red!4}{\strut Coordinates} \colorbox{red!0}{\strut 340322N} \colorbox{red!0}{\strut 1173604W} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 34.05611N} \colorbox{red!0}{\strut 117.60111W} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 34.05611} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -117.60111} \colorbox{red!0}{\strut Website} \colorbox{red!0}{\strut www.lawa.orgont} \colorbox{red!10}{\strut Runways} \colorbox{red!5}{\strut Direction} \colorbox{red!1}{\strut Length} \colorbox{red!1}{\strut Surface} \colorbox{red!0}{\strut ft} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut 8L26R} \colorbox{red!0}{\strut 12,197} \colorbox{red!0}{\strut 3,718} \colorbox{red!0}{\strut Concrete} \colorbox{red!0}{\strut 8R26L} \colorbox{red!0}{\strut 10,200} \colorbox{red!0}{\strut 3,109} \colorbox{red!0}{\strut Concrete} \colorbox{red!0}{\strut Statistics} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 2006} \colorbox{red!2}{\strut .} \colorbox{red!7}{\strut Aircraft} \colorbox{red!7}{\strut operations} \colorbox{red!0}{\strut 136,410} \colorbox{red!3}{\strut Based} \colorbox{red!7}{\strut aircraft} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut Source} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut Federal} \colorbox{red!3}{\strut Aviation} \colorbox{red!1}{\strut Administration} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Terminal} \colorbox{red!1}{\strut 2} \colorbox{red!3}{\strut at} \colorbox{red!40}{\strut ONT} \colorbox{red!0}{\strut LAOntario} \colorbox{red!22}{\strut International} \colorbox{red!96}{\strut Airport} \colorbox{red!1}{\strut .} \colorbox{red!7}{\strut IATA} \colorbox{red!2}{\strut .} \colorbox{red!40}{\strut ONT} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut ICAO} \colorbox{red!2}{\strut .} \colorbox{red!20}{\strut KONT} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut FAA} \colorbox{red!3}{\strut LID} \colorbox{red!2}{\strut .} \colorbox{red!40}{\strut ONT} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut .} \colorbox{red!3}{\strut formerly} \colorbox{red!94}{\strut Ontario} \colorbox{red!22}{\strut International} \colorbox{red!96}{\strut Airport} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut is} \colorbox{red!1}{\strut a} \colorbox{red!5}{\strut public} \colorbox{red!96}{\strut airport} \colorbox{red!0}{\strut located} \colorbox{red!1}{\strut two} \colorbox{red!4}{\strut miles} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!2}{\strut km} \colorbox{red!2}{\strut .} \colorbox{red!5}{\strut east} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!4}{\strut central} \colorbox{red!2}{\strut business} \colorbox{red!2}{\strut district} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut CBD} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut of} \colorbox{red!94}{\strut Ontario} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut a} \colorbox{red!10}{\strut city} \colorbox{red!4}{\strut in} \colorbox{red!3}{\strut San} \colorbox{red!0}{\strut Bernardino} \colorbox{red!7}{\strut County} \colorbox{red!2}{\strut ,} \colorbox{red!33}{\strut California} \colorbox{red!2}{\strut ,} \colorbox{red!8}{\strut USA} \colorbox{red!2}{\strut .} \colorbox{red!1}{\strut This} \colorbox{red!96}{\strut airport} \colorbox{red!1}{\strut is} \colorbox{red!11}{\strut owned} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut operated} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut the} \colorbox{red!13}{\strut Los} \colorbox{red!12}{\strut Angeles} \colorbox{red!6}{\strut World} \colorbox{red!0}{\strut Airports} \colorbox{red!2}{\strut ,} \colorbox{red!2}{\strut an} \colorbox{red!4}{\strut agency} \colorbox{red!2}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!10}{\strut City} \colorbox{red!2}{\strut of} \colorbox{red!13}{\strut Los} \colorbox{red!12}{\strut Angeles} \colorbox{red!2}{\strut .} \colorbox{red!4}{\strut In} \colorbox{red!0}{\strut 2008} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut 6.2} \colorbox{red!0}{\strut million} \colorbox{red!5}{\strut passengers} \colorbox{red!0}{\strut used} \colorbox{red!2}{\strut the} \colorbox{red!96}{\strut airport} \colorbox{red!2}{\strut ,} \colorbox{red!1}{\strut a} \colorbox{red!0}{\strut decline} \colorbox{red!2}{\strut of} \colorbox{red!0}{\strut 13.5} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!96}{\strut airport} \colorbox{red!1}{\strut is} \colorbox{red!0}{\strut dominated} \colorbox{red!0}{\strut by} \colorbox{red!4}{\strut Southwest} \colorbox{red!23}{\strut Airlines} \colorbox{red!5}{\strut who} \colorbox{red!4}{\strut carried} \colorbox{red!0}{\strut 49.38} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut of} \colorbox{red!5}{\strut passengers} \colorbox{red!4}{\strut in} \colorbox{red!0}{\strut 2007} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut The} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut four} \colorbox{red!23}{\strut airlines} \colorbox{red!4}{\strut in} \colorbox{red!2}{\strut the} \colorbox{red!0}{\strut top} \colorbox{red!1}{\strut five} \colorbox{red!0}{\strut were} \colorbox{red!11}{\strut United} \colorbox{red!0}{\strut AirlinesUnited} \colorbox{red!6}{\strut Express} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 8.64} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!9}{\strut Delta} \colorbox{red!6}{\strut Air} \colorbox{red!4}{\strut Lines} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 7.93} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!3}{\strut US} \colorbox{red!4}{\strut Airways} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 7.08} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut American} \colorbox{red!23}{\strut Airlines} \colorbox{red!1}{\strut .} \colorbox{red!0}{\strut 6.18} \colorbox{red!1}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!2}{\strut .} \colorbox{red!3}{\strut Expressjet} \colorbox{red!0}{\strut operated} \colorbox{red!1}{\strut a} \colorbox{red!2}{\strut hub} \colorbox{red!3}{\strut at} 
}}}
\end{CJK*}

92:airports, 82:ontario, 72:california, 26:aviation, 23:state, 18:new, 17:usa, 15:maine, 14:runways, 14:photovalet


\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut PHOTOVALET} \colorbox{red!1}{\strut .} \colorbox{red!4}{\strut tm} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Enter} \colorbox{red!2}{\strut search} \colorbox{red!2}{\strut term} \colorbox{red!4}{\strut PHOTOVAULT} \colorbox{red!10}{\strut AVIATION} \colorbox{red!4}{\strut Museum} \colorbox{red!37}{\strut Airports} \colorbox{red!0}{\strut .} \colorbox{red!33}{\strut Ontario} \colorbox{red!29}{\strut California} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut Customs} \colorbox{red!1}{\strut ,} \colorbox{red!4}{\strut Traffic} \colorbox{red!2}{\strut Control} \colorbox{red!1}{\strut ,} \colorbox{red!5}{\strut Runways} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut .} \colorbox{red!5}{\strut images} \colorbox{red!1}{\strut by} \colorbox{red!2}{\strut Wernher} \colorbox{red!2}{\strut Krutein} \colorbox{red!1}{\strut and} \colorbox{red!4}{\strut PHOTOVAULT} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut contains} \colorbox{red!2}{\strut samples} \colorbox{red!1}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!3}{\strut picture} \colorbox{red!3}{\strut files} \colorbox{red!37}{\strut Airports} \colorbox{red!0}{\strut .} \colorbox{red!33}{\strut Ontario} \colorbox{red!29}{\strut California} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut These} \colorbox{red!0}{\strut pictures} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut available} \colorbox{red!1}{\strut for} \colorbox{red!2}{\strut licensing} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!2}{\strut media} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut For} \colorbox{red!2}{\strut Pricing} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut General} \colorbox{red!2}{\strut Guidelines} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!2}{\strut Delivery} \colorbox{red!1}{\strut information} \colorbox{red!0}{\strut click} \colorbox{red!1}{\strut here} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut You} \colorbox{red!0}{\strut may} \colorbox{red!2}{\strut contact} \colorbox{red!1}{\strut us} \colorbox{red!1}{\strut thru} \colorbox{red!2}{\strut email} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut by} \colorbox{red!2}{\strut phone} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut more} \colorbox{red!1}{\strut information} \colorbox{red!1}{\strut on} \colorbox{red!1}{\strut the} \colorbox{red!0}{\strut use} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut These} \colorbox{red!0}{\strut pictures} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut and} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut others} \colorbox{red!1}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!3}{\strut files} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut shown} \colorbox{red!1}{\strut here} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Please} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut ask} \colorbox{red!1}{\strut us} \colorbox{red!1}{\strut for} \colorbox{red!1}{\strut free} \colorbox{red!0}{\strut use} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut These} \colorbox{red!0}{\strut pictures} \colorbox{red!1}{\strut !} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut .} \colorbox{red!1}{\strut Included} \colorbox{red!1}{\strut in} \colorbox{red!1}{\strut the} \colorbox{red!4}{\strut PHOTOVAULT} \colorbox{red!10}{\strut AVIATION} \colorbox{red!4}{\strut Museum} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut Airport} \colorbox{red!5}{\strut images} \colorbox{red!1}{\strut from} \colorbox{red!0}{\strut -} \colorbox{red!6}{\strut USA} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Adak} \colorbox{red!1}{\strut ,} \colorbox{red!3}{\strut Albuquerque} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Alton} \colorbox{red!5}{\strut Bay} \colorbox{red!7}{\strut New} \colorbox{red!2}{\strut Hampshire} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Anchorage} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Atlanta} \colorbox{red!1}{\strut Hartsfield} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Austin} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Bakersfield} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Baltimore} \colorbox{red!3}{\strut Washington} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Boise} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Boulder} \colorbox{red!3}{\strut Nevada} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Burbank} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Calistoga} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Canyonlands} \colorbox{red!3}{\strut Field} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Catalina} \colorbox{red!3}{\strut Island} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Chandler} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Charlotte} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Charleston} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Chester} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Chicago} \colorbox{red!1}{\strut Midway} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Chicago} \colorbox{red!0}{\strut Ohare} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Cincinnati} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Concord} \colorbox{red!29}{\strut California} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Dallas} \colorbox{red!2}{\strut Fort} \colorbox{red!2}{\strut Worth} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Dallas} \colorbox{red!0}{\strut Love} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Denver} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Detroit} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Dulles} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut El} \colorbox{red!1}{\strut Paso} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut El} \colorbox{red!1}{\strut Toro} \colorbox{red!29}{\strut California} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Fairbanks} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Fortuna} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Fremont} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Fresno} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut General} \colorbox{red!1}{\strut Mitchell} \colorbox{red!1}{\strut Intl} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Grand} \colorbox{red!1}{\strut Junction} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Gulfport} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Hailey} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Half} \colorbox{red!1}{\strut Moon} \colorbox{red!5}{\strut Bay} \colorbox{red!29}{\strut California} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Hampton} \colorbox{red!7}{\strut New} \colorbox{red!1}{\strut H} \colorbox{red!0}{\strut ampshire} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Hayward} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Hilo} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Honolulu} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Houston} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Jackson} \colorbox{red!0}{\strut Hole} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut F.} \colorbox{red!1}{\strut Kennedy} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut John} \colorbox{red!1}{\strut Wayne} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Kahului} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Kansas} \colorbox{red!4}{\strut City} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Kauai} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Knox} \colorbox{red!2}{\strut County} \colorbox{red!6}{\strut Maine} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Kona} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut La} \colorbox{red!0}{\strut Guardia} \colorbox{red!1}{\strut ,} \colorbox{red!2}{\strut Lake} \colorbox{red!1}{\strut Tahoe} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Las} \colorbox{red!1}{\strut Vegas} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Lawrence} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Lebanon} \colorbox{red!7}{\strut New} \colorbox{red!2}{\strut Hampshire} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Little} \colorbox{red!2}{\strut Rock} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Livermore} \colorbox{red!1}{\strut ,} \colorbox{red!0}{\strut Logan} \colorbox{red!1}{\strut ,} \colorbox{red!1}{\strut Long} \colorbox{red!2}{\strut Beach} \colorbox{red!1}{\strut ,} 
}}}
\end{CJK*}



==> sections/visualization/loss.tex <==
query: what constitutional clause prohibits a state from drawing unreasonable distinctions between its own residents and those of persons living in other states

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Chapter} \colorbox{red!0}{\strut 4} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut Quiz} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 47} \colorbox{red!0}{\strut terms} \colorbox{red!0}{\strut hannahmcclary8Chapter} \colorbox{red!0}{\strut 4} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut QuizLearn} \colorbox{red!0}{\strut Flashcards} \colorbox{red!0}{\strut Write} \colorbox{red!0}{\strut Spell} \colorbox{red!0}{\strut Test} \colorbox{red!0}{\strut MatchGravityAdvertisementUpgrade} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut remove} \colorbox{red!0}{\strut adsLike} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut study} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Create} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut it.Create} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut accountMaybe} \colorbox{red!0}{\strut laterSortThe} \colorbox{red!0}{\strut 10th} \colorbox{red!0}{\strut Amendment} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut division} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut powersFederalism} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut government} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut written} \colorbox{red!1}{\strut constitution} \colorbox{red!0}{\strut does} \colorbox{red!4}{\strut what} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut divides} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut powers} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut government} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut national} \colorbox{red!6}{\strut government} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut regional} \colorbox{red!0}{\strut governmentsWhat} \colorbox{red!6}{\strut powers} \colorbox{red!3}{\strut given} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut spelled} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Constitution} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut expressed} \colorbox{red!0}{\strut powersWhich} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut NOT} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut concern} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Framers} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut limited} \colorbox{red!6}{\strut government} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut strong} \colorbox{red!0}{\strut central} \colorbox{red!6}{\strut government} \colorbox{red!0}{\strut helps} \colorbox{red!0}{\strut ensure} \colorbox{red!0}{\strut personal} \colorbox{red!0}{\strut freedom.The} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut powers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut expressed} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut implied} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut inherent} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut delegatedWhat} \colorbox{red!6}{\strut powers} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut exercised} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut exclusive} \colorbox{red!0}{\strut powersWhat} \colorbox{red!6}{\strut powers} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut given} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut national} \colorbox{red!6}{\strut government} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut sovereign} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut inherent} \colorbox{red!0}{\strut powersWhat} \colorbox{red!6}{\strut powers} \colorbox{red!3}{\strut given} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut reasonably} \colorbox{red!0}{\strut suggested} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Constitution} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut implied} \colorbox{red!0}{\strut powersWhat} \colorbox{red!6}{\strut powers} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut exercised} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut concurrent} \colorbox{red!0}{\strut powersWhat} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut powers} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Constitution} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut grant} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut deny} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut reserved} \colorbox{red!0}{\strut powersWhich} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut NOT} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut domestic} \colorbox{red!0}{\strut Violence} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Constitution} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut invasionWhat} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut grants} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut federal} \colorbox{red!0}{\strut money} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut States} \colorbox{red!0}{\strut andor} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut cities} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut counties} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut units} \colorbox{red!0}{\strut called} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut grants-in-aid} \colorbox{red!0}{\strut programsWhat} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut grants} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut broadly} \colorbox{red!0}{\strut defined} \colorbox{red!0}{\strut purpose} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut health} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut services} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut welfare} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut block} \colorbox{red!0}{\strut grantsWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut restriction} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Constitution} \colorbox{red!0}{\strut places} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut National} \colorbox{red!6}{\strut Government} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut admission} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut states} \colorbox{red!0}{\strut into} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut clauses} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!5}{\strut Constitution} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedianavigation} \colorbox{red!0}{\strut searchThis} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut citations} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut verification} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut improve} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut citations} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reliable} \colorbox{red!0}{\strut sources} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Unsourced} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut challenged} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut removed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut February} \colorbox{red!0}{\strut 2017} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Learn} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut remove} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut template} \colorbox{red!0}{\strut message} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!5}{\strut Constitution} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut its} \colorbox{red!2}{\strut amendments} \colorbox{red!0}{\strut comprise} \colorbox{red!0}{\strut hundreds} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut clauses} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut outline} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut functioning} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!1}{\strut Federal} \colorbox{red!1}{\strut Government} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut political} \colorbox{red!0}{\strut relationship} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut states} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut national} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut affect} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!1}{\strut States} \colorbox{red!1}{\strut federal} \colorbox{red!0}{\strut court} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut interprets} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut law} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut When} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut particular} \colorbox{red!5}{\strut clause} \colorbox{red!0}{\strut becomes} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut contentious} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut law} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ease} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut reference.Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!5}{\strut Clauses} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Articles2} \colorbox{red!5}{\strut Clauses} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Amendments2.1} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut Amendment2.2} \colorbox{red!0}{\strut Fourth} \colorbox{red!0}{\strut Amendment2.3} \colorbox{red!0}{\strut Fifth} \colorbox{red!0}{\strut Amendment2.4} \colorbox{red!0}{\strut Sixth} \colorbox{red!0}{\strut Amendment2.5} \colorbox{red!0}{\strut Eighth} \colorbox{red!0}{\strut Amendment2.6} \colorbox{red!0}{\strut Fourteenth} \colorbox{red!0}{\strut Amendment2.7} \colorbox{red!0}{\strut Recurring} \colorbox{red!0}{\strut Clauses3} \colorbox{red!0}{\strut References4} \colorbox{red!0}{\strut NotesClauses} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Articles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut Name} \colorbox{red!0}{\strut Article} \colorbox{red!0}{\strut Section} \colorbox{red!0}{\strut Clause1808} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut 1Admissions} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut IV} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut 1Advice} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Consent} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut II} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 2Appointments} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut II} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 2Arisings} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut III} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 1Basket} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut 18Case} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Controversy} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut III} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 1Coefficient} \colorbox{red!5}{\strut Clause} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut 18Comity} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut IV} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 1Commerce} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut 3Compact} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut 3Contract} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut 1Copyright} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut 8Diversity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Citizenship} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut III} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 1Elastic} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut 18Emoluments} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut 2Emolument} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut 8Enclave} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut 17Excepting} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut II} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 2Exceptions} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut III} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 2Export} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut 2Extradition} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut IV} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 2Faithful} \colorbox{red!0}{\strut Execution} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut II} \colorbox{red!0}{\strut 3Faithfully} \colorbox{red!0}{\strut Executed} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut II} \colorbox{red!0}{\strut 3Foreign} \colorbox{red!0}{\strut Commerce} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut 3Fugitive} \colorbox{red!0}{\strut Slave} \colorbox{red!5}{\strut Clause} \colorbox{red!0}{\strut IV} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut 3Full} \colorbox{red!0}{\strut Faith} \colorbox{red!0}{\strut and} 
}}}
\end{CJK*}

query: what is diflorasone diacetate cream used for

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Diflorasone} \colorbox{red!0}{\strut Diacetate} \colorbox{red!0}{\strut Uses} \colorbox{red!0}{\strut .} \colorbox{red!37}{\strut Skin} \colorbox{red!0}{\strut ChannelTopicsAllergic} \colorbox{red!4}{\strut Contact} \colorbox{red!0}{\strut DermatitisAlopecia} \colorbox{red!0}{\strut AreataAtopic} \colorbox{red!0}{\strut DermatitisBody} \colorbox{red!0}{\strut LiceBreast} \colorbox{red!0}{\strut CellulitisCellulitisContact} \colorbox{red!0}{\strut DermatitisDermatitis} \colorbox{red!0}{\strut HerpetiformisFacial} \colorbox{red!0}{\strut CellulitisHot} \colorbox{red!0}{\strut Tub} \colorbox{red!0}{\strut RashImpetigoIrritant} \colorbox{red!4}{\strut Contact} \colorbox{red!0}{\strut DermatitisLeg} \colorbox{red!0}{\strut CellulitisLiceLichen} \colorbox{red!0}{\strut SclerosusOrbital} \colorbox{red!0}{\strut CellulitisPerianal} \colorbox{red!0}{\strut CellulitisPeriorbital} \colorbox{red!0}{\strut CellulitisSkinSkin} \colorbox{red!0}{\strut ExamStaph} \colorbox{red!0}{\strut InfectionSwimmer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut ItchVitiligoMedicationsAbobotulinumtoxinAAcitretinAdapaleneBenzoyl} \colorbox{red!0}{\strut PeroxideAlclometasoneAlefaceptAltabaxAmcinonideAquaphorAvageAzelaic} \colorbox{red!0}{\strut Acid} \colorbox{red!0}{\strut GelAzficel-TBenzyl} \colorbox{red!0}{\strut Alcohol} \colorbox{red!0}{\strut LotionBetamethasone} \colorbox{red!0}{\strut Valerate} \colorbox{red!0}{\strut FoamBotulinum} \colorbox{red!4}{\strut Toxin} \colorbox{red!4}{\strut Type} \colorbox{red!0}{\strut ABrimonidine} \colorbox{red!0}{\strut GelCalcipotrieneCalcipotrieneBetamethasone} \colorbox{red!0}{\strut DipropionateCalcitriol} \colorbox{red!0}{\strut OintmentCapexCinryzeClemastineClindamycinBenzoyl} \colorbox{red!0}{\strut PeroxideClobetasol} \colorbox{red!0}{\strut PropionateClobetasol} \colorbox{red!0}{\strut Propionate} \colorbox{red!0}{\strut FoamClobexCordran} \colorbox{red!0}{\strut SP} \colorbox{red!0}{\strut CreamCutivate} \colorbox{red!0}{\strut LotionDacarbazineDecadronDenileukin} \colorbox{red!0}{\strut DiftitoxDermatopDesonateDesonide} \colorbox{red!0}{\strut CreamDesoximetasoneDesoximetasone} \colorbox{red!0}{\strut SprayDiclofenac} \colorbox{red!0}{\strut GelDiflorasone} \colorbox{red!0}{\strut DiacetateDiflorasone} \colorbox{red!0}{\strut Emollient} \colorbox{red!0}{\strut CreamElidelErythromycinBenzoyl} \colorbox{red!0}{\strut PeroxideExtinaFirazyrFluocinolone} \colorbox{red!0}{\strut OilFluocinonideFlurandrenolide} \colorbox{red!0}{\strut LotionFluticasone} \colorbox{red!0}{\strut Propionate} \colorbox{red!0}{\strut CreamHalogHydrocortisone} \colorbox{red!0}{\strut ButyrateHydrogen} \colorbox{red!0}{\strut PeroxideHydroxyzineImiquimodIncobotulinumtoxinAInjectable} \colorbox{red!0}{\strut Poly-L} \colorbox{red!0}{\strut Lactic} \colorbox{red!0}{\strut AcidIstodaxIvermectin} \colorbox{red!0}{\strut LotionKalbitorKenalog} \colorbox{red!0}{\strut OintmentLamisilLidexMangosteenMetronidazole} \colorbox{red!0}{\strut GelMometasoneMometasone} \colorbox{red!0}{\strut Furoate} \colorbox{red!0}{\strut OintmentMupirocinNeosporinOnabotulinumtoxinAPicatoPromethazineProtopicRheumatrexSpinosadTazarotene} \colorbox{red!0}{\strut FoamTerbinafineTopical} \colorbox{red!0}{\strut Fluticasone} \colorbox{red!0}{\strut PropionateTriamcinoloneTriamcinolone} \colorbox{red!0}{\strut Acetonide} \colorbox{red!0}{\strut CreamUltravateUstekinumabVerdesoVorinostatXolegelZyclaraAdvertisementQuicklinksSkinLiceCellulitisVitiligoAlopecia} \colorbox{red!0}{\strut AreataLichen} \colorbox{red!0}{\strut SclerosisAtopic} \colorbox{red!0}{\strut DermatitisContact} \colorbox{red!0}{\strut DermatitisBody} \colorbox{red!0}{\strut LiceLamisilTriamcinoloneMangosteenHydroxyzinePromethazineStaph} \colorbox{red!0}{\strut InfectionImpetigoHydrogen} \colorbox{red!0}{\strut PeroxideRelated} \colorbox{red!0}{\strut ChannelsPsoriasisRosaceaSkin} \colorbox{red!0}{\strut CancerScabiesKidsPregnancyAdvertisementTweetSkin} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Diflorasone} \colorbox{red!0}{\strut Diacetate} \colorbox{red!0}{\strut UsesDiflorasone} \colorbox{red!0}{\strut Diacetate} \colorbox{red!0}{\strut UsesYour} \colorbox{red!0}{\strut healthcare} \colorbox{red!0}{\strut provider} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut recommend} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut diflorasone} \colorbox{red!0}{\strut diacetate} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut relieve} \colorbox{red!0}{\strut inflammation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut itching} \colorbox{red!0}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut various} \colorbox{red!37}{\strut skin} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Specifically} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut topical} \colorbox{red!37}{\strut skin} \colorbox{red!0}{\strut medicine} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut approved} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut treating} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut dermatitis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eczema} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut poison} \colorbox{red!0}{\strut ivy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut works} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut suppressing} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut overactive} \colorbox{red!0}{\strut immune} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut reducing} \colorbox{red!0}{\strut inflammation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut approved} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut adults} \colorbox{red!0}{\strut only.Interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Discount} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Diflorasone} \colorbox{red!0}{\strut Diacetate} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Our} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut DiscountRx} \colorbox{red!0}{\strut savings} \colorbox{red!0}{\strut card} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut family} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut money} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut prescriptions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut card} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut accepted} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut major} \colorbox{red!0}{\strut chain} \colorbox{red!0}{\strut pharmacies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut nationwide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Enter} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut address} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut receive} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut savings} \colorbox{red!0}{\strut card.Enter} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut NameEnter} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut AddressCLICK} \colorbox{red!0}{\strut HERE} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut eMedTV.comWhat} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut Diflorasone} \colorbox{red!0}{\strut Diacetate} \colorbox{red!0}{\strut Used} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Diflorasone} \colorbox{red!0}{\strut diacetate} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut prescription} \colorbox{red!37}{\strut skin} \colorbox{red!0}{\strut medication} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut treat} \colorbox{red!0}{\strut inflammation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut itching} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut wide} \colorbox{red!0}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Such} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Atopic} \colorbox{red!0}{\strut dermatitisContact} \colorbox{red!0}{\strut dermatitisEczemaPsoriasisPoison} \colorbox{red!0}{\strut ivySeborrhea.Specifically} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut diflorasone} \colorbox{red!0}{\strut diacetate} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut approved} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut treat} \colorbox{red!0}{\strut any} \colorbox{red!37}{\strut skin} \colorbox{red!0}{\strut condition} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut responsive} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut corticosteroids} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut diflorasone} \colorbox{red!0}{\strut diacetate} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut corticosteroid} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut broad} \colorbox{red!0}{\strut indication} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut medication} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut probably} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut treating} \colorbox{red!0}{\strut psoriasis} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut severe} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Label} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut DIFLORASONE} \colorbox{red!0}{\strut DIACETATE-} \colorbox{red!9}{\strut diflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!5}{\strut cream} \colorbox{red!0}{\strut NDC} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 51672-1296-1} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 51672-1296-2} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 51672-1296-3Packager} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Taro} \colorbox{red!0}{\strut Pharmaceuticals} \colorbox{red!0}{\strut U.S.A.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.Category} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut HUMAN} \colorbox{red!1}{\strut PRESCRIPTION} \colorbox{red!1}{\strut DRUG} \colorbox{red!0}{\strut LABELDEA} \colorbox{red!0}{\strut Schedule} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NoneMarketing} \colorbox{red!0}{\strut Status} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Abbreviated} \colorbox{red!0}{\strut New} \colorbox{red!1}{\strut Drug} \colorbox{red!0}{\strut ApplicationDrug} \colorbox{red!1}{\strut Label} \colorbox{red!0}{\strut InformationUpdated} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 31} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2015If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut consumer} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut patient} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut version.Download} \colorbox{red!1}{\strut DRUG} \colorbox{red!1}{\strut LABEL} \colorbox{red!0}{\strut INFO} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PDF} \colorbox{red!0}{\strut XML} \colorbox{red!0}{\strut Official} \colorbox{red!1}{\strut Label} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Printer} \colorbox{red!0}{\strut Friendly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut SectionsSPL} \colorbox{red!0}{\strut UNCLASSIFIED} \colorbox{red!0}{\strut SECTIONRx} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut Only} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Not} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Ophthalmic} \colorbox{red!0}{\strut Use.DESCRIPTIONDiflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!5}{\strut cream} \colorbox{red!1}{\strut USP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 0.05} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut contains} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut active} \colorbox{red!0}{\strut compound} \colorbox{red!9}{\strut diflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut synthetic} \colorbox{red!2}{\strut corticosteroid} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut topical} \colorbox{red!0}{\strut dermatological} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Chemically} \colorbox{red!0}{\strut ,} \colorbox{red!9}{\strut diflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut CLINICAL} \colorbox{red!0}{\strut PHARMACOLOGYLike} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut topical} \colorbox{red!1}{\strut corticosteroids} \colorbox{red!0}{\strut ,} \colorbox{red!9}{\strut diflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut anti-inflammatory} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anti-pruritic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut vasoconstrictive} \colorbox{red!0}{\strut actions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut mechanism} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut anti-inflammatory} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut topical} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut INDICATION} \colorbox{red!0}{\strut AND} \colorbox{red!0}{\strut USAGEDiflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!5}{\strut cream} \colorbox{red!1}{\strut USP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 0.05} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut potency} \colorbox{red!2}{\strut corticosteroid} \colorbox{red!0}{\strut indicated} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut relief} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut inflammatory} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut pruritic} \colorbox{red!0}{\strut manifestations} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut corticosteroid-responsive} \colorbox{red!0}{\strut dermatoses} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut CONTRAINDICATIONSDiflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!5}{\strut cream} \colorbox{red!1}{\strut USP} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut contraindicated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut history} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut hypersensitivity} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut components} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut preparation.PRECAUTIONSGeneral} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Systemic} \colorbox{red!0}{\strut absorption} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut topical} \colorbox{red!1}{\strut corticosteroids} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut produce} \colorbox{red!0}{\strut reversible} \colorbox{red!0}{\strut hypothalamic-pituitary-adrenal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut HPA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut axis} \colorbox{red!0}{\strut suppression} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut potential} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut ADVERSE} \colorbox{red!0}{\strut REACTIONSThe} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut local} \colorbox{red!1}{\strut adverse} \colorbox{red!0}{\strut reactions} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut infrequently} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut topical} \colorbox{red!1}{\strut corticosteroids} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut occur} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut frequently} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut occlusive} \colorbox{red!0}{\strut dressings} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut OVERDOSAGETopically} \colorbox{red!0}{\strut applied} \colorbox{red!9}{\strut diflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!5}{\strut cream} \colorbox{red!1}{\strut USP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 0.05} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut absorbed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut sufficient} \colorbox{red!0}{\strut amounts} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut produce} \colorbox{red!0}{\strut systemic} \colorbox{red!0}{\strut effects} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut PRECAUTIONS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .DOSAGE} \colorbox{red!0}{\strut AND} \colorbox{red!0}{\strut ADMINISTRATIONDiflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!5}{\strut cream} \colorbox{red!1}{\strut USP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 0.05} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut applied} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut affected} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut twice} \colorbox{red!0}{\strut daily.HOW} \colorbox{red!0}{\strut SUPPLIEDDiflorasone} \colorbox{red!8}{\strut diacetate} \colorbox{red!5}{\strut cream} \colorbox{red!1}{\strut USP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 0.05} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut g} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NDC} \colorbox{red!0}{\strut 51672-1296-1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut g} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NDC} \colorbox{red!0}{\strut 51672-1296-2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} 
}}}
\end{CJK*}

query: general izzam

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Board} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Directors} \colorbox{red!2}{\strut Board} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut DirectorsAmir} \colorbox{red!0}{\strut AhamedChairman} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut President} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CEOAmir} \colorbox{red!0}{\strut Ahamed} \colorbox{red!2}{\strut founded} \colorbox{red!0}{\strut The} \colorbox{red!21}{\strut Regency} \colorbox{red!8}{\strut Group} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 1983} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut firm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut President} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut CEO} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Amir} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut responsible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut operations} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Group.He} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut grown} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut real} \colorbox{red!0}{\strut estate} \colorbox{red!0}{\strut holdings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut multi-family} \colorbox{red!0}{\strut residential} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut commercial} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut retail} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut OEM} \colorbox{red!0}{\strut franchises} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut dealerships} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut peak} \colorbox{red!0}{\strut of} \colorbox{red!21}{\strut Regency} \colorbox{red!8}{\strut Auto} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut managing} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut investments} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut operating} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Amir} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut held} \colorbox{red!0}{\strut principal} \colorbox{red!0}{\strut responsibility} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut operations} \colorbox{red!0}{\strut of} \colorbox{red!21}{\strut Regency} \colorbox{red!8}{\strut Auto} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut 1983} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut driving} \colorbox{red!0}{\strut force} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut The} \colorbox{red!21}{\strut Regency} \colorbox{red!0}{\strut Group.In} \colorbox{red!0}{\strut 1998} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Amir} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut awarded} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Ernst} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Young} \colorbox{red!0}{\strut Entrepreneur} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Year} \colorbox{red!0}{\strut award} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut with} \colorbox{red!21}{\strut Regency} \colorbox{red!8}{\strut Auto} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Amir} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut chaired} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Lexus} \colorbox{red!0}{\strut Communications} \colorbox{red!0}{\strut Team} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Canada} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut active} \colorbox{red!2}{\strut board} \colorbox{red!0}{\strut member} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut BC} \colorbox{red!0}{\strut Cancer} \colorbox{red!0}{\strut Foundation} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut Collingwood} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Vice} \colorbox{red!0}{\strut Chairman} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Chairman} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Building} \colorbox{red!0}{\strut Committee} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut campus} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Wentworth} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Aleem} \colorbox{red!0}{\strut AhamedManaging} \colorbox{red!0}{\strut DirectorAleem} \colorbox{red!0}{\strut Ahamed} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut Managing} \colorbox{red!2}{\strut Director} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut holds} \colorbox{red!0}{\strut responsibility} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut managing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut existing} \colorbox{red!0}{\strut investment} \colorbox{red!0}{\strut portfolio} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut sourcing} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut opportunities.Aleem} \colorbox{red!0}{\strut joined} \colorbox{red!0}{\strut The} \colorbox{red!21}{\strut Regency} \colorbox{red!8}{\strut Group} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2013} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut spending} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut financial} \colorbox{red!0}{\strut services} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Aleem} \colorbox{red!0}{\strut worked} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Bank} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Montreal} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut capacities} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut Vancouver} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Toronto} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut Commercial} \colorbox{red!0}{\strut Banking} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Real} \colorbox{red!0}{\strut Estate} \colorbox{red!0}{\strut Finance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Corporate} \colorbox{red!0}{\strut Finance} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut spending} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Chicago} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut IL} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Milwaukee} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut WI} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut worked} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut acquisition} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut integration} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Marshall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ilsley} \colorbox{red!1}{\strut Bank} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut closed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Following} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Bank} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Montreal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Aleem} \colorbox{red!0}{\strut worked} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Aver} \colorbox{red!0}{\strut Media} \colorbox{red!0}{\strut LP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut media} \colorbox{red!1}{\strut bank} \colorbox{red!2}{\strut founded} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut partially} \colorbox{red!0}{\strut owned} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pension} \colorbox{red!0}{\strut fund} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut responsibilities} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!13}{\strut generalize} \colorbox{red!13}{\strut generalize} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut jen} \colorbox{red!0}{\strut -er-} \colorbox{red!0}{\strut uh} \colorbox{red!0}{\strut -lahyz} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SpellSyllablesExamples} \colorbox{red!1}{\strut Word} \colorbox{red!0}{\strut OriginSee} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut synonyms} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Thesaurus.comverb} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut object} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut generalized} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut generalizing.1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut infer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut general} \colorbox{red!1}{\strut principle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut trend} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut particular} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut statistics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut like.2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut infer} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut general} \colorbox{red!1}{\strut principle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut opinion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut conclusion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut examples} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut like.3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut give} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut general} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut character} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut to.4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut make} \colorbox{red!12}{\strut general} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut bring} \colorbox{red!0}{\strut into} \colorbox{red!12}{\strut general} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut knowledge.verb} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut without} \colorbox{red!1}{\strut object} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut generalized} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut generalizing.5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut form} \colorbox{red!12}{\strut general} \colorbox{red!1}{\strut principles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut opinions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc.6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut deal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut speak} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut generalities.7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut make} \colorbox{red!12}{\strut general} \colorbox{red!0}{\strut inferences.ExpandAlso} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut British} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut generalise.Origin} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut generalizeExpand1745-1755First} \colorbox{red!0}{\strut recorded} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1745-55} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut general} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -izeRelated} \colorbox{red!0}{\strut formsExpandgeneralizable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adjectivegeneralizer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut nounnongeneralized} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adjectiveungeneralized} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adjectiveungeneralizing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adjectiveDictionary.com} \colorbox{red!0}{\strut Unabridged} \colorbox{red!0}{\strut Based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Random} \colorbox{red!0}{\strut House} \colorbox{red!0}{\strut Dictionary} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Random} \colorbox{red!0}{\strut House} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut 2018} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Cite} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut SourceExamples} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Web} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut generalizeExpandContemporary} \colorbox{red!0}{\strut ExamplesTel} \colorbox{red!0}{\strut Aviv} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!13}{\strut generalize} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut slightly} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut dislikes} \colorbox{red!0}{\strut Netanyahu} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fears} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut future} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut personifies.Resigned} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Loss} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut Optimism} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Center-LeftFania} \colorbox{red!0}{\strut Oz-SalzbergerJanuary} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2013I} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut safe} \colorbox{red!0}{\strut to} \colorbox{red!13}{\strut generalize} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut therein.Jennie} \colorbox{red!0}{\strut Ketcham} \colorbox{red!0}{\strut Interview} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Recovering} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Sex} \colorbox{red!0}{\strut AddictionRachel} \colorbox{red!0}{\strut Kramer} \colorbox{red!0}{\strut BusselJuly} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut impossible} \colorbox{red!0}{\strut to} \colorbox{red!13}{\strut generalize} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut issue} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Jewish} \colorbox{red!0}{\strut councils.Claude} \colorbox{red!0}{\strut Lanzmann} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Shoah} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut His} \colorbox{red!0}{\strut Memoir} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Banality} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut EvilClmence} \colorbox{red!0}{\strut BoulouqueJune} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012Not} \colorbox{red!0}{\strut to} \colorbox{red!13}{\strut generalize} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut seems} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut everyone} \colorbox{red!0}{\strut drinks} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut drunk} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut vodka.Lights} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Camera} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut CocktailsBrody} \colorbox{red!0}{\strut BrownOctober} \colorbox{red!0}{\strut 29} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2011Can} \colorbox{red!0}{\strut we} \colorbox{red!13}{\strut generalize} \colorbox{red!0}{\strut about} 
}}}
\end{CJK*}

query: what in skin care is linked to thyroid problems

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Solutions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!1}{\strut Reasons} \colorbox{red!0}{\strut To} \colorbox{red!2}{\strut Ditch} \colorbox{red!5}{\strut Toxic} \colorbox{red!13}{\strut Dryer} \colorbox{red!12}{\strut Sheets} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Solutions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!1}{\strut Reasons} \colorbox{red!0}{\strut To} \colorbox{red!2}{\strut Ditch} \colorbox{red!5}{\strut Toxic} \colorbox{red!13}{\strut Dryer} \colorbox{red!0}{\strut SheetsBy} \colorbox{red!0}{\strut kim} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 16th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Freshly} \colorbox{red!0}{\strut dried} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut awesomely} \colorbox{red!0}{\strut clean} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut nice} \colorbox{red!0}{\strut smelling} \colorbox{red!0}{\strut clothes} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut lovely} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Yea} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut making} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut lovely} \colorbox{red!0}{\strut fresh} \colorbox{red!0}{\strut washed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dried} \colorbox{red!0}{\strut clothes} \colorbox{red!0}{\strut reeeeeaaally} \colorbox{red!0}{\strut soft} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut skin} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut !} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut accomplish} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut softening} \colorbox{red!0}{\strut effect} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut washer} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!13}{\strut dryer} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!13}{\strut dryer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut probably} \colorbox{red!13}{\strut dryer} \colorbox{red!12}{\strut sheets} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut THE} \colorbox{red!0}{\strut BAD} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Solutions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!1}{\strut Reasons} \colorbox{red!0}{\strut To} \colorbox{red!2}{\strut Ditch} \colorbox{red!5}{\strut Toxic} \colorbox{red!13}{\strut Dryer} \colorbox{red!0}{\strut SheetsLeave} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut comment} \colorbox{red!0}{\strut Nervous} \colorbox{red!0}{\strut System} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Skin} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut Problems} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Toxins} \colorbox{red!0}{\strut healthy} \colorbox{red!0}{\strut lifestyle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut bad} \colorbox{red!0}{\strut news} \colorbox{red!0}{\strut about} \colorbox{red!13}{\strut dryer} \colorbox{red!12}{\strut sheets} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut thyroid} \colorbox{red!0}{\strut health} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut thyroid} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut thyroid} \colorbox{red!1}{\strut symptoms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut toxinsThyroid} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Avoid} \colorbox{red!5}{\strut Toxic} \colorbox{red!3}{\strut Deodorants} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Switching} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Limes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Lemons} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut kim} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 7th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2013} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut health} \colorbox{red!0}{\strut depends} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut multitude} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut things} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut toxins} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut skin} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut pollutants} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut escape} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut air} \colorbox{red!0}{\strut pollutions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut smoke} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Right} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut lotions} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut deodorant.It} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut feel} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut raise} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut sleeveless} \colorbox{red!0}{\strut arms} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut public} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Avoid} \colorbox{red!5}{\strut Toxic} \colorbox{red!3}{\strut Deodorants} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Switching} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Limes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Lemons} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut Hypothyroidism} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Women} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Skin} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut healthy} \colorbox{red!0}{\strut lifestyle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lemon} \colorbox{red!3}{\strut deodorant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lime} \colorbox{red!3}{\strut deodorant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut non-toxic} \colorbox{red!0}{\strut natural} \colorbox{red!3}{\strut deodorant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut toxinsThyroid} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Affects} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Iron} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut Thyroid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut T4} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut T3By} \colorbox{red!0}{\strut kim} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 21st} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Skin} \colorbox{red!1}{\strut Conditions} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Thyroid} \colorbox{red!1}{\strut Health} \colorbox{red!6}{\strut Skin} \colorbox{red!1}{\strut Conditions} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Thyroid} \colorbox{red!0}{\strut HealthPublished} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut 2014It} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut quite} \colorbox{red!2}{\strut common} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut thyroid} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut autoimmune} \colorbox{red!6}{\strut thyroid} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!2}{\strut dry} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut dry} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut problems} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut common} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut acne} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eczema} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut psoriasis} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Skin} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut common} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut hypothyroidism} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Hashimoto} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut Thyroiditis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut hyperthyroidism} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Graves} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Disease} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut discuss} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut relationship} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut common} \colorbox{red!6}{\strut skin} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut thyroid} \colorbox{red!0}{\strut health.Dry} \colorbox{red!6}{\strut Skin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Although} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut hyperthyroid} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut experience} \colorbox{red!2}{\strut dry} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut common} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut hypothyroid} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Thyroid} \colorbox{red!1}{\strut hormone} \colorbox{red!0}{\strut plays} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut role} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut maintaining} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut health} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut So} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut thyroid} \colorbox{red!1}{\strut hormone} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut begin} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut decrease} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut integrity} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut affected} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut hypothyroidism} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Hashimoto} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!5}{\strut Thyroiditis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut balancing} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut thyroid} \colorbox{red!1}{\strut hormone} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut help} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut dry} \colorbox{red!0}{\strut skin.When} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut Graves} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Disease} \colorbox{red!0}{\strut has} \colorbox{red!2}{\strut dry} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut typically} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut autoimmune} \colorbox{red!0}{\strut component} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut condition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut imbalance} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut thyroid} \colorbox{red!1}{\strut hormone} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut hyperthyroid} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut opposite} \colorbox{red!0}{\strut problem} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut their} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut appear} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut moist} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut excessive} \colorbox{red!0}{\strut sweating} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hyperhydrosis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut increase} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut metabolism} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut addressing} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut autoimmune} \colorbox{red!0}{\strut component} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut key} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut helping} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut Graves} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Disease} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut has} \colorbox{red!6}{\strut skin} \colorbox{red!0}{\strut problems.Acne} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Acne} \colorbox{red!0}{\strut vulgaris} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!2}{\strut common} \colorbox{red!6}{\strut skin} \colorbox{red!1}{\strut disorder} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Conventional} \colorbox{red!1}{\strut medical} \colorbox{red!1}{\strut treatment} \colorbox{red!0}{\strut involves} \colorbox{red!0}{\strut topical} \colorbox{red!0}{\strut retinoids} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut topical} \colorbox{red!0}{\strut antimicrobials} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut azelaic} \colorbox{red!0}{\strut acid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut oral} \colorbox{red!0}{\strut antibiotics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut hormonal} \colorbox{red!0}{\strut therapies} 
}}}
\end{CJK*}

query: highest dose of glimepiride

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Glimepiride} \colorbox{red!0}{\strut Dosing} \colorbox{red!40}{\strut Endocrine} \colorbox{red!32}{\strut System} \colorbox{red!0}{\strut ChannelTopicsAcromegalyAddison} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut DiseaseAddisonian} \colorbox{red!0}{\strut CrisisAdrenal} \colorbox{red!0}{\strut InsufficiencyCortisolCushing} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut DiseaseCushing} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut SyndromeEmpty} \colorbox{red!0}{\strut Sella} \colorbox{red!0}{\strut SyndromeHigh} \colorbox{red!8}{\strut Prolactin} \colorbox{red!0}{\strut LevelsHyperthyroidismHypothyroidismPituitary} \colorbox{red!0}{\strut AdenomaPituitary} \colorbox{red!0}{\strut MacroadenomaPituitary} \colorbox{red!0}{\strut MicroadenomaPituitary} \colorbox{red!0}{\strut TumorProlactinomaMedicationsAcarboseActoplus} \colorbox{red!0}{\strut Met} \colorbox{red!0}{\strut XRAlogliptinAlogliptin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut MetforminAlogliptin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut PioglitazoneArmour} \colorbox{red!0}{\strut ThyroidCanagliflozinCytomelExenatideExtended-Release} \colorbox{red!0}{\strut ExenatideGlimepirideGlipizide} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut MetforminGlucaGenGlucophageGlucophage} \colorbox{red!0}{\strut XRGlucotrolGlyburide} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut MetforminHumalog} \colorbox{red!0}{\strut Mix7525Inhaled} \colorbox{red!0}{\strut InsulinInsulin} \colorbox{red!0}{\strut AspartInsulin} \colorbox{red!0}{\strut DetemirInsulin} \colorbox{red!0}{\strut GlargineInsulin} \colorbox{red!0}{\strut GlulisineInsulin} \colorbox{red!0}{\strut LisproInsulin} \colorbox{red!0}{\strut Lispro} \colorbox{red!0}{\strut ProtamineInsulin} \colorbox{red!0}{\strut LisproJanumetKorlymLevothyroxineLinagliptinLinagliptinMetforminLiraglutideMethimazoleMetoclopramideNateglinideNovolin} \colorbox{red!0}{\strut NNovoLog} \colorbox{red!0}{\strut Mix} \colorbox{red!0}{\strut 7030NPH} \colorbox{red!0}{\strut InsulinRegular} \colorbox{red!0}{\strut InsulinPioglitazonePioglitazone} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut GlimepiridePioglitazone} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut MetforminPramlintidePropylthiouracilRegular} \colorbox{red!0}{\strut InsulinRepaglinideRepaglinide} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut MetforminRosiglitazoneRosiglitazone} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut GlimepirideRosiglitazone} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut MetforminSaxagliptinSaxagliptinMetformin} \colorbox{red!0}{\strut ERSitagliptinSitagliptin} \colorbox{red!0}{\strut and} \colorbox{red!32}{\strut Metformin} \colorbox{red!0}{\strut Extended-ReleaseSynthroidTestosterone} \colorbox{red!0}{\strut Topical} \colorbox{red!0}{\strut SolutionTirosintWesthroidAdvertisementQuicklinksCushing} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut DiseaseAddison} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut DiseaseAcromegalyProlactinomaAdrenal} \colorbox{red!0}{\strut InsufficiencyPituitary} \colorbox{red!0}{\strut TumorEmpty} \colorbox{red!0}{\strut Sella} \colorbox{red!0}{\strut SyndromeGlucophageExenatideSynthroidLevothyroxineCytomelMetoclopramideHypothyroidismHypothyroidism} \colorbox{red!0}{\strut DietHyperthyroidismRelated} \colorbox{red!0}{\strut ChannelsDiabetesDepressionHeart} \colorbox{red!0}{\strut DiseaseBlood} \colorbox{red!0}{\strut PressureCholesterolAdvertisementTweetEndocrine} \colorbox{red!32}{\strut System} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Glimepiride} \colorbox{red!0}{\strut DosingGlimepiride} \colorbox{red!0}{\strut DosingThe} \colorbox{red!0}{\strut recommended} \colorbox{red!0}{\strut starting} \colorbox{red!0}{\strut glimepiride} \colorbox{red!0}{\strut dose} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut generally} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut healthcare} \colorbox{red!0}{\strut provider} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut determine} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut glimepiride} \colorbox{red!0}{\strut dosing} \colorbox{red!0}{\strut guidelines} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut factors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut age} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut medical} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut medications} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Glimepiride} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lower} \colorbox{red!0}{\strut dose} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut slowly} \colorbox{red!0}{\strut increased} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut weeks} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut necessary} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut medication} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut combination} \colorbox{red!0}{\strut with} \colorbox{red!56}{\strut insulin} \colorbox{red!0}{\strut injections.Your} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Healthy} \colorbox{red!0}{\strut Living} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut DiabetesGet} \colorbox{red!0}{\strut tips} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut read} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut healthy} \colorbox{red!0}{\strut living} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut diabetes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in-depth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut eMedTV} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut experts.Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut Overview} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Glimepiride} \colorbox{red!0}{\strut DosingThe} \colorbox{red!0}{\strut dose} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut glimepiride} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Amaryl} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut healthcare} \colorbox{red!0}{\strut provider} \colorbox{red!0}{\strut prescribes} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut factors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut ageOther} \colorbox{red!0}{\strut medical} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut haveOther} \colorbox{red!0}{\strut medications} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut taking.As} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut adjust} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut dose} \colorbox{red!0}{\strut unless} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut healthcare} \colorbox{red!0}{\strut provider} \colorbox{red!0}{\strut specifically} \colorbox{red!0}{\strut instructs} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut so.Glimepiride} \colorbox{red!0}{\strut Dosage} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Type} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut DiabetesGlimepiride} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut dose} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut increased} \colorbox{red!0}{\strut slowly} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut instructions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut recommended} \colorbox{red!0}{\strut starting} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut glimepiride} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut glimepiride} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut day.The} \colorbox{red!0}{\strut recommended} \colorbox{red!0}{\strut starting} \colorbox{red!0}{\strut dose} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut elderly} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut people} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!28}{\strut Glimepiride} \colorbox{red!0}{\strut GlimepirideDosage} \colorbox{red!0}{\strut Form} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut tabletOverview} \colorbox{red!6}{\strut Side} \colorbox{red!4}{\strut Effects} \colorbox{red!6}{\strut Dosage} \colorbox{red!0}{\strut Professional} \colorbox{red!0}{\strut Tips} \colorbox{red!0}{\strut Interactions} \colorbox{red!3}{\strut Pregnancy} \colorbox{red!0}{\strut WarningsMoreBreastfeeding} \colorbox{red!0}{\strut WarningsUser} \colorbox{red!0}{\strut ReviewsDrug} \colorbox{red!0}{\strut ImagesSupport} \colorbox{red!0}{\strut Group} \colorbox{red!0}{\strut Q} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut APricing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CouponsOn} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut PageIndications} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut UsageDosage} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut AdministrationDosage} \colorbox{red!0}{\strut Forms} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut StrengthsContraindicationsWarnings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut PrecautionsAdverse} \colorbox{red!0}{\strut ReactionsDrug} \colorbox{red!0}{\strut InteractionsUse} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Specific} \colorbox{red!0}{\strut PopulationsOverdosageDescriptionClinical} \colorbox{red!0}{\strut PharmacologyNonclinical} \colorbox{red!0}{\strut ToxicologyClinical} \colorbox{red!0}{\strut StudiesHow} \colorbox{red!0}{\strut SuppliedStorage} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut HandlingPatient} \colorbox{red!0}{\strut Counseling} \colorbox{red!0}{\strut InformationOn} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut PageIndications} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut UsageDosage} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut AdministrationDosage} \colorbox{red!0}{\strut Forms} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut StrengthsContraindicationsWarnings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut PrecautionsAdverse} \colorbox{red!0}{\strut ReactionsDrug} \colorbox{red!0}{\strut InteractionsUse} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Specific} \colorbox{red!0}{\strut PopulationsOverdosageDescriptionClinical} \colorbox{red!0}{\strut PharmacologyNonclinical} \colorbox{red!0}{\strut ToxicologyClinical} \colorbox{red!0}{\strut StudiesHow} \colorbox{red!0}{\strut SuppliedStorage} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut HandlingPatient} \colorbox{red!0}{\strut Counseling} \colorbox{red!0}{\strut InformationIndications} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut Usage} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut GlimepirideGlimepiride} \colorbox{red!3}{\strut tablets} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut indicated} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut adjunct} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut diet} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut improve} \colorbox{red!6}{\strut glycemic} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut adults} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut 2} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut mellitus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut Clinical} \colorbox{red!0}{\strut Studies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 14.1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Important} \colorbox{red!0}{\strut Limitations} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut UseGlimepiride} \colorbox{red!3}{\strut tablets} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut treatment} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut 1} \colorbox{red!3}{\strut diabetes} \colorbox{red!0}{\strut mellitus} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut diabetic} \colorbox{red!0}{\strut ketoacidosis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!3}{\strut effective} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut settings.SlideshowAging} \colorbox{red!0}{\strut Issues} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut Common} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Concerns} \colorbox{red!0}{\strut Affecting} \colorbox{red!0}{\strut SeniorsGlimepiride} \colorbox{red!6}{\strut Dosage} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut AdministrationRecommended} \colorbox{red!0}{\strut DosingGlimepiride} \colorbox{red!3}{\strut tablets} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut administered} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut breakfast} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut main} \colorbox{red!0}{\strut meal} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut day.The} \colorbox{red!5}{\strut recommended} \colorbox{red!3}{\strut starting} \colorbox{red!13}{\strut dose} \colorbox{red!0}{\strut of} \colorbox{red!28}{\strut Glimepiride} \colorbox{red!3}{\strut tablets} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut once} \colorbox{red!4}{\strut daily} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Patients} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut increased} \colorbox{red!0}{\strut risk} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut hypoglycemia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut e.g.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut elderly} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut renal} \colorbox{red!0}{\strut impairment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut once} \colorbox{red!4}{\strut daily} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut Warnings} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut Precautions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5.1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Specific} \colorbox{red!0}{\strut Populations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8.5} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 8.6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .After} \colorbox{red!0}{\strut reaching} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut daily} \colorbox{red!13}{\strut dose} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut further} \colorbox{red!13}{\strut dose} \colorbox{red!3}{\strut increases} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut increments} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut mg} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut upon} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut patient} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!6}{\strut glycemic} \colorbox{red!0}{\strut response} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Uptitration} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut occur} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut frequently} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut weeks} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut conservative} \colorbox{red!0}{\strut titration} \colorbox{red!0}{\strut scheme} \colorbox{red!0}{\strut is} \colorbox{red!5}{\strut recommended} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut increased} \colorbox{red!0}{\strut risk} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut hypoglycemia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut Warnings} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut Precautions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5.1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Specific} \colorbox{red!0}{\strut Populations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8.5} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 8.6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .The} \colorbox{red!4}{\strut maximum} 
}}}
\end{CJK*}

query: who starred in movie reckless?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Reckless} \colorbox{red!0}{\strut 1984} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut placing} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut playing} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut video} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut agree} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut Terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sold} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Amazon} \colorbox{red!0}{\strut Digital} \colorbox{red!0}{\strut Services} \colorbox{red!0}{\strut LLC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Additional} \colorbox{red!0}{\strut taxes} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut apply.Customers} \colorbox{red!15}{\strut who} \colorbox{red!0}{\strut watched} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut item} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut watchedFire} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut Fire} \colorbox{red!0}{\strut Thief} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut Hearts} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Kids} \colorbox{red!0}{\strut Tuff} \colorbox{red!0}{\strut Turf} \colorbox{red!0}{\strut Afterburn} \colorbox{red!0}{\strut Aftershock} \colorbox{red!0}{\strut Hollywood} \colorbox{red!0}{\strut Dirt} \colorbox{red!0}{\strut Blink} \colorbox{red!0}{\strut Dogfight} \colorbox{red!0}{\strut Ribbons} \colorbox{red!0}{\strut Permanent} \colorbox{red!0}{\strut Record} \colorbox{red!0}{\strut Moving} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!1}{\strut Born} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Accident} \colorbox{red!0}{\strut Perfect} \colorbox{red!0}{\strut Commandments} \colorbox{red!2}{\strut Jersey} \colorbox{red!4}{\strut Girl} \colorbox{red!0}{\strut Tomboy} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Trouble} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut Mistletoe} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Night} \colorbox{red!0}{\strut Before} \colorbox{red!0}{\strut Vision} \colorbox{red!0}{\strut Quest} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut Small} \colorbox{red!0}{\strut AffairProduct} \colorbox{red!0}{\strut detailsGenres} \colorbox{red!0}{\strut DramaDirector} \colorbox{red!0}{\strut James} \colorbox{red!0}{\strut FoleyStarring} \colorbox{red!6}{\strut Aidan} \colorbox{red!4}{\strut Quinn} \colorbox{red!0}{\strut ,} \colorbox{red!11}{\strut Daryl} \colorbox{red!6}{\strut Hannah} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Kenneth} \colorbox{red!0}{\strut McmillanSupporting} \colorbox{red!2}{\strut actors} \colorbox{red!0}{\strut Cliff} \colorbox{red!0}{\strut De} \colorbox{red!0}{\strut YoungStudio} \colorbox{red!0}{\strut MGMMPAA} \colorbox{red!0}{\strut rating} \colorbox{red!0}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Restricted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Captions} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut subtitles} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DetailsAudio} \colorbox{red!0}{\strut EnglishPurchase} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut Stream} \colorbox{red!0}{\strut instantly} \colorbox{red!0}{\strut DetailsFormat} \colorbox{red!1}{\strut Prime} \colorbox{red!1}{\strut Video} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut streaming} \colorbox{red!0}{\strut online} \colorbox{red!1}{\strut video} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Devices} \colorbox{red!0}{\strut Available} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut watch} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut supported} \colorbox{red!0}{\strut devicesOther} \colorbox{red!0}{\strut formatsDVD} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 13.72Customer} \colorbox{red!0}{\strut Reviews4.6} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut 1304.6} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut stars5} \colorbox{red!1}{\strut star} \colorbox{red!0}{\strut 72} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!1}{\strut star} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!1}{\strut star} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut star2} \colorbox{red!1}{\strut star} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!1}{\strut star} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut thoughts} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut customersWrite} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut customer} \colorbox{red!0}{\strut reviewSee} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut 130} \colorbox{red!0}{\strut customer} \colorbox{red!0}{\strut reviewsRead} \colorbox{red!0}{\strut reviews} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut mentionquinn} \colorbox{red!6}{\strut hannah} \colorbox{red!6}{\strut aidan} \colorbox{red!1}{\strut dvd} \colorbox{red!11}{\strut daryl} \colorbox{red!28}{\strut movies} \colorbox{red!0}{\strut youngschool} \colorbox{red!0}{\strut scene} \colorbox{red!0}{\strut classic} \colorbox{red!0}{\strut saw} \colorbox{red!0}{\strut soundtrack} \colorbox{red!0}{\strut johnnydance} \colorbox{red!0}{\strut early} \colorbox{red!0}{\strut teen} \colorbox{red!0}{\strut scenes} \colorbox{red!0}{\strut void} \colorbox{red!4}{\strut girl} \colorbox{red!0}{\strut rebelTop} \colorbox{red!0}{\strut customer} \colorbox{red!0}{\strut reviewsClaire4.0} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut Better} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut ways} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012Format} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut DVD} \colorbox{red!0}{\strut Verified} \colorbox{red!0}{\strut PurchaseI} \colorbox{red!0}{\strut saw} \colorbox{red!0}{\strut this} \colorbox{red!26}{\strut movie} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut high} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1988} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut came} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut tv} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut edited} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut nudity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Just} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut though} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut editing} \colorbox{red!0}{\strut did} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut take} \colorbox{red!3}{\strut away} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!26}{\strut movie} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Rebel} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut A} \colorbox{red!1}{\strut Cause} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Romeo} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Juliet} \colorbox{red!0}{\strut love} \colorbox{red!0}{\strut story} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut inspired} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut wish} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!11}{\strut Daryl} \colorbox{red!6}{\strut Hannah} \colorbox{red!3}{\strut running} \colorbox{red!3}{\strut away} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut motorcycle} \colorbox{red!0}{\strut wrapped} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!40}{\strut Zipper} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FULL} \colorbox{red!5}{\strut CAST} \colorbox{red!0}{\strut AND} \colorbox{red!0}{\strut CREW} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut TRIVIA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut USER} \colorbox{red!0}{\strut REVIEWS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut IMDbPro} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MORESHARE5.7} \colorbox{red!0}{\strut 105,536Rate} \colorbox{red!0}{\strut ThisZipper} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1h} \colorbox{red!0}{\strut 52min} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Drama} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thriller} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 28} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 2015} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut USA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 221} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Trailer3} \colorbox{red!0}{\strut VIDEOS} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut IMAGESWatch} \colorbox{red!0}{\strut NowFrom} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.99} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut SD} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Prime} \colorbox{red!0}{\strut VideoA} \colorbox{red!0}{\strut successful} \colorbox{red!0}{\strut family} \colorbox{red!0}{\strut man} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut blossoming} \colorbox{red!0}{\strut political} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut loses} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut sense} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut morality} \colorbox{red!3}{\strut when} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut becomes} \colorbox{red!0}{\strut addicted} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut escort} \colorbox{red!0}{\strut agency.Director} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Mora} \colorbox{red!0}{\strut StephensWriters} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Mora} \colorbox{red!0}{\strut Stephens} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Joel} \colorbox{red!0}{\strut Viertel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut credits} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Stars} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Patrick} \colorbox{red!0}{\strut Wilson} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lena} \colorbox{red!0}{\strut Headey} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ray} \colorbox{red!0}{\strut Winstone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut full} \colorbox{red!5}{\strut cast} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut crew} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 39MetascoreFrom} \colorbox{red!0}{\strut metacritic.comReviews26} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 39} \colorbox{red!0}{\strut criticAre} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Team} \colorbox{red!0}{\strut Emily} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Team} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Emily} \colorbox{red!0}{\strut Blunt} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut Krasinski} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Who} \colorbox{red!0}{\strut would} \colorbox{red!3}{\strut survive} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut post-apocalyptic} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut cast} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Quiet} \colorbox{red!0}{\strut Place} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut bets.Watch} \colorbox{red!0}{\strut nowRelated} \colorbox{red!0}{\strut NewsJohn} \colorbox{red!0}{\strut Cho} \colorbox{red!0}{\strut Joins} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Cast} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Fox} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut Exorcist} \colorbox{red!0}{\strut Season} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Plot} \colorbox{red!0}{\strut Details} \colorbox{red!0}{\strut Revealed08} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 2017} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DailyDeadDVD} \colorbox{red!0}{\strut Review} \colorbox{red!0}{\strut .} \colorbox{red!16}{\strut Reckless} \colorbox{red!3}{\strut .} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 2016} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FlickeringmythGlee} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut star} \colorbox{red!0}{\strut Dianna} \colorbox{red!0}{\strut Agron} \colorbox{red!0}{\strut thriller} \colorbox{red!3}{\strut heads} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut WestEnd12} \colorbox{red!0}{\strut February} \colorbox{red!0}{\strut 2016} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ScreenDailySee} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Around} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut WebPowered} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut ZergNetEditorial} \colorbox{red!0}{\strut ListsRelated} \colorbox{red!3}{\strut lists} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut IMDb} \colorbox{red!0}{\strut editorsSundance} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Distribution} \colorbox{red!0}{\strut Dealsa} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 33} \colorbox{red!3}{\strut titles} \colorbox{red!0}{\strut updated} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut Feb} \colorbox{red!0}{\strut 2015Sundance} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Premieresa} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut images} \colorbox{red!0}{\strut updated} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut Jan} \colorbox{red!0}{\strut 2015Sundance} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Premieresa} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 18} \colorbox{red!3}{\strut titles} \colorbox{red!0}{\strut updated} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut Dec} \colorbox{red!0}{\strut 2014Create} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut User} \colorbox{red!0}{\strut ListsRelated} \colorbox{red!3}{\strut lists} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut IMDb} \colorbox{red!0}{\strut users2017} \colorbox{red!12}{\strut Movies} \colorbox{red!0}{\strut watcheda} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 43} \colorbox{red!3}{\strut titles} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut 02} \colorbox{red!0}{\strut Jan} \colorbox{red!0}{\strut 20175.7} \colorbox{red!3}{\strut Rated} \colorbox{red!0}{\strut Filmsa} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 24} \colorbox{red!3}{\strut titles} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut months} \colorbox{red!0}{\strut agoRay} \colorbox{red!0}{\strut Winstone} \colorbox{red!0}{\strut Moviesa} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 49} \colorbox{red!3}{\strut titles} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut months} \colorbox{red!0}{\strut agoJune} \colorbox{red!0}{\strut 16a} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 24} \colorbox{red!3}{\strut titles} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut 04} \colorbox{red!0}{\strut Jun} \colorbox{red!0}{\strut 2016Favourite} \colorbox{red!5}{\strut Films} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2015a} \colorbox{red!3}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 30} \colorbox{red!3}{\strut titles} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut 07} \colorbox{red!0}{\strut Jan} \colorbox{red!0}{\strut 2016See} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut related} \colorbox{red!3}{\strut lists} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Related} 
}}}
\end{CJK*}

query: where is the corral club located in reliant stadium

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!15}{\strut NRG} \colorbox{red!14}{\strut Stadium} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Formerly} \colorbox{red!0}{\strut Reliant} \colorbox{red!14}{\strut Stadium} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Seating} \colorbox{red!0}{\strut Chart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ticket} \colorbox{red!0}{\strut Info} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A3} \colorbox{red!0}{\strut A4} \colorbox{red!0}{\strut A2} \colorbox{red!0}{\strut A5} \colorbox{red!0}{\strut A1} \colorbox{red!0}{\strut A6} \colorbox{red!0}{\strut B3} \colorbox{red!0}{\strut B4} \colorbox{red!0}{\strut 109} \colorbox{red!0}{\strut 124} \colorbox{red!0}{\strut 108} \colorbox{red!0}{\strut 125} \colorbox{red!0}{\strut 107} \colorbox{red!0}{\strut 126} \colorbox{red!0}{\strut B2} \colorbox{red!0}{\strut B5} \colorbox{red!0}{\strut 106} \colorbox{red!0}{\strut 127} \colorbox{red!0}{\strut B1} \colorbox{red!0}{\strut B6} \colorbox{red!0}{\strut 105} \colorbox{red!0}{\strut 128} \colorbox{red!0}{\strut 104} \colorbox{red!0}{\strut 129} \colorbox{red!0}{\strut 110} \colorbox{red!0}{\strut 123} \colorbox{red!0}{\strut 103} \colorbox{red!0}{\strut 130} \colorbox{red!0}{\strut 312} \colorbox{red!0}{\strut 335} \colorbox{red!0}{\strut 311} \colorbox{red!0}{\strut 336} \colorbox{red!0}{\strut 102} \colorbox{red!0}{\strut 131} \colorbox{red!0}{\strut 310} \colorbox{red!0}{\strut 337} \colorbox{red!0}{\strut 309} \colorbox{red!0}{\strut 338} \colorbox{red!0}{\strut 101} \colorbox{red!0}{\strut 132} \colorbox{red!0}{\strut 308} \colorbox{red!0}{\strut 339} \colorbox{red!0}{\strut 307} \colorbox{red!0}{\strut 340} \colorbox{red!0}{\strut 133} \colorbox{red!0}{\strut 140} \colorbox{red!0}{\strut C3} \colorbox{red!0}{\strut C4} \colorbox{red!0}{\strut 306} \colorbox{red!0}{\strut C2} \colorbox{red!0}{\strut C5} \colorbox{red!0}{\strut 334} \colorbox{red!0}{\strut 341} \colorbox{red!0}{\strut 305} \colorbox{red!0}{\strut C1} \colorbox{red!0}{\strut C6} \colorbox{red!0}{\strut 134} \colorbox{red!0}{\strut 139} \colorbox{red!0}{\strut 342} \colorbox{red!0}{\strut 304} \colorbox{red!0}{\strut 510} \colorbox{red!0}{\strut 532} \colorbox{red!0}{\strut 343} \colorbox{red!0}{\strut 111} \colorbox{red!0}{\strut 122} \colorbox{red!0}{\strut 509} \colorbox{red!0}{\strut 135} \colorbox{red!0}{\strut 136} \colorbox{red!0}{\strut 137} \colorbox{red!0}{\strut 138} \colorbox{red!0}{\strut 303} \colorbox{red!0}{\strut 533} \colorbox{red!0}{\strut 344} \colorbox{red!0}{\strut 508} \colorbox{red!0}{\strut 534} \colorbox{red!0}{\strut 302} \colorbox{red!0}{\strut 313} \colorbox{red!0}{\strut 345} \colorbox{red!0}{\strut 507} \colorbox{red!0}{\strut 535} \colorbox{red!0}{\strut 301} \colorbox{red!0}{\strut 346} \colorbox{red!0}{\strut 506} \colorbox{red!0}{\strut 536} \colorbox{red!0}{\strut 356} \colorbox{red!0}{\strut 333} \colorbox{red!0}{\strut 505} \colorbox{red!0}{\strut 347} \colorbox{red!0}{\strut 537} \colorbox{red!0}{\strut 531} \colorbox{red!0}{\strut 355} \colorbox{red!0}{\strut 504} \colorbox{red!0}{\strut 633} \colorbox{red!0}{\strut 610} \colorbox{red!0}{\strut 348} \colorbox{red!0}{\strut 538} \colorbox{red!0}{\strut 609} \colorbox{red!0}{\strut 634} \colorbox{red!0}{\strut 354} \colorbox{red!0}{\strut 503} \colorbox{red!0}{\strut 539} \colorbox{red!0}{\strut 349} \colorbox{red!0}{\strut 608} \colorbox{red!0}{\strut 635} \colorbox{red!0}{\strut 502} \colorbox{red!0}{\strut 350} \colorbox{red!0}{\strut 351} \colorbox{red!0}{\strut 352} \colorbox{red!0}{\strut 353} \colorbox{red!0}{\strut 540} \colorbox{red!0}{\strut 607} \colorbox{red!0}{\strut 636} \colorbox{red!0}{\strut 501} \colorbox{red!0}{\strut 511} \colorbox{red!0}{\strut 606} \colorbox{red!0}{\strut 541} \colorbox{red!0}{\strut 637} \colorbox{red!0}{\strut 632} \colorbox{red!0}{\strut 605} \colorbox{red!0}{\strut 552} \colorbox{red!0}{\strut 638} \colorbox{red!0}{\strut 542} \colorbox{red!0}{\strut 604} \colorbox{red!0}{\strut 530} \colorbox{red!0}{\strut 639} \colorbox{red!0}{\strut 551} \colorbox{red!0}{\strut 543} \colorbox{red!0}{\strut 603} \colorbox{red!0}{\strut 611} \colorbox{red!0}{\strut 332} \colorbox{red!0}{\strut 112} \colorbox{red!0}{\strut 640} \colorbox{red!0}{\strut 121} \colorbox{red!0}{\strut 550} \colorbox{red!0}{\strut 544} \colorbox{red!0}{\strut 602} \colorbox{red!0}{\strut 641} \colorbox{red!0}{\strut 545} \colorbox{red!0}{\strut 546} \colorbox{red!0}{\strut 547} \colorbox{red!0}{\strut 548} \colorbox{red!0}{\strut 549} \colorbox{red!0}{\strut 601} \colorbox{red!0}{\strut 631} \colorbox{red!0}{\strut 642} \colorbox{red!0}{\strut 314} \colorbox{red!0}{\strut 652} \colorbox{red!0}{\strut 643} \colorbox{red!0}{\strut 651} \colorbox{red!0}{\strut 644} \colorbox{red!0}{\strut 650} \colorbox{red!0}{\strut 645} \colorbox{red!0}{\strut 529} \colorbox{red!0}{\strut 646} \colorbox{red!0}{\strut 647} \colorbox{red!0}{\strut 648} \colorbox{red!0}{\strut 649} \colorbox{red!0}{\strut 630} \colorbox{red!0}{\strut 612} \colorbox{red!0}{\strut 512} \colorbox{red!0}{\strut 331} \colorbox{red!0}{\strut 717} \colorbox{red!0}{\strut 718} \colorbox{red!0}{\strut 719} \colorbox{red!0}{\strut 720} \colorbox{red!0}{\strut 721} \colorbox{red!0}{\strut 722} \colorbox{red!0}{\strut 723} \colorbox{red!0}{\strut 724} \colorbox{red!0}{\strut 725} \colorbox{red!0}{\strut 726} \colorbox{red!0}{\strut 743} \colorbox{red!0}{\strut 744} \colorbox{red!0}{\strut 746} \colorbox{red!0}{\strut 747} \colorbox{red!0}{\strut 748} \colorbox{red!0}{\strut 749} \colorbox{red!0}{\strut 750} \colorbox{red!0}{\strut 751} \colorbox{red!0}{\strut 752} \colorbox{red!0}{\strut 745} \colorbox{red!0}{\strut 629} \colorbox{red!0}{\strut 528} \colorbox{red!0}{\strut 613} \colorbox{red!0}{\strut 113} \colorbox{red!0}{\strut 114} \colorbox{red!0}{\strut 115} \colorbox{red!0}{\strut 116} \colorbox{red!0}{\strut 117} \colorbox{red!0}{\strut 118} \colorbox{red!0}{\strut 119} \colorbox{red!0}{\strut 120} \colorbox{red!0}{\strut 628} \colorbox{red!0}{\strut 315} \colorbox{red!0}{\strut 316} \colorbox{red!0}{\strut 317} \colorbox{red!0}{\strut 318} \colorbox{red!0}{\strut 319} \colorbox{red!0}{\strut 320} \colorbox{red!0}{\strut 321} \colorbox{red!0}{\strut 322} \colorbox{red!0}{\strut 323} \colorbox{red!0}{\strut 324} \colorbox{red!0}{\strut 325} \colorbox{red!0}{\strut 326} \colorbox{red!0}{\strut 327} \colorbox{red!0}{\strut 328} \colorbox{red!0}{\strut 329} \colorbox{red!0}{\strut 330} \colorbox{red!0}{\strut 513} \colorbox{red!0}{\strut 514} \colorbox{red!0}{\strut 515} \colorbox{red!0}{\strut 516} \colorbox{red!0}{\strut 517} \colorbox{red!0}{\strut 518} \colorbox{red!0}{\strut 519} \colorbox{red!0}{\strut 520} \colorbox{red!0}{\strut 521} \colorbox{red!0}{\strut 522} \colorbox{red!0}{\strut 523} \colorbox{red!0}{\strut 524} \colorbox{red!0}{\strut 525} \colorbox{red!0}{\strut 526} \colorbox{red!0}{\strut 527} \colorbox{red!0}{\strut 620} \colorbox{red!0}{\strut 621} \colorbox{red!0}{\strut 622} \colorbox{red!0}{\strut 623} \colorbox{red!0}{\strut 624} \colorbox{red!0}{\strut 625} \colorbox{red!0}{\strut 626} \colorbox{red!0}{\strut 627} \colorbox{red!0}{\strut 614} \colorbox{red!0}{\strut 615} \colorbox{red!0}{\strut 616} \colorbox{red!0}{\strut 617} \colorbox{red!0}{\strut 618} \colorbox{red!0}{\strut 619Seating} \colorbox{red!0}{\strut ConfigurationsStandard} \colorbox{red!0}{\strut Concert} \colorbox{red!0}{\strut Basketball} \colorbox{red!1}{\strut Houston} \colorbox{red!0}{\strut TexansHouston} \colorbox{red!1}{\strut Texans} \colorbox{red!15}{\strut Seating} \colorbox{red!0}{\strut Chart} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut NRG} \colorbox{red!14}{\strut Stadium} \colorbox{red!14}{\strut Seat} \colorbox{red!0}{\strut ViewsWelcome} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut TickPick} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Houston} \colorbox{red!1}{\strut Texans} \colorbox{red!15}{\strut Seating} \colorbox{red!0}{\strut Chart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut cover} \colorbox{red!0}{\strut everything} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut knwo} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut purchasing} \colorbox{red!0}{\strut Cheap} \colorbox{red!1}{\strut Houston} \colorbox{red!1}{\strut Texans} \colorbox{red!1}{\strut Tickets} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!15}{\strut NRG} \colorbox{red!14}{\strut Stadium} \colorbox{red!0}{\strut row} \colorbox{red!0}{\strut and} \colorbox{red!14}{\strut seat} \colorbox{red!4}{\strut numbers} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Texans} \colorbox{red!14}{\strut seat} \colorbox{red!0}{\strut views} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut club} \colorbox{red!3}{\strut seats} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut texans} \colorbox{red!5}{\strut club} \colorbox{red!3}{\strut seats} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut texansRam} \colorbox{red!0}{\strut KingSubscribe} \colorbox{red!0}{\strut 7Add} \colorbox{red!0}{\strut toShareMore3,855} \colorbox{red!0}{\strut views02Published} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Nov} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2010This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut view} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Club} \colorbox{red!2}{\strut Seat} \colorbox{red!1}{\strut section} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Reliant} \colorbox{red!0}{\strut StadiumShow} \colorbox{red!0}{\strut moreLoading} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut AutoplayUp} \colorbox{red!0}{\strut nextHouston} \colorbox{red!0}{\strut 20-25} \colorbox{red!0}{\strut Oakland} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Reliant} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Houston} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Club} \colorbox{red!0}{\strut Section.aldjazairi11,899} \colorbox{red!0}{\strut views244Inside} \colorbox{red!2}{\strut Reliant} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut IEPA0000124,718} \colorbox{red!0}{\strut views302Reliant} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut Minuteminutemaps20,646} \colorbox{red!0}{\strut views116Club} \colorbox{red!3}{\strut Seats} \colorbox{red!1}{\strut Pats} \colorbox{red!0}{\strut GameGene} \colorbox{red!0}{\strut Brown1,703} \colorbox{red!0}{\strut views033NRG} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Walking} \colorbox{red!0}{\strut Into} \colorbox{red!1}{\strut Section} \colorbox{red!0}{\strut 606DoktorStrangelove3,487} \colorbox{red!0}{\strut views028TEXANS} \colorbox{red!1}{\strut BULLS} \colorbox{red!0}{\strut ON} \colorbox{red!0}{\strut PARADE} \colorbox{red!0}{\strut COMING} \colorbox{red!0}{\strut OUT} \colorbox{red!0}{\strut OF} \colorbox{red!0}{\strut THE} \colorbox{red!0}{\strut TUNNEL} \colorbox{red!0}{\strut LIVE} \colorbox{red!0}{\strut SATELLITE} \colorbox{red!0}{\strut FEEDsatellite} \colorbox{red!0}{\strut pro30,288} \colorbox{red!0}{\strut views550121110} \colorbox{red!2}{\strut Reliant} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut turf} \colorbox{red!0}{\strut lapseMarc} \colorbox{red!0}{\strut Herklotz26,296} \colorbox{red!0}{\strut views145Reliant} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Houston} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Texas} \colorbox{red!0}{\strut Not} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut bad} \colorbox{red!2}{\strut seat} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut theHouse} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Elmer} \colorbox{red!0}{\strut Mudguaard1,332} \colorbox{red!0}{\strut views041Panoramic} \colorbox{red!1}{\strut view} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Reliant} \colorbox{red!0}{\strut StadiumJCLIVE325877} \colorbox{red!0}{\strut views039Monster} \colorbox{red!0}{\strut Jam} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut 1414} \colorbox{red!1}{\strut Relient} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Houston} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Texas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut WhosZappo7,171} \colorbox{red!0}{\strut views1236NRG} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut -} \colorbox{red!4}{\strut Houston} \colorbox{red!2}{\strut Texans} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut NFL} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut Zone19,528} \colorbox{red!0}{\strut views119Panthers} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut Tours} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut Club} \colorbox{red!0}{\strut Seatschiefkeith14,758} \colorbox{red!0}{\strut views622Houston} \colorbox{red!2}{\strut Texans} \colorbox{red!0}{\strut 360} \colorbox{red!0}{\strut Player} \colorbox{red!0}{\strut EntranceFamous} \colorbox{red!0}{\strut Group1,798} \colorbox{red!0}{\strut views360107NRG} \colorbox{red!8}{\strut Stadium} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut Rich} \colorbox{red!0}{\strut Eisen} \colorbox{red!0}{\strut Show} \colorbox{red!0}{\strut 10914The} \colorbox{red!1}{\strut Rich} \colorbox{red!0}{\strut Eisen} \colorbox{red!0}{\strut Show2,214} \colorbox{red!0}{\strut views201FSU} \colorbox{red!5}{\strut Club} \colorbox{red!3}{\strut Seats} \colorbox{red!0}{\strut 60} \colorbox{red!0}{\strut secChampions} \colorbox{red!0}{\strut Campaign14,285} \colorbox{red!0}{\strut views101View} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Suite} \colorbox{red!0}{\strut Level} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Cowboys} \colorbox{red!0}{\strut Stadiumhoutexusa23,420} \colorbox{red!0}{\strut views055Walking} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!3}{\strut seats} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut Lexus} \colorbox{red!0}{\strut Diamond} \colorbox{red!5}{\strut Club} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut woahjophill2460} \colorbox{red!0}{\strut views031BASE} \colorbox{red!0}{\strut jump} \colorbox{red!0}{\strut inside} \colorbox{red!2}{\strut Reliant} \colorbox{red!0}{\strut Stadiumredbullusa123,880} \colorbox{red!0}{\strut views1218} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut 13} \colorbox{red!2}{\strut Texans} \colorbox{red!0}{\strut Video} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut PrezoMichael} \colorbox{red!0}{\strut Williams4,411} \colorbox{red!0}{\strut views406A} \colorbox{red!0}{\strut walk} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Club} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut at} \colorbox{red!4}{\strut Houston} \colorbox{red!0}{\strut Rodeo} \colorbox{red!0}{\strut 2012Bandit44TA1,278} \colorbox{red!0}{\strut views035Show} \colorbox{red!0}{\strut more} 
}}}
\end{CJK*}

query: what is the charter of french liberties

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Charter} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut 1814} \colorbox{red!0}{\strut Alternative} \colorbox{red!0}{\strut Title} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Charte} \colorbox{red!0}{\strut ConstitutionnelleCharter} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut 1814} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut French} \colorbox{red!2}{\strut Charte} \colorbox{red!1}{\strut Constitutionnelle} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut French} \colorbox{red!20}{\strut constitution} \colorbox{red!1}{\strut issued} \colorbox{red!0}{\strut by} \colorbox{red!4}{\strut Louis} \colorbox{red!2}{\strut XVIII} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut became} \colorbox{red!2}{\strut king} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!3}{\strut Bourbon} \colorbox{red!2}{\strut Restoration} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut charter} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut revised} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1830} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut remained} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut effect} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut 1848} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut preserved} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut liberties} \colorbox{red!0}{\strut won} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut French} \colorbox{red!1}{\strut Revolution} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!1}{\strut established} \colorbox{red!0}{\strut a} \colorbox{red!18}{\strut constitutional} \colorbox{red!1}{\strut monarchy} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut bicameral} \colorbox{red!0}{\strut parliament} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut guaranteed} \colorbox{red!0}{\strut civil} \colorbox{red!0}{\strut liberties} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut proclaimed} \colorbox{red!0}{\strut religious} \colorbox{red!0}{\strut toleration} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut acknowledged} \colorbox{red!0}{\strut Catholicism} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut religion.Learn} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut articles} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Bourbon} \colorbox{red!0}{\strut RestorationBourbon} \colorbox{red!2}{\strut Restoration} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 181430} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut France} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut began} \colorbox{red!4}{\strut when} \colorbox{red!2}{\strut Napoleon} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut abdicated} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Bourbon} \colorbox{red!0}{\strut monarchs} \colorbox{red!0}{\strut were} \colorbox{red!1}{\strut restored} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut throne} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut First} \colorbox{red!2}{\strut Restoration} \colorbox{red!0}{\strut occurred} \colorbox{red!4}{\strut when} \colorbox{red!2}{\strut Napoleon} \colorbox{red!0}{\strut fell} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut power} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut Louis} \colorbox{red!2}{\strut XVIII} \colorbox{red!0}{\strut became} \colorbox{red!2}{\strut king} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Louis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut reign} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut interrupted} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut Napoleon} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut return} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut France} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut Hundred} \colorbox{red!0}{\strut Days} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut NapoleonRead} \colorbox{red!0}{\strut MoreFrance} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Louis} \colorbox{red!2}{\strut XVIII} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 181524refused} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut scrap} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Charter} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut 1814} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut spite} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut ultra} \colorbox{red!0}{\strut pressure} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut When} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut Chamber} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Deputies} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut elected} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 1815} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ultras} \colorbox{red!0}{\strut scored} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut sweeping} \colorbox{red!0}{\strut victory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut surprised} \colorbox{red!2}{\strut king} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut who} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut feared} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut surge} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut antimonarchical} \colorbox{red!0}{\strut sentiment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut greeted} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut legislature} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut la} \colorbox{red!0}{\strut chambre} \colorbox{red!0}{\strut introuvable} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut incomparableRead} \colorbox{red!0}{\strut MoreSpain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut failure} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut liberalismconstitution} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut French} \colorbox{red!1}{\strut Charter} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut 1814} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut give} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut representation} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut upper} \colorbox{red!0}{\strut classes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut totally} \colorbox{red!0}{\strut unacceptable} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut king} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut prison} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!20}{\strut constitution} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1812} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut king} \colorbox{red!0}{\strut gave} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut movement} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut cowardly} \colorbox{red!0}{\strut fashion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut disowned} \colorbox{red!0}{\strut aRead} \colorbox{red!0}{\strut MoreLouis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut marquis} \colorbox{red!0}{\strut de} \colorbox{red!0}{\strut Fontanescommission} \colorbox{red!0}{\strut appointed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut draft} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Charte} \colorbox{red!1}{\strut Constitutionnelle} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Louis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!20}{\strut constitution} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut 1817} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut a} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut 1830} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut French} \colorbox{red!11}{\strut Charter} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut 1830} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Key} \colorbox{red!0}{\strut DocumentsRelated} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Francis} \colorbox{red!0}{\strut LieberCollection} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Laws} \colorbox{red!0}{\strut ,} \colorbox{red!7}{\strut Charters} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Constitutions} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Bills} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut RightSource} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Appendix} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Francis} \colorbox{red!0}{\strut Lieber} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut On} \colorbox{red!1}{\strut Civil} \colorbox{red!1}{\strut Liberty} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Self-Government,3rd} \colorbox{red!0}{\strut revised} \colorbox{red!0}{\strut edition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Theodore} \colorbox{red!0}{\strut D.} \colorbox{red!0}{\strut Woolsey} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Philadelphia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut J.B.} \colorbox{red!0}{\strut Lippincott} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Co.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1883} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .APPENDIX} \colorbox{red!0}{\strut XII.french} \colorbox{red!11}{\strut charter} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut louis} \colorbox{red!1}{\strut xviii} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut adopted} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut 1830.The} \colorbox{red!1}{\strut following} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut charter} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut 1830} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut translated} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut work} \colorbox{red!1}{\strut published} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Boston} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut title} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Events} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Paris} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut 26th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 27th} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut 28th} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut 29th} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut July} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut translated} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut French.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!11}{\strut charter} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut August} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut 1830} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut substance} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut charter} \colorbox{red!1}{\strut of} \colorbox{red!2}{\strut Louis} \colorbox{red!1}{\strut XVIII} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut such} \colorbox{red!1}{\strut changes} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut chambers} \colorbox{red!1}{\strut adopted} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut favor} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut liberty} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut articles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut amendments} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut ones} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut printed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut italics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut readings} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut suppressed} \colorbox{red!1}{\strut articles} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut notes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut paper} \colorbox{red!0}{\strut exhibits} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut charters.FRENCH} \colorbox{red!11}{\strut CHARTER} \colorbox{red!1}{\strut OF} \colorbox{red!0}{\strut 1830.The} \colorbox{red!0}{\strut whole} \colorbox{red!1}{\strut preamble} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut ancient} \colorbox{red!11}{\strut charter} \colorbox{red!0}{\strut was} \colorbox{red!3}{\strut suppressed} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut containing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut principle} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut concession} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut octroi} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut grant} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut incompatible} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut acknowledgment} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut national} \colorbox{red!0}{\strut sovereignty.The} \colorbox{red!1}{\strut following} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut substitution} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut preamble} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut declaration} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut chamber} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut deputies.The} \colorbox{red!1}{\strut chamber} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut deputies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut consideration} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut imperious} \colorbox{red!0}{\strut necessity} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut events} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut 26th} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 27th} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut 28th} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut 29th} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut July} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut following} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut situation} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut which} \colorbox{red!2}{\strut France} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut placed} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut consequence} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut violation} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut constitutional} \colorbox{red!11}{\strut charter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Considering} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut moreover} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut violation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut heroic} \colorbox{red!0}{\strut resistance} \colorbox{red!1}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut citizens} \colorbox{red!1}{\strut of} \colorbox{red!1}{\strut Paris} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut majesty} 
}}}
\end{CJK*}

query: do clouds form in the vab

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut NASA} \colorbox{red!2}{\strut Vehicle} \colorbox{red!3}{\strut Assembly} \colorbox{red!13}{\strut Building} \colorbox{red!2}{\strut Titusville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut FloridaNASA} \colorbox{red!2}{\strut Vehicle} \colorbox{red!3}{\strut Assembly} \colorbox{red!0}{\strut BuildingA} \colorbox{red!13}{\strut building} \colorbox{red!0}{\strut so} \colorbox{red!1}{\strut large} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut weather.Edit} \colorbox{red!0}{\strut EntryAdd} \colorbox{red!0}{\strut PhotoBeen} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 691Want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Visit} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 149Exterior} \colorbox{red!0}{\strut view} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Vehicle} \colorbox{red!3}{\strut Assembly} \colorbox{red!13}{\strut Building} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut upload.wikimedia.orgwikipediacomm} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut Vehicle} \colorbox{red!3}{\strut Assembly} \colorbox{red!13}{\strut Building} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut VAB} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut NASA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Kennedy} \colorbox{red!2}{\strut Space} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Florida} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut fourth} \colorbox{red!12}{\strut largest} \colorbox{red!13}{\strut building} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut volume} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Completed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1966} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut VAB} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut holds} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut record} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut largest} \colorbox{red!0}{\strut one-story} \colorbox{red!13}{\strut building} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tallest} \colorbox{red!13}{\strut building} \colorbox{red!0}{\strut outside} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut urban} \colorbox{red!1}{\strut center} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States.Top} \colorbox{red!0}{\strut Places} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut TitusvilleTitusville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut FloridaAmerican} \colorbox{red!2}{\strut Space} \colorbox{red!0}{\strut Museum28.6105} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut -80.8087Titusville} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut FloridaWindover} \colorbox{red!0}{\strut Archeological} \colorbox{red!0}{\strut Site28.5386} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut -80.8433See} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut things} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut Titusville} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut astonishing} \colorbox{red!0}{\strut 160} \colorbox{red!0}{\strut meters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 525} \colorbox{red!0}{\strut feet} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut tall} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 218} \colorbox{red!0}{\strut meters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 716} \colorbox{red!0}{\strut feet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut long} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 158} \colorbox{red!0}{\strut meters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 518} \colorbox{red!0}{\strut feet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut wide} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut VAB} \colorbox{red!0}{\strut covers} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut eight} \colorbox{red!0}{\strut acres} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut encloses} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut volume} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 3,665,000} \colorbox{red!0}{\strut cubic} \colorbox{red!0}{\strut meters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 129,428,000} \colorbox{red!0}{\strut cubic} \colorbox{red!0}{\strut feet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut idea} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut how} \colorbox{red!1}{\strut large} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut volume} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut VAB} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 3.75} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Manhattan} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Empire} \colorbox{red!0}{\strut State} \colorbox{red!13}{\strut Building} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut enough} \colorbox{red!2}{\strut space} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fit} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut volume} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Pentagon} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut plenty} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut room} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut VAB} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut so} \colorbox{red!1}{\strut large} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut fact} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut weather} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut humid} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut clouds} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ceiling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut requiring} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 10,000} \colorbox{red!0}{\strut tons} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut air} \colorbox{red!0}{\strut conditioning} \colorbox{red!0}{\strut equipment} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut moisture} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut setup} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut volume} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut air} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!13}{\strut building} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut replaced} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut hour.The} \colorbox{red!0}{\strut records} \colorbox{red!0}{\strut held} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut VAB} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut interior} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut exterior} \colorbox{red!0}{\strut boasts} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut largest} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Cloud} \colorbox{red!4}{\strut Formation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Brief} \colorbox{red!0}{\strut Explanation} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut How} \colorbox{red!1}{\strut Do} \colorbox{red!9}{\strut Clouds} \colorbox{red!6}{\strut Form} \colorbox{red!9}{\strut Cloud} \colorbox{red!4}{\strut Formation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Brief} \colorbox{red!0}{\strut Explanation} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut How} \colorbox{red!1}{\strut Do} \colorbox{red!9}{\strut Clouds} \colorbox{red!0}{\strut FormClouds} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut interesting} \colorbox{red!2}{\strut natural} \colorbox{red!1}{\strut phenomenon} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut observe} \colorbox{red!0}{\strut everyday} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Interestingly} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut clouds} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut substances} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut ice} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut condensed} \colorbox{red!0}{\strut form.Weather} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut predicted} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut certain} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut studying} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut clouds} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut planet} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut solar} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut has} \colorbox{red!1}{\strut atmosphere} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut definitely} \colorbox{red!0}{\strut have} \colorbox{red!9}{\strut clouds} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Besides} \colorbox{red!1}{\strut Earth} \colorbox{red!0}{\strut ,} \colorbox{red!9}{\strut clouds} \colorbox{red!1}{\strut exist} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut planets} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut Venus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mars} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Jupiter} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Saturn} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut nothing} \colorbox{red!0}{\strut but} \colorbox{red!1}{\strut condensed} \colorbox{red!0}{\strut droplets} \colorbox{red!0}{\strut suspended} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut atmosphere} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut surface} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut planet.Processes} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut Cloud} \colorbox{red!0}{\strut FormationClouds} \colorbox{red!0}{\strut are} \colorbox{red!7}{\strut formed} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut air} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut atmosphere} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut saturated} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut water} \colorbox{red!1}{\strut vapor} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut hold} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut may} \colorbox{red!1}{\strut happen} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut viz.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut air} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut cooled} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut point} \colorbox{red!1}{\strut where} \colorbox{red!1}{\strut condensation} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut bound} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut take} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut air} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut expanded} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut lost} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut considerable} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut moisture} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut quantity} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut atmosphere} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut increased} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut extent} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut air} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut capacity} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut hold} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut atmosphere} \colorbox{red!0}{\strut may} \colorbox{red!1}{\strut rise} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut factors} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut evaporation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Though} \colorbox{red!9}{\strut cloud} \colorbox{red!4}{\strut formation} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut seem} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut simple} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut condensation} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut water} \colorbox{red!1}{\strut vapor} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut air} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut reality} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut entire} \colorbox{red!1}{\strut process} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut complicated} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut water} \colorbox{red!1}{\strut vapor} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut condense} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut particular} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut form} \colorbox{red!9}{\strut clouds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut moist} \colorbox{red!1}{\strut air} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut rises} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut earth} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut surface} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut undergo} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut processes} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Clouds} \colorbox{red!0}{\strut thus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!7}{\strut formed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut five} \colorbox{red!1}{\strut different} \colorbox{red!1}{\strut ways} 
}}}
\end{CJK*}

query: when allocating service department costs, the method which ignores serviced provided to other service departments is called

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Examining} \colorbox{red!0}{\strut methods} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut allocating} \colorbox{red!7}{\strut overhead} \colorbox{red!6}{\strut costs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Examining} \colorbox{red!0}{\strut methods} \colorbox{red!0}{\strut for} \colorbox{red!4}{\strut allocating} \colorbox{red!7}{\strut overhead} \colorbox{red!0}{\strut costsPrintReference} \colorbox{red!0}{\strut thisPublished} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 23rd} \colorbox{red!0}{\strut March} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2015Disclaimer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut essay} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut submitted} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut student} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut professional} \colorbox{red!0}{\strut essay} \colorbox{red!0}{\strut writers.Any} \colorbox{red!0}{\strut opinions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut findings} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut conclusions} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut recommendations} \colorbox{red!0}{\strut expressed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut authors} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut necessarily} \colorbox{red!0}{\strut reflect} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut views} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut UK} \colorbox{red!0}{\strut Essays.Overhead} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut ongoing} \colorbox{red!1}{\strut expense} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut operating} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut group} \colorbox{red!0}{\strut expenses} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut necessary} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut continued} \colorbox{red!0}{\strut functioning} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut immediately} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut productsservices} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut offered} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut costs} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut directly} \colorbox{red!0}{\strut generate} \colorbox{red!0}{\strut profits.Overhead} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut indirect} \colorbox{red!1}{\strut product} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut indirect} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut responsibility} \colorbox{red!0}{\strut centre} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Indirect} \colorbox{red!1}{\strut product} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut manufacturing} \colorbox{red!7}{\strut overhead} \colorbox{red!0}{\strut whereas} \colorbox{red!0}{\strut indirect} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut responsibility} \colorbox{red!0}{\strut centre} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut non-manufacturing} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Manufacturing} \colorbox{red!7}{\strut overhead} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut those} \colorbox{red!1}{\strut manufacturing} \colorbox{red!6}{\strut costs} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut incurred} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut traced} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut individual} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut depreciation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut insurance} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut manufacturing} \colorbox{red!0}{\strut equipment} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut occupying} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut managing} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut maintaining} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut production} \colorbox{red!0}{\strut facility} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Manufacturing} \colorbox{red!7}{\strut overhead} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut traced} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut individual} \colorbox{red!1}{\strut product} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut worth} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut trouble} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut like} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut lubricants} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut glue} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Manufacturing} \colorbox{red!7}{\strut overhead} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut include} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut appropriately} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut treated} \colorbox{red!0}{\strut as} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut outputs} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut overtime} \colorbox{red!0}{\strut premium} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut idle} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut utilities} \colorbox{red!0}{\strut cost.Non-manufacturing} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut customer} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut marketing} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut cost.ALLOCATING} \colorbox{red!7}{\strut OVERHEAD} \colorbox{red!0}{\strut COSTSNormally} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut only} \colorbox{red!1}{\strut manufacturing} \colorbox{red!7}{\strut overhead} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut allocated} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut obtain} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut comprehensive} \colorbox{red!0}{\strut estimates} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut product} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut management} \colorbox{red!0}{\strut accountant} \colorbox{red!0}{\strut may} \colorbox{red!3}{\strut allocate} \colorbox{red!0}{\strut non-manufacturing} \colorbox{red!6}{\strut cost} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut is} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut Reciprocal} \colorbox{red!6}{\strut Method} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Cost} \colorbox{red!1}{\strut Allocation} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Service} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut Costing} \colorbox{red!7}{\strut Reciprocal} \colorbox{red!6}{\strut Method} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Cost} \colorbox{red!1}{\strut Allocation} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Service} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut CostingDefinition} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Reciprocal} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut allocating} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut department} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut gives} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut recognition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut interdepartmental} \colorbox{red!0}{\strut services.Explanation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut reciprocal} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut gives} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut recognition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut interdepartmental} \colorbox{red!1}{\strut services} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Under} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut step} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut partial} \colorbox{red!0}{\strut recognition} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut interdepartmental} \colorbox{red!1}{\strut services} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut possible} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut step} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut always} \colorbox{red!1}{\strut allocates} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut forward} \colorbox{red!0}{\strut never} \colorbox{red!0}{\strut backward} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut reciprocal} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut contrast} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut allocates} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut department} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut directions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut reciprocal} \colorbox{red!1}{\strut allocation} \colorbox{red!0}{\strut requires} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut simultaneous} \colorbox{red!1}{\strut equations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut algebraic} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut simultaneous} \colorbox{red!1}{\strut equations} \colorbox{red!0}{\strut method.Under} \colorbox{red!0}{\strut this} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut true} \colorbox{red!5}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut computed} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut simultaneous} \colorbox{red!1}{\strut equations} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut distributed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut producing} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut basis} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut ratio} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Remember} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut true} \colorbox{red!5}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut department} \colorbox{red!0}{\strut means} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut department} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut original} \colorbox{red!5}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut department} \colorbox{red!0}{\strut plus} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut share} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut department} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut main} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!6}{\strut method} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut accurate} \colorbox{red!1}{\strut distribution} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut single} \colorbox{red!0}{\strut step} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut distribution} \colorbox{red!0}{\strut summary} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Example} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut company} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut two} \colorbox{red!1}{\strut service} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut producing} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut two} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut serve} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut producing} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut departmental} \colorbox{red!0}{\strut estimates} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut follows.Producing} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut B} \colorbox{red!1}{\strut Service} \colorbox{red!1}{\strut departments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut X} \colorbox{red!0}{\strut Y} \colorbox{red!0}{\strut 50,000} \colorbox{red!0}{\strut 40,000} \colorbox{red!0}{\strut 10,000} \colorbox{red!0}{\strut 8,800The} \colorbox{red!1}{\strut service} \colorbox{red!1}{\strut departments} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut distributed} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut X} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut B} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Y} \colorbox{red!5}{\strut Cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Y} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut B} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut XRequired} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Transfer} 
}}}
\end{CJK*}

query: define user maintenance

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Automatic} \colorbox{red!11}{\strut Maintenance} \colorbox{red!9}{\strut Automatic} \colorbox{red!0}{\strut MaintenanceMaintenance} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut refers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut application} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut helps} \colorbox{red!0}{\strut maintain} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut health} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Windows} \colorbox{red!1}{\strut PC} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Maintenance} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut keeping} \colorbox{red!1}{\strut Windows} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut applications} \colorbox{red!0}{\strut up-to-date} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut checking} \colorbox{red!0}{\strut security} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut running} \colorbox{red!0}{\strut scans} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut malware} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Windows} \colorbox{red!9}{\strut Automatic} \colorbox{red!1}{\strut Management} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut WAM} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut enhancements} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Task} \colorbox{red!1}{\strut Scheduler} \colorbox{red!0}{\strut API} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut link} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut applications} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Windows} \colorbox{red!11}{\strut maintenance} \colorbox{red!1}{\strut schedule} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Specifically} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut WAM} \colorbox{red!0}{\strut allows} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut activities} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut require} \colorbox{red!0}{\strut regular} \colorbox{red!1}{\strut scheduling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut exact} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut requirements} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Instead} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut WAM} \colorbox{red!0}{\strut relies} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut operating} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut appropriate} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut activate} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut task} \colorbox{red!0}{\strut throughout} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut chooses} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut minimal} \colorbox{red!0}{\strut impact} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut PC} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut energy} \colorbox{red!0}{\strut efficiency.How} \colorbox{red!1}{\strut Scheduled} \colorbox{red!11}{\strut Maintenance} \colorbox{red!0}{\strut WorksWindows} \colorbox{red!9}{\strut Automatic} \colorbox{red!11}{\strut Maintenance} \colorbox{red!0}{\strut minimizes} \colorbox{red!0}{\strut impact} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut PC} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut scheduling} \colorbox{red!11}{\strut maintenance} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut PC} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut idle} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut default} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut performs} \colorbox{red!11}{\strut maintenance} \colorbox{red!0}{\strut daily} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut starting} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut AM} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Note} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut re-schedule} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut maintenance} \colorbox{red!0}{\strut occurs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut daily} \colorbox{red!0}{\strut session} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut maximum} \colorbox{red!0}{\strut duration} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut hour} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut attempt} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut actively} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut machine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut defers} \colorbox{red!11}{\strut maintenance} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut suspends} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut executing} \colorbox{red!11}{\strut maintenance} \colorbox{red!1}{\strut task} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut returns} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut PC.The} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut restarts} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut suspended} \colorbox{red!11}{\strut maintenance} \colorbox{red!1}{\strut task} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut idle} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut suspend} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut task} \colorbox{red!0}{\strut marked} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut critical} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Instead} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut allows} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut critical} \colorbox{red!1}{\strut task} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut complete} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut regardless} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut action.Due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nature} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut scheduling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut some} \colorbox{red!1}{\strut scheduled} \colorbox{red!0}{\strut tasks} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut finish} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut perhaps} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut scheduled} \colorbox{red!0}{\strut events} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fit} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut hour} \colorbox{red!11}{\strut maintenance} \colorbox{red!1}{\strut window} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut maybe} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut computer} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut User-defined} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut User-defined} \colorbox{red!0}{\strut functionFrom} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedianavigation} \colorbox{red!0}{\strut searchA} \colorbox{red!0}{\strut user-defined} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut UDF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut user} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut program} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut environment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut context} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut usual} \colorbox{red!0}{\strut assumption} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!9}{\strut functions} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut built} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut program} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut environment.Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut BASIC} \colorbox{red!0}{\strut language2} \colorbox{red!0}{\strut Databases2.1} \colorbox{red!1}{\strut SQL} \colorbox{red!0}{\strut Server} \colorbox{red!0}{\strut 20002.2} \colorbox{red!0}{\strut Apache} \colorbox{red!0}{\strut Hive3} \colorbox{red!0}{\strut References4} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut linksBASIC} \colorbox{red!1}{\strut language} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut implementations} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut BASIC} \colorbox{red!1}{\strut programming} \colorbox{red!1}{\strut language} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut user-defined} \colorbox{red!9}{\strut functions} \colorbox{red!0}{\strut are} \colorbox{red!9}{\strut defined} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DEF} \colorbox{red!0}{\strut FN} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut syntax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut modern} \colorbox{red!0}{\strut dialects} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut BASIC} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut influenced} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut structured} \colorbox{red!1}{\strut programming} \colorbox{red!0}{\strut paradigm} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut user-defined} \colorbox{red!9}{\strut functions} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut procedures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut concept} \colorbox{red!0}{\strut becomes} \colorbox{red!0}{\strut practically} \colorbox{red!0}{\strut redundant.Databases} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut relational} \colorbox{red!1}{\strut database} \colorbox{red!0}{\strut management} \colorbox{red!0}{\strut systems} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut user-defined} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut mechanism} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut extending} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut functionality} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut database} \colorbox{red!0}{\strut server} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut evaluated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut standard} \colorbox{red!0}{\strut query} \colorbox{red!1}{\strut language} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut usually} \colorbox{red!1}{\strut SQL} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut statements} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut SQL} \colorbox{red!0}{\strut standard} \colorbox{red!0}{\strut distinguishes} \colorbox{red!0}{\strut between} \colorbox{red!1}{\strut scalar} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut table} \colorbox{red!9}{\strut functions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!1}{\strut scalar} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut returns} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut single} \colorbox{red!0}{\strut value} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut NULL} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut whereas} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut table} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut returns} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut relational} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut table} \colorbox{red!0}{\strut comprising} \colorbox{red!0}{\strut zero} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut rows} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut row} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut columns.User-defined} \colorbox{red!9}{\strut functions} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut SQL} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut declared} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut CREATE} \colorbox{red!9}{\strut FUNCTION} \colorbox{red!0}{\strut statement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut converts} \colorbox{red!1}{\strut Celsius} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Fahrenheit} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut declared} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut CREATE} \colorbox{red!9}{\strut FUNCTION} \colorbox{red!0}{\strut dbo} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CtoF} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Celsius} \colorbox{red!0}{\strut FLOAT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RETURNS} \colorbox{red!0}{\strut FLOATRETURN} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Celsius} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 32Once} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut user-defined} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut expressions} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut SQL} \colorbox{red!0}{\strut statements} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut invoked} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut intrinsic} \colorbox{red!9}{\strut functions} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut allowed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut SELECT} \colorbox{red!0}{\strut statements} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut function} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut against} 
}}}
\end{CJK*}

query: mia nrt distance

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Distance} \colorbox{red!0}{\strut from} \colorbox{red!14}{\strut Miami} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MIA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Narita} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut NRT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Distance} \colorbox{red!0}{\strut from} \colorbox{red!14}{\strut Miami} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MIA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Narita} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut NRT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut flight} \colorbox{red!0}{\strut distance} \colorbox{red!0}{\strut from} \colorbox{red!14}{\strut Miami} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Narita} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 7437} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11968} \colorbox{red!0}{\strut kilometers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6462} \colorbox{red!0}{\strut nautical} \colorbox{red!0}{\strut miles.Search} \colorbox{red!0}{\strut airportsSearch} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut airport} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut city} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut IATA} \colorbox{red!0}{\strut airport} \colorbox{red!0}{\strut code.From} \colorbox{red!0}{\strut AirportTo} \colorbox{red!0}{\strut AirportMultiple} \colorbox{red!0}{\strut airportsAdd} \colorbox{red!0}{\strut AirportRemove} \colorbox{red!0}{\strut AirportDistanceFrom} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut ToMiami} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MIA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!15}{\strut Tokyo} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut NRT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mi7437km11968NM6462MapABFlight} \colorbox{red!0}{\strut durationEstimated} \colorbox{red!2}{\strut flight} \colorbox{red!14}{\strut time} \colorbox{red!0}{\strut from} \colorbox{red!14}{\strut Miami} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MIA} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Narita} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Airport} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut NRT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 14} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut 34} \colorbox{red!0}{\strut minutes.Time} \colorbox{red!13}{\strut difference} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut current} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut timesThe} \colorbox{red!14}{\strut time} \colorbox{red!13}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!14}{\strut Miami} \colorbox{red!0}{\strut and} \colorbox{red!15}{\strut Tokyo} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Tokyo} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut ahead} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Miami.Time} \colorbox{red!0}{\strut DifferenceMiamiTokyoMiami205308} \colorbox{red!0}{\strut EDTFriday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 6th} \colorbox{red!0}{\strut 2018Tokyo095308} \colorbox{red!0}{\strut JSTSaturday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 7th} \colorbox{red!0}{\strut 2018Airport} \colorbox{red!0}{\strut informationA} \colorbox{red!14}{\strut Miami} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut AirportCity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MiamiCountry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut StatesIATA} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut MIAICAO} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut KMIACoordinates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 254735N} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 801726WB} \colorbox{red!1}{\strut Narita} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut AirportCity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut TokyoCountry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut JapanIATA} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NRTICAO} \colorbox{red!0}{\strut Code} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RJAACoordinates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 354552N} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 140239EFrequent} \colorbox{red!0}{\strut Flyer} \colorbox{red!0}{\strut Miles} \colorbox{red!0}{\strut Calculator} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut MIA} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut NRTElite} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut bonus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Booking} \colorbox{red!0}{\strut class} \colorbox{red!0}{\strut bonus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Air} \colorbox{red!0}{\strut miles7437Elite} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut bonus0Booking} \colorbox{red!0}{\strut class} \colorbox{red!0}{\strut bonus0In} \colorbox{red!0}{\strut totalTotal} \colorbox{red!0}{\strut frequent} \colorbox{red!0}{\strut flyer} \colorbox{red!0}{\strut miles7437CalculateRound} \colorbox{red!0}{\strut trip} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut No} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!1}{\strut driving} \colorbox{red!4}{\strut distance} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut Fort} \colorbox{red!0}{\strut Lauderdale-Hollywood} \colorbox{red!1}{\strut International} \colorbox{red!2}{\strut Airport} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Miami} \colorbox{red!1}{\strut International} \colorbox{red!2}{\strut Airport} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut driving} \colorbox{red!4}{\strut distance} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut Fort} \colorbox{red!0}{\strut Lauderdale-Hollywood} \colorbox{red!1}{\strut International} \colorbox{red!2}{\strut Airport} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Miami} \colorbox{red!1}{\strut International} \colorbox{red!2}{\strut Airport} \colorbox{red!0}{\strut is32} \colorbox{red!1}{\strut miles} \colorbox{red!0}{\strut 51} \colorbox{red!0}{\strut kmCity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Check-in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Check-out} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rooms} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Travelers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Fort} \colorbox{red!10}{\strut Lauderdale} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Miami} \colorbox{red!0}{\strut road} \colorbox{red!0}{\strut tripMap} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut driving} \colorbox{red!1}{\strut directions} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAClick} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut show} \colorbox{red!0}{\strut mapDrag} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut map} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut calculate} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut driving} \colorbox{red!4}{\strut distance} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut route.If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut verify} \colorbox{red!0}{\strut these} \colorbox{red!1}{\strut driving} \colorbox{red!1}{\strut directions} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut possible} \colorbox{red!0}{\strut route} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut try} \colorbox{red!0}{\strut Google} \colorbox{red!0}{\strut Maps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Bing} \colorbox{red!0}{\strut Maps} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut MapQuest.More} \colorbox{red!0}{\strut trip} \colorbox{red!0}{\strut calculationsdriving} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAcost} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut driving} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAreverse} \colorbox{red!1}{\strut drive} \colorbox{red!4}{\strut distance} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut MIA} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut FLLhalfway} \colorbox{red!0}{\strut between} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut MIAstopping} \colorbox{red!0}{\strut points} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAhotels} \colorbox{red!0}{\strut near} \colorbox{red!0}{\strut MIAflight} \colorbox{red!4}{\strut distance} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAflight} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAfly} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut drive} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAairports} \colorbox{red!0}{\strut near} \colorbox{red!0}{\strut MIAairlines} \colorbox{red!1}{\strut flying} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAnonstop} \colorbox{red!1}{\strut flights} \colorbox{red!0}{\strut from} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut MIAtime} \colorbox{red!1}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!10}{\strut FLL} \colorbox{red!0}{\strut and} \colorbox{red!10}{\strut MIA} 
}}}
\end{CJK*}

query: how many 1000 in 1 million

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut How} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answers.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut WikiAnswers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Categories} \colorbox{red!0}{\strut Science} \colorbox{red!0}{\strut Math} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Arithmetic} \colorbox{red!0}{\strut Mathematical} \colorbox{red!0}{\strut Analysis} \colorbox{red!4}{\strut How} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut FlagHow} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Rob} \colorbox{red!0}{\strut Flanders} \colorbox{red!0}{\strut Confidence} \colorbox{red!0}{\strut votes} \colorbox{red!0}{\strut 31.2KANSWER} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1000} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 000} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 000} \colorbox{red!0}{\strut 1000} \colorbox{red!4}{\strut millions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut billion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1,000,000,000} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut billions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut trillion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1,000,000,000,000} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut thousand} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut one} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut Proof} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut multiplied} \colorbox{red!0}{\strut together} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,000,000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut one} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,0001,000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,000,00067} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut usefulWas} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut useful} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut YesSomewhatNoUser00987} \colorbox{red!0}{\strut 126,341} \colorbox{red!0}{\strut ContributionsHow} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut makes} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!5}{\strut thousand} \colorbox{red!5}{\strut thousand} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,000,000Matthew} \colorbox{red!0}{\strut Burgess} \colorbox{red!0}{\strut 396,785} \colorbox{red!0}{\strut ContributionsA} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut equals} \colorbox{red!4}{\strut how} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousand} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut One} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut equal} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut thousands.Anand} \colorbox{red!0}{\strut Vijayakumar} \colorbox{red!0}{\strut 363,997} \colorbox{red!0}{\strut ContributionsHow} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut dollars} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 1000000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1000} \colorbox{red!0}{\strut A} \colorbox{red!5}{\strut thousand} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut called} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut dollars.Anand} \colorbox{red!0}{\strut Mehta} \colorbox{red!0}{\strut 278,423} \colorbox{red!0}{\strut Contributionsmehtamatics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mathematics} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut differenceHow} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 31.92} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 319204} \colorbox{red!0}{\strut JAYS} \colorbox{red!0}{\strut 2,010,442} \colorbox{red!0}{\strut ContributionsMathematics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut definitions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut conversions} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut physics} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut interests} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Answers.comHow} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut one} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut 1,000} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut million.Anand} \colorbox{red!0}{\strut Mehta} \colorbox{red!0}{\strut 278,423} \colorbox{red!0}{\strut Contributionsmehtamatics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mathematics} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut differenceHow} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 17.5} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 17500How} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut hundred} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut why} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Because} \colorbox{red!0}{\strut 100,000} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,000,000Sandalian} \colorbox{red!0}{\strut 919} \colorbox{red!0}{\strut ContributionsHow} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut 10} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut ten} \colorbox{red!5}{\strut thousands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut million.4} \colorbox{red!0}{\strut JAYS} \colorbox{red!0}{\strut 2,010,442} \colorbox{red!0}{\strut ContributionsMathematics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut definitions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut conversions} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut physics} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut interests} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Answers.comHow} \colorbox{red!0}{\strut many} \colorbox{red!5}{\strut thousand} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 0.3} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 0.3} \colorbox{red!0}{\strut trillion} \colorbox{red!0}{\strut equals} \colorbox{red!0}{\strut 300} \colorbox{red!5}{\strut million} \colorbox{red!0}{\strut thousands.4} \colorbox{red!0}{\strut JAYS} \colorbox{red!0}{\strut 2,010,442} \colorbox{red!0}{\strut ContributionsMathematics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut facts} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut What} \colorbox{red!0}{\strut does} \colorbox{red!4}{\strut trillion} \colorbox{red!1}{\strut equal} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Nasiruddin} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut ContributionsWhat} \colorbox{red!0}{\strut does} \colorbox{red!4}{\strut trillion} \colorbox{red!1}{\strut equal} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 1,000,000,000,000What} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut 1000} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut thousand} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut quadrillion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut figure} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut byknowing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut numbers} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut zeroes} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut 12.Since} \colorbox{red!3}{\strut 1000} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut zeroes} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut 1000} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut 1000} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut trillion} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut quatrillionAnna} \colorbox{red!0}{\strut Rino} \colorbox{red!0}{\strut 36,058} \colorbox{red!0}{\strut ContributionsHow} \colorbox{red!0}{\strut many} \colorbox{red!3}{\strut 1000} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Number} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut 1000} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut billionWhat} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut 1000} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut billions} \colorbox{red!0}{\strut or} \colorbox{red!4}{\strut trillions} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut 1000} \colorbox{red!1}{\strut million} \colorbox{red!1}{\strut equals} \colorbox{red!1}{\strut 1} \colorbox{red!4}{\strut billion} \colorbox{red!0}{\strut 1,000,000,000} \colorbox{red!3}{\strut 1000} \colorbox{red!4}{\strut billion} \colorbox{red!1}{\strut equals} \colorbox{red!1}{\strut 1} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut 1,000,000,000,000Al} \colorbox{red!0}{\strut Cohen} \colorbox{red!0}{\strut 126,337} \colorbox{red!0}{\strut ContributionsSenior} \colorbox{red!0}{\strut Fellow} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Electrical} \colorbox{red!0}{\strut EngineeringDoes} \colorbox{red!3}{\strut 1000} \colorbox{red!1}{\strut million} \colorbox{red!1}{\strut equal} \colorbox{red!1}{\strut 1} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,000} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!4}{\strut billion} \colorbox{red!0}{\strut 1,000} \colorbox{red!4}{\strut billion} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut trillionWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut value} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut 1000} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 1000,000,00,00,000,001000} \colorbox{red!4}{\strut trillion} \colorbox{red!1}{\strut equal} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut Indian} \colorbox{red!0}{\strut rupees} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut 1000} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut indian1000} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut equal} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut what} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut quadrillion} \colorbox{red!0}{\strut exactly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pcig} \colorbox{red!0}{\strut morfil} \colorbox{red!0}{\strut 39,268} \colorbox{red!0}{\strut ContributionsWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut times} \colorbox{red!3}{\strut 1000} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut short} \colorbox{red!0}{\strut scale} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut x} \colorbox{red!3}{\strut 1000} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut quadrillion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut long} \colorbox{red!0}{\strut scales} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Europe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut x} \colorbox{red!3}{\strut 1000} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 1} \colorbox{red!0}{\strut thousand} \colorbox{red!0}{\strut Prasang} \colorbox{red!0}{\strut ghanshyam} \colorbox{red!0}{\strut 348} \colorbox{red!0}{\strut ContributionsHow} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut 1000} \colorbox{red!4}{\strut trillion} \colorbox{red!1}{\strut equal} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut crore} \colorbox{red!0}{\strut crores4} \colorbox{red!0}{\strut JAYS} \colorbox{red!0}{\strut 2,010,442} \colorbox{red!0}{\strut ContributionsMathematics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut facts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut definitions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut conversions} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut physics} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut interests} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Answers.comWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!3}{\strut 1000} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut words} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut thousand} \colorbox{red!4}{\strut trillion} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is the voltage in israel

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Aliyah} \colorbox{red!0}{\strut .} \colorbox{red!13}{\strut Electrical} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FAQ} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Aliyah} \colorbox{red!0}{\strut .} \colorbox{red!13}{\strut Electrical} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FAQ} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut LAST} \colorbox{red!0}{\strut UPDATED} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 21,2006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CLICK} \colorbox{red!0}{\strut ON} \colorbox{red!0}{\strut QUESTION} \colorbox{red!0}{\strut TO} \colorbox{red!0}{\strut GO} \colorbox{red!0}{\strut TO} \colorbox{red!0}{\strut ANSWER} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut main} \colorbox{red!6}{\strut differences} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut the} \colorbox{red!13}{\strut electrical} \colorbox{red!5}{\strut power} \colorbox{red!2}{\strut supplied} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut power} \colorbox{red!2}{\strut supplied} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut 110V} \colorbox{red!0}{\strut refrigerator} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut What} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut buying} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut 110V} \colorbox{red!1}{\strut washer} \colorbox{red!0}{\strut andor} \colorbox{red!1}{\strut dryer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut 110v} \colorbox{red!0}{\strut small} \colorbox{red!1}{\strut appliances} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut transformer} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut transformer} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut converter} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut power} \colorbox{red!1}{\strut supply} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut convert} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut voltage} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut computer} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut I} \colorbox{red!1}{\strut bring} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut lighting} \colorbox{red!0}{\strut fixtures} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut purchase} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 12VDC} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut 110VAC} \colorbox{red!1}{\strut inverter} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 220VAC} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12VDC} \colorbox{red!5}{\strut power} \colorbox{red!0}{\strut pack} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut supply} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut DC} \colorbox{red!1}{\strut voltage} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut stereo} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut 60Hz} \colorbox{red!14}{\strut electricity} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut planning} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut bring} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut equipment} \colorbox{red!1}{\strut which} \colorbox{red!1}{\strut uses} \colorbox{red!1}{\strut 110V} \colorbox{red!0}{\strut 60Hz} \colorbox{red!1}{\strut motors} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut motors} \colorbox{red!1}{\strut converted} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 220V} \colorbox{red!0}{\strut 50Hz} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut done} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut costly} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut 110V} \colorbox{red!1}{\strut computer} \colorbox{red!0}{\strut monitor} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut ?} \colorbox{red!11}{\strut What} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut printer} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut came} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Israel} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut stacked} \colorbox{red!0}{\strut Maytag} \colorbox{red!0}{\strut washerdryer} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut told} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 30A} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut electrician} \colorbox{red!0}{\strut told} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut big} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut huge} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut outlet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut company} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut installing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut appliance} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut install} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut sheka} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Search} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut Ceptics} \colorbox{red!1}{\strut 2} \colorbox{red!4}{\strut USB} \colorbox{red!4}{\strut Israel} \colorbox{red!3}{\strut Travel} \colorbox{red!4}{\strut Adapter} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1} \colorbox{red!2}{\strut Power} \colorbox{red!3}{\strut Plug} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Type} \colorbox{red!1}{\strut H} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Universal} \colorbox{red!0}{\strut Socketby} \colorbox{red!0}{\strut Ceptics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12.99} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut 99FREE} \colorbox{red!1}{\strut Shipping} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut eligible} \colorbox{red!0}{\strut orders} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut promotion4.4} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut 509OREI} \colorbox{red!4}{\strut Israel} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Palestine} \colorbox{red!3}{\strut Travel} \colorbox{red!3}{\strut Plug} \colorbox{red!4}{\strut Adapter} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Dual} \colorbox{red!4}{\strut USB} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Surge} \colorbox{red!1}{\strut Protection} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Type} \colorbox{red!1}{\strut H} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut U2U-14} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Does} \colorbox{red!0}{\strut Not} \colorbox{red!3}{\strut Convert} \colorbox{red!0}{\strut Voltageby} \colorbox{red!0}{\strut Orei} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19.99} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19} \colorbox{red!0}{\strut 99Only} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut stock} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut order} \colorbox{red!0}{\strut soon.FREE} \colorbox{red!1}{\strut Shipping} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut eligible} \colorbox{red!0}{\strut orders4.4} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut 257Amazon} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut ChoiceCeptics} \colorbox{red!0}{\strut CT-14} \colorbox{red!2}{\strut USA} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut Israel} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Palestine} \colorbox{red!3}{\strut Travel} \colorbox{red!4}{\strut Adapter} \colorbox{red!3}{\strut Plug} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Type} \colorbox{red!1}{\strut H} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Pack} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Dual} \colorbox{red!0}{\strut Inputs} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Ultra} \colorbox{red!1}{\strut Compact} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Does} \colorbox{red!0}{\strut Not} \colorbox{red!3}{\strut Convert} \colorbox{red!2}{\strut Voltage} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Ceptics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9.99} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut 99More} \colorbox{red!0}{\strut Buying} \colorbox{red!0}{\strut Choices} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8.24} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut offers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FREE} \colorbox{red!1}{\strut Shipping} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut eligible} \colorbox{red!0}{\strut orders} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut promotion4.8} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut 3,746Ceptics} \colorbox{red!0}{\strut CTU-14} \colorbox{red!2}{\strut USA} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut Israel} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Palestine} \colorbox{red!3}{\strut Travel} \colorbox{red!4}{\strut Adapter} \colorbox{red!3}{\strut Plug} \colorbox{red!0}{\strut With} \colorbox{red!1}{\strut Dual} \colorbox{red!4}{\strut USB} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Type} \colorbox{red!1}{\strut H} \colorbox{red!0}{\strut -} \colorbox{red!1}{\strut Ultra} \colorbox{red!0}{\strut Compactby} \colorbox{red!0}{\strut Ceptics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12.99} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut 99} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 14.99More} \colorbox{red!0}{\strut Buying} \colorbox{red!0}{\strut Choices} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11.37} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut offers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FREE} \colorbox{red!1}{\strut Shipping} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut eligible} \colorbox{red!0}{\strut orders4.7} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut 2,193VCT} \colorbox{red!0}{\strut VP-5} \colorbox{red!4}{\strut Israel} \colorbox{red!4}{\strut Adapter} \colorbox{red!3}{\strut Plug} \colorbox{red!3}{\strut Converts} \colorbox{red!2}{\strut USA} \colorbox{red!3}{\strut Plug} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut Israel} \colorbox{red!0}{\strut Plugby} \colorbox{red!0}{\strut VCT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6.50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut 50More} \colorbox{red!0}{\strut Buying} \colorbox{red!0}{\strut Choices} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut offers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FREE} \colorbox{red!1}{\strut Shipping} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut eligible} \colorbox{red!0}{\strut orders3.9} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut 94Ceptics} \colorbox{red!4}{\strut Israel} \colorbox{red!3}{\strut Travel} \colorbox{red!3}{\strut Plug} \colorbox{red!4}{\strut Adapter} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Type} \colorbox{red!1}{\strut H} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Pack} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Grounded} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Universal} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GP-14-3PK} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Ceptics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7.99} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut 99FREE} \colorbox{red!1}{\strut Shipping} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut eligible} \colorbox{red!0}{\strut orders} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut promotion4.5} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5} \colorbox{red!1}{\strut stars} \colorbox{red!0}{\strut 7,042Orei} \colorbox{red!4}{\strut Israel} \colorbox{red!1}{\strut 2} \colorbox{red!4}{\strut USB} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.4A17W} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Travel} \colorbox{red!0}{\strut Charger} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut iPhone} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut iPad} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Samsung} \colorbox{red!0}{\strut Galaxy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Android} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut HTC} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Motorola} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut LG} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut W2U-H} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Orei} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11.99} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is the butler's name in the addams family

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!23}{\strut Lurch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut Addams} \colorbox{red!1}{\strut Family} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedianavigation} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut multiple} \colorbox{red!0}{\strut issues} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut improve} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut discuss} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut issues} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut talk} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Learn} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut remove} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut template} \colorbox{red!0}{\strut messages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut citations} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut verification} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut possibly} \colorbox{red!0}{\strut contains} \colorbox{red!1}{\strut original} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut LurchTed} \colorbox{red!1}{\strut Cassidy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!23}{\strut Lurch} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Jackie} \colorbox{red!0}{\strut Coogan} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut Uncle} \colorbox{red!1}{\strut Fester} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .First} \colorbox{red!1}{\strut appearance} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut New} \colorbox{red!0}{\strut Yorker} \colorbox{red!2}{\strut cartoon} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1938} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Created} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Charles} \colorbox{red!0}{\strut AddamsPortrayed} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Ted} \colorbox{red!0}{\strut CassidyJim} \colorbox{red!0}{\strut CummingsCarel} \colorbox{red!0}{\strut StruyckenJohn} \colorbox{red!0}{\strut DeSantisRyan} \colorbox{red!0}{\strut Jacob} \colorbox{red!0}{\strut WoodInformationGender} \colorbox{red!0}{\strut MaleOccupation} \colorbox{red!0}{\strut ServantNationality} \colorbox{red!0}{\strut AmericanLurch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut whose} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut name} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut unknown} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fictional} \colorbox{red!1}{\strut character} \colorbox{red!1}{\strut created} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut cartoonist} \colorbox{red!1}{\strut Charles} \colorbox{red!2}{\strut Addams} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut manservant} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut Addams} \colorbox{red!1}{\strut Family} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut original} \colorbox{red!0}{\strut television} \colorbox{red!1}{\strut series} \colorbox{red!0}{\strut ,} \colorbox{red!23}{\strut Lurch} \colorbox{red!0}{\strut was} \colorbox{red!6}{\strut played} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Ted} \colorbox{red!1}{\strut Cassidy} \colorbox{red!0}{\strut ,} \colorbox{red!18}{\strut who} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut famous} \colorbox{red!0}{\strut catchphrase} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut rang} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut similar} \colorbox{red!0}{\strut phrase} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut trademark} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut character} \colorbox{red!0}{\strut Maynard} \colorbox{red!0}{\strut G.} \colorbox{red!1}{\strut Krebs} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut Loves} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Dobie} \colorbox{red!0}{\strut Gillis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Cartoons2} \colorbox{red!0}{\strut Characterization3} \colorbox{red!0}{\strut Backstory4} \colorbox{red!0}{\strut Influence5} \colorbox{red!0}{\strut ReferencesCartoons} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!1}{\strut Charles} \colorbox{red!2}{\strut Addams} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut original} \colorbox{red!2}{\strut cartoons} \colorbox{red!0}{\strut ,} \colorbox{red!23}{\strut Lurch} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut accompanying} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rest} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Family} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut carrying} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut feather-duster} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut couple} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut illustrations} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Family} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut decorating} \colorbox{red!23}{\strut Lurch} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Christmas} \colorbox{red!0}{\strut tree.Characterization} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut personal} \colorbox{red!0}{\strut reflection} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut opinion} \colorbox{red!0}{\strut essay} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut editor} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut personal} \colorbox{red!0}{\strut feelings} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut topic} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut improve} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut rewriting} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut encyclopedic} \colorbox{red!0}{\strut style} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Learn} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut remove} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut template} \colorbox{red!0}{\strut message} \colorbox{red!0}{\strut .} \colorbox{red!23}{\strut Lurch} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut ft} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2.05} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!11}{\strut Addams} \colorbox{red!10}{\strut Family} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1964} \colorbox{red!0}{\strut publicity} \colorbox{red!0}{\strut photo} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut TV} \colorbox{red!1}{\strut series} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Lisa} \colorbox{red!0}{\strut Loring} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut Wednesday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut Astin} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut Gomez} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ted} \colorbox{red!0}{\strut Cassidy} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut Lurch} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Carolyn} \colorbox{red!0}{\strut Jones} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut Morticia} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Ken} \colorbox{red!0}{\strut Weatherwax} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut Pugsley.The} \colorbox{red!11}{\strut Addams} \colorbox{red!10}{\strut Family} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut eccentric} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut macabre} \colorbox{red!0}{\strut fictional} \colorbox{red!10}{\strut family} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut were} \colorbox{red!1}{\strut created} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut American} \colorbox{red!0}{\strut cartoonist} \colorbox{red!1}{\strut Charles} \colorbox{red!11}{\strut Addams} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut appeared} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut single-panel} \colorbox{red!2}{\strut cartoons} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut New} \colorbox{red!0}{\strut Yorker} \colorbox{red!1}{\strut magazine} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1938.The} \colorbox{red!0}{\strut extremely} \colorbox{red!0}{\strut wealthy} \colorbox{red!10}{\strut family} \colorbox{red!1}{\strut live} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut mansion} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut somewhat} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut giving} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut appearance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut typical} \colorbox{red!0}{\strut haunted} \colorbox{red!0}{\strut house} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!10}{\strut family} \colorbox{red!0}{\strut consists} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut husband} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut wife} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut young} \colorbox{red!1}{\strut children} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut older} \colorbox{red!1}{\strut relatives} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut butler} \colorbox{red!3}{\strut who} \colorbox{red!0}{\strut resembles} \colorbox{red!1}{\strut Frankenstein} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut monster} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut played} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Boris} \colorbox{red!0}{\strut Karloff} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 1931} \colorbox{red!1}{\strut movie} \colorbox{red!1}{\strut Frankenstein} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut other} \colorbox{red!10}{\strut family} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut visited} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut time.The} \colorbox{red!1}{\strut characters} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut unnamed} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Charles} \colorbox{red!11}{\strut Addams} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut cartoons} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut TV} \colorbox{red!0}{\strut comedy} \colorbox{red!1}{\strut series} \colorbox{red!1}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut characters} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut developed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1964} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Charles} \colorbox{red!11}{\strut Addams} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut asked} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!2}{\strut names} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!2}{\strut named} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut butler} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Lurch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut husband} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut wife} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Gomez} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Morticia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut older} \colorbox{red!1}{\strut relatives} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Uncle} \colorbox{red!1}{\strut Fester} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Grandmama} \colorbox{red!1}{\strut Frump} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut children} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Wednesday} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pubert} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pubert} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut rejected} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut show} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut producers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut character} \colorbox{red!0}{\strut was} \colorbox{red!2}{\strut named} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Pugsley} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut instead} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pubert} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Gomez} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Morticia} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut third} \colorbox{red!1}{\strut child} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 1993} \colorbox{red!1}{\strut movie} \colorbox{red!0}{\strut The} \colorbox{red!11}{\strut Addams} \colorbox{red!10}{\strut Family} \colorbox{red!0}{\strut Values} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Grandmama} 
}}}
\end{CJK*}

query: consolidate function

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!10}{\strut Consolidate} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut multiple} \colorbox{red!2}{\strut worksheets} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut summarize} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut separate} \colorbox{red!2}{\strut worksheets} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!10}{\strut consolidate} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut master} \colorbox{red!2}{\strut worksheet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut worksheets} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!1}{\strut workbook} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut master} \colorbox{red!2}{\strut worksheet} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut workbooks} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut you} \colorbox{red!10}{\strut consolidate} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut assembling} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut easily} \colorbox{red!0}{\strut update} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut aggregate} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut needed.For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut expense} \colorbox{red!2}{\strut worksheet} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut regional} \colorbox{red!0}{\strut offices} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut use} \colorbox{red!10}{\strut consolidation} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut roll} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut master} \colorbox{red!0}{\strut corporate} \colorbox{red!0}{\strut expense} \colorbox{red!2}{\strut worksheet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut master} \colorbox{red!2}{\strut worksheet} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut contain} \colorbox{red!0}{\strut sales} \colorbox{red!0}{\strut totals} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut averages} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut current} \colorbox{red!0}{\strut inventory} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut highest} \colorbox{red!0}{\strut selling} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut entire} \colorbox{red!0}{\strut enterprise.Tip} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut frequently} \colorbox{red!10}{\strut consolidate} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut base} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut worksheets} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut worksheet} \colorbox{red!0}{\strut template} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut uses} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut consistent} \colorbox{red!0}{\strut layout} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut learn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut Templates} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Create} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut template} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut ideal} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut template} \colorbox{red!0}{\strut with} \colorbox{red!3}{\strut Excel} \colorbox{red!0}{\strut tables.There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut ways} \colorbox{red!0}{\strut to} \colorbox{red!10}{\strut consolidate} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Category} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Position.Consolidation} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut position} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut source} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut arranged} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut uses} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut labels} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut method} \colorbox{red!0}{\strut to} \colorbox{red!10}{\strut consolidate} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut worksheets} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut departmental} \colorbox{red!0}{\strut budget} \colorbox{red!2}{\strut worksheets} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut created} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut template.Consolidation} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut category} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut source} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut arranged} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut uses} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut labels} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut method} \colorbox{red!0}{\strut to} \colorbox{red!10}{\strut consolidate} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut worksheets} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut layouts} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut labels.Consolidating} \colorbox{red!6}{\strut data} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut category} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut similar} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut creating} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut PivotTable} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut PivotTable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut easily} \colorbox{red!0}{\strut reorganize} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut categories} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut flexible} \colorbox{red!10}{\strut consolidation} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut category} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!11}{\strut Consolidate} \colorbox{red!0}{\strut in} \colorbox{red!11}{\strut Excel} \colorbox{red!0}{\strut Edit} \colorbox{red!0}{\strut ArticleHow} \colorbox{red!0}{\strut to} \colorbox{red!11}{\strut Consolidate} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut ExcelFour} \colorbox{red!2}{\strut Methods} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Consolidate} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Position} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!11}{\strut Excel} \colorbox{red!0}{\strut WorksheetIdentify} \colorbox{red!0}{\strut Categories} \colorbox{red!0}{\strut to} \colorbox{red!11}{\strut Consolidate} \colorbox{red!11}{\strut Excel} \colorbox{red!1}{\strut Data} \colorbox{red!0}{\strut Use} \colorbox{red!1}{\strut Formulas} \colorbox{red!0}{\strut to} \colorbox{red!11}{\strut Consolidate} \colorbox{red!11}{\strut Excel} \colorbox{red!0}{\strut DataAccess} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut PivotTable} \colorbox{red!1}{\strut function} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut Q} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut AMicrosoft} \colorbox{red!1}{\strut Office} \colorbox{red!11}{\strut Excel} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut customizing} \colorbox{red!1}{\strut tables} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut charts} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut important} \colorbox{red!1}{\strut data} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut program} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut offers} \colorbox{red!1}{\strut efficient} \colorbox{red!1}{\strut ways} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut combine} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut summarize} \colorbox{red!1}{\strut data} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut multiple} \colorbox{red!1}{\strut files} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut worksheets} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Common} \colorbox{red!2}{\strut methods} \colorbox{red!0}{\strut to} \colorbox{red!11}{\strut consolidate} \colorbox{red!0}{\strut in} \colorbox{red!11}{\strut Excel} \colorbox{red!0}{\strut include} \colorbox{red!1}{\strut consolidating} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut position} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut category} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut formula} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut using} \colorbox{red!11}{\strut Excel} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Pivot} \colorbox{red!1}{\strut Table} \colorbox{red!0}{\strut feature} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Scroll} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut jump} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!7}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!11}{\strut consolidate} \colorbox{red!0}{\strut in} \colorbox{red!11}{\strut Excel} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut appears} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut master} \colorbox{red!1}{\strut worksheet} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut reference} \colorbox{red!0}{\strut whenever} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut generate} \colorbox{red!0}{\strut reports} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what do partnerships file tax in michigan

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Pay} \colorbox{red!2}{\strut Taxes} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Limited} \colorbox{red!1}{\strut Liability} \colorbox{red!1}{\strut Corporation} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Michigan} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut limited} \colorbox{red!1}{\strut liability} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Michigan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!2}{\strut tax} \colorbox{red!0}{\strut obligations} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut IRS} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Tax} \colorbox{red!0}{\strut obligations} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut LLCs} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut whether} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut sell} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut rent} \colorbox{red!0}{\strut goods} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut employees} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut After} \colorbox{red!1}{\strut registering} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!1}{\strut state} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut determining} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut your} \colorbox{red!11}{\strut LLC} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut responsible} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut business} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut paid} \colorbox{red!0}{\strut online} \colorbox{red!0}{\strut via} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut Michigan} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Treasury} \colorbox{red!0}{\strut website} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut mail.Registration} \colorbox{red!0}{\strut for} \colorbox{red!8}{\strut Michigan} \colorbox{red!0}{\strut TaxesNew} \colorbox{red!1}{\strut businesses} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Michigan} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut Form} \colorbox{red!0}{\strut 518} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Registration} \colorbox{red!0}{\strut for} \colorbox{red!8}{\strut Michigan} \colorbox{red!2}{\strut Taxes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut register} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Indicate} \colorbox{red!0}{\strut whether} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut sell} \colorbox{red!0}{\strut tangible} \colorbox{red!0}{\strut property} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut liable} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut sales} \colorbox{red!2}{\strut tax} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut lease} \colorbox{red!0}{\strut property} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!1}{\strut requires} \colorbox{red!0}{\strut payment} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut use} \colorbox{red!2}{\strut tax} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Michigan} \colorbox{red!0}{\strut also} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut tobacco} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut motor} \colorbox{red!0}{\strut fuels} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut business} \colorbox{red!0}{\strut sells} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Treasury} \colorbox{red!0}{\strut suggests} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut register} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut those} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!8}{\strut Michigan} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Treasury} \colorbox{red!0}{\strut recommends} \colorbox{red!0}{\strut Form} \colorbox{red!0}{\strut 518} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut mailed} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut six} \colorbox{red!0}{\strut weeks} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut begin} \colorbox{red!0}{\strut doing} \colorbox{red!1}{\strut business} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut state.Ready} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut start} \colorbox{red!0}{\strut your} \colorbox{red!11}{\strut LLC} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Start} \colorbox{red!0}{\strut an} \colorbox{red!11}{\strut LLC} \colorbox{red!0}{\strut Online} \colorbox{red!0}{\strut NowEmployer} \colorbox{red!0}{\strut ObligationsIf} \colorbox{red!0}{\strut your} \colorbox{red!11}{\strut LLC} \colorbox{red!0}{\strut employes} \colorbox{red!0}{\strut personnel} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut register} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut employer-related} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut unemployment} \colorbox{red!0}{\strut insurance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut required} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut withhold} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut federal} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut state} \colorbox{red!1}{\strut income} \colorbox{red!2}{\strut tax} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut After} \colorbox{red!1}{\strut registering} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!1}{\strut state} \colorbox{red!2}{\strut taxes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut send} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut personalized} \colorbox{red!2}{\strut tax} \colorbox{red!0}{\strut returns} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut withheld} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut file} \colorbox{red!0}{\strut Form} \colorbox{red!0}{\strut 165} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut withheld} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut copies} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut W-2} \colorbox{red!0}{\strut forms} \colorbox{red!0}{\strut distributed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut employee} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut IRS.Federal} \colorbox{red!0}{\strut TaxesMichigan} \colorbox{red!1}{\strut requires} \colorbox{red!1}{\strut businesses} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut complete} \colorbox{red!0}{\strut federal} \colorbox{red!2}{\strut tax} \colorbox{red!0}{\strut returns} \colorbox{red!0}{\strut before} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut returns} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut file} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut federal} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Steps} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Filing} \colorbox{red!3}{\strut Partnership} \colorbox{red!6}{\strut Taxes} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Steps} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Filing} \colorbox{red!3}{\strut Partnership} \colorbox{red!0}{\strut Taxesby} \colorbox{red!0}{\strut Jane} \colorbox{red!0}{\strut Haskins} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Esq} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Freelance} \colorbox{red!0}{\strut writerPartnerships} \colorbox{red!0}{\strut don} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut t} \colorbox{red!1}{\strut pay} \colorbox{red!1}{\strut federal} \colorbox{red!1}{\strut income} \colorbox{red!6}{\strut tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Instead} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut losses} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut deductions} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut credits} \colorbox{red!0}{\strut pass} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut partners} \colorbox{red!0}{\strut themselves} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut amountsand} \colorbox{red!1}{\strut pay} \colorbox{red!6}{\strut taxes} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut themas} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut personal} \colorbox{red!1}{\strut income} \colorbox{red!6}{\strut tax} \colorbox{red!0}{\strut returns.Even} \colorbox{red!0}{\strut though} \colorbox{red!5}{\strut partnerships} \colorbox{red!0}{\strut aren} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut t} \colorbox{red!6}{\strut taxed} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut must} \colorbox{red!1}{\strut file} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut tax} \colorbox{red!2}{\strut return} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut unless} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut no} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut expenses} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut return} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut show} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut total} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut deductions} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut credits} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Partnerships} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut must} \colorbox{red!1}{\strut prepare} \colorbox{red!1}{\strut schedules} \colorbox{red!0}{\strut showing} \colorbox{red!0}{\strut each} \colorbox{red!1}{\strut partner} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut share} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut business} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut loss} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut file} \colorbox{red!1}{\strut state} \colorbox{red!6}{\strut tax} \colorbox{red!2}{\strut returns} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut certain} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut taxes.Whether} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut operate} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut general} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut limited} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut follow} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut basic} \colorbox{red!0}{\strut procedure} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut filing} \colorbox{red!1}{\strut business} \colorbox{red!6}{\strut taxes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut limited} \colorbox{red!1}{\strut partners} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut slightly} \colorbox{red!0}{\strut different} \colorbox{red!6}{\strut tax} \colorbox{red!0}{\strut treatment} \colorbox{red!0}{\strut than} \colorbox{red!1}{\strut general} \colorbox{red!0}{\strut partners.Here} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut five} \colorbox{red!0}{\strut steps} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut follow} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut file} \colorbox{red!1}{\strut business} \colorbox{red!6}{\strut taxes} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut partnership.1} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Prepare} \colorbox{red!1}{\strut Form} \colorbox{red!0}{\strut 1065} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut U.S.} \colorbox{red!2}{\strut Return} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Partnership} \colorbox{red!0}{\strut IncomeEvery} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut must} \colorbox{red!1}{\strut prepare} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut federal} \colorbox{red!3}{\strut partnership} \colorbox{red!6}{\strut tax} \colorbox{red!2}{\strut return} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Internal} \colorbox{red!0}{\strut Revenue} \colorbox{red!0}{\strut Servicer} \colorbox{red!1}{\strut Form} \colorbox{red!0}{\strut 1065} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut form} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut asked} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut total} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut loss} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut list} \colorbox{red!1}{\strut deductions} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut salaries} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut guaranteed} \colorbox{red!0}{\strut payments} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut partners} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut repairs} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut taxes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut depreciation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut employee} \colorbox{red!1}{\strut benefit} \colorbox{red!0}{\strut programs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!3}{\strut partnership} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut total} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut deductions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut ordinary} \colorbox{red!1}{\strut business} \colorbox{red!0}{\strut income.You} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fill} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut several} \colorbox{red!1}{\strut Form} \colorbox{red!0}{\strut 1065} \colorbox{red!1}{\strut schedules} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Schedule} \colorbox{red!0}{\strut B} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut partnershipfrom} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut partners} 
}}}
\end{CJK*}

query: against what part of the electromagnetic spectrum does sunscreen protect?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Critical} \colorbox{red!8}{\strut Wavelength} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Broad} \colorbox{red!1}{\strut Spectrum} \colorbox{red!1}{\strut UV} \colorbox{red!1}{\strut Protection} \colorbox{red!8}{\strut Critical} \colorbox{red!8}{\strut Wavelength} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Broad} \colorbox{red!1}{\strut Spectrum} \colorbox{red!1}{\strut UV} \colorbox{red!1}{\strut Protection} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut informational} \colorbox{red!0}{\strut pages} \colorbox{red!0}{\strut on} \colorbox{red!3}{\strut sunscreens} \colorbox{red!0}{\strut and} \colorbox{red!8}{\strut critical} \colorbox{red!8}{\strut wavelength} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Karl} \colorbox{red!0}{\strut Gruber} \colorbox{red!0}{\strut MD} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Founder} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut LUCA} \colorbox{red!0}{\strut SunscreenWhat} \colorbox{red!0}{\strut Is} \colorbox{red!8}{\strut Critical} \colorbox{red!8}{\strut Wavelength} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!8}{\strut critical} \colorbox{red!8}{\strut wavelength} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut why} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ask} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Critical} \colorbox{red!8}{\strut wavelength} \colorbox{red!0}{\strut identifies} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut UVA} \colorbox{red!1}{\strut protection} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut given} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut offers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut define} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut broad} \colorbox{red!1}{\strut spectrum} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut protection} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Critical} \colorbox{red!8}{\strut wavelength} \colorbox{red!1}{\strut measurements} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut therefore} \colorbox{red!0}{\strut extremely} \colorbox{red!0}{\strut beneficial} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut consumer} \colorbox{red!0}{\strut seeking} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut maximum} \colorbox{red!1}{\strut protection} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut sun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut harmful} \colorbox{red!0}{\strut rays} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut worksMeasuring} \colorbox{red!1}{\strut UV} \colorbox{red!1}{\strut Absorbance} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut UV} \colorbox{red!1}{\strut absorbance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut determined} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut vitro} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut entire} \colorbox{red!1}{\strut UV} \colorbox{red!1}{\strut spectrum} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 290nm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 400nm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut substrate} \colorbox{red!0}{\strut spectrophotometry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut uniform} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut thickness} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut applied} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut slide} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut exposed} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut UV} \colorbox{red!0}{\strut light} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut absorbance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut UV} \colorbox{red!0}{\strut radiation} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut measured} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut graph} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut approximates} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut absorbance} \colorbox{red!0}{\strut curves} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut UVB} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2-EHMC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut UVA} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut TDSA} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut broad} \colorbox{red!1}{\strut spectrum} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut Zinc} \colorbox{red!0}{\strut Oxide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .The} \colorbox{red!0}{\strut shape} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut resultant} \colorbox{red!1}{\strut absorbance} \colorbox{red!0}{\strut curve} \colorbox{red!0}{\strut represents} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut efficiency} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut sunscreen} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut blocks} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut given} \colorbox{red!1}{\strut UV} \colorbox{red!8}{\strut wavelength} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut respect} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut UV} \colorbox{red!1}{\strut absorbance} \colorbox{red!0}{\strut curve} \colorbox{red!0}{\strut demonstrates} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut amplitude} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut breadth} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut protection} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 290nm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 400nm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut UV} \colorbox{red!0}{\strut spectrum.Interpreting} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Absorbance} \colorbox{red!0}{\strut Curve} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut amplitude} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut absorbance} \colorbox{red!0}{\strut curve} \colorbox{red!0}{\strut reflects} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut degree} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut protection} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut higher} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut amplitude} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut curve} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut greater} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut absorbance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut protection} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut radio} \colorbox{red!0}{\strut wavesAshley} \colorbox{red!0}{\strut Holden} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut ContributionsWhat} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Radio} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Microwave} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Infrared} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Visible} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut colours} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Ultraviolet} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut X-ray} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Gamma} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut remember} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rabbits} \colorbox{red!0}{\strut Mate} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Very} \colorbox{red!0}{\strut Unusual} \colorbox{red!0}{\strut eXpens} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut consists} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut non-visible} \colorbox{red!0}{\strut radiation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut visible} \colorbox{red!0}{\strut light} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut radio} \colorbox{red!0}{\strut waves} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut examples} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut Gamma} \colorbox{red!0}{\strut rays} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut x-rays} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ultraviolet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut UHF} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut VHF} \colorbox{red!0}{\strut bandwidt} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut Ellis} \colorbox{red!0}{\strut Hartford} \colorbox{red!0}{\strut 21,476} \colorbox{red!0}{\strut ContributionsWhat} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut visible} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut colors} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut see.Jack177} \colorbox{red!0}{\strut 784} \colorbox{red!0}{\strut ContributionsThe} \colorbox{red!4}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut visible} \colorbox{red!0}{\strut light} \colorbox{red!0}{\strut 790-400} \colorbox{red!0}{\strut nmCommon} \colorbox{red!0}{\strut properties} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut x} \colorbox{red!0}{\strut u} \colorbox{red!0}{\strut v} \colorbox{red!0}{\strut i} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut rPetethemeerkat} \colorbox{red!0}{\strut 1,289} \colorbox{red!0}{\strut ContributionsList} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Radio} \colorbox{red!0}{\strut waves} \colorbox{red!0}{\strut Microwaves} \colorbox{red!0}{\strut Infrared} \colorbox{red!0}{\strut Visible} \colorbox{red!0}{\strut light} \colorbox{red!0}{\strut Ultraviolet} \colorbox{red!0}{\strut X} \colorbox{red!0}{\strut rays} \colorbox{red!0}{\strut Gamma} \colorbox{red!0}{\strut raysJohn} \colorbox{red!0}{\strut Ellis} \colorbox{red!0}{\strut Hartford} \colorbox{red!0}{\strut 21,476} \colorbox{red!0}{\strut ContributionsWhat} \colorbox{red!4}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut color} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut called} \colorbox{red!0}{\strut visible} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut red} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut frequency} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut violet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut frequency} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Identify} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut school} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut outWhy} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut sound} \colorbox{red!0}{\strut not} \colorbox{red!4}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Sound} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut medium} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut travel} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut thus} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Usually} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut travel} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut vacuum} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!0}{\strut spectrum.Kevinkendall} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut ContributionsWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut hear} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut Electromagnetic} \colorbox{red!4}{\strut spectrum} \colorbox{red!0}{\strut consists} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut radiations} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut wavelengths} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut frequency} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut visible} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut invisible} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut forms} 
}}}
\end{CJK*}

query: what is a buddy test

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut See} \colorbox{red!4}{\strut What} \colorbox{red!0}{\strut Our} \colorbox{red!9}{\strut ACT} \colorbox{red!8}{\strut Test} \colorbox{red!5}{\strut Watch} \colorbox{red!0}{\strut Customers} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut Saying} \colorbox{red!9}{\strut ACT} \colorbox{red!8}{\strut Test} \colorbox{red!0}{\strut WatchOur} \colorbox{red!0}{\strut revolutionary} \colorbox{red!0}{\strut timing} \colorbox{red!0}{\strut device} \colorbox{red!0}{\strut gives} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut effective} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut manage} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ACT.Order} \colorbox{red!0}{\strut NowQuestion} \colorbox{red!0}{\strut TrackingNotifies} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut exactly} \colorbox{red!4}{\strut what} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut remain} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut track.View} \colorbox{red!0}{\strut NowPre-ProgrammedOur} \colorbox{red!9}{\strut ACT} \colorbox{red!8}{\strut Test} \colorbox{red!5}{\strut watch} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut pre-programmed} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut sections} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ACT.View} \colorbox{red!0}{\strut NowSection} \colorbox{red!0}{\strut TrackingQuickly} \colorbox{red!0}{\strut know} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut elapsed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut remains} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut section.View} \colorbox{red!0}{\strut NowApproved} \colorbox{red!8}{\strut Test} \colorbox{red!0}{\strut Watch100} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut legal} \colorbox{red!9}{\strut ACT} \colorbox{red!0}{\strut pacing} \colorbox{red!5}{\strut watch} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut practice} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut real} \colorbox{red!0}{\strut ACT.View} \colorbox{red!0}{\strut NowThe} \colorbox{red!8}{\strut Test} \colorbox{red!0}{\strut Buddy} \colorbox{red!9}{\strut ACT} \colorbox{red!8}{\strut Test} \colorbox{red!0}{\strut WatchThe} \colorbox{red!8}{\strut Test} \colorbox{red!1}{\strut Buddy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut for} \colorbox{red!9}{\strut ACT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut gives} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ability} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut precisely} \colorbox{red!0}{\strut manage} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut ACT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut device} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut five} \colorbox{red!0}{\strut preset} \colorbox{red!0}{\strut timing} \colorbox{red!0}{\strut functions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut test} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut revolutionary} \colorbox{red!0}{\strut questionpassage} \colorbox{red!0}{\strut tracking} \colorbox{red!0}{\strut feature} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut allows} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut passage} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut completed} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut given} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut passed.The} \colorbox{red!8}{\strut Test} \colorbox{red!1}{\strut Buddy} \colorbox{red!0}{\strut Video} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut browser} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut recognize} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut formats} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut frequently} \colorbox{red!0}{\strut asked} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut HTML5} \colorbox{red!0}{\strut video.Top} \colorbox{red!0}{\strut TimerMeasures} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut passed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut particular} \colorbox{red!0}{\strut section.Bottom} \colorbox{red!0}{\strut TimerDenotes} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut specific} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut test.Fraction} \colorbox{red!0}{\strut TimerFraction} \colorbox{red!0}{\strut timer} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut bottom} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut screen} \colorbox{red!0}{\strut displays} \colorbox{red!4}{\strut what} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut regards} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut section.Exam} \colorbox{red!0}{\strut SectionsThe} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut displays} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut E} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Math} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut R} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Reading} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut S} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Science} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut W} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut WritingStart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stop} \colorbox{red!0}{\strut ButtonAllows} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut stop} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut timer} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut respective} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut test.Mode} \colorbox{red!0}{\strut ButtonUsed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut toggle} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut five} \colorbox{red!0}{\strut sections} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut ACT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Math} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Reading} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Science} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Writing.ACT} \colorbox{red!5}{\strut Watch} \colorbox{red!0}{\strut SolutionThe} \colorbox{red!8}{\strut Test} \colorbox{red!1}{\strut Buddy} \colorbox{red!0}{\strut Has} \colorbox{red!0}{\strut Been} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut an} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddy} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut an} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddy} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut When} \colorbox{red!7}{\strut anchoring} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Columbia} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut my} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddy} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut thingy} \colorbox{red!0}{\strut invented} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Oregon} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut works} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut giant} \colorbox{red!0}{\strut bungee} \colorbox{red!0}{\strut cord} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut boat} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut deep} \colorbox{red!1}{\strut water} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut keep} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut beached} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut tides} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut yacht} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut ship} \colorbox{red!0}{\strut wakes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut wind} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut tutorial} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut an} \colorbox{red!7}{\strut Anchor} \colorbox{red!0}{\strut buddy.I} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Danforth} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut Fortress} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut shackle} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 3} \colorbox{red!1}{\strut feet} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut chain} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Connect} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut blue} \colorbox{red!1}{\strut ropes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!7}{\strut anchor} \colorbox{red!1}{\strut chain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut connecting} \colorbox{red!0}{\strut two} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddies} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut boat} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Now} \colorbox{red!1}{\strut attach} \colorbox{red!0}{\strut 150} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 200} \colorbox{red!1}{\strut feet} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 38} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut 516} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut nylon} \colorbox{red!1}{\strut rope} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut finally} \colorbox{red!0}{\strut buy} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut helix} \colorbox{red!7}{\strut anchor} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut ground} \colorbox{red!7}{\strut anchor} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut attach} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rope.Now} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut say} \colorbox{red!0}{\strut 50-100} \colorbox{red!1}{\strut feet} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut shore} \colorbox{red!0}{\strut chuck} \colorbox{red!0}{\strut your} \colorbox{red!7}{\strut anchor} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut drink} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Slowly} \colorbox{red!0}{\strut motor} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut shore} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut Anchor} \colorbox{red!7}{\strut Buddy} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut rope} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut sucked} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut prop} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut shore} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut toss} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rest} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut rope} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut ground} \colorbox{red!7}{\strut anchor} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut beach.Now} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut grab} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut rope} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut start} \colorbox{red!1}{\strut pulling} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut goes} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut anchor} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut pull} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut tight} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut then} \colorbox{red!1}{\strut attach} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut bow} \colorbox{red!0}{\strut cleat} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut half} \colorbox{red!0}{\strut hitches.It} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut this.Note} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut picture} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut foot} \colorbox{red!0}{\strut firmly} 
}}}
\end{CJK*}

query: is the louisiana sales tax 4.75

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 2017} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut Income} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut Property} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut Corporate} \colorbox{red!0}{\strut Tax2017} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!0}{\strut TaxLocal} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Jefferson} \colorbox{red!0}{\strut Parish9.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2017} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut taxExact} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut itemsTax} \colorbox{red!0}{\strut Jurisdiction} \colorbox{red!2}{\strut Sales} \colorbox{red!0}{\strut TaxLouisiana} \colorbox{red!0}{\strut State} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut 5.00} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut County} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut City} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut NASpecial} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut NACombined} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut 9.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut data} \colorbox{red!0}{\strut incorrect} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Download} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rates} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut zip} \colorbox{red!0}{\strut codeThe} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 9.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut consisting} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5.00} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut state} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut taxes.The} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut consists} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut county} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut tax.The} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut collected} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut merchant} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut qualifying} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut within} \colorbox{red!3}{\strut Jefferson} \colorbox{red!0}{\strut ParishGroceries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut exempt} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut state} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut taxesJefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut collects} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut maximum} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut allowed} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut lawJefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lower} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 59.6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut cities} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut countiesJefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut ExemptionsIn} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut essential} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut medicine} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut groceries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut exempted} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut eligible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lower} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut collect} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut groceries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Certain} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut alcohol} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cigarettes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut gasoline} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut excise} \colorbox{red!3}{\strut taxes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut tax.Note} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut alcohol} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut prepared} \colorbox{red!0}{\strut food} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut restaurant} \colorbox{red!0}{\strut meals} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut premade} \colorbox{red!0}{\strut supermarket} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut charged} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut higher} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rate} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rates} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut commonly} \colorbox{red!0}{\strut exempted} \colorbox{red!0}{\strut categories} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut Sales} \colorbox{red!5}{\strut Tax} \colorbox{red!2}{\strut Holidays} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2013} \colorbox{red!5}{\strut Louisiana} \colorbox{red!5}{\strut Taxes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Income} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Sales} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Property} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Corporate} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Excise} \colorbox{red!0}{\strut TaxesLouisiana} \colorbox{red!4}{\strut Sales} \colorbox{red!5}{\strut Tax} \colorbox{red!2}{\strut Holidays} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2013A} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut special} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut allowed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut purchase} \colorbox{red!0}{\strut certain} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut buy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 500.00} \colorbox{red!0}{\strut worth} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut goods} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20.00.Louisiana} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut five} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut throughout} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut goods} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut calendar} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut lists} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut major} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut item} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut applies} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut purchase} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut person} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Sale} \colorbox{red!0}{\strut Dates} \colorbox{red!2}{\strut Sale} \colorbox{red!0}{\strut Item} \colorbox{red!2}{\strut Sale} \colorbox{red!0}{\strut Maximum} \colorbox{red!0}{\strut Cost} \colorbox{red!2}{\strut Sale} \colorbox{red!0}{\strut Start} \colorbox{red!0}{\strut YearSeptember} \colorbox{red!0}{\strut 6th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 8th} \colorbox{red!0}{\strut Ammunition} \colorbox{red!0}{\strut NO} \colorbox{red!0}{\strut LIMIT} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 6th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 8th} \colorbox{red!0}{\strut Firearms} \colorbox{red!0}{\strut NO} \colorbox{red!0}{\strut LIMIT} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 6th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 8th} \colorbox{red!0}{\strut Hunting} \colorbox{red!0}{\strut Supplies} \colorbox{red!0}{\strut NO} \colorbox{red!0}{\strut LIMIT} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 25th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 26th} \colorbox{red!0}{\strut Hurricane} \colorbox{red!0}{\strut Preparedness} \colorbox{red!0}{\strut Items} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,500.00} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 2nd} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 3rd} \colorbox{red!0}{\strut TPP} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2,500.00} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Why} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut have} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut dozen} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut throughout} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut these} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut promotions} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut promote} \colorbox{red!0}{\strut desirable} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut energy-star} \colorbox{red!0}{\strut rated} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut emergency} \colorbox{red!0}{\strut preparedness} \colorbox{red!0}{\strut supplies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut hold} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut correspond} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut back-to-school} \colorbox{red!0}{\strut shopping} \colorbox{red!0}{\strut season} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut books} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut clothing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut school} \colorbox{red!0}{\strut supplies.In} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}



==> sections/visualization/loss2.tex <==
query: is the louisiana sales tax 4.75

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 2017} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut Income} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut Property} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut Corporate} \colorbox{red!0}{\strut Tax2017} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!0}{\strut TaxLocal} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut -} \colorbox{red!3}{\strut Jefferson} \colorbox{red!0}{\strut Parish9.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2017} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut taxExact} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut itemsTax} \colorbox{red!0}{\strut Jurisdiction} \colorbox{red!2}{\strut Sales} \colorbox{red!0}{\strut TaxLouisiana} \colorbox{red!0}{\strut State} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut 5.00} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut County} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut City} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut NASpecial} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut NACombined} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut 9.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut data} \colorbox{red!0}{\strut incorrect} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Download} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rates} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut zip} \colorbox{red!0}{\strut codeThe} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 9.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut consisting} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 5.00} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut state} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut taxes.The} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut consists} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut county} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut tax.The} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut collected} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut merchant} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut qualifying} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut within} \colorbox{red!3}{\strut Jefferson} \colorbox{red!0}{\strut ParishGroceries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut exempt} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut state} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut taxesJefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut collects} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 4.75} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut maximum} \colorbox{red!0}{\strut local} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut allowed} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut lawJefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lower} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 59.6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut cities} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut countiesJefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut Louisiana} \colorbox{red!2}{\strut Sales} \colorbox{red!3}{\strut Tax} \colorbox{red!0}{\strut ExemptionsIn} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut essential} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut medicine} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut groceries} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut exempted} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut eligible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lower} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Jefferson} \colorbox{red!3}{\strut Parish} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut collect} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut groceries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Certain} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut alcohol} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cigarettes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut gasoline} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut additional} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut excise} \colorbox{red!3}{\strut taxes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut sales} \colorbox{red!0}{\strut tax.Note} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut alcohol} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut prepared} \colorbox{red!0}{\strut food} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut restaurant} \colorbox{red!0}{\strut meals} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut premade} \colorbox{red!0}{\strut supermarket} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut charged} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut higher} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rate} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Louisiana} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut sales} \colorbox{red!3}{\strut tax} \colorbox{red!1}{\strut rates} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut commonly} \colorbox{red!0}{\strut exempted} \colorbox{red!0}{\strut categories} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut listed} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut Sales} \colorbox{red!5}{\strut Tax} \colorbox{red!2}{\strut Holidays} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2013} \colorbox{red!5}{\strut Louisiana} \colorbox{red!5}{\strut Taxes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Income} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Sales} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Property} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Corporate} \colorbox{red!5}{\strut Tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Excise} \colorbox{red!0}{\strut TaxesLouisiana} \colorbox{red!4}{\strut Sales} \colorbox{red!5}{\strut Tax} \colorbox{red!2}{\strut Holidays} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2013A} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut special} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut allowed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut purchase} \colorbox{red!0}{\strut certain} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut pay} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut buy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 500.00} \colorbox{red!0}{\strut worth} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut goods} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20.00.Louisiana} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut five} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut throughout} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut goods} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut calendar} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut lists} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut major} \colorbox{red!5}{\strut Louisiana} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut item} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut applies} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut purchase} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut holiday} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut person} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Sale} \colorbox{red!0}{\strut Dates} \colorbox{red!2}{\strut Sale} \colorbox{red!0}{\strut Item} \colorbox{red!2}{\strut Sale} \colorbox{red!0}{\strut Maximum} \colorbox{red!0}{\strut Cost} \colorbox{red!2}{\strut Sale} \colorbox{red!0}{\strut Start} \colorbox{red!0}{\strut YearSeptember} \colorbox{red!0}{\strut 6th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 8th} \colorbox{red!0}{\strut Ammunition} \colorbox{red!0}{\strut NO} \colorbox{red!0}{\strut LIMIT} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 6th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 8th} \colorbox{red!0}{\strut Firearms} \colorbox{red!0}{\strut NO} \colorbox{red!0}{\strut LIMIT} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 6th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 8th} \colorbox{red!0}{\strut Hunting} \colorbox{red!0}{\strut Supplies} \colorbox{red!0}{\strut NO} \colorbox{red!0}{\strut LIMIT} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 25th} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 26th} \colorbox{red!0}{\strut Hurricane} \colorbox{red!0}{\strut Preparedness} \colorbox{red!0}{\strut Items} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,500.00} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 2nd} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 3rd} \colorbox{red!0}{\strut TPP} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2,500.00} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Why} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut have} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut dozen} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut throughout} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut these} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut promotions} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut promote} \colorbox{red!0}{\strut desirable} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut energy-star} \colorbox{red!0}{\strut rated} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut emergency} \colorbox{red!0}{\strut preparedness} \colorbox{red!0}{\strut supplies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut hold} \colorbox{red!4}{\strut sales} \colorbox{red!5}{\strut tax} \colorbox{red!2}{\strut holidays} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut correspond} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut back-to-school} \colorbox{red!0}{\strut shopping} \colorbox{red!0}{\strut season} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut books} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut clothing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut school} \colorbox{red!0}{\strut supplies.In} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

query: percentage of people with security clearance

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Security} \colorbox{red!9}{\strut Clearance} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Who} \colorbox{red!0}{\strut Needs} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut Security} \colorbox{red!9}{\strut Clearance} \colorbox{red!0}{\strut Help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Who} \colorbox{red!0}{\strut Needs} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Few} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut realize} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut issues} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut affect} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut ability} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut obtain} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut security} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut applicant} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut interest} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut advance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut decide} \colorbox{red!0}{\strut early} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut help.Security} \colorbox{red!0}{\strut ClearanceWilliam} \colorbox{red!0}{\strut Henderson} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mar} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012Sign} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Cleared} \colorbox{red!0}{\strut Brief} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Latest} \colorbox{red!4}{\strut security} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut news} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut delivered} \colorbox{red!0}{\strut monthly.19Many} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut themselves} \colorbox{red!0}{\strut filling} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Standard} \colorbox{red!0}{\strut Form} \colorbox{red!0}{\strut 86} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SF86} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Questionnaire} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut National} \colorbox{red!4}{\strut Security} \colorbox{red!0}{\strut Positions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut security} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut vague} \colorbox{red!0}{\strut understanding} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut what} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut affect} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut eligibility} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut receive} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut scour} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut internet} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Others} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut rely} \colorbox{red!0}{\strut entirely} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut guidance} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut sponsor} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!4}{\strut security} \colorbox{red!0}{\strut officer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut thorough} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Few} \colorbox{red!0}{\strut seek} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut assistance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut security} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut consultant} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut attorney.The} \colorbox{red!1}{\strut average} \colorbox{red!4}{\strut security} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut denial} \colorbox{red!0}{\strut rate} \colorbox{red!0}{\strut among} \colorbox{red!0}{\strut federal} \colorbox{red!0}{\strut agencies} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 2.5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut doesn} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut mean} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut 97.5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut population} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut eligible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut means} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut final} \colorbox{red!0}{\strut stages} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut security} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2.5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut denied} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut don} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut bother} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut apply} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut jobs} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut require} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut believe} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut factors} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut life} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut inevitably} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut denial} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut potential} \colorbox{red!0}{\strut applicants} \colorbox{red!0}{\strut fail} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut receive} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut sponsorship} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut screened} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut prospective} \colorbox{red!0}{\strut employers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Others} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut initially} \colorbox{red!0}{\strut receive} \colorbox{red!0}{\strut sponsorship} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut sponsorship} \colorbox{red!0}{\strut withdrawn} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut final} \colorbox{red!9}{\strut clearance} \colorbox{red!0}{\strut decision} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut fail} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut receive} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut interim} \colorbox{red!9}{\strut clearance} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Bankruptcy} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Security} \colorbox{red!8}{\strut Clearance} \colorbox{red!0}{\strut Issues} \colorbox{red!3}{\strut Bankruptcy} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Security} \colorbox{red!8}{\strut Clearance} \colorbox{red!0}{\strut IssuesWhat} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut My} \colorbox{red!4}{\strut Security} \colorbox{red!8}{\strut Clearance} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut done} \colorbox{red!1}{\strut bankruptcies} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut hundreds} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut people} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut have} \colorbox{red!4}{\strut security} \colorbox{red!8}{\strut clearances} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut told} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut their} \colorbox{red!4}{\strut security} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut would} \colorbox{red!2}{\strut lose} \colorbox{red!0}{\strut their} \colorbox{red!8}{\strut clearance} \colorbox{red!0}{\strut unless} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut filed} \colorbox{red!3}{\strut bankruptcy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Having} \colorbox{red!0}{\strut trouble} \colorbox{red!1}{\strut paying} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut debts} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut automatic} \colorbox{red!0}{\strut grounds} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut losing} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut clearancebecause} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut desperate} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut money} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut selling} \colorbox{red!0}{\strut things} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut don} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut t} \colorbox{red!0}{\strut belong} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut agree} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut probably} \colorbox{red!0}{\strut don} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut t} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut six} \colorbox{red!1}{\strut people} \colorbox{red!1}{\strut who} \colorbox{red!1}{\strut lost} \colorbox{red!0}{\strut their} \colorbox{red!4}{\strut security} \colorbox{red!8}{\strut clearance} \colorbox{red!0}{\strut after} \colorbox{red!1}{\strut filing} \colorbox{red!3}{\strut bankruptcy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Three} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut ignoring} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut bills} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dragging} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut bad} \colorbox{red!0}{\strut credit} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut doing} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut review} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut stupid} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut trusted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Bankruptcy} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut itself} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut deny} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut security} \colorbox{red!8}{\strut clearance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut against} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut combination} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut worked} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut perhaps} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!3}{\strut secure} \colorbox{red!0}{\strut location} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut t} \colorbox{red!0}{\strut explain.I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut several} \colorbox{red!1}{\strut people} \colorbox{red!1}{\strut who} \colorbox{red!1}{\strut did} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut have} \colorbox{red!8}{\strut clearances} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut denied} \colorbox{red!0}{\strut interim} \colorbox{red!8}{\strut clearances} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut applied} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut bankruptcy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut fought} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Fourth} \colorbox{red!0}{\strut Circuit} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut lost.Security} \colorbox{red!8}{\strut Clearances} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut BankruptcyAs} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut rule} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut people} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut clearance} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut aren} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut t} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut trouble} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut else} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!2}{\strut lose} \colorbox{red!0}{\strut their} \colorbox{red!8}{\strut clearances} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut bankruptcy} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut People} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut applying} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut clearance} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut everything} \colorbox{red!0}{\strut possible} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!0}{\strut everything} \colorbox{red!0}{\strut current} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut clearance} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut approved.In} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut parts} \colorbox{red!0}{\strut of} 
}}}
\end{CJK*}

query: what is the hormone that makes you fat

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Simple} \colorbox{red!0}{\strut Way} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Fix} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Hormones} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut Make} \colorbox{red!0}{\strut You} \colorbox{red!4}{\strut Fat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!21}{\strut cause} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut obesityYour} \colorbox{red!0}{\strut browser} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut recognize} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut formats} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut frequently} \colorbox{red!0}{\strut asked} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut HTML5} \colorbox{red!0}{\strut video.000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1556} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Insulin} \colorbox{red!0}{\strut shunts} \colorbox{red!2}{\strut sugar} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut fat} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Insulin} \colorbox{red!0}{\strut makes} \colorbox{red!4}{\strut fat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!3}{\strut insulin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut more} \colorbox{red!4}{\strut fat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Period} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut involved} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut nutrition} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut probably} \colorbox{red!0}{\strut heard} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Dr.} \colorbox{red!0}{\strut Robert} \colorbox{red!0}{\strut Lustig.He} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pediatric} \colorbox{red!0}{\strut endocrinologist} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut expert} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut childhood} \colorbox{red!21}{\strut obesity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut became} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut viral} \colorbox{red!0}{\strut YouTube} \colorbox{red!0}{\strut lecture} \colorbox{red!0}{\strut called} \colorbox{red!2}{\strut Sugar} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Bitter} \colorbox{red!0}{\strut Truth.In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut interviewed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Dr.} \colorbox{red!0}{\strut Andreas} \colorbox{red!0}{\strut Eenfeldt} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut about} \colorbox{red!10}{\strut what} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut believes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut true} \colorbox{red!21}{\strut cause} \colorbox{red!0}{\strut of} \colorbox{red!21}{\strut obesity} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut diseases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut civilization.There} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Biochemical} \colorbox{red!0}{\strut Forces} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut Make} \colorbox{red!0}{\strut Us} \colorbox{red!2}{\strut Eat} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Exercise} \colorbox{red!0}{\strut LessSome} \colorbox{red!1}{\strut people} \colorbox{red!0}{\strut believe} \colorbox{red!0}{\strut that} \colorbox{red!21}{\strut obesity} \colorbox{red!0}{\strut is} \colorbox{red!20}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut eating} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut exercising} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut little.In} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut words} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut behavior} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut driving} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut weight} \colorbox{red!1}{\strut gain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut individual} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut fault} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut happened.However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Lustig} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut believe} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut majority} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut people.He} \colorbox{red!0}{\strut believes} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut behavior} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut increased} \colorbox{red!1}{\strut food} \colorbox{red!0}{\strut intake} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut decreased} \colorbox{red!1}{\strut exercise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut secondary} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut changes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut function} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut hormones} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .It} \colorbox{red!0}{\strut turns} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut defined} \colorbox{red!0}{\strut biological} \colorbox{red!0}{\strut mechanisms} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut explain} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut foods} \colorbox{red!0}{\strut we} \colorbox{red!2}{\strut eat} \colorbox{red!0}{\strut disrupt} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut function} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut hormones} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut makes} \colorbox{red!0}{\strut us} \colorbox{red!2}{\strut eat} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut gain} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .In} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut words} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut getting} \colorbox{red!4}{\strut fat} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut re} \colorbox{red!3}{\strut eating} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut re} \colorbox{red!3}{\strut eating} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut getting} \colorbox{red!0}{\strut fat.Insulin} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Leptin} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut Two} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Major} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Fat} \colorbox{red!6}{\strut Cells} \colorbox{red!4}{\strut Make} \colorbox{red!6}{\strut Estrogen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Fat} \colorbox{red!6}{\strut Cells} \colorbox{red!4}{\strut Make} \colorbox{red!6}{\strut Estrogen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut November} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut Breast} \colorbox{red!1}{\strut Cancer} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Nutrition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Breast} \colorbox{red!1}{\strut Cancer} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Obesity} \colorbox{red!0}{\strut breast} \colorbox{red!1}{\strut cancer} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut obesity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut breast} \colorbox{red!1}{\strut cancer} \colorbox{red!0}{\strut blog} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut fat} \colorbox{red!6}{\strut cells} \colorbox{red!4}{\strut make} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut fat} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut hormones} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fatTweetImage} \colorbox{red!0}{\strut source} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut freedigitalphotos.net} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Master} \colorbox{red!0}{\strut Isolated} \colorbox{red!0}{\strut ImagesFat} \colorbox{red!6}{\strut Cells} \colorbox{red!4}{\strut Make} \colorbox{red!6}{\strut Estrogen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Why} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut continually} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut told} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut cut} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut breast} \colorbox{red!1}{\strut cancer} \colorbox{red!0}{\strut risk} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut lose} \colorbox{red!0}{\strut weight} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Because} \colorbox{red!2}{\strut fat} \colorbox{red!6}{\strut cells} \colorbox{red!4}{\strut make} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut cause} \colorbox{red!0}{\strut big} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut why.The} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut carry} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut more} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut produce} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut vice} \colorbox{red!0}{\strut versa} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut biggest} \colorbox{red!0}{\strut majority} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut breast} \colorbox{red!1}{\strut cancer} \colorbox{red!0}{\strut tumors} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut fueled} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut over-abundance} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut circulating} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut body} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut complicate} \colorbox{red!0}{\strut matters} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut fat} \colorbox{red!6}{\strut cells} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut loaded} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut aromatase} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut enzyme} \colorbox{red!0}{\strut required} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut biosynthesis} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut higher} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut body} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut more} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut produce} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut fatter} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut unless} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut stop} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut cycle} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut nutrition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut stress} \colorbox{red!0}{\strut reduction} \colorbox{red!0}{\strut steps.Estrogen} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut come} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut abundance} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut sources} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut body} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut own} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut High} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut estrogen} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut come} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut stress} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut cortisol} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut hormone} \colorbox{red!0}{\strut secreted} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut stress} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut causes} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut body} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut store} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut belly} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut More} \colorbox{red!2}{\strut fat} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut estrogen.Estrogen} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut come} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut xenoestrogens} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut false} \colorbox{red!6}{\strut estrogens} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut environment} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut chemically-laden} \colorbox{red!1}{\strut body} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut Protect} \colorbox{red!0}{\strut Yourself} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Xenoestrogens} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Estrogen} \colorbox{red!0}{\strut Dominance} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut subject.High} \colorbox{red!0}{\strut calorie} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fat-filled} \colorbox{red!1}{\strut foods} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut blame} \colorbox{red!0}{\strut for} 
}}}
\end{CJK*}

query: how many years back to the clinton tax returns go

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Hillary} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut Releases} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut Years} \colorbox{red!0}{\strut Of} \colorbox{red!7}{\strut Tax} \colorbox{red!1}{\strut Returns} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Enlarge} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut imageDemocratic} \colorbox{red!1}{\strut presidential} \colorbox{red!1}{\strut hopeful} \colorbox{red!8}{\strut Hillary} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut campaign} \colorbox{red!0}{\strut event} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Iowa} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut week.Scott} \colorbox{red!0}{\strut OlsonGetty} \colorbox{red!0}{\strut ImagesThis} \colorbox{red!0}{\strut post} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut updated} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut 645} \colorbox{red!0}{\strut p.m.} \colorbox{red!0}{\strut ETDemocratic} \colorbox{red!1}{\strut presidential} \colorbox{red!1}{\strut hopeful} \colorbox{red!8}{\strut Hillary} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut released} \colorbox{red!0}{\strut eight} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut worth} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut tax} \colorbox{red!1}{\strut returns} \colorbox{red!0}{\strut Friday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut showing} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut husband} \colorbox{red!1}{\strut Bill} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut earned} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 139} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut paid} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 44} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut federal} \colorbox{red!7}{\strut taxes} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut couple} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut effective} \colorbox{red!0}{\strut federal} \colorbox{red!7}{\strut tax} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut ranged} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2007} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 36} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut year.The} \colorbox{red!8}{\strut Clintons} \colorbox{red!0}{\strut paid} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut state} \colorbox{red!1}{\strut income} \colorbox{red!7}{\strut taxes} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut gave} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut charity.Much} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut couple} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut came} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut giving} \colorbox{red!0}{\strut paid} \colorbox{red!0}{\strut speeches.HillaryClinton.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut long} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut going} \colorbox{red!0}{\strut door-to-door} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Children} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Defense} \colorbox{red!0}{\strut Fund} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut earning} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16,450} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut young} \colorbox{red!0}{\strut law} \colorbox{red!0}{\strut professor} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Arkansas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Hillary} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut owe} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut opportunities} \colorbox{red!0}{\strut America} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut couple} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut released} \colorbox{red!7}{\strut tax} \colorbox{red!1}{\strut returns} \colorbox{red!0}{\strut dating} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 1977.Republican} \colorbox{red!1}{\strut presidential} \colorbox{red!0}{\strut candidate} \colorbox{red!0}{\strut Jeb} \colorbox{red!1}{\strut Bush} \colorbox{red!0}{\strut released} \colorbox{red!0}{\strut decades} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut tax} \colorbox{red!1}{\strut returns} \colorbox{red!0}{\strut earlier} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut month} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut showing} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut effective} \colorbox{red!0}{\strut federal} \colorbox{red!7}{\strut tax} \colorbox{red!4}{\strut rate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut roughly} \colorbox{red!0}{\strut 36} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bush} \colorbox{red!0}{\strut lives} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Florida} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut state} \colorbox{red!1}{\strut income} \colorbox{red!0}{\strut tax.Hillary} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut complained} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut statement} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut federal} \colorbox{red!7}{\strut tax} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut loopholes} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut allow} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut wealthiest} \colorbox{red!0}{\strut Americans} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut powerful} \colorbox{red!0}{\strut corporations} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut game} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut avoid} \colorbox{red!0}{\strut paying} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut fair} \colorbox{red!0}{\strut share} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut sign} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut either} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut Bush} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut taken} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut loopholes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut though} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Both} \colorbox{red!0}{\strut candidates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut effective} \colorbox{red!7}{\strut tax} \colorbox{red!4}{\strut rates} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut Americans} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Clinton} \colorbox{red!6}{\strut Foundation} \colorbox{red!4}{\strut amends} \colorbox{red!0}{\strut four} \colorbox{red!1}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut tax} \colorbox{red!3}{\strut returns} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PresidentialClinton} \colorbox{red!6}{\strut Foundation} \colorbox{red!4}{\strut amends} \colorbox{red!0}{\strut four} \colorbox{red!1}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut tax} \colorbox{red!0}{\strut returnsPublished} \colorbox{red!0}{\strut November} \colorbox{red!0}{\strut 17} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2015} \colorbox{red!1}{\strut Fox} \colorbox{red!0}{\strut NewsFacebook} \colorbox{red!0}{\strut Twitter} \colorbox{red!0}{\strut livefyre} \colorbox{red!0}{\strut EmailThe} \colorbox{red!8}{\strut Clinton} \colorbox{red!6}{\strut Foundation} \colorbox{red!0}{\strut announced} \colorbox{red!0}{\strut late} \colorbox{red!0}{\strut Monday} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut had} \colorbox{red!5}{\strut amended} \colorbox{red!0}{\strut its} \colorbox{red!3}{\strut tax} \colorbox{red!3}{\strut return} \colorbox{red!0}{\strut forms} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut four} \colorbox{red!0}{\strut separate} \colorbox{red!1}{\strut years} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut errors} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut reporting} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut donations} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut foreign} \colorbox{red!0}{\strut governments.ADVERTISEMENTFoundation} \colorbox{red!2}{\strut President} \colorbox{red!1}{\strut Donna} \colorbox{red!0}{\strut Shalala} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut statement} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut returns} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut revised} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut voluntary} \colorbox{red!0}{\strut review} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut charity} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut past} \colorbox{red!3}{\strut tax} \colorbox{red!3}{\strut returns} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut She} \colorbox{red!0}{\strut added} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut corrections} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut required} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut law} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut change} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut bottom} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut numbers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut assets} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut liabilities} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut net} \colorbox{red!0}{\strut assets} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Shalala} \colorbox{red!0}{\strut wrote} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut statement} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut foundation} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut supporters} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut obtained} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Reuters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut nothing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut suggest} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut Foundation} \colorbox{red!0}{\strut intended} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut conceal} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut receipt} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut grants} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut website} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut amended} \colorbox{red!1}{\strut Form} \colorbox{red!0}{\strut 990} \colorbox{red!3}{\strut tax} \colorbox{red!3}{\strut returns} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut years} \colorbox{red!0}{\strut 2010} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2011} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 2013} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut affiliated} \colorbox{red!0}{\strut charity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut Health} \colorbox{red!0}{\strut Access} \colorbox{red!0}{\strut Initiative} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!5}{\strut amended} \colorbox{red!0}{\strut its} \colorbox{red!3}{\strut returns} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 2013.The} \colorbox{red!6}{\strut foundation} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut reports} \colorbox{red!1}{\strut receiving} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut funds} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 2010} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 2013} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut foreign} \colorbox{red!1}{\strut governments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!6}{\strut foundation} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut neglected} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut government} \colorbox{red!1}{\strut funding} \colorbox{red!0}{\strut separately} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut funding} \colorbox{red!0}{\strut sources} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut original} \colorbox{red!0}{\strut returns.More} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Emails} \colorbox{red!0}{\strut reveal} \colorbox{red!0}{\strut influence} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut Clinton} \colorbox{red!6}{\strut Foundation} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut State} \colorbox{red!0}{\strut Dept.The} \colorbox{red!6}{\strut foundation} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut revealed} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut raised} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 177} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut before} \colorbox{red!3}{\strut Hillary} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut announced} \colorbox{red!0}{\strut her} \colorbox{red!1}{\strut run} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut presidency.The} \colorbox{red!8}{\strut Clinton} \colorbox{red!6}{\strut Foundation} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut fundraising} \colorbox{red!0}{\strut efforts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut particularly} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut involving} \colorbox{red!1}{\strut foreign} \colorbox{red!1}{\strut governments} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut scrutiny} \colorbox{red!0}{\strut as} \colorbox{red!8}{\strut Clinton} \colorbox{red!0}{\strut moves} \colorbox{red!0}{\strut toward} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Democratic} \colorbox{red!1}{\strut presidential} \colorbox{red!0}{\strut nomination} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Critics} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut foundation} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut dealings} 
}}}
\end{CJK*}

query: chance of rain pembroke pines

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!19}{\strut Pembroke} \colorbox{red!19}{\strut Pines} \colorbox{red!19}{\strut Weather} \colorbox{red!3}{\strut Forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Monday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 09} \colorbox{red!19}{\strut Pembroke} \colorbox{red!19}{\strut Pines} \colorbox{red!19}{\strut Weather} \colorbox{red!3}{\strut Forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Monday} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 09Countries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Florida} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 33028The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 59} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut South.80Monday} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 0984Tuesday} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 1080Wednesday} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 1178Thursday} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 1281Friday} \colorbox{red!0}{\strut April} \colorbox{red!0}{\strut 13Current} \colorbox{red!0}{\strut Conditionssubmit} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut forecast80Hourly} \colorbox{red!0}{\strut Forecast0am743am736am729am7412am803pm826pm819pm80Weather} \colorbox{red!0}{\strut Photosadd} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut photoHourly} \colorbox{red!3}{\strut Forecast} \colorbox{red!0}{\strut Detailed0am} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 74} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Southwest.3am} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 73} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 86} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut East.6am} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 72} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut South-Southwest.9am} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 74} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 78} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut South.12am} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 59} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut South.3pm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 82} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 58} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut South.6pm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 81} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 57} \colorbox{red!0}{\strut percentage} \colorbox{red!0}{\strut chance} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 9} \colorbox{red!0}{\strut mph} \colorbox{red!0}{\strut winds} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut South-Southwest.9pm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut 33028} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut FL} \colorbox{red!3}{\strut forecast} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 09} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Partly} \colorbox{red!0}{\strut cloudy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Pembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Pembroke} \colorbox{red!0}{\strut PinesPembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut FLFavoriteShareMoreNearbyDirectionsSponsored} \colorbox{red!0}{\strut TopicsDescriptionPembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Broward} \colorbox{red!6}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Florida} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut population} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 154,750} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 2010} \colorbox{red!0}{\strut census} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut making} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut populous} \colorbox{red!1}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Broward} \colorbox{red!6}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tenth} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut populous} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut Florida} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 150th} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut populous} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Its} \colorbox{red!0}{\strut official} \colorbox{red!0}{\strut motto} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Join} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Progress} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Us} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Pembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut named} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut best} \colorbox{red!1}{\strut cities} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut live} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut America} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Pembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut won} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut National} \colorbox{red!0}{\strut Civic} \colorbox{red!0}{\strut League} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut coveted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All-America} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut Award} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2004} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut finalist} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2003} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Pembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut received} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut outstanding} \colorbox{red!0}{\strut achievement} \colorbox{red!0}{\strut award} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2005} \colorbox{red!1}{\strut City} \colorbox{red!0}{\strut Livability} \colorbox{red!0}{\strut Awards} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Program} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sponsored} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut Conference} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Mayors} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut Pembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut schools} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut received} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Five} \colorbox{red!0}{\strut Star} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut Award} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut Florida} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Education} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut schools} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut shown} \colorbox{red!0}{\strut evidence} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut exemplary} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut involvement} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Pembroke} \colorbox{red!8}{\strut Pines} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut incorporated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1960} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut took} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut name} \colorbox{red!8}{\strut Pembroke} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut location} \colorbox{red!0}{\strut along} \colorbox{red!8}{\strut Pembroke} \colorbox{red!0}{\strut Road} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut many} \colorbox{red!7}{\strut pine} \colorbox{red!0}{\strut trees} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut name} \colorbox{red!8}{\strut Pembroke} \colorbox{red!0}{\strut dates} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut name} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut early} \colorbox{red!0}{\strut landowner} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Britain} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Earl} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut Pembroke} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: average salary for firefighters in az

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Phoenix} \colorbox{red!7}{\strut Fire} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Arizona} \colorbox{red!7}{\strut Firefighter} \colorbox{red!8}{\strut Salaries} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!4}{\strut Phoenix} \colorbox{red!7}{\strut Fire} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Arizona} \colorbox{red!7}{\strut Firefighter} \colorbox{red!8}{\strut Salaries} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States1} \colorbox{red!8}{\strut Salary} \colorbox{red!0}{\strut Updated} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2012United} \colorbox{red!0}{\strut States} \colorbox{red!4}{\strut Phoenix} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AZ} \colorbox{red!0}{\strut AreaAny} \colorbox{red!0}{\strut Experience0-1} \colorbox{red!0}{\strut Years1-3} \colorbox{red!0}{\strut Years4-6} \colorbox{red!0}{\strut Years7-9} \colorbox{red!0}{\strut Years10-14} \colorbox{red!0}{\strut Years15} \colorbox{red!0}{\strut YearsSearchBase} \colorbox{red!0}{\strut Pay} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 48K} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 53KTotal} \colorbox{red!0}{\strut Pay} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 49K} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 52KAdditional} \colorbox{red!0}{\strut PayNo} \colorbox{red!0}{\strut ReportsCash} \colorbox{red!0}{\strut Bonus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Stock} \colorbox{red!0}{\strut Bonus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Profit} \colorbox{red!0}{\strut Sharing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Commission} \colorbox{red!0}{\strut Sharing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Tips} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut roleRelated} \colorbox{red!0}{\strut Searches} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!7}{\strut Firefighter} \colorbox{red!8}{\strut Salaries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!4}{\strut Phoenix} \colorbox{red!7}{\strut Fire} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Arizona} \colorbox{red!0}{\strut SalariesFirefighter} \colorbox{red!8}{\strut salaries} \colorbox{red!0}{\strut at} \colorbox{red!4}{\strut Phoenix} \colorbox{red!7}{\strut Fire} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Arizona} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 48,040-} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 52,512} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut estimate} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut upon} \colorbox{red!0}{\strut 1} \colorbox{red!4}{\strut Phoenix} \colorbox{red!7}{\strut Fire} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Arizona} \colorbox{red!7}{\strut Firefighter} \colorbox{red!8}{\strut salary} \colorbox{red!0}{\strut report} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut employees} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut estimated} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut upon} \colorbox{red!0}{\strut statistical} \colorbox{red!0}{\strut methods} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut all} \colorbox{red!7}{\strut Firefighter} \colorbox{red!8}{\strut salaries} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut learn} \colorbox{red!1}{\strut how} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut stacks} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut market.Are} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut paid} \colorbox{red!0}{\strut fairly} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut personalized} \colorbox{red!8}{\strut salary} \colorbox{red!0}{\strut estimate} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut today} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut marketGet} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut EstimateSalaries} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Firefighter} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Phoenix} \colorbox{red!7}{\strut Fire} \colorbox{red!1}{\strut Department} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut Arizona} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Embed} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut report} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut Firefighter} \colorbox{red!8}{\strut Salaries} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Mesa} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AZ} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Firefighter} \colorbox{red!8}{\strut Salaries} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Mesa} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AZSalary} \colorbox{red!0}{\strut estimated} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 224} \colorbox{red!1}{\strut employees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut users} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut present} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut advertisements} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Indeed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut 36} \colorbox{red!0}{\strut months} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Last} \colorbox{red!0}{\strut updated} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut March} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2018LocationPopular} \colorbox{red!1}{\strut Jobs} \colorbox{red!7}{\strut Average} \colorbox{red!8}{\strut Salary} \colorbox{red!8}{\strut Salary} \colorbox{red!0}{\strut DistributionCustom} \colorbox{red!1}{\strut Protection} \colorbox{red!0}{\strut Officer170} \colorbox{red!8}{\strut salaries} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12.91} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut hourMost} \colorbox{red!0}{\strut Reported} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7.25} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 22.45Custom} \colorbox{red!1}{\strut Protection} \colorbox{red!1}{\strut Officer} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Mesa} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AZEmergency} \colorbox{red!1}{\strut Medicine} \colorbox{red!0}{\strut Physician17} \colorbox{red!8}{\strut salaries} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 61,333} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 14,500} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 44,900Emergency} \colorbox{red!1}{\strut Medicine} \colorbox{red!1}{\strut Physician} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Mesa} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AZPhysician5} \colorbox{red!8}{\strut salaries} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 46.64} \colorbox{red!0}{\strut per} \colorbox{red!1}{\strut hour} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7.25} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 22.45Physician} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Mesa} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut AZWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut average} \colorbox{red!8}{\strut salary} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut jobs} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut firefighter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut average} \colorbox{red!8}{\strut salary} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut firefighter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ranges} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut approximately} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 12.91} \colorbox{red!0}{\strut per} \colorbox{red!1}{\strut hour} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Custom} \colorbox{red!1}{\strut Protection} \colorbox{red!1}{\strut Officer} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 46.64} \colorbox{red!0}{\strut per} \colorbox{red!1}{\strut hour} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Physician.Salary} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 224} \colorbox{red!0}{\strut data} \colorbox{red!0}{\strut points} \colorbox{red!0}{\strut collected} \colorbox{red!0}{\strut directly} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut employees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut users} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut present} \colorbox{red!1}{\strut job} \colorbox{red!0}{\strut advertisements} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Indeed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut 36} \colorbox{red!0}{\strut months.Please} \colorbox{red!0}{\strut note} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut all} \colorbox{red!8}{\strut salary} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut approximations} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut upon} \colorbox{red!0}{\strut third} \colorbox{red!0}{\strut party} \colorbox{red!0}{\strut submissions} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Indeed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Indeed} \colorbox{red!0}{\strut users} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut purpose} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut generalized} \colorbox{red!0}{\strut comparison} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Minimum} \colorbox{red!1}{\strut wage} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut differ} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut jurisdiction} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut consult} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut employer} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut actual} \colorbox{red!8}{\strut salary} \colorbox{red!0}{\strut figures} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what to do when you run out of storage on lg optimus

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut SD} \colorbox{red!9}{\strut Card} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut LG} \colorbox{red!1}{\strut Optimus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Home} \colorbox{red!0}{\strut Buying} \colorbox{red!0}{\strut Guides} \colorbox{red!1}{\strut Cell} \colorbox{red!6}{\strut Phones} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Accessories} \colorbox{red!1}{\strut Cell} \colorbox{red!6}{\strut Phones} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SmartphonesHow} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut SD} \colorbox{red!9}{\strut Card} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut LG} \colorbox{red!0}{\strut OptimuseBay} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Likes} \colorbox{red!0}{\strut LikeSeptember} \colorbox{red!0}{\strut 19} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2016There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut cell} \colorbox{red!6}{\strut phones} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut market} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut individual} \colorbox{red!0}{\strut brands} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut array} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut devices} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut technical} \colorbox{red!0}{\strut specifications} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut LG} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut those} \colorbox{red!1}{\strut cell} \colorbox{red!6}{\strut phone} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut LG} \colorbox{red!0}{\strut markets} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut Optimus} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut smartphones} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut consumers} \colorbox{red!0}{\strut according} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut economic} \colorbox{red!1}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut early} \colorbox{red!1}{\strut Optimus} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut lacking} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut models} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut flagship} \colorbox{red!8}{\strut LG} \colorbox{red!1}{\strut Optimus} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut high-tech} \colorbox{red!0}{\strut mobile} \colorbox{red!6}{\strut phones} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut incorporates} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut SD} \colorbox{red!9}{\strut card} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut removable} \colorbox{red!0}{\strut data} \colorbox{red!0}{\strut storage} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut allows} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut greater} \colorbox{red!0}{\strut adaptability} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut how} \colorbox{red!0}{\strut files} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut removable} \colorbox{red!0}{\strut storage} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut phone} \colorbox{red!0}{\strut depends} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut chosen} \colorbox{red!0}{\strut model} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut eBay} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut host} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut LG} \colorbox{red!0}{\strut memory} \colorbox{red!9}{\strut cards} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut data} \colorbox{red!0}{\strut capacities} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut GB} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 64} \colorbox{red!0}{\strut GB} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut enabling} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!6}{\strut SD} \colorbox{red!9}{\strut card} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Those} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut data} \colorbox{red!0}{\strut space} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut opt} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut GB} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut GB} \colorbox{red!0}{\strut size} \colorbox{red!0}{\strut device} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut expensive} \colorbox{red!0}{\strut model} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut LG} \colorbox{red!1}{\strut Optimus} \colorbox{red!0}{\strut L70} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut robust} \colorbox{red!1}{\strut smartphone} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut sleek} \colorbox{red!0}{\strut black} \colorbox{red!0}{\strut design} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut priced} \colorbox{red!0}{\strut fairly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Much} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Mac} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut jailbreaking} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut frees} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut limitations} \colorbox{red!0}{\strut imposed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut software} \colorbox{red!0}{\strut team} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Androids} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut rooting} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut root} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Android} \colorbox{red!6}{\strut phone} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut an} \colorbox{red!8}{\strut LG} \colorbox{red!1}{\strut Optimus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut unlocks} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut data} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut so} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Memory} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SD} \colorbox{red!3}{\strut card} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut LG} \colorbox{red!4}{\strut Optimus} \colorbox{red!5}{\strut L9} \colorbox{red!1}{\strut Learn} \colorbox{red!8}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut task} \colorbox{red!2}{\strut manager} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut view} \colorbox{red!1}{\strut free} \colorbox{red!0}{\strut space} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut free} \colorbox{red!0}{\strut up} \colorbox{red!3}{\strut memory} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut storage} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut LG} \colorbox{red!4}{\strut Optimus} \colorbox{red!5}{\strut L9} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut sd} \colorbox{red!3}{\strut card} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Internal} \colorbox{red!3}{\strut memory} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut RAM} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Internal} \colorbox{red!2}{\strut storage} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut ROM} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut SD} \colorbox{red!0}{\strut cardInternal} \colorbox{red!3}{\strut memory} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut RAM} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Manage} \colorbox{red!0}{\strut memoryTo} \colorbox{red!3}{\strut manage} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut internal} \colorbox{red!3}{\strut memory} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut follow} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut steps} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Restart} \colorbox{red!1}{\strut device} \colorbox{red!0}{\strut regularlyNote} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut should} \colorbox{red!1}{\strut restart} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut phone} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut day.Press} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut hold} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Power} \colorbox{red!0}{\strut key.Tap} \colorbox{red!1}{\strut Power} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut restart.Reduce} \colorbox{red!3}{\strut memory} \colorbox{red!0}{\strut useNote} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut phone} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut running} \colorbox{red!0}{\strut slow} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut reduce} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut memory} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut using.Reduce} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut RAM} \colorbox{red!1}{\strut clear} \colorbox{red!0}{\strut periodFrom} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut screen} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut press} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut hold} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut key.Tap} \colorbox{red!2}{\strut Task} \colorbox{red!0}{\strut Manager.Tap} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Menu} \colorbox{red!1}{\strut key} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!1}{\strut tap} \colorbox{red!1}{\strut Settings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Note} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Make} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Check} \colorbox{red!0}{\strut box} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Auto} \colorbox{red!1}{\strut Clear} \colorbox{red!3}{\strut RAM} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut selected.Tap} \colorbox{red!0}{\strut Auto-clear} \colorbox{red!0}{\strut period.Tap} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut desired} \colorbox{red!0}{\strut setting} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut determines} \colorbox{red!8}{\strut how} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut RAM} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut cleared.Remove} \colorbox{red!0}{\strut widgets} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Animated} \colorbox{red!0}{\strut widgets} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut widgets} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut update} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!3}{\strut memory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut desired} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut screen} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut touch} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut hold} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut widget.Drag} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut widget} \colorbox{red!0}{\strut over} \colorbox{red!1}{\strut Remove} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut release} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut finger.Replace} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Live} \colorbox{red!0}{\strut wallpaperFrom} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut screen} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut touch} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut hold} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut screen} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!1}{\strut tap} \colorbox{red!0}{\strut Wallpapers.Tap} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut Gallery} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Wallpaper} \colorbox{red!0}{\strut thumbnail} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Live} \colorbox{red!0}{\strut Wallpapers.Follow} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut prompts} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut set} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut wallpaper} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut replaces} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut current} \colorbox{red!1}{\strut Live} \colorbox{red!0}{\strut wallpaper.Remove} \colorbox{red!0}{\strut unused} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut screensFrom} \colorbox{red!0}{\strut any} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut screen} \colorbox{red!1}{\strut tap} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Menu} \colorbox{red!1}{\strut key} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!1}{\strut tap} \colorbox{red!0}{\strut Edit} \colorbox{red!1}{\strut home} \colorbox{red!0}{\strut screens.Touch} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut hold} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Home} \colorbox{red!1}{\strut screen} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut deleted.Drag} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut over} \colorbox{red!1}{\strut Remove} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut release} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut finger} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tap} \colorbox{red!0}{\strut OK.Manage} \colorbox{red!0}{\strut applicationsNote} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Manage} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut applications} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut keep} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut device} \colorbox{red!1}{\strut running} \colorbox{red!0}{\strut smoothly.Research} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut monitor} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut applications} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut installRead} \colorbox{red!1}{\strut Play} \colorbox{red!0}{\strut Store} \colorbox{red!1}{\strut application} \colorbox{red!0}{\strut reviews} \colorbox{red!0}{\strut before} \colorbox{red!1}{\strut installing} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is agave?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!27}{\strut Agave} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!27}{\strut Agave} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut genus} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut succulent} \colorbox{red!2}{\strut plants} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 200} \colorbox{red!1}{\strut species} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut native} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut source} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut food} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fiber} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ornamentation} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut hundreds} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut spread} \colorbox{red!0}{\strut far} \colorbox{red!0}{\strut beyond} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut original} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut thanks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut migrating} \colorbox{red!0}{\strut peoples} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut brought} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut plant} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut modern} \colorbox{red!1}{\strut uses} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut plant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut widely} \colorbox{red!0}{\strut cultivated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut warm} \colorbox{red!0}{\strut regions} \colorbox{red!2}{\strut where} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut exposed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut frost} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut gardeners} \colorbox{red!0}{\strut also} \colorbox{red!2}{\strut plant} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut water} \colorbox{red!0}{\strut gardens} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut succulent} \colorbox{red!0}{\strut looks} \colorbox{red!0}{\strut attractive} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut requires} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut water.While} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut of} \colorbox{red!27}{\strut agave} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut member} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut cactus} \colorbox{red!0}{\strut family} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut actually} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut closely} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut lilies} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut other} \colorbox{red!1}{\strut succulent} \colorbox{red!2}{\strut plants} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Typically} \colorbox{red!0}{\strut ,} \colorbox{red!27}{\strut agave} \colorbox{red!2}{\strut grows} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut form} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut rosette} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut thick} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fleshy} \colorbox{red!1}{\strut leaves} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut toothed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut terminate} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut spikes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!1}{\strut species} \colorbox{red!1}{\strut flower} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut putting} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tall} \colorbox{red!0}{\strut stalk} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut aromatic} \colorbox{red!1}{\strut flowers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut dying} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Since} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut plants} \colorbox{red!0}{\strut tend} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut grow} \colorbox{red!0}{\strut runners} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut offshoots} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut smaller} \colorbox{red!2}{\strut plants} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut left} \colorbox{red!0}{\strut behind} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut parent} \colorbox{red!0}{\strut dies.AdThe} \colorbox{red!2}{\strut plant} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut extremely} \colorbox{red!0}{\strut slow} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut mature} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut demonstrated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut century} \colorbox{red!2}{\strut plant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut slow} \colorbox{red!2}{\strut growing} \colorbox{red!1}{\strut species} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut flowers} \colorbox{red!0}{\strut intermittently} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut plant} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut highly} \colorbox{red!0}{\strut useful} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut dense} \colorbox{red!1}{\strut leaves} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut often} \colorbox{red!1}{\strut edible} \colorbox{red!1}{\strut flowers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut plantations} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut specific} \colorbox{red!1}{\strut species} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut blue} \colorbox{red!27}{\strut agave} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut warm} \colorbox{red!0}{\strut regions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Mexico} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Southwest.The} \colorbox{red!1}{\strut leaves} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!27}{\strut agave} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut beaten} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut fiber} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut generate} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut foamy} \colorbox{red!0}{\strut material} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut like} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!21}{\strut agave} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut agavenoun} \colorbox{red!0}{\strut agave} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -g-v} \colorbox{red!0}{\strut Popularity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Bottom} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut words} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Updated} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 2018Trending} \colorbox{red!0}{\strut Now} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut oligarch} \colorbox{red!0}{\strut glib} \colorbox{red!0}{\strut depose} \colorbox{red!0}{\strut omnibus} \colorbox{red!0}{\strut acrimonyALLTime} \colorbox{red!0}{\strut Traveler} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Explore} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut word} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut appearedDefinition} \colorbox{red!0}{\strut of} \colorbox{red!21}{\strut agave} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut genus} \colorbox{red!0}{\strut .} \colorbox{red!21}{\strut Agave} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut family} \colorbox{red!0}{\strut Agavaceae} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!21}{\strut agave} \colorbox{red!1}{\strut family} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut plants} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut spiny-margined} \colorbox{red!0}{\strut leaves} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut tall} \colorbox{red!0}{\strut spreading} \colorbox{red!0}{\strut panicles} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut cultivated} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut fiber} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut sap} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ornamentSee} \colorbox{red!21}{\strut agave} \colorbox{red!1}{\strut defined} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut kidsRecent} \colorbox{red!0}{\strut Examples} \colorbox{red!0}{\strut of} \colorbox{red!21}{\strut agave} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut WebMezcal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut hand} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut made} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 30} \colorbox{red!2}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut agave.} \colorbox{red!0}{\strut sam} \colorbox{red!0}{\strut dangremond} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Town} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Country} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut What} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Difference} \colorbox{red!0}{\strut Between} \colorbox{red!0}{\strut Tequila} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Mezcal} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut Mar} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2018Mash} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut avocado} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lime} \colorbox{red!0}{\strut juice} \colorbox{red!0}{\strut ,} \colorbox{red!21}{\strut agave} \colorbox{red!0}{\strut nectar} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut salt.} \colorbox{red!0}{\strut San} \colorbox{red!0}{\strut Antonio} \colorbox{red!0}{\strut Express-News} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Recipe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Avocado} \colorbox{red!0}{\strut Deviled} \colorbox{red!0}{\strut Eggs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut Mar} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2018Or} \colorbox{red!0}{\strut try} \colorbox{red!0}{\strut succulents} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut jade} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut hens} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut chicks} \colorbox{red!0}{\strut ,} \colorbox{red!21}{\strut agave} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut require} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut water} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fertilize} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut Fertilizer} \colorbox{red!0}{\strut encourages} \colorbox{red!0}{\strut blooms} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut prevents} \colorbox{red!0}{\strut leggy} \colorbox{red!0}{\strut shoots.} \colorbox{red!0}{\strut rose} \colorbox{red!0}{\strut shilling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Houston} \colorbox{red!0}{\strut Chronicle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut professional} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut flower} \colorbox{red!1}{\strut planters} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut Mar} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2018These} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut sentences} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut selected} \colorbox{red!0}{\strut automatically} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut online} \colorbox{red!0}{\strut news} \colorbox{red!0}{\strut sources} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut reflect} \colorbox{red!0}{\strut current} \colorbox{red!0}{\strut usage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut word} \colorbox{red!0}{\strut agave} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Views} \colorbox{red!0}{\strut expressed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut examples} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut represent} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut opinion} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Merriam-Webster} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut editors} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Send} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut feedback.Illustration} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut agaveOrigin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Etymology} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut agaveborrowed} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Latin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut borrowed} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Greek} \colorbox{red!0}{\strut agau} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut feminine} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut agaus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut admirable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut illustrious} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut brilliant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut uncertain} \colorbox{red!2}{\strut origin} \colorbox{red!0}{\strut Note} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut distinguished} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut genus} \colorbox{red!0}{\strut separate} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut aloe} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Linnaeus} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Hortus} \colorbox{red!0}{\strut Upsaliensis} \colorbox{red!0}{\strut v.} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Stockholm} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1748} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut p.} \colorbox{red!0}{\strut 87-88} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: determining marginal cost from total cost equation

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Marginal} \colorbox{red!9}{\strut Cost} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Definition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Equation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Formula} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut error} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut iframe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut lesson} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut play} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut secondsAdd} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Timeline} \colorbox{red!0}{\strut Autoplay} \colorbox{red!0}{\strut 529K} \colorbox{red!0}{\strut viewsCreate} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut todayTry} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Create} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut AccountRecommended} \colorbox{red!0}{\strut Lessons} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Courses} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut YouRelated} \colorbox{red!0}{\strut Lessons} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut CoursesMarginal} \colorbox{red!0}{\strut Revenue} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Definition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Equation} \colorbox{red!0}{\strut Average} \colorbox{red!0}{\strut Total} \colorbox{red!9}{\strut Cost} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Definition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Formula} \colorbox{red!0}{\strut Average} \colorbox{red!0}{\strut Variable} \colorbox{red!9}{\strut Cost} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut AVC} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Definition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Function} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Equation} \colorbox{red!0}{\strut Total} \colorbox{red!9}{\strut Cost} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Economics} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Definition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut FormulaLesson} \colorbox{red!0}{\strut TranscriptInstructor} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Shawn} \colorbox{red!0}{\strut GrimsleyMarginal} \colorbox{red!9}{\strut cost} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut concept} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut lesson} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut learn} \colorbox{red!3}{\strut what} \colorbox{red!9}{\strut marginal} \colorbox{red!9}{\strut costs} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut standard} \colorbox{red!0}{\strut formula} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut illustrative} \colorbox{red!0}{\strut examples} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut short} \colorbox{red!0}{\strut quiz} \colorbox{red!0}{\strut follows} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lesson.Key} \colorbox{red!0}{\strut Concepts} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut Marginal} \colorbox{red!0}{\strut CostsMarginal} \colorbox{red!9}{\strut cost} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut increase} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut decrease} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!9}{\strut cost} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut incur} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut producing} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut unit} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut serving} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut customer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut plot} \colorbox{red!9}{\strut marginal} \colorbox{red!9}{\strut costs} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut graph} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut U-shaped} \colorbox{red!0}{\strut curve} \colorbox{red!0}{\strut where} \colorbox{red!9}{\strut costs} \colorbox{red!0}{\strut start} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut increases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut rise} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut manufacturing} \colorbox{red!0}{\strut endeavors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut marginal} \colorbox{red!9}{\strut costs} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut decreases} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut volume} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut increases} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut economies} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut scale} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Costs} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut lower} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut advantage} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut discounts} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut bulk} \colorbox{red!0}{\strut purchases} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut raw} \colorbox{red!0}{\strut materials} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut machinery} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut engage} \colorbox{red!0}{\strut specialized} \colorbox{red!0}{\strut labor.However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut reach} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut diseconomies} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut scale} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut picture} \colorbox{red!0}{\strut and} \colorbox{red!9}{\strut marginal} \colorbox{red!9}{\strut costs} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut begin} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut rise} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Costs} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut rise} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut hire} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut management} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut buy} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut equipment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut tapped} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut source} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Relationship} \colorbox{red!0}{\strut Between} \colorbox{red!4}{\strut Marginal} \colorbox{red!4}{\strut Cost} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Total} \colorbox{red!4}{\strut Cost} \colorbox{red!0}{\strut ?} \colorbox{red!4}{\strut Marginal} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut terms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut manufacturing} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut providers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fixed} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut marginal} \colorbox{red!0}{\strut variation} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut considered} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut determining} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut encompass} \colorbox{red!4}{\strut marginal} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut average} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut generally} \colorbox{red!0}{\strut decrease} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut minimum} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut increasing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut forming} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut U-shape} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Marginal} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut intersect} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut graph} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut although} \colorbox{red!4}{\strut marginal} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut curves} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut shapes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut process.When} \colorbox{red!0}{\strut determining} \colorbox{red!4}{\strut marginal} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut companies} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut calculate} \colorbox{red!0}{\strut upfront} \colorbox{red!0}{\strut fees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fixed} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut varied} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut necessary} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut occur} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Examples} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut rent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut manufacturing} \colorbox{red!0}{\strut equipment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut minimum} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut employees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut other} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut change} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut output} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut ultimately} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut marginal} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut factor} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut average} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut unit} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut with} \colorbox{red!4}{\strut marginal} \colorbox{red!0}{\strut cost.AdAn} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut marginal} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut drug} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fixed} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut upfront} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut incredibly} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut everything} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut hiring} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut specialists} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut conducting} \colorbox{red!0}{\strut experiments} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut purchasing} \colorbox{red!0}{\strut manufacturing} \colorbox{red!0}{\strut equipment} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut medications} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Additional} \colorbox{red!0}{\strut fixed} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut contribute} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut total} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut clinical} \colorbox{red!0}{\strut trials} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut marketing} \colorbox{red!0}{\strut campaigns} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut costs} \colorbox{red!0}{\strut involved} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut regulation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut certification} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut necessary} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut generate} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut income} \colorbox{red!0}{\strut stream} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut units} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut drug} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut produced.Marginal} \colorbox{red!4}{\strut cost} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut low} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut producing} \colorbox{red!0}{\strut extra} \colorbox{red!0}{\strut units} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut drug} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Once} \colorbox{red!0}{\strut the} 
}}}
\end{CJK*}

query: serve define

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!25}{\strut serve} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1serveverb} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut srv} \colorbox{red!0}{\strut Popularity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut words} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Updated} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 2018Trending} \colorbox{red!0}{\strut Now} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut oligarch} \colorbox{red!1}{\strut glib} \colorbox{red!0}{\strut depose} \colorbox{red!0}{\strut omnibus} \colorbox{red!0}{\strut acrimonyALLExamples} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut serve} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut SentenceTime} \colorbox{red!0}{\strut Traveler} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Explore} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut word} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut appearedDefinition} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut serveserved} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut servingintransitive} \colorbox{red!0}{\strut verb1} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut servantb} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!1}{\strut military} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut naval} \colorbox{red!0}{\strut service2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut assist} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut celebrant} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut server} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut mass3} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut usein} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut day} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut write} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut seals} \colorbox{red!25}{\strut served} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut signaturesElizabeth} \colorbox{red!0}{\strut W.} \colorbox{red!0}{\strut Kingb} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut favorable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut opportune} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut convenientc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut worthy} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut reliance} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut trustif} \colorbox{red!0}{\strut memory} \colorbox{red!0}{\strut servesd} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut hold} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut office} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut discharge} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut duty} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut functionserve} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut jury4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut prove} \colorbox{red!0}{\strut adequate} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut satisfactory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut sufficeit} \colorbox{red!0}{\strut will} \colorbox{red!25}{\strut serve} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut task5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut persons} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut food} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut asa} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut wait} \colorbox{red!0}{\strut at} \colorbox{red!1}{\strut tableb} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut portions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut food} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut drink6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut wait} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut customers7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut put} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ball} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut shuttlecock} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut play} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut games} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut tennis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut volleyball} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut badminton} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut transitive} \colorbox{red!0}{\strut verb1} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut servant} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut attendb} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut give} \colorbox{red!0}{\strut the} \colorbox{red!21}{\strut service} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut respect} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut superior} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut c} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut comply} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut commands} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut demands} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut gratifyd} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut give} \colorbox{red!1}{\strut military} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut naval} \colorbox{red!21}{\strut service} \colorbox{red!0}{\strut toe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut perform} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut duties} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut office} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut post} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut act} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut server} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut mass} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut archaic} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut pay} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lover} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut suitor} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut court} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lady} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut gentle} \colorbox{red!0}{\strut lady} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut whom} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut love} \colorbox{red!0}{\strut and} \colorbox{red!25}{\strut serve} \colorbox{red!0}{\strut Edmund} \colorbox{red!0}{\strut Spenser4} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut term} \colorbox{red!0}{\strut of} \colorbox{red!21}{\strut service} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut b} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut put} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut term} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut imprisonment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut served} \colorbox{red!10}{\strut market} \colorbox{red!0}{\strut Full} \colorbox{red!0}{\strut TextPrevious} \colorbox{red!0}{\strut Entry} \colorbox{red!0}{\strut Next} \colorbox{red!0}{\strut Entryserved} \colorbox{red!0}{\strut marketDerek} \colorbox{red!0}{\strut F.} \colorbox{red!0}{\strut ChannonSubject} \colorbox{red!1}{\strut Business} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut International} \colorbox{red!0}{\strut Management} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Strategic} \colorbox{red!0}{\strut ManagementExtractThe} \colorbox{red!9}{\strut served} \colorbox{red!10}{\strut market} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut segment} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!10}{\strut market} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut firm} \colorbox{red!0}{\strut actively} \colorbox{red!0}{\strut attempts} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut serve} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut difficult} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut define} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut concept} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut essential} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut measurement} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut variables} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut relative} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut absolute} \colorbox{red!10}{\strut market} \colorbox{red!1}{\strut share} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut growth} \colorbox{red!0}{\strut rate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut therefore} \colorbox{red!0}{\strut imperative} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut task} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut undertaken} \colorbox{red!0}{\strut creatively} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut embarking} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut precise} \colorbox{red!0}{\strut strategy} \colorbox{red!0}{\strut formulation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut observers} \colorbox{red!0}{\strut cite} \colorbox{red!10}{\strut market} \colorbox{red!1}{\strut share} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut relative} \colorbox{red!10}{\strut market} \colorbox{red!1}{\strut share} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut key} \colorbox{red!0}{\strut determinants} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut business} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut profitability} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut fail} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut define} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut market} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut illustrated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut figure} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut served} \colorbox{red!10}{\strut market} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut defined} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut intersection} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut class} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut customers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut firm} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut service} \colorbox{red!0}{\strut offering} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut desired} \colorbox{red!0}{\strut geographic} \colorbox{red!0}{\strut coverage} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Figure} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut served} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut market} \colorbox{red!1}{\strut concept} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Channon} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1986} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut each} \colorbox{red!10}{\strut market} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut firm} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut engaged} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut sufficiently} \colorbox{red!2}{\strut defined} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut answered} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Who} \colorbox{red!0}{\strut precisely} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut customers} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut needs} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut What} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut services} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut firm} \colorbox{red!0}{\strut offer} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut meet} \colorbox{red!0}{\strut these} \colorbox{red!1}{\strut needs} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Can} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut efficiently} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut profitably} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut acceptable} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut risk} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut What} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut firm} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut deliver} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut products} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut services} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut How} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut resources} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut managed} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut evaluate} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut potential} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut served} \colorbox{red!10}{\strut market} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut desirable} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut complete} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut customerproduct} \colorbox{red!1}{\strut needs} \colorbox{red!0}{\strut grid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut segments} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut subdivided} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut needs} \colorbox{red!0}{\strut established} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut key} \colorbox{red!0}{\strut customer} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut log} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut subscribe} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut read} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut textLog} \colorbox{red!0}{\strut InYou} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut logged-in} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Blackwell} \colorbox{red!0}{\strut Reference} \colorbox{red!0}{\strut OnlineIf} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut institution} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut subscription} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} 
}}}
\end{CJK*}

query: what grade on final do i need

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut What} \colorbox{red!7}{\strut Grade} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut Need} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Final} \colorbox{red!2}{\strut Exam} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut What} \colorbox{red!7}{\strut Grade} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut Need} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Final} \colorbox{red!2}{\strut Exam} \colorbox{red!0}{\strut ?} \colorbox{red!9}{\strut What} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut final} \colorbox{red!2}{\strut exam} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut frequent} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut asked} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut What} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut final} \colorbox{red!2}{\strut exam} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut B} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut C} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut other} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut desired} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut involves} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut math} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut student} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut apply} \colorbox{red!0}{\strut successfully} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Determine} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut Grading} \colorbox{red!1}{\strut Scale} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut determine} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut grading} \colorbox{red!1}{\strut scale} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut class} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut typically} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut syllabus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut scores} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut earning} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut B} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!1}{\strut classes} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut successfully} \colorbox{red!0}{\strut complete} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut class} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut minimum} \colorbox{red!2}{\strut score} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut successful} \colorbox{red!0}{\strut completion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Once} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut write} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lowest} \colorbox{red!1}{\strut number} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut range} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut unsure} \colorbox{red!9}{\strut what} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut grading} \colorbox{red!1}{\strut scale} \colorbox{red!0}{\strut looks} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 7-point} \colorbox{red!5}{\strut grading} \colorbox{red!1}{\strut scale} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Letter} \colorbox{red!7}{\strut Grade} \colorbox{red!1}{\strut Range} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut ScoresA} \colorbox{red!0}{\strut 93-100B} \colorbox{red!0}{\strut 86-92C} \colorbox{red!0}{\strut 79-85D} \colorbox{red!0}{\strut 72-78F} \colorbox{red!0}{\strut 0-71In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut minimum} \colorbox{red!2}{\strut scores} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut desired} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut achieve} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut C} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut final} \colorbox{red!1}{\strut average} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 79.If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut achieve} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut B} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut final} \colorbox{red!1}{\strut average} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 86.If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut achieve} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut grade} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut final} \colorbox{red!1}{\strut average} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 93.Determine} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Weighting} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut Grades} \colorbox{red!0}{\strut Next} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut determine} \colorbox{red!0}{\strut whether} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut not} \colorbox{red!2}{\strut scores} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut weighted} \colorbox{red!0}{\strut differently} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut sections} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut class} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Final} \colorbox{red!4}{\strut grade} \colorbox{red!4}{\strut calculator} \colorbox{red!4}{\strut Final} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut calculatorFind} \colorbox{red!2}{\strut what} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut final} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Grade} \colorbox{red!4}{\strut calculator} \colorbox{red!4}{\strut Final} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut calculatorSelect} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Current} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Required} \colorbox{red!0}{\strut class} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Final} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CalculateResetFinal} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut needed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Grade} \colorbox{red!4}{\strut calculator} \colorbox{red!0}{\strut Final} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut calculationExample} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1Current} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 70} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut C-} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Final} \colorbox{red!1}{\strut exam} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Required} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut B-} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Calculation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut final} \colorbox{red!1}{\strut exam} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut equal} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut required} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut minus} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut minus} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut final} \colorbox{red!1}{\strut exam} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut w} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut times} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut current} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut g} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut divided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut final} \colorbox{red!1}{\strut exam} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut w} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Final} \colorbox{red!1}{\strut exam} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut required} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut w} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut current} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut w} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 70} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut So} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut final} \colorbox{red!1}{\strut exam} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut A-} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Example} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2Assigment} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut weight150} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut grade116} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 20.Assigment} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut weight230} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut max} \colorbox{red!0}{\strut grade30.Assigment} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut weight320} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut max} \colorbox{red!0}{\strut grade40.Find} \colorbox{red!1}{\strut average} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut assignments} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut needed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut class} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 85} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Calculation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Current} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Assignment} \colorbox{red!0}{\strut 1} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut grade1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut max} \colorbox{red!0}{\strut grade1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1620} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0.8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Required} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 85} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Final} \colorbox{red!1}{\strut exam} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut w} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut weight2weight3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Final} \colorbox{red!1}{\strut exam} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut required} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut w} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut current} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut w} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 85} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut mean} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut average} \colorbox{red!4}{\strut grade} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut assignments} \colorbox{red!0}{\strut 2} 
}}}
\end{CJK*}

query: most secluded beach north carolina

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Secluded} \colorbox{red!1}{\strut North} \colorbox{red!2}{\strut Carolina} \colorbox{red!0}{\strut Beaches} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Secluded} \colorbox{red!0}{\strut spots} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut North} \colorbox{red!2}{\strut Carolina} \colorbox{red!1}{\strut coast} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut scenic} \colorbox{red!0}{\strut beauty} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut moments} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut solitude.Home} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Cape} \colorbox{red!2}{\strut Hatteras} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Cape} \colorbox{red!0}{\strut Lookout} \colorbox{red!1}{\strut national} \colorbox{red!1}{\strut seashores} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rugged} \colorbox{red!1}{\strut Outer} \colorbox{red!0}{\strut Banks} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut North} \colorbox{red!2}{\strut Carolina} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut share} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut secluded} \colorbox{red!0}{\strut shorelines} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut 300} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut beach} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut its} \colorbox{red!2}{\strut barrier} \colorbox{red!16}{\strut islands} \colorbox{red!0}{\strut alone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut special} \colorbox{red!1}{\strut sandy} \colorbox{red!0}{\strut spots} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Tar} \colorbox{red!0}{\strut Heel} \colorbox{red!1}{\strut State} \colorbox{red!0}{\strut stand} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut natural} \colorbox{red!0}{\strut scenic} \colorbox{red!0}{\strut beauty} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut glimpses} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut wildlife} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut laid-back} \colorbox{red!0}{\strut atmosphere.Pea} \colorbox{red!17}{\strut Island} \colorbox{red!1}{\strut National} \colorbox{red!1}{\strut Wildlife} \colorbox{red!0}{\strut RefugePea} \colorbox{red!17}{\strut Island} \colorbox{red!1}{\strut National} \colorbox{red!1}{\strut Wildlife} \colorbox{red!1}{\strut Refuge} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pristine} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut undeveloped} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Cape} \colorbox{red!2}{\strut Hatteras} \colorbox{red!1}{\strut National} \colorbox{red!1}{\strut Seashore} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Outer} \colorbox{red!0}{\strut Banks} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lies} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut N.C.} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut Hatteras} \colorbox{red!17}{\strut Island} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut between} \colorbox{red!2}{\strut Oregon} \colorbox{red!1}{\strut Inlet} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Rodanthe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut refuge} \colorbox{red!0}{\strut boasts} \colorbox{red!0}{\strut almost} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut beach} \colorbox{red!4}{\strut where} \colorbox{red!0}{\strut vehicles} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut allowed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut popular} \colorbox{red!0}{\strut activities} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut shelling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut swimming} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut relaxing} \colorbox{red!0}{\strut walks} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut secluded} \colorbox{red!1}{\strut shore} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fishing} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Pamlico} \colorbox{red!0}{\strut Sound} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Atlantic} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut refuge} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut visitor} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut center} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut freshwater} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut brackish} \colorbox{red!0}{\strut ponds} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut wetlands} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut nature} \colorbox{red!0}{\strut trails} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Overnight} \colorbox{red!0}{\strut options} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut national} \colorbox{red!1}{\strut seashore} \colorbox{red!0}{\strut s} \colorbox{red!2}{\strut Oregon} \colorbox{red!1}{\strut Inlet} \colorbox{red!0}{\strut campground} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut miles} \colorbox{red!1}{\strut north} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut selection} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut motels} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rental} \colorbox{red!0}{\strut homes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut campgrounds} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut cabins} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Rodanthe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut away.Portsmouth} \colorbox{red!0}{\strut IslandPortsmouth} \colorbox{red!17}{\strut Island} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut lies} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut south} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Okracoke} \colorbox{red!17}{\strut Island} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Cape} \colorbox{red!0}{\strut Lookout} \colorbox{red!1}{\strut National} \colorbox{red!1}{\strut Seashore} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut home} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut thriving} \colorbox{red!0}{\strut port} \colorbox{red!0}{\strut village} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut served} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut largest} \colorbox{red!0}{\strut European} \colorbox{red!0}{\strut settlement} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Outer} \colorbox{red!0}{\strut Banks} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut uninhabited} \colorbox{red!17}{\strut island} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut accessible} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut private} \colorbox{red!0}{\strut boat} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut private} \colorbox{red!0}{\strut ferry} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Okracoke} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Atlantic} \colorbox{red!0}{\strut --} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut home} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut beach} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!17}{\strut island} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut homes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut stores} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut businesses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut although} \colorbox{red!0}{\strut self-guided} \colorbox{red!0}{\strut tours} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut allow} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut tour} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Carova} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut North} \colorbox{red!2}{\strut Carolina} \colorbox{red!1}{\strut Named} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Secluded} \colorbox{red!10}{\strut Beach} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!2}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Home} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Vacationer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Guide} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut Beach} \colorbox{red!0}{\strut Buzz} \colorbox{red!0}{\strut Carova} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut North} \colorbox{red!2}{\strut Carolina} \colorbox{red!1}{\strut Named} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut Secluded} \colorbox{red!10}{\strut Beach} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!0}{\strut StatesTags} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Best} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut OBXRoads} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Who} \colorbox{red!0}{\strut Needs} \colorbox{red!1}{\strut Roads} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Sherman} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Travel} \colorbox{red!0}{\strut recently} \colorbox{red!0}{\strut released} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut 10} \colorbox{red!7}{\strut Secluded} \colorbox{red!10}{\strut Beaches} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut United} \colorbox{red!2}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Tranquil} \colorbox{red!10}{\strut beaches} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Hawaii} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut California} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut list} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Outer} \colorbox{red!0}{\strut Banks} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut own} \colorbox{red!8}{\strut Carova} \colorbox{red!10}{\strut Beach} \colorbox{red!0}{\strut took} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!1}{\strut spot} \colorbox{red!0}{\strut !} \colorbox{red!1}{\strut Located} \colorbox{red!0}{\strut just} \colorbox{red!1}{\strut north} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Corolla} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut NC} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut south} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Virginia} \colorbox{red!0}{\strut border} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Carova} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut truly} \colorbox{red!0}{\strut unique} \colorbox{red!1}{\strut vacation} \colorbox{red!1}{\strut destination} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut warned} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut sense} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut adventure} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut necessity} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut paved} \colorbox{red!1}{\strut roads} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Carova} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut 4-wheel} \colorbox{red!1}{\strut drive} \colorbox{red!0}{\strut vehicle} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut drive} \colorbox{red!0}{\strut directly} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut sand} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut guy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut decides} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut mini} \colorbox{red!0}{\strut van} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut onto} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut beach} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ends} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut needing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tow} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Driving} \colorbox{red!0}{\strut conditions} \colorbox{red!0}{\strut fluctuate} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tides} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut weather} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut drive} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tracks} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut vehicles} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut gone} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut access} \colorbox{red!8}{\strut Carova} \colorbox{red!1}{\strut vacation} \colorbox{red!1}{\strut homes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!1}{\strut drive} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut dune} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut onto} \colorbox{red!0}{\strut back} \colorbox{red!1}{\strut roads} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut sand} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dirt.If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut nightlife} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut shopping} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut best} \colorbox{red!0}{\strut steer} \colorbox{red!0}{\strut clear} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut Carova} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut NC} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut What} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut pristine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut undeveloped} \colorbox{red!0}{\strut coastline} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut lush} \colorbox{red!0}{\strut maritime} \colorbox{red!0}{\strut forest} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Mother} \colorbox{red!0}{\strut Nature} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut main} \colorbox{red!0}{\strut attraction} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut Carova} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rolling} \colorbox{red!0}{\strut waves} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Atlantic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut peaceful} \colorbox{red!0}{\strut waters} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Currituck} \colorbox{red!0}{\strut Sound} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut natural} \colorbox{red!0}{\strut landscape} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut breathtaking} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut wild} \colorbox{red!0}{\strut horses} \colorbox{red!0}{\strut roaming} 
}}}
\end{CJK*}

query: which event nearly caused nuclear war?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut New} \colorbox{red!0}{\strut Study} \colorbox{red!0}{\strut Suggests} \colorbox{red!13}{\strut Solar} \colorbox{red!7}{\strut Storm} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut 1967} \colorbox{red!0}{\strut Nearly} \colorbox{red!11}{\strut Caused} \colorbox{red!2}{\strut Nuclear} \colorbox{red!1}{\strut War} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut StoriesNew} \colorbox{red!0}{\strut Study} \colorbox{red!0}{\strut Suggests} \colorbox{red!13}{\strut Solar} \colorbox{red!7}{\strut Storm} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut 1967} \colorbox{red!0}{\strut Nearly} \colorbox{red!11}{\strut Caused} \colorbox{red!2}{\strut Nuclear} \colorbox{red!0}{\strut WarHistory} \colorbox{red!0}{\strut StoriesNew} \colorbox{red!0}{\strut Study} \colorbox{red!0}{\strut Suggests} \colorbox{red!13}{\strut Solar} \colorbox{red!7}{\strut Storm} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut 1967} \colorbox{red!0}{\strut Nearly} \colorbox{red!11}{\strut Caused} \colorbox{red!2}{\strut Nuclear} \colorbox{red!0}{\strut WarBy} \colorbox{red!0}{\strut Sarah} \colorbox{red!0}{\strut Pruitt} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2016The} \colorbox{red!0}{\strut sun} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 23} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut 1967} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut powerful} \colorbox{red!0}{\strut flare} \colorbox{red!0}{\strut erupted} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut bright} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut top-center} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!13}{\strut solar} \colorbox{red!0}{\strut disk} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Credit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut National} \colorbox{red!13}{\strut Solar} \colorbox{red!0}{\strut Observatory} \colorbox{red!0}{\strut historical} \colorbox{red!0}{\strut archive} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut CiteOn} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 23} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut 1967} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut midst} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Cold} \colorbox{red!1}{\strut War} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut Air} \colorbox{red!0}{\strut Force} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut preparing} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut nuclear-armed} \colorbox{red!0}{\strut aircraft} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut takeoff} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut believing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Soviet} \colorbox{red!0}{\strut Union} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut committed} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut act} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut war} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut jamming} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut surveillance} \colorbox{red!0}{\strut radar} \colorbox{red!0}{\strut systems} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut planes} \colorbox{red!0}{\strut never} \colorbox{red!0}{\strut took} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut averting} \colorbox{red!9}{\strut what} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut catastrophic} \colorbox{red!0}{\strut military} \colorbox{red!0}{\strut conflict} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut What} \colorbox{red!1}{\strut happened} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut reveals} \colorbox{red!0}{\strut military} \colorbox{red!0}{\strut space-weather} \colorbox{red!0}{\strut forecasters} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut intervened} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut informing} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Air} \colorbox{red!0}{\strut Force} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut disturbance} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut radar} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut radio} \colorbox{red!0}{\strut communications} \colorbox{red!0}{\strut was} \colorbox{red!11}{\strut caused} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Soviets} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut powerful} \colorbox{red!0}{\strut eruption} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut radiation} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sun.In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut late} \colorbox{red!0}{\strut 1950s} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut branches} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut military} \colorbox{red!0}{\strut began} \colorbox{red!0}{\strut monitoring} \colorbox{red!13}{\strut solar} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut space} \colorbox{red!1}{\strut weather} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut disturbances} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Earth} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut magnetic} \colorbox{red!0}{\strut field} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut upper} \colorbox{red!0}{\strut atmosphere} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut interfere} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut radio} \colorbox{red!0}{\strut transmissions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut power} \colorbox{red!0}{\strut lines} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut technologies} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 60s} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut branch} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut Air} \colorbox{red!0}{\strut Force} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Air} \colorbox{red!1}{\strut Weather} \colorbox{red!0}{\strut Service} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut AWS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut dedicated} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut monitoring} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sun} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut watching} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut brief} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut powerful} \colorbox{red!0}{\strut eruptions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut radiation} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut surface} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!13}{\strut solar} \colorbox{red!2}{\strut flares} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut network} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut observers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut abroad} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Aerospace} \colorbox{red!0}{\strut Defense} \colorbox{red!0}{\strut Command} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NORAD} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut joint} \colorbox{red!0}{\strut U.S.-Canadian} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Which} \colorbox{red!10}{\strut event} \colorbox{red!10}{\strut resulted} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut greatest} \colorbox{red!10}{\strut threat} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut nuclear} \colorbox{red!10}{\strut war} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A.} \colorbox{red!0}{\strut U.S} \colorbox{red!0}{\strut military} \colorbox{red!0}{\strut aid} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Vietnam} \colorbox{red!0}{\strut B.} \colorbox{red!0}{\strut outbreak} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut war} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Middle} \colorbox{red!0}{\strut East} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut Soviet} \colorbox{red!0}{\strut Union} \colorbox{red!0}{\strut launched} \colorbox{red!0}{\strut Sputnik} \colorbox{red!0}{\strut D.} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut naval} \colorbox{red!1}{\strut blockade} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Cuba} \colorbox{red!0}{\strut High} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut pointsWhich} \colorbox{red!10}{\strut event} \colorbox{red!10}{\strut resulted} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut greatest} \colorbox{red!10}{\strut threat} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut nuclear} \colorbox{red!10}{\strut war} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A.} \colorbox{red!0}{\strut U.S} \colorbox{red!0}{\strut military} \colorbox{red!0}{\strut aid} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Vietnam} \colorbox{red!0}{\strut B.} \colorbox{red!0}{\strut outbreak} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut war} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Middle} \colorbox{red!0}{\strut East} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut Soviet} \colorbox{red!0}{\strut Union} \colorbox{red!0}{\strut launched} \colorbox{red!0}{\strut Sputnik} \colorbox{red!0}{\strut D.} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut naval} \colorbox{red!1}{\strut blockade} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut CubaAsk} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut details} \colorbox{red!0}{\strut Follow} \colorbox{red!0}{\strut Reportby} \colorbox{red!0}{\strut LeannLoriammabbyS} \colorbox{red!0}{\strut 09272016Only} \colorbox{red!0}{\strut registered} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut access} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut verified} \colorbox{red!0}{\strut answersJoin} \colorbox{red!0}{\strut nowAnswersmeerkat18} \colorbox{red!0}{\strut AmbitiousThe} \colorbox{red!0}{\strut correct} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut among} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut choice} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut D.} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut naval} \colorbox{red!1}{\strut blockade} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Cuba} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!10}{\strut event} \colorbox{red!10}{\strut resulted} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut greatest} \colorbox{red!10}{\strut threat} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut nuclear} \colorbox{red!10}{\strut war} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Thank} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut posting} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut hope} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut helped} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Let} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut help.Comments} \colorbox{red!0}{\strut Report4.9} \colorbox{red!0}{\strut 19} \colorbox{red!0}{\strut votesThanks} \colorbox{red!0}{\strut 43The} \colorbox{red!0}{\strut Brain} \colorbox{red!0}{\strut HelperNot} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut answersLearn} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Brainly} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Having} \colorbox{red!0}{\strut trouble} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut homework} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut 80} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut answered} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut minutesAnswers} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut explanations} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut learnAnswer} \colorbox{red!0}{\strut quality} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ensured} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut expertsI} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut !} 
}}}
\end{CJK*}

query: who created the song danny boy

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!15}{\strut Danny} \colorbox{red!15}{\strut Boy} \colorbox{red!0}{\strut Lyrics} \colorbox{red!0}{\strut And} \colorbox{red!1}{\strut Chords} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Song} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Danny} \colorbox{red!15}{\strut Boy} \colorbox{red!0}{\strut Lyrics} \colorbox{red!0}{\strut And} \colorbox{red!1}{\strut Chords} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut SongWritten} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Frederic} \colorbox{red!0}{\strut Weatherly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Set} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut tune} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Derry} \colorbox{red!0}{\strut Air} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut published} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1913} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Alternative} \colorbox{red!1}{\strut chords} \colorbox{red!0}{\strut for} \colorbox{red!15}{\strut Danny} \colorbox{red!15}{\strut Boy} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut key} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut CG} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut FC} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut C7G7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut key} \colorbox{red!0}{\strut changer} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut key} \colorbox{red!0}{\strut changes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut suit} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut voice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Celtic} \colorbox{red!0}{\strut Fusion} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Stephen} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut guitar} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Tony} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut vocals.Sheet} \colorbox{red!0}{\strut Music} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut Tin} \colorbox{red!0}{\strut Whistle} \colorbox{red!0}{\strut NotesOh} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Danny} \colorbox{red!15}{\strut boy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut pipes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut pipes} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut calling} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut glen} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut glen} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut mountain} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut side} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut gone} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dying} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut bide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut back} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut meadow} \colorbox{red!0}{\strut Or} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C7} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut valley} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hushed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut white} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut snow} \colorbox{red!0}{\strut t} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut sunshine} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut sha} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Am} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dow} \colorbox{red!0}{\strut Oh} \colorbox{red!15}{\strut Danny} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut boy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut oh} \colorbox{red!15}{\strut Danny} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut boy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut love} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut dying} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut dead} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut dead} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut lying} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut kneel} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut say} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ave} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!12}{\strut Danny} \colorbox{red!11}{\strut Boy} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Danny} \colorbox{red!0}{\strut Boynavigation} \colorbox{red!0}{\strut searchDanny} \colorbox{red!11}{\strut Boy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1913} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Frederick} \colorbox{red!0}{\strut Weatherlyinformation} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut edition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Danny} \colorbox{red!11}{\strut Boy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut song} \colorbox{red!0}{\strut whose} \colorbox{red!1}{\strut lyrics} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Irish} \colorbox{red!1}{\strut tune} \colorbox{red!0}{\strut Londonderry} \colorbox{red!1}{\strut Air} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut lyrics} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut originally} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut different} \colorbox{red!1}{\strut tune} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1910} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Frederick} \colorbox{red!1}{\strut Weatherly} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut lawyer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut modified} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut fit} \colorbox{red!0}{\strut Londonderry} \colorbox{red!1}{\strut Air} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1913} \colorbox{red!2}{\strut when} \colorbox{red!1}{\strut Weatherly} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut sent} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut copy} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut tune} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut sister.The} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut recording} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Ernestine} \colorbox{red!0}{\strut Schumann-Heink} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1915} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Weatherly} \colorbox{red!0}{\strut gave} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut song} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Elsie} \colorbox{red!0}{\strut Griffin} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut who} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut popular} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut century} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Weatherly} \colorbox{red!0}{\strut later} \colorbox{red!0}{\strut suggested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1928} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut verse} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fitting} \colorbox{red!0}{\strut requiem} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut actress} \colorbox{red!0}{\strut Ellen} \colorbox{red!0}{\strut Terry.} \colorbox{red!0}{\strut Excerpted} \colorbox{red!0}{\strut from} \colorbox{red!12}{\strut Danny} \colorbox{red!11}{\strut Boy} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia.Oh} \colorbox{red!0}{\strut ,} \colorbox{red!12}{\strut Danny} \colorbox{red!11}{\strut Boy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut pipes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut pipes} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut calling} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut glen} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut glen} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut mountain} \colorbox{red!0}{\strut side} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut gone} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut roses} \colorbox{red!0}{\strut falling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut bide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut ye} \colorbox{red!0}{\strut back} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut summer} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut meadow} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Or} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut valley} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut hushed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut white} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut snow} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut sunshine} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut shadow} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Oh} \colorbox{red!0}{\strut ,} \colorbox{red!12}{\strut Danny} \colorbox{red!11}{\strut Boy} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut oh} \colorbox{red!12}{\strut Danny} \colorbox{red!11}{\strut Boy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut love} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut But} \colorbox{red!2}{\strut when} \colorbox{red!0}{\strut ye} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut flowers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut dying} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut dead} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut dead} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Ye} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut place} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut lying} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut kneel} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut say} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Ave} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut shall} \colorbox{red!0}{\strut hear} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut though} \colorbox{red!0}{\strut soft} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut tread} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut grave} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut warmer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sweeter} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

query: does adult acne rosacea give you blepharitis

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut About} \colorbox{red!2}{\strut Dry} \colorbox{red!6}{\strut Eyes} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Blepharitis} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Ocular} \colorbox{red!1}{\strut Rosacea} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut About} \colorbox{red!2}{\strut Dry} \colorbox{red!6}{\strut Eyes} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Blepharitis} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut Ocular} \colorbox{red!0}{\strut RosaceaWhat} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut Blepharitis} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut Blepharitis} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut common} \colorbox{red!0}{\strut disorder} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut eyelids} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut tiny} \colorbox{red!2}{\strut oil} \colorbox{red!3}{\strut glands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut eyelids} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut openings} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut behind} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut eyelashes} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut edge} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut our} \colorbox{red!8}{\strut eyelids} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!3}{\strut glands} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut produce} \colorbox{red!2}{\strut oil} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut moisturizes} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut eyes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut prevents} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut tears} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut evaporating} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut quickly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sometimes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut oil} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut thick} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut plug} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut openings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut trapping} \colorbox{red!0}{\strut bacteria} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut naturally} \colorbox{red!0}{\strut live} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut skin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut glands} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut leads} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut chronic} \colorbox{red!0}{\strut infection} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut eyelids} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut redness} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut crusty} \colorbox{red!1}{\strut discharge} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut morning} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut gland} \colorbox{red!0}{\strut becomes} \colorbox{red!0}{\strut completely} \colorbox{red!1}{\strut plugged} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut pustule} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut stye} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut it.What} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut Ocular} \colorbox{red!1}{\strut Rosacea} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Rosacea} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut facial} \colorbox{red!1}{\strut skin} \colorbox{red!0}{\strut condition} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!4}{\strut cause} \colorbox{red!0}{\strut adult} \colorbox{red!1}{\strut acne} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut blepharitis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut blocked} \colorbox{red!2}{\strut oil} \colorbox{red!3}{\strut glands} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lids} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut affect} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut skin} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut entire} \colorbox{red!1}{\strut face} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut leading} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut redness} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut pustule} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut pimple} \colorbox{red!0}{\strut formation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Exposure} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut sunlight} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut drinking} \colorbox{red!0}{\strut excess} \colorbox{red!0}{\strut alcohol} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut caffeinated} \colorbox{red!0}{\strut beverages} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eating} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lot} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut greasy} \colorbox{red!0}{\strut foods} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut factors} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut making} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut condition} \colorbox{red!0}{\strut worse} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut These} \colorbox{red!0}{\strut factors} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut completely} \colorbox{red!0}{\strut avoided} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut When} \colorbox{red!1}{\strut rosacea} \colorbox{red!1}{\strut affects} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut eyes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut called} \colorbox{red!1}{\strut ocular} \colorbox{red!1}{\strut rosacea} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Blepharitis} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut dryness} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut eyes} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut severe} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut condition.What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut symptoms} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut blepharitis} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Common} \colorbox{red!2}{\strut symptoms} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut blepharitis} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut redness} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut eyelids} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut eyes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut crusty} \colorbox{red!1}{\strut discharge} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut eyelids} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dandruff} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut eyelids} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut burning} \colorbox{red!0}{\strut tears} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut dry} \colorbox{red!6}{\strut eyes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sometimes} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut blepharitis} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut styes} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut eyelids} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Blepharitis} \colorbox{red!0}{\strut and} \colorbox{red!8}{\strut Rosacea} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut Blepharitis} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut RosaceaTreato} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut 494} \colorbox{red!0}{\strut discussions} \colorbox{red!0}{\strut about} \colorbox{red!8}{\strut Rosacea} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Blepharitis} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut web.Symptoms} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut mentioned} \colorbox{red!0}{\strut with} \colorbox{red!6}{\strut Blepharitis} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut patients} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut discussionsDry} \colorbox{red!7}{\strut Eyes} \colorbox{red!2}{\strut Pain} \colorbox{red!1}{\strut Allergy} \colorbox{red!3}{\strut Inflammation} \colorbox{red!2}{\strut Itching} \colorbox{red!8}{\strut Rosacea} \colorbox{red!1}{\strut Infection} \colorbox{red!0}{\strut SwellingRedness} \colorbox{red!2}{\strut Ocular} \colorbox{red!0}{\strut RosaceaAbout} \colorbox{red!0}{\strut Blepharitis13,520} \colorbox{red!0}{\strut discussionsBlepharitis} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut ocular} \colorbox{red!1}{\strut condition} \colorbox{red!1}{\strut characterized} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut chronic} \colorbox{red!3}{\strut inflammation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut eyelid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut severity} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut var} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut WikipediaAbout} \colorbox{red!0}{\strut Rosacea144,278} \colorbox{red!0}{\strut discussionsRosacea} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut long-term} \colorbox{red!1}{\strut disease} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut affects} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut skin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut your} \colorbox{red!7}{\strut eyes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!6}{\strut causes} \colorbox{red!1}{\strut redness} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut pimples} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Rosacea} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut common} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut women} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut fair} \colorbox{red!2}{\strut skin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut often} \colorbox{red!1}{\strut affects} \colorbox{red!0}{\strut middle-aged} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut older} \colorbox{red!0}{\strut adults} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Read} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut MedlinePlus.gov.See} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut aboutBlepharitis} \colorbox{red!0}{\strut RosaceaDiscussions} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut webFilter} \colorbox{red!0}{\strut byGenderM} \colorbox{red!0}{\strut FRolePatient} \colorbox{red!0}{\strut CaregiverAgeAllAdd} \colorbox{red!0}{\strut topicWe} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut 494} \colorbox{red!0}{\strut discussionsShare} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut experienceMark} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut questionHopefully} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut wo} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut family} \colorbox{red!0}{\strut physician} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut February} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2018} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut englishforum.ch} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut quite} \colorbox{red!0}{\strut surprised} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut She} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut insisting} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut treating} \colorbox{red!0}{\strut my} \colorbox{red!8}{\strut rosacea} \colorbox{red!0}{\strut herself} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut that} \colorbox{red!8}{\strut rosacea} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut normally} \colorbox{red!1}{\strut treated} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut dermatologist} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Switzerland} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut looking} \colorbox{red!8}{\strut rosacea} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut talking} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut good} \colorbox{red!0}{\strut friend} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Canada} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!1}{\strut conditions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut indicates} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut treatment} \colorbox{red!0}{\strut options} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!7}{\strut what} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut root} \colorbox{red!6}{\strut cause} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut seems} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut important} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Comment} \colorbox{red!0}{\strut Helpful} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut SaveI} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut inner} \colorbox{red!6}{\strut eyelid} \colorbox{red!3}{\strut inflammation} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut August} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut healthboards.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut did} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut know} \colorbox{red!2}{\strut Dry} \colorbox{red!7}{\strut Eyes} \colorbox{red!0}{\strut can} \colorbox{red!6}{\strut cause} \colorbox{red!1}{\strut inner} \colorbox{red!6}{\strut eyelid} \colorbox{red!3}{\strut inflammation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut inner} \colorbox{red!6}{\strut eyelid} \colorbox{red!3}{\strut inflammation} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut burning} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut lessen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut bottom} \colorbox{red!1}{\strut eyelids} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut thick} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut maybe} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut How} \colorbox{red!1}{\strut long} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut gotten} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut ?} 
}}}
\end{CJK*}

query: what do you do in a film production club

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Does} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut Have} \colorbox{red!0}{\strut a} \colorbox{red!13}{\strut Film} \colorbox{red!4}{\strut Production} \colorbox{red!1}{\strut Club} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Does} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut School} \colorbox{red!0}{\strut Have} \colorbox{red!0}{\strut a} \colorbox{red!13}{\strut Film} \colorbox{red!4}{\strut Production} \colorbox{red!1}{\strut Club} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut Our} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Central} \colorbox{red!0}{\strut Educational} \colorbox{red!1}{\strut Center} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut located} \colorbox{red!0}{\strut 35} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut south} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Atlanta} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut rapidly} \colorbox{red!0}{\strut becoming} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Hollywood} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut south.The} \colorbox{red!14}{\strut Walking} \colorbox{red!13}{\strut Dead} \colorbox{red!0}{\strut is} \colorbox{red!11}{\strut filmed} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut away} \colorbox{red!0}{\strut Pinewood} \colorbox{red!1}{\strut Studios} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut located} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut away} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Raleigh} \colorbox{red!0}{\strut Studios} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 6} \colorbox{red!11}{\strut films} \colorbox{red!0}{\strut were} \colorbox{red!1}{\strut shot} \colorbox{red!0}{\strut nearby} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut past} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Hunger} \colorbox{red!0}{\strut Games} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Atlanta} \colorbox{red!0}{\strut metro} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut major} \colorbox{red!10}{\strut movie} \colorbox{red!4}{\strut production} \colorbox{red!0}{\strut complexes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut coming} \colorbox{red!0}{\strut year.We} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut input} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut setting} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut a} \colorbox{red!13}{\strut film} \colorbox{red!4}{\strut production} \colorbox{red!1}{\strut club} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut open} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut high} \colorbox{red!1}{\strut schools} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut county} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut college} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut academy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut charter} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut county} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut gets} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut student} \colorbox{red!0}{\strut body} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut high} \colorbox{red!1}{\strut schools} \colorbox{red!0}{\strut throughout} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut vocational} \colorbox{red!0}{\strut high} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut county} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut trying} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut attract} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut kids} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut career} \colorbox{red!0}{\strut choices} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Students} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut choice} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut classes} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut base} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut vocational} \colorbox{red!0}{\strut classes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!13}{\strut film} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut television} \colorbox{red!4}{\strut production} \colorbox{red!0}{\strut pathway} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut courses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut looking} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut grow} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut hoping} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut additional} \colorbox{red!13}{\strut Film} \colorbox{red!4}{\strut Production} \colorbox{red!1}{\strut Club} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut attract} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut opportunities.The} \colorbox{red!0}{\strut idea} \colorbox{red!0}{\strut behind} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut club} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut opportunity} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut train} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut students} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut the} \colorbox{red!13}{\strut film} \colorbox{red!4}{\strut production} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut talking} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut producers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut directors} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut 7} \colorbox{red!16}{\strut Things} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut Need} \colorbox{red!0}{\strut to} \colorbox{red!15}{\strut Stop} \colorbox{red!10}{\strut Doing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Be} \colorbox{red!0}{\strut More} \colorbox{red!16}{\strut Productive} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Backed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Science} \colorbox{red!1}{\strut 7} \colorbox{red!16}{\strut Things} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut Need} \colorbox{red!0}{\strut to} \colorbox{red!15}{\strut Stop} \colorbox{red!10}{\strut Doing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Be} \colorbox{red!0}{\strut More} \colorbox{red!16}{\strut Productive} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Backed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut ScienceBY} \colorbox{red!0}{\strut CAMMI} \colorbox{red!1}{\strut PHAM} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut appeared} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut personal} \colorbox{red!0}{\strut blogWhen} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut 17} \colorbox{red!0}{\strut years} \colorbox{red!2}{\strut old} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut work} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut study} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 20} \colorbox{red!1}{\strut hours} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut went} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut did} \colorbox{red!0}{\strut my} \colorbox{red!1}{\strut homework} \colorbox{red!0}{\strut during} \colorbox{red!1}{\strut breaks} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut managed} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut not-for-profit} \colorbox{red!0}{\strut organization} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut night} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut working} \colorbox{red!1}{\strut hard} \colorbox{red!1}{\strut landed} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut countless} \colorbox{red!0}{\strut national} \colorbox{red!0}{\strut campaigns} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut opportunities} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut work} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut A-list} \colorbox{red!1}{\strut organizations} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut successful} \colorbox{red!1}{\strut career} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut older} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!2}{\strut started} \colorbox{red!1}{\strut thinking} \colorbox{red!0}{\strut differently} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut realized} \colorbox{red!0}{\strut that} \colorbox{red!10}{\strut working} \colorbox{red!0}{\strut harder} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut path} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut success} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sometimes} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut working} \colorbox{red!0}{\strut less} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut actually} \colorbox{red!0}{\strut produce} \colorbox{red!0}{\strut better} \colorbox{red!1}{\strut results} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: is death a natural disaster

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Natural} \colorbox{red!10}{\strut Disasters} \colorbox{red!9}{\strut Natural} \colorbox{red!0}{\strut DisastersNatural} \colorbox{red!0}{\strut DisastersIntroduction-} \colorbox{red!6}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut natural} \colorbox{red!10}{\strut disaster} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut definition} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut catastrophic} \colorbox{red!0}{\strut event} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!9}{\strut nature} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut natural} \colorbox{red!0}{\strut processes} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut earth} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut severity} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!10}{\strut disaster} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut measured} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut lives} \colorbox{red!0}{\strut lost} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut economic} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ability} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut population} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut rebuild} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Events} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut occur} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut unpopulated} \colorbox{red!0}{\strut areas} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut considered} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut So} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut flood} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut uninhabited} \colorbox{red!0}{\strut island} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut count} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!10}{\strut disaster} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut flood} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut populated} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut called} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut natural} \colorbox{red!0}{\strut disaster.All} \colorbox{red!9}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!1}{\strut cause} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut severity} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lives} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut lost} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Falling} \colorbox{red!0}{\strut buildings} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut trees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut freezing} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut death} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut washed} \colorbox{red!0}{\strut away} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut heat} \colorbox{red!0}{\strut stroke} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut deadly} \colorbox{red!0}{\strut effects} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!10}{\strut disasters} \colorbox{red!1}{\strut cause} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut life} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut population} \colorbox{red!0}{\strut density} \colorbox{red!0}{\strut affects} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut death} \colorbox{red!0}{\strut count} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well.Natural} \colorbox{red!0}{\strut Disasters} \colorbox{red!0}{\strut Asteroid} \colorbox{red!0}{\strut Avalanche} \colorbox{red!0}{\strut Blizzard} \colorbox{red!0}{\strut Thunderstorm} \colorbox{red!0}{\strut Earthquake} \colorbox{red!0}{\strut Flood} \colorbox{red!0}{\strut Gamma-Ray} \colorbox{red!0}{\strut Burst} \colorbox{red!0}{\strut Volcano} \colorbox{red!0}{\strut Eruption} \colorbox{red!0}{\strut Heat} \colorbox{red!0}{\strut Wave} \colorbox{red!0}{\strut Hurricane} \colorbox{red!0}{\strut Landslide} \colorbox{red!0}{\strut Solar} \colorbox{red!0}{\strut Flare} \colorbox{red!0}{\strut Drought} \colorbox{red!0}{\strut Tornado} \colorbox{red!0}{\strut Tsunami} \colorbox{red!0}{\strut Hail} \colorbox{red!0}{\strut WildfireThen} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut property} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut affects} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut living} \colorbox{red!0}{\strut quarters} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut transportation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut livelihood} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut means} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut live} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fields} \colorbox{red!0}{\strut saturated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut salt} \colorbox{red!0}{\strut water} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut tsunamis} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut grow} \colorbox{red!0}{\strut crops} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Homes} \colorbox{red!0}{\strut destroyed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut floods} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut hurricanes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cyclones} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut landslides} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut avalanches} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut volcanic} \colorbox{red!0}{\strut eruption} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut earthquake} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut beyond} \colorbox{red!0}{\strut repair} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lot} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut livable} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Personal} \colorbox{red!0}{\strut effects} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut memorabilia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut vehicles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut documents} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut hit} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut many} \colorbox{red!9}{\strut natural} \colorbox{red!0}{\strut disasters.The} \colorbox{red!9}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut affect} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut worldwide} \colorbox{red!0}{\strut tend} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut intense} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Frequency} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut earthquakes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mega} \colorbox{red!0}{\strut storms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut heat} \colorbox{red!0}{\strut waves} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut gone} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut death} \colorbox{red!1}{\strut toll} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut death} \colorbox{red!0}{\strut tollFrom} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedianavigation} \colorbox{red!0}{\strut searchA} \colorbox{red!8}{\strut natural} \colorbox{red!10}{\strut disaster} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut sudden} \colorbox{red!1}{\strut event} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut causes} \colorbox{red!0}{\strut widespread} \colorbox{red!0}{\strut destruction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lots} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut collateral} \colorbox{red!0}{\strut damage} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut life} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut brought} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut forces} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut acts} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut human} \colorbox{red!0}{\strut beings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!8}{\strut natural} \colorbox{red!10}{\strut disaster} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut earthquakes} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut flooding} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut volcanic} \colorbox{red!1}{\strut eruption} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut landslide} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut hurricanes} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut classified} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!10}{\strut disaster} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut profound} \colorbox{red!0}{\strut environmental} \colorbox{red!1}{\strut effect} \colorbox{red!0}{\strut andor} \colorbox{red!1}{\strut human} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut frequently} \colorbox{red!0}{\strut incurs} \colorbox{red!0}{\strut financial} \colorbox{red!0}{\strut loss.Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!8}{\strut natural} \colorbox{red!0}{\strut disasters2} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!8}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut 19003} \colorbox{red!1}{\strut Lists} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut cause3.1} \colorbox{red!1}{\strut Deadliest} \colorbox{red!0}{\strut earthquakes3.2} \colorbox{red!1}{\strut Deadliest} \colorbox{red!0}{\strut famines3.3} \colorbox{red!1}{\strut Deadliest} \colorbox{red!1}{\strut impact} \colorbox{red!0}{\strut events3.4} \colorbox{red!1}{\strut Deadliest} \colorbox{red!0}{\strut limnic} \colorbox{red!0}{\strut eruptions3.5} \colorbox{red!1}{\strut Deadliest} \colorbox{red!0}{\strut wildfires} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut bushfires3.6} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!0}{\strut avalanches3.7} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!0}{\strut blizzards3.8} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!1}{\strut floods} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut landslides3.9} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!0}{\strut heat} \colorbox{red!0}{\strut waves3.10} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!0}{\strut storms} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut non-cyclones} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.11} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!0}{\strut tornadoes3.12} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!1}{\strut tropical} \colorbox{red!0}{\strut cyclones3.13} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!0}{\strut tsunamis3.14} \colorbox{red!0}{\strut Ten} \colorbox{red!1}{\strut deadliest} \colorbox{red!0}{\strut volcanic} \colorbox{red!0}{\strut eruptions4} \colorbox{red!0}{\strut Notes5} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also6} \colorbox{red!0}{\strut References7} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut linksTen} \colorbox{red!1}{\strut deadliest} \colorbox{red!8}{\strut natural} \colorbox{red!10}{\strut disasters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Notes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut list} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut volcanic} \colorbox{red!1}{\strut eruptions} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut uncertain} \colorbox{red!1}{\strut death} \colorbox{red!0}{\strut tolls} \colorbox{red!0}{\strut resulting} \colorbox{red!0}{\strut from} \colorbox{red!1}{\strut collateral} \colorbox{red!1}{\strut effects} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut crop} \colorbox{red!0}{\strut failures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut though} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut numbered} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut millions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut see} \colorbox{red!1}{\strut List} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut volcanic} \colorbox{red!1}{\strut eruptions} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut death} \colorbox{red!1}{\strut toll} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut list} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut man-made} \colorbox{red!0}{\strut 1938} \colorbox{red!0}{\strut Yellow} \colorbox{red!0}{\strut River} \colorbox{red!1}{\strut flood} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut caused} \colorbox{red!0}{\strut entirely} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut deliberate} \colorbox{red!0}{\strut man-made} \colorbox{red!0}{\strut act} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut act} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut war} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut destroying} \colorbox{red!0}{\strut dikes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut alternative} \colorbox{red!1}{\strut listing} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Peter} \colorbox{red!0}{\strut Hough} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut 2008} \colorbox{red!0}{\strut book} \colorbox{red!0}{\strut Global} \colorbox{red!0}{\strut Security} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Rank} \colorbox{red!1}{\strut Death} \colorbox{red!1}{\strut toll} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut estimate} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Event} \colorbox{red!1}{\strut Location} \colorbox{red!0}{\strut Date1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,000,0004,000,000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut nb} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1931} \colorbox{red!0}{\strut China} \colorbox{red!1}{\strut floods} \colorbox{red!0}{\strut China} \colorbox{red!0}{\strut July} \colorbox{red!0}{\strut 19312} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 900,0002,000,000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1887} \colorbox{red!0}{\strut Yellow} \colorbox{red!0}{\strut River} 
}}}
\end{CJK*}

query: copperhead snake bite effects

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut long} \colorbox{red!10}{\strut term} \colorbox{red!7}{\strut effects} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut copperhead} \colorbox{red!10}{\strut snake} \colorbox{red!10}{\strut venom} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Answers.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut WikiAnswers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Categories} \colorbox{red!0}{\strut Animal} \colorbox{red!0}{\strut Life} \colorbox{red!0}{\strut Reptiles} \colorbox{red!10}{\strut Snakes} \colorbox{red!2}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut long} \colorbox{red!10}{\strut term} \colorbox{red!7}{\strut effects} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut copperhead} \colorbox{red!10}{\strut snake} \colorbox{red!10}{\strut venom} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut FlagWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut long} \colorbox{red!10}{\strut term} \colorbox{red!7}{\strut effects} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut copperhead} \colorbox{red!10}{\strut snake} \colorbox{red!10}{\strut venom} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answered} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut WikiAnswers} \colorbox{red!0}{\strut CommunityAnswers.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut making} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut time.I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut bitten} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!10}{\strut copperhead} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1981} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut foot} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut bite} \colorbox{red!0}{\strut immed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut started} \colorbox{red!0}{\strut swelling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lots} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut pain} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut super} \colorbox{red!0}{\strut bee} \colorbox{red!0}{\strut sting} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut stop} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut feeling} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut throwing} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut went} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ER} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut around} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut bite} \colorbox{red!0}{\strut fangs} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut turning} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut blue} \colorbox{red!0}{\strut red} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut cent} \colorbox{red!0}{\strut piece} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut ER} \colorbox{red!0}{\strut tested} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut anivemon} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut arm} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut swelling} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut thigh} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut received} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut injections} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut thigh} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 100lbs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut leg} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut packed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut ice} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut IV} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut leg} \colorbox{red!0}{\strut continued} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut swell} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut again} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut dose} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut buttocks} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut foot} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut bigger} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut football} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut shinny} \colorbox{red!0}{\strut tight} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut swelling} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut bend} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut toes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ankle} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut bend} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut knee} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut fang} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut skin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tissue} \colorbox{red!0}{\strut turned} \colorbox{red!0}{\strut black} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ability} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut bend} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PINKY} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut toe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut constant} \colorbox{red!0}{\strut pain} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut RSD} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut foot} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut hike} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut several} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut foot} \colorbox{red!0}{\strut swells} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Not} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut Since} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut bite} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut anemic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut taking} \colorbox{red!0}{\strut supplements} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut healthy} \colorbox{red!0}{\strut diet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut daily} \colorbox{red!0}{\strut to} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut Copperhead} \colorbox{red!6}{\strut Bites} \colorbox{red!5}{\strut Copperhead} \colorbox{red!0}{\strut BitesVenom} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut copperheads} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut deadly} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut die} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut copperhead} \colorbox{red!4}{\strut snake} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut due} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut allergic} \colorbox{red!0}{\strut reaction} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut People} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut weak} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut young} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut significant} \colorbox{red!0}{\strut impact} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut body} \colorbox{red!0}{\strut functions} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut copperhead} \colorbox{red!4}{\strut snake} \colorbox{red!6}{\strut bite} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut copperhead} \colorbox{red!0}{\strut injects} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut venom} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut ducts} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut fangs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Its} \colorbox{red!1}{\strut venom} \colorbox{red!0}{\strut disrupts} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut red} \colorbox{red!1}{\strut blood} \colorbox{red!0}{\strut cells} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut prey} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut turn} \colorbox{red!0}{\strut becomes} \colorbox{red!0}{\strut completely} \colorbox{red!0}{\strut subdued} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut Copperhead} \colorbox{red!4}{\strut snakes} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut jaws} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut flexible} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut swallow} \colorbox{red!0}{\strut prey} \colorbox{red!0}{\strut larger} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut twice} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut diameter.Copperhead} \colorbox{red!6}{\strut Bite} \colorbox{red!0}{\strut StatisticsAccording} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut poison} \colorbox{red!0}{\strut centers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 769} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut copperheads} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2001} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut those} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 37} \colorbox{red!1}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut venomous} \colorbox{red!4}{\strut snake} \colorbox{red!0}{\strut bites4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Figure} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Copperhead} \colorbox{red!4}{\strut Snake} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut painful} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut experts} \colorbox{red!0}{\strut suggest} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut seek} \colorbox{red!0}{\strut medical} \colorbox{red!0}{\strut advice} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut bite.Figure} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Approximately} \colorbox{red!0}{\strut 37} \colorbox{red!1}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut venomous} \colorbox{red!4}{\strut snake} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut copperheads.Copperhead} \colorbox{red!6}{\strut Bite} \colorbox{red!0}{\strut StatisticsIn} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut percentage} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut venomous} \colorbox{red!4}{\strut snake} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Agkistrodon} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut higher} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 40-year} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut North} \colorbox{red!0}{\strut Carolina} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 64} \colorbox{red!1}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut venomous} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut copperhead} \colorbox{red!4}{\strut snake} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut surprised} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Virginia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Carolina} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Tennessee.Swelling} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tissue} \colorbox{red!0}{\strut injuryCopperhead} \colorbox{red!4}{\strut snake} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut cause} \colorbox{red!0}{\strut swelling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut tissue} \colorbox{red!0}{\strut injury} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut abnormally} \colorbox{red!0}{\strut low} \colorbox{red!1}{\strut blood} \colorbox{red!0}{\strut pressure} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lack} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut blood} \colorbox{red!0}{\strut clotting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut general} \colorbox{red!0}{\strut pain} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut limbs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut recent} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut reports} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut deadly} \colorbox{red!6}{\strut bites} \colorbox{red!0}{\strut from} \colorbox{red!5}{\strut copperheads} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut former} \colorbox{red!0}{\strut police} \colorbox{red!0}{\strut officer} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Madison} \colorbox{red!0}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Texas} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut died} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut poison} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut copperhead} \colorbox{red!4}{\strut snake} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2006} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut victim} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut probably} \colorbox{red!0}{\strut allergic} \colorbox{red!0}{\strut to} 
}}}
\end{CJK*}

query: how many days to defrost

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut How} \colorbox{red!8}{\strut Long} \colorbox{red!0}{\strut Does} \colorbox{red!0}{\strut It} \colorbox{red!7}{\strut Take} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut Defrost} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut Turkey} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut BHG.com} \colorbox{red!0}{\strut Recipes} \colorbox{red!9}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Cook} \colorbox{red!1}{\strut Cooking} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PoultryHow} \colorbox{red!8}{\strut Long} \colorbox{red!0}{\strut Does} \colorbox{red!0}{\strut It} \colorbox{red!7}{\strut Take} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut Defrost} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut Turkey} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Plan} \colorbox{red!0}{\strut ahead} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut helpful} \colorbox{red!0}{\strut how-to} \colorbox{red!0}{\strut guide} \colorbox{red!0}{\strut for} \colorbox{red!6}{\strut defrosting} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut turkey} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut fridge} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut wonder} \colorbox{red!9}{\strut how} \colorbox{red!8}{\strut long} \colorbox{red!0}{\strut it} \colorbox{red!6}{\strut takes} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut defrost} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut frozen} \colorbox{red!8}{\strut turkey} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut answers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Plus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut tips} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut cooking} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut carving} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut turkey.PinFacebook} \colorbox{red!0}{\strut Twitter} \colorbox{red!0}{\strut Google} \colorbox{red!0}{\strut Plus} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut PrintHow} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut Days} \colorbox{red!0}{\strut Does} \colorbox{red!0}{\strut It} \colorbox{red!7}{\strut Take} \colorbox{red!0}{\strut to} \colorbox{red!7}{\strut Defrost} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut Turkey} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Refrigerator} \colorbox{red!0}{\strut ?} \colorbox{red!6}{\strut Defrosting} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut turkey} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut refrigerator} \colorbox{red!0}{\strut will} \colorbox{red!7}{\strut take} \colorbox{red!0}{\strut approximately} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut size} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut turkey.Allow} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut thawing} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut refrigerator} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut pounds} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut turkey.continue} \colorbox{red!0}{\strut reading} \colorbox{red!0}{\strut belowHelpful} \colorbox{red!8}{\strut Turkey} \colorbox{red!0}{\strut TipsHow} \colorbox{red!8}{\strut Long} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut Cook} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut TurkeyHow} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Thaw} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut TurkeyTurkey} \colorbox{red!0}{\strut Carving} \colorbox{red!0}{\strut GuideTurkey} \colorbox{red!0}{\strut Carving} \colorbox{red!0}{\strut 101NETWORK} \colorbox{red!0}{\strut ERRORCannot} \colorbox{red!0}{\strut Contact} \colorbox{red!0}{\strut ServerRELOAD} \colorbox{red!0}{\strut YOUR} \colorbox{red!0}{\strut SCREEN} \colorbox{red!0}{\strut OR} \colorbox{red!0}{\strut TRY} \colorbox{red!0}{\strut SELECTING} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut DIFFERENT} \colorbox{red!0}{\strut VIDEOHow} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Carve} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut TurkeyPinFacebook} \colorbox{red!0}{\strut Twitter} \colorbox{red!0}{\strut Google} \colorbox{red!0}{\strut Plus} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut Print} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!10}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Defrost} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut Meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Facebook} \colorbox{red!0}{\strut PinterestFreezeChillHow} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Defrost} \colorbox{red!0}{\strut Any} \colorbox{red!0}{\strut MeatMatt} \colorbox{red!0}{\strut Duckor} \colorbox{red!0}{\strut 04.14.15Photo} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Charles} \colorbox{red!0}{\strut Masters} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Food} \colorbox{red!0}{\strut Styling} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Sue} \colorbox{red!0}{\strut LiShareShare} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Defrost} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut Meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Facebook} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Defrost} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut Meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Twitter} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Defrost} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut Meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut Pinterest} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Defrost} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut Meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Google} \colorbox{red!0}{\strut Email} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut Defrost} \colorbox{red!0}{\strut Any} \colorbox{red!1}{\strut Meat} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut pageYou} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut options.The} \colorbox{red!1}{\strut freezer} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut favorite} \colorbox{red!0}{\strut assets} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut kitchen} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut constantly} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut ours} \colorbox{red!0}{\strut stocked} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut frozen} \colorbox{red!0}{\strut sausages} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut fish} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut ground} \colorbox{red!1}{\strut beef} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut proteins} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut quick} \colorbox{red!0}{\strut weeknight} \colorbox{red!0}{\strut meals} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pinch} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut grocery} \colorbox{red!0}{\strut store.There} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Integrate} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut freezer} \colorbox{red!0}{\strut pantry} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut home} \colorbox{red!2}{\strut cooking} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ll} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!10}{\strut defrosting} \colorbox{red!0}{\strut pro} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Yes} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut cooking} \colorbox{red!0}{\strut directly} \colorbox{red!0}{\strut from} \colorbox{red!2}{\strut frozen} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut technically} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut option} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut doing} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut result} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut watery} \colorbox{red!1}{\strut protein} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut overall} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut quality.Essentially} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut choices} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut safely} \colorbox{red!1}{\strut thawing} \colorbox{red!1}{\strut protein} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Which} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut down} \colorbox{red!0}{\strut to} \colorbox{red!10}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have.IDEAL} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut RefrigeratorSay} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut planned} \colorbox{red!0}{\strut ahead} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut tomorrow} \colorbox{red!0}{\strut night} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut dinner} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut absolute} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut safest} \colorbox{red!1}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut defrost} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut frozen} \colorbox{red!1}{\strut meat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut refrigeratoryour} \colorbox{red!1}{\strut meat} \colorbox{red!0}{\strut will} \colorbox{red!9}{\strut defrost} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut consistent} \colorbox{red!1}{\strut temperature} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut USDA} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut magical} \colorbox{red!0}{\strut safety} \colorbox{red!0}{\strut mark} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut F.Simply} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut meateither} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut plastic} \colorbox{red!0}{\strut packaging} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut removed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut covered} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut plastic} \colorbox{red!0}{\strut wrapon} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut plate} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut fridge} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut night} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut cooking} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut plate} \colorbox{red!0}{\strut ensures} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut moisture} \colorbox{red!0}{\strut produced} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut thawing} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut does} 
}}}
\end{CJK*}

query: monster types

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!3}{\strut Monster} \colorbox{red!9}{\strut Type} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Category} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut RaceMonster} \colorbox{red!0}{\strut TypeName} \colorbox{red!0}{\strut DescriptionDragonkind} \colorbox{red!10}{\strut Dragons} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut kith} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut kinFayThe} \colorbox{red!1}{\strut fairiefolke} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut sometimes} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut fayefolk} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut simply} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!12}{\strut fay} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut comprised} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut diverse} \colorbox{red!12}{\strut fay} \colorbox{red!6}{\strut races} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Wisps} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut pixies} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut brownies} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut rhym} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut fae} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut fairy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut treants} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut sirens} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut dryads} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut nymphs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut all} \colorbox{red!8}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut fairiefolke} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut exist} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Norrath.MagicalEncounters} \colorbox{red!1}{\strut created} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut intervention} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Magic} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut creatures} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut category} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut animated} \colorbox{red!0}{\strut candlestick} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut sings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut talks} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut French} \colorbox{red!0}{\strut accent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Frankenstein} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Monster.Mechanimagical} \colorbox{red!0}{\strut Various} \colorbox{red!0}{\strut mechanized} \colorbox{red!5}{\strut beings} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut clockworks} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut robotsNaturalThe} \colorbox{red!1}{\strut Natural} \colorbox{red!1}{\strut animals} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut beasts} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut real} \colorbox{red!1}{\strut world} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sizes} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut things} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut insects} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut bit} \colorbox{red!0}{\strut bigger} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut expect.PlanarPlanar} \colorbox{red!5}{\strut Beings} \colorbox{red!0}{\strut are} \colorbox{red!8}{\strut creatures} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Planes} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut than} \colorbox{red!7}{\strut Norrath} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Material} \colorbox{red!0}{\strut Plane} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Plant} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut various} \colorbox{red!6}{\strut races} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut flora} \colorbox{red!9}{\strut type} \colorbox{red!4}{\strut monsters} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut corners} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut Norrath} \colorbox{red!0}{\strut .Sentient} \colorbox{red!8}{\strut Creatures} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut self-awareness} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut andor} \colorbox{red!0}{\strut intelligence.Undead} \colorbox{red!0}{\strut That} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut once} \colorbox{red!0}{\strut living} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut yet} \colorbox{red!0}{\strut still} \colorbox{red!0}{\strut moves} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut tries} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut kill} \colorbox{red!0}{\strut you.Were} \colorbox{red!8}{\strut Creatures} \colorbox{red!0}{\strut afflicted} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut lycanthropy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut thus} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut turn} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut form.See} \colorbox{red!0}{\strut Also} \colorbox{red!0}{\strut EditMonstersMonsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut DifficultyMonsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut TierMonsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut UpdateMonsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut ZoneNamed} \colorbox{red!0}{\strut MonstersNamed} \colorbox{red!4}{\strut Monsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut DifficultyNamed} \colorbox{red!4}{\strut Monsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut TierNamed} \colorbox{red!4}{\strut Monsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut UpdateNamed} \colorbox{red!4}{\strut Monsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut ZoneFactionsFaction} \colorbox{red!0}{\strut MonstersNamed} \colorbox{red!0}{\strut Faction} \colorbox{red!0}{\strut MonstersMonsters} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut GroupMonsters} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut Monster} \colorbox{red!0}{\strut TypeTop} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut B} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut D} \colorbox{red!0}{\strut E} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut G} \colorbox{red!0}{\strut H} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut J} \colorbox{red!0}{\strut K} \colorbox{red!0}{\strut L} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut N} \colorbox{red!0}{\strut O} \colorbox{red!0}{\strut P} \colorbox{red!0}{\strut Q} \colorbox{red!0}{\strut R} \colorbox{red!0}{\strut S} \colorbox{red!0}{\strut T} \colorbox{red!0}{\strut U} \colorbox{red!0}{\strut V} \colorbox{red!0}{\strut W} \colorbox{red!0}{\strut X} \colorbox{red!0}{\strut Y} \colorbox{red!0}{\strut Z} \colorbox{red!0}{\strut SubcategoriesThis} \colorbox{red!1}{\strut category} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut subcategories} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut total.D} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Dragonkind} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut F} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!12}{\strut Fay} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut C} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut M} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Magical} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 34} \colorbox{red!0}{\strut C} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!22}{\strut Monster} \colorbox{red!10}{\strut Types} \colorbox{red!0}{\strut .} \colorbox{red!22}{\strut Monster} \colorbox{red!2}{\strut Codex} \colorbox{red!0}{\strut .} \colorbox{red!22}{\strut Monster} \colorbox{red!0}{\strut TypesThese} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut major} \colorbox{red!10}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!22}{\strut monsters} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!3}{\strut creatures} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!10}{\strut types} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut none} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut fall} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut category} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut appear} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut outsiders} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut humanoid} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut appearance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .Description} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Vision} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut darkvision} \colorbox{red!0}{\strut low-light} \colorbox{red!0}{\strut vision} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Breathing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sleeping} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut eatingWeapon} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut armor} \colorbox{red!0}{\strut proficiencyWhether} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut magical} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut non-magicalSentienceDescription} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut preferred} \colorbox{red!0}{\strut skillsDescription} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut defensesAdditional} \colorbox{red!0}{\strut notesAny} \colorbox{red!0}{\strut inherent} \colorbox{red!0}{\strut immunity} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut creature} \colorbox{red!10}{\strut type} \colorbox{red!0}{\strut hasAberrationThese} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut strange} \colorbox{red!0}{\strut abominations} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut necessarily} \colorbox{red!0}{\strut fit} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut theme} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut typically} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut amorphous} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut many} \colorbox{red!2}{\strut appendages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Often} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut tentacles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut multiple} \colorbox{red!0}{\strut heads} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut reside} \colorbox{red!0}{\strut undergroundDarkvision} \colorbox{red!0}{\strut 60Aberrations} \colorbox{red!0}{\strut breathe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sleep} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut eatProficient} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut any} \colorbox{red!2}{\strut weapon} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut described} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut wielding} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut armor} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut described} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut wearing} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut proficient} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut natural} \colorbox{red!0}{\strut weapons.Aberrations} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut unnatural} \colorbox{red!3}{\strut creatures} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut magical} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut natureAberrations} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut either} \colorbox{red!2}{\strut sentient} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut non-sentientPreferred} \colorbox{red!2}{\strut skills} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Acrobatics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Athletics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Escape} \colorbox{red!0}{\strut artist} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Intimidate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut knowledge} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Perception} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Stealth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut SurvivalHigh} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fortitude} \colorbox{red!0}{\strut defense} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut poor} \colorbox{red!0}{\strut dodgeAberrations} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut powers} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut usually} \colorbox{red!0}{\strut deal} \colorbox{red!0}{\strut multiple} \colorbox{red!0}{\strut attacks.AnimalNon-human} \colorbox{red!3}{\strut creatures} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut reality} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!2}{\strut animals} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut creatures} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut exist} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut reality} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut existed} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut point.Low-light} \colorbox{red!0}{\strut visionAnimals} \colorbox{red!0}{\strut breath} \colorbox{red!0}{\strut sleep} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut eatAnimals} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut proficient} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut any} \colorbox{red!2}{\strut weapon} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut armor} \colorbox{red!0}{\strut aside} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut natural} \colorbox{red!0}{\strut weapons} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut animals} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut trained} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut proficient} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut special} \colorbox{red!10}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut armor.Animals} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut non-magical} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut natureAnimals} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut non-sentient} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut granted} \colorbox{red!2}{\strut sentience} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut magicPreferred} \colorbox{red!2}{\strut skills} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Acrobatics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Athletics} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Perception} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut StealthLow} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut defenseConstructMechanical} \colorbox{red!0}{\strut creations} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut not} \colorbox{red!2}{\strut living} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut given} \colorbox{red!0}{\strut life} \colorbox{red!0}{\strut through} \colorbox{red!2}{\strut magical} \colorbox{red!2}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Unlike} \colorbox{red!2}{\strut undead} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut animated} \colorbox{red!0}{\strut through} \colorbox{red!2}{\strut magic} 
}}}
\end{CJK*}

query: current fad diet

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Top} \colorbox{red!0}{\strut 5} \colorbox{red!7}{\strut Fad} \colorbox{red!10}{\strut Diets} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Top} \colorbox{red!0}{\strut 5} \colorbox{red!7}{\strut Fad} \colorbox{red!10}{\strut Diets} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2015Whether} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut counting} \colorbox{red!0}{\strut carbs} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut drinking} \colorbox{red!0}{\strut herbal} \colorbox{red!0}{\strut tea} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut lose} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut fad} \colorbox{red!10}{\strut diet} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut fits} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut particular} \colorbox{red!0}{\strut inclinations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut real} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut And} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut forever} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut Report} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!7}{\strut fad} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut loss} \colorbox{red!10}{\strut diets} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut rise} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rest} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut ring} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut new} \colorbox{red!7}{\strut fad} \colorbox{red!10}{\strut diets} \colorbox{red!0}{\strut emerge} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut fade} \colorbox{red!0}{\strut away.Topping} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut fad} \colorbox{red!10}{\strut diets} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut 2015} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut Weight} \colorbox{red!0}{\strut Watchers} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut currently} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut widely-adopted} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut loss} \colorbox{red!10}{\strut diet} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut country} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Aside} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut big} \colorbox{red!0}{\strut WW} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut top} \colorbox{red!7}{\strut fad} \colorbox{red!10}{\strut diets} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2015.1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Biggest} \colorbox{red!0}{\strut Loser} \colorbox{red!0}{\strut DietThis} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut proven} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut contestants} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut popular} \colorbox{red!0}{\strut TV} \colorbox{red!0}{\strut show} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut emphasizes} \colorbox{red!0}{\strut filling} \colorbox{red!1}{\strut foods} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut sources} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut fruits} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut vegetables} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lean} \colorbox{red!0}{\strut protein} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut whole} \colorbox{red!0}{\strut grains} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Portion} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut food} \colorbox{red!0}{\strut journaling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut jumping} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut sofa} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut key} \colorbox{red!0}{\strut components} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut top} \colorbox{red!7}{\strut fad} \colorbox{red!10}{\strut diet} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut uses} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut food} \colorbox{red!0}{\strut pyramid} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut suggestions} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut exercising} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut lists} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut calories} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut burn} \colorbox{red!0}{\strut doing} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut abundance} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut recipes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut enjoy} \colorbox{red!0}{\strut Mexican} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Italian} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Asian} \colorbox{red!0}{\strut cuisines-as} \colorbox{red!0}{\strut long} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut overboard.2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Spark} \colorbox{red!0}{\strut SolutionThis} \colorbox{red!0}{\strut plan} \colorbox{red!0}{\strut brings} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut community} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Sparkpeople} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut fad} \colorbox{red!10}{\strut diet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Spark} \colorbox{red!0}{\strut Solution} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut playbook} \colorbox{red!0}{\strut containing} \colorbox{red!0}{\strut meal} \colorbox{red!0}{\strut plans} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut daily} \colorbox{red!0}{\strut guidance} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut food} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut decisions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut employs} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut basic} \colorbox{red!0}{\strut building} \colorbox{red!0}{\strut blocks} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut weight} \colorbox{red!0}{\strut loss} \colorbox{red!10}{\strut diet} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut healthy} \colorbox{red!0}{\strut eating} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sparkpeople} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut success} \colorbox{red!0}{\strut stories} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Current} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut 5} \colorbox{red!11}{\strut Fad} \colorbox{red!13}{\strut Diets} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Current} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut 5} \colorbox{red!11}{\strut Fad} \colorbox{red!0}{\strut Dietsby} \colorbox{red!0}{\strut Kristen} \colorbox{red!0}{\strut Ciuba} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Sep} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2014TweetIf} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut sounds} \colorbox{red!0}{\strut too} \colorbox{red!1}{\strut good} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut probably} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut How} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut times} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut heard} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut warning} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut things} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut life} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut weight-loss} \colorbox{red!0}{\strut promise} \colorbox{red!0}{\strut sounds} \colorbox{red!0}{\strut too} \colorbox{red!1}{\strut good} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut true} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut probably} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Lose} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut pounds} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut week} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Eat} \colorbox{red!6}{\strut what} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut still} \colorbox{red!1}{\strut lose} \colorbox{red!2}{\strut weight} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Try} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Chocolate} \colorbox{red!13}{\strut Diet} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut seen} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut claims} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut counted} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut real} \colorbox{red!0}{\strut weight-loss} \colorbox{red!13}{\strut diets} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut are} \colorbox{red!8}{\strut fads} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Jared} \colorbox{red!0}{\strut Rice} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut MS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut RD} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut HFS} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Washington} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut D.C.} \colorbox{red!0}{\strut area-based} \colorbox{red!1}{\strut nutrition} \colorbox{red!0}{\strut expert} \colorbox{red!0}{\strut warns} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut So} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut times} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut see} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut getting} \colorbox{red!0}{\strut pulled} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut so-called} \colorbox{red!11}{\strut fad} \colorbox{red!13}{\strut diets} \colorbox{red!0}{\strut simply} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut others} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut saying} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut thinking} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut healthy.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut definition} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!11}{\strut fad} \colorbox{red!13}{\strut diet} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut over-emphasizes} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut bans} \colorbox{red!0}{\strut one} \colorbox{red!2}{\strut food} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut food} \colorbox{red!0}{\strut group} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut guarantees} \colorbox{red!0}{\strut rapid} \colorbox{red!0}{\strut weight-loss} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut promises} \colorbox{red!0}{\strut quick} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut easy} \colorbox{red!0}{\strut solutions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut ever} \colorbox{red!0}{\strut lost} \colorbox{red!2}{\strut weight} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut maintained} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut lasting} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut quick} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut easy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Here} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut review} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut current} \colorbox{red!0}{\strut top} \colorbox{red!0}{\strut 5} \colorbox{red!11}{\strut fad} \colorbox{red!13}{\strut diets} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut why} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut long-term} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut derail} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut weight-loss} \colorbox{red!0}{\strut efforts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut harmful} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut health.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut High} \colorbox{red!0}{\strut ProteinProtein} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut essential} \colorbox{red!0}{\strut nutrient} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut helps} \colorbox{red!0}{\strut repair} \colorbox{red!0}{\strut muscles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut aids} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut recovery} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut injury} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut maintains} \colorbox{red!1}{\strut healthy} \colorbox{red!0}{\strut hair} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut nails} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!1}{\strut consuming} \colorbox{red!0}{\strut too} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut unhealthy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut high-protein} \colorbox{red!13}{\strut diet} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut stress} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut kidneys} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut organs} \colorbox{red!0}{\strut responsible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut metabolizing} \colorbox{red!1}{\strut protein} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut While} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut protein-rich} \colorbox{red!2}{\strut foods} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut lean} \colorbox{red!1}{\strut meats} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut non-fat} \colorbox{red!0}{\strut yogurt} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut edamame} \colorbox{red!0}{\strut and} 
}}}
\end{CJK*}



==> sections/visualization/rel.tex <==
query: which gas is produced when mg(s) is added to hcl(aq

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!19}{\strut reaction} \colorbox{red!0}{\strut between} \colorbox{red!31}{\strut HCl} \colorbox{red!1}{\strut and} \colorbox{red!38}{\strut Mg} \colorbox{red!20}{\strut produces} \colorbox{red!8}{\strut Hydrogen} \colorbox{red!11}{\strut gas} \colorbox{red!1}{\strut and} \colorbox{red!7}{\strut Magnesium} \colorbox{red!8}{\strut Chloride} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut balanced} \colorbox{red!1}{\strut equation} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!19}{\strut reaction} \colorbox{red!0}{\strut :} \colorbox{red!38}{\strut Mg} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut +2HCl} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut l} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut âH2} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut g} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut +MgCl2} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut l} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Quick} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!16}{\strut chemical} \colorbox{red!20}{\strut reaction} \colorbox{red!0}{\strut between} \colorbox{red!13}{\strut hydrochloric} \colorbox{red!10}{\strut acid} \colorbox{red!0}{\strut and} \colorbox{red!21}{\strut magnesium} \colorbox{red!14}{\strut produces} \colorbox{red!21}{\strut magnesium} \colorbox{red!4}{\strut chloride} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut hydrogen} \colorbox{red!3}{\strut gas} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut balanced} \colorbox{red!16}{\strut chemical} \colorbox{red!2}{\strut equation} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!20}{\strut reaction} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut Mg} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut s} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut +} \colorbox{red!0}{\strut 2} \colorbox{red!2}{\strut HCl} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut aq} \colorbox{red!0}{\strut )} \colorbox{red!14}{\strut produces} \colorbox{red!2}{\strut MgCl2} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut aq} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut +} \colorbox{red!0}{\strut H2} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut g} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut letter} \colorbox{red!2}{\strut s} \colorbox{red!0}{\strut stands} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut solid} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut g} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut gas} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut aq} \colorbox{red!0}{\strut represents} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut aqueous} \colorbox{red!0}{\strut solution} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Keep} \colorbox{red!0}{\strut Learning} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what values do zoos serve

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!54}{\strut Zoos} \colorbox{red!9}{\strut serve} \colorbox{red!0}{\strut several} \colorbox{red!58}{\strut puposes} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ask} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut Park/Garden} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut Some} \colorbox{red!54}{\strut zoos} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut similar} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut botanical} \colorbox{red!4}{\strut garden} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut city} \colorbox{red!3}{\strut park} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut give} \colorbox{red!1}{\strut people} \colorbox{red!1}{\strut living} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut crowded} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut noisy} \colorbox{red!3}{\strut cities} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut walk} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut beautiful} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut maintained} \colorbox{red!1}{\strut outdoor} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut animal} \colorbox{red!1}{\strut exhibits} \colorbox{red!0}{\strut create} \colorbox{red!0}{\strut interesting} \colorbox{red!0}{\strut scenery} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fun} \colorbox{red!0}{\strut excursion} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut NO} \colorbox{red!12}{\strut purebred} \colorbox{red!17}{\strut Bengal} \colorbox{red!34}{\strut tigers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut only} \colorbox{red!12}{\strut purebred} \colorbox{red!34}{\strut tigers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut AZA} \colorbox{red!4}{\strut zoos} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut 133} \colorbox{red!2}{\strut Amur} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut AKA} \colorbox{red!2}{\strut Siberian} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 73} \colorbox{red!0}{\strut Sumatran} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 50} \colorbox{red!0}{\strut Malayan} \colorbox{red!34}{\strut tigers} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Species} \colorbox{red!0}{\strut Survival} \colorbox{red!0}{\strut Plan} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut U.S.} \colorbox{red!2}{\strut captive} \colorbox{red!34}{\strut tigers} \colorbox{red!0}{\strut are} \colorbox{red!5}{\strut inbred} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cross} \colorbox{red!2}{\strut bred} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut serve} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut conservation} \colorbox{red!0}{\strut value} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what types of trees are in maryland

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!95}{\strut MARYLAND} \colorbox{red!101}{\strut TREES} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!1}{\strut Birch} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut River} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Betula} \colorbox{red!0}{\strut nigra} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Blackgum} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Sour} \colorbox{red!0}{\strut Gum} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Nyssa} \colorbox{red!0}{\strut sylvatica} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Butternut} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut White} \colorbox{red!1}{\strut Walnut} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Juglans} \colorbox{red!0}{\strut cinerea} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut Cedar} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Atlantic} \colorbox{red!1}{\strut White} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Chamaecyparis} \colorbox{red!0}{\strut thyoides} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Cedar} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Eastern} \colorbox{red!0}{\strut Red} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Juniperus} \colorbox{red!0}{\strut virginiana} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut Cherry} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Black} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Prunus} \colorbox{red!0}{\strut serotina} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut Chestnut} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Castanea} \colorbox{red!0}{\strut dentata} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut Chinkapin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Allegheny} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Castanea} \colorbox{red!0}{\strut pumila} \colorbox{red!0}{\strut )} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Over} \colorbox{red!0}{\strut 60} \colorbox{red!5}{\strut species} \colorbox{red!0}{\strut of} \colorbox{red!27}{\strut trees} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut cataloged} \colorbox{red!0}{\strut as} \colorbox{red!5}{\strut native} \colorbox{red!0}{\strut to} \colorbox{red!27}{\strut Maryland} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut White} \colorbox{red!2}{\strut Oak} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Quercus} \colorbox{red!0}{\strut alba} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut State} \colorbox{red!27}{\strut tree} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Magnolia} \colorbox{red!0}{\strut blossom} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Annapolis} \colorbox{red!0}{\strut ,} \colorbox{red!27}{\strut Maryland} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut June} \colorbox{red!0}{\strut 1999} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Diane} \colorbox{red!0}{\strut P.} \colorbox{red!0}{\strut Frese} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 100} \colorbox{red!4}{\strut Poisonous} \colorbox{red!9}{\strut Plants} \colorbox{red!0}{\strut of} \colorbox{red!27}{\strut Maryland} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!27}{\strut Maryland} \colorbox{red!0}{\strut )} 
}}}
\end{CJK*}

query: what is the training wage

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!26}{\strut Training} \colorbox{red!27}{\strut minimum} \colorbox{red!26}{\strut wage} \colorbox{red!0}{\strut The} \colorbox{red!26}{\strut training} \colorbox{red!27}{\strut minimum} \colorbox{red!26}{\strut wage} \colorbox{red!0}{\strut :} \colorbox{red!1}{\strut applies} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut employees} \colorbox{red!5}{\strut aged} \colorbox{red!0}{\strut 20} \colorbox{red!1}{\strut years} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut whose} \colorbox{red!2}{\strut employment} \colorbox{red!0}{\strut agreement} \colorbox{red!0}{\strut states} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 60} \colorbox{red!1}{\strut credits} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut industry} \colorbox{red!26}{\strut training} \colorbox{red!0}{\strut programme} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!1}{\strut qualified} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut working} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut 5330582702602} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thanks} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut question.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thanks} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut question.} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!30}{\strut average} \colorbox{red!28}{\strut salary} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!33}{\strut McDonald} \colorbox{red!0}{\strut 's} \colorbox{red!13}{\strut restaurant} \colorbox{red!21}{\strut employee} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut ,} \colorbox{red!28}{\strut salary} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut pay} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut staff} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut training} \colorbox{red!21}{\strut employee} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut hourly} \colorbox{red!3}{\strut rate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Behind} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Job} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut 's} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut work} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Wages} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 5330582702602} 
}}}
\end{CJK*}

query: what is the suprachiasmatic nucleus and what is its function?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut That} \colorbox{red!9}{\strut internal} \colorbox{red!7}{\strut clock} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut body} \colorbox{red!2}{\strut does} \colorbox{red!0}{\strut indeed} \colorbox{red!3}{\strut exist} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!8}{\strut called} \colorbox{red!0}{\strut the} \colorbox{red!27}{\strut suprachiasmatic} \colorbox{red!23}{\strut nucleus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Our} \colorbox{red!11}{\strut body} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!1}{\strut advanced} \colorbox{red!6}{\strut system} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut provision} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut our} \colorbox{red!2}{\strut needs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Through} \colorbox{red!1}{\strut evolution} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut our} \colorbox{red!9}{\strut bodies} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut developed} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut timetable} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut our} \colorbox{red!9}{\strut internal} \colorbox{red!9}{\strut functions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 24-hour} \colorbox{red!2}{\strut cycle} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut night} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut implementation} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut synchronization} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut timetable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut according} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut external} \colorbox{red!1}{\strut stimuli} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut controlled} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!23}{\strut nucleus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut our} \colorbox{red!12}{\strut brain} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Many} \colorbox{red!1}{\strut tissues} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut body} \colorbox{red!0}{\strut will} \colorbox{red!1}{\strut follow} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut circadian} \colorbox{red!1}{\strut pattern} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut primary} \colorbox{red!2}{\strut coordinator} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut brain} \colorbox{red!4}{\strut called} \colorbox{red!0}{\strut the} \colorbox{red!14}{\strut suprachiasmatic} \colorbox{red!15}{\strut nucleus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut the} \colorbox{red!14}{\strut Suprachiasmatic} \colorbox{red!15}{\strut Nucleus} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut Brain} \colorbox{red!0}{\strut 's} \colorbox{red!3}{\strut Hypothalamus} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!14}{\strut suprachiasmatic} \colorbox{red!15}{\strut nucleus} \colorbox{red!0}{\strut is} \colorbox{red!7}{\strut located} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut forward} \colorbox{red!2}{\strut region} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut brain} \colorbox{red!4}{\strut called} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut hypothalamus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!1}{\strut contains} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut group} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut nerve} \colorbox{red!1}{\strut cells} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut or} \colorbox{red!2}{\strut neurons} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut body} \colorbox{red!0}{\strut 's} \colorbox{red!2}{\strut circadian} \colorbox{red!1}{\strut rhythm} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!14}{\strut suprachiasmatic} \colorbox{red!15}{\strut nucleus} \colorbox{red!0}{\strut lies} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut shallow} \colorbox{red!0}{\strut impression} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut optic} \colorbox{red!0}{\strut chiasm} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut nerves} \colorbox{red!0}{\strut extending} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut each} \colorbox{red!1}{\strut eye} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut brain} \colorbox{red!0}{\strut cross} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut thus} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut highly} \colorbox{red!0}{\strut influenced} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut input} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut light} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Role} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut SCN} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Normal} \colorbox{red!0}{\strut Sleep} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Circadian} \colorbox{red!0}{\strut Rhythms} 
}}}
\end{CJK*}

query: what is the perimeter of triangle

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!32}{\strut perimeter} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!32}{\strut triangle} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut sum} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut sides} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!32}{\strut triangle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut determine} \colorbox{red!0}{\strut the} \colorbox{red!32}{\strut perimeter} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut any} \colorbox{red!32}{\strut triangle} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lengths} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut three} \colorbox{red!2}{\strut sides} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Since} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut isosceles} \colorbox{red!32}{\strut triangle} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut ...} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Remember} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut formula} \colorbox{red!0}{\strut for} \colorbox{red!6}{\strut finding} \colorbox{red!0}{\strut the} \colorbox{red!24}{\strut perimeter} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!26}{\strut triangle} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut a} \colorbox{red!26}{\strut triangle} \colorbox{red!0}{\strut with} \colorbox{red!4}{\strut sides} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut b} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut c} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!24}{\strut perimeter} \colorbox{red!5}{\strut P} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut defined} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut :} \colorbox{red!5}{\strut P} \colorbox{red!0}{\strut =} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut +} \colorbox{red!2}{\strut b} \colorbox{red!0}{\strut +} \colorbox{red!0}{\strut c.} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut formula} \colorbox{red!4}{\strut means} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut simpler} \colorbox{red!2}{\strut terms} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut to} \colorbox{red!5}{\strut find} \colorbox{red!0}{\strut the} \colorbox{red!24}{\strut perimeter} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!26}{\strut triangle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut together} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lengths} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut 3} \colorbox{red!4}{\strut sides} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is the job description for cashiers?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!88}{\strut Cashier} \colorbox{red!58}{\strut Job} \colorbox{red!27}{\strut Description} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!2}{\strut Managing} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut cash} \colorbox{red!2}{\strut transactions} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut workplace} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Maintaining} \colorbox{red!2}{\strut daily} \colorbox{red!1}{\strut account} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut daily} \colorbox{red!2}{\strut transactions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Balancing} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut daily} \colorbox{red!1}{\strut account} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut end} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!1}{\strut Checking} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut daily} \colorbox{red!3}{\strut cash} \colorbox{red!0}{\strut balance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Interacting} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut customers} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut counter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut Solving} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut cash} \colorbox{red!0}{\strut related} \colorbox{red!0}{\strut queries} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut duties} \colorbox{red!18}{\strut head} \colorbox{red!23}{\strut cashier} \colorbox{red!3}{\strut job} \colorbox{red!2}{\strut description} \colorbox{red!18}{\strut head} \colorbox{red!23}{\strut cashier} \colorbox{red!3}{\strut job} \colorbox{red!2}{\strut description} \colorbox{red!2}{\strut example} \colorbox{red!18}{\strut head} \colorbox{red!23}{\strut cashier} \colorbox{red!3}{\strut job} \colorbox{red!2}{\strut description} \colorbox{red!0}{\strut sample} \colorbox{red!18}{\strut head} \colorbox{red!23}{\strut cashier} \colorbox{red!6}{\strut role} \colorbox{red!3}{\strut responsibilities} \colorbox{red!3}{\strut tasks} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: who is susan boyle

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Amateur} \colorbox{red!5}{\strut vocalist} \colorbox{red!83}{\strut Susan} \colorbox{red!85}{\strut Boyle} \colorbox{red!0}{\strut became} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut overnight} \colorbox{red!1}{\strut sensation} \colorbox{red!0}{\strut after} \colorbox{red!2}{\strut appearing} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut round} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut 's} \colorbox{red!2}{\strut popular} \colorbox{red!0}{\strut U.K.} \colorbox{red!3}{\strut reality} \colorbox{red!7}{\strut show} \colorbox{red!0}{\strut Britain} \colorbox{red!0}{\strut 's} \colorbox{red!4}{\strut Got} \colorbox{red!4}{\strut Talent} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Best} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut a} \colorbox{red!38}{\strut troll} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut generally} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut tries} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!2}{\strut attention} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut posting} \colorbox{red!0}{\strut things} \colorbox{red!0}{\strut everyone} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut disagree} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut going} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!19}{\strut susan} \colorbox{red!3}{\strut boyle} \colorbox{red!0}{\strut fan} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut writing} \colorbox{red!19}{\strut susan} \colorbox{red!3}{\strut boyle} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ugly} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut wall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut usually} \colorbox{red!0}{\strut 14-16} \colorbox{red!0}{\strut year} \colorbox{red!5}{\strut olds} \colorbox{red!0}{\strut who} \colorbox{red!3}{\strut crave} \colorbox{red!0}{\strut attention.Source} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut est} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut a} \colorbox{red!38}{\strut troll} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut generally} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut tries} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!2}{\strut attention} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut posting} \colorbox{red!0}{\strut things} \colorbox{red!0}{\strut everyone} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut disagree} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut going} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!19}{\strut susan} \colorbox{red!3}{\strut boyle} \colorbox{red!0}{\strut fan} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut writing} \colorbox{red!19}{\strut susan} \colorbox{red!3}{\strut boyle} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ugly} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut wall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut are} \colorbox{red!3}{\strut usually} \colorbox{red!0}{\strut 14-16} \colorbox{red!0}{\strut year} \colorbox{red!5}{\strut olds} \colorbox{red!0}{\strut who} \colorbox{red!3}{\strut crave} \colorbox{red!2}{\strut attention} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Source} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut :} 
}}}
\end{CJK*}

query: who is the king of scotland today

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Following} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Jacobite} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!27}{\strut current} \colorbox{red!64}{\strut King} \colorbox{red!0}{\strut of} \colorbox{red!74}{\strut Scotland} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut Franz} \colorbox{red!0}{\strut Bonaventura} \colorbox{red!1}{\strut Adalbert} \colorbox{red!0}{\strut Maria} \colorbox{red!3}{\strut Herzog} \colorbox{red!1}{\strut von} \colorbox{red!3}{\strut Bayern} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut whose} \colorbox{red!0}{\strut great-grandfather} \colorbox{red!1}{\strut Ludwig} \colorbox{red!0}{\strut III} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut last} \colorbox{red!2}{\strut Bavarian} \colorbox{red!15}{\strut monarch} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut deposed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1918} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Now} \colorbox{red!0}{\strut 77} \colorbox{red!0}{\strut years} \colorbox{red!4}{\strut old} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut his} \colorbox{red!3}{\strut heir} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut younger} \colorbox{red!2}{\strut brother} \colorbox{red!0}{\strut Max} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 74} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut Sophie} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut eldest} \colorbox{red!0}{\strut niece} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut From} \colorbox{red!4}{\strut Scottish} \colorbox{red!2}{\strut Mael} \colorbox{red!0}{\strut MÃ¡el} \colorbox{red!8}{\strut coluim} \colorbox{red!0}{\strut which} \colorbox{red!14}{\strut means} \colorbox{red!2}{\strut disciple} \colorbox{red!0}{\strut Of} \colorbox{red!2}{\strut SAINT} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Columba} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!23}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut four} \colorbox{red!15}{\strut kings} \colorbox{red!0}{\strut Of} \colorbox{red!9}{\strut scotland} \colorbox{red!2}{\strut starting} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut 10th} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut century} \colorbox{red!0}{\strut Including} \colorbox{red!3}{\strut MALCOLM} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut iii} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut became} \colorbox{red!14}{\strut king} \colorbox{red!0}{\strut after} \colorbox{red!2}{\strut Killing} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut macbeth} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut usurper} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut murdered} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut fatherhis} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!23}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut four} \colorbox{red!15}{\strut kings} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut Scotland} \colorbox{red!2}{\strut starting} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut 10th} \colorbox{red!2}{\strut century} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!3}{\strut Malcolm} \colorbox{red!2}{\strut III} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut became} \colorbox{red!14}{\strut king} \colorbox{red!0}{\strut after} \colorbox{red!2}{\strut killing} \colorbox{red!3}{\strut Macbeth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut usurper} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut murdered} \colorbox{red!0}{\strut his} \colorbox{red!2}{\strut father} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is terminal f

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!67}{\strut Terminal} \colorbox{red!58}{\strut F} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!22}{\strut good} \colorbox{red!14}{\strut condition} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pretty} \colorbox{red!22}{\strut good} \colorbox{red!1}{\strut place} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut kill} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut day} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut age} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut more} \colorbox{red!8}{\strut charging} \colorbox{red!4}{\strut plugs} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut public} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut 4} \colorbox{red!2}{\strut stars} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!16}{\strut new} \colorbox{red!18}{\strut international} \colorbox{red!37}{\strut terminal} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!16}{\strut new} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 1.4} \colorbox{red!0}{\strut billion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1.2} \colorbox{red!0}{\strut million-square-foot} \colorbox{red!4}{\strut Maynard} \colorbox{red!0}{\strut H.} \colorbox{red!9}{\strut Jackson} \colorbox{red!18}{\strut International} \colorbox{red!37}{\strut Terminal} \colorbox{red!6}{\strut opens} \colorbox{red!0}{\strut May} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut introducing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut front} \colorbox{red!0}{\strut door} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!19}{\strut airport} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut a} \colorbox{red!16}{\strut new} \colorbox{red!0}{\strut 12-gate} \colorbox{red!3}{\strut Concourse} \colorbox{red!2}{\strut F} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is ryan seacrest sc

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!24}{\strut Ryan} \colorbox{red!25}{\strut Seacrest} \colorbox{red!0}{\strut 's} \colorbox{red!1}{\strut Height} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut 5ft} \colorbox{red!0}{\strut 7.25in} \colorbox{red!25}{\strut Seacrest} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut Usher} \colorbox{red!0}{\strut Raymond} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut 's} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 5'7} \colorbox{red!24}{\strut Ryan} \colorbox{red!1}{\strut John} \colorbox{red!25}{\strut Seacrest} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut American} \colorbox{red!0}{\strut radio} \colorbox{red!0}{\strut personality} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut television} \colorbox{red!1}{\strut host} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut producer} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut hosting} \colorbox{red!1}{\strut American} \colorbox{red!0}{\strut Top} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut American} \colorbox{red!1}{\strut Idol} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut Air} \colorbox{red!0}{\strut with} \colorbox{red!24}{\strut Ryan} \colorbox{red!25}{\strut Seacrest} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Live} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut Kelly} \colorbox{red!0}{\strut and} \colorbox{red!24}{\strut Ryan} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut claimed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut 5'8} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 5'8.5} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut 5'9} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Related} \colorbox{red!14}{\strut Ryan} \colorbox{red!14}{\strut Seacrest} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut What} \colorbox{red!12}{\strut cologne} \colorbox{red!0}{\strut does} \colorbox{red!14}{\strut Ryan} \colorbox{red!14}{\strut Seacrest} \colorbox{red!13}{\strut wear} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut what} \colorbox{red!12}{\strut cologne} \colorbox{red!14}{\strut Ryan} \colorbox{red!12}{\strut wears} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut American} \colorbox{red!1}{\strut Idol} \colorbox{red!1}{\strut host} \colorbox{red!14}{\strut Ryan} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Does} \colorbox{red!14}{\strut ryan} \colorbox{red!14}{\strut seacrest} \colorbox{red!13}{\strut wear} \colorbox{red!0}{\strut lifts} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut .} \colorbox{red!14}{\strut Ryan} \colorbox{red!0}{\strut John} \colorbox{red!14}{\strut Seacrest} \colorbox{red!0}{\strut Date} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Birth} \colorbox{red!0}{\strut December} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut 1974} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Atlanta} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Georgia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ...} 
}}}
\end{CJK*}

query: what is net gain

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!25}{\strut Net} \colorbox{red!24}{\strut gain} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut refer} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut :} \colorbox{red!25}{\strut Net} \colorbox{red!24}{\strut gain} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut telecommunications} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut overall} \colorbox{red!24}{\strut gain} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut transmission} \colorbox{red!0}{\strut circuit} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Net} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut economics} \colorbox{red!0}{\strut )} \colorbox{red!25}{\strut Net} \colorbox{red!1}{\strut profit} \colorbox{red!0}{\strut ;} \colorbox{red!25}{\strut Net} \colorbox{red!1}{\strut income} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!17}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut a} \colorbox{red!20}{\strut net} \colorbox{red!20}{\strut gain} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!20}{\strut net} \colorbox{red!19}{\strut loss} \colorbox{red!0}{\strut ?} \colorbox{red!20}{\strut Net} \colorbox{red!20}{\strut gain} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut income} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut greater} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut expenses} \colorbox{red!0}{\strut ,} \colorbox{red!20}{\strut net} \colorbox{red!19}{\strut loss} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut when} \colorbox{red!3}{\strut expenses} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut greater} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut your} \colorbox{red!3}{\strut income} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut Spending} \colorbox{red!2}{\strut Plan} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut document} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut record} \colorbox{red!1}{\strut planned} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut actual} \colorbox{red!3}{\strut income} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut expenses} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut time} 
}}}
\end{CJK*}

query: what is hold mail

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut exists} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut alternate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!38}{\strut Hold} \colorbox{red!39}{\strut Mail} \colorbox{red!22}{\strut Service} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!22}{\strut service} \colorbox{red!0}{\strut offered} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut persons} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut going} \colorbox{red!1}{\strut away} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut local} \colorbox{red!0}{\strut address} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut request} \colorbox{red!0}{\strut to} \colorbox{red!38}{\strut hold} \colorbox{red!0}{\strut their} \colorbox{red!39}{\strut mail} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut without} \colorbox{red!1}{\strut returning} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut sender} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut they} \colorbox{red!1}{\strut returns} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!93}{\strut MimeCast} \colorbox{red!0}{\strut ?} \colorbox{red!93}{\strut MimeCast} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut front-end} \colorbox{red!8}{\strut service} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut defense} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut e-mail} \colorbox{red!6}{\strut filtering} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut level} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut e-mails} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut act} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut our} \colorbox{red!0}{\strut archive} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut holding} \colorbox{red!0}{\strut e-mails} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is force fluids mean

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!47}{\strut Fluid} \colorbox{red!45}{\strut force} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!47}{\strut fluid} \colorbox{red!8}{\strut dynamics} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut description} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut theforce} \colorbox{red!0}{\strut applied} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut object} \colorbox{red!0}{\strut by} \colorbox{red!47}{\strut fluid} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut motion} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!24}{\strut Convection} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut classified} \colorbox{red!0}{\strut as} \colorbox{red!8}{\strut natural} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut or} \colorbox{red!4}{\strut free} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut and} \colorbox{red!10}{\strut forced} \colorbox{red!24}{\strut convection} \colorbox{red!1}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut fluid} \colorbox{red!2}{\strut motion} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut initiated} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!8}{\strut natural} \colorbox{red!24}{\strut convection} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut any} \colorbox{red!3}{\strut fluid} \colorbox{red!2}{\strut motion} \colorbox{red!0}{\strut is} \colorbox{red!6}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!8}{\strut natural} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut buoyancy} \colorbox{red!2}{\strut effect} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut i.e} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut rise} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut warmer} \colorbox{red!3}{\strut fluid} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut fall} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut cooler} \colorbox{red!3}{\strut fluid} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Whereas} \colorbox{red!0}{\strut in} \colorbox{red!10}{\strut forced} \colorbox{red!24}{\strut convection} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut fluid} \colorbox{red!0}{\strut is} \colorbox{red!10}{\strut forced} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut flow} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut surface} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tube} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut external} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pump} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut fan} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is elbaite

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!82}{\strut Elbaite} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut sodium} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut lithium} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut aluminium} \colorbox{red!0}{\strut boro-silicate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut chemical} \colorbox{red!9}{\strut composition} \colorbox{red!1}{\strut Na} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Li} \colorbox{red!0}{\strut 1.5} \colorbox{red!0}{\strut Al} \colorbox{red!0}{\strut 1.5} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut Al} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut Si} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut O} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut BO} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut OH} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut mineral} \colorbox{red!3}{\strut species} \colorbox{red!0}{\strut belonging} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut six-member} \colorbox{red!0}{\strut ring} \colorbox{red!0}{\strut cyclosilicate} \colorbox{red!0}{\strut tourmaline} \colorbox{red!3}{\strut group} \colorbox{red!0}{\strut .} \colorbox{red!82}{\strut Elbaite} \colorbox{red!0}{\strut forms} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut dravite} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut fluor-liddicoatite} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut schorl} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Dakota} \colorbox{red!1}{\strut Matrix} \colorbox{red!7}{\strut Minerals} \colorbox{red!1}{\strut Google} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut for} \colorbox{red!15}{\strut Elbaite} \colorbox{red!1}{\strut Excalibur} \colorbox{red!7}{\strut Mineral} \colorbox{red!0}{\strut Corp.} \colorbox{red!1}{\strut Google} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut for} \colorbox{red!15}{\strut Elbaite} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut Betts} \colorbox{red!0}{\strut Fine} \colorbox{red!7}{\strut Minerals} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut for} \colorbox{red!15}{\strut Elbaite} \colorbox{red!1}{\strut McDougall} \colorbox{red!7}{\strut Minerals} \colorbox{red!1}{\strut Google} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut for} \colorbox{red!15}{\strut Elbaite} \colorbox{red!7}{\strut Mineral} \colorbox{red!0}{\strut News} \colorbox{red!0}{\strut Website} \colorbox{red!0}{\strut Link} \colorbox{red!1}{\strut Rock} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut Mineral} \colorbox{red!0}{\strut Shows} \colorbox{red!1}{\strut Google} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut for} \colorbox{red!15}{\strut Elbaite} \colorbox{red!1}{\strut Weinrich} \colorbox{red!7}{\strut Minerals} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!1}{\strut Google} \colorbox{red!1}{\strut Search} \colorbox{red!0}{\strut for} \colorbox{red!15}{\strut Elbaite} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Ask} \colorbox{red!0}{\strut about} \colorbox{red!15}{\strut Elbaite} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut Ask-A-Mineralogist} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Mineralogical} \colorbox{red!0}{\strut Society} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut America} \colorbox{red!0}{\strut Mindat.org} \colorbox{red!0}{\strut 's} \colorbox{red!0}{\strut Discussion} \colorbox{red!0}{\strut Groups} \colorbox{red!0}{\strut Original} \colorbox{red!0}{\strut Rockhounds} \colorbox{red!0}{\strut Discussion} \colorbox{red!0}{\strut Group} \colorbox{red!0}{\strut Rockhounds} \colorbox{red!0}{\strut Discussion} \colorbox{red!0}{\strut Group} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut Yahoo} \colorbox{red!0}{\strut Groups} \colorbox{red!7}{\strut Mineral} \colorbox{red!0}{\strut Discussion} \colorbox{red!0}{\strut Forum} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Fabre} \colorbox{red!7}{\strut Minerals} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut available} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut EspaÃ±ol} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Print} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Cut-and-Paste} \colorbox{red!0}{\strut your} \colorbox{red!15}{\strut Elbaite} \colorbox{red!0}{\strut Specimen} \colorbox{red!0}{\strut Label} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut :} 
}}}
\end{CJK*}

query: what is considered the love apple

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!81}{\strut Love} \colorbox{red!83}{\strut apple} \colorbox{red!30}{\strut definition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tropical} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tender} \colorbox{red!4}{\strut plant} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Solanum} \colorbox{red!0}{\strut aculeatissimum} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nightshade} \colorbox{red!0}{\strut family} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut prickly} \colorbox{red!0}{\strut leaves} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut clusters} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut star-shaped} \colorbox{red!0}{\strut white} \colorbox{red!2}{\strut flowers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut red} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tomatolike} \colorbox{red!1}{\strut fruit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Answers.com} \colorbox{red!0}{\strut Â®} \colorbox{red!0}{\strut WikiAnswers} \colorbox{red!0}{\strut Â®} \colorbox{red!4}{\strut Categories} \colorbox{red!22}{\strut Food} \colorbox{red!0}{\strut \&} \colorbox{red!3}{\strut Cooking} \colorbox{red!28}{\strut Fruits} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut Vegetables} \colorbox{red!30}{\strut Apples} \colorbox{red!0}{\strut What} \colorbox{red!29}{\strut fruit} \colorbox{red!0}{\strut is} \colorbox{red!24}{\strut Known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!27}{\strut love} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!29}{\strut apple} \colorbox{red!0}{\strut ?} 
}}}
\end{CJK*}

query: composite object definition

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut In} \colorbox{red!13}{\strut programming} \colorbox{red!7}{\strut languages} \colorbox{red!0}{\strut ,} \colorbox{red!44}{\strut composite} \colorbox{red!28}{\strut objects} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut usually} \colorbox{red!1}{\strut expressed} \colorbox{red!0}{\strut by} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut references} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut one} \colorbox{red!33}{\strut object} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut language} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!2}{\strut references} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut attributes} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut fields} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut members} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut properties} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut resulting} \colorbox{red!2}{\strut composition} \colorbox{red!0}{\strut as} \colorbox{red!44}{\strut composite} \colorbox{red!3}{\strut type} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut storage} \colorbox{red!1}{\strut record} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut structure} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tuple} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut user-defined} \colorbox{red!3}{\strut type} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut UDT} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!38}{\strut Definition} \colorbox{red!0}{\strut :} \colorbox{red!80}{\strut Perspective} \colorbox{red!0}{\strut (} \colorbox{red!19}{\strut compositional} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut In} \colorbox{red!35}{\strut photography} \colorbox{red!0}{\strut âperspectiveâ} \colorbox{red!0}{\strut refers} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sense} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut width} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut height} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut depth} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut creates} \colorbox{red!0}{\strut three} \colorbox{red!5}{\strut dimensional} \colorbox{red!0}{\strut relationships} \colorbox{red!0}{\strut between} \colorbox{red!6}{\strut objects} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut photograph} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: why are clouds flat at the bottom

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!43}{\strut Clouds} \colorbox{red!0}{\strut are} \colorbox{red!28}{\strut flat} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!33}{\strut bottom} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut transition} \colorbox{red!1}{\strut point} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut temperature} \colorbox{red!0}{\strut \&} \colorbox{red!4}{\strut pressure} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut point} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut air} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut hold} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut 's} \colorbox{red!5}{\strut water} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut gaseous} \colorbox{red!1}{\strut form} \colorbox{red!0}{\strut (} \colorbox{red!43}{\strut clouds} \colorbox{red!0}{\strut are} \colorbox{red!7}{\strut made} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut water} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut liquid} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut solid} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut increase} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut altitude} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut temperature} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut atmospheric} \colorbox{red!4}{\strut pressure} \colorbox{red!0}{\strut decrease} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Before} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut why} \colorbox{red!34}{\strut clouds} \colorbox{red!0}{\strut are} \colorbox{red!15}{\strut flat} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!13}{\strut bottom} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut little} \colorbox{red!0}{\strut review} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut how} \colorbox{red!34}{\strut clouds} \colorbox{red!10}{\strut form} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut exactly} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut a} \colorbox{red!34}{\strut cloud} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut helpful} \colorbox{red!0}{\strut .} \colorbox{red!34}{\strut Clouds} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut condensed} \colorbox{red!3}{\strut water} \colorbox{red!3}{\strut vapor} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut atmosphere} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut liquid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut solid} \colorbox{red!10}{\strut form} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is baking chocolate

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!39}{\strut Baking} \colorbox{red!48}{\strut chocolate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut most} \colorbox{red!1}{\strut traditional} \colorbox{red!1}{\strut form} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut unsweetened} \colorbox{red!48}{\strut chocolate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut That} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut 's} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut percent} \colorbox{red!48}{\strut chocolate} \colorbox{red!3}{\strut liquor} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut aka} \colorbox{red!1}{\strut processed} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ground} \colorbox{red!2}{\strut cocoa} \colorbox{red!1}{\strut beans} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut added} \colorbox{red!2}{\strut sugar} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut flavoring} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut 's} \colorbox{red!0}{\strut extra} \colorbox{red!1}{\strut bitter} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut extra} \colorbox{red!0}{\strut unpleasant} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut bite} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!2}{\strut Best} \colorbox{red!28}{\strut chocolate} \colorbox{red!0}{\strut for} \colorbox{red!7}{\strut baking} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!23}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!7}{\strut unsweetened} \colorbox{red!0}{\strut ,} \colorbox{red!11}{\strut bittersweet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut semi-sweet} \colorbox{red!0}{\strut and} \colorbox{red!15}{\strut milk} \colorbox{red!28}{\strut chocolate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut what} \colorbox{red!3}{\strut type} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut baked} \colorbox{red!4}{\strut goods} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut ittersweet} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut semi-sweet} \colorbox{red!28}{\strut chocolate} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut varying} \colorbox{red!0}{\strut amounts} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut sugar} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut flavourings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut extra} \colorbox{red!0}{\strut cocoa} \colorbox{red!2}{\strut butter} \colorbox{red!0}{\strut added} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!28}{\strut chocolate} \colorbox{red!0}{\strut liquor} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Many} \colorbox{red!0}{\strut bakers} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut interchangeably} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is at the base of the aorta

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Name} \colorbox{red!0}{\strut the} \colorbox{red!39}{\strut valve} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!31}{\strut base} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!37}{\strut aorta} \colorbox{red!0}{\strut a.} \colorbox{red!2}{\strut Semilunar} \colorbox{red!39}{\strut valve} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Anti} \colorbox{red!2}{\strut backflow} \colorbox{red!38}{\strut valves} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut which} \colorbox{red!2}{\strut blood} \colorbox{red!1}{\strut vessels} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut the} \colorbox{red!17}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!23}{\strut artery} \colorbox{red!21}{\strut passing} \colorbox{red!21}{\strut inferiorly} \colorbox{red!2}{\strut from} \colorbox{red!2}{\strut the} \colorbox{red!12}{\strut base} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut ascending} \colorbox{red!12}{\strut aorta} \colorbox{red!2}{\strut and} \colorbox{red!16}{\strut following} \colorbox{red!2}{\strut the} \colorbox{red!14}{\strut course} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut the} \colorbox{red!8}{\strut sulcus} \colorbox{red!2}{\strut between} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut right} \colorbox{red!5}{\strut auricle} \colorbox{red!2}{\strut and} \colorbox{red!2}{\strut the} \colorbox{red!9}{\strut right} \colorbox{red!4}{\strut ventricle} \colorbox{red!0}{\strut ?} 
}}}
\end{CJK*}

query: why do neptune and uranus appear blue

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!28}{\strut Uranus} \colorbox{red!0}{\strut and} \colorbox{red!27}{\strut Neptune} \colorbox{red!25}{\strut appear} \colorbox{red!28}{\strut blue} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a.} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut atmospheres} \colorbox{red!2}{\strut absorb} \colorbox{red!28}{\strut blue} \colorbox{red!3}{\strut light} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut efficiently} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut b.} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut small} \colorbox{red!1}{\strut masses} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Jovian} \colorbox{red!14}{\strut planets} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut c.} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut surfaces} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut covered} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut water} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut clouds} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut thin} \colorbox{red!0}{\strut d.} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut atmospheres} \colorbox{red!2}{\strut absorb} \colorbox{red!0}{\strut red} \colorbox{red!3}{\strut light} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut efficiently} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut e.} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut wind} \colorbox{red!0}{\strut speeds} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut high} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut show} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut strong} \colorbox{red!28}{\strut blue} \colorbox{red!0}{\strut shift} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Why} \colorbox{red!0}{\strut do} \colorbox{red!28}{\strut Uranus} \colorbox{red!0}{\strut and} \colorbox{red!20}{\strut Neptune} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut characteristic} \colorbox{red!0}{\strut blue-green} \colorbox{red!27}{\strut color} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut Methane} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut their} \colorbox{red!2}{\strut atmosphere} \colorbox{red!2}{\strut absorbs} \colorbox{red!0}{\strut red} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut yellow} \colorbox{red!3}{\strut light} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Neptune} \colorbox{red!2}{\strut emits} \colorbox{red!0}{\strut more} \colorbox{red!2}{\strut energy} \colorbox{red!0}{\strut into} \colorbox{red!2}{\strut space} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut receives} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Sun} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut whereas} \colorbox{red!28}{\strut Uranus} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut What} \colorbox{red!2}{\strut visible} \colorbox{red!2}{\strut effect} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut appearance} \colorbox{red!0}{\strut of} \colorbox{red!20}{\strut Neptune} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut of} \colorbox{red!28}{\strut Uranus} \colorbox{red!0}{\strut ?} 
}}}
\end{CJK*}

query: what is a variable factor

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut a} \colorbox{red!30}{\strut variable} \colorbox{red!30}{\strut factor} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut experiment} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut change} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut control} \colorbox{red!30}{\strut factor} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut kept} \colorbox{red!0}{\strut constant} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut whole} \colorbox{red!4}{\strut experiment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!30}{\strut variable} \colorbox{red!30}{\strut factor} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!4}{\strut experiment} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut change} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut control} \colorbox{red!30}{\strut factor} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut kept} \colorbox{red!0}{\strut constant} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut whole} \colorbox{red!4}{\strut experiment} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!21}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut a} \colorbox{red!22}{\strut factor} \colorbox{red!0}{\strut and} \colorbox{red!19}{\strut variable} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!22}{\strut factor} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!9}{\strut experiment} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut controlled} \colorbox{red!2}{\strut independent} \colorbox{red!19}{\strut variable} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut a} \colorbox{red!19}{\strut variable} \colorbox{red!0}{\strut whose} \colorbox{red!0}{\strut the} \colorbox{red!21}{\strut differences} \colorbox{red!0}{\strut between} \colorbox{red!2}{\strut means} \colorbox{red!0}{\strut for} \colorbox{red!21}{\strut different} \colorbox{red!1}{\strut levels} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut one} \colorbox{red!22}{\strut factor} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Edit} \colorbox{red!0}{\strut Share} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut :} 
}}}
\end{CJK*}

query: what is a tag sale

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Those} \colorbox{red!0}{\strut Girls} \colorbox{red!0}{\strut '} \colorbox{red!20}{\strut Tag} \colorbox{red!0}{\strut \&} \colorbox{red!4}{\strut Estate} \colorbox{red!20}{\strut Sale} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Lincoln} \colorbox{red!0}{\strut NE} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Tag} \colorbox{red!20}{\strut Sale} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut A} \colorbox{red!20}{\strut sale} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut second-hand} \colorbox{red!1}{\strut items} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut estate} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut moving} \colorbox{red!20}{\strut sale} \colorbox{red!0}{\strut where} \colorbox{red!1}{\strut items} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut tagged/priced} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut displayed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut house} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Tag} \colorbox{red!20}{\strut Sale} \colorbox{red!1}{\strut Procedure} \colorbox{red!0}{\strut :} \colorbox{red!1}{\strut Customers} \colorbox{red!0}{\strut pick} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut number} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut front} \colorbox{red!0}{\strut door} \colorbox{red!0}{\strut before} \colorbox{red!0}{\strut the} \colorbox{red!20}{\strut sale} \colorbox{red!0}{\strut starts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 2} \colorbox{red!1}{\strut numbers} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut handed} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut individual} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut spouse} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut 20-25} \colorbox{red!1}{\strut customers} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut numbers} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut home} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut shop} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut customers} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut numerical} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut every} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut minutes} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Category} \colorbox{red!0}{\strut :} \colorbox{red!13}{\strut Jamberry} \colorbox{red!13}{\strut Nails} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tagged} \colorbox{red!0}{\strut :} \colorbox{red!13}{\strut jamberry} \colorbox{red!13}{\strut nail} \colorbox{red!4}{\strut shields} \colorbox{red!0}{\strut ,} \colorbox{red!13}{\strut jamberry} \colorbox{red!13}{\strut nails} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut new} \colorbox{red!1}{\strut direct} \colorbox{red!1}{\strut sales} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut are} \colorbox{red!13}{\strut jamberry} \colorbox{red!13}{\strut nail} \colorbox{red!4}{\strut shields} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut are} \colorbox{red!13}{\strut jamberry} \colorbox{red!13}{\strut nails} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut is} \colorbox{red!13}{\strut jamberry} \colorbox{red!13}{\strut nails} \colorbox{red!0}{\strut .} \colorbox{red!13}{\strut Jamberry} \colorbox{red!13}{\strut Nails} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut newest} \colorbox{red!1}{\strut direct} \colorbox{red!1}{\strut sales} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut 's} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut launched} \colorbox{red!0}{\strut nationally} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is a preliminary source

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut The} \colorbox{red!25}{\strut preliminary} \colorbox{red!14}{\strut source} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut mom} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut name} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!19}{\strut author} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut s} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut [} \colorbox{red!0}{\strut if} \colorbox{red!1}{\strut available} \colorbox{red!0}{\strut ]} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut followed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut period} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut last} \colorbox{red!7}{\strut name} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut first} \colorbox{red!7}{\strut name} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut second} \colorbox{red!19}{\strut author} \colorbox{red!0}{\strut 's} \colorbox{red!7}{\strut name} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!3}{\strut inverted} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .The} \colorbox{red!8}{\strut title} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut article} \colorbox{red!0}{\strut or} \colorbox{red!1}{\strut section} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut site.â¦} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut in} \colorbox{red!21}{\strut quotation} \colorbox{red!4}{\strut marks} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut followed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut period} \colorbox{red!0}{\strut placed} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!21}{\strut quotation} \colorbox{red!4}{\strut marks} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut The} \colorbox{red!8}{\strut title} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut website} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut After} \colorbox{red!5}{\strut connecting} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut power} \colorbox{red!5}{\strut source} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!16}{\strut PDC} \colorbox{red!0}{\strut you} \colorbox{red!3}{\strut conduct} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut preliminary} \colorbox{red!18}{\strut test} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut find} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!27}{\strut voltage} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!36}{\strut B} \colorbox{red!36}{\strut phase} \colorbox{red!18}{\strut test} \colorbox{red!4}{\strut point} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut next} \colorbox{red!6}{\strut step} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut document} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut discrepancy} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut refer} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut T.O} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Edit} 
}}}
\end{CJK*}

query: what is a pedicle flap

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!44}{\strut pedicle} \colorbox{red!45}{\strut flap} \colorbox{red!0}{\strut a} \colorbox{red!45}{\strut flap} \colorbox{red!0}{\strut consisting} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut full} \colorbox{red!0}{\strut thickness} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut skin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut subcutaneous} \colorbox{red!2}{\strut tissue} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut attached} \colorbox{red!0}{\strut by} \colorbox{red!2}{\strut tissue} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut it} \colorbox{red!1}{\strut receives} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut blood} \colorbox{red!0}{\strut supply} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut rope} \colorbox{red!45}{\strut flap} \colorbox{red!0}{\strut one} \colorbox{red!1}{\strut made} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut elevating} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut long} \colorbox{red!1}{\strut strip} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut tissue} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut bed} \colorbox{red!0}{\strut except} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut ends} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut cut} \colorbox{red!0}{\strut edges} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut being} \colorbox{red!1}{\strut sutured} \colorbox{red!0}{\strut together} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tube} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!12}{\strut Flaps} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut Skin} \colorbox{red!0}{\strut and/or} \colorbox{red!2}{\strut Deep} \colorbox{red!6}{\strut Tissue} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut Whatâs} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut major} \colorbox{red!11}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut adjacent} \colorbox{red!6}{\strut tissue} \colorbox{red!3}{\strut transfer} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut pedicle} \colorbox{red!12}{\strut flap} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut an} \colorbox{red!6}{\strut adjacent} \colorbox{red!6}{\strut tissue} \colorbox{red!3}{\strut transfer} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut flap} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut developed} \colorbox{red!0}{\strut immediately} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut defect} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut then} \colorbox{red!1}{\strut rotated} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut advanced} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut that} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!12}{\strut pedicle} \colorbox{red!12}{\strut flap} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut developed} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut an} \colorbox{red!1}{\strut area} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut short} \colorbox{red!1}{\strut distance} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut defect} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut once} \colorbox{red!1}{\strut elevated} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut flap} \colorbox{red!0}{\strut remains} \colorbox{red!1}{\strut attached} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut pedicle} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut maintains} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut blood} \colorbox{red!0}{\strut supply} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut that} \colorbox{red!12}{\strut flap} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut keep} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut viable} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Once} \colorbox{red!0}{\strut the} \colorbox{red!12}{\strut pedicle} \colorbox{red!12}{\strut flap} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!3}{\strut transferred} \colorbox{red!0}{\strut into} \colorbox{red!1}{\strut wound} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut sutured} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what is a composite dental procedure

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!30}{\strut dental} \colorbox{red!47}{\strut composite} \colorbox{red!38}{\strut procedure} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut variety} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut reasons} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut cosmetic} \colorbox{red!1}{\strut reasons} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut fix} \colorbox{red!0}{\strut a} \colorbox{red!12}{\strut tooth} \colorbox{red!1}{\strut structure} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut severely} \colorbox{red!2}{\strut decayed} \colorbox{red!12}{\strut tooth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut help} \colorbox{red!1}{\strut bond} \colorbox{red!12}{\strut tooth} \colorbox{red!1}{\strut veneers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut closing} \colorbox{red!0}{\strut a} \colorbox{red!30}{\strut dental} \colorbox{red!0}{\strut gap} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut fillings} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut correct} \colorbox{red!0}{\strut minor} \colorbox{red!3}{\strut cosmetic} \colorbox{red!0}{\strut imperfections} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut patients} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut worry} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut bit} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut the} \colorbox{red!17}{\strut cosmetic} \colorbox{red!27}{\strut dental} \colorbox{red!43}{\strut bonding} \colorbox{red!13}{\strut procedure} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut what} \colorbox{red!4}{\strut patients} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut forward} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut strong} \colorbox{red!5}{\strut composite} \colorbox{red!8}{\strut resin} \colorbox{red!10}{\strut material} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut placed} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut front} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut back} \colorbox{red!18}{\strut teeth} \colorbox{red!0}{\strut dr} \colorbox{red!0}{\strut leo} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut apply} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut thin} \colorbox{red!5}{\strut coating} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut composite} \colorbox{red!8}{\strut resin} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut front} \colorbox{red!0}{\strut surface} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut problem} \colorbox{red!14}{\strut tooth} 
}}}
\end{CJK*}

query: what does wintergreen blend well with

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!86}{\strut Wintergreen} \colorbox{red!6}{\strut blends} \colorbox{red!0}{\strut nicely} \colorbox{red!0}{\strut with} \colorbox{red!12}{\strut Ravensara} \colorbox{red!0}{\strut and/or} \colorbox{red!8}{\strut Eucalyptus} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!3}{\strut effect} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!2}{\strut pale} \colorbox{red!7}{\strut yellow} \colorbox{red!68}{\strut oil} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut intense} \colorbox{red!0}{\strut sweet-woody} \colorbox{red!1}{\strut aroma} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!3}{\strut diluted} \colorbox{red!0}{\strut significantly} \colorbox{red!0}{\strut before} \colorbox{red!2}{\strut topical} \colorbox{red!0}{\strut application} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fine} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut formulas} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut supporting} \colorbox{red!0}{\strut joint} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut muscular} \colorbox{red!0}{\strut aches} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut pains} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut CHEMICAL} \colorbox{red!3}{\strut CONSTITUENTS} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut main} \colorbox{red!9}{\strut chemical} \colorbox{red!3}{\strut components} \colorbox{red!0}{\strut of} \colorbox{red!19}{\strut wintergreen} \colorbox{red!18}{\strut oil} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut menthyl} \colorbox{red!1}{\strut salicylate} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut gaultherilene} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut PRECAUTIONS} \colorbox{red!0}{\strut :} \colorbox{red!19}{\strut Wintergreen} \colorbox{red!18}{\strut oil} \colorbox{red!0}{\strut is} \colorbox{red!5}{\strut toxic} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut taken} \colorbox{red!0}{\strut internally} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut fatal} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut BLENDS} \colorbox{red!0}{\strut :} \colorbox{red!2}{\strut Blends} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut Oregano} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Peppermint} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Thyme} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Cajuput} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Eucalyptus} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Niaoli} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Ylang} \colorbox{red!0}{\strut Ylang} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut suggested} \colorbox{red!0}{\strut that} \colorbox{red!19}{\strut Wintergreen} \colorbox{red!18}{\strut Oil} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Aromatherapy} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut highly} \colorbox{red!5}{\strut toxic} \colorbox{red!2}{\strut properties} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut many} \colorbox{red!2}{\strut Essential} \colorbox{red!18}{\strut Oils} \colorbox{red!0}{\strut .} \colorbox{red!19}{\strut wintergreen} 
}}}
\end{CJK*}

query: what does unlock my device mean

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!66}{\strut Unlocking} \colorbox{red!0}{\strut a} \colorbox{red!56}{\strut device} \colorbox{red!1}{\strut refers} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut disabling} \colorbox{red!7}{\strut software} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut would} \colorbox{red!2}{\strut prevent} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut consumer} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut attempting} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut activate} \colorbox{red!0}{\strut a} \colorbox{red!56}{\strut device} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut provider} \colorbox{red!0}{\strut 's} \colorbox{red!2}{\strut network} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut provider} \colorbox{red!0}{\strut 's} \colorbox{red!2}{\strut network} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut that} \colorbox{red!2}{\strut network} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut technologically} \colorbox{red!0}{\strut compatible} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut Does} \colorbox{red!45}{\strut Jailbreaking} \colorbox{red!39}{\strut Mean} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Why} \colorbox{red!0}{\strut Should} \colorbox{red!0}{\strut I} \colorbox{red!43}{\strut Jailbreak} \colorbox{red!0}{\strut My} \colorbox{red!7}{\strut iPhone} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut iPod} \colorbox{red!4}{\strut Touch} \colorbox{red!0}{\strut ,} \colorbox{red!6}{\strut iPad} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Everything} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut Know} \colorbox{red!0}{\strut About} \colorbox{red!45}{\strut Jailbreaking} \colorbox{red!0}{\strut And} \colorbox{red!6}{\strut Unlocking} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut November} \colorbox{red!0}{\strut 25} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2009} \colorbox{red!0}{\strut By} \colorbox{red!0}{\strut Jaden} \colorbox{red!0}{\strut Easton-Ellett} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut Comments} 
}}}
\end{CJK*}

query: what does the bank for international settlements help

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!39}{\strut Bank} \colorbox{red!0}{\strut for} \colorbox{red!41}{\strut International} \colorbox{red!43}{\strut Settlements} \colorbox{red!0}{\strut would} \colorbox{red!2}{\strut act} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut lender} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut German} \colorbox{red!3}{\strut central} \colorbox{red!39}{\strut bank} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut case} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut German} \colorbox{red!3}{\strut currency} \colorbox{red!0}{\strut weakened} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut government} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut itself} \colorbox{red!0}{\strut unable} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut make} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut reparations} \colorbox{red!2}{\strut payment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut give} \colorbox{red!0}{\strut steps} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut proceed} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut case} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut German} \colorbox{red!1}{\strut default} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!20}{\strut difference} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut a} \colorbox{red!22}{\strut correspondent} \colorbox{red!18}{\strut bank} \colorbox{red!0}{\strut and} \colorbox{red!21}{\strut intermediary} \colorbox{red!18}{\strut bank} \colorbox{red!0}{\strut ?} \colorbox{red!22}{\strut Correspondent} \colorbox{red!0}{\strut and} \colorbox{red!21}{\strut intermediary} \colorbox{red!19}{\strut banks} \colorbox{red!0}{\strut serve} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut third-party} \colorbox{red!19}{\strut banks} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut coordinate} \colorbox{red!0}{\strut with} \colorbox{red!2}{\strut beneficiary} \colorbox{red!19}{\strut banks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut facilitate} \colorbox{red!1}{\strut international} \colorbox{red!0}{\strut fund} \colorbox{red!0}{\strut transfers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut transaction} \colorbox{red!0}{\strut settlements} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what does conservatorship mean in real estate?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!48}{\strut conservatorship} \colorbox{red!9}{\strut estate} \colorbox{red!5}{\strut assets} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut typically} \colorbox{red!2}{\strut invested} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut produce} \colorbox{red!7}{\strut income} \colorbox{red!0}{\strut sufficient} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut care} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut minor} \colorbox{red!0}{\strut 's} \colorbox{red!1}{\strut needs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut likely} \colorbox{red!3}{\strut require} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!45}{\strut conservator} \colorbox{red!0}{\strut must} \colorbox{red!3}{\strut prepare} \colorbox{red!0}{\strut and} \colorbox{red!10}{\strut file} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut yearly} \colorbox{red!7}{\strut income} \colorbox{red!13}{\strut tax} \colorbox{red!9}{\strut return} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut behalf} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut minor} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut pay} \colorbox{red!0}{\strut any} \colorbox{red!12}{\strut taxes} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!3}{\strut due} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut does} \colorbox{red!74}{\strut REIT} \colorbox{red!51}{\strut stand} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut It} \colorbox{red!14}{\strut means} \colorbox{red!8}{\strut Real} \colorbox{red!8}{\strut Estate} \colorbox{red!6}{\strut Investment} \colorbox{red!7}{\strut Trust} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut entity} \colorbox{red!0}{\strut designed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut serve} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut interests} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut group} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut real} \colorbox{red!8}{\strut estate} \colorbox{red!5}{\strut investors} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: cat torque converter replacement cost

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!28}{\strut replacement} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!60}{\strut torque} \colorbox{red!56}{\strut converter} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut both} \colorbox{red!2}{\strut parts} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut labor} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut anywhere} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 500} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 1,000} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut hand} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut relatively} \colorbox{red!0}{\strut inexpensive} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut only} \colorbox{red!52}{\strut cost} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 150} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 450} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut depending} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut vehicle} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut It} \colorbox{red!0}{\strut will} \colorbox{red!14}{\strut cost} \colorbox{red!0}{\strut approximately} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 520} \colorbox{red!0}{\strut to} \colorbox{red!8}{\strut replace} \colorbox{red!0}{\strut the} \colorbox{red!16}{\strut torque} \colorbox{red!16}{\strut converter} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!11}{\strut Lexus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!16}{\strut torque} \colorbox{red!16}{\strut converter} \colorbox{red!0}{\strut will} \colorbox{red!14}{\strut cost} \colorbox{red!0}{\strut approximately} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 160} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut require} \colorbox{red!0}{\strut six} \colorbox{red!0}{\strut hours} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut labor} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut install} \colorbox{red!0}{\strut .} \colorbox{red!16}{\strut torque} \colorbox{red!16}{\strut converter} \colorbox{red!0}{\strut can} \colorbox{red!14}{\strut cost} \colorbox{red!0}{\strut anywhere} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 129} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 249} \colorbox{red!0}{\strut dollars} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!16}{\strut torque} \colorbox{red!16}{\strut converter} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut allows} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut transmission} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut shift} \colorbox{red!1}{\strut gears} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what do you learn in nursing school

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut In} \colorbox{red!39}{\strut nursing} \colorbox{red!29}{\strut school} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut 'll} \colorbox{red!3}{\strut learn} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut history} \colorbox{red!0}{\strut of} \colorbox{red!39}{\strut nursing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut plethora} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut disease} \colorbox{red!0}{\strut processes} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lifespan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pharmacology} \colorbox{red!0}{\strut ,} \colorbox{red!39}{\strut nursing} \colorbox{red!7}{\strut skills} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut do} \colorbox{red!39}{\strut nursing} \colorbox{red!0}{\strut procedures} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut talk} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut patients} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut therapeutic} \colorbox{red!0}{\strut manner} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut a} \colorbox{red!36}{\strut Nurse} \colorbox{red!27}{\strut Technician} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut How} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut Become} \colorbox{red!0}{\strut a} \colorbox{red!36}{\strut Nurse} \colorbox{red!23}{\strut Tech} \colorbox{red!0}{\strut ?} \colorbox{red!2}{\strut Learn} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut education} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut preparation} \colorbox{red!0}{\strut needed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut a} \colorbox{red!36}{\strut nurse} \colorbox{red!27}{\strut technician} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Get} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut quick} \colorbox{red!0}{\strut view} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut requirements} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut details} \colorbox{red!0}{\strut about} \colorbox{red!2}{\strut schooling} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut job} \colorbox{red!0}{\strut duties} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut registration} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut career} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Essential} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what causes the li

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!47}{\strut Causes} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Li-Fraumeni} \colorbox{red!44}{\strut syndrome} \colorbox{red!0}{\strut Li-Fraumeni} \colorbox{red!44}{\strut syndrome} \colorbox{red!0}{\strut is} \colorbox{red!47}{\strut caused} \colorbox{red!0}{\strut by} \colorbox{red!5}{\strut mutations} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut TP53} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut CHEK2} \colorbox{red!2}{\strut genes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut both} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut produce} \colorbox{red!2}{\strut tumor} \colorbox{red!0}{\strut suppressor} \colorbox{red!2}{\strut genes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!5}{\strut mutations} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut uncontrolled} \colorbox{red!0}{\strut growth} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut cells} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut tumors} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut BU-808} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!10}{\strut Prolong} \colorbox{red!0}{\strut Lithium-based} \colorbox{red!32}{\strut Batteries} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Discover} \colorbox{red!0}{\strut what} \colorbox{red!8}{\strut causes} \colorbox{red!0}{\strut Li-ion} \colorbox{red!0}{\strut to} \colorbox{red!8}{\strut age} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut the} \colorbox{red!32}{\strut battery} \colorbox{red!0}{\strut user} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut to} \colorbox{red!10}{\strut prolong} \colorbox{red!0}{\strut its} \colorbox{red!4}{\strut life} \colorbox{red!0}{\strut .} \colorbox{red!32}{\strut Battery} \colorbox{red!0}{\strut research} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut focusing} \colorbox{red!0}{\strut on} \colorbox{red!14}{\strut lithium} \colorbox{red!3}{\strut chemistries} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut imagine} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut the} \colorbox{red!32}{\strut battery} \colorbox{red!0}{\strut future} \colorbox{red!0}{\strut lies} \colorbox{red!0}{\strut solely} \colorbox{red!0}{\strut in} \colorbox{red!14}{\strut lithium} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: what are the signs of kidney failure in dogs with dm?

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut PetMD} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut common} \colorbox{red!6}{\strut signs} \colorbox{red!0}{\strut of} \colorbox{red!53}{\strut kidney} \colorbox{red!45}{\strut failure} \colorbox{red!0}{\strut in} \colorbox{red!48}{\strut dogs} \colorbox{red!0}{\strut include} \colorbox{red!1}{\strut depression} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lethargy} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut lack} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut appetite} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut vomiting} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut diarrhea} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut constipation} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut weight} \colorbox{red!0}{\strut loss} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Other} \colorbox{red!43}{\strut symptoms} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut increased} \colorbox{red!0}{\strut thirst} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ...} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut But} \colorbox{red!0}{\strut surprisingly} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut main} \colorbox{red!22}{\strut cause} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut chronic} \colorbox{red!24}{\strut kidney} \colorbox{red!13}{\strut failure} \colorbox{red!0}{\strut in} \colorbox{red!23}{\strut dogs} \colorbox{red!0}{\strut is} \colorbox{red!3}{\strut dental} \colorbox{red!2}{\strut disease} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Bacteria} \colorbox{red!0}{\strut associated} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut advanced} \colorbox{red!3}{\strut dental} \colorbox{red!2}{\strut disease} \colorbox{red!0}{\strut enter} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut blood} \colorbox{red!0}{\strut stream} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut invades} \colorbox{red!0}{\strut multiple} \colorbox{red!2}{\strut organs} \colorbox{red!0}{\strut ,} \colorbox{red!22}{\strut causing} \colorbox{red!0}{\strut irreversible} \colorbox{red!2}{\strut damage} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut heart} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut liver} \colorbox{red!0}{\strut and} \colorbox{red!23}{\strut kidneys} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut Are} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut Signs} \colorbox{red!0}{\strut of} \colorbox{red!24}{\strut Kidney} \colorbox{red!3}{\strut Problems} \colorbox{red!0}{\strut in} \colorbox{red!23}{\strut Dogs} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut â¢} \colorbox{red!0}{\strut Change} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut water} \colorbox{red!0}{\strut consumption} 
}}}
\end{CJK*}

query: what are the road c

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut C-ROADS} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut free} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut award-winning} \colorbox{red!38}{\strut computer} \colorbox{red!85}{\strut simulator} \colorbox{red!0}{\strut that} \colorbox{red!4}{\strut helps} \colorbox{red!0}{\strut people} \colorbox{red!8}{\strut understand} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut long-term} \colorbox{red!19}{\strut climate} \colorbox{red!0}{\strut impacts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut actions} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut reduce} \colorbox{red!8}{\strut greenhouse} \colorbox{red!0}{\strut gas} \colorbox{red!4}{\strut emissions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut rapidly} \colorbox{red!0}{\strut test} \colorbox{red!0}{\strut strategies} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut tackling} \colorbox{red!19}{\strut climate} \colorbox{red!12}{\strut change} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!64}{\strut main} \colorbox{red!62}{\strut goal} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!65}{\strut Crusades} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut open} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Silk} \colorbox{red!0}{\strut Roads} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut traders} \colorbox{red!0}{\strut B} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!4}{\strut take} \colorbox{red!0}{\strut Mecca} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Islamic} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut C.} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut save} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Byzantine} \colorbox{red!0}{\strut Empire} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut invaders} \colorbox{red!0}{\strut D.} \colorbox{red!0}{\strut To} \colorbox{red!4}{\strut take} \colorbox{red!0}{\strut ...} 
}}}
\end{CJK*}

query: what are hcp

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!124}{\strut HCP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Inc.} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut real} \colorbox{red!8}{\strut estate} \colorbox{red!4}{\strut investment} \colorbox{red!6}{\strut trust} \colorbox{red!0}{\strut which} \colorbox{red!3}{\strut invests} \colorbox{red!0}{\strut primarily} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut real} \colorbox{red!8}{\strut estate} \colorbox{red!0}{\strut serving} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut healthcare} \colorbox{red!0}{\strut industry} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut States} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut acquires} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut develops} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut leases} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sells} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut manages} \colorbox{red!5}{\strut healthcare} \colorbox{red!8}{\strut real} \colorbox{red!8}{\strut estate} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut provides} \colorbox{red!0}{\strut mortgage} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!3}{\strut financing} \colorbox{red!0}{\strut to} \colorbox{red!5}{\strut healthcare} \colorbox{red!0}{\strut providers} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!15}{\strut goal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut stated} \colorbox{red!0}{\strut by} \colorbox{red!54}{\strut HCP} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut to} \colorbox{red!5}{\strut create} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut portfolio} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut stable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut high-quality} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut private-pay} \colorbox{red!10}{\strut assets} \colorbox{red!0}{\strut .} \colorbox{red!54}{\strut HCP} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut previously} \colorbox{red!0}{\strut estimated} \colorbox{red!0}{\strut what} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut post-spinoff} \colorbox{red!6}{\strut portfolio} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut look} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut sure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!16}{\strut company} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut 800} \colorbox{red!9}{\strut properties} \colorbox{red!0}{\strut spread} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut 43} \colorbox{red!9}{\strut states} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 94} \colorbox{red!0}{\strut \%} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut private-pay} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut read} \colorbox{red!0}{\strut :} \colorbox{red!8}{\strut stable} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: the function of the olfactory nerve concerns

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!11}{\strut Function} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!20}{\strut Olfactory} \colorbox{red!21}{\strut Nerve} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!20}{\strut olfactory} \colorbox{red!21}{\strut nerve} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut responsible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut sense} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut smell} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut partially} \colorbox{red!4}{\strut responsible} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut your} \colorbox{red!2}{\strut sense} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut taste} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!2}{\strut cranial} \colorbox{red!21}{\strut nerve} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut shortest} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut cranial} \colorbox{red!21}{\strut nerves} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut two} \colorbox{red!21}{\strut nerves} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut optic} \colorbox{red!21}{\strut nerve} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut bypass} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut brain} \colorbox{red!0}{\strut stem} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut connect} \colorbox{red!0}{\strut directly} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut brain} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!19}{\strut olfactory} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut pertaining} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut smell} \colorbox{red!0}{\strut .} \colorbox{red!19}{\strut olfactory} \colorbox{red!3}{\strut nerve} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut cranial} \colorbox{red!3}{\strut nerve} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut purely} \colorbox{red!1}{\strut sensory} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut concerned} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut sense} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut smell} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut nerve} \colorbox{red!2}{\strut cell} \colorbox{red!0}{\strut bodies} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut situated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!19}{\strut olfactory} \colorbox{red!2}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut mucous} \colorbox{red!1}{\strut membrane} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut nose.lfactory} \colorbox{red!2}{\strut system} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut includes} \colorbox{red!0}{\strut the} \colorbox{red!19}{\strut olfactory} \colorbox{red!2}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut nasal} \colorbox{red!2}{\strut mucosa} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!19}{\strut olfactory} \colorbox{red!3}{\strut nerves} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!19}{\strut olfactory} \colorbox{red!1}{\strut bulbs} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut cerebrum} \colorbox{red!0}{\strut .} \colorbox{red!19}{\strut olfactory} \colorbox{red!2}{\strut tract} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut band} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut white} \colorbox{red!3}{\strut nerve} \colorbox{red!0}{\strut fibers} \colorbox{red!0}{\strut visible} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ventral} \colorbox{red!0}{\strut surface} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut brain} \colorbox{red!0}{\strut running} \colorbox{red!0}{\strut caudally} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!19}{\strut olfactory} \colorbox{red!1}{\strut bulbs} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: sore synonyms

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!100}{\strut sore} \colorbox{red!0}{\strut |} \colorbox{red!86}{\strut synonyms} \colorbox{red!0}{\strut :} \colorbox{red!3}{\strut aching} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut acute} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut aggravating} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut agonizing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut anguishing} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut annoying} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut arduous} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut besetting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut biting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut bitter} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut bothersome} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut burdensome} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cramping} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cruel} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut crushing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cutting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut disagreeable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut distressful} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut excruciating} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut gnawing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut grievous} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut grueling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut harrowing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut horrendous} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut hurtful} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut inflaming} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut insufferable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut irksome} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut irritating} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut miserable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut odious} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut offensive} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut oppressive} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut painful} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut piercing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut severe} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut stabbing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut stinging} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut throbbing} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut tormenting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut torturing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut troublesome} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut trying} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut unbearable} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut uncomfortable} \colorbox{red!0}{\strut ...} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!20}{\strut Synonyms} \colorbox{red!0}{\strut for} \colorbox{red!21}{\strut sore} \colorbox{red!21}{\strut loser} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!1}{\strut thesaurus} \colorbox{red!0}{\strut page} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut possible} \colorbox{red!20}{\strut synonyms} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut equivalent} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut same} \colorbox{red!3}{\strut meaning} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut similar} \colorbox{red!2}{\strut words} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut term} \colorbox{red!21}{\strut sore} \colorbox{red!21}{\strut loser} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut n't} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut direct} \colorbox{red!20}{\strut synonyms} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut term} \colorbox{red!21}{\strut sore} \colorbox{red!21}{\strut loser} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: qualify definition

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!36}{\strut Definition} \colorbox{red!0}{\strut of} \colorbox{red!62}{\strut qualify} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut entitled} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut particular} \colorbox{red!1}{\strut benefit} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut privilege} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut fulfilling} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut necessary} \colorbox{red!0}{\strut condition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut officially} \colorbox{red!0}{\strut recognized} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut practition} \colorbox{red!36}{\strut Definition} \colorbox{red!0}{\strut of} \colorbox{red!62}{\strut qualify} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut entitled} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut particular} \colorbox{red!1}{\strut benefit} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut privilege} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut fulfilling} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut necessary} \colorbox{red!0}{\strut condition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut officially} \colorbox{red!0}{\strut recognized} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut practition} \colorbox{red!0}{\strut dictionary} \colorbox{red!0}{\strut thesaurus} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!17}{\strut Definition} \colorbox{red!0}{\strut of} \colorbox{red!32}{\strut qualify} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Definitions.net} \colorbox{red!5}{\strut dictionary} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Meaning} \colorbox{red!0}{\strut of} \colorbox{red!32}{\strut qualify} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut does} \colorbox{red!32}{\strut qualify} \colorbox{red!14}{\strut mean} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut translations} \colorbox{red!0}{\strut of} \colorbox{red!32}{\strut qualify} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut comprehensive} \colorbox{red!5}{\strut dictionary} \colorbox{red!18}{\strut definitions} \colorbox{red!0}{\strut resource} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut web} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: product level activity define

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Product-level} \colorbox{red!36}{\strut activity} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut called} \colorbox{red!0}{\strut product-sustaining} \colorbox{red!36}{\strut activity} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut service-sustaining} \colorbox{red!36}{\strut activity} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!36}{\strut activity} \colorbox{red!1}{\strut performed} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut support} \colorbox{red!2}{\strut production} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut specific} \colorbox{red!45}{\strut product} \colorbox{red!0}{\strut or} \colorbox{red!6}{\strut service} \colorbox{red!0}{\strut regardless} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut batches} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut run} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut produced} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!4}{\strut Define} \colorbox{red!0}{\strut :} \colorbox{red!25}{\strut Flexible} \colorbox{red!26}{\strut Budget} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!25}{\strut flexible} \colorbox{red!26}{\strut budget} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!26}{\strut budget} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!2}{\strut adjusted} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut any} \colorbox{red!2}{\strut activity} \colorbox{red!2}{\strut level} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut shows} \colorbox{red!0}{\strut how} \colorbox{red!3}{\strut costs} \colorbox{red!0}{\strut vary} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut volume} \colorbox{red!0}{\strut .} \colorbox{red!26}{\strut Budgeted} \colorbox{red!2}{\strut Total} \colorbox{red!3}{\strut Costs} \colorbox{red!0}{\strut =} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut Variable} \colorbox{red!2}{\strut Cost} \colorbox{red!0}{\strut per} \colorbox{red!2}{\strut unit} \colorbox{red!0}{\strut x} \colorbox{red!2}{\strut activity} \colorbox{red!2}{\strut level} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut +} \colorbox{red!2}{\strut fixed} \colorbox{red!3}{\strut costs} \colorbox{red!2}{\strut Fixed} \colorbox{red!3}{\strut costs} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut total} \colorbox{red!0}{\strut are} \colorbox{red!2}{\strut constant} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut relevant} \colorbox{red!0}{\strut range} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut activity} \colorbox{red!2}{\strut level} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut î} \colorbox{red!0}{\strut î} \colorbox{red!0}{\strut î} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: population of greater concepcion, chile

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut concepcion.cl} \colorbox{red!0}{\strut Satellite} \colorbox{red!0}{\strut image} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Greater} \colorbox{red!0}{\strut ConcepciÃ³n} \colorbox{red!3}{\strut Gran} \colorbox{red!0}{\strut ConcepciÃ³n} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut second} \colorbox{red!17}{\strut largest} \colorbox{red!18}{\strut conurbation} \colorbox{red!0}{\strut in} \colorbox{red!113}{\strut Chile} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut after} \colorbox{red!2}{\strut Greater} \colorbox{red!5}{\strut Santiago} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut 945,650} \colorbox{red!38}{\strut inhabitants} \colorbox{red!0}{\strut according} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 2012} \colorbox{red!0}{\strut pre} \colorbox{red!0}{\strut census} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut ConcepciÃ³n} \colorbox{red!4}{\strut lies} \colorbox{red!0}{\strut in} \colorbox{red!6}{\strut Central} \colorbox{red!51}{\strut Chile} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 500} \colorbox{red!0}{\strut kilometres} \colorbox{red!0}{\strut south} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut capital} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut Santiago} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!8}{\strut city} \colorbox{red!0}{\strut sits} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut larger} \colorbox{red!0}{\strut urban} \colorbox{red!4}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Greater} \colorbox{red!10}{\strut Concepcion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut a} \colorbox{red!22}{\strut population} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1,026,425} \colorbox{red!0}{\strut reside} \colorbox{red!0}{\strut across} \colorbox{red!0}{\strut 10} \colorbox{red!13}{\strut municipalities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 11th} \colorbox{red!6}{\strut largest} \colorbox{red!13}{\strut municipality} \colorbox{red!0}{\strut in} \colorbox{red!51}{\strut Chile} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ConcepciÃ³n} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut home} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 231,233} \colorbox{red!5}{\strut people} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: barbados: history definition

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!127}{\strut Barbados} \colorbox{red!61}{\strut definition} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut an} \colorbox{red!7}{\strut island} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut E} \colorbox{red!0}{\strut West} \colorbox{red!0}{\strut Indies} \colorbox{red!0}{\strut constituting} \colorbox{red!0}{\strut an} \colorbox{red!3}{\strut independent} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Commonwealth} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Nations} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut formerly} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut British} \colorbox{red!1}{\strut colony} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 166} \colorbox{red!0}{\strut sq} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut 430} \colorbox{red!0}{\strut sq} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Dictionary.com} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!18}{\strut Eat} \colorbox{red!0}{\strut \&} \colorbox{red!18}{\strut Drink} \colorbox{red!0}{\strut .} \colorbox{red!18}{\strut Eat} \colorbox{red!0}{\strut \&} \colorbox{red!18}{\strut Drink} \colorbox{red!0}{\strut in} \colorbox{red!19}{\strut Barbados} \colorbox{red!0}{\strut .} \colorbox{red!18}{\strut Eat} \colorbox{red!0}{\strut and} \colorbox{red!18}{\strut Drink} \colorbox{red!0}{\strut in} \colorbox{red!19}{\strut Barbados} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!2}{\strut island} \colorbox{red!0}{\strut of} \colorbox{red!19}{\strut Barbados} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut swamped} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut culture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut history} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut architecture} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut endless} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!15}{\strut eats} \colorbox{red!0}{\strut and} \colorbox{red!18}{\strut drinks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut choose} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: average time to sit on the toilet

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut ready} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut bet} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut poster} \colorbox{red!0}{\strut âTAB67â} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut i} \colorbox{red!0}{\strut can} \colorbox{red!8}{\strut crap} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 15} \colorbox{red!2}{\strut seconds} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!8}{\strut crap} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 15} \colorbox{red!1}{\strut minutes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Itâs} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut myth} \colorbox{red!0}{\strut that} \colorbox{red!3}{\strut people} \colorbox{red!0}{\strut who} \colorbox{red!15}{\strut sit} \colorbox{red!0}{\strut a} \colorbox{red!39}{\strut long} \colorbox{red!10}{\strut time} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!23}{\strut toilet} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut actually} \colorbox{red!3}{\strut shitting} \colorbox{red!0}{\strut more} \colorbox{red!1}{\strut volume} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut those} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut \&} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!14}{\strut bathroom} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut People} \colorbox{red!0}{\strut who} \colorbox{red!8}{\strut stay} \colorbox{red!0}{\strut a} \colorbox{red!39}{\strut long} \colorbox{red!10}{\strut time} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!14}{\strut bathroom} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut constipated} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut Comfort} \colorbox{red!21}{\strut Height} \colorbox{red!0}{\strut :} \colorbox{red!9}{\strut Comfort} \colorbox{red!21}{\strut height} \colorbox{red!21}{\strut toilets} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut slightly} \colorbox{red!1}{\strut taller} \colorbox{red!0}{\strut than} \colorbox{red!5}{\strut standard} \colorbox{red!21}{\strut toilets} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut making} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut more} \colorbox{red!5}{\strut comfortable} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut average-sized} \colorbox{red!3}{\strut adults} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut sit} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut stand} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Comfort} \colorbox{red!21}{\strut height} \colorbox{red!21}{\strut toilets} \colorbox{red!3}{\strut measure} \colorbox{red!0}{\strut anywhere} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut 1/2} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 19} \colorbox{red!0}{\strut inches} \colorbox{red!0}{\strut in} \colorbox{red!21}{\strut height} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: how much protein and iron does fish have

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!4}{\strut median} \colorbox{red!2}{\strut value} \colorbox{red!0}{\strut of} \colorbox{red!58}{\strut Iron} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!13}{\strut Fish} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut salmon} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut pink} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut cooked} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut dry} \colorbox{red!5}{\strut heat} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut 100g} \colorbox{red!6}{\strut contains} \colorbox{red!0}{\strut 0.45} \colorbox{red!2}{\strut mg} \colorbox{red!0}{\strut of} \colorbox{red!58}{\strut Iron} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut corresponds} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut \%} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut recommended} \colorbox{red!5}{\strut daily} \colorbox{red!1}{\strut allowance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut this} \colorbox{red!2}{\strut serving} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut Calories} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 153} \colorbox{red!1}{\strut kcal} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Protein} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 24.58} \colorbox{red!0}{\strut g} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Fat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 5.28} \colorbox{red!0}{\strut g} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut Carbohydrate} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut g} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Does} \colorbox{red!22}{\strut fish} \colorbox{red!0}{\strut have} \colorbox{red!23}{\strut protein} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Indeed} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lots} \colorbox{red!0}{\strut !} \colorbox{red!22}{\strut Fish} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut 6} \colorbox{red!1}{\strut times} \colorbox{red!0}{\strut more} \colorbox{red!23}{\strut protein} \colorbox{red!0}{\strut than} \colorbox{red!5}{\strut milk} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut making} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut best} \colorbox{red!2}{\strut sources} \colorbox{red!0}{\strut of} \colorbox{red!23}{\strut protein} \colorbox{red!2}{\strut available} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut put} \colorbox{red!0}{\strut together} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut list} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut best} \colorbox{red!22}{\strut fish} \colorbox{red!2}{\strut available} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut eat} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut find} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!23}{\strut protein} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut favourite} \colorbox{red!22}{\strut fish} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: how much does a bar of gold worth

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut A} \colorbox{red!22}{\strut gold} \colorbox{red!20}{\strut bar} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut international} \colorbox{red!0}{\strut standards} \colorbox{red!2}{\strut weighs} \colorbox{red!0}{\strut ~} \colorbox{red!0}{\strut 400} \colorbox{red!1}{\strut troy} \colorbox{red!2}{\strut ounces} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut 27.4} \colorbox{red!2}{\strut pounds} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut 4/25/08} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut value} \colorbox{red!0}{\strut of} \colorbox{red!22}{\strut gold} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 891} \colorbox{red!0}{\strut per} \colorbox{red!1}{\strut troy} \colorbox{red!2}{\strut oz} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Therefore} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!22}{\strut gold} \colorbox{red!20}{\strut bar} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut be} \colorbox{red!10}{\strut worth} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut \$} \colorbox{red!0}{\strut 356,400} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut \_\_\_\_\_\_\_\_\_\_} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut value} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!22}{\strut gold} \colorbox{red!20}{\strut bar} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut slightly} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut spot} \colorbox{red!8}{\strut price} \colorbox{red!0}{\strut of} \colorbox{red!22}{\strut gold} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Add} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut \%} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut How} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut one} \colorbox{red!26}{\strut bar} \colorbox{red!0}{\strut of} \colorbox{red!23}{\strut gold} \colorbox{red!0}{\strut at} \colorbox{red!14}{\strut fort} \colorbox{red!18}{\strut knox} \colorbox{red!17}{\strut weigh} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!26}{\strut bar} \colorbox{red!9}{\strut worth} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut us} \colorbox{red!3}{\strut currency} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Me} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut friends} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut watching} \colorbox{red!2}{\strut die} \colorbox{red!0}{\strut hard} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut wondering} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!5}{\strut sam} \colorbox{red!7}{\strut jackson} \colorbox{red!4}{\strut lost} \colorbox{red!0}{\strut by} \colorbox{red!4}{\strut leaving} \colorbox{red!0}{\strut that} \colorbox{red!26}{\strut bar} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut back} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut p.o.s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut they} \colorbox{red!3}{\strut left} \colorbox{red!0}{\strut behind} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut please} \colorbox{red!3}{\strut leave} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut dollar} \colorbox{red!3}{\strut amount} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut n't} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut thank} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: how much debt does china have as % of gdp

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!28}{\strut China} \colorbox{red!0}{\strut 's} \colorbox{red!27}{\strut debt} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut 250} \colorbox{red!1}{\strut \%} \colorbox{red!0}{\strut of} \colorbox{red!22}{\strut GDP} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 'could} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut fatal} \colorbox{red!0}{\strut '} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut says} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut expert} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Chinaâs} \colorbox{red!1}{\strut total} \colorbox{red!27}{\strut debt} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut double} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut gross} \colorbox{red!0}{\strut domestic} \colorbox{red!0}{\strut product} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut 2015} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut government} \colorbox{red!0}{\strut economist} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut said} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut warning} \colorbox{red!0}{\strut that} \colorbox{red!27}{\strut debt} \colorbox{red!3}{\strut linkages} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut state} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut industry} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut âfatalâ} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut worldâs} \colorbox{red!0}{\strut second} \colorbox{red!1}{\strut largest} \colorbox{red!3}{\strut economy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut countryâs} \colorbox{red!27}{\strut debt} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut ballooned} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut almost} \colorbox{red!1}{\strut 250} \colorbox{red!1}{\strut \%} \colorbox{red!0}{\strut of} \colorbox{red!22}{\strut GDP} \colorbox{red!0}{\strut thanks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Beijingâs} \colorbox{red!0}{\strut repeated} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut cheap} \colorbox{red!0}{\strut credit} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut stimulate} \colorbox{red!0}{\strut slowing} \colorbox{red!0}{\strut growth} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut unleashing} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut massive} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut debt-fuelled} \colorbox{red!0}{\strut spending} \colorbox{red!0}{\strut binge} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut How} \colorbox{red!0}{\strut much} \colorbox{red!32}{\strut debt} \colorbox{red!0}{\strut does} \colorbox{red!30}{\strut Australia} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut ?} \colorbox{red!6}{\strut Net} \colorbox{red!32}{\strut debt} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut gross} \colorbox{red!2}{\strut domestic} \colorbox{red!2}{\strut product} \colorbox{red!0}{\strut (} \colorbox{red!6}{\strut GDP} \colorbox{red!0}{\strut )} \colorbox{red!4}{\strut ratio} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut counting} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut much} \colorbox{red!2}{\strut national} \colorbox{red!32}{\strut debt} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut country} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut value} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut economy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!2}{\strut measured} \colorbox{red!0}{\strut by} \colorbox{red!6}{\strut GDP} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut one} \colorbox{red!2}{\strut indicator} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut economic} \colorbox{red!0}{\strut sustainability} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut countryâs} \colorbox{red!32}{\strut debt} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: health effects of styrofoam cups

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Researchers} \colorbox{red!1}{\strut found} \colorbox{red!0}{\strut that} \colorbox{red!48}{\strut Styrofoam} \colorbox{red!29}{\strut cups} \colorbox{red!18}{\strut lose} \colorbox{red!22}{\strut weight} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut use} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut meaning} \colorbox{red!0}{\strut that} \colorbox{red!37}{\strut styrene} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut oozing} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut foods} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut drinks} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut consume} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut then} \colorbox{red!0}{\strut ends} \colorbox{red!0}{\strut up} \colorbox{red!2}{\strut stored} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut our} \colorbox{red!2}{\strut fatty} \colorbox{red!1}{\strut tissue} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut build} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut levels} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut can} \colorbox{red!16}{\strut cause} \colorbox{red!1}{\strut fatigue} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut nervousness} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut difficulty} \colorbox{red!1}{\strut sleeping} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut blood} \colorbox{red!0}{\strut abnormalities} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut even} \colorbox{red!3}{\strut carcinogenic} \colorbox{red!3}{\strut effects} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!0}{\strut âstyreneâ} \colorbox{red!3}{\strut present} \colorbox{red!0}{\strut in} \colorbox{red!12}{\strut Styrofoam} \colorbox{red!5}{\strut cups} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut such} \colorbox{red!4}{\strut containers} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ability} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut percolate} \colorbox{red!0}{\strut the} \colorbox{red!31}{\strut food} \colorbox{red!0}{\strut or} \colorbox{red!4}{\strut beverages} \colorbox{red!5}{\strut carried} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!30}{\strut foods} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ranging} \colorbox{red!0}{\strut from} \colorbox{red!3}{\strut hot} \colorbox{red!0}{\strut or} \colorbox{red!4}{\strut cold} \colorbox{red!10}{\strut drinks} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut snacks} \colorbox{red!0}{\strut ,} \colorbox{red!5}{\strut alcohols} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut acidic} \colorbox{red!4}{\strut eatables} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Styrene} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut suspected} \colorbox{red!9}{\strut carcinogen} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut neurotoxin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!7}{\strut carries} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut host} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut other} \colorbox{red!3}{\strut adverse} \colorbox{red!4}{\strut health} \colorbox{red!6}{\strut effects} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut :} 
}}}
\end{CJK*}

query: are lesser apes hylobates

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!69}{\strut lesser} \colorbox{red!79}{\strut apes} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut gibbon} \colorbox{red!14}{\strut family} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut Hylobatidae} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut sixteen} \colorbox{red!10}{\strut species} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut are} \colorbox{red!4}{\strut native} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Asia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Their} \colorbox{red!0}{\strut major} \colorbox{red!8}{\strut differentiating} \colorbox{red!5}{\strut characteristic} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut long} \colorbox{red!2}{\strut arms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut brachiate} \colorbox{red!0}{\strut through} \colorbox{red!1}{\strut trees} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut How} \colorbox{red!0}{\strut the} \colorbox{red!35}{\strut Apes} \colorbox{red!18}{\strut Evolved} \colorbox{red!0}{\strut The} \colorbox{red!3}{\strut other} \colorbox{red!9}{\strut African} \colorbox{red!7}{\strut anthropoid} \colorbox{red!8}{\strut lineage} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut hominoids} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!3}{\strut includes} \colorbox{red!0}{\strut the} \colorbox{red!35}{\strut apes} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut hominids} \colorbox{red!0}{\strut (} \colorbox{red!5}{\strut humans} \colorbox{red!0}{\strut andtheir} \colorbox{red!3}{\strut direct} \colorbox{red!7}{\strut ancestors} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!6}{\strut living} \colorbox{red!35}{\strut apes} \colorbox{red!3}{\strut consist} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut gib-bon} \colorbox{red!0}{\strut (} \colorbox{red!4}{\strut genus} \colorbox{red!0}{\strut Hylobates} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut orangutan} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Pongo} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut gorilla} \colorbox{red!0}{\strut (} \colorbox{red!4}{\strut Gorilla} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut chimpanzee} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut Pan} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut figure} \colorbox{red!0}{\strut 23.5} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: green fielding meaning

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 'Green} \colorbox{red!40}{\strut Field} \colorbox{red!25}{\strut Investment} \colorbox{red!0}{\strut '} \colorbox{red!0}{\strut A} \colorbox{red!42}{\strut green} \colorbox{red!40}{\strut field} \colorbox{red!25}{\strut investment} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut foreign} \colorbox{red!0}{\strut direct} \colorbox{red!25}{\strut investment} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut parent} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut builds} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut operations} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut foreign} \colorbox{red!0}{\strut country} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ground} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut construction} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut production} \colorbox{red!0}{\strut facilities} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut projects} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut building} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut distribution} \colorbox{red!0}{\strut hubs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut offices} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut living} \colorbox{red!0}{\strut quarters} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!29}{\strut Definition} \colorbox{red!0}{\strut :} \colorbox{red!72}{\strut Cut} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut several} \colorbox{red!27}{\strut meanings} \colorbox{red!0}{\strut in} \colorbox{red!63}{\strut golf} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut reduction} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut tournament} \colorbox{red!0}{\strut field} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut shot} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut controlled} \colorbox{red!0}{\strut fade} \colorbox{red!0}{\strut ;} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut position} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut hole} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut green} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: does flomax cause liver damage

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!18}{\strut medication} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut less} \colorbox{red!20}{\strut side} \colorbox{red!21}{\strut effects} \colorbox{red!0}{\strut than} \colorbox{red!45}{\strut Flomax} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!1}{\strut hard} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!16}{\strut liver} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut n't} \colorbox{red!8}{\strut cause} \colorbox{red!1}{\strut loss} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut strength} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut drowsiness} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut confusion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut relieving} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut symptoms} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut BPH} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut provide} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut brand} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut generic} \colorbox{red!1}{\strut names} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!18}{\strut medications} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut print} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!20}{\strut side} \colorbox{red!21}{\strut effects} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Some} \colorbox{red!32}{\strut Flomax} \colorbox{red!2}{\strut warnings} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut precautions} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut aware} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut 1} \colorbox{red!32}{\strut Flomax} \colorbox{red!0}{\strut can} \colorbox{red!21}{\strut cause} \colorbox{red!4}{\strut dizziness} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!3}{\strut spinning} \colorbox{red!3}{\strut sensation} \colorbox{red!0}{\strut (} \colorbox{red!3}{\strut vertigo} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!4}{\strut fainting} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut first} \colorbox{red!4}{\strut standing} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut Very} \colorbox{red!0}{\strut rarely} \colorbox{red!0}{\strut ,} \colorbox{red!32}{\strut Flomax} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!2}{\strut reported} \colorbox{red!0}{\strut to} \colorbox{red!21}{\strut cause} \colorbox{red!6}{\strut priapism} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!6}{\strut painful} \colorbox{red!4}{\strut erection} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut penis} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut go} \colorbox{red!4}{\strut away} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Even} \colorbox{red!0}{\strut though} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut seem} \colorbox{red!0}{\strut embarrassing} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut seek} \colorbox{red!0}{\strut medical} \colorbox{red!0}{\strut attention} \colorbox{red!0}{\strut right} \colorbox{red!4}{\strut away} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!6}{\strut priapism} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut made} \colorbox{red!0}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut permanent} \colorbox{red!0}{\strut damage} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut penis} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: do atoms make up dna

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!23}{\strut DNA} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut 5} \colorbox{red!4}{\strut different} \colorbox{red!22}{\strut atoms} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut carbon} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut hydrogen} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut oxygen} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut nitrogen} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut phosphorous} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut estimation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 204} \colorbox{red!0}{\strut billion} \colorbox{red!22}{\strut atoms} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut each} \colorbox{red!23}{\strut DNA} \colorbox{red!0}{\strut .} \colorbox{red!23}{\strut DNA} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut 5} \colorbox{red!4}{\strut different} \colorbox{red!22}{\strut atoms} \colorbox{red!0}{\strut -} \colorbox{red!2}{\strut carbon} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut hydrogen} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut oxygen} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut nitrogen} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut phosphorous} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut According} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut estimation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut 204} \colorbox{red!0}{\strut billion} \colorbox{red!22}{\strut atoms} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut each} \colorbox{red!23}{\strut DNA} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!46}{\strut Genomics} \colorbox{red!0}{\strut in} \colorbox{red!10}{\strut Theory} \colorbox{red!0}{\strut and} \colorbox{red!6}{\strut Practice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!46}{\strut Genomics} \colorbox{red!0}{\strut .} \colorbox{red!46}{\strut Genomics} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut study} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut genomes} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut organisms} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!3}{\strut main} \colorbox{red!0}{\strut task} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!4}{\strut determine} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut entire} \colorbox{red!3}{\strut sequence} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut DNA} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut composition} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut atoms} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut DNA} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut chemical} \colorbox{red!0}{\strut bonds} \colorbox{red!0}{\strut between} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut DNA} \colorbox{red!3}{\strut atoms} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: definition of sadducees

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut The} \colorbox{red!158}{\strut Sadducees} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut ;} \colorbox{red!8}{\strut Hebrew} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut á¹¢ÄdÃ»qÃ®m} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut a} \colorbox{red!7}{\strut sect} \colorbox{red!0}{\strut or} \colorbox{red!3}{\strut group} \colorbox{red!0}{\strut of} \colorbox{red!5}{\strut Jews} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut was} \colorbox{red!2}{\strut active} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut Judea} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Second} \colorbox{red!2}{\strut Temple} \colorbox{red!0}{\strut period} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut starting} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut century} \colorbox{red!0}{\strut BCE} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut destruction} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Temple} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 70} \colorbox{red!0}{\strut CE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!7}{\strut sect} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut identified} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Josephus} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut upper} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut economic} \colorbox{red!0}{\strut echelon} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Judean} \colorbox{red!0}{\strut society} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!52}{\strut Sadducees} \colorbox{red!0}{\strut The} \colorbox{red!47}{\strut origin} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!31}{\strut Jewish} \colorbox{red!35}{\strut sect} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut definitely} \colorbox{red!0}{\strut be} \colorbox{red!9}{\strut traced} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!6}{\strut probably} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut outcome} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut influence} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Grecian} \colorbox{red!7}{\strut customs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut philosophy} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut period} \colorbox{red!0}{\strut of} \colorbox{red!7}{\strut Greek} \colorbox{red!0}{\strut domination} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: definition of anthropology

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut LINK} \colorbox{red!0}{\strut /} \colorbox{red!1}{\strut CITE} \colorbox{red!0}{\strut ADD} \colorbox{red!0}{\strut TO} \colorbox{red!1}{\strut WORD} \colorbox{red!0}{\strut LIST} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!45}{\strut definition} \colorbox{red!0}{\strut of} \colorbox{red!75}{\strut anthropology} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut study} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut elements} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut humans} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut biology} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut culture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut understand} \colorbox{red!1}{\strut human} \colorbox{red!0}{\strut origin} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut evolution} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut beliefs} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut customs} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut An} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut someone} \colorbox{red!0}{\strut who} \colorbox{red!2}{\strut studies} \colorbox{red!75}{\strut anthropology} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Ruth} \colorbox{red!0}{\strut Benedict} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut Define} \colorbox{red!33}{\strut anthropological} \colorbox{red!0}{\strut .} \colorbox{red!33}{\strut anthropological} \colorbox{red!5}{\strut synonyms} \colorbox{red!0}{\strut ,} \colorbox{red!33}{\strut anthropological} \colorbox{red!2}{\strut pronunciation} \colorbox{red!0}{\strut ,} \colorbox{red!33}{\strut anthropological} \colorbox{red!2}{\strut translation} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut English} \colorbox{red!2}{\strut dictionary} \colorbox{red!14}{\strut definition} \colorbox{red!0}{\strut of} \colorbox{red!33}{\strut anthropological} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut n.} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut scientific} \colorbox{red!0}{\strut study} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut origin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut behavior} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut physical} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut cultural} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut humans} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Christian} \colorbox{red!0}{\strut theology} \colorbox{red!0}{\strut ...} 
}}}
\end{CJK*}

query: age not to take off shoes at airline security

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut 're} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut the} \colorbox{red!45}{\strut age} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 13} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut generally} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!47}{\strut remove} \colorbox{red!0}{\strut your} \colorbox{red!55}{\strut shoes} \colorbox{red!0}{\strut during} \colorbox{red!0}{\strut the} \colorbox{red!34}{\strut security} \colorbox{red!0}{\strut screening.You} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut multiple} \colorbox{red!0}{\strut passes} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut metal} \colorbox{red!2}{\strut detector} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut advanced} \colorbox{red!0}{\strut technology} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut your} \colorbox{red!11}{\strut hands} \colorbox{red!4}{\strut swabbed} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!14}{\strut United} \colorbox{red!10}{\strut Airlines} \colorbox{red!4}{\strut passengers} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut now} \colorbox{red!1}{\strut notified} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut advance} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut their} \colorbox{red!10}{\strut boarding} \colorbox{red!12}{\strut pass} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut they} \colorbox{red!2}{\strut qualify} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut expedited} \colorbox{red!3}{\strut security} \colorbox{red!0}{\strut via} \colorbox{red!7}{\strut TSA} \colorbox{red!7}{\strut Precheck} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut CLEVELAND} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut Ohio} \colorbox{red!0}{\strut -} \colorbox{red!14}{\strut United} \colorbox{red!10}{\strut Airlines} \colorbox{red!4}{\strut passengers} \colorbox{red!0}{\strut hoping} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut sail} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut faster} \colorbox{red!7}{\strut TSA} \colorbox{red!7}{\strut Precheck} \colorbox{red!1}{\strut lanes} \colorbox{red!0}{\strut at} \colorbox{red!3}{\strut airport} \colorbox{red!3}{\strut security} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut now} \colorbox{red!1}{\strut know} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut 're} \colorbox{red!2}{\strut eligible} \colorbox{red!0}{\strut simply} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut glancing} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut their} \colorbox{red!10}{\strut boarding} \colorbox{red!11}{\strut passes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut That} \colorbox{red!0}{\strut beats} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut wait} \colorbox{red!0}{\strut until} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut TSA} \colorbox{red!0}{\strut agent} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut kiosk} \colorbox{red!0}{\strut scans} \colorbox{red!0}{\strut your} \colorbox{red!10}{\strut boarding} \colorbox{red!12}{\strut pass} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut know} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut 're} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut limited} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut passengers} \colorbox{red!0}{\strut who} \colorbox{red!2}{\strut qualify} \colorbox{red!0}{\strut for} \colorbox{red!7}{\strut Precheck} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut every} \colorbox{red!3}{\strut flight} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut n't} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut take} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut their} \colorbox{red!1}{\strut shoes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut belts} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut jackets} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut can} \colorbox{red!1}{\strut leave} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut laptops} \colorbox{red!0}{\strut inside} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut computer} \colorbox{red!0}{\strut bags} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: definition of western european time zone

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut Western} \colorbox{red!6}{\strut European} \colorbox{red!29}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!8}{\strut WET} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut UTCÂ±00:00} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!29}{\strut time} \colorbox{red!17}{\strut zone} \colorbox{red!0}{\strut covering} \colorbox{red!0}{\strut parts} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut western} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut northwestern} \colorbox{red!9}{\strut Europe} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut All} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut above} \colorbox{red!0}{\strut countries} \colorbox{red!0}{\strut except} \colorbox{red!2}{\strut Iceland} \colorbox{red!0}{\strut implement} \colorbox{red!1}{\strut daylight} \colorbox{red!1}{\strut saving} \colorbox{red!29}{\strut time} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut summer} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut switching} \colorbox{red!0}{\strut to} \colorbox{red!6}{\strut Western} \colorbox{red!6}{\strut European} \colorbox{red!2}{\strut Summer} \colorbox{red!29}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut WEST} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut UTC+1} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!1}{\strut hour} \colorbox{red!0}{\strut ahead} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut WET} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!11}{\strut Iceland} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!11}{\strut Time} \colorbox{red!6}{\strut Zone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!1}{\strut Standard} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut WET} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Greenwich} \colorbox{red!1}{\strut Mean} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut GMT} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Iceland} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!11}{\strut Time} \colorbox{red!6}{\strut Zone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!1}{\strut Standard} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut WET} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Greenwich} \colorbox{red!1}{\strut Mean} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut GMT} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .celand} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!11}{\strut Time} \colorbox{red!6}{\strut Zone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!1}{\strut Standard} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut WET} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Greenwich} \colorbox{red!1}{\strut Mean} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut GMT} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} \colorbox{red!11}{\strut Iceland} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!11}{\strut Time} \colorbox{red!6}{\strut Zone} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Western} \colorbox{red!1}{\strut European} \colorbox{red!1}{\strut Standard} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut WET} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Greenwich} \colorbox{red!1}{\strut Mean} \colorbox{red!11}{\strut Time} \colorbox{red!0}{\strut (} \colorbox{red!1}{\strut GMT} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: age requirements for name change

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut These} \colorbox{red!22}{\strut requirements} \colorbox{red!0}{\strut include} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut must} \colorbox{red!2}{\strut currently} \colorbox{red!4}{\strut reside} \colorbox{red!0}{\strut in} \colorbox{red!27}{\strut California} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut must} \colorbox{red!2}{\strut currently} \colorbox{red!5}{\strut live} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut County} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!29}{\strut name} \colorbox{red!40}{\strut change} \colorbox{red!2}{\strut action} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut filed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut an} \colorbox{red!5}{\strut adult} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 18} \colorbox{red!0}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!14}{\strut age} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut older} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut You} \colorbox{red!1}{\strut must} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut under} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut jurisdiction} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!27}{\strut California} \colorbox{red!0}{\strut Department} \colorbox{red!0}{\strut of} \colorbox{red!6}{\strut Corrections} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut state} \colorbox{red!2}{\strut prison} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut on} \colorbox{red!2}{\strut parole} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Tips} \colorbox{red!0}{\strut \&} \colorbox{red!0}{\strut Warnings} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut 18} \colorbox{red!2}{\strut years} \colorbox{red!0}{\strut of} \colorbox{red!16}{\strut age} \colorbox{red!0}{\strut to} \colorbox{red!9}{\strut legally} \colorbox{red!22}{\strut change} \colorbox{red!0}{\strut your} \colorbox{red!21}{\strut name} \colorbox{red!0}{\strut in} \colorbox{red!18}{\strut Texas} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut State} \colorbox{red!0}{\strut law} \colorbox{red!1}{\strut requires} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut different} \colorbox{red!0}{\strut petition} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut procedure} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!2}{\strut minor} \colorbox{red!4}{\strut child} \colorbox{red!0}{\strut 's} \colorbox{red!21}{\strut name} \colorbox{red!22}{\strut change} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut child} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut the} \colorbox{red!16}{\strut age} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 10} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut must} \colorbox{red!0}{\strut agree} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!21}{\strut name} \colorbox{red!22}{\strut change} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: do you need a certification to become a mindfulness meditation practitioner

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut SR-FLEX} \colorbox{red!20}{\strut MBSR} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Mind-Body} \colorbox{red!15}{\strut Medicine} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Intensive} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 7-day} \colorbox{red!1}{\strut residential} \colorbox{red!6}{\strut program} \colorbox{red!2}{\strut teaching} \colorbox{red!19}{\strut mindfulness} \colorbox{red!15}{\strut meditation} \colorbox{red!1}{\strut practice} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut taught} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!10}{\strut CFM} \colorbox{red!0}{\strut Mindfulness-Based} \colorbox{red!3}{\strut Stress} \colorbox{red!1}{\strut Reduction} \colorbox{red!1}{\strut Clinic} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut MBSR} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Mind-Body} \colorbox{red!15}{\strut Medicine} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut SR-FLEX} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!10}{\strut required} \colorbox{red!0}{\strut for} \colorbox{red!10}{\strut CFM} \colorbox{red!12}{\strut Teacher} \colorbox{red!16}{\strut Certification} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut completed} \colorbox{red!0}{\strut any} \colorbox{red!2}{\strut time} \colorbox{red!0}{\strut prior} \colorbox{red!0}{\strut to} \colorbox{red!16}{\strut Certification} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Â©} \colorbox{red!0}{\strut Bob} \colorbox{red!2}{\strut Stockfield} \colorbox{red!0}{\strut .} \colorbox{red!39}{\strut Meditation} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!4}{\strut mind} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut body} \colorbox{red!4}{\strut practice} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!16}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!39}{\strut meditation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut which} \colorbox{red!4}{\strut originated} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut ancient} \colorbox{red!0}{\strut religious} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut spiritual} \colorbox{red!0}{\strut traditions} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Some} \colorbox{red!3}{\strut forms} \colorbox{red!0}{\strut of} \colorbox{red!39}{\strut meditation} \colorbox{red!2}{\strut instruct} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut practitioner} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut become} \colorbox{red!3}{\strut mindful} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut thoughts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut feelings} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sensations} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut observe} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut nonjudgmental} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Featured} \colorbox{red!39}{\strut Meditation} \colorbox{red!0}{\strut :} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut Depth} 
}}}
\end{CJK*}

query: does excessive spinach consumption cause kidney stones

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut Low} \colorbox{red!0}{\strut in} \colorbox{red!5}{\strut calories} \colorbox{red!0}{\strut but} \colorbox{red!4}{\strut high} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut vitamins} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut minerals} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut fiber} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut versatile} \colorbox{red!0}{\strut addition} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!5}{\strut healthy} \colorbox{red!11}{\strut diet} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut rare} \colorbox{red!0}{\strut cases} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut consuming} \colorbox{red!9}{\strut excessive} \colorbox{red!1}{\strut amounts} \colorbox{red!0}{\strut of} \colorbox{red!52}{\strut spinach} \colorbox{red!0}{\strut can} \colorbox{red!2}{\strut lead} \colorbox{red!0}{\strut to} \colorbox{red!40}{\strut kidney} \colorbox{red!24}{\strut stones} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut issues} \colorbox{red!0}{\strut with} \colorbox{red!5}{\strut iron} \colorbox{red!1}{\strut absorption} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut gastrointestinal} \colorbox{red!0}{\strut difficulties} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Maintaining} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut balanced} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut varied} \colorbox{red!11}{\strut diet} \colorbox{red!0}{\strut will} \colorbox{red!6}{\strut help} \colorbox{red!0}{\strut you} \colorbox{red!2}{\strut avoid} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!16}{\strut Home} \colorbox{red!17}{\strut Remedies} \colorbox{red!0}{\strut for} \colorbox{red!25}{\strut Kidney} \colorbox{red!23}{\strut Stones} \colorbox{red!0}{\strut .} \colorbox{red!25}{\strut Kidney} \colorbox{red!23}{\strut stones} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut very} \colorbox{red!2}{\strut common} \colorbox{red!2}{\strut health} \colorbox{red!2}{\strut problem} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut chemicals} \colorbox{red!0}{\strut in} \colorbox{red!4}{\strut urine} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut uric} \colorbox{red!0}{\strut acid} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut phosphorous} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut calcium} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut oxalic} \colorbox{red!0}{\strut acid} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Other} \colorbox{red!2}{\strut common} \colorbox{red!9}{\strut causes} \colorbox{red!0}{\strut of} \colorbox{red!25}{\strut kidney} \colorbox{red!23}{\strut stones} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut excessive} \colorbox{red!0}{\strut consumption} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut vitamin} \colorbox{red!0}{\strut D} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut mineral} \colorbox{red!0}{\strut imbalance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut dehydration} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut gout} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut improper} \colorbox{red!0}{\strut diet} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: does insulin give you constipation

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!28}{\strut Insulin} \colorbox{red!0}{\strut and} \colorbox{red!31}{\strut Constipation} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut from} \colorbox{red!3}{\strut FDA} \colorbox{red!0}{\strut reports} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Summary} \colorbox{red!0}{\strut .} \colorbox{red!31}{\strut Constipation} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut found} \colorbox{red!0}{\strut among} \colorbox{red!2}{\strut people} \colorbox{red!0}{\strut who} \colorbox{red!2}{\strut take} \colorbox{red!28}{\strut Insulin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut people} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut female} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 60+} \colorbox{red!1}{\strut old} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!2}{\strut taking} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut drug} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut <} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut month} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut also} \colorbox{red!2}{\strut take} \colorbox{red!2}{\strut medication} \colorbox{red!2}{\strut Lasix} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut have} \colorbox{red!3}{\strut Diabetes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut review} \colorbox{red!0}{\strut analyzes} \colorbox{red!0}{\strut which} \colorbox{red!2}{\strut people} \colorbox{red!0}{\strut have} \colorbox{red!31}{\strut Constipation} \colorbox{red!0}{\strut with} \colorbox{red!28}{\strut Insulin} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!39}{\strut Diabetes} \colorbox{red!0}{\strut and} \colorbox{red!29}{\strut Constipation} \colorbox{red!0}{\strut or} \colorbox{red!32}{\strut Diarrhea} \colorbox{red!0}{\strut .} \colorbox{red!39}{\strut Diabetes} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!9}{\strut disease} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut body} \colorbox{red!0}{\strut either} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!4}{\strut produce} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut unable} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut the} \colorbox{red!5}{\strut hormone} \colorbox{red!5}{\strut insulin} \colorbox{red!0}{\strut properly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!6}{\strut pancreas} \colorbox{red!4}{\strut produces} \colorbox{red!5}{\strut insulin} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut which} \colorbox{red!4}{\strut helps} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut body} \colorbox{red!0}{\strut use} \colorbox{red!3}{\strut sugar} \colorbox{red!0}{\strut (} \colorbox{red!3}{\strut glucose} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut from} \colorbox{red!4}{\strut foods} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: effects of hyperthyroidism

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!2}{\strut serious} \colorbox{red!69}{\strut effects} \colorbox{red!0}{\strut of} \colorbox{red!69}{\strut hyperthyroidism} \colorbox{red!3}{\strut impact} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut heartâs} \colorbox{red!8}{\strut function} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Rapid} \colorbox{red!11}{\strut heart} \colorbox{red!2}{\strut rate} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut atrial} \colorbox{red!1}{\strut fibrillation} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut which} \colorbox{red!3}{\strut occurs} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!11}{\strut heart} \colorbox{red!2}{\strut beat} \colorbox{red!0}{\strut is} \colorbox{red!2}{\strut abnormal} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut congestive} \colorbox{red!11}{\strut heart} \colorbox{red!3}{\strut failure} \colorbox{red!0}{\strut (} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut body} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut unable} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut circulate} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut blood} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut occur} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut according} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Mayo} \colorbox{red!0}{\strut Clinic} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!11}{\strut Hyperdynamic} \colorbox{red!6}{\strut circulation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut cardiac} \colorbox{red!11}{\strut effects} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut hyperthyroidism} \colorbox{red!1}{\strut commonly} \colorbox{red!3}{\strut cause} \colorbox{red!2}{\strut increased} \colorbox{red!1}{\strut preload} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut low} \colorbox{red!1}{\strut systemic} \colorbox{red!2}{\strut vascular} \colorbox{red!1}{\strut resistance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut high} \colorbox{red!2}{\strut heart} \colorbox{red!2}{\strut rate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut increased} \colorbox{red!4}{\strut cardiac} \colorbox{red!2}{\strut muscle} \colorbox{red!1}{\strut oxygen} \colorbox{red!1}{\strut consumption} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut short} \colorbox{red!2}{\strut term} \colorbox{red!10}{\strut hyperthyroidism} \colorbox{red!0}{\strut these} \colorbox{red!11}{\strut effects} \colorbox{red!1}{\strut result} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut increased} \colorbox{red!2}{\strut heart} \colorbox{red!2}{\strut rate} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut high} \colorbox{red!4}{\strut cardiac} \colorbox{red!0}{\strut output.yperdynamic} \colorbox{red!6}{\strut circulation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut cardiac} \colorbox{red!11}{\strut effects} \colorbox{red!0}{\strut of} \colorbox{red!10}{\strut hyperthyroidism} \colorbox{red!1}{\strut commonly} \colorbox{red!3}{\strut cause} \colorbox{red!2}{\strut increased} \colorbox{red!1}{\strut preload} \colorbox{red!0}{\strut with} \colorbox{red!1}{\strut low} \colorbox{red!1}{\strut systemic} \colorbox{red!2}{\strut vascular} \colorbox{red!1}{\strut resistance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut high} \colorbox{red!2}{\strut heart} \colorbox{red!2}{\strut rate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut increased} \colorbox{red!4}{\strut cardiac} \colorbox{red!2}{\strut muscle} \colorbox{red!1}{\strut oxygen} \colorbox{red!1}{\strut consumption} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut short} \colorbox{red!2}{\strut term} \colorbox{red!10}{\strut hyperthyroidism} \colorbox{red!0}{\strut these} \colorbox{red!11}{\strut effects} \colorbox{red!1}{\strut result} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut an} \colorbox{red!2}{\strut increased} \colorbox{red!2}{\strut heart} \colorbox{red!2}{\strut rate} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut high} \colorbox{red!4}{\strut cardiac} \colorbox{red!1}{\strut output} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: geranium rose essential oil benefits

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut slide} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!29}{\strut Benefits} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut Uses} \colorbox{red!41}{\strut Rose} \colorbox{red!44}{\strut geranium} \colorbox{red!28}{\strut essential} \colorbox{red!44}{\strut oil} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut primarily} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut in} \colorbox{red!3}{\strut skin} \colorbox{red!1}{\strut care} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut treat} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut problems} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!1}{\strut acne} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut bruises} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut insect} \colorbox{red!0}{\strut bites} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut cuts} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut scrapes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut minor} \colorbox{red!0}{\strut burns} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut athlete} \colorbox{red!0}{\strut 's} \colorbox{red!1}{\strut foot} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut psoriasis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut impetigo} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut eczema} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Research} \colorbox{red!0}{\strut suggests} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut significantly} \colorbox{red!0}{\strut reduce} \colorbox{red!0}{\strut nerve} \colorbox{red!1}{\strut pain} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut follows} \colorbox{red!1}{\strut shingles} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!21}{\strut Geranium} \colorbox{red!17}{\strut Essential} \colorbox{red!24}{\strut Oil} \colorbox{red!0}{\strut :} \colorbox{red!3}{\strut Uses} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Benefits} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!2}{\strut Precautions} \colorbox{red!0}{\strut .} \colorbox{red!21}{\strut Geranium} \colorbox{red!24}{\strut oil} \colorbox{red!0}{\strut (} \colorbox{red!2}{\strut Pelargonium} \colorbox{red!2}{\strut graveolens} \colorbox{red!0}{\strut )} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut beautiful} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut floral} \colorbox{red!17}{\strut essential} \colorbox{red!24}{\strut oil} \colorbox{red!0}{\strut often} \colorbox{red!0}{\strut referred} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut poor} \colorbox{red!0}{\strut man} \colorbox{red!0}{\strut 's} \colorbox{red!3}{\strut rose} \colorbox{red!24}{\strut oil} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut similar} \colorbox{red!2}{\strut properties} \colorbox{red!0}{\strut and} \colorbox{red!3}{\strut uses} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut 's} \colorbox{red!1}{\strut sweet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rose-like} \colorbox{red!0}{\strut aroma} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut long-lasting} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut potent} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut 'll} \colorbox{red!2}{\strut smell} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut days} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}



==> sections/visualization/win.tex <==
query: synonyms for the word discipline

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut another} \colorbox{red!2}{\strut word} \colorbox{red!0}{\strut for} \colorbox{red!25}{\strut discipline} \colorbox{red!0}{\strut ?} \colorbox{red!9}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut another} \colorbox{red!2}{\strut word} \colorbox{red!0}{\strut for} \colorbox{red!25}{\strut discipline} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut 871} \colorbox{red!22}{\strut synonyms} \colorbox{red!0}{\strut foundPronunciation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dspln} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dspln} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut dspln} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut TweetSee} \colorbox{red!25}{\strut DISCIPLINE} \colorbox{red!3}{\strut definition} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut Dictionary.net} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Find} \colorbox{red!0}{\strut antonyms} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut word} \colorbox{red!25}{\strut DISCIPLINE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Enter} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut text} \colorbox{red!0}{\strut below} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut find} \colorbox{red!22}{\strut synonyms} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut click} \colorbox{red!0}{\strut hereSynonyms} \colorbox{red!0}{\strut for} \colorbox{red!25}{\strut Discipline} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut command} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut authority} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut charge} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut command} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut commission} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut coordination} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut direction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut domination} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut government} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut grasp} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut grip} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut hold} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut law} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut management} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mandate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mastery} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut power} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut prowess} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut reign} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rule} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sovereignty} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut supremacy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut sway} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut will.control} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut administration} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut bridle} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut conn} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut harness} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut helm} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut leadership} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut oversight} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut subjection.eastern} \colorbox{red!0}{\strut poison} \colorbox{red!0}{\strut oak} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Champaign} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut control} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut deserts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut disciplining} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut domain} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut domestication} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut drill} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut duress} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut effort} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut exercise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut field} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut meticulousness} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut nurture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut payment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut practice} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pressure} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut demesne} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut lesson} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut speciality} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut warm-up} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut science} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut self-control} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut willpower} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut education} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut spit} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut polish} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut terrain.education} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut schooling} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pedagogy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut inculcation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut apprenticeship.instruction} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut instruction.method} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut approach} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut course} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut manner} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut mechanism} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut method} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut procedure} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut process} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut program} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut schema} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut scheme} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut tactic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut technique} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut trajectory} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut way.order} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut law} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut order.penalty} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut abatement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut chastisement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut correction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut deduction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut encumbrance} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut forfeiture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut judgment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut penalty} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut premium} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut punishment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut retribution.preparation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut training.punishment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut affliction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut agony} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut castigation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut chastisement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut confinement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut crucifixion} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut execution} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut imprisonment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut incarceration} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut payment} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut penalty} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut persecution} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut price} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!3}{\strut Synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Word} \colorbox{red!0}{\strut games} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Submit} \colorbox{red!0}{\strut new} \colorbox{red!1}{\strut word} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut WidgetSynonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0,00} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut votesThe} \colorbox{red!3}{\strut synonym} \colorbox{red!10}{\strut discipline} \colorbox{red!1}{\strut synonymous} \colorbox{red!1}{\strut definition} \colorbox{red!1}{\strut words} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut verb} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut punish} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut subdue} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut penalise} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut penalize} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut castigate} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut limit} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut chastise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut correctSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut disciplineAds} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut verb} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut instruct} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut exercise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut prepare} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut drill} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut control} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut harden} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut educateSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut disciplinediscipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut training} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut cultivation} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut drill} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut exercise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut instruction} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut practiceSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut disciplinediscipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut rules} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut codeSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut disciplinediscipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut punishment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut castigation} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut chastisement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut correctionSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut disciplinediscipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut control} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut limitation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut government} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut order} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut regulation} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut subjection} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut subjugationSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut disciplineFurther} \colorbox{red!0}{\strut results} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut word} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut breed} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut verb} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut foster} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut bring} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut educate} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut instruct} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut nurture} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut raiseSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut breedcensure} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut verb} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut condemn} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut fault} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut disciplineSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut censurechastise} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut verb} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut punish} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut subdue} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut penalise} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut penalize} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut castigate} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut limit} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut disciplineSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut chastisecode} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut noun} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut principle} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut rules} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut statutesSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut codecondition} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut verb} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut prepare} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut equip} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut train} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut coach} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adapt} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut treatSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut conditiondrill} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut verb} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut means} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut activity} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut practise} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut rehearse} \colorbox{red!0}{\strut ,} \colorbox{red!10}{\strut discipline} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut teach} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut train} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut coachSubmit} \colorbox{red!3}{\strut synonym} \colorbox{red!0}{\strut for} 
}}}
\end{CJK*}

query: node js import

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Could} \colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut import} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut CSV} \colorbox{red!1}{\strut files} \colorbox{red!0}{\strut into} \colorbox{red!14}{\strut MySQL} \colorbox{red!0}{\strut quicker} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut Load} \colorbox{red!1}{\strut Data} \colorbox{red!0}{\strut Infile} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Simon} \colorbox{red!0}{\strut Dowdles} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Full} \colorbox{red!0}{\strut stack} \colorbox{red!0}{\strut web} \colorbox{red!0}{\strut developer} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut strong} \colorbox{red!0}{\strut focus} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut heavy} \colorbox{red!1}{\strut WordPress} \colorbox{red!0}{\strut customizationAnswered} \colorbox{red!0}{\strut Nov} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2015No} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut becuase} \colorbox{red!0}{\strut even} \colorbox{red!0}{\strut the} \colorbox{red!14}{\strut MySQL} \colorbox{red!17}{\strut node} \colorbox{red!1}{\strut module} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut still} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut driver} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut gets} \colorbox{red!1}{\strut data} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut your} \colorbox{red!17}{\strut node} \colorbox{red!0}{\strut instance} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut core} \colorbox{red!14}{\strut MySQL} \colorbox{red!1}{\strut system} \colorbox{red!0}{\strut level} \colorbox{red!1}{\strut operations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut So} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut essence} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut bridge} \colorbox{red!0}{\strut further} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut core} \colorbox{red!14}{\strut MySQL} \colorbox{red!1}{\strut system} \colorbox{red!1}{\strut operations} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut otherwise} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut command} \colorbox{red!0}{\strut line} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut slower} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut maybe} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut nano} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut same} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut faster} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Load} \colorbox{red!1}{\strut Data} \colorbox{red!0}{\strut Infile} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut perfectly} \colorbox{red!0}{\strut okay} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut half} \colorbox{red!0}{\strut decent} \colorbox{red!0}{\strut amount} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut processing} \colorbox{red!0}{\strut power} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut ram} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut suggest} \colorbox{red!0}{\strut splitting} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut 5-10} \colorbox{red!0}{\strut smaller} \colorbox{red!1}{\strut files} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!0}{\strut imported} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut 600,000} \colorbox{red!0}{\strut rows} \colorbox{red!0}{\strut merely} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut mysqdump} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut piped} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut to} \colorbox{red!14}{\strut mysql} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut took} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut matter} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut seconds} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut VPS.1.7k} \colorbox{red!0}{\strut ViewsRelated} \colorbox{red!0}{\strut Questions} \colorbox{red!0}{\strut More} \colorbox{red!0}{\strut Answers} \colorbox{red!0}{\strut BelowWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut best} \colorbox{red!14}{\strut MySQL} \colorbox{red!0}{\strut ORM} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut ?} \colorbox{red!9}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut with} \colorbox{red!14}{\strut MySql} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut How} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut unzip} \colorbox{red!0}{\strut large} \colorbox{red!1}{\strut files} \colorbox{red!0}{\strut using} \colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut ?} \colorbox{red!3}{\strut How} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut use} \colorbox{red!14}{\strut MySQL} \colorbox{red!0}{\strut database} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut declining} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Ask} \colorbox{red!0}{\strut New} \colorbox{red!0}{\strut QuestionSalvatore} \colorbox{red!0}{\strut Garbesi} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut http} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut salvatore.garbesi.comAnswered} \colorbox{red!0}{\strut Apr} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2014It} \colorbox{red!0}{\strut depends} \colorbox{red!9}{\strut what} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut comparing} \colorbox{red!0}{\strut Node.js} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut automated} \colorbox{red!0}{\strut scripts} \colorbox{red!0}{\strut running} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut parse} \colorbox{red!0}{\strut CSV} \colorbox{red!1}{\strut files} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 100} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut lines} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut import} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut directly} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut Elasticsearch} \colorbox{red!0}{\strut ,} \colorbox{red!14}{\strut MySQL} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Redis} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CC} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut definitely} \colorbox{red!0}{\strut almost} \colorbox{red!0}{\strut always} \colorbox{red!0}{\strut overrule} \colorbox{red!0}{\strut performance} \colorbox{red!0}{\strut wise} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut likely} \colorbox{red!0}{\strut comes} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut play} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut maintenance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut writing} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut majority} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut JavaScriptNode.js} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut make} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut best} \colorbox{red!0}{\strut Node.js} \colorbox{red!7}{\strut host} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Rohit} \colorbox{red!0}{\strut Mishra} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut Years} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Experience} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Web} \colorbox{red!0}{\strut HostingAnswered} \colorbox{red!0}{\strut Sep} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2017} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Author} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut 88} \colorbox{red!0}{\strut answers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 16.3k} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut viewsI} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut Best} \colorbox{red!0}{\strut totally} \colorbox{red!0}{\strut depends} \colorbox{red!0}{\strut upon} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut individual} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut requirement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut people} \colorbox{red!2}{\strut best} \colorbox{red!1}{\strut web} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut low} \colorbox{red!2}{\strut price} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Some} \colorbox{red!0}{\strut thinks} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut customer} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut should} \colorbox{red!0}{\strut be} \colorbox{red!1}{\strut good} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut So} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut definition} \colorbox{red!0}{\strut of} \colorbox{red!2}{\strut best} \colorbox{red!0}{\strut changes} \colorbox{red!0}{\strut person} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut person} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut But} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut best} \colorbox{red!1}{\strut node} \colorbox{red!9}{\strut js} \colorbox{red!8}{\strut hosting} \colorbox{red!1}{\strut company} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut easily} \colorbox{red!7}{\strut host} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut node} \colorbox{red!9}{\strut js} \colorbox{red!0}{\strut applications.According} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut me} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut research} \colorbox{red!1}{\strut A2HOSTING} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut best} \colorbox{red!1}{\strut node} \colorbox{red!9}{\strut js} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut providers.I} \colorbox{red!0}{\strut am} \colorbox{red!0}{\strut saying} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut researched} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut lot} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut web} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut applications} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut gone} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut social} \colorbox{red!0}{\strut media} \colorbox{red!0}{\strut accounts} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut hosting} \colorbox{red!1}{\strut companies} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut clarity} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut experience} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut customers.Let} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut Why} \colorbox{red!1}{\strut A2hosting} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut bestThe} \colorbox{red!8}{\strut Hosting} \colorbox{red!2}{\strut price} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut A2hosting} \colorbox{red!1}{\strut starts} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.92} \colorbox{red!0}{\strut per} \colorbox{red!1}{\strut month} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut shared} \colorbox{red!0}{\strut hostingA2hosting} \colorbox{red!1}{\strut provides} \colorbox{red!1}{\strut shared} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut vps} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut dedicated} \colorbox{red!1}{\strut server} \colorbox{red!8}{\strut hosting} \colorbox{red!1}{\strut service} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut any} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut time} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut upgrade} \colorbox{red!0}{\strut your} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut easilyUnlimited} \colorbox{red!1}{\strut webspace} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut bandwidth} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut A2hostingFree} \colorbox{red!0}{\strut SSL} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut SSD} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut every} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut accounA2} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut accelerator} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut helps} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut increase} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut website} \colorbox{red!0}{\strut speedAnytime} \colorbox{red!0}{\strut money} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut guarantee} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut A2hostingA2hosting} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut among} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!1}{\strut company} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut provide} \colorbox{red!1}{\strut Node} \colorbox{red!9}{\strut js} \colorbox{red!8}{\strut hosting} \colorbox{red!0}{\strut serviceI} \colorbox{red!0}{\strut hope} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut hosting} \colorbox{red!1}{\strut service} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Node} \colorbox{red!0}{\strut JS544} \colorbox{red!0}{\strut Views} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut View} \colorbox{red!0}{\strut Upvoters} 
}}}
\end{CJK*}

query: what generation is pokemon diamond and pearl

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Pokmon} \colorbox{red!15}{\strut Diamond} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut PearlPokmon} \colorbox{red!15}{\strut Diamond} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Pearl} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut thre} \colorbox{red!0}{\strut fourth} \colorbox{red!1}{\strut Generation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Pokmon} \colorbox{red!1}{\strut games} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Having} \colorbox{red!0}{\strut come} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut new} \colorbox{red!1}{\strut Nintendo} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Nintendo} \colorbox{red!1}{\strut DS} \colorbox{red!0}{\strut ,} \colorbox{red!15}{\strut Diamond} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Pearl} \colorbox{red!0}{\strut makes} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut DS} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut functions} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut TouchScreen} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut WiFi} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Diamond} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Pearl} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut brings} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut features} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Gold} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Silver} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut since} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut removed.Bringing} \colorbox{red!0}{\strut 107} \colorbox{red!1}{\strut New} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut mix} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut bringing} \colorbox{red!0}{\strut us} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 493} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut evolutions} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut old} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut ,} \colorbox{red!15}{\strut Diamond} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Pearl} \colorbox{red!0}{\strut completely} \colorbox{red!0}{\strut overhauls} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut battling} \colorbox{red!0}{\strut system} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut No} \colorbox{red!0}{\strut longer} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut move} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut stats} \colorbox{red!0}{\strut based} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut type} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut rather} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut move} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut individually} \colorbox{red!0}{\strut allocated} \colorbox{red!0}{\strut being} \colorbox{red!0}{\strut Physical} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Special.Diamond} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Pearl} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut set} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut far} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut land} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Sinnoh} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut playing} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Rookie} \colorbox{red!0}{\strut trainer} \colorbox{red!0}{\strut wanting} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut Sinnoh} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut beat} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Gyms} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut best} \colorbox{red!0}{\strut trainer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut throughout} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut travels} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut encounter} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut rivals} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut evil} \colorbox{red!0}{\strut Team} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut land} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Team} \colorbox{red!0}{\strut Galactic} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut whom} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut bent} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut obtaining} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut special} \colorbox{red!0}{\strut legendary} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut version.Diamond} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Pearl} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut 400} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut obtainable} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut making} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut biggest} \colorbox{red!0}{\strut Pokmon} \colorbox{red!1}{\strut game} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut date} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut methods} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut find} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut game} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Inserting} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut GBA} \colorbox{red!1}{\strut Game} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Wild} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Swarms} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut PokRadar} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut Mansion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut However} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut capable} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut transferring} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut teams} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut GBA} \colorbox{red!0}{\strut Versions} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut Pal} \colorbox{red!0}{\strut Park} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut however} \colorbox{red!0}{\strut one-way.Diamond} \colorbox{red!0}{\strut .} \colorbox{red!15}{\strut Pearl} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut brings} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut whole} \colorbox{red!1}{\strut new} \colorbox{red!0}{\strut thing} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Pokmon} \colorbox{red!0}{\strut World} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut online} \colorbox{red!0}{\strut battling} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut trading} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Using} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut critically} \colorbox{red!0}{\strut acclaimed} \colorbox{red!1}{\strut Nintendo} \colorbox{red!0}{\strut WiFi} \colorbox{red!0}{\strut Connection} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut capable} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut sharing} \colorbox{red!0}{\strut Friend} \colorbox{red!0}{\strut Codes} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut friends} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut battling} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut them} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut hedgehog} \colorbox{red!1}{\strut Pokemon} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut diamond} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut pearl} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answers.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut WikiAnswers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Categories} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Arts} \colorbox{red!0}{\strut Toys} \colorbox{red!1}{\strut Pokemon} \colorbox{red!1}{\strut Pokemon} \colorbox{red!1}{\strut XD} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Colosseum} \colorbox{red!7}{\strut What} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut hedgehog} \colorbox{red!1}{\strut Pokemon} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut diamond} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut pearl} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut FlagWhat} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!7}{\strut hedgehog} \colorbox{red!1}{\strut Pokemon} \colorbox{red!0}{\strut in} \colorbox{red!7}{\strut diamond} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut pearl} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answered} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut WikiAnswers} \colorbox{red!0}{\strut CommunityAnswers.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut making} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut better} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut time.The} \colorbox{red!1}{\strut cute} \colorbox{red!0}{\strut little} \colorbox{red!7}{\strut hedgehog} \colorbox{red!1}{\strut Pokemon} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut Shaymin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sheimi} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Japanese} \colorbox{red!0}{\strut games} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut green} \colorbox{red!0}{\strut spines} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut pink} \colorbox{red!0}{\strut nose} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut fairly} \colorbox{red!0}{\strut short} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut legendary} \colorbox{red!1}{\strut Pokemon} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut pure} \colorbox{red!0}{\strut grass-type.19} \colorbox{red!0}{\strut people} \colorbox{red!1}{\strut found} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut usefulWas} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut useful} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut YesSomewhatNoCan} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut Deoxys} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Pokemon} \colorbox{red!7}{\strut Diamond} \colorbox{red!0}{\strut or} \colorbox{red!7}{\strut pearl} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut There} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!0}{\strut way} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut Deoxys} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut Pokemon} \colorbox{red!7}{\strut diamond} \colorbox{red!0}{\strut or} \colorbox{red!7}{\strut pearl} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut onlyway} \colorbox{red!0}{\strut i} \colorbox{red!0}{\strut know} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut action} \colorbox{red!0}{\strut replay} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut know} \colorbox{red!7}{\strut what} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut isyour} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut right} \colorbox{red!0}{\strut spot} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut find} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut alright} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut Wiggleytuff} \colorbox{red!0}{\strut 84} \colorbox{red!0}{\strut 1,218} \colorbox{red!0}{\strut ContributionsWhen} \colorbox{red!0}{\strut comes} \colorbox{red!1}{\strut Pokemon} \colorbox{red!7}{\strut Diamond} \colorbox{red!0}{\strut or} \colorbox{red!7}{\strut pearl} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut country} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut delay} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut they} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut desided} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut translate} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut send} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut If} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut still} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut o} \colorbox{red!0}{\strut Randomnessish} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut ContributionsHow} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!1}{\strut fossils} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Pokemon} \colorbox{red!7}{\strut Diamond} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut Pearl} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut In} \colorbox{red!1}{\strut Pokemon} \colorbox{red!7}{\strut Diamond} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut Pearl} \colorbox{red!0}{\strut versions} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut fossils} \colorbox{red!0}{\strut are} \colorbox{red!1}{\strut found} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut theunderground} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut may} \colorbox{red!0}{\strut access} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut underground} \colorbox{red!0}{\strut if} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut go} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Eterna} \colorbox{red!0}{\strut City} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut talk} \colorbox{red!0}{\strut tothe} \colorbox{red!0}{\strut underground} \colorbox{red!0}{\strut man} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut hou} \colorbox{red!0}{\strut Dark} \colorbox{red!0}{\strut void95} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut ContributionsHow} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut Darkrai} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut Pokemon} \colorbox{red!7}{\strut Diamond} \colorbox{red!0}{\strut and} \colorbox{red!7}{\strut Pearl} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut darkai} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut obtained} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut event} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut japan} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut u} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut action} \colorbox{red!0}{\strut replay} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut use} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut walk} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut walls} \colorbox{red!0}{\strut cheat} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Members} \colorbox{red!0}{\strut Pass} \colorbox{red!0}{\strut cheat} \colorbox{red!0}{\strut if} 
}}}
\end{CJK*}

query: who are net a porter founders

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut Multimillionaire} \colorbox{red!0}{\strut Net-a-Porter} \colorbox{red!2}{\strut founder} \colorbox{red!0}{\strut Dame} \colorbox{red!14}{\strut Natalie} \colorbox{red!14}{\strut Massenet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 52} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut welcomes} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut first} \colorbox{red!2}{\strut son} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut partner} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 38} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut thanks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut generous} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut surrogate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Multimillionaire} \colorbox{red!0}{\strut Net-a-Porter} \colorbox{red!2}{\strut founder} \colorbox{red!0}{\strut Dame} \colorbox{red!14}{\strut Natalie} \colorbox{red!14}{\strut Massenet} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 52} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut welcomes} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut first} \colorbox{red!2}{\strut son} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut partner} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 38} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut thanks} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut generous} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut surrogateLA-born} \colorbox{red!0}{\strut fashion} \colorbox{red!1}{\strut entrepreneur} \colorbox{red!0}{\strut announced} \colorbox{red!0}{\strut birth} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut first} \colorbox{red!2}{\strut son} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut InstagramJet} \colorbox{red!0}{\strut Everest} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut child} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut photographer} \colorbox{red!0}{\strut partner} \colorbox{red!0}{\strut Erik} \colorbox{red!0}{\strut Torstensson} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 38Shares} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut daughters} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut husband} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Isabella} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 17} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Ava} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 11Dame} \colorbox{red!14}{\strut Natalie} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut current} \colorbox{red!0}{\strut chairman} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut British} \colorbox{red!0}{\strut Fashion} \colorbox{red!0}{\strut CouncilBy} \colorbox{red!0}{\strut Siofra} \colorbox{red!0}{\strut Brennan} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut MailonlinePublished} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1410} \colorbox{red!0}{\strut EDT} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 2017} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Updated} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1118} \colorbox{red!0}{\strut EDT} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 27} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 2017237shares571View} \colorbox{red!0}{\strut commentsDame} \colorbox{red!14}{\strut Natalie} \colorbox{red!0}{\strut Sara} \colorbox{red!14}{\strut Massenet} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut journalist} \colorbox{red!5}{\strut who} \colorbox{red!0}{\strut formed} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut hugely} \colorbox{red!0}{\strut successful} \colorbox{red!0}{\strut luxury} \colorbox{red!0}{\strut fashion} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Net-a-porter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut welcomed} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut first} \colorbox{red!2}{\strut son} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut age} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 52.The} \colorbox{red!0}{\strut fashion} \colorbox{red!1}{\strut entrepreneur} \colorbox{red!0}{\strut announced} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut happy} \colorbox{red!0}{\strut news} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut Jet} \colorbox{red!0}{\strut Everest} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut arrival} \colorbox{red!0}{\strut on} \colorbox{red!1}{\strut Instagram} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut revealing} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut been} \colorbox{red!1}{\strut born} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut generous} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut surrogate.She} \colorbox{red!0}{\strut already} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut daughters} \colorbox{red!0}{\strut Isabella} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 17} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Ava} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut marriage} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!3}{\strut Jet} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut baby} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut Swedish} \colorbox{red!0}{\strut photographer} \colorbox{red!0}{\strut partner} \colorbox{red!0}{\strut Erik} \colorbox{red!0}{\strut Torstensson} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 38.The} \colorbox{red!0}{\strut businesswoman} \colorbox{red!1}{\strut founded} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut luxury} \colorbox{red!0}{\strut fashion} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut sold} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 950} \colorbox{red!0}{\strut million} \colorbox{red!0}{\strut with} \colorbox{red!14}{\strut Natalie} \colorbox{red!0}{\strut receiving} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut reported} \colorbox{red!0}{\strut 100M} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut stake.The} \colorbox{red!0}{\strut only} \colorbox{red!0}{\strut child} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut English} \colorbox{red!0}{\strut mother} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut father} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Mrs} \colorbox{red!14}{\strut Massenet} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut raised} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Paris} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut moved} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Los} \colorbox{red!0}{\strut Angeles} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut live} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut father} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut age} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 11.But} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut husband} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut tempted} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut London} \colorbox{red!1}{\strut where} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut based.9Dame} \colorbox{red!14}{\strut Natalie} \colorbox{red!0}{\strut Sara} \colorbox{red!14}{\strut Massenet} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut journalist} \colorbox{red!5}{\strut who} \colorbox{red!0}{\strut formed} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut hugely} \colorbox{red!0}{\strut successful} \colorbox{red!0}{\strut luxury} \colorbox{red!0}{\strut fashion} \colorbox{red!0}{\strut site} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Net-a-porter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut has} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!8}{\strut YOOX} \colorbox{red!0}{\strut Net-a-Porter} \colorbox{red!7}{\strut Group} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut YOOX} \colorbox{red!0}{\strut Net-a-Porter} \colorbox{red!0}{\strut GroupFrom} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedia} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Redirected} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut Net-a-Porter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut navigation} \colorbox{red!0}{\strut searchYOOX} \colorbox{red!0}{\strut NET-A-PORTER} \colorbox{red!7}{\strut GROUP} \colorbox{red!0}{\strut S.p.AType} \colorbox{red!0}{\strut Societ} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut AzioniTraded} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut BIT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut YNAPIndustry} \colorbox{red!4}{\strut Fashion} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut leisureFounded} \colorbox{red!0}{\strut 2015Founder} \colorbox{red!0}{\strut Federico} \colorbox{red!0}{\strut MarchettiHeadquarters} \colorbox{red!0}{\strut Milan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut ItalyKey} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut Federico} \colorbox{red!0}{\strut Marchetti} \colorbox{red!0}{\strut CEOProducts} \colorbox{red!4}{\strut Fashion} \colorbox{red!0}{\strut productsRevenue} \colorbox{red!0}{\strut 1.82} \colorbox{red!0}{\strut Billion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2016} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Number} \colorbox{red!0}{\strut of} \colorbox{red!3}{\strut employees} \colorbox{red!0}{\strut 4300} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Subsidiaries} \colorbox{red!0}{\strut UK} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut US} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Japan} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut France} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Spain} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut China} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Hong} \colorbox{red!0}{\strut KongWebsite} \colorbox{red!0}{\strut www.ynap.comYoox} \colorbox{red!0}{\strut Net-A-Porter} \colorbox{red!7}{\strut Group} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut MTA} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut YNAP} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Italian} \colorbox{red!0}{\strut online} \colorbox{red!4}{\strut fashion} \colorbox{red!3}{\strut retailer} \colorbox{red!5}{\strut created} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut October} \colorbox{red!0}{\strut 2015} \colorbox{red!0}{\strut after} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut merger} \colorbox{red!0}{\strut between} \colorbox{red!8}{\strut Yoox} \colorbox{red!7}{\strut GROUP} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut THE} \colorbox{red!0}{\strut NET-A-PORTER} \colorbox{red!7}{\strut GROUP} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Yoox} \colorbox{red!0}{\strut was} \colorbox{red!5}{\strut founded} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Federico} \colorbox{red!0}{\strut Marchetti} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Bologna} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut become} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut e-commerce} \colorbox{red!4}{\strut company} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut serves} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut 180} \colorbox{red!0}{\strut countries} \colorbox{red!0}{\strut worldwide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!8}{\strut Yoox} \colorbox{red!0}{\strut Net-A-Porter} \colorbox{red!7}{\strut Group} \colorbox{red!0}{\strut history1.1} \colorbox{red!8}{\strut Yoox} \colorbox{red!7}{\strut Group} \colorbox{red!0}{\strut history1.2} \colorbox{red!0}{\strut Net-A-Porter} \colorbox{red!7}{\strut Group} \colorbox{red!0}{\strut history1.3} \colorbox{red!0}{\strut Merger2} \colorbox{red!0}{\strut Distribution3} \colorbox{red!3}{\strut Corporate} \colorbox{red!0}{\strut structure4} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also5} \colorbox{red!0}{\strut ReferencesYoox} \colorbox{red!0}{\strut Net-A-Porter} \colorbox{red!7}{\strut Group} \colorbox{red!0}{\strut history} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut Yoox} \colorbox{red!7}{\strut Group} \colorbox{red!0}{\strut history} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut name} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Yoox} \colorbox{red!0}{\strut which} \colorbox{red!0}{\strut was} \colorbox{red!5}{\strut created} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Federico} \colorbox{red!0}{\strut Marchetti} \colorbox{red!0}{\strut composed} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut male} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Y} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut female} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut X} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut chromosome} \colorbox{red!0}{\strut letters} \colorbox{red!0}{\strut linked} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut OO} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut infinity} \colorbox{red!0}{\strut symbol} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut zero} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut binary} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut fundamental} \colorbox{red!0}{\strut language} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut digital} \colorbox{red!0}{\strut age} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut YOOX} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut concept} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut buy} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut overstocked} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut unsold} \colorbox{red!0}{\strut items} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut previous} \colorbox{red!0}{\strut seasons} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut a} \colorbox{red!0}{\strut direct} \colorbox{red!0}{\strut relationship} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut renowned} \colorbox{red!4}{\strut fashion} \colorbox{red!0}{\strut houses} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut Dolce} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Gabbana} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Diesel} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Gucci} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Armani} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Cavalli} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 8} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut well} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut manufacturers} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut authorized} \colorbox{red!0}{\strut dealers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut sell} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut online} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut discounted} \colorbox{red!0}{\strut outlet} \colorbox{red!0}{\strut prices} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

query: who sang the song i had the time of my life

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!1}{\strut Had} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!17}{\strut Time} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut My} \colorbox{red!17}{\strut Life} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!1}{\strut Had} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!17}{\strut Time} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut LifeFrom} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedianavigation} \colorbox{red!0}{\strut search} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!1}{\strut Had} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!17}{\strut Time} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut My} \colorbox{red!17}{\strut Life} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Single} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Bill} \colorbox{red!0}{\strut Medley} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Jennifer} \colorbox{red!0}{\strut Warnesfrom} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut album} \colorbox{red!1}{\strut Dirty} \colorbox{red!0}{\strut DancingB-side} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Love} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut Strange} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Mickey} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SylviaReleased} \colorbox{red!0}{\strut September} \colorbox{red!0}{\strut 1987Format7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut single} \colorbox{red!0}{\strut 12} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut maxi} \colorbox{red!0}{\strut cassetteCD} \colorbox{red!0}{\strut singleRecorded} \colorbox{red!0}{\strut 1987Genre} \colorbox{red!0}{\strut Soft} \colorbox{red!0}{\strut rock} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut adult} \colorbox{red!0}{\strut contemporary} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut popLength} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 47} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut LP} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut single} \colorbox{red!0}{\strut version} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 646} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut extended} \colorbox{red!0}{\strut version} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Label} \colorbox{red!0}{\strut RCA} \colorbox{red!0}{\strut RecordsSongwriter} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut DeNicola} \colorbox{red!0}{\strut Donald} \colorbox{red!0}{\strut MarkowitzFranke} \colorbox{red!0}{\strut PreviteProducer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Michael} \colorbox{red!0}{\strut LloydMusic} \colorbox{red!0}{\strut video} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!1}{\strut Had} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!17}{\strut Time} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut My} \colorbox{red!17}{\strut Life} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut YouTubeAlternative} \colorbox{red!0}{\strut cover7} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ve} \colorbox{red!1}{\strut Had} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!17}{\strut Time} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut My} \colorbox{red!17}{\strut Life} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut 1987} \colorbox{red!6}{\strut song} \colorbox{red!0}{\strut composed} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Franke} \colorbox{red!0}{\strut Previte} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut John} \colorbox{red!0}{\strut DeNicola} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Donald} \colorbox{red!0}{\strut Markowitz} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut recorded} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Bill} \colorbox{red!0}{\strut Medley} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Jennifer} \colorbox{red!0}{\strut Warnes} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut used} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut theme} \colorbox{red!6}{\strut song} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 1987} \colorbox{red!0}{\strut film} \colorbox{red!1}{\strut Dirty} \colorbox{red!1}{\strut Dancing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!6}{\strut song} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut won} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut awards} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut including} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut Academy} \colorbox{red!0}{\strut Award} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Best} \colorbox{red!0}{\strut Original} \colorbox{red!6}{\strut Song} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Golden} \colorbox{red!0}{\strut Globe} \colorbox{red!0}{\strut Award} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Best} \colorbox{red!0}{\strut Original} \colorbox{red!6}{\strut Song} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Grammy} \colorbox{red!0}{\strut Award} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Best} \colorbox{red!0}{\strut Pop} \colorbox{red!0}{\strut Performance} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Duo} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Group} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut Vocals.Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut History2} \colorbox{red!1}{\strut Music} \colorbox{red!0}{\strut video3} \colorbox{red!0}{\strut Personnel4} \colorbox{red!0}{\strut Chart} \colorbox{red!0}{\strut performance5} \colorbox{red!0}{\strut Awards6} \colorbox{red!0}{\strut Cover} \colorbox{red!0}{\strut versions} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut samples7} \colorbox{red!0}{\strut Formats} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut track} \colorbox{red!0}{\strut listings8} \colorbox{red!0}{\strut Charts8.1} \colorbox{red!0}{\strut Weekly} \colorbox{red!0}{\strut charts8.2} \colorbox{red!0}{\strut Year-end} \colorbox{red!0}{\strut charts8.3} \colorbox{red!0}{\strut Certifications9} \colorbox{red!0}{\strut See} \colorbox{red!0}{\strut also10} \colorbox{red!0}{\strut ReferencesHistory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Singer-songwriter} \colorbox{red!0}{\strut Previte} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut lead} \colorbox{red!1}{\strut singer} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut band} \colorbox{red!0}{\strut Franke} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Knockouts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!1}{\strut had} \colorbox{red!0}{\strut success} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut song} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Sweetheart} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut in} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!7}{\strut Who} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut song} \colorbox{red!7}{\strut How} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut I} \colorbox{red!7}{\strut Live} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Answers.com} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut WikiAnswers} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Categories} \colorbox{red!0}{\strut Entertainment} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Arts} \colorbox{red!0}{\strut Music} \colorbox{red!0}{\strut Music} \colorbox{red!0}{\strut Genres} \colorbox{red!7}{\strut Who} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut song} \colorbox{red!7}{\strut How} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut I} \colorbox{red!7}{\strut Live} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut FlagWho} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut song} \colorbox{red!7}{\strut How} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut I} \colorbox{red!7}{\strut Live} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Answer} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Answers} \colorbox{red!0}{\strut Publisher} \colorbox{red!0}{\strut Confidence} \colorbox{red!0}{\strut votes} \colorbox{red!0}{\strut 415K} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!7}{\strut How} \colorbox{red!0}{\strut Do} \colorbox{red!0}{\strut I} \colorbox{red!7}{\strut Live} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut originally} \colorbox{red!1}{\strut performed} \colorbox{red!0}{\strut by} \colorbox{red!1}{\strut Leann} \colorbox{red!0}{\strut Rimes} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Trish} \colorbox{red!0}{\strut Yearwood} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut re-released} \colorbox{red!0}{\strut this} \colorbox{red!1}{\strut song} \colorbox{red!0}{\strut shortly} \colorbox{red!0}{\strut after} \colorbox{red!1}{\strut Leann} \colorbox{red!0}{\strut Rimes} \colorbox{red!1}{\strut did} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut written} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Diane} \colorbox{red!0}{\strut Warren.5} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut usefulWas} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut answer} \colorbox{red!0}{\strut useful} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut YesSomewhatNoTxswimmerjbb13} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut ContributionsWho} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 90s} \colorbox{red!0}{\strut techno} \colorbox{red!1}{\strut song} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Well} \colorbox{red!0}{\strut considering} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut techno} \colorbox{red!0}{\strut songs..} \colorbox{red!0}{\strut i} \colorbox{red!0}{\strut bet} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut talking} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut George} \colorbox{red!0}{\strut Lamond} \colorbox{red!0}{\strut version.Just1minit} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut ContributionWho} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut ca} \colorbox{red!0}{\strut nt} \colorbox{red!7}{\strut live} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut believe} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut Eric} \colorbox{red!0}{\strut Carmen..} \colorbox{red!0}{\strut And} \colorbox{red!7}{\strut who} \colorbox{red!0}{\strut else} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Ckanyuto} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut ContributionWhat} \colorbox{red!0}{\strut artists} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut Ca} \colorbox{red!0}{\strut nt} \colorbox{red!7}{\strut Live} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut One} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut favorite} \colorbox{red!1}{\strut songs} \colorbox{red!0}{\strut Ca} \colorbox{red!0}{\strut nt} \colorbox{red!7}{\strut Live} \colorbox{red!0}{\strut if} \colorbox{red!7}{\strut Living} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut theme} \colorbox{red!1}{\strut song} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut movie} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Goodbye} \colorbox{red!0}{\strut Maggie} \colorbox{red!0}{\strut Cole} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut starring} \colorbox{red!0}{\strut Susan} \colorbox{red!0}{\strut Hayward} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut original} \colorbox{red!0}{\strut person} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut sing} \colorbox{red!1}{\strut t} \colorbox{red!0}{\strut Who} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut song} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Without} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut was} \colorbox{red!1}{\strut sung} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Usher} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut artist} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut David} \colorbox{red!0}{\strut Guetta.What} \colorbox{red!0}{\strut group} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut song} \colorbox{red!0}{\strut titled} \colorbox{red!7}{\strut LIVE} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut group} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut called} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Merry} \colorbox{red!0}{\strut Go} \colorbox{red!0}{\strut Round} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut lyrics} \colorbox{red!0}{\strut follow} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Oh} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut re} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut kind} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut girl} \colorbox{red!0}{\strut -} \colorbox{red!7}{\strut who} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut stopped} \colorbox{red!0}{\strut yourself} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut having} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut ball} \colorbox{red!0}{\strut Oh} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut you} \colorbox{red!7}{\strut live} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut but} \colorbox{red!7}{\strut how} \colorbox{red!0}{\strut ca} \colorbox{red!0}{\strut Bill} \colorbox{red!0}{\strut Grifenhagen} \colorbox{red!0}{\strut 19,554} \colorbox{red!0}{\strut ContributionsWho} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut ca} \colorbox{red!0}{\strut nt} \colorbox{red!7}{\strut live} \colorbox{red!0}{\strut if} \colorbox{red!7}{\strut living} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut without} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut ?} \colorbox{red!1}{\strut Originally} \colorbox{red!0}{\strut done} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Badfinger} \colorbox{red!0}{\strut Much} \colorbox{red!0}{\strut bigger} \colorbox{red!0}{\strut hit} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut NilssonWho} \colorbox{red!1}{\strut sang} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut song} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut words} \colorbox{red!7}{\strut live} \colorbox{red!7}{\strut live} \colorbox{red!7}{\strut live} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut many} \colorbox{red!1}{\strut song} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut it} 
}}}
\end{CJK*}

query: cambridge  wi in what county

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!20}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut Wisconsin} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut WisconsinFrom} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedianavigation} \colorbox{red!0}{\strut searchCambridge} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut WisconsinVillageLooking} \colorbox{red!0}{\strut east} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut downtown} \colorbox{red!0}{\strut CambridgeLocation} \colorbox{red!0}{\strut of} \colorbox{red!20}{\strut Cambridge} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Jefferson} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Wisconsin.Coordinates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 43015N} \colorbox{red!0}{\strut 8912WCoordinates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 43015N} \colorbox{red!0}{\strut 8912WCountry} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut StatesState} \colorbox{red!0}{\strut WisconsinCounties} \colorbox{red!0}{\strut Dane} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut JeffersonGovernment} \colorbox{red!0}{\strut Type} \colorbox{red!0}{\strut Village} \colorbox{red!0}{\strut Board} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Trustees} \colorbox{red!0}{\strut President} \colorbox{red!0}{\strut Steven} \colorbox{red!0}{\strut R.} \colorbox{red!0}{\strut StrussArea} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Total} \colorbox{red!0}{\strut 1.44} \colorbox{red!0}{\strut sq} \colorbox{red!0}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.73} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Land} \colorbox{red!0}{\strut 1.43} \colorbox{red!0}{\strut sq} \colorbox{red!0}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3.70} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Water} \colorbox{red!0}{\strut 0.01} \colorbox{red!0}{\strut sq} \colorbox{red!0}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0.03} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Elevation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 850} \colorbox{red!0}{\strut ft} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 259} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Population} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2010} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Total} \colorbox{red!0}{\strut 1,457} \colorbox{red!0}{\strut Estimate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2016} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1,509} \colorbox{red!0}{\strut Density} \colorbox{red!0}{\strut 1,018.9sq} \colorbox{red!0}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 393.4km} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Time} \colorbox{red!0}{\strut zone} \colorbox{red!0}{\strut Central} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CST} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut UTC-6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Summer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DST} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CDT} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut UTC-5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Area} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 608FIPS} \colorbox{red!0}{\strut code} \colorbox{red!0}{\strut 55-12225} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GNIS} \colorbox{red!0}{\strut feature} \colorbox{red!0}{\strut ID} \colorbox{red!0}{\strut 1562561} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Website} \colorbox{red!0}{\strut www} \colorbox{red!0}{\strut .ci} \colorbox{red!0}{\strut .cambridge} \colorbox{red!0}{\strut .wi} \colorbox{red!0}{\strut .usLooking} \colorbox{red!0}{\strut east} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut entering} \colorbox{red!0}{\strut CambridgeCambridge} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut village} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Dane} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut mostly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Jefferson} \colorbox{red!13}{\strut counties} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut of} \colorbox{red!4}{\strut Wisconsin} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut population} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut 1,457} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 2010} \colorbox{red!0}{\strut census} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1,348} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Dane} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 109} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Jefferson} \colorbox{red!0}{\strut County.The} \colorbox{red!0}{\strut Dane} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut portion} \colorbox{red!0}{\strut of} \colorbox{red!20}{\strut Cambridge} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Madison} \colorbox{red!0}{\strut Metropolitan} \colorbox{red!0}{\strut Statistical} \colorbox{red!0}{\strut Area} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut while} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Jefferson} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut portion} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut part} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Watertown} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Fort} \colorbox{red!0}{\strut Atkinson} \colorbox{red!0}{\strut Micropolitan} \colorbox{red!0}{\strut Statistical} \colorbox{red!0}{\strut Area.Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut History1.1} \colorbox{red!0}{\strut Settlement-18901.2} \colorbox{red!0}{\strut 1900s-2000s1.3} \colorbox{red!0}{\strut 2000s-present2} \colorbox{red!0}{\strut Geography3} \colorbox{red!0}{\strut Demographics3.1} \colorbox{red!0}{\strut 2010} \colorbox{red!0}{\strut census3.2} \colorbox{red!0}{\strut 2000} \colorbox{red!0}{\strut census4} \colorbox{red!0}{\strut Media5} \colorbox{red!0}{\strut Notable} \colorbox{red!0}{\strut people6} \colorbox{red!0}{\strut Images7} \colorbox{red!0}{\strut References8} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut linksHistory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Settlement-1890} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!20}{\strut Cambridge} \colorbox{red!0}{\strut settlement} \colorbox{red!0}{\strut dates} \colorbox{red!0}{\strut back} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut October} \colorbox{red!0}{\strut 15} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1847} \colorbox{red!0}{\strut when} \colorbox{red!0}{\strut farmer} \colorbox{red!0}{\strut Joseph} \colorbox{red!0}{\strut Keyes} \colorbox{red!0}{\strut filed} \colorbox{red!0}{\strut plans} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Register} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Deeds} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Dane} \colorbox{red!15}{\strut County} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut structure} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut dam} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut northern} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut WIPROPERTY} \colorbox{red!0}{\strut PROFILE} \colorbox{red!0}{\strut Properties} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut ,} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut WI136} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 137} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 139} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523160} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 166} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 173} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523176} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 19} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 215} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523229} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 243} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 279} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523306} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 372} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 384} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523385} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 385} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Apt} \colorbox{red!0}{\strut 1} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 385} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut Apt} \colorbox{red!0}{\strut 2} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523501} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 501} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 503} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523510} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 593} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 60} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523650} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut 75} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut N3975} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523N3993} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut N4007} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut N4039} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523N4045} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut N4137} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut N4146} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523N4149} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut N4161} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} \colorbox{red!0}{\strut 53523} \colorbox{red!0}{\strut N4185} \colorbox{red!0}{\strut County} \colorbox{red!1}{\strut Road} \colorbox{red!0}{\strut A} \colorbox{red!3}{\strut Cambridge} \colorbox{red!0}{\strut ,} \colorbox{red!2}{\strut WI} 
}}}
\end{CJK*}

query: where is quincy located

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut LocationClimate} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut ProfileCommunity} \colorbox{red!0}{\strut OverviewLocationClimateFinancialPopulationHonors} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut AwardsDemographic} \colorbox{red!0}{\strut LinksHome} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Government} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut City} \colorbox{red!0}{\strut Departments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Planning} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Development} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Community} \colorbox{red!0}{\strut Profile} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut LocationClimateLocationClimateThe} \colorbox{red!1}{\strut western} \colorbox{red!0}{\strut most} \colorbox{red!2}{\strut city} \colorbox{red!0}{\strut in} \colorbox{red!22}{\strut Illinois} \colorbox{red!0}{\strut ,} \colorbox{red!70}{\strut Quincy} \colorbox{red!0}{\strut is} \colorbox{red!16}{\strut located} \colorbox{red!0}{\strut along} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut eastern} \colorbox{red!0}{\strut bank} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Mississippi} \colorbox{red!0}{\strut River} \colorbox{red!0}{\strut atop} \colorbox{red!0}{\strut 90} \colorbox{red!0}{\strut foot} \colorbox{red!0}{\strut limestone} \colorbox{red!0}{\strut bluffs} \colorbox{red!1}{\strut which} \colorbox{red!0}{\strut overlook} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut wide} \colorbox{red!0}{\strut expanse} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut river} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut natural} \colorbox{red!0}{\strut harbor.Residents} \colorbox{red!0}{\strut enjoy} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut moderate} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut four} \colorbox{red!0}{\strut season} \colorbox{red!1}{\strut climate} \colorbox{red!36}{\strut where} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut sun} \colorbox{red!0}{\strut shines} \colorbox{red!0}{\strut nearly} \colorbox{red!0}{\strut 68} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut of} \colorbox{red!22}{\strut Illinois} \colorbox{red!0}{\strut receives} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut average} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 36.86} \colorbox{red!0}{\strut inches} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut rainfall} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut an} \colorbox{red!4}{\strut average} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut inches} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut snowfall} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!4}{\strut average} \colorbox{red!0}{\strut winter} \colorbox{red!4}{\strut temperature} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 28} \colorbox{red!0}{\strut degrees} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut average} \colorbox{red!0}{\strut summer} \colorbox{red!4}{\strut temperature} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut 79} \colorbox{red!0}{\strut degrees.Quick} \colorbox{red!0}{\strut LinksCity} \colorbox{red!0}{\strut PermitsCity} \colorbox{red!0}{\strut Licenses2013} \colorbox{red!0}{\strut Land} \colorbox{red!0}{\strut Use} \colorbox{red!0}{\strut Plan2018} \colorbox{red!0}{\strut Plan} \colorbox{red!0}{\strut Commission} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut ZBA} \colorbox{red!0}{\strut Meeting} \colorbox{red!0}{\strut Schedule} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut Indiana} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut IndianaCommunity} \colorbox{red!0}{\strut ProfileNearby} \colorbox{red!0}{\strut CensusGenealogy} \colorbox{red!0}{\strut HelperCemeteriesTidbits} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Trivia} \colorbox{red!0}{\strut Local} \colorbox{red!0}{\strut Newspapers} \colorbox{red!0}{\strut TripAdvisor} \colorbox{red!0}{\strut Links} \colorbox{red!0}{\strut Interactive} \colorbox{red!0}{\strut Map} \colorbox{red!0}{\strut Wish} \colorbox{red!0}{\strut List} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut IN} \colorbox{red!0}{\strut CommunitiesThe} \colorbox{red!1}{\strut location} \colorbox{red!0}{\strut of} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut GPS} \colorbox{red!0}{\strut coordinates} \colorbox{red!0}{\strut provided} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut GNIS} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Click} \colorbox{red!0}{\strut here} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut interactive} \colorbox{red!0}{\strut map} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut surrounding} \colorbox{red!0}{\strut area.Learn} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Commemorative} \colorbox{red!0}{\strut Quarter} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut IndianaCensus} \colorbox{red!0}{\strut Data} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut As} \colorbox{red!0}{\strut far} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut tell} \colorbox{red!0}{\strut ,} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut included} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut past} \colorbox{red!1}{\strut Census} \colorbox{red!0}{\strut counts} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut no} \colorbox{red!4}{\strut population} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut community.While} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut have} \colorbox{red!1}{\strut census} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut might} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut interested} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut some} \colorbox{red!0}{\strut nearby} \colorbox{red!1}{\strut communities} \colorbox{red!2}{\strut where} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Community2016} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!4}{\strut Population} \colorbox{red!0}{\strut Direction} \colorbox{red!0}{\strut Distance} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Bloomington} \colorbox{red!0}{\strut 84,465} \colorbox{red!1}{\strut SE} \colorbox{red!0}{\strut 22} \colorbox{red!0}{\strut miles} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 35.4} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Owen} \colorbox{red!8}{\strut County} \colorbox{red!0}{\strut ...} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut is} \colorbox{red!1}{\strut located} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Owen} \colorbox{red!0}{\strut County.For} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut please} \colorbox{red!0}{\strut visit} \colorbox{red!0}{\strut our} \colorbox{red!1}{\strut Census} \colorbox{red!0}{\strut Page} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Owen} \colorbox{red!0}{\strut County.Population} \colorbox{red!0}{\strut Rings} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut identify} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut live} \colorbox{red!0}{\strut in} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut surrounding} \colorbox{red!0}{\strut area} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut we} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut drawn} \colorbox{red!0}{\strut concentric} \colorbox{red!0}{\strut rings} \colorbox{red!0}{\strut centered} \colorbox{red!0}{\strut on} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut counted} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut number} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut communities} \colorbox{red!0}{\strut within} \colorbox{red!0}{\strut each} \colorbox{red!0}{\strut ring} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut summed} \colorbox{red!0}{\strut their} \colorbox{red!3}{\strut populations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut We} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut population} \colorbox{red!0}{\strut of} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut so} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut people} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut included.RadiusNo} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Communities2016} \colorbox{red!0}{\strut PopulationChange} \colorbox{red!0}{\strut Since} \colorbox{red!0}{\strut 201010} \colorbox{red!1}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 16} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut 3,549} \colorbox{red!0}{\strut -2.95} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 15} \colorbox{red!1}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 24} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 11} \colorbox{red!0}{\strut 30,507} \colorbox{red!0}{\strut 1.22} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!1}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 32} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut 42,421} \colorbox{red!0}{\strut 1.34} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 25} \colorbox{red!1}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 40} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 30} \colorbox{red!0}{\strut 189,209} \colorbox{red!0}{\strut 5.32} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 30} \colorbox{red!1}{\strut mi} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 48} \colorbox{red!0}{\strut km} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 38} \colorbox{red!0}{\strut 219,493} \colorbox{red!0}{\strut 8.68} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Miscellaneous} \colorbox{red!0}{\strut Information} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut Quincy} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut Federal} \colorbox{red!0}{\strut government} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut assigned} \colorbox{red!0}{\strut various} \colorbox{red!0}{\strut identifying} \colorbox{red!0}{\strut codes} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut each} \colorbox{red!1}{\strut community} \colorbox{red!0}{\strut ,} \colorbox{red!8}{\strut county} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut state} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut At} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut another} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut US} \colorbox{red!1}{\strut Census} \colorbox{red!0}{\strut Bureau} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut referenced} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut identifiers} \colorbox{red!0}{\strut when} 
}}}
\end{CJK*}

query: what is university of sioux falls federal id number

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut University} \colorbox{red!0}{\strut Of} \colorbox{red!12}{\strut Sioux} \colorbox{red!12}{\strut Falls} \colorbox{red!0}{\strut in} \colorbox{red!12}{\strut Sioux} \colorbox{red!12}{\strut Falls} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut South} \colorbox{red!0}{\strut Dakota} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut SD} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Table} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut OverviewDetailed} \colorbox{red!0}{\strut ReportsChecklistStatements} \colorbox{red!0}{\strut Regarding} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut IRS} \colorbox{red!0}{\strut Filings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Tax} \colorbox{red!0}{\strut ComplianceCompensation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Officers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Directors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Trustees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Key} \colorbox{red!0}{\strut Employees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Highest} \colorbox{red!0}{\strut Compensated} \colorbox{red!0}{\strut Employees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Independent} \colorbox{red!0}{\strut ContractorsStatement} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut RevenueStatement} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Functional} \colorbox{red!0}{\strut ExpensesBalance} \colorbox{red!0}{\strut SheetReason} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Public} \colorbox{red!0}{\strut Charity} \colorbox{red!0}{\strut StatusRevenue} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Expenses} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Changes} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Net} \colorbox{red!0}{\strut Assets} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Fund} \colorbox{red!0}{\strut BalancesStatement} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Functional} \colorbox{red!0}{\strut ExpensesBalance} \colorbox{red!0}{\strut SheetsReconciliation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Revenue} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut Audited} \colorbox{red!0}{\strut Financial} \colorbox{red!0}{\strut Statements} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut Revenue} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut ReturnReconciliation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Expenses} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut Audited} \colorbox{red!0}{\strut Financial} \colorbox{red!0}{\strut Statements} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut Expenses} \colorbox{red!0}{\strut per} \colorbox{red!0}{\strut ReturnCurrent} \colorbox{red!0}{\strut Officers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Directors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Trustees} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Key} \colorbox{red!0}{\strut EmployeesOther} \colorbox{red!0}{\strut InformationAnalysis} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Income-Producing} \colorbox{red!0}{\strut ActivitiesInformation} \colorbox{red!0}{\strut Regarding} \colorbox{red!0}{\strut Taxable} \colorbox{red!0}{\strut Subsidiaries} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Disregarded} \colorbox{red!0}{\strut EntitiesCompensation} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Five} \colorbox{red!0}{\strut Highest} \colorbox{red!0}{\strut Paid} \colorbox{red!0}{\strut Employees} \colorbox{red!0}{\strut Other} \colorbox{red!0}{\strut Than} \colorbox{red!0}{\strut Officers} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Directors} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut TrusteesStatements} \colorbox{red!0}{\strut About} \colorbox{red!0}{\strut ActivitiesReason} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Non-Private} \colorbox{red!0}{\strut Foundation} \colorbox{red!0}{\strut StatusSupport} \colorbox{red!0}{\strut ScheduleLobbying} \colorbox{red!0}{\strut Expenditures} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut Electing} \colorbox{red!0}{\strut Public} \colorbox{red!0}{\strut CharitiesUnrelated} \colorbox{red!0}{\strut Trade} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut IncomeDeductions} \colorbox{red!0}{\strut Not} \colorbox{red!0}{\strut Taken} \colorbox{red!0}{\strut ElsewhereOrganizations} \colorbox{red!0}{\strut performing} \colorbox{red!0}{\strut similar} \colorbox{red!0}{\strut types} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut workOrganization} \colorbox{red!0}{\strut representatives} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut corrected} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut new} \colorbox{red!0}{\strut information} \colorbox{red!0}{\strut about} \colorbox{red!6}{\strut University} \colorbox{red!0}{\strut Of} \colorbox{red!12}{\strut Sioux} \colorbox{red!12}{\strut Falls} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Non-representatives} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut about} \colorbox{red!6}{\strut University} \colorbox{red!0}{\strut Of} \colorbox{red!12}{\strut Sioux} \colorbox{red!12}{\strut Falls} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut University} \colorbox{red!0}{\strut Of} \colorbox{red!12}{\strut Sioux} \colorbox{red!0}{\strut FallsEmployer} \colorbox{red!0}{\strut Identification} \colorbox{red!1}{\strut Number} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut EIN} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 460224600Name} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Organization} \colorbox{red!6}{\strut University} \colorbox{red!0}{\strut Of} \colorbox{red!12}{\strut Sioux} \colorbox{red!0}{\strut FallsIn} \colorbox{red!0}{\strut Care} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Name} \colorbox{red!6}{\strut University} \colorbox{red!0}{\strut Of} \colorbox{red!12}{\strut Sioux} \colorbox{red!0}{\strut FallsAddress} \colorbox{red!0}{\strut 1101} \colorbox{red!0}{\strut W} \colorbox{red!0}{\strut 22nd} \colorbox{red!0}{\strut St} \colorbox{red!0}{\strut ,} \colorbox{red!12}{\strut Sioux} \colorbox{red!12}{\strut Falls} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut SD} \colorbox{red!0}{\strut 57105-1600Activities} \colorbox{red!0}{\strut Private} \colorbox{red!0}{\strut school} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut School} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut college} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut trade} \colorbox{red!0}{\strut school} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut etc.Subsection} \colorbox{red!0}{\strut Educational} \colorbox{red!0}{\strut OrganizationRuling} \colorbox{red!0}{\strut Date} \colorbox{red!0}{\strut 021950Deductibility} \colorbox{red!0}{\strut Contributions} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut deductibleFoundation} \colorbox{red!0}{\strut SchoolOrganization} \colorbox{red!0}{\strut CorporationExempt} \colorbox{red!1}{\strut Organization} \colorbox{red!1}{\strut Status} \colorbox{red!0}{\strut Unconditional} \colorbox{red!0}{\strut ExemptionTax} \colorbox{red!0}{\strut Period} \colorbox{red!0}{\strut 062013Assets} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50,000,000} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut greaterIncome} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 10,000,000} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 49,999,999Filing} \colorbox{red!0}{\strut Requirement} \colorbox{red!0}{\strut 990} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut 990EZ} \colorbox{red!0}{\strut returnAsset} \colorbox{red!0}{\strut Amount} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 75,156,503Amount} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut Income} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 41,961,321Form} \colorbox{red!0}{\strut 990} \colorbox{red!0}{\strut Revenue} \colorbox{red!0}{\strut Amount} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 37,150,134National} \colorbox{red!0}{\strut Taxonomy} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut Exempt} \colorbox{red!0}{\strut Entities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NTEE} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Educational} \colorbox{red!0}{\strut Institutions} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Related} \colorbox{red!0}{\strut Activities} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Undergraduate} \colorbox{red!0}{\strut College} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4-year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Non-representatives} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut add} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut First} \colorbox{red!0}{\strut Name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Last} \colorbox{red!0}{\strut Name} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut E-mail} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut displayed} \colorbox{red!0}{\strut publicly} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Public} \colorbox{red!0}{\strut comments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 50-4000} \colorbox{red!0}{\strut characters} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!9}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut Sioux} \colorbox{red!9}{\strut Falls} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut From} \colorbox{red!0}{\strut Wikipedia} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut free} \colorbox{red!0}{\strut encyclopedianavigation} \colorbox{red!0}{\strut searchThis} \colorbox{red!0}{\strut article} \colorbox{red!0}{\strut contains} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut advertisement} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Please} \colorbox{red!0}{\strut help} \colorbox{red!0}{\strut improve} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut removing} \colorbox{red!0}{\strut promotional} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut inappropriate} \colorbox{red!0}{\strut external} \colorbox{red!0}{\strut links} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut adding} \colorbox{red!0}{\strut encyclopedic} \colorbox{red!0}{\strut content} \colorbox{red!0}{\strut written} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut neutral} \colorbox{red!0}{\strut point} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut view} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut January} \colorbox{red!0}{\strut 2018} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Learn} \colorbox{red!0}{\strut how} \colorbox{red!0}{\strut and} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut remove} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut template} \colorbox{red!0}{\strut message} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut Sioux} \colorbox{red!0}{\strut FallsFormer} \colorbox{red!0}{\strut names} \colorbox{red!1}{\strut Dakota} \colorbox{red!0}{\strut Collegiate} \colorbox{red!0}{\strut Institute} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 18831885} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Sioux} \colorbox{red!9}{\strut Falls} \colorbox{red!9}{\strut University} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 18851931} \colorbox{red!0}{\strut .} \colorbox{red!9}{\strut Sioux} \colorbox{red!9}{\strut Falls} \colorbox{red!0}{\strut College} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19311995} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Motto} \colorbox{red!0}{\strut Culture} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut ServiceType} \colorbox{red!0}{\strut PrivateEstablished} \colorbox{red!0}{\strut 1883Affiliation} \colorbox{red!0}{\strut American} \colorbox{red!0}{\strut Baptist} \colorbox{red!0}{\strut Churches} \colorbox{red!0}{\strut USAPresident} \colorbox{red!0}{\strut Brett} \colorbox{red!0}{\strut BradfieldAcademic} \colorbox{red!0}{\strut staff} \colorbox{red!0}{\strut 103Students} \colorbox{red!0}{\strut 1,419Location} \colorbox{red!9}{\strut Sioux} \colorbox{red!9}{\strut Falls} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut South} \colorbox{red!1}{\strut Dakota} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut United} \colorbox{red!0}{\strut StatesColors} \colorbox{red!0}{\strut Purple} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut WhiteAthletics} \colorbox{red!0}{\strut NCAA} \colorbox{red!0}{\strut Division} \colorbox{red!0}{\strut II} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut NSICNickname} \colorbox{red!0}{\strut CougarsMascot} \colorbox{red!0}{\strut Cooper} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut CougarWebsite} \colorbox{red!0}{\strut www.usiouxfalls.eduCoordinates} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 433150.8N} \colorbox{red!0}{\strut 964419.3WFounded} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1883} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut University} \colorbox{red!0}{\strut of} \colorbox{red!9}{\strut Sioux} \colorbox{red!9}{\strut Falls} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut USF} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut Christian} \colorbox{red!0}{\strut liberal} \colorbox{red!0}{\strut arts} \colorbox{red!9}{\strut university} \colorbox{red!1}{\strut located} \colorbox{red!0}{\strut in} \colorbox{red!9}{\strut Sioux} \colorbox{red!9}{\strut Falls} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!1}{\strut state} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut South} \colorbox{red!1}{\strut Dakota} \colorbox{red!0}{\strut .} \colorbox{red!3}{\strut USF} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut mission} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut foster} \colorbox{red!0}{\strut academic} \colorbox{red!0}{\strut excellence} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut development} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut mature} \colorbox{red!0}{\strut Christian} \colorbox{red!0}{\strut persons} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut service} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut God} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut humankind} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut fall} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!9}{\strut University} \colorbox{red!1}{\strut enrolled} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 1,108} \colorbox{red!0}{\strut undergraduate} \colorbox{red!1}{\strut students} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut 311} \colorbox{red!0}{\strut graduate} \colorbox{red!1}{\strut students} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Contents} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut hide} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut History1.1} \colorbox{red!1}{\strut Founding} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Early} \colorbox{red!0}{\strut History1.2} \colorbox{red!0}{\strut Expansion1.3} \colorbox{red!1}{\strut Name} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Future1.4} \colorbox{red!0}{\strut Investments} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Technology2} \colorbox{red!0}{\strut Academics2.1} \colorbox{red!0}{\strut Academic} \colorbox{red!0}{\strut Offerings3} \colorbox{red!0}{\strut Mission4} \colorbox{red!0}{\strut Student} \colorbox{red!0}{\strut life4.1} \colorbox{red!0}{\strut Student} \colorbox{red!0}{\strut Groups} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Organizations4.2} \colorbox{red!0}{\strut Service} \colorbox{red!0}{\strut Opportunities4.3} \colorbox{red!0}{\strut Student} \colorbox{red!0}{\strut Media5} \colorbox{red!0}{\strut Buildings} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Facilities5.1} \colorbox{red!0}{\strut Residence} \colorbox{red!0}{\strut Halls5.2} \colorbox{red!1}{\strut Campus} \colorbox{red!0}{\strut Buildings6} \colorbox{red!3}{\strut USF} \colorbox{red!0}{\strut Presidents7} \colorbox{red!0}{\strut Athletics7.1} \colorbox{red!0}{\strut Women} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Teams7.2} \colorbox{red!0}{\strut Men} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut Teams8} \colorbox{red!0}{\strut Alumni9} \colorbox{red!0}{\strut References10} \colorbox{red!0}{\strut External} \colorbox{red!0}{\strut linksHistory} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut Founding} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Early} \colorbox{red!0}{\strut History} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut edit} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut On} \colorbox{red!0}{\strut June} \colorbox{red!0}{\strut 5} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1872} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut pastors} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut delegates} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut nine} \colorbox{red!0}{\strut Baptist} \colorbox{red!0}{\strut churches} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut Dakota} \colorbox{red!0}{\strut Territory} \colorbox{red!0}{\strut gathered} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut Vermillion} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut South} \colorbox{red!1}{\strut Dakota} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut meeting} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut Baptist} \colorbox{red!0}{\strut Association} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut They} \colorbox{red!0}{\strut adopted} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut resolution} 
}}}
\end{CJK*}

query: what is usaid

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!6}{\strut United} \colorbox{red!7}{\strut States} \colorbox{red!12}{\strut Agency} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut International} \colorbox{red!7}{\strut Development} \colorbox{red!0}{\strut .} \colorbox{red!21}{\strut USAID} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!6}{\strut United} \colorbox{red!7}{\strut States} \colorbox{red!12}{\strut Agency} \colorbox{red!0}{\strut for} \colorbox{red!11}{\strut International} \colorbox{red!7}{\strut Development} \colorbox{red!0}{\strut .} \colorbox{red!21}{\strut USAID} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut DefinitionPopular} \colorbox{red!0}{\strut TermsAn} \colorbox{red!0}{\strut independent} \colorbox{red!1}{\strut federal} \colorbox{red!12}{\strut agency} \colorbox{red!1}{\strut established} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut Foreign} \colorbox{red!0}{\strut Assistance} \colorbox{red!0}{\strut Act} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1961} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut purpose} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut extending} \colorbox{red!1}{\strut economic} \colorbox{red!0}{\strut assistance} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut developing} \colorbox{red!0}{\strut countries} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Its} \colorbox{red!0}{\strut stated} \colorbox{red!1}{\strut purpose} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut support} \colorbox{red!0}{\strut long-term} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut equitable} \colorbox{red!1}{\strut economic} \colorbox{red!0}{\strut growth} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut advance} \colorbox{red!0}{\strut U.S.} \colorbox{red!3}{\strut foreign} \colorbox{red!0}{\strut policy} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut conflict} \colorbox{red!0}{\strut prevention} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut humanitarian} \colorbox{red!0}{\strut assistance.immediate} \colorbox{red!0}{\strut famil} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut dislocated} \colorbox{red!0}{\strut work} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut businessglobalizationmarginal} \colorbox{red!0}{\strut benefi} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut revenueproductelasticity} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut ...} \colorbox{red!1}{\strut economic} \colorbox{red!0}{\strut systemYou} \colorbox{red!0}{\strut Also} \colorbox{red!0}{\strut Might} \colorbox{red!0}{\strut Like} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Leo} \colorbox{red!0}{\strut SunGovernment} \colorbox{red!0}{\strut Aide} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut Minority} \colorbox{red!0}{\strut Small} \colorbox{red!0}{\strut Business} \colorbox{red!0}{\strut OwnersIn} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut United} \colorbox{red!7}{\strut States} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut civil} \colorbox{red!0}{\strut rights} \colorbox{red!0}{\strut movement} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut 1960s} \colorbox{red!0}{\strut opened} \colorbox{red!0}{\strut doors} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut minority} \colorbox{red!0}{\strut entrepreneurs} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut who} \colorbox{red!0}{\strut had} \colorbox{red!0}{\strut previously} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut widely} \colorbox{red!0}{\strut marginalized} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut affluent} \colorbox{red!0}{\strut white} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut owners} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut President} \colorbox{red!0}{\strut Nixon} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut ball} \colorbox{red!0}{\strut rolling} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 1969} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut jayhawkBusiness} \colorbox{red!0}{\strut Dictionary} \colorbox{red!0}{\strut s} \colorbox{red!1}{\strut Term} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Tax} \colorbox{red!0}{\strut InversionTax} \colorbox{red!0}{\strut Inversions} \colorbox{red!0}{\strut With} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut U.S.} \colorbox{red!0}{\strut corporate} \colorbox{red!0}{\strut tax} \colorbox{red!0}{\strut rate} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 39} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut highest} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut developed} \colorbox{red!0}{\strut world} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut large} \colorbox{red!0}{\strut corporations} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut their} \colorbox{red!0}{\strut headquarters} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!6}{\strut United} \colorbox{red!7}{\strut States} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut considered} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut tax} \colorbox{red!0}{\strut inversion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut corporate} \colorbox{red!0}{\strut inversion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut ADVERTISEMENTLeo} \colorbox{red!0}{\strut SunFive} \colorbox{red!0}{\strut Ways} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut Become} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut Multinational} \colorbox{red!0}{\strut CompanyCongratulations} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut grown} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut tiny} \colorbox{red!0}{\strut office} \colorbox{red!0}{\strut block} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut now} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut enough} \colorbox{red!0}{\strut cash} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut go} \colorbox{red!1}{\strut multinational} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut time} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut expand} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut countries} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut make} \colorbox{red!0}{\strut your} \colorbox{red!0}{\strut brand} \colorbox{red!0}{\strut known} \colorbox{red!0}{\strut worldwide} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut basic} \colorbox{red!0}{\strut options} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut fledgling} \colorbox{red!0}{\strut ...} \colorbox{red!0}{\strut Jeffrey} \colorbox{red!0}{\strut GlenCollege} \colorbox{red!0}{\strut vs.} \colorbox{red!0}{\strut University} \colorbox{red!0}{\strut .} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!1}{\strut Top} \colorbox{red!8}{\strut USAID} \colorbox{red!2}{\strut contractors} \colorbox{red!0}{\strut for} \colorbox{red!2}{\strut 2015} \colorbox{red!0}{\strut Children} \colorbox{red!0}{\strut wear} \colorbox{red!0}{\strut baseball} \colorbox{red!0}{\strut caps} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut U.S.} \colorbox{red!2}{\strut Agency} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut International} \colorbox{red!1}{\strut Development} \colorbox{red!0}{\strut logo} \colorbox{red!0}{\strut .} \colorbox{red!2}{\strut Which} \colorbox{red!2}{\strut contractors} \colorbox{red!2}{\strut secured} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!7}{\strut funding} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut aid} \colorbox{red!2}{\strut agency} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut fiscal} \colorbox{red!0}{\strut year} \colorbox{red!2}{\strut 2015} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Photo} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Karima} \colorbox{red!0}{\strut Rhanem} \colorbox{red!0}{\strut .} \colorbox{red!8}{\strut USAID} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut CC} \colorbox{red!0}{\strut BY-NCThe} \colorbox{red!0}{\strut U.S.} \colorbox{red!2}{\strut Agency} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut International} \colorbox{red!1}{\strut Development} \colorbox{red!1}{\strut obligated} \colorbox{red!2}{\strut contract} \colorbox{red!7}{\strut funding} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut fiscal} \colorbox{red!2}{\strut 2015} \colorbox{red!0}{\strut reached} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 4.8} \colorbox{red!0}{\strut billion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut billion} \colorbox{red!1}{\strut increase} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut its} \colorbox{red!0}{\strut total} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut 26} \colorbox{red!0}{\strut percent} \colorbox{red!1}{\strut budget} \colorbox{red!0}{\strut surge} \colorbox{red!0}{\strut marks} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut upward} \colorbox{red!0}{\strut movement} \colorbox{red!0}{\strut in} \colorbox{red!8}{\strut USAID} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut s} \colorbox{red!2}{\strut contract} \colorbox{red!1}{\strut spending} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut last} \colorbox{red!0}{\strut three} \colorbox{red!0}{\strut years.Despite} \colorbox{red!8}{\strut USAID} \colorbox{red!0}{\strut .} \colorbox{red!1}{\strut s} \colorbox{red!0}{\strut focus} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut channeling} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut foreign} \colorbox{red!1}{\strut aid} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut local} \colorbox{red!1}{\strut organizations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut most} \colorbox{red!0}{\strut notably} \colorbox{red!0}{\strut through} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut USAID} \colorbox{red!0}{\strut Forward} \colorbox{red!0}{\strut initiative} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!2}{\strut agency} \colorbox{red!0}{\strut continues} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut award} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut bulk} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut its} \colorbox{red!1}{\strut contracts} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut American} \colorbox{red!1}{\strut firms} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!2}{\strut 2015} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut top} \colorbox{red!0}{\strut 20} \colorbox{red!1}{\strut recipients} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut USAID} \colorbox{red!7}{\strut funding} \colorbox{red!0}{\strut were} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut U.S.-based} \colorbox{red!1}{\strut organizations} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Combined} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut transactions} \colorbox{red!0}{\strut account} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut 70} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut total} \colorbox{red!8}{\strut USAID} \colorbox{red!1}{\strut spending} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut obligated} \colorbox{red!1}{\strut contracts} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut slightly} \colorbox{red!0}{\strut from} \colorbox{red!0}{\strut 67} \colorbox{red!0}{\strut percent} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2014.The} \colorbox{red!0}{\strut consortium} \colorbox{red!0}{\strut Partnerships} \colorbox{red!0}{\strut for} \colorbox{red!1}{\strut Supply} \colorbox{red!1}{\strut Chain} \colorbox{red!1}{\strut Management} \colorbox{red!1}{\strut received} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut most} \colorbox{red!8}{\strut USAID} \colorbox{red!2}{\strut contract} \colorbox{red!7}{\strut funding} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut while} \colorbox{red!1}{\strut international} \colorbox{red!1}{\strut development} \colorbox{red!1}{\strut consulting} \colorbox{red!1}{\strut firm} \colorbox{red!0}{\strut Chemonics} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut second} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!2}{\strut 2015} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut Chemonics} \colorbox{red!2}{\strut secured} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut indefinite} \colorbox{red!0}{\strut delivery} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut indefinite} \colorbox{red!0}{\strut quantity} \colorbox{red!0}{\strut agreement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut IDIQ} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut with} \colorbox{red!8}{\strut USAID} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut tune} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 9.5} \colorbox{red!0}{\strut billion} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut largest} \colorbox{red!8}{\strut USAID} \colorbox{red!1}{\strut award} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut date} \colorbox{red!2}{\strut which} \colorbox{red!0}{\strut could} \colorbox{red!0}{\strut lift} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut firm} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut top} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut next} \colorbox{red!0}{\strut year.Meanwhile} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut four} \colorbox{red!1}{\strut organizations} \colorbox{red!0}{\strut managed} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut break} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut top} \colorbox{red!0}{\strut 20} \colorbox{red!0}{\strut in} \colorbox{red!1}{\strut fiscal} \colorbox{red!2}{\strut 2015} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Checchi} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut Co.} \colorbox{red!0}{\strut more} \colorbox{red!0}{\strut than} \colorbox{red!0}{\strut doubled} \colorbox{red!0}{\strut its} \colorbox{red!2}{\strut contract} \colorbox{red!7}{\strut funding} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 44} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut compared} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 19} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut 2014} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut consulting} \colorbox{red!1}{\strut firm} \colorbox{red!0}{\strut Dexis} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut formerly} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut small} \colorbox{red!0}{\strut business} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut received} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 48} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut in} \colorbox{red!2}{\strut 2015} \colorbox{red!0}{\strut versus} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 22} \colorbox{red!1}{\strut million} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut previous} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Morganti} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut meanwhile} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut significantly} \colorbox{red!0}{\strut increased} 
}}}
\end{CJK*}

query: when do kids start writing sentences

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 1} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 12Old} \colorbox{red!0}{\strut 09-16-2009} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1019} \colorbox{red!0}{\strut PM} \colorbox{red!0}{\strut -} \colorbox{red!0}{\strut Thread} \colorbox{red!0}{\strut StarteraishamamaJoin} \colorbox{red!0}{\strut Date} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Jun} \colorbox{red!0}{\strut 2009Posts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 286Mentioned} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tagged} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Thread} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Quoted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Does} \colorbox{red!0}{\strut anyone} \colorbox{red!0}{\strut know} \colorbox{red!9}{\strut what} \colorbox{red!0}{\strut the} \colorbox{red!4}{\strut typical} \colorbox{red!12}{\strut age} \colorbox{red!0}{\strut is} \colorbox{red!5}{\strut when} \colorbox{red!3}{\strut children} \colorbox{red!3}{\strut start} \colorbox{red!13}{\strut writing} \colorbox{red!12}{\strut sentences} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut wondering} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut Yusuf} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut also} \colorbox{red!1}{\strut types} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut computer} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut This} \colorbox{red!0}{\strut morning} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut got} \colorbox{red!0}{\strut up} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut my} \colorbox{red!0}{\strut husband} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut sleeping} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut other} \colorbox{red!0}{\strut lo} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut When} \colorbox{red!0}{\strut dh} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut leaving} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut found} \colorbox{red!0}{\strut Yusuf} \colorbox{red!0}{\strut at} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut computer} \colorbox{red!1}{\strut typing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut It} \colorbox{red!0}{\strut was} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut simple} \colorbox{red!13}{\strut sentence} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Yusuf} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut big} \colorbox{red!0}{\strut boy} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut spaces} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut usually} \colorbox{red!13}{\strut writes} \colorbox{red!12}{\strut sentences} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut doodleboard} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut really} \colorbox{red!0}{\strut want} \colorbox{red!0}{\strut him} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut type} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut out} \colorbox{red!0}{\strut as} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut d} \colorbox{red!0}{\strut like} \colorbox{red!0}{\strut him} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut improve} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut handwriting} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Is} \colorbox{red!0}{\strut that} \colorbox{red!9}{\strut what} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut all} \colorbox{red!0}{\strut would} \colorbox{red!0}{\strut recommend} \colorbox{red!0}{\strut ?} \colorbox{red!9}{\strut What} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut you} \colorbox{red!0}{\strut doing} \colorbox{red!0}{\strut int} \colorbox{red!0}{\strut his} \colorbox{red!0}{\strut regard} \colorbox{red!0}{\strut and} \colorbox{red!9}{\strut what} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut the} \colorbox{red!3}{\strut normal} \colorbox{red!12}{\strut age} \colorbox{red!0}{\strut that} \colorbox{red!4}{\strut typical} \colorbox{red!3}{\strut children} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut ?} \colorbox{red!0}{\strut Mama} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut 3} \colorbox{red!0}{\strut boys} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 6} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 4} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut one} \colorbox{red!0}{\strut baby} \colorbox{red!0}{\strut girl} \colorbox{red!0}{\strut !} \colorbox{red!0}{\strut aishamama} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut offline} \colorbox{red!0}{\strut Quote} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut 12Old} \colorbox{red!0}{\strut 09-16-2009} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut 1154} \colorbox{red!0}{\strut PMno5no5Join} \colorbox{red!0}{\strut Date} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Feb} \colorbox{red!0}{\strut 2008Posts} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 2,557Mentioned} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Tagged} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Thread} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Quoted} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut 0} \colorbox{red!0}{\strut Post} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut My} \colorbox{red!0}{\strut DD} \colorbox{red!0}{\strut has} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut able} \colorbox{red!0}{\strut to} \colorbox{red!13}{\strut write} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut over} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut year} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut just} \colorbox{red!0}{\strut does} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut much} \colorbox{red!0}{\strut interest} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut m} \colorbox{red!0}{\strut not} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut least} \colorbox{red!0}{\strut bit} \colorbox{red!0}{\strut concerned} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut nt} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut anything} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut encouragediscourage} \colorbox{red!13}{\strut writing} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Well} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut did} \colorbox{red!0}{\strut get} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut own} \colorbox{red!0}{\strut email} \colorbox{red!0}{\strut address} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut case} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut wanted} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut place} \colorbox{red!0}{\strut to} \colorbox{red!13}{\strut write} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut but} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut novelty} \colorbox{red!0}{\strut wore} \colorbox{red!0}{\strut off} \colorbox{red!0}{\strut very} \colorbox{red!0}{\strut quickly} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut I} \colorbox{red!0}{\strut think} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut s} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut weeks} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut more} 
}}}
\end{CJK*}

\begin{CJK*}{UTF8}{gbsn}
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.9\textwidth}{
\colorbox{red!5}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Teach} \colorbox{red!1}{\strut Kids} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Write} \colorbox{red!8}{\strut Sentences} \colorbox{red!2}{\strut Writing} \colorbox{red!0}{\strut .} \colorbox{red!5}{\strut How} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Teach} \colorbox{red!1}{\strut Kids} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Write} \colorbox{red!0}{\strut SentencesHow} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut Teach} \colorbox{red!1}{\strut Kids} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Write} \colorbox{red!0}{\strut SentencesTeaching} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut kid} \colorbox{red!5}{\strut how} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut write} \colorbox{red!1}{\strut complete} \colorbox{red!8}{\strut sentences} \colorbox{red!0}{\strut can} \colorbox{red!0}{\strut be} \colorbox{red!0}{\strut challenging} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut especially} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut great} \colorbox{red!0}{\strut deal} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut common} \colorbox{red!0}{\strut speech} \colorbox{red!0}{\strut consists} \colorbox{red!0}{\strut of} \colorbox{red!8}{\strut sentence} \colorbox{red!1}{\strut fragments} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut In} \colorbox{red!0}{\strut spite} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut techniques} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut been} \colorbox{red!0}{\strut shown} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut work} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut To} \colorbox{red!0}{\strut successfully} \colorbox{red!2}{\strut help} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut child} \colorbox{red!2}{\strut learn} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut write} \colorbox{red!1}{\strut complete} \colorbox{red!8}{\strut sentences} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut consider} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut tips.Teaching} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut Child} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut Write} \colorbox{red!0}{\strut SentencesPutting} \colorbox{red!1}{\strut Basic} \colorbox{red!8}{\strut Sentences} \colorbox{red!0}{\strut TogetherLearning} \colorbox{red!0}{\strut to} \colorbox{red!3}{\strut write} \colorbox{red!8}{\strut sentences} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut gradual} \colorbox{red!1}{\strut process} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut all} \colorbox{red!1}{\strut kids} \colorbox{red!0}{\strut because} \colorbox{red!0}{\strut there} \colorbox{red!0}{\strut are} \colorbox{red!0}{\strut many} \colorbox{red!0}{\strut steps} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut stages} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Your} \colorbox{red!1}{\strut child} \colorbox{red!0}{\strut first} \colorbox{red!0}{\strut needs} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut understand} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut sentence} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut series} \colorbox{red!0}{\strut of} \colorbox{red!1}{\strut words} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut form} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut statement} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut question} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut command} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut an} \colorbox{red!0}{\strut exclamation} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Then} \colorbox{red!0}{\strut he} \colorbox{red!0}{\strut or} \colorbox{red!0}{\strut she} \colorbox{red!0}{\strut can} \colorbox{red!2}{\strut learn} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut sentence} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut typically} \colorbox{red!0}{\strut composed} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut predicate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut sentence} \colorbox{red!0}{\strut is} \colorbox{red!4}{\strut what} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut sentence} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut about} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!1}{\strut predicate} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut whatever} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut stated} \colorbox{red!0}{\strut in} \colorbox{red!0}{\strut relationship} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut subject.When} \colorbox{red!2}{\strut teaching} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut child} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut a} \colorbox{red!1}{\strut common} \colorbox{red!0}{\strut method} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut present} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut with} \colorbox{red!8}{\strut sentence} \colorbox{red!1}{\strut fragments} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut put} \colorbox{red!0}{\strut together} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut You} \colorbox{red!0}{\strut do} \colorbox{red!0}{\strut this} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut dividing} \colorbox{red!0}{\strut a} \colorbox{red!8}{\strut sentence} \colorbox{red!0}{\strut by} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut relating} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut subject} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut section} \colorbox{red!0}{\strut relating} \colorbox{red!0}{\strut to} \colorbox{red!0}{\strut the} \colorbox{red!1}{\strut predicate} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut For} \colorbox{red!0}{\strut example} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut take} \colorbox{red!0}{\strut the} \colorbox{red!8}{\strut sentence} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut girl} \colorbox{red!0}{\strut walks} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut Divide} \colorbox{red!0}{\strut it} \colorbox{red!0}{\strut into} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut following} \colorbox{red!0}{\strut two} \colorbox{red!0}{\strut sections} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut The} \colorbox{red!0}{\strut girl} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut and} \colorbox{red!0}{\strut walks} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut school} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut After} \colorbox{red!0}{\strut showing} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut child} \colorbox{red!0}{\strut a} \colorbox{red!0}{\strut few} \colorbox{red!0}{\strut of} \colorbox{red!0}{\strut these} \colorbox{red!0}{\strut exercises} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut have} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut begin} \colorbox{red!0}{\strut to} \colorbox{red!1}{\strut complete} \colorbox{red!0}{\strut them} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut her} \colorbox{red!0}{\strut own.Expanding} \colorbox{red!0}{\strut on} \colorbox{red!0}{\strut the} \colorbox{red!0}{\strut BasicsEnsure} \colorbox{red!0}{\strut that} \colorbox{red!0}{\strut your} \colorbox{red!1}{\strut child} \colorbox{red!0}{\strut is} \colorbox{red!0}{\strut familiar} \colorbox{red!0}{\strut with} \colorbox{red!0}{\strut interrogative} \colorbox{red!1}{\strut words} \colorbox{red!0}{\strut for} \colorbox{red!0}{\strut asking} \colorbox{red!0}{\strut questions} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut such} \colorbox{red!0}{\strut as} \colorbox{red!1}{\strut who} \colorbox{red!0}{\strut ,} \colorbox{red!4}{\strut what} \colorbox{red!0}{\strut ,} \colorbox{red!0}{\strut where} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut when} \colorbox{red!0}{\strut ,} \colorbox{red!1}{\strut why} \colorbox{red!0}{\strut and} \colorbox{red!5}{\strut how} \colorbox{red!0}{\strut .} \colorbox{red!0}{\strut He} \colorbox{red!0}{\strut will} \colorbox{red!0}{\strut also} \colorbox{red!0}{\strut need} \colorbox{red!0}{\strut to} \colorbox{red!2}{\strut learn} \colorbox{red!0}{\strut about} \colorbox{red!1}{\strut verbs} \colorbox{red!0}{\strut ,} 
}}}
\end{CJK*}


